Unveiling complex magnetic field configurations in red giant stars

Recent measurements of magnetic field strength inside the radiative interior of red giant stars open the way towards the characterization of the geometry of stable large-scale magnetic fields. However, current measurements do not properly constrain the topology of magnetic fields due to degeneracies on the observed magnetic field signature on such $\ell=1$ mode frequencies. Efforts focused towards unambiguous detections of magnetic field configurations are now key to better understand angular momentum transport in stars. We investigate the detectability of complex magnetic field topologies inside the radiative interior of red giants. We focus on a field composed of a combination of a dipole and a quadrupole (quadrudipole), and on an offset field. We explore the potential of probing such magnetic field topologies from a combined measurement of magnetic signatures on $\ell=1$ and quadrupolar ($\ell=2$) mixed mode oscillation frequencies. We first derive the asymptotic theoretical formalism for computing the asymmetric signature in frequency pattern for $\ell=2$ modes due to a quadrudipole magnetic field. The degeneracy of the quadrudipole with a dipole is lifted when considering both $\ell=1$ and $\ell=2$ mode frequencies. In addition to the analytical derivation for the quadrudipole, we present the prospect for complex magnetic field inversions using magnetic sensitivity kernels from standard perturbation analysis for forward modeling. Using this method, we demonstrate that offset fields may be mistaken for weak and centered magnetic fields, resulting in underestimating magnetic field strength in stellar cores. We emphasize the need to characterize $\ell=2$ mixed-mode frequencies, (along with the currently characterized $\ell=1$ mixed modes), to unveil the higher-order components of the geometry of buried magnetic fields, and better constrain angular momentum transport inside stars.

==> newcommands.tex <==
\newcommand{\xiv}{\boldsymbol{\xi}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand\basisvec[1]{\hat{\boldsymbol{e}}_{#1}}
\newcommand{\bnabla}{\boldsymbol{\nabla}}
\newcommand{\solint}{\int_0^{R_{\odot}} \mathrm{d}r\,}
\newcommand{\wigred}[3]{\bigg(\begin{smallmatrix} \ell' & s & \ell \\ #1 & #2 & #3 \end{smallmatrix}\bigg)\,}
\newcommand{\om}[2]{\Omega_{#1}^{#2}\,}
\newcommand{\tj}[6]{\left(\begin{array}{ccr}
#1 & #2 & #3\\
#4 & #5 & #6 \end{array}\right)}

==> references_old <==
@article{2018,
  title = {{{OUP}} Accepted Manuscript},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/sty1010},
  urldate = {2023-10-02},
  abstract = {Recent detections of g-mode pulsations in subdwarf B (sdB) stars from the space missions CoRoT and Kepler have verified that nearly all of these pulsators have regular period spacings. This discovery has been extensively applied to mode identification for the observed g-mode sdB pulsators. However, the discovery of regular period spacings apparently contradicts the strong g-mode trapping structure expected in canonical sdB models, which is caused by steep chemical gradients in such evolved stars. Although the mode trapping efficiency could be reduced somewhat by taking into account the diffusion effect during the sdB phase, it is still difficult to explain the regular period spacings of g-mode sdB pulsators, especially in the shortperiod range. We suggest that the regular period spacings may arise earlier in the evolution of sdB stars rather than during the sdB stage itself. As for a canonical sdB star, it is evolved from a low-mass star and is considered to have gone through the He flash. The He flash causes extensive and aggressive convection that extends very close to the He/H transition zone. When considering a proper convective overshoot during the He-flash stage, the chemical profile in the He/H transition zone becomes smoother. Detailed model calculations show that the mode trapping efficiency could be reduced to approximately the level of observations throughout the observed period range by taking the He-flash overshoot into account.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/6N6ZGR6K/2018 - OUP accepted manuscript.pdf}
}

@article{2241978,
  title = {Period {{Determination Using Phase Dispersion Minimization}}},
  author = {Stellingwerf, R.F.},
  year = {1978},
  journal = {The Astrophysical Journal},
  volume = {224},
  pages = {953--960},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ANETXCFS/Stellingwerf - 1978.pdf}
}

@article{A,
  title = {Theoretical Amplitudes of Solar G-Modes},
  author = {Andersen, B. N.},
  year = {1996},
  journal = {Astronomy \& Astrophysics},
  volume = {312},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RI6Y4V3F/Andersen - 1996.pdf}
}

@article{Abdul-Masih2016,
  title = {Kepler {{Eclipsing Binary Stars}}. {{VIII}}. {{Identification}} of {{False Positive Eclipsing Binaries}} and {{Re-extraction}} of {{New Light Curves}}},
  author = {{Abdul-Masih}, Michael and Prsa, Andrej and Conroy, Kyle and Bloemen, Steven and Boyajian, Tabetha and Doyle, Laurance R. and Johnston, Cole and Kostov, Veselin and Latham, David W. and Matijevic, Gal and Shporer, Avi and Southworth, John},
  year = {2016},
  eprint = {1602.05932},
  pages = {1--21},
  doi = {10.3847/0004-6256/151/4/101},
  abstract = {The Kepler Mission has provided unprecedented, nearly continuous photometric data of \$\textbackslash sim\$200,000 objects in the \$\textbackslash sim\$105 deg\$\^\{2\}\$ field of view from the beginning of science operations in May of 2009 until the loss of the second reaction wheel in May of 2013. The Kepler Eclipsing Binary Catalog contains information including but not limited to ephemerides, stellar parameters and analytical approximation fits for every known eclipsing binary system in the Kepler Field of View. Using Target Pixel level data collected from Kepler in conjunction with the Kepler Eclipsing Binary Catalog, we identify false positives among eclipsing binaries, i.e. targets that are not eclipsing binaries themselves, but are instead contaminated by eclipsing binary sources nearby on the sky and show eclipsing binary signatures in their light curves. We present methods for identifying these false positives and for extracting new light curves for the true source of the observed binary signal. For each source, we extract three separate light curves for each quarter of available data by optimizing the signal-to-noise ratio, the relative percent eclipse depth and the flux eclipse depth. We present 289 new eclipsing binaries in the Kepler Field of View that were not targets for observation, and these have been added to the Catalog. An online version of this Catalog with downloadable content and visualization tools is maintained at http://keplerEBs.villanova.edu.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9SQUVEDR/Abdul-Masih et al. - 2016.pdf}
}

@book{Abramowitz1972,
  title = {Handbook of {{Mathematical Functions}}},
  author = {Abramowitz, M. and Stegun, I.A.},
  year = {1972},
  publisher = {{New York: Dover}},
  urldate = {2020-08-10},
  keywords = {notion,notion-database}
}

@article{Abrial2008,
  title = {{{CMB}} Data Analysis and Sparsity},
  author = {Abrial, P. and Moudden, Y. and Starck, J. L. and Fadili, J. and Delabrouille, J. and Nguyen, M. K.},
  year = {2008},
  journal = {Statistical Methodology},
  volume = {5},
  number = {4},
  pages = {289--298},
  issn = {15723127},
  doi = {10.1016/j.stamet.2007.11.005},
  abstract = {The statistical analysis of the soon to come Planck satellite CMB data will help set tighter bounds on major cosmological parameters. On the way, a number of practical difficulties need to be tackled, notably that several other astrophysical sources emit radiation in the frequency range of CMB observations. Some level of residual contributions, most significantly in the galactic region and at the locations of strong radio point sources will unavoidably contaminate the estimated spherical CMB map. Masking out these regions is common practice but the gaps in the data need proper handling. In order to restore the stationarity of a partly incomplete CMB map and thus lower the impact of the gaps on non-local statistical tests, we developed an inpainting algorithm on the sphere based on a sparse representation of the data, to fill in and interpolate across the masked regions. \textcopyright{} 2007 Elsevier B.V. All rights reserved.},
  keywords = {Cosmic microwave background,notion,notion-database,Overcomplete dictionary,Sparse representation,Sphere},
  file = {/Users/lbugnet/Zotero/storage/ARC4VRY9/Abrial et al. - 2008.pdf}
}

@article{Acevedo-Arreguin2013,
  title = {Dynamics of the Solar Tachocline-{{III}}. {{Numerical}} Solutions of the Gough and Mcintyre Model},
  author = {{Acevedo-Arreguin}, L. A. and Garaud, P. and Wood, T. S.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {434},
  number = {1},
  eprint = {1304.3167},
  pages = {720--741},
  issn = {00358711},
  doi = {10.1093/mnras/stt1065},
  abstract = {We present the first numerical simulations of the solar interior to exhibit a tachocline consistent with the Gough and McIntyre model. We find non-linear, axisymmetric, steady-state numerical solutions in which: (1) a large-scale primordial field is confined within the radiation zone by downwelling meridional flows that are gyroscopically pumped in the convection zone; (2) the radiation zone is in almost uniform rotation, with a rotation rate consistent with observations; (3) the bulk of the high-latitude tachocline is in thermal-wind balance, and the Lorentz force plays a negligible role in its dynamics; (4) the interaction between the field and the flows takes place within a very thin magnetic boundary layer, the tachopause, located at the bottom of the tachocline. We show that the thickness of the high-latitude tachocline scales with the amplitude of the meridional flows exactly as predicted by Gough and McIntyre. We also determine the parameter range in which such solutions can be obtained, and provide a simple explanation for the failure of previous numerical attempts at reproducing the Gough and McIntyre model. Finally, we discuss the implications of our findings for future numerical models of the solar interior, and for future observations of the Sun and other stars. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {MHD,notion,notion-database,Sun:interior,Sun:rotation},
  file = {/Users/lbugnet/Zotero/storage/R7G9J4T9/Acevedo-Arreguin, Garaud, Wood - 2013.pdf}
}

@article{Adamow2012a,
  title = {{{BD}}+48 740-{{Li}} Overabundant Giant Star with a Planet: {{A}} Case of Recent Engulfment?},
  author = {Adam{\'o}w, M. and Niedzielski, A. and Villaver, E. and Nowak, G. and Wolszczan, A.},
  year = {2012},
  journal = {Astrophysical Journal Letters},
  volume = {754},
  number = {1},
  issn = {20418205},
  doi = {10.1088/2041-8205/754/1/L15},
  abstract = {We report the discovery of a unique object, BD+48 740, a lithium overabundant giant with A(Li) = 2.33 {$\pm$} 0.04 (where A(Li) = log n Li/n H + 12), that exhibits radial velocity (RV) variations consistent with a 1.6 MJ companion in a highly eccentric, e = 0.67 {$\pm$} 0.17, and extended, a = 1.89AU (P = 771days), orbit. The high eccentricity of the planet is uncommon among planetary systems orbiting evolved stars and so is the high lithium abundance in a giant star. The ingestion by the star of a putative second planet in the system originally in a closer orbit could possibly allow for a single explanation to these two exceptional facts. If the planet candidate is confirmed by future RV observations, it might represent the first example of the remnant of a multiple planetary system recently affected by stellar evolution. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,planet-star interactions,planets and satellites: detection,stars: atmospheres,stars: fundamental parameters,stars: individual (BD+48 740),stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/YMNGEERC/Adamów et al. - 2012.pdf}
}

@article{Adelberger1998,
  title = {Solar Fusion Cross Sections},
  author = {Adelberger, Eric G. and Austin, Sam M. and Bahcall, John N. and Balantekin, A. B. and Bogaert, Gilles and Brown, Lowell S. and Buchmann, Lothar and Cecil, F. Edward and Champagne, Arthur E. and De Braeckeleer, Ludwig and Duba, Charles A. and Elliott, Steven R. and Freedman, Stuart J. and Gai, Moshe and Goldring, G. and Gould, Christopher R. and Gruzinov, Andrei and Haxton, Wick C. and Heeger, Karsten M. and Henley, Ernest and Johnson, Calvin W. and Kamionkowski, Marc and Kavanagh, Ralph W. and Koonin, Steven E. and Kubodera, Kuniharu and Langanke, Karlheinz and Motobayashi, Tohru and Pandharipande, Vijay and Parker, Peter and Robertson, R. G.H. and Rolfs, Claus and Sawyer, R. F. and Shaviv, N. and Shoppa, T. D. and Snover, K. A. and Swanson, Erik and Tribble, Robert E. and {Turck-Chi{\`e}ze}, Sylvaine and Wilkerson, John F.},
  year = {1998},
  journal = {Reviews of Modern Physics},
  volume = {70},
  number = {4 PART II},
  eprint = {astro-ph/9805121},
  pages = {1265--1291},
  issn = {00346861},
  doi = {10.1103/revmodphys.70.1265},
  abstract = {We review and analyze the available information on the nuclear-fusion cross sections that are most important for solar energy generation and solar neutrino production. We provide best values for the low-energy cross-section factors and, wherever possible, estimates of the uncertainties. We also describe the most important experiments and calculations that are required in order to improve our knowledge of solar fusion rates. \textcopyright{} 1998 The American Physical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SVTDAC9L/Adelberger et al. - 1998.pdf}
}

@article{Aerts1999,
  title = {Selection of a Sample of Bright Southern {{Slowly Pulsating B Stars}} for Long-Term Photometric and Spectroscopic Monitoring},
  author = {Aerts, C and Decat, P and Peeters, E and Decin, L and De Ridder, J and Kolenberg, K and Meeus, G and Van Winckel, H and Cuypers, J and Waelkens, C},
  year = {1999},
  journal = {ASTRONOMY AND ASTROPHYSICS},
  volume = {343},
  pages = {872--882},
  urldate = {2020-04-09},
  abstract = {The photometric experiment on Hipparcos has led to the discovery of, among other types of variables, a large amount of new Slowly Pulsating B Stars. We have selected twelve bright southern stars of this sample, together with five previously known Slowly Pulsating B Stars, for spectroscopic and photometric monitoring. These seventeen stars have spectral types ranging from B 2 up to B 9 and thus fully cover the instability strip. We here present the results of a preliminary analysis of our data and show that our sample is an extremely important one to perform seismology of intermediate-massive stars. In particular, we find that all but one of the selected stars exhibit clear line-profile variability. The broader-lined Slowly Pulsating B Stars tend to have more complex line-profile variations. One of the previously known Slowly Pulsating B stars was known to be a binary. Besides this star, another six of the selected Slowly Pulsating B stars turn out to be multiple systems. Five of these seven binaries have large rotational velocities and complicated line-profile variations with moving subfeatures. It is not yet clear whether or not the binarity results in a particular spectrum of excited modes.},
  keywords = {binaries,early-type,general-stars,notion,notion-database,oscillations-stars,spectro-scopic-stars,stars,variables},
  file = {/Users/lbugnet/Zotero/storage/8JAFKI4I/full-text.pdf}
}

@article{Aerts2008,
  title = {The Current Status of Asteroseismology},
  author = {Aerts, C. and {Christensen-Dalsgaard}, J. and Cunha, M. and Kurtz, D. W.},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  eprint = {0803.3527},
  pages = {3--20},
  issn = {00380938},
  doi = {10.1007/s11207-008-9182-z},
  abstract = {Stellar evolution, a fundamental bedrock of modern astrophysics, is driven by the physical processes in stellar interiors. While we understand these processes in general terms, we lack some important ingredients. Seemingly small uncertainties in the input physics of the models (e.g., the opacities or the amount of mixing and of interior rotation) have large consequences for the evolution of stars. The goal of asteroseismology is to improve the description of the interior physics of stars by means of their oscillations, just as global helioseismology led to a huge step forward in our knowledge about the internal structure of the Sun. In this paper we present the current status of asteroseismology by considering case studies of stars with a variety of masses and evolutionary stages. In particular, we outline how the confrontation between the observed oscillation frequencies and those predicted by the models allows us to pinpoint limitations of the input physics of current models and improve them to a level that cannot be reached with any other current method. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {Instrumentation and data management,{Interior, convective zone},{Interior, core},notion,notion-database,{Oscillations, stellar}},
  file = {/Users/lbugnet/Zotero/storage/QKU5RUB8/Aerts et al. - 2008.pdf}
}

@book{Aerts2010,
  title = {Asteroseismology},
  author = {Aerts, C. and {Christensen-Dalsgaard}, J. and Kurtz, D. W.},
  year = {2010},
  publisher = {{Springer Netherlands}},
  address = {{Dordrecht}},
  doi = {10.1007/978-1-4020-5803-5},
  urldate = {2020-03-03},
  isbn = {978-1-4020-5178-4},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9SZ3T554/full-text.pdf}
}

@article{Aerts2015,
  title = {The Age and Interior Rotation of Stars from Asteroseismology},
  author = {Aerts, C.},
  year = {2015},
  journal = {Astronomische Nachrichten},
  volume = {336},
  number = {5},
  eprint = {1503.06690},
  pages = {477--486},
  issn = {15213994},
  doi = {10.1002/asna.201512177},
  abstract = {We provide a status report on the determination of stellar ages from asteroseismology for stars of various masses and evolutionary stages. The ability to deduce the ages of stars with a relative precision of typically 10 to 20\% is a unique opportunity for stellar evolution and also of great value for both galactic and exoplanet studies. Further, a major uncalibrated ingredient that makes stellar evolution models uncertain, is the stellar interior rotation frequency {$\Omega$}(r) and its evolution during stellar life. We summarize the recent achievements in the derivation of {$\Omega$}(r) for different types stars, offering stringent observational constraints on theoretical models. Core-to-envelope rotation rates during the red-giant stage are far lower than theoretical predictions, pointing towards the need to include new physical ingredients that allow strong and efficient coupling between the core and the envelope in the models of low-mass stars in the evolutionary phase prior to core helium burning. Stars are subject to efficient mixing phenomena, even at low rotation rates. Young massive stars with seismically determined interior rotation frequency reveal low core-to-envelope rotation values. (\textcopyright{} 2015 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim).},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,stars: evolution,stars: interiors,stars: oscillations,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/WPVWBDUH/Aerts - 2015.pdf}
}

@techreport{Aerts2018,
  title = {Angular {{Momentum Transport}} in {{Stellar Interiors}}},
  author = {Aerts, Conny and Mathis, St{\'e}phane and Rogers, Tamara M},
  year = {2018},
  eprint = {1809.07779v1},
  doi = {10.1146/((please)},
  urldate = {2020-03-04},
  abstract = {Stars lose a significant amount of angular momentum between birth and death, implying that efficient processes transporting it from the core to the surface are active. Space asteroseismology delivered the interior rotation rates of more than a thousand low-and intermediate-mass stars, revealing that: 1) single stars rotate nearly uniformly during the core hydrogen and core helium burning phases; 2) stellar cores spin up to a factor 10 faster than the envelope during the red giant phase; 3) the angular momentum of the helium-burning core of stars is in agreement with the angular momentum of white dwarfs. Observations reveal a strong decrease of core angular momentum when stars have a con-vective core. Current theory of angular momentum transport fails to explain this. We propose improving the theory with a data-driven approach , whereby angular momentum prescriptions derived from multi-dimensional (magneto)hydrodynamical simulations and theoretical considerations are continously tested against modern observations. The TESS and PLATO space missions have the potential to derive the interior rotation of large samples of stars, including high-mass and metal-poor stars in binaries and clusters. This will provide the powerful observational constraints needed to improve theory and simulations.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,stars: evolution,stars: interiors,stars: oscillations (including pulsations),stars: rotation,waves},
  file = {/Users/lbugnet/Zotero/storage/NUVZ5HTL/full-text.pdf}
}

@article{Aerts2019,
  title = {Angular {{Momentum Transport}} in {{Stellar Interiors}}},
  author = {Aerts, Conny and Mathis, St{\'e}phane and Rogers, Tamara M},
  year = {2019},
  month = nov,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {57},
  pages = {35},
  issn = {['0066-4146']},
  doi = {10.1146/annurev-astro-091918-104359},
  abstract = {Stars lose a significant amount of angular momentum between birth and death, implying that efficient processes transporting it from the core to the surface are active. Space asteroseismology delivered the interior rotation rates of more than a thousand low- and intermediate-mass stars, revealing the following: Single stars rotate nearly uniformly during the core-hydrogen and core-helium burning phases. Stellar cores spin up to a factor of 10 faster than the envelope during the red giant phase. The angular momentum of the helium-burning core of stars is in agreement with the angular momentum of white dwarfs.Observations reveal a strong decrease of core angular momentum when stars have a convective core. Current theory of angular momentum transport fails to explain this. We propose improving the theory with a data-driven approach, whereby angular momentum prescriptions derived frommultidimensional (magneto)hydrodynamical simulations and theoretical considerations are continuously tested against modern observations. The TESS and PLATO space missions have the potential to derive the interior rotation of large samples of stars, including high-mass and metal-poor stars in binaries and clusters. This will provide the powerful observational constraints needed to improve theory and simulations.},
  langid = {english},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/D78L8QPP/m-api-1374c832-479d-fc1d-1a77-e15dbb95014a.pdf}
}

@article{Aerts2019a,
  title = {Angular {{Momentum Transport}} in {{Stellar Interiors}}},
  author = {Aerts, Conny and Mathis, St{\'e}phane and Rogers, Tamara M.},
  year = {2019},
  month = aug,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {57},
  number = {1},
  eprint = {1809.07779},
  pages = {35--78},
  publisher = {{Annual Reviews}},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-091918-104359},
  abstract = {Stars lose a significant amount of angular momentum between birth and death, implying that efficient processes transporting it from the core to the surface are active. Space asteroseismology delivered the interior rotation rates of more than a thousand low- and intermediate-mass stars, revealing the following: {$\blacksquare$} Single stars rotate nearly uniformly during the core-hydrogen and core-helium burning phases. {$\blacksquare$} Stellar cores spin up to a factor of 10 faster than the envelope during the red giant phase. {$\blacksquare$} The angular momentum of the helium-burning core of stars is in agreement with the angular momentum of white dwarfs. Observations reveal a strong decrease of core angular momentum when stars have a convective core. Current theory of angular momentum transport fails to explain this. We propose improving the theory with a data-driven approach, whereby angular momentum prescriptions derived frommultidimensional (magneto)hydrodynamical simulations and theoretical considerations are continuously tested against modern observations. The TESS and PLATO space missions have the potential to derive the interior rotation of large samples of stars, including high-mass and metal-poor stars in binaries and clusters. This will provide the powerful observational constraints needed to improve theory and simulations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@techreport{Aerts2019b,
  title = {Probing the Interior Physics of Stars through Asteroseismology},
  author = {Aerts, C.},
  year = {2019},
  month = dec,
  eprint = {1912.12300},
  urldate = {2020-03-09},
  abstract = {Years-long high-precision brightness measurements assembled with telescopes operating in space have become available for thousands of stars. Such data made it possible to measure the physics of stellar interiors via nonradial oscillations, opening a new avenue to study the stars in the Universe. Asteroseismology, the interpretation of the characteristics of oscillation modes in terms of the physical properties of the stellar interior, brought entirely new insights in how stars rotate and how they build up their chemistry throughout their evolution. We discuss how data-driven space asteroseismology has allowed us to improve our knowledge of stellar physics. This delivered a drastic increase in the reliability of computer models mimicking the evolution of stars born with a variety of masses and metalicities. Such models are critical ingredients for modern physics as a whole, because they are used throughout various contemporary and multidisciplinary research fields in space science, including the search for life outside the solar system, archeological studies of the Milky Way, and supernova explosions of single and binary stars, among which future gravitational wave sources. We illustrate the specific role and potential of asteroseismology for those modern research fields. We end with current limitations of asteroseismology and highlight how they can be overcome with ongoing and future large infrastructures for survey astronomy combined with new theoretical research in the era of high-performance computing. This review presents some of the results obtained thanks to major community efforts over the past decade. These breakthroughs were achieved in a collaborative and inclusive spirit so characteristic of the asteroseismology community. The aim was to write it in a way so as to make this research field well accessible.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Aerts2021,
  title = {Probing the Interior Physics of Stars through Asteroseismology},
  author = {Aerts, C.},
  year = {2021},
  month = jan,
  journal = {Reviews of Modern Physics},
  volume = {93},
  number = {1},
  eprint = {1912.12300},
  pages = {015001},
  publisher = {{American Physical Society}},
  issn = {15390756},
  doi = {10.1103/RevModPhys.93.015001},
  urldate = {2022-01-20},
  abstract = {Yearslong time series of high-precision brightness measurements have been assembled for thousands of years with telescopes operating in space. Such data have allowed astronomers to measure the physics of stellar interiors via nonradial oscillations, opening a new avenue to study the stars in the Universe. Asteroseismology, the interpretation of the characteristics of oscillation modes in terms of the physical properties of the stellar interior, brought entirely new insights in how stars rotate and how they build up their chemistry throughout their evolution. Data-driven space asteroseismology has delivered a drastic increase in the reliability of computer models mimicking the evolution of stars born with a variety of masses and metallicities. Such models are critical ingredients for modern physics as a whole because they are used throughout various contemporary and multidisciplinary research fields in space science, including the search for life outside the Solar System, archaeological studies of the Milky Way, and the study of single and binary supernova progenitors, among which are future gravitational wave sources. The specific role and potential of asteroseismology for those modern research fields are illustrated. The review concludes with current limitations of asteroseismology and highlights how they can be overcome with ongoing and future large infrastructures for survey astronomy combined with new theoretical research in the era of high-performance computing. This review presents results obtained through major community efforts over the past decade. These breakthroughs were achieved in a collaborative and inclusive spirit that is characteristic of the asteroseismology community. The review's aim is to make this research field accessible to graduate students and readers coming from other fields of physics, with incentives to enjoy and join future applications in this domain of astrophysics.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics}
}

@article{Aerts2021a,
  title = {Probing the Interior Physics of Stars through Asteroseismology},
  author = {Aerts, C.},
  year = {2021},
  month = jan,
  journal = {Reviews of Modern Physics},
  volume = {93},
  pages = {015001},
  issn = {0034-6861},
  doi = {10.1103/RevModPhys.93.015001},
  urldate = {2023-09-28},
  abstract = {Yearslong time series of high-precision brightness measurements have been assembled for thousands of stars with telescopes operating in space. Such data have allowed astronomers to measure the physics of stellar interiors via nonradial oscillations, opening a new avenue to study the stars in the Universe. Asteroseismology, the interpretation of the characteristics of oscillation modes in terms of the physical properties of the stellar interior, brought entirely new insights in how stars rotate and how they build up their chemistry throughout their evolution. Data-driven space asteroseismology has delivered a drastic increase in the reliability of computer models mimicking the evolution of stars born with a variety of masses and metallicities. Such models are critical ingredients for modern physics as a whole because they are used throughout various contemporary and multidisciplinary research fields in space science, including the search for life outside the Solar System, archaeological studies of the Milky Way, and the study of single and binary supernova progenitors, among which are future gravitational wave sources. The specific role and potential of asteroseismology for those modern research fields are illustrated. The review concludes with current limitations of asteroseismology and highlights how they can be overcome with ongoing and future large infrastructures for survey astronomy combined with new theoretical research in the era of high-performance computing. This review presents results obtained through major community efforts over the past decade. These breakthroughs were achieved in a collaborative and inclusive spirit that is characteristic of the asteroseismology community. The review's aim is to make this research field accessible to graduate students and readers coming from other fields of physics, with incentives to enjoy and join future applications in this domain of astrophysics.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2021RvMP...93a5001A},
  file = {/Users/lbugnet/Zotero/storage/59PLNM7A/Aerts - 2021 - Probing the interior physics of stars through aste.pdf;/Users/lbugnet/Zotero/storage/5FN2M47U/Aerts - 2021 - Probing the interior physics of stars through aste.pdf}
}

@article{Aerts2023,
  title = {Mode Coupling Coefficients between the Convective Core and Radiative Envelope of {\emph{{$\gamma$}}} {{Doradus}} and Slowly Pulsating {{B}} Stars},
  author = {Aerts, C. and Mathis, S.},
  year = {2023},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {677},
  pages = {A68},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202347196},
  urldate = {2023-09-28},
  abstract = {Methods. We used asteroseismic forward models of two samples consisting of 26 SPB stars and 37 {$\gamma$} Dor stars to infer their numerical values of {$\epsilon$} and {$\epsilon$}\texttildelow. For both samples, we also computed: the linear correlation coefficients between {$\epsilon$} or {$\epsilon$}\texttildelow{} and the near-core rotation frequency, the chemical gradient, the evolutionary stage, the convective core masses and radii, and the Sch\"onberg-Chandrasekhar limiting mass representing the maximum mass of an inert helium core at central hydrogen exhaustion that can still withstand the pressure of the overlaying envelope. Results. The asteroseismically inferred values of {$\epsilon$} and {$\epsilon$}\texttildelow{} for the two samples are between 0.0 and 0.34. While {$\epsilon$} is most strongly correlated with the near-core rotation frequency for {$\gamma$} Dor stars, the fractional radius of the convective core instead provides the tightest correlation for SPB stars. We find {$\epsilon$} to decrease mildly as the stars evolve. For the SPB stars, {$\epsilon$} and {$\epsilon$}\texttildelow{} have similar moderate correlations with respect to the core properties. For the {$\gamma$} Dor stars, {$\epsilon$}\texttildelow{} reveals systematically lower and often no correlation to the core properties; their {$\epsilon$} is mainly determined by the near-core rotation frequency. The Sch\"onberg-Chandrasekar limit is already surpassed by the more massive SPB stars, while none of the {$\gamma$} Dor stars have reached it yet. Conclusions. Our asteroseismic results for the mode coupling support the theoretical interpretation and reveal that young, fast-rotating {$\gamma$} Dor stars are most suitable for undergoing couplings between inertial modes in the rotating convective core and gravito-inertial modes in the radiative envelope. The phenomenon has been found in 2.4\% of such pulsators with detected period spacing patterns, whereas it has not been seen in any of the SPB stars so far.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/Y8FQ5LJN/Aerts and Mathis - 2023 - Mode coupling coefficients between the convective .pdf}
}

@article{Agnew2002,
  title = {History of {{Seismology}}},
  author = {Agnew, Duncan Carr},
  year = {2002},
  journal = {International Geophysics},
  volume = {81},
  pages = {3--11},
  urldate = {2020-02-28},
  isbn = {0124406521},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TQKLXTEX/full-text.pdf}
}

@techreport{agnolonPLATODefinitionsMethodology2015,
  title = {{{PLATO}} Definitions and Methodology Handbook {{Title PLATO}} Definitions and Methodology Handbook {{Issue}} 1},
  author = {Agnolon, D and Heras Heike Rauer, Ana},
  year = {2015},
  urldate = {2021-04-06},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JMIFSAAR/full-text.pdf}
}

@article{Aguirre2014,
  title = {Old Puzzle, New Insights: {{A}} Lithium-Rich Giant Quietly Burning Helium in Its Core},
  author = {Aguirre, V. Silva and Ruchti, G. R. and Hekker, S. and Cassisi, S. and {Christensen-Dalsgaard}, J. and Datta, A. and Jendreieck, A. and {Jessen-Hansen}, J. and Mazumdar, A. and Mosser, B. and Stello, D. and Beck, P. G. and De Ridder, J.},
  year = {2014},
  journal = {Astrophysical Journal Letters},
  volume = {784},
  number = {1},
  issn = {20418205},
  doi = {10.1088/2041-8205/784/1/L16},
  abstract = {About 1\% of giant stars have been shown to have large surface Li abundances, which is unexpected according to standard stellar evolution models. Several scenarios for lithium production have been proposed, but it is still unclear why these Li-rich giants exist. A missing piece in this puzzle is the knowledge of the exact stage of evolution of these stars. Using low- and-high-resolution spectroscopic observations, we have undertaken a survey of lithium-rich giants in the Kepler field. In this Letter, we report the finding of the first confirmed Li-rich core-helium-burning giant, as revealed by asteroseismic analysis. The evolutionary timescales constrained by its mass suggest that Li production most likely took place through non-canonical mixing at the RGB tip, possibly during the helium flash. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  keywords = {asteroseismology,notion,notion-database,stars: abundances,stars: individual (KIC 5000307),stars: late-type,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/CLVWIIW3/Aguirre et al. - 2014.pdf}
}

@article{Aguirre2016,
  title = {Standing on the Shoulders of {{Dwarfs}}: The {{Kepler}} Asteroseismic {{LEGACY}} Sample {{II}} - Radii, Masses, and Ages},
  author = {Aguirre, Victor Silva and Lund, Mikkel N. and Antia, H. M. and Ball, Warrick H. and Basu, Sarbani and {Christensen-Dalsgaard}, J{\o}rgen and Lebreton, Yveline and Reese, Daniel R. and Verma, Kuldeep and Casagrande, Luca and Justesen, Anders B. and Mosumgaard, Jakob R. and Chaplin, William J. and Bedding, Timothy R. and Davies, Guy R. and Handberg, Rasmus and Houdek, G{\"u}nter and Huber, Daniel and Kjeldsen, Hans and Latham, David W. and White, Timothy R. and Coelho, Hugo R. and Miglio, Andrea and Rendle, Ben},
  year = {2016},
  month = nov,
  eprint = {1611.08776},
  doi = {10.3847/1538-4357/835/2/173},
  urldate = {2020-07-04},
  abstract = {We use asteroseismic data from the Kepler satellite to determine fundamental stellar properties of the 66 main-sequence targets observed for at least one full year by the mission. We distributed tens of individual oscillation frequencies extracted from the time series of each star among seven modelling teams who applied different methods to determine radii, masses, and ages for all stars in the sample. Comparisons among the different results reveal a good level of agreement in all stellar properties, which is remarkable considering the variety of codes, input physics and analysis methods employed by the different teams. Average uncertainties are of the order of \$\textbackslash sim\$2\textbackslash\% in radius, \$\textbackslash sim\$4\textbackslash\% in mass, and \$\textbackslash sim\$10\textbackslash\% in age, making this the best-characterised sample of main-sequence stars available to date. Our predicted initial abundances and mixing-length parameters are checked against inferences from chemical enrichment laws \$\textbackslash Delta Y / \textbackslash Delta Z\$ and predictions from 3D atmospheric simulations. We test the accuracy of the determined stellar properties by comparing them to the Sun, angular diameter measurements, Gaia parallaxes, and binary evolution, finding excellent agreement in all cases and further confirming the robustness of asteroseismically-determined physical parameters of stars when individual frequencies of oscillation are available. Baptised as the Kepler dwarfs LEGACY sample, these stars are the solar-like oscillators with the best asteroseismic properties available for at least another decade. All data used in this analysis and the resulting stellar parameters are made publicly available for the community.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DJZP4LXV/full-text.pdf}
}

@article{Aguirre2017,
  title = {Standing on the {{Shoulders}} of {{Dwarfs}}: The {{Kepler Asteroseismic LEGACY Sample}}. {{II}}. {{Radii}}, {{Masses}}, and {{Ages}}},
  author = {Aguirre, V{\'i}ctor Silva and Lund, Mikkel N. and Antia, H. M. and Ball, Warrick H. and Basu, Sarbani and {Christensen-Dalsgaard}, J{\o}rgen and Lebreton, Yveline and Reese, Daniel R. and Verma, Kuldeep and Casagrande, Luca and Justesen, Anders B. and Mosumgaard, Jakob R. and Chaplin, William J. and Bedding, Timothy R. and Davies, Guy R. and Handberg, Rasmus and Houdek, G{\"u}nter and Huber, Daniel and Kjeldsen, Hans and Latham, David W. and White, Timothy R. and Coelho, Hugo R. and Miglio, Andrea and Rendle, Ben},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {835},
  number = {2},
  eprint = {1611.08776},
  pages = {173},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/835/2/173},
  abstract = {We use asteroseismic data from the Kepler satellite to determine fundamental stellar properties of the 66 main-sequence targets observed for at least one full year by the mission. We distributed tens of individual oscillation frequencies extracted from the time series of each star among seven modelling teams who applied different methods to determine radii, masses, and ages for all stars in the sample. Comparisons among the different results reveal a good level of agreement in all stellar properties, which is remarkable considering the variety of codes, input physics and analysis methods employed by the different teams. Average uncertainties are of the order of \$\textbackslash sim\$2\textbackslash\% in radius, \$\textbackslash sim\$4\textbackslash\% in mass, and \$\textbackslash sim\$10\textbackslash\% in age, making this the best-characterised sample of main-sequence stars available to date. Our predicted initial abundances and mixing-length parameters are checked against inferences from chemical enrichment laws \$\textbackslash Delta Y / \textbackslash Delta Z\$ and predictions from 3D atmospheric simulations. We test the accuracy of the determined stellar properties by comparing them to the Sun, angular diameter measurements, Gaia parallaxes, and binary evolution, finding excellent agreement in all cases and further confirming the robustness of asteroseismically-determined physical parameters of stars when individual frequencies of oscillation are available. Baptised as the Kepler dwarfs LEGACY sample, these stars are the solar-like oscillators with the best asteroseismic properties available for at least another decade. All data used in this analysis and the resulting stellar parameters are made publicly available for the community.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JA4FNLWH/Aguirre et al. - 2017.pdf}
}

@article{Aguirre2019,
  title = {Detection and Characterisation of Oscillating Red Giants: First Results from the {{TESS}} Satellite},
  author = {Aguirre, V{\'i}ctor Silva and Stello, Dennis and Stokholm, Amalie and Mosumgaard, Jakob R. and Ball, Warrick and Basu, Sarbani and Bossini, Diego and Bugnet, Lisa and Buzasi, Derek and Campante, Tiago L. and Carboneau, Lindsey and Chaplin, William J. and Corsaro, Enrico and Davies, Guy R. and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Gaulme, Patrick and Hall, Oliver J. and Handberg, Rasmus and Hon, Marc and Kallinger, Thomas and Kang, Liu and Lund, Mikkel N. and Mathur, Savita and Mints, Alexey and Mosser, Benoit and Orhan, Zeynep {\c C}elik and Rodrigues, Tha{\'i}se S. and Vrard, Mathieu and Y{\i}ld{\i}z, Mutlu and Zinn, Joel C. and {\"O}rtel, Sibel and Beck, Paul G. and Bell, Keaton J. and Guo, Zhao and Jiang, Chen and Kuszlewicz, James S. and Kuehn, Charles A. and Li, Tanda and Lundkvist, Mia S. and Pinsonneault, Marc and Tayar, Jamie and Cunha, Margarida S. and Hekker, Saskia and Huber, Daniel and Miglio, Andrea and Monteiro, Mario J. P. F. G. and Slumstrup, Ditte and Winther, Mark L. and Angelou, George and Benomar, Othman and B{\'o}di, Attila and De Moura, Bruno L. and Deheuvels, S{\'e}bastien and Derekas, Aliz and Di Mauro, Maria Pia and Dupret, Marc-Antoine and Jim{\'e}nez, Antonio and Lebreton, Yveline and Matthews, Jaymie and Nardetto, Nicolas and do Nascimento,, Jose D. and Pereira, Filipe and D{\'i}az, Luisa F. Rodr{\'i}guez and Serenelli, Aldo M. and Spitoni, Emanuele and Stonkut{\.e}, Edita and Su{\'a}rez, Juan Carlos and Szab{\'o}, Robert and Van Eylen, Vincent and Ventura, Rita and Verma, Kuldeep and Weiss, Achim and Wu, Tao and Barclay, Thomas and {Christensen-Dalsgaard}, J{\o}rgen and Jenkins, Jon M. and Kjeldsen, Hans and Ricker, George R. and Seager, Sara and Vanderspek, Roland},
  year = {2019},
  month = dec,
  eprint = {1912.07604},
  doi = {10.3847/2041-8213/ab6443},
  urldate = {2020-06-19},
  abstract = {Since the onset of the `space revolution' of high-precision high-cadence photometry, asteroseismology has been demonstrated as a powerful tool for informing Galactic archaeology investigations. The launch of the NASA TESS mission has enabled seismic-based inferences to go full sky -- providing a clear advantage for large ensemble studies of the different Milky Way components. Here we demonstrate its potential for investigating the Galaxy by carrying out the first asteroseismic ensemble study of red giant stars observed by TESS. We use a sample of 25 stars for which we measure their global asteroseimic observables and estimate their fundamental stellar properties, such as radius, mass, and age. Significant improvements are seen in the uncertainties of our estimates when combining seismic observables from TESS with astrometric measurements from the Gaia mission compared to when the seismology and astrometry are applied separately. Specifically, when combined we show that stellar radii can be determined to a precision of a few percent, masses to 5-10\% and ages to the 20\% level. This is comparable to the precision typically obtained using end-of-mission Kepler data},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NFHZMIBQ/Aguirre et al. - 2019(2).pdf;/Users/lbugnet/Zotero/storage/P7ULIKGA/full-text.pdf}
}

@article{Ahlborn2020,
  title = {Asteroseismic Sensitivity to Internal Rotation along the Red-Giant Branch},
  author = {Ahlborn, F. and Bellinger, E. P. and Hekker, S. and Basu, S. and Angelou, G. C.},
  year = {2020},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {639},
  pages = {A98},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201936947},
  urldate = {2023-11-06},
  abstract = {Context. Transport of angular momentum in stellar interiors is currently not well understood. Asteroseismology can provide us with estimates of internal rotation of stars and thereby advances our understanding of angular momentum transport. Aims: We can measure core-rotation rates in red-giant stars and we can place upper bounds on surface-rotation rates using measurements of dipole (l = 1) modes. Here, we aim to determine the theoretical sensitivity of modes of different spherical degree towards the surface rotation. Additionally, we aim to identify modes that can potentially add sensitivity at intermediate radii. Methods: We used asteroseismic rotational inversions to probe the internal stellar rotation profiles in red-giant models from the base of the red-giant branch up to the luminosity bump. We used the inversion method of multiplicative optimally localised averages to assess how well internal and surface rotation rates can be recovered from different mode sets and different synthetic rotation profiles. Results: We confirm that dipole mixed modes are sufficient to set constraints on the average core-rotation rates in red giants. However, surface-rotation rates estimated with only dipole mixed modes are contaminated by the core rotation. We show that the sensitivity to surface rotation decreases from the base of the red-giant branch until it reaches a minimum at 60-80\% of the bump luminosity due to a glitch in the buoyancy frequency. Thereafter, a narrow range of increased surface sensitivity just below the bump luminosity exists. Quadrupole and octopole modes have more sensitivity in the outer parts of the star. To obtain accurate estimates of rotation rates at intermediate radii (i.e. a fractional radius of {$\sim$}0.4), acoustic oscillation modes with a spherical degree of l {$\approx$} 10 are needed. Conclusions: We find a minimum and subsequent maximum in the sensitivity to the surface rotation rate in red giants below the luminosity bump. Furthermore, we show that, if observed, quadrupole and octopole modes enable us to distinguish between differential and solid body rotation in the convection zone. This will be important when investigating the transport of angular momentum between the core and the envelope.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2020A\&A...639A..98A},
  file = {/Users/lbugnet/Zotero/storage/ICSEN7XH/Ahlborn et al. - 2020 - Asteroseismic sensitivity to internal rotation alo.pdf}
}

@article{ahlbornAsteroseismicSensitivityInternal2020,
  title = {Asteroseismic Sensitivity to Internal Rotation along the Red-Giant Branch},
  author = {Ahlborn, F. and Bellinger, E. P. and Hekker, S. and Basu, S. and Angelou, G. C.},
  year = {2020},
  month = jul,
  journal = {Astronomy and Astrophysics},
  volume = {639},
  pages = {A98},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201936947},
  urldate = {2023-05-28},
  abstract = {Context. Transport of angular momentum in stellar interiors is currently not well understood. Asteroseismology can provide us with estimates of internal rotation of stars and thereby advances our understanding of angular momentum transport. Aims: We can measure core-rotation rates in red-giant stars and we can place upper bounds on surface-rotation rates using measurements of dipole (l = 1) modes. Here, we aim to determine the theoretical sensitivity of modes of different spherical degree towards the surface rotation. Additionally, we aim to identify modes that can potentially add sensitivity at intermediate radii. Methods: We used asteroseismic rotational inversions to probe the internal stellar rotation profiles in red-giant models from the base of the red-giant branch up to the luminosity bump. We used the inversion method of multiplicative optimally localised averages to assess how well internal and surface rotation rates can be recovered from different mode sets and different synthetic rotation profiles. Results: We confirm that dipole mixed modes are sufficient to set constraints on the average core-rotation rates in red giants. However, surface-rotation rates estimated with only dipole mixed modes are contaminated by the core rotation. We show that the sensitivity to surface rotation decreases from the base of the red-giant branch until it reaches a minimum at 60-80\% of the bump luminosity due to a glitch in the buoyancy frequency. Thereafter, a narrow range of increased surface sensitivity just below the bump luminosity exists. Quadrupole and octopole modes have more sensitivity in the outer parts of the star. To obtain accurate estimates of rotation rates at intermediate radii (i.e. a fractional radius of {$\sim$}0.4), acoustic oscillation modes with a spherical degree of l {$\approx$} 10 are needed. Conclusions: We find a minimum and subsequent maximum in the sensitivity to the surface rotation rate in red giants below the luminosity bump. Furthermore, we show that, if observed, quadrupole and octopole modes enable us to distinguish between differential and solid body rotation in the convection zone. This will be important when investigating the transport of angular momentum between the core and the envelope.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2020A\&A...639A..98A},
  file = {/Users/lbugnet/Zotero/storage/8R6BXJ87/Ahlborn et al. - 2020 - Asteroseismic sensitivity to internal rotation alo.pdf}
}

@article{ahlbornAsteroseismicSensitivityInternal2020a,
  title = {Asteroseismic Sensitivity to Internal Rotation along the Red-Giant Branch},
  author = {Ahlborn, F. and Bellinger, E. P. and Hekker, S. and Basu, S. and Angelou, G. C.},
  year = {2020},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {639},
  pages = {A98},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201936947},
  urldate = {2023-06-01},
  abstract = {Methods. We used asteroseismic rotational inversions to probe the internal stellar rotation profiles in red-giant models from the base of the red-giant branch up to the luminosity bump. We used the inversion method of multiplicative optimally localised averages to assess how well internal and surface rotation rates can be recovered from different mode sets and different synthetic rotation profiles. Results. We confirm that dipole mixed modes are sufficient to set constraints on the average core-rotation rates in red giants. However, surface-rotation rates estimated with only dipole mixed modes are contaminated by the core rotation. We show that the sensitivity to surface rotation decreases from the base of the red-giant branch until it reaches a minimum at 60\textendash 80\% of the bump luminosity due to a glitch in the buoyancy frequency. Thereafter, a narrow range of increased surface sensitivity just below the bump luminosity exists. Quadrupole and octopole modes have more sensitivity in the outer parts of the star. To obtain accurate estimates of rotation rates at intermediate radii (i.e. a fractional radius of {$\sim$}0.4), acoustic oscillation modes with a spherical degree of l {$\approx$} 10 are needed. Conclusions. We find a minimum and subsequent maximum in the sensitivity to the surface rotation rate in red giants below the luminosity bump. Furthermore, we show that, if observed, quadrupole and octopole modes enable us to distinguish between differential and solid body rotation in the convection zone. This will be important when investigating the transport of angular momentum between the core and the envelope.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/3F2FJA78/Ahlborn et al. - 2020 - Asteroseismic sensitivity to internal rotation alo.pdf}
}

@article{Ahmad2001,
  title = {Measurement of the Rate of ve + d \textrightarrow{} p + p + E- Interactions Produced by {{8B}} Solar Neutrinos at the Sudbury Neutrino Observatory},
  author = {Ahmad, Q. R. and Allen, R. C. and Andersen, T. C. and Anglin, J. D. and B{\"u}hler, G. and Barton, J. C. and Beier, E. W. and Bercovitch, M. and Bigu, J. and Biller, S. and Black, R. A. and Blevis, I. and Boardman, R. J. and Boger, J. and Bonvin, E. and Boulay, M. G. and Bowler, M. G. and Bowles, T. J. and Brice, S. J. and Browne, M. C. and Bullard, T. V. and Burritt, T. H. and Cameron, K. and Cameron, J. and Chan, Y. D. and Chen, M. and Chen, H. H. and Chen, X. and Chon, M. C. and Cleveland, B. T. and Clifford, E. T.H. and Cowan, J. H.M. and Cowen, D. F. and Cox, G. A. and Dai, Y. and Dai, X. and {Dalnoki-Veress}, F. and Davidson, W. F. and Doe, P. J. and Doucas, G. and Dragowsky, M. R. and Duba, C. A. and Duncan, F. A. and Dunmore, J. and Earle, E. D. and Elliott, S. R. and Evans, H. C. and Ewan, G. T. and Farine, J. and Fergani, H. and Ferraris, A. P. and Ford, R. J. and Fowler, M. M. and Frame, K. and Frank, E. D. and Frati, W. and Germani, J. V. and Gil, S. and Goldschmidt, A. and Grant, D. R. and Hahn, R. L. and Hallin, A. L. and Hallman, E. D. and Hamer, A. and Hamian, A. A. and Haq, R. U. and Hargrove, C. K. and Harvey, P. J. and Hazama, R. and Heaton, R. and Heeger, K. M. and Heintzelman, W. J. and Heise, J. and Helmer, R. L. and Hepburn, J. D. and Heron, H. and Hewett, J. and Hime, A. and Howe, M. and Hykawy, J. G. and Isaac, M. C.P. and Jagam, P. and Jelley, N. A. and Jillings, C. and Jonkmans, G. and Karn, J. and Keener, P. T. and Kirch, K. and Klein, J. R. and Knox, A. B. and Komar, R. J. and Kouzes, R. and Kutter, T. and Kyba, C. C.M. and Law, J. and Lawson, I. T. and Lay, M. and Lee, H. W. and Lesko, K. T. and Leslie, J. R. and Levine, I. and Locke, W. and Lowry, M. M. and Luoma, S. and Lyon, J. and Majerus, S. and Mak, H. B. and Marino, A. D. and McCauley, N. and McDonald, A. B. and McDonald, D. S. and McFarlane, K. and McGregor, G. and McLatchie, W. and Drees Meijer, R. and Mes, H. and Mifflin, C. and Miller, G. G. and Milton, G. and Moffat, B. A. and Moorhead, M. and Nally, C. W. and Neubauer, M. S. and Newcomer, F. M. and Ng, H. S. and Noble, A. J. and Norman, E. B. and Novikov, V. M. and O'Neill, M. and Okada, C. E. and Ollerhead, R. W. and Omori, M. and Orrell, J. L. and Oser, S. M. and Poon, A. W.P. and Radcliffe, T. J. and Roberge, A. and Robertson, B. C. and Robertson, R. G.H. and Rowley, J. K. and Rusu, V. L. and Saettler, E. and Schaffer, K. K. and Schuelke, A. and Schwendener, M. H. and Seifert, H. and Shatkay, M. and Simpson, J. J. and Sinclair, D. and Skensved, P. and Smith, A. R. and Smith, M. W.E. and Starinsky, N. and Steiger, T. D. and Stokstad, R. G. and Storey, R. S. and Sur, B. and Tafirout, R. and Tagg, N. and Tanner, N. W. and Taplin, R. K. and Thorman, M. and Thornewell, P. and Trent, P. T. and Tserkovnyak, Y. I. and Van Berg, R. and {Van de Water}, R. G. and Virtue, C. J. and Waltham, C. E. and Wang, J. X. and Wark, D. L. and West, N. and Wilhelmy, J. B. and Wilkerson, J. F. and Wilson, J. and Wittich, P. and Wouters, J. M. and Yeh, M.},
  year = {2001},
  journal = {Physical Review Letters},
  volume = {87},
  number = {7},
  eprint = {nucl-ex/0106015},
  pages = {71301-1-71301-4},
  issn = {10797114},
  doi = {10.1103/PhysRevLett.87.071301},
  abstract = {Solar neutrinos from 8B decay have been detected at the Sudbury Neutrino Observatory via the charged current (CC) reaction on deuterium and the elastic scattering (ES) of electrons. The flux of {$\nu$}e's is measured by the CC reaction rate to be {$\varphi$}CC(ve) = 1.75 {$\pm$} 0.07(stat)+0.12-0.11(syst) {$\pm$} 0.05(theor) \texttimes{} 106 cm-2s-1. Comparison of {$\varphi$}CC(ve) to the Super-Kamiokande Collaboration's precision value of the flux inferred from the ES reaction yields a 3.3{$\sigma$} difference, assuming the systematic uncertainties are normally distributed, providing evidence of an active non-ve component in the solar flux. The total flux of active 8B neutrinos is determined to be 5.44 {$\pm$} 0.99 \texttimes{} 106 cm-2s-1. \textcopyright{} 2001 The American Physical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2JD88HAB/Ahmad et al. - 2001.pdf}
}

@article{Ahuir2021,
  title = {Magnetic and Tidal Migration of Close-in Planets. {{Influence}} of Secular Evolution on Their Population},
  author = {Ahuir, J. and Strugarek, A. and Brun, A. -S. and Mathis, S.},
  year = {2021},
  month = jun,
  journal = {Astronomy \& Astrophysics},
  volume = {650},
  pages = {A126},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202040173},
  urldate = {2023-11-04},
  abstract = {Context. Over the last two decades, a large population of close-in planets has been detected around a wide variety of host stars. Such exoplanets are likely to undergo planetary migration through magnetic and tidal interactions. Aims: We aim to follow the orbital evolution of a planet along the structural and rotational evolution of its host star, simultaneously taking into account tidal and magnetic torques, in order to explain some properties of the distribution of observed close-in planets. Methods: We rely on a numerical model of a coplanar circular star-planet system called ESPEM, which takes into account stellar structural changes, wind braking, and star-planet interactions. We browse the parameter space of the star-planet system configurations and assess the relative influence of magnetic and tidal torques on its secular evolution. We then synthesize star-planet populations and compare their distribution in orbital and stellar rotation periods to Kepler satellite data. Results: Magnetic and tidal interactions act together on planetary migration and stellar rotation. Furthermore, both interactions can dominate secular evolution depending on the initial configuration of the system and the evolutionary phase considered. Indeed, tidal effects tend to dominate for high stellar and planetary masses as well as low semi-major axis; they also govern the evolution of planets orbiting fast rotators while slower rotators evolve essentially through magnetic interactions. Moreover, three populations of star-planet systems emerge from the combined action of both kinds of interactions. First, systems undergoing negligible migration define an area of influence of star-planet interactions. For sufficiently large planetary magnetic fields, the magnetic torque determines the extension of this region. Next, planets close to fast rotators migrate efficiently during the pre-main sequence, which engenders a depleted region at low rotation and orbital periods. Then, the migration of planets close to slower rotators, which happens during the main sequence, may lead to a break in gyrochronology for high stellar and planetary masses. This also creates a region at high rotation periods and low orbital periods not populated by star-planet systems. We also find that star-planet interactions significantly impact the global distribution in orbital periods by depleting more planets for higher planetary masses and planetary magnetic fields. However, the global distribution in stellar rotation periods is marginally affected, as around 0.5\% of G-type stars and 0.1\% of K-type stars may spin up because of planetary engulfment. More precisely, star-planet magnetic interactions significantly affect the distribution of super-Earths around stars with a rotation period higher than around 5 days, which improves the agreement between synthetic populations and observations at orbital periods of less than 1 day. Tidal effects for their part shape the distribution of giant planets.},
  keywords = {Astrophysics - Earth and Planetary Astrophysics,Astrophysics - Solar and Stellar Astrophysics,planet-star interactions,stars: evolution,stars: rotation,stars: solar-type},
  annotation = {ADS Bibcode: 2021A\&A...650A.126A},
  file = {/Users/lbugnet/Zotero/storage/UK9KTT5Y/Ahuir et al. - 2021 - Magnetic and tidal migration of close-in planets. .pdf}
}

@article{Aigrain2015,
  title = {Testing the Recovery of Stellar Rotation Signals from {{Kepler}} Light Curves Using a Blind Hare-and-Hounds Exercise},
  author = {Aigrain, S. and Llama, J. and Ceillier, T. and Das Chagas, M. L. and Davenport, J. R.A. and Garc{\'i}a, R. A. and Hay, K. L. and Lanza, A. F. and McQuillan, A. and Mazeh, T. and De Medeiros, J. R. and Nielsen, M. B. and Reinhold, T.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {450},
  number = {3},
  eprint = {1504.04029},
  pages = {3211--3226},
  issn = {13652966},
  doi = {10.1093/mnras/stv853},
  abstract = {We present the results of a blind exercise to test the recoverability of stellar rotation and differential rotation in Kepler light curves. The simulated light curves lasted 1000 d and included activity cycles, Sun-like butterfly patterns, differential rotation and spot evolution. The range of rotation periods, activity levels and spot lifetime were chosen to be representative of the Kepler data of solar-like stars. Of the 1000 simulated light curves, 770 were injected into actual quiescent Kepler light curves to simulate Kepler noise. The test also included five 1000-d segments of the Sun's total irradiance variations at different points in the Sun's activity cycle. Five teams took part in the blind exercise, plus two teams who participated after the content of the light curves had been released. The methods used included Lomb-Scargle periodograms and variants thereof, autocorrelation function and wavelet-based analyses, plus spot modelling to search for differential rotation. The results show that the 'overall' period is well recovered for stars exhibiting low and moderate activity levels. Most teams reported values within 10 per cent of the true value in 70 per cent of the cases. There was, however, little correlation between the reported and simulated values of the differential rotation shear, suggesting that differential rotation studies based on full-disc light curves alone need to be treated with caution, at least for solar-type stars. The simulated light curves and associated parameters are available online for the community to test their own methods.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: rotation,Starspots,Surveys,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/4GJ85U9H/Aigrain et al. - 2015.pdf}
}

@article{Aigrain2016,
  title = {{{K2SC}}: {{Flexible}} Systematics Correction and Detrending of {{K2}} Light Curves Using {{Gaussian}} Process Regression},
  author = {Aigrain, S. and Parviainen, H. and Pope, B. J.S.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {459},
  number = {3},
  eprint = {1603.09167},
  pages = {2408--2419},
  issn = {13652966},
  doi = {10.1093/mnras/stw706},
  abstract = {We present k2sc (K2 Systematics Correction), a python pipeline to model instrumental systematics and astrophysical variability in light curves from the K2 mission. k2sc uses Gaussian Process regression to model position-dependent systematics and time-dependent variability simultaneously, enabling the user to remove both (e.g. for transit searches) or to remove systematics while preserving variability (for variability studies). For periodic variables, k2sc automatically computes estimates of the period, amplitude and evolution time-scale of the variability. We apply k2sc to publicly available K2 data from Campaigns 3-5 showing that we obtain photometric precision approaching that of the original Kepler mission. We compare our results to other publicly available K2 pipelines, showing that we obtain similar or better results, on average. We use transit injection and recovery tests to evaluate the impact of k2sc on planetary transit searches in K2 Pre-search Data Conditioning data, for planet-to-star radius ratios down to Rp/R* = 0.01 and periods up to P = 40 d, and show that k2sc significantly improves the ability to distinguish between true and false detections, particularly for small planets. k2sc can be run automatically on many light curves, or manually tailored for specific objects such as pulsating stars or large amplitude eclipsing binaries. It can be run on ASCII and FITS light-curve files, regardless of their origin. Both the code and the processed light curves are publicly available, and we provide instructions for downloading and using them. The methodology used by k2sc will be applicable to future transit search missions such as TESS and PLATO.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Planetary systems,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/H4UXTFHK/Aigrain, Parviainen, Pope - 2016.pdf}
}

@article{Aizenman1977,
  title = {Avoided {{Crossing}} of {{Modes}} of {{Non-radiel Stellar Oscillations}}},
  author = {Aizenman, M. and Smeyers, P. and Weigert, A.},
  year = {1977},
  journal = {Astronomy \& Astrophysics},
  volume = {58},
  pages = {41--46},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/K34YFQQK/Aizenman, Smeyers, Weigert - 1977.pdf}
}

@article{Akgun2013,
  title = {Stability of Magnetic Fields in Non-Barotropic Stars: {{An}} Analytic Treatment},
  author = {Akg{\"u}n, T. and Reisenegger, A. and Mastrano, A. and Marchant, P.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {433},
  number = {3},
  eprint = {1302.0273},
  pages = {2445--2466},
  issn = {00358711},
  doi = {10.1093/mnras/stt913},
  urldate = {2020-06-19},
  abstract = {Magnetic fields in upper main-sequence stars, white dwarfs and neutron stars are known to persist for time-scales comparable to their lifetimes. From a theoretical perspective this is problematic, as it can be shown that simple magnetic field configurations are always unstable. In non-barotropic stars, stable stratification allows for a much wider range of magnetic field structures than in barotropic stars, and helps stabilize them by making it harder to induce radial displacements. Recent simulations by Braithwaite and collaborators have shown that, in stably stratified stars, random initial magnetic fields evolve into nearly axisymmetric configurations with both poloidal and toroidal components, which then remain stable for some time. It is desirable to provide an analytic study of the stability of such fields. We write an explicit expression for a plausible equilibrium structure of an axially symmetric magnetic field with both poloidal and toroidal components of adjustable strengths, in a non-barotropic, non-rotating, fluid star, and study its stability using the energy principle. We construct a displacement field that should be a reasonable approximation to the most unstable mode of a toroidal field, and confirm Braithwaite's result that a given toroidal field can be stabilized by a poloidal field containing much less energy than the former, as given through the condition Epol/Etor {$\sigma$} 2aE tor/Egrav, where Epol and Etor are the energies of the poloidal and toroidal fields, respectively, and E grav is the gravitational binding energy of the star. We find that a {$\approx$} 7.4 for main-sequence stars, and a {$\sim$} 200 for neutron stars. Since Epol/EgraV {$<<$} 1, we conclude that the energy of the toroidal field can be substantially larger than that of the poloidal field, which is consistent with the speculation that the toroidal field is the main reservoir powering magnetar activity. The deformation of a neutron star caused by the hidden toroidal field can also cause emission of gravitational waves. \textcopyright{} 2013 The Authors.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,Magnetic fields,MHD,notion,notion-database,Stars: Magnetic field,Stars: Neutron,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/UC3Z9A3G/full-text.pdf}
}

@article{Alam2015,
  title = {{{THE ELEVENTH}} and {{TWELFTH DATA RELEASES}} of the {{SLOAN DIGITAL SKY SURVEY}}: {{FINAL DATA}} from {{SDSS-III}}},
  author = {Alam, Shadab and Albareti, Franco D. and Prieto, Carlos Allende and Anders, F. and Anderson, Scott F. and Anderton, Timothy and Andrews, Brett H. and Armengaud, Eric and Aubourg, {\'E}ric and Bailey, Stephen and Basu, Sarbani and Bautista, Julian E. and Beaton, Rachael L. and Beers, Timothy C. and Bender, Chad F. and Berlind, Andreas A. and Beutler, Florian and Bhardwaj, Vaishali and Bird, Jonathan C. and Bizyaev, Dmitry and Blake, Cullen H. and Blanton, Michael R. and Blomqvist, Michael and Bochanski, John J. and Bolton, Adam S. and Bovy, Jo and Bradley, A. Shelden and Brandt, W. N. and Brauer, D. E. and Brinkmann, J. and Brown, Peter J. and Brownstein, Joel R. and Burden, Angela and Burtin, Etienne and Busca, Nicol{\'a}s G. and Cai, Zheng and Capozzi, Diego and Rosell, Aurelio Carnero and Carr, Michael A. and Carrera, Ricardo and Chambers, K. C. and Chaplin, William James and Chen, Yen Chi and Chiappini, Cristina and Chojnowski, S. Drew and Chuang, Chia Hsun and Clerc, Nicolas and Comparat, Johan and Covey, Kevin and Croft, Rupert A.C. and Cuesta, Antonio J. and Cunha, Katia and Costa, Luiz N.Da and Rio, Nicola Da and Davenport, James R.A. and Dawson, Kyle S. and Lee, Nathan De and Delubac, Timoth{\'e}e and Deshpande, Rohit and Dhital, Saurav and {Dutra-Ferreira}, Let{\'i}cia and Dwelly, Tom and Ealet, Anne and Ebelke, Garrett L. and Edmondson, Edward M. and Eisenstein, Daniel J. and Ellsworth, Tristan and Elsworth, Yvonne and Epstein, Courtney R. and Eracleous, Michael and Escoffier, Stephanie and Esposito, Massimiliano and Evans, Michael L. and Fan, Xiaohui and {Fern{\'a}ndez-Alvar}, Emma and Feuillet, Diane and Ak, Nurten Filiz and Finley, Hayley and Finoguenov, Alexis and Flaherty, Kevin and Fleming, Scott W. and {Font-Ribera}, Andreu and Foster, Jonathan and Frinchaboy, Peter M. and {Galbraith-Frew}, J. G. and Garc{\'i}a, Rafael A. and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and P{\'e}rez, Ana E.Garc{\'i}a and Gaulme, Patrick and Ge, Jian and {G{\'e}nova-Santos}, R. and Georgakakis, A. and Ghezzi, Luan and Gillespie, Bruce A. and Girardi, L{\'e}o and Goddard, Daniel and Gontcho, Satya Gontcho A. and Hern{\'a}ndez, Jonay I.Gonz{\'a}lez and Grebel, Eva K. and Green, Paul J. and Grieb, Jan Niklas and Grieves, Nolan and Gunn, James E. and Guo, Hong and Harding, Paul and Hasselquist, Sten and Hawley, Suzanne L. and Hayden, Michael and Hearty, Fred R. and Hekker, Saskia and Ho, Shirley and Hogg, David W. and {Holley-Bockelmann}, Kelly and Holtzman, Jon A. and Honscheid, Klaus and Huber, Daniel and Huehnerhoff, Joseph and Ivans, Inese I. and Jiang, Linhua and Johnson, Jennifer A. and Kinemuchi, Karen and Kirkby, David and Kitaura, Francisco and Klaene, Mark A. and Knapp, Gillian R. and Kneib, Jean Paul and Koenig, Xavier P. and Lam, Charles R. and Lan, Ting Wen and Lang, Dustin and Laurent, Pierre and Goff, Jean Marc Le and Leauthaud, Alexie and Lee, Khee Gan and Lee, Young Sun and Licquia, Timothy C. and Liu, Jian and Long, Daniel C. and {L{\'o}pez-Corredoira}, Mart{\'i}n and {Lorenzo-Oliveira}, Diego and Lucatello, Sara and Lundgren, Britt and Lupton, Robert H. and Iii, Claude E.Mack and Mahadevan, Suvrath and Maia, Marcio A.G. and Majewski, Steven R. and Malanushenko, Elena and Malanushenko, Viktor and Manchado, A. and Manera, Marc and Mao, Qingqing and Maraston, Claudia and Marchwinski, Robert C. and Margala, Daniel and Martell, Sarah L. and Martig, Marie and Masters, Karen L. and Mathur, Savita and McBride, Cameron K. and McGehee, Peregrine M. and McGreer, Ian D. and McMahon, Richard G. and M{\'e}nard, Brice and Menzel, Marie Luise and Merloni, Andrea and M{\'e}sz{\'a}ros, Szabolcs and Miller, Adam A. and {Miralda-Escud{\'e}}, Jordi and Miyatake, Hironao and {Montero-Dorta}, Antonio D. and More, Surhud and Morganson, Eric and {Morice-Atkinson}, Xan and Morrison, Heather L. and Mosser, Benoit and Muna, Demitri and Myers, Adam D. and Nandra, Kirpal and Newman, Jeffrey A. and Neyrinck, Mark and Nguyen, Duy Cuong and Nichol, Robert C. and Nidever, David L. and Noterdaeme, Pasquier and Nuza, Sebasti{\'a}n E. and O'Connell, Julia E. and O'Connell, Robert W. and O'Connell, Ross and Ogando, Ricardo L.C. and Olmstead, Matthew D. and Oravetz, Audrey E. and Oravetz, Daniel J. and Osumi, Keisuke and Owen, Russell and Padgett, Deborah L. and Padmanabhan, Nikhil and Paegert, Martin and {Palanque-Delabrouille}, Nathalie and Pan, Kaike and Parejko, John K. and P{\^a}ris, Isabelle and Park, Changbom and Pattarakijwanich, Petchara and {Pellejero-Ibanez}, M. and Pepper, Joshua and Percival, Will J. and {P{\'e}rez-Fournon}, Ismael and {P{\'e}rez-Ra'Fols}, Ignasi and Petitjean, Patrick and Pieri, Matthew M. and Pinsonneault, Marc H. and Mello, Gustavo F.Porto De and Prada, Francisco and Prakash, Abhishek and {Price-Whelan}, Adrian M. and Protopapas, Pavlos and Raddick, M. Jordan and Rahman, Mubdi and Reid, Beth A. and Rich, James and Rix, Hans Walter and Robin, Annie C. and Rockosi, Constance M. and Rodrigues, Tha{\'i}se S. and {Rodr{\'i}guez-Torres}, Sergio and Roe, Natalie A. and Ross, Ashley J. and Ross, Nicholas P. and Rossi, Graziano and Ruan, John J. and {Rubi{\~n}o-Mart{\'i}n}, J. A. and Rykoff, Eli S. and {Salazar-Albornoz}, Salvador and Salvato, Mara and Samushia, Lado and S{\'a}nchez, Ariel G. and Santiago, Bas{\'i}lio and Sayres, Conor and Schiavon, Ricardo P. and Schlegel, David J. and Schmidt, Sarah J. and Schneider, Donald P. and Schultheis, Mathias and Schwope, Axel D. and Sc{\'o}ccola, C. G. and Scott, Caroline and Sellgren, Kris and Seo, Hee Jong and Serenelli, Aldo and Shane, Neville and Shen, Yue and Shetrone, Matthew and Shu, Yiping and Aguirre, V. Silva and Sivarani, Thirupathi and Skrutskie, M. F. and Slosar, An{\v z}e and Smith, Verne V. and Sobreira, Fl{\'a}via and Souto, Diogo and Stassun, Keivan G. and Steinmetz, Matthias and Stello, Dennis and Strauss, Michael A. and Streblyanska, Alina and Suzuki, Nao and Swanson, Molly E.C. and Tan, Jonathan C. and Tayar, Jamie and Terrien, Ryan C. and Thakar, Aniruddha R. and Thomas, Daniel and Thomas, Neil and Thompson, Benjamin A. and Tinker, Jeremy L. and Tojeiro, Rita and Troup, Nicholas W. and {Vargas-Maga{\~n}a}, Mariana and Vazquez, Jose A. and Verde, Licia and Viel, Matteo and Vogt, Nicole P. and Wake, David A. and Wang, Ji and Weaver, Benjamin A. and Weinberg, David H. and Weiner, Benjamin J. and White, Martin and Wilson, John C. and Wisniewski, John P. and {Wood-Vasey}, W. M. and Ye'Che, Christophe and York, Donald G. and Zakamska, Nadia L. and Zamora, O. and Zasowski, Gail and Zehavi, Idit and Zhao, Gong Bo and Zheng, Zheng and Zhou, Xu and Zhou, Zhimin and Zou, Hu and Zhu, Guangtun},
  year = {2015},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {219},
  number = {1},
  eprint = {1501.00963},
  issn = {00670049},
  doi = {10.1088/0067-0049/219/1/12},
  abstract = {The third generation of the Sloan Digital Sky Survey (SDSS-III) took data from 2008 to 2014 using the original SDSS wide-field imager, the original and an upgraded multi-object fiber-fed optical spectrograph, a new near-infrared high-resolution spectrograph, and a novel optical interferometer. All of the data from SDSS-III are now made public. In particular, this paper describes Data Release 11 (DR11) including all data acquired through 2013 July, and Data Release 12 (DR12) adding data acquired through 2014 July (including all data included in previous data releases), marking the end of SDSS-III observing. Relative to our previous public release (DR10), DR12 adds one million new spectra of galaxies and quasars from the Baryon Oscillation Spectroscopic Survey (BOSS) over an additional 3000 deg2 of sky, more than triples the number of H-band spectra of stars as part of the Apache Point Observatory (APO) Galactic Evolution Experiment (APOGEE), and includes repeated accurate radial velocity measurements of 5500 stars from the Multi-object APO Radial Velocity Exoplanet Large-area Survey (MARVELS). The APOGEE outputs now include the measured abundances of 15 different elements for each star. In total, SDSS-III added 5200 deg2 of ugriz imaging; 155,520 spectra of 138,099 stars as part of the Sloan Exploration of Galactic Understanding and Evolution 2 (SEGUE-2) survey; 2,497,484 BOSS spectra of 1,372,737 galaxies, 294,512 quasars, and 247,216 stars over 9376 deg2; 618,080 APOGEE spectra of 156,593 stars; and 197,040 MARVELS spectra of 5513 stars. Since its first light in 1998, SDSS has imaged over 1/3 of the Celestial sphere in five bands and obtained over five million astronomical spectra.},
  archiveprefix = {arxiv},
  keywords = {atlases,catalogs,notion,notion-database,surveys},
  file = {/Users/lbugnet/Zotero/storage/U29RBPVX/Alam et al. - 2015.pdf}
}

@article{alexandrae.l.thomasImpactMagneticActivity2021,
  title = {Impact of Magnetic Activity on Inferred Stellar Properties of Main-Sequence {{Sun-like}} Stars},
  author = {{Alexandra E. L. Thomas} and {William J. Chaplin} and {Sarbani Basu} and {Ben Rendle} and {Guy Davies} and {Andrea Miglio}},
  year = {2021},
  journal = {MNRAS},
  volume = {502},
  pages = {5808--5820},
  urldate = {2021-11-11},
  keywords = {notion,notion-database}
}

@article{Alfven1937,
  title = {Versuch Zu Einer {{Theorie}} \"Uber Die {{Entstehung}} Der Kosmischen {{Strahlung}}. {{II}}},
  author = {Alfv{\'e}n, Hannes},
  year = {1937},
  month = sep,
  journal = {Zeitschrift f\"ur Physik},
  volume = {107},
  number = {9-10},
  pages = {579--588},
  publisher = {{Springer-Verlag}},
  issn = {14346001},
  doi = {10.1007/BF01339294},
  urldate = {2020-07-03},
  keywords = {notion,notion-database}
}

@article{AllendePrieto2002,
  title = {Signatures of {{Convection}} in the {{Spectrum}} of {{Procyon}}: {{Fundamental Parameters}} and {{Iron Abundance}}},
  author = {Allende Prieto, Carlos and Asplund, Martin and Lopez, Ramon J. Garcia and Lambert, David L.},
  year = {2002},
  journal = {The Astrophysical Journal},
  volume = {567},
  number = {1},
  pages = {544--565},
  issn = {0004-637X},
  doi = {10.1086/338248},
  abstract = {We have observed the spectrum of Procyon A (F5 IV) from 4559 to 5780 \AA{} with a signal-to-noise ratio of \textasciitilde 103 and a resolving power of 2\texttimes 105. We have measured the line bisectors and relative line shifts of a large number of Fe I and Fe II lines, comparing them to those found in the solar spectrum. A three-dimensional hydrodynamical model atmosphere has been computed and is tested against observations. The model reproduces in detail most of the features observed, although we identify some room for improvement. At all levels, the comparison of the three-dimensional time-dependent calculations with the observed spectral lines shows a much better agreement than for classical homogeneous models, making it possible to refine previous estimates of the iron abundance, the projected rotational velocity, the limb darkening, and the systemic velocity of the Procyon binary system. The difference between the iron abundance determined with the three-dimensional model and its one-dimensional counterpart is {$<\sptilde$}0.05 dex. We find consistency between the iron abundance derived from Fe I and Fe II lines, suggesting that departures from LTE in the formation of the studied lines are relatively small. The scatter in the iron abundance determined from different lines still exceeds the expectations from the uncertainties in the atomic data, pointing out that one or more components in the modeling can be refined further.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BIVAC2S3/Allende Prieto et al. - 2002.pdf}
}

@article{Alonso2009,
  title = {Special Feature {{The}} Secondary Eclipse of {{CoRoT-1b}}},
  author = {Alonso, R and Alapini, A and Aigrain, S and Auvergne, M and Baglin, A and Barbieri, M and Barge, P and Bonomo, A S and Bord{\'e}, P},
  year = {2009},
  volume = {358},
  pages = {353--358},
  keywords = {notion,notion-database,photometric,planetary systems,{planetary systems, techniques: photometric},techniques},
  file = {/Users/lbugnet/Zotero/storage/N7H8UBTU/Alonso et al. - 2009.pdf}
}

@article{Althaus2013,
  title = {New Evolutionary Sequences for Extremely Low-Mass White Dwarfs. {{Homogeneous}} Mass and Age Determinations and Asteroseismic Prospects},
  author = {Althaus, Leandro G. and Miller Bertolami, Marcelo M. and C{\'o}rsico, Alejandro H.},
  year = {2013},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {557},
  pages = {A19},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201321868},
  urldate = {2023-10-02},
  abstract = {Context. The number of detected extremely low-mass (ELM) white dwarf stars has increased drastically in recent years, thanks to the results of many surveys. In addition, some of these stars have been found to exhibit pulsations, making them potential targets for asteroseismology. Aims: We provide a fine and homogeneous grid of evolutionary sequences for helium (He) core white dwarfs for the whole range of their expected masses (0.15 {$\lessequivlnt$} M{${_\ast}$}/M{$\odot$} {$\lessequivlnt$} 0.45), including the mass range for ELM white dwarfs (M{${_\ast}$}/M{$\odot$} {$\lessequivlnt$} 0.20). The grid is appropriate for mass and age determination of these stars, as well as for studying their adiatabic pulsational properties. Methods: White dwarf sequences have been computed by performing full evolutionary calculations that consider the main energy sources and processes of chemical abundance changes during white dwarf evolution. Realistic initial models for the evolving white dwarfs have been obtained by computing the nonconservative evolution of a binary system consisting of an initially 1 M{$\odot$} ZAMS star and a 1.4 M{$\odot$} neutron star for various initial orbital periods. To derive cooling ages and masses for He-core white dwarfs, we perform a least square fitting of the M(Teff,g) and Age(Teff,g) relations provided by our sequences by using a scheme that takes into account the time spent by models in different regions of the Teff - g plane. This is particularly useful when multiple solutions for cooling age and mass determinations are possible in the case of CNO-flashing sequences. We also explore in a preliminary way the adiabatic pulsational properties of models near the critical mass for the development of CNO flashes (\textasciitilde 0.2 M{$\odot$}). This is motivated by the discovery of pulsating white dwarfs with stellar masses near this threshold value. Results: We obtain reliable and homogeneous mass and cooling age determinations for 58 very low-mass white dwarfs, including three pulsating stars. Also, we find substantial differences in the period spacing distributions of g-modes for models with stellar masses near \textasciitilde{} 0.2 M{$\odot$}, which could be used as a seismic tool to distinguish stars that have undergone CNO flashes in their early cooling phase from those that have not. Finally, for an easy application of our results, we provide a reduced grid of values useful to obtain the masses and ages of He-core white dwarfs. Table 2 is available in electronic form at http://www.aanda.orgThe tracks and the data presented in the middle and lower panels of Figs. 5, 6 are available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr (ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/557/A19},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: general,stars: evolution,stars: interiors,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2013A\&A...557A..19A},
  file = {/Users/lbugnet/Zotero/storage/GBTANN4K/Althaus et al. - 2013 - New evolutionary sequences for extremely low-mass .pdf}
}

@phdthesis{Alvan,
  title = {Ondes Internes de Gravit\'e Dans Les \'Etoiles de Type Solaire. {{Excitation}}, Propagation et Transport de Moment Cin\'etique.},
  author = {Alvan, L.},
  year = {2014},
  keywords = {notion,notion-database}
}

@article{Alvan2013,
  title = {Coupling between Internal Waves and Shear-Induced Turbulence in Stellar Radiation Zones: {{The}} Critical Layers},
  author = {Alvan, L. and Mathis, S. and Decressin, T.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {553},
  eprint = {1303.1715},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321210},
  urldate = {2020-04-19},
  abstract = {Context. Internal gravity waves (IGW) are known as one of the candidates for explaining the angular velocity profile in the Sun and in solar-type main-sequence and evolved stars due to their role in the transport of angular momentum. Our contribution deals with critical layers, which are defined as the locations where the Doppler-shifted frequency of the wave approaches zero (i.e., they correspond to corotation resonances). Aims. The IGW propagate through stably stratified radiative regions, where they extract or deposit angular momentum through two processes: radiative and viscous dampings and critical layers. Our goal is to obtain a complete picture of the effects of these processes. Methods. First, we expose a mathematical resolution of the equation of propagation for IGW in adiabatic and non-adiabatic cases near critical layers. Then, the use of a dynamical stellar evolution code, which treats the secular transport of angular momentum, allows us to apply these results to the case of a solar-like star. Results. The analysis reveals two cases depending on the value of the Richardson number at critical layers: a stable one, where IGW are attenuated as they pass through a critical level, and an unstable turbulent case, where they can be reflected/transmitted by the critical level with a coefficient larger than one. Such over-reflection/transmission can have strong implications on our vision of angular momentum transport in stellar interiors. Conclusions. This paper highlights the existence of two regimes defining the interaction between an IGW and a critical layer. An application exposes the effect of the first regime, showing a strengthening of the damping of the wave. Moreover, this work opens up new ways concerning the coupling between IGW and shear instabilities in stellar interiors. \textcopyright{} 2013 ESO.},
  archiveprefix = {arxiv},
  keywords = {Hydrodynamics,notion,notion-database,Stars: evolution,Stars: rotation,Turbulence,Waves},
  file = {/Users/lbugnet/Zotero/storage/GWNARUSK/full-text.pdf}
}

@article{Alvan2014,
  title = {{{3D}} Simulations of Internal Gravity Waves in Solar-like Stars},
  author = {Alvan, Lucie and Brun, Allan Sacha and Mathis, St{\'e}phane},
  year = {2014},
  journal = {Proceedings of the International Astronomical Union},
  volume = {9},
  number = {S301},
  pages = {375--376},
  issn = {17439213},
  doi = {10.1017/S1743921313014622},
  abstract = {We perform numerical simulations of the whole Sun using the 3D anelastic spherical harmonic (ASH) code. In such models, the radiative and convective zones are non-linearly coupled and in the radiative interior a wave-like pattern is observed. For the first time, we are thus able to model in 3D the excitation and propagation of internal gravity waves (IGWs) in a solar-like star's radiative zone. We compare the properties of our waves to theoretical predictions and results of oscillation calculations. The obtained good agreement allows us to validate the consistency of our approach and to study the characteristics of IGWs. We find that a wave's spectrum is excited up to radial order n=58. This spectrum evolves with depth and time; we show that the lifetime of the highest-frequency modes must be greater than 550 days. We also test the sensitivity of waves to rotation and are able to retrieve the rotation rate to within 5\% error by measuring the frequency splitting. Copyright \textcopyright{} International Astronomical Union 2014.},
  isbn = {9781107045170},
  keywords = {hydrodynamics,methods: numerical,notion,notion-database,stellar dynamics,waves},
  file = {/Users/lbugnet/Zotero/storage/2ITIUR37/Alvan, Brun, Mathis - 2014.pdf}
}

@article{Amard2016,
  title = {Rotating Models of Young Solar-Type Stars: {{Exploring}} Braking Laws and Angular Momentum Transport Processes},
  author = {Amard, L. and Palacios, A. and Charbonnel, C. and Gallet, F. and Bouvier, J.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {587},
  number = {27349},
  eprint = {1601.01904},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527349},
  abstract = {Context. Understanding the angular momentum evolution of stars is one of the greatest challenges of modern stellar physics. Aims. We study the predicted rotational evolution of solar-type stars from the pre-main sequence to the solar age with 1D rotating evolutionary models including physical ingredients. Methods. We computed rotating evolution models of solar-type stars including an external stellar wind torque and internal transport of angular momentum following the method of Maeder and Zahn with the code STAREVOL. We explored different formalisms and prescriptions available from the literature. We tested the predictions of the models against recent rotational period data from extensive photometric surveys, lithium abundances of solar-mass stars in young clusters, and the helioseismic rotation profile of the Sun. Results. We find a best-matching combination of prescriptions for both internal transport and surface extraction of angular momentum. This combination provides a very good fit to the observed evolution of rotational periods for solar-type stars from early evolution to the age of the Sun. Additionally, we show that fast rotators experience a stronger coupling between their radiative region and the convective envelope. Regardless of the set of prescriptions, however, we cannot simultaneously reproduce surface angular velocity and the internal profile of the Sun or the evolution of lithium abundance. Conclusions. We confirm the idea that additional transport mechanisms must occur in solar-type stars until they reach the age of the Sun. Whether these processes are the same as those needed to explain recent asteroseismic data in more advanced evolutionary phases is still an open question.},
  archiveprefix = {arxiv},
  keywords = {Hydrodynamics,notion,notion-database,stars: evolution,stars: magnetic field,stars: pre-main sequence,stars: rotation,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/HK65Q9JJ/Amard et al. - 2016.pdf}
}

@article{Amard2019,
  title = {First Grids of Low-Mass Stellar Models and Isochrones with Self-Consistent Treatment of Rotation: {{From}} 0.2 to 1.5 {{M}} {$\cdot$} at Seven Metallicities from {{PMS}} to {{TAMS}}},
  author = {Amard, L. and Palacios, A. and Charbonnel, C. and Gallet, F. and Georgy, C. and Lagarde, N. and Siess, L.},
  year = {2019},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {631},
  eprint = {1905.08516},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201935160},
  urldate = {2020-07-06},
  abstract = {Aims. We present an extended grid of state-of-the art stellar models for low-mass stars including updated physics (nuclear reaction rates, surface boundary condition, mass-loss rate, angular momentum transport, rotation-induced mixing, and torque prescriptions). We evaluate the impact of wind braking, realistic atmospheric treatment, rotation, and rotation-induced mixing on the structural and rotational evolution from the pre-main sequence (PMS) to the turn-off. Methods. Using the STAREVOL code, we provide an updated PMS grid. We computed stellar models for seven different metallicities, from [Fe/H] = -1 dex to [Fe/H] = +0.3 dex with a solar composition corresponding to Z = 0.0134. The initial stellar mass ranges from 0.2 to 1.5 M{$\cdot$} with extra grid refinement around one solar mass. We also provide rotating models for three different initial rotation rates (slow, median, and fast) with prescriptions for the wind braking and disc-coupling timescale calibrated on observed properties of young open clusters. The rotational mixing includes the most recent description of the turbulence anisotropy in stably stratified regions. Results. The overall behaviour of our models at solar metallicity, and their constitutive physics, are validated through a detailed comparison with a variety of distributed evolutionary tracks. The main differences arise from the choice of surface boundary conditions and initial solar composition. The models including rotation with our prescription for angular momentum extraction and self-consistent formalism for angular momentum transport are able to reproduce the rotation period distribution observed in young open clusters over a wide range of mass values. These models are publicly available and can be used to analyse data coming from present and forthcoming asteroseismic and spectroscopic surveys such as Gaia, TESS, and PLATO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: low-mass,Stars: pre-main sequence,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/IPV9NXMT/full-text.pdf}
}

@article{Amard2020,
  title = {The {{Impact}} of {{Metallicity}} on the {{Evolution}} of the {{Rotation}} and {{Magnetic Activity}} of {{Sun-like Stars}}},
  author = {Amard, Louis and Matt, Sean P.},
  year = {2020},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {889},
  number = {2},
  eprint = {2001.10404},
  pages = {108},
  publisher = {{American Astronomical Society}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/ab6173},
  urldate = {2020-06-08},
  abstract = {The rotation rates and magnetic activity of Sun-like and low-mass ({$<$} 1.4 Msun) main-sequence stars are known to decline with time, and there now exist several models for the evolution of rotation and activity. However, the role that chemical composition plays during stellar spin-down has not yet been explored. In this work, we use a structural evolution code to compute the rotational evolution of stars with three different masses (0.7, 1.0, and 1.3Msun and six different metallicities, ranging from [Fe/H]=-1.0 to [Fe/H]=+0.5. We also implement three different wind-braking formulations from the literature (two modern and one classical) and compare their predictions for rotational evolution. The effect that metallicity has on stellar structural properties, and in particular the convective turnover timescale, leads the two modern wind-braking formulations to predict a strong dependence of the torque on metallicity. Consequently, they predict that metal rich stars spin-down more effectively at late ages ({$>$} 1 Gyr) than metal poor stars, and the effect is large enough to be detectable with current observing facilities. For example, the formulations predict that a Sun-like (solar-mass and solar-aged) star with [Fe/H]=-0.3 will have a rotation period of less than 20 days. Even though old, metal poor stars are predicted to rotate more rapidly at a given age, they have larger Rossby numbers and are thus expected to have lower magnetic activity levels. Finally, the different wind-braking formulations predict quantitative differences in the metallicity-dependence of stellar rotation, which may be used to test them.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Ambastha2003,
  title = {Flare-Induced Excitation of Solar p Modes},
  author = {Ambastha, Ashok and Basu, Sarbani and Antia, H. M.},
  year = {2003},
  journal = {Solar Physics},
  volume = {218},
  number = {1-2},
  pages = {151--172},
  issn = {00380938},
  doi = {10.1023/b:sola.0000013043.45512.20},
  abstract = {Solar flares release large amounts of energy at different layers of the solar atmosphere, including at the photosphere in the case of exceptionally major events. Therefore, it is expected that large flares would be able to excite acoustic waves on the solar surface, thereby affecting the p-mode oscillation characteristics. We have applied the ring-diagram analysis technique to 3-D power spectra obtained for different flare regions in order to study how flares affect the amplitude, frequency and width of the acoustic modes. Data from the Michelson Doppler Imager (MDI) on board the Solar and Heliospheric Observatory (SOHO) has been used. We have used data obtained for several active regions of the current solar cycle that have produced flares. In most cases, during the period of high flare activity, power in p modes appears to be larger when compared to that in non-flaring regions of similar magnetic field strength.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VED8N94B/Ambastha, Basu, Antia - 2003.pdf}
}

@article{Amit1997,
  title = {Communicated by {{Shimon Ullman Shape Quantization}} and {{Recognition}} with {{Randomized Trees}}},
  author = {Amit, Yali and Geman, Donald},
  year = {1997},
  journal = {Neural Computation},
  volume = {9},
  pages = {1545--1588},
  urldate = {2020-03-23},
  abstract = {We explore a new approach to shape recognition based on a virtually infinite family of binary features (queries) of the image data, designed to accommodate prior information about shape invariance and regularity. Each query corresponds to a spatial arrangement of several local topographic codes (or tags), which are in themselves too primitive and common to be informative about shape. All the discriminating power derives from relative angles and distances among the tags. The important attributes of the queries are a natural partial ordering corresponding to increasing structure and complexity; semi-invariance, meaning that most shapes of a given class will answer the same way to two queries that are successive in the ordering; and stability, since the queries are not based on distinguished points and substructures. No classifier based on the full feature set can be evaluated, and it is impossible to determine a priori which arrangements are informative. Our approach is to select informative features and build tree classifiers at the same time by inductive learning. In effect, each tree provides an approximation to the full posterior where the features chosen depend on the branch that is traversed. Due to the number and nature of the queries, standard decision tree construction based on a fixed-length feature vector is not feasible. Instead we entertain only a small random sample of queries at each node, constrain their complexity to increase with tree depth, and grow multiple trees. The terminal nodes are labeled by estimates of the corresponding posterior distribution over shape classes. An image is classified by sending it down every tree and aggregating the resulting distributions. The method is applied to classifying handwritten digits and synthetic linear and nonlinear deformations of three hundred L A T E X symbols. State-of-the-art error rates are achieved on the National Institute of Standards and Technology database of digits. The principal goal of the experiments on L A T E X symbols is to analyze invariance, generalization error and related issues, and a comparison with artificial neural networks methods is presented in this context.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FY6FMK83/full-text.pdf}
}

@article{Anders2017,
  title = {Galactic Archaeology with Asteroseismology and Spectroscopy: {{Red}} Giants Observed by {{CoRoT}} and {{APOGEE}}},
  author = {Anders, F. and Chiappini, C. and Rodrigues, T. S. and Miglio, A. and Montalb{\'a}n, J. and Mosser, B. and Girardi, L. and Valentini, M. and Noels, A. and Morel, T. and Johnson, J. A. and Schultheis, M. and Baudin, F. and De Assis Peralta, R. and Hekker, S. and Theme{\ss}l, N. and Kallinger, T. and Garc{\'i}a, R. A. and Mathur, S. and Baglin, A. and Santiago, B. X. and Martig, M. and Minchev, I. and Steinmetz, M. and Da Costa, L. N. and Maia, M. A.G. and Prieto, C. Allende and Cunha, K. and Beers, T. C. and Epstein, C. and P{\'e}rez, A. E.Garc{\'i}a and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Harding, P. and Holtzman, J. and Majewski, S. R. and M{\'e}sz{\'a}ros, Sz and Nidever, D. and Pan, K. and Pinsonneault, M. and Schiavon, R. P. and Schneider, D. P. and Shetrone, M. D. and Stassun, K. and Zamora, O. and Zasowski, G.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {597},
  eprint = {1604.07763},
  pages = {1--27},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527204},
  abstract = {With the advent of the space missions CoRoT and Kepler, it has recently become feasible to determine precise asteroseismic masses and relative ages for large samples of red giant stars. We present the CoRoGEE dataset, obtained from CoRoT light curves for 606 red giants in two fields of the Galactic disc that have been co-observed by the Apache Point Observatory Galactic Evolution Experiment (APOGEE). We used the Bayesian parameter estimation code PARAM to calculate distances, extinctions, masses, and ages for these stars in a homogeneous analysis, resulting in relative statistical uncertainties of {$\leq$} 2\% in distance, {$\sim$}4\% in radius, {$\sim$}9\% in mass and {$\sim$}25\% in age. We also assessed systematic age uncertainties stemming from different input physics and mass loss. We discuss the correlation between ages and chemical abundance patterns of field stars over a broad radial range of the Milky Way disc (5 kpc},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Galaxy: abundances,Galaxy: disk,Galaxy: evolution,notion,notion-database,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/NUHID3A4/Anders et al. - 2017.pdf}
}

@article{Anders2022,
  title = {Stellar {{Convective Penetration}}: {{Parameterized Theory}} and {{Dynamical Simulations}}},
  shorttitle = {Stellar {{Convective Penetration}}},
  author = {Anders, Evan H. and Jermyn, Adam S. and Lecoanet, Daniel and Brown, Benjamin P.},
  year = {2022},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {926},
  pages = {169},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac408d},
  urldate = {2023-10-14},
  abstract = {Most stars host convection zones in which heat is transported directly by fluid motion, but the behavior of convective boundaries is not well-understood. Here, we present 3D numerical simulations that exhibit penetration zones: regions where the entire luminosity could be carried by radiation, but where the temperature gradient is approximately adiabatic and convection is present. To parameterize this effect, we define the "penetration parameter" \$\{ \textbackslash mathcal P \}\$ , which compares how far the radiative gradient deviates from the adiabatic gradient on either side of the Schwarzschild convective boundary. Following Roxburgh and Zahn, we construct an energy-based theoretical model in which \$\{ \textbackslash mathcal P \}\$ controls the extent of penetration. We test this theory using 3D numerical simulations that employ a simplified Boussinesq model of stellar convection. The convection is driven by internal heating, and we use a height-dependent radiative conductivity. This allows us to separately specify \$\{ \textbackslash mathcal P \}\$ and the stiffness \$\{ \textbackslash mathcal S \}\$ of the radiative-convective boundary. We find significant convective penetration in all simulations. Our simple theory describes the simulations well. Penetration zones can take thousands of overturn times to develop, so long simulations or accelerated evolutionary techniques are required. In stars, we expect \$\{ \textbackslash mathcal P \}\textbackslash approx 1\$ , and in this regime, our results suggest that convection zones may extend beyond the Schwarzschild boundary by up to \textasciitilde 20\%-30\% of a mixing length. We present a MESA stellar model of the Sun that employs our parameterization of convective penetration as a proof of concept. Finally, we discuss prospects for extending these results to more realistic stellar contexts.},
  keywords = {101,1606,1631,1963,1998,299,300,301,767,Astrophysics - Solar and Stellar Astrophysics,Physics - Fluid Dynamics},
  annotation = {ADS Bibcode: 2022ApJ...926..169A},
  file = {/Users/lbugnet/Zotero/storage/IJBDXYLC/Anders et al. - 2022 - Stellar Convective Penetration Parameterized Theo.pdf}
}

@article{Anders2022a,
  title = {Stellar {{Convective Penetration}}: {{Parameterized Theory}} and {{Dynamical Simulations}}},
  shorttitle = {Stellar {{Convective Penetration}}},
  author = {Anders, Evan H. and Jermyn, Adam S. and Lecoanet, Daniel and Brown, Benjamin P.},
  year = {2022},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {926},
  pages = {169},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac408d},
  urldate = {2023-10-14},
  abstract = {Most stars host convection zones in which heat is transported directly by fluid motion, but the behavior of convective boundaries is not well-understood. Here, we present 3D numerical simulations that exhibit penetration zones: regions where the entire luminosity could be carried by radiation, but where the temperature gradient is approximately adiabatic and convection is present. To parameterize this effect, we define the "penetration parameter" \$\{ \textbackslash mathcal P \}\$ , which compares how far the radiative gradient deviates from the adiabatic gradient on either side of the Schwarzschild convective boundary. Following Roxburgh and Zahn, we construct an energy-based theoretical model in which \$\{ \textbackslash mathcal P \}\$ controls the extent of penetration. We test this theory using 3D numerical simulations that employ a simplified Boussinesq model of stellar convection. The convection is driven by internal heating, and we use a height-dependent radiative conductivity. This allows us to separately specify \$\{ \textbackslash mathcal P \}\$ and the stiffness \$\{ \textbackslash mathcal S \}\$ of the radiative-convective boundary. We find significant convective penetration in all simulations. Our simple theory describes the simulations well. Penetration zones can take thousands of overturn times to develop, so long simulations or accelerated evolutionary techniques are required. In stars, we expect \$\{ \textbackslash mathcal P \}\textbackslash approx 1\$ , and in this regime, our results suggest that convection zones may extend beyond the Schwarzschild boundary by up to \textasciitilde 20\%-30\% of a mixing length. We present a MESA stellar model of the Sun that employs our parameterization of convective penetration as a proof of concept. Finally, we discuss prospects for extending these results to more realistic stellar contexts.},
  keywords = {101,1606,1631,1963,1998,299,300,301,767,Astrophysics - Solar and Stellar Astrophysics,Physics - Fluid Dynamics},
  annotation = {ADS Bibcode: 2022ApJ...926..169A}
}

@article{Anders2022b,
  title = {Convective {{Boundary Mixing Processes}}},
  author = {Anders, Evan H. and Jermyn, Adam S. and Lecoanet, Daniel and Fuentes, J. R. and Korre, Lydia and Brown, Benjamin P. and Oishi, Jeffrey S.},
  year = {2022},
  month = feb,
  journal = {Research Notes of the AAS},
  volume = {6},
  number = {2},
  pages = {41},
  publisher = {{The American Astronomical Society}},
  issn = {2515-5172},
  doi = {10.3847/2515-5172/ac5892},
  urldate = {2023-10-18},
  abstract = {Convective motions extend beyond the nominal boundaries of a convection zone. These motions mix fluid through multiple mechanisms collectively called ``convective boundary mixing.'' In this note, we discuss three distinct fluid dynamical processes: convective overshoot, entrainment, and penetrative convection. We describe the structure of a convective boundary that these processes create. To resolve discrepancies between models and observations, the stellar astrophysics community should distinguish between these processes and parameterize each of them separately in 1D evolutionary models.},
  langid = {english}
}

@article{Anders2023,
  title = {The Photometric Variability of Massive Stars Due to Gravity Waves Excited by Core Convection},
  author = {Anders, Evan H. and Lecoanet, Daniel and Cantiello, Matteo and Burns, Keaton J. and Hyatt, Benjamin A. and Kaufman, Emma and Townsend, Richard H. D. and Brown, Benjamin P. and Vasil, Geoffrey M. and Oishi, Jeffrey S. and Jermyn, Adam S.},
  year = {2023},
  month = jul,
  journal = {Nature Astronomy},
  eprint = {2306.08023},
  primaryclass = {astro-ph, physics:physics},
  issn = {2397-3366},
  doi = {10.1038/s41550-023-02040-7},
  urldate = {2023-10-16},
  abstract = {Massive stars die in catastrophic explosions, which seed the interstellar medium with heavy elements and produce neutron stars and black holes. Predictions of the explosion's character and the remnant mass depend on models of the star's evolutionary history. Models of massive star interiors can be empirically constrained by asteroseismic observations of gravity wave oscillations. Recent photometric observations reveal a ubiquitous red noise signal on massive main sequence stars; a hypothesized source of this noise is gravity waves driven by core convection. We present the first 3D simulations of massive star convection extending from the star's center to near its surface, with realistic stellar luminosities. Using these simulations, we make the first prediction of photometric variability due to convectively-driven gravity waves at the surfaces of massive stars, and find that gravity waves produce photometric variability of a lower amplitude and lower characteristic frequency than the observed red noise. We infer that the photometric signal of gravity waves excited by core convection is below the noise limit of current observations, so the red noise must be generated by an alternative process.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,Physics - Fluid Dynamics},
  file = {/Users/lbugnet/Zotero/storage/IVZI6CIV/Anders et al. - 2023 - The photometric variability of massive stars due t.pdf;/Users/lbugnet/Zotero/storage/XA79FRXI/2306.html}
}

@article{Anders2023a,
  title = {The Photometric Variability of Massive Stars Due to Gravity Waves Excited by Core Convection},
  author = {Anders, Evan H. and Lecoanet, Daniel and Cantiello, Matteo and Burns, Keaton J. and Hyatt, Benjamin A. and Kaufman, Emma and Townsend, Richard H. D. and Brown, Benjamin P. and Vasil, Geoffrey M. and Oishi, Jeffrey S. and Jermyn, Adam S.},
  year = {2023},
  month = jul,
  journal = {Nature Astronomy},
  issn = {2397-3366},
  doi = {10.1038/s41550-023-02040-7},
  urldate = {2023-10-16},
  abstract = {Massive stars die in catastrophic explosions that seed the interstellar medium with heavy elements and produce neutron stars and black holes. Predictions of the explosion's character and the remnant mass depend on models of the star's evolutionary history. Models of massive star interiors can be empirically constrained by asteroseismic observations of gravity wave oscillations. Recent photometric observations reveal a ubiquitous red noise signal on massive main sequence stars; a hypothesized source of this noise is gravity waves driven by core convection. We present three-dimensional simulations of massive star convection extending from the star's centre to near its surface, with realistic stellar luminosities. Using these simulations, we predict the photometric variability due to convectively driven gravity waves at the surfaces of massive stars, and find that gravity waves produce photometric variability of a lower amplitude and lower characteristic frequency than the observed red noise. We infer that the photometric signal of gravity waves excited by core convection is below the noise limit of current observations, and thus the red noise must be generated by an alternative process.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,Physics - Fluid Dynamics},
  annotation = {ADS Bibcode: 2023NatAs.tmp..170A},
  file = {/Users/lbugnet/Zotero/storage/4ZH8S3IX/Anders et al. - 2023 - The photometric variability of massive stars due t.pdf}
}

@article{Anderson1977,
  title = {Seismology on {{Mars}}},
  author = {Anderson, Don L. and Miller, W. F. and Latham, G. V. and Nakamura, Y. and Toks{\"o}z, M. N. and Dainty, A. M. and Duennebier, F. K. and Lazarewicz, A. R. and Kovach, R. L. and Knight, T. C. D.},
  year = {1977},
  month = sep,
  journal = {Journal of Geophysical Research},
  volume = {82},
  number = {28},
  pages = {4524--4546},
  publisher = {{American Geophysical Union (AGU)}},
  issn = {0148-0227},
  doi = {10.1029/js082i028p04524},
  urldate = {2020-03-06},
  abstract = {DON L. ANDERSON, \textbullet{} W. F. MILLER, \textbullet{} G. V. LATHAM, 2 Y. NAKAMURA, 2 M. N. TOKSOZ, a A.M. DAINTY, a F. K. DUENNEBIER, 4 A. R. LAZAREWICZ, 4 R. L. KOVACH, 5 AND T. C. D. KNIGHT 6 A three-axis short-period seismometer has been operating on the surface of Mars in the Utopia Planitia region since September 4, 1976. During the first 5 months of operation, approximately 640 hours of high-quality data, uncontaminated by lander or wind noise, have been obtained. The detection threshold is estimated to be magnitude 3 to about 200 km and about 6.5 for the planet as a whole. No large events have been seen during this period, a result indicating that Mars is less seismically active than earth. Wind is the major source of noise during the day, although the noise level was at or below the sensitivity threshold of the seismometer for most of the night during the early part of the mission. Winds and therefore the seismic background started to intrude into the nighttime hours starting on sol 119 (a sol is a Martian day). The seismic background correlates well with wind velocity and is proportional to the square of the wind velocity, as is appropriate for turbulent flow. The seismic envelope power spectral density is proportional to frequency to the -0.66 to -0.90 power during windy periods. A possible local seismic event was detected on sol 80. No wind data were obtained at the time, so a wind disturbance cannot be ruled out. However, this event has some unusual characteristics and is similar to local events recorded on earth through a Viking seismometer system. If it is interpreted as a natural seismic event, it has a magnitude of 3 and a distance of 110 km. Preliminary interpretation of later arrivals in the signal suggest a crustal thickness of 15 km at the Utopia Planitia site which is within the range of crustal models derived from the gravity field. More events must be recorded before a firm interpretation can be made of seismicity or crustal structure. One firm conclusion is that the natural background noise on Mars is low and that the wind is the prime noise source. It will be possible to reduce this noise by a factor of l0 s on future missions by removing the seismometer from the lander, operation of an extremely sensitive seismometer thus being possible on the surface.},
  keywords = {Background Noise,Lunar and Planetary Exploration,Mars (Planet),Noise Reduction,notion,notion-database,Planetary Crusts,Planetary Mantles,Planetary Structure,Planetology,Seismology,Viking Lander Spacecraft,Wind Effects}
}

@article{Ando1985,
  title = {Examination of {{Wave}} Behaviors in the {{Differentially Rpotating Systems}}},
  author = {Ando, Hiroyasu},
  year = {1985},
  journal = {PASJ},
  volume = {37},
  pages = {47--68},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/I4XAUEUT/Ando - 1985.pdf}
}

@article{Andrae2018,
  title = {Gaia {{Data Release}} 2 {{First}} Stellar Parameters from {{Apsis}}},
  author = {Andrae, Ren{\'e} and Fouesneau, Morgan and Creevey, Orlagh and Ordenovic, Christophe and Mary, Nicolas and Burlacu, Alexandru and Chaoul, Laurence and {Jean-Antoine-Piccolo}, Anne and Kordopatis, Georges and Korn, Andreas and Lebreton, Yveline and Panem, Chantal and Pichon, Bernard and Th{\'e}venin, Fr{\'e}d{\'e}ric and Walmsley, Gavin and {Bailer-Jones}, Coryn A L},
  year = {2018},
  journal = {Astronomy and Astrophysics},
  volume = {616},
  doi = {10.1051/0004-6361/201732516},
  urldate = {2020-03-31},
  abstract = {The second Gaia data release (Gaia DR2) contains, beyond the astrometry, three-band photometry for 1.38 billion sources. One band is the G band, the other two were obtained by integrating the Gaia prism spectra (BP and RP). We have used these three broad photometric bands to infer stellar effective temperatures, T eff , for all sources brighter than G = 17 mag with T eff in the range 3000-10 000 K (some 161 million sources). Using in addition the parallaxes, we infer the line-of-sight extinction, A G , and the reddening, E(BP-RP), for 88 million sources. Together with a bolometric correction we derive luminosity and radius for 77 million sources. These quantities as well as their estimated uncertainties are part of Gaia DR2. Here we describe the procedures by which these quantities were obtained, including the underlying assumptions, comparison with literature estimates, and the limitations of our results. Typical accuracies are of order 324 K (T eff), 0.46 mag (A G), 0.23 mag (E(BP-RP)), 15\% (luminosity), and 10\% (radius). Being based on only a small number of observable quantities and limited training data, our results are necessarily subject to some extreme assumptions that can lead to strong systematics in some cases (not included in the aforementioned accuracy estimates). One aspect is the non-negativity contraint of our estimates, in particular extinction, which we discuss. Yet in several regions of parameter space our results show very good performance, for example for red clump stars and solar analogues. Large uncertainties render the extinctions less useful at the individual star level, but they show good performance for ensemble estimates. We identify regimes in which our parameters should and should not be used and we define a "clean" sample. Despite the limitations, this is the largest catalogue of uniformly-inferred stellar parameters to date. More precise and detailed astrophysical parameters based on the full BP/RP spectrophotometry are planned as part of the third Gaia data release.},
  keywords = {data analysis-methods,fundamental parameters-methods,notion,notion-database,stars,statistical-surveys-catalogs}
}

@misc{Andre2018,
  title = {The Effects of Rotation on Wave-Induced Transport in Stars: From Weakly to Strongly Stratified Radiative Zones},
  shorttitle = {The Effects of Rotation on Wave-Induced Transport in Stars},
  author = {Andr{\'e}, Q. and Mathis, S. and Amard, L.},
  year = {2018},
  month = nov,
  number = {arXiv:1811.02818},
  eprint = {1811.02818},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-08-16},
  abstract = {Internal waves propagating in stellar radiative zones can lead to efficient angular momentum transport, that should occur throughout the whole lifetime of stars. They thus play a key role in shaping the internal rotation profile of these regions, that can be probed by asteroseismology. We present a new analytical study of their propagation and dissipation near the equatorial plane. We include the effects of rotation and differential rotation without making any assumption on their relative strength relative to that of the background stable stratification. This analytical framework allows in principle to scan the efficiency of the wave-induced transport of angular momentum. The computations goes from the pre-main sequence, during which the restoring forces associated with rotation and stratification can be of the same order, to the later stages of evolution, for which stratification tends to dominate over rotation. A first application to the case of a sun-like star is finally discussed.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/HIFLSDTQ/André et al. - 2018 - The effects of rotation on wave-induced transport .pdf;/Users/lbugnet/Zotero/storage/3CGFWKAU/1811.html}
}

@article{Andronov2013,
  title = {Program {{WWZ}}: {{Wavelet}} Analysis of {{Astronomical SIgnals}} with Irregularly Aspaced Arguments},
  author = {Andronov, Ivan L. and Naumova, Alevtina V.},
  year = {2013},
  journal = {Odessa Astronomical Publications},
  volume = {26},
  number = {1},
  isbn = {9783540773405},
  keywords = {cillations,data analysis,directions of modern astrophysics,is,long-period pulsating variables,notion,notion-database,one of the main,quasi-periodic and cyclic os-,u del,variable stars,wavelet analysis},
  file = {/Users/lbugnet/Zotero/storage/4WICD4KA/Andronov, Naumova - 2013.pdf}
}

@article{Angel1981,
  title = {The Magnetic Fields of White Dwarfs},
  author = {Angel, J.R..P. and Borra, Ermanno F. and {Lands}},
  year = {1981},
  journal = {The Astrophysical Journal},
  volume = {45},
  eprint = {1011.1669v3},
  pages = {457--474},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ULPSE32I/Angel, Borra, Lands - 1981.pdf}
}

@article{Angerhausen2015,
  title = {A {{Comprehensive Study}} of {{Kepler Phase Curves}} and {{Secondary Eclipses}}: {{Temperatures}} and {{Albedos}} of {{Confirmed Kepler Giant Planets}}},
  author = {Angerhausen, Daniel and DeLarme, Em and Morse, Jon A.},
  year = {2015},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {127},
  number = {957},
  eprint = {1404.4348},
  pages = {1113--1130},
  issn = {00046280},
  doi = {10.1086/683797},
  abstract = {We present a comprehensive study of phase curves and secondary eclipses in the Kepler data set using all data from 16 quarters that were available in 2013-2014. Our sample consists of 20 confirmed planets with R\_p {$>$} 4 R\_e ,P {$<$} 10d, V\_mag {$<$} 15. Here we derive their temperatures and albedos, with an eye towards constraining models for the formation and evolution of such planets. Where there was overlap our results confirm parameters derived by previous studies, whereas we present new results for Kepler 1b-8b, 12b-15b, 17b, 40b, 41b, 43b, 44b, 76b, 77b, and 412b derived in a consistent manner. We also present lightcurve analyses for Kepler 91b and Kepler 74b, which both show extra dimmings at times other than from the expected primary and secondary eclipses. Corrected for thermal emission we find most of the massive planets from our sample to be low in albedo ({$<$}0.1) with a few having higher albedo ({$>$}0.1).},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JEFTNM8R/Angerhausen, DeLarme, Morse - 2015.pdf}
}

@article{Anguera1992,
  title = {The Low l Solar P-Mode Spectrum at Maximum and Minimum Solar Activity},
  author = {Anguera Gubau, M. and Pall{\'e}, Pere L. and Regulo, C. and Roca Cortes, T.},
  year = {1992},
  journal = {Astronomy \& Astrophysics},
  volume = {255},
  number = {363-372},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QA9UMI7T/Anguera Gubau et al. - 1992.pdf}
}

@article{Angulo1999,
  title = {A Compilation of Charged-Particle Induced Thermonuclear Reaction Rates},
  author = {Angulo, C. and Arnould, M. and Rayet, M. and Descouvemont, P. and Baye, D. and {Leclercq-Willain}, C. and Coc, A. and Barhoumi, S. and Aguer, P. and Rolfs, C. and Kunz, R. and Hammer, J. W. and Mayer, A. and Paradellis, T. and Kossionides, S. and Chronidou, C. and Spyrou, K. and Degl'Innocenti, S. and Fiorentini, G. and Ricci, B. and Zavatarelli, S. and Providencia, C. and Wolters, H. and Soares, J. and Grama, C. and Rahighi, J. and Shotter, A. and Lamehi Rachti, M.},
  year = {1999},
  journal = {Nuclear Physics A},
  volume = {656},
  number = {1},
  pages = {3--183},
  issn = {03759474},
  doi = {10.1016/S0375-9474(99)00030-5},
  abstract = {Low-energy cross section data for 86 charged-particle induced reactions involving light (1 {$\leq$} {$Z$} {$\leq$} 14), mostly stable, nuclei are compiled. The corresponding Maxwellian-averaged thermonuclear reaction rates of relevance in astrophysical plasmas at temperatures in the range from 106 {$K$} to 1010 {$K$} are calculated. These evaluations assume either that the target nuclei are in their ground state, or that the target states are thermally populated following a Maxwell-Boltzmann distribution, except in some cases involving isomeric states. Adopted values complemented with lower and upper limits of the rates are presented in tabular form. Analytical approximations to the adopted rates, as well as to the inverse/direct rate ratios, are provided. \textcopyright{} 1999 Elsevier Science B.V. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GDN7FVVH/Angulo et al. - 1999.pdf}
}

@article{Angus2015,
  title = {Calibrating Gyrochronology Using {{Kepler}} Asteroseismic Targets},
  author = {Angus, Ruth and Aigrain, Suzanne and {Foreman-Mackey}, Daniel and McQuillan, Amy},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {450},
  number = {2},
  eprint = {1502.06965},
  pages = {1787--1798},
  issn = {13652966},
  doi = {10.1093/mnras/stv423},
  abstract = {Among the available methods for dating stars, gyrochronology is a powerful one because it requires knowledge of only the star's mass and rotation period. Gyrochronology relations have previously been calibrated using young clusters, with the Sun providing the only age dependence, and are therefore poorly calibrated at late ages. We used rotation period measurements of 310 Kepler stars with asteroseismic ages, 50 stars from the Hyades and Coma Berenices clusters and 6 field stars (including the Sun) with precise age measurements to calibrate the gyrochronology relation, whilst fully accounting for measurement uncertainties in all observable quantities. We calibrated a relation of the form P = A\textsuperscript{n} \texttimes{} (B - V - c)\textsuperscript{b}, where P is rotation period in days, A is age in Myr, B and V are magnitudes and a, b and n are the free parameters of our model. We found a = 0.40\textsuperscript{+0.3}{$<$}inf{$>$}-0.05{$<$}/inf{$>$}, b = 0.31\textsuperscript{+0.05}{$<$}inf{$>$}-0.02{$<$}/inf{$>$} and n = 0.55\textsuperscript{+0.02}{$<$}inf{$>$}-0.09{$<$}/inf{$>$}. Markov Chain Monte Carlo methods were used to explore the posterior probability distribution functions of the gyrochronology parameters and we carefully checked the effects of leaving out parts of our sample, leading us to find that no single relation between rotation period, colour and age can adequately describe all the subsets of our data. The Kepler asteroseismic stars, cluster stars and local field stars cannot all be described by the same gyrochronology relation. The Kepler asteroseismic stars may be subject to observational biases; however, the clusters show unexpected deviations from the predicted behaviour, providing concerns for the overall reliability of gyrochronology as a dating method.},
  archiveprefix = {arxiv},
  keywords = {Methods: statistical,notion,notion-database,Stars: evolution,Stars: fundamental parameters,Stars: oscillations,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/YWPRILR9/Angus et al. - 2015.pdf}
}

@article{Angus2016,
  title = {Probabilistic {{Inference}} of {{Basic Stellar Parameters}}: {{Application To Flickering Stars}}},
  author = {Angus, Ruth and Kipping, {\relax David}. M.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {823},
  number = {1},
  pages = {L9},
  publisher = {{IOP Publishing}},
  issn = {2041-8213},
  doi = {10.3847/2041-8205/823/1/l9},
  abstract = {The relations between observable stellar parameters are usually assumed to be deterministic. That is, given an infinitely precise measurement of independent variable, `\$x\$', and some model, the value of dependent variable, `\$y\$' can be known exactly. In practise this assumption is rarely valid and intrinsic stochasticity means that two stars with exactly the same `\$x\$', will have slightly different `\$y\$'s. The relation between short-timescale brightness fluctuations (flicker) of stars and both surface gravity and stellar density are two such stochastic relations that have, until now, been treated as deterministic ones. We recalibrate these relations in a probabilistic framework, using Hierarchical Bayesian Modelling (HBM) to constrain the intrinsic scatter in the relations. We find evidence for additional scatter in the relationships, that cannot be accounted for by the observational uncertainties alone. The scatter in surface gravity and stellar density does not depend on flicker, suggesting that using flicker as a proxy for \$\textbackslash log g\$ and \$\textbackslash rho\_\textbackslash star\$ is equally valid for dwarf and giant stars, despite the fact that the observational uncertainties tend to be larger for dwarfs.},
  keywords = {fundamental parameters,methods,methods: statistical,notion,notion-database,photometric,stars,stars: fundamental parameters,statistical,techniques,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/3XTJF8C6/Angus, Kipping - 2016.pdf}
}

@article{Angus2018,
  title = {Inferring Probabilistic Stellar Rotation Periods Using {{Gaussian}} Processes},
  author = {Angus, Ruth and Morton, Timothy and Aigrain, Suzanne and {Foreman-Mackey}, Daniel and Rajpaul, Vinesh},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {474},
  number = {2},
  eprint = {1706.05459},
  issn = {13652966},
  doi = {10.1093/mnras/stx2109},
  abstract = {Variability in the light curves of spotted, rotating stars is often non-sinusoidal and quasiperiodic - spots move on the stellar surface and have finite lifetimes, causing stellar flux variations to slowly shift in phase. A strictly periodic sinusoid therefore cannot accurately model a rotationally modulated stellar light curve. Physical models of stellar surfaces have many drawbacks preventing effective inference, such as highly degenerate or high-dimensional parameter spaces. In this work, we test an appropriate effective model: a Gaussian Process with a quasi-periodic covariance kernel function. This highly flexible model allows sampling of the posterior probability density function of the periodic parameter, marginalizing over the other kernel hyperparameters using a Markov Chain Monte Carlo approach. To test the effectiveness of this method, we infer rotation periods from 333 simulated stellar light curves, demonstrating that the Gaussian process method produces periods that are more accurate than both a sinefitting periodogram and an autocorrelation function method. We also demonstrate that it works well on real data, by inferring rotation periods for 275 Kepler stars with previously measured periods. We provide a table of rotation periods for these and many more, altogether 1102 Kepler objects of interest, and their posterior probability density function samples. Because this method delivers posterior probability density functions, it will enable hierarchical studies involving stellar rotation, particularly those involving population modelling, such as inferring stellar ages, obliquities in exoplanet systems, or characterizing star-planet interactions. The code used to implement this method is available online.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Angus2019,
  title = {Towards Precise Stellar Ages: Combining Isochrone Fitting with Empirical Gyrochronology},
  author = {Angus, Ruth and Morton, Timothy D and {Foreman-Mackey}, Daniel and Van Saders, Jennifer and Curtis, Jason and Kane, Stephen R and Bedell, Megan and Kiman, Rocio and Hogg, David W and Brewer, John},
  year = {2019},
  eprint = {1908.07528v1},
  urldate = {2020-03-08},
  abstract = {We present a new age-dating technique that combines gyrochronology with isochrone fitting to infer ages for FGKM main-sequence and subgiant field stars. Gyrochronology and isochrone fitting are each capable of providing relatively precise ages for field stars in certain areas of the Hertzsprung-Russell diagram: gyrochronology works optimally for cool main-sequence stars, and isochrone fitting can provide precise ages for stars near the main-sequence turnoff. Combined , these two age-dating techniques can provide precise and accurate ages for a broader range of stellar masses and evolutionary stages than either method used in isolation. We demonstrate that the position of a star on the Hertzsprung-Russell or color-magnitude diagram can be combined with its rotation period to infer a precise age via both isochrone fitting and gyrochronology simultaneously. We show that incorporating rotation periods with 5\% uncertainties into stellar evolution models improves age precision for FGK stars on the main sequence , and can, on average, provide age estimates up to three times more precise than isochrone fitting alone. In addition, we provide a new gyrochronology-2-relation, calibrated to the Praesepe cluster and the Sun, that includes a variance model to capture the rotational behavior of stars whose rotation periods do not lengthen with the square-root of time, and parts of the Hertzsprung-Russell diagram where gyrochronology has not been calibrated. This publication is accompanied by an open source Python package, stardate, for inferring the ages of main-sequence and subgiant FGKM stars from rotation periods, spectroscopic parameters and/or apparent magnitudes and parallaxes.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YIAFU2SP/full-text.pdf}
}

@article{Antia1994,
  title = {Nonasymptotic Helioseismic Inversion for Solar Structure. - {{NASA}}/{{ADS}}},
  author = {Antia, H. M. and Basu, Sarbani},
  year = {1994},
  journal = {Astronomy \& Astrophysics Supplement Series},
  volume = {107},
  pages = {421--444},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TXY4YEXV/Antia, Basu - 1994.pdf}
}

@article{Antia2000,
  title = {The {{Sun}}'s Acoustic Asphericity and Magnetic Fields in the Solar Convection Zone},
  author = {Antia, H. M. and Chitre, S. M. and Thompson, M. J.},
  year = {2000},
  month = may,
  eprint = {astro-ph/0005587},
  urldate = {2020-07-03},
  abstract = {The observed splittings of solar oscillation frequencies can be employed to separate the effects of internal solar rotation and to estimate the contribution from a large-scale magnetic field or any latitude-dependent thermal perturbation inside the Sun. The surface distortion estimated from the rotation rate in the solar interior is found to be in good agreement with the observed oblateness at solar surface. After subtracting out the estimated contribution from rotation, there is some residual signal in the even splitting coefficients, which may be explained by a magnetic field of approximately 20 kG strength located at a depth of 30000 km below the surface or an equivalent aspherical thermal perturbation. An upper limit of 300 kG is derived for a toroidal field near the base of the convection zone.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WJ42FNDF/full-text.pdf}
}

@article{Antia2010,
  title = {Solar Rotation Rate during the Cycle 24 Minimum in Activity},
  author = {Antia, H. M. and Basu, Sarbani},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {720},
  number = {1},
  eprint = {1008.1787},
  pages = {494--502},
  issn = {15384357},
  doi = {10.1088/0004-637X/720/1/494},
  abstract = {The minimum of solar cycle 24 is significantly different from most other minima in terms of its duration as well as its abnormally low levels of activity. Using available helioseismic data that cover epochs from the minimum of cycle 23 to now, we study the differences in the nature of the solar rotation between the minima of cycles 23 and 24. We find that there are significant differences between the rotation rates during the two minima. There are differences in the zonal-flow pattern too. We find that the band of fast rotating region close to the equator bifurcated around 2005 and recombined by 2008. This behavior is different from that during the cycle 23 minimum. By autocorrelating the zonal-flow pattern with a time shift, we find that in terms of solar dynamics, solar cycle 23 lasted for a period of 11.7 years, consistent with the result of Howe et al. (2009). The autocorrelation coefficient also confirms that the zonal-flow pattern penetrates through the convection zone. \textcopyright{} 2010. The American Astronomical Society. All rights reserved. Printed in the U.S.A.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/L8MGGD4K/Antia, Basu - 2010.pdf}
}

@article{Antia2011,
  title = {Revisiting the Solar Tachocline: {{Average}} Properties and Temporal Variations},
  author = {Antia, H. M. and Basu, Sarbani},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {735},
  number = {2},
  eprint = {1107.1004},
  pages = {1--13},
  issn = {20418205},
  doi = {10.1088/2041-8205/735/2/L45},
  abstract = {The tachocline is believed to be the region where the solar dynamo operates. With over a solar cycle's worth of data available from the Michelson Doppler Imager and Global Oscillation Network Group instruments, we are in a position to investigate not merely the average structure of the solar tachocline, but also its time variations. We determine the properties of the tachocline as a function of time by fitting a two-dimensional model that takes latitudinal variations of the tachocline properties into account. We confirm that if we consider the central position of the tachocline, it is prolate. Our results show that the tachocline is thicker at latitudes higher than the equator, making the overall shape of the tachocline more complex. Of the tachocline properties examined, the transition of the rotation rate across the tachocline, and to some extent the position of the tachocline, show some temporal variations. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/Q49IPVAK/Antia, Basu - 2011.pdf}
}

@article{Antoci2011,
  title = {The Excitation of Solar-like Oscillations in a {$\delta$} {{Sct}} Star by Efficient Envelope Convection},
  author = {Antoci, V. and Handler, G. and Campante, T. L. and Thygesen, A. O. and Moya, A. and Kallinger, T. and Stello, D. and Grigahc{\`e}ne, A. and Kjeldsen, H. and Bedding, T. R. and L{\"u}ftinger, T. and {Christensen-Dalsgaard}, J. and Catanzaro, G. and Frasca, A. and De Cat, P. and Uytterhoeven, K. and Bruntt, H. and Houdek, G. and Kurtz, D. W. and Lenz, P. and Kaiser, A. and Van Cleve, J. and Allen, C. and Clarke, B. D.},
  year = {2011},
  journal = {Nature},
  volume = {477},
  number = {7366},
  eprint = {1109.4285},
  pages = {570--573},
  issn = {14764687},
  doi = {10.1038/nature10389},
  abstract = {Delta Scuti ({$\delta$}Sct)1 stars are opacity-driven pulsators with masses of 1.5-2.5M {\.O}, their pulsations resulting from the varying ionization of helium. In less massive stars such as the Sun, convection transports mass and energy through the outer 30 per cent of the star and excites a rich spectrum of resonant acoustic modes. Based on the solar example, with no firm theoretical basis, models predict that the convective envelope in {$\delta$}Sct stars extends only about 1per cent of the radius, but with sufficient energy to excite solar-like oscillations. This was not observed before the Kepler mission, so the presence of a convective envelope in the models has been questioned. Here we report the detection of solar-like oscillations in the {$\delta$}Sct star HD187547, implying that surface convection operates efficiently in stars about twice as massive as the Sun, as the ad hoc models predicted. \textcopyright{} 2011 Macmillan Publishers Limited. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/A23PIIJ9/Antoci et al. - 2011.pdf}
}

@article{Antoci2019,
  title = {The First View of {$\delta$} {{Scuti}} and {$\gamma$} {{Doradus}} Stars with the {{TESS}} Mission},
  author = {Antoci, V. and Cunha, M. S. and Bowman, D. M. and Murphy, S. J. and Kurtz, D. W. and Bedding, T. R. and Borre, C. C. and Christophe, S. and {Daszy{\'n}ska-Daszkiewicz}, J. and {Fox-Machado}, L. and Garc{\'i}a Hern{\'a}ndez, A. and Ghasemi, H. and Handberg, R. and Hansen, H. and Hasanzadeh, A. and Houdek, G. and Johnston, C. and Justesen, A. B. and Kahraman Alicavus, F. and Kotysz, K. and Latham, D. and Matthews, J. M. and M{\o}nster, J. and Niemczura, E. and Paunzen, E. and S{\'a}nchez Arias, J. P. and Pigulski, A. and Pepper, J. and {Richey-Yowell}, T. and Safari, H. and Seager, S. and Smalley, B. and Shutt, T. and S{\'o}dor, A. and Su{\'a}rez, J. -C. and Tkachenko, A. and Wu, T. and Zwintz, K. and Barcel{\'o} Forteza, S. and Brunsden, E. and Bogn{\'a}r, Z. and Buzasi, D. L. and Chowdhury, S. and De Cat, P. and Evans, J. A. and Guo, Z. and Guzik, J. A. and Jevtic, N. and Lampens, P. and Lares Martiz, M. and Lovekin, C. and Li, G. and Mirouh, G. M. and Mkrtichian, D. and Monteiro, M. J. P. F. G. and Nemec, J. M. and Ouazzani, R. -M. and {Pascual-Granado}, J. and Reese, D. R. and Rieutord, M. and Rodon, J. R. and Skarka, M. and Sowicka, P. and Stateva, I. and Szab{\'o}, R. and Weiss, W. W.},
  year = {2019},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {490},
  pages = {4040--4059},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz2787},
  urldate = {2023-10-17},
  abstract = {We present the first asteroseismic results for {$\delta$} Scuti and {$\gamma$} Doradus stars observed in Sectors 1 and 2 of the TESS mission. We utilize the 2-min cadence TESS data for a sample of 117 stars to classify their behaviour regarding variability and place them in the Hertzsprung-Russell diagram using Gaia DR2 data. Included within our sample are the eponymous members of two pulsator classes, {$\gamma$} Doradus and SX Phoenicis. Our sample of pulsating intermediate-mass stars observed by TESS also allows us to confront theoretical models of pulsation driving in the classical instability strip for the first time and show that mixing processes in the outer envelope play an important role. We derive an empirical estimate of 74 per cent for the relative amplitude suppression factor as a result of the redder TESS passband compared to the Kepler mission using a pulsating eclipsing binary system. Furthermore, our sample contains many high-frequency pulsators, allowing us to probe the frequency variability of hot young {$\delta$} Scuti stars, which were lacking in the Kepler mission data set, and identify promising targets for future asteroseismic modelling. The TESS data also allow us to refine the stellar parameters of SX Phoenicis, which is believed to be a blue straggler.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: chemically peculiar,stars: interiors,stars: variables: {$\delta$} Scuti,techniques: photometric},
  annotation = {ADS Bibcode: 2019MNRAS.490.4040A},
  file = {/Users/lbugnet/Zotero/storage/9YY5KDZB/Antoci et al. - 2019 - The first view of δ Scuti and γ Doradus stars with.pdf}
}

@article{Appourchaux1997,
  title = {In-Flight Performance of the Virgo Luminosity Oscillations Imager Aboard Soho},
  author = {Appourchaux, Thierry and Andersen, B. O.N. and Fr{\"o}hlich, Claus and Jim{\'e}nez, Antonio and Telljohann, Udo and Wehrli, Christoph},
  year = {1997},
  journal = {Solar Physics},
  volume = {170},
  number = {1},
  pages = {27--41},
  issn = {00380938},
  doi = {10.1023/A:1004999005915},
  abstract = {The Luminosity Oscillations Imager (LOI) is a part of the VIRGO instrument aboard the Solar and Heliospheric Observatory (SOHO). The scientific objective of the LOI experiment is to identify and characterize pressure and internal gravity oscillations of the Sun by observing the radiance variations. The LOI is a low-resolution imager with 12 pixels, for the measurement of the radiance distribution over the solar disk at 500 nm. The low resolution capability of the instrument allows the identification of individual azimuthal orders for l = 0 to 7, without suffering the mixing that affects integrated solar disk instruments. The performance, calibrations and instrumental effects of the LOI are described together with the procedures for extracting the solar p modes.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LZFEWUIN/Appourchaux et al. - 1997.pdf}
}

@article{Appourchaux1998a,
  title = {The Art of Fitting P-Mode Spectra. {{I}}. {{Maximum}} Likelihood Estimation},
  author = {Appourchaux, T. and Gizon, L. and {Rabello-Soares}, M. C.},
  year = {1998},
  journal = {Astronomy and Astrophysics Supplement Series},
  volume = {132},
  number = {1},
  eprint = {astro-ph/9710082},
  pages = {107--119},
  issn = {03650138},
  doi = {10.1051/aas:1998441},
  abstract = {In this article we present our state of the art of fitting helioseismic p-mode spectra. We give a step by step recipe for fitting the spectra: statistics of the spectra both for spatially unresolved and resolved data, the use of Maximum Likelihood estimates, the statistics of the p-mode parameters, the use of Monte-Carlo simulation and the significance of fitted parameters. The recipe is applied to synthetic low-resolution data, similar to those of the LOI, using Monte-Carlo simulations. For such spatially resolved data, the statistics of the Fourier spectrum is assumed to be a multi-normal distribution; the statistics of the power spectrum is not a {$\chi$}2 with 2 degrees of freedom. Results for l = 1 shows that all parameters describing the p modes can be obtained with negligible bias and with minimum variance provided that the leakage matrix is known. Systematic errors due to an imperfect knowledge of the leakage matrix are derived for all the p-mode parameters.},
  archiveprefix = {arxiv},
  keywords = {Methods: analytical; data analysis; statistical,notion,notion-database,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/BNC6BL7W/Appourchaux, Gizon, Rabello-Soares - 1998.pdf}
}

@article{Appourchaux2000,
  title = {Observational {{Upper Limits}} to {{Low}}-{{Degree Solar}} g -{{Modes}}},
  author = {Appourchaux, T. and Frohlich, C. and Andersen, B. and Berthomieu, G. and Chaplin, W. J. and Elsworth, Y. and Finsterle, W. and Gough, D. O. and Hoeksema, J. T. and Isaak, G. R. and Kosovichev, A. G. and Provost, J. and Scherrer, P. H. and Sekii, T. and Toutain, T.},
  year = {2000},
  journal = {The Astrophysical Journal},
  volume = {538},
  number = {1},
  pages = {401--414},
  issn = {0004-637X},
  doi = {10.1086/309124},
  abstract = {Observations made by the Michelson Doppler Imager (MDI) and Variability of solar IRradiance and Gravity Oscillations (VIRGO) on the Solar and Heliospheric Observatory (SOHO) and by the ground-based Birmingham Solar Oscillations Network (BiSON) and Global Oscillations Network Group (GONG) have been used in a concerted effort to search for solar gravity oscillations. All spectra are dominated by solar noise in the frequency region from 100 to 1000 {$\mu$}Hz, where g-modes are expected to be found. Several methods have been used in an effort to extract any g-mode signal present. These include (1) the correlation of data-both full-disk and imaged (with different spatial-mask properties)-collected over different time intervals from the same instrument, (2) the correlation of near-contemporaneous data from different instruments, and (3) the extraction-through the application of complex filtering techniques-of the coherent part of data collected at different heights in the solar atmosphere. The detection limit is set by the loss of coherence caused by the temporal evolution and the motion (e.g., rotation) of superficial structures. Although we cannot identify any g-mode signature, we have nevertheless set a firm upper limit to the amplitudes of the modes: at 200 {$\mu$}Hz, they are below 10 mm s-1 in velocity, and below 0.5 parts per million in intensity. The velocity limit corresponds very approximately to a peak-to-peak vertical displacement of {$\delta$}R/Rsolar=2.3\texttimes 10-8 at the solar surface. These levels which are much lower than prior claims, are consistent with theoretical predictions.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GNINWCHV/Appourchaux et al. - 2000.pdf}
}

@article{Appourchaux2003a,
  title = {On {{Maximum Likelihood Estimation}} of Averaged Power Spectra},
  author = {Appourchaux, T.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {412},
  number = {3},
  pages = {903--904},
  issn = {00046361},
  doi = {10.1051/0004-6361:20034401},
  abstract = {It is custom in helioseismology to assume that the power spectra of time series of solar radial velocity or of solar intensity have {$\chi$}2 with 2 degrees of freedom statistics. This assumption is regularly used in helioseismology for using Maximum Likelihood Estimators for single power spectra with that assumed statistics. When independent power spectra are added, it is also custom to assume that the resulting power spectra can be approximated by a Gaussian distribution. Here we show that this approximation is irrelevant, and that the software code developed for fitting single power spectra can be used without any approximation after proper normalization of the added power spectra.},
  keywords = {Methods: analytical,Methods: data analysis,Methods: statistical,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/P92AVSJS/Appourchaux - 2003.pdf}
}

@article{Appourchaux2004,
  title = {On Detecting Short-Lived p Modes in a Stellar Oscillation Spectrum},
  author = {Appourchaux, T.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {428},
  number = {3},
  pages = {1039--1042},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041682},
  abstract = {The false alarm probability for detecting peaks embedded in a power spectrum of noise was given by Scargle (1982). This test has been used in helioseismology to detect long-lived modes such as g modes (Appourchaux et al. 2000). With the development of asteroseismology, there is now a need to define a similar test but for short-lived p modes. In this article, I define a false alarm test for detecting short-lived p modes, and I give the probability of detecting such modes given their signal-to-noise ratio, their linewidths and the duration of observation.},
  keywords = {Methods: statistical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/487J7N8Z/Appourchaux - 2004.pdf}
}

@article{Appourchaux2007a,
  title = {On Cross-Spectrum Capabilities for Detecting Stellar Oscillation Modes},
  author = {Appourchaux, T. and Leibacher, J. and Boumier, P.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {463},
  number = {3},
  pages = {1211--1214},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065271},
  abstract = {Aims. Long-lived stellar oscillation modes are usually detected using Fourier transforms of time series of stellar radial velocities or brightness. It is commonly thought that one could use the cross spectrum of the two signals, or alternatively use the interleaved series of a single signal, to considerably improve the detection level by reducing the noise level. Methods. We use a statistical analysis of the cross spectrum to compute its mean value and rms value, and use the associated signal-to-noise ratio for stochastically excited modes. Results. Here, we demonstrate that the gain in the signal-to-noise ratio can indeed be improved for modes with a shorter lifetime than the observation time, but not those with a longer lifetime than the observation time. \textcopyright{} ESO 2007.},
  keywords = {Methods: analytical,Methods: statistical,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/T4RVDMHL/Appourchaux, Leibacher, Boumier - 2007.pdf}
}

@article{Appourchaux2007b,
  title = {On Understanding the Meaning of 1 = 2 and 3 P-Mode Frequencies as Measured by Various Helioseismic Instruments ({{Research Note}})},
  author = {Appourchaux, T. and Chaplin, W. J.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {469},
  number = {3},
  pages = {1151--1154},
  issn = {00046361},
  doi = {10.1051/0004-6361:20077492},
  abstract = {Aims. Frequencies of the low-degree p-mode oscillations of the Sun may be extracted either from data collected by instruments that make full-disc observations of the Sun as a star, or from data collected by instruments that resolve, or image, the Sun's surface onto many detector elements. The two methods can show marked differences in their sensitivity to modes having certain combinations of degree and azimuthal order. These different sensitivities lead to differences in measurements of the central frequencies of the modes, which must be properly accounted for if data from two different instruments are to be compared, or combined. Methods. We perform an analytical derivation of the p-mode frequency offsets expected between contemporaneous Sun-as-a-star and resolved-Sun data. Results. Here, we demonstrate that the empirical factors derived by Chaplin et al. (2004, A\&A, 424, 713) are reproduced by our analysis, but with a more marked dependence upon the mode linewidth. \textcopyright{} ESO 2007.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ANGLYLRH/Appourchaux, Chaplin - 2007.pdf}
}

@article{Appourchaux2008,
  title = {Bayesian Approach for G-Mode Detection, or How to Restrict Our Imagination},
  author = {Appourchaux, T.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  eprint = {0711.0435},
  pages = {485--489},
  issn = {00046337},
  doi = {10.1002/asna.200710981},
  abstract = {Nowadays, g-mode detection is based upon a priori theoretical knowledge. By doing so, detection becomes more restricted to what we can imagine. De facto, the universe of possibilities ismade narrower. Such an approach is pertinent for Bayesian statisticians. Examples of how Bayesian inferences can be applied to spectral analysis and helioseismic power spectra are given. Our intention is not to give the full statistical framework (much too ambitious) but to provide an appetizer for going further in the direction of a proper Bayesian inference, especially for detecting gravity modes. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  archiveprefix = {arxiv},
  keywords = {Methods: statistical,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WQ87FAJ4/Appourchaux - 2008.pdf}
}

@article{Appourchaux2008a,
  title = {{{CoRoT}} Sounds the Stars: {{P-mode}} Parameters of {{Sun-like}} Oscillations on {{HD}} 49933},
  author = {Appourchaux, T. and Michel, E. and Auvergne, M. and Baglin, A. and Toutain, T. and Baudin, F. and Benomar, O. and Chaplin, W. J. and Deheuvels, S. and Samadi, R. and Verner, G. A. and Boumier, P. and Garc{\'i}a, R. A. and Mosser, B. and Hulot, J. C. and Ballot, J. and Barban, C. and Elsworth, Y. and {Jim{\'e}nez-Reyes}, S. J. and Kjeldsen, H. and R{\'e}gulo, C. and Roxburgh, I. W.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {488},
  number = {2},
  pages = {705--714},
  issn = {00046361},
  doi = {10.1051/0004-6361:200810297},
  abstract = {Context: The first asteroseismology results from CoRoT are presented, on a star showing Sun-like oscillations. We have analyzed a 60 day lightcurve of high-quality photometric data collected by CoRoT on the F5 V star HD 49933. The data reveal a rich spectrum of overtones of low-degree p modes. Aims: Our aim was to extract robust estimates of the key parameters of the p modes observed in the power spectrum of the lightcurve. Methods: Estimation of the mode parameters was performed using maximum likelihood estimation of the power spectrum. A global fitting strategy was adopted whereby 15 mode orders of the mode spectrum (45 modes) were fitted simultaneously. Results: The parameter estimates that we list include mode frequencies, peak linewidths, mode amplitudes, and a mean rotational frequency splitting. We find that the average large frequency (overtone) spacing derived from the fitted mode frequencies is 85.9 0.15 Hz. The frequency of maximum amplitude of the radial modes is at 1760 Hz, where the observed rms mode amplitude is 3.75 0.23 ppm. The mean rotational splitting of the non-radial modes appears to be in the range 2.7 Hz to 3.4 Hz. The angle of inclination offered by the star, as determined by fits to the amplitude ratios of the modes, appears to be in the range degrees to degrees.. \textcopyright{} 2008 ESO.},
  keywords = {Methods: observational,Methods: statistical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/Y6KH6TRZ/Appourchaux et al. - 2008.pdf}
}

@article{Appourchaux2010,
  title = {The Quest for the Solar g Modes},
  author = {Appourchaux, T. and Belkacem, K. and Broomhall, A. M. and Chaplin, W. J. and Gough, D. O. and Houdek, G. and Provost, J. and Baudin, F. and Boumier, P. and Elsworth, Y. and Garc{\'i}a, R. A. and Andersen, B. N. and Finsterle, W. and Fr{\"o}hlich, C. and Gabriel, A. and Grec, G. and Jim{\'e}nez, A. and Kosovichev, A. and Sekii, T. and Toutain, T. and {Turck-Chi{\`e}ze}, S.},
  year = {2010},
  journal = {Astronomy and Astrophysics Review},
  volume = {18},
  number = {1-2},
  eprint = {0910.0848},
  pages = {197--277},
  issn = {09354956},
  doi = {10.1007/s00159-009-0027-z},
  abstract = {Solar gravity modes (or g modes)-oscillations of the solar interior on which buoyancy acts as the restoring force-have the potential to provide unprecedented inference on the structure and dynamics of the solar core, inference that is not possible with the well-observed acoustic modes (or p modes). The relative high amplitude of the g-mode eigenfunctions in the core and the evanesence of the modes in the convection zone make the modes particularly sensitive to the physical and dynamical conditions in the core. Owing to the existence of the convection zone, the g modes have very low amplitudes at photospheric levels, which makes the modes extremely hard to detect. In this article, we review the current state of play regarding attempts to detect g modes. We review the theory of g modes, including theoretical estimation of the g-mode frequencies, amplitudes and damping rates. Then we go on to discuss the techniques that have been used to try to detect g modes. We review results in the literature, and finish by looking to the future, and the potential advances that can be made-from both data and data-analysis perspectives-to give unambiguous detections of individual g modes. The review ends by concluding that, at the time of writing, there is indeed a consensus amongst the authors that there is currently no undisputed detection of solar g modes. \textcopyright{} 2010 Springer-Verlag.},
  archiveprefix = {arxiv},
  keywords = {Data analysis,G modes,notion,notion-database,Sun,Theory},
  file = {/Users/lbugnet/Zotero/storage/LF4A4WUR/Appourchaux et al. - 2010.pdf}
}

@article{Appourchaux2012,
  title = {Oscillation Mode Frequencies of 61 Main-Sequence and Subgiant Stars Observed by {{Kepler}}},
  author = {Appourchaux, T. and Chaplin, W. J. and Garc{\'i}a, R. A. and Gruberbauer, M. and Verner, G. A. and Antia, H. M. and Benomar, O. and Campante, T. L. and Davies, G. R. and Deheuvels, S. and Handberg, R. and Hekker, S. and Howe, R. and R{\'e}gulo, C. and Salabert, D. and Bedding, T. R. and White, T. R. and Ballot, J. and Mathur, S. and Silva Aguirre, V. and Elsworth, Y. P. and Basu, S. and L Gilliland, R. and {Christensen-Dalsgaard}, J. and Kjeldsen, H. and Uddin, K. and Stumpe, M. C. and Barclay, T.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {543},
  eprint = {1204.3147},
  issn = {00046361},
  doi = {10.1051/0004-6361/201218948},
  abstract = {Context. Solar-like oscillations have been observed by Kepler and CoRoT in several solar-type stars, thereby providing a way to probe the stars using asteroseismology Aims. We provide the mode frequencies of the oscillations of various stars required to perform a comparison with those obtained from stellar modelling. Methods. We used a time series of nine months of data for each star. The 61 stars observed were categorised in three groups: simple, F-like, and mixed-mode. The simple group includes stars for which the identification of the mode degree is obvious. The F-like group includes stars for which the identification of the degree is ambiguous. The mixed-mode group includes evolved stars for which the modes do not follow the asymptotic relation of low-degree frequencies. Following this categorisation, the power spectra of the 61 main-sequence and subgiant stars were analysed using both maximum likelihood estimators and Bayesian estimators, providing individual mode characteristics such as frequencies, linewidths, and mode heights. We developed and describe a methodology for extracting a single set of mode frequencies from multiple sets derived by different methods and individual scientists. We report on how one can assess the quality of the fitted parameters using the likelihood ratio test and the posterior probabilities. Results. We provide the mode frequencies of 61 stars (with their 1-{$\sigma$} error bars), as well as their associated \'echelle diagrams. \textcopyright{} 2012 ESO.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/UI8GS7G7/Appourchaux et al. - 2012.pdf}
}

@article{Appourchaux2013,
  title = {The History of G-Mode Detection},
  author = {Appourchaux, T. and Pall{\'e}, P.},
  year = {2013},
  eprint = {1309.3835},
  pages = {1--11},
  abstract = {The quest for the solar gravity modes (or g modes) is key for the understanding of the structure and dynamics of the solar core. In this paper, we review the history of the solar g-mode detection which is separated in three nearly distinct era which corresponds to: the theory of g modes, the detections from the ground and the detections from space. The prospects of definitive solar g-mode detection are also discussed.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GEGZHNVY/Appourchaux, Pallé - 2013.pdf}
}

@article{Appourchaux2014,
  title = {Oscillation Mode Linewidths and Heights of 23 Main-Sequence Stars Observed by {{Kepler}}},
  author = {Appourchaux, T. and Antia, H. M. and Benomar, O. and Campante, T. L. and Davies, G. R. and Handberg, R. and Howe, R. and R{\'e}gulo, C. and Belkacem, K. and Houdek, G. and Garc{\'i}a, R. A. and Chaplin, W. J.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {566},
  pages = {1--35},
  issn = {14320746},
  doi = {10.1051/0004-6361/201323317},
  abstract = {Context. Solar-like oscillations have been observed by Kepler and CoRoT in many solar-type stars, thereby providing a way to probe the stars using asteroseismology. Aims. We provide the mode linewidths and mode heights of the oscillations of various stars as a function of frequency and of effective temperature. Methods. We used a time series of nearly two years of data for each star. The 23 stars observed belong to the simple or F-like category. The power spectra of the 23 main-sequence stars were analysed using both maximum likelihood estimators and Bayesian estimators, providing individual mode characteristics such as frequencies, linewidths, and mode heights. We study the source of systematic errors in the mode linewidths and mode heights, and we present a way to correct these errors with respect to a common reference fit. Results. Using the correction, we can explain all sources of systematic errors, which could be reduced to less than {$\pm$}15\% for mode linewidths and heights, and less than {$\pm$}5\% for amplitude, when compared to the reference fit. The effect of a different estimated stellar background and a different estimated splitting will provide frequency-dependent systematic errors that might affect the comparison with theoretical mode linewidth and mode height, therefore affecting the understanding of the physical nature of these parameters. All other sources of relative systematic errors are less dependent upon frequency. We also provide the dependence of the so-called linewidth dip in the middle of the observed frequency range as a function of effective temperature. We show that the depth of the dip decreases with increasing effective temperature. The dependence of the dip on effective temperature may imply that the mixing length parameter {$\alpha$} or the convective flux may increase with effective temperature. \textcopyright{} ESO, 2014.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: interiors},
  file = {/Users/lbugnet/Zotero/storage/DCNFT3NC/Appourchaux et al. - 2014(2).pdf;/Users/lbugnet/Zotero/storage/GSRMMBPF/Appourchaux et al. - 2014.pdf}
}

@article{Appourchaux2015,
  title = {A Seismic and Gravitationally Bound Double Star Observed by {{Kepler}}: {{Implication}} for the Presence of a Convective Core},
  author = {Appourchaux, T. and Antia, H. M. and Ball, W. and Creevey, O. and Lebreton, Y. and Verma, K. and Vorontsov, S. and Campante, T. L. and Davies, G. R. and Gaulme, P. and R{\'e}gulo, C. and Horch, E. and Howell, S. and Everett, M. and Ciardi, D. and Fossati, L. and Miglio, A. and Montalb{\'a}n, J. and Chaplin, W. J. and Garc{\'i}a, R. A. and Gizon, L.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {582},
  pages = {1--19},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526610},
  abstract = {Context. Solar-like oscillations have been observed by Kepler and CoRoT in many solar-type stars, thereby providing a way to probe stars using asteroseismology. Aims. The derivation of stellar parameters has usually been done with single stars. The aim of the paper is to derive the stellar parameters of a double-star system (HIP93511), for which an interferometric orbit has been observed along with asteroseismic measurements. Methods. We used a time series of nearly two years of data for the double star to detect the two oscillation-mode envelopes that appear in the power spectrum. Using a new scaling relation based on luminosity, we derived the radius and mass of each star. We derived the age of each star using two proxies: one based upon the large frequency separation and a new one based upon the small frequency separation. Using stellar modelling, the mode frequencies allowed us to derive the radius, the mass, and the age of each component. In addition, speckle interferometry performed since 2006 has enabled us to recover the orbit of the system and the total mass of the system. Results. From the determination of the orbit, the total mass of the system is 2.34-0.33+0.45 M{$\odot$}. The total seismic mass using scaling relations is 2.47 {$\pm$} 0.07 M{$\odot$}. The seismic age derived using the new proxy based upon the small frequency separation is 3.5 {$\pm$} 0.3 Gyr. Based on stellar modelling, the mean common age of the system is 2.7-3.9 Gyr. The mean total seismic mass of the system is 2.34-2.53 M{$\odot$} consistent with what we determined independently with the orbit. The stellar models provide the mean radius, mass, and age of the stars as RA = 1.82-1.87R{$\odot$}, MA = 1.25-1.39 M{$\odot$}, AgeA = 2.6-3.5 Gyr; RB = 1.22-1.25 R{$\odot$}, MB = 1.08-1.14 M{$\odot$}, AgeB = 3.35-4.21 Gyr. The models provide two sets of values for Star A: [1.25-1.27] M{$\odot$} and [1.34-1.39] M{$\odot$}. We detect a convective core in Star A, while Star B does not have any. For the metallicity of the binary system of Z {$\approx$} 0.02, we set the limit between stars having a convective core in the range [1.14-1.25] M{$\odot$}.},
  keywords = {asteroseismology,astrometry,binaries: general,notion,notion-database,stars: evolution,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/R6N3KJS2/Appourchaux et al. - 2015.pdf}
}

@article{Appourchaux2018,
  title = {Searching for g Modes: {{Part I}}. {{A}} New Calibration of the {{GOLF}} Instrument},
  author = {Appourchaux, T. and Boumier, P. and Leibacher, J. W. and Corbard, T.},
  year = {2018},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {607},
  number = {A108},
  eprint = {1807.00998},
  doi = {10.1051/0004-6361/201833535},
  urldate = {2020-07-29},
  abstract = {The recent claims of g-mode detection have restarted the search for these potentially extremely important modes. These claims can be reassessed in view of the different data sets available from the SoHO instruments and ground-based instruments. We produce a new calibration of the GOLF data with a more consistent p-mode amplitude and a more consistent time shift correction compared to the time series used in the past. The calibration of 22 years of GOLF data is done with a simpler approach that uses only the predictive radial velocity of the SoHO spacecraft as a reference. Using p modes, we measure and correct the time shift between ground- and space-based instruments and the GOLF instrument. The p-mode velocity calibration is now consistent to within a few percent with other instruments. The remaining time shifts are within \$\textbackslash pm\$ 5 s for 99.8\% of the time series. Accepted by A\&A on June 29, 2018},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/A9SAVXDK/full-text.pdf}
}

@article{Arentoft2008,
  title = {A {{Multisite Campaign}} to {{Measure Solar}}-like {{Oscillations}} in {{Procyon}}. {{I}}. {{Observations}}, {{Data Reduction}}, and {{Slow Variations}}},
  author = {Arentoft, Torben and Kjeldsen, Hans and Bedding, Timothy R. and Bazot, Micha{\"e}l and Christensen-Dalsgaard, J{\o}rgen and Dall, Thomas H. and Karoff, Christoffer and Carrier, Fabien and Eggenberger, Patrick and Sosnowska, Danuta and Wittenmyer, Robert A. and Endl, Michael and Metcalfe, Travis S. and Hekker, Saskia and Reffert, Sabine and Butler, R. Paul and Bruntt, Hans and Kiss, L{\'a}szl{\'o} L. and O'Toole, Simon J. and Kambe, Eiji and Ando, Hiroyasu and Izumiura, Hideyuki and Sato, Bun'ei and Hartmann, Michael and Hatzes, Artie and Bouchy, Francois and Mosser, Benoit and Appourchaux, Thierry and Barban, Caroline and Berthomieu, Gabrielle and Garcia, Rafael A. and Michel, Eric and Provost, Janine and Turck-Chi{\`e}ze, Sylvaine and Marti{\'c}, Milena and Lebrun, Jean-Claude and Schmitt, Jerome and Bertaux, Jean-Loup and Bonanno, Alfio and Benatti, Serena and Claudi, Riccardo U. and Cosentino, Rosario and Leccia, Silvio and Frandsen, S{\o}ren and Brogaard, Karsten and Glowienka, Lars and Grundahl, Frank and Stempels, Eric},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {687},
  number = {2},
  pages = {1180--1190},
  issn = {0004-637X},
  doi = {10.1086/592040},
  abstract = {We have carried out a multisite campaign to measure oscillations in the F5 star Procyon A. We obtained high-precision velocity observations over more than three weeks with 11 telescopes, with almost continuous coverage for the central 10 days. This represents the most extensive campaign so far organized on any solar-type oscillator. We describe in detail the methods we used for processing and combining the data. These involved calculating weights for the velocity time series from the measurement uncertainties and adjusting them in order to minimize the noise level of the combined data. The time series of velocities for Procyon shows the clear signature of oscillations, with a plateau of excess power that is centered at 0.9 mHz and is broader than has been seen for other stars. The mean amplitude of the radial modes is 38.1 {$\pm$} 1.3 cm s -1 (2.0 times solar), which is consistent with previous detections from the ground and by the WIRE spacecraft, and also with the upper limit set by the MOST spacecraft. The variation of the amplitude during the observing campaign allows us to estimate the mode lifetime to be 1.5-0.8 +1.9 days. We also find a slow variation in the radial velocity of Procyon, with good agreement between different telescopes. These variations are remarkably similar to those seen in the Sun, and we interpret them as being due to rotational modulation from active regions on the stellar surface. The variations appear to have a period of about 10 days, which presumably equals the stellar rotation period or, perhaps, half of it. The amount of power in these slow variations indicates that the fractional area of Procyon covered by active regions is slightly higher than for the Sun. \textcopyright{} 2008. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QSTPND2P/Arentoft et al. - 2008.pdf}
}

@article{Arlt2010,
  title = {Amplification and Stability of Magnetic Fields and Dynamo Effect in Young {{A}} Stars},
  author = {Arlt, R. and Ruediger, G.},
  year = {2010},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {412},
  number = {1},
  eprint = {1010.3899},
  pages = {107--119},
  doi = {10.1111/j.1365-2966.2010.17889.x},
  urldate = {2020-07-02},
  abstract = {This study is concerned with the early evolution of magnetic fields and differential rotation of intermediate-mass stars which may evolve into Ap stars. We report on simulations of the interplay of differential rotation and magnetic fields, the stability limits and non-linear evolution of such configurations, and the prospects of dynamo action from the unstable cases. The axisymmetric problem delivers a balance between field amplification and back-reaction of the magnetic field on the differential rotation. The non-axisymmetric case involves also the Tayler instability of the amplified toroidal fields. We consider limits for field amplification and apply these to young A stars. Apart from its application to Ap stars, the instability is scrutinized for the fundamental possibility of a dynamo. We are not looking for a dynamo as an explanation for the Ap star phenomenon. The kinetic helicity is concentrated near the tangent cylinder of the inner sphere of the computational domain and is negative in the northern hemisphere. This appears to be a ubiquitous effect not special to the Tayler instability. The latter is actually connected with a positive current helicity in the bulk of the spherical shell giving rise to a small, but non-vanishing alpha-effect in non-linear evolution of the instability.},
  archiveprefix = {arxiv},
  keywords = {MHD - stars: chemically peculiar,notion,notion-database,Stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/ZYPAR5B8/full-text.pdf}
}

@article{Arlt2013,
  title = {Sunspot Positions and Sizes for 1825-1867 from the Observations by {{Samuel Heinrich Schwabe}}},
  author = {Arlt, R. and Leussu, R. and Giese, N. and Mursula, K. and Usoskin, I. G.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {433},
  number = {4},
  eprint = {1305.7400},
  pages = {3165--3172},
  issn = {00358711},
  doi = {10.1093/mnras/stt961},
  abstract = {Samuel Heinrich Schwabe made 8486 drawings of the solar disc with sunspots in the period from 1825 November 5 to 1867 December 29. We have measured sunspot sizes and heliographic positions on digitized images of these drawings. A total of about 135 000 measurements of individual sunspots are available in a data base. Positions are accurate to about 5 per cent of the solar radius or to about 3\textdegree{} in heliographic coordinates in the solar-disc centre. Sizes were given in 12 classes as estimated visually with circular cursor shapes on the screen. Most of the drawings show a coordinate grid aligned with the celestial coordinate system. A subset of 1168 drawings have no indication of their orientation. We have used a Bayesian estimator to infer the orientations of the drawings as well as the average heliographic spot positions from a chain of drawings of several days, using the rotation profile of the present Sun. The data base also includes all information available from Schwabe on spotless days. \textcopyright{} 2013 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sunspots},
  file = {/Users/lbugnet/Zotero/storage/WVDEN7TR/Arlt et al. - 2013.pdf}
}

@article{Arlt2014,
  title = {Solar Activity in the Past and the Chaotic Behaviour of the Dynamo},
  author = {Arlt, R. and Weiss, N.},
  year = {2014},
  month = jun,
  journal = {Space Science Reviews},
  volume = {186},
  number = {1-4},
  eprint = {1406.7628},
  pages = {525--533},
  publisher = {{Kluwer Academic Publishers}},
  doi = {10.1007/s11214-014-0063-5},
  urldate = {2020-07-13},
  abstract = {The record of solar activity is reviewed here with emphasis on peculiarities. Since sunspot positions tell us a lot more about the solar dynamo than the various global sunspot numbers, we first focus on the records of telescopic observations of sunspots leading to positional information. Then we turn to the proxy record from cosmogenic isotope abundances, which shows recurrent grand minima over the last 9500 years. The apparent distinction between episodes of strong modulation, and intervening episodes with milder modulation and weaker overall activity, hints at the solar dynamo following a variety of solutions, with different symmetries, over the course of millennia.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Solar activity,Solar dynamo}
}

@article{Armstrong2002,
  title = {K2 {{Variable Catalogue II}}: {{Machine Learning Classification}} of {{Variable Stars}} and {{Eclipsing Binaries}} in {{K2 Fields}} 0-4},
  author = {Armstrong, D J and Kirk, J and Lam, K W F and Mccormac, J and Osborn, H P and Spake, J and Walker, S and Brown, D J A and Kristiansen, M H and Pollacco, D and West, R and Wheatley, P J},
  year = {2002},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {000},
  eprint = {1512.01246v2},
  urldate = {2020-04-09},
  abstract = {We are entering an era of unprecedented quantities of data from current and planned survey telescopes. To maximise the potential of such surveys, automated data analysis techniques are required. Here we implement a new methodology for variable star classification, through the combination of Kohonen Self Organising Maps (SOM, an unsupervised machine learning algorithm) and the more common Random Forest (RF) supervised machine learning technique. We apply this method to data from the K2 mission fields 0-4, finding 154 ab-type RR Lyraes (10 newly discovered), 377 {$\delta$} Scuti pulsators, 133 {$\gamma$} Doradus pulsators, 183 detached eclipsing binaries, 290 semi-detached or contact eclipsing binaries and 9399 other periodic (mostly spot-modulated) sources, once class significance cuts are taken into account. We present lightcurve features for all K2 stellar targets, including their three strongest detected frequencies, which can be used to study stellar rotation periods where the observed variability arises from spot modulation. The resulting catalogue of variable stars, classes, and associated data features are made available online. We publish our SOM code in Python as part of the open source PyMVPA package, which in combination with already available RF modules can be easily used to recreate the method.},
  archiveprefix = {arxiv},
  keywords = {data analysis-binaries,eclipsing-techniques,general-catalogues-methods,notion,notion-database,photometric,stars,variable},
  file = {/Users/lbugnet/Zotero/storage/ZQQR2JWD/full-text.pdf}
}

@article{Armstrong2015,
  title = {Astrophysics {{K2 Variable Catalogue}}: {{Variable}} Stars and Eclipsing Binaries in {{K2}} Campaigns 1 and 0},
  author = {Armstrong, D J and Kirk, J and Lam, K W F and Mccormac, J and Walker, S R and Brown, D J A and Osborn, H P and Pollacco, D L and Spake, J},
  year = {2015},
  journal = {A\&A},
  volume = {579},
  pages = {19},
  doi = {10.1051/0004-6361/201525889},
  urldate = {2020-03-27},
  abstract = {Aims. We have created a catalogue of variable stars found from a search of the publicly available K2 mission data from Campaigns 1 and 0. This catalogue provides the identifiers of 8395 variable stars, including 199 candidate eclipsing binaries with periods up to 60 d and 3871 periodic or quasi-periodic objects, with periods up to 20 d for Campaign 1 and 15 d for Campaign 0. Methods. Lightcurves are extracted and detrended from the available data. These are searched using a combination of algorithmic and human classification, leading to a classifier for each object as an eclipsing binary, sinusoidal periodic, quasi periodic, or aperiodic variable. The source of the variability is not identified, but could arise in the non-eclipsing binary cases from pulsation or stellar activity. Each object is cross-matched against variable star related guest observer proposals to the K2 mission, which specifies the variable type in some cases. The detrended lightcurves are also compared to lightcurves currently publicly available. Results. The resulting catalogue gives the ID, type, period, semi-amplitude, and range of the variation seen. We also make available the detrended lightcurves for each object.},
  keywords = {eclipsing,general-binaries,general-catalogs-stars,notion,notion-database,stars,variables}
}

@article{Armstrong2016,
  title = {K2 Variable Catalogue-{{II}}. {{Machine}} Learning Classification of Variable Stars and Eclipsing Binaries in {{K2}} Fields 0-4},
  author = {Armstrong, D J and Kirk, J and Lam, K W F and Mccormac, J and Osborn, H P and Spake, J and Walker, S and Brown, D J A and Kristiansen, M H and Pollacco, D and West, R and Wheatley, P J},
  year = {2016},
  journal = {MNRAS},
  volume = {456},
  pages = {2260--2272},
  doi = {10.1093/mnras/stv2836},
  urldate = {2020-01-16},
  abstract = {We are entering an era of unprecedented quantities of data from current and planned survey telescopes. To maximize the potential of such surveys, automated data analysis techniques are required. Here we implement a new methodology for variable star classification, through the combination of Kohonen Self-Organizing Maps (SOMs, an unsupervised machine learning algorithm) and the more common Random Forest (RF) supervised machine learning technique. We apply this method to data from the K2 mission fields 0-4, finding 154 ab-type RR Lyraes (10 newly discovered), 377 {$\delta$} Scuti pulsators, 133 {$\gamma$} Doradus pulsators, 183 detached eclipsing binaries, 290 semidetached or contact eclipsing binaries and 9399 other periodic (mostly spot-modulated) sources, once class significance cuts are taken into account. We present light-curve features for all K2 stellar targets, including their three strongest detected frequencies, which can be used to study stellar rotation periods where the observed variability arises from spot modulation. The resulting catalogue of variable stars, classes, and associated data features are made available online. We publish our SOM code in PYTHON as part of the open source PYMVPA package, which in combination with already available RF modules can be easily used to recreate the method.},
  keywords = {data analysis-techniques,eclips-ing-stars,general,methods,notion,notion-database,photometric-catalogues-binaries,variables},
  file = {/Users/lbugnet/Zotero/storage/7K43J9MG/full-text.pdf}
}

@article{Ashton2018,
  title = {Hierarchical Multistage {{MCMC}} Follow-up of Continuous Gravitational Wave Candidates},
  author = {Ashton, G. and Prix, R.},
  year = {2018},
  journal = {Physical Review D},
  volume = {97},
  number = {10},
  eprint = {1802.05450},
  issn = {24700029},
  doi = {10.1103/PhysRevD.97.103020},
  abstract = {Leveraging Markov chain Monte Carlo optimization of the F statistic, we introduce a method for the hierarchical follow-up of continuous gravitational wave candidates identified by wide-parameter space semicoherent searches. We demonstrate parameter estimation for continuous wave sources and develop a framework and tools to understand and control the effective size of the parameter space, critical to the success of the method. Monte Carlo tests of simulated signals in noise demonstrate that this method is close to the theoretical optimal performance.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/7JCZB4JV/Ashton, Prix - 2018.pdf}
}

@article{Asplund2000,
  title = {Line Formation in Solar Granulation: {{II}}. {{The}} Photospheric {{Fe}} Abundance},
  author = {Asplund, M. and Nordlund, {\AA} and Trampedach, R. and Stein, R. F.},
  year = {2000},
  journal = {Astronomy and Astrophysics},
  volume = {359},
  number = {2},
  eprint = {astro-ph/0005321},
  pages = {743--754},
  issn = {00046361},
  abstract = {The solar photospheric Fe abundance has been determined using realistic ab initio 3D, time-dependent, hydrodynamical model atmospheres. The study is based on the excellent agreement between the predicted and observed line profiles directly rather than equivalent widths, since the intrinsic Doppler broadening from the convective motions and oscillations provide the necessary non-thermal broadening. Thus, three of the four hotly debated parameters (equivalent widths, microturbulence and damping enhancement factors) in the center of the recent solar Fe abundance dispute regarding Fe I lines no longer enter the analysis, leaving the transition probabilities as the main uncertainty. Both Fe I (using the samples of lines of both the Oxford and Kiel studies) and Fen lines have been investigated, which give consistent results: log {$\epsilon$}FeI = 7.44{$\pm$}0.05 and log {$\epsilon$}FeII = 7.45 {$\pm$} 0.10. Also the wings of strong Fe I lines return consistent abundances, log {$\epsilon$}FeII = 7.42 {$\pm$} 0.03, but due to the uncertainties inherent in analyses of strong lines we give this determination lower weight than the results from weak and intermediate strong lines. In view of the recent slight downward revision of the meteoritic Fe abundance log {$\epsilon$}Fe = 7.46 {$\pm$} 0.01, the agreement between the meteoritic and photospheric values is very good, thus appearingly settling the debate over the photospheric Fe abundance from Fe I lines.},
  archiveprefix = {arxiv},
  keywords = {Convection,Hydrodynamics,Line: formation,notion,notion-database,Sun: abundances,Sun: granulation,Sun: photosphere},
  file = {/Users/lbugnet/Zotero/storage/2K9FHECS/Asplund et al. - 2000.pdf}
}

@article{Asplund2009,
  title = {The {{Chemical Composition}} of the {{Sun}}},
  author = {Asplund, Martin and Grevesse, Nicolas and Sauval, A. Jacques and Scott, Pat},
  year = {2009},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {47},
  number = {1},
  eprint = {0909.0948},
  pages = {481--522},
  issn = {0066-4146},
  doi = {10.1146/annurev.astro.46.060407.145222},
  abstract = {The solar chemical composition is an important ingredient in our understanding of the formation, structure and evolution of both the Sun and our solar system. Furthermore, it is an essential reference standard against which the elemental contents of other astronomical objects are compared. In this review we evaluate the current understanding of the solar photospheric composition. In particular, we present a re-determination of the abundances of nearly all available elements, using a realistic new 3-dimensional (3D), time-dependent hydrodynamical model of the solar atmosphere. We have carefully considered the atomic input data and selection of spectral lines, and accounted for departures from LTE whenever possible. The end result is a comprehensive and homogeneous compilation of the solar elemental abundances. Particularly noteworthy findings are significantly lower abundances of carbon, nitrogen, oxygen and neon compared with the widely-used values of a decade ago. The new solar chemical composition is supported by a high degree of internal consistency between available abundance indicators, and by agreement with values obtained in the solar neighborhood and from the most pristine meteorites. There is, however, a stark conflict with standard models of the solar interior according to helioseismology, a discrepancy that has yet to find a satisfactory resolution.},
  archiveprefix = {arxiv},
  keywords = {abstract the solar chemical,both the sun and,composition is an important,convection,ingredient in our under-,meteoritic abundances,notion,notion-database,our solar system,solar abundances,solar atmosphere,spectral line formation,standing of the formation,structure and evolution of,sun},
  file = {/Users/lbugnet/Zotero/storage/SVEH52GA/Asplund et al. - 2009.pdf}
}

@article{Astoul2019,
  title = {Does Magnetic Field Impact Tidal Dynamics inside the Convective Zone of Low-Mass Stars along Their Evolution?},
  author = {Astoul, A. and Mathis, S. and Baruteau, C. and Gallet, F. and Strugarek, A. and Augustson, K. C. and Brun, A. S. and Bolmont, E.},
  year = {2019},
  journal = {Astronomy and Astrophysics},
  volume = {631},
  eprint = {1909.10490},
  pages = {A111},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201936477},
  abstract = {Context. The dissipation of the kinetic energy of wave-like tidal flows within the convective envelope of low-mass stars is one of the key physical mechanisms that shapes the orbital and rotational dynamics of short-period exoplanetary systems. Although low-mass stars are magnetically active objects, the question of how the star's magnetic field impacts large-scale tidal flows and the excitation, propagation and dissipation of tidal waves still remains open. Aims. Our goal is to investigate the impact of stellar magnetism on the forcing of tidal waves, and their propagation and dissipation in the convective envelope of low-mass stars as they evolve. Methods. We have estimated the amplitude of the magnetic contribution to the forcing and dissipation of tidally induced magneto-inertial waves throughout the structural and rotational evolution of low-mass stars (from M to F-type). For this purpose, we have used detailed grids of rotating stellar models computed with the stellar evolution code STAREVOL. The amplitude of dynamo-generated magnetic fields is estimated via physical scaling laws at the base and the top of the convective envelope. Results. We find that the large-scale magnetic field of the star has little influence on the excitation of tidal waves in the case of nearly-circular orbits and coplanar hot-Jupiter planetary systems, but that it has a major impact on the way waves are dissipated. Our results therefore indicate that a full magneto-hydrodynamical treatment of the propagation and dissipation of tidal waves is needed to properly assess the impact of star-planet tidal interactions throughout the evolutionary history of low-mass stars hosting short-period massive planets.},
  archiveprefix = {arxiv},
  keywords = {evolution,magnetic field,magnetohydrodynamics,magnetohydrodynamics (MHD),mhd,notion,notion-database,planet-star int,planet-star interactions,stars,waves},
  file = {/Users/lbugnet/Zotero/storage/3MCJMPZW/Astoul et al. - 2019.pdf}
}

@article{Audenaert2021,
  title = {{{TESS Data}} for {{Asteroseismology}} ({{T}}'{{DA}}) {{Stellar Variability Classification Pipeline}}: {{Setup}} and {{Application}} to the {{Kepler Q9 Data}}},
  author = {Audenaert, J. and Kuszlewicz, J. S. and Handberg, R. and Tkachenko, A. and Armstrong, D. J. and Hon, M. and Kgoadi, R. and Lund, M. N. and Bell, K. J. and Bugnet, L. and Bowman, D. M. and Johnston, C. and Garc{\'i}a, R. A. and Stello, D. and Moln{\'a}r, L. and Plachy, E. and Buzasi, D. and Aerts, C. and Collaboration, The T'DA},
  year = {2021},
  month = oct,
  journal = {The Astronomical Journal},
  volume = {162},
  number = {5},
  pages = {209},
  publisher = {{IOP Publishing}},
  issn = {1538-3881},
  doi = {10.3847/1538-3881/AC166A},
  urldate = {2021-10-24},
  keywords = {notion,notion-database}
}

@article{Augustson2012,
  title = {Convection and {{Differential Rotation}} in {{F-type Stars}}},
  author = {Augustson, Kyle C. and Brown, Benjamin P. and Brun, Allan Sacha and Miesch, Mark S. and Toomre, Juri},
  year = {2012},
  journal = {The Astrophysical Journal},
  volume = {756},
  number = {2},
  pages = {169},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/756/2/169},
  urldate = {2020-06-19},
  keywords = {convection,hydrodynamics,notion,notion-database,stars: interiors,stars: rotation,stars: solar,type},
  file = {/Users/lbugnet/Zotero/storage/5K9Y37U4/full-text.pdf}
}

@article{Augustson2015,
  title = {{{GRAND MINIMA}} and {{EQUATORWARD PROPAGATION}} in {{A CYCLING STELLAR CONVECTIVE DYNAMO}}},
  author = {Augustson, Kyle and Brun, Allan Sacha and Miesch, Mark and Toomre, Juri},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {809},
  number = {2},
  eprint = {1410.6547},
  issn = {15384357},
  doi = {10.1088/0004-637X/809/2/149},
  abstract = {The 3D MHD Anelastic Spherical Harmonic code, using slope-limited diffusion, is employed to capture convective and dynamo processes achieved in a global-scale stellar convection simulation for a model solar-mass star rotating at three times the solar rate. The dynamo-generated magnetic fields possesses many timescales, with a prominent polarity cycle occurring roughly every 6.2 years. The magnetic field forms large-scale toroidal wreaths, whose formation is tied to the low Rossby number of the convection in this simulation. The polarity reversals are linked to the weakened differential rotation and a resistive collapse of the large-scale magnetic field. An equatorial migration of the magnetic field is seen, which is due to the strong modulation of the differential rotation rather than a dynamo wave. A poleward migration of magnetic flux from the equator eventually leads to the reversal of the polarity of the high-latitude magnetic field. This simulation also enters an interval with reduced magnetic energy at low latitudes lasting roughly 16 years (about 2.5 polarity cycles), during which the polarity cycles are disrupted and after which the dynamo recovers its regular polarity cycles. An analysis of this grand minimum reveals that it likely arises through the interplay of symmetric and antisymmetric dynamo families. This intermittent dynamo state potentially results from the simulation's relatively low magnetic Prandtl number. A mean-field-based analysis of this dynamo simulation demonstrates that it is of the {$\alpha$}-{$\Omega$} type. The timescales that appear to be relevant to the magnetic polarity reversal are also identified.},
  archiveprefix = {arxiv},
  keywords = {convection,magnetohydrodynamics (MHD),notion,notion-database,stars: magnetic field,stars: rotation,turbulence},
  file = {/Users/lbugnet/Zotero/storage/F9IMZ4XY/Augustson et al. - 2015.pdf}
}

@article{Augustson2016,
  title = {The {{Magnetic Furnace}}: {{Intense Core Dynamos}} in {{B-stars}}},
  author = {Augustson, Kyle C. and Brun, Allan Sacha and Toomre, Juri},
  year = {2016},
  month = mar,
  journal = {ApJ},
  volume = {829},
  number = {2},
  eprint = {1603.03659},
  pages = {92},
  doi = {10.3847/0004-637X/829/2/92},
  urldate = {2020-06-19},
  abstract = {The dynamo action achieved in the convective cores of main-sequence massive stars is explored here through 3D global simulations of convective core dynamos operating within a young \$\textbackslash Msun\{10\}\$ B-type star, using the anelastic spherical harmonic (ASH) code. These simulations capture the inner 65\textbackslash\% of this star by radius, encompassing the convective nuclear-burning core (about 23\textbackslash\% by radius) and a portion of the overlying radiative envelope. Eight rotation rates are considered, ranging from 0.05\textbackslash\% to 16\textbackslash\% of the surface breakup velocity, thereby capturing both convection that barely senses the effects of rotation and other situations in which the Coriolis forces are prominent. The vigorous dynamo action realized within all of these turbulent convective cores builds magnetic fields with peak strengths exceeding a megagauss, with the overall magnetic energy (ME) in the faster rotators reaching super-equipartition levels compared to the convective kinetic energy (KE). The core convection typically involves turbulent columnar velocity structures roughly aligned with the rotation axis, with magnetic fields threading through these rolls and possessing complex linkages throughout the core. The very strong fields are able to coexist with the flows without quenching them through Lorentz forces. The velocity and magnetic fields achieve such a state by being nearly co-aligned, and with peak magnetic islands being somewhat displaced from the fastest flows as the intricate evolution proceeds. As the rotation rate is increased, the primary force balance shifts from nonlinear advection balancing Lorentz forces to a magnetostrophic balance between Coriolis and Lorentz forces.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,convection,dynamo,magnetohydrodynamics: MHD,notion,notion-database,Solar and Stellar Astrophysics,stars: massive},
  file = {/Users/lbugnet/Zotero/storage/BILZ4F8W/full-text.pdf}
}

@inproceedings{Augustson2018,
  title = {Perturbations of {{Stellar Oscillations}}: A {{General Magnetic Field}}},
  booktitle = {{{SF2A-2018}}: {{Proceedings}} of the {{Annual Meeting}} of the {{French Society}} of {{Astronomy}} and {{Astrophysics}}},
  author = {Augustson, Kyle and Mathis, St{\'e}phane},
  year = {2018},
  month = nov,
  eprint = {1811.04416},
  urldate = {2020-07-29},
  abstract = {The purpose of this short paper is to give a summary of the derivation of a perturbative method to assess the impact of an arbitrary 3D magnetic field configuration, whose energy is everywhere small relative to the gravitational binding energy, on the form and value of the eigenfrequencies and eigenfunctions of stellar oscillations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TZSNIY8B/full-text.pdf}
}

@article{Augustson2019,
  title = {Rossby and {{Magnetic Prandtl Number Scaling}} of {{Stellar Dynamos}} - {{NASA}}/{{ADS}}},
  author = {Augustson, K. C.; and Brun, A. S.; and Toomre, J.},
  year = {2019},
  journal = {The Astrophysical Journal},
  volume = {876},
  number = {1},
  urldate = {2020-06-19},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/F9M5CAB5/Augustson, Brun, Toomre - 2019.pdf}
}

@article{Augustson2020,
  title = {A {{Model}} of {{Rotating Convection}} in {{Stellar}} and {{Planetary Interiors}}. {{II}}. {{Gravito-inertial Wave Generation}}},
  author = {Augustson, K. C. and Mathis, S. and Astoul, A.},
  year = {2020},
  month = nov,
  journal = {The Astrophysical Journal},
  volume = {903},
  number = {2},
  eprint = {2009.10473},
  pages = {90},
  publisher = {{American Astronomical Society}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/abba1c},
  urldate = {2021-01-02},
  abstract = {Gravito-inertial waves are excited at the interface of convective and radiative regions and by the Reynolds stresses in the bulk of the convection zones of rotating stars and planets. Such waves have notable asteroseismic signatures in the frequency spectra of rotating stars, particularly among rapidly rotating early-type stars, which provides a means of probing their internal structure and dynamics. They can also transport angular momentum, chemical species, and energy from the excitation region to where they dissipate in radiative regions. To estimate the excitation and convective parameter dependence of the amplitude of those waves, a monomodal model for stellar and planetary convection as described in Paper I is employed, which provides the magnitude of the rms convective velocity as a function of rotation rate. With this convection model, two channels for wave driving are considered: excitation at a boundary between convectively stable and unstable regions and excitation due to Reynolds-stresses. Parameter regimes are found where the sub-inertial waves may carry a significant energy flux, depending upon the convective Rossby number, the interface stiffness, and the wave frequency. The super-inertial waves can also be enhanced, but only for convective Rossby numbers near unity. Interfacially excited waves have a peak energy flux near the lower cutoff frequency when the convective Rossby number of the flows that excite them are below a critical Rossby number that depends upon the stiffness of the interface, whereas that flux decreases when the convective Rossby number is larger than this critical Rossby number.},
  archiveprefix = {arxiv},
  keywords = {1596,1617,1621,1629,301,Astrophysics,Earth and Planetary Astrophysics,Fluid Dynamics,notion,notion-database,Physics,Solar and Stellar Astrophysics,Stellar convective zones,Stellar dynamics,Stellar oscillations,Stellar physics,Stellar rotation}
}

@article{Auriere2007,
  title = {Weak Magnetic Fields in {{Ap}}/{{Bp}} Stars: {{Evidence}} for a Dipole Field Lower Limit and a Tentative Interpretation of the Magnetic Dichotomy},
  author = {Auriere, M. and Wade, G. A. and Silvester, J. and Lignieres, F. and Bagnulo, S. and Bale, K. and Dintrans, B. and Donati, J. F. and Folsom, C. P. and Gruberbauer, M. and Hoa, A. Hui Bon and Jeffers, S. and Johnson, N. and Landstreet, J. D. and Lebre, A. and Lueftinger, T. and Marsden, S. and Mouillet, D. and Naseri, S. and Paletou, F. and Petit, P. and Power, J. and Rincon, F. and Strasser, S. and Toque, N.},
  year = {2007},
  month = oct,
  journal = {Astronomy and Astrophysics},
  volume = {475},
  number = {3},
  eprint = {0710.1554},
  pages = {1053--1065},
  doi = {10.1051/0004-6361:20078189},
  urldate = {2020-07-03},
  abstract = {We have investigated a sample of 28 well-known spectroscopically-identified magnetic Ap/Bp stars, with weak, poorly-determined or previously undetected magnetic fields, with the aim of exploring the weak part of the magnetic field distribution of Ap/Bp stars. Using the MuSiCoS and NARVAL spectropolarimeters we have obtained 282 LSD Stokes V signatures of our 28 sample stars. All stars were detected, showing clearly that when observed with sufficient precision, all firmly classified Ap/Bp stars show detectable surface magnetic fields. To better characterise the surface magnetic field intensities and geometries of the sample, we have inferred the dipolar field intensity and the magnetic obliquity. The distribution of derived dipole strengths for these stars exhibits a plateau at about 1 kG, falling off to larger and smaller field strengths. Remarkably, in this sample of stars selected for their presumably weak magnetic fields, we find only 2 stars for which the derived dipole strength is weaker than 300 G. We interpret this "magnetic threshold" as a critical value necessary for the stability of large-scale magnetic fields, and develop a simple quantitative model that is able to approximately reproduce the observed threshold characteristics. This scenario leads to a natural explanation of the small fraction of intermediate-mass magnetic stars. It may also explain the near-absence of magnetic fields in more massive B and O-type stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: chemically peculiar,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/WTEVLSJA/full-text.pdf}
}

@article{Auriere2009,
  title = {Discovery of a Weak Magnetic Field in the Photosphere of the Single Giant {{Pollux}}},
  author = {Auri{\`e}re, M. and Wade, G. A. and {Konstantinova-Antova}, R. and Charbonnel, C. and Catala, C. and Weiss, W. W. and Roudier, T. and Petit, P. and Donati, J. -F. and Alecian, E. and Cabanac, R. and Van Eck, S. and Folsom, C. P. and Power, J.},
  year = {2009},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {504},
  number = {1},
  eprint = {0907.1423},
  pages = {231--237},
  doi = {10.1051/0004-6361/200912050},
  urldate = {2020-05-15},
  abstract = {Aims: We observe the nearby, weakly-active single giant, Pollux, in order to directly study and infer the nature of its magnetic field. Methods: We used the new generation spectropolarimeters ESPaDOnS and NARVAL to observe and detect circular polarization within the photospheric absorption lines of Pollux. Our observations span 18 months from 2007-2009. We treated the spectropolarimetric data using the Least-Squares Deconvolution method to create high signal-to-noise ratio mean Stokes V profiles. We also measured the classical activity indicator S-index for the Ca H\&K lines, and the stellar radial velocity (RV). Results: We have unambiguously detected a weak Stokes V signal in the spectral lines of Pollux, and measured the related surface-averaged longitudinal magnetic field Bl. The longitudinal field averaged over the span of the observations is below one gauss. Our data suggest variations of the longitudinal magnetic field, but no significant variation of the S-index. We observe variations of RV which are qualitatively consistent with the published ephemeris for a proposed exoplanet orbiting Pollux. The observed variations of Bl appear to mimic those of RV, but additional data for this relationship to be established. Using evolutionary models including the effects of rotation, we derive the mass of Pollux and we discuss its evolutionary status and the origin of its magnetic field. Conclusions: This work presents the first direct detection of the magnetic field of Pollux, and demonstrates that ESPaDOnS and NARVAL are capable of obtaining sub-G measurements of the surface-averaged longitudinal magnetic field of giant stars, and of directly studying the relationships between magnetic activity, stellar evolution and planet hosting of these stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YHTGKTYU/full-text.pdf}
}

@book{Auriere2014,
  title = {Descendants of Magnetic and Non-Magnetic {{A-type}} Stars},
  author = {Auri{\`e}re, M. and Ligni{\`e}res, F. and {Konstantinova-Antova}, R. and Charbonnel, C. and Petit, P. and Tsvetkova, S. and Wade, G.},
  year = {2014},
  month = nov,
  pages = {444--450},
  address = {{eprint: arXiv:1310.6942}},
  doi = {10.48550/arXiv.1310.6942},
  urldate = {2023-10-06},
  abstract = {We have studied the magnetic fields of about 50 active or non-active single G-K-type red giants by means of spectropolarimetry with Narval and ESPaDOnS. Thirty giants show significant Zeeman signals. A close examination of the 17 giants with known rotational periods shows that the measured magnetic field strength is correlated with the rotation, and in particular with the Rossby number. Four giants for which the magnetic field has been found to be outstandingly strong with respect to the rotational period or the evolutionary state are identified as probable Ap star descendants. We give details of their magnetic properties, and propose criteria to identify Ap star descendants.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2014psce.conf..444A}
}

@article{Auriere2015,
  title = {The Magnetic Fields at the Surface of Active Single {{G-K}} Giants},
  author = {Auri{\`e}re, M. and {Konstantinova-Antova}, R. and Charbonnel, C. and Wade, G. A. and Tsvetkova, S. and Petit, P. and Dintrans, B. and Drake, N. A. and Decressin, T. and Lagarde, N. and Donati, J. F. and Roudier, T. and Ligni{\`e}res, F. and Schr{\"o}der, K. P. and Landstreet, J. D. and L{\`e}bre, A. and Weiss, W. W. and Zahn, J. P.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {574},
  pages = {1--30},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424579},
  abstract = {Aims. We investigate the magnetic field at the surface of 48 red giants selected as promising for detection of Stokes V Zeeman signatures in their spectral lines. In our sample, 24 stars are identified from the literature as presenting moderate to strong signs of magnetic activity. An additional 7 stars are identified as those in which thermohaline mixing appears not to have occured, which could be due to hosting a strong magnetic field. Finally, we observed 17 additional very bright stars which enable a sensitive search to be performed with the spectropolarimetric technique. Methods. We use the spectropolarimeters Narval and ESPaDOnS to detect circular polarization within the photospheric absorption lines of our targets. We treat the spectropolarimetric data using the least-squares deconvolution method to create high signal-to-noise ratio mean Stokes V profiles. We also measure the classical S-index activity indicator for the Ca ii H\&K lines, and the stellar radial velocity. To infer the evolutionary status of our giants and to interpret our results, we use state-of-the-art stellar evolutionary models with predictions of convective turnover times. Results. We unambiguously detect magnetic fields via Zeeman signatures in 29 of the 48 red giants in our sample. Zeeman signatures are found in all but one of the 24 red giants exhibiting signs of activity, as well as 6 out of 17 bright giant stars. However no detections were obtained in the 7 thermohaline deviant giants. The majority of the magnetically detected giants are either in the first dredge up phase or at the beginning of core He burning, i.e. phases when the convective turnover time is at a maximum: this corresponds to a "magnetic strip" for red giants in the Hertzsprung-Russell diagram. A close study of the 16 giants with known rotational periods shows that the measured magnetic field strength is tightly correlated with the rotational properties, namely to the rotational period and to the Rossby number Ro. Our results show that the magnetic fields of these giants are produced by a dynamo, possibly of {$\alpha$}-{$\omega$} origin since Ro is in general smaller than unity. Four stars for which the magnetic field is measured to be outstandingly strong with respect to that expected from the rotational period/magnetic field relation or their evolutionary status are interpreted as being probable descendants of magnetic Ap stars. In addition to the weak-field giant Pollux, 4 bright giants (Aldebaran, Alphard, Arcturus, {$\eta$} Psc) are detected with magnetic field strength at the sub-Gauss level. Besides Arcturus, these stars were not considered to be active giants before this study and are very similar in other respects to ordinary giants, with S-index indicating consistency with basal chromospheric flux.},
  keywords = {notion,notion-database,Stars: evolution,Stars: late-type,Stars: magnetic field,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/BV55SEVJ/Aurière et al. - 2015.pdf;/Users/lbugnet/Zotero/storage/HYLPTJCB/Aurière et al. - 2014.pdf}
}

@article{Austin2019a,
  title = {References and {{Notes}}},
  author = {Austin, James H.},
  year = {2019},
  journal = {Meditating Selflessly},
  number = {December},
  pages = {1217--1220},
  doi = {10.7551/mitpress/8876.003.0036},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YEA4JLWS/Austin - 2019.pdf}
}

@misc{AustralianSurvivorS09E04,
  title = {Australian {{Survivor S09E04}} - Video {{Dailymotion}}},
  urldate = {2023-06-05},
  howpublished = {https://www.dailymotion.com/video/x87p1hz}
}

@article{Auvergne2009,
  title = {Special Feature {{The CoRoT}} Satellite in Flight : Description and Performance},
  author = {Auvergne, M and Bodin, P and Boisnard, L and Buey, J and Chaintreuil, S and Epstein, G and Jouret, M},
  year = {2009},
  volume = {424},
  pages = {411--424},
  keywords = {instrumentation,{instrumentation: photometers, stars: planetary sys},notion,notion-database,oscillations,photometers,planetary systems,stars},
  file = {/Users/lbugnet/Zotero/storage/KIAYJ5Z5/Auvergne et al. - 2009.pdf}
}

@article{Ayres2015,
  title = {The Far-Ultraviolet Ups and Downs of {{Alpha Centauri}}},
  author = {Ayres, Thomas R.},
  year = {2015},
  journal = {Astronomical Journal},
  volume = {149},
  number = {2},
  eprint = {1411.0038},
  issn = {00046256},
  doi = {10.1088/0004-6256/149/2/58},
  abstract = {Four years (2010-2014) of semiannual pointings by the Hubble Space Telescope Imaging Spectrograph (STIS) on nearby Alpha Centauri have yielded a detailed time history of far-ultraviolet (FUV: 1150-1700 \AA ) emissions of the solarlike primary (A: G2 V) and the cooler but more active secondary ( B: K1 V). This period saw A climbing out of a prolonged coronal X-ray minimum, as documented contemporaneously by Chandra, while B was rising to, then falling from, a peak of its long-term ({$\sim$}8 year) starspot cycle. The FUV fluxes of the primary were steady over most of the STIS period, although the [Fe XII] {$\lambda$}1242 coronal forbidden line (T {$\sim$} 1.5 MK) partly mirrored the slowly rising X-ray fluxes. The FUV emissions of the secondary more closely tracked the rise and fall of its coronal luminosities, especially the "hot lines" Si IV, C IV, and N V (T {$\sim$} 0.8 -2 \texttimes{} 105 K ), and coronal [Fe XII] itself. The hot lines of both stars were systematically redshifted, relative to narrow chromospheric emissions, by several km s-1, showing little change in amplitude over the four-year period, especially for {$\alpha$} Cen B, despite the significant evolution of its coronal activity. Further, the hot lines of both stars, individually and epoch-averaged, displayed non-Gaussian shapes, which most trivially could be decomposed into two components, one narrow (FWHM {$\sim$}25-45 km s-1), the other broad (60-80 km s-1). A bimodal Gaussian strategy had been applied previously to the {$\alpha$} Cen stars, but this was the first opportunity to evaluate any time dependence. In fact, not much variation of the component properties was seen, even over the major cycle changes of B. Curiously, the line fluxes were about equally divided between the narrow and broad components for both stars. The fact that there is minimal activity dependence of the narrow/broad flux partition, as well as densities derived from O IV] line ratios, either during the cycle evolution of B or between A and B, suggests that there is a dominant "quantum" of FUV surface activity that is relatively unchanged during the cycle, aside from the fractional area covered.},
  archiveprefix = {arxiv},
  keywords = {Binaries: visual,notion,notion-database,{Stars: individual (HD 128620, HD 128621, G191B2B,},Ultraviolet: stars},
  file = {/Users/lbugnet/Zotero/storage/FLSEQJCC/Ayres - 2015.pdf}
}

@article{Babcock1961,
  title = {The {{Topology}} of the {{Sun}}'s {{Magnetic Field}} and the 22-{{YEAR Cycle}}.},
  author = {Babcock, H. W.},
  year = {1961},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {133},
  pages = {572},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/147060},
  urldate = {2020-05-14},
  abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein-protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-{$\alpha$}-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD {$\leq$} 2.0 \AA{} for the interface backbone atoms) increased from 21\% with default Glide SP settings to 58\% with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63\% success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40\% of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
  keywords = {notion,notion-database}
}

@inproceedings{Baglin2006,
  title = {The Seismology Program of the {{CoRoT}} Mi},
  booktitle = {Proceedings of {{SOHO}} 18/{{GONG}} 2006/{{HELAS I}}, {{Beyond}} the Spherical {{Sun}} ({{ESA SP-624}}).},
  author = {Baglin, Annie and Michel, Eric and Auvergne, Michel and Team, CoRoT},
  year = {2006},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MD9NAEW6/full-text.pdf}
}

@book{Bagnulo2015,
  title = {Stellar Magnetic Fields},
  author = {Bagnulo, Stefano and Landstreet, John D.},
  year = {2015},
  journal = {Polarimetry of Stars and Planetary Systems},
  number = {March 2018},
  issn = {0365-0138},
  doi = {10.1017/CBO9781107358249.014},
  abstract = {Magnetic fields are detected by polarimetry in a large variety of stars across the entire Hertzsprung-Russell (HR) diagram. They deeply influence many evolutionary stages, from the collapse of the protostellar material, to the end of the star's life as a white dwarf or neutron star. Stellar magnetic fields are detected and studied through the analysis of the Zeeman effect (Zeeman 1897) on the Stokes profiles of photospheric spectral lines. The actual detection of stellar magnetic fields is rather difficult, and although the clear signature of the Zeeman effect was found in the spectra of sunspots more than a century ago (Hale 1908), almost 40 years passed before a field was found in any other star (the chemically peculiar A-type star 78 Vir; Babcock 1947), 60 years before the first neutron star (Hewish et al. 1968) and white dwarf (Kemp et al. 1970) fields were discovered, and 70 years before another field in a Sun-like star was detected (Robinson et al. 1980). During the last decade, stellar magnetism has attracted the interest of a varied scientific community with different specific backgrounds. While 15 years ago stellar magnetism was considered mainly in the context of studies of chemically peculiar stars and white dwarfs, today we actively discuss the role of magnetic fields in, for example, solar-type, cool, and ultra-cool stars; accretion disks; phenomena of stellar winds and mass loss; massive stars; the atmospheres of the extrasolar planets; and even in the context of astrobiology. Our knowledge of stellar magnetic fields has rapidly evolved thanks to the introduction, starting from the late 1990s, of modern and accurate spectro-polarimeters, and to the development of sophisticated methods for field detection and modeling capable of extracting crucial information even from very noisy signals. These latest developments have been reviewed in recent articles, for example, by Donati and Landstreet (2009) and Reiners (2012).},
  isbn = {978-1-107-35824-9},
  keywords = {notion,notion-database}
}

@article{Bagnulo2021,
  title = {New Insight into the Magnetism of Degenerate Stars from the Analysis of a Volume-Limited Sample of White Dwarfs},
  author = {Bagnulo, S. and Landstreet, J. D.},
  year = {2021},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {507},
  pages = {5902--5951},
  issn = {0035-8711},
  doi = {10.1093/mnras/stab2046},
  urldate = {2023-10-05},
  abstract = {Many stars evolve into magnetic white dwarfs (MWDs), and observations may help to understand when the magnetic field appears at the stellar surface, if and how it evolves during the cooling phase, and, above all, what are the mechanisms that generate it. After obtaining new spectropolarimetric observations and combining them with previous literature data, we have checked almost the entire population of about 152 WDs within 20 pc from the Sun for the presence of magnetic fields, with a sensitivity that ranges from better than 1 kG for most of the stars of spectral class DA, to 1 MG for some of the featureless white dwarfs (WDs). We find that 33 WDs of the local 20 pc volume are magnetic. Statistically, the data are consistent with the possibility that the frequency of the magnetic field occurrence is similar in stars of all spectral classes, except that in the local 20 pc volume, either DQ stars are more frequently magnetic or host much stronger fields than average. The distribution of the observed field strength ranges from 40 kG to 300 MG and is uniform per decade, in striking contrast to the field frequency distribution resulting from spectroscopic surveys. Remarkably, no fields weaker than 40 kG are found. We confirm that magnetic fields are more frequent in WDs with higher than average mass, especially in younger stars. We find a marked deficiency of MWDs younger than 0.5 Gyr, and we find that the frequency of the occurrence of the magnetic field is significantly higher in WDs that have undergone the process of core crystallization than in WDs with fully liquid core. There is no obvious evidence of field strength decay with time. We discuss the implications of our findings in relation to some of the proposals that have been put forward to explain the origin and evolution of magnetic fields in degenerate stars, in particular those that predict the presence of a dynamo acting during the crystallization phase.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,polarization,stars: magnetic field,white dwarfs},
  annotation = {ADS Bibcode: 2021MNRAS.507.5902B},
  file = {/Users/lbugnet/Zotero/storage/HBEK5AD3/Bagnulo and Landstreet - 2021 - New insight into the magnetism of degenerate stars.pdf}
}

@article{Bagnulo2022,
  title = {Multiple {{Channels}} for the {{Onset}} of {{Magnetism}} in {{Isolated White Dwarfs}}},
  author = {Bagnulo, Stefano and Landstreet, John D.},
  year = {2022},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {935},
  pages = {L12},
  issn = {0004-637X},
  doi = {10.3847/2041-8213/ac84d3},
  urldate = {2023-10-05},
  abstract = {The presence of a strong magnetic field is a feature common to a significant fraction of degenerate stars, yet little is understood about the field's origin and evolution. New observational constraints from volume-limited surveys point to a more complex situation than a single mechanism valid for all stars. We show that in high-mass white dwarfs, which are probably the results of mergers, magnetic fields are extremely common and very strong and appear immediately in the cooling phase. These fields may have been generated by a dynamo active during the merging. Lower-mass white dwarfs, which are often the product of single-star evolution, are rarely detectably magnetic at birth, but fields appear very slowly, and very weakly, in about a quarter of them. What we may see is an internal field produced in an earlier evolutionary stage that gradually relaxes to the surface from the interior. The frequency and strength of magnetic fields continue to increase to eventually rival those of highly massive stars, particularly after the stars cool past the start of core crystallization, an effect that could be responsible for a dynamo mechanism similar to the one that is active in Earth's interior.},
  keywords = {1799,1973,995,Astrophysics - Solar and Stellar Astrophysics,Magnetic stars,Spectropolarimetry,White dwarf stars},
  annotation = {ADS Bibcode: 2022ApJ...935L..12B},
  file = {/Users/lbugnet/Zotero/storage/CLF37X7U/Bagnulo and Landstreet - 2022 - Multiple Channels for the Onset of Magnetism in Is.pdf}
}

@article{Bagnulo2022a,
  title = {Multiple {{Channels}} for the {{Onset}} of {{Magnetism}} in {{Isolated White Dwarfs}}},
  author = {Bagnulo, Stefano and Landstreet, John D.},
  year = {2022},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {935},
  pages = {L12},
  issn = {0004-637X},
  doi = {10.3847/2041-8213/ac84d3},
  urldate = {2023-10-12},
  abstract = {The presence of a strong magnetic field is a feature common to a significant fraction of degenerate stars, yet little is understood about the field's origin and evolution. New observational constraints from volume-limited surveys point to a more complex situation than a single mechanism valid for all stars. We show that in high-mass white dwarfs, which are probably the results of mergers, magnetic fields are extremely common and very strong and appear immediately in the cooling phase. These fields may have been generated by a dynamo active during the merging. Lower-mass white dwarfs, which are often the product of single-star evolution, are rarely detectably magnetic at birth, but fields appear very slowly, and very weakly, in about a quarter of them. What we may see is an internal field produced in an earlier evolutionary stage that gradually relaxes to the surface from the interior. The frequency and strength of magnetic fields continue to increase to eventually rival those of highly massive stars, particularly after the stars cool past the start of core crystallization, an effect that could be responsible for a dynamo mechanism similar to the one that is active in Earth's interior.},
  keywords = {1799,1973,995,Astrophysics - Solar and Stellar Astrophysics,Magnetic stars,Spectropolarimetry,White dwarf stars},
  annotation = {ADS Bibcode: 2022ApJ...935L..12B},
  file = {/Users/lbugnet/Zotero/storage/QNYAN8NE/Bagnulo and Landstreet - 2022 - Multiple Channels for the Onset of Magnetism in Is.pdf}
}

@article{Bagnulo2022b,
  title = {The {{Isolated Magnetic White Dwarfs}}},
  author = {Bagnulo, S. and Landstreet, J. D.},
  year = {2022},
  month = mar,
  journal = {The Messenger},
  volume = {186},
  pages = {14--18},
  issn = {0722-6691},
  doi = {10.18727/0722-6691/5257},
  urldate = {2023-10-12},
  abstract = {About one star in four will end its life as a magnetic white dwarf. Although magnetism is a very common feature in degenerate stars, we still do not know much about its origin and evolution. Our volume-limited spectropolarimetric survey of white dwarfs reveals statistical characteristics that may help to understand it.},
  annotation = {ADS Bibcode: 2022Msngr.186...14B},
  file = {/Users/lbugnet/Zotero/storage/YT4XDBDT/Bagnulo and Landstreet - 2022 - The Isolated Magnetic White Dwarfs.pdf}
}

@article{Bahcall1995,
  title = {Progress and Prospects in Neutrino Astrophysics},
  author = {Bahcall, John N. and Lande, Kenneth and Lanou, Robert E. and Learned, John G. and Robertson, R. G.Hamish and Wolfenstein, Lincoln},
  year = {1995},
  journal = {Nature},
  volume = {375},
  number = {6526},
  pages = {29--34},
  issn = {00280836},
  doi = {10.1038/375029a0},
  abstract = {Four separate experiments to detect neutrinos from the Sun have now confirmed a deficit in the flux relative to the predictions of standard theories of nuclear physics. Future experiments with new neutrino detectors promise to reveal the explanation for this shortfall. The planned detectors may also engender a new field of astronomy, based on the observation of neutrino emission from distant, energetic astrophysical sources. \textcopyright{} 1995 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/N7UGQ9ZJ/Bahcall et al. - 1995.pdf}
}

@article{Bahcall1995a,
  title = {Solar Models with Helium and Heavy-Element Diffusion},
  author = {Bahcall, John N. and Pinsonneault, M. H. and Wasserburg, G. J.},
  year = {1995},
  journal = {Reviews of Modern Physics},
  volume = {67},
  number = {4},
  pages = {781--808},
  issn = {00346861},
  doi = {10.1103/RevModPhys.67.781},
  abstract = {Helium and heavy-element diffusion are both included in precise calculations of solar models. In addition, improvements in the input data for solar interior models are described for nuclear reaction rates, the solar luminosity, the solar age, heavy-element abundances, radiative opacities, helium and metal diffusion rates, and neutrino interaction cross sections. The effects on the neutrino fluxes of each change in the input physics are evaluated separately by constructing a series of solar models with one additional improvement added at each stage. The effective 1 {$\sigma$} uncertainties in the individual input quantities are estimated and used to evaluate the uncertainties in the calculated neutrino fluxes and the calculated event rates for solar neutrino experiments. The calculated neutrino event rates, including all of the improvements, are 9.3-1.4+1.2 SNU for the Cl37 experiment and 137-7+8 SNU for the Ga71 experiments. The calculated flux of Be7 neutrinos is 5.1 (1.00-0.07+0.06)\texttimes 109 cm-2 s-1 and the flux of B8 neutrinos is 6.6(1.00-0.17+0.14)\texttimes 106 cm-2 s-1. The primordial helium abundance found for this model is Y=0.278. The present-day surface abundance of the model is Ys=0.247, in agreement with the helioseismological measurement of Ys=0.242{$\pm$}0.003 determined by Hernandez and Christensen-Dalsgaard (1994). The computed depth of the convective zone is R=0.712R, in agreement with the observed value determined from p-mode oscillation data of R=0.713{$\pm$}0.003R found by Christensen-Dalsgaard et al. (1991). Although the present results increase the predicted event rate in the four operating solar neutrino experiments by almost 1 {$\sigma$} (theoretical uncertainty), they only slightly increase the difficulty of explaining the existing experiments with standard physics (i.e., by assuming that nothing happens to the neutrinos after they are created in the center of the sun). For an extreme model in which all diffusion (helium and heavy-element diffusion) is neglected, the event rates are 7.0-1.0+0.9 SNU for the Cl37 experiment and 126-6+6 SNU for the Ga71 experiments, while the Be7 and B8 neutrino fluxes are, respectively, 4.5(1.00-0.07+0.06)\texttimes 109 cm-2 s-1 and 4.9(1.00-0.17+0.14)\texttimes 106 cm-2 s-1. For the no-diffusion model, the computed value of the depth of the convective zone is R=0.726R, which disagrees with the observed helioseismological value. The calculated surface abundance of helium, Ys=0.268, is also in disagreement with the p-mode measurement. The authors conclude that helioseismology provides strong evidence for element diffusion and therefore for the somewhat larger solar neutrino event rates calculated in this paper. \textcopyright{} 1995 The American Physical Society.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XF2DQR5M/Bahcall, Pinsonneault, Wasserburg - 1995.pdf}
}

@article{Bahcall1997,
  title = {Are Standard Solar Models Reliable?},
  author = {Bahcall, John N. and Pinsonneault, M. H. and Basu, Sarbani and {Christensen-Dalsgaard}, J.},
  year = {1997},
  journal = {Physical Review Letters},
  volume = {78},
  number = {2},
  pages = {171--174},
  issn = {10797114},
  doi = {10.1103/PhysRevLett.78.171},
  abstract = {The sound speeds of solar models that include element diffusion agree with helioseismological measurements to a rms discrepancy of better than 0.2\% throughout almost the entire Sun. Models that do not include diffusion, or in which the interior of the Sun is assumed to be significantly mixed, are effectively ruled out by helioseismology. Standard solar models predict the measured properties of the Sun more accurately than is required for applications involving solar neutrinos. \textcopyright{} 1997 The American Physical Society.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SQRRISPK/Bahcall et al. - 1997.pdf}
}

@article{Bahcall2004,
  title = {What Do We (Not) Know Theoretically about Solar Neutrino Fluxes?},
  author = {Bahcall, John N. and Pinsonneault, M. H.},
  year = {2004},
  journal = {Physical Review Letters},
  volume = {92},
  number = {12},
  eprint = {astro-ph/0402114},
  pages = {1--4},
  issn = {00319007},
  doi = {10.1103/PhysRevLett.92.121301},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/N8GV9WBW/Bahcall, Pinsonneault - 2004.pdf}
}

@article{Bahcall2004a,
  title = {Helioseismological {{Implications}} of {{Recent Solar Abundance Determinations}}},
  author = {Bahcall, John N. and Basu, Sarbani and Pinsonneault, Marc and Serenelli, Aldo M.},
  year = {2004},
  eprint = {astro-ph/0407060},
  doi = {10.1086/426070},
  abstract = {We show that standard solar models are in good agreement with the helioseismologically determined sound speed and density as a function of solar radius, the depth of the convective zone, and the surface helium abundance, as long as those models do not incorporate the most recent heavy element abundance determinations. However, sophisticated new analyses of the solar atmosphere infer lower abundances of the lighter metals (like C, N, O, Ne, and Ar) than the previously widely used surface abundances. We show that solar models that include the lower heavy element abundances disagree with the solar profiles of sound speed and density as well as the depth of the convective zone and the helium abundance. The disagreements for models with the new abundances range from factors of several to many times the quoted uncertainties in the helioseismological measurements. The disagreements are at temperatures below what is required for solar interior fusion reactions and therefore do not significantly affect solar neutrino emission. If errors in thecalculated OPAL opacities are solely responsible for the disagreements, then the corrections in the opacity must extend from 2 times 10\^6 K (R = 0.7R\_Sun)to 5 times 10\^6 K (R = 0.4 R\_Sun), with opacity increases of order 10\%.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/B4YEZWCI/Bahcall et al. - 2004.pdf}
}

@article{Bahcall2005,
  title = {What {{Is}} the {{Neon Abundance}} of the {{Sun}}?},
  author = {Bahcall, John N. and Basu, Sarbani and Serenelli, Aldo M.},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {631},
  number = {2},
  eprint = {astro-ph/0502563},
  pages = {1281--1285},
  issn = {0004-637X},
  doi = {10.1086/431926},
  abstract = {We have evolved a series of thirteen complete solar models that utilize different assumed heavy element compositions. Models that are based upon the heavy element abundances recently determined by Asplund, Grevesse, and Sauval (2005) are inconsistent with helioseismological measurements. However, models in which the neon abundance is increased by 0.4-0.5 dex to log N(Ne) = 8.29 +- 0.05 (on the scale in which log N(H) = 12) are consistent with the helioseismological measurements even though the other heavy element abundances are in agreement with the determinations of Asplund et al. (2005). These results sharpen and strengthen an earlier study by Antia and Basu (2005). The predicted solar neutrino fluxes are affected by the uncertainties in the composition by less than their 1sigma theoretical uncertainties.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FAEXGQ47/Bahcall, Basu, Serenelli - 2005.pdf}
}

@article{Bahcall2006,
  title = {10,000 {{Standard Solar Models}}: {{A Monte Carlo Simulation}}},
  author = {Bahcall, John N. and Serenelli, Aldo M. and Basu, Sarbani},
  year = {2006},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {165},
  number = {1},
  eprint = {astro-ph/0511337},
  pages = {400--431},
  issn = {0067-0049},
  doi = {10.1086/504043},
  abstract = {We have evolved 10,000 solar models using 21 input parameters that are randomly drawn for each model from separate probability distributions for every parameter. We use the results of these models to determine the theoretical uncertainties in the predicted surface helium abundance, the profile of the sound speed versus radius, the profile of the density versus radius, the depth of the solar convective zone, the eight principal solar neutrino fluxes, and the fractions of nuclear reactions that occur in the CNO cycle or in the three branches of the p-p chains. We also determine the correlation coefficients of the neutrino fluxes for use in analysis of solar neutrino oscillations. Our calculations include the most accurate available input parameters, including radiative opacity, equation of state, and nuclear cross sections. We incorporate both the recently determined heavy element abundances recommended by Asplund, Grevesse \& Sauval (2005) and the older (higher) heavy element abundances recommended by Grevesse \& Sauval (1998). We present best-estimates of many characteristics of the standard solar model for both sets of recommended heavy element compositions.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3LMGGFXW/Bahcall, Serenelli, Basu - 2006.pdf}
}

@article{Bailey1902,
  title = {Miscellaneous {{Variables}} and {{NCG}} 7078, 6656, {{M3}}, {{M5}}},
  author = {Bailey, Solon Irving and Irving, Solon},
  year = {1902},
  journal = {phae},
  volume = {6},
  pages = {2290},
  urldate = {2020-04-14},
  keywords = {Harvard College Observatory,notion,notion-database,Project PHAEDRA}
}

@article{Baines2016,
  title = {Spectroscopic and {{Interferometric Measurements}} of {{Nine K Giant Stars}}},
  author = {Baines, Ellyn K. and D{\"o}llinger, Michaela P. and Guenther, Eike W. and Hatzes, Artie P. and Hrudkovu, Marie and {van Belle}, Gerard T.},
  year = {2016},
  eprint = {1609.02379},
  doi = {10.3847/0004-6256/152/3/66},
  abstract = {We present spectroscopic and interferometric measurements for a sample of nine K giant stars. These targets are of particular interest because they are slated for stellar oscillation observations. Our improved parameters will directly translate into reduced errors in the final masses for these stars when interferometric radii and asteroseismic densities are combined. Here we determine each star's limb-darkened angular diameter, physical radius, luminosity, bolometric flux, effective temperature, surface gravity, metallicity, and mass. When we compare our interferometric and spectroscopic results, we find no systematic offsets in the diameters and the values generally agree within the errors. Our interferometric temperatures for seven of the nine stars are hotter than those determined from spectroscopy with an average difference of about 380 K.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G9W7LZTB/Baines et al. - 2016.pdf}
}

@article{Balbus1991,
  title = {A Powerful Local Shear Instability in Weakly Magnetized Disks. {{I}} - {{Linear}} Analysis. {{II}} - {{Nonlinear}} Evolution},
  author = {Balbus, Steven A. and Hawley, John F.},
  year = {1991},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {376},
  pages = {214},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/170270},
  urldate = {2020-07-02},
  abstract = {applicability for this approach.},
  keywords = {ACCRETION,Accretion Disks,Astrophysics,Boussinesq Approximation,Computational Astrophysics,HYDRODYNAMICS,HYDROMAGNETICS,INSTABILITIES,Linear Systems,Magnetohydrodynamic Stability,notion,notion-database,Stellar Magnetic Fields,Stellar Mass Accretion}
}

@article{Balbus1994,
  title = {The {{Stability}} of {{Differentially Rotating Weakly Magnetized Stellar Radiative Zones}} - {{NASA}}/{{ADS}}},
  author = {Balbus, S.A. and Hawley, J.F.},
  year = {1994},
  journal = {MNRAS},
  volume = {266},
  urldate = {2020-03-09},
  keywords = {notion,notion-database}
}

@article{Baliun1995a,
  title = {Are Variations in the Length of the Activity Cycle Related to Changes in Brightness in Solar-Type Stars ?},
  author = {Baliunas, Sallie and Soon, Willie},
  year = {1995},
  journal = {The Astrophysical Journal},
  volume = {450},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ATLE6HNB/Baliunas, Soon - 1995.pdf}
}

@article{Baliunas1990a,
  title = {Evidence for Long-Term Brightness Changes of Solar-Type Stars},
  author = {Baliunas, Sallie and Jastrow, Robert},
  year = {1990},
  journal = {Nature},
  volume = {348},
  number = {6301},
  pages = {520--523},
  issn = {00280836},
  doi = {10.1038/348520a0},
  abstract = {CHANGES in the brightness of the Sun may introduce further uncertainties into forecasts of global warming by the greenhouse effect. The Sun is known to vary in brightness, on a timescale of years, by 0.1\% in phase with changes in magnetic activity during the solar cycle1-3, and variations of up to 0.4\%, also correlated with surface magnetic activity, have been found in stars similar to the Sun4. To delimit the magnitude of solar luminosity variations on a timescale of centuries, we have looked at the magnetic behaviour of a number of solar-type stars over several years. Observed in random phases of their long-term variability, they give a sample of the behaviour of a solar-type star over a long period of time. We find indirect evidence that these stars undergo brightness changes of more than the 0.1\% observed during the last solar cycle, a result that calls into question the assumption of a constant Sun in calculations using general circulation models for climate forecasting. \textcopyright{} 1990 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Y9CN96MC/Baliunas, Jastrow - 1990.pdf}
}

@article{Baliunas1995,
  title = {Chromospheric Variations in Main-Sequence Stars. {{II}}.},
  author = {et al. Baliunas, Sallie L.},
  year = {1995},
  journal = {The Astrophysical Journal},
  volume = {438},
  pages = {269--287},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/83QT6APJ/Baliunas - 1995.pdf}
}

@article{Baliunas1996,
  title = {A {{Dynamo Interpretation}} of {{Stellar Activity Cycles}}},
  author = {Baliunas, S. L. and {Nesme-Ribes}, E. and Sokoloff, D. and Soon, W. H.},
  year = {1996},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {460},
  pages = {848},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/177014},
  urldate = {2020-07-02},
  abstract = {Twenty-five-year records of Ca II H and K chromospheric emission fluxes measured in single lower main-sequence stars at Mount Wilson Observatory reveal surface magnetic activity cycles in one-third of the sample of roughly 100 stars. For those stars with cycles, we compare the ratio of the observed periods of the cycle of magnetic activity and axial rotation, Pcyc/Prot, to predictions available from stellar dynamo theory. Theoretical considerations suggest that the ratio is the observational equivalent of the stellar dynamo number, D. The stellar sample is comprised of two groups separated by their mean level of activity, {$\langle$}R{${'}$}HK{$\rangle$}, and rotation, Prot: one group has high levels of average activity and fast rotation, while the other group has relatively low levels of activity and slower rotation. Both groups also occupy different regions on the diagram of X-ray flux versus stellar dynamo number. For the older group of stars (ages {$\greaterequivlnt$}2 Gyr) which includes the current Sun, we find a statistically significant inverse relation between the intensity of the cycle, c = {$\Delta$}R{${'}$}HK/{$\langle$}R{${'}$}HK{$\rangle$}, and the stellar dynamo number, empirically determined to be D {$\sim$} (Pcyc/Prot)1.35+0.65/-0.35. \textcopyright{} 1996. The American Astronomical Society. All rights reserved.},
  keywords = {MAGNETOHYDRODYNAMICS: MHD,notion,notion-database,STARS: ACTIVITY,STARS: MAGNETIC FIELDS,STARS: ROTATION}
}

@article{Ball2017,
  title = {Surface-Effect Corrections for Oscillation Frequencies of Evolved Stars},
  author = {Ball, W. H. and Gizon, L.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {600},
  issn = {14320746},
  doi = {10.1051/0004-6361/201630260},
  abstract = {Context. Accurate modelling of solar-like oscillators requires that modelled mode frequencies are corrected for the systematic shift caused by improper modelling of the near-surface layers, known as the surface effect. Several parametrizations of the surface effect are now available but they have not yet been systematically compared with observations of stars showing modes with mixed g- and p-mode character. Aims. We investigate how much additional uncertainty is introduced to stellar model parameters by our uncertainty about the functional form of the surface effect. At the same time, we test whether any of the parametrizations is significantly better or worse at modelling observed subgiants and low-luminosity red giants. Methods. We model six stars observed by Kepler that show clear mixed modes. We fix the input physics of the stellar models and vary the choice of surface correction between five parametrizations. Results. Models using a solar-calibrated power law correction consistently fit the observations more poorly than the other four corrections. Models with the remaining four corrections generally fit the observations about equally well, with the combined surface correction by Ball \& Gizon perhaps being marginally superior. The fits broadly agree on the model parameters within about the 2{$\sigma$} uncertainties, with discrepancies between the modified Lorentzian and free power law corrections occasionally exceeding the 3{$\sigma$} level. Relative to the best-fitting values, the total uncertainties on the masses, radii and ages of the stars are all less than 2, 1 and 6 per cent, respectively. Conclusions. A solar-calibrated power law, as formulated by Kjeldsen et al., appears unsuitable for use with more evolved solar-like oscillators. Among the remaining surface corrections, the uncertainty in the model parameters introduced by the surface effects is about twice as large as the uncertainty in the individual fits for these six stars. Though the fits are thus somewhat less certain because of our uncertainty of how to manage the surface effect, these results also demonstrate that it is feasible to model the individual mode frequencies of subgiants and low-luminosity red giants, and hence also use these individual stars to help to constrain stellar models.},
  keywords = {notion,notion-database}
}

@article{Ballot2004,
  title = {Seismic Extraction of the Convective Extent in Solar-like Stars: {{The}} Observational Point of View},
  author = {Ballot, J. and {Turck-Chi{\`e}ze}, S. and Garc{\'i}a, R. A.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {423},
  number = {3},
  pages = {1051--1061},
  issn = {00046361},
  doi = {10.1051/0004-6361:20035898},
  abstract = {Convection is the first manifestation of macroscopic motions in stars. In the next decade, the extent of the external convective zone of solar-like stars will have to be derived from the eigenfrequencies of their low-degree ({$\mathscr{l}$} = 0, 1 and 2) acoustic modes. In this paper, we compare different tracers of the base of the convective zone (BCZ) and show that the second difference {$\delta\delta$}2v stays simple and well suited for analyzing real data. We suggest the use of {\~t}BCZ = (2{$<\Delta$}v{$>$}) -1 - {$\tau\tilde$}BCZ as a quasinon-biased indicator of the BCZ acoustic radius. The method is first checked on a long-time solar observation with GOLF, then on shorter real observations by VIRGO and 10000 simulated observations of solar-like stars, We present results for different observational duration and stellar masses. The intrinsic error due to the method on the convective extent is smaller than 1.5\% (in units of stellar acoustic radius) for stars with masses between 0.9 and 1.3 M{$\odot$}. The limited observational interval adds a supplementary uncertainty of about 1.6\% for a 150-day long simulated observation. In this study, we have also analyzed the effects of stochastic excitation and of non-continuous runs of shorter lengths. We discuss how to take into account the variations in activity.},
  keywords = {Convection,Methods: data analysis,notion,notion-database,Stars: interiors,Stars: oscillations,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/LE2JFM87/Ballot, Turck-Chièze, García - 2004.pdf}
}

@article{Ballot2006a,
  title = {Rotation Speed and Stellar Axis Inclination from p Modes: {{How CoRoT}} Would See Other Suns},
  author = {Ballot, J. and Garc{\'i}a, R. A. and Lambert, P.},
  year = {2006},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {369},
  number = {3},
  pages = {1281--1286},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2006.10375.x},
  abstract = {In the context of future space-based asteroseismic missions, we have studied the problem of extracting the rotation speed and the rotation-axis inclination of solar-like stars from the expected data. We have focused on slow rotators (at most twice solar rotation speed), first, because they constitute the most difficult case and, secondly, because some of the Convection Rotation and planetary Transits (CoRoT) main targets are expected to have slow rotation rates. Our study of the likelihood function has shown a correlation between the estimates of inclination of the rotation axis i and the rotational splitting {$\delta\nu$} of the star. By using the parameters, i and , we propose and discuss new fitting strategies. Monte Carlo simulations have shown that we can extract a mean splitting and the rotation-axis inclination down to solar rotation rates. However, at the solar rotation rate we are not able to correctly recover the angle i, although we are still able to measure a correct with a dispersion less than 40 nHz. \textcopyright{} 2006 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: oscillations,Stars: rotation,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/KYR3TT8E/Ballot, García, Lambert - 2006.pdf}
}

@article{Ballot2008,
  title = {On Deriving P-Mode Parameters for Inclined Solar-like Stars},
  author = {Ballot, J. and Appourchaux, T. and Toutain, T. and Guittet, M.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {486},
  number = {3},
  pages = {867--875},
  issn = {00046361},
  doi = {10.1051/0004-6361:20079343},
  abstract = {Context. Thanks to their high quality, new and upcoming asteroseismic observations, with CoRoT, Kepler, and from the ground, benefit from experience gained with helioseismology. Aims. We focus, in this paper, on solar-like oscillations, for which the inclination of the rotation axis is unknown. We present a theoretical study of the errors of p-mode parameters determined by means of a maximum-likelihood estimator, and we also analyze correlations and biases. Methods. We used different, complementary approaches: we performed either semi-analytical computation of the Hessian matrix, fitting of single mean profiles, or Monte Carlo simulations. Results. First, we give analytical approximations for the errors of frequency, inclination and rotational splitting. The determination of the inclination is very challenging for the common case of slow rotators (like the Sun), making the determination of a reliable rotational splitting difficult. Moreover, due to the numerous correlations, biases - more or less significant - can appear in the determination of various parameters in the case of bad inclination fittings, especially when a locking at 90\textdegree{} occurs. We also discuss this issue. Nevertheless, the central frequency and some derived parameters, such as the total power of the mode, are free of such biases. \textcopyright{} ESO 2008.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/BGVJ4ZTU/Ballot et al. - 2008.pdf}
}

@article{Ballot2010,
  title = {Current Methods for Analyzing Light Curves of Solar-like Stars},
  author = {Ballot, J.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  eprint = {1008.0495},
  pages = {933--939},
  issn = {00046337},
  doi = {10.1002/asna.201011430},
  abstract = {CoRoT has allowed a quantitative leap for the solar-like-star seismology thanks to 5-month-long uninterrupted timeseries of high-precision photometric data. Kepler is also starting to deliver similar data. Now, several F and G main-sequence stars have been analyzed. The techniques developed to interpret light curves directly inherit from the experience got on the Sun with helioseismology. I describe in this review the methods currently used to analyze these light curves. First, these data provide an accurate determination of the stellar rotation rate. This is possible thanks to the magnetic activity of stars. The power spectra of light curves put also constraints on the stellar granulation, which can be directly compared to 3-D stellar atmosphere models; this shows still unexplained discrepancies. I then detailed a standard method for extracting p-mode characteristics (frequency, amplitude and lifetime). CoRoT has revealed unexpected short life times for F stars. Last, I also discuss errors and biases of mode frequencies, especially the ones due to the simplified description of the rotation generally used (\textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim) Copyright \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: activity,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/58V25KUF/Ballot - 2010.pdf}
}

@article{Ballot2011,
  title = {Accurate P-Mode Measurements of the {{G0V}} Metal-Rich {{CoRoT}}*target {{HD}} 52265},
  author = {Ballot, J. and Gizon, L. and Samadi, R. and Vauclair, G. and Benomar, O. and Bruntt, H. and Mosser, B. and Stahn, T. and Verner, G. A. and Campante, T. L. and Garc{\'i}a, R. A. and Mathur, S. and Salabert, D. and Gaulme, P. and R{\'e}gulo, C. and Roxburgh, I. W. and Appourchaux, T. and Baudin, F. and Catala, C. and Chaplin, W. J. and Deheuvels, S. and Michel, E. and Bazot, M. and Creevey, O. and Dolez, N. and Elsworth, Y. and Sato, K. H. and Vauclair, S. and Auvergne, M. and Baglin, A.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {530},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116547},
  abstract = {Context. The star HD 52265 is a G0V metal-rich exoplanet-host star observed in the seismology field of the CoRoT space telescope from November 2008 to March 2009. The satellite collected 117 days of high-precision photometric data on this star, showing that it presents solar-like oscillations. HD 52265 was also observed in spectroscopy with the Narval spectrograph at the same epoch. Aims. We characterise HD 52265 using both spectroscopic and seismic data. Methods. The fundamental stellar parameters of HD 52265 were derived with the semi-automatic software VWA, and the projected rotational velocity was estimated by fitting synthetic profiles to isolated lines in the observed spectrum. The parameters of the observed p modes were determined with a maximum-likelihood estimation. We performed a global fit of the oscillation spectrum, over about ten radial orders, for degrees l = 0 to 2. We also derived the properties of the granulation, and analysed a signature of the rotation induced by the photospheric magnetic activity. Results. Precise determinations of fundamental parameters have been obtained: Teff = 6100 {$\pm$} 60 K, logg = 4.35 {$\pm$} 0.09, [M/H] = 0.19 {$\pm$} 0.05, as well as \textbackslash vsini=3.6+0.3-1.0\textbackslash kms\vphantom\{\}. We have measured a mean rotation period Prot = 12.3 {$\pm$} 0.15 days, and find a signature of differential rotation. The frequencies of 31 modes are reported in the range 1500-2550 {$\mu$}Hz. The large separation exhibits a clear modulation around the mean value \textbackslash hbox\{\$\textbackslash Dnu=98.3\textbackslash,\textbackslash pm\textbackslash,0. 1{$\sim$}muHz\$\}. Mode widths vary with frequency along an S-shape with a clear local maximum around 1800 {$\mu$}Hz. We deduce lifetimes ranging between 0.5 and 3 days for these modes. Finally, we find a maxim al bolometric amplitude of about 3.96 {$\pm$} 0.24 ppm for radial modes. \textcopyright{} 2011 ESO.},
  keywords = {asteroseismology,notion,notion-database,stars: fundamental parameters,stars: individual: HD 52265,stars: rotation,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/HZRNPIVS/Ballot et al. - 2011.pdf}
}

@article{Ballot2011a,
  title = {Visibilities and Bolometric Corrections for Stellar Oscillation Modes Observed by {{Kepler}}: ({{Research}} Note)},
  author = {Ballot, J. and Barban, C. and {Van'T Veer-Menneret}, C.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {531},
  pages = {1--5},
  issn = {00046361},
  doi = {10.1051/0004-6361/201016230},
  abstract = {Context.Kepler produces a large amount of data used for asteroseismological analyses, particularly of solar-like stars and red giants. The mode amplitudes observed in the Kepler spectral band have to be converted into bolometric amplitudes to be compared to models. Aims. We give a simple bolometric correction for the amplitudes of radial modes observed with Kepler, as well as the relative visibilities of non-radial modes. Methods. We numerically compute the bolometric correction cK-bol and mode visibilities for different effective temperatures Teff within the range 4000-7500 K, using a similar approach to a recent one from the literature. Results. We derive a law for the correction to bolometric values: cK - bol = 1 + a 1(Teff - To) + a2(Teff - To)2, with To = 5934 K, a1 = 1.349 \texttimes{} 10-4 K-1, and a2 = -3.120 \texttimes{} 10-9 K-2 or, alternatively, as the power law c K - bol = (Teff/To){$\alpha$} with {$\alpha$} = 0.80. We give tabulated values for the mode visibilities based on limb-darkening (LD), computed from ATLAS9 model atmospheres for Teff [4000,7500] K, log g [2.5,4.5], and [M/H] [- 1.0, + 1.0]. We show that using LD profiles already integrated over the spectral band provides quick and good approximations for visibilities. We point out the limits of these classical visibility estimations. \textcopyright{} 2011 ESO.},
  keywords = {asteroseismology,notion,notion-database,stars: atmospheres,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/WQYNTMAV/Ballot, Barban, Van'T Veer-Menneret - 2011.pdf}
}

@article{Balmforth1992,
  title = {Solar Pulsational Stability - {{III}}. {{Acoustical}} Excitation by Turbulent Convection},
  author = {Balmforth J., N.},
  year = {1992},
  journal = {MNRAS},
  volume = {255},
  number = {4},
  pages = {639},
  publisher = {{Oxford University Press}},
  issn = {0035-8711},
  doi = {10.1093/MNRAS/255.4.639},
  urldate = {2022-01-26},
  abstract = {Current opinion presumes that solar five-minute oscillations are intrinsically damped and excited as a consequence of the emission of acoustical radiation by turbulent convective flows. Prescriptions modelling this process are employed to estimate modal mean amplitudes. The resulting oscillation power spectra can be made to agree with observation by adjusting various theoretical parameters. Whilst this ruins the predictive power of the theory, it does demonstrate that the hypothesis of stochastic excitation is plausible. Uncertainties in the theory are shown to have substantial repercussions on the mean amplitudes.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/A3CFHVBW/full-text.pdf}
}

@article{Balona2011,
  title = {Kepler Observations of Rapidly Oscillating {{Ap}}, {$\delta$} {{Scuti}} and {$\gamma$} {{Doradus}} Pulsations in {{Ap}} Stars},
  author = {Balona, L. A. and Cunha, M. S. and Kurtz, D. W. and Brand{\~a}o, I. M. and Gruberbauer, M. and Saio, H. and {\O}stensen, R. and Elkin, V. G. and Borucki, W. J. and {Christensen-Dalsgaard}, J. and Kjeldsen, H. and Koch, D. G. and Bryson, S. T.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {410},
  number = {1},
  eprint = {1006.4013},
  pages = {517--524},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2010.17461.x},
  abstract = {Observations of the A5p star KIC 8677585 obtained during the Kepler 10-d commissioning run with 1-min time resolution show that it is a rapidly oscillating Ap (roAp) star with several frequencies with periods near 10 min. In addition, a low frequency at 3.142 d-1 is also clearly present. Multiperiodic {$\gamma$} Doradus ({$\gamma$}Dor) and {$\delta$} Scuti ({$\delta$} Sct) pulsations, never before seen in any Ap star, are present in Kepler observations of at least three other Ap stars. Since {$\gamma$} Dor pulsations are seen in Ap stars, it is likely that the low frequency in KIC 8677585 is also a {$\gamma$} Dor pulsation. The simultaneous presence of both {$\gamma$} Dor and roAp pulsations and the unexpected detection of {$\delta$} Sct and {$\gamma$} Dor pulsations in Ap stars present new opportunities and challenges for the interpretation of these stars. Since it is easy to confuse Am and Ap stars at classification dispersions, the nature of these Ap stars in the Kepler field needs to be confirmed. \textcopyright{} 2010 The Authors. Journal compilation \textcopyright{} 2010 RAS.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: chemically peculiar,Stars: individual: BD+44 3063,Stars: oscillations,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/XRPUENCW/Balona et al. - 2011.pdf}
}

@article{Balona2011a,
  title = {Kepler Observations of the Variability in {{B-type}} Stars},
  author = {Balona, L. A. and Pigulski, A. and Cat, P. De and Handler, G. and {Guti{\'e}rrez-Soto}, J. and Engelbrecht, C. A. and Frescura, F. and Briquet, M. and Cuypers, J. and {Daszy{\'n}ska-Daszkiewicz}, J. and Degroote, P. and Dukes, R. J. and Garcia, R. A. and Green, E. M. and Heber, U. and Kawaler, S. D. and Lehmann, H. and Leroy, B. and {Molenda-Zakowicz}, J. and Neiner, C. and Noels, A. and Nuspl, J. and {\O}stensen, R. and Pricopi, D. and Roxburgh, I. and Salmon, S. and Smith, M. A. and Su{\'a}rez, J. C. and Suran, M. and Szab{\'o}, R. and Uytterhoeven, K. and {Christensen-Dalsgaard}, S. and Kjeldsen, H. and Caldwell, D. A. and Girouard, F. R. and Sanderfer, D. T.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {413},
  number = {4},
  pages = {2403--2420},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.18311.x},
  abstract = {The analysis of the light curves of 48 B-type stars observed by Kepler is presented. Among these are 15 pulsating stars, all of which show low frequencies, characteristic of slowly pulsating B (SPB) stars. Seven of these stars also show a few weak, isolated high frequencies and they could be considered as SPB/{$\beta$} Cephei ({$\beta$} Cep) hybrids. In all cases, the frequency spectra are quite different from what is seen from ground-based observations. We suggest that this is because most of the low frequencies are modes of high degree which are predicted to be unstable in models of mid-B stars. We find that there are non-pulsating stars within the {$\beta$} Cep and SPB instability strips. Apart from the pulsating stars, we can identify stars with frequency groupings similar to what is seen in Be stars but which are not Be stars. The origin of the groupings is not clear, but may be related to rotation. We find periodic variations in other stars which we attribute to proximity effects in binary systems or possibly rotational modulation. We find no evidence for pulsating stars between the cool edge of the SPB and the hot edge of the {$\delta$} Sct instability strips. None of the stars shows the broad features which can be attributed to stochastically excited modes as recently proposed. Among our sample of B stars are two chemically peculiar stars, one of which is a HgMn star showing rotational modulation in the light curve. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {notion,notion-database,Stars: early-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/JUSU7F56/Balona et al. - 2011(2).pdf;/Users/lbugnet/Zotero/storage/R8KVCH93/Balona et al. - 2011(2).pdf}
}

@article{Balona2011b,
  title = {Kepler Observations of {$\delta$} {{Scuti}} Stars},
  author = {Balona, L. A. and Dziembowski, W. A.},
  year = {2011},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {417},
  number = {1},
  pages = {591--601},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.19301.x},
  urldate = {2020-03-27},
  abstract = {We analyse observations of 1568 {$\delta$} Scuti stars in the public archive of the Kepler satellite. We compare the location of these stars in the Hertzsprung-Russell (HR) diagram with that calculated by linear, non-adiabatic pulsation models. There is generally a good agreement and it appears that many of the hotter {$\delta$} Scuti stars are pulsating in overtones as high as radial order n= 8. Models predict unstable modes of intermediate and high spherical harmonic, l, which are trapped in the envelope. The instability strip for these modes extends well beyond the blue edge for l{$\leq$} 4 and should be visible in the Kepler data. However, stars with these predicted properties are not seen. Moreover, we find that the observed frequency range does not agree with the models. Another challenge is to understand why more than half of the stars in the {$\delta$} Sct instability strip are not pulsating. The distribution of amplitudes argues strongly against the notion that the pulsation amplitudes are below the Kepler detection limit. The mode density of {$\delta$} Scuti stars is surprisingly low and suggests that modes of a high degree are not common. We do not find any stars with mode densities as high as that found in the CoRoT observations of HD 50844. The periodograms of stars in the same part of the HR diagram vary widely. However, we have identified a group of {$\delta$} Scuti stars characterized by a single dominant frequency in which a period-luminosity law is present. In many cases the dominant frequency is accompanied by a close frequency of lower amplitude. The problem of low frequencies in hot {$\delta$} Scuti stars remains unresolved. We confirm that these frequencies have long lifetimes and are not likely to be of stochastic origin. By carefully examining the periodograms of {$\delta$} Sct stars in the low-frequency regime, we were able to identify a group of {$\delta$} Sct stars with low-frequency peaks closely resembling those attributed to pure {$\gamma$} Dor stars. These stars lie in the region of the HR diagram where ground-based {$\gamma$} Dor stars are located. None is found hotter than the blue edge of {$\gamma$} Dor pulsation. We suspect that these are genuine {$\gamma$} Dor/{$\delta$} Sct hybrids. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {notion,notion-database,Stars: oscillations,Stars: variables: {$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/JJ52BWC3/full-text.pdf}
}

@article{Balona2011c,
  title = {The {{Kepler}} View of {$\gamma$} {{Doradus}} Stars},
  author = {Balona, L. A. and Guzik, J. A. and Uytterhoeven, K. and Smith, J. C. and Tenenbaum, P. and Twicken, J. D.},
  year = {2011},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {415},
  number = {4},
  pages = {3531--3538},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.18973.x},
  urldate = {2020-03-27},
  abstract = {Visual classification of over 10000 stars in the Kepler data base has revealed a class of stars with almost monoperiodic light variations and characteristic beating. A subset of these stars have a larger light amplitude and asymmetric light curves with larger variation in maximum brightness than in minimum brightness. The beating is mostly a result of two dominant, closely spaced frequencies. A third group of stars shows multiple low frequencies of comparable amplitudes. All three types of star fall in the region of the Hertzsprung-Russell diagram where {$\gamma$} Dor stars are found and we therefore identify them as {$\gamma$} Dor variables. However, stars with migrating star-spots also have symmetric light curves with beats, so it is likely that the sample is contaminated by non-pulsating stars of this type. If we assume that the dominant frequency in stars with beats is the rotational frequency, the resulting distribution of equatorial rotational velocities matches that of field stars of similar temperature and luminosity. We therefore conclude that the pulsation periods of these stars must be close to their rotational periods. The third group with multiple frequencies may be slowly rotating {$\gamma$} Dor stars. This investigation is closely related to the presence of low frequencies in {$\delta$} Scuti stars which we briefly discuss. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {notion,notion-database,Stars: oscillations,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/TLRIXIZ7/full-text.pdf}
}

@article{Balona2013,
  title = {Long Periods in Two {{Kepler roAp}} Stars},
  author = {Balona, L. A.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {436},
  number = {2},
  pages = {1415--1421},
  issn = {00358711},
  doi = {10.1093/mnras/stt1660},
  abstract = {We analyse over three years of Kepler photometry for the two roAp stars KIC 10483436 and KIC 10195926. Our aim is to detect possible unexpected low frequencies and to determine the frequency and amplitude variations of the roAp pulsations. Both stars have frequencies close to, but not exactly equal to, half the frequency of rotation with highly variable amplitudes. The origin of this variation is at present not known. In KIC 10483436, the main roAp pulsation is highly variable in frequency, but none of the other modes vary in this way. \textcopyright{} 2013 The Author published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {notion,notion-database,Stars:chemically peculiar,stars:oscillations},
  file = {/Users/lbugnet/Zotero/storage/SBGEF6I3/Balona - 2013.pdf}
}

@article{Balona2018,
  title = {Gaia Luminosities of Pulsating {{A-F}} Stars in the {{Kepler}} Field},
  author = {Balona, L. A.},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {479},
  number = {1},
  eprint = {1806.02622},
  pages = {183--191},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/sty1511},
  abstract = {All stars in the Kepler field brighter than 12.5 mag have been classified according to variability type. A catalogue of {$\delta$} Scuti and {$\gamma$} Doradus stars is presented. The problem of low frequencies in {$\delta$} Sct stars, which occurs in over 98 percent of these stars, is discussed. Gaia DR2 parallaxes were used to obtain precise luminosities, enabling the instability strips of the two classes of variable to be precisely defined. Surprisingly, it turns out that the instability region of the {$\gamma$} Dor stars is entirely within the {$\delta$} Sct instability strip. Thus, {$\gamma$} Dor stars should not be considered a separate class of variable. The observed red and blue edges of the instability strip do not agree with recent model calculations. Stellar pulsation occurs in less than half of the stars in the instability region and arguments are presented to show that this cannot be explained by assuming pulsation at a level too low to be detected. Precise Gaia DR2 luminosities of high-amplitude {$\delta$} Sct stars (HADS) show that most of these are normal {$\delta$} Sct stars and not transition objects. It is argued that current ideas on A star envelopes need to be revised.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Parallaxes,Stars: oscillations,Stars: variables: {$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/YT3SD76M/Balona - 2018.pdf}
}

@article{Banyai2013,
  title = {Variability of {{M}} Giant Stars Based on {{Kepler}} Photometry: {{General}} Characteristics},
  author = {B{\'a}nyai, E. and Kiss, L. L. and Bedding, T. R. and Bellamy, B. and Benko, J. M. and B{\'o}di, A. and Callingham, J. R. and Compton, D. and Cs{\'a}nyi, I. and Derekas, A. and Dorval, J. and Huber, D. and Shrier, O. and Simon, A. E. and Stello, D. and Szab{\'o}, Gy M. and Szab{\'o}, R. and Szatm{\'a}ry, K.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {436},
  number = {2},
  eprint = {1309.1012},
  pages = {1576--1587},
  issn = {00358711},
  doi = {10.1093/mnras/stt1685},
  abstract = {Mgiants are among the longest period pulsating stars which iswhy their studies were traditionally restricted to analyses of low-precision visual observations, and, more recently, accurate ground-based data. Here we present an overview of M giant variability on a wide range of time-scales (hours to years), based on the analysis of 13 quarters of Kepler long-cadence observations (one point per every 29.4 min), with a total time-span of over 1000 d. About two-thirds of the sample stars have been selected from the All Sky Automated Survey (ASAS)-North survey of the Kepler field, with the rest supplemented from a randomly chosenMgiant control sample. We first describe the correction of the light curves from different quarters, which was found to be essential. We use Fourier analysis to calculate multiple frequencies for all stars in the sample. Over 50 stars show a relatively strong signal with a period equal to the Kepler-year and a characteristic phase dependence across the whole field of view. We interpret this as a so far unidentified systematic effect in the Kepler data. We discuss the presence of regular patterns in the distribution of multiple periodicities and amplitudes. In the period-amplitude plane we find that it is possible to distinguish between solar-like oscillations and larger amplitude pulsations which are characteristic for Mira/semiregular stars. This may indicate the region of the transition between two types of oscillations as we move upward along the giant branch. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars:AGB and post-AGB,Stars:Variables:General,Techniques: Photometric},
  file = {/Users/lbugnet/Zotero/storage/8W4I9D6R/Bányai et al. - 2013.pdf}
}

@article{Baraffe2003,
  title = {Evolutionary Models for Cool Brown Dwarfs and Extrasolar Giant Planets. {{The}} Case of {{HD}} 209458},
  author = {Baraffe, I. and Chabrier, G. and Barman, T. S. and Allard, F. and Hauschildt, P. H.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {402},
  number = {2},
  eprint = {astro-ph/0302293},
  pages = {701--712},
  publisher = {{EDP Sciences}},
  issn = {00046361},
  doi = {10.1051/0004-6361:20030252},
  urldate = {2020-03-23},
  abstract = {We present evolutionary models for cool brown dwarfs and extra-solar giant planets. The models reproduce the main trends of observed methane dwarfs in near-IR color-magnitude diagrams. We also present evolutionary models for irradiated planets, coupling for the first time irradiated atmosphere profiles and inner structures. We focus on HD 209458-like systems and show that irradiation effects can substantially affect the radius of sub-jovian mass giant planets. Irradiation effects, however, cannot alone explain the large observed radius of HD 209458b. Adopting assumptions which optimise irradiation effects and taking into account the extension of the outer atmospheric layers, we still find {$\sim$}20\% discrepancy between observed and theoretical radii. An extra source of energy seems to be required to explain the observed value of the first transit planet.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: brown dwarfs,Stars: evolution,Stars: individual (HD 209458)},
  file = {/Users/lbugnet/Zotero/storage/SPQHA8DR/full-text.pdf}
}

@article{Baran2005,
  title = {Multicolour Photometry of {{Balloon}} 090100001: Linking the Two Classes of Pulsating Hot Subdwarfs},
  shorttitle = {Multicolour Photometry of {{Balloon}} 090100001},
  author = {Baran, A. and Pigulski, A. and Kozie{\l}, D. and Og{\l}oza, W. and Silvotti, R. and Zo{\l}a, S.},
  year = {2005},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {360},
  pages = {737--747},
  issn = {0035-8711},
  doi = {10.1111/j.1365-2966.2005.09066.x},
  urldate = {2023-10-09},
  abstract = {We present results of multicolour UBVR photometry of the high-amplitude EC14026-type star Balloon090100001. The data span over a month and consist of more than a hundred hours of observations. Fourier analysis of these data led us to the detection of at least 30 modes of pulsation of which 22 are independent. The frequencies of 13 detected modes group in three narrow ranges, around 2.8, 3.8 and 4.7 mHz, where the radial fundamental mode and the first and second overtones are likely to occur. Surprisingly, we also detect nine independent modes in the low-frequency domain, between 0.15 and 0.4 mHz. These modes are typical for pulsations found in PG1716+426-type stars, discovered recently among cool B-type subdwarfs. The modes found in these stars are attributed to the high-order g modes. As both kinds of pulsations are observed in Balloon090100001, it represents a link between the two classes of pulsating hot subdwarfs. At present, it is probably the most suitable target for testing evolutionary scenarios and internal constitution models of these stars by means of asteroseismology. Three of the modes that we discovered form an equidistant frequency triplet which can be explained by invoking rotational splitting of an l= 1 mode. The splitting amounts to about 1.58 {$\mu$}Hz, leading to a rotation period of 7.1 +/- 0.1d.},
  keywords = {Astrophysics,stars: individual: Balloon 090100001,stars: oscillations,subdwarfs},
  annotation = {ADS Bibcode: 2005MNRAS.360..737B},
  file = {/Users/lbugnet/Zotero/storage/XDHLTWXZ/Baran et al. - 2005 - Multicolour photometry of Balloon 090100001 linki.pdf}
}

@article{Baran2012,
  title = {A Pulsation Zoo in the Hot Subdwarf {{B}} Star {{KIC10139564}} Observed by {{Kepler}}},
  author = {Baran, A. S. and Reed, M. D. and Stello, D. and {\O}stensen, R. H. and Telting, J. H. and Pak{\v s}tiene, E. and O'Toole, S. J. and Silvotti, R. and Degroote, P. and Bloemen, S. and Hu, H. and Van Grootel, V. and Clarke, B. D. and Van Cleve, J. and Thompson, S. E. and Ka{\'e}aler, S. D.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {424},
  number = {4},
  eprint = {1206.3841},
  pages = {2686--2700},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.21355.x},
  abstract = {We present our analyses of 15 months of Kepler data on KIC 10139564. We detected 57 periodicities with a variety of properties not previously observed all together in one pulsating subdwarf B (sdB) star. Ten of the periodicities were found in the low-frequency region, and we associate them with nonradial g modes. The other periodicities were found in the high-frequency region, which are likely p modes. We discovered that most of the periodicities are components of multiplets with a common spacing. Assuming that multiplets are caused by rotation, we derive a rotation period of 25.6 {$\pm$} 1.8 d. The multiplets also allow us to identify the pulsations to an unprecedented extent for this class of pulsator. We also detect l = 2 multiplets, which are sensitive to the pulsation inclination and can constrain limb darkening via geometric cancellation factors. While most periodicities are stable, we detected several regions that show complex patterns. Detailed analyses showed that these regions are complicated by several factors. Two are combination frequencies that originate in the super-Nyquist region and were found to be reflected below the Nyquist frequency. The Fourier peaks are clear in the super-Nyquist region, but the orbital motion of Kepler smears the Nyquist frequency in the barycentric reference frame and this effect is passed on to the sub-Nyquist reflections. Others are likely multiplets but unstable in amplitudes and/or frequencies. The density of periodicities also makes KIC 10139564 challenging to explain using published models. This menagerie of properties should provide tight constraints on structural models, making this sdB star the most promising for applying asteroseismology. To support our photometric analysis, we have obtained spectroscopic radial-velocity measurements of KIC 10139564 using low-resolution spectra in the Balmer-line region. We did not find any radial-velocity variation. We used our high signal-to-noise average spectrum to improve the atmospheric parameters of the sdB star, deriving Teff = 31 859 K and log g = 5.673 dex. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  archiveprefix = {arxiv},
  keywords = {\'d Asteroseismology,notion,notion-database,Stars: oscillation,Subd\'earfs,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/MCFFT272/Baran et al. - 2012.pdf}
}

@article{Baran2021,
  title = {A Search for Variable Subdwarf {{B}} Stars in {{TESS Full Frame Images}} - {{II}}. {{Variable}} Objects in the Northern Ecliptic Hemisphere},
  author = {Baran, A. S. and Sahoo, S. K. and Sanjayan, S. and Ostrowski, J.},
  year = {2021},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {503},
  pages = {3828--3847},
  issn = {0035-8711},
  doi = {10.1093/mnras/stab668},
  urldate = {2023-10-22},
  abstract = {We report the results of our search for pulsating subdwarf B stars in Full Frame Images collected during Year 2 of the TESS mission and covering the northern ecliptic hemisphere. This is a continuation of our effort we presented in Paper I. We found 13 likely new pulsating subdwarf B stars, 10 pulsating candidates that are identified as other hot subdwarfs, and 30 spectroscopically unclassified objects that show amplitude spectra typical of pulsating subdwarf B stars. We found 506 variable objects, most of them spectroscopically unclassified, hence their specific variability class yet to be confirmed. Eclipsing binaries with sharp eclipses sample comprises 33 systems. For 12 of them we derived precise orbital periods and checked their stabilities. We identified one known and five new candidate HW Vir systems. The amplitude spectra of the 13 likely sdB pulsators are not rich in modes, hence any further analysis is not possible. However, we selected three candidates for pulsating subdwarf B stars that show the richest amplitude spectra and we performed a mode identification deriving modal degrees of most of the detected modes. In total, in both ecliptic hemispheres, we found 15 likely pulsating pulsating subdwarf B stars, additional 10 candidates for pulsating subdwarf B stars, 66 other variable subdwarf B stars, 2076 spectroscopically unconfirmed variable stars, and 123 variable non-sdB stars.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: general,stars: oscillations (including pulsations),stars: variables: general,subdwarfs,surveys},
  annotation = {ADS Bibcode: 2021MNRAS.503.3828B},
  file = {/Users/lbugnet/Zotero/storage/YKEV43JC/Baran et al. - 2021 - A search for variable subdwarf B stars in TESS Ful.pdf}
}

@article{Baran2023,
  title = {Short-Period Pulsating Hot-Subdwarf Stars Observed by {{TESS}} - {{I}}. {{Southern}} Ecliptic Hemisphere},
  author = {Baran, A. S. and Grootel, V. Van and {\O}stensen, R. H. and Worters, H. L. and Sahoo, S. K. and Sanjayan, S. and Charpinet, S. and Nemeth, P. and Telting, J. H. and Kilkenny, D.},
  year = {2023},
  month = jan,
  journal = {Astronomy \& Astrophysics},
  volume = {669},
  pages = {A48},
  publisher = {{EDP Sciences}},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202244888},
  urldate = {2023-10-14},
  abstract = {We present results of a Transiting Exoplanet Survey Satellite (TESS) search for short-period pulsations in compact stellar objects observed in years 1 and 3 of the TESS mission, during which the southern ecliptic hemisphere was targeted. We describe the TESS data used and the details of the search method. For many of the targets, we use unpublished spectroscopic observations to classify the objects. From the TESS photometry, we clearly identify 43 short-period hot-subdwarf pulsators, including 32 sdB stars, eight sdOB stars, two sdO stars, and, significantly, one He-sdOB star, which is the first of this kind to show short-period pulsations. Eight stars show signals at both low and high frequencies, and are therefore ``hybrid'' pulsators. We report the list of prewhitened frequencies and we show the amplitude spectra calculated from the TESS data. We make an attempt to identify possible multiplets caused by stellar rotation, and we select four candidates with rotation periods between 1 and 12.9 days. The most interesting targets discovered in this survey should be observed throughout the remainder of the TESS mission and from the ground. Asteroseismic investigations of these data sets will be invaluable in revealing the interior structure of these stars and will boost our understanding of their evolutionary history. We find three additional new variable stars but their spectral and variability types remain to be constrained.},
  copyright = {\textcopyright{} The Authors 2023},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/DTRQK9ZM/Baran et al. - 2023 - Short-period pulsating hot-subdwarf stars observed.pdf}
}

@article{Baranne1979,
  title = {Coravel- {{A}} New Tool for Radial Velocity Measurements},
  author = {Baranne, A. and Mayor, M. and Poncet, J. L.},
  year = {1979},
  journal = {Vistas in Astronomy},
  volume = {23},
  number = {PART 4},
  pages = {279--316},
  issn = {00836656},
  doi = {10.1016/0083-6656(79)90016-3},
  abstract = {CORAVEL is a Cassegrain spectrophotometer for determining stellar radial velocities by cross-correlation. This is done between the spectrum and a suitable mask located in the focal surface. Before discussing the design of the spectrometer and in particular the use of an echelle grating, the process of optimization of the mask is described. The radial velocities determined by CORAVEL depend only on the calibration of the optics; this process is presented with some details. Finally, other quantities such as stellar rotation, v sini, and metallicities, [M/H] can be derived simultaneously from the cross-correlation function. \textcopyright{} 1980.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QXJJ4LRU/Baranne, Mayor, Poncet - 1979.pdf}
}

@article{Barban2007,
  title = {Detection of Solar-like Oscillations in the Red Giant Star {$\epsilon$} {{Ophiuchi}} by {{MOST}} Spacebased Photometry},
  author = {Barban, C. and Matthews, J. M. and De Ridder, J. and Baudin, F. and Kuschnig, R. and Mazumdar, A. and Samadi, R. and Guenther, D. B. and Moffat, A. F.J. and Rucinski, S. M. and Sasselov, D. and Walker, G. A.H. and Weiss, W. W.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {468},
  number = {3},
  pages = {1033--1038},
  issn = {00046361},
  doi = {10.1051/0004-6361:20066716},
  abstract = {Context. Solar-like oscillations have been discovered in a few red giants, including {$\epsilon$} Oph, through spectroscopy. Acoustic modes around 60 {$\mu$}Hz were clearly seen in this star, but daily aliasing of the groundbased data made it impossible to unambiguously isolate the p-mode frequencies in the eigenspectrum, and hence the correct value of the large spacing, to asteroseismically constrain the mass of this pulsating star. Aims, We obtained about 28 days of contiguous high-precision photometry of {$\epsilon$} Oph in May-June 2005 with the MOST (Microvariability \& Oscillations of STars) satellite. The thorough time sampling removes the ambiguity of the frequency identifications based on the groundbased discovery data. Methods. We identify equidistant peaks in the Fourier spectrum of the MOST photometry in the range where the p-modes were seen spectroscopically. Those peaks are searched by autocorrelation of the power spectrum to estimate the value of the large separation in the p-mode eigenspectrum. Having isolated the oscillation modes, we determine their mode parameters (frequency, amplitude and line width) by fitting the distribution of peaks to Lorentzian profiles. Results. The clear series of equidistant peaks in the power spectrum, with amplitudes from about 30 to 130 ppm, are consistent with radial modes spaced by a mean value of (5.3 {$\pm$}0.1) {$\mu$}Hz. This large separation matches one of the two possibilities allowed by the groundbased observations thus constraining the stellar models to a much greater extent than previously possible. The line widths and Lorentzian fits indicate a rather short average mode lifetime: (2.7-0.8+0.6) days. \textcopyright{} ESO 2007.},
  keywords = {notion,notion-database,Stars: individual: {$\epsilon$} Ophiuchi,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/JLGIPKZH/Barban et al. - 2007.pdf}
}

@article{Barban2009,
  title = {Solar-like Oscillations in {{HD}} 181420: {{Data}} Analysis of 156 Days of {{CoRoT}} Data},
  author = {Barban, C. and Deheuvels, S. and Baudin, F. and Appourchaux, T. and Auvergne, M. and Ballot, J. and Boumier, P. and Chaplin, W. J. and Garc{\'i}a, R. A. and Gaulme, P. and Michel, E. and Mosser, B. and R{\'e}gulo, C. and Roxburgh, I. W. and Verner, G. and Baglin, A. and Catala, C. and Samadi, R. and Bruntt, H. and Elsworth, Y. and Mathur, S.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {51--56},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911937},
  abstract = {Context. The estimate of solar-like oscillation properties, such as their frequencies, amplitudes and lifetimes, is challenging because of their low amplitudes and will benefit from long and uninterrupted observing runs. The space telescope CoRoT allows us to obtain high-performance photometric data over a long and quasi continuous period. Among its main targets are stars for which we expect solar-like oscillations. Aims. HD 181420, an F2 main sequence star, has been observed by CoRoT during its first long run covering about 156 days. With this unprecedently high-quality set of data, our aim is to derive the p-mode parameters that can be used to probe the stellar interior. Methods. The CoRoT data obtained on HD 181420 is analysed using a classical Fourier approach for the search for the p mode signature. The p-mode parameters are then derived using global fitting of the power spectrum by a Lorentzian model, as used widely in the solar case. Results. From the p-mode frequencies, the mean value of the large spacing is estimated to be 75 {$\mu$}Hz. The p-mode amplitudes are slightly less than 4 ppm with a line width of about 8 {$\mu$}Hz at the maximum of the p modes. The inclination angle is estimated to be around 45\textdegree. The large mode line-width combined with the observed mode spacing make it difficult to identify the {$\mathscr{l}$} = 2 modes and to estimate the rotational splitting. We explore two scenarios for the identification of the modes.},
  keywords = {notion,notion-database,Stars: individual: HD 181420,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/AVZQMH8V/Barban et al. - 2009.pdf}
}

@article{BarceloForteza2015,
  title = {Evidence of Amplitude Modulation Due to Resonant Mode Coupling in the {$\delta$} {{Scuti}} Star {{KIC}} 5892969: {{A}} Particular or a General Case?},
  author = {Barcel{\'o} Forteza, S. and Michel, E. and Roca Cort{\'e}s, T. and Garci{\'a}, R. A.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {579},
  pages = {1--8},
  issn = {14320746},
  doi = {10.1051/0004-6361/201425507},
  abstract = {A study of the star KIC 5892969 observed by the Kepler satellite is presented. Its three highest amplitude modes present a strong amplitude modulation. The aim of this work is to investigate amplitude variations in this star and their possible cause. Using the 4 years-long observations available, we obtained the frequency content of the full light curve. Then, we studied the amplitude and phase variations with time using shorter time stamps. The results obtained are compared with the predicted ones for resonant mode coupling of an unstable mode with lower frequency stable modes. Our conclusion is that resonant mode coupling is consistent as an amplitude limitation mechanism in several modes of KIC 5892969 and we discuss to which extent it might play an important role for other {$\delta$} Scuti stars.},
  keywords = {Asteroseismology,notion,notion-database,Stars: individual: KIC 5892969,Stars: oscillations,Stars: variables:{$\delta$}Scuti},
  file = {/Users/lbugnet/Zotero/storage/EDNIIRHB/Barceló Forteza et al. - 2015.pdf}
}

@article{Barclay2013,
  title = {A Super-Earth-Sized Planet Orbiting in or near the Habitable Zone around a Sun-like Star},
  author = {Barclay, Thomas and Burke, Christopher J. and Howell, Steve B. and Rowe, Jason F. and Huber, Daniel and Isaacson, Howard and Jenkins, Jon M. and Kolbl, Rea and Marcy, Geoffrey W. and Quintana, Elisa V. and Still, Martin and Twicken, Joseph D. and Bryson, Stephen T. and Borucki, William J. and Caldwell, Douglas A. and Ciardi, David and Clarke, Bruce D. and Christiansen, Jessie L. and Coughlin, Jeffrey L. and Fischer, Debra A. and Li, Jie and Haas, Michael R. and Hunter, Roger and Lissauer, Jack J. and Mullally, Fergal and Sabale, Anima and Seader, Shawn E. and Smith, Jeffrey C. and Tenenbaum, Peter and Kamal Uddin, A. K.M. and Thompson, Susan E.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {768},
  number = {2},
  eprint = {1304.4941},
  pages = {1--8},
  issn = {15384357},
  doi = {10.1088/0004-637X/768/2/101},
  abstract = {We present the discovery of a super-Earth-sized planet in or near the habitable zone of a Sun-like star. The host is Kepler-69, a 13.7 mag G4V-type star. We detect two periodic sets of transit signals in the 3-year flux time series of Kepler-69, obtained with the Kepler spacecraft. Using the very high precision Kepler photometry, and follow-up observations, our confidence that these signals represent planetary transits is {$>$}99.3\%. The inner planet, Kepler-69b, has a radius of R{$\oplus$} and orbits the host star every 13.7 days. The outer planet, Kepler-69c, is a super-Earth-sized object with a radius of R{$\oplus$} and an orbital period of 242.5 days. Assuming an Earth-like Bond albedo, Kepler-69c has an equilibrium temperature of 299 {$\pm$} 19 K, which places the planet close to the habitable zone around the host star. This is the smallest planet found by Kepler to be orbiting in or near the habitable zone of a Sun-like star and represents an important step on the path to finding the first true Earth analog. \textcopyright{} 2013. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,planetary systems,stars: fundamental parameters,{stars: individual (Kepler-69, KIC 8692861, KOI-172},stars: statistics,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/LFJNHU7W/Barclay et al. - 2013.pdf}
}

@article{Barclay2013a,
  title = {A Sub-{{Mercury-sized}} Exoplanet},
  author = {Barclay, Thomas and Rowe, Jason F. and Lissauer, Jack J. and Huber, Daniel and Fressin, Fran{\c c}ois and Howell, Steve B. and Bryson, Stephen T. and Chaplin, William J. and D{\'e}sert, Jean Michel and Lopez, Eric D. and Marcy, Geoffrey W. and Mullally, Fergal and Ragozzine, Darin and Torres, Guillermo and Adams, Elisabeth R. and Agol, Eric and Barrado, David and Basu, Sarbani and Bedding, Timothy R. and Buchhave, Lars A. and Charbonneau, David and Christiansen, Jessie L. and {Christensen-Dalsgaard}, J{\o}rgen and Ciardi, David and Cochran, William D. and Dupree, Andrea K. and Elsworth, Yvonne and Everett, Mark and Fischer, Debra A. and Ford, Eric B. and Fortney, Jonathan J. and Geary, John C. and Haas, Michael R. and Handberg, Rasmus and Hekker, Saskia and Henze, Christopher E. and Horch, Elliott and Howard, Andrew W. and Hunter, Roger C. and Isaacson, Howard and Jenkins, Jon M. and Karoff, Christoffer and Kawaler, Steven D. and Kjeldsen, Hans and Klaus, Todd C. and Latham, David W. and Li, Jie and {Lillo-Box}, Jorge and Lund, Mikkel N. and Lundkvist, Mia and Metcalfe, Travis S. and Miglio, Andrea and Morris, Robert L. and Quintana, Elisa V. and Stello, Dennis and Smith, Jeffrey C. and Still, Martin and Thompson, Susan E.},
  year = {2013},
  journal = {Nature},
  volume = {494},
  number = {7438},
  pages = {452--454},
  issn = {14764687},
  doi = {10.1038/nature11914},
  abstract = {Since the discovery of the first exoplanets, it has been known that other planetary systems can look quite unlike our own. Until fairly recently, we have been able to probe only the upper range of the planet size distribution, and, since last year, to detect planets that are the size of Earth or somewhat smaller. Hitherto, no planets have been found that are smaller than those we see in the Solar System. Here we report a planet significantly smaller than Mercury. This tiny planet is the innermost of three that orbit the Sun-like host star, which we have designated Kepler-37. Owing to its extremely small size, similar to that of the Moon, and highly irradiated surface, the planet, Kepler-37b, is probably rocky with no atmosphere or water, similar to Mercury. \textcopyright{} 2013 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AKNPLDAB/Barclay et al. - 2013(2).pdf}
}

@article{barclayCatalogStarsObserved2018,
  title = {A Catalog of Stars Observed Simultaneously by {{Kepler}} and {{TESS}}},
  author = {Barclay, Thomas and Barentsen, Geert},
  year = {2018},
  eprint = {1810.08835v1},
  doi = {10.6084/m9.figshare.7227260.v1},
  urldate = {2021-08-15},
  abstract = {The Kepler spacecraft provided the first long-baseline, high-precision photometry for large numbers of stars (Borucki et al.},
  archiveprefix = {arxiv},
  keywords = {catalogs,notion,notion-database,surveys},
  file = {/Users/lbugnet/Zotero/storage/SUHBCIQM/full-text.pdf}
}

@article{Barker2009,
  title = {On the Tidal Evolution of {{Hot Jupiters}} on Inclined Orbits},
  author = {Barker, Adrian J. and Ogilvie, Gordon I.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {395},
  number = {4},
  pages = {2268--2287},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.14694.x},
  abstract = {Tidal friction is thought to be important in determining the long-term spin-orbit evolution of short-period extrasolar planetary systems. Using a simple model of the orbit-averaged effects of tidal friction, we study the evolution of close-in planets on inclined orbits, due to tides. We analyse the effects of the inclusion of stellar magnetic braking by performing a phase-plane analysis of a simplified system of equations, including the braking torque. The inclusion of magnetic braking is found to be important, and its neglect can result in a very different system history. We then present the results of numerical integrations of the tidal evolution equations, where we find that it is essential to consider coupled evolution of the orbital and rotational elements, including dissipation in both the star and planet, to accurately model the evolution. The main result of our integrations is that for typical Hot Jupiters, tidal friction aligns the stellar spin with the orbit on a similar time as it causes the orbit to decay. This tells us that if a planet is observed to be aligned, then it probably formed coplanar. This reinforces the importance of Rossiter-McLaughlin effect observations in determining the degree of spin-orbit alignment in transiting systems. We apply these results to the only observed system with a spin-orbit misalignment, XO-3, and constrain the efficiency of tidal dissipation (i.e. the modified tidal quality factors Q{${'}$}) in both the star and the planet in this system. Using a model in which inertial waves are excited by tidal forcing in the outer convective envelope and dissipated by turbulent viscosity, we calculate Q{${'}$} for a range of F-star models, and find it to vary considerably within this class of stars. This means that using a single Q{${'}$}, and assuming that it applies to all stars, is probably incorrect. In addition, we propose an explanation for the survival of two of the planets on the tightest orbits, WASP-12 b and OGLE-TR-56 b, in terms of weak dissipation in the star, as a result of their internal structures and slow rotation periods. \textcopyright{} 2009 RAS.},
  keywords = {Binaries: close,Celestial mechanics,notion,notion-database,Planetary systems,Stars: individual: XO-3,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/7VPT7QZ9/Barker, Ogilvie - 2009.pdf}
}

@article{Barker2014,
  title = {{{THEORY AND SIMULATIONS OF ROTATING CONVECTION}}},
  author = {Barker, Adrian J and Dempsey, Adam M and Lithwick, Yoram},
  year = {2014},
  journal = {The Astrophysical Journal},
  volume = {791},
  number = {13},
  doi = {10.1088/0004-637X/791/1/13},
  urldate = {2022-01-26},
  abstract = {We study thermal convection in a rotating fluid in order to better understand the properties of convection zones in rotating stars and planets. We first derive a mixing-length theory for rapidly rotating convection, arriving at the results of Stevenson via simple physical arguments. The theory predicts the properties of convection as a function of the imposed heat flux and rotation rate, independent of microscopic diffusivities. In particular, it predicts the mean temperature gradient, the rms velocity and temperature fluctuations, and the size of the eddies that dominate heat transport. We test all of these predictions with high resolution three-dimensional hydrodynamical simulations of Boussinesq convection in a Cartesian box. The results agree remarkably well with the theory across more than two orders of magnitude in rotation rate. For example, the temperature gradient is predicted to scale as the rotation rate to the four-fifths power at fixed flux, and the simulations yield 0.75 {$\pm$} 0.06. We conclude that the mixing-length theory is a solid foundation for understanding the properties of convection zones in rotating stars and planets.},
  keywords = {convection-hydrodynamics-stars,interiors-stars,notion,notion-database,rotation-turbulence}
}

@article{Barker2019,
  title = {Angular Momentum Transport by the {{GSF}} Instability: Non-Linear Simulations at the Equator},
  author = {Barker, A J and Jones, C A and Tobias, S M},
  year = {2019},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {487},
  number = {2},
  eprint = {1905.06962},
  pages = {1777--1794},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz1386},
  urldate = {2020-07-05},
  abstract = {We present an investigation into the nonlinear evolution of the Goldreich-Schubert-Fricke (GSF) instability using axisymmetric and three-dimensional simulations near the equator of a differentially rotating radiation zone. This instability may provide an important contribution to angular momentum transport in stars and planets. We adopt a local Boussinesq Cartesian shearing box model, which represents a small patch of a differentially rotating stellar radiation zone. Complementary simulations are also performed with stress-free, impenetrable boundaries in the local radial direction. The linear and nonlinear evolution of the equatorial axisymmetric instability is formally equivalent to the salt fingering instability. This is no longer the case in 3D, but we find that the instability behaves nonlinearly in a similar way to salt fingering. Axisymmetric simulations -- and those in 3D with short dimensions along the local azimuthal direction -- quickly develop strong jets along the rotation axis, which inhibit the instability and lead to predator-prey-like temporal dynamics. In 3D, the instability initially produces homogeneous turbulence and enhanced momentum transport, though in some cases jets form on a much longer timescale. We propose and validate numerically a simple theory for nonlinear saturation of the GSF instability and its resulting angular momentum transport. This theory is straightforward to implement in stellar evolution codes incorporating rotation. We estimate that the GSF instability could contribute towards explaining the missing angular momentum transport required in red giant stars, and play a role in the long-term evolution of the solar tachocline.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Barnes1999,
  title = {Angular {{Momentum Transport}} in {{Magnetized Stellar Radiative Zones}}. {{III}}. {{The Solar Light}}-{{Element Abundances}}},
  author = {Barnes, G. and Charbonneau, P. and MacGregor, K. B.},
  year = {1999},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {511},
  number = {1},
  pages = {466--480},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/306639},
  urldate = {2020-06-19},
  abstract = {We calculate the depletion of the trace elements lithium and beryllium within a solar-mass star during the course of its evolution from the zero-age main sequence to the age of the present-day Sun. In the radiative layers beneath the convection zone, we assume that these elements are transported by the turbulent fluid motions that result from instability of the shear flow associated with internal differential rotation. This turbulent mixing is modeled as a diffusion process, using a diffusion coefficient that is taken to be proportional to the gradient of the angular velocity distribution inside the star. We study the evolution of the light-element abundances produced by rotational mixing for models in which internal angular momentum redistribution takes place either by hydrodynamic or by hydromagnetic means. Since models based on these alternative mechanisms for angular-momentum transport predict similar surface rotation rates late in the evolution, we explore the extent to which light-element abundances make it possible to distinguish between them. In the case of an internally magnetized star, our computations indicate that both the details of the surface abundance evolution and the magnitude of the depletion at solar age can depend sensitively on the assumed strength and configuration of the poloidal magnetic field inside the star. For a configuration with no direct magnetic coupling between the radiative and convective portions of the stellar interior, the depletion of lithium calibrated to the solar lithium depletion at the solar age is similar at all ages to the lithium depletion of a model in which angular-momentum transport occurs solely by hydrodynamical processes. However, the two models can be distinguished on the basis of their respective beryllium depletions, with the depletion of the magnetic model being significantly smaller than that of the nonmagnetic model.},
  keywords = {notion,notion-database,Sun: Abundances,SUN: ABUNDANCES,Sun: Interior,SUN: INTERIOR,Sun: Magnetic Fields,SUN: MAGNETIC FIELDS,Sun: Rotation,SUN: ROTATION},
  file = {/Users/lbugnet/Zotero/storage/UN5M4VS2/full-text.pdf}
}

@article{Barnes2003,
  title = {On the {{Rotational Evolution}} of {{Solar}}- and {{Late}}-{{Type Stars}}, {{Its Magnetic Origins}}, and the {{Possibility}} of {{Stellar Gyrochronology}}},
  author = {Barnes, Sydney A.},
  year = {2003},
  journal = {The Astrophysical Journal},
  volume = {586},
  number = {1},
  eprint = {astro-ph/0303631},
  pages = {464--479},
  issn = {0004-637X},
  doi = {10.1086/367639},
  abstract = {We propose a simple interpretation of the rotation period data for solar- and late-type stars. The open cluster and Mt. Wilson star observations suggest that rotating stars lie primarily on two sequences, initially called I and C. Some stars lie in the intervening gap. These sequences, and the fractional numbers of stars on each sequence evolve systematically with cluster age, enabling us to construct crude rotational isochrones allowing `stellar gyrochronology', a procedure, upon improvement, likely to yield ages for individual field stars. The age and color dependences of the sequences allow the identification of the underlying mechanism, which appears to be primarily magnetic. The majority of solar- and late-type stars possess a dominant Sun-like, or Interface magnetic field, which connects the convective envelope both to the radiative interior of the star and to the exterior where winds can drain off angular momentum. These stars spin down Skumanich-style. An age-decreasing fraction of young G, K, and M stars, which are rapid rotators, possess only a Convective field which is not only inefficient in depleting angular momentum, but also incapable of coupling the surface convection zone to the inner radiative zone, so that only the outer zone is spun down, and on an exponential timescale. These stars do not yet possess large-scale dynamos. The large-scale magnetic field associated with the dynamo, apparently created by the shear between the decoupled radiative and convective zones, (re)couples the convective and radiative zones and drives a star from the Convective to the Interface sequence through the gap on a timescale that increases as stellar mass decreases. (Abstract is truncated here.)},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HK9HTUNC/Barnes - 2003.pdf}
}

@article{Barnes2005,
  title = {Cosmic {{Abundances}} as {{Records}} of {{Stellar Evolution}} and {{Nucleosynthesis}}},
  author = {Barnes, Thomas G and Bash, Frank N and Asplund, Martin and Grevesse, Nicolas and Sauval, A Jacques},
  year = {2005},
  journal = {Lambert ASP Conference Series},
  volume = {336},
  pages = {25--38},
  abstract = {We review our current knowledge of the solar chemical composition as determined from photospheric absorption lines. In particular we describe the recent significant revisions of the solar abundances as a result of the application of a time-dependent, 3D hydrodynamical model of the solar atmosphere instead of 1D hydrostatic models. This has decreased the metal content in the solar convection zone by almost a factor of two compared with the widely used compilation by Anders \& Grevesse (1989). While resolving a number of long-standings problems, the new 3D-based element abundances also pose serious challenges, most notably for helioseismology.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LPX5G9E4/Barnes et al. - 2005.pdf}
}

@article{Barnes2007,
  title = {Ages for {{Illustrative Field Stars Using Gyrochronology}}: {{Viability}}, {{Limitations}}, and {{Errors}}},
  author = {Barnes, Sydney A.},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {669},
  number = {2},
  eprint = {0704.3068},
  pages = {1167--1189},
  issn = {0004-637X},
  doi = {10.1086/519295},
  abstract = {We here develop an improved way of using a rotating star as a clock, set it using the Sun, and demonstrate that it keeps time well. This technique, called gyrochronology, permits the derivation of ages for solar- and late-type main sequence stars using only their rotation periods and colors. The technique is clarified and developed here, and used to derive ages for illustrative groups of nearby, late-type field stars with measured rotation periods. We first demonstrate the reality of the interface sequence, the unifying feature of the rotational observations of cluster and field stars that makes the technique possible, and extends it beyond the proposal of Skumanich by specifying the mass dependence of rotation for these stars. We delineate which stars it cannot currently be used on. We then calibrate the age dependence using the Sun. The errors are propagated to understand their dependence on color and period. Representative age errors associated with the technique are estimated at \textasciitilde 15\% (plus possible systematic errors) for late-F, G, K, \& early-M stars. Ages derived via gyrochronology for the Mt. Wilson stars are shown to be in good agreement with chromospheric ages for all but the bluest stars, and probably superior. Gyro ages are then calculated for each of the active main sequence field stars studied by Strassmeier and collaborators where other ages are not available. These are shown to be mostly younger than 1Gyr, with a median age of 365Myr. The sample of single, late-type main sequence field stars assembled by Pizzolato and collaborators is then assessed, and shown to have gyro ages ranging from under 100Myr to several Gyr, and a median age of 1.2Gyr. Finally, we demonstrate that the individual components of the three wide binaries XiBooAB, 61CygAB, \& AlphaCenAB yield substantially the same gyro ages.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,Galaxy: Open Clusters and Associations: General,notion,notion-database,Stars: Activity,Stars: Evolution,Stars: Late,Stars: Magnetic Fields,Stars: Rotation,Type},
  file = {/Users/lbugnet/Zotero/storage/JBSWBWN6/Barnes - 2007.pdf;/Users/lbugnet/Zotero/storage/WJIR2E98/full-text.pdf}
}

@article{Barnes2008,
  title = {Gyrochronology and Its Usage for Main Sequence Field Star Ages},
  author = {Barnes, Sydney A.},
  year = {2008},
  journal = {Proceedings of the International Astronomical Union},
  volume = {4},
  number = {S258},
  eprint = {0906.2386},
  pages = {345--356},
  issn = {1743-9213},
  doi = {10.1017/s1743921309032001},
  abstract = {The construction of all age indicators consists of certain basic steps which lead to the identification of the properties desirable for stellar age indicators. Prior age indicators for main sequence field stars possess only some of these properties. The measured rotation periods of cool stars are particularly useful in this respect because they have well-defined dependencies that allow stellar ages to be determined with \textasciitilde 20\% errors. This method, called gyrochronology, is explained informally in this talk, shown to have the desired properties, compared to prior methods, and used to derive ages for samples of main sequence field stars.},
  archiveprefix = {arxiv},
  keywords = {36 oph,61 cyg,activity,binaries,evolution,fundamental parameters,individual,late-type,notion,notion-database,rotation,stars,{$\alpha$} cen,{$\xi$} boo},
  file = {/Users/lbugnet/Zotero/storage/8BRG9W8R/Barnes - 2008.pdf}
}

@article{Barnes2010,
  title = {A {{SIMPLE NONLINEAR MODEL FOR THE ROTATION OF MAIN-SEQUENCE COOL STARS}}. {{I}}. {{INTRODUCTION}}, {{IMPLICATIONS FOR GYROCHRONOLOGY}}, {{AND COLOR-PERIOD DIAGRAMS}}},
  author = {Barnes, Sydney A},
  year = {2010},
  journal = {The Astrophysical Journal},
  volume = {722},
  number = {1},
  pages = {222--234},
  doi = {10.1088/0004-637X/722/1/222},
  urldate = {2020-07-02},
  abstract = {We here introduce a simple nonlinear model to describe the rotational evolution of cool stars on the main sequence. It is formulated only in terms of the Rossby number (Ro = P /{$\tau$}), its inverse, and two dimensionless constants which we specify using solar and open-cluster data. The model has two limiting cases of stellar rotation, previously called C and I, that correspond to two observed sequences of fast and slowly rotating stars in young open clusters. The model describes the evolution of stars from C-type, with particular mass and age dependencies, to I-type, with different mass and age dependencies, through the rotational gap, g, separating them. The proposed model explains various aspects of stellar rotation, and provides an exact expression for the age of a rotating cool star in terms of P and {$\tau$} , thereby generalizing gyrochronology. Using it, we calculate the time interval required for stars to reach the rotational gap-a monotonically increasing, mildly nonlinear function of {$\tau$}. Beginning with the range of initial periods indicated by observations, we show that the (mass-dependent) dispersion in rotation period initially increases, and then decreases rapidly with the passage of time. The initial dispersion in period contributes up to 128 Myr to the gyro-age errors of solar-mass field stars. Finally, we transform to color-period space, calculate appropriate isochrones, and show that this model explains some detailed features in the observed color-period diagrams of open clusters, including the positions and shapes of the sequences, and the observed density of stars across these diagrams.},
  keywords = {analytical-open clusters and associations,Convection,convection-methods,evolution-stars,general-stars,late-type-stars,Methods: Analytical,notion,notion-database,Open clusters and associations: General,rotation,Stars: Evolution,Stars: Late-type,Stars: Rotation},
  file = {/Users/lbugnet/Zotero/storage/JBXITT49/full-text.pdf}
}

@article{Barnes2010a,
  title = {Angular Momentum Loss from Cool Stars: {{An}} Empirical Expression and Connection to Stellar Activity},
  author = {Barnes, Sydney A. and Kim, Yong Cheol},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {721},
  number = {1},
  eprint = {1104.2350},
  pages = {675--685},
  issn = {15384357},
  doi = {10.1088/0004-637X/721/1/675},
  abstract = {We show here that the rotation period data in open clusters allow the empirical determination of an expression for the rate of loss of angular momentum from cool stars on the main sequence. One significant component of the expression, the dependence on rotation rate, persists from prior work; others do not. The expression has a bifurcation, as before, that corresponds to an observed bifurcation in the rotation periods of coeval open cluster stars. The dual dependencies of this loss rate on stellarmass are captured by two functions, f (B-V ) and T (B-V ), that can be determined from the rotation period observations. Equivalent masses and other [UBVRIJHK] colors are provided in Table 1. Dimensional considerations and a comparison with appropriate calculated quantities suggest interpretations for f and T, both of which appear to be related closely (but differently) to the calculated convective turnover timescale, tc, in cool stars. This identification enables us to write down symmetrical expressions for the angular momentum loss rate and the deceleration of cool stars and also to revive the convective turnover timescale as a vital connection between stellar rotation and stellar activity physics. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Convection,notion,notion-database,Open clusters and associations: general,Stars: activity,Stars: evolution,Stars: late-type,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/DGIRKJI3/Barnes, Kim - 2010.pdf}
}

@article{Barrere2023,
  title = {Numerical Simulations of the {{Tayler-Spruit}} Dynamo in Proto-Magnetars},
  author = {Barr{\`e}re, Paul and Guilet, J{\'e}r{\^o}me and Raynaud, Rapha{\"e}l and {Reboul-Salze}, Alexis},
  year = {2023},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {526},
  pages = {L88-L93},
  issn = {0035-8711},
  doi = {10.1093/mnrasl/slad120},
  urldate = {2023-10-11},
  abstract = {The Tayler-Spruit dynamo is one of the most promising mechanisms proposed to explain angular momentum transport during stellar evolution. Its development in proto-neutron stars spun-up by supernova fallback has also been put forward as a scenario to explain the formation of very magnetized neutron stars called magnetars. Using three-dimensional direct numerical simulations, we model the proto-neutron star interior as a stably stratified spherical Couette flow with the outer sphere that rotates faster than the inner one. We report the existence of two subcritical dynamo branches driven by the Tayler instability. They differ by their equatorial symmetry (dipolar or hemispherical) and the magnetic field scaling, which is in agreement with different theoretical predictions (by Fuller and Spruit, respectively). The magnetic dipole of the dipolar branch is found to reach intensities compatible with observational constraints on magnetars.},
  keywords = {Astrophysics - High Energy Astrophysical Phenomena,Astrophysics - Solar and Stellar Astrophysics,instabilities,magnetic fields,MHD,Physics - Fluid Dynamics,stars: magnetars,supernovae: general},
  annotation = {ADS Bibcode: 2023MNRAS.526L..88B},
  file = {/Users/lbugnet/Zotero/storage/Y23XCASE/Barrère et al. - 2023 - Numerical simulations of the Tayler-Spruit dynamo .pdf}
}

@article{Barstow2014,
  title = {White Paper: {{Gaia}} and the End States of Stellar Evolution},
  author = {Barstow, M. A and Casewell, S. L. and Catalan, S. and Copperwheat, C. and Gaensicke, B. and {Garcia-Berro}, E. and Hambly, N. and Heber, U. and Holberg, J. and Isern, J. and Jeffery, S. and Jordan, S. and Lawrie, K. A. and {Lynas-Gray}, A. E. and Maccarone, T. and Marsh, T. and Parsons, S. and Silvotti, R. and Subasavage, J. and Torres, S. and Wheatley, P.},
  year = {2014},
  month = jul,
  eprint = {1407.6163},
  urldate = {2020-03-06},
  abstract = {This is the product of a Gaia GREAT workshop on "Gaia and the end states of stellar evolution" held at the University of Leicester in April 2011.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/B8E53DSP/full-text.pdf}
}

@article{Basri2005,
  title = {The {{Kepler Mission}}: {{A}} Wide-Field Transit Search for Terrestrial Planets},
  author = {Basri, Gibor and Borucki, William J. and Koch, David},
  year = {2005},
  journal = {New Astronomy Reviews},
  volume = {49},
  number = {7-9},
  pages = {478--485},
  issn = {13876473},
  doi = {10.1016/j.newar.2005.08.026},
  abstract = {The Kepler Mission is a NASA Discovery mission which will continuously monitor the brightness of at least 100,000 main sequence stars, to detect the transits of terrestrial and larger planets. It is scheduled to be launched in 2007 into an Earth-trailing heliocentric orbit. It is a wide-field photometer with a Schmidt-type telescope and array of 42 CCDs covering the 100 square degree field-of-view. It has a 1-m aperture which enables a differential photometric precision of 2 parts in 100,000 for 12th magnitude solar-like stars over a 6.5-hour transit duration. It will continuously observe dwarf stars from 8th to 15th magnitude in the Cygnus constellation, for a period of four years, with a cadence of 4 measurements per hour. Hundreds of terrestrial planets should be detected if they are common around solar-type stars. Ground-based spectrometry of stars with planetary candidates will help eliminate false-positives, and determine stellar characteristics such as mass and metallicity. A null result would imply that terrestrial planets are rare. \textcopyright{} 2005 Published by Elsevier B.V.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/T5BXE6VP/Basri, Borucki, Koch - 2005.pdf}
}

@article{Basri2010a,
  title = {Photometric Variability in Kepler Target Stars: {{The}} Sun among Stars - {{A}} First Look},
  author = {Basri, Gibor and Walkowicz, Lucianne M. and Batalha, Natalie and Gilliland, Ronald L. and Jenkins, Jon and Borucki, William J. and Koch, David and Caldwell, Doug and Dupree, Andrea K. and Latham, David W. and Meibom, S{\o}ren and Howell, Steve and Brown, Tim},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0414},
  pages = {1--13},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L155},
  abstract = {The Kepler mission provides an exciting opportunity to study the light curves of stars with unprecedented precision and continuity of coverage. This is the first look at a large sample of stars with photometric data of a quality that has heretofore been only available for our Sun. It provides the first opportunity to compare the irradiance variations of our Sun to a large cohort of stars ranging from very similar to rather different stellar properties, at a wide variety of ages. Although Kepler data are in an early phase of maturity, and we only analyze the first month of coverage, it is sufficient to garner the first meaningful measurements of our Sun's variability in the context of a large cohort of main-sequence stars in the solar neighborhood. We find that nearly half of the full sample is more active than the active Sun, although most of them are not more than twice as active. The active fraction is closer to a third for the stars most similar to the Sun, and rises to well more than half for stars cooler than mid-K spectral types. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: statistics,Starspots},
  file = {/Users/lbugnet/Zotero/storage/CTT8VL34/Basri et al. - 2010.pdf}
}

@article{Basri2011,
  title = {Photometric Variability in {{Kepler}} Target Stars. {{II}}. {{An}} Overview of Amplitude, Periodicity, and Rotation in First Quarter Data},
  author = {Basri, Gibor and Walkowicz, Lucianne M. and Batalha, Natalie and Gilliland, Ronald L. and Jenkins, Jon and Borucki, William J. and Koch, David and Caldwell, Doug and Dupree, Andrea K. and Latham, David W. and Marcy, Geoffrey W. and Meibom, Soeren and Brown, Tim},
  year = {2011},
  journal = {Astronomical Journal},
  volume = {141},
  number = {1},
  eprint = {1008.1092},
  pages = {1--21},
  issn = {00046256},
  doi = {10.1088/0004-6256/141/1/20},
  abstract = {We provide an overview of stellar variability in the first quarter data from the Kepler mission. The intent of this paper is to examine the entire sample of over 150,000 target stars for periodic behavior in their light curves and relate this to stellar characteristics. This data set constitutes an unprecedented study of stellar variability given its great precision and complete time coverage (with a half hour cadence). Because the full Kepler pipeline is not currently suitable for a study of stellar variability of this sort, we describe our procedures for treating the "raw" pipeline data. About half of the total sample exhibits convincing periodic variability up to two weeks, with amplitudes ranging from differential intensity changes of less than 10-4 up to more than 10\%. K and M dwarfs have a greater fraction of period behavior than G dwarfs. The giants in the sample have distinctive quasi-periodic behavior, but are not periodic in the way we define it. Not all periodicities are due to rotation, and the most significant period is not necessarily the rotation period. We discuss properties of the light curves, and in particular look at a sample of very clearly periodic G dwarfs. It is clear that a large number of them do vary because of rotation and starspots, but it will take further analysis to fully exploit this. \textcopyright{} 2011 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: rotation,Stars: solar-type,Stars: statistics,Stars: variables: general,Starspots},
  file = {/Users/lbugnet/Zotero/storage/JLHP55YL/Basri et al. - 2011.pdf}
}

@article{Basri2013,
  title = {Comparison of Kepler Photometric Variability with the Sun on Different Timescales},
  author = {Basri, Gibor and Walkowicz, Lucianne M. and Reiners, Ansgar},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {769},
  number = {1},
  eprint = {1304.0136},
  pages = {1--45},
  issn = {15384357},
  doi = {10.1088/0004-637X/769/1/37},
  abstract = {We utilize Kepler data to study the precision differential photometric variability of solar-type and cooler stars at different timescales, ranging from half an hour to three months. We define a diagnostic that characterizes the median differential intensity change between data bins of a given timescale. We apply the same diagnostics to Solar and Heliospheric Observatory data that has been rendered comparable to Kepler. The Sun exhibits similar photometric variability on all timescales as comparable solar-type stars in the Kepler field. The previously defined photometric "range" serves as our activity proxy (driven by starspot coverage). We revisit the fraction of comparable stars in the Kepler field that are more active than the Sun. The exact active fraction depends on what is meant by "more active than the Sun" and on the magnitude limit of the sample of stars considered. This active fraction is between a quarter and a third (depending on the timescale). We argue that a reliable result requires timescales of half a day or longer and stars brighter than MKep of 14, otherwise non-stellar noise distorts it. We also analyze main sequence stars grouped by temperature from 6500 to 3500 K. As one moves to cooler stars, the active fraction of stars becomes steadily larger (greater than 90\% for early M dwarfs). The Sun is a good photometric model at all timescales for those cooler stars that have long-term variability within the span of solar variability. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: activity,stars: late-type,stars: solar-type,stars: variables: general,Sun: activity},
  file = {/Users/lbugnet/Zotero/storage/YRL7NIW3/Basri, Walkowicz, Reiners - 2013.pdf}
}

@article{Basri2018,
  title = {Double {{Dipping}}: {{A New Relation}} between {{Stellar Rotation}} and {{Starspot Activity}}},
  author = {Basri, Gibor and Nguyen, Hieu T.},
  year = {2018},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {863},
  number = {2},
  eprint = {1805.04587},
  pages = {190},
  publisher = {{American Astronomical Society}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aad3b6},
  urldate = {2020-07-02},
  abstract = {We report the discovery of a new relationship between a simple morphological characteristic of light curves produced by starspots and stellar rotation periods. The characteristic we examine is whether the light curve exhibits one dip or two during a single rotation. We analyze thousands of Kepler light curves of main sequence stars from 3200-6200K. Almost all the stars exhibit segments of their light curve that contain either single or double dip segments (very few have more than two significant dips per rotation). We define a variable, the "single/double ratio" (SDR) that expresses the ratio of the time spent in single mode to the time spent in double mode. Unexpectedly, there is a strong relationship between the SDR and the stellar rotation period, in the sense that longer periods come with a larger fraction of double segments. Even more unexpectedly, the slopes of the SDR-Period relations are a clear function of stellar temperature. We also show that the relationships of spot variability amplitude (R\_var) to rotation period have similar levels of scatter, slopes, and dependence on temperature as the SDR-Period relations. Finally, the median R\_var of single segments tends to be about twice that of double segments in a given light curve. We offer some tentative interpretations of these new results in terms of starspot coverage and lifetimes. It will be fruitful to look further into this novel "rotation-activity" relation, and better understand what information these aspects of light curve morphology bring to our knowledge of stellar magnetic activity.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VTA9A64G/full-text.pdf}
}

@article{Bass2016,
  title = {Supervised {{Ensemble Classification}} of {{Kepler Variable Stars}}},
  author = {Bass, Gideon and Borne, Kirk},
  year = {2016},
  month = apr,
  eprint = {1604.01355},
  doi = {10.1093/mnras/stw810},
  urldate = {2020-04-09},
  abstract = {Variable star analysis and classification is an important task in the understanding of stellar features and processes. While historically classifications have been done manually by highly skilled experts, the recent and rapid expansion in the quantity and quality of data has demanded new techniques, most notably automatic classification through supervised machine learning. We present an expansion of existing work on the field by analyzing variable stars in the \{\textbackslash em Kepler\} field using an ensemble approach, combining multiple characterization and classification techniques to produce improved classification rates. Classifications for each of the roughly 150,000 stars observed by \{\textbackslash em Kepler\} are produced separating the stars into one of 14 variable star classes.},
  archiveprefix = {arxiv},
  keywords = {(),notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2IZKFVXC/full-text.pdf}
}

@article{Bastien2013,
  title = {An Observational Correlation between Stellar Brightness Variations and Surface Gravity},
  author = {Bastien, Fabienne A. and Stassun, Keivan G. and Basri, Gibor and Pepper, Joshua},
  year = {2013},
  month = aug,
  journal = {Nature},
  volume = {500},
  number = {7463},
  eprint = {1308.4728},
  pages = {427--430},
  doi = {10.1038/nature12419},
  urldate = {2020-03-16},
  abstract = {Surface gravity is one of a star's basic properties, but it is difficult to measure accurately, with typical uncertainties of 25-50 per cent if measured spectroscopically and 90-150 per cent photometrically. Asteroseismology measures gravity with an uncertainty of about two per cent but is restricted to relatively small samples of bright stars, most of which are giants. The availability of high-precision measurements of brightness variations for {$>$}150,000 stars provides an opportunity to investigate whether the variations can be used to determine surface gravities. The Fourier power of granulation on a star's surface correlates physically with surface gravity; if brightness variations on timescales of hours arise from granulation, then such variations should correlate with surface gravity. Here we report an analysis of archival data that reveals an observational correlation between surface gravity and the root-mean-square brightness variations on timescales of less than eight hours for stars with temperatures of 4500-6750K, log of surface gravities of 2.5-4.5 (cgs units), and having overall brightness variations {$<$}3 parts per thousand. A straightforward observation of optical brightness variations therefore allows a determination of the surface gravity with a precision of {$<$}25 percent for inactive Sun-like stars at main-sequence to giant stages of evolution.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/5B2V464J/full-text.pdf}
}

@article{Bastien2016,
  title = {A {{Granulation}} ``{{Flicker}}''-{{Based Measure}} of {{Stellar Surface Gravity}}},
  author = {Bastien, Fabienne A. and Stassun, Keivan G. and Basri, Gibor and Pepper, Joshua},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {818},
  number = {1},
  eprint = {1512.03454},
  pages = {43},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/818/1/43},
  abstract = {In Bastien et al. (2013) we found that high quality light curves, such as those obtained by Kepler, may be used to measure stellar surface gravity via granulation-driven light curve "flicker". Here, we update and extend the relation originally presented in Bastien et al. (2013) after calibrating flicker against a more robust set of asteroseismically derived surface gravities. We describe in detail how we extract the flicker signal from the light curves, including how we treat phenomena, such as exoplanet transits and shot noise, that adversely affect the measurement of flicker. We examine the limitations of the technique, and, as a result, we now provide an updated treatment of the flicker-based logg error. We briefly highlight further applications of the technique, such as astrodensity profiling or its use in other types of stars with convective outer layers. We discuss potential uses in current and upcoming space-based photometric missions. Finally, we supply flicker-based logg values, and their uncertainties, for 27 628 Kepler stars not identified as transiting-planet hosts, with 4500},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics,stars: fundamental parameters,stars: general,stars: solar,techniques: photometric,type},
  file = {/Users/lbugnet/Zotero/storage/5F5GYP8T/full-text.pdf;/Users/lbugnet/Zotero/storage/SJWMF5QZ/Bastien et al. - 2016.pdf}
}

@article{Basu1997,
  title = {Seismology of the Base of the Solar Convection Zone - {{NASA}}/{{ADS}}},
  author = {{Basu}},
  year = {1997},
  journal = {MNRAS},
  volume = {288},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RHNVM957/Basu - 1997.pdf}
}

@article{Basu2000,
  title = {Structure of the {{Solar Core}}: {{Effect}} of {{Asymmetry}} of {{Peak Profiles}}},
  author = {Basu, S. and Turck-Chieze, S. and Berthomieu, G. and Brun, A. S. and Corbard, T. and Gonczi, G. and Christensen-Dalsgaard, J. and Provost, J. and Thiery, S. and Gabriel, A. H. and Boumier, P.},
  year = {2000},
  journal = {The Astrophysical Journal},
  volume = {535},
  number = {2},
  eprint = {astro-ph/0001208},
  pages = {1078--1084},
  issn = {0004-637X},
  doi = {10.1086/308875},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IPWUPJRN/Basu et al. - 2000.pdf}
}

@article{Basu2003,
  title = {Temporal Variations in the Rotation Rate in the Solar Interior},
  author = {Basu, Sarbani and Antia, H. M.},
  year = {2003},
  journal = {European Space Agency, (Special Publication) ESA SP},
  number = {517},
  eprint = {astro-ph/0004335},
  pages = {235--238},
  issn = {03796566},
  doi = {10.1086/309421},
  abstract = {The frequency splittings obtained from GONG and MDI observations over the last 7 years are used to study how the rotation rate of the solar convection zone has evolved with time. The bands of faster and slower than average rotation rate are found to move towards the equator at low latitudes, while at high latitudes they move towards the poles. The low latitude bands also move upwards with time, and they extend almost to the base of the convection zone. We find no significant temporal variation in the rotation rate in the tachocline region.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: interior,Sun: oscillations,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/83EG7Y6C/Basu, Antia - 2003.pdf}
}

@article{Basu2007,
  title = {Solar {{Abundances}} and {{Helioseismology}}: {{Fine}}-{{Structure Spacings}} and {{Separation Ratios}} of {{Low}}-{{Degree}} p -{{Modes}}},
  author = {Basu, Sarbani and Chaplin, William J. and Elsworth, Yvonne and New, Roger and Serenelli, Aldo M. and Verner, Graham A.},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {655},
  number = {1},
  eprint = {astro-ph/0610052},
  pages = {660--671},
  issn = {0004-637X},
  doi = {10.1086/509820},
  abstract = {We have used 4752 days of data collected by the Birmingham Solar-Oscillations Network (BiSON) to determine very precise oscillation frequencies of acoustic low-degree modes that probe the solar core. We compare the fine (small frequency) spacings and frequency separation ratios formed from these data with those of different solar models. We find that models constructed with low metallicity are incompatible with the observations. The results provide strong support for lowering the theoretical uncertainties on the neutrino fluxes. These uncertainties had recently been raised due to the controversy over the solar abundances.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KJWD86GL/Basu et al. - 2007.pdf}
}

@article{Basu2009,
  title = {Fresh Insights on the Structure of the Solar Core},
  author = {Basu, Sarbani and Chaplin, William J. and Elsworth, Yvonne and New, Roger and Serenelli, Aldo M.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {699},
  number = {2},
  eprint = {0905.0651},
  pages = {1403--1417},
  issn = {15384357},
  doi = {10.1088/0004-637X/699/2/1403},
  abstract = {We present new results on the structure of the solar core, obtained with new sets of frequencies of solar low-degree p modes obtained from the BiSON network. We find that different methods used in extracting the different sets of frequencies cause shifts in frequencies, but the shifts are not large enough to affect solar structure results. We find that the BiSON frequencies show that the solar sound speed in the core is slightly larger than that inferred from data from Michelson Doppler Imager low-degree modes, and the uncertainties on the inversion results are smaller. Density results also change by a larger amount, and we find that solar models now tend to show smaller differences in density compared to the Sun. The result is seen at all radii, a result of the fact that conservation of mass implies that density differences in one region have to cancel out density differences in others, since our models are constructed to have the same mass as the Sun. The uncertainties on the density results are much smaller too. We attribute the change in results to having more, and lower frequency, low-degree mode frequencies available. These modes provide greater sensitivity to conditions in the core. \textcopyright{} 2009. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: abundances,Sun: helioseismology,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/HJXWZZ88/Basu et al. - 2009.pdf}
}

@article{Basu2010,
  title = {Determination of Stellar Radii from Asteroseismic Data},
  author = {Basu, Sarbani and Chaplin, William J. and Elsworth, Yvonne},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {710},
  number = {2},
  eprint = {0909.0506},
  pages = {1596--1609},
  issn = {15384357},
  doi = {10.1088/0004-637X/710/2/1596},
  abstract = {The NASA Kepler mission is designed to find planets through transits. Accurate and precise radii of the detected planets depend on knowing the radius of the host star accurately, which is difficult unless the temperature and luminosity of the star are known precisely. Kepler, however, has an asteroseismology program that will provide seismic variables that can characterize stellar radii easily, accurately, and extremely precisely. In this paper, we describe the Yale-Birmingham (YB) method to determine stellar radii using a combination of seismic and conventional variables and analyze the effect of these variables on the result. We find that for main-sequence stars, a knowledge of the parallax is not important to get accurate radii using the YB method: we can get results to an accuracy and precision of better than a few percent if we know the effective temperature and the seismic parameters for these stars. Metallicity does not make much difference either. However, good estimates of the effective temperature and metallicity, along with those of the seismic parameters, are essential to determine radii of subgiants properly. On the other hand, for red giants we find that determining radii properly is not possible without a good estimate of the parallax. We find that the so-called "surface term" in the seismic data has minimal effect on the inferred radii. Uncertainties in the convective mixing length can matter under some circumstances and can cause a systematic shift in the inferred radii. Blind tests with data simulated to match those expected from the asteroseismic survey phase of Kepler show that it will be possible to infer stellar radii successfully using our method. \textcopyright{} 2010. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/62WXU2DM/Basu, Chaplin, Elsworth - 2010.pdf}
}

@article{Basu2011,
  title = {Sounding Open Clusters: {{Asteroseismic}} Constraints from Kepler on the Properties of {{NGC6791}} and {{NGC6819}}},
  author = {Basu, Sarbani and Grundahl, Frank and Stello, Dennis and Kallinger, Thomas and Hekker, Saskia and Mosser, Benoit and Garc{\'i}a, Rafael A. and Mathur, Savita and Brogaard, Karsten and Bruntt, Hans and Chaplin, William J. and Gai, Ning and Elsworth, Yvonne and Esch, Lisa and Ballot, Jerome and Bedding, Timothy R. and Gruberbauer, Michael and Huber, Daniel and Miglio, Andrea and Yildiz, Mutlu and Kjeldsen, Hans and {Christensen-Dalsgaard}, J{\o}rgen and Gilliland, Ronald L. and Fanelli, Michael M. and Ibrahim, Khadeejah A. and Smith, Jeffrey C.},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {729},
  number = {1 PART II},
  issn = {20418213},
  doi = {10.1088/2041-8205/729/1/L10},
  abstract = {We present initial results on some of the properties of open clusters NGC6791 and NGC6819 derived from asteroseismic data obtained by NASA's Kepler mission. In addition to estimating the mass, radius, and log g of stars on the red giant branch (RGB) of these clusters, we estimate the distance to the clusters and their ages. Our model-independent estimate of the distance modulus of NGC6791 is (m - M)0 = 13.11 0.06. We find (m - M)0 = 11.85 0.05 for NGC6819. The average mass of stars on the RGB of NGC6791 is 1.20 0.01 M, while that of NGC6819 is 1.68 0.03 M. It should be noted that we do not have data that cover the entire RGB and the actual mass will be somewhat lower. We have determined model-dependent estimates of ages of these clusters. We find ages between 6.8 and 8.6 Gyr for NGC6791, however, most sets of models give ages around 7 Gyr. We obtain ages between 2 and 2.4 Gyr for NGC6819. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,open clusters and associations: individual (NGC 68,stars: fundamental parameters,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ECNNLX6R/Basu et al. - 2011.pdf}
}

@article{Basu2012,
  title = {Thinning of the {{Sun}}'s Magnetic Layer: {{The}} Peculiar Solar Minimum Could Have Been Predicted},
  author = {Basu, Sarbani and Broomhall, Anne Marie and Chaplin, William J. and Elsworth, Yvonne},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {758},
  number = {1},
  eprint = {1208.5493},
  pages = {1--15},
  issn = {15384357},
  doi = {10.1088/0004-637X/758/1/43},
  abstract = {The solar magnetic activity cycle causes changes in the Sun on timescales that are equivalent to human lifetimes. The minimum solar activity that preceded the current solar cycle (cycle 24) was deeper and quieter than any other recent minimum. Using data from the Birmingham Solar Oscillations Network (BiSON), we show that the structure of the solar sub-surface layers during the descending phase of the preceding cycle (cycle 23) was very different from that during cycle 22. This leads us to believe that a detailed examination of the data would have led to the prediction that the cycle 24 minimum would be out of the ordinary. The behavior of the oscillation frequencies allows us to infer that changes in the Sun that affected the oscillation frequencies in cycle 23 were localized mainly to layers above about 0.996R{$\odot$}, depths shallower than about 3000km. In cycle 22, on the other hand, the changes must have also occurred in the deeper-lying layers. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/UKJ8D2MK/Basu et al. - 2012.pdf}
}

@book{basuAsteroseismicDataAnalysis2017,
  title = {Asteroseismic Data Analysis : Foundations and Techniques},
  author = {Basu, Sarbani and Chaplin, William J.},
  year = {2017},
  urldate = {2021-09-01},
  abstract = {Includes index. Studies of stars and stellar populations, and the discovery and characterization of exoplanets, are being revolutionized by new satellite and telescope observations of unprecedented quality and scope. Some of the most significant advances have been in the field of asteroseismology, the study of stars by observation of their oscillations. Asteroseismic Data Analysis gives a comprehensive technical introduction to this discipline. This book not only helps students and researchers learn about asteroseismology; it also serves as an essential instruction manual for those entering the field. The book presents readers with the foundational techniques used in the analysis and interpretation of asteroseismic data on cool stars that show solar-like oscillations. The techniques have been refined, and in some cases developed, to analyze asteroseismic data collected by the NASA Kepler mission. Topics range from the analysis of time-series observations to extract seismic data for stars to the use of those data to determine global and internal properties of the stars. Reading lists and problem sets are provided, and data necessary for the problem sets are available online. The first book to describe in detail the different techniques used to analyze the data on stellar oscillations, Asteroseismic Data Analysis offers an invaluable window into the hearts of stars. Introduces the asteroseismic study of stars and the theory of stellar oscillationsDescribes the analysis of observational (time-domain) dataExamines how seismic parameters are extracted from observationsExplores how stellar properties are determined from seismic dataLooks at the "inverse problem," where frequencies are used to infer internal structures of stars Cover; Title; Copyright; Contents; Preface and Acknowledgments; 1 Introduction; 1.1 The Different Types of Pulsators; 1.2 A Brief History of the Study of Solar-Type Oscillations; 1.3 Overview of the Data; 1.4 Scope of This Book; 1.5 Further Reading; 1.6 Exercises; 2 Theoretical Underpinnings: Modeling Stars; 2.1 The Equations of Stellar Structure and Evolution; 2.2 The Question of {$\nabla$}; 2.3 Other Physical Processes; 2.4 Boundary Conditions; 2.5 Inputs to Stellar Models; 2.6 Modeling a Star; 2.7 Constructing Solar Models; 2.8 Constructing Stellar Models of a Given Mass, Radius, and Teff 2.9 Further Reading2.10 Exercises; 3 Theoretical Underpinnings: Stellar Oscillations; 3.1 The Equations of Stellar Oscillations; 3.2 Properties of Stellar Oscillations; 3.3 Changes in Frequencies in Response to Changes in Stellar Structure; 3.4 The Effects of Acoustic Glitches; 3.5 The Effects of Rotation; 3.6 Mode Excitation; 3.7 Further Reading; 3.8 Exercises; 4 Observational Data: Overview and Fundamentals; 4.1 Spatial Response of the Observations; 4.2 Photometric and Doppler Velocity Observations; 4.3 Other Contributions to the Observed Data; 4.4 Further Reading; 4.5 Exercises 5 Observational Data: Detailed Characteristics in the Frequency Domain5.1 Power Spectrum Estimation; 5.2 Statistics of the Power Spectrum; 5.3 Solar-Like Oscillations in the Frequency Domain; 5.4 Global Properties of the Oscillation Spectrum; 5.5 Frequency Spectrum of Granulation and Active-Region Signal; 5.6 Harmonic Structure from Transits, Eclipses, and Stellar Rotation; 5.7 Super-Nyquist Asteroseismology; 5.8 Further Reading; 5.9 Exercises; 6 Observational Data: Analysis of the Frequency Spectrum; 6.1 Statistical Tests: Example of Detection of Signatures of Individual Modes 6.2 Automated Detection of Oscillation Spectra6.3 Fundamentals of Peak-Bagging: Extraction of Individual Mode Parameters; 6.4 Peak-Bagging: Practicalities and Challenges; 6.5 Challenges for Peak-Bagging Posed by Mixed Modes; 6.6 Further Reading; 6.7 Exercises; 7 Drawing Inferences from Average Seismic Parameters; 7.1 The Direct Method; 7.2 Grid-Based Modeling; 7.3 Further Reading; 7.4 Exercises; 8 Interpreting Frequencies of Individual Modes: Comparing Frequencies; 8.1 Choosing the Physics of Models; 8.2 Effects of Different Model Parameters; 8.3 A Complicating Factor: The Surface Term 8.4 Common Ways of Constructing Models to Fit Frequencies8.5 Dealing with Avoided Crossings in Subgiants; 8.6 Modeling Red Giants; 8.7 Alternative Methods for Fitting Frequencies; 8.8 Analysis of Rotation; 8.9 Further Reading; 8.10 Exercises; 9 Interpreting Frequencies of Individual Modes: Other Diagnostics; 9.1 Learning from Combinations of Frequencies; 9.2 Fitting and Interpreting the Signature of Acoustic Glitches; 9.3 Analysis of Red Giants; 9.4 Further Reading; 9.5 Exercises; 10 Inverting Mode Frequencies; 10.1 The Inversion Equation; 10.2 The Regularized Least Squares Technique},
  isbn = {978-0-691-16292-8},
  keywords = {notion,notion-database}
}

@article{basuUnveilingStructureDynamics2020,
  title = {Unveiling the {{Structure}} and {{Dynamics}} of {{Red Giants With Asteroseismology}}},
  author = {Basu, Sarbani and Hekker, Saskia},
  year = {2020},
  journal = {Frontiers in Astronomy and Space Sciences},
  volume = {7},
  issn = {2296-987X},
  urldate = {2022-07-22},
  abstract = {The Kepler mission observed many thousands of red giants. The long time series, some as long as the mission itself, have allowed us to study red giants with unprecedented detail. Given that red giants are intrinsically luminous, and hence can be observed from very large distances, knowing the properties of red giants, in particular ages, is of immense value for studies of the formation and evolution of the Galaxy, an endeavor known as ``Galactic archaeology.'' In this article we review what we have learned about red giants using asteroseismic data. We start with the properties of the power spectrum and move on to internal structure and dynamics of these stars; we also touch upon unsolved issues in red-giant asteroseismology and the prospects of making further progress in understanding these stars.},
  file = {/Users/lbugnet/Zotero/storage/YLRNWUQV/Basu et Hekker - 2020 - Unveiling the Structure and Dynamics of Red Giants.pdf}
}

@article{Batalha2010,
  title = {Selection, Prioritization, and Characteristics of Kepler Target Stars},
  author = {Batalha, Natalie M. and Borucki, William J. and Koch, David G. and Bryson, Stephen T. and Haas, Michael R. and Brown, Timothy M. and Caldwell, Douglas A. and Hall, Jennifer R. and Gilliland, Ronald L. and Latham, David W. and Meibom, Soren and Monet, David G.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0349},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L109},
  abstract = {The Kepler Mission began its 3.5 year photometric monitoring campaign in 2009 May on a select group of approximately 150,000 stars. The stars were chosen from the {$\sim$}half million in the field of view that are brighter than 16th magnitude. The selection criteria are quantitative metrics designed to optimize the scientific yield of the mission with regard to the detection of Earth-size planets in the habitable zone. This yields more than 90,000 G-type stars on or close to the main sequence, {$>$}20, 000 of which are brighter than 14th magnitude. At the temperature extremes, the sample includes approximately 3000 M-type dwarfs and a small sample of O- and B-type MS stars ({$<$}200). The small numbers of giants are included in the sample: 5000 stars with surface gravities log(g) {$<$} 3.5. We present a brief summary of the selection process and the stellar populations it yields in terms of surface gravity, effective temperature, and apparent magnitude. In addition to the primary, statistically derived target set, several ancillary target lists were manually generated to enhance the science of the mission, examples being: known eclipsing binaries, open cluster members, and high proper motion stars. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: statistics},
  file = {/Users/lbugnet/Zotero/storage/FYPNCD4F/Batalha et al. - 2010.pdf}
}

@article{Batalha2011,
  title = {Kepler's First Rocky Planet: {{Kepler-10b}}},
  author = {Batalha, Natalie M. and Borucki, William J. and Bryson, Stephen T. and Buchhave, Lars A. and Caldwell, Douglas A. and {Christensen-Dalsgaard}, J{\o}rgen and Ciardi, David and Dunham, Edward W. and Fressin, Francois and Gautier, Thomas N. and Gilliland, Ronald L. and Haas, Michael R. and Howell, Steve B. and Jenkins, Jon M. and Kjeldsen, Hans and Koch, David G. and Latham, Davidw and Lissauer, Jack J. and Marcy, Geoffrey W. and Rowe, Jason F. and Sasselov, Dimitar D. and Seager, Sara and Steffen, Jasonh and Torres, Guillermo and Basri, Gibor S. and Brown, Timothy M. and Charbonneau, David and Christiansen, Jessie and Clarke, Bruce and Cochran, William D. and Dupree, Andrea and Fabrycky, Daniel C. and Fischer, Debra and Ford, Eric B. and Fortney, Jonathan and Girouard, Forrest R. and Holman, Matthew J. and Johnson, John and Isaacson, Howard and Klaus, Todd C. and MacHalek, Pavel and Moorehead, Althea V. and Morehead, Robert C. and Ragozzine, Darin and Tenenbaum, Peter and Twicken, Joseph and Quinn, Samuel and Vancleve, Jeffrey and Walkowicz, Lucianne M. and Welsh, Williamf and Devore, Edna and Gould, Alan},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {729},
  number = {1},
  eprint = {1102.0605},
  issn = {15384357},
  doi = {10.1088/0004-637X/729/1/27},
  abstract = {NASA's Kepler Mission uses transit photometry to determine the frequency of Earth-size planets in or near the habitable zone of Sun-like stars. The mission reached a milestone toward meeting that goal: the discovery of its first rocky planet, Kepler-10b. Two distinct sets of transit events were detected: (1) a 152 4 ppm dimming lasting 1.811 0.024 hr with ephemeris T[BJD] =2454964.57375 +0.00060-0.00082 + N*0.837495+0.000004-0.000005 days and (2) a 376 9ppm dimming lasting 6.86 0.07 hr with ephemeris T[BJD] =2454971.6761+0.0020-0.0023 + N*45.29485+0.00065-0.00076 days. Statistical tests on the photometric and pixel flux time series established the viability of the planet candidates triggering ground-based follow-up observations. Forty precision Doppler measurements were used to confirm that the short-period transit event is due to a planetary companion. The parent star is bright enough for asteroseismic analysis. Photometry was collected at 1 minute cadence for {$>$}4 months from which we detected 19 distinct pulsation frequencies. Modeling the frequencies resulted in precise knowledge of the fundamental stellar properties. Kepler-10 is a relatively old (11.9 4.5Gyr) but otherwise Sun-like main-sequence star with T eff = 5627 44K, M = 0.895 0.060 M, and R = 1.056 0.021 R. Physical models simultaneously fit to the transit light curves and the precision Doppler measurements yielded tight constraints on the properties of Kepler-10b that speak to its rocky composition: M P = 4.56+1.17-1.29 M {$\oplus$}, R P = 1.416+0.033-0.036 R {$\oplus$}, and {$\rho$}P = 8.8+2.1-2.9gcm-3. Kepler-10b is the smallest transiting exoplanet discovered to date. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,planetary systems,techniques: photometric,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/K3EEA3ZQ/Batalha et al. - 2011.pdf}
}

@article{Batalha2013,
  title = {Planetary Candidates Observed by Kepler. {{III}}. {{Analysis}} of the First 16 Months of Data},
  author = {Batalha, Natalie M. and Rowe, Jason F. and Bryson, Stephen T. and Barclay, Thomas and Burke, Christopher J. and Caldwell, Douglas A. and Christiansen, Jessie L. and Mullally, Fergal and Thompson, Susan E. and Brown, Timothy M. and Dupree, Andrea K. and Fabrycky, Daniel C. and Ford, Eric B. and Fortney, Jonathan J. and Gilliland, Ronald L. and Isaacson, Howard and Latham, David W. and Marcy, Geoffrey W. and Quinn, Samuel N. and Ragozzine, Darin and Shporer, Avi and Borucki, William J. and Ciardi, David R. and Gautier, Thomas N. and Haas, Michael R. and Jenkins, Jon M. and Koch, David G. and Lissauer, Jack J. and Rapin, William and Basri, Gibor S. and Boss, Alan P. and Buchhave, Lars A. and Carter, Joshua A. and Charbonneau, David and {Christensen-Dalsgaard}, Joergen and Clarke, Bruce D. and Cochran, William D. and Demory, Brice Olivier and Desert, Jean Michel and Devore, Edna and Doyle, Laurance R. and Esquerdo, Gilbert A. and Everett, Mark and Fressin, Francois and Geary, John C. and Girouard, Forrest R. and Gould, Alan and Hall, Jennifer R. and Holman, Matthew J. and Howard, Andrew W. and Howell, Steve B. and Ibrahim, Khadeejah A. and Kinemuchi, Karen and Kjeldsen, Hans and Klaus, Todd C. and Li, Jie and Lucas, Philip W. and Meibom, Soren and Morris, Robert L. and Pr{\v s}a, Andrej and Quintana, Elisa and Sanderfer, Dwight T. and Sasselov, Dimitar and Seader, Shawn E. and Smith, Jeffrey C. and Steffen, Jason H. and Still, Martin and Stumpe, Martin C. and Tarter, Jill C. and Tenenbaum, Peter and Torres, Guillermo and Twicken, Joseph D. and Uddin, Kamal and Van Cleve, Jeffrey and Walkowicz, Lucianne and Welsh, William F.},
  year = {2013},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {204},
  number = {2},
  eprint = {1202.5852},
  issn = {00670049},
  doi = {10.1088/0067-0049/204/2/24},
  abstract = {New transiting planet candidates are identified in 16 months (2009 May-2010 September) of data from the Kepler spacecraft. Nearly 5000 periodic transit-like signals are vetted against astrophysical and instrumental false positives yielding 1108 viable new planet candidates, bringing the total count up to over 2300. Improved vetting metrics are employed, contributing to higher catalog reliability. Most notable is the noise-weighted robust averaging of multi-quarter photo-center offsets derived from difference image analysis that identifies likely background eclipsing binaries. Twenty-two months of photometry are used for the purpose of characterizing each of the candidates. Ephemerides (transit epoch, T 0, and orbital period, P) are tabulated as well as the products of light curve modeling: reduced radius (R P/R*), reduced semimajor axis (d/R *), and impact parameter (b). The largest fractional increases are seen for the smallest planet candidates (201\% for candidates smaller than 2 R{$\oplus$} compared to 53\% for candidates larger than 2 R{$\oplus$}) and those at longer orbital periods (124\% for candidates outside of 50 day orbits versus 86\% for candidates inside of 50 day orbits). The gains are larger than expected from increasing the observing window from 13 months (Quarters 1-5) to 16 months (Quarters 1-6) even in regions of parameter space where one would have expected the previous catalogs to be complete. Analyses of planet frequencies based on previous catalogs will be affected by such incompleteness. The fraction of all planet candidate host stars with multiple candidates has grown from 17\% to 20\%, and the paucity of short-period giant planets in multiple systems is still evident. The progression toward smaller planets at longer orbital periods with each new catalog release suggests that Earth-size planets in the habitable zone are forthcoming if, indeed, such planets are abundant. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {eclipses,notion,notion-database,planetary systems,space vehicles,techniques: photometric,words: catalogs},
  file = {/Users/lbugnet/Zotero/storage/2JMJ2LBZ/Batalha et al. - 2013.pdf}
}

@article{Batygin2015,
  title = {Jupiter's Decisive Role in the Inner {{Solar System}}'s Early Evolution},
  author = {Batygin, Konstantin and Laughlin, Greg},
  year = {2015},
  month = apr,
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  volume = {112},
  number = {14},
  eprint = {1503.06945},
  pages = {4214--4217},
  publisher = {{National Academy of Sciences}},
  issn = {10916490},
  doi = {10.1073/pnas.1423252112},
  urldate = {2020-02-27},
  abstract = {The statistics of extrasolar planetary systems indicate that the default mode of planet formation generates planets with orbital periods shorter than 100 days and masses substantially exceeding that of the Earth. When viewed in this context, the Solar System is unusual. Here, we present simulations which show that a popular formation scenario for Jupiter and Saturn, in which Jupiter migrates inward from a {$>$} 5 astronomical units (AU) to a {$\approx$} 1.5 AU before reversing direction, can explain the low overall mass of the Solar System's terrestrial planets, as well as the absence of planets with a {$<$} 0.4 AU. Jupiter's inward migration entrained s {$\greaterequivlnt$} 10-100 km planetesimals into low-order mean motion resonances, shepherding and exciting their orbits. The resulting collisional cascade generated a planetesimal disk that, evolving under gas drag, would have driven any preexisting short-period planets into the Sun. In this scenario, the Solar System's terrestrial planets formed from gas-starved mass-depleted debris that remained after the primary period of dynamical evolution.},
  archiveprefix = {arxiv},
  keywords = {Extrasolar planets,notion,notion-database,Planetary dynamics,Solar System formation},
  file = {/Users/lbugnet/Zotero/storage/LC5IKT8M/full-text.pdf}
}

@article{Baudin2005,
  title = {Inferred Acoustic Rates of Solar p Modes from Several Helioseismic Instruments},
  author = {Baudin, F. and Samadi, R. and Goupil, M. J. and Appourchaux, T. and Barban, C. and Boumier, P. and Chaplin, W. J. and Gouttebroze, P.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {433},
  number = {1},
  pages = {349--356},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041229},
  abstract = {Acoustic rates of excitation of solar p modes can be estimated from observations in order to place constraints on the modelling of the excitation process and the layers where it occurs in the star. For several reasons (including a poor signal to noise ratio and mode overlap), this estimation is difficult. In this work, we use three completely independent datasets to obtain robust estimates in the solar case for l = 1 modes. We also show that the height in the solar atmosphere where the modes are observed must be taken into account. Our three sets of results are shown to be consistent, particularly in the lower part of the p-mode spectrum (from 1.8 mHz to 2.8 mHz). At higher frequencies, the agreement is not as good, because of a larger dispersion of the measurements and also because of some systematic differences which might be due to observation height estimation or to a systematic influence of the noise. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: oscillation},
  file = {/Users/lbugnet/Zotero/storage/GPM6ZDDQ/Baudin et al. - 2005.pdf}
}

@article{Baudin2007,
  title = {A Contribution to the Understanding of Chromospheric Oscillations},
  author = {Baudin, F. and Ibarra, E. and Avrett, E. H. and Vial, J. C. and Bocchialini, K. and Costa, A. and Lemaire, P. and Rovira, M.},
  year = {2007},
  journal = {Solar Physics},
  volume = {241},
  number = {1},
  pages = {39--51},
  issn = {00380938},
  doi = {10.1007/s11207-007-0006-3},
  abstract = {We present SUMER/SOHO UV measurements of chromospheric oscillations of intensity, velocity, and linewidth observed in C i, S i, O i, and C ii lines, which are formed in the altitude range from 1000 km to 2000 km above {$\tau$} 500=1. Oscillations in lines originating at similar altitudes exhibit different behaviors which we discuss in terms of the formation of the lines. \textcopyright{} Springer 2007.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WTDNWBEW/Baudin et al. - 2007.pdf}
}

@article{Baudin2008,
  title = {Searching for P-Modes in {{MOST}}* {{Procyon}} Data: {{Another}} View},
  author = {Baudin, F. and Appourchaux, T. and Boumier, P. and Kuschnig, R. and Leibacher, J. W. and Matthews, J. M.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {478},
  number = {2},
  pages = {461--465},
  issn = {00046361},
  doi = {10.1051/0004-6361:20077683},
  abstract = {Context: Photometry of Procyon obtained by the MOST satellite in 2004 has been searched for p modes by several groups, with sometimes contradictory interpretations. Aims:We explore two possible factors that complicate the analysis and may lead to erroneous reports of p modes in these data. Methods: Two methods are used to illustrate the role of subtle instrumental effects in the photometry: time-frequency analysis, and a search for regularly spaced peaks in a Fourier spectrum based on the echelle diagramme approach. Results: We find no convincing evidence of a p-mode signal in the MOST Procyon data. We can account for an apparent excess of power close to the p-mode frequency range and signs of structure in an echelle diagramme in terms of instrumental effects. \textcopyright{} ESO 2008.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TCNEBHQZ/Baudin et al. - 2008.pdf}
}

@article{Baudin2011,
  title = {Amplitudes and Lifetimes of Solar-like Oscillations Observed by {{CoRoT}} ( {{Corrigendum}} )},
  author = {Baudin, F. and Barban, C. and Belkacem, K. and Hekker, S. and Morel, T. and Samadi, R. and Benomar, O. and Goupil, M.-J. and Carrier, F. and Ballot, J. and Deheuvels, S. and De Ridder, J. and Hatzes, A. P. and Kallinger, T. and Weiss, W. W.},
  year = {2011},
  journal = {Astronomy \& Astrophysics},
  volume = {535},
  pages = {C1},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201014037e},
  abstract = {Context. The advent of space-borne missions such as CoRoT or Kepler providing photometric data has brought new possibilities for asteroseismology across the H-R diagram. Solar-like oscillations are now observed in many stars, including red giants and main-sequence stars. Aims. Based on several hundred identified pulsating red giants, we aim to characterize their oscillation amplitudes and widths. These observables are compared with those of main-sequence stars in order to test trends and scaling laws for these parameters for main-sequence stars and red giants. Methods. An automated fitting procedure is used to analyze several hundred Fourier spectra. For each star, a modeled spectrum is fitted to the observed oscillation spectrum, and mode parameters are derived. Results. Amplitudes and widths of red-giant solar-like oscillations are estimated for several hundred modes of oscillation. Amplitudes are relatively high (several hundred ppm) and widths relatively small (very few tenths of a \textmu Hz). Conclusions. Widths measured in main-sequence stars show a different variation with the effective temperature from red giants. A single scaling law is derived for mode amplitudes of red giants and main-sequence stars versus their luminosity to mass ratio. However, our results suggest that two regimes may also be compatible with the observations.},
  keywords = {asteroseismology,data analysis,methods,notion,notion-database,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/DLJRX6BJ/Baudin et al. - 2011.pdf}
}

@article{Bazilevskaya2014,
  title = {A {{Combined Analysis}} of the {{Observational Aspects}} of the {{Quasi-biennial Oscillation}} in {{Solar Magnetic Activity}}},
  author = {Bazilevskaya, G. and Broomhall, A. M. and Elsworth, Y. and Nakariakov, V. M.},
  year = {2014},
  journal = {Space Science Reviews},
  volume = {186},
  number = {1-4},
  pages = {359--386},
  issn = {15729672},
  doi = {10.1007/s11214-014-0068-0},
  abstract = {Solar quasi-biennial oscillations (QBOs) with the time scale of 0.6\textendash 4 yrs appear to be a basic feature of the Sun's activity. Observational aspects of QBOs are reviewed on the basis of recent publications. Solar QBOs are shown to be ubiquitous and very variable. We demonstrate that many features of QBOs are common to different observations. These features include variable periodicity and intermittence with signs of stochastisity, a presence at all levels of the solar atmosphere and even in the convective zone, independent development in the northern and southern solar hemispheres, most pronounced amplitudes during the maximum phase of the 11-yr cycle and the transition of QBOs into interplanetary space. Temporal weakening of solar activity around the maximum of the 11-yr cycle (Gnevyshev Gap) can be considered an integral part of QBOs. The exact mechanism by which the solar QBO is produced is poorly understood. We describe some of the most plausible theoretical mechanisms and discuss observational features that support/contradict the theory. QBOs have an important meaning as a benchmark of solar activity, not only for investigation of the solar dynamo but also in terms of space weather.},
  keywords = {notion,notion-database,Sun: activity,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/4BV93PGV/Bazilevskaya et al. - 2014.pdf}
}

@article{Bazot2004,
  title = {Asteroseismology of Exoplanets Hosts Stars: {{Tests}} of Internal Metallicity},
  author = {Bazot, M. and Vauclair, S.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {427},
  number = {3},
  pages = {965--973},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041528},
  abstract = {Exoplanet host stars present a clear metallicity excess compared to stars without detected planets, with an average overabundance of 0.2 dex. This excess may be primordial, in which case the stars should be overmetallic down to their center, or it may be due to accretion in the early phases of planetary formation, in which case the stars would be overmetallic only in their outer layers. In the present paper, we show the differences in the internal structure of stars, according to the chosen scenario. Namely two stars with the same observable parameters (luminosity, effective temperature, outer chemical composition) are completely different in their interiors according to their past histories, which we reconstitute through the computations of their evolutionary tracks. It may happen that stars with an initial overmetallicity have a convective core while the stars which suffered accretion do not. We claim that asteroseismic studies of these exoplanet host stars can give clues about their internal structures and metallicities, which may help in understanding planetary formation.},
  keywords = {Abundances - Stars,Formation - Stars,notion,notion-database,Oscillations,Planetary systems,Stars},
  file = {/Users/lbugnet/Zotero/storage/VX6IK6EX/Bazot, Vauclair - 2004.pdf}
}

@article{Bazot2005,
  title = {Seismic Analysis of the Planet-Hosting Star \textmu{} {{Arae}}},
  author = {Bazot, M and Vauclair, S and Bouchy, F and Santos, N C},
  year = {2005},
  volume = {621},
  pages = {615--621},
  keywords = {abundances,formation,hd 160691,notion,notion-database,oscillations,planetary systems,stars,supernovae individual},
  file = {/Users/lbugnet/Zotero/storage/NL4PBPI3/Bazot et al. - 2005.pdf}
}

@article{Bazot2007,
  title = {Asteroseismology of {$\alpha$} {{Centauri A}} Evidence of Rotational Splitting},
  author = {Bazot, M. and Bouchy, F. and Kjeldsen, H. and Charpinet, S. and Laymand, M. and Vauclair, S.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {470},
  number = {1},
  pages = {295--302},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065694},
  abstract = {Context. Asteroseismology provides a unique tool for studying stellar interiors. Recently p modes have been detected on the bright solar-like star {$\alpha$} Cen A thanks to high-precision radial-velocity measurements. However, a better characterisation of these p modes is clearly needed to constrain theoretical models. Aims. We observed {$\alpha$} Cen A during five nights using the HARPS spectrograph in order to improve our knowledge of the seismic properties of this star. Methods. We performed high-precision radial-velocity sequences and computed the acoustic spectrum of {$\alpha$} Cen A. Results. We identify 34 p modes with angular degree l = 0-3 in the frequency range 1.8-2.9 mHz and amplitude range 13-48 cms-1, in agreement with previous seismic studies. We find an enhancement of the frequency scatter with the angular degree l that indicates, considering the high inclination axis of {$\alpha$} Cen A, rotational splitting and explains the low values of previously suggested mode lifetimes. We also derive new values for the small separations that take the effect of rotational splitting into account. Conclusions. Our seismic study of {$\alpha$} Cen A leads to a list of now well-identified p-mode frequencies and shows the importance of taking the rotation into account in order to properly characterise the p modes even in quite short campaigns. \textcopyright{} ESO 2007.},
  keywords = {notion,notion-database,Stars: individual: {$\alpha$} Centauri A,Stars: oscillations,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/JY24387J/Bazot et al. - 2007.pdf}
}

@article{Bazot2011,
  title = {Astrophysics {{L}} Etter to the {{E}} Ditor {{The}} Radius and Mass of the Close Solar Twin 18 {{Scorpii}} Derived from Asteroseismology and Interferometry},
  author = {Bazot, M and Ireland, M J and Huber, D and Bedding, T R and Broomhall, A and Campante, T L and Carfantan, H},
  year = {2011},
  volume = {4},
  pages = {2--5},
  keywords = {18 sco,data analysis,individual,interferometric,methods,notion,notion-database,oscillations,radial velocities,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/W7743XMP/Bazot et al. - 2011.pdf}
}

@article{Bazot2012,
  title = {Estimating the P-Mode Frequencies of the Solar Twin 18 {{Scorpii}}},
  author = {Bazot, M. and Campante, T. L. and Chaplin, W. J. and Carfantan, H. and Bedding, T. R. and Dumusque, X. and Broomhall, A. M. and Petit, P. and Th{\'e}ado, S. and Van Grootel, V. and Arentoft, T. and Castro, M. and {Christensen-Dalsgaard}, J. and Do Nascimento, J. D. and Dintrans, B. and Kjeldsen, H. and Monteiro, M. J.P.F.G. and Santos, N. C. and Sousa, S. and Vauclair, S.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {544},
  pages = {1--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117963},
  abstract = {Solar twins have been a focus of attention for more than a decade, because their structure is extremely close to that of the Sun. Today, thanks to high-precision spectrometers, it is possible to use asteroseismology to probe their interiors. Our goal is to use time series obtained from the HARPS spectrometer to extract the oscillation frequencies of 18 Sco, the brightest solar twin. We used the tools of spectral analysis to estimate these quantities. We estimate 52 frequencies using an MCMC algorithm. After examination of their probability densities and comparison with results from direct MAP optimization, we obtain a minimal set of 21 reliable modes. The identification of each pulsation mode is straightforwardly accomplished by comparing to the well-established solar pulsation modes. We also derived some basic seismic indicators using these values. These results offer a good basis to start a detailed seismic analysis of 18 Sco using stellar models. \textcopyright{} 2012 ESO.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: individual: 18 Sco,Stars: oscillations,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/B7YSS7KY/Bazot et al. - 2012.pdf}
}

@article{Bazot2018,
  title = {Butterfly Diagram of a {{Sun-like}} Star Observed Using Asteroseismology},
  author = {Bazot, M. and Nielsen, M. B. and Mary, D. and {Christensen-Dalsgaard}, J. and Benomar, O. and Petit, P. and Gizon, L. and Sreenivasan, K. R. and White, T. R.},
  year = {2018},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {619},
  eprint = {1810.08630},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201834251},
  urldate = {2020-07-21},
  abstract = {Stellar magnetic fields are poorly understood, but are known to be important for stellar evolution and exoplanet habitability. They drive stellar activity, which is the main observational constraint on theoretical models for magnetic field generation and evolution. Starspots are the main manifestation of the magnetic fields at the stellar surface. In this study we measured the variation in their latitude with time, called a butterfly diagram in the solar case, for the solar analogue HD 173701 (KIC 8006161). To this end, we used Kepler data to combine starspot rotation rates at different epochs and the asteroseismically determined latitudinal variation in the stellar rotation rates. We observe a clear variation in the latitude of the starspots. It is the first time such a diagram has been constructed using asteroseismic data.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: individual: HD173701,Stars: oscillations,Stars: rotation,Stars: solar-type,Starspots},
  file = {/Users/lbugnet/Zotero/storage/G73RTX6Q/full-text.pdf}
}

@article{Beaudoin2018,
  title = {Differential {{Rotation}} in {{Solar-like Convective Envelopes}}: {{Influence}} of {{Overshoot}} and {{Magnetism}}},
  author = {Beaudoin, Patrice and Strugarek, Antoine and Charbonneau, Paul},
  year = {2018},
  doi = {10.3847/1538-4357/aabfef},
  urldate = {2020-07-05},
  abstract = {We present a set of four global Eulerian/semi-Lagrangian fluid solver (EULAG) hydrodynamical (HD) and magnetohydrodynamical (MHD) simulations of solar convection, two of which are restricted to the nominal convection zone, and the other two include an underlying stably stratified fluid layer. While all four simulations generate reasonably solar-like latitudinal differential rotation profiles where the equatorial region rotates faster than the polar regions, the rotational isocontours vary significantly among them. In particular, the purely HD simulation with a stable layer alone can break the Taylor-Proudman theorem and produce approximately radially oriented rotational isocontours at medium to high latitudes. We trace this effect to the buildup of a significant latitudinal temperature gradient in the stable fluid immediately beneath the convection zone, which imprints itself on the lower convection zone. It develops naturally in our simulations as a consequence of convective overshoot and rotational influence of rotation on convective energy fluxes. This favors the establishment of a thermal wind balance that allows evading the Taylor-Proudman constraint. A much smaller latitudinal temperature gradient develops in the companion MHD simulation that includes a stable fluid layer, reflecting the tapering of deep convective overshoot that occurs at medium to high latitudes, which is caused by the strong magnetic fields that accumulate across the base of the convection zone. The stable fluid layer also has a profound impact on the large-scale magnetic cycles developing in the two MHD simulations. Even though both simulations operate in the same convective parameter regime, the simulation that includes a stable layer eventually loses cyclicity and transits to a non-solar, steady quadrupolar state.},
  keywords = {convection,magnetohydrodynamics (MHD),notion,notion-database,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/7D522V7N/full-text.pdf}
}

@article{Becerra2022,
  title = {Stability of Axially Symmetric Magnetic Fields in Stars},
  author = {Becerra, Laura and Reisenegger, Andreas and Valdivia, Juan Alejandro and Gusakov, Mikhail},
  year = {2022},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {517},
  pages = {560--568},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac2704},
  urldate = {2023-07-25},
  abstract = {The magnetic fields observed in Ap stars, white dwarfs, and neutron stars are known to be stable for long times. However, the physical conditions inside the stellar interiors that allow these states are still a matter of research. It has been formally demonstrated that both purely toroidal and purely poloidal magnetic fields develop instabilities at some point in the star. On the other hand, numerical simulations have proved the stability of roughly axisymmetric magnetic field configurations inside stably stratified stars. These configurations consist of mutually stabilizing toroidal and poloidal components in a twisted torus shape. Previous studies have proposed rough upper and lower bounds on the ratio of the magnetic energy in the toroidal and poloidal components of the magnetic field. With the purpose of mapping out the parameter space under which such configurations remain stable, we used the PENCIL CODE to perform 3D magnetohydrodynamic simulations of the evolution of the magnetic field in non-rotating, non-degenerate stars in which viscosity is the only dissipation mechanism, both for stars with a uniform (barotropic) and radially increasing (stably stratified) specific entropy. Furthermore, we considered different conditions regarding the degree of stable stratification and the magnetic energy in each component, roughly confirming the previously suggested stability boundaries for the magnetic field.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,MHD,software: simulations,stars: magnetic field,stars: massive,stars: neutron,white dwarfs},
  annotation = {ADS Bibcode: 2022MNRAS.517..560B Cite key: Becerra2022},
  file = {/Users/lbugnet/Zotero/storage/IITXMYPM/Becerra et al. - 2022 - Stability of axially symmetric magnetic fields in .pdf}
}

@article{Becerra2022a,
  title = {Evolution of Random Initial Magnetic Fields in Stably Stratified and Barotropic Stars},
  author = {Becerra, Laura and Reisenegger, Andreas and Valdivia, Juan Alejandro and Gusakov, Mikhail E},
  year = {2022},
  month = feb,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {511},
  number = {1},
  pages = {732--745},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/stac102},
  urldate = {2023-08-16},
  abstract = {ABSTRACT             Long-lived magnetic fields are known to exist in upper main-sequence stars, white dwarfs, and neutron stars. In order to explore possible equilibrium configurations of the magnetic field inside these stars, we have performed 3D magnetohydrodynamic simulations of the evolution of initially random magnetic fields in stably stratified and barotropic stars with an ideal-gas equation~of state using the pencil code, a high-order finite-difference code for compressible hydrodynamic flows in the presence of magnetic fields. In barotropic (isentropic) stars, we confirm previous results in the sense that all initial magnetic fields we tried decay away, unable to reach a stable equilibrium. In the case of stably stratified stars (with radially increasing specific entropy), initially random magnetic fields appear to always evolve to a stable equilibrium. However, the nature of this equilibrium depends on the dissipation mechanisms considered. If magnetic diffusivity (or hyper-diffusivity) is included, the final state is more axially symmetric and dominated by large wavelengths than the initial state, whereas this is not the case if only viscosity (or hyper-viscosity) is present. In real stars, the main mechanism allowing them to relax to equilibrium is likely to be phase mixing, which we argue is more closely mimicked by viscosity. Therefore, we conclude that, depending on its formation mechanism, the equilibrium magnetic field in these stars could in principle be very asymmetric.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/CK5TWGY5/Becerra et al. - 2022 - Evolution of random initial magnetic fields in sta.pdf}
}

@article{Beck1993,
  title = {A Study of the Contrast of Sunspots from Photometric Images},
  author = {Beck, John G. and Chapman, Gary A.},
  year = {1993},
  journal = {Solar Physics},
  volume = {146},
  number = {1},
  pages = {49--60},
  issn = {00380938},
  doi = {10.1007/BF00662169},
  abstract = {The thermal contrast {$\alpha$}, and the umbra-penumbra Au/Ap, were calculated for 63 sunspots of various sizes and morphologies. Contrary to the assumptions of the PSI model, {$\alpha$} and Au/Ap were found to be quite variable. The values of {$\alpha$} ranged from 0.1807 to 0.4266;Au/Ap ranged from 0.0089 to 0.4899. The values of {$\alpha$} and Au/Ap correlated well (r = 0.6018;p{$<$}0.005) and the regression for {$\alpha$} and Au/Ap was obtained: {$\alpha$} = (0.220 {$\pm$} 0.016) + (0.340 {$\pm$} O.06)Au/Ap. The values of {$\alpha$} and Au/Ap were then compared with complexity ratings, magnetic field strength, time, and {$\mu$}. The quantities {$\alpha$} and Au/Ap were found to be independent of the complexity, magnetic field strength, and time factors. The correlation between {$\alpha$} and Au/Ap lead to the proposed division of {$\alpha$} into an umbral thermal contrast {$\alpha$}u, and a penumbral thermal contrast {$\alpha$}p. These values were calculated from the photometric data: {$\alpha$}u = 0.57 {$\pm$} 0.01 and {$\alpha$}p = 0.26 {$\pm$} 0.006. \textcopyright{} 1993 Kluwer Academic Publishers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ECAS5AQL/Beck, Chapman - 1993.pdf}
}

@article{Beck2011,
  title = {Kepler Detected Gravity-Mode Period Spacings in a Red Giant Star},
  author = {Beck, P. G. and Bedding, T. R. and Mosser, B. and Stello, D. and Garcia, R. A. and Kallinger, T. and Hekker, S. and Elsworth, Y. and Frandsen, S. and Carrier, F. and De Ridder, J. and Aerts, C. and White, T. R. and Huber, D. and Dupret, M. A. and Montalb{\'a}n, J. and Miglio, A. and Noels, A. and Chaplin, W. J. and Kjeldsen, H. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Brown, T. M. and Kawaler, S. D. and Mathur, S. and Jenkins, J. M.},
  year = {2011},
  journal = {Science},
  volume = {332},
  number = {6026},
  pages = {205},
  issn = {00368075},
  doi = {10.1126/science.1201939},
  keywords = {ASTRONOMY,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WCDI45AD/Beck et al. - 2011.pdf}
}

@article{Beck2012,
  title = {Fast Core Rotation in Red-Giant Stars as Revealed by Gravity-Dominated Mixed Modes},
  author = {Beck, Paul G. and Montalban, Josefina and Kallinger, Thomas and De Ridder, Joris and Aerts, Conny and Garc{\'i}a, Rafael A. and Hekker, Saskia and Dupret, Marc Antoine and Mosser, Benoit and Eggenberger, Patrick and Stello, Dennis and Elsworth, Yvonne and Frandsen, S{\o}ren and Carrier, Fabien and Hillen, Michel and Gruberbauer, Michael and {Christensen-Dalsgaard}, J{\o}rgen and Miglio, Andrea and Valentini, Marica and Bedding, Timothy R. and Kjeldsen, Hans and Girouard, Forrest R. and Hall, Jennifer R. and Ibrahim, Khadeejah A.},
  year = {2012},
  journal = {Nature},
  volume = {481},
  number = {7379},
  pages = {55--57},
  issn = {00280836},
  doi = {10.1038/nature10612},
  abstract = {When the core hydrogen is exhausted during stellar evolution, the central region of a star contracts and the outer envelope expands and cools, giving rise to a red giant. Convection takes place over much of the star's radius. Conservation of angular momentum requires that the cores of these stars rotate faster than their envelopes; indirect evidence supports this. Information about the angular-momentum distribution is inaccessible to direct observations, but it can be extracted from the effect of rotation on oscillation modes that probe the stellar interior. Here we report an increasing rotation rate from the surface of the star to the stellar core in the interiors of red giants, obtained using the rotational frequency splitting of recently detected 'mixed modes'. By comparison with theoretical stellar models, we conclude that the core must rotate at least ten times faster than the surface. This observational result confirms the theoretical prediction of a steep gradient in the rotation profile towards the deep stellar interior. \textcopyright{} 2012 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4DU2C9FV/Beck et al. - 2012.pdf}
}

@book{Beck2013a,
  title = {Asteroseismology of {{Red-Giant Stars}}: {{Mixed Modes}}, {{Differential Rotation}}, and {{Eccentric Binaries}}},
  author = {Beck, Paul~G.},
  year = {2013},
  journal = {PhD Thesis},
  number = {December},
  issn = {0027-8424},
  abstract = {Astronomers are aware of rotation in stars since Galileo Galilei attributed the movement of sunspots to rotation of the Sun in 1613. In contrast to the Sun, whose surface can be resolved by small telescopes or even the (protected) eye, we detect stars as point sources with no spatial information. Numerous techniques have been developed to derive information about stellar rotation. Unfortunately, most observational data allow only for the surface rotational rate to be inferred. The internal rotational profile, which has a great effect on the stellar structure and evolution, remains hidden below the top layers of the star - the essential is hidden to the eyes.  Asteroseismology allows us to "sense" indirectly deep below the stellar surface. Oscillations that propagate through the star provide information about the deep stellar interiors while they also distort the stellar surface in characteristic patterns leading to detectable brightness or velocity variations. Also, certain oscillation modes are sensitive to internal rotation and carry information on how the star is spinning deep inside. Thanks to the unprecedented quality of NASA's space telescope Kepler, numerous detailed observations of stars in various evolutionary stages are available. Such high quality data allow that for many stars, rotation can not only be constrained from surface rotation, but also investigated through seismic studies.  The work presented in this thesis focuses on the oscillations and internal rotational gradient of evolved single and binary stars. It is shown that the seismic analysis can reach the cores of oscillating red-giant stars and that these cores are rapidly rotating, while nested in a slowly rotating convective envelope.},
  isbn = {978-90-8649-677-8},
  pmid = {17556540},
  keywords = {Asteroseismology,Eccentric Binaries,Mixed Modes,Multi-Site Campaign,NASA Kepler Space telescope,Non-Rigid Rotation,notion,notion-database,Red Giant Stars},
  file = {/Users/lbugnet/Zotero/storage/HPWZVCJY/Beck - 2013.pdf;/Users/lbugnet/Zotero/storage/JGK5GAAW/Beck - 2013.pdf;/Users/lbugnet/Zotero/storage/T3K6NWE6/Beck - 2013.pdf}
}

@article{Beck2014,
  title = {Pulsating Red Giant Stars in Eccentric Binary Systems Discovered from {{Kepler}} Space-Based Photometry: {{A}} Sample Study and the Analysis of {{KIC}} 5006817},
  author = {Beck, P. G. and Hambleton, K. and Vos, J. and Kallinger, T. and Bloemen, S. and Tkachenko, A. and Garc{\'i}a, R. A. and {\O}stensen, R. H. and Aerts, C. and Kurtz, D. W. and De Ridder, J. and Hekker, S. and Pavlovski, K. and Mathur, S. and De Smedt, K. and Derekas, A. and Corsaro, E. and Mosser, B. and Van Winckel, H. and Huber, D. and Degroote, P. and Davies, G. R. and Pr{\v s}a, A. and Debosscher, J. and Elsworth, Y. and Nemeth, P. and Siess, L. and Schmid, V. S. and P{\'a}pics, P. I. and De Vries, B. L. and Van Marle, A. J. and {Marcos-Arenal}, P. and Lobel, A.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {564},
  pages = {1--18},
  issn = {14320746},
  doi = {10.1051/0004-6361/201322477},
  abstract = {Context. The unparalleled photometric data obtained by NASA's Kepler Space Telescope has led to improved understanding of red giant stars and binary stars. Seismology allows us to constrain the properties of red giants. In addition to eclipsing binaries, eccentric non-eclipsing binaries that exhibit ellipsoidal modulations have been detected with Kepler. Aims. We aim to study the properties of eccentric binary systems containing a red giant star and to derive the parameters of the primary giant component. Methods. We applied asteroseismic techniques to determine the masses and radii of the primary component of each system. For a selected target, light and radial velocity curve modelling techniques were applied to extract the parameters of the system and its primary component. Stellar evolution and its effects on the evolution of the binary system were studied from theoretical models. Results. The paper presents the asteroseismic analysis of 18 pulsating red giants in eccentric binary systems, for which masses and radii were constrained. The orbital periods of these systems range from 20 to 440 days. The results of our ongoing radial velocity monitoring programme with the Hermes spectrograph reveal an eccentricity range of e = 0.2 to 0.76. As a case study we present a detailed analysis of KIC 5006817, whose rich oscillation spectrum allows for detailed seismic analysis. From seismology we constrain the rotational period of the envelope to be at least 165 d, which is roughly twice the orbital period. The stellar core rotates 13 times faster than the surface. From the spectrum and radial velocities we expect that the Doppler beaming signal should have a maximum amplitude of 300 ppm in the light curve. Fixing the mass and radius to the asteroseismically determined values, we find from our binary modelling a value of the gravity darkening exponent that is significantly larger than expected. Through binary modelling, we determine the mass of the secondary component to be 0.29 {$\pm$} 0.03 Mmiddot;. Conclusions. For KIC 5006817 we exclude pseudo-synchronous rotation of the red giant with the orbit. The comparison of the results from seismology and modelling of the light curve shows a possible alignment of the rotational and orbital axis at the 2{$\sigma$} level. Red giant eccentric systems could be progenitors of cataclysmic variables and hot subdwarf B stars. \textcopyright{} 2014 ESO.},
  keywords = {Asteroseismology,Binaries: general,notion,notion-database,Stars: individual: KIC5006817,Stars: rotation,Stars: solar-type,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/G47VBWMX/Beck et al. - 2014.pdf}
}

@article{Beck2016,
  title = {The {{HERMES}} Solar Atlas and the Spectroscopic Analysis of the Seismic Solar Analogue {{KIC}} 3241581},
  author = {Beck, P. G. and Allende Prieto, C. and Van Reeth, T. and Tkachenko, A. and Raskin, G. and Van Winckel, H. and Do Nascimento, J. D. and Salabert, D. and Corsaro, E. and Garc{\'i}a, R. A.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {589},
  eprint = {1511.06583},
  pages = {1--12},
  issn = {14320746},
  doi = {10.1051/0004-6361/201425423},
  abstract = {Context. Solar-analogue stars provide an excellent resource to study the Sun's evolution, i.e. the changes with time in stellar structure, activity, or rotation for solar-like stars. The unparalleled photometric data from the NASA space telescope Kepler allows us to study and characterise solar-like stars through asteroseismology. Aims. We aim to spectroscopically investigate the fundamental parameter and chromospheric activity of solar analogues and twins, based on observations obtained with the HERMES spectrograph and combine them with asteroseismology. Therefore, we need to build a solar atlas for the spectrograph, to provide accurate calibrations of the spectroscopically determined abundances of solar- and late-type stars observed with this instrument and thus perform differential spectroscopic comparisons. Methods. We acquire high-resolution and high signal-to-noise (S/N) spectroscopy to construct three solar reference spectra by observing the reflected light of the asteroids Vesta and Victoria and the jovian moon Europa (100 {$\leq$} S/N {$\leq$} 450) with the HERMES spectrograph. We then observe the Kepler solar analogue KIC 3241581 (S/N \textasciitilde{} 170). For this star, the fundamental spectral parameters are extracted using a differential analysis. Sufficient S/N in the near ultraviolet allows us to investigate the chromospheric magnetic activity in both objects. Results. We constructed three solar spectrum atlases from 385 to 900 nm, obtained with the HERMES spectrograph from observations of two bright asteroids and a jovian moon. A comparison between our solar spectra atlas to the Kurucz and HARPS solar spectrum shows an excellent agreement. KIC 3241581 was found to be a long-periodic binary system. The fundamental parameter for the stellar primary component are Teff = 5689 {$\pm$} 11 K, log g = 4.385 {$\pm$} 0.005, [Fe/H] = + 0.22 {$\pm$} 0.01, being in agreement with the published global seismic values, which confirms its status as solar analogue. The chromospheric activity level is compatible with the solar magnetic activity observed during 2014 and 2015. Conclusions. Our solar atlas is an essential tool for the analysis of solar-like stars and to characterise solar analogues and twins with HERMES. The differential analysis, using the presented solar atlas from HERMES observations allows us to obtain the fundamental parameters with very high accuracy. KIC 3241581 is a metal-rich solar analogue with a solar-like activity level in a binary system of unknown period.},
  archiveprefix = {arxiv},
  keywords = {Methods: observational,notion,notion-database,Stars: fundamental parameters,Stars: solar-type,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/G2VQIXUE/Beck et al. - 2016.pdf}
}

@article{Beckers1968,
  title = {Photospheric Brightness Differences Associated with the Solar Supergranulation},
  author = {Beckers, Jacques M.},
  year = {1968},
  month = nov,
  journal = {Solar Physics},
  volume = {5},
  number = {3},
  pages = {309--322},
  publisher = {{Kluwer Academic Publishers}},
  issn = {00380938},
  doi = {10.1007/BF00147143},
  urldate = {2020-03-23},
  abstract = {The large scale ({$>$} 5000 km) intensity structure of the photosphere has been examined. The power per frequency unit indicates a continuous increase towards smaller spatial frequency. No excess power exists at wavelengths near the size of the supergranulation (30000 km) or at any other wavelength between 5000 and 100000 km. However, direct measurement of the intensity distribution in 1652 supergranulation cells shows a very small increase of the intensity towards the cell boundary. The amount of this increase is larger near the solar limb. It is probably due to a weak continuum emission associated with the chromospheric network. Any temperature difference arising from the supergranulation convection is obscured by this emission and is probably less than 1 K. \textcopyright{} 1968 D. Reidel Publishing Company.},
  keywords = {notion,notion-database}
}

@article{Beckers1975,
  title = {The Line Response Fucntion of the Stellar Atmospheres and the Effective Depth of Line Formation},
  author = {Beckers, Jacques M. and Milkey, Robert W.},
  year = {1975},
  journal = {Solar Physics},
  volume = {43},
  eprint = {1011.1669v3},
  pages = {289--292},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/7ZEFL4VB/Beckers, Milkey - 1975.pdf}
}

@article{Bedding2004,
  title = {Oscillation {{Frequencies}} and {{Mode Lifetimes}} in {$\alpha$} {{Centauri A}}},
  author = {Bedding, Timothy R. and Kjeldsen, Hans and Butler, R. Paul and McCarthy, Chris and Marcy, Geoffrey W. and O'Toole, Simon J. and Tinney, Christopher G. and Wright, Jason T.},
  year = {2004},
  journal = {The Astrophysical Journal},
  volume = {614},
  number = {1},
  eprint = {astro-ph/0406471},
  pages = {380--385},
  issn = {0004-637X},
  doi = {10.1086/423484},
  abstract = {We analyse our recently-published velocity measurements of alpha Cen A (Butler et al. 2004). After adjusting the weights on a night-by-night basis in order to optimize the window function to minimize sidelobes, we extract 42 oscillation frequencies with l=0 to 3 and measure the large and small frequency separations. We give fitted relations to these frequencies that can be compared with theoretical models and conclude that the observed scatter about these fits is due to the finite lifetimes of the oscillation modes. We estimate the mode lifetimes to be 1-2 d, substantially shorter than in the Sun.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WRDNR55X/Bedding et al. - 2004.pdf}
}

@article{Bedding2005,
  title = {The Non-Detection of Oscillations in {{Procyon}} by {{MOST}}: {{Is}} It Really a Surprise?},
  author = {Bedding, T. R. and Kjeldsen, H. and Bouchy, F. and Bruntt, H. and Butler, R. P. and Buzasi, D. L. and {Christensen-Dalsgaard}, J. and Frandsen, S. and Lebrun, J. C. and Marti{\'c}, M. and Schou, J.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {432},
  number = {2},
  pages = {43--48},
  issn = {00046361},
  doi = {10.1051/0004-6361:200500019},
  abstract = {We argue that the non-detection of oscillations in Procyon by the MOST satellite reported by Matthews et al. (2004) is fully consistent with published ground-based velocity observations of this star. We also examine the claims that the MOST observations represent the best photometric precision so far reported in the literature by about an order of magnitude and are the most sensitive data set for asteroseismology available for any star other than the Sun. These statements are not correct, with the most notable exceptions being observations of oscillations in {$\alpha$} Cen A that are far superior. We further disagree that the hump of excess power seen repeatedly from velocity observations of Procyon can be explained as an artefact caused by gaps in the data. The MOST observations failed to reveal oscillations clearly because their noise level is too high, possibly from scattered Earthlight in the instrument. We did find an excess of strong peaks in the MOST amplitude spectrum that is inconsistent with a simple noise source such as granulation, and may perhaps indicate oscillations at roughly the expected level. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Stars: individual: Procyon,Stars: oscillations,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ARXQBKH2/Bedding et al. - 2005.pdf}
}

@article{Bedding2006,
  title = {Joint {{Discussion}} 17 {{Highlights}} of Recent Progress in the Seismology of the {{Sun}} and {{Sun-like}} Stars},
  author = {Bedding, Timothy R. and Brun, Allan S. and {Christensen-Dalsgaard}, J{\o}rgen and Crouch, Ashley and De Cat, Peter and Garc{\'i}a, Raphael A. and Gizon, Laurent and Hill, Frank and Kjeldsen, Hans and Leibacher, John W. and Maillard, Jean Pierre and Mathis, S. and {Rabello-Soares}, M. Cristina and Rozelot, Jean Pierre and Rempel, Matthias and Roxburgh, Ian W. and Samadi, R{\'e}za and Talon, Suzanne and Thompson, Michael J.},
  year = {2006},
  journal = {Proceedings of the International Astronomical Union},
  volume = {2},
  number = {14},
  pages = {491--516},
  issn = {17439213},
  doi = {10.1017/S1743921307011635},
  abstract = {The seismology and physics of localized structures beneath the surface of the Sun takes on a special significance with the completion in 2006 of a solar cycle of observations by the ground-based Global Oscillation Network Group (GONG) and by the instruments on board the Solar and Heliospheric Observatory (SOHO). Of course, the spatially unresolved Birmingham Solar Oscillation Network (BiSON) has been observing for even longer. At the same time, the testing of models of stellar structure moves into high gear with the extension of deep probes from the Sun to other solar-like stars and other multi-mode pulsators, with ever-improving observations made from the ground, the success of the MOST satellite, and the recently launched CoRoT satellite. Here we report the current state of the two closely related and rapidly developing fields of helio- and asteroseimology. \textcopyright{} 2007 International Astronomical Union.},
  keywords = {notion,notion-database,Space vehicles: instruments,Stars: interiors,Stars: oscillations (including pulsations),Stars: rotation,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/CLMZVA6M/Bedding et al. - 2006(2).pdf}
}

@article{Bedding2006a,
  title = {Solar-like {{Oscillations}} in the {{Metal}}-poor {{Subgiant}} {$\nu$} {{Indi}}: {{Constraining}} the {{Mass}} and {{Age Using Asteroseismology}}},
  author = {Bedding, Timothy R. and Butler, R. Paul and Carrier, Fabien and Bouchy, Francois and Brewer, Brendon J. and Eggenberger, Patrick and Grundahl, Frank and Kjeldsen, Hans and McCarthy, Chris and Nielsen, Tine Bjorn and Retter, Alon and Tinney, Christopher G.},
  year = {2006},
  journal = {The Astrophysical Journal},
  volume = {647},
  number = {1},
  eprint = {astro-ph/0604453},
  pages = {558--563},
  issn = {0004-637X},
  doi = {10.1086/505295},
  abstract = {Asteroseismology is a powerful method for determining fundamental properties of stars. We report the first application to a metal-poor object, namely the subgiant star nu Ind. We measured precise velocities from two sites, allowing us to detect oscillations and infer a large frequency separation of Delta\_nu = 24.25 +/- 0.25 microHz. Combining this value with the location of the star in the H-R diagram and comparing with standard evolutionary models, we were able to place constraints on the stellar parameters. In particular, our results indicate that nu Ind has a low mass (0.85 +/- 0.04 M\_sun) and is at least 9 Gyr old.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4N6F45CG/Bedding et al. - 2006.pdf}
}

@article{Bedding2007,
  title = {Observations of Solar-like Oscillations},
  author = {Bedding, Timothy R and Kjeldsen, Hans},
  year = {2007},
  volume = {150},
  number = {F5 V},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NAZGKKYQ/Bedding, Kjeldsen - 2007.pdf}
}

@article{Bedding2007a,
  title = {Solar-like {{Oscillations}} in the {{G2 Subgiant}} {$\beta$} {{Hydri}} from {{Dual}}-{{Site Observations}}},
  author = {Bedding, Timothy R. and Kjeldsen, Hans and Arentoft, Torben and Bouchy, Francois and Brandbyge, Jacob and Brewer, Brendon J. and Butler, R. Paul and Christensen-Dalsgaard, Jorgen and Dall, Thomas and Frandsen, Soren and Karoff, Christoffer and Kiss, Laszlo L. and Monteiro, Mario J. P. F. G. and Pijpers, Frank P. and Teixeira, Teresa C. and Tinney, C. G. and Baldry, Ivan K. and Carrier, Fabien and O'Toole, Simon J.},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {663},
  number = {2},
  eprint = {astro-ph/0703747},
  pages = {1315--1324},
  issn = {0004-637X},
  doi = {10.1086/518593},
  abstract = {We have observed oscillations in the nearby G2 subgiant star beta Hyi using high-precision velocity observations obtained over more than a week with the HARPS and UCLES spectrographs. The oscillation frequencies show a regular comb structure, as expected for solar-like oscillations, but with several l=1 modes being strongly affected by avoided crossings. The data, combined with those we obtained five years earlier, allow us to identify 28 oscillation modes. By scaling the large frequency separation from the Sun, we measure the mean density of beta Hyi to an accuracy of 0.6\%. The amplitudes of the oscillations are about 2.5 times solar and the mode lifetime is 2.3 d. A detailed comparison of the mixed l=1 modes with theoretical models should allow a precise estimate of the age of the star.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5AXT4DB6/Bedding et al. - 2007.pdf}
}

@article{Bedding2010,
  title = {A Multi-Site Campaign to Measure Solar-like Oscillations in {{Procyon}}. {{II}}. Mode Frequencies},
  author = {Bedding, Timothy R. and Kjeldsen, Hans and Campante, Tiago L. and Appourchaux, Thierry and Bonanno, Alfio and Chaplin, William J. and Garcia, Rafael A. and Marti{\'c}, Milena and Mosser, Benoit and Butler, R. Paul and Bruntt, Hans and Kiss, Lszl{\'o} L. and O'Toole, Simon J. and Kambe, Eiji and Ando, Hiroyasu and Izumiura, Hideyuki and Sato, Bun'Ei and Hartmann, Michael and Hatzes, Artie and Barban, Caroline and Berthomieu, Gabrielle and Michel, Eric and Provost, Janine and {Turck-Chi{\`e}ze}, Sylvaine and Lebrun, Jean Claude and Schmitt, Jerome and Bertaux, Jean Loup and Benatti, Serena and Claudi, Riccardo U. and Cosentino, Rosario and Leccia, Silvio and Frandsen, S{\o}ren and Brogaard, Karsten and Glowienka, Lars and Grundahl, Frank and Stempels, Eric and Arentoft, Torben and Bazot, Micha{\"e}l and {Christensen-Dalsgaard}, J{\o}rgen and Dall, Thomas H. and Karoff, Christoffer and {Lundgreen-Nielsen}, Jens and Carrier, Fabien and Eggenberger, Patrick and Sosnowska, Danuta and Wittenmyer, Robert A. and Endl, Michael and Metcalfe, Travis S. and Hekker, Saskia and Reffert, Sabine},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {713},
  number = {2},
  pages = {935--949},
  issn = {15384357},
  doi = {10.1088/0004-637X/713/2/935},
  abstract = {We have analyzed data from a multi-site campaign to observe oscillations in the F5 star Procyon. The data consist of high-precision velocities that we obtained over more than three weeks with 11 telescopes. A new method for adjusting the data weights allows us to suppress the sidelobes in the power spectrum. Stacking the power spectrum in a so-called \'echelle diagram reveals two clear ridges, which we identify with even and odd values of the angular degree (l = 0 and 2, and l = 1 and 3, respectively). We interpret a strong, narrow peak at 446{$\mu$}Hz that lies close to the l = 1 ridge as a mode with mixed character. We show that the frequencies of the ridge centroids and their separations are useful diagnostics for asteroseismology. In particular, variations in the large separation appear to indicate a glitch in the sound-speed profile at an acoustic depth of 1000s. We list frequencies for 55 modes extracted from the data spanning 20 radial orders, a range comparable to the best solar data, which will provide valuable constraints for theoretical models. A preliminary comparison with published models shows that the offset between observed and calculated frequencies for the radial modes is very different for Procyon than for the Sun and other cool stars. We find the mean lifetime of the modes in Procyon to be 1.29+0.55-0.49days, which is significantly shorter than the 2-4days seen in the Sun. \textcopyright{} 2010 The American Astronomical Society.},
  keywords = {notion,notion-database,Stars: individual (Procyon A),Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/CRPMD69M/Bedding et al. - 2010.pdf}
}

@article{Bedding2010a,
  title = {Solar-like Oscillations in Low-Luminosity Red Giants: {{First}} Results from Kepler},
  author = {Bedding, T. R. and Huber, D. and Stello, D. and Elsworth, Y. P. and Hekker, S. and Kallinger, T. and Mathur, S. and Mosser, B. and Preston, H. L. and Ballot, J. and Barban, C. and Broomhall, A. M. and Buzasi, D. L. and Chaplin, W. J. and Garc{\'i}a, R. A. and Gruberbauer, M. and Hale, S. J. and De Ridder, J. and Frandsen, S. and Borucki, W. J. and Brown, T. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Jenkins, J. M. and Kjeldsen, H. and Koch, D. and Belkacem, K. and Bildsten, L. and Bruntt, H. and Campante, T. L. and Deheuvels, S. and Derekas, A. and Dupret, M. A. and Goupil, M. J. and Hatzes, A. and Houdek, G. and Ireland, M. J. and Jiang, C. and Karoff, C. and Kiss, L. L. and Lebreton, Y. and Miglio, A. and Montalbn, J. and Noels, A. and Roxburgh, I. W. and Sangaralingam, V. and Stevens, I. R. and Suran, M. D. and Tarrant, N. J. and Weiss, A.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0229},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L176},
  abstract = {We have measured solar-like oscillations in red giants using time-series photometry from the first 34 days of science operations of the Kepler Mission. The light curves, obtained with 30 minute sampling, reveal clear oscillations in a large sample of G and K giants, extending in luminosity from the red clump down to the bottom of the giant branch. We confirm a strong correlation between the large separation of the oscillations ({$\Delta\nu$}) and the frequency of maximum power ({$\nu$}max). We focus on a sample of 50 low-luminosity stars ({$\nu$}max {$>$} 100 {$\mu$}Hz, L {$\lessequivlnt$} 30L) having high signal-to-noise ratios and showing the unambiguous signature of solar-like oscillations. These are H-shell-burning stars, whose oscillations should be valuable for testing models of stellar evolution and for constraining the star formation rate in the local disk. We use a new technique to compare stars on a single \'echelle diagram by scaling their frequencies and find well-defined ridges corresponding to radial and non-radial oscillations, including clear evidence for modes with angular degree l = 3. Measuring the small separation between l = 0 and l = 2 allows us to plot the so-called C-D diagram of {$\delta\nu$}02 versus {$\Delta\nu$}. The small separation {$\delta\nu$}01 of l = 1 from the midpoint of adjacent l = 0 modes is negative, contrary to the Sun and solar-type stars. The ridge for l = 1 is notably broadened, which we attribute to mixed modes, confirming theoretical predictions for low-luminosity giants. Overall, the results demonstrate the tremendous potential of Kepler data for asteroseismology of red giants. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/C5GZ3N32/Bedding et al. - 2010(2).pdf}
}

@article{Bedding2011,
  title = {Gravity Modes as a Way to Distinguish between Hydrogen- and Helium-Burning Red Giant Stars},
  author = {Bedding, Timothy R. and Mosser, Benoit and Huber, Daniel and Montalb{\'a}n, Josefina and Beck, Paul and {Christensen-Dalsgaard}, J{\o}rgen and Elsworth, Yvonne P. and Garc{\'i}a, Rafael A. and Miglio, Andrea and Stello, Dennis and White, Timothy R. and De Ridder, Joris and Hekker, Saskia and Aerts, Conny and Barban, Caroline and Belkacem, Kevin and Broomhall, Anne Marie and Brown, Timothy M. and Buzasi, Derek L. and Carrier, Fabien and Chaplin, William J. and Di Mauro, Maria Pia and Dupret, Marc Antoine and Frandsen, S{\"o}ren and Gilliland, Ronald L. and Goupil, Marie Jo and Jenkins, Jon M. and Kallinger, Thomas and Kawaler, Steven and Kjeldsen, Hans and Mathur, Savita and Noels, Arlette and Aguirre, Victor Silva and Ventura, Paolo},
  year = {2011},
  journal = {Nature},
  volume = {471},
  number = {7340},
  eprint = {1103.5805},
  pages = {608--611},
  issn = {00280836},
  doi = {10.1038/nature09935},
  abstract = {Red giants are evolved stars that have exhausted the supply of hydrogen in their cores and instead burn hydrogen in a surrounding shell. Once a red giant is sufficiently evolved, the helium in the core also undergoes fusion. Outstanding issues in our understanding of red giants include uncertainties in the amount of mass lost at the surface before helium ignition and the amount of internal mixing from rotation and other processes. Progress is hampered by our inability to distinguish between red giants burning helium in the core and those still only burning hydrogen in a shell. Asteroseismology offers a way forward, being a powerful tool for probing the internal structures of stars using their natural oscillation frequencies. Here we report observations of gravity-mode period spacings in red giants that permit a distinction between evolutionary stages to be made. We use high-precision photometry obtained by the Kepler spacecraft over more than a year to measure oscillations in several hundred red giants. We find many stars whose dipole modes show sequences with approximately regular period spacings. These stars fall into two clear groups, allowing us to distinguish unambiguously between hydrogen-shell-burning stars (period spacing mostly -450seconds) and those that are also burning helium (period spacing-100 to 300 seconds). \textcopyright{} 2011 Macmillan Publishers Limited. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6XSZHQ2C/Bedding et al. - 2011.pdf}
}

@article{Bedding2014,
  title = {Solar-like {{Oscillations}}},
  author = {Bedding, Timothy R and Kjeldsen, Hans},
  year = {2014},
  journal = {Asteroseismology, 22nd Canary Islands Winter School of Astrophysics.},
  pages = {203--212},
  keywords = {notion,notion-database,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/8G3SDT82/Bedding, Kjeldsen - 2019.pdf}
}

@article{Bedding2020,
  title = {Very Regular High-Frequency Pulsation Modes in Young Intermediate-Mass Stars},
  author = {Bedding, Timothy R. and Murphy, Simon J. and Hey, Daniel R. and Huber, Daniel and Li, Tanda and Smalley, Barry and Stello, Dennis and White, Timothy R. and Ball, Warrick H. and Chaplin, William J. and Colman, Isabel L. and Fuller, Jim and Gaidos, Eric and Harbeck, Daniel R. and Hermes, J. J. and Holdsworth, Daniel L. and Li, Gang and Li, Yaguang and Mann, Andrew W. and Reese, Daniel R. and Sekaran, Sanjay and Yu, Jie and Antoci, Victoria and Bergmann, Christoph and Brown, Timothy M. and Howard, Andrew W. and Ireland, Michael J. and Isaacson, Howard and Jenkins, Jon M. and Kjeldsen, Hans and McCully, Curtis and Rabus, Markus and Rains, Adam D. and Ricker, George R. and Tinney, Christopher G. and Vanderspek, Roland K.},
  year = {2020},
  month = may,
  journal = {Nature},
  volume = {581},
  number = {7807},
  eprint = {2005.06157},
  pages = {147--151},
  publisher = {{Nature Research}},
  issn = {14764687},
  doi = {10.1038/s41586-020-2226-8},
  abstract = {Asteroseismology probes the internal structures of stars by using their natural pulsation frequencies1. It relies on identifying sequences of pulsation modes that can be compared with theoretical models, which has been done successfully for many classes of pulsators, including low-mass solar-type stars2, red giants3, high-mass stars4 and white dwarfs5. However, a large group of pulsating stars of intermediate mass\textemdash the so-called {$\delta$} Scuti stars\textemdash have rich pulsation spectra for which systematic mode identification has not hitherto been possible6,7. This arises because only a seemingly random subset of possible modes are excited and because rapid rotation tends to spoil regular patterns8\textendash 10. Here we report the detection of remarkably regular sequences of high-frequency pulsation modes in 60 intermediate-mass main-sequence stars, which enables definitive mode identification. The space motions of some of these stars indicate that they are members of known associations of young stars, as confirmed by modelling of their pulsation spectra.},
  archiveprefix = {arxiv},
  pmid = {32405022},
  keywords = {notion,notion-database}
}

@article{Beeck2015,
  title = {Three-Dimensional Simulations of near-Surface Convection in Main-Sequence Stars: {{IV}}. {{Effect}} of Small-Scale Magnetic Flux Concentrations on Centre-to-Limb Variation and Spectral Lines},
  author = {Beeck, B. and Sch{\"u}ssler, M. and Cameron, R. H. and Reiners, A.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {581},
  eprint = {1505.04744},
  pages = {1--16},
  issn = {14320746},
  doi = {10.1051/0004-6361/201525874},
  abstract = {Context. Magnetic fields affect the local structure of the photosphere of stars. They can considerably influence the radiative properties near the optical surface, flow velocities, and the temperature and pressure profiles. This has an impact on observables such as limb darkening and spectral line profiles. Aims. We aim at understanding qualitatively the influence of small magnetic flux concentrations in unipolar plage regions on the centre-to-limb variation of the intensity and its contrast and on the shape of spectral line profiles in cool main-sequence stars. Methods. We analyse the bolometric and continuum intensity and its angular dependence of 24 radiative magnetohydrodynamic simulations of the near-surface layers of main-sequence stars with six different sets of stellar parameters (spectral types F to early M) and four different average magnetic field strengths (including the non-magnetic case). We also calculated disc-integrated profiles of three spectral lines. Results. The small magnetic flux concentrations formed in the magnetic runs of simulations have a considerable impact on the intensity and its centre-to-limb variation. In some cases, the difference in limb darkening between magnetic and non-magnetic runs is larger than the difference between the spectral types. Spectral lines are not only broadened owing to the Zeeman effect, but are also strongly affected by the modified thermodynamical structure and flow patterns. This indirect magnetic impact on the line profiles is often bigger than that of the Zeeman effect. Conclusions. The effects of the magnetic field on the radiation leaving the star can be considerable and is not restricted to spectral line broadening and polarisation by the Zeeman effect. The inhomogeneous structure of the magnetic field on small length scales and its impact on (and spatial correlation with) the local thermodynamical structure and the flow field near the surface influence the measurement of the global field properties and stellar parameters. These effects need to be taken into account in the interpretation of observations.},
  archiveprefix = {arxiv},
  keywords = {line: profiles,magnetic fields,magnetohydrodynamics (MHD),notion,notion-database,radiative transfer,stars: low-mass,stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/PGQYCC66/Beeck et al. - 2015.pdf}
}

@article{Bekki2022,
  title = {Theory of Solar Oscillations in the Inertial Frequency Range: {{Linear}} Modes of the Convection Zone},
  author = {Bekki, Yuto and Cameron, Robert H and Gizon, Laurent},
  year = {2022},
  journal = {Astronomy \& Astrophysics},
  eprint = {2203.04442v1},
  urldate = {2022-04-05},
  abstract = {Context. On the one hand, several types of global-scale inertial modes of oscillation have been observed on the Sun. They include the equatorial Rossby modes, critical-latitude modes, and high-latitude modes. On the other hand, the columnar convective modes (predicted by simulations; also known as banana cells or thermal Rossby waves) remain elusive. Aims. We aim to investigate the influence of turbulent diffusivities, non-adiabatic stratification, differential rotation, and a latitudinal entropy gradient on the linear global modes of the rotating solar convection zone. Methods. We solve numerically for the eigenmodes of a rotating compressible fluid inside a spherical shell. The model takes into account the solar stratification, turbulent diffusivities, differential rotation (determined by helioseismology), and the latitudinal entropy gradient. As a starting point, we restrict ourselves to a superadiabaticity and turbulent diffusivities that are uniform in space. We identify modes in the inertial frequency range including the columnar convective modes, as well as modes of mixed character. The corresponding mode dispersion relations and eigenfunctions are computed for azimuthal orders m {$\leq$} 16. Results. The three main results are as follows. Firstly, we find that, for m 5, the radial dependence of the equatorial Rossby modes with no radial node (n = 0) is radically changed from the traditional expectation (r m) for turbulent diffusivities 10 12 cm 2 s -1. Secondly, we find mixed modes, i.e. modes that share properties of the equatorial Rossby modes with one radial node (n = 1) and the columnar convective modes, which are not substantially affected by turbulent diffusion. Thirdly, we show that the m = 1 high-latitude mode in the model is consistent with the solar observations when the latitudinal entropy gradient corresponding to a thermal wind balance is included (baroclinally unstable mode). Conclusions. To our knowledge, this work is the first realistic eigenvalue calculation of the global modes of the rotating solar con-vection zone. This calculation reveals a rich spectrum of modes in the inertial frequency range, which can be directly compared to the observations. In turn, the observed modes can inform us about the solar convection zone.},
  archiveprefix = {arxiv},
  keywords = {convection-Sun,helioseismology,interior-Sun,notion,notion-database,rotation-Sun},
  file = {/Users/lbugnet/Zotero/storage/GH6W56NL/full-text.pdf}
}

@article{Belkacem2006,
  title = {A Closure Model with Plumes {{I}}. {{The}} Solar Convection},
  author = {Belkacem, K. and Samadi, R. and Goupil, M. J. and Kupka, F.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {460},
  number = {1},
  pages = {173--182},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065369},
  abstract = {Context. Oscillations of stellar p modes, excited by turbulent convection, are investigated. In the uppermost part of the solar convection zone, radiative cooling is responsible for the formation of turbulent plumes, hence the medium is modelled with downdrafts and updrafts. Aims. We take into account the asymmetry of the up- and downflows created by turbulent plumes through an adapted closure model. In a companion paper, we apply it to the formalism of excitation of solar p modes developed by Samadi \& Goupil (2001). Methods. Using results from 3D numerical simulations of the uppermost part of the solar convection zone, we show that the two-scale mass-flux model (TFM) is valid only for quasi-laminar or highly skewed flows (Gryanik \& Hartmann 2002) and does not reproduce turbulent properties of the medium such as velocity-correlation products. We build a generalized two-scale mass-flux Model (GTFM) model that takes both the skew introduced by the presence of two flows and the effects of turbulence in each flow into account. In order to apply the GTFM to the solar case, we introduce the plume dynamics as modelled by Rieutord \& Zahn (1995) and construct a closure model with plumes (CMP). Results. The CMP enables expressing the third- and fourth-order correlation products in terms of second-order ones. When compared with 3D simulation results, the CMP improves the agreement for the fourth-order moments by a factor of two approximately compared with the use of the quasi-normal approximation or a skewness computed with the classical TFM. Conclusions. The asymmetry of turbulent convection in the solar case has an important impact on the vertical-velocity fourth-order moment, which has to be accounted for by models. The CMP is a significant improvement and is expected to improve the modelling of solar p-mode excitation. \textcopyright{} ESO 2006.},
  keywords = {Convection,notion,notion-database,Sun: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/CSUTQ5WU/Belkacem et al. - 2006.pdf}
}

@article{Belkacem2006a,
  title = {A Closure Model for Turbulent Convection. {{Application}} to the Excitation of p Modes},
  author = {Belkacem, K. and Samadi, R. and Goupil, M. J. and Kupka, F. and Baudin, F.},
  year = {2006},
  journal = {Proceedings of the International Astronomical Union},
  volume = {2},
  number = {S239},
  pages = {376--378},
  issn = {17439213},
  doi = {10.1017/S1743921307000762},
  abstract = {Oscillations of stellar p modes excited by turbulent convection are investigated. In the uppermost part of the solar convection zone, radiative cooling is responsible for the formation of turbulent plumes, hence the medium is characterized with downdrafts and updrafts. The motivation is to take the asymmetry of up- and downflows created by turbulent plumes into account through an adapted closure model. We built a generalized two-scale mass-flux model (GTFM) that considers both the skew introduced by the presence of two flows and the effect of turbulence onto each flow. In order to apply the GTFM to the solar case, we introduce the plume dynamics as modelled by Rieutord \& Zahn (1995) and construct a closure model with plumes (CMP). The CMP enables to express third- and fourth-order velocity correlation products in terms of the second-order ones. When comparing with 3D numerical simulation results, the CMP improves the agreement for the fourth order moments in comparison with the quasi-normal approximation (QNA) or the classical mass-flux model (MFM). This excitation model reproduces the maximum of the power supplied to solar p modes, when compared with GOLF observations. \textcopyright{} 2007 International Astronomical Union.},
  keywords = {Convection,notion,notion-database,Sun: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/VFJ9QVL9/Belkacem et al. - 2006(2).pdf}
}

@article{Belkacem2008,
  title = {Stochastic Excitation of Non-Radial Modes: {{I}}. {{High-angular-degree}} p Modes},
  author = {Belkacem, K. and Samadi, R. and Goupil, M. J. and Dupret, M. A.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {478},
  number = {1},
  pages = {163--174},
  issn = {00046361},
  doi = {10.1051/0004-6361:20077775},
  abstract = {Context.Turbulent motions in stellar convection zones generate acoustic energy, part of which is then supplied to normal modes of the star. Their amplitudes result from a balance between the efficiencies of excitation and damping processes in the convection zones. Aims.We develop a formalism that provides the excitation rates of non-radial global modes excited by turbulent convection. As a first application, we estimated the impact of non-radial effects on excitation rates and amplitudes of the high-angular-degree modes that are observed on the Sun. Methods.A model of stochastic excitation by turbulent convection was developed to compute the excitation rates and then successfully applied to solar radial modes. We generalise this approach to the case of non-radial global modes. This enables us to estimate the energy supplied to high-() acoustic modes. Qualitative arguments, as well as numerical calculations, are used to illustrate the results. Results.We find that non-radial effects for modes are non-negligible: - For high- modes (i.e. typically n {$>$} 3) and for high values of , the power supplied to the oscillations depends on the mode inertia. - For low- modes, independent of the value of , the excitation is dominated by the non-radial components of the Reynolds stress term. Conclusions.Our numerical investigation of high- modes shows that the validity of the present formalism is limited to {$<$} 500 due to the spatial separation of scale assumption. Thus, a model for very high- -mode excitation rates calls for further theoretical developments; however, the formalism is valid for solar modes, which will be investigated in a paper in preparation. \textcopyright{} 2008 ESO.},
  keywords = {Convection,notion,notion-database,Sun: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/95NXG7WC/Belkacem et al. - 2008.pdf}
}

@article{Belkacem2009,
  title = {Solar-like Oscillations in Massive Main-Sequence Stars. {{I}}. {{Asteroseismic}} Signatures of the Driving and Damping Regions},
  author = {Belkacem, K. and Dupret, M. A. and Noels, A.},
  year = {2009},
  month = nov,
  eprint = {0911.0908},
  doi = {10.1051/0004-6361/200913221},
  urldate = {2020-06-26},
  abstract = {Motivated by the recent detection of stochastically excited modes in the massive star V1449 Aql (Belkacem et al., 2009b), already known to be a \$\textbackslash beta\$ Cephei, we theoretically investigate the driving by turbulent convection. By using a full non-adiabatic computation of the damping rates, together with a computation of the energy injection rates, we provide an estimate of the amplitudes of modes excited by both the convective region induced by the iron opacity bump and the convective core. Despite uncertainties in the dynamical properties of such convective regions, we demonstrate that both are able to efficiently excite \$p\$ modes above the CoRoT observational threshold and the solar amplitudes. In addition, we emphasise the potential asteroseismic diagnostics provided by each convective region, which we hope will help to identify the one responsible for solar-like oscillations, and to give constraints on this convective zone. A forthcoming work will be dedicated to an extended investigation of the likelihood of solar-like oscillations across the Hertzsprung-Russell diagram.},
  archiveprefix = {arxiv},
  keywords = {convection-waves-stars,notion,notion-database,oscillations},
  file = {/Users/lbugnet/Zotero/storage/AY82WQPJ/full-text.pdf}
}

@article{Belkacem2009a,
  title = {Mode Excitation by Turbulent Convection in Rotating Stars},
  author = {Belkacem, K. and Mathis, S. and Goupil, M. J. and Samadi, R.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {508},
  number = {1},
  pages = {345--353},
  issn = {00046361},
  doi = {10.1051/0004-6361/200912284},
  abstract = {We focus on the influence of the Coriolis acceleration on the stochastic excitation of oscillation modes in convective regions of rotating stars. Our aim is to estimate the asymmetry between excitation rates of prograde and retrograde modes. We extend the formalism derived for obtaining stellar p-and g-mode amplitudes (Samadi \& Goupil 2001, A\&A, 370, 136; Belkacem et al. 2008, A\&A, 478, 163) to include the effect of the Coriolis acceleration. We then study the special case of uniform rotation for slowly rotating stars by performing a perturbative analysis. This allows us to consider the cases of the Sun and the CoRoT target HD49933. We find that, in the subsonic regime, the influence of rotation as a direct contribution to mode driving is negligible compared to the Reynolds stress contribution. In slow rotators, the indirect effect of the modification of the eigenfunctions on mode excitation is investigated by performing a perturbative analysis of the excitation rates. The excitation of solar p modes is found to be affected by rotation with excitation-rate asymmetries between prograde and retrograde modes of the order of several percent. Solar low-order g modes are also affected by uniform rotation and their excitation-rate asymmetries are found to reach 10\%. The CoRoT target HD49933 is rotating more rapidly than the Sun ({$\sigma$}/{$\sigma$} {$\approx$} 8), and we show that the resulting excitation-rate asymmetry is about 10\% for the excitation rates of p modes. We demonstrate that p and g mode excitation rates are modified by uniform rotation through the Coriolis acceleration. A study of the effect of differential rotation will be presented in a forthcoming paper. \textcopyright{} 2009 ESO.},
  keywords = {Convection,convection-turbulence-stars,notion,notion-database,oscillations,Stars: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/YWTUXWA4/Belkacem et al. - 2009.pdf}
}

@article{Belkacem2009b,
  title = {Solar-like Oscillations in a Massive Star},
  author = {Belkacem, K{\'e}vin and Samadi, R{\'e}za and Goupil, Marie Jo and Lef{\`e}vre, Laure and Baudin, Fr{\'e}deric and Deheuvels, S{\'e}bastien and Dupret, Marc Antoine and Appourchaux, Thierry and Scuflaire, Richard and Auvergne, Michel and Catala, Claude and Michel, Eric and Miglio, Andrea and Montalban, Josefina and Thoul, Anne and Talon, Suzanne and Baglin, Annie and Noels, Arlette},
  year = {2009},
  journal = {Science},
  volume = {324},
  number = {5934},
  pages = {1540--1542},
  issn = {00368075},
  doi = {10.1126/science.1171913},
  abstract = {Seismology of stars provides insight into the physical mechanisms taking place in their interior, with modes of oscillation probing different layers. Low-amplitude acoustic oscillations excited by turbulent convection were detected four decades ago in the Sun and more recently in low-mass main-sequence stars. Using data gathered by the Convection Rotation and Planetary Transits mission, we report here on the detection of solar-like oscillations in a massive star, V1449 Aql, which is a known large-amplitude ({$\beta$} Cephei) pulsator.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SQATZWST/Belkacem et al. - 2009(3).pdf}
}

@article{Belkacem2009c,
  title = {Stochastic Excitation of Nonradial Modes {{II}}. {{Are}} Solar Asymptotic Gravity Modes Detectable?},
  author = {Belkacem, K. and Samadi, R. and Goupil, M. J. and Dupret, M. A. and Brun, A. S. and Baudin, F.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {494},
  number = {1},
  pages = {191--204},
  issn = {00046361},
  doi = {10.1051/0004-6361:200810827},
  abstract = {Context. Detection of solar gravity modes remains a major challenge to our understanding of the inner parts of the Sun. Their frequencies would enable the derivation of constraints on the core physical properties, while their amplitudes can put severe constraints on the properties of the inner convective region. Aims. Our purpose is to determine accurate theoretical amplitudes of solar g modes and estimate the SOHO observation duration for an unambiguous detection of individual modes. We also explain differences in theoretical amplitudes derived from previous works. Methods. We investigate the stochastic excitation of modes by turbulent convection, as well as their damping. Input from a 3D global simulation of the solar convective zone is used for the kinetic turbulent energy spectrum. Damping is computed using a parametric description of the nonlocal, time-dependent, convection-pulsation interaction. We then provide a theoretical estimation of the intrinsic, as well as apparent, surface velocity. Results. Asymptotic g-mode velocity amplitudes are found to be orders of magnitude higher than previous works. Using a 3D numerical simulation from the ASH code, we attribute this to the temporal-correlation between the modes and the turbulent eddies, which is found to follow a Lorentzian law rather than a Gaussian one, as previously used. We also find that damping rates of asymptotic gravity modes are dominated by radiative losses, with a typical life time of 3 \texttimes{} 105 years for the {$\mathscr{l}$}= 1 mode at {$\nu$} = 60 {$\mu$}Hz. The maximum velocity in the considered frequency range (10-100 {$\mu$}Hz) is obtained for the {$\mathscr{l}$} = 1 mode at {$\nu$} = 60 {$\mu$}Hz and for the {$\mathscr{l}$} = 2 at {$\nu$} = 100 {$\mu$}Hz. Due to uncertainties in the modeling, amplitudes at maximum i.e. for {$\mathscr{l}$} = 1 at 60 {$\mu$}Hz can range from 3 to 6 mm s-1. The upper limit is too high, as g modes would have been easily detected with SOHO, the GOLF instrument, and this sets an upper constraint mainly on the convective velocity in the Sun. \textcopyright{} ESO 2009.},
  keywords = {Convection,notion,notion-database,Sun: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/VZ7F8CCX/Belkacem et al. - 2009(2).pdf}
}

@article{Belkacem2011,
  title = {The Underlying Physical Meaning of the {$\nu$} Max-{$\nu$} c Relation},
  author = {Belkacem, K. and Goupil, M. J. and Dupret, M. A. and Samadi, R. and Baudin, F. and Noels, A. and Mosser, B.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {530},
  pages = {1--8},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116490},
  abstract = {Asteroseismology of stars that exhibit solar-like oscillations are enjoying a growing interest with the wealth of observational results obtained with the CoRoT and Kepler missions. In this framework, scaling laws between asteroseismic quantities and stellar parameters are becoming essential tools to study a rich variety of stars. However, the physical underlying mechanisms of those scaling laws are still poorly known. Our objective is to provide a theoretical basis for the scaling between the frequency of the maximum in the power spectrum ({$\nu$}max) of solar-like oscillations and the cut-off frequency ({$\nu$}c). Using the SoHO GOLF observations together with theoretical considerations, we first confirm that the maximum of the height in oscillation power spectrum is determined by the so-called plateau of the damping rates. The physical origin of the plateau can be traced to the destabilizing effect of the Lagrangian perturbation of entropy in the upper-most layers, which becomes important when the modal period and the local thermal relaxation time-scale are comparable. Based on this analysis, we then find a linear relation between {$\nu$}max and {$\nu$}c, with a coefficient that depends on the ratio of the Mach number of the exciting turbulence to the third power to the mixing-length parameter. \textcopyright{} 2011 ESO.},
  keywords = {convection,notion,notion-database,stars: interiors,stars: oscillations,turbulence},
  file = {/Users/lbugnet/Zotero/storage/FG74TW2F/Belkacem et al. - 2011.pdf}
}

@article{Belkacem2012,
  title = {Damping Rates of Solar-like Oscillations across the {{HR}} Diagram. {{Theoretical}} Calculations Confronted to {{CoRoT}} and {{Kepler}} Observations},
  author = {Belkacem, K. and Dupret, M. A. and Baudin, F. and Appourchaux, T. and Marques, J. P. and Samadi, R.},
  year = {2012},
  month = mar,
  journal = {Astronomy \& Astrophysics},
  volume = {540},
  number = {L7},
  eprint = {1203.1737},
  doi = {10.1051/0004-6361/201218890},
  urldate = {2020-06-26},
  abstract = {Space-borne missions CoRoT and \{\textbackslash it Kepler\} are providing a rich harvest of high-quality constraints on solar-like pulsators. Among the seismic parameters, mode damping rates remains poorly understood and thus barely used to infer physical properties of stars. Nevertheless, thanks to CoRoT and \{\textbackslash it Kepler\} space-crafts it is now possible to measure damping rates for hundreds of main-sequence and thousands of red-giant stars with an unprecedented precision. By using a non-adiabatic pulsation code including a time-dependent convection treatment, we compute damping rates for stellar models representative for solar-like pulsators from the main-sequence to the red-giant phase. This allows us to reproduce the observations of both CoRoT and \{\textbackslash it Kepler\}, which validates our modeling of mode damping rates and thus the underlying physical mechanisms included in the modeling. Actually, by considering the perturbations of turbulent pressure and entropy (including perturbation of the dissipation rate of turbulent energy into heat) by the oscillation in our computation, we succeed in reproducing the observed relation between damping rates and effective temperature. Moreover, we discuss the physical reasons for mode damping rates to scale with effective temperature, as observationally exhibited. Finally, this opens the way for the use of mode damping rates to probe turbulent convection in solar-like stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Q4T4I38N/Belkacemetal2012.pdf}
}

@article{Belkacem2015,
  title = {Angular Momentum Redistribution by Mixed Modes in Evolved Low-Mass Stars: {{I}}. {{Theoretical}} Formalism},
  author = {Belkacem, K. and Marques, J. P. and Goupil, M. J. and Sonoi, T. and Ouazzani, R. M. and Dupret, M. A. and Mathis, S. and Mosser, B. and Grosjean, M.},
  year = {2015},
  journal = {Astronomy \& Astrophysics},
  volume = {579},
  pages = {1--12},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526042},
  abstract = {Seismic observations by the space-borne mission Kepler have shown that the core of red giant stars slows down while evolving, requiring an efficient physical mechanism to extract angular momentum from the inner layers. Current stellar evolution codes fail to reproduce the observed rotation rates by several orders of magnitude and instead predict a drastic spin-up of red giant cores. New efficient mechanisms of angular momentum transport are thus required. In this framework, our aim is to investigate the possibility that mixed modes extract angular momentum from the inner radiative regions of evolved low-mass stars. To this end, we consider the transformed Eulerian mean (TEM) formalism, which allows us to consider the combined effect of both the wave momentum flux in the mean angular momentum equation and the wave heat flux in the mean entropy equation as well as their interplay with the meridional circulation. In radiative layers of evolved low-mass stars, the quasi-adiabatic approximation, the limit of slow rotation, and the asymptotic regime can be applied for mixed modes and enable us to establish a prescription for the wave fluxes in the mean equations. The formalism is finally applied to a 1.3 M{$\odot$} benchmark model, representative of observed CoRoT and Kepler oscillating evolved stars. We show that the influence of the wave heat flux on the mean angular momentum is not negligible and that the overall effect of mixed modes is to extract angular momentum from the innermost region of the star. A quantitative and accurate estimate requires realistic values of mode amplitudes. This is provided in a companion paper.},
  keywords = {evolution,interiors-Stars,notion,notion-database,oscillations-Stars,rotation-Stars,Stars: evolution,Stars: interiors,Stars: oscillations,Stars: rotation,Waves,Waves-Stars},
  file = {/Users/lbugnet/Zotero/storage/B4XAL4FM/full-text.pdf;/Users/lbugnet/Zotero/storage/ZAUDFPUT/Belkacem et al. - 2015.pdf}
}

@article{Belkacem2015b,
  title = {Angular Momentum Redistribution by Mixed Modes in Evolved Low-Mass Stars {{II}}. {{Spin-down}} of the Core of Red Giants Induced by Mixed Modes},
  author = {Belkacem, K and Marques, J P and Goupil, M J and Mosser, B and Sonoi, T and Ouazzani, R M and Dupret, M A and Mathis, S and Grosjean, M},
  year = {2015},
  journal = {Astronomy \& Astrophysics},
  volume = {579},
  number = {A31},
  eprint = {1505.05452v1},
  urldate = {2020-05-13},
  abstract = {The detection of mixed modes in subgiants and red giants by the CoRoT and Kepler space-borne missions allows us to investigate the internal structure of evolved low-mass stars, from the end of the main sequence to the central helium-burning phase. In particular, the measurement of the mean core rotation rate as a function of the evolution places stringent constraints on the physical mechanisms responsible for the angular momentum redistribution in stars. It showed that the current stellar evolution codes including the modelling of rotation fail to reproduce the observations. An additional physical process that efficiently extracts angular momentum from the core is thus necessary. Our aim is to assess the ability of mixed modes to do this. To this end, we developed a formalism that provides a modelling of the wave fluxes in both the mean angular momentum and the mean energy equations in a companion paper. In this article, mode amplitudes are modelled based on recent asteroseismic observations, and a quantitative estimate of the angular momentum transfer is obtained. This is performed for a benchmark model of 1.3 M at three evolutionary stages, representative of the evolved pulsating stars observed by CoRoT and Kepler. We show that mixed modes extract angular momentum from the innermost regions of subgiants and red giants. However, this transport of angular momentum from the core is unlikely to counterbalance the effect of the core contraction in subgiants and early red giants. In contrast, for more evolved red giants, mixed modes are found efficient enough to balance and exceed the effect of the core contraction, in particular in the hydrogen-burning shell. Our results thus indicate that mixed modes are a promising candidate to explain the observed spin-down of the core of evolved red giants, but that an other mechanism is to be invoked for subgiants and early red giants.},
  archiveprefix = {arxiv},
  keywords = {interiors-Stars,notion,notion-database,oscillations-Stars,rotation,Waves-Stars},
  file = {/Users/lbugnet/Zotero/storage/PU6Y73L5/full-text.pdf}
}

@article{Belkacem2019,
  title = {Transport of Angular Momentum by Waves in Stars},
  author = {Belkacem, Kevin},
  year = {2019},
  month = oct,
  eprint = {1910.11778},
  urldate = {2020-03-09},
  abstract = {Transport of angular momentum is a long-standing problem in stellar physics which recently became more acute thanks to the observations of the space-borne mission \textbackslash emph\{Kepler\}. Indeed, the need for an efficient mechanism able to explain the rotation profile of low-mass stars has been emphasized by asteroseimology and waves are among the potential candidates to do so. In this article, our objective is not to review all the literature related to the transport of angular momentum by waves but rather to emphasize the way it is to be computed in stellar models. We stress that to model wave transport of angular momentum is a non-trivial issue that requires to properly account for interactions between meridional circulation and waves. Also, while many authors only considered the effect of the wave momentum flux in the mean momentum equation, we show that this is an incomplete picture that prevents from grasping the main physics of the problem. We thus present the Transform Eulerian Formalism (TEM) which enable to properly address the problem.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZXW7ARA8/full-text.pdf}
}

@article{Bell2015,
  title = {{{SDSS J1618}}+3854: {{The Sixth Extremely Low-Mass White Dwarf Pulsator}}},
  shorttitle = {{{SDSS J1618}}+3854},
  author = {Bell, Keaton J. and Kepler, S. O. and Montgomery, M. H. and Hermes, J. J. and Harrold, Samuel T. and Winget, D. E.},
  year = {2015},
  month = jun,
  journal = {19th European Workshop on White Dwarfs},
  volume = {493},
  pages = {217},
  urldate = {2023-10-09},
  abstract = {We announce the discovery of the sixth-known pulsating extremely low-mass (ELM; {$\sim$}0.25 M{$\odot$}) white dwarf star (WD). SDSS J1618+3854 exhibits nonlinear pulse shapes that enable us to asteroseimically investigate the convective properties of ELM WDs for the first time. We present the light curve, its Fourier transform, and our very preliminary findings regarding convection.},
  annotation = {ADS Bibcode: 2015ASPC..493..217B},
  file = {/Users/lbugnet/Zotero/storage/NKEZMAIU/Bell et al. - 2015 - SDSS J1618+3854 The Sixth Extremely Low-Mass Whit.pdf}
}

@article{Bell2017,
  title = {Pruning {{The ELM Survey}}: {{Characterizing Candidate Low-mass White Dwarfs}} through {{Photometric Variability}}},
  shorttitle = {Pruning {{The ELM Survey}}},
  author = {Bell, Keaton J. and Gianninas, A. and Hermes, J. J. and Winget, D. E. and Kilic, Mukremin and Montgomery, M. H. and Castanheira, B. G. and Vanderbosch, Z. and Winget, K. I. and Brown, Warren R.},
  year = {2017},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {835},
  pages = {180},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/835/2/180},
  urldate = {2023-10-09},
  abstract = {We assess the photometric variability of nine stars with spectroscopic Teff and log g values from the ELM Survey that locates them near the empirical extremely low-mass (ELM) white dwarf instability strip. We discover three new pulsating stars: SDSS J135512.34+195645.4, SDSS J173521.69+213440.6, and SDSS J213907.42+222708.9. However, these are among the few ELM Survey objects that do not show radial velocity (RV) variations that confirm the binary nature expected of helium-core white dwarfs. The dominant 4.31 hr pulsation in SDSS J135512.34+195645.4 far exceeds the theoretical cut-off for surface reflection in a white dwarf, and this target is likely a high-amplitude {$\delta$} Scuti pulsator with an overestimated surface gravity. We estimate the probability to be less than 0.0008 that the lack of measured RV variations in four of eight other pulsating candidate ELM white dwarfs could be due to low orbital inclination. Two other targets exhibit variability as photometric binaries. Partial coverage of the 19.342 hr orbit of WD J030818.19+514011.5 reveals deep eclipses that imply a primary radius {$>$}0.4 R{$\odot$}\textemdash too large to be consistent with an ELM white dwarf. The only object for which our time series photometry adds support to ELM white dwarf classification is SDSS J105435.78-212155.9, which has consistent signatures of Doppler beaming and ellipsoidal variations. We conclude that the ELM Survey contains multiple false positives from another stellar population at Teff {$\lessequivlnt$} 9000 K, possibly related to the sdA stars recently reported from SDSS spectra.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: eclipsing,stars: oscillations: including pulsations,stars: variables: delta Scuti,white dwarfs},
  annotation = {ADS Bibcode: 2017ApJ...835..180B},
  file = {/Users/lbugnet/Zotero/storage/BSM2J5CR/Bell et al. - 2017 - Pruning The ELM Survey Characterizing Candidate L.pdf}
}

@article{Bellinger2019,
  title = {A Seismic Scaling Relation for Stellar Age},
  author = {Bellinger, Earl Patrick},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {486},
  number = {4},
  eprint = {1903.03110},
  issn = {13652966},
  doi = {10.1093/mnras/stz714},
  abstract = {A simple solar scaling relation for estimating the ages of main-sequence stars from asteroseismic and spectroscopic data is developed. New seismic scaling relations for estimating mass and radius are presented as well, including a purely seismic radius scaling relation (i.e. no dependence on temperature). The relations show substantial improvement over the classical scaling relations and perform similarly well to grid-based modelling.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@book{Belloche2011,
  title = {The End of Star Formation in {{Chamaeleon I}}?: {{A LABOCA}} Census of Starless and Protostellar Cores},
  author = {Belloche, A. and Schuller, F. and Parise, B. and Andr{\'e}, Ph and Hatchell, J. and J{\o}rgensen, J. K. and Bontemps, S. and Wei{\ss}, A. and Menten, K. M. and Muders, D.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {527},
  eprint = {1101.0718},
  issn = {14320746},
  doi = {10.1051/0004-6361/201015733},
  abstract = {Context. Chamaeleon I is the most active region in terms of star formation in the Chamaeleon molecular cloud complex. Although it is one of the nearest low-mass star forming regions, its population of prestellar and protostellar cores is not known and a controversy exists concerning its history of star formation. Aims. Our goal is to search for prestellar and protostellar cores and characterize the earliest stages of star formation in this cloud. Methods. We used the bolometer array LABOCA at the APEX telescope to map the cloud in dust continuum emission at 870 {$\mu$}m with a high sensitivity. This deep, unbiased survey was performed based on an extinction map derived from 2MASS data. The 870 {$\mu$}m map is compared with the extinction map and C18O observations, and decomposed with a multiresolution algorithm. The extracted sources are analysed by carefully taking into account the spatial filtering inherent in the data reduction process. A search for associations with young stellar objects is performed using Spitzer data and the SIMBAD database. Results. Most of the detected 870 {$\mu$}m emission is distributed in five filaments. We identify 59 starless cores, one candidate first hydrostatic core, and 21 sources associated with more evolved young stellar objects. The estimated 90\% completeness limit of our survey is 0.22 M{\.o} for the starless cores. The latter are only found above a visual extinction threshold of 5 mag. They are less dense than those detected in other nearby molecular clouds by a factor of a few on average, maybe because of the better sensitivity of our survey. The core mass distribution is consistent with the IMF at the high-mass end but is overpopulated at the low-mass end. In addition, at most 17\% of the cores have a mass larger than the critical Bonnor-Ebert mass. Both results suggest that a large fraction of the starless cores may not be prestellar in nature. Based on the census of prestellar cores, Class 0 protostars, and more evolved young stellar objects, we conclude that the star formation rate has decreased with time in this cloud. Conclusions. The low fraction of candidate prestellar cores among the population of starless cores, the small number of Class 0 protostars, the high global star formation efficiency, the decrease of the star formation rate with time, and the low mass per unit length of the detected filaments all suggest that we may be witnessing the end of the star formation process in Chamaeleon I. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  isbn = {1-110-11417-6},
  keywords = {{evolution - dust, extinction},ISM: individual objects: Chamaeleon I,ISM: structure,notion,notion-database,stars: formation,stars: protostars},
  file = {/Users/lbugnet/Zotero/storage/8MLAEFEU/Belloche et al. - 2011.pdf}
}

@article{Benbakoura2019,
  title = {Evolution of Star-Planet Systems under Magnetic Braking and Tidal Interaction},
  author = {Benbakoura, M. and R{\'e}ville, V. and Brun, A. S. and {Le Poncin-Lafitte}, C. and Mathis, S.},
  year = {2019},
  month = jan,
  journal = {Astronomy and Astrophysics},
  volume = {621},
  eprint = {1811.06354},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201833314},
  urldate = {2020-03-06},
  abstract = {Context. With the discovery over the last two decades of a large diversity of exoplanetary systems, it is now of prime importance to characterize star-planet interactions and how such systems evolve. Aims. We address this question by studying systems formed by a solar-like star and a close-in planet. We focus on the stellar wind spinning down the star along its main-sequence phase and tidal interaction causing orbital evolution of the systems. Despite recent significant advances in these fields, all current models use parametric descriptions to study at least one of these effects. Our objective is to introduce ab initio prescriptions of the tidal and braking torques simultaneously, so as to improve our understanding of the underlying physics. Methods. We develop a one-dimensional (1D) numerical model of coplanar circular star-planet systems taking into account stellar structural changes, wind braking, and tidal interaction and implement it in a code called ESPEM. We follow the secular evolution of the stellar rotation and of the semi-major axis of the orbit, assuming a bilayer internal structure for the former. After comparing our predictions to recent observations and models, we perform tests to emphasize the contribution of ab initio prescriptions. Finally, we isolate four significant characteristics of star-planet systems: Stellar mass, initial stellar rotation period, planetary mass and initial semi-major axis; and browse the parameter space to investigate the influence of each of them on the fate of the system. Results. Our secular model of stellar wind braking accurately reproduces the recent observations of stellar rotation in open clusters. Our results show that a planet can affect the rotation of its host star and that the resulting spin-up or spin-down depends on the orbital semi-major axis and on the joint influence of magnetic and tidal effects. The ab initio prescription for tidal dissipation that we used predicts fast outward migration of massive planets orbiting fast-rotating young stars. Finally, we provide the reader with a criterion based on the characteristics of the system that allows us to assess whether or not the planet will undergo orbital decay due to tidal interaction.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planet-star interactions,Planetary systems,Stars: Evolution,Stars: Low-mass,Stars: Rotation,Stars: Solar-type},
  file = {/Users/lbugnet/Zotero/storage/EGN6GWRG/full-text.pdf}
}

@techreport{Benbakoura2020,
  title = {Spectroscopic and Seismic Analysis of Red Giants in Eclipsing Binaries Discovered by {{Kepler}}},
  author = {Benbakoura, M and Gaulme, P and Mckeever, J and Sekaran, S and Beck, P G and Spada, F and Jackiewicz, J and Mathis, S and Mathur, S and Tkachenko, A and Garc{\'i}a, R A},
  year = {2020},
  journal = {Astronomy \& Astrophysics},
  pages = {1--30},
  keywords = {asteroseismology,binaries,eclipsing,fundamental parameters,notion,notion-database,oscillations,spectroscopic,stars},
  file = {/Users/lbugnet/Zotero/storage/BT8YZLYB/Benbakoura et al. - 2020.pdf}
}

@article{Benevolenskaya1995,
  title = {Double Magnetic Cycle of Solar Activity},
  author = {Benevolenskaya, E. E.},
  year = {1995},
  journal = {Solar Physics},
  volume = {161},
  number = {1},
  pages = {1--8},
  issn = {00380938},
  doi = {10.1007/BF00732080},
  abstract = {The source of the poloidal magnetic field was fixed using a uniform series of surface low-resolution magnetic field observations begun at Wilcox Solar Observatory at Stanford. The results obtained confirm the idea that low-frequency dynamo waves with a period approximately equal to 22 years and a high-frequency wave of a quasi-two-year period can coexist. It seems that an interaction between these components in the convection zone takes place on the Sun. Surface large-scale solar magnetic fields are analyzed using a two-dimensional Fourier method technique to study the poloidal field distribution. The first harmonic approximately equals the period of the magnetic cycle, appears at all latitudes, and reaches its the maximum value in the polar regions. Moreover, spectral analyses of axisymmetric magnetic field derivative in time found that the second important harmonic of a period approximately equal to two years appears at all latitudes. This second high-frequency harmonic dominates the polar latitude regions at the same time as the low-frequency one. \textcopyright{} 1995 Kluwer Academic Publishers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XP3YZ55E/Benevolenskaya - 1995.pdf}
}

@article{Benoit2006,
  title = {Duty Cycle of {{Doppler}} Ground-Based Asteroseismic Observations},
  author = {Benoit, Mosser and Eric, Aristidi},
  year = {2006},
  eprint = {astro-ph/0612506},
  pages = {1--18},
  abstract = {We report the observations of the clear sky fraction at the Concordia station during winter 2006, and derive from it the duty cycle for astronomical observations. Performance in duty cycle and observation duration promotes Dome C for efficient asteroseismic observations. This performance is analyzed and compared to network observation. For network observations, simulations were run considering the helioseismic network GONG as a reference. Observations with 1 site in Antarctica provide performance similar or better than with a 6-site network, since the duty cycle limited by meteorology is as high as 92\%. On bright targets, a 100-day long time series with a duty cycle about 87\% can be observed, what network observation cannot.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Z33ZL3CF/Benoit, Eric - 2006.pdf}
}

@article{Benomar2009a,
  title = {The Solar-like Oscillations of {{HD49933}}: {{A Bayesian}} Approach},
  author = {Benomar, O. and Appourchaux, T. and Baudin, F.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {15--32},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911657},
  abstract = {Context. Asteroseismology has entered a new era with the availability of continuous observations from space-borne missions such as MOST, CoRoT and Kepler. However, the low amplitude and the complexity of the observed spectrum make the exploitation of these data sets difficult. Aims. The use of robust methods to estimate the parameters of stellar oscillation eigenmodes is necessary to fully exploit these new data sets. These parameters include in particular the frequency, the width and the energy of the eigenmodes, all being required for a seismic interpretation of the stellar internal structure or excitation of the eigenmodes. Methods. A Bayesian approach, coupled with a Markov chain Monte Carlo (MCMC) algorithm, is presented. Such a method allows the use of a priori knowledge to improve the parameter estimation. It also provides complete information on the probability distribution of the fitted parameters. The method is tested on simulated time series and then applied to CoRoT observations of HD49933. Results. The simulated time series allow the validation of the method for conditions similar to those of the observations in terms of spectral complexity and signal-to-noise ratio. However, a very important problem in the analysis of the HD49933 mode spectrum is the l degree identification of the modes. The degree identification has little impact on the large frequency separation, rotational splitting, energy and width estimation, whereas individual frequencies and the star inclination angle evaluation are strongly affected. From a statistical point of view, we provide a quantitative ranking of the four models considered. The most probable model includes only modes of degree 0 and 1. Two other models include modes with degree up to 2 and have a non negligible level of significance. The last model includes modes of degree 0 and 1 but has an alternate degree identification and can be definitively rejected. In conclusion, the significance of the resulting probabilities is not sufficient to draw a definite conclusion.},
  keywords = {Methods: observational,Methods: statistical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/KA7CAQDW/Benomar, Appourchaux, Baudin - 2009.pdf}
}

@article{Benomar2009b,
  title = {A Fresh Look at the Seismic Spectrum of {{HD49933}}: {{Analysis}} of 180 Days of {{CoRoT}} Photometry},
  author = {Benomar, O. and Baudin, F. and Campante, T. L. and Chaplin, W. J. and Garc{\'i}a, R. A. and Gaulme, P. and Toutain, T. and Verner, G. A. and Appourchaux, T. and Ballot, J. and Barban, C. and Elsworth, Y. and Mathur, S. and Mosser, B. and R{\'e}gulo, C. and Roxburgh, I. W. and Auvergne, M. and Baglin, A. and Catala, C. and Michel, E. and Samadi, R.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {507},
  number = {1},
  eprint = {0910.3060},
  issn = {14320746},
  doi = {10.1051/0004-6361/200913111},
  abstract = {Context. Solar-like oscillations have now been observed in several stars, thanks to ground-based spectroscopic observations and space-borne photometry. CoRoT, which has been in orbit since December 2006, has observed the star HD49933 twice. The oscillation spectrum of this star has proven difficult to interpret. Aims. Thanks to a new timeseries provided by CoRoT, we aim to provide a robust description of the oscillations in HD49933, i.e., to identify the degrees of the observed modes, and to measure mode frequencies, widths, amplitudes and the average rotational splitting.Methods. Several methods were used to model the Fourier spectrum: Maximum Likelihood Estimators and Bayesian analysis using Markov Chain Monte-Carlo techniques.Results. The different methods yield consistent result, and allow us to make a robust identification of the modes and to extract precise mode parameters. Only the rotational splitting remains difficult to estimate precisely, but is clearly relatively large (several {$\mu$}Hz in size). \textcopyright{} 2009 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/6EVQ4DHM/Benomar et al. - 2009.pdf}
}

@article{Benomar2012,
  title = {Masses of Subgiant Stars from Asteroseismology Using the Coupling Strengths of Mixed Modes},
  author = {Benomar, O. and Bedding, T. R. and Stello, D. and Deheuvels, S. and White, T. R. and {Christensen-Dalsgaard}, J.},
  year = {2012},
  journal = {Astrophysical Journal Letters},
  volume = {745},
  number = {2},
  eprint = {1201.1067},
  issn = {20418205},
  doi = {10.1088/2041-8205/745/2/L33},
  abstract = {For a few decades now, asteroseismology, the study of stellar oscillations, has enabled us to probe the interiors of stars with great precision. It allows stringent tests of stellar models and can provide accurate radii, masses, and ages for individual stars. Of particular interest are the mixed modes that occur in subgiant solar-like stars since they can place very strong constraints on stellar ages. Here, we measure the characteristics of the mixed modes, particularly the coupling strength, using a grid of stellar models for stars with masses between 0.9 and 1.5 M {$\odot$}. We show that the coupling strength of the {$\mathscr{l}$} = 1 mixed modes is predominantly a function of stellar mass and appears to be independent of metallicity. This should allow an accurate mass evaluation, further increasing the usefulness of mixed modes in subgiants as asteroseismic tools. \textcopyright{} 2012. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {methods: data analysis,notion,notion-database,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/XRJBERCE/Benomar et al. - 2012.pdf}
}

@article{Benomar2012a,
  title = {Acoustic Spectrum Fitting for a Large Set of Solar-like Pulsators},
  author = {Benomar, O. and Baudin, F. and Chaplin, W. J. and Elsworth, Y. and Appourchaux, T.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {420},
  number = {3},
  pages = {2178--2189},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.20184.x},
  abstract = {Asteroseismology provides the means both to constrain the global properties and to probe the internal structures of stars. Asteroseismic data are now available on large numbers of solar-type stars, thanks in particular to theCoRoTandKeplerspace missions, and automated data-analysis pipelines are needed to provide efficient and timely results. Here, we present an automated algorithm that is able to extract mode parameters under low signal-to-noise ratio conditions. We use a Bayesian framework to ensure the robustness of the algorithm. We discuss the efficiency of the method and test it using Variability of Solar Irradiance and Gravity Oscillations (VIRGO) Sun-as-a-star photometry data and the artificial Astero Fitting at Low Angular degree Group (asteroFLAG)Keplerensemble. Analysis of the VIRGO data shows that it is possible to track variations of the individual mode parameters (frequency, height, width) through the solar cycle, using short time series (30 days). The present analysis also revealed a modulation of the degreel= 2 relative height through the solar cycle. Applied on asteroFLAG data, we show that the pipeline extracts accurately the central frequency and the large separation. It is also able to identify the degree of the modes in 78 per cent of stars. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {Methods: statistical,notion,notion-database,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/NFABVMIL/Benomar et al. - 2012(2).pdf}
}

@article{Benomar2013,
  title = {Properties of Oscillation Modes in Subgiant Stars Observed by Kepler},
  author = {Benomar, O. and Bedding, T. R. and Mosser, B. and Stello, D. and Belkacem, K. and Garcia, R. A. and White, T. R. and Kuehn, C. A. and Deheuvels, S. and {Christensen-Dalsgaard}, J.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {767},
  number = {2},
  eprint = {1302.4143},
  issn = {15384357},
  doi = {10.1088/0004-637X/767/2/158},
  abstract = {Mixed modes seen in evolved stars carry information on their deeper layers that can place stringent constraints on their physics and on their global properties (mass, age, etc.). In this study, we present a method to identify and measure all oscillatory mode characteristics (frequency, height, width). Analyzing four subgiant stars, we present the first measure of the effect of the degree of mixture on the {$\mathscr{l}$} = 1 mixed mode characteristics. We also show that some stars have measurable {$\mathscr{l}$} = 2 mixed modes and discuss the interest of their measure to constrain the deeper layers of stars. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VZFPC9DH/Benomar et al. - 2013.pdf}
}

@article{Benomar2014,
  title = {Inferring Mode Inertias in Evolved Solar-like Stars},
  author = {Benomar, Othman and Belkacem, Kevin and Bedding, Timothy R. and Stello, Dennis and Di Mauro, Maria Pia and Ventura, R. and Mosser, Beno{\^i}t and Goupil, M. J. and Samadi, R{\'e}za and Garcia, R. A.},
  year = {2014},
  journal = {The Astrophysical Journal},
  volume = {781},
  number = {2},
  eprint = {1401.5152},
  pages = {L29},
  issn = {2041-8205},
  doi = {10.1088/2041-8205/781/2/L29},
  abstract = {Asteroseismology of evolved solar-like stars is experiencing a growing interest due to the wealth of observational data from space-borne instruments such as the \textbackslash emph\{CoRoT\} and \textbackslash emph\{Kepler\} spacecraft. In particular, the recent detection of mixed modes, which probe both the innermost and uppermost layers of stars, paves the way for inferring the internal structure of stars along their evolution through the subgiant and red giant phases. Mixed modes can also place stringent constraints on the physics of such stars and on their global properties (mass, age, etc...). Here, using two \textbackslash emph\{Kepler\} stars (KIC 4351319 and KIC 6442183), we demonstrate that measurements of mixed mode characteristics allow us to estimate the mode inertias, providing a new and additional diagnostics on the mode trapping and subsequently on the internal structure of evolved stars. We however stress that the accuracy may be sensitive to non-adiabatic effects.},
  archiveprefix = {arxiv},
  keywords = {color figures,data analysis,interiors,methods,notion,notion-database,online-only material,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/ZUDCA5AM/Benomar et al. - 2014.pdf}
}

@article{Benomar2015a,
  title = {Nearly Uniform Internal Rotation of Solar-like Main-Sequence Stars Revealed by Space-Based Asteroseismology and Spectroscopic Measurements},
  author = {Benomar, O. and Takata, M. and Shibahashi, H. and Ceillier, T. and Garc{\'i}a, R. A.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {452},
  number = {3},
  pages = {2654--2674},
  issn = {13652966},
  doi = {10.1093/mnras/stv1493},
  abstract = {The rotation rates in the deep interior and at the surface of 22 main-sequence stars with masses between 1.0 and 1.6 M{$\odot$} are constrained by combining asteroseismological analysis with spectroscopic measurements. The asteroseismic data of each star are taken by the Kepler or CoRoT space mission. It is found that the difference between the surface rotation rate and the average rotation rate (excluding the convective core) of most of stars is small enough to suggest that an efficient process of angular momentum transport operates during and/or before the main-sequence stage of stars. If each of the surface convective zone and the underlying radiative zone, for individual stars, is assumed to rotate uniformly, the difference in the rotation rate between the two zones turns out to be no more than a factor of 2 in most of the stars independently of their ages.},
  keywords = {Asteroseismology -methods: data analysis,notion,notion-database,Stars: interiors,Stars: oscillations,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/C86G4VPW/Benomar et al. - 2015.pdf}
}

@article{Benomar2018,
  title = {Asteroseismic Detection of Latitudinal Differential Rotation in 13 {{Sun-like}} Stars},
  author = {Benomar, O. and Bazot, M. and Nielsen, M. B. and Gizon, L. and Sekii, T. and Takata, M. and Hotta, H. and Hanasoge, S. and Sreenivasan, K. R. and {Christensen-Dalsgaard}, J.},
  year = {2018},
  month = sep,
  journal = {Science},
  volume = {361},
  number = {6408},
  eprint = {1809.07938},
  pages = {1231--1234},
  publisher = {{American Association for the Advancement of Science}},
  issn = {10959203},
  doi = {10.1126/science.aao6571},
  urldate = {2020-07-17},
  abstract = {The differentially rotating outer layers of stars are thought to play a role in driving their magnetic activity, but the underlying mechanisms that generate and sustain differential rotation are poorly understood. We report the measurement using asteroseismology of latitudinal differential rotation in the convection zones of 40 Sun-like stars. For the most significant detections, the stars' equators rotate approximately twice as fast as their midlatitudes. The latitudinal shear inferred from asteroseismology is much larger than predictions from numerical simulations.},
  archiveprefix = {arxiv},
  pmid = {30237352},
  keywords = {ASTRONOMY,Astrophysics,notion,notion-database,PHYSICS,Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/HZNSXIC7/full-text.pdf}
}

@article{Bercovici1987,
  title = {Jovian Seismology},
  author = {Bercovici, D. and Schubert, G.},
  year = {1987},
  month = mar,
  journal = {Icarus},
  volume = {69},
  number = {3},
  pages = {557--565},
  publisher = {{Academic Press}},
  issn = {10902643},
  doi = {10.1016/0019-1035(87)90024-8},
  urldate = {2020-05-21},
  abstract = {Standing acoustic waves, with periods between about 4.5 and 9 min, may be trapped in a wave duct beneath Jupiter's tropopause. Detection of these oscillations by observations of Doppler shifting of infrared and ultraviolet absorption lines would offer a new important method for probing the giant planet's deep atmosphere and interior. Information would be revealed on Jupiter's thermal and density structure and the depth to which its zonal winds penetrate. Standing oscillations in the molecular hydrogen envelope are modeled and their theoretical eigenfrequencies are presented as they might appear in actual data analysis. Several forcing functions for wave generation are considered. These include coupling with turbulent and convective motions, thermal overstability due to radiative transfer, effects of wave propagation in a saturated atmosphere, and consequences of ortho- to parahydrogen conversion. Altjough the forcing mechanisms couple well with the acoustic waves, allowing for possible maintenance of the oscillations, the contribution they make to velocity amplitudes is very small, between 1.0 and 0.1 m sec-1. This implies that the Doppler shifting caused by the waves may be unresolvable except, perhaps, by methods of superposing time records of oscillations to enhance acoustic signals and diminish random noise. \textcopyright{} 1987.},
  keywords = {notion,notion-database}
}

@article{Berdyugina2002,
  title = {Magnetic Activity in the Young Solar Analog {{LQ}} Hydrae. {{I}}. {{Active}} Longitudes and Cycles},
  author = {Berdyugina, S. V. and Pelt, J. and Tuominen, I.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {394},
  number = {2},
  pages = {505--515},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021179},
  abstract = {We present the first evidence that a single active dwarf of solar type can show a long-lived, nonaxisymmetric spot distribution - active longitudes on opposite hemispheres, similar to evolved, rapidly rotating RS CVn-type binary stars. We analyse new as well as published photometric observations of the young active dwarf LQ Hya, spanning almost 20 years. We find that activity of the star has three activity cycles: a 5.2-yr "flip-flop" cycle, a 7.7-yr period in the amplitude modulation of the brightness and an approximately 15-yr period in variations of the mean brightness. The two shorter cycles are related to the alternating active longitudes and are similar to cycles observed in RS CVn-type stars. The 15-yr cycle reflects periodic changes of the mean spottedness of the star and resembles the solar 11-year cycle. The spot rotation period (about 1.6 days) changes during the 15-yr cycle, indicating the presence of small differential rotation. The lengths of the three cycles are related as 3:2:1, with the repetition of the spot configuration after 15 years. We discuss the possibility that the observed spot cycles represent two different magnetic dynamo modes operating in LQ Hya: an axisymmetric mode, as in the Sun, and a nonaxisymmetric higher order mode with two cycles in spot patterns. Our results suggest that young stars exhibit their cycles in spot distribution, as seen in LQ Hya. This is in contrast to the conclusion based on the analysis of Ca II H\&K emission from plages. The results suggest also that the Vaughn-Preston gap represents a transition from a multiple-mode dynamo to a single-mode dynamo.},
  keywords = {notion,notion-database,Stars: activity,Stars: magnetic fields,Stars: starspots},
  file = {/Users/lbugnet/Zotero/storage/3HDNMDN4/Berdyugina, Pelt, Tuominen - 2002.pdf}
}

@article{Berdyugina2006,
  title = {Flip-Flop Cycles in Solar and Stellar Activity},
  author = {Berdyugina, Svetlana V.},
  year = {2006},
  journal = {Proceedings of the International Astronomical Union},
  volume = {2},
  number = {14},
  pages = {275--276},
  issn = {17439213},
  doi = {10.1017/S1743921307010563},
  abstract = {We discuss flip-flop cycles in solar and stellar activity. \textcopyright{} 2007 International Astronomical Union.},
  keywords = {notion,notion-database,Stars: activity,Stars: late-type,Stars: spots,Sun: activity},
  file = {/Users/lbugnet/Zotero/storage/QDXBENHA/Berdyugina - 2006.pdf}
}

@article{Berdyugina2006a,
  title = {Active Longitudes, Nonaxisymmetric Dynamos and Phase Mixing},
  author = {Berdyugina, S. V. and Moss, D. and Sokoloff, D. and Usoskin, I. G.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {445},
  number = {2},
  pages = {703--714},
  issn = {14320746},
  doi = {10.1051/0004-6361:20053454},
  abstract = {We discuss the problem of solar active longitudes from the viewpoint of dynamo theory. We start from a recent observational analysis of the problem undertaken by Berdyugina \& Usoskin (2003, A\&A, 405, 1121) and Usoskin et al. (2005, A\&A, 441, 347) who demonstrated from a study of sunspot data that solar active longitudes rotate differentially, with a small but significant asynchrony between northern and southern hemispheres. We suggest two concepts by which the underlying magnetic structure could lead to the observed phenomenology - the true differential rotation of a nonaxisymmetric magnetic structure and a stroboscopic effect. In the latter case, a solid body rotation of nonaxisymmetric magnetic structure is illuminated by an activity wave propagating from middle latitudes to the solar equator, and so mimics a differential rotation. We then discuss several mechanisms which could in principle lead to the excitation of active longitudes. In particular, we consider dynamo excitation of nonaxisymmetric magnetic modes, nonaxisymmetric structures as a manifestation of a relic magnetic field in the solar core, nonaxisymmetric solar hydrodynamics and nonlinear instabilities that lack axial symmetry. We conclude that these mechanisms all provide ways to explain the phenomenology, provided the stroboscopic interpretation is accepted. Of course, a quantitative explanation in the framework of any scenario requires ultimately a detailed numerical simulation. The interpretation of the available observations as a true differential rotation appears to provide a much more severe challenge for theorists. We are unable to suggest a plausible mechanism of this kind; however we can not exclude in principle such an explanation. We relate the phenomenon of solar active longitudes to the information available concerning stellar active longitudes, and also consider evidence from other tracers of solar activity. \textcopyright{} ESO 2005.},
  keywords = {Magnetic fields,notion,notion-database,Stars: magnetic fields,Sun: activity,Sun: magnetic fields,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/QV6JAMCA/Berdyugina et al. - 2006.pdf}
}

@article{Berdyugina2007,
  title = {Butterfly {{Diagram}} and {{Activity Cycles}} in {{HR}} 1099},
  author = {Berdyugina, Svetlana V. and Henry, Gregory W.},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {659},
  number = {2},
  eprint = {astro-ph/0703530},
  pages = {L157-L160},
  issn = {0004-637X},
  doi = {10.1086/517881},
  abstract = {We analyze photometric data of the active RS CVn--type star HR 1099 for the years 1975--2006 with an inversion technique and reveal the nature of two activity cycles of 15--16 yr and 5.3\$\textbackslash pm\$0.1 yr duration. The 16 yr cycle is related to variations of the total spot area and is coupled with the differential rotation, while the 5.3 yr cycle is caused by the symmetric redistribution of the spotted area between the opposite stellar hemispheres (flip-flop cycle). We recover long-lived active regions comprising two active longitudes that migrate in the orbital reference frame with a variable rate because of the differential rotation along with changes in the mean spot latitudes. The migration pattern is periodic with the 16 yr cycle. Combining the longitudinal migration of the active regions with a previously measured differential rotation law, we recover the first stellar butterfly diagram without an assumption about spot shapes. We find that mean latitudes of active regions at opposite longitudes change antisymmetrically in the course of the 16 yr cycle: while one active region migrates to the pole, the other approaches the equator. This suggests a precession of the global magnetic field with respect to the stellar rotational axis.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6TWJZCED/Berdyugina, Henry - 2007.pdf}
}

@article{Berger2018,
  title = {Revised {{Radii}} of {{Kepler Stars}} and {{Planets Using Gaia Data Release}} 2},
  author = {Berger, Travis A. and Huber, Daniel and Gaidos, Eric and {van Saders}, Jennifer L.},
  year = {2018},
  journal = {The Astrophysical Journal},
  volume = {866},
  number = {2},
  eprint = {1805.00231},
  pages = {99},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aada83},
  abstract = {One bottleneck for the exploitation of data from the \$Kepler\$ mission for stellar astrophysics and exoplanet research has been the lack of precise radii and evolutionary states for most of the observed stars. We report revised radii of 177,911 \$Kepler\$ stars derived by combining parallaxes from \$Gaia\$ Data Release 2 with the DR25 \$Kepler\$ Stellar Properties Catalog. The median radius precision is \$\textbackslash approx\$ 8\%, a typical improvement by a factor of 4-5 over previous estimates for typical \$Kepler\$ stars. We find that \$\textbackslash approx\$ 67\% (\$\textbackslash approx\$ 120,000) of all \$Kepler\$ targets are main-sequence stars, \$\textbackslash approx\$ 21\% (\$\textbackslash approx\$ 37,000) are subgiants, and \$\textbackslash approx\$ 12\% (\$\textbackslash approx\$ 21,000) are red giants, demonstrating that subgiant contamination is less severe than some previous estimates and that Kepler targets are mostly main-sequence stars. Using the revised stellar radii, we recalculate the radii for 2123 confirmed and 1922 candidate exoplanets. We confirm the presence of a gap in the radius distribution of small, close-in planets, but find that the gap is mostly limited to incident fluxes \${$>\$$} 200\$F\_\textbackslash oplus\$ and its location may be at a slightly larger radius (closer to \$\textbackslash approx\$ 2\$R\_\textbackslash oplus\$) when compared to previous results. Further, we find several confirmed exoplanets occupying a previously-described "hot super-Earth desert" at high irradiance, show the relation between gas-giant planet radius and incident flux, and establish a bona-fide sample of eight confirmed planets and 30 planet candidates with \$R\_\{\textbackslash mathrm\{p\}\}\$ \${$<\$$} 2\$R\_\textbackslash oplus\$ in circumstellar "habitable zones" (incident fluxes between 0.25--1.50 \$F\_\textbackslash oplus\$). The results presented here demonstrate the potential for transformative characterization of stellar and exoplanet populations using \$Gaia\$ data.},
  archiveprefix = {arxiv},
  keywords = {catalogs,fundamental parameters,notion,notion-database,photometric,planetary systems,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/Y62SMQQL/Berger et al. - 2018.pdf}
}

@article{bergerGaiaKeplerStellarProperties2020,
  title = {The {{Gaia-Kepler Stellar Properties Catalog}}. {{I}}. {{Homogeneous Fundamental Properties}} for 186,301 {{Kepler Stars}}},
  author = {Berger, Travis A and Huber, Daniel and Van Saders, Jennifer L and Gaidos, Eric and Tayar, Jamie and Kraus, Adam L},
  year = {2020},
  journal = {The Astronomical Journal},
  volume = {159},
  pages = {280},
  doi = {10.3847/1538-3881/159/6/280},
  urldate = {2021-08-01},
  abstract = {An accurate and precise Kepler Stellar Properties Catalog is essential for the interpretation of the Kepler exoplanet survey results. Previous Kepler Stellar Properties Catalogs have focused on reporting the best-available parameters for each star, but this has required combining data from a variety of heterogeneous sources. We present the Gaia-Kepler Stellar Properties Catalog, a set of stellar properties of 186,301 Kepler stars, homogeneously derived from isochrones and broadband photometry, Gaia Data Release 2 parallaxes, and spectroscopic metallicities, where available. Our photometric effective temperatures, derived from g K to s colors, are calibrated on stars with interferometric angular diameters. Median catalog uncertainties are 112 K for T eff , 0.05 dex for g log , 4\% for  R , 7\% for  M , 13\% for r  , 10\% for  L , and 56\% for stellar age. These precise constraints on stellar properties for this sample of stars will allow unprecedented investigations into trends in stellar and exoplanet properties as a function of stellar mass and age. In addition, our homogeneous parameter determinations will permit more accurate calculations of planet occurrence and trends with stellar properties. Unified Astronomy Thesaurus concepts: Catalogs (205); Fundamental parameters of stars (555); Exoplanet systems (484) Supporting material: machine-readable tables},
  keywords = {Catalogs,Exoplanet systems,Fundamental parameters of stars,notion,notion-database}
}

@article{Bernstein1958,
  title = {An Energy Principle for Hydromagnetic Stability Problems},
  author = {Bernstein, I. B. and Frieman, E. A. and Kruskal, M. D. and Kulsrud, R. M.},
  year = {1958},
  month = feb,
  journal = {Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
  volume = {244},
  number = {1236},
  pages = {17--40},
  publisher = {{The Royal Society}},
  issn = {0080-4630},
  doi = {10.1098/rspa.1958.0023},
  urldate = {2020-07-02},
  abstract = {The problem of the stability of static, highly conducting, fully ionized plasmas is investigated by means of an energy principle developed from one introduced by Lundquist. The derivation of the principle and the conditions under which it applies are given. The method is applied to find complete stability criteria for two types of equilibrium situations. The first concerns plasmas which are completely separated from the magnetic field by an interface. The second is the general axisymmetric system.},
  keywords = {notion,notion-database}
}

@article{Bertello2012,
  title = {Signature of Differential Rotation in {{Sun-as-a-star Ca II K}} Measurements},
  author = {Bertello, L. and Pevtsov, A. A. and Pietarila, A.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {761},
  number = {1},
  eprint = {1210.5556},
  issn = {15384357},
  doi = {10.1088/0004-637X/761/1/11},
  abstract = {The characterization of solar surface differential rotation (SDR) from disk-integrated chromospheric measurements has important implications for the study of differential rotation and dynamo processes in other stars. Some chromospheric lines, such as Ca II K, are very sensitive to the presence of activity on the disk and are an ideal choice for investigating SDR in Sun-as-a-star observations. Past studies indicate that when the activity is low, the determination of Sun's differential rotation from integrated-sunlight measurements becomes uncertain. However, our study shows that using the proper technique, SDR can be detected from these type of measurements even during periods of extended solar minima. This paper describes results from the analysis of the temporal variations of Ca II K line profiles observed by the Integrated Sunlight Spectrometer during the declining phase of Cycle 23 and the rising phase of Cycle 24, and discusses the signature of SDR in the power spectra computed from time series of parameters derived from these profiles. The methodology described is quite general, and could be applied to photometric time series of other main-sequence stars for detecting differential rotation. \textcopyright{} 2012. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: rotation,Sun: activity,Sun: rotation,Sun: surface magnetism},
  file = {/Users/lbugnet/Zotero/storage/2Y6VH7DR/Bertello, Pevtsov, Pietarila - 2012.pdf}
}

@article{Bigot2000,
  title = {Non-Axisymmetric Oscillations of {{roAp}} Stars},
  author = {Bigot, L. and Provost, J. and Berthomieu, G. and Dziembowski, W. A. and Goode, P. R.},
  year = {2000},
  journal = {Astronomy \& Astrophysics},
  volume = {356},
  pages = {218--233},
  issn = {0004-6361},
  urldate = {2020-08-10},
  keywords = {notion,notion-database,STARS: CHEMICALLY PECULIAR,STARS: INTERIORS,STARS: MAGNETIC FIELDS,STARS: OSCILLATIONS}
}

@article{Blazko1907,
  title = {Mitteilung \"Uber Ver\"anderliche {{Sterne}}},
  author = {Bla{\v z}ko, S.},
  year = {1907},
  journal = {Astronomische Nachrichten},
  volume = {175},
  number = {20},
  pages = {327--330},
  issn = {15213994},
  doi = {10.1002/asna.19071752003},
  urldate = {2020-03-31},
  keywords = {notion,notion-database}
}

@article{Bloecker1995,
  title = {Stellar Evolution of Low and Intermediate-Mass Stars. {{I}}. {{Mass}} Loss on the {{AGB}} and Its Consequences for Stellar Evolution.},
  author = {Bloecker, T. and {T.}},
  year = {1995},
  journal = {A\&A},
  volume = {297},
  pages = {727},
  issn = {0004-6361},
  urldate = {2020-07-13},
  keywords = {AGB,notion,notion-database,POST,STARS: AGB,STARS: EVOLUTION,STARS: MASS LOSS}
}

@article{Blomme2011,
  title = {Improved Methodology for the Automated Classification of Periodic Variable Stars},
  author = {Blomme, J and Sarro, L M and O'donovan, F T and Debosscher, J and Brown, T and Lopez, M and Dubath, P and Rimoldini, L and Charbonneau, D and Dunham, E and Mandushev, G and Ciardi, D R and De Ridder, J and Aerts, C},
  year = {2011},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {418},
  pages = {96--106},
  doi = {10.1111/j.1365-2966.2011.19466.x},
  urldate = {2020-04-09},
  abstract = {We present a novel automated methodology to detect and classify periodic variable stars in a large data base of photometric time series. The methods are based on multivariate Bayesian statistics and use a multistage approach. We applied our method to the ground-based data of the TransAtlantic Exoplanet Survey (TrES) Lyr1 field, which is also observed by the Kepler satellite, covering {$\sim$}26 000 stars. We found many eclipsing binaries as well as classical non-radial pulsators, such as slowly pulsating B stars, {$\gamma$} Doradus, {$\beta$} Cephei and {$\delta$} Scuti stars. Also a few classical radial pulsators were found.},
  keywords = {data analysis-methods,methods,notion,notion-database,photometric,statistical-techniques},
  file = {/Users/lbugnet/Zotero/storage/DWU7I4JB/full-text.pdf}
}

@article{Bodenheimer2003,
  title = {On the {{Radii}} of {{Extrasolar Giant Planets}}},
  author = {Bodenheimer, P. and Laughlin, G. and Lin, D. N. C.},
  year = {2003},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {592},
  number = {1},
  eprint = {astro-ph/0303541},
  pages = {555--563},
  publisher = {{IOP Publishing}},
  doi = {10.1086/375565},
  urldate = {2020-03-23},
  abstract = {We have computed evolutionary models for extrasolar planets which range in mass from 0.1 to 3.0 Jovian Masses, and which range in equilibrium temperature from 113 K to 2000 K. We present four sequences of models, designed to show the structural effects of a solid core and of internal heating due to the conversion of kinetic to thermal energy at pressures of tens of bars. The model planetary radii are intended for comparisons with radii derived from observations of transiting extrasolar planets. To provide such comparisons, we expect that of order 10 transiting planets with orbital periods less than 200 days can be detected around bright (V{$<$}10) main-sequence stars for which accurate, well-sampled radial velocity measurements can be readily accumulated. Through these observations, structural properties of the planets will be derivable, particularly for low-mass, high-temperature planets. Implications regarding the transiting companion to OGLE-TR-56 recently announced by Konacki et al. are discussed. With regard to the confirmed transiting planet, HD 209458b, we find, in accordance with other recent calculations, that models without internal heating predict a radius that is 35 percent smaller than the observed radius. We explore the possibility that HD 209458b owes its large size to dissipation of energy arising from ongoing tidal circularization of the orbit. We show that residual scatter in the current radial velocity data set for HD 209458b is consistent with the presence of an as-of-yet undetected second companion, and that further radial velocity monitoring of the star is indicated.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Planets and Satellites: General,Stars: Planetary Systems},
  file = {/Users/lbugnet/Zotero/storage/RKZ7V273/full-text.pdf}
}

@article{Bogart1995,
  title = {The {{SOHO}} Mission ( {{Domingo}} et al ., 1995 ) Emphasizes Three Principal Ar- Eas of Scientific Investigation : ( 1 ) Probing the Solar Interior Using the Tech- Niques of Helioseismology , ( 2 ) Determining the Heating Mechanism of the Solar Corona , and ( 3},
  author = {Bogart, R S and Bush, R I and Hoeksema, J T and Schou, J and Experimental, W W Hansen and Tarbell, T D and Zayer, I and Palo, Lockheed and Alto, Palo},
  year = {1995},
  pages = {129--188},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/24NVM937/Bogart et al. - 1995.pdf}
}

@article{Bognar2020,
  title = {{{TESS}} First Look at Evolved Compact Pulsators: {{Known ZZ Ceti}} Stars of the Southern Ecliptic Hemisphere as Seen by {{TESS}}},
  shorttitle = {{{TESS}} First Look at Evolved Compact Pulsators},
  author = {Bogn{\'a}r, {\relax Zs}. and Kawaler, S. D. and Bell, K. J. and Schrandt, C. and Baran, A. S. and Bradley, P. A. and Hermes, J. J. and Charpinet, S. and Handler, G. and Mullally, S. E. and Murphy, S. J. and Raddi, R. and S{\'o}dor, {\'A}. and Tremblay, P.-E. and Uzundag, M. and Zong, W.},
  year = {2020},
  month = jun,
  journal = {Astronomy \& Astrophysics},
  volume = {638},
  pages = {A82},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202037470},
  urldate = {2023-10-05},
  abstract = {Context. We present our findings on 18 previously known ZZ Ceti stars observed by the TESS space telescope in 120 s cadence mode during the survey observation of the southern ecliptic hemisphere. Aims. We focus on the frequency analysis of the space-based observations, comparing the results with findings of previous groundbased measurements. The frequencies detected by the TESS observations can serve as inputs for future asteroseismic analyses. Methods. We performed standard pre-whitening of the data sets to derive the possible pulsation frequencies of the different targets. In some cases, we fit Lorentzians to the frequency groups that emerged as the result of short-term amplitude or phase variations that occurred during the TESS observations.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/9DC7QIFS/Bognár et al. - 2020 - TESS first look at evolved compact pulsators Know.pdf}
}

@article{Bolmont2012,
  title = {Effect of the Stellar Spin History on the Tidal Evolution of Close-in Planets},
  author = {Bolmont, E. and Raymond, S. N. and Leconte, J. and Matt, S. P.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {544},
  pages = {1--11},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219645},
  abstract = {Context. The spin rate of stars evolves substantially during their lifetime, owing to the evolution of their internal structure and to external torques arising from the interaction of stars with their environments and stellar winds. Aims. We investigate how the evolution of the stellar spin rate affects, and is affected by, planets in close orbits via star-planet tidal interactions. Methods. We used a standard equilibrium tidal model to compute the orbital evolution of single planets orbiting both Sun-like stars and very low-mass stars (0.1 M {$\cdot$}). We tested two stellar spin evolution profiles, one with fast initial rotation (1.2 day rotation period) and one with slow initial rotation (8 day period). We tested the effect of varying the stellar and planetary dissipations, and the planet's mass and initial orbital radius. Results. For Sun-like stars, the different tidal evolution between initially rapidly and slowly rotating stars is only evident for extremely close-in gas giants orbiting highly dissipative stars. However, for very low-mass stars the effect of the initial rotation of the star on the planet's evolution is apparent for less massive (1 M {$\odot$}) planets and typical dissipation values. We also find that planetary evolution can have significant effects on the stellar spin history. In particular, when a planet falls onto the star, it can cause the star to spin up. Conclusions. Tidal evolution allows us to differentiate between the early behaviors of extremely close-in planets orbiting either a rapidly rotating star or a slowly rotating star. The early spin-up of the star allows the close-in planets around fast rotators to survive the early evolution. For planets around M-dwarfs, surviving the early evolution means surviving on Gyr timescales, whereas for Sun-like stars the spin-down brings about late mergers of Jupiter planets. In the light of this study, we can say that differentiating one type of spin evolution from another given the present position of planets can be very tricky. Unless we can observe some markers of former evolution, it is nearly impossible to distinguish the two very different spin profiles, let alone intermediate spin-profiles. Nevertheless, some conclusions can still be drawn about statistical distributions of planets around fully convective M-dwarfs. If tidal evolution brings about a merger late in the stellar history, it can also entail a noticeable acceleration of the star at late ages, so that it is possible to have old stars that spin rapidly. This raises the question of how the age of stars can be more tightly constrained. \textcopyright{} 2012 ESO.},
  keywords = {notion,notion-database,Planet-star interactions,Planets and satellites: dynamical evolution and st,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/MNX73DHN/Bolmont et al. - 2012.pdf}
}

@article{Bolmont2016,
  title = {Effect of the Rotation and Tidal Dissipation History of Stars on the Evolution of Close-in Planets},
  author = {Bolmont, Emeline and Mathis, St{\'e}phane},
  year = {2016},
  month = nov,
  journal = {Celestial Mechanics and Dynamical Astronomy},
  volume = {126},
  number = {1-3},
  pages = {275--296},
  publisher = {{Springer Netherlands}},
  issn = {15729478},
  doi = {10.1007/s10569-016-9690-3},
  urldate = {2020-07-17},
  abstract = {Since 20~years, a large population of close-in planets orbiting various classes of low-mass stars (from M-type to A-type stars) has been discovered. In such systems, the dissipation of the kinetic energy of tidal flows in the host star may modify its rotational evolution and shape the orbital architecture of the surrounding planetary system. In this context, recent observational and theoretical works demonstrated that the amplitude of this dissipation can vary over several orders of magnitude as a function of stellar mass, age and rotation. In addition, stellar spin-up occurring during the Pre-Main-Sequence (PMS) phase because of the contraction of stars and their spin-down because of the torque applied by magnetized stellar winds strongly impact angular momentum exchanges within star\textendash planet systems. Therefore, it is now necessary to take into account the structural and rotational evolution of stars when studying the orbital evolution of close-in planets. At the same time, the presence of planets may modify the rotational dynamics of the host stars and as a consequence their evolution, magnetic activity and mixing. In this work, we present the first study of the dynamics of close-in planets of various masses orbiting low-mass stars (from 0.6M{$\odot$} to 1.2M{$\odot$}) where we compute the simultaneous evolution of the star's structure, rotation and tidal dissipation in its external convective envelope. We demonstrate that tidal friction due to the stellar dynamical tide, i.e. tidal inertial waves excited in the convection zone, can be larger by several orders of magnitude than the one of the equilibrium tide currently used in Celestial Mechanics, especially during the PMS phase. Moreover, because of this stronger tidal friction in the star, the orbital migration of the planet is now more pronounced and depends more on the stellar mass, rotation and age. This would very weakly affect the planets in the habitable zone because they are located at orbital distances such that stellar tide-induced migration happens on very long timescales. We also demonstrate that the rotational evolution of host stars is only weakly affected by the presence of planets except for massive companions.},
  keywords = {Gaseous planets,notion,notion-database,Planet\textendash star interactions,Planets and satellites: dynamical evolution and st,Stars: evolution,Stars: rotation,Terrestrial planets},
  file = {/Users/lbugnet/Zotero/storage/FK44YDG5/full-text.pdf}
}

@article{Bommier1994,
  title = {Complete Determination of the Magnetic Field Vector and of the Electron Density in 14 Prominences from Linear Polarizaton Measurements in the {{HeI D3}} and {{H}} {$\alpha$} Lines},
  author = {Bommier, V{\'e}ronique and Degl'Innocenti, Egidio Landi and Leroy, Jean Louis and {Sahal-Br{\'e}chot}, Sylvie},
  year = {1994},
  month = oct,
  journal = {Solar Physics},
  volume = {154},
  number = {2},
  pages = {231--260},
  publisher = {{Kluwer Academic Publishers}},
  issn = {00380938},
  doi = {10.1007/BF00681098},
  urldate = {2020-07-13},
  abstract = {The present paper is devoted to the interpretation of linear polarization data obtained in 14 quiescent prominences with the Pic-du-Midi coronagraph-polarimeter by J. L. Leroy, in the two lines He i D3 and H{$\alpha$} quasi-simultaneously. The linear polarization of the lines is due to scattering of the anisotropic photospheric radiation, modified by the Hanle effect due to the local magnetic field. The interpretation of the polarization data in the two lines is able to provide the 3 components of the magnetic field vector, and one extra parameter, namely the electron density, because the linear polarization of H {$\alpha$} is also sensitive to the depolarizing effect of collisions with the electrons and protons of the medium. Moreover, by using two lines with different optical thicknesses, namely He i D3, which is optically thin, and H {$\alpha$}, which is optically thick ({$\tau$} = 1), it is possible to solve the fundamental ambiguity, each line providing two field vector solutions that are symmetrical in direction with respect to the line of sight in the case of the optically thin line, and which have a different symmetry in the case of the optically thick line. It is then possible to determine without ambiguity the polarity of the prominence magnetic field with respect to that of the photospheric field: 12 prominences are found to be Inverse polarity prominences, whereas 2 prominences are found to be Normal polarity prominences. It must be noticed that in 12 of the 14 cases, the line-of-sight component of the magnetic field vector has a Normal polarity (to the extent that the notion of polarity of a vector component is meaningful; no polarity can be derived in the 2 remaining cases); this may explain the controversy between the results obtained with methods based on the Hanle effect with results obtained through the Zeeman effect. A dip of the magnetic field lines across the prominence has been assumed, to which the optically thick H {$\alpha$} line is sensitive, and the optically thin He i D3 line is insensitive. For the Inverse prominences, the average field strength is 7.5{$\pm$}1.2 G, the average angle, {$\alpha$}, between the field vector and the prominence long axis is 36\textdegree{} {$\pm$} 15\textdegree, the average angle, {$\zeta$}, between the outgoing field lines and the solar surface at the prominence boundary is 29\textdegree{} {$\pm$} 20\textdegree, and the average electron density is 2.1 \texttimes{} 1010 {$\pm$} 0.7 \texttimes{} 1010 cm-3. For the Normal prominences, the average field strength is 13.2{$\pm$}2.0 G, the average angle, {$\alpha$}, between the field vector and the prominence long axis is 53\textdegree{} {$\pm$} 15\textdegree, the average angle, {$\zeta$}, between the outgoing field lines and the solar surface at the prominence boundary is 0\textdegree{} {$\pm$} 20\textdegree{} (horizontal field), and the average electron density is 8.7 \texttimes{} 109 {$\pm$} 3.0 \texttimes{} 109 cm-3. \textcopyright{} 1994 Kluwer Academic Publishers.},
  keywords = {Astronomical Polarimetry,Coronagraphs,Deuterium,Electron Density (Concentration),Helium,Line Spectra,Linear Polarization,notion,notion-database,Polarimeters,Solar Magnetic Field,Solar Physics,Solar Prominences,Solar Spectra,Vectors (Mathematics)}
}

@article{Bonanno2007,
  title = {Seismic Inference of Differential Rotation in {{Procyon A}}},
  author = {Bonanno, A and K{\"u}ker, M and Patern{\`o}, L},
  year = {2007},
  volume = {1037},
  pages = {1031--1037},
  keywords = {evolution,individual,interiors,notion,notion-database,oscillations,procyon a,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/W4P6CG7N/Bonanno, Küker, Paternò - 2007.pdf}
}

@article{Bonanno2014,
  title = {Magnetic Activity, Differential Rotation, and Dynamo Action in the Pulsating {{F9IV}} Star {{KIC}} 5955122},
  author = {Bonanno, A. and Fr{\"o}hlich, H. E. and Karoff, C. and Lund, M. N. and Corsaro, E. and Frasca, A.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {569},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424371},
  abstract = {We present photometric spot modeling of the nearly four-year long light-curve of the Kepler target KIC 5955122 in terms of persisting dark circular surface features. With a Bayesian technique, we produced a plausible surface map that shows dozens of small spots. After some artifacts are removed, the residuals are at {$\pm$} 0.16'mmag. The shortest rotational period found is P = 16.4 {$\pm$} 0.2 days. The equator-to-pole extrapolated differential rotation is 0.25 {$\pm$} 0.02 rad/d. The spots are roughly half as bright as the unperturbed stellar photosphere. Spot latitudes are restricted to the zone {$\pm$}60\textdegree{} latitude. There is no indication for any near-pole spots. In addition, the p-mode pulsations enabled us to determine the evolutionary status of the star, the extension of the convective zone, and its radius and mass. We discuss the possibility that the clear signature of active regions in the light curve of the F9IV star KIC 5955122 is produced by a flux-transport dynamo action at the base of the convection zone. In particular, we argue that this star has evolved from an active to a quiet status during the Q0-Q16 period of observation, and we predict, according to our dynamo model, that the characteristic activity cycle is of the order of the solar one.},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Stars: activity,Stars: individual: KIC 5955122,Stars: magnetic field,Stars: rotation,Starspots},
  file = {/Users/lbugnet/Zotero/storage/9VJHTJMD/Bonanno et al. - 2014.pdf}
}

@article{Bonanno2014a,
  title = {Asteroseismic Stellar Activity Relations},
  author = {Bonanno, A. and Corsaro, E. and Karoff, C.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {571},
  pages = {1--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424632},
  abstract = {Context. In asteroseismology an important diagnostic of the evolutionary status of a star is the small frequency separation which is sensitive to the gradient of the mean molecular weight in the stellar interior. It is thus interesting to discuss the classical age-activity relations in terms of this quantity. Moreover, as the photospheric magnetic field tends to suppress the amplitudes of acoustic oscillations, it is important to quantify the importance of this effect by considering various activity indicators. Aims. We propose a new class of age-activity relations that connects the Mt. Wilson S index and the average scatter in the light curve with the small frequency separation and the amplitude of the p-mode oscillations. Methods. We used a Bayesian inference to compute the posterior probability of various empirical laws for a sample of 19 solar-like active stars observed by the Kepler telescope. Results. We demonstrate the presence of a clear correlation between the Mt. Wilson S index and the relative age of the stars as indicated by the small frequency separation, as well as an anti-correlation between the S index and the oscillation amplitudes. We argue that the average activity level of the stars shows a stronger correlation with the small frequency separation than with the absolute age that is often considered in the literature. Conclusions. The phenomenological laws discovered in this paper have the potential to become new important diagnostics to link stellar evolution theory with the dynamics of global magnetic fields. In particular we argue that the relation between the Mt. Wilson S index and the oscillation amplitudes is in good agreement with the findings of direct numerical simulations of magneto-convection.},
  keywords = {Methods: statistical,notion,notion-database,Stars: activity,Stars: chromospheres,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WK5D67ZR/Bonanno, Corsaro, Karoff - 2014.pdf}
}

@article{Bono1998,
  title = {On the {{Theoretical Period-Radius Relation}} of {{Classical Cepheids}}},
  author = {Bono, Giuseppe and Caputo, Filippina and Marconi, Marcella},
  year = {1998},
  journal = {The Astrophysical Journal},
  volume = {497},
  number = {1},
  eprint = {astro-ph/9801242},
  pages = {L43-L46},
  issn = {0004637X},
  doi = {10.1086/311270},
  abstract = {We present the results of a comprehensive theoretical investigation of the period-radius relation of classical Cepheids based on new sequences of full-amplitude, nonlinear, convective models constructed by adopting a wide range of both stellar masses and chemical compositions. In the period range , very good 0.9 {$\leq$} log P {$\leq$} 1.8 agreement is found between theoretical predictions and current available data, whereas outside this range, at both shorter and longer periods, nonlinear radii attain intermediate values between empirical relations based on different Baade-Wesselink methods and photometric bandpasses.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IFRNX9UT/Bono, Caputo, Marconi - 1998.pdf}
}

@techreport{Borne2009,
  title = {Astroinformatics: {{A}} 21st {{Century Approach}} to {{Astronomy}}},
  author = {Borne, Kirk D},
  year = {2009},
  urldate = {2020-04-11},
  abstract = {Data volumes from multiple sky surveys have grown from gigabytes into terabytes during the past decade, and will grow from terabytes into tens (or hundreds) of petabytes in the next decade. This exponential growth of new data both enables and challenges effective astronomical research, requiring new approaches. Thus far, astronomy has tended to address these challenges in an informal and ad hoc manner, with the necessary special expertise being assigned to e-Science or survey science. However, we see an even wider scope and therefore promote a broader vision of this data-driven revolution in astronomical research. For astronomy to effectively cope with and reap the maximum scientific return from existing and future large sky surveys, facilities, and data-producing projects, we need our own information science specialists. We therefore recommend the formal creation, recognition, and support of a major new discipline, which we call Astroinformatics. Astroinformatics includes a set of naturally-related specialties including data organization, data description, astronomical classification taxonomies, astronomical concept ontologies, data mining, machine learning, visualization, and astrostatistics. By virtue of its new stature, we propose that astronomy now needs to integrate Astroinformatics as a formal sub-discipline within agency funding plans, university departments, research programs, graduate training, and undergraduate education. Now is the time for the recognition of Astroinformatics as an essential methodology of astronomical research. The future of astronomy depends on it.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MNQ6AMKS/full-text.pdf}
}

@article{Borucki2008,
  title = {{{KEPLER}}: {{Search}} for Earth-Size Planets in the Habitable Zone},
  author = {Borucki, William and Koch, David and Batalha, Natalie and Caldwell, Douglas and {Christensen-Dalsgaard}, Jorgen and Cochran, William D. and Dunham, Edward and Gautier, Thomas N. and Geary, John and Gilliland, Ronald and Jenkins, Jon and Kjeldsen, Hans and Lissauer, Jack J. and Rowe, Jason},
  year = {2008},
  journal = {Proceedings of the International Astronomical Union},
  volume = {4},
  number = {S253},
  pages = {289--299},
  issn = {17439213},
  doi = {10.1017/S1743921308026513},
  abstract = {The Kepler Mission is a space-based mission whose primary goal is to determine the frequency of Earth-size and larger planets in the habitable zone of solar-like stars. The mission will monitor more than 100,000 stars for patterns of transits with a differential photometric precision of 20 ppm at V = 12 for a 6.5 hour transit. It will also provide asteroseismic results on several thousand dwarf stars. It is specifically designed to continuously observe a single field of view of greater than 100 square degrees for 3.5 or more years. This paper provides a short overview of the mission, a brief history of the mission development, expected results, new investigations by the recently chosen Participating Scientists, and the plans for the Guest Observer and Astrophysical Data Programs. \textcopyright{} 2009 International Astronomical Union.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FDPCDQMG/Borucki et al. - 2008.pdf}
}

@article{Borucki2010,
  title = {Kepler Planet-Detection Mission: {{Introduction}} and First Results},
  author = {Borucki, William J. and Koch, David and Basri, Gibor and Batalha, Natalie and Brown, Timothy and Caldwell, Douglas and Caldwell, John and {Christensen-Dalsgaard}, Jo{\o}rgen and Cochran, William D. and Devore, Edna and Dunham, Edward W. and Dupree, Andrea K. and Gautier, Thomas N. and Geary, John C. and Gilliland, Ronald and Gould, Alan and Howell, Steve B. and Jenkins, Jon M. and Kondo, Yoji and Latham, David W. and Marcy, Geoffrey W. and Meibom, Soren and Kjeldsen, Hans and Lissauer, Jack J. and Monet, David G. and Morrison, David and Sasselov, Dimitar and Tarter, Jill and Boss, Alan and Brownlee, Don and Owen, Toby and Buzasi, Derek and Charbonneau, David and Doyle, Laurance and Fortney, Jonathan and Ford, Eric B. and Holman, Matthew J. and Seager, Sara and Steffen, Jason H. and Welsh, William F. and Rowe, Jason and Anderson, Howard and Buchhave, Lars and Ciardi, David and Walkowicz, Lucianne and Sherry, William and Horch, Elliott and Isaacson, Howard and Everett, Mark E. and Fischer, Debra and Torres, Guillermo and Johnson, John Asher and Endl, Michael and MacQueen, Phillip and Bryson, Stephen T. and Dotson, Jessie and Haas, Michael and Kolodziejczak, Jeffrey and Van Cleve, Jeffrey and Chandrasekaran, Hema and Twicken, Joseph D. and Quintana, Elisa V. and Clarke, Bruce D. and Allen, Christopher and Li, Jie and Wu, Haley and Tenenbaum, Peter and Verner, Ekaterina and Bruhweiler, Frederick and Barnes, Jason and Prsa, Andrej},
  year = {2010},
  journal = {Science},
  volume = {327},
  number = {5968},
  pages = {977--980},
  issn = {00368075},
  doi = {10.1126/science.1185402},
  abstract = {The Kepler mission was designed to determine the frequency of Earth-sized planets in and near the habitable zone of Sun-like stars. The habitable zone is the region where planetary temperatures are suitable for water to exist on a planet's surface. During the first 6 weeks of observations, Kepler monitored 156,000 stars, and five new exoplanets with sizes between 0.37 and 1.6 Jupiter radii and orbital periods from 3.2 to 4.9 days were discovered. The density of the Neptune-sized Kepler-4b is similar to that of Neptune and GJ 436b, even though the irradiation level is 800,000 times higher. Kepler-7b is one of the lowest-density planets ({$\sim$}0.17 gram per cubic centimeter) yet detected. Kepler-5b, -6b, and -8b confirm the existence of planets with densities lower than those predicted for gas giant planets.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5MCXLSLD/Borucki et al. - 2010.pdf}
}

@article{Borucki2012,
  title = {Kepler-22b: {{A}} 2.4 Earth-Radius Planet in the Habitable Zone of a Sun-like Star},
  author = {Borucki, William J. and Koch, David G. and Batalha, Natalie and Bryson, Stephen T. and Rowe, Jason and Fressin, Francois and Torres, Guillermo and Caldwell, Douglas A. and {Christensen-Dalsgaard}, J{\o}rgen and Cochran, William D. and Devore, Edna and Gautier, Thomas N. and Geary, John C. and Gilliland, Ronald and Gould, Alan and Howell, Steve B. and Jenkins, Jon M. and Latham, David W. and Lissauer, Jack J. and Marcy, Geoffrey W. and Sasselov, Dimitar and Boss, Alan and Charbonneau, David and Ciardi, David and Kaltenegger, Lisa and Doyle, Laurance and Dupree, Andrea K. and Ford, Eric B. and Fortney, Jonathan and Holman, Matthew J. and Steffen, Jason H. and Mullally, Fergal and Still, Martin and Tarter, Jill and Ballard, Sarah and Buchhave, Lars A. and Carter, Josh and Christiansen, Jessie L. and Demory, Brice Olivier and D{\'e}sert, Jean Michel and Dressing, Courtney and Endl, Michael and Fabrycky, Daniel and Fischer, Debra and Haas, Michael R. and Henze, Christopher and Horch, Elliott and Howard, Andrew W. and Isaacson, Howard and Kjeldsen, Hans and Johnson, John Asher and Klaus, Todd and Kolodziejczak, Jeffery and Barclay, Thomas and Li, Jie and Meibom, S{\o}ren and Prsa, Andrej and Quinn, Samuel N. and Quintana, Elisa V. and Robertson, Paul and Sherry, William and Shporer, Avi and Tenenbaum, Peter and Thompson, Susan E. and Twicken, Joseph D. and Van Cleve, Jeffrey and Welsh, William F. and Basu, Sarbani and Chaplin, William and Miglio, Andrea and Kawaler, Steven D. and Arentoft, Torben and Stello, Dennis and Metcalfe, Travis S. and Verner, Graham A. and Karoff, Christoffer and Lundkvist, Mia and Lund, Mikkel N. and Handberg, Rasmus and Elsworth, Yvonne and Hekker, Saskia and Huber, Daniel and Bedding, Timothy R. and Rapin, William},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {745},
  number = {2},
  issn = {15384357},
  doi = {10.1088/0004-637X/745/2/120},
  abstract = {A search of the time-series photometry from NASA's Kepler spacecraft reveals a transiting planet candidate orbiting the 11th magnitude G5 dwarf KIC 10593626 with a period of 290 days. The characteristics of the host star are well constrained by high-resolution spectroscopy combined with an asteroseismic analysis of the Kepler photometry, leading to an estimated mass and radius of 0.970 0.060 M and 0.979 0.020 R. The depth of 492 10 ppm for the three observed transits yields a radius of 2.38 0.13 Re for the planet. The system passes a battery of tests for false positives, including reconnaissance spectroscopy, high-resolution imaging, and centroid motion. A full BLENDER analysis provides further validation of the planet interpretation by showing that contamination of the target by an eclipsing system would rarely mimic the observed shape of the transits. The final validation of the planet is provided by 16 radial velocities (RVs) obtained with the High Resolution Echelle Spectrometer on Keck I over a one-year span. Although the velocities do not lead to a reliable orbit and mass determination, they are able to constrain the mass to a 3{$\sigma$} upper limit of 124 M {$\oplus$}, safely in the regime of planetary masses, thus earning the designation Kepler-22b. The radiative equilibrium temperature is 262 K for a planet in Kepler-22b's orbit. Although there is no evidence that Kepler-22b is a rocky planet, it is the first confirmed planet with a measured radius to orbit in the habitable zone of any star other than the Sun. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,planetary systems,stars: fundamental parameters,{stars: individual (Kepler-22, KIC 10593626)}},
  file = {/Users/lbugnet/Zotero/storage/MC6F79P2/Borucki et al. - 2012(2).pdf}
}

@article{Borucki2012a,
  title = {Radii in the {{Habitable Zone}}},
  author = {Borucki, William J and Agol, Eric and Fressin, Francois and Kaltenegger, Lisa and Rowe, Jason and Fischer, Debra and Batalha, Natalie and Lissauer, Jack J and Marcy, Geoffrey W and D{\'e}sert, Jean-michel and Bryson, Stephen T and Barclay, Thomas and Bastien, Fabienne and Charbonneau, David and Crepp, Justin R and {Christensen-dalsgaard}, J{\o}rgen and Jessie, L and Ciardi, David and Cochran, William D and Devore, Edna and Doyle, Laurance and Andrea, K and Endl, Michael and Everett, Mark E and Ford, Eric B and Fortney, Jonathan and Thomas, N and Iii, Gautier and Geary, John C and Gould, Alan and Haas, Michael and Henze, Christopher and Andrew, W and Howell, Steve B and Huber, Daniel and Jenkins, Jon M and Kjeldsen, Hans and Kolbl, Rea and Latham, David W and Lee, Brian L and Lopez, Eric and Mullally, Fergal and Jerome, A and Prsa, Andrej and Quintana, Elisa V and Sasselov, Dimitar and Seader, Shawn and Shporer, Avi and Steffen, Jason H and Still, Martin and Tenenbaum, Peter and Thompson, Susan E and Torres, Guillermo and Twicken, Joseph D and Welsh, William F and Winn, Joshua N},
  year = {2012},
  journal = {Science},
  volume = {340},
  number = {May},
  pages = {1--34},
  doi = {10.1126/science.1234702},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZNNNHHEX/Borucki et al. - 2012.pdf}
}

@article{Bossini2016,
  title = {{{ASTEROSEISMOLOGY OF RED GIANT STARS}} : {{A TOOL FOR CONSTRAINING}} By},
  author = {Bossini, Diego},
  year = {2016},
  number = {June},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZTAQH8T6/Bossini - 2016.pdf}
}

@article{Boston2023,
  title = {Relativistic {{Corrections}} in {{White Dwarf Asteroseismology}}},
  author = {Boston, S. Reece and Evans, Charles R. and Clemens, J. Christopher},
  year = {2023},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {952},
  pages = {87},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/acd446},
  urldate = {2023-09-19},
  abstract = {With the precision now afforded by modern space-based photometric observations from the retired K2 and current TESS missions, the effects of general relativity (GR) may be detectable in the light curves of pulsating white dwarfs (WDs). Almost all WD models are calculated using a Newtonian description of gravity and hydrodynamics. To determine if the inclusion of GR leads to observable effects, we used idealized models of compact stars and made side-by-side comparisons of mode periods computed using a: (i) Newtonian and (ii) GR description of the equilibrium structure and nonradial pulsations. For application to WDs, it is only necessary to include the first post-Newtonian (1PN) approximation to GR. The mathematical nature of the linear nonradial pulsation problem is then qualitatively unchanged and the GR corrections can be written as extensions of the classic Dziembowski equations. As such, GR effects might easily be included in existing asteroseismology codes. The idealized stellar models are (i) 1PN relativistic polytropes and (ii) stars with a cold degenerate electron equation of state featuring a near-surface chemical transition from {$\mu$} e = 2 to {$\mu$} e = 1, simulating a surface hydrogen layer. A comparison of Newtonian and 1PN normal mode periods reveals fractional differences in the order of the surface gravitational redshift z. For a typical WD, this fractional difference is \textasciitilde 10-4 and is greater than the period uncertainty {$\sigma$} {$\Pi$}/{$\Pi$} of many WD pulsation modes observed by TESS. Consistent theoretical modeling of periods observed in these stars should, in principle, include GR effects to 1PN order.},
  keywords = {1799,641,661,73,Asteroseismology,Astrophysics - High Energy Astrophysical Phenomena,Astrophysics - Solar and Stellar Astrophysics,General relativity,General Relativity and Quantum Cosmology,Gravitation,White dwarf stars},
  annotation = {ADS Bibcode: 2023ApJ...952...87B},
  file = {/Users/lbugnet/Zotero/storage/94QMUR4T/Boston et al. - 2023 - Relativistic Corrections in White Dwarf Asteroseis.pdf}
}

@techreport{Bostrom2007,
  title = {Calibrating {{Random Forests}}},
  author = {Bostr{\"o}m, Henrik},
  year = {2007},
  urldate = {2020-04-11},
  abstract = {When using the output of classifiers to calculate the expected utility of different alternatives in decision situations, the correctness of predicted class probabilities may be of crucial importance. However, even very accurate classifiers may output class probabilities of rather poor quality. One way of overcoming this problem is by means of calibration, i.e., mapping the original class probabilities to more accurate ones. Previous studies have however indicated that random forests are difficult to calibrate by standard calibration methods. In this work, a novel calibration method is introduced, which is based on a recent finding that probabilities predicted by forests of classification trees have a lower squared error compared to those predicted by forests of probability estimation trees (PETs). The novel calibration method is compared to the two standard methods, Platt scaling and isotonic regression, on 34 datasets from the UCI repository. The experiment shows that random forests of PETs calibrated by the novel method significantly outper-form uncalibrated random forests of both PETs and classification trees, as well as random forests calibrated with the two standard methods, with respect to the squared error of predicted class probabilities.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IACPHZ6V/full-text.pdf}
}

@article{Bostrom2008,
  title = {Calibrating {{Random Forests}}},
  author = {Bostr{\"o}m, Henrik},
  year = {2008},
  journal = {IEEE Xplore},
  urldate = {2020-04-04},
  abstract = {When using the output of classifiers to calculate the expected utility of different alternatives in decision situations, the correctness of predicted class probabilities may be of crucial importance. However, even very accurate classifiers may output class probabilities of rather poor quality. One way of overcoming this problem is by means of calibration, i.e., mapping the original class probabilities to more accurate ones. Previous studies have however indicated that random forests are difficult to calibrate by standard calibration methods. In this work, a novel calibration method is introduced, which is based on a recent finding that probabilities predicted by forests of classification trees have a lower squared error compared to those predicted by forests of probability estimation trees (PETs). The novel calibration method is compared to the two standard methods, Platt scaling and isotonic regression, on 34 datasets from the UCI repository. The experiment shows that random forests of PETs calibrated by the novel method significantly outper-form uncalibrated random forests of both PETs and classification trees, as well as random forests calibrated with the two standard methods, with respect to the squared error of predicted class probabilities.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GHDAPZAA/full-text.pdf}
}

@article{Bostrom2012,
  title = {Forests of Probability Estimation Trees},
  author = {Bostr{\"o}m, Henrik},
  year = {2012},
  month = mar,
  journal = {International Journal of Pattern Recognition and Artificial Intelligence},
  volume = {26},
  number = {2},
  publisher = {{World Scientific Publishing Company}},
  issn = {02180014},
  doi = {10.1142/S0218001412510019},
  urldate = {2020-04-11},
  abstract = {Probability estimation trees (PETs) generalize classification trees in that they assign class probability distributions instead of class labels to examples that are to be classified. This property has been demonstrated to allow PETs to outperform classification trees with respect to ranking performance, as measured by the area under the ROC curve (AUC). It has further been shown that the use of probability correction improves the performance of PETs. This has lead to the use of probability correction also in forests of PETs. However, it was recently observed that probability correction may in fact deteriorate performance of forests of PETs. A more detailed study of the phenomenon is presented and the reasons behind this observation are analyzed. An empirical investigation is presented, comparing forests of classification trees to forests of both corrected and uncorrected PETS on 34 data sets from the UCI repository. The experiment shows that a small forest (10 trees) of probability corrected PETs gives a higher AUC than a similar-sized forest of classification trees, hence providing evidence in favor of using forests of probability corrected PETs. However, the picture changes when increasing the forest size, as the AUC is no longer improved by probability correction. For accuracy and squared error of predicted class probabilities (Brier score), probability correction even leads to a negative effect. An analysis of the mean squared error of the trees in the forests and their variance, shows that although probability correction results in trees that are more correct on average, the variance is reduced at the same time, leading to an overall loss of performance for larger forests. The main conclusions are that probability correction should only be employed in small forests of PETs, and that for larger forests, classification trees and PETs are equally good alternatives. \textcopyright{} 2012 World Scientific Publishing Company.},
  keywords = {accuracy,area under ROC curve,Brier score,notion,notion-database,probability estimation trees,Random forests}
}

@article{Bouabid2013,
  title = {Effects of the {{Coriolis}} Force on High-Order g Modes in {$\gamma$} {{Doradus}} Stars},
  author = {Bouabid, M. P. and Dupret, M. A. and Salmon, S. and Montalb{\'a}n, J. and Miglio, A. and Noels, A.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {429},
  number = {3},
  pages = {2500--2514},
  issn = {00358711},
  doi = {10.1093/mnras/sts517},
  abstract = {{$\gamma$} Doradus stars pulsate with high-order gravity modes having typical frequencies which can be comparable to or higher than their rotation frequencies. Therefore, rotation has a nonnegligible effect on their oscillation properties. To explore the rotation-pulsation coupling in {$\gamma$} Dor stars, we perform a non-adiabatic study including the traditional approximation of rotation on a grid of spherical stellar models covering the mass range 1.4 {$<$} M* {$<$} 2.1M{$\odot$}. This approximation allows us to treat the effect of the Coriolis force on the frequencies and the stability of high-order g modes. The effect of the Coriolis force depends on the kind of mode considered (prograde sectoral or not) and increases with their periods. As a consequence, we first find that the period spacing between modes is no longer periodically oscillating around a constant value. Secondly, we showthat the frequency gap (5-15 cycles day-1) arising from stablemodes between {$\gamma$} Dor-type high-order g modes and {$\delta$} Scuti-type modes can be easily filled by g-mode frequencies shifted to higher values by the rotation. Thirdly, we analyse the combined effect of diffusive mixing and the Coriolis force on the period spacings. And finally, we predict a slight broadening of the {$\gamma$} Dor instability strip. \textcopyright{} 2013 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {General,notion,notion-database,Oscillations-Stars,Rotation-Stars,Stars,Variables},
  file = {/Users/lbugnet/Zotero/storage/HTYDZPQV/Bouabid et al. - 2013.pdf}
}

@article{Bouchy2001,
  title = {P-Mode Observations on {{Alpha Cen A}}},
  author = {Bouchy, Francois and Carrier, Fabien},
  year = {2001},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {374},
  number = {1},
  eprint = {astro-ph/0107099},
  pages = {L5-L8},
  publisher = {{EDP Sciences}},
  doi = {10.1051/0004-6361:20010792},
  urldate = {2020-03-08},
  abstract = {We have made a clear detection of p-mode oscillations in the nearest solar-like G2V star \$\textbackslash alpha\$ Cen A with the CORALIE spectrograph on the 1.2-m Swiss telescope at the ESO La Silla Observatory. We report the 5 nights of observation on this star in May 2001 during which 1260 high precision radial velocity measurements were obtained. The power spectrum clearly shows several identifiable peaks between 1.7 and 3 mHz. The average large splitting of 105.7 \$\textbackslash mu\$Hz and the amplitude of about 35 cm s\$\^\{-1\}\$ of these modes are in agreement with theoretical expectations.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,STARS: INDIVIDUAL: ALPHA CEN A,STARS: OSCILLATIONS,TECHNIQUES: RADIAL VELOCITIES},
  file = {/Users/lbugnet/Zotero/storage/YACME2N6/full-text.pdf}
}

@article{Bouchy2002,
  title = {The Acoustic Spectrum of {$\alpha$} {{Cen A}}},
  author = {Bouchy, F. and Carrier, F.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {390},
  number = {1},
  pages = {205--212},
  issn = {00046361},
  doi = {10.1051/0004-6361:20020706},
  abstract = {This paper presents the analysis of Doppler p-mode observations of the G2V star {$\alpha$} Cen A obtained with the spectrograph CORALIE in May 2001. Thirteen nights of observations have made it possible to collect 1850 radial velocity measurements with a standard deviation of about 1.5 m s-1. Twenty-eight oscillation modes have been identified in the power spectrum between 1.8 and 2.9 mHz with amplitudes in the range 12 to 44 cm s-1. The average large and small spacing are respectively equal to 105.5 and 5.6 {$\mu$}Hz. A comparison with stellar models of {$\alpha$} Cen A is presented.},
  keywords = {notion,notion-database,Stars: individual,Stars: oscillations,{$\alpha$} Cen A},
  file = {/Users/lbugnet/Zotero/storage/R8T9ZSGD/Bouchy, Carrier - 2002.pdf}
}

@article{Boumier2014,
  title = {Seismic Analysis of {{HD 43587Aa}}, a Solar-like Oscillator in a Multiple System},
  author = {Boumier, P. and Benomar, O. and Baudin, F. and Verner, G. and Appourchaux, T. and Lebreton, Y. and Gaulme, P. and Chaplin, W. and Garc{\'i}a, R. A. and Hekker, S. and Regulo, C. and Salabert, D. and Stahn, T. and Elsworth, Y. and Gizon, L. and Hall, M. and Mathur, S. and Michel, E. and Morel, T. and Mosser, B. and Poretti, E. and Rainer, M. and Roxburgh, I. and Do Nascimento, J. D. and Samadi, R. and Auvergne, M. and Chaintreuil, S. and Baglin, A. and Catala, C.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {564},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/201322478},
  abstract = {Context. The object HD 43587Aa is a G0V star observed during the 145-day LRa03 run of the COnvection, ROtation and planetary Transits space mission (CoRoT), for which complementary High Accuracy Radial velocity Planet Searcher (HARPS) spectra with S/N {$>$} 300 were also obtained. Its visual magnitude is 5.71, and its effective temperature is close to 5950 K. It has a known companion in a highly eccentric orbit and is also coupled with two more distant companions. Aims. We undertake a preliminary investigation of the internal structure of HD 43587Aa. Methods. We carried out a seismic analysis of the star, using maximum likelihood estimators and Markov chain Monte Carlo methods. Results. We established the first table of the eigenmode frequencies, widths, and heights for HD 43587Aa. The star appears to have a mass and a radius slightly larger than the Sun, and is slightly older (5.6 Gyr). Two scenarios are suggested for the geometry of the star: either its inclination angle is very low, or the rotation velocity of the star is very low. Conclusions. A more detailed study of the rotation and of the magnetic and chromospheric activity for this star is needed, and will be the subject of a further study. New high resolution spectrometric observations should be performed for at least several months in duration. \textcopyright{} 2014 ESO.},
  keywords = {Asteroseismology,Binaries: general,Methods: data analysis,notion,notion-database,Stars: individual: HD 43587Aa,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/GJRANQ5T/Boumier et al. - 2014.pdf}
}

@article{Bourguignon2007,
  title = {{{SparSpec}}: {{A}} New Method for Fitting Multiple Sinusoids with Irregularly Sampled Data},
  author = {Bourguignon, S. and Carfantan, H. and B{\"o}hm, T.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {462},
  number = {1},
  pages = {379--387},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065452},
  abstract = {Context: The location of pure frequencies in the spectrum of an irregularly sampled time series is an important topic in astrophysical data analysis. Especially in the domain of asteroseismology, a highly precise and unambiguous study of frequencies in photometric light or radial velocity curves is required. Aims: Due to sampling irregularities and large observational gaps, the classic methods for frequency estimation (prewhitening techniques, CLEAN, CLEANEST, etc.) sometimes suffer false detections. We propose a new framework for this problem that allows a more precise and unambiguous frequency location. Methods: Multisine fitting is addressed as the sparse representation of the data in an overcomplete dictionary of frequencies, hence the name SparSpec for the method. We model the data as the sum of an arbitrarily large number of pure frequencies, discretised on a fixed grid. Among all the many representations fitting the data, we seek the one with the fewest non-zero amplitudes. This solution can be computed by minimising a convex criterion with no local minima. A computationally efficient and convergent optimisation strategy is derived and a user-friendly software implementing SparSpec is provided online at http://www.ast.obs-mip.fr/Softwares. Results: The method is first illustrated on a simple test example where SparSpec correctly locates the frequencies while classic methods fail. Then, simulations on more realistic artificial time series reveal the interest of this new methodology in terms of robustness toward sampling aliases. An application to the radial velocity curve of the pre-main sequence Herbig Ae star HD 104237 is finally presented, where the method is able to determine oscillation frequencies even in the presence of strong low-frequency perturbations such as orbital movements. While SparSpec mainly confirms previously published studies for the four more important frequencies, it suggests some ambiguity about the position of a fifth frequency. Additional simulations show that the SparSpec results are more plausible. \textcopyright{} ESO 2007.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: individual: HD 104237,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WD7RKF4I/Bourguignon, Carfantan, Böhm - 2007.pdf}
}

@article{Boury1971,
  title = {Les Progr\`es de La Th\'eorie de l'\'evolution Stellaire - {{NASA}}/{{ADS}}},
  author = {Boury, A. and Gabriel, M.},
  year = {1971},
  journal = {C\&T},
  volume = {87},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8L75ZLSP/Boury, Gabriel - 1971.pdf}
}

@techreport{Bouvier1997,
  title = {The Angular Momentum Evolution of Low-Mass Stars},
  author = {Bouvier, J and Forestini, M and Allain, S},
  year = {1997},
  journal = {Astronomy \& Astrophysics},
  volume = {326},
  pages = {1023--1043},
  issn = {0004-6361},
  urldate = {2020-07-17},
  abstract = {We present a model for the evolution of surface rotation of stars in the mass range from 0.5 to 1.1M , from their first appearance in the HR diagram as T Tauri stars up to the age of the Sun. The model is based on 3 assumptions: i) nearly solid-body rotation, ii) pre-main sequence disk locking, iii) wind braking. The initial conditions and the calibration of the braking law are completely determined from observations. The model includes only 2 adjustable parameters: the distribution of disk lifetimes in the pre-main sequence and the velocity at which saturation of the angular momentum losses due to the stellar wind occurs. We review all the observational results, including the most recent ones, that can be used to constrain the models, as well as theoretical work that puts limits onto the parameter space. We show that the currently available distributions of vsini for PMS, ZAMS and MS stars can be reasonably well reproduced by the model assuming solid-body rotation for stars in the mass-range from 0.5 to 1.1M. We deduce a median lifetime of 3 Myr for circumstellar accretion disks around pre-main sequence stars. By an age of 20 Myr, only 10\% of the stars are still surrounded by disks. Stars with long disk lifetimes and low initial rota-tional velocities account for the large fraction of slow rotators (vsini{$\leq$}20 km s -1) observed in young clusters. On the opposite, stars with short-lived disk reach the ZAMS with velocities up to 200 km s -1 over the whole mass range investigated here. In agreement with other models, we find that a mass-dependent saturation velocity for the angular momentum losses is required to account for the longer spin down timescale of lower mass stars on the zero-age main sequence. We argue that this assumption provides an alternative to the hypothesis of ra-diative core-convective envelope decoupling, which has been used in other models. Both the rapid spin down of fast rotators on the ZAMS and its mass-dependency are accounted for in the present solid-body rotation models. In particular, we show that the model predicts a distribution of rotational periods at the age of the Hyades for 0.5-1.1M stars that is in close agreement with the observations. We conclude that the observed evolution of moderate and fast rotators on the early main sequence requires physical processes that lead to the redistribution of angular momentum Send offprint requests to: J. Bouvier in stellar interiors on a timescale much shorter than evolutionary timescales, such as dynamical rotational instabilities, gravity waves or MHD torques. The evolution of slow rota-tors (vsini{$\leq$}10 km s -1), however, remains uncertain due to the currently uncomplete vsini distribution. Precise vsini measurements for slow rotators in young clusters, rather than upper limits, are required.},
  keywords = {notion,notion-database,pre-main sequence,rotation-stars,stars},
  file = {/Users/lbugnet/Zotero/storage/Q93RTCUI/full-text.pdf}
}

@article{Bouvier2007,
  title = {The Rotational Evolution of Young Low Mass Stars},
  author = {Bouvier, J{\'e}r{\^o}me},
  year = {2007},
  journal = {Proceedings of the International Astronomical Union},
  volume = {3},
  number = {1 S243},
  pages = {231--240},
  issn = {17439213},
  doi = {10.1017/S1743921307009593},
  abstract = {Abstract Star-disk interaction is thought to drive the angular momentum evolution of young stars. In this review, I present the latest results obtained on the rotational properties of low mass and very low mass pre-main sequence stars. I discuss the evidence for extremely efficient angular momentum removal over the first few Myr of pre-main sequence evolution and describe recent results that support an accretion-driven braking mechanism. Angular momentum evolution models are presented and their implication for accretion disk lifetimes discussed. \textcopyright{} 2007 International Astronomical Union.},
  isbn = {1743921307009},
  keywords = {Accretion,Accretion disks,notion,notion-database,Stars: premain-sequence,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/D33QPZLI/Bouvier - 2007.pdf}
}

@book{Bouvier2014,
  title = {Angular {{Momentum Evolution}} of {{Young Low-Mass Stars}} and {{Brown Dwarfs}}: {{Observations}} and {{Theory}}},
  shorttitle = {Angular {{Momentum Evolution}} of {{Young Low-Mass Stars}} and {{Brown Dwarfs}}},
  author = {Bouvier, J. and Matt, S. P. and Mohanty, S. and Scholz, A. and Stassun, K. G. and Zanni, C.},
  year = {2014},
  month = jan,
  pages = {433--450},
  address = {{eprint: arXiv:1309.7851}},
  doi = {10.2458/azu_uapress_9780816531240-ch019},
  urldate = {2023-10-26},
  abstract = {This chapter aims at providing the most complete review of both the emerging concepts and the latest observational results regarding the angular momentum evolution of young low-mass stars and brown dwarfs. In the time since Protostars and Planets V (Reipurth et al., 2007) (PPV), there have been major developments in the availability of rotation-period measurements at multiple ages and in different star-forming environments that are essential for testing theory. In parallel, substantial theoretical developments have been carried out in the last few years, including the physics of the star-disk interaction, numerical simulations of stellar winds, and the investigation of angular momentum transport processes in stellar interiors. This chapter reviews both the recent observational and theoretical advances that prompted the development of renewed angular momentum evolution models for cool stars and brown dwarfs. While the main observational trends of the rotational history of low-mass objects seem to be accounted for by these new models, a number of critical open issues remain that are outlined in this review.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2014prpl.conf..433B},
  file = {/Users/lbugnet/Zotero/storage/A88ZV4TW/Bouvier et al. - 2014 - Angular Momentum Evolution of Young Low-Mass Stars.pdf}
}

@article{Bovy2014,
  title = {The Apogee Red-Clump Catalog: {{Precise}} Distances, Velocities, and High-Resolution Elemental Abundances over a Large Area of the Milky Way's Disk},
  author = {Bovy, Jo and Nidever, David L. and Rix, Hans Walter and Girardi, L{\'e}o and Zasowski, Gail and Chojnowski, S. Drew and Holtzman, Jon and Epstein, Courtney and Frinchaboy, Peter M. and Hayden, Michael R. and Rodrigues, Tha{\'i}se S. and Majewski, Steven R. and Johnson, Jennifer A. and Pinsonneault, Marc H. and Stello, Dennis and Allende Prieto, Carlos and Andrews, Brett and Basu, Sarbani and Beers, Timothy C. and Bizyaev, Dmitry and Burton, Adam and Chaplin, William J. and Cunha, Katia and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and {Garc{\'i}a-Her{\'n}andez}, Domingo A. and Garc{\'i}a P{\'e}rez, Ana E. and Hearty, Fred R. and Hekker, Saskia and Kallinger, Thomas and Kinemuchi, Karen and Koesterke, Lars and M{\'e}sz{\'a}ros, Szabolcs and Mosser, Beno{\^i}t and O'Connell, Robert W. and Oravetz, Daniel and Pan, Kaike and Robin, Annie C. and Schiavon, Ricardo P. and Schneider, Donald P. and Schultheis, Mathias and Serenelli, Aldo and Shetrone, Matthew and Silva Aguirre, Victor and Simmons, Audrey and Skrutskie, Michael and Smith, Verne V. and Stassun, Keivan and Weinberg, David H. and Wilson, John C. and Zamora, Olga},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {790},
  number = {2},
  eprint = {1405.1032},
  issn = {15384357},
  doi = {10.1088/0004-637X/790/2/127},
  abstract = {The Sloan Digital Sky Survey III's Apache Point Observatory Galactic Evolution Experiment (APOGEE) is a high-resolution near-infrared spectroscopic survey covering all of the major components of the Galaxy, including the dust-obscured regions of the inner Milky Way disk and bulge. Here we present a sample of 10,341 likely red-clump stars (RC) from the first two years of APOGEE operations, selected based on their position in color-metallicity-surface- gravity-effective-temperature space using a new method calibrated using stellar evolution models and high-quality asteroseismology data. The narrowness of the RC locus in color-metallicity-luminosity space allows us to assign distances to the stars with an accuracy of 5\%-10\%. The sample extends to typical distances of about 3 kpc from the Sun, with some stars out to 8 kpc, and spans a volume of approximately 100 kpc3 over 5 kpc {$\lessequivlnt$} R {$\lessequivlnt$} 14 kpc, |Z| {$\lessequivlnt$} 2 kpc, and -15\textdegree{} {$\lessequivlnt$} Galactocentric azimuth {$\lessequivlnt$} 30\textdegree. The APOGEE red-clump (APOGEE-RC) catalog contains photometry from the Two Micron All Sky Survey, reddening estimates, distances, line-of-sight velocities, stellar parameters and elemental abundances determined from the high-resolution APOGEE spectra, and matches to major proper motion catalogs. We determine the survey selection function for this data set and discuss how the RC selection samples the underlying stellar populations. We use this sample to limit any azimuthal variations in the median metallicity within the 45\textdegree azimuthal region covered by the current sample to be {$\leq$}0.02 dex, which is more than an order of magnitude smaller than the radial metallicity gradient. This result constrains coherent non-axisymmetric flows within a few kiloparsecs from the Sun. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {Galaxy: abundances,Galaxy: disk,Galaxy: stellar content,Galaxy: structure,notion,notion-database,stars: distances,stars: general},
  file = {/Users/lbugnet/Zotero/storage/ND4J6N7W/Bovy et al. - 2014.pdf}
}

@techreport{Bowman2016,
  title = {Amplitude Modulation and Energy Conservation of Pulsation Modes in Delta {{Scuti}} Stars},
  author = {Bowman, Dominic M},
  year = {2016},
  urldate = {2020-03-24},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TJH99MJI/full-text.pdf}
}

@misc{Bowman2022,
  title = {Asteroseismology Reveals the Near-Core Magnetic Field Strength in the Early-{{B}} Star {{HD}} 43317},
  author = {Bowman, D. M. and Lecoanet, D. and Van Reeth, T.},
  year = {2022},
  month = jul,
  number = {arXiv:2207.08526},
  eprint = {2207.08526},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-05-09},
  abstract = {Spectropolarimetic campaigns have established that large-scale magnetic fields are present at the surfaces of approximately 10\% of massive dwarf stars. However, there is a dearth of magnetic field measurements for their deep interiors. Asteroseismology of gravity-mode pulsations combined with rotating magneto-hydrodynamical calculations of the early-B main-sequence star HD 43317 constrain its magnetic field strength to be approximately \$5\textbackslash times10\^\{5\}\$ G just outside its convective core. This proof-of-concept study for magneto-asteroseismology opens a new window into the observational characterisation of magnetic fields inside massive stars.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/E9AGS2A2/Bowman et al. - 2022 - Asteroseismology reveals the near-core magnetic fi.pdf;/Users/lbugnet/Zotero/storage/GJGNH5B2/2207.html}
}

@article{Bradshaw2014,
  title = {On Sunspot and Starspot Lifetimes},
  author = {Bradshaw, S. J. and Hartigan, P.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {795},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/795/1/79},
  abstract = {We consider the lifetimes of spots on the Sun and other stars from the standpoint of magnetic diffusion. While normal magnetic diffusivity predicts lifetimes of sunspots that are too large by at least two orders of magnitude, turbulent magnetic diffusivity accounts for both the functional form of the solar empirical spot-lifetime relation and for the observed sunspot lifetimes, provided that the relevant diffusion length is the supergranule size. Applying this relation to other stars, the value of turbulent diffusivity depends almost entirely on supergranule size, with very weak dependence on other variables such as magnetic field strength and density. Overall, the best observational data for other stars is consistent with the extension of the solar relation, provided that stellar supergranule sizes for some stars are significantly larger than they are on the Sun.},
  keywords = {magnetic fields,notion,notion-database,{stars: variables: T Tauri, Herbig Ae/Be},starspots,Sun: photosphere,sunspots},
  file = {/Users/lbugnet/Zotero/storage/VGNQPJR6/Bradshaw, Hartigan - 2014.pdf}
}

@techreport{Braithwaite,
  title = {Magnetic Fields in Non-Convective Regions of Stars},
  author = {Braithwaite, Jonathan and Spruit, Henk C},
  eprint = {1510.03198v4},
  urldate = {2020-05-01},
  abstract = {We review the current state of knowledge of magnetic fields inside stars, concentrating on recent developments concerning magnetic fields in stably stratified (zones of) stars, leaving out convec-tive dynamo theories and observations of convective envelopes. We include the observational properties of A, B and O-type main-sequence stars, which have radiative envelopes, and the fossil field model which is normally invoked to explain the strong fields sometimes seen in these stars. Observations seem to show that Ap-type stable fields are excluded in stars with con-vective envelopes. Most stars contain both radiative and convective zones, and there are potentially important effects arising from the interaction of magnetic fields at the boundaries between them. Related to this, we discuss whether the Sun could harbour a magnetic field in its core. Recent developments regarding the various convective and radiative layers near the surfaces of early-type stars and their observational effects are examined. We look at possible dynamo mechanisms that run on differential rotation rather than con-vection. Finally we turn to neutron stars with a discussion of the possible origins for their magnetic fields.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/M5V8USZW/full-text.pdf}
}

@article{Braithwaite2004,
  title = {A Fossil Origin for the Magnetic Field in {{A}} Stars and White Dwarfs},
  author = {Braithwaite, Jonathan and Spruit, Hendrik C.},
  year = {2004},
  journal = {Nature},
  volume = {431},
  number = {7010},
  pages = {819--821},
  issn = {00280836},
  doi = {10.1038/nature02934},
  abstract = {Some main-sequence stars of spectral type A are observed to have a strong (0.03-3 tesla), static, large-scale magnetic field, of a chiefly dipolar shape: they are known as 'Ap stars', such as Alioth, the fifth star in the Big Dipper. Following the discovery of these fields, it was proposed that they are remnants of the star's formation, a 'fossil' field. An alternative suggestion is that they could be generated by a dynamo process in the star's convective core. The dynamo hypothesis, however, has difficulty explaining high field strengths and the observed lack of a correlation with rotation. The weakness of the fossil-field theory has been the absence of field configurations stable enough to survive in a star over its lifetime. Here we report numerical simulations that show that stable magnetic field configurations, with properties agreeing with those observed, can develop through evolution from arbitrary, unstable initial fields. The results are applicable equally to Ap stars, magnetic white dwarfs and some highly magnetized neutron stars known as magnetars. This establishes fossil fields as the natural, unifying explanation for the magnetism of all these stars.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NBYX4RNF/Braithwaite, Spruit - 2004.pdf}
}

@article{Braithwaite2006,
  title = {The Stability of Toroidal Fields in Stars},
  author = {Braithwaite, Jonathan},
  year = {2006},
  month = dec,
  journal = {Astronomy and Astrophysics},
  volume = {453},
  number = {2},
  eprint = {astro-ph/0512182},
  pages = {687--698},
  doi = {10.1051/0004-6361:20041282},
  urldate = {2020-06-19},
  abstract = {We present numerical models of hydromagnetic instabilities under the conditions prevailing in a stably stratified, non-convective stellar interior, and compare them with previous results of analytic work on instabilities in purely toroidal fields. We confirm that an \$m=1\$ mode (`kink') is the dominant instability in a toroidal field in which the field strength is proportional to distance from the axis, such as the field formed by the winding up of a weak field by differential rotation. We measure the growth rate of the instability as a function of field strength and rotation rate \$\textbackslash Omega\$, and investigate the effects of a stabilising thermal stratification as well as magnetic and thermal diffusion on the stability. Where comparison is computationally feasible, the results agree with analytic predictions.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,Magnetohydrodynamics (MHD),notion,notion-database,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/R74ZRSDD/full-text.pdf}
}

@article{Braithwaite2006a,
  title = {Stable Magnetic Fields in Stellar Interiors},
  author = {Braithwaite, J. and Nordlund, A},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {450},
  number = {3},
  eprint = {astro-ph/0510316},
  pages = {1077--1095},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041980},
  abstract = {We investigate the 50-year old hypothesis that the magnetic fields of the Ap stars are stable equilibria that have survived in these stars since their formation. With numerical simulations we find that stable magnetic field configurations indeed appear to exist under the conditions in the radiative interior of a star. Confirming a hypothesis by Prendergast (1956, ApJ, 123, 498), the configurations have roughly equal poloidal and toroidal field strengths. We find that tori of such twisted fields can form as remnants of the decay of an unstable random initial field. In agreement with observations, the appearance at the surface is an approximate dipole with smaller contributions from higher multipoles, and the surface field strength can increase with the age of the star. The results of this paper were summarised by Braithwaite \& Spruit (2004, Nature, 431, 891). \textcopyright{} ESO 2006.},
  archiveprefix = {arxiv},
  keywords = {Instabilities - magnetohydrodynamics (MHD) - stars,Magnetic fields,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TYKNMM5G/Braithwaite, Nordlund - 2006.pdf}
}

@article{Braithwaite2007a,
  title = {The Stability of Poloidal Magnetic Fields in Rotating Stars},
  author = {Braithwaite, J.},
  year = {2007},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {469},
  number = {1},
  eprint = {0705.0185},
  pages = {275--284},
  doi = {10.1051/0004-6361:20065903},
  urldate = {2020-05-01},
  abstract = {The stability of large-scale magnetic fields in rotating stars is explored, using 3D numerical hydrodynamics to follow the evolution of an initial poloidal field. It is found that the field is subject to an instability, located initially on the magnetic equator, whereby the gas is displaced in a direction parallel to the magnetic axis. If the magnetic axis is parallel to the rotation axis, the rotation does not affect the initial linear growth of the instability, but does restrict the growth of the instability outside of the equatorial zone. The magnetic energy decays on a timescale which is a function of the Alfv\textbackslash 'en crossing time and the rotation speed, but short compared to any evolutionary timescale. No evidence is found for a possible stable end state to evolve from an initial axisymmetric poloidal field. The field of an oblique rotator is similarly unstable, in both cases regardless of the rotation speed.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,Magnetohydrodynamics (MHD),notion,notion-database,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/ULK3P2HB/full-text.pdf}
}

@article{Braithwaite2008a,
  title = {On Non-Axisymmetric Magnetic Equilibria in Stars},
  author = {Braithwaite, J.},
  year = {2008},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {386},
  number = {4},
  eprint = {0810.1049},
  pages = {1947--1958},
  doi = {10.1111/j.1365-2966.2008.14034.x},
  urldate = {2020-05-01},
  abstract = {In this third paper in a series on stable magnetic equilibria in stars, I look at the stability of axisymmetric field configurations and in particular at the relative strengths of the toroidal and poloidal components. Both toroidal and poloidal fields are unstable on their own, and stability is achieved by adding the two together in some ratio. I use Tayler's (1973) stability conditions for toroidal fields and other analytic tools to predict the range of stable ratios and then check these predictions by running numerical simulations. It is found that while the poloidal field can account for no more than approximately 80\% of the total energy, it can account for a very small fraction of the energy, i.e. that the toroidal field can be -- and is likely to be -- significantly stronger than the poloidal. Furthermore, the weaker the field, the weaker the poloidal component can be in relation to the toroidal. The implications of this result are discussed in various contexts such as the emission of gravitational waves by neutron stars, free precession, and a `hidden' energy source for magnetars.},
  archiveprefix = {arxiv},
  keywords = {MHD,notion,notion-database,Stars: chemically peculiar,Stars: magnetic fields,Stars: neutron,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/LZGI39DG/full-text.pdf}
}

@article{Braithwaite2009,
  title = {Axisymmetric Magnetic Fields in Stars: {{Relative}} Strengths of Poloidal and Toroidal Components},
  author = {Braithwaite, Jonathan},
  year = {2009},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {397},
  number = {2},
  eprint = {0810.1049},
  pages = {763--774},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2008.14034.x},
  urldate = {2020-07-13},
  abstract = {In this third paper in a series on stable magnetic equilibria in stars, I look at the stability of axisymmetric field configurations and, in particular, the relative strengths of the toroidal and poloidal components. Both toroidal and poloidal fields are unstable on their own, and stability is achieved by adding the two together in some ratio. I use Tayler's stability conditions for toroidal fields and other analytic tools to predict the range of stable ratios and then check these predictions by running numerical simulations. If the energy in the poloidal component as a fraction of the total magnetic energy is written as Ep/E, it is found that the stability condition is a(E/U) {$<$} Ep/E {$\lessequivlnt$} 0.8 where E/U is the ratio of magnetic to gravitational energy in the star and a is some dimensionless factor whose value is of order 10 in a main-sequence star and of order 103 in a neutron star. In other words, whilst the poloidal component cannot be significantly stronger than the toroidal, the toroidal field can be very much stronger than the poloidal-given that in realistic stars we expect E/U {$<$} 10-6. The implications of this result are discussed in various contexts such as the emission of gravitational waves by neutron stars, free precession and a 'hidden' energy source for magnetars. \textcopyright{} 2009 RAS.},
  archiveprefix = {arxiv},
  keywords = {MHD,notion,notion-database,Stars: chemically peculiar,Stars: magnetic fields,Stars: neutron,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/JACWV7IZ/full-text.pdf}
}

@article{Braithwaite2013,
  title = {Weak Magnetic Fields in Early-Type Stars: Failed Fossils},
  author = {Braithwaite, Jonathan and Cantiello, Matteo},
  year = {2013},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {428},
  number = {4},
  eprint = {1201.5646v1},
  pages = {2789--2794},
  urldate = {2020-07-03},
  abstract = {Weak magnetic fields have recently been detected in Vega and Sirius. Here, we explore the possibility that these fields are the remnants of some field inherited or created during or shortly after star formation and, unlike true fossil fields, are still evolving as we observe them. The timescale of this evolution is given in terms of the Alfv\'en timescale and the rotation frequency by {$\tau$} evol {$\sim$} {$\tau$} 2 A {$\Omega$}, which would be comparable to the age of the star. It is shown that it is likely that all intermediate-and high-mass stars contain fields of at least the strength found so far in Vega and Sirius. Faster rotators are expected to have stronger magnetic fields. Stars may experience an increase in surface field strength during their early main sequence, but for most of their lives field strength will decrease slowly. The length scale of the magnetic structure on the surface may be small in very young stars but should quickly increase to at least very approximately a fifth of the stellar radius.},
  archiveprefix = {arxiv},
  keywords = {(magnetohydrodynamics) MHD-star,early-type-stars,magnetic fields,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8QDYBN8N/full-text.pdf}
}

@article{Braithwaite2017,
  title = {Magnetic Fields in Non-Convective Regions of Stars},
  author = {Braithwaite, Jonathan and Spruit, Henk C.},
  year = {2017},
  journal = {Royal Society Open Science},
  volume = {4},
  number = {2},
  eprint = {1510.03198},
  pages = {1--48},
  issn = {20545703},
  doi = {10.1098/rsos.160271},
  abstract = {We review the current state of knowledge of magnetic fields inside stars, concentrating on recent developments concerning magnetic fields in stably stratified (zones of) stars, leaving out convective dynamo theories and observations of convective envelopes. We include the observational properties of A, B and O-type main-sequence stars, which have radiative envelopes, and the fossil fieldmodel which is normally invoked to explain the strong fields sometimes seen in these stars. Observations seem to show that Ap-type stable fields are excluded in stars with convective envelopes. Most stars contain both radiative and convective zones, and there are potentially important effects arising from the interaction of magnetic fields at the boundaries between them; the solar cycle being one of the better known examples. Related to this, we discuss whether the Sun could harbour a magnetic field in its core. Recent developments regarding the various convective and radiative layers near the surfaces of early-type stars and their observational effects are examined. We look at possible dynamo mechanisms that run on differential rotation rather than convection. Finally, we turn to neutron stars with a discussion of the possible origins for their magnetic fields.},
  archiveprefix = {arxiv},
  keywords = {Magnetohydrodynamics,notion,notion-database,Stars: magnetic fields,Stars: neutron},
  file = {/Users/lbugnet/Zotero/storage/K76D9DWE/Braithwaite, Spruit - 2017.pdf}
}

@article{Braithwaite2017a,
  title = {Magnetic Fields in Non-Convective Regions of Stars},
  author = {Braithwaite, Jonathan and Spruit, Henk C.},
  year = {2017},
  month = feb,
  journal = {Royal Society Open Science},
  volume = {4},
  pages = {160271},
  doi = {10.1098/rsos.160271},
  urldate = {2023-10-06},
  abstract = {We review the current state of knowledge of magnetic fields inside stars, concentrating on recent developments concerning magnetic fields in stably stratified (zones of) stars, leaving out convective dynamo theories and observations of convective envelopes. We include the observational properties of A, B and O-type main-sequence stars, which have radiative envelopes, and the fossil field model which is normally invoked to explain the strong fields sometimes seen in these stars. Observations seem to show that Ap-type stable fields are excluded in stars with convective envelopes. Most stars contain both radiative and convective zones, and there are potentially important effects arising from the interaction of magnetic fields at the boundaries between them; the solar cycle being one of the better known examples. Related to this, we discuss whether the Sun could harbour a magnetic field in its core. Recent developments regarding the various convective and radiative layers near the surfaces of early-type stars and their observational effects are examined. We look at possible dynamo mechanisms that run on differential rotation rather than convection. Finally, we turn to neutron stars with a discussion of the possible origins for their magnetic fields.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2017RSOS....460271B},
  file = {/Users/lbugnet/Zotero/storage/S2KSF3PV/Braithwaite and Spruit - 2017 - Magnetic fields in non-convective regions of stars.pdf}
}

@article{Braithwaite2018,
  title = {Axisymmetric Magnetic Fields in Stars: Relative Strengths of Poloidal and Toroidal Components},
  author = {Braithwaite, Jonathan},
  year = {2018},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {000},
  number = {0000},
  eprint = {0810.1049v3},
  pages = {1--13},
  urldate = {2020-05-01},
  abstract = {In this third paper in a series on stable magnetic equilibria in stars, I look at the stability of axisymmetric field configurations and in particular at the relative strengths of the toroidal and poloidal components. Both toroidal and poloidal fields are unstable on their own, and stability is achieved by adding the two together in some ratio. I use Tayler's (1973) stability conditions for toroidal fields and other analytic tools to predict the range of stable ratios and then check these predictions by running numerical simulations. It is found that while the poloidal field can account for no more than approximately 80\% of the total energy, it can account for a very small fraction of the energy, i.e. that the toroidal field can be-and is likely to be-significantly stronger than the poloidal. Furthermore, the weaker the field, the weaker the poloidal component can be in relation to the toroidal. The implications of this result are discussed in various contexts such as the emission of gravitational waves by neutron stars, free precession, and a 'hidden' energy source for magnetars.},
  archiveprefix = {arxiv},
  keywords = {(magnetohydrodynamics) MHD-stars,) white dwarfs,chemically pe-culiar-stars,magnetic fields-stars,neutron-(stars,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JEF56B4C/full-text.pdf}
}

@article{Brandenburg2005a,
  title = {Astrophysical Magnetic Fields and Nonlinear Dynamo Theory},
  author = {Brandenburg, Axel and Subramanian, Kandaswamy},
  year = {2005},
  journal = {Physics Reports},
  volume = {417},
  number = {1-4},
  eprint = {astro-ph/0405052},
  pages = {1--209},
  issn = {03701573},
  doi = {10.1016/j.physrep.2005.06.005},
  abstract = {The current understanding of astrophysical magnetic fields is reviewed, focusing on their generation and maintenance by turbulence. In the astrophysical context this generation is usually explained by a self-excited dynamo, which involves flows that can amplify a weak 'seed' magnetic field exponentially fast. Particular emphasis is placed on the nonlinear saturation of the dynamo. Analytic and numerical results are discussed both for small scale dynamos, which are completely isotropic, and for large scale dynamos, where some form of parity breaking is crucial. Central to the discussion of large scale dynamos is the so-called alpha effect which explains the generation of a mean field if the turbulence lacks mirror symmetry, i.e. if the flow has kinetic helicity. Large scale dynamos produce small scale helical fields as a waste product that quench the large scale dynamo and hence the alpha seffect. With this in mind, the microscopic theory of the alpha effect is revisited in full detail and recent results for the loss of helical magnetic fields are reviewed. \textcopyright{} 2005 Elsevier B.V. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Dynamos,Magnetohydrodynamics,Mean field theory,notion,notion-database,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/RGXBI6LH/Brandenburg, Subramanian - 2005.pdf}
}

@article{Braun2008,
  title = {{{PROSPECTS FOR THE DETECTION OF THE DEEP SOLAR MERIDIONAL CIRCULATION D}}. {{C}}. {{Braun}} and {{A}}. {{C}}. {{Birch}}},
  author = {Braun, D C and Birch, A C},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {689},
  pages = {161--165},
  abstract = {We perform helioseismic holography to assess the noise in p-mode travel-time shifts which would form the basis of inferences of large-scale flows throughout the solar convection zone. We also derive the expected travel times from a parameterized return (equatorward) flow component of the meridional circulation at the base of the convection zone from forward models under the assumptions of the ray and Born approximations. From estimates of the signal-to-noise ratio for measurements focused near the base of the convection zone, we conclude that the helioseismic detection of the deep meridional flow including the return component may not be possible using travel-time measurements spanning an interval less than a solar cycle. We speculate that this conclusion may be generally true for other helioseismic methods under the assumption that the underlying measurements are equiv- alently limited by solar realization noise.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/34IWNTQD/Braun, Birch - 2008.pdf}
}

@article{Braun2008c,
  title = {Surface-Focused Seismic Holography of Sunspots: {{I}}. {{Observations}}},
  author = {Braun, D. C. and Birch, A. C.},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  pages = {267--289},
  issn = {00380938},
  doi = {10.1007/s11207-008-9152-5},
  abstract = {We present a comprehensive set of observations of the interaction of p-mode oscillations with sunspots using surface-focused seismic holography. Maps of travel-time shifts, relative to quiet-Sun travel times, are shown for incoming and outgoing p modes as well as their mean and difference. We compare results using phase-speed filters with results obtained with filters that isolate single p-mode ridges, and we further divide the data into multiple temporal frequency bandpasses. The f mode is removed from the data. The variations of the resulting travel-time shifts with magnetic-field strength and with the filter parameters are explored. We find that spatial averages of these shifts within sunspot umbrae, penumbrae, and surrounding plage often show strong frequency variations at fixed phase speed. In addition, we find that positive values of the mean and difference travel-time shifts appear exclusively in waves observed with phase-speed filters that are dominated by power in the low-frequency wing of the p 1 ridge. We assess the ratio of incoming to outgoing p-mode power using the ridge filters and compare surface-focused holography measurements with the results of earlier published p-mode scattering measurements using Fourier-Hankel decomposition. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  keywords = {Active regions,Helioseismology,Magnetic fields,notion,notion-database,Observations},
  file = {/Users/lbugnet/Zotero/storage/YZ288WPS/Braun, Birch - 2008(2).pdf}
}

@techreport{Breger2000,
  title = {Delta {{Scuti}} Stars},
  author = {Breger, Michel},
  year = {2000},
  urldate = {2020-03-31},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FMIL72DR/full-text.pdf}
}

@inproceedings{Breger2010,
  title = {The {{Blazhko Effect}} in {{Delta Scuti}} and Other {{Groups}} of {{Pulsating Stars}}},
  booktitle = {B.{{V}}. {{Kukarkin Centenary Conference}}: {{Variable Stars}} the {{Galactic Halo}} and {{Galaxy Formation}}},
  author = {Breger, Michel},
  year = {2010},
  month = jan,
  eprint = {1001.4443},
  urldate = {2020-04-09},
  abstract = {Amplitude and period variations have been detected in almost all types of pulsating stars. Many of these modulations are nearly periodic. In RR Lyrae stars the phenomenon in known as the Blazhko Effect. Because of the observed similarities, we propose to extend the definition to other groups. We illustrate the Blazhko Effect with examples from Cepheids, RR Lyrae stars, White Dwarfs, sdB stars and delta Scuti variables. For delta Scuti stars the present results indicate the presence of at least two effects: beating of independent modes with close frequencies and stellar cycles. For period and amplitude changes with timescales less than one year, the beating hypothesis explains the observed modulations very well. This has been shown by the correctly correlated relationship between amplitude and phase changes as well as the repetitions of these cycles. However, the observed period variations with longer timescales cannot be due to simple beating between two close frequencies. For the star AI CVn (= 4 CVn), we can derive accurate annual frequency values for a number of radial and nonradial modes from 1974 to 2009. For prograde and retrograde modes, the frequency variations are of similar size, but with opposite signs. The radial mode shows no (or little) changes. Fur- thermore, all frequency variations show a reversal around 1990. These results are consistent with long-term cycles affecting individual modes differently with some common systematic behavior. The observed change in the size of rotational splitting is interpreted as a change in the differential rotation during the stellar cycle.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/P3TNRJZI/full-text.pdf}
}

@book{Breiman1984,
  title = {Classification {{And Regression Trees}}},
  author = {Breiman, Leo and Friedman, Jerome and Stone, Charles J. and Olsen, R.A.},
  editor = {{Taylor \& Francis}},
  year = {1984},
  journal = {Chapman \& Hall/Crc},
  urldate = {2020-03-20},
  abstract = {\textbullet{} גרינבלט, י. (2012). ענף הקיווי: תמונת מצב 2012, עלון הנוטע שה``מ, מחוז צפון, משרד החקלאות.},
  isbn = {978-0-412-04841-8},
  keywords = {notion,notion-database}
}

@article{Breiman2001,
  title = {Random Forests},
  author = {Breiman, Leo},
  year = {2001},
  month = oct,
  journal = {Machine Learning},
  volume = {45},
  number = {1},
  pages = {5--32},
  publisher = {{Springer}},
  issn = {08856125},
  doi = {10.1023/A:1010933404324},
  urldate = {2020-03-09},
  abstract = {Random forests are a combination of tree predictors such that each tree depends on the values of a random vector sampled independently and with the same distribution for all trees in the forest. The generalization error for forests converges a.s. to a limit as the number of trees in the forest becomes large. The generalization error of a forest of tree classifiers depends on the strength of the individual trees in the forest and the correlation between them. Using a random selection of features to split each node yields error rates that compare favorably to Adaboost (Y. Freund \& R. Schapire, Machine Learning: Proceedings of the Thirteenth International conference, * * *, 148-156), but are more robust with respect to noise. Internal estimates monitor error, strength, and correlation and these are used to show the response to increasing the number of features used in the splitting. Internal estimates are also used to measure variable importance. These ideas are also applicable to regression.},
  keywords = {Classification,Ensemble,notion,notion-database,Regression},
  file = {/Users/lbugnet/Zotero/storage/ZNPKHAZD/full-text.pdf}
}

@inproceedings{Breton2019,
  title = {Determining Surface Rotation Periods of Solar-like Stars Observed by the {{Kepler}} Mission Using Machine Learning Techniques},
  booktitle = {Proceedings of the 2019 {{SF2A}} Meeting},
  author = {Breton, S. N. and Bugnet, L. and Santos, A. R. G. and Saux, A. Le and Mathur, S. and Palle, P. L. and Garcia, R. A.},
  year = {2019},
  eprint = {1906.09609},
  abstract = {For a solar-like star, the surface rotation evolves with time, allowing in principle to estimate the age of a star from its surface rotation period. Here we are interested in measuring surface rotation periods of solar-like stars observed by the NASA Kepler mission. Different methods have been developed to track rotation signals in Kepler photometric light curves: time-frequency analysis based on wavelet techniques, autocorrelation and composite spectrum. We use the learning abilities of random forest classifiers to take decisions during two crucial steps of the analysis. First, given some input parameters, we discriminate the considered Kepler targets between rotating MS stars, non-rotating MS stars, red giants, binaries and pulsators. We then use a second classifier only on the MS rotating targets to decide the best data-analysis treatment.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,kepler,machine learning,notion,notion-database,random forest,rotation,solar-like stars},
  file = {/Users/lbugnet/Zotero/storage/N7MJNW56/Breton et al. - 2019.pdf}
}

@article{Breton2020,
  title = {{{ROOSTER}}},
  author = {Breton, S. and Bugnet, L and Santos, A.},
  year = {2020},
  journal = {A\&A, accepted},
  keywords = {notion,notion-database}
}

@article{Breton2021,
  title = {{{ROOSTER}}: {{A}} Machine-Learning Analysis Tool for {{Kepler}} Stellar Rotation Periods},
  author = {Breton, S. N. and Santos, A. R.G. and Bugnet, L. and Mathur, S. and Garc{\'i}a, R. A. and Pall{\'e}, P. L.},
  year = {2021},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {647},
  eprint = {2101.10152},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/202039947},
  urldate = {2021-12-29},
  abstract = {In order to understand stellar evolution, it is crucial to efficiently determine stellar surface rotation periods. Indeed, while they are of great importance in stellar models, angular momentum transport processes inside stars are still poorly understood today. Surface rotation, which is linked to the age of the star, is one of the constraints needed to improve the way those processes are modelled. Statistics of the surface rotation periods for a large sample of stars of different spectral types are thus necessary. An efficient tool to automatically determine reliable rotation periods is needed when dealing with large samples of stellar photometric datasets. The objective of this work is to develop such a tool. For this purpose, machine learning classifiers constitute relevant bases to build our new methodology. Random forest learning abilities are exploited to automate the extraction of rotation periods in Kepler light curves. Rotation periods and complementary parameters are obtained via three different methods: a wavelet analysis, the autocorrelation function of the light curve, and the composite spectrum. We trained three different classifiers: one to detect if rotational modulations are present in the light curve, one to flag close binary or classical pulsators candidates that can bias our rotation period determination, and finally one classifier to provide the final rotation period. We tested our machine learning pipeline on 23 431 stars of the Kepler K and M dwarf reference rotation catalogue for which 60\% of the stars have been visually inspected. For the sample of 21 707 stars where all the input parameters are provided to the algorithm, 94.2\% of them are correctly classified (as rotating or not). Among the stars that have a rotation period in the reference catalogue, the machine learning provides a period that agrees within 10\% of the reference value for 95.3\% of the stars. Moreover, the yield of correct rotation periods is raised to 99.5\% after visually inspecting 25.2\% of the stars. Over the two main analysis steps, rotation classification and period selection, the pipeline yields a global agreement with the reference values of 92.1\% and 96.9\% before and after visual inspection. Random forest classifiers are efficient tools to determine reliable rotation periods in large samples of stars. The methodology presented here could be easily adapted to extract surface rotation periods for stars with different spectral types or observed by other instruments such as K2, TESS or by PLATO in the near future.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: activity,Stars: rotation,Stars: solar-type,Starspots},
  file = {/Users/lbugnet/Zotero/storage/7GA7BT8Z/full-text.pdf;/Users/lbugnet/Zotero/storage/95GNER2W/abstract.html}
}

@book{bretonAnalysingKeplerStellar2021,
  title = {Analysing {{Kepler}} Stellar Surface Rotation and Activity with {{ROOSTER}}},
  author = {Breton, S. N. and Santos, A. R. G. and Mathur, S. and Garc{\'i}a, R. A. and Bugnet, L. and Pall{\'e}, P. L.},
  year = {2021},
  month = dec,
  pages = {363--366},
  urldate = {2022-07-18},
  abstract = {It is crucial for our knowledge of stellar evolution to be able to efficiently determine stellar surface rotation periods in large stellar samples. Random forest (RF) learning abilities are exploited to automate the extraction of rotation periods in Kepler light curves. We train three different classifiers: one to detect if rotational modulation is present in the light curve; one to select the rotation period among estimates provided by ACF and wavelet analysis methods; and finally one to flag classical pulsators or close binary candidates that can bias our rotation-period determination. We test our machine learning pipeline, ROOSTER, on the Kepler K and M dwarf sample using the most up-to-date reference catalog. We show that we are able to detect rotational modulations with an accuracy of 94.2\% and to retrieve final rotation periods with an accuracy of 95.3\%. This value is raised to 99.5\% after visually inspecting 25.2\% of the stars. Over the two main analysis steps, the pipeline yields a global accuracy of 92.1\% before visual checks, 96.9\% after. The method is then applied to analyse the F and G stars observed by Kepler. The methodology presented here can be adapted to extract surface rotation periods for stars observed by other missions, like K2, TESS, and PLATO.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: activity,Stars: rotation,Stars: solar-type,starspots},
  annotation = {ADS Bibcode: 2021sf2a.conf..363B},
  file = {/Users/lbugnet/Zotero/storage/7X8R59QU/Breton et al. - 2021 - Analysing Kepler stellar surface rotation and acti.pdf}
}

@article{bretonComparisonGlobalHelioseismicInstrument2020,
  title = {A {{Comparison}} of {{Global Helioseismic-Instrument Performances}}: {{Solar-SONG}}, {{GOLF}} and {{VIRGO}}},
  shorttitle = {A {{Comparison}} of {{Global Helioseismic-Instrument Performances}}},
  author = {Breton, S. N. and Garc{\'i}a, R. A. and Pall{\'e}, P. L. and Mathur, S. and Hill, F. and Jain, K. and Jim{\'e}nez, A. and Tripathy, S. C. and Grundahl, F. and {Fredslund-Andersen}, M. and Santos, A. R. G.},
  year = {2020},
  month = jan,
  volume = {57},
  pages = {327--328},
  doi = {10.1007/978-3-030-55336-4_45},
  urldate = {2022-07-18},
  abstract = {The SONG spectrograph has recently demonstrated its ability to perform solar radial velocity measurement during the first test run of the Solar-SONG initiative. A preliminary assessment of its performance is carried out here by comparing the results of Solar-SONG during the summer 2018 test run, with GOLF and VIRGO/SPM taken as reference instruments.},
  keywords = {notion,notion-database},
  annotation = {ADS Bibcode: 2020ASSP...57..327B}
}

@misc{bretonDeterminingSurfaceRotation2019,
  title = {Determining Surface Rotation Periods of Solar-like Stars Observed by the Kepler Mission Using Machine Learning Techniques},
  author = {Breton, S.N. and Bugnet, L. and Santos, A.R.G. and Le Saux, A. and Mathur, S. and Pall{\'e}, P.L. and Garc{\'i}a, R.A.},
  year = {2019},
  journal = {arXiv},
  abstract = {Copyright \textcopyright{} 2019, arXiv, All rights reserved. For a solar-like star, the surface rotation evolves with time, allowing in principle to estimate the age of a star from its surface rotation period. Here we are interested in measuring surface rotation periods of solar-like stars observed by the NASA mission Kepler. Different methods have been developed to track rotation signals in Kepler photometric light curves: time-frequency analysis based on wavelet techniques, autocorrelation and composite spectrum. We use the learning abilities of random forest classifiers to take decisions during two crucial steps of the analysis. First, given some input parameters, we discriminate the considered Kepler targets between rotating MS stars, non-rotating MS stars, red giants, binaries and pulsators. We then use a second classifier only on the MS rotating targets to decide the best data-analysis treatment.},
  keywords = {Asteroseismology,Kepler,Machine learning,notion,notion-database,Random forest,Rotation,Solar-like stars}
}

@article{Brett2004,
  title = {The Automated Classification of Astronomical Light Curves Using {{Kohonen}} Self-Organizing Maps},
  author = {Brett, David R. and West, Richard G. and Wheatley, Peter J.},
  year = {2004},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {353},
  number = {2},
  pages = {369--376},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2004.08093.x},
  urldate = {2020-07-11},
  abstract = {We apply the technique of self-organizing maps to the automated classification of singly periodic astronomical light curves. We find that our maps readily distinguish between light curve types in both synthetic and real data sets, and that the resulting maps do not depend sensitively on the chosen learning parameters. Automated data analysis techniques are likely to be become increasingly important as the size of astronomical data sets continues to increase, particularly with the advent of ultra-wide-field survey telescopes such as WASP, RAPTOR and ASAS.},
  keywords = {Astronomical data bases: miscellaneous,Binaries: general,Methods: data analysis,notion,notion-database,Stars: general,Surveys,Techniques: miscellaneous}
}

@article{Briquet2012a,
  title = {Multisite Spectroscopic Seismic Study of the {$\beta$} {{Cep}} Star {{V2052 Ophiuchi}}: {{Inhibition}} of Mixing by Its Magnetic Field},
  author = {Briquet, M. and Neiner, C. and Aerts, C. and Morel, T. and Mathis, S. and Reese, D. R. and Lehmann, H. and Costero, R. and Echevarria, J. and Handler, G. and Kambe, E. and Hirata, R. and Masuda, S. and Wright, D. and Yang, S. and Pintado, O. and Mkrtichian, D. and Lee, B. C. and Han, I. and Bruch, A. and De Cat, P. and Uytterhoeven, K. and Lefever, K. and Vanautgaerden, J. and {de Batz}, B. and Fr{\'e}mat, Y. and Henrichs, H. and Geers, V. C. and Martayan, C. and Hubert, A. M. and Thizy, O. and Tijani, A.},
  year = {2012},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {427},
  number = {1},
  pages = {483--493},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.21933.x},
  abstract = {We used extensive ground-based multisite and archival spectroscopy to derive observational constraints for a seismic modelling of the magnetic {$\beta$} Cep star V2052 Ophiuchi. The line-profile variability is dominated by a radial mode (f 1 = 7.14846d -1) and by rotational modulation (P rot = 3.638833d). Two non-radial low-amplitude modes (f 2 = 7.75603d -1 and f 3 = 6.82308d -1) are also detected. The four periodicities that we found are the same as the ones discovered from a companion multisite photometric campaign and known in the literature. Using the photometric constraints on the degrees {$\mathscr{l}$} of the pulsation modes, we show that both f 2 and f 3 are prograde modes with ({$\mathscr{l}$}, m) = (4, 2) or (4, 3). These results allowed us to deduce ranges for the mass (M {$\in$} [8.2, 9.6]M {$\odot$}) and central hydrogen abundance (X c {$\in$} [0.25, 0.32]) of V2052 Oph, to identify the radial orders n 1 = 1, n 2 = -3 and n 3 = -2, and to derive an equatorial rotation velocity v eq {$\in$} [71, 75]kms -1. The model parameters are in full agreement with the effective temperature and surface gravity deduced from spectroscopy. Only models with no or mild core overshooting ({$\alpha$} ov {$\in$} [0, 0.15] local pressure scale heights) can account for the observed properties. Such a low overshooting is opposite to our previous modelling results for the non-magnetic {$\beta$} Cep star \texttheta{} Oph having very similar parameters, except for a slower surface rotation rate. We discuss whether this result can be explained by the presence of a magnetic field in V2052 Oph that inhibits mixing in its interior. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {notion,notion-database,Stars: early-type,Stars: individual: V2052 Oph,Stars: interiors,Stars: magnetic field,Starspots},
  file = {/Users/lbugnet/Zotero/storage/RI5U9TY6/427-1-483-1.pdf}
}

@article{Briquet2013,
  title = {Discovery of a Magnetic Field in the {{CoRoT}} Hybrid {{B-type}} Pulsator {{HD}} 43317},
  author = {Briquet, M. and Neiner, C. and Leroy, B. and P{\'a}pics, P. I. and {collaboration}, the MiMeS},
  year = {2013},
  month = aug,
  eprint = {1308.4636},
  doi = {10.1051/0004-6361/201321779},
  urldate = {2020-06-29},
  abstract = {A promising way of testing the impact of a magnetic field on internal mixing (core overshooting, internal rotation) in main-sequence B-type stars is to perform asteroseismic studies of a sample of magnetic pulsators. The CoRoT satellite revealed that the B3IV star HD 43317 is a hybrid SPB/beta Cep-type pulsator that has a wealth of pulsational constraints on which one can perform a seismic modelling, in particular, probing the extent of its convective core and mixing processes. Moreover, indirect indicators of a magnetic field in the star were observed: rotational modulation due to chemical or temperature spots and X-ray emission. Our goal was to directly investigate the field in HD 43317 and, if it is magnetic, to characterise it. We collected data with the Narval spectropolarimeter installed at TBL (T\textbackslash 'elescope Bernard Lyot, Pic du Midi, France) and applied the least-squares deconvolution technique to measure the circular polarisation of the light emitted from HD 43317. We modelled the longitudinal field measurements directly with a dipole. Zeeman signatures in the Stokes V profiles of HD 43317 are clearly detected and rotationally modulated, which proves that this star exhibits an oblique magnetic field. The modulation with the rotation period deduced from the CoRoT light curve is also confirmed, and we found a field strength at the poles of about 1 kG. Our result must be taken into account in future seismic modelling work of this star.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8B85R4FA/full-text.pdf}
}

@article{Broderick2007,
  title = {Magnetic {{Helicity}} and the {{Relaxation}} of {{Fossil Fields}}},
  author = {Broderick, Avery E. and Narayan, Ramesh},
  year = {2007},
  month = feb,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {383},
  number = {3},
  eprint = {astro-ph/0702128},
  pages = {943--956},
  doi = {10.1111/j.1365-2966.2007.12634.x},
  urldate = {2020-05-14},
  abstract = {In the absence of an active dynamo, purely poloidal magnetic field configurations are unstable to large-scale dynamical perturbations, and decay via reconnection on an Alfvenic timescale. Nevertheless, a number of classes of dynamo-free stars do exhibit significant, long-lived, surface magnetic fields. Numerical simulations suggest that the large-scale poloidal field in these systems is stabilized by a toroidal component of the field in the stellar interior. Using the principle of conservation of total helicity, we develop a variational principle for computing the structure of the magnetic field inside a conducting sphere surrounded by an insulating vacuum. We show that, for a fixed total helicity, the minimum energy state corresponds to a force-free configuration. We find a simple class of axisymmetric solutions, parametrized by angular and radial quantum numbers. However, these solutions have a discontinuity in the toroidal magnetic field at the stellar surface which will exert a toroidal stress on the surface of the star. We then describe two other classes of solutions, the standard spheromak solutions and ones with fixed surface magnetic fields, the latter being relevant for neutron stars with rigid crusts. We discuss the implications of our results for the structure of neutron star magnetic fields, the decay of fields, and the origin of variability and outbursts in magnetars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: flare,Stars: magnetic fields,Stars: neutron},
  file = {/Users/lbugnet/Zotero/storage/NBZDU99W/full-text.pdf}
}

@article{Broomhall2007,
  title = {Needles in Haystacks: {{How}} to Use Contemporaneous Data in the Search for Low-Frequency Modes of Oscillation of the {{Sun}}},
  author = {Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. and Appourchaux, T.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {379},
  number = {1},
  pages = {2--10},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.11905.x},
  abstract = {We show how to take advantage of contemporaneous data from two different instruments in the search for low-frequency modes of oscillation of the Sun. Contemporaneous data allow searches to be made for prominent, sharp concentrations of power which are coincident in frequency. Crucial to determining objective measures of the joint probability of the random occurrence of such features, which are potential candidates for modes, is a good understanding of the characteristics of the background noise. In this paper we show how to make proper allowance, in the calculation of the probability, for noise that is common to data from different instruments. This common noise is solar in origin, and comes from the solar granulation. Its presence makes calculation of the probability a non-trivial problem. We demonstrate application of the technique in searches for low-frequency p modes. The data we searched comprised 3071 d of contemporaneous Sun-as-a-star Doppler velocity observations made by the ground-based Birmingham Solar-Oscillations Network (BiSON), and the GOLF instrument onboard the ESA/NASA SOHO spacecraft. \textcopyright{} 2007 RAS.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/T3GUW65Q/Broomhall et al. - 2007.pdf}
}

@article{Broomhall2008,
  title = {The Visibility of Low-Frequency Solar Acoustic Modes},
  author = {Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. and Fletcher, S. T.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  pages = {461--469},
  issn = {00046337},
  doi = {10.1002/asna.200710988},
  abstract = {We make predictions of the detectability of low-frequency p modes. Estimates of the powers and damping times of these low-frequency modes are found by extrapolating the observed powers and widths of higher-frequency modes with large observed signal-to-noise ratios. The extrapolations predict that the low-frequency modes will have small signal-to-noise ratios and narrow widths in a frequency-power spectrum. Monte Carlo simulations were then performed where timeseries containing mode signals and normally distributed Gaussian noise were produced. The mode signals were simulated to have the powers and damping times predicted by the extrapolations. Various statistical tests were then performed on the frequency-amplitude spectra formed from these timeseries to investigate the fraction of spectra in which the modes could be detected. The results of these simulations were then compared to the number of p-modes candidates observed in real Sun-as-a-star data at low frequencies. The fraction of simulated spectra in which modes were detected decreases rapidly as the frequency of modes decreases and so the fraction of simulations in which the low-frequency modes were detected was very small. However, increasing the signal-to-noise (S/N) ratio of the low-frequency modes by a factor of 2 above the extrapolated values led to significantly more detections. Therefore efforts should continue to further improve the quality of solar data that is currently available. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {Methods: statistical,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WIU23JTQ/Broomhall et al. - 2008.pdf}
}

@article{Broomhall2009a,
  title = {Is the Current Lack of Solar Activity Only Skin Deep?},
  author = {Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. and Fletcher, S. T. and New, R.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {700},
  number = {2 PART 2},
  pages = {162--165},
  issn = {15384357},
  doi = {10.1088/0004-637X/700/2/L162},
  abstract = {The Sun is a variable star whose magnetic activity and total irradiance vary on a timescale of approximately 11 years. The current activity minimum has attracted considerable interest because of its unusual duration and depth. This raises the question: what might be happening beneath the surface where the magnetic activity ultimately originates? The surface activity can be linked to the conditions in the solar interior by the observation and analysis of the frequencies of the Sun's natural seismic modes of oscillation - the p modes. These seismic frequencies respond to changes in activity and are probes of conditions within the Sun. The Birmingham Solar-Oscillations Network (BiSON) has made measurements of p-mode frequencies over the last three solar activity cycles, and so is in a unique position to explore the current unusual and extended solar minimum. We show that the BiSON data reveal significant variations of the p-mode frequencies during the current minimum. This is in marked contrast to the surface activity observations, which show little variation over the same period. The level of the minimum is significantly deeper in the p-mode frequencies than in the surface observations. We observe a quasi-biennial signal in the p-mode frequencies, which has not previously been observed at mid- and low-activity levels. The stark differences in the behavior of the frequencies and the surface activity measures point to activity-related processes occurring in the solar interior, which are yet to reach the surface, where they may be attenuated. \textcopyright{} 2009. The American Astronomical Society.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: activity,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4KJ9Q38D/Broomhall et al. - 2009.pdf}
}

@article{Broomhall2009b,
  title = {New Aspects of {{Doppler}} Imaging in {{Sun-as-a-star}} Observations},
  author = {Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. and New, R.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {397},
  number = {2},
  pages = {793--801},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.15011.x},
  abstract = {Birmingham Solar Oscillations Network (BiSON) instruments use resonant scattering spectrometers to make unresolved Doppler velocity observations of the Sun. Unresolved measurements are not homogenous across the solar disc and so the observed data do not represent a uniform average over the entire surface. The influence on the inhomogeneity of the solar rotation and limb darkening has been considered previously and is well understood. Here, we consider a further effect that originates from the instrumentation itself. The intensity of light observed from a particular region on the solar disc is dependent on the distance between that region on the image of the solar disc formed in the instrument and the detector. The majority of BiSON instruments have two detectors positioned on opposite sides of the image of the solar disc and the observations made by each detector are weighted towards differing regions of the disc. Therefore, the visibility and amplitudes of the solar oscillations and the realization of the solar noise observed by each detector will differ. We find that the modelled bias is sensitive to many different parameters such as the width of solar absorption lines, the strength of the magnetic field in the resonant scattering spectrometer, the orientation of the Sun's rotation axis, the size of the image observed by the instrument and the optical depth in the vapour cell. We find that the modelled results best match the observations when the optical depth at the centre of the vapour cell is 0.55. The inhomogeneous weighting means that a 'velocity offset' is introduced into unresolved Doppler velocity observations of the Sun, which varies with time, and so has an impact on the long-term stability of the observations. \textcopyright{} 2009 RAS.},
  keywords = {Methods: observational,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RRWS8KP8/Broomhall et al. - 2009(2).pdf}
}

@article{Broomhall2009c,
  title = {Definitive {{Sun-as-a-star}} p-Mode Frequencies: 23 Years of {{BiSON}} Observations},
  author = {Broomhall, A. M. and Chaplin, W. J. and Davies, G. R. and Elsworth, Y. and Fletcher, S. T. and Hale, S. J. and Miller, B. and New, R.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {396},
  number = {1},
  pages = {100--104},
  issn = {17453933},
  doi = {10.1111/j.1745-3933.2009.00672.x},
  abstract = {We present a list of 'best possible' estimates of low-degree p-mode frequencies from 8640 days of observations made by the Birmingham Solar-Oscillations Network (BiSON). This is the longest stretch of helioseismic data ever used for this purpose, giving exquisite precision in the estimated frequencies. Every effort has been made in the analysis to ensure that the frequency estimates are also accurate. In addition to presenting the raw best-fitting frequencies from our 'peak-bagging' analysis, we also provide tables of corrected frequencies pertinent to the quiet-Sun and an intermediate level of solar activity. \textcopyright{} 2009 The Authors. Journal compilation \textcopyright{} 2009 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/8JM38UTZ/Broomhall et al. - 2009(3).pdf}
}

@article{Broomhall2010a,
  title = {A Comparison of Frequentist and {{Bayesian}} Inference: {{Searching}} for Low-Frequency p Modes and g Modes in {{Sun-as-a-star}} Data},
  author = {Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. and Appourchaux, T. and New, R.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {406},
  number = {2},
  eprint = {1004.4505},
  pages = {767--781},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2010.16743.x},
  abstract = {We describe and use two different statistical approaches to try and detect low-frequency solar oscillations in Sun-as-a-star data: a frequentist approach and a Bayesian approach. We have used frequentist statistics to search contemporaneous Sun-as-a-star data for coincident, statistically prominent features. However, we find that this approach leads to numerous false detections. We have also used Bayesian statistics to search for evidence of low-frequency p modes and g modes in Sun-as-a-star data. We describe how Bayesian statistics can be used to search near-contemporaneous data for coincident prominent features. Near-contemporaneous data were used to circumvent the difficulties in deriving probabilities that occur when common noise is present in the data. We find that the Bayesian approach, which is reliant on the assumptions made when determining the posterior probability, leads to significantly fewer false detections and those that are observed can be discredited using a priori knowledge. Therefore, we have more confidence in the mode candidates found with Bayesian statistics. \textcopyright{} 2010 The Authors. Journal compilation \textcopyright{} 2010 RAS.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/BQSNT3CQ/Broomhall et al. - 2010.pdf}
}

@article{Broomhall2011,
  title = {Are Short-Term Variations in Solar Oscillation Frequencies the Signature of a Second Solar Dynamo?},
  author = {Broomhall, Anne Marie and Fletcher, Stephen T. and Salabert, David and Basu, Sarbani and Chaplin, William J. and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Jim{\'e}nez, Antonio and New, Roger},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012025},
  abstract = {In addition to the well-known 11-year solar cycle, the Sun's magnetic activity also shows significant variation on shorter time scales, e.g. between one and two years. We observe a quasi-biennial (2-year) signal in the solar p-mode oscillation frequencies, which are sensitive probes of the solar interior. The signal is visible in Sun-as-a-star data observed by different instruments and here we describe the results obtained using BiSON, GOLF, and VIRGO data. Our results imply that the 2-year signal is susceptible to the influence of the main 11-year solar cycle. However, the source of the signal appears to be separate from that of the 11-year cycle. We speculate as to whether it might be the signature of a second dynamo, located in the region of near-surface rotational shear. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6HYSZXHB/Broomhall et al. - 2011.pdf}
}

@article{Broomhall2012,
  title = {Misleading Variations in Estimated Rotational Frequency Splittings of Solar p Modes: {{Consequences}} for Helioseismology and Asteroseismology},
  author = {Broomhall, Anne Marie and Salabert, David and Chaplin, William J. and Garc{\'i}a, Rafael A. and Elsworth, Yvonne and Howe, Rachel and Mathur, Savita},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {422},
  number = {4},
  pages = {3564--3573},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.20868.x},
  abstract = {The aim of this paper is to investigate whether there are any 11-yr or quasi-biennial solar-cycle-related variations in solar rotational splitting frequencies of low-degree solar p modes. Although no 11-yr signals were observed, variations on a shorter time-scale ({$\sim$}2yr) were apparent. We show that the variations arose from complications/artefacts associated with the realization noise in the data and the process by which the data were analysed. More specifically, the realization noise was observed to have a larger effect on the rotational splittings than accounted for by the formal uncertainties. When used to infer the rotation profile of the Sun these variations are not important. The outer regions of the solar interior can be constrained using higher degree modes. While the variations in the low-l splittings do make large differences to the inferred rotation rate of the core, the core rotation rate is so poorly constrained, even by low-l modes, that the different inferred rotation profiles still agree within their respective 1{$\sigma$} uncertainties. By contrast, in asteroseismology, only low-l modes are visible and so higher l modes cannot be used to constrain the rotation profile of stars. Furthermore, we usually only have one data set from which to measure the observed low-l splitting. In such circumstances the inferred internal rotation rate of a main-sequence star could differ significantly from estimates of the surface rotation rate, hence leading to spurious conclusions. Therefore, extreme care must be taken when using only the splittings of low-l modes to draw conclusions about the average internal rotation rate of a star. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: oscillations,Sun: activity,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/IUEJL2YP/Broomhall et al. - 2012.pdf}
}

@article{Broomhall2014,
  title = {The {{Sun}}'s {{Interior Structure}} and {{Dynamics}}, and the {{Solar Cycle}}},
  author = {Broomhall, A. M. and Chatterjee, P. and Howe, R. and Norton, A. A. and Thompson, M. J.},
  year = {2014},
  journal = {Space Science Reviews},
  volume = {186},
  number = {1-4},
  eprint = {1411.5941},
  pages = {191--225},
  issn = {15729672},
  doi = {10.1007/s11214-014-0101-3},
  abstract = {The Sun's internal structure and dynamics can be studied with helioseismology, which uses the Sun's natural acoustic oscillations to build up a profile of the solar interior. We discuss how solar acoustic oscillations are affected by the Sun's magnetic field. Careful observations of these effects can be inverted to determine the variations in the structure and dynamics of the Sun's interior as the solar cycle progresses. Observed variations in the structure and dynamics can then be used to inform models of the solar dynamo, which are crucial to our understanding of how the Sun's magnetic field is generated and maintained.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: interior,Sun: magnetic fields,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/NW29YUGB/Broomhall et al. - 2014.pdf}
}

@article{Broomhall2015,
  title = {A {{Comparison Between Global Proxies}} of the {{Sun}}'s {{Magnetic Activity Cycle}}: {{Inferences}} from {{Helioseismology}}},
  author = {Broomhall, A. M. and Nakariakov, V. M.},
  year = {2015},
  journal = {Solar Physics},
  volume = {290},
  number = {11},
  eprint = {1507.02854},
  pages = {3095--3111},
  publisher = {{Springer Science+Business Media Dordrecht}},
  issn = {1573093X},
  doi = {10.1007/s11207-015-0728-6},
  abstract = {The last solar minimum was, by recent standards, unusually deep and long. We are now close to the maximum of the subsequent solar cycle, which is relatively weak. In this article we make comparisons between different global (unresolved) measures of the Sun's magnetic activity to investigate how they are responding to this weak-activity epoch. We focus on helioseismic data, which are sensitive to conditions, including the characteristics of the magnetic field, in the solar interior. Also considered are measures of the magnetic field in the photosphere (sunspot number and sunspot area), the chromosphere and corona (10.7~cm radio flux and 530.3 nm green coronal index), and two measures of the Sun's magnetic activity closer to Earth (the interplanetary magnetic field and the galactic cosmic-ray intensity). Scaled versions of the activity proxies diverge from the helioseismic data around 2000, indicating a change in relationship between the proxies. The degree of divergence varies from proxy to proxy, with sunspot area and 10.7~cm flux showing only small deviations, while sunspot number, coronal index, and the two interplanetary proxies show much larger departures. In Cycle 24 the deviations in the solar proxies and the helioseismic data decrease, raising the possibility that the deviations observed in Cycle 23 are just symptomatic of a 22-year Hale cycle. However, the deviations in the helioseismic data and the interplanetary proxies increase in Cycle 24. Interestingly, the divergence in the solar proxies and the helioseismic data are not reflected in the shorter-term variations (often referred to as quasi-biennial oscillations) observed on top of the dominant 11-year solar cycle. However, despite being highly correlated in Cycle 22, the short-term variations in the interplanetary proxies show very little correlation with the helioseismic data during Cycles 23 and 24.},
  archiveprefix = {arxiv},
  keywords = {{Helioseismology, Observations},Integrated Sun Observations,notion,notion-database,{Oscillations, Solar},{Solar Cycle, Observations}},
  file = {/Users/lbugnet/Zotero/storage/4KGL3UDQ/Broomhall, Nakariakov - 2015.pdf}
}

@article{Broomhall2015a,
  title = {Solar Cycle Variations in the Powers and Damping Rates of Low-Degree Solar Acoustic Oscillations},
  author = {Broomhall, A. M. and Pugh, C. E. and Nakariakov, V. M.},
  year = {2015},
  journal = {Advances in Space Research},
  volume = {56},
  number = {12},
  pages = {2706--2712},
  publisher = {{COSPAR}},
  issn = {18791948},
  doi = {10.1016/j.asr.2015.04.018},
  abstract = {Helioseismology uses the Sun's natural resonant oscillations to study the solar interior. The properties of the solar oscillations are sensitive to the Sun's magnetic activity cycle. Here we examine variations in the powers, damping rates, and energy supply rates of the most prominent acoustic oscillations in unresolved, Sun-as-a-star data, obtained by the Birmingham Solar Oscillations Network (BiSON) during solar cycles 22, 23, and the first half of 24. The variations in the helioseismic parameters are compared to the 10.7 cm flux, a well-known global proxy of solar activity. As expected the oscillations are most heavily damped and the mode powers are at a minimum at solar activity maximum. The 10.7 cm flux was linearly regressed using the fractional variations of damping rates and powers observed during cycle 23. In general, good agreement is found between the damping rates and the 10.7 cm flux. However, the linearly regressed 10.7 cm flux and fractional variation in powers diverge in cycles 22 and 24, indicating that the relationship between the mode powers and the 10.7 cm flux is not consistent from one cycle to the next. The energy supply rate of the oscillations, which is usually approximately constant, also decreases at this time. We have determined that this discrepancy is not because of the first-order bias introduced by an increase in the level of background noise or gaps in the data. Although we cannot categorically rule out an instrumental origin, the divergence observed in cycle 24, when the data were of high quality and the data coverage was over 80\%, raises the possibility that the effect may be solar in origin.},
  keywords = {Helioseismology,notion,notion-database,Solar cycle,Sun},
  file = {/Users/lbugnet/Zotero/storage/R8BXIPRR/Broomhall, Pugh, Nakariakov - 2015.pdf}
}

@article{Brott2011,
  title = {Rotating Massive Main-Sequence Stars. {{I}}. {{Grids}} of Evolutionary Models and Isochrones},
  author = {Brott, I. and {de Mink}, S. E. and Cantiello, M. and Langer, N. and {de Koter}, A. and Evans, C. J. and Hunter, I. and Trundle, C. and Vink, J. S.},
  year = {2011},
  month = jun,
  journal = {Astronomy \& Astrophysics},
  volume = {530},
  pages = {A115},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201016113},
  urldate = {2023-10-09},
  abstract = {We present a dense grid of evolutionary tracks and isochrones of rotating massive main-sequence stars. We provide three grids with different initial compositions tailored to compare with early OB stars in the Small and Large Magellanic Clouds and in the Galaxy. Each grid covers masses ranging from 5 to 60 M{$\odot$} and initial rotation rates between 0 and about 600 km s-1. To calibrate our models we used the results of the VLT-FLAMES Survey of Massive Stars. We determine the amount of convective overshooting by using the observed drop in rotation rates for stars with surface gravities log g {$<$} 3.2 to determine the width of the main sequence. We calibrate the efficiency of rotationally induced mixing using the nitrogen abundance determinations for B stars in the Large Magellanic cloud. We describe and provide evolutionary tracks and the evolution of the central and surface abundances. In particular, we discuss the occurrence of quasi-chemically homogeneous evolution, i.e. the severe effects of efficient mixing of the stellar interior found for the most massive fast rotators. We provide a detailed set of isochrones for rotating stars. Rotation as an initial parameter leads to a degeneracy between the age and the mass of massive main sequence stars if determined from its observed location in the Hertzsprung-Russell diagram. We show that the consideration of surface abundances can resolve this degeneracy. Model data is made available at the CDS via anonymous ftp to cdsarc.u-strasbg.fr (130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/530/A115},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: abundances,stars: early-type,stars: evolution,stars: massive,stars: rotation},
  annotation = {ADS Bibcode: 2011A\&A...530A.115B},
  file = {/Users/lbugnet/Zotero/storage/M4YKGVXN/Brott et al. - 2011 - Rotating massive main-sequence stars. I. Grids of .pdf}
}

@article{Brown1985,
  title = {Solar Rotation as a Function of Depth and Latitude},
  author = {Brown, Timothy M.},
  year = {1985},
  journal = {Nature},
  volume = {317},
  number = {6038},
  pages = {591--594},
  issn = {00280836},
  doi = {10.1038/317591a0},
  abstract = {A 5-day series of two-dimensional velocity images of the Sun is analysed to yield frequencies of solar p-mode oscillations with degrees between 8 and 50, with all azimuthal orders for each degree. The frequency splitting between modes with the same degree and radial order is related to the latitudinal variation of rotation, averaged over a depth range that depends on the degree. The observed splittings indicate that for 0.3R{$\odot$} l{$\sim$}rl{$\sim$}0.7R{$\odot$} the solar latitudinal differential rotation is much smaller than at the surface (rotation roughly constant on spheres), and moreover that the rotation rate is close to the surface equatorial value. \textcopyright{} 1985 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VUSU4MNS/Brown - 1985.pdf}
}

@article{Brown1987,
  title = {Depth and Latitude Dependence of Solar Rotation},
  author = {Brown, T. M. and Morrow, Cherilynn A.},
  year = {1987},
  journal = {The Astrophysical Journal},
  volume = {314},
  eprint = {1011.1669v3},
  pages = {21--26},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XB6RBUDC/Brown, Morrow - 1987.pdf}
}

@article{Brown1990,
  title = {A Technique for Estimating Complicated Power Spectra from Time Series with Gaps},
  author = {Brown, Timothy M. and {Christensen-Dalsgaard}, Jorgen},
  year = {1990},
  journal = {The Astrophysical Journal},
  volume = {349},
  pages = {667},
  issn = {0004-637X},
  doi = {10.1086/168354},
  abstract = {Fahlman and Ulrych (1982) describe a method for estimating the power and phase spectra of gapped time series, using a maximum-entropy reconstruction of the data in the gaps. It has proved difficult to apply this technique to solar oscillations data, because of the great complexity of the solar oscillations spectrum. We describe a means for avoiding this difficulty and report the results of a series of blind tests of the modified technique.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LI3AYQSS/Brown, Christensen-Dalsgaard - 1990.pdf}
}

@article{Brown2010,
  title = {Persistent {{Magnetic Wreaths}} in a {{Rapidly Rotating Sun}}},
  author = {Brown, Benjamin P. and Browning, Matthew K. and Brun, Allen Sacha and Miesch, Mark S. and Toomre, Juri},
  year = {2010},
  month = nov,
  journal = {The Astrophysical Journal},
  volume = {711},
  number = {1},
  eprint = {1011.2831},
  pages = {424--438},
  doi = {10.1088/0004-637X/711/1/424},
  urldate = {2020-07-06},
  abstract = {When our Sun was young it rotated much more rapidly than now. Observations of young, rapidly rotating stars indicate that many possess substantial magnetic activity and strong axisymmetric magnetic fields. We conduct simulations of dynamo action in rapidly rotating suns with the 3-D MHD anelastic spherical harmonic (ASH) code to explore the complex coupling between rotation, convection and magnetism. Here we study dynamo action realized in the bulk of the convection zone for a system rotating at three times the current solar rotation rate. We find that substantial organized global-scale magnetic fields are achieved by dynamo action in this system. Striking wreaths of magnetism are built in the midst of the convection zone, coexisting with the turbulent convection. This is a surprise, for it has been widely believed that such magnetic structures should be disrupted by magnetic buoyancy or turbulent pumping. Thus, many solar dynamo theories have suggested that a tachocline of penetration and shear at the base of the convection zone is a crucial ingredient for organized dynamo action, whereas these simulations do not include such tachoclines. We examine how these persistent magnetic wreaths are maintained by dynamo processes and explore whether a classical mean-field \$\textbackslash alpha\$-effect explains the regeneration of poloidal field.},
  archiveprefix = {arxiv},
  keywords = {convection-magnetohydrodynamics (MHD)-stars,interior,interiors-stars,magnetic field-stars,notion,notion-database,rotation-Sun},
  file = {/Users/lbugnet/Zotero/storage/JEVD3JYK/full-text.pdf}
}

@article{Brown2011,
  title = {Magnetic Cycles in a Convective Dynamo Simulation of a Young Solar-Type Star},
  author = {Brown, Benjamin P. and Miesch, Mark S. and Browning, Matthew K. and Brun, Allan Sacha and Toomre, Juri},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {731},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/731/1/69},
  abstract = {Young solar-type stars rotate rapidly and many are magnetically active. Some appear to undergo magnetic cycles similar to the 22 yr solar activity cycle. We conduct simulations of dynamo action in rapidly rotating suns with the three-dimensional magnetohydrodynamic anelastic spherical harmonic (ASH) code to explore dynamo action achieved in the convective envelope of a solar-type star rotating at five times the current solar rotation rate. We find that dynamo action builds substantial organized global-scale magnetic fields in the midst of the convection zone. Striking magnetic wreaths span the convection zone and coexist with the turbulent convection. A surprising feature of this wreath-building dynamo is its rich time dependence. The dynamo exhibits cyclic activity and undergoes quasi-periodic polarity reversals where both the global-scale poloidal and toroidal fields change in sense on a roughly 1500day timescale. These magnetic activity patterns emerge spontaneously from the turbulent flow and are more organized temporally and spatially than those realized in our previous simulations of the solar dynamo. We assess in detail the competing processes of magnetic field creation and destruction within our simulations that contribute to the global-scale reversals. We find that the mean toroidal fields are built primarily through an {$\Omega$}-effect, while the mean poloidal fields are built by turbulent correlations which are not well represented by a simple {$\alpha$}-effect. During a reversal the magnetic wreaths propagate toward the polar regions, and this appears to arise from a poleward propagating dynamo wave. As the magnetic fields wax and wane in strength and flip in polarity, the primary response in the convective flows involves the axisymmetric differential rotation which varies on similar timescales. Bands of relatively fast and slow fluid propagate toward the poles on timescales of roughly 500days and are associated with the magnetic structures that propagate in the same fashion. In the Sun, similar patterns are observed in the poleward branch of the torsional oscillations, and these may represent poleward propagating magnetic fields deep below the solar surface. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  keywords = {convection,magnetohydrodynamics (MHD),notion,notion-database,stars: interiors,stars: magnetic field,stars: rotation,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/NQUWD2MF/Brown et al. - 2011.pdf}
}

@article{Brown2011a,
  title = {Kepler Input Catalog: {{Photometric}} Calibration and Stellar Classification},
  author = {Brown, Timothy M. and Latham, David W. and Everett, Mark E. and Esquerdo, Gilbert A.},
  year = {2011},
  journal = {Astronomical Journal},
  volume = {142},
  number = {4},
  eprint = {1102.0342},
  issn = {00046256},
  doi = {10.1088/0004-6256/142/4/112},
  abstract = {We describe the photometric calibration and stellar classification methods used by the Stellar Classification Project to produce the Kepler Input Catalog (KIC). The KIC is a catalog containing photometric and physical data for sources in the Kepler mission field of view; it is used by the mission to select optimal targets. Four of the visible-light (g, r, i, z) magnitudes used in the KIC are tied to Sloan Digital Sky Survey magnitudes; the fifth (D51) is an AB magnitude calibrated to be consistent with Castelli \& Kurucz (CK) model atmosphere fluxes. We derived atmospheric extinction corrections from hourly observations of secondary standard fields within the Kepler field of view. For these filters and extinction estimates, repeatability of absolute photometry for stars brighter than magnitude 15 is typically 2\%. We estimated stellar parameters \{T eff, log (g), log (Z), E B - V\} using Bayesian posterior probability maximization to match observed colors to CK stellar atmosphere models. We applied Bayesian priors describing the distribution of solar-neighborhood stars in the color-magnitude diagram, in log (Z), and in height above the galactic plane. Several comparisons with samples of stars classified by other means indicate that for 4500K {$\leq$}T eff {$\leq$} 6500 K, our classifications are reliable within about 200 K and 0.4 dex in log (g) for dwarfs, with somewhat larger log (g) uncertainties for giants. It is difficult to assess the reliability of our log (Z) estimates, but there is reason to suspect that it is poor, particularly at extreme T eff. Comparisons between the CK models and observed colors are generally satisfactory with some exceptions, notably for stars cooler than 4500K. Of great importance for the Kepler mission, for T eff {$\leq$} 5400 K, comparison with asteroseismic results shows that the distinction between main-sequence stars and giants is reliable with about 98\% confidence. Larger errors in log (g) occur for warmer stars, for which our filter set provides inadequate gravity diagnostics. The KIC is available through the MAST data archive. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {catalogs,methods: data analysis,notion,notion-database,surveys,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/BPHX9M64/Brown et al. - 2011(2).pdf}
}

@article{Brown2012,
  title = {The {{ELM Survey}}. {{III}}. {{A Successful Targeted Survey}} for {{Extremely Low Mass White Dwarfs}}},
  author = {Brown, Warren R. and Kilic, Mukremin and Allende Prieto, Carlos and Kenyon, Scott J.},
  year = {2012},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {744},
  pages = {142},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/744/2/142},
  urldate = {2023-10-02},
  abstract = {Extremely low mass (ELM) white dwarfs (WDs) with masses {$<$} 0.25 M {$\odot$} are rare objects that result from compact binary evolution. Here, we present a targeted spectroscopic survey of ELM WD candidates selected by color. The survey is 71\% complete and has uncovered 18 new ELM WDs. Of the seven ELM WDs with follow-up observations, six are short-period binaries and four have merger times less than 5 Gyr. The most intriguing object, J1741+6526, likely has either a pulsar companion or a massive WD companion making the system a possible supernova Type Ia or an Ia progenitor. The overall ELM survey has now identified 19 double degenerate binaries with {$<$}10 Gyr merger times. The significant absence of short orbital period ELM WDs at cool temperatures suggests that common envelope evolution creates ELM WDs directly in short period systems. At least one-third of the merging systems are halo objects, thus ELM WD binaries continue to form and merge in both the disk and the halo. Based on observations obtained at the MMT Observatory, a joint facility of the Smithsonian Institution and the University of Arizona.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,binaries: close,Galaxy: stellar content,stars: individual: SDSS J011210.25+183503.7 SDSS J015213.77+074913.9 SDSS J144342.74+150938.6 SDSS J151826.68+065813.2 SDSS J174140.49+652638.7 SDSS J184037.78+642312.3,stars: neutron,white dwarfs},
  annotation = {ADS Bibcode: 2012ApJ...744..142B},
  file = {/Users/lbugnet/Zotero/storage/2QNK7MDS/Brown et al. - 2012 - The ELM Survey. III. A Successful Targeted Survey .pdf}
}

@article{Brown2016,
  title = {Gaia Data Release 1},
  author = {Gaia, Collaboration and A Brown, A G and Vallenari, A and Prusti, T and {de Bruijne}, J HJ and Mignard, F and Drimmel, R and Babusiaux, C and {Bailer-Jones}, C AL and Bastian, U and Biermann, M and Evans, D W and Eyer, L and Jansen, F and Jordi, C and Katz, D and Klioner, S A and Lammers, U and Lindegren, L and Luri, X and Panem, C and Pourbaix, D and Randich, S and Sartoretti, P and Siddiqui, H I and Soubiran, C and Valette, V and {van Leeuwen}, F and Walton, N A and Aerts, C and Arenou, F and Cropper, M and H{\o}g, E and Lattanzi, M G and Grebel, E K and Holland, A D and Huc, C and Passot, X and Perryman, M and Bramante, L and Cacciari, C and Casta{\~n}eda, J and Chaoul, L and Cheek, N and De Angeli, F and Fabricius, C and Guerra, R and Hern{\'a}ndez, J and {Jean-Antoine-Piccolo}, A and Masana, E and Messineo, R and Mowlavi, N and Nienartowicz, K and {Ord{\'o}{\~n}ez-Blanco}, D and Panuzzo, P and Portell, J and Richards, P J and Riello, M and Seabroke, G M and Tanga, P and Th{\'e}venin, F and Torra, J and Els, S G and {Gracia-Abril}, G and Comoretto, G and {Garcia-Reinaldos}, M and Lock, T and Mercier, E and Altmann, M and Andrae, R and Astraatmadja, T L and {Bellas-Velidis}, I and Benson, K and Berthier, J and Blomme, R and Busso, G and Carry, B and Cellino, A and Clementini, G and Cowell, S and Creevey, O and Cuypers, J and Davidson, M and De Ridder, J and {de Torres}, A and Delchambre, L and Dell, A and Ducourant, C and Fr{\'e}mat, Y and {Garc{\'i}a-Torres}, M and Gosset, E and Halbwachs, J-l and Hambly, N C and Harrison, D L and Hauser, M and Hestroffer, D and Hodgkin, S T and Huckle, H E and Hutton, A and Jasniewicz, G and Jordan, S and Kontizas, M and Korn, A J and Lanzafame, A C and Manteiga, M and Moitinho, A and Muinonen, K and Osinde, J and Pancino, E and Pauwels, T and Petit, J-m and {Recio-Blanco}, A and Robin, A C and Sarro, L M and Siopis, C and Smith, M and Smith, K W and Sozzetti, A and Thuillot, W and {van Reeven}, W and Viala, Y and Abbas, U and Abreu Aramburu, A and Accart, S and Aguado, J J and Allan, P M and Allasia, W and Altavilla, G and {\'A}lvarez, M A and Alves, J and Anderson, R I and Andrei, A H and Anglada Varela, E and Antiche, E and Antoja, T and Ant{\'o}n, S and Arcay, B and Bach, N and Baker, S G and {Balaguer-N{\'u}{\~n}ez}, L and Barache, C and Barata, C and Barbier, A and Barblan, F and Barrado Navascu{\'e}s, D and Barros, M and Barstow, M A and Becciani, U and Bellazzini, M and Bello Garc{\'i}a, A and Belokurov, V and Bendjoya, P and Berihuete, A and Bianchi, L and Bienaym{\'e}, O and Billebaud, F and Blagorodnova, N and {Blanco-Cuaresma}, S and Boch, T and Bombrun, A and Borrachero, R and Bouquillon, S and Bourda, G and Bouy, H and Bragaglia, A and Breddels, M A and Brouillet, N and Br{\"u}semeister, T and Bucciarelli, B and Burgess, P and Burgon, R and Burlacu, A and Busonero, D and Buzzi, R and Caffau, E and Cambras, J and Campbell, H and Cancelliere, R and {Cantat-Gaudin}, T and Carlucci, T and Carrasco, J M and Castellani, M and Charlot, P and Charnas, J and Chiavassa, A and Clotet, M and Cocozza, G and Collins, R S and Costigan, G and Crifo, F and Cross, N JG and Crosta, M and Crowley, C and Dafonte, C and Damerdji, Y and Dapergolas, A and David, P and David, M and De Cat, P and {de Felice}, F and {de Laverny}, P and De Luise, F and De March, R and {de Martino}, D and {de Souza}, R and Debosscher, J and {del Pozo}, E and Delbo, M and Delgado, A and Delgado, H E and Di Matteo, P and Diakite, S and Distefano, E and Dolding, C and Dos Anjos, S and Drazinos, P and Duran, J and Dzigan, Y and Edvardsson, B and Enke, H and Evans, N W and Eynard Bontemps, G and Fabre, C and Fabrizio, M and Faigler, S and Falc{\~a}o, A J and Farr{\`a}s Casas, M and Federici, L and Fedorets, G and {Fern{\'a}ndez-Hern{\'a}ndez}, J and Fernique, P and Fienga, A and Figueras, F and Filippi, F and Findeisen, K and Fonti, A and Fouesneau, M and Fraile, E and Fraser, M and Fuchs, J and Gai, M and Galleti, S and Galluccio, L and Garabato, D and {Garc{\'i}a-Sedano}, F and Garofalo, A and Garralda, N and Gavras, P and Gerssen, J and Geyer, R and Gilmore, G and Girona, S and Giuffrida, G and Gomes, M and {Gonz{\'a}lez-Marcos}, A and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J and {Gonz{\'a}lez-Vidal}, J J and Granvik, M and Guerrier, A and Guillout, P and Guiraud, J and G{\'u}rpide, A and {Guti{\'e}rrez-S{\'a}nchez}, R and Guy, L P and Haigron, R and Hatzidimitriou, D and Haywood, M and Heiter, U and Helmi, A and Hobbs, D and Hofmann, W and Holl, B and Holland, G and Hunt, J AS and Hypki, A and Icardi, V and Irwin, M and {Jevardat de Fombelle}, G and Jofr{\'e}, P and Jonker, P G and Jorissen, A and Julbe, F and Karampelas, A and Kochoska, A and Kohley, R and Kolenberg, K and Kontizas, E and Koposov, S E and Kordopatis, G and Koubsky, P and {Krone-Martins}, A and Kudryashova, M and Kull, I and Bachchan, R K and {Lacoste-Seris}, F and Lanza, A F and Lavigne, J-b and {Le Poncin-Lafitte}, C and Lebreton, Y and Lebzelter, T and Leccia, S and Leclerc, N and {Lecoeur-Taibi}, I and Lemaitre, V and Lenhardt, H and Leroux, F and Liao, S and Licata, E and Lindstr{\o}m, H EP and Lister, T A and Livanou, E and Lobel, A and L{\"o}ffler, W and L{\'o}pez, M and Lorenz, D and MacDonald, I and Magalh{\~a}es Fernandes, T and Managau, S and Mann, R G and Mantelet, G and Marchal, O and Michalik, D and Millar, N R and H Miranda, B M and Molina, D and Molinaro, R and Pentik{\"a}inen, H and Pichon, B and Piersimoni, A M and Pineau, F-x and Plachy, E and Plum, G and Poujoulet, E and Pr{\v s}a, A and Pulone, L and Ragaini, S and Rago, S and Rambaux, N and {Ramos-Lerate}, M and Ranalli, P and Rauw, G and Read, A and Regibo, S and Reyl{\'e}, C and Ribeiro, R A and Rimoldini, L and Ripepi, V and Riva, A and Rixon, G and Roelens, M and {Romero-G{\'o}mez}, M and Rowell, N and Royer, F and {Ruiz-Dern}, L and Sadowski, G and Sagrist{\`a} Sell{\'e}s, T and Sahlmann, J and Salgado, J and Salguero, E and Sarasso, M and Savietto, H and Schultheis, M and Sciacca, E and Segol, M and Segovia, J C and Segransan, D and Shih, I-c and Smareglia, R and Smart, R L and Solano, E and Solitro, F and Sordo, R and Soria Nieto, S and Souchay, J and Spagna, A and Spoto, F and Stampa, U and Steele, I A and Steidelm{\"u}ller, H and Stephenson, C A and Stoev, H and Suess, F F and S{\"u}veges, M and Surdej, J and Szabados, L and {Szegedi-Elek}, E and Tapiador, D and Taris, F and Tauran, G and Taylor, M B and Teixeira, R and Terrett, D and Tingley, B and Trager, S C and Turon, C and Ulla, A and Utrilla, E and Valentini, G and {van Elteren}, A and Van Hemelryck, E and {van Leeuwen}, M and Varadi, M and Vecchiato, A and Veljanoski, J and Via, T and Vicente, D and Vogt, S and Voss, H and Votruba, V and Voutsinas, S and Walmsley, G and Weiler, M and Weingrill, K and Wevers, T and Wyrzykowski, {\L} and Yoldas, A and {\v Z}erjal, M and Zucker, S and Zurbach, C and Zwitter, T and Alecu, A and Allen, M and Allende Prieto, C and Amorim, A and {Anglada-Escud{\'e}}, G and Arsenijevic, V and Azaz, S and Balm, P and Beck, M and Bernstein, H-h and Bigot, L and Bijaoui, A and Blasco, C and Bonfigli, M and Bono, G and Boudreault, S and Bressan, A and Brown, S and Brunet, P-m and Bunclark, P and Buonanno, R and Butkevich, A G and Carret, C and Carrion, C and Chemin, L and Ch{\'e}reau, F and Corcione, L and Darmigny, E and {de Boer}, K S and {de Teodoro}, P and {de Zeeuw}, P T and Delle Luche, C and Domingues, C D and Dubath, P and Fodor, F and Fr{\'e}zouls, B and Fries, A and Fustes, D and Fyfe, D and Gallardo, E and Gallegos, J and Gardiol, D and Gebran, M and Gomboc, A and G{\'o}mez, A and Grux, E and Gueguen, A and Heyrovsky, A and Munari, U and Nguyen, A-t and Nordlander, T and Ocvirk, P and Olias Sanz, A and Ortiz, P and Osorio, J and Oszkiewicz, D and Ouzounis, A and Palmer, M and Park, P and Pasquato, E and Peltzer, C and Peralta, J and P{\'e}turaud, F and Pieniluoma, T and Pigozzi, E and Ziaeepour, H and Zschocke, S},
  year = {2016},
  month = sep,
  journal = {Astronomische Nachrichten},
  volume = {337},
  number = {8-9},
  eprint = {1601.01313},
  pages = {944--948},
  publisher = {{Wiley-VCH Verlag}},
  issn = {15213994},
  doi = {10.1002/asna.201612404},
  urldate = {2020-03-06},
  abstract = {The main goal of Galactic Archaeology is understanding the formation and evolution of the basic Galactic components. This requires sophisticated chemo-dynamical modeling, where disc asymmetries (e.g., perturbations from the central bar, spirals arms, and infalling satellites) and non-equilibrium processes are taken into account self-consistently. Here we discuss the current status of Galactic chemo-dynamical modeling and focus on a recent hybrid technique, which helps circumvent traditional problems with chemical enrichment and star formation encountered in fully self-consistent cosmological simulations. We show that this model can account for a number of chemo-kinematic relations in the Milky Way. In addition, we demonstrate that (1) our model matches well the observed age-[{$\alpha$}/Fe] and age-[Fe/H] relations and (2) that the scatter in the age-[Fe/H] relation cannot be simply explained by blurring (stars on apo- and pericenters visiting the solar vicinity) but significant radial migration (stars born elsewhere but ending up at the solar vicinity today because of a change in guiding radius) is needed. We emphasize the importance of accurate stellar ages, such as those obtained through asteroseismology by the CoRoT and Kepler missions, for breaking the degeneracy among different Galactic evolution scenarios.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: abundances,Galaxy: disk,Galaxy: evolution,Galaxy: formation,Galaxy: kinematics and dynamics,notion,notion-database}
}

@article{Brown2016a,
  title = {Most {{Double Degenerate Low-mass White Dwarf Binaries Merge}}},
  author = {Brown, Warren R. and Kilic, Mukremin and Kenyon, Scott J. and Gianninas, A.},
  year = {2016},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {824},
  pages = {46},
  issn = {0004-637X},
  doi = {10.3847/0004-637X/824/1/46},
  urldate = {2023-10-09},
  abstract = {We estimate the merger rate of double degenerate binaries containing extremely low mass (ELM; 0.3 M {$\odot$}) white dwarfs (WDs) in the Galaxy. Such WDs are detectable for timescales of 0.1-1 Gyr in the ELM Survey; the binaries they reside in have gravitational wave merger times of 0.001-100 Gyr. To explain the observed distribution requires that most ELM WD binary progenitors detach from the common envelope phase with {$<$}1 hr orbital periods. We calculate the local space density of ELM WD binaries and estimate a merger rate of 3 \texttimes{} 10-3 yr-1 over the entire disk of the Milky Way; the merger rate in the halo is 10 times smaller. The ELM WD binary merger rate exceeds by a factor of 40 the formation rate of stable mass transfer AM CVn binaries, marginally exceeds the rate of underluminous supernovae, and is identical to the formation rate of R CrB stars. On this basis, we conclude that ELM WD binaries can be the progenitors of all observed AM CVn and possibly underluminous supernovae; however, the majority of He+CO WD binaries go through unstable mass transfer and merge, e.g., into single massive {$\sim$}1 M {$\odot$} WDs.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,binaries: close,Galaxy: stellar content,white dwarfs},
  annotation = {ADS Bibcode: 2016ApJ...824...46B},
  file = {/Users/lbugnet/Zotero/storage/GCHDXFCI/Brown et al. - 2016 - Most Double Degenerate Low-mass White Dwarf Binari.pdf}
}

@article{Browning2006a,
  title = {Dynamo {{Action}} in the {{Solar Convection Zone}} and {{Tachocline}}: {{Pumping}} and {{Organization}} of {{Toroidal Fields}}},
  author = {Browning, Matthew K. and Miesch, Mark S. and Brun, Allan Sacha and Toomre, Juri},
  year = {2006},
  journal = {The Astrophysical Journal},
  volume = {648},
  number = {2},
  eprint = {astro-ph/0609153},
  pages = {L157-L160},
  issn = {0004-637X},
  doi = {10.1086/507869},
  abstract = {We present the first results from three-dimensional spherical shell simulations of magnetic dynamo action realized by turbulent convection penetrating downward into a tachocline of rotational shear. This permits us to assess several dynamical elements believed to be crucial to the operation of the solar global dynamo, variously involving differential rotation resulting from convection, magnetic pumping, and amplification of fields by stretching within the tachocline. The simulations reveal that strong axisymmetric toroidal magnetic fields (about 3000 G in strength) are realized within the lower stable layer, unlike in the convection zone where fluctuating fields are predominant. The toroidal fields in the stable layer possess a striking persistent antisymmetric parity,with fields in the northern hemisphere largely of opposite polarity to those in the southern hemisphere. The associatedmean poloidalmagnetic fields there have a clear dipolar geometry, but we have not yet observed any distinctive reversals or latitudinal propagation. The presence of these deep magnetic fields appears to stabilize the sense ofmean fields produced by vigorous dynamo action in the bulk of the convection zone.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8U9UE2F4/Browning et al. - 2006.pdf}
}

@article{Browning2008,
  title = {Simulations of {{Dynamo Action}} in {{Fully Convective Stars}}},
  author = {Browning, Matthew K.},
  year = {2008},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {676},
  number = {2},
  eprint = {0712.1603},
  pages = {1262--1280},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/527432},
  urldate = {2020-06-19},
  abstract = {We present three-dimensional nonlinear magnetohydrodynamic simulations of the interiors of fully convective M-dwarfs. Our models consider 0.3 solar-mass stars using the Anelastic Spherical Harmonic code, with the spherical computational domain extending from 0.08-0.96 times the overall stellar radius. Like previous authors, we find that fully convective stars can generate kG-strength magnetic fields (in rough equipartition with the convective flows) without the aid of a tachocline of shear. Although our model stars are everywhere unstably stratified, the amplitudes and typical pattern sizes of the convective flows vary strongly with radius, with the outer regions of the stars hosting vigorous convection and field amplification while the deep interiors are more quiescent. Modest differential rotation is established in hydrodynamic calculations, but -- unlike in some prior work --strongly quenched in MHD simulations because of the Maxwell stresses exerted by the dynamo-generated magnetic fields. Despite the lack of strong differential rotation, the magnetic fields realized in the simulations possess significant mean (axisymmetric) components, which we attribute partly to the strong influence of rotation upon the slowly overturning flows.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,brown dwarfs,convection,mass,MHD,notion,notion-database,stars: low,stars: magnetic fields,turbulence},
  file = {/Users/lbugnet/Zotero/storage/QPLUFC3C/full-text.pdf}
}

@article{Browning2015,
  title = {{{THEORETICAL LIMITS ON MAGNETIC FIELD STRENGTHS IN LOW-MASS STARS}}},
  author = {Browning, Matthew K and Weber, Maria A and Chabrier, Gilles and Massey, Angela P},
  year = {2015},
  doi = {10.3847/0004-637X/818/2/189},
  urldate = {2020-10-05},
  abstract = {Observations have suggested that some low-mass stars have larger radii thanpredicted by 1D structure models. Some theoretical models have invoked very strong interior magnetic fields (of order 1 MG or more) as a possible cause of such large radii. Whether fields of that strength could in principle begenerated by dynamo action in these objects is unclear, and we do not address the matter directly. Instead, we examine whether such fields could remain in the interior of a low-mass object for a significant amount of time, and whether they would have any other obvious signatures. First, we estimate the timescales for the loss of strong fields by magnetic buoyancy instabilities. We consider a range of field strengths and simple morphologies, including both idealized flux tubes and smooth layers of field. We confirm some of our analytical estimates using thin flux tube magnetohydrodynamic simulations of the rise of buoyant fields in a fully convective M-dwarf. Separately, we consider the Ohmic dissipation of such fields. We find that dissipation provides a complementary constraint to buoyancy: while small-scale, fibril fields might be regenerated faster than they rise, the dissipative heating associated with such fields would in some cases greatly exceed the luminosity of the star. We show how these constraints combine to yield limits on the internal field strength and morphology in low-mass stars. In particular, we find that for stars of 0.3 solar masses, no fields in flux tubes stronger than about 800 kG are simultaneously consistent with both constraints.},
  keywords = {convection,magnetohydrodynamics (MHD),notion,notion-database,stars: low-mass,stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/TXZDQMAZ/full-text.pdf}
}

@article{Bruevich2014,
  title = {Changed {{Relation}} between {{Solar}} 10.7-Cm {{Radio Flux}} and Some {{Activity Indices}} Which Describe the {{Radiation}} at {{Different Altitudes}} of {{Atmosphere}} during {{Cycles}} 21\textendash 23},
  author = {Bruevich, E. A. and Bruevich, V. V. and Yakunina, G. V.},
  year = {2014},
  journal = {Journal of Astrophysics and Astronomy},
  volume = {35},
  number = {1},
  pages = {1--15},
  issn = {09737758},
  doi = {10.1007/s12036-014-9258-0},
  abstract = {The correlation coefficients of the linear regression of six solar indices versus 10.7 cm radio flux F{$<$}inf{$>$}10.7{$<$}/inf{$>$} were analysed in solar cycles 21, 22 and 23. We also analysed the interconnection between these indices and F{$<$}inf{$>$}10.7{$<$}/inf{$>$} with help of approximation by polynomials of second order. The indices we have studied in this paper are: the relative sunspot numbers \textendash{} SSN, 530.3 nm coronal line flux \textendash{} F{$<$}inf{$>$}530{$<$}/inf{$>$}, the total solar irradiance \textendash{} TSI, Mg II 280 nm core-to-wing ratio UV-index, the Flare Index \textendash{} FI and the counts of flares. In most cases the regressions of these solar indices vs. F{$<$}inf{$>$}10.7{$<$}/inf{$>$} are close to the linear regression except the moments of time near the minimums and maximums of the 11-year activity. For the linear regressions, we found that correlation coefficients K{$<$}inf{$>$}corr{$<$}/inf{$>$}(t) for the solar indices vs. F{$<$}inf{$>$}10.7{$<$}/inf{$>$} and SSN dropped to their minimum values twice during each 11-year cycle.},
  keywords = {notion,notion-database,Solar cycle: observations\textemdash solar activity indices},
  file = {/Users/lbugnet/Zotero/storage/RXZW2EMT/Bruevich, Bruevich, Yakunina - 2014.pdf}
}

@article{Brun1998,
  title = {Standard Solar Models in the Light of New Helioseismic Constraints. i. the Solar Core a. s. Brun and s. Turck-Chie ` Ze},
  author = {Brun, A. S. and {Turck-Chieze}, S. and Morel, P.},
  year = {1998},
  journal = {The Astrophysical Journal},
  volume = {20},
  number = {506},
  pages = {913--925},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9VRJVAH7/Brun, Turck-Chieze, Morel - 1998.pdf}
}

@article{Brun2000,
  title = {Erratum {{Standard Solar Models}} in the {{Light}} of {{New Helioseismic Constraints}}. {{II}}. {{Mixing}} below the {{Convective Zone}}},
  author = {Brun, A. S. and Turck-Chieze, S. and Zahn, J. P.},
  year = {2000},
  journal = {The Astrophysical Journal},
  volume = {536},
  number = {2},
  pages = {1005--1005},
  issn = {0004-637X},
  doi = {10.1086/308988},
  abstract = {In previous work, we have shown that recent updated standard solar models cannot reproduce the radial profile of the sound speed at the base of the convective zone and fail to predict the photospheric lithium abundance. In parallel, helioseismology has shown that the transition from differential rotation in the convective zone to almost uniform rotation in the radiative solar interior occurs in a shallow layer called the tachocline. This layer is presumably the seat of a large-scale circulation and of turbulent motions. Here we introduce a macroscopic transport term in the structure equations that is based on a hydrodynamical description of the tachocline proposed by Spiegel \& Zahn, and we calculate the mixing induced within this layer. We discuss the influence of different parameters that represent the tachocline thickness, the Brunt-V\"ais\"al\"a frequency at the base of the convective zone, and the time dependence of this mixing process along the Sun's evolution. We show that the introduction of such a process inhibits the microscopic diffusion by about 25\%. Starting from models including a pre-main-sequence evolution, we obtain (1) a good agreement with observed photospheric chemical abundance of light elements such as 3He, 4He, 7Li, and 9Be; (2) a smooth composition gradient at the base of the convective zone; and (3) a significant improvement of the sound-speed square difference between the seismic Sun and the models in this transition region when we allow the photospheric heavy-element abundance to adjust, within the observational incertitude, as a result of the action of this mixing process. The impact on neutrino predictions is also discussed.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XIPACT97/Brun, Turck‐Chieze, Zahn - 2000.pdf}
}

@article{Brun2004,
  title = {Global-{{Scale Turbulent Convection}} and {{Magnetic Dynamo Action}} in the {{Solar Envelope}}},
  author = {Brun, Allan Sacha and Miesch, Mark S. and Toomre, Juri},
  year = {2004},
  journal = {The Astrophysical Journal},
  volume = {614},
  number = {2},
  pages = {1073--1098},
  issn = {0004-637X},
  doi = {10.1086/423835},
  abstract = {The operation of the solar global dynamo appears to involve many dynamical elements. Self-consistent MHD simulations which realistically incorporate all of these processes are not yet computationally feasible, though some elements can now be studied with reasonable fidelity. Here we consider the manner in which turbulent compressible convection within the bulk of the solar convection zone can generate large-scale magnetic fields through dynamo action. We accomplish this through a series of three-dimensional numerical simulations of MHD convection within rotating spherical shells using our ASH code on massively parallel supercomputers. Since differential rotation is a key ingredient in all dynamo models, we also examine here the nature of the rotation profiles that can be sustained within the deep convection zone as strong magnetic fields are built and maintained. We find that the convection is able to maintain a solar-like angular velocity profile despite the influence of Maxwell stresses which tend to oppose Reynolds stresses and thus reduce the latitudinal angular velocity contrast throughout the convection zone. The dynamo-generated magnetic fields exhibit a complex structure and evolution, with radial fields concentrated in downflow lanes and toroidal fields organized into twisted ribbons which are extended in longitude and which achieve field strengths of up to 5000 G. The flows and fields exhibit substantial kinetic and magnetic helicity although systematic hemispherical patterns are only apparent in the former. Fluctuating fields dominate the magnetic energy and account for most of the back-reaction on the flow via Lorentz forces. Mean fields are relatively weak and do not exhibit systematic latitudinal propagation or periodic polarity reversals as in the sun. This may be attributed to the absence of a tachocline.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/C2MIZITY/Brun, Miesch, Toomre - 2004.pdf}
}

@article{Brun2005,
  title = {Simulations of {{Core Convection}} in {{Rotating A}}-{{Type Stars}}: {{Magnetic Dynamo Action}}},
  author = {Brun, Allan Sacha and Browning, Matthew K. and Toomre, Juri},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {629},
  number = {1},
  eprint = {astro-ph/0610072},
  pages = {461--481},
  issn = {0004-637X},
  doi = {10.1086/430430},
  abstract = {Core convection and dynamo activity deep within rotating A-type stars of 2 Msolar are studied with three-dimensional nonlinear simulations. Our modeling considers the inner 30\% by radius of such stars, thus capturing within a spherical domain the convective core and a modest portion of the surrounding radiative envelope. The magnetohydrodynamic (MHD) equations are solved using the anelastic spherical harmonic (ASH) code to examine turbulent flows and magnetic fields, both of which exhibit intricate time dependence. By introducing small seed magnetic fields into our progenitor hydrodynamic models rotating at 1 and 4 times the solar rate, we assess here how the vigorous convection can amplify those fields and sustain them against ohmic decay. Dynamo action is indeed realized, ultimately yielding magnetic fields that possess energy densities comparable to that of the flows. Such magnetism reduces the differential rotation obtained in the progenitors, partly by Maxwell stresses that transport angular momentum poleward and oppose the Reynolds stresses in the latitudinal balance. In contrast, in the radial direction we find that the Maxwell and Reynolds stresses may act together to transport angular momentum. The central columns of slow rotation established in the progenitors are weakened, with the differential rotation waxing and waning in strength as the simulations evolve. We assess the morphology of the flows and magnetic fields, their complex temporal variations, and the manner in which dynamo action is sustained. Differential rotation and helical convection are both found to play roles in giving rise to the magnetic fields. The magnetism is dominated by strong fluctuating fields throughout the core, with the axisymmetric (mean) fields there relatively weak. The fluctuating magnetic fields decrease rapidly with radius in the region of overshooting, and the mean toroidal fields less so due to stretching by rotational shear.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,Convection,Magnetohydrodynamics: MHD,notion,notion-database,Stars: Evolution,Stars: Interiors,Stars: Magnetic Fields},
  file = {/Users/lbugnet/Zotero/storage/D2YF7GWM/Brun, Browning, Toomre - 2005.pdf;/Users/lbugnet/Zotero/storage/QK9VDZ4F/full-text.pdf}
}

@article{Brun2006,
  title = {Magnetic Confinement of the Solar Tachocline},
  author = {Brun, A. S. and Zahn, J. -P.},
  year = {2006},
  month = oct,
  journal = {Astronomy \& Astrophysics},
  volume = {457},
  pages = {665--674},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20053908},
  urldate = {2023-10-18},
  abstract = {Context: .We study the physics of the solar tachocline (i.e. the thin transition layer between differential rotation in the convection zone and quasi uniform rotation in the radiative interior), and related MHD instabilities. Aims: .We have performed 3D MHD simulations of the solar radiative interior to check whether a fossil magnetic field is able to prevent the spread of the tachocline. Methods: .Starting with a purely poloidal magnetic field and a latitudinal shear meant to be imposed by the convection zone at the top of the radiation zone, we have investigated the interactions between magnetic fields, rotation and shear, using the spectral code ASH on massively parallel supercomputers. Results: .In all cases we have explored, the fossil field diffuses outward and ends up connecting with the convection zone, whose differential rotation is then imprinted at latitudes above {$\approx$}40\textdegree{} throughout the radiative interior, according to Ferraro's law of isorotation. Rotation remains uniform in the lower latitude region which is contained within closed field lines. We find that the meridional flow cannot stop the inward progression of the differential rotation. Further, we observe the development of non-axisymmetric magnetohydrodynamic instabilities, first due to the initial poloidal configuration of the fossil field, and later to the toroidal field produced by shearing the poloidal field through the differential rotation. We do not find dynamo action as such in the radiative interior, since the mean poloidal field is not regenerated. But the instability persists during the whole evolution, while slowly decaying with the mean poloidal field; it is probably sustained by small departures from isorotation. Conclusions: .According to our numerical simulations, a fossil magnetic field cannot prevent the radiative spread of the tachocline, and thus it is unable to enforce uniform rotation in the radiation zone. Neither can the observed thinness of that layer be invoked as a proof for such an internal fossil magnetic field.},
  keywords = {Astrophysics,magnetohydrodynamics (MHD),stars: evolution,stars: rotation,Sun: rotation,turbulence},
  annotation = {ADS Bibcode: 2006A\&A...457..665B},
  file = {/Users/lbugnet/Zotero/storage/JVRIZ79R/Brun and Zahn - 2006 - Magnetic confinement of the solar tachocline.pdf}
}

@article{Brun2006a,
  title = {Magnetic Confinement of the Solar Tachocline},
  author = {Brun, A. S. and Zahn, J. -P.},
  year = {2006},
  month = oct,
  journal = {Astronomy and Astrophysics},
  volume = {457},
  number = {2},
  eprint = {astro-ph/0610069},
  pages = {665--674},
  doi = {10.1051/0004-6361:20053908},
  urldate = {2020-08-11},
  abstract = {We study the physics of the solar tachocline and related MHD instabilities. We have performed 3-D MHD simulations of the solar radiative interior to check whether a fossil magnetic field is able to prevent the spread of the tachocline. Starting with a purely poloidal magnetic field and a latitudinal shear meant to be imposed by the convection zone at the top of the radiation zone, we have investigated the interactions between magnetic fields, rotation and shear, using the spectral code ASH on massive parallel supercomputers. In all cases we have explored, the fossil field diffuses outward and ends up connecting with the convection zone, whose differential rotation is then imprinted at latitudes above 40 deg throughout the radiative interior, according to Ferraro's law of isorotation. Rotation remains uniform in the lower latitude region which is contained within closed field lines. We find that the meridional flow cannot stop the inward progression of the differential rotation. Further, we observe the development of non-axisymmetric magnetohydrodynamic instabilities, first due to the initial poloidal configuration of the fossil field, and later to the toroidal field produced by shearing the poloidal field through the differential rotation. We do not find dynamo action as such in the radiative interior, since the mean poloidal field is not regenerated. But the instability persists during the whole evolution, while slowly decaying with the mean poloidal field. According to our numerical simulations, a fossil magnetic field cannot prevent the radiative spread of the tachocline, and thus it is unable to enforce uniform rotation in the radiation zone. Neither can the observed thinness of that layer be invoked as a proof for such an internal fossil magnetic field.},
  archiveprefix = {arxiv},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Stars: Evolution,Stars: Rotation,Sun: Rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/B4SNDNZ6/full-text.pdf}
}

@article{Brun2009,
  title = {Numerical Simulations of a Rotating Red Giant Star. {{I}}. {{Three-dimensional}} Models of Turbulent Convection and Associated Mean Flows},
  author = {Brun, A. S. and Palacios, A.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {702},
  number = {2},
  pages = {1078--1097},
  issn = {15384357},
  doi = {10.1088/0004-637X/702/2/1078},
  abstract = {With the development of one-dimensional stellar evolution codes including rotation and the increasing number of observational data for stars of various evolutionary stages, it becomes more and more possible to follow the evolution of the rotation profile and angular momentum distribution in stars. In this context, understanding the interplay between rotation and convection in the very extended envelopes of giant stars is very important considering that all low- and intermediate-mass stars become red giants after the central hydrogen burning phase. In this paper, we analyze the interplay between rotation and convection in the envelope of red giant stars using three-dimensional numerical experiments. We make use of the Anelastic Spherical Harmonics code to simulate the inner 50\% of the envelope of a low-mass star on the red giant branch. We discuss the organization and dynamics of convection, and put a special emphasis on the distribution of angular momentum in such a rotating extended envelope. To do so, we explore two directions of the parameter space, namely, the bulk rotation rate and the Reynolds number with a series of four simulations. We find that turbulent convection in red giant stars is dynamically rich, and that it is particularly sensitive to the rotation rate of the star. Reynolds stresses and meridional circulation establish various differential rotation profiles (either cylindrical or shellular) depending on the convective Rossby number of the simulations, but they all agree that the radial shear is large. Temperature fluctuations are found to be large and in the slowly rotating cases, a dominant {$\mathscr{l}$} = 1 temperature dipole influences the convective motions. Both baroclinic effects and turbulent advection are strong in all cases and mostly oppose one another. \textcopyright{} 2009. The American Astronomical Society. All rights reserved.},
  keywords = {Convection,Evolution,Hydrodynamics,Interiors,Methods,notion,notion-database,Numerical,Rotation,Stars},
  file = {/Users/lbugnet/Zotero/storage/E36FEAQ7/Brun, Palacios - 2009.pdf}
}

@article{Brun2010,
  title = {Modelling the {{Sun}} and {{Stars}} in 3-{{D}}},
  author = {Brun, A. S.},
  year = {2010},
  journal = {EAS Publications Series},
  volume = {44},
  pages = {81--95},
  issn = {16334760},
  doi = {10.1051/eas/1044015},
  abstract = {Stars can be seen as modern physics laboratory from which fundamental processes as diverse as atomic physics or turbulence can be studied and understood. Being able to model accurately their structure, dynamic and evolution is thus of fundamental importance and is the subject of intense research. In this short review we will present some of the numerical simulations in three dimensions performed in recent years to model such complex and nonlinear objects, focussing mostly our discussion on results obtained with the anelastic spherical harmonic (ASH) code. Using the Sun as a reference star, we wish to gain insight and to constrain magnetohydrodynamical processes (such as Reynolds and Maxwell stresses, meridional circulations, differential rotation (i.e. {$\omega$}-effect), thermal wind, {$\alpha$}-effect) at the origin of the solar small and large scale dynamics and magnetism. We will then extend our study to other stars, such as young Suns, massive stars or evolved RGB stars in order to identify which processes are at the origin of their significantly different dynamics. \textcopyright{} EAS, EDP Sciences 2011.},
  isbn = {9782759806065},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Z3PQ2CSL/Brun - 2010.pdf}
}

@article{Brun2017,
  title = {On {{Differential Rotation}} and {{Overshooting}} in {{Solar-like Stars}}},
  author = {Brun, Allan Sacha and Strugarek, Antoine and Varela, Jacobo and Matt, Sean P. and Augustson, Kyle C. and Emeriau, Constance and DoCao, Olivier Long and Brown, Benjamin and Toomre, Juri},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {836},
  number = {2},
  eprint = {1702.06598},
  pages = {192},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aa5c40},
  abstract = {We seek to characterize how the change of global rotation rate influences the overall dynamics and large scale flows arising in the convective envelopes of stars covering stellar spectral types from early G to late K. We do so through numerical simulations with the ASH code, where we consider stellar convective envelopes coupled to a radiative interior with various global properties. As solar-like stars spin down over the course of their main sequence evolution, such change must have a direct impact on their dynamics and rotation state. We indeed find that three main states of rotation may exist for a given star: anti-solar-like (fast poles, slow equator), solar-like (fast equator, slow poles), or a cylindrical rotation profile. Under increasingly strict rotational constraints, the latter profile can further evolve into a Jupiter-like profile, with alternating prograde and retrograde zonal jets. We have further assessed how far the convection and meridional flows overshoot into the radiative zone and investigated the morphology of the established tachocline. Using simple mixing length arguments, we are able to construct a scaling of the fluid Rossby number \$R\_\{of\} = \textbackslash tilde\{\textbackslash omega\}/2\textbackslash Omega\_* \textbackslash sim \textbackslash tilde\{v\}/2\textbackslash Omega\_* R\_*\$, which we calibrate based on our 3-D ASH simulations. We can use this scaling to map the behavior of differential rotation versus the global parameters of stellar mass and rotation rate. Finally, we isolate a region on this map (\$R\_\{of\} \textbackslash gtrsim 1.5-2\$) where we posit that stars with an anti-solar differential rotation may exist in order to encourage observers to hunt for such targets.},
  archiveprefix = {arxiv},
  keywords = {activity,convection,hydrodynamics,notion,notion-database,rotation,solar-type,stars,stars: activity,stars: rotation,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/LP26DENU/Brun et al. - 2017.pdf}
}

@article{Brun2017a,
  title = {Magnetism, Dynamo Action and the Solar-Stellar Connection},
  author = {Brun, Allan Sacha and Browning, Matthew K.},
  year = {2017},
  month = dec,
  journal = {Living Reviews in Solar Physics},
  volume = {14},
  number = {1},
  pages = {1--133},
  publisher = {{Springer Science and Business Media LLC}},
  issn = {2367-3648},
  doi = {10.1007/s41116-017-0007-8},
  urldate = {2020-05-22},
  abstract = {The Sun and other stars are magnetic: magnetism pervades their interiors and affects their evolution in a variety of ways. In the Sun, both the fields themselves and their influence on other phenomena can be uncovered in exquisite detail, but these observations sample only a moment in a single star's life. By turning to observations of other stars, and to theory and simulation, we may infer other aspects of the magnetism-e.g., its dependence on stellar age, mass, or rotation rate-that would be invisible from close study of the Sun alone. Here, we review observations and theory of magnetism in the Sun and other stars, with a partial focus on the "Solar-stellar connec-tion": i.e., ways in which studies of other stars have influenced our understanding of the Sun and vice versa. We briefly review techniques by which magnetic fields can be measured (or their presence otherwise inferred) in stars, and then highlight some key observational findings uncovered by such measurements, focusing (in many cases) on those that offer particularly direct constraints on theories of how the fields are built and maintained. We turn then to a discussion of how the fields arise in different objects: first, we summarize some essential elements of convection and dynamo theory, including a very brief discussion of mean-field theory and related concepts. Next we turn to simulations of convection and magnetism in stellar interiors, highlighting both some peculiarities of field generation in different types of stars and some unifying physical processes that likely influence dynamo action in general. We conclude with a brief summary of what we have learned, and a sampling of issues that remain uncertain or unsolved.},
  keywords = {Astronomy,Astrophysics and Astroparticles,Astrophysics and Cosmology,notion,notion-database,Plasma Physics,Space Exploration and Astronautics),Space Sciences (including Extraterrestrial Physics},
  file = {/Users/lbugnet/Zotero/storage/JJR22KX7/full-text.pdf}
}

@article{Bruntt2005,
  title = {Evidence for {{Granulation}} and {{Oscillations}} in {{Procyon}} from {{Photometry}} with the {{WIRE Satellite}}},
  author = {Bruntt, H. and Kjeldsen, H. and Buzasi, D. L. and Bedding, T. R.},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {633},
  number = {1},
  eprint = {astro-ph/0504469},
  pages = {440--446},
  issn = {0004-637X},
  doi = {10.1086/462401},
  abstract = {We report evidence for the granulation signal in the star Procyon A, based on two photometric time series from the star tracker on the WIRE satellite. The power spectra show evidence of excess power around 1 milliHz, consistent with the detection of p-modes reported from radial velocity measurements. We see a significant increase in the noise level below 3 milliHz, which we interpret as the granulation signal. We have made a large set of numerical simulations to constrain the amplitude and timescale of the granulation signal and the amplitude of the oscillations. We find that the timescale for granulation is T(gran) = 750(200) s, the granulation amplitude is 1.8(0.3) times solar, and the amplitude of the p-modes is 8(3) ppm. We found the distribution of peak heights in the observed power spectra to be consistent with that expected from p-mode oscillations. However, the quality of the data is not sufficient to measure the large separation or detect a comb-like structure, as seen in the p-modes of the Sun. Comparison with the recent negative result from the MOST satellite reveal that the MOST data must have an additional noise source that prevented the detection of oscillations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6GJN2SNZ/Bruntt et al. - 2005.pdf}
}

@article{Bruntt2007,
  title = {Multisite Campaign on the Open Cluster {{M67}} - {{III}}. {$\delta$} {{Scuti}} Pulsations in the Blue Stragglers},
  author = {Bruntt, H. and Stello, D. and Su{\'a}rez, J. C. and Arentoft, T. and Bedding, T. R. and Bouzid, M. Y. and Csubry, Z. and Dall, T. H. and Dind, Z. E. and Frandsen, S. and Gilliland, R. L. and Jacob, A. P. and Jensen, H. R. and Kang, Y. B. and Kim, S. L. and Kiss, L. L. and Kjeldsen, H. and Koo, J. R. and Lee, J. A. and Lee, C. U. and Nuspl, J. and Sterken, C. and Szab{\'o}, R.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {378},
  number = {4},
  pages = {1371--1384},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.11865.x},
  abstract = {We have made an asteroseismic analysis of the variable blue stragglers in the open cluster M67. The data set consists of photometric time-series from eight sites using nine 0.6-2.1 m telescopes with a time-baseline of 43 d. In two stars, EW Cnc and EX Cnc, we detect the highest number of frequencies (41 and 26) detected in {$\delta$} Scuti stars belonging to a stellar cluster, and EW Cnc has the second highest number of frequencies detected in any {$\delta$} Scuti star. We have computed a grid of pulsation models that take the effects of rotation into account. The distribution of observed and theoretical frequencies shows that in a wide frequency range a significant fraction of the radial and non-radial low-degree modes are excited to detectable amplitudes. Despite the large number of observed frequencies we cannot constrain the fundamental parameters of the stars. To make progress we need to identify the degrees of some of the modes from either multicolour photometry or spectroscopy. \textcopyright{} 2007 RAS.},
  keywords = {Blue stragglers,notion,notion-database,Open clusters and associations: individual: M67 (N,Stars: individual: EW Cnc,Stars: individual: EX Cnc,{$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/69MU6WU9/Bruntt et al. - 2007.pdf}
}

@article{Bruntt2008,
  title = {A Spectroscopic Study of Southern (Candidate) {$\gamma$} {{Doradus}} Stars: {{II}}. {{Detailed}} Abundance Analysis and Fundamental Parameters},
  author = {Bruntt, H. and De Cat, P. and Aerts, C.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {478},
  number = {2},
  pages = {487--496},
  issn = {00046361},
  doi = {10.1051/0004-6361:20078523},
  abstract = {Context: The {$\gamma$} Doradus stars are a recent class of variable main sequence F-type stars located on the red edge of the Cepheid instability strip. They pulsate in gravity modes, and this makes them particularly interesting for detailed asteroseismic analysis, which can provide fundamental knowledge of properties near the convective cores of intermediate-mass main sequence stars. Aims: To improve current understanding of {$\gamma$} Dor stars through theoretical modelling, additional constraints are needed. Our aim is to estimate the fundamental atmospheric parameters and determine the chemical composition of these stars. Detailed analyses of single stars have previously suggested links to Am and {$\lambda$} Boo stars, so we wish to explore this interesting connection between chemical peculiarity and pulsation. Methods: We analysed a sample of {$\gamma$} Dor stars for the first time, including nine bona fide and three candidate members of the class. We determined the fundamental atmospheric parameters and compared the abundance pattern with other A-type stars. We used the semi-automatic software package VWA for the analysis. This code relies on the calculation of synthetic spectra and thus takes lineblending into account. This is important because of the fast rotation in some of the sample stars, and we made a thorough analysis of how VWA performs when increasing {$\nu$} sin i. We obtained good results in agreement with previously derived fundamental parameters and abundances in a few selected reference stars with properties similar to the {$\gamma$} Dor stars. Results: We find that the abundance pattern in the {$\gamma$} Dor stars is not distinct from the constant A-and F-type stars we analysed. \textcopyright{} ESO 2008.},
  keywords = {notion,notion-database,Stars: abundances,Stars: chemically peculiar,Stars: early-type,Stars: fundamental parameters,Stars: oscillations,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/I77QPCDC/Bruntt, De Cat, Aerts - 2008.pdf}
}

@article{Bruntt2009,
  title = {Accurate Fundamental Parameters of {{CoRoT}} Asteroseismic Targets},
  author = {Bruntt, H.},
  year = {2009},
  journal = {Astronomy \& Astrophysics},
  volume = {506},
  number = {1},
  pages = {235--244},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/200911925},
  abstract = {Context: The CoRoT satellite has provided high-quality light curves of several solar-like stars. Analysis of these light curves provides oscillation frequencies that make it possible to probe the interior of the stars. However, additional constraints on the fundamental parameters of the stars are important for the theoretical modelling to be successful. Aims: We estimate the fundamental parameters (mass, radius, and luminosity) of the first four solar-like targets to be observed in the asteroseismic field. In addition, we determine their effective temperature, metallicity, and detailed abundance patterns. Methods: To constrain the stellar mass, radius and age we used the shotgun software, which compares the location of the stars in the Hertzsprung-Russell diagram with theoretical evolution models. This method takes the uncertainties of the observed parameters into account, including the large separation determined from the solar-like oscillations. We determined the effective temperatures and abundance patterns in the stars from the analysis of high-resolution spectra obtained with the HARPS, NARVAL, ELODIE and FEROS spectrographs. Results: We determined the mass, radius, and luminosity of the four CoRoT targets to within 5\{-\}10\%, 2\{-\}4\% and 5\{-\}13\%, respectively. The quality of the stellar spectra determines how well we can constrain the effective temperature. For the two best spectra we get 1-{$\sigma$} uncertainties below 60 K and 100\{-\}150 K for the other two. The uncertainty on the surface gravity is less than 0.08 dex for three stars, while it is 0.15 dex for HD 181906. The reason for the larger uncertainty is that the spectrum has two components with a luminosity ratio of L\_p/Ls = 0.50{$\pm$}0.15. While Hipparcos astrometric data strongly suggest it is a binary star, we find evidence that the fainter star may be a background star, since it is less luminous but hotter.},
  keywords = {abundances,binaries,fundamental parameters,notion,notion-database,spectroscopic,stars,{stars: fundamental parameters, binaries: spectrosc}},
  file = {/Users/lbugnet/Zotero/storage/R33574HC/Bruntt - 2009.pdf}
}

@article{Bruntt2010,
  title = {Accurate Fundamental Parameters for 23 Bright Solar-Type Stars},
  author = {Bruntt, H. and Bedding, T. R. and Quirion, P. O. and Lo Curto, G. and Carrier, F. and Smalley, B. and Dall, T. H. and Arentoft, T. and Bazot, M. and Butler, R. P.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {405},
  number = {3},
  pages = {1907--1923},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2010.16575.x},
  abstract = {We combine results from interferometry, asteroseismology and spectroscopy to determine accurate fundamental parameters of 23 bright solar-type stars, from spectral type F5 to K2 and luminosity classes III-V. For some stars we can use direct techniques to determine the mass, radius, luminosity and effective temperature, and we compare with indirect methods that rely on photometric calibrations or spectroscopic analyses. We use the asteroseismic information available in the literature to infer an indirect mass with an accuracy of 4-15 per cent. From indirect methods we determine luminosity and radius to 3 per cent. We find evidence that the luminosity from the indirect method is slightly overestimated ({$\approx$} 5 per cent) for the coolest stars, indicating that their bolometric corrections (BCs) are too negative. For Teff we find a slight offset of -40 {$\pm$} 20 K between the spectroscopic method and the direct method, meaning the spectroscopic temperatures are too high. From the spectroscopic analysis we determine the detailed chemical composition for 13 elements, including Li, C and O. The metallicity ranges from [Fe/H]=-1.7 to +0.4, and there is clear evidence for {$\alpha$}-element enhancement in the metal-poor stars. We find no significant offset between the spectroscopic surface gravity and the value from combining asteroseismology with radius estimates. From the spectroscopy we also determine v sin i and we present a new calibration of macroturbulence and microturbulence. From the comparison between the results from the direct and spectroscopic methods we claim that we can determine Teff, log and [Fe/H] with absolute accuracies of 80 K, 0.08 and 0.07 dex. Photometric calibrations of Str\"omgren indices provide accurate results for Teff and [Fe/H] but will be more uncertain for distant stars when interstellar reddening becomes important. The indirect methods are important to obtain reliable estimates of the fundamental parameters of relatively faint stars when interferometry cannot be used. This paper is the first to compare direct and indirect methods for a large sample of stars, and we conclude that indirect methods are valid, although slight corrections may be needed. \textcopyright{} 2010 The Authors. Journal compilation \textcopyright{} 2010 RAS.},
  keywords = {notion,notion-database,Stars: abundances,Stars: fundamental parameters,Stars: solar-type,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/3WTM7BTF/Bruntt et al. - 2010.pdf}
}

@article{Bruntt2012,
  title = {Accurate Fundamental Parameters and Detailed Abundance Patterns from Spectroscopy of 93 Solar-Type {{Kepler}} Targets},
  author = {Bruntt, H. and Basu, S. and Smalley, B. and Chaplin, W. J. and Verner, G. A. and Bedding, T. R. and Catala, C. and Gazzano, J. C. and {Molenda-Zakowicz}, J. and Thygesen, A. O. and Uytterhoeven, K. and Hekker, S. and Huber, D. and Karoff, C. and Mathur, S. and Mosser, B. and Appourchaux, T. and Campante, T. L. and Elsworth, Y. and Garc{\'i}a, R. A. and Handberg, R. and Metcalfe, T. S. and Quirion, P. O. and R{\'e}gulo, C. and Roxburgh, I. W. and Stello, D. and {Christensen-Dalsgaard}, J. and Kawaler, S. D. and Kjeldsen, H. and Morris, R. L. and Quintana, E. V. and Sanderfer, D. T.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {423},
  number = {1},
  pages = {122--131},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.20686.x},
  abstract = {We present a detailed spectroscopic study of 93 solar-type stars that are targets of the NASA/Kepler mission and provide detailed chemical composition of each target. We find that the overall metallicity is well represented by Fe lines. Relative abundances of light elements (CNO) and {$\alpha$} elements are generally higher for low-metallicity stars. Our spectroscopic analysis benefits from the accurately measured surface gravity from the asteroseismic analysis of the Kepler light curves. The accuracy on the logg parameter is better than 0.03 dex and is held fixed in the analysis. We compare our T eff determination with a recent colour calibration of V T-K S [TYCHO V magnitude minus Two Micron All Sky Survey (2MASS) K S magnitude] and find very good agreement and a scatter of only 80K, showing that for other nearby Kepler targets, this index can be used. The asteroseismic logg values agree very well with the classical determination using Fei-Feii balance, although we find a small systematic offset of 0.08 dex (asteroseismic logg values are lower). The abundance patterns of metals, {$\alpha$} elements and the light elements (CNO) show that a simple scaling by [Fe/H] is adequate to represent the metallicity of the stars, except for the stars with metallicity below -0.3, where {$\alpha$}-enhancement becomes important. However, this is only important for a very small fraction of the Kepler sample. We therefore recommend that a simple scaling with [Fe/H] be employed in the asteroseismic analyses of large ensembles of solar-type stars. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {notion,notion-database,Stars: abundances,Stars: atmospheres,Stars: fundamental parameters,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/Z64PVD2U/Bruntt et al. - 2012.pdf}
}

@incollection{Bt1989,
  title = {Unno:List of Symbols},
  author = {Unno, Wasaburo},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZC3BDNAM/Unno - 1989(8).pdf}
}

@article{buderGALAHSurveySecond2018,
  title = {The {{GALAH Survey}}: Second Data Release},
  author = {Buder, Sven and Asplund, Martin and Duong, Ly and Kos, Janez and Lind, Karin and Ness, Melissa K and Sharma, Sanjib and {Bland-Hawthorn}, Joss and Casey, Andrew R and De Silva, Gayandhi M and Orazi, Valentina D ' and Freeman, Ken C and Lewis, Geraint F and Lin, Jane and Martell, Sarah L and Schlesinger, Katharine J and Simpson, Jeffrey D and Zucker, Daniel B and Zwitter, Toma{\v z} and Amarsi, Anish M and Anguiano, Borja and Carollo, Daniela and Casagrande, Luca and Cotar, Kleme{\v n} and Cottrell, Peter L and Da Costa, Gary and Gao, Xudong D and Hayden, Michael R and Horner, Jonathan and Ireland, Michael J and Kafle, Prajwal R and Munari, Ulisse and Nataf, David M and Nordlander, Thomas and Stello, Dennis and Ting, Yuan-Sen and Traven, Gregor and Watson, Fred and Wittenmyer, Robert A and Wyse, Rosemary F G and Yong, David and Zinn, Joel C and Maru{\v s}a{\v z}erjal, Maru{\v s}a Maru{\v s}a{\textasciicaron}},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {478},
  pages = {4513--4552},
  doi = {10.1093/mnras/sty1281},
  urldate = {2021-08-12},
  abstract = {The Galactic Archaeology with HERMES (GALAH) survey is a large-scale stellar spectro-scopic survey of the Milky Way, designed to deliver complementary chemical information to a large number of stars covered by the Gaia mission. We present the GALAH second public data release (GALAH DR2) containing 342 682 stars. For these stars, the GALAH collaboration provides stellar parameters and abundances for up to 23 elements to the community. Here we present the target selection, observation, data reduction, and detailed explanation of how the spectra were analysed to estimate stellar parameters and element abundances. For the stellar analysis, we have used a multistep approach. We use the physics-driven spectrum synthesis of Spectroscopy Made Easy (SME) to derive stellar labels (T eff , log g, [Fe/H], [X/Fe], v mic , vsin i, A K S) for a representative training set of stars. This information is then propagated to the whole sample with the data-driven method of The Cannon. Special care has been exercised in the spectral synthesis to only consider spectral lines that have reliable atomic input data and are little affected by blending lines. Departures from local thermodynamic equilibrium (LTE) are considered for several key elements, including Li, O, Na, Mg, Al, Si, and Fe, using 1D MARCS stellar atmosphere models. Validation tests including repeat observations, Gaia benchmark stars, open and globular clusters, and K2 asteroseismic targets lend confidence to our methods and results. Combining the GALAH DR2 catalogue with the kinematic information from Gaia will enable a wide range of Galactic Archaeology studies, with unprecedented detail, dimensionality, and scope.},
  keywords = {abundances,data analysis-stars,fundamental parameters-stars,notion,notion-database,observational-methods,Surveys-the Galaxy-methods}
}

@article{buderGALAHSurveyThird2021,
  title = {The {{GALAH}}+ Survey: {{Third}} Data Release},
  author = {Buder, Sven and Sharma, Sanjib and Kos, Janez and Amarsi, Anish M and Nordlander, Thomas and Lind, Karin and Martell, Sarah L and Asplund, Martin and {Bland-Hawthorn}, Joss and Casey, Andrew R and De Silva, Gayandhi M and Orazi, Valentina D ' and Freeman, Ken C and Hayden, Michael R and Lewis, Geraint F and Lin, Jane and Schlesinger, Katharine J and Simpson, Jeffrey D and Stello, Dennis and Zucker, Daniel B and Zwitter, Toma{\v z} and Beeson, Kevin L and Buck, Tobias and Casagrande, Luca and Clark, Jake T and Cotar, Kleme{\v n} and Da Costa, Gary S and De Grijs, Richard and Feuillet, Diane and Horner, Jonathan and Kafle, Prajwal R and Khanna, Shourya and Kobayashi, Chiaki and Liu, Fan and Montet, Benjamin T and Nandakumar, Govind and Nataf, David M and Ness, Melissa K and Spina, Lorenzo and {Tepper-Garc{\'i}a}, Thor and Ting, Yuan-Sen and Traven, Gregor and Vogrin{\v c}i{\v c}, Rok and Wittenmyer, Robert A and Wyse, Rosemary F G and Maru{\v s}a{\v z}erjal, Maru{\v s}a Maru{\v s}a{\textasciicaron}},
  year = {2021},
  journal = {MNRAS},
  volume = {506},
  pages = {150--201},
  doi = {10.1093/mnras/stab1242},
  urldate = {2021-08-12},
  abstract = {The ensemble of chemical element abundance measurements for stars, along with precision distances and orbit properties, provides high-dimensional data to study the evolution of the Milky Way. With this third data release of the Galactic Archaeology with HERMES (GALAH) survey, we publish 678 423 spectra for 588 571 mostly nearby stars (81.2 per cent of stars are within {$<$}2 kpc), observed with the HERMES spectrograph at the Anglo-Australian Telescope. This release (hereafter GALAH+ DR3) includes all observations from GALAH Phase 1 (bright, main, and faint survey, 70 per cent), K2-HERMES (17 per cent), TESS-HERMES (5 per cent), and a subset of ancillary observations (8 per cent) including the bulge and {$>$}75 stellar clusters. We derive stellar parameters T eff , log g, [Fe/H], v mic , v broad , and v rad using our modified version of the spectrum synthesis code Spectroscopy Made Easy (SME) and 1D MARCS model atmospheres. We break spectroscopic degeneracies in our spectrum analysis with astrometry from Gaia DR2 and photometry from 2MASS. We report abundance ratios [X/Fe] for 30 different elements (11 of which are based on non-LTE computations) covering five nucleosynthetic pathways. We describe validations for accuracy and precision, flagging of peculiar stars/measurements and recommendations for using our results. Our catalogue comprises 65 per cent dwarfs, 34 per cent giants, and 1 per cent other/unclassified stars. Based on unflagged chemical composition and age, we find 62 per cent young low-{$\alpha$}, 9 per cent young high-{$\alpha$}, 27 per cent old high-{$\alpha$}, and 2 per cent stars with [Fe/H] {$\leq$} -1. Based on kinematics, 4 per cent are halo stars. Several Value-Added-Catalogues, including stellar ages and dynamics, updated after Gaia eDR3, accompany this release and allow chrono-chemodynamic analyses, as we showcase.},
  keywords = {abundances \ding{72} Contact,abundances-stars,data analysis-methods,data analysis-stars,fundamental parameters,fundamental parameters-stars,methods,notion,notion-database,observational-methods,observational-surveys-stars,Surveys-the Galaxy-methods},
  file = {/Users/lbugnet/Zotero/storage/Y8I84Y7J/full-text.pdf}
}

@inproceedings{Bugnet2017,
  title = {Fliper: {{Checking}} the Reliability of Global Seismic Parameters from Automatic Pipelines},
  booktitle = {{{SF2A-2017}}: {{Proceedings}} of the {{Annual Meeting}} of the {{French Society}} of {{Astronomy}} and {{Astrophysics}}},
  author = {Bugnet, L. and Garc{\'i}a, R.A. and Davies, G.R. and Mathur, S. and Corsaro, E.},
  year = {2017},
  abstract = {Our understanding of stars through asteroseismic data analysis is limited by our ability to take advantage of the huge amount of observed stars provided by space missions such as CoRoT, Kepler, K2, and soon TESS and PLATO. Global seismic pipelines provide global stellar parameters such as mass and radius using the mean seismic parameters, as well as the effective temperature. These pipelines are commonly used automatically on thousands of stars observed by K2 for 3 months (and soon TESS for at least {$\sim$} 1 month). However, pipelines are not immune from misidentifying noise peaks and stellar oscillations. Therefore, new validation techniques are required to assess the quality of these results. We present a new metric called FliPer (Flicker in Power), which takes into account the average variability at all measured time scales. The proper calibration of FliPer enables us to obtain good estimations of global stellar parameters such as surface gravity that are robust against the influence of noise peaks and hence are an excellent way to find faults in asteroseismic pipelines.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations}
}

@article{Bugnet2018,
  title = {{{FliPer}}: {{A}} Global Measure of Power Density to Estimate Surface Gravities of Main-Sequence Solar-like Stars and Red Giants},
  author = {Bugnet, L. and Garc{\'i}a, R. A. and Davies, G. R. and Mathur, S. and Corsaro, E. and Hall, O. J. and Rendle, B. M.},
  year = {2018},
  journal = {Astronomy \& Astrophysics},
  volume = {620},
  eprint = {1809.05105},
  pages = {1--9},
  issn = {14320746},
  doi = {10.1051/0004-6361/201833106},
  abstract = {Asteroseismology provides global stellar parameters such as masses, radii, or surface gravities using mean global seismic parameters and effective temperature for thousands of low-mass stars (0.8 M{$\odot$} {$<$} M {$<$} 3 M{$\odot$}). This methodology has been successfully applied to stars in which acoustic modes excited by turbulent convection are measured. Other methods such as the Flicker technique can also be used to determine stellar surface gravities, but only works for log g above 2.5 dex. In this work, we present a new metric called FliPer (Flicker in spectral power density, in opposition to the standard Flicker measurement which is computed in the time domain); it is able to extend the range for which reliable surface gravities can be obtained (0.1 {$<$} log g {$<$} 4.6 dex) without performing any seismic analysis for stars brighter than Kp {$<$} 14. FliPer takes into account the average variability of a star measured in the power density spectrum in a given range of frequencies. However, FliPer values calculated on several ranges of frequency are required to better characterize a star. Using a large set of asteroseismic targets it is possible to calibrate the behavior of surface gravity with FliPer through machine learning. This calibration made with a random forest regressor covers a wide range of surface gravities from main-sequence stars to subgiants and red giants, with very small uncertainties from 0.04 to 0.1 dex. FliPer values can be inserted in automatic global seismic pipelines to either give an estimation of the stellar surface gravity or to assess the quality of the seismic results by detecting any outliers in the obtained {$\nu$}max values. FliPer also constrains the surface gravities of main-sequence dwarfs using only long-cadence data for which the Nyquist frequency is too low to measure the acoustic-mode properties.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ETKHWUF8/Bugnet et al. - 2018.pdf}
}

@article{Bugnet2019a,
  title = {{{FliPerClass}}: {{In}} Search of Solar-like Pulsators among {{TESS}} Targets},
  author = {Bugnet, L. and Garc{\'i}a, R. A. and Mathur, S. and Davies, G. R. and Hall, O. J. and Lund, M. N. and Rendle, B. M.},
  year = {2019},
  journal = {Astronomy \& Astrophysics},
  volume = {624},
  eprint = {1902.09854},
  pages = {1--8},
  issn = {14320746},
  doi = {10.1051/0004-6361/201834780},
  abstract = {The NASA Transiting Exoplanet Survey Satellite (TESS) is about to provide full-frame images of almost the entire sky. The amount of stellar data to be analysed represents hundreds of millions stars, which is several orders of magnitude more than the number of stars observed by the Convection, Rotation and planetary Transits satellite (CoRoT), and NASA Kepler and K2 missions. We aim at automatically classifying the newly observed stars with near real-time algorithms to better guide the subsequent detailed studies. In this paper, we present a classification algorithm built to recognise solar-like pulsators among classical pulsators. This algorithm relies on the global amount of power contained in the power spectral density (PSD), also known as the flicker in spectral power density (FliPer). Because each type of pulsating star has a characteristic background or pulsation pattern, the shape of the PSD at different frequencies can be used to characterise the type of pulsating star. The FliPer classifier (FliPerClass) uses different FliPer parameters along with the effective temperature as input parameters to feed a ML algorithm in order to automatically classify the pulsating stars observed by TESS. Using noisy TESS-simulated data from the TESS Asteroseismic Science Consortium (TASC), we classify pulsators with a 98\% accuracy. Among them, solar-like pulsating stars are recognised with a 99\% accuracy, which is of great interest for a further seismic analysis of these stars, which are like our Sun. Similar results are obtained when we trained our classifier and applied it to 27-day subsets of real Kepler data. FliPerClass is part of the large TASC classification pipeline developed by the TESS Data for Asteroseismology (T'DA) classification working group.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/QMMR6U5Y/Bugnet et al. - 2019.pdf}
}

@inproceedings{Bugnet2020a,
  title = {The Impact of a Fossil Magnetic Field on Dipolar Mixed-Mode Frequencies in Sub- and Red-Giant Stars},
  booktitle = {Dynamics of the {{Sun}} and {{Stars}}: {{Honoring}} the {{Life}} and {{Work}} of {{Michael J}}. {{Thompson}}},
  author = {Bugnet, L. and Prat, V. and Mathis, S. and Garc{\'i}a, R. A. and Mathur, S. and Augustson, K. and Neiner, C. and Thompson, M. J.},
  year = {2020},
  month = dec,
  eprint = {2012.08684},
  urldate = {2021-01-06},
  abstract = {Stars more massive than \$\textbackslash sim 1.3\$ M\$\_\textbackslash odot\$ are known to develop a convective core during the main-sequence: the dynamo process triggered by this convection could be the origin of a strong magnetic field inside the core of the star, trapped when it becomes stably stratified and for the rest of its evolution. The presence of highly magnetized white dwarfs strengthens the hypothesis of buried fossil magnetic fields inside the core of evolved low-mass stars. If such a fossil field exists, it should affect the mixed modes of red giants as they are sensitive to processes affecting the deepest layers of these stars. The impact of a magnetic field on dipolar oscillations modes was one of Pr. Michael J. Thompson's research topics during the 90s when preparing the helioseismic SoHO space mission. As the detection of gravity modes in the Sun is still controversial, the investigation of the solar oscillation modes did not provide any hint of the existence of a magnetic field in the solar radiative core. Today we have access to the core of evolved stars thanks to the asteroseismic observation of mixed modes from CoRoT, Kepler, K2 and TESS missions. The idea of applying and generalizing the work done for the Sun came from discussions with Pr. Michael Thompson in early 2018 before we loss him. Following the path we drew together, we theoretically investigate the effect of a stable axisymmetric mixed poloidal and toroidal magnetic field, aligned with the rotation axis of the star, on the mixed modes frequencies of a typical evolved low-mass star. This enables us to estimate the magnetic perturbations to the eigenfrequencies of mixed dipolar modes, depending on the magnetic field strength and the evolutionary state of the star. We conclude that strong magnetic fields of \$\textbackslash sim\$ 1MG should perturbe the mixed-mode frequency pattern enough for its effects to be detectable inside current asteroseismic data.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Bugnet2021,
  title = {Magnetic Signatures on Mixed-Mode Frequencies {{I}}. {{An}} Axisymmetric Fossil Field inside the Core of Red Giants},
  author = {Bugnet, L and Prat, V and Mathis, S and Astoul, A and Augustson, K and Garc{\'i}a, R A and Mathur, S and Amard, L and Neiner, C},
  year = {2021},
  journal = {Astronomy \& Astrophysics},
  volume = {650},
  pages = {53},
  doi = {10.1051/0004-6361/202039159},
  urldate = {2021-10-15},
  abstract = {Context. The discovery of moderate differential rotation between the core and the envelope of evolved solar-like stars could be the signature of a strong magnetic field trapped inside the radiative interior. The population of intermediate-mass red giants presenting surprisingly low-amplitude mixed modes (i.e. oscillation modes that behave as acoustic modes in their external envelope and as gravity modes in their core) could also arise from the effect of an internal magnetic field. Indeed, stars more massive than about 1.1 solar masses are known to develop a convective core during their main sequence. The field generated by the dynamo triggered by this con-vection could be the progenitor of a strong fossil magnetic field trapped inside the core of the star for the remainder of its evolution. Aims. Observations of mixed modes can constitute an excellent probe of the deepest layers of evolved solar-like stars, and magnetic fields in those regions can impact their propagation. The magnetic perturbation on mixed modes may therefore be visible in astero-seismic data. To unravel which constraints can be obtained from observations, we theoretically investigate the effects of a plausible mixed axisymmetric magnetic field with various amplitudes on the mixed-mode frequencies of evolved solar-like stars. Methods. First-order frequency perturbations due to an axisymmetric magnetic field were computed for dipolar and quadrupolar mixed modes. These computations were carried out for a range of stellar ages, masses, and metallicities. Conclusions. We show that typical fossil-field strengths of 0.1-1 MG, consistent with the presence of a dynamo in the convective core during the main sequence, provoke significant asymmetries on mixed-mode frequency multiplets during the red giant branch. We provide constraints and methods for the detectability of such magnetic signatures. We show that these signatures may be detectable in asteroseismic data for field amplitudes small enough for the amplitude of the modes not to be affected by the conversion of gravity into Alfv\'en waves inside the magnetised interior. Finally, we infer an upper limit for the strength of the field and the associated lower limit for the timescale of its action in order to redistribute angular momentum in stellar interiors.},
  keywords = {evolution-stars,interiors-stars,magnetic field-stars,notion,notion-database,oscillations-stars,rotation,stars},
  annotation = {shorthand: B+2021},
  file = {/Users/lbugnet/Zotero/storage/FH76PNNT/full-text.pdf}
}

@article{Bugnet2022,
  title = {Magnetic Signatures on Mixed-Mode Frequencies. {{II}}. {{Period}} Spacings as a Probe of the Internal Magnetism of Red Giants},
  author = {Bugnet, L.},
  year = {2022},
  month = nov,
  journal = {Astronomy \& Astrophysics},
  volume = {667},
  pages = {A68},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202243167},
  urldate = {2023-10-09},
  abstract = {Context. Theoretical works have looked into the various topologies and amplitudes, as well as the stability of the magnetic field that is expected to be present in the radiative interior of stars evolving after the main sequence. From these studies, we know that strong stable "fossil" fields might be trapped inside evolved stars. These could trigger the strong transport of angular momentum from the core to the envelope, a process that is not generally included in state-of-the-art stellar models. This may therefore have a substantial impact on the mixing and the inferred stellar parameters. Such internal magnetic fields have never been observed in evolved stars. As a result, there is a major piece missing from our global picture of stars as dynamical bodies. Aims: Asteroseismology has opened a window onto stellar internal dynamics, as oscillation frequencies, amplitudes, and lifetimes are affected by processes that are taking place inside the star. The detection of buried magnetic fields could therefore be possible through the measurement of their impact on the oscillations of stars. This advancement would be groundbreaking for our knowledge of stellar dynamics. In this scope, magnetic signatures on mixed-mode frequencies have recently been characterized, but the task of detection remains challenging as the mixed-mode frequency pattern is highly complex and affected by rotational effects, while modes of different radial orders are often intertwined. In this work, we aim to build a bridge between theoretical prescriptions and complex asteroseismic data analysis to facilitate a future search and characterization of internal magnetism with asteroseismology. Methods: We investigated the effect of magnetic fields inside evolved stars with solar-like oscillations on the estimation of the period spacing of gravity-mode (g-mode) components of simulated mixed gravito-acoustic modes. We derived a new corrected stretching function of the power spectrum density to account for the presence of magnetic signatures on their frequencies. Results: We demonstrate that the strong dependency of the amplitude of the magnetic signature with mixed-mode frequencies leads to biased estimates of period spacings towards lower values. We also show that a careful analysis of the oscillation frequency pattern through various period spacing estimates and across a broad frequency range might lead to the first detection of magnetic fields inside red giants and at the same time, we adjust the measured value of g-mode period spacing.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: magnetic field,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2022A\&A...667A..68B},
  file = {/Users/lbugnet/Zotero/storage/K9KQ9IP2/Bugnet - 2022 - Magnetic signatures on mixed-mode frequencies. II..pdf}
}

@book{bugnetDynamicsSunStars2021,
  title = {Dynamics of the {{Sun}} and {{Stars}}},
  author = {Bugnet, L. and Prat, V. and Mathis, S. and Garc{\'i}a, R and Mathur, S and Neiner, C and Thompson, M.J.},
  editor = {Monteiro, M{\'a}rio J P F G and Garc{\'i}a, Rafael A and {Christensen-Dalsgaard}, J{\o}rgen and Mcintosh Editors, Scott W},
  year = {2021},
  journal = {Dynamics of the Sun and Stars},
  volume = {57},
  publisher = {{Springer}},
  urldate = {2021-01-17},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HQIZ8CFM/bok-978-3-030-55336-4.pdf}
}

@misc{bugnetFliPerGlobalMeasure2018,
  title = {{{FliPer}}: {{A}} Global Measure of Power Density to Estimate Surface Gravities of Main-Sequence {{Solar-like}} Stars and Red Giants},
  author = {Bugnet, L. and Garc{\'i}a, R.A. and Davies, G.R. and Mathur, S. and Corsaro, E. and Hall, O.J. and Rendle, B.M.},
  year = {2018},
  journal = {arXiv},
  abstract = {Copyright \textcopyright{} 2018, arXiv, All rights reserved. Asteroseismology provides global stellar parameters such as masses, radii or surface gravities using the mean global seismic parameters as well as the eective temperature for thousands of low-mass stars (0:8M M 3M). This methodology has been successfully applied to stars in which acoustic modes excited by turbulent convection are measured. Other techniques such as the Flicker can also be used to determine stellar surface gravities, but only works for log g above 2:5 dex. In this work, we present a new metric called FliPer (the acronym stands for Flicker in spectral power density, in opposition to the standard Flicker measurement which is computed in the time domain) that is able to extend the range for which reliable surface gravities can be obtained (0:1 log g 4:6 dex) without performing any seismic analysis for stars brighter than Kp 14. FliPer takes into account the average variability of a star measured in the power density spectrum in a given range of frequencies. However, FliPer values calculated on several ranges of frequency are required to better characterize a star. Using a large set of asteroseismic targets it is possible to calibrate the behavior of surface gravity with FliPer through machine learning. This calibration made with a random forest regressor covers a wide range of surface gravities from main-sequence stars to subgiants and red giants, with very small uncertainties from 0:04 to 0:1 dex. FliPer values can be inserted in automatic global seismic pipelines to either give an estimation of the stellar surface gravity or to assess the quality of the seismic results by detecting any outliers in the obtained max values. FliPer also constrain the surface gravities of main-sequence dwarfs using only long cadence data for which the Nyquist frequency is too low to measure the acoustic-mode properties.},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,stars: oscillations}
}

@article{bugnetImpactFossilMagnetic2020,
  title = {The Impact of a Fossil Magnetic Field on Dipolar Mixed-Mode Frequencies in Sub- and Red-Giant Stars},
  author = {Bugnet, L. and Prat, V. and Mathis, S. and Garc{\'i}a, R.A. and Mathur, S. and Augustson, K. and Neiner, C. and Thompson, M.J.},
  year = {2020},
  journal = {arXiv},
  issn = {23318422},
  abstract = {Copyright \textcopyright{} 2020, The Authors. All rights reserved. The recent discovery of low-amplitude dipolar oscillation mixed modes in massive red giants indicate the presence of a missing physical process inside their cores. Stars more massive than {$\sim$} 1.3 M{$\Sun$} are known to develop a convective core during the main-sequence: the dynamo process triggered by this convection could be the origin of a strong magnetic field inside the core of the star, trapped when it becomes stably stratified and for the rest of its evolution. The presence of highly magnetized white dwarfs strengthens the hypothesis of buried fossil magnetic fields inside the core of evolved low-mass stars. If such a fossil field exists, it should affect the mixed modes of red giants as they are sensitive to processes affecting the deepest layers of these stars. The impact of a magnetic field on dipolar oscillations modes was one of Pr. Michael J. Thompson's research topics during the 90s when preparing the helioseismic SoHO space mission. As the detection of gravity modes in the Sun is still controversial, the investigation of the solar oscillation modes did not provide any hint of the existence of a magnetic field in the solar radiative core. Today we have access to the core of evolved stars thanks to the asteroseismic observation of mixed modes from CoRoT, Kepler, K2 and TESS missions. The idea of applying and generalizing the work done for the Sun came from discussions with Pr. Michael Thompson in early 2018 before we loss him. Following the path we drew together, we theoretically investigate the effect of a stable axisymmetric mixed poloidal and toroidal magnetic field, aligned with the rotation axis of the star, on the mixed modes frequencies of a typical evolved low-mass star. This enables us to estimate the magnetic perturbations to the eigenfrequencies of mixed dipolar modes, depending on the magnetic field strength and the evolutionary state of the star. We conclude that strong magnetic fields of {$\sim$} 1MG should perturbe the mixed-mode frequency pattern enough for its effects to be detectable inside current asteroseismic data.},
  keywords = {notion,notion-database}
}

@article{Buldgen2016,
  title = {In-Depth Study of {{16CygB}} Using Inversion Techniques},
  author = {Buldgen, G. and Salmon, S. J.A.J. and Reese, D. R. and Dupret, M. A.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {596},
  issn = {14320746},
  doi = {10.1051/0004-6361/201628773},
  abstract = {Context. The 16Cyg binary system hosts the solar-like Kepler targets with the most stringent observational constraints. Indeed, we benefit from very high quality oscillation spectra, as well as spectroscopic and interferometric observations. Moreover, this system is particularly interesting since both stars are very similar in mass but the A component is orbited by a red dwarf, whereas the B component is orbited by a Jovian planet and thus could have formed a more complex planetary system. In our previous study, we showed that seismic inversions of integrated quantities could be used to constrain microscopic diffusion in the A component. In this study, we analyse the B component in the light of a more regularised inversion. Aims. We wish to analyse independently the B component of the 16Cyg binary system using the inversion of an indicator dedicated to analyse core conditions, denoted tu. Using this independent determination, we wish to analyse any differences between both stars due to the potential influence of planetary formation on stellar structure and/or their respective evolution. Methods. First, we recall the observational constraints for 16CygB and the method we used to generate reference stellar models of this star. We then describe how we improved the inversion and how this approach could be used for future targets with a sufficient number of observed frequencies. The inversion results were then used to analyse the differences between the A and B components. Results. The inversion of the tu indicator for 16CygB shows a disagreement with models including microscopic diffusion and sharing the chemical composition previously derived for 16CygA. We show that small changes in chemical composition are insufficient to solve the problem but that extra mixing can account for the differences seen between both stars. We use a parametric approach to analyse the impact of extra mixing in the form of turbulent diffusion on the behaviour of the tu values. We conclude on the necessity of further investigations using models with a physically motivated implementation of extra mixing processes including additional constraints to further improve the accuracy with which the fundamental parameters of this system are determined.},
  keywords = {Asteroseismology,notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WDG32UL8/Buldgen et al. - 2016.pdf}
}

@article{Buldgen2017,
  title = {Analysis of the Linear Approximation of Seismic Inversions for Various Structural Pairs},
  author = {Buldgen, G. and Reese, D. R. and Dupret, M. A.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {598},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629485},
  abstract = {Context. Thanks to the space-based photometry missions CoRoT and Kepler, we now benefit from a wealth of seismic data for stars other than the sun. In the future, K2, Tess, and Plato will complement this data and provide observations in addition to those already at hand. The availability of this data leads to questions on how it is feasible to extend kernel-based, linear structural inversion techniques to stars other than the sun. Linked to the inversion problem is the question of the validity of the linear assumption. In this study, we analyse the limitations of this assumption with respect to changes of structural variables. Aims. We wish to provide a more extended theoretical background to structural linear inversions by doing a study of the validity of the linear assumption for various structural variables. We thus point towards limitations in inversion techniques in the asteroseismic and helioseismic cases. Methods. First, we recall the origins of the linear assumption for structural stellar inversions and explain its importance for asteroseismic studies. We also briefly recall the impact of unknown structural quantities such as the mass and the radius of the star on structural inversion results. We then explain how kernels for new structural variables can be derived using two methods, one suited to asteroseismic targets, the other to helioseismic targets. For this second method, we present a new structural pair, namely the (A,Y) structural kernels. The kernels are then tested in various numerical experiments that enable us to evaluate the weaknesses of different structural pairs and the domains of validity of their respective linear regime. Results. The numerical tests we carry out allow us to disentangle the impact of various uncertainties in stellar models on the verification of the linear integral relations. We show the importance of metallicity, the impact of the equation of state, extra-mixing, and inaccuracies in the microphysics on the verification of these relations. We also discuss the limitations of the method of conjugated functions due to the lack of extremely precise determinations of masses or radii in the asteroseismic context.},
  keywords = {Asteroseismology,notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TLEDE68M/Buldgen, Reese, Dupret - 2017.pdf}
}

@article{Buldgen2019,
  title = {Progress in {{Global Helioseismology}}: {{A New Light}} on the {{Solar Modeling Problem}} and {{Its Implications}} for {{Solar-Like Stars}}},
  author = {Buldgen, Ga{\"e}l and Salmon, S{\'e}bastien and Noels, Arlette},
  year = {2019},
  month = jul,
  journal = {Frontiers in Astronomy and Space Sciences},
  volume = {6},
  pages = {42},
  publisher = {{Frontiers Media S.A.}},
  issn = {2296987X},
  doi = {10.3389/fspas.2019.00042},
  urldate = {2020-03-02},
  abstract = {Since the first observations of solar oscillations in 1960, helioseismology has probably been one of the most successful fields of astrophysics. Data of unprecedented quality were obtained through the implementation of networks of ground-based observatories such as the GONG project or the BiSON network, coupled with space-based telescopes such as SOHO and SDO missions and more data is expected from the Solar Orbiter mission. Besides the improvement of observational data, solar seismologists developed sophisticated techniques to infer the internal structure of the Sun from its eigenfrequencies. These methods, then already extensively used in the field of Geophysics, are called inversion techniques. They allowed to precisely determine the position of the solar convective envelope, the helium abundance in this region and the internal radial profiles of given thermodynamic quantities. Back in 1990s these comparisons showed a very high agreement between solar models and the Sun. However, the downward revision of the CNO surface abundances in the Sun in 2005, confirmed in 2009, induced a drastic reduction of this agreement leading to the so-called solar modeling problem. More than 10 years later, in the era of the space-based photometry missions which have established asteroseismology of solar-like stars as a standard approach to obtain their masses, radii and ages, the solar modeling problem still awaits a solution. In this paper, we will present the results of new helioseismic inversions, discuss the current uncertainties of solar models as well as some possible solutions to the solar modeling problem. We will show how helioseismology can help us grasp what is amiss in our solar models. We will also show that, far from being an argument about details of solar models, the solar problem has significant implications for seismology of solar-like stars, on the main sequence and beyond, impacting asteroseismology as a whole as well as the fields requiring precise and accurate knowledge of stellar masses, radii and ages, such as Galactic archaeology and exoplanetology.},
  keywords = {asteroseismology,helioseismology,notion,notion-database,solar abundances,solar-like stars,stellar structure and evolution,the Sun},
  file = {/Users/lbugnet/Zotero/storage/B84SF3NK/full-text.pdf}
}

@article{Burns2020,
  title = {Dedalus: {{A}} Flexible Framework for Numerical Simulations with Spectral Methods},
  author = {Burns, Keaton J. and Vasil, Geoffrey M. and Oishi, Jeffrey S. and Lecoanet, Daniel and Brown, Benjamin P.},
  year = {2020},
  month = apr,
  journal = {Physical Review Research},
  volume = {2},
  number = {2},
  pages = {023068},
  publisher = {{American Physical Society}},
  doi = {10.1103/PhysRevResearch.2.023068},
  urldate = {2021-10-15},
  abstract = {Numerical solutions of partial differential equations enable a broad range of scientific research. The Dedalus project is a flexible, open-source, parallelized computational framework for solving general partial differential equations using spectral methods. Dedalus translates plain-text strings describing partial differential equations into efficient solvers. This paper details the numerical method that enables this translation, describes the design and implementation of the codebase, and illustrates its capabilities with a variety of example problems. The numerical method is a first-order generalized tau formulation that discretizes equations into banded matrices. This method is implemented with an object-oriented design. Classes for spectral bases and domains manage the discretization and automatic parallel distribution of variables. Discretized fields and mathematical operators are symbolically manipulated with a basic computer algebra system. Initial value, boundary value, and eigenvalue problems are efficiently solved using high-performance linear algebra, transform, and parallel communication libraries. Custom analysis outputs can also be specified in plain text and stored in self-describing portable formats. The performance of the code is evaluated with a parallel scaling benchmark and a comparison to a finite-volume code. The features and flexibility of the codebase are illustrated by solving several examples: The nonlinear Schr\"odinger equation on a graph, a supersonic magnetohydrodynamic vortex, quasigeostrophic flow, Stokes flow in a cylindrical annulus, normal modes of a radiative atmosphere, and diamagnetic levitation.},
  keywords = {doi:10.1103/PhysRevResearch.2.023068 url:https://d,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JHFID9QL/full-text.pdf}
}

@article{Buysschaert2016,
  title = {Testing the Asymptotic Relation for Period Spacings from Mixed Modes of Red Giants Observed with the {{Kepler}} Mission},
  author = {Buysschaert, B. and Beck, P. G. and Corsaro, E. and {Christensen-Dalsgaard}, J. and Aerts, C. and Arentoft, T. and Kjeldsen, H. and Garc{\'i}a, R. A. and Silva Aguirre, V. and Degroote, P.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {588},
  pages = {1--14},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527055},
  abstract = {Context. Dipole mixed pulsation modes of consecutive radial order have been detected for thousands of low-mass red-giant stars with the NASA space telescope Kepler. These modes have the potential to reveal information on the physics of the deep stellar interior. Aims. Different methods have been proposed to derive an observed value for the gravity-mode period spacing, the most prominent one relying on a relation derived from asymptotic pulsation theory applied to the gravity-mode character of the mixed modes. Our aim is to compare results based on this asymptotic relation with those derived from an empirical approach for three pulsating red-giant stars. Methods. We developed a data-driven method to perform frequency extraction and mode identification. Next, we used the identified dipole mixed modes to determine the gravity-mode period spacing by means of an empirical method and by means of the asymptotic relation. In our methodology we consider the phase offset, g, of the asymptotic relation as a free parameter. Results. Using the frequencies of the identified dipole mixed modes for each star in the sample, we derived a value for the gravity-mode period spacing using the two different methods. These values differ by less than 5\%. The average precision we achieved for the period spacing derived from the asymptotic relation is better than 1\%, while that of our data-driven approach is 3\%. Conclusions. Good agreement is found between values for the period spacing derived from the asymptotic relation and from the empirical method. The achieved uncertainties are small, but do not support the ultra-high precision claimed in the literature. The precision from our data-driven method is mostly affected by the differing number of observed dipole mixed modes. For the asymptotic relation, the phase offset, g, remains ill defined, but enables a more robust analysis of both the asymptotic period spacing and the dimensionless coupling factor. However, its estimation might still offer a valuable observational diagnostic for future theoretical modeling.},
  keywords = {Asteroseismology,notion,notion-database,Stars: interiors,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/5JZVN6BU/Buysschaert et al. - 2016.pdf}
}

@article{Buysschaert2016a,
  title = {Testing the Asymptotic Relation for Period Spacings from Mixed Modes of Red Giants Observed with the {{{\emph{Kepler}}}} Mission},
  author = {Buysschaert, B. and Beck, P. G. and Corsaro, E. and {Christensen-Dalsgaard}, J. and Aerts, C. and Arentoft, T. and Kjeldsen, H. and Garc{\'i}a, R. A. and Silva Aguirre, V. and Degroote, P.},
  year = {2016},
  month = apr,
  journal = {Astronomy \& Astrophysics},
  volume = {588},
  pages = {A82},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201527055},
  urldate = {2023-09-27},
  abstract = {Methods. We developed a data-driven method to perform frequency extraction and mode identification. Next, we used the identified dipole mixed modes to determine the gravity-mode period spacing by means of an empirical method and by means of the asymptotic relation. In our methodology we consider the phase offset, g, of the asymptotic relation as a free parameter. Results. Using the frequencies of the identified dipole mixed modes for each star in the sample, we derived a value for the gravitymode period spacing using the two different methods. These values differ by less than 5\%. The average precision we achieved for the period spacing derived from the asymptotic relation is better than 1\%, while that of our data-driven approach is 3\%. Conclusions. Good agreement is found between values for the period spacing derived from the asymptotic relation and from the empirical method. The achieved uncertainties are small, but do not support the ultra-high precision claimed in the literature. The precision from our data-driven method is mostly affected by the differing number of observed dipole mixed modes. For the asymptotic relation, the phase offset, g, remains ill defined, but enables a more robust analysis of both the asymptotic period spacing and the dimensionless coupling factor. However, its estimation might still offer a valuable observational diagnostic for future theoretical modeling.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/C9993CSV/Buysschaert et al. - 2016 - Testing the asymptotic relation for period spacing.pdf}
}

@article{Buysschaert2017,
  title = {Magnetic Characterization of the {{SPB}}/\$\textbackslash mathbf\{\textbackslash beta\}\$ {{Cep}} Hybrid Pulsator {{HD}} 43317},
  author = {Buysschaert, B. and Neiner, C. and Briquet, M. and Aerts, C.},
  year = {2017},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {605},
  number = {A104},
  eprint = {1707.09148},
  doi = {10.1051/0004-6361/201731012},
  urldate = {2020-06-29},
  abstract = {Large-scale magnetic fields at the surface of massive stars do not only influence the outer-most layers of the star, but also have consequences for the deep interior, only observationally accessible through asteroseismology. We performed a detailed characterization of the dipolar magnetic field at the surface of the B3.5V star HD 43317, a SPB/\$\textbackslash beta\$ Cep hybrid pulsator, by studying the rotationally modulated magnetic field of archival and new Narval spectropolarimetry. Additionally, we employed a grid-based approach to compare the Zeeman signatures with model profiles. By studying the rotational modulation of the He lines in both the Narval and HARPS spectroscopy caused by co-rotating surface abundance inhomogeneities, we updated the rotation period to \$0.897673\textbackslash pm0.000004\$d. The inclination angle between the rotation axis and the observer's line of sight remains ill-defined, because of the low level of variability in Stokes V and deformations in the intensity profiles by stellar pulsation modes. The obliquity angle between the rotation and magnetic axes is constrained to \$\textbackslash beta \textbackslash in [67,90]\^\{\textbackslash circ\}\$, and the strength of the dipolar magnetic field is of the order of 1kG to 1.5kG. This magnetic field at the stellar surface is sufficiently strong to warrant a uniformly rotating radiative envelope, causing less convective core overshooting, which should be visible in future forward seismic modeling.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Buysschaert2018,
  title = {Forward Seismic Modelling of the Pulsating Magnetic {{B-type}} Star {{HD}} 43317},
  author = {Buysschaert, B. and Aerts, C. and Bowman, D. M. and Johnston, C. and Van Reeth, T. and Pedersen, M. G. and Mathis, S. and Neiner, C.},
  year = {2018},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {616},
  number = {A148},
  eprint = {1805.00802},
  doi = {10.1051/0004-6361/201832642},
  urldate = {2020-06-29},
  abstract = {The large-scale magnetic fields detected at the surface of about 10\% of hot stars extend into the stellar interior, where they may alter the structure. Deep inner regions of stars are only observable using asteroseismology. Here, we investigated the pulsating magnetic B3.5V star HD43317, inferred its interior properties and assessed whether the dipolar magnetic field with a surface strength of \$B\_p = 1312 \textbackslash pm 332\$G caused different properties compared to those of non-magnetic stars. We analysed the latest version of the star's 150d CoRoT light curve and extracted 35 significant frequencies, 28 of which were determined to be independent and not related to the known surface rotation period of \$P\_\{\textbackslash rm rot\} = 0.897673\$d. We performed forward seismic modelling based on non-magnetic, non-rotating 1D MESA models and the adiabatic module of the pulsation code GYRE, utilizing a grid-based approach. Our aim was to estimate the stellar mass, age, and convective core overshooting. The GYRE calculations were done for uniform rotation with \$P\_\{\textbackslash rm rot\}\$. This modelling was able to explain 16 of the 28 frequencies as gravity modes belonging to retrograde modes with \$(\textbackslash ell, m) = (1, -1)\$ and \$(2, -1)\$ period spacing patterns and one distinct prograde \$(2,2)\$ mode. The modelling resulted in a stellar mass \$M\_\{\textbackslash star\} = 5.8\^\{+0.1\}\_\{-0.2\}\$\$\textbackslash mathrm\{M\_\{\textbackslash odot\}\}\$, a central hydrogen mass fraction \$X\_c = 0.54\^\{+0.01\}\_\{-0.02\}\$, and exponential convective core overshooting parameter \$f\_\{\textbackslash rm ov\} = 0.004\^\{+0.014\}\_\{-0.002\}\$. The low value for \$f\_\{\textbackslash rm ov\}\$ is compatible with the suppression of near-core mixing due to a magnetic field but the uncertainties are too large to pinpoint such suppression as the sole physical interpretation. \$[...]\$},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YW3LKP5X/full-text.pdf}
}

@article{Buysschaert2018a,
  title = {Detection of Magnetic Fields in Chemically Peculiar Stars Observed with the {{K2}} Space Mission},
  author = {Buysschaert, B and Neiner, C and Martin, A J and Aerts, C and Bowman, D M and Oksala, M E and Van~Reeth, T},
  year = {2018},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {478},
  number = {2},
  pages = {2777--2793},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/sty1190},
  urldate = {2023-09-27},
  abstract = {We report the results of an observational study aimed at searching for magnetic pulsating hot stars suitable for magneto-asteroseismology. A sample of 16 chemically peculiar stars was selected and analysed using both high-resolution spectropolarimetry with ESPaDOnS and K2 high-precision space photometry. For all stars, we derive the effective temperature, surface gravity, rotational, and non-rotational line broadening from our spectropolarimetric data. High-quality K2 light curves were obtained for 13 of the 16 stars and revealed rotational modulation, providing accurate rotation periods. Two stars show evidence for roAp pulsations, and one star shows signatures of internal gravity waves or unresolved g-mode pulsations. We confirm the presence of a large-scale magnetic field for 11 of the studied stars, of which nine are first detections. Further, we report one marginal detection and four non-detections. Two of the stars with a non-detected magnetic field show rotational modulation due to surface abundance inhomogeneities in the K2 light curve, and we confirm that the other two are chemically peculiar. Thus, these five stars likely host a weak (undetected) large-scale magnetic field.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/IM9D65MC/Buysschaert et al. - 2018 - Detection of magnetic fields in chemically peculia.pdf}
}

@article{Buysschaert2018b,
  title = {Forward Seismic Modeling of the Pulsating Magnetic {{B-type}} Star {{HD}} 43317},
  author = {Buysschaert, B. and Aerts, C. and Bowman, D. M. and Johnston, C. and Van Reeth, T. and Pedersen, M. G. and Mathis, S. and Neiner, C.},
  year = {2018},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {616},
  pages = {A148},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201832642},
  urldate = {2023-09-28},
  abstract = {The large-scale magnetic fields detected at the surface of about 10\% of hot stars extend into the stellar interior, where they may alter the structure. Deep inner regions of stars are only observable using asteroseismology. Here, we investigate the pulsating magnetic B3.5V star HD 43317, infer its interior properties and assess whether the dipolar magnetic field with a surface strength of Bp = 1312 {$\pm$} 332 G causes different properties compared to those of non-magnetic stars. We analyze the latest version of the star's 150 d CoRoT light curve and extract 35 significant frequencies, 28 of which are found to be independent and not related to the known surface rotation period of Prot = 0.897673 d. We perform forward seismic modeling based on non-magnetic, non-rotating 1D MESA models and the adiabatic module of the pulsation code GYRE, using a grid-based approach. Our aim was to estimate the stellar mass, age, and convective core overshooting. The GYRE calculations were done for uniform rotation with Prot. This modeling is able to explain 16 of the 28 frequencies as gravity modes belonging to retrograde modes with ({$\mathscr{l}$}, m) = (1, -1) and (2, -1) period spacing patterns and one distinct prograde (2, +2) mode. The modeling resulted in a stellar mass M{$\star$} = 5.8-0.2+0.1 M{$\odot$}, a central hydrogen mass fraction Xc = 0.54-0.02+0.01, and exponential convective core overshooting parameter fov = 0.004-0.002+0.014. The low value for fov is compatible with the suppression of near-core mixing due to a magnetic field but the uncertainties are too large to pinpoint such suppression as the sole physical interpretation. We assess the frequency shifts of pulsation modes caused by the Lorentz and the Coriolis forces and find magnetism to have a lower impact than rotation for this star. Including magnetism in future pulsation computations would be highly relevant to exploit current and future photometric time series spanning at least one year, such as those assembled by the Kepler space telescope and expected from the TESS (Continuous Viewing Zone) and PLATO space missions.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: early-type,stars: individual: HD 43317,stars: magnetic field,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2018A\&A...616A.148B},
  file = {/Users/lbugnet/Zotero/storage/7C9HV369/Buysschaert et al. - 2018 - Forward seismic modeling of the pulsating magnetic.pdf}
}

@article{Buysschaert2019,
  title = {Magnetic Characterization and Variability Study of the Magnetic {{SPB}} Star {\emph{o}} {{Lupi}}},
  author = {Buysschaert, B. and Neiner, C. and Martin, A. J. and Oksala, M. E. and Aerts, C. and Tkachenko, A. and Alecian, E. and {the MiMeS Collaboration}},
  year = {2019},
  month = feb,
  journal = {Astronomy \& Astrophysics},
  volume = {622},
  pages = {A67},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201731913},
  urldate = {2023-09-27},
  abstract = {Thanks to large dedicated surveys, large-scale magnetic fields have been detected for about 10\% of early-type stars. We aim to precisely characterize the large-scale magnetic field of the magnetic component of the wide binary o Lupi, by using high-resolution ESPaDOnS and HARPSpol spectropolarimetry to analyze the variability of the measured longitudinal magnetic field. In addition, we have investigated the periodic variability using space-based photometry collected with the BRITE-Constellation by means of iterative prewhitening. The rotational variability of the longitudinal magnetic field indicates a rotation period Prot = 2.95333(2) d and that the large-scale magnetic field is dipolar, but with a significant quadrupolar contribution. Strong differences in the strength of the measured magnetic field occur for various chemical elements as well as rotational modulation for Fe and Si absorption lines, suggesting a inhomogeneous surface distribution of chemical elements. Estimates of the geometry of the large-scale magnetic field indicate i = 27 {$\pm$} 10{$\smwhtcircle$}, {$\beta$} = 74+-79{$\smwhtcircle$}, and a polar field strength of at least 5.25 kG. The BRITE photometry reveals the rotation frequency and several of its harmonics, as well as two gravity mode pulsation frequencies. The high-amplitude g-mode pulsation at f = 1.1057 d-1dominates the line-profile variability of the majority of the spectroscopic absorption lines. We do not find direct observational evidence of the secondary in the spectroscopy. Therefore, we attribute the pulsations and the large-scale magnetic field to the B5IV primary of the o Lupi system, but we discuss the implications should the secondary contribute to or cause the observed variability.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/H39BJ6EF/Buysschaert et al. - 2019 - Magnetic characterization and variability study of.pdf}
}

@article{Cacciani1978a,
  title = {The Magneto-Optical Filter},
  author = {Cacciani, A. and Fofi, M.},
  year = {1978},
  journal = {Solar Physics},
  volume = {59},
  number = {1},
  pages = {179--189},
  issn = {0038-0938},
  doi = {10.1007/bf00154941},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8HBF4FPX/Cacciani, Fofi - 1978.pdf}
}

@article{Caiazzo2023,
  title = {A Rotating White Dwarf Shows Different Compositions on Its Opposite Faces},
  author = {Caiazzo, Ilaria and Burdge, Kevin B. and Tremblay, Pier-Emmanuel and Fuller, James and Ferrario, Lilia and G{\"a}nsicke, Boris T. and Hermes, J. J. and Heyl, Jeremy and Kawka, Adela and Kulkarni, S. R. and Marsh, Thomas R. and Mr{\'o}z, Przemek and Prince, Thomas A. and Richer, Harvey B. and Rodriguez, Antonio C. and {van Roestel}, Jan and Vanderbosch, Zachary P. and Vennes, St{\'e}phane and Wickramasinghe, Dayal and Dhillon, Vikram S. and Littlefair, Stuart P. and Munday, James and Pelisoli, Ingrid and Perley, Daniel and Bellm, Eric C. and Breedt, Elm{\'e} and Brown, Alex J. and Dekany, Richard and Drake, Andrew and Dyer, Martin J. and Graham, Matthew J. and Green, Matthew J. and Laher, Russ R. and Kerry, Paul and Parsons, Steven G. and Riddle, Reed L. and Rusholme, Ben and Sahman, Dave I.},
  year = {2023},
  month = aug,
  journal = {Nature},
  volume = {620},
  pages = {61--66},
  issn = {0028-0836},
  doi = {10.1038/s41586-023-06171-9},
  urldate = {2023-09-22},
  abstract = {White dwarfs, the extremely dense remnants left behind by most stars after their death, are characterized by a mass comparable to that of the Sun compressed into the size of an Earth-like planet. In the resulting strong gravity, heavy elements sink towards the centre and the upper layer of the atmosphere contains only the lightest element present, usually hydrogen or helium1,2. Several mechanisms compete with gravitational settling to change a white dwarf's surface composition as it cools3, and the fraction of white dwarfs with helium atmospheres is known to increase by a factor of about 2.5 below a temperature of about 30,000 kelvin4-8; therefore, some white dwarfs that appear to have hydrogen-dominated atmospheres above 30,000 kelvin are bound to transition to be helium-dominated as they cool below it. Here we report observations of ZTF J203349.8+322901.1, a transitioning white dwarf with two faces: one side of its atmosphere is dominated by hydrogen and the other one by helium. This peculiar nature is probably caused by the presence of a small magnetic field, which creates an inhomogeneity in temperature, pressure or mixing strength over the surface9-11. ZTF J203349.8+322901.1 might be the most extreme member of a class of magnetic, transitioning white dwarfs\textemdash together with GD 323 (ref. 12), a white dwarf that shows similar but much more subtle variations. This class of white dwarfs could help shed light on the physical mechanisms behind the spectral evolution of white dwarfs.},
  keywords = {Astrophysics - Earth and Planetary Astrophysics,Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2023Natur.620...61C},
  file = {/Users/lbugnet/Zotero/storage/T642WJ6Z/Caiazzo et al. - 2023 - A rotating white dwarf shows different composition.pdf}
}

@article{caiazzoIntermediateMassStarsBecome2020,
  title = {Intermediate-{{Mass}} Stars Become Magnetic White Dwarfs},
  author = {Caiazzo, Ilaria and Heyl, Jeremy and Richer, Harvey and Cummings, Jeffrey and Fleury, Leesa and Hegarty, James and Kalirai, Jason and Kerr, Ronan and Thiele, Sarah and Tremblay, Pier Emmanuel and Villanueva, Michael},
  year = {2020},
  month = sep,
  journal = {arXiv},
  volume = {901},
  number = {1},
  eprint = {2009.03374},
  pages = {L14},
  publisher = {{arXiv}},
  issn = {23318422},
  doi = {10.3847/2041-8213/abb5f7},
  urldate = {2021-02-24},
  abstract = {When a star exhausts its nuclear fuel, it either explodes as a supernova or more quiescently becomes a white dwarf, an object about half the mass of our Sun with a radius of about that of the Earth. About one fifth of white dwarfs exhibit the presence of magnetic fields, whose origin has long been debated as either the product of previous stages of evolution or of binary interactions. We here report the discovery of two massive and magnetic white dwarf members of young star clusters in the Gaia DR2 database, while a third massive and magnetic cluster white dwarf was already reported in a previous paper. These stars are most likely the product of single-star evolution and therefore challenge the merger scenario as the only way to produce magnetic white dwarfs. The progenitor masses of these stars are all above 5 solar masses, and there are only two other cluster white dwarfs whose distances have been unambiguously measured with Gaia and whose progenitors' masses fall in this range. This high incidence of magnetic white dwarfs indicates that intermediate-mass progenitors are more likely to produce magnetic remnants and that a fraction of magnetic white dwarfs forms from intermediate-mass stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Calcaferro2023,
  title = {Exploring the Internal Rotation of the Extremely Low-Mass {{He-core}} White Dwarf {{GD}} 278 with {{TESS}} Asteroseismology},
  author = {Calcaferro, Leila M. and C{\'o}rsico, Alejandro H. and Althaus, Leandro G. and Lopez, Isaac D. and Hermes, J. J.},
  year = {2023},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {673},
  pages = {A135},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202346007},
  urldate = {2023-10-02},
  abstract = {Context. The advent of high-quality space-based photometry, brought about by missions such as Kepler/K2 and TESS, makes it possible to unveil the fundamental parameters and properties of the interiors of white dwarf stars, particularly extremely low-mass white dwarfs, using the tools of asteroseismology. Aims: We present an exploration of the internal rotation of GD 278, the first known pulsating extremely low-mass white dwarf to show rotational splittings within its periodogram. Methods: We assessed the theoretical frequency splittings expected for different rotation profiles and compared them to the observed frequency splittings of GD 278. To this aim, we employed an asteroseismological model representative of the pulsations of this star, obtained by using the LPCODE stellar evolution code and the LP-PUL non-radial pulsation code. We also derived a rotation profile that results from detailed evolutionary calculations carried out with the MESA stellar evolution code and used it to infer the expected theoretical frequency splittings. Results: We find that the best-fitting solution when assuming linear profiles for the rotation of GD 278 leads to angular velocity values at the surface and center that are only slightly differential, and still compatible with rigid rotation. Additionally, the values of the angular velocity at the surface and the center for the simple linear rotation profiles and for the rotation profile derived from evolutionary calculations are in very good agreement. Also, the resulting theoretical frequency splittings are compatible with the observed frequency splittings, in general, for both cases. Conclusions: The results obtained from the different approaches followed in this work to derive the internal rotation of GD 278 agree. The fact that they were obtained by employing two independent stellar evolution codes gives our results robustness. Our results suggest only a marginally differential behavior for the internal rotation in GD 278 and, considering the uncertainties involved, this is very compatible with the rigid case, as has been observed previously for white dwarfs and pre-white dwarfs. The rotation periods derived for this star are also in line with the values determined asteroseismologically for white dwarfs and pre-white dwarfs in general.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: individual: GD 278,stars: interiors,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2023A\&A...673A.135C},
  file = {/Users/lbugnet/Zotero/storage/2JMNZXU7/Calcaferro et al. - 2023 - Exploring the internal rotation of the extremely l.pdf}
}

@article{Calcaferro2023a,
  title = {Exploring the Internal Rotation of the Extremely Low-Mass {{He-core}} White Dwarf {{GD}} 278 with {{TESS}} Asteroseismology},
  author = {Calcaferro, Leila M. and C{\'o}rsico, Alejandro H. and Althaus, Leandro G. and Lopez, Isaac D. and Hermes, J. J.},
  year = {2023},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {673},
  pages = {A135},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202346007},
  urldate = {2023-10-14},
  abstract = {Context. The advent of high-quality space-based photometry, brought about by missions such as Kepler/K2 and TESS, makes it possible to unveil the fundamental parameters and properties of the interiors of white dwarf stars, particularly extremely low-mass white dwarfs, using the tools of asteroseismology. Aims: We present an exploration of the internal rotation of GD 278, the first known pulsating extremely low-mass white dwarf to show rotational splittings within its periodogram. Methods: We assessed the theoretical frequency splittings expected for different rotation profiles and compared them to the observed frequency splittings of GD 278. To this aim, we employed an asteroseismological model representative of the pulsations of this star, obtained by using the LPCODE stellar evolution code and the LP-PUL non-radial pulsation code. We also derived a rotation profile that results from detailed evolutionary calculations carried out with the MESA stellar evolution code and used it to infer the expected theoretical frequency splittings. Results: We find that the best-fitting solution when assuming linear profiles for the rotation of GD 278 leads to angular velocity values at the surface and center that are only slightly differential, and still compatible with rigid rotation. Additionally, the values of the angular velocity at the surface and the center for the simple linear rotation profiles and for the rotation profile derived from evolutionary calculations are in very good agreement. Also, the resulting theoretical frequency splittings are compatible with the observed frequency splittings, in general, for both cases. Conclusions: The results obtained from the different approaches followed in this work to derive the internal rotation of GD 278 agree. The fact that they were obtained by employing two independent stellar evolution codes gives our results robustness. Our results suggest only a marginally differential behavior for the internal rotation in GD 278 and, considering the uncertainties involved, this is very compatible with the rigid case, as has been observed previously for white dwarfs and pre-white dwarfs. The rotation periods derived for this star are also in line with the values determined asteroseismologically for white dwarfs and pre-white dwarfs in general.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: individual: GD 278,stars: interiors,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2023A\&A...673A.135C},
  file = {/Users/lbugnet/Zotero/storage/JE46JY7J/Calcaferro et al. - 2023 - Exploring the internal rotation of the extremely l.pdf}
}

@article{Calcaferro2023b,
  title = {Exploring the Internal Rotation of the Extremely Low-Mass {{He-core}} White Dwarf {{GD}} 278 with {{TESS}} Asteroseismology},
  author = {Calcaferro, Leila M. and C{\'o}rsico, Alejandro H. and Althaus, Leandro G. and Lopez, Isaac D. and Hermes, J. J.},
  year = {2023},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {673},
  pages = {A135},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202346007},
  urldate = {2023-10-14},
  abstract = {Context. The advent of high-quality space-based photometry, brought about by missions such as Kepler/K2 and TESS, makes it possible to unveil the fundamental parameters and properties of the interiors of white dwarf stars, particularly extremely low-mass white dwarfs, using the tools of asteroseismology. Aims: We present an exploration of the internal rotation of GD 278, the first known pulsating extremely low-mass white dwarf to show rotational splittings within its periodogram. Methods: We assessed the theoretical frequency splittings expected for different rotation profiles and compared them to the observed frequency splittings of GD 278. To this aim, we employed an asteroseismological model representative of the pulsations of this star, obtained by using the LPCODE stellar evolution code and the LP-PUL non-radial pulsation code. We also derived a rotation profile that results from detailed evolutionary calculations carried out with the MESA stellar evolution code and used it to infer the expected theoretical frequency splittings. Results: We find that the best-fitting solution when assuming linear profiles for the rotation of GD 278 leads to angular velocity values at the surface and center that are only slightly differential, and still compatible with rigid rotation. Additionally, the values of the angular velocity at the surface and the center for the simple linear rotation profiles and for the rotation profile derived from evolutionary calculations are in very good agreement. Also, the resulting theoretical frequency splittings are compatible with the observed frequency splittings, in general, for both cases. Conclusions: The results obtained from the different approaches followed in this work to derive the internal rotation of GD 278 agree. The fact that they were obtained by employing two independent stellar evolution codes gives our results robustness. Our results suggest only a marginally differential behavior for the internal rotation in GD 278 and, considering the uncertainties involved, this is very compatible with the rigid case, as has been observed previously for white dwarfs and pre-white dwarfs. The rotation periods derived for this star are also in line with the values determined asteroseismologically for white dwarfs and pre-white dwarfs in general.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: individual: GD 278,stars: interiors,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2023A\&A...673A.135C}
}

@article{Cameron2007,
  title = {Differential Rotation on Rapidly Rotating Stars},
  author = {Cameron, A. Collier},
  year = {2007},
  journal = {Astronomische Nachrichten},
  volume = {328},
  number = {10},
  pages = {1030--1033},
  issn = {00046337},
  doi = {10.1002/asna.200710880},
  abstract = {Theories of meridional circulation and differential rotation in stellar convective zones predict trends in surface flow patterns on main-sequence stars that are amenable to direct observational testing. Here I summarise progress made in the last few years in determining surface differential rotation patterns on rapidly-rotating young main-sequence stars of spectral types F, G, K and M. Differential rotation increases strongly with increasing effective temperature along the main sequence. The shear rate appears to increase with depth in the sub-photospheric layers. Tidal locking in close binaries appears to suppress differential rotation, but better statistics are needed before this conclusion can be trusted. \textcopyright{} 2007 WILEY-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {notion,notion-database,Stars: activity,Stars: imaging,Stars: rotation,Starspots},
  file = {/Users/lbugnet/Zotero/storage/2FJ9Y4MI/Cameron - 2007.pdf}
}

@article{Campante2010,
  title = {Modelling the Autocovariance of the Power Spectrum of a Solar-Type Oscillator},
  author = {Campante, T. L. and Karoff, C. and Chaplin, W. J. and Elsworth, Y. P. and Handberg, R. and Hekker, S.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {408},
  number = {1},
  pages = {542--550},
  issn = {0035-8711},
  doi = {10.1111/j.1365-2966.2010.17141.x},
  abstract = {Asteroseismology is able to conduct studies on the interiors of solar-type stars from the analysis of stellar acoustic spectra. However, such an analysis process often has to rely upon subjective choices made throughout. A recurring problem is to determine whether a signal in the acoustic spectrum originates from a radial or a dipolar oscillation mode. In order to overcome this problem, we present a procedure for modelling and fitting the autocovariance of the power spectrum which can be used to obtain global seismic parameters of solar-type stars, doing so in an automated fashion without the need to make subjective choices. From the set of retrievable global seismic parameters we emphasize the mean small frequency separation and, depending on the intrinsic characteristics of the power spectrum, the mean rotational frequency splitting. Since this procedure is automated, it can serve as a useful tool in the analysis of the more than one thousand solar-type stars expected to be observed as part of the Kepler Asteroseismic Investigation (KAI). We apply the aforementioned procedure to simulations of the Sun. Assuming different apparent magnitudes, we address the issues of how accurately and how precisely we can retrieve the several global seismic parameters were the Sun to be observed as part of the KAI.},
  keywords = {1 i n t,and evolution,data analysis,is a powerful tool,methods,notion,notion-database,oscillations,ro d u c,seismology of solar-type oscillators,stars,statistical,t i o n,that can be,understanding of stellar structure,used to increase our},
  file = {/Users/lbugnet/Zotero/storage/PRXFZZDS/Campante et al. - 2010.pdf}
}

@article{Campante2011,
  title = {Asteroseismology from Multi-Month Kepler Photometry: {{The}} Evolved Sun-like Stars {{KIC}} 10273246 and {{KIC}} 10920273},
  author = {Campante, T. L. and Handberg, R. and Mathur, S. and Appourchaux, T. and Bedding, T. R. and Chaplin, W. J. and Garc{\'i}a, R. A. and Mosser, B. and Benomar, O. and Bonanno, A. and Corsaro, E. and Fletcher, S. T. and Gaulme, P. and Hekker, S. and Karoff, C. and R{\'e}gulo, C. and Salabert, D. and Verner, G. A. and White, T. R. and Houdek, G. and Brand{\~a}o, I. M. and Creevey, O. L. and Do{\^g}an, G. and Bazot, M. and {Christensen-Dalsgaard}, J. and Cunha, M. S. and Elsworth, Y. and Huber, D. and Kjeldsen, H. and Lundkvist, M. and {Molenda-Zakowicz}, J. and Monteiro, M. J.P.F.G. and Stello, D. and Clarke, B. D. and Girouard, F. R. and Hall, J. R.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {534},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116620},
  abstract = {Context. The evolved main-sequence Sun-like stars KIC 10273246 (F-type) and KIC 10920273 (G-type) were observed with the NASA Kepler satellite for approximately ten months with a duty cycle in excess of 90\%. Such continuous and long observations are unprecedented for solar-type stars other than the Sun. Aims. We aimed mainly at extracting estimates of p-mode frequencies-as well as of other individual mode parameters-from the power spectra of the light curves of both stars, thus providing scope for a full seismic characterization. Methods. The light curves were corrected for instrumental effects in a manner independent of the Kepler science pipeline. Estimation of individual mode parameters was based both on the maximization of the likelihood of a model describing the power spectrum and on a classic prewhitening method. Finally, we employed a procedure for selecting frequency lists to be used in stellar modeling. Results. A total of 30 and 21 modes of degree l = 0,1,2-spanning at least eight radial orders-have been identified for KIC 10273246 and KIC 10920273, respectively. Two avoided crossings (l = 1 ridge) have been identified for KIC 10273246, whereas one avoided crossing plus another likely one have been identified for KIC 10920273. Good agreement is found between observed and predicted mode amplitudes for the F-type star KIC 10273246, based on a revised scaling relation. Estimates are given of the rotational periods, the parameters describing stellar granulation and the global asteroseismic parameters {$\Delta\nu$} and {$\nu$}max. \textcopyright{} 2011 ESO.},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,stars: individual: KIC 10273246,stars: individual: KIC 10920273,stars: oscillations,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/7PZSJNRC/Campante et al. - 2011.pdf}
}

@article{Campante2014,
  title = {Limits on Surface Gravities of Kepler Planet-Candidate Host Stars from Non-Detection of Solar-like Oscillations},
  author = {Campante, T. L. and Chaplin, W. J. and Lund, M. N. and Huber, D. and Hekker, S. and Garc{\'i}a, R. A. and Corsaro, E. and Handberg, R. and Miglio, A. and Arentoft, T. and Basu, S. and Bedding, T. R. and {Christensen-Dalsgaard}, J. and Davies, G. R. and Elsworth, Y. P. and Gilliland, R. L. and Karoff, C. and Kawaler, S. D. and Kjeldsen, H. and Lundkvist, M. and Metcalfe, T. S. and Silva Aguirre, V. and Stello, D.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {783},
  number = {2},
  eprint = {1401.6324},
  issn = {15384357},
  doi = {10.1088/0004-637X/783/2/123},
  abstract = {We present a novel method for estimating lower-limit surface gravities (log g) of Kepler targets whose data do not allow the detection of solar-like oscillations. The method is tested using an ensemble of solar-type stars observed in the context of the Kepler Asteroseismic Science Consortium. We then proceed to estimate lower-limit log g for a cohort of Kepler solar-type planet-candidate host stars with no detected oscillations. Limits on fundamental stellar properties, as provided by this work, are likely to be useful in the characterization of the corresponding candidate planetary systems. Furthermore, an important byproduct of the current work is the confirmation that amplitudes of solar-like oscillations are suppressed in stars with increased levels of surface magnetic activity. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {methods: statistical,notion,notion-database,planetary systems,stars: late-type,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/8TNM59KG/Campante et al. - 2014.pdf}
}

@article{Campante2015,
  title = {An Ancient Extrasolar System with Five Sub-Earth-Size Planets},
  author = {Campante, T. L. and Barclay, T. and Swift, J. J. and Huber, D. and Adibekyan, V. Zh and Cochran, W. and Burke, C. J. and Isaacson, H. and Quintana, E. V. and Davies, G. R. and Aguirre, V. Silva and Ragozzine, D. and Riddle, R. and Baranec, C. and Basu, S. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Metcalfe, T. S. and Bedding, T. R. and Handberg, R. and Stello, D. and Brewer, J. M. and Hekker, S. and Karoff, C. and Kolbl, R. and Law, N. M. and Lundkvist, M. and Miglio, A. and Rowe, J. F. and Santos, N. C. and Van Laerhoven, C. and Arentoft, T. and Elsworth, Y. P. and Fischer, D. A. and Kawaler, S. D. and Kjeldsen, H. and Lund, M. N. and Marcy, G. W. and Sousa, S. G. and Sozzetti, A. and White, T. R.},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {799},
  number = {2},
  eprint = {1501.06227},
  issn = {15384357},
  doi = {10.1088/0004-637X/799/2/170},
  abstract = {The chemical composition of stars hosting small exoplanets (with radii less than four Earth radii) appears to be more diverse than that of gas-giant hosts, which tend to be metal-rich. This implies that small, including Earth-size, planetsmay have readily formed at earlier epochs in the universe's history when metals were more scarce.We report Kepler spacecraft observations of Kepler-444, a metal-poor Sun-like star from the old population of the Galactic thick disk and the host to a compact system of five transiting planets with sizes between those of Mercury and Venus. We validate this system as a true five-planet system orbiting the target star and provide a detailed characterization of its planetary and orbital parameters based on an analysis of the transit photometry. Kepler-444 is the densest star with detected solar-like oscillations. We use asteroseismology to directly measure a precise age of 11.2 {$\pm$} 1.0 Gyr for the host star, indicating that Kepler-444 formed when the universe was less than 20\% of its current age and making it the oldest known system of terrestrial-size planets. We thus show that Earth-size planets have formed throughout most of the universe's 13.8 billion year history, leaving open the possibility for the existence of ancient life in the Galaxy. The age of Kepler-444 not only suggests that thick-disk stars were among the hosts to the first Galactic planets, but may also help to pinpoint the beginning of the era of planet formation.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: disk,notion,notion-database,Planetary systems,Stars: individual (HIP 94931),Stars: late-type,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/UEXANNGV/Campante et al. - 2015.pdf}
}

@article{Campante2016,
  title = {Spin\textendash{{Orbit Alignment}} of {{Exoplanet Systems}}: {{Ensemble Analysis Using Asteroseismology}}},
  author = {Campante, T. L. and Lund, M. N. and Kuszlewicz, J. S. and Davies, G. R. and Chaplin, W. J. and Albrecht, S. and Winn, J. N. and Bedding, T. R. and Benomar, O. and Bossini, D. and Handberg, R. and Santos, A. R. G. and Van Eylen, V. and Basu, S. and {Christensen-Dalsgaard}, J. and Elsworth, Y. P. and Hekker, S. and Hirano, T. and Huber, D. and Karoff, C. and Kjeldsen, H. and Lundkvist, M. S. and North, T. S. H. and Silva Aguirre, V. and Stello, D. and White, T. R.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {819},
  number = {1},
  eprint = {1601.06052},
  pages = {85},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/819/1/85},
  abstract = {The angle \$\textbackslash psi\$ between a planet's orbital axis and the spin axis of its parent star is an important diagnostic of planet formation, migration, and tidal evolution. We seek empirical constraints on \$\textbackslash psi\$ by measuring the stellar inclination \$i\_\{\textbackslash rm s\}\$ via asteroseismology for an ensemble of 25 solar-type hosts observed with NASA's Kepler satellite. Our results for \$i\_\{\textbackslash rm s\}\$ are consistent with alignment at the 2-\$\textbackslash sigma\$ level for all stars in the sample, meaning that the system surrounding the red-giant star Kepler-56 remains as the only unambiguous misaligned multiple-planet system detected to date. The availability of a measurement of the projected spin-orbit angle \$\textbackslash lambda\$ for two of the systems allows us to estimate \$\textbackslash psi\$. We find that the orbit of the hot-Jupiter HAT-P-7b is likely to be retrograde (\$\textbackslash psi=116.4\^\{+30.2\}\_\{-14.7\}\textbackslash :\{\textbackslash rm deg\}\$), whereas that of Kepler-25c seems to be well aligned with the stellar spin axis (\$\textbackslash psi=12.6\^\{+6.7\}\_\{-11.0\}\textbackslash :\{\textbackslash rm deg\}\$). While the latter result is in apparent contradiction with a statement made previously in the literature that the multi-transiting system Kepler-25 is misaligned, we show that the results are consistent, given the large associated uncertainties. Finally, we perform a hierarchical Bayesian analysis based on the asteroseismic sample in order to recover the underlying distribution of \$\textbackslash psi\$. The ensemble analysis suggests that the directions of the stellar spin and planetary orbital axes are correlated, as conveyed by a tendency of the host stars to display large inclination values.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,general,methods,methods: statistical,notion,notion-database,photometric,planetary systems,planets and satellites,planets and satellites: general,solar-type,stars,stars: solar-type,statistical,techniques,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/LWS4P7GL/Campante et al. - 2016.pdf}
}

@article{Campante2016a,
  title = {The {{Asteroseismic Potential}} of {{Tess}} : {{Exoplanet-Host Stars}}},
  author = {Campante, T. L. and Schofield, M. and Kuszlewicz, J. S. and Bouma, L. and Chaplin, W. J. and Huber, D. and {Christensen-Dalsgaard}, J. and Kjeldsen, H. and Bossini, D. and North, T. S. H. and Appourchaux, T. and Latham, D. W. and Pepper, J. and Ricker, G. R. and Stassun, K. G. and Vanderspek, R. and Winn, J. N.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {830},
  number = {2},
  eprint = {1608.01138},
  pages = {138},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/830/2/138},
  abstract = {New insights on stellar evolution and stellar interiors physics are being made possible by asteroseismology. Throughout the course of the Kepler mission, asteroseismology has also played an important role in the characterization of exoplanet-host stars and their planetary systems. The upcoming NASA Transiting Exoplanet Survey Satellite (TESS) will be performing a near all-sky survey for planets that transit bright nearby stars. In addition, its excellent photometric precision, combined with its fine time sampling and long intervals of uninterrupted observations, will enable asteroseismology of solar-type and red-giant stars. Here we develop a simple test to estimate the detectability of solar-like oscillations in TESS photometry of any given star. Based on an all-sky stellar and planetary synthetic population, we go on to predict the asteroseismic yield of the TESS mission, placing emphasis on the yield of exoplanet-host stars for which we expect to detect solar-like oscillations. This is done for both the target stars (observed at a 2-min cadence) and the full-frame-image stars (observed at a 30-min cadence). A similar exercise is also conducted based on a compilation of known host stars. We predict that TESS will detect solar-like oscillations in a few dozen target hosts (mainly subgiant stars but also in a smaller number of F dwarfs), in up to 200 low-luminosity red-giant hosts, and in over 100 solar-type and red-giant known hosts, thereby leading to a threefold improvement in the asteroseismic yield of exoplanet-host stars when compared to Kepler's.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,detection,instruments,notion,notion-database,photometric,planets and satellites,space vehicles,surveys,techniques},
  file = {/Users/lbugnet/Zotero/storage/DHNHGNE7/Campante et al. - 2016(2).pdf}
}

@article{Campbell1900,
  title = {A List of Nine Stars Whose Velocities in the Line of Sight Are Variable.},
  author = {Campbell, W. W. and Wright, W. H.},
  year = {1900},
  month = nov,
  journal = {The Astrophysical Journal},
  volume = {12},
  pages = {254},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/140765},
  urldate = {2020-03-07},
  keywords = {notion,notion-database}
}

@article{Campbell1986,
  title = {Stellar Oscillations in the Presence of a Magnetic Field},
  author = {Campbell, C. G. and Papaloizou, J. C. B.},
  year = {1986},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {220},
  number = {3},
  pages = {577--591},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/220.3.577},
  urldate = {2020-08-10},
  keywords = {A Stars,Astrophysics,Boundary Value Problems,Magnetic Stars,Magnetohydrodynamic Waves,notion,notion-database,Propagation Modes,Stellar Magnetic Fields,Stellar Models,Stellar Oscillations,Wave Propagation},
  file = {/Users/lbugnet/Zotero/storage/3C52GAYS/full-text.pdf}
}

@article{Cantiello2002a,
  title = {Rotation and {{Asteroseismology}} : {{SPIDER Network}}},
  author = {Cantiello, Matteo and Mankovich, Chris and Bildsten, Lars and Paxton, Bill and Fuller, Jim and Lecoanet, Daniel and Brown, Ben},
  year = {2002},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2SI7F4KK/Cantiello et al. - 2002.pdf}
}

@article{Cantiello2014a,
  title = {Angular Momentum Transport within Evolved Low-Mass Stars},
  author = {Cantiello, Matteo and Mankovich, Christopher and Bildsten, Lars and {Christensen-Dalsgaard}, J{\o}rgen and Paxton, Bill},
  year = {2014},
  journal = {The Astrophysical Journal},
  volume = {788},
  number = {1},
  pages = {1--7},
  issn = {15384357},
  doi = {10.1088/0004-637X/788/1/93},
  abstract = {Asteroseismology of 1.0-2.0 M red giants by the Kepler satellite has enabled the first definitive measurements of interior rotation in both first ascent red giant branch (RGB) stars and those on the helium burning clump. The inferred rotation rates are 10-30 days for the 0.2 M He degenerate cores on the RGB and 30-100 days for the He burning core in a clump star. Using the Modules for Experiments in Stellar Evolution code, we calculate state-of-the-art stellar evolution models of low mass rotating stars from the zero-age main sequence to the cooling white dwarf (WD) stage. We include transport of angular momentum due to rotationally induced instabilities and circulations, as well as magnetic fields in radiative zones (generated by the Tayler-Spruit dynamo). We find that all models fail to predict core rotation as slow as observed on the RGB and during core He burning, implying that an unmodeled angular momentum transport process must be operating on the early RGB of low mass stars. Later evolution of the star from the He burning clump to the cooling WD phase appears to be at nearly constant core angular momentum. We also incorporate the adiabatic pulsation code, ADIPLS, to explicitly highlight this shortfall when applied to a specific Kepler asteroseismic target, KIC8366239. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  keywords = {asteroseismology,methods: numerical,notion,notion-database,stars: evolution,stars: interiors,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/T7NRAJG3/Cantiello et al. - 2014.pdf}
}

@article{Cantiello2016,
  title = {Asteroseismic {{Signatures}} of {{Evolving Internal Stellar Magnetic Fields}}},
  author = {Cantiello, Matteo and Fuller, Jim and Bildsten, Lars},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {824},
  number = {1},
  pages = {14},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/824/1/14},
  abstract = {Recent asteroseismic analyses have revealed the presence of strong (B 10 5 G) magnetic fields in the cores of many red giant stars. Here, we examine the implications of these results for the evolution of stellar magnetic fields, and we make predictions for future observations. Those stars with suppressed dipole modes indicative of strong core fields should exhibit moderate but detectable quadrupole mode suppression. The long magnetic diffusion times within stellar cores ensure that dynamo-generated fields are confined to mass coordinates within the main sequence convective core, and the observed sharp increase in dipole mode suppression rates above 1.5 M may be explained by the larger convective core masses and faster rotation of these more massive stars. In clump stars, core fields of {$\sim$} 10 5 G can suppress dipole modes, whose visibility should be equal to or less than the visibility of suppressed modes in ascending red giants. High dipole mode suppression rates in low-mass (M 2 M) clump stars would indicate that magnetic fields generated during the main sequence can withstand subsequent convective phases and survive into the compact remnant phase. Finally, we discuss implications for observed magnetic fields in white dwarfs and neutron stars, as well as the effects of magnetic fields in various types of pulsating stars.},
  keywords = {asteroseismology,evolution,interiors,magnetic fi eld,notion,notion-database,oscillations,stars,stars: evolution,stars: interiors,stars: magnetic field,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4C7RUPGA/Cantiello, Fuller, Bildsten - 2016.pdf}
}

@article{Cao2023,
  title = {Core-Envelope {{Decoupling Drives Radial Shear Dynamos}} in {{Cool Stars}}},
  author = {Cao, Lyra and Pinsonneault, Marc H. and {van Saders}, Jennifer L.},
  year = {2023},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {951},
  pages = {L49},
  issn = {0004-637X},
  doi = {10.3847/2041-8213/acd780},
  urldate = {2023-10-18},
  abstract = {Differential rotation is thought to be responsible for the dynamo process in stars like our Sun, driving magnetic activity and starspots. We report that starspot measurements in the Praesepe open cluster are strongly enhanced only for stars that depart from standard models of rotational evolution. A decoupling of the spin-down history between the core and envelope explains both the activity and rotation anomalies: surface rotational evolution is stalled by interior angular momentum redistribution, and the resultant radial shears enhance starspot activity. These anomalies provide evidence for an evolving front of shear-enhanced activity affecting the magnetic and rotational evolution of cool stars and the high-energy environments of their planetary companions for hundreds of millions to billions of years on the main sequence.},
  keywords = {1572,1580,1599,1610,1629,Astrophysics - Solar and Stellar Astrophysics,Starspots,Stellar activity,Stellar evolution,Stellar magnetic fields,Stellar rotation},
  annotation = {ADS Bibcode: 2023ApJ...951L..49C},
  file = {/Users/lbugnet/Zotero/storage/TK9BK8S9/Cao et al. - 2023 - Core-envelope Decoupling Drives Radial Shear Dynam.pdf}
}

@article{Carlberg2009,
  title = {The {{Role}} of {{Planet Accretion}} in {{Creating}} the {{Next Generation}} of {{Red Giant Rapid Rotators}}},
  author = {Carlberg, Joleen K. and Majewski, Steven R. and Arras, Phil},
  year = {2009},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {700},
  number = {1},
  eprint = {0906.1587},
  pages = {832--843},
  doi = {10.1088/0004-637X/700/1/832},
  urldate = {2020-07-13},
  abstract = {Rapid rotation in field red giant stars is a relatively rare but well-studied phenomenon; here we investigate the potential role of planet accretion in spinning up these stars. Using Zahn's theory of tidal friction and stellar evolution models, we compute the decay of a planet's orbit into its evolving host star and the resulting transfer of angular momentum into the stellar convective envelope. This experiment assesses the frequency of planet ingestion and rapid rotation on the red giant branch (RGB) for a sample of 99 known exoplanet host stars. We find that the known exoplanets are indeed capable of creating rapid rotators; however, the expected fraction due to planet ingestion is only \textasciitilde 10\% of the total seen in surveys of present-day red giants. Of the planets ingested, we find that those with smaller initial semimajor axes are more likely to create rapid rotators because these planets are accreted when the stellar moment of inertia is smallest. We also find that many planets may be ingested prior to the RGB phase, contrary to the expectation that accretion would generally occur when the stellar radii expand significantly as giants. Finally, our models suggest that the rapid rotation signal from ingested planets is most likely to be seen on the lower RGB, which is also where alternative mechanisms for spin-up, e.g., angular momentum dredged up from the stellar core, do not operate. Thus, rapid rotators on the lower RGB are the best candidates to search for definitive evidence of systems that have experienced planet accretion.},
  archiveprefix = {arxiv},
  keywords = {evolution-stars,notion,notion-database,planetary systems-stars,rotation},
  file = {/Users/lbugnet/Zotero/storage/Y8GKL4TA/full-text.pdf}
}

@article{Carlberg2011,
  title = {The Frequency of Rapid Rotation among {{K}} Giant Stars},
  author = {Carlberg, Joleen K. and Majewski, Steven R. and Patterson, Richard J. and Bizyaev, Dmitry and Smith, Verne V. and Cunha, Katia},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {732},
  number = {1},
  eprint = {1103.1387},
  pages = {1--25},
  issn = {15384357},
  doi = {10.1088/0004-637X/732/1/39},
  abstract = {We present the results of a search for unusually rapidly rotating giant stars in a large sample of K giants ({$\sim$}1300 stars) that had been spectroscopically monitored as potential targets for the Space Interferometry Mission's Astrometric Grid. The stars in this catalog are much fainter and typically more metal-poor than those of other catalogs of red giant star rotational velocities, but the spectra generally only have signal-to-noise ratio (S/N) of {$\sim$}20-60, making the measurement of the widths of individual lines difficult. To compensate for this, we have developed a cross-correlation method to derive rotational velocities in moderate S/N echelle spectra to efficiently probe this sample for rapid rotator candidates. We have discovered 28 new red giant rapid rotators as well as one extreme rapid rotator with a vsin i of 86.4kms-1. Rapid rotators comprise 2.2\% of our sample, which is consistent with other surveys of brighter, more metal-rich K giant stars. Although we find that the temperature distribution of rapid rotators is similar to that of the slow rotators, this may not be the case with the distributions of surface gravity and metallicity. The rapid rotators show a slight overabundance of low-gravity stars and as a group are significantly more metal-poor than the slow rotators, which may indicate that the rotators are tidally locked binaries. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: late-type,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/BNUNT5JX/Carlberg et al. - 2011.pdf}
}

@article{Carlberg2012,
  title = {Observable Signatures of Planet Accretion in Red Giant Stars. {{I}}. {{Rapid}} Rotation and Light Element Replenishment},
  author = {Carlberg, Joleen K. and Cunha, Katia and Smith, Verne V. and Majewski, Steven R.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {757},
  number = {2},
  issn = {15384357},
  doi = {10.1088/0004-637X/757/2/109},
  abstract = {The orbital angular momentum of a close-orbiting giant planet can be sufficiently large that, if transferred to the envelope of the host star during the red giant branch (RGB) evolution, it can spin-up the star's rotation to unusually large speeds. This spin-up mechanism is one possible explanation for the rapid rotators detected among the population of generally slow-rotating red giant stars. These rapid rotators thus comprise a unique stellar sample suitable for searching for signatures of planet accretion in the form of unusual stellar abundances due to the dissemination of the accreted planet in the stellar envelope. In this study, we look for signatures of replenishment in the Li abundances and (to a lesser extent) 12C/13C, which are both normally lowered during RGB evolution. Accurate abundances were measured from high signal-to-noise echelle spectra for samples of both slow and rapid rotator red giant stars. We find that the rapid rotators are on average enriched in lithium compared to the slow rotators, but both groups of stars have identical distributions of 12C/13C within our measurement precision. Both of these abundance results are consistent with the accretion of planets of only a few Jupiter masses. We also explore alternative scenarios for understanding the most Li-rich stars in our sample - particularly Li regeneration during various stages of stellar evolution. Finally, we find that our stellar samples show non-standard abundances even at early RGB stages, suggesting that initial protostellar Li abundances and 12C/ 13C may be more variable than originally thought. \textcopyright{} \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,stars: abundances,stars: atmospheres,stars: chemically peculiar,stars: late-type,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/FGXWXUTH/Carlberg et al. - 2012.pdf}
}

@article{Carlberg2014,
  title = {Rotational and Radial Velocities of 1.3-2.2 {{M}}{$\odot$} Red Giants in Open Clusters},
  author = {Carlberg, Joleen K.},
  year = {2014},
  journal = {Astronomical Journal},
  volume = {147},
  number = {6},
  issn = {00046256},
  doi = {10.1088/0004-6256/147/6/138},
  abstract = {This study presents the rotational distribution of red giant (RG) stars in 11 old to intermediate age open clusters. The masses of these stars are all above the Kraft break, so they lose negligible amounts of their birth angular momentum (AM) during the main-sequence (MS) evolution. However, they do span a mass range with quite different AM distributions imparted during formation, with the stars less massive than {$\sim$}1.6M {$\odot$} arriving on the MS with lower rotation rates than the more massive stars. The majority of RGs in this study are slow rotators across the entire red giant branch regardless of mass, supporting the picture that intermediate-mass stars rapidly spin down when they evolve off the MS and develop convection zones capable of driving a magnetic dynamo. Nevertheless, a small fraction of RGs in open clusters show some level of enhanced rotation, and faster rotators are as common in these clusters as in the field RG population. Most of these enhanced rotators appear to be red clump stars, which is also true of the underlying stellar sample, while others are clearly RGs that are above or below the clump. In addition to rotational velocities, the radial velocities (RVs) and membership probabilities of individual stars are also presented. Cluster heliocentric RVs for NGC 6005 and Pismis 18 are reported for the first time. \textcopyright{} 2014. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,open clusters and associations: general,stars: evolution,stars: late-type,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/E25P6RTK/Carlberg - 2014.pdf}
}

@article{Carrier2005,
  title = {New Seismological Results on the {{G0 IV}} {$\eta$} {{Bootis}}},
  author = {Carrier, F. and Eggenberger, P. and Bouchy, F.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {434},
  number = {3},
  pages = {1085--1095},
  issn = {00046361},
  doi = {10.1051/0004-6361:20042140},
  abstract = {Several attempts have been made to detect solar-like oscillations in the GO IV star {$\eta$} Boo. We present here new observations on this star simultaneously conducted with two spectrographs: CORALIE mounted on the 1.2-m Swiss telescope at the ESO La Silla Observatory (Chile) and ELODIE based on the 1.93-m telescope at the Observatoire de Haute-Provence (France). In total, 1239 spectra were collected over 13 nights. The power spectrum of the high precision velocity time series clearly presents several identifiable peaks between 0.4 and 1.0 mHz showing regularity with a large and small separation of {$\Delta$}v = 39.9 {$\mu$}Hz and {$\delta$}v02 = 3.95 {$\mu$}Hz respectively. Twenty-two individual frequencies have been identified. Detailed models based on these measurements and non-asteroseismic observables were computed using the Geneva evolution code including shellular rotation and atomic diffusion. By combining these seismological data with non-asteroseismic observations, we determine the following global parameters for {$\eta$} Boo: a mass of 1.57 {$\pm$} 0.07 M {$\odot$}, an age t = 2.67 {$\pm$} 0.10 Gyr and an initial metallicity (Z/X)i = 0.0391 {$\pm$} 0.0070. We also show that the mass of {$\eta$} Boo is very sensitive to the choice of the observed metallicity, while the age of {$\eta$} Boo depends on the input physics used. Indeed, a higher metallicity favours a higher mass, while non-rotating models without overshooting predict a smaller age. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Stars variables: general,Stars: fundamental parameters,Stars: individual: {$\eta$} Boo,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/BHLGCJ2W/Carrier, Eggenberger, Bouchy - 2005.pdf}
}

@article{Carrier2010,
  title = {Non-Radial Oscillations in the Red Giant {{HR}} 7349 Measured by {{CoRoT}}},
  author = {Carrier, F. and De Ridder, J. and Baudin, F. and Barban, C. and Hatzes, A. P. and Hekker, S. and Kallinger, T. and Miglio, A. and Montalb{\'a}n, J. and Morel, T. and Weiss, W. W. and Auvergne, M. and Baglin, A. and Catala, C. and Michel, E. and Samadi, R.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {509},
  number = {1},
  pages = {1--7},
  issn = {14320746},
  doi = {10.1051/0004-6361/200912749},
  abstract = {Context: Convection in red giant stars excites resonant acoustic waves whose frequencies depend on the sound speed inside the star, which in turn depends on the properties of the stellar interior. Therefore, asteroseismology is the most robust available method for probing the internal structure of red giant stars. Aims: Solar-like oscillations in the red giant HR 7349 are investigated. Methods: Our study is based on a time series of 380 760 photometric measurements spread over 5 months obtained with the CoRoT satellite. Mode parameters were estimated using maximum likelihood estimation of the power spectrum. Results: The power spectrum of the high-precision time series clearly exhibits several identifiable peaks between 19 and 40 {$\mu$}Hz showing regularity with a mean large and small spacing of {$\Delta$}? = 3.47 {$\pm$} 0.12 {$\mu$}Hz and {$\delta$}?02 = 0.65 {$\pm$} 0.10 {$\mu$}Hz. Nineteen individual modes are identified with amplitudes in the range from 35 to 115 ppm. The mode damping time is estimated to be 14.7+-2.94.7 days. \textcopyright{} 2010 ESO.},
  keywords = {General - Stars,HR 7349,Individual,Interiors - Stars,notion,notion-database,Oscillations - Stars,Stars,Variables},
  file = {/Users/lbugnet/Zotero/storage/8CKX2LZZ/Carrier et al. - 2010.pdf}
}

@article{Carrier2010b,
  title = {The Red-Giant {{CoRoT}} Target {{HR}} 7349},
  author = {Carrier, F. and Morel, T. and Miglio, A. and Montalb{\'a}n, J. and Auvergne, M. and Baglin, A. and Baudin, F. and Barban, C. and Catala, C. and D'Antona, F. and De Ridder, J. and Eggenberger, P. and Hatzes, A. P. and Hekker, S. and Kallinger, T. and Michel, E. and Noels, A. and Poretti, E. and Rainer, M. and Samadi, R. and Ventura, P. and Weiss, W. W.},
  year = {2010},
  journal = {Astrophysics and Space Science},
  volume = {328},
  number = {1},
  pages = {83--86},
  issn = {0004640X},
  doi = {10.1007/s10509-009-0171-y},
  abstract = {HR7349 is a bright [V = 5.8] red giant observed by CoRoT in the seismofield of the first long run. The outstanding CoRoT light curve allowed the detection of several solar-like oscillation modes (both radial and non-radial). On top of these seismic constraints, our observational knowledge on HR7349 benefits as well from a precise parallax and detailed spectroscopic constraints. We present all the observational constraints that are available for the theoretical modelling of this most promising target. \textcopyright{} 2009 Springer Science+Business Media B.V.},
  isbn = {1050900901},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations,Stars: variables},
  file = {/Users/lbugnet/Zotero/storage/T9HADPKE/Carrier et al. - 2010(2).pdf}
}

@article{Carter2012,
  title = {References and {{Notes}} 1.},
  author = {Carter, Joshua A and Agol, Eric and Chaplin, William J and Basu, Sarbani and Bedding, Timothy R and Fabrycky, Daniel C and Ford, Eric B and Fortney, Jonathan J and Hale, Steven J and Handberg, Rasmus},
  year = {2012},
  volume = {337},
  number = {August},
  pages = {556--560},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/P3Y87WFM/Carter et al. - 2012.pdf}
}

@article{Casagrande2016,
  title = {Measuring the Vertical Age Structure of the {{Galactic}} Disc Using Asteroseismology and {{SAGA}}},
  author = {Casagrande, L. and Silva Aguirre, V. and Schlesinger, K. J. and Stello, D. and Huber, D. and Serenelli, A. M. and Sch{\"o}nrich, R. and Cassisi, S. and Pietrinferni, A. and Hodgkin, S. and Milone, A. P. and Feltzing, S. and Asplund, M.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {455},
  number = {1},
  pages = {987--1007},
  issn = {13652966},
  doi = {10.1093/mnras/stv2320},
  abstract = {The existence of a vertical age gradient in the Milky Way disc has been indirectly known for long. Here, wemeasure it directly for the first time with seismic ages, using red giants observed by Kepler. We use Str\"omgren photometry to gauge the selection function of asteroseismic targets, and derive colour and magnitude limits where giants with measured oscillations are representative of the underlying population in the field. Limits in the 2MASS system are also derived. We lay out a method to assess and correct for target selection effects independent of Galaxy models. We find that low-mass, i.e. old red giants dominate at increasing Galactic heights, whereas closer to theGalactic plane they exhibit a wide range of ages and metallicities. Parametrizing this as a vertical gradient returns approximately 4 Gyr kpc-1 for the disc we probe, although with a large dispersion of ages at all heights. The ages of stars show a smooth distribution over the last {$\simeq$}10 Gyr, consistent with a mostly quiescent evolution for the Milky Way disc since a redshift of about 2. We also find a flat age-metallicity relation for disc stars. Finally, we show how to use secondary clump stars to estimate the present-day intrinsic metallicity spread, and suggest using their number count as a new proxy for tracing the ageing of the disc. This work highlights the power of asteroseismology for Galactic studies; however, we also emphasize the need for better constraints on stellar mass-loss, which is a major source of systematic age uncertainties in red giant stars.},
  keywords = {Asteroseismology,Disc,Distances,Evolution,Fundamental parameters,Galaxy,General,notion,notion-database,Stars},
  file = {/Users/lbugnet/Zotero/storage/WL9S7WV9/Casagrande et al. - 2016.pdf}
}

@article{Castanheira2004,
  title = {Observations of the {{Pulsating White Dwarf G}} 185\textendash 32},
  author = {Castanheira, B. G. and Kepler, S. O. and Moskalik, P. and Zo{\l}a, S. and Pajdosz, G. and Krzesi{\'n}ski, J. and O'Donoghue, D. and Katz, M. and Buckley, D. and Vauclair, G. and Dolez, N. and Chevreton, M. and Barstow, M. A. and Kanaan, A. and Giovannini, O. and Provencal, J. and Kawaler, S. D. and Clemens, J. C. and Nather, R. E. and Winget, D. E. and Watson, T. K. and Yanagida, K. and Dixson, J. S. and Hansen, C. J. and Bradley, P. A. and Wood, M. A. and Sullivan, D. J. and Kleinman, S. J. and Meistas, E. and Solheim, J.-E. and Bruvold, A. and Leibowitz, E. and Mazeh, T. and Koester, D. and Montgomery, M. H.},
  year = {2004},
  month = jan,
  journal = {Astronomy \& Astrophysics},
  volume = {413},
  number = {2},
  pages = {623--634},
  publisher = {{EDP Sciences}},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361:20031567},
  urldate = {2023-10-12},
  abstract = {We observed the pulsating hydrogen atmosphere white dwarf G 185\textendash 32 with the Whole Earth Telescope in 1992. We report on a weighted Fourier transform of the data detecting 18 periodicities in its light curve. Using the Hubble Space Telescope Faint Object Spectrograph time resolved spectroscopy, and the wavelength dependence of the relative amplitudes, we identify the spherical harmonic degree () for 14 pulsation signals. We also compare the determinations of effective temperature and surface gravity using the excited modes and atmospheric methods, obtaining \emph{{$\pm<$}i/{$>$} 80 K, \emph{{$\pm<$}i/{$>$} 0.04 and \emph{{$\pm<$}i/{$>$} .}}}},
  copyright = {\textcopyright{} ESO, 2004},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/PKTM7EE7/Castanheira et al. - 2004 - Observations of the Pulsating White Dwarf G 185–32.pdf}
}

@article{Catala2008,
  title = {{{PLATO}}: {{PLAnetary Transits}} and {{Oscillations}} of Stars},
  author = {Catala, Claude and Consortium, The Plato},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012040},
  abstract = {The PLAnetary Transits and Oscillations of stars Mission (PLATO), presented to ESA in the framework of its Cosmic Vision programme, will detect and characterize exoplanets by means of their transit signature in front of a very large sample of bright stars, and measure the seismic oscillations of the parent stars orbited by these planets in order to understand the properties of the exoplanetary systems. PLATO is the next-generation planet finder, building on the accomplishments of CoRoT and Kepler. i) it will observe significantly more stars, ii) its targets will be 2 to 3 magnitudes brighter (hence the precision of the measurements will be correspondingly greater as will be those of post-detection investigations, e.g. spectroscopy, asteroseismology, and eventually imaging), iii) it will be capable of observing significantly smaller exoplanets. The space-based observations will be complemented by ground- and space-based follow-up observations. These goals will be achieved by a long-term (5 years), high-precision, high-time-resolution, high-duty-cycle monitoring in visible photometry of a sample of more than 100,000 relatively bright (my {$\leq$} 12) stars and another 400,000 down to my 14. Two different mission concepts are proposed for PLATO: i) a staring concept with 100 small, very wide-field telescopes, assembled on a single platform and all looking at the same 26\textdegree{} diameter field, and ii) a spinning concept with three moderate-size telescopes covering more than 1400 degree2. \textcopyright{} 2008 IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G9ZX6TYL/Catala, Consortium - 2008.pdf}
}

@inproceedings{Catala2009,
  title = {Stellar Rotation: {{New}} Insight from {{CoRoT}}},
  booktitle = {{{AIP Conference Proceedings}}},
  author = {Catala, C. and Goupil, M. J. and Michel, E. and Baglin, A. and De Medeiros, J. Renan and Gondoin, Ph and Team, Corot},
  year = {2009},
  volume = {1094},
  pages = {87--94},
  issn = {0094243X},
  doi = {10.1063/1.3099257},
  urldate = {2020-07-04},
  abstract = {We present an overview of the new insight provided by the CoRoT satellite on stellar rotation. Thanks to its ultra-high precision, high duty cycle, long photometric monitoring of thousands of stars, CoRoT gives us a powerful tool to study stellar rotational modulation, and therefore to measure stellar rotational periods and to study active structures at the surface of stars. This paper presents preliminary results concerning this type of study. CoRoT will also provide us with an insight of internal stellar rotation via the measurement and exploitation of rotational splittings of oscillation modes. This approach to stellar rotation with CoRoT will require a careful analysis of the oscillation power spectra, which is in progress, but prospects for such measurements are presented. \textcopyright{} 2009 American Institute of Physics.},
  keywords = {notion,notion-database,{Photometric, polarimetric, and spectroscopic instr},{Space-based ultraviolet, optical, and infrared tel},Stellar activity,Stellar rotation,{Stellar structure, interiors, evolution, nucleosyn}}
}

@article{Catala2011,
  title = {{{PLATO}} : {{PLAnetary Transits}} and {{Oscillations}} of Stars},
  author = {Catala, Claude and Appourchaux, Thierry},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012084},
  abstract = {PLATO is a M-class candidate in the ESA Cosmic Vision program. PLATO's objective is to characterize exoplanets and their host stars in the solar neighbourhood. While it builds on the heritage from CoRoT and Kepler, the major breakthrough will come from its strong focus on bright targets (mV {$\leq$} 11). The PLATO targets will also include a large number of very bright (mV {$\leq$} 8) and nearby stars. The prime science goals of PLATO are: (i) the detection and characterization of exoplanetary systems of all kinds, including both the planets and their host stars, reaching down to small, terrestrial planets in the habitable zone; (ii) the identification of suitable targets for future, more detailed characterization, including a spectroscopic search for bio-markers in nearby habitable exoplanets. These ambitious goals will be reached by ultra-high precision, long (few years), uninterrupted photometric monitoring in the visible of very large samples of bright stars, which can only be done from space. The resulting high quality light curves will be used on the one hand to detect planetary transits, as well as to measure their characteristics, and on the other hand to provide a seismic analysis of the host stars of the detected planets, from which precise measurements of their radii, masses, and ages will be derived. The PLATO space-based data will be complemented by ground-based follow-up observations, in particular very precise radial velocity monitoring, which will be used to confirm the planetary nature of the detected events and to measure the planet masses. The full set of parameters of exoplanetary systems will thus be measured, including all characteristics of the host stars and the orbits, radii, masses, and ages of the planets, allowing us to derive planet mean densities, and estimate their temperature and radiation environment. Finally, the knowledge of the age of the exoplanetary systems will allow us to put them in an evolutionary perspective. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/W7DA929V/Catala, Appourchaux - 2011.pdf}
}

@article{Catelan2007,
  title = {Structure and Evolution of Low-Mass Stars: {{An}} Overview and Some Open Problems},
  author = {Catelan, M{\'a}rcio},
  year = {2007},
  journal = {AIP Conference Proceedings},
  volume = {930},
  eprint = {astro-ph/0703724},
  pages = {39--90},
  issn = {0094243X},
  doi = {10.1063/1.2790333},
  abstract = {A review is presented of some of the ingredients, assumptions and techniques that are used in the computation of the structure and evolution of low-mass stars. Emphasis is placed on several ingredients which are still subject to considerable uncertainty. An overview of the evolution of low-mass stars is also presented, from the cloud collapse phase all the way to the white dwarf cooling curve. \textcopyright{} 2007 American Institute of Physics.},
  archiveprefix = {arxiv},
  isbn = {0735404402},
  keywords = {notion,notion-database,Stars: evolution,Stars: general,Stars: Hertzsprung-Russell diagram,Stars: interiors,Stars: low-mass},
  file = {/Users/lbugnet/Zotero/storage/BYHCNPD7/Catelan - 2007.pdf}
}

@article{Cattaneo2001,
  title = {On the {{Origin}} of the {{Solar Mesogranulation}}},
  author = {Cattaneo, Fausto and Lenz, Dawn and Weiss, Nigel},
  year = {2001},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {563},
  number = {1},
  pages = {L91-L94},
  publisher = {{IOP Publishing}},
  issn = {0004637X},
  doi = {10.1086/338355},
  urldate = {2020-03-14},
  abstract = {The observed properties of mesogranules are related to structures found in idealized numerical experiments on turbulent convection. We describe results obtained for three-dimensional Boussinesq convection in a layer with a very large aspect ratio. There are two distinct cellular patterns at the surface. Energy-transporting convection cells (corresponding to granules in the solar photosphere) have diameters comparable to the layer depth, while macrocells (corresponding to mesogranules) are several times larger. The motion acts as a small-scale turbulent dynamo, generating a disordered magnetic field that is concentrated at macrocellular corners and, to a lesser extent, in the lanes that join them. These results imply that mesogranules owe their origin to collective interactions between the granules.},
  keywords = {notion,notion-database,Sun: Granulation,Sun: Magnetic Fields,Sun: Photosphere},
  file = {/Users/lbugnet/Zotero/storage/HZBPL3DD/full-text.pdf}
}

@article{Ceillier2012,
  title = {Attempts to Reproduce the Rotation Profile of the Red Giant {{KIC}} 7341231 Observed by {{Kepler}}},
  author = {Ceillier, T. and Eggenberger, P. and Garc{\'i}a, R. A. and Mathis, S.},
  year = {2012},
  journal = {Astronomische Nachrichten},
  volume = {333},
  number = {10},
  eprint = {1210.5880},
  pages = {971--974},
  issn = {00046337},
  doi = {10.1002/asna.201211806},
  abstract = {Thanks to the asteroseimic study of the red giant star KIC 7341231 observed by Kepler, it has been possible to infer its radial differential rotation profile (Deheuvels et al. 2012). This opens new ways to constrain the physical mechanisms responsible of the angular momentum transport in stellar interiors by directly comparing this radial rotation profile with the ones computed using stellar evolution codes including dynamical processes. In this preliminary work, we computed different models of KIC 7341231 with the Geneva stellar evolution code that includes transport mechanisms due to a shellular rotation and the associated large-scale meridional circulation and shear-induced turbulence. Once the global parameters of the star had been established, we modified some of the model's input parameters in order to understand their effects on the predicted rotation profile of the modeled star. As a result, we find a discrepancy between the rotation profile deduced from asteroseismic measurements and the profiles predicted from models including shellular rotation and related meridional flows and turbulence. This indicates that a most powerful mechanism is in action to extract angular momentum from the core of this star. \textcopyright{} 2012 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual (KIC 7341231),Stars: interiors,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/CZTA3J3E/Ceillier et al. - 2012.pdf}
}

@article{Ceillier2013,
  title = {Understanding Angular Momentum Transport in Red Giants: {{The}} Case of {{KIC}} 7341231},
  author = {Ceillier, T. and Eggenberger, P. and Garc{\'i}a, R. A. and Mathis, S.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {555},
  eprint = {1305.5630},
  pages = {1--8},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321473},
  abstract = {Context. Thanks to recent asteroseismic observations, it has been possible to infer the radial differential rotation profile of subgiants and red giants. Aims. We want to reproduce the observed rotation profile of the early red giant KIC 7341231 through modeling and constrain the physical mechanisms responsible for angular momentum transport in stellar interiors. Methods. We computed models of KIC 7341231 including a treatment of shellular rotation, and we compared the rotation profiles obtained with the one derived from observations. We then modify some modeling parameters in order to quantify their effect on the obtained rotation profile. Moreover, we mimicked a powerful angular momentum transport during the main sequence and studied its effect on the evolution of the rotation profile during the subgiant and red giant phases. Results. We show that meridional circulation and shear mixing alone produce a rotation profile for KIC 7341231 that is too steep compared to the observed one. An additional mechanism is then needed to increase the internal transport of angular momentum. We find that this undetermined mechanism has to be efficient not only during the main sequence but also during the much quicker subgiant phase. Moreover, we point out the importance of studying the whole rotational history of a star to explain its rotation profile during the red giant evolution. \textcopyright{} 2013 ESO.},
  archiveprefix = {arxiv},
  keywords = {Evolution,notion,notion-database,Oscillations-Stars,Rotation-Stars,Stars},
  file = {/Users/lbugnet/Zotero/storage/C3ALDAMM/Ceillier et al. - 2013.pdf}
}

@article{Ceillier2016,
  title = {Rotation Periods and Seismic Ages of {{KOIs}} - Comparison with Stars without Detected Planets from {{Kepler}} Observations},
  author = {Ceillier, T. and {van Saders}, J. and Garc{\'i}a, R. A. and Metcalfe, T. S. and Creevey, O. and Mathis, S. and Mathur, S. and Pinsonneault, M. H. and Salabert, D. and Tayar, J.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {456},
  number = {1},
  eprint = {1510.09023},
  pages = {119--125},
  issn = {13652966},
  doi = {10.1093/mnras/stv2622},
  abstract = {One of the most difficult properties to derive for stars is their age. For cool main-sequence stars, gyrochronology relations can be used to infer stellar ages from measured rotation periods and Hertzsprung Russell diagram positions. These relations have few calibrators with known ages for old, long rotation period stars. There is a significant sample of old Kepler objects of interest, or KOIs, which have both measurable surface rotation periods and precise asteroseismic measurements from which ages can be accurately derived. In this work, we determine the age and the rotation period of solar-like pulsating KOIs to both compare the rotation properties of stars with and without known planets and enlarge the gyrochronology calibration sample for old stars. We use Kepler photometric light curves to derive the stellar surface rotation periods while ages are obtained with asteroseismology using the Asteroseismic Modelling Portal in which individual mode frequencies are combined with high-resolution spectroscopic parameters. We thus determine surface rotation periods and ages for 11 planet-hosting stars, all over 2 Gyr old. We find that the planet-hosting stars exhibit a rotational behaviour that is consistent with the latest age-rotation models and similar to the rotational behaviour of stars without detected planets. We conclude that these old KOIs can be used to test and calibrate gyrochronology along with stars not known to host planets.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planet,Star interactions,Stars: evolution,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/FYUP33IL/Ceillier et al. - 2016.pdf}
}

@article{Ceillier2017,
  title = {Surface Rotation of {{Kepler}} Red Giant Stars},
  author = {Ceillier, T. and Tayar, J. and Mathur, S. and Salabert, D. and Garc{\'i}a, R. A. and Stello, D. and Pinsonneault, M. H. and Van Saders, J. and Beck, P. G. and Bloemen, S.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {605},
  eprint = {1707.05989},
  pages = {1--11},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629884},
  abstract = {Kepler allows the measurement of starspot variability in a large sample of field red giants for the first time. With a new method that combines autocorrelation and wavelet decomposition, we measure 361 rotation periods from the full set of 17 377 oscillating red giants in our sample. This represents 2.08\% of the stars, consistent with the fraction of spectroscopically detected rapidly rotating giants in the field. The remaining stars do not show enough variability to allow us to measure a reliable surface rotation period. Because the stars with detected rotation periods have measured oscillations, we can infer their global properties, e.g. mass and radius, and quantitatively evaluate the predictions of standard stellar evolution models as a function of mass. Consistent with results for cluster giants when we consider only the 4881 intermediate-mass stars, M {$>$} 2.0 M{$\odot$} from our full red giant sample, we do not find the enhanced rates of rapid rotation expected from angular momentum conservation. We therefore suggest that either enhanced angular momentum loss or radial differential rotation must be occurring in these stars. Finally, when we examine the 575 low-mass (M{$<$} 1.1 M{$\odot$}) red clump stars in our sample, which were expected to exhibit slow (non-detectable) rotation, 15\% of them actually have detectable rotation. This suggests a high rate of interactions and stellar mergers on the red giant branch.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: evolution,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/TSPBE44P/Ceillier et al. - 2017.pdf}
}

@article{Chaname2012a,
  title = {Toward Precise Ages for Single Stars in the Field. {{Gyrochronology}} Constraints at Several {{Gyr}} Using Wide Binaries. {{I}}. {{Ages}} for Initial Sample},
  author = {Chanam{\'e}, Julio and Ram{\'i}rez, Iv{\'a}n},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {746},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/746/1/102},
  abstract = {We present a program designed to obtain age-rotation measurements of solar-type dwarfs to be used in the calibration of gyrochronology relations at ages of several Gyr. This is a region of parameter space crucial for the large-scale study of the Milky Way, and where the only constraint available today is that provided by the Sun. Our program takes advantage of a set of wide binaries selected so that one component is an evolved star and the other is a main-sequence star of FGK type. In this way, we obtain the age of the system from the evolved star, while the rotational properties of the main-sequence component provide the information relevant for gyrochronology regarding the spin-down of solar-type stars. By mining currently available catalogs of wide binaries, we assemble a sample of 37 pairs well positioned for our purposes: 19 with turnoff or subgiant primaries and 18 with white dwarf components. Using high-resolution optical spectroscopy, we measure precise stellar parameters for a subset of 15 of the pairs with turnoff/subgiant components and use these to derive isochronal ages for the corresponding systems. Ages for 16 of the 18 pairs with white dwarf components are taken from the literature. The ages of this initial sample of 31 wide binaries range from 1 to 9Gyr, with precisions better than 20\% for almost half of these systems. When combined with measurements of the rotation period of their main-sequence components, these wide binary systems would potentially provide a similar number of points useful for the calibration of gyrochronology relations at very old ages. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {binaries: general,Galaxy: stellar content,notion,notion-database,stars: evolution,stars: fundamental parameters,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/FNBTVAH8/Chanamé, Ramírez - 2012.pdf}
}

@article{Chandrasekhar1958,
  title = {{{ON THE EQUILIBRIUM CONFIGURATIONS OF AN INCOMPRESSIBLE FLUID WITH AXISYMMETRIC MOTIONS AND MAGNETIC FIELDS}}},
  author = {Chandrasekhar, S.},
  year = {1958},
  month = sep,
  journal = {Proceedings of the National Academy of Sciences},
  volume = {44},
  number = {9},
  pages = {842--847},
  publisher = {{Proceedings of the National Academy of Sciences}},
  issn = {0027-8424},
  doi = {10.1073/pnas.44.9.842},
  urldate = {2020-06-19},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/S5NQUZ57/full-text.pdf}
}

@article{Chandrasekhar1960,
  title = {{{THE STABILITY OF NON-DISSIPATIVE COUETTE FLOW IN HYDROMAGNETICS}}},
  author = {Chandrasekhar, S.},
  year = {1960},
  month = feb,
  journal = {Proceedings of the National Academy of Sciences},
  volume = {46},
  number = {2},
  pages = {253--257},
  publisher = {{Proceedings of the National Academy of Sciences}},
  issn = {0027-8424},
  doi = {10.1073/pnas.46.2.253},
  urldate = {2020-07-02},
  abstract = {Not Available},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MQ6RNTNG/full-text.pdf}
}

@article{Chaplin1996,
  title = {{{BiSon}} Performance},
  author = {Chaplin, William J. and Elsworth, Yvonne and Howe, Rachel and Isaak, George R. and McLeod, Clive P. and Miller, Brek A. and Van Der Raay, H. B. and Wheeler, Sarah J. and New, Roger},
  year = {1996},
  journal = {Solar Physics},
  volume = {168},
  number = {1},
  pages = {1--18},
  publisher = {{Springer Netherlands}},
  issn = {00380938},
  doi = {10.1007/BF00145821},
  urldate = {2020-03-08},
  abstract = {Since 1981 we have been operating the Birmingham Solar-Oscillations Network (BiSON), a global network of resonant-scattering spectrometers, observing the low-l solar p modes. Here we discuss historical developments, culminating in the establishment of a 6-station network in 1992 September, and the subsequent performance of that network. The data record of each station from 1992 to 1994 has been analysed in terms of weather and equipment breakdowns. Our early experience suggests that the best long-term coverage possible with a 6-station network is limited in practice to about 80\%, which falls short of previous predictions. \textcopyright{} 1996 Kluwer Academic Publishers.},
  keywords = {notion,notion-database}
}

@article{Chaplin1999,
  title = {Skew-Symmetric Solar p Modes in Low-{$\mathscr{l}$} {{BiSON}} Data},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Miller, B. A. and New, R.},
  year = {1999},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {308},
  number = {2},
  pages = {424--430},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.1999.02719.x},
  abstract = {The p-mode oscillations of the Sun are manifestations of resonantly trapped acoustic waves propagating within its interior. The effective size of the resulting resonant cavity changes with the properties of the modes - the interaction of this phenomenon with a highly localized excitation source in the upper layers of the convection zone gives rise to skew-symmetric resonant profiles whose degree of asymmetry changes with frequency. Here, we have fitted low-angular-degree (low-{$\mathscr{l}$}) resonant p-mode peaks - in a power spectrum generated from 32 months of BiSON Doppler velocity observations of the visible solar disc - to a skew-symmetric formalism to account for this effect. We present the fitted frequencies, fine-structure spacings [d0(n) and d1(n)] and mode-skewness estimates; and discuss the quantitative impact of fitting a skew, rather than symmetric, limit model. We also consider the reliability of the extracted parameters through the application of a useful statistical test, and extensive Monte Carlo fits to artificial data.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: interior,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/LRBAQWRP/Chaplin et al. - 1999.pdf}
}

@article{Chaplin2000,
  title = {Variations in the Excitation and Damping of Low-{$\mathscr{l}$} Solar p Modes over the Solar Activity Cycle},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Miller, B. A. and New, R.},
  year = {2000},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {313},
  number = {1},
  pages = {32--42},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2000.03176.x},
  abstract = {We have searched helioseismic data collected by the Birmingham Solar Oscillations Network (BiSON) for solar-cycle changes to those low-{$\mathscr{l}$} p-mode parameters that relate to the excitation and damping of the resonances. These data - collected between 1991 and 1997 - cover the complete declining phase of solar activity cycle 22 (up to and including the cycle 22/23 boundary). Over the range 2600 {$\leq$} v {$\leq$} 3600 {$\mu$}Hz, we uncover a mean 24 {$\pm$} 3 per cent increase in the frequency-domain linewidths; a mean decrease of 46 {$\pm$} 5 per cent decrease in the mode heights, and a mean decrease of 22 {$\pm$} 3 per cent in the modal velocity powers. The rate at which energy is supplied to the modes remains constant, at the level of precision of the observations (measured change 0 {$\pm$} 4 per cent). We use expressions derived from the equation of a damped harmonic oscillator to illustrate the diagnostic properties of the observables: these indicate that both the signs and relative sizes of the extracted variations can arise from changes solely to the net damping; the net forcing of the modes need not change. The results possibly hint at the changes being maximal at frequencies near {$\sim$}3100 {$\mu$}Hz. They might therefore suggest an origin for the observed variations that is peaked in the superadiabatic layer of the convection zone, which couples most strongly to the eigenfunctions of modes at the centre of the p-mode spectrum.},
  keywords = {notion,notion-database,Sun: activity,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/937VXF6D/Chaplin et al. - 2000.pdf}
}

@article{Chaplin2001,
  title = {Changes to Low-{$\mathscr{l}$} Solar p-Mode Frequencies over the Solar Cycle: {{Correlations}} on Different Time-Scales},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Marchenkov, K. I. and Miller, B. A. and New, R.},
  year = {2001},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {322},
  number = {1},
  pages = {22--30},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2001.04098.x},
  abstract = {We have studied variations in the frequencies of low-{$\mathscr{l}$} solar p modes through the analysis of nine years of helioseismic data collected by the Birmingham Solar Oscillations Network (BiSON)\textdagger. This is the first time that such a long data set has been explored with the extra accuracy afforded by fitting the modes to asymmetric profiles. The epoch covered (1991-99) spans the declining activity phase of solar cycle 22, and a substantial portion of the initial activity increase during cycle 23. The complete time series has been split into contiguous segments of length 27, 54, 108 and 216 d in order to facilitate the study of changes occurring on different time-scales. Further, we have characterized the observed shifts as a function of six well-known indicators of solar activity. These indices reflect changes taking place in the photosphere, chromosphere and corona, but only over the visible hemisphere of the Sun. Since the low-{$\mathscr{l}$} eigenfrequencies respond to global variations in activity, we discuss the implications of this mismatch for the analyses performed. We demonstrate that, as expected, the low-{$\mathscr{l}$} modes adjust to changes in the activity measures on time-scales as short as a few months. Our analysis indicates that all six proxies correlate equally well (at the level of precision of the data) with the measured shifts. Further, the sensitivity of the shifts to changes in five of the activity indices is the same, to within {$\sim$}15 per cent (1{$\sigma$}) or so, on the falling and rising phases considered. There is, however, a slight suggestion that the sensitivity to changes in the disc-averaged line-of-sight magnetic field component (as determined from daily Kitt Peak magnetograms) may be higher on the rising phase of the cycle.},
  keywords = {notion,notion-database,Sun: activity,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/C6U2PBRY/Chaplin et al. - 2001.pdf}
}

@article{Chaplin2001a,
  title = {The Phenomenology of Solar-Cycle-Induced Acoustic Eigenfrequency Variations: {{A}} Comparative and Complementary Analysis of {{GONG}}, {{BiSON}} and {{VIRGO}}/{{LOI}} Data},
  author = {Chaplin, W. J. and Appourchaux, T. and Elsworth, Y. and Isaak, G. R. and New, R.},
  year = {2001},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {324},
  number = {4},
  pages = {910--916},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2001.04357.x},
  abstract = {We use high-quality helioseismic data collected by three different observational programmes during the declining phase of activity cycle 22, and a substantial portion of the rising phase of the current cycle (23), to study the phenomenological nature of the cycle-induced (centroid) eigenfrequency variations. We have analysed the frequency dependence of the shifts by fitting a power law of the form {$\delta\nu$}nl {$\propto$} ({$\nu$}nl){$\alpha$}/Enl to the data (where the Enl are the mode inertias, and a is the power-law index to be extracted). Previous studies have suggested that a relation with {$\alpha$} = 0 provides an adequate description of the shifts up to {$\nu$} {$\approx$} 3500 {$\mu$}Hz. However, here we show that while nevertheless describing the shifts well up to {$\sim$}2500 {$\mu$}Hz, the linear scaling breaks down conspicuously at higher frequencies. Above this threshold, the shifts follow a power-law dependence with {$\alpha$} {$\sim$} 2. Our analyses (for 1600 {$\leq$} {$\nu$} {$\leq$} 4000 {$\mu$}Hz) make use of observations made by the ground-based GONG over the angular degree range 4 {$\leq$} l {$\leq$} 150; the ground-based BiSON over 0 {$\leq$} l {$\leq$} 2; and the VIRGO/LOI instrument on board the ESA/NASA SOHO satellite over 0 {$\leq$} l {$\leq$} 8. We show that GONG shifts averaged over different ranges in l, together with the BiSON and LOI data averaged over their full quoted ranges, all scale at fixed frequency with the normalized mode inertia ratio Qnl. This is to be expected if the solar-cycle perturbation affecting the modes is confined in the surface layers; the excellent agreement also reflects favourably on the external consistency of the different observations.},
  keywords = {notion,notion-database,Sun: activity,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/PADNTJPB/Chaplin et al. - 2001(2).pdf}
}

@article{Chaplin2001b,
  title = {Rigid Rotation of the Solar Core? {{On}} the Reliable Extraction of Low-{$\mathscr{l}$} Rotational p-Mode Splittings from Full-Disc Observations of the {{Sun}}},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Marchenkov, K. I. and Miller, B. A. and New, R.},
  year = {2001},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {327},
  number = {4},
  pages = {1127--1136},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2001.04805.x},
  abstract = {We present low-{$\mathscr{l}$} rotational p-mode splittings from the analysis of 8 yr of observations made by the Birmingham Solar-Oscillations Network (BiSON) of the full solar disc. These data are presented in the light of a thorough investigation of the fitting techniques used to extract them. Particular attention is paid to both the origin and magnitude of bias present in these estimates. An extensive Monte Carlo strategy has been adopted to facilitate this study - in all, several thousand complete, artificial proxies of the 96-month data set have been generated to test the analysis of real 'full-disc' data. These simulations allow for an assessment of any complications in the analysis which might arise from variations in the properties of the p modes over the 11-yr solar activity cycle. The use of such an extended data set affords greater precision in the splittings, and by implication the rotation rate inferred from these data, and reduces bias inherent in the analysis, thereby giving a more accurate determination of the rotation. The grand, weighted sidereal average of the BiSON set is 434 {$\pm$} 2 nHz, a value consistent with that expected were the deep radiative interior (r/R {$<$} 0.5) to rotate at the same frequency, and in the same 'rigid' manner, as the more precisely and accurately studied outer part of the radiative zone.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: interior,Sun: oscillations,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/VJXIWTIE/Chaplin et al. - 2001(3).pdf}
}

@article{Chaplin2002,
  title = {Peak Finding at Low Signal-to-Noise Ratio: {{Low-$\mathscr{l}$}} Solar Acoustic Eigenmodes at n {$\leq$} 9 from the Analysis of {{BiSON}} Data},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Marchenkov, K. I. and Miller, B. A. and New, R. N. and Pinter, B. and Appourchaux, T.},
  year = {2002},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {336},
  number = {3},
  pages = {979--991},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2002.05834.x},
  abstract = {We make use of 9 yr of full-disc helioseismic data - as collected by the ground-based Birmingham Solar-Oscillations Network (BiSON) - to search for low-frequency, low-angular-degree (low-{$\mathscr{l}$}) acoustic modes. A range of tests are applied to the power spectrum of the observations that search for prominent mode-like structure: strong spikes, structure spanning several bins signifying the presence of width (from damping), and the occurrence of prominent multiplet structure at {$\mathscr{l}$} {$\geq$} 1 arising principally from the solar rotation and made from several spikes separated suitably in frequency. For each test we present analytical expressions that allow the probability that the uncovered structure is part of the broad-band noise background to be assessed. These make use of the cumulative binomial (Bernoulli) distribution and serve to provide an objective measure of the significance of the detections. This work has to date uncovered nine significant detections of non-broad-band origin that we have identified as low-{$\mathscr{l}$} modes with radial overtone numbers n {$\leq$} 9.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Sun: interior,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/UYVC4QEK/Chaplin et al. - 2002.pdf}
}

@article{Chaplin2003,
  title = {Observation of , and Temporal Variations in , Solar p-Mode Multiplet Frequency Asymmetries at = 2 3 {{DATA A N D F I T T I N G P R O C E D U R E}} 2 {{S TAT E M E N T O F T H E P RO B L E M}}},
  author = {Chaplin, W J and Elsworth, Y and Isaak, G R and Miller, B A and New, R and Thiery, S and Boumier, P and Gabriel, A H},
  year = {2003},
  volume = {352},
  pages = {343--352},
  keywords = {activity,data analysis,methods,notion,notion-database,oscillations,sun},
  file = {/Users/lbugnet/Zotero/storage/7VC63LNS/Chaplin et al. - 2003.pdf}
}

@article{Chaplin2004,
  title = {The Solar Cycle as Seen by Low-{$\mathscr{l}$} p-Mode Frequencies: {{Comparison}} with Global and Decomposed Activity Proxies},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Miller, B. A. and New, R.},
  year = {2004},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {352},
  number = {4},
  pages = {1102--1108},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2004.07998.x},
  abstract = {We present a detailed study of variations observed in low-angular degree solar p-mode frequencies during solar cycles 22 and 23, and their relation to global and spatially decomposed proxies of the surface activity. To do so, we have analysed 11 yr of unresolved (Sun-as-a-star) Doppler velocity observations of the solar disc made by the Birmingham Solar-Oscillations Network (BiSON). The sensitivity of these observations to different azimuthal orders, m, is such that for the degree range studied (0 {$\leq$} {$\mathscr{l}$} {$\leq$} 2) extracted frequencies can be regarded as providing a measure of the response of the sectoral modes (with |m| = {$\mathscr{l}$}). After allowing for the dependence of the frequency shifts on mode frequency and inertia, we find the average {$\mathscr{l}$} = 0 shift is significantly weaker than that at {$\mathscr{l}$} = 2; the magnitude of the average {$\mathscr{l}$} = 1 shift lies in between the two, The comparative sizes of the shifts are observed to match those of the corresponding spherical harmonic (Legendre) components of both the Kitt Peak magnetogram (KPMI) and He I equivalent width activity indices, and reflect, therefore, the sensitivity of the observed mode components to the distribution of activity over the solar surface (i.e. a 'spatial' contribution to the shifts). When the falling and rising parts of the cycles are analysed independently, we uncover a significant difference in behaviour at {$\mathscr{l}$} = 1. Possible reasons for this are discussed.},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/4UXHIWY6/Chaplin et al. - 2004.pdf}
}

@article{Chaplin2004b,
  title = {Solar P-Mode Frequencies at {$\mathscr{l}$} = 2: {{What}} Do Analyses of Unresolved Observations Actually Measure?},
  author = {Chaplin, W. J. and Appourchauz, T. and Elsworth, Y. and Isaak, G. R. and Miller, B. A. and New, R. and Toutain, T.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {416},
  number = {1},
  pages = {341--351},
  issn = {00046361},
  doi = {10.1051/0004-6361:20034465},
  abstract = {We have studied in detail the extraction of estimates of {$\mathscr{l}$} = 2 p-mode frequencies from unresolved observations of the visible disc of the Sun. Examples of data of this type include ground-based observations made by the Birmingham Solar-Oscillations Network (BiSON), and space-borne observations made by the GOLF and VIRGO/SPM instruments on board the ESA/NASA SOHO satellite. The fitting of the modes is complicated in practice by the asymmetric arrangement in frequency of the three components (m = -2, 0 and 2) that are prominent in such data. In order to investigate the effect of this we used a series of 10-yr artificial datasets into which varying degrees of asymmetry were introduced. The sets were designed to mimic the characteristics of the BiSON and GOLF data, and were analyzed both with and without the BiSON window function from the period 1992 through 2001. Since reliable estimates of the asymmetry have only recently been extracted from unresolved observations (Chaplin et al. 2003a) it has for a long time been standard practice to fit the {$\mathscr{l}$} = 2 modes to a model that assumes a symmetrically arranged multiplet. We have tested the impact of this on the accuracy of the extracted frequencies. Furthermore, we demonstrate that asymmetric models can be successfully applied, provided the data are of sufficient length and quality. We also discuss the implications of our simulations for analyses of real solar data.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/RJEVG5H9/Chaplin et al. - 2004(2).pdf}
}

@article{Chaplin2004c,
  title = {Impact of Observational Duty Cycle on the Measurement of Low-{$\mathscr{l}$} Solar p-Mode Frequencies},
  author = {Chaplin, W. J. and Elsworth, Y. and Isaak, G. R. and Miller, B. A. and New, R. and Salabert, D.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {424},
  number = {1},
  pages = {301--309},
  issn = {00046361},
  doi = {10.1051/0004-6361:20040372},
  abstract = {We investigate the impact of a multi-site, ground-based observational window function on the extraction of estimates of the frequencies of low-angular-degree (low-{$\mathscr{l}$}) solar p modes from decade-long datasets. To effect this study we have made use of some {$\approx$}10 yr of full-disc, "Sun-as-a-star" Doppler velocity data collected by the Birmingham-Solar Oscillations Network (BiSON). A coherent combination of observations made by all six BiSON sites provided the principal time series of data. This set was then modulated by a whole series of different window functions and the resulting sets analyzed. The windows were made from different combinations and numbers of BiSON stations. We find that for the majority of low-{$\mathscr{l}$} modes the bias in the frequencies given by the effects of the window function is not significant. However, for modes above {$\approx$}3300 {$\mu$}Hz, and some {$\mathscr{l}$} = 2 modes near {$\approx$}2500 {$\mu$}Hz, the bias is important when the frequencies are extracted from long datasets.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/U2H8MZZ7/Chaplin et al. - 2004(3).pdf}
}

@article{Chaplin2004d,
  title = {On the Detectability of a Rotation-Rate Gradient in the Solar Core},
  author = {Chaplin, W. J. and Sekii, T. and Elsworth, Y. and Gough, D. O.},
  year = {2004},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {355},
  number = {2},
  pages = {535--542},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2004.08338.x},
  abstract = {We consider the problem of uncovering a possible gradient of rotation in the solar core using seismic frequency splittings of low-degree p-modes. The data are presumed to come from full-disc observations of the Sun. In particular, we formulate an approach for determining the diagnostic potential of a low-l splitting set to uncover, by inversion, a difference in rotation between two target radii: one deep in the core, the other in the mid-regions of the radiative zone. Our formulation assumes the underlying rotation rate to be flat in the outer part of the zone, but to vary linearly in the core (with the breakpoint in behaviour located between the two target radii). Artificial data are used to test the formulation, and to investigate the relative importance at low l of deeply penetrating, high-order modes and relatively shallow, low-order modes. Our results suggest that in order to detect a significant difference between the rotation at r = 0.1 R and 0.35 R - with the input splitting data coming from a 10-yr set of high-quality observations - that difference would need to be a significant fraction of the rotation rate itself.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/SJ94ASDQ/Chaplin et al. - 2004(4).pdf}
}

@article{Chaplin2006,
  title = {Solar {{FLAG}} Here and Hounds: {{On}} the Extraction of Rotational p-Mode Splittings from Seismic, {{Sun-as-a-star}} Data},
  author = {Chaplin, W. J. and Appourchaux, T. and Baudin, F. and Boumier, P. and Elsworth, Y. and Fletcher, S. T. and Fossat, E. and Garc{\'i}a, R. A. and Isaak, G. R. and Jim{\'e}nez, A. and {Jim{\'e}nez-Reyes}, S. J. and Lazrek, M. and Leibacher, J. W. and Lochard, J. and New, R. and Pall{\'e}, P. and R{\'e}gulo, C. and Salabert, D. and Seghouani, N. and Toutain, T. and Wachter, R.},
  year = {2006},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {369},
  number = {2},
  pages = {985--996},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2006.10358.x},
  abstract = {We report on results from the first solar Fitting at Low-Angular degree Group (solar FLAG) hare-and-hounds exercise. The group is concerned with the development of methods for extracting the parameters of low-l solar p-mode data ('peak bagging'), collected by Sun-as-a-star observations. Accurate and precise estimation of the fundamental parameters of the p modes is a vital pre-requisite of all subsequent studies. Nine members of the FLAG (the 'hounds') fitted an artificial 3456-d data set. The data set was made by the 'hare' (WJC) to simulate full-disc Doppler velocity observations of the Sun. The rotational frequency splittings of the l = 1, 2 and 3 modes were the first parameter estimates chosen for scrutiny. Significant differences were uncovered at l = 2 and 3 between the fitted splittings of the hounds. Evidence is presented that suggests this unwanted bias had its origins in several effects. The most important came from the different way in which the hounds modelled the visibility ratio of the different rotationally split components. Our results suggest that accurate modelling of the ratios is vital to avoid the introduction of significant bias in the estimated splittings. This is of importance not only for studies of the Sun, but also of the solar analogues that will be targets for asteroseismic campaigns. \textcopyright{} 2006 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/PW8YRH8Z/Chaplin et al. - 2006.pdf}
}

@article{Chaplin2007,
  title = {Solar {{Heavy}}-{{Element Abundance}}: {{Constraints}} from {{Frequency Separation Ratios}} of {{Low}}-{{Degree}} p -{{Modes}}},
  author = {Chaplin, William J. and Serenelli, Aldo M. and Basu, Sarbani and Elsworth, Yvonne and New, Roger and Verner, Graham A.},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {670},
  number = {1},
  eprint = {0705.3154},
  pages = {872--884},
  issn = {0004-637X},
  doi = {10.1086/522578},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Y23XQFP8/Chaplin et al. - 2007.pdf}
}

@article{Chaplin2007a,
  title = {On Prospects for Sounding Activity Cycles of {{Sun-like}} Stars with Acoustic Modes},
  author = {Chaplin, W. J. and Elsworth, Y. and Houdek, G. and New, R.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {377},
  number = {1},
  pages = {17--29},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.11581.x},
  abstract = {Data are now available on the Sun-like, p-mode oscillations of a growing number of late-type stars. With extension of these observations to dedicated, long-term campaigns, it will soon become possible to probe acoustically magnetic activity, and stellar cycles, by observation of systematic shifts in the mode frequencies giving additional information to the stellar dynamo theorists. Here, we use model computations of the damping rates of stochastically excited radial p modes to make predictions of the precision with which it will be possible to measure stellar-cycle frequency shifts of Sun-like stars along the lower main sequence. We assume the first analyses will average shifts across the most prominent modes to reduce uncertainties. We also make some predictions of the expected frequency shifts, based on existing stellar Ca ii H\& K data. Our main conclusion is that the basic properties of the acoustic signatures of the cycles should be measurable to reasonably high precision given only a few multimonth segments of data. It should also be possible to make inference on the surface distribution of the activity, through measurement of shifts of modes of different degree. Our computations also reveal an interesting feature in the predicted appearance of the acoustic mode spectra of stars cooler than about 5400 K: the modelled power spectral density of the modes shows two maxima, at different frequencies. By computing average shifts of modes across the two maxima, where the signal-to-noise ratio is highest, it should be possible to get the first measures of the frequency dependence of the p-mode shifts. This dependence provides information on the mechanism responsible for driving these shifts. \textcopyright{} 2007 RAS.},
  keywords = {notion,notion-database,Stars: activity,Stars: oscillations,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/XHR2WQDA/Chaplin et al. - 2007(2).pdf}
}

@article{Chaplin2008a,
  title = {Uncovering the Bias in Low-Degree p-Mode Linewidth Fitting},
  author = {Chaplin, W. J. and Elsworth, Y. and Miller, B. A. and New, R. and Verner, G. A.},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  pages = {189--196},
  issn = {00380938},
  doi = {10.1007/s11207-008-9215-7},
  abstract = {Obtaining reliable estimates of linewidths in the power spectra of low-degree p modes is problematic at low frequency. In this regime, the mode coherence time increases with decreasing frequency, often causing the modes to be unresolved in relatively long duration spectra. The signal-to-noise ratio is also less favourable at low frequency, resulting in fits to power spectra underestimating the true linewidth of the p modes owing to the tails of the Lorentzian peaks becoming dominated by the background noise. We use a numerical simulation approach to assess the effect of this bias on the fitted widths of p-mode peaks and calculate observational duration limits required to obtain an unbiased estimate of the p-mode linewidth as a function of frequency. This is done in four different cases, where the precision of the artificial data is set at 0.25, 0.50, 0.75, and 1.00 ms-1 by adding randomscatter to increase the sample standard deviation per 40-second measurement. In all cases, the observational duration required to accurately obtain width estimates increases beyond that required for sufficient spectral resolution below a certain threshold frequency. For modes at {$\approx$}1500 {$\mu$}Hz, with an amplitude of approximately ten times the background, observations of up to 972 days are required to obtain an unbiased estimate of the linewidth. This is equivalent to {$\approx$}18 times the coherence time of the corresponding p modes. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  isbn = {1120700892},
  keywords = {Helioseismology: Observations,notion,notion-database,Oscillations: Solar},
  file = {/Users/lbugnet/Zotero/storage/Q8WF9EVA/Chaplin et al. - 2008.pdf}
}

@article{Chaplin2008b,
  title = {A Devil in the Detail: {{Parameter}} Cross-Talk from the Solar Cycle and Estimation of Solar p-Mode Frequencies},
  author = {Chaplin, W. J. and {Jim{\'e}nez-Reyes}, S. J. and {Eff-Darwich}, A. and Elsworth, Y. and New, R.},
  year = {2008},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {385},
  number = {3},
  pages = {1605--1612},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2008.12942.x},
  abstract = {Frequencies, powers and damping rates of the solar p modes are all observed to vary over the 11-yr solar activity cycle. Here, we show that simultaneous variations in these parameters give rise to a subtle cross-talk effect, which we call the 'devil in the detail', that biases p-mode frequencies estimated from analysis of long power frequency spectra. We also show that the resonant peaks observed in the power frequency spectra show small distortions due to the effect. Most of our paper is devoted to a study of the effect for Sun-as-a-star observations of the low-l p modes. We show that for these data the significance of the effect is marginal. We also touch briefly on the likely l dependence of the effect, and discuss the implications of these results for solar structure inversions. \textcopyright{} 2008 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/95QYD2U4/Chaplin et al. - 2008(2).pdf}
}

@article{Chaplin2008d,
  title = {Distortion of the P-Mode Peak Profiles by the Solar-Cycle Frequency Shifts: Do We Need to Worry?},
  author = {Chaplin, W. J. and Elsworth, Y. and New, R. and Toutain, T.},
  year = {2008},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {384},
  number = {4},
  pages = {1668--1674},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.12833.x},
  abstract = {We seek to address whether solar-cycle frequency shifts of the Sun's low-l p modes 'distort' the underlying shapes of the mode peaks, when those peaks are observed in power frequency spectra made from data spanning large fractions, or more, of the cycle period. We present analytical descriptions of the expected profiles, and validate the predictions through use of artificial seismic time-series data, in which temporal variations of the oscillator frequencies are introduced. Our main finding is that for the Sun-like frequency shifts the distortion of the asymmetrical Lorentzian-like profiles is very small, but also just detectible. Our analysis indicates that by fitting modes to the usual Lorentzian-like models - which do not allow for the distortion - rather than new models we derive, there is a bias in the mode height and linewidth parameters that is comparable in size to the observational uncertainties given by multi-year data sets. Bias in the frequency parameter gives much less cause for worry, being over an order of magnitude smaller than the corresponding frequency uncertainties. The distortion discussed in this paper may need to be considered when multiyear Sun-like asteroseismic data sets are analysed on stars showing strong activity cycles. \textcopyright{} 2008 RAS.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/5KEDU6KA/Chaplin et al. - 2008(3).pdf}
}

@article{Chaplin2008e,
  title = {{{AsteroFLAG}} - {{From}} the {{Sun}} to the Stars},
  author = {Chaplin, W. J. and Appourchaux, T. and Arentoft, T. and Ballot, J. and Baudin, F. and Bazot, M. and Bedding, T. R. and {Christensen-Dalsgaard}, J. and Creevey, O. L. and Duez, V. and Elsworth, Y. and Fletcher, S. T. and Garc{\'i}a, R. A. and Gough, D. O. and Jim{\'e}nez, A. and {Jim{\'e}nez-Reyes}, S. J. and Houdek, G. and Kjeldsen, H. and Lazrek, M. and Leibacher, W. and Monteiro, M. J.P.F.G. and Neiner, C. and New, R. and R{\'e}gulo, C. and Salabert, D. and Samadi, R. and Sekii, T. and Sousa, S. G. and Toutain, T. and {Turck-Chi{\`e}ze}, S.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012048},
  abstract = {We stand on the threshold of a critical expansion of asteroseismology of Sun-like stars, the study of stellar interiors by observation and analysis of their global acoustic modes of oscillation. The Sun-like oscillations give a very rich spectrum allowing the internal structure and dynamics to be probed down into the stellar cores to very high precision. Asteroseismic observations of many stars will allow multiple-point tests of crucial aspects of stellar evolution and dynamo theory. The aims of the asteroFLAG collaboration are to help the community to refine existing, and to develop new, methods for analysis of the asteroseismic data on the Sun-like oscillators. \textcopyright{} 2008 IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VMJX3S48/Chaplin et al. - 2008(4).pdf}
}

@article{Chaplin2008f,
  title = {{{AsteroFLAG}}: {{First}} Results from Hare-and-Hounds Exercise \#1},
  author = {Chaplin, W. J. and Appourchaux, T. and Arentoft, T. and Ballot, J. and {Christensen-Dalsgaard}, J. and Creevey, O. L. and Elsworth, Y. and Fletcher, S. T. and Garc{\'i}a, R. A. and Houdek, G. and {Jim{\'e}nez-Reyes}, S. J. and Kjeldsen, H. and New, R. and R{\'e}gulo, C. and Salabert, D. and Sekii, T. and Sousa, S. G. and Toutain, T.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  pages = {549--557},
  issn = {00046337},
  doi = {10.1002/asna.200710995},
  abstract = {We report on initial results from the first phase of Exercise \#1 of the asteroFLAG hare and hounds. The asteroFLAG group is helping to prepare for the asteroseismology component of NASA's Kepler mission, and the first phase of Exercise \#1 is concerned with testing extraction of estimates of the large and small frequency spacings of the low-degree p modes from Kepler-like artificial data. These seismic frequency spacings will provide key input for complementing the exoplanet search data. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {notion,notion-database,Space vehicles: instruments,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/77AZ5CB9/Chaplin et al. - 2008(6).pdf}
}

@article{Chaplin2008g,
  title = {Challenges for Asteroseismic Analysis of {{Sun-like}} Stars},
  author = {Chaplin, W. J. and Houdek, G. and Appourchaux, T. and Elsworth, Y. and New, R. and Toutain, T.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {485},
  number = {3},
  pages = {813--822},
  issn = {14320746},
  doi = {10.1051/0004-6361:200809695},
  abstract = {Context. Asteroseismology of Sun-like stars is undergoing rapid expansion with, for example, new data from the CoRoT mission and continuation of ground-based campaigns. There is also the exciting upcoming prospect of NASA's Kepler mission, which will allow the asteroseismic study of several hundred Sun-like targets, in some cases for periods lasting up to a few years. Aims. The seismic mode parameters are the input data needed for making inference on stars and their internal structures. In this paper we discuss the ease with which it will be possible to extract estimates of individual mode parameters, dependent on the mass, age, and visual brightness of the star. Our results are generally applicable; however, we look at mode detectability in the context of the upcoming Kepler observations. Methods. To inform our discussions we make predictions of various seismic parameters. To do this we use simple empirical scaling relations and detailed pulsation computations of the stochastic excitation and damping characteristics of the Sun-like p modes. Results. The issues related to parameter extraction on individual p modes discussed here are mode detectability, the detectability and impact of stellar activity cycles, and the ability to measure properties of rotationally split components, which is dependent on the relative importance of the rotational characteristics of the star and the damping of the stochastically excited p modes.},
  keywords = {Methods: Data analysis,notion,notion-database,Stars: Activity,Stars: Interiors,Stars: Oscillations,Sun: Helioseismology},
  file = {/Users/lbugnet/Zotero/storage/QEHA7J49/Chaplin et al. - 2008(5).pdf}
}

@article{Chaplin2008h,
  title = {Perspectives in Global Helioseismology and the Road Ahead},
  author = {Chaplin, William J. and Basu, Sarbani},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  eprint = {0801.4213},
  pages = {53--75},
  issn = {00380938},
  doi = {10.1007/s11207-008-9136-5},
  abstract = {We review the impact of global helioseismology on key questions concerning the internal structure and dynamics of the Sun and consider the exciting challenges the field faces as it enters a fourth decade of science exploitation. We do so with an eye on the past, looking at the perspectives global helioseismology offered in its earlier phases, in particular the mid-to-late 1970s and the 1980s. We look at how modern, higher quality, longer datasets coupled with new developments in analysis have altered, refined, and changed some of those perspectives and opened others that were not previously available for study. We finish by discussing outstanding challenges and questions for the field. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {Abundances,Activity,Magnetic fields,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/J5L5XQ84/Chaplin, Basu - 2008.pdf}
}

@article{Chaplin2009,
  title = {Mode Lifetimes of Stellar Oscillations {{Implications}} for Asteroseismology},
  author = {Chaplin, W. J. and Houdek, G. and Karoff, C. and Elsworth, Y. and New, R.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {500},
  number = {2},
  pages = {10--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/200911952},
  abstract = {Context. Successful inference from, asteroseismology relies on at least two factors: that the oscillations in the stars have amplitudes large enough to be clearly observable, and that the oscillations themselves be stable enough to enable precise measurements of mode frequencies and other parameters. Solar-like p modes are damped by convection, and hence the stability of the modes depends on the lifetime. Aims. We seek a simple scaling relation between the mean lifetime of the most prominent solar-like p modes in stars, and the fundamental stellar parameters. Methods. We base our search for a relation on the use of stellar equilibrium, and pulsation computations of a grid of stellar models, and the first asteroseismic results on lifetimes of main-sequence, sub-giant and red-giant stars. Results. We find that the mean lifetimes of all three classes of solar-like stars scale like T-4eff (where T eff is the effective temperature). When this relation is combined with the well-known scaling relation of Kjeldsen \& Bedding for mode amplitudes observed in narrowband intensity observations, we obtain the unexpected result that the height (the maximum power spectral density) of mode peaks in the frequency power spectrum, scales as g-2 (where g is the surface gravity). As it is the mode height (and not the amplitude) that fixes the S/N at which the modes can be measured, and as g changes only slowly along the main, sequence, this suggests that stars cooler than the Sun might be as good targets for asteroseismology as their hotter counterparts. When observations are instead, made in Doppler velocity, our results imply that mode height does increase with increasing effective temperature. \textcopyright{} ESO 2009.},
  keywords = {Convection,Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/429FRYM9/Chaplin et al. - 2009.pdf}
}

@article{Chaplin2009a,
  title = {Excitation and {{Damping}} of P-Mode {{Oscillations}} of {$\alpha$} {{Cen B}}},
  author = {Chaplin, W. J. and Houdek, G. and Elsworth, Y. and New, R. and Bedding, T. R. and Kjeldsen, H.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {692},
  number = {1},
  pages = {531--537},
  issn = {15384357},
  doi = {10.1088/0004-637X/692/1/531},
  abstract = {This paper presents an analysis of observational data on the p-mode spectrum of the star {$\alpha$} Cen B, and a comparison with theoretical computations of the stochastic excitation and damping of the modes. We find that at frequencies {$\greaterequivlnt$}4500 {$\mu$}Hz, the model damping rates appear to be too weak to explain the observed shape of the power spectral density of {$\alpha$} Cen B. The conclusion rests on the assumption that most of the disagreement is due to problems modeling the damping rates, not the excitation rates, of the modes. This assumption is supported by a parallel analysis of BiSON Sun-as-a-star data, for which it is possible to use analysis of very long timeseries to place tight constraints on the assumption. The BiSON analysis shows that there is a similar high-frequency disagreement between theory and observation in the Sun. We demonstrate that by using suitable comparisons of theory and observation it is possible to make inference on the dependence of the p-mode linewidths on frequency, without directly measuring those linewidths, even though the {$\alpha$} Cen B dataset is only a few nights long. Use of independent measures from a previous study of the {$\alpha$} Cen B linewidths in two parts of its spectrum also allows us to calibrate our linewidth estimates for the star. The resulting calibrated linewidth curve looks similar to a frequency-scaled version of its solar cousin, with the scaling factor equal to the ratio of the respective acoustic cut-off frequencies of the two stars. The ratio of the frequencies at which the onset of high-frequency problems is seen in both stars is also given approximately by the same scaling factor. \textcopyright{} 2009. The American Astronomical Society. All rights reserved.},
  keywords = {methods: data analysis,notion,notion-database,stars: activity,stars: oscillations,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/ZJNU8KSS/Chaplin et al. - 2009(2).pdf}
}

@article{Chaplin2010,
  title = {The Asteroseismic Potential of Kepler: {{First}} Results for Solar-Type Stars},
  author = {Chaplin, W. J. and Appourchaux, T. and Elsworth, Y. and Garc{\'i}a, R. A. and Houdek, G. and Karoff, C. and Metcalfe, T. S. and {Molenda-Akowicz}, J. and Monteiro, M. J.P.F.G. and Thompson, M. J. and Brown, T. M. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kjeldsen, H. and Borucki, W. J. and Koch, D. and Jenkins, J. M. and Ballot, J. and Basu, S. and Bazot, M. and Bedding, T. R. and Benomar, O. and Bonanno, A. and Brand{\~a}o, I. M. and Bruntt, H. and Campante, T. L. and Creevey, O. L. and Mauro, M. P.Di and Doan, G. and Dreizler, S. and Eggenberger, P. and Esch, L. and Fletcher, S. T. and Frandsen, S. and Gai, N. and Gaulme, P. and Handberg, R. and Hekker, S. and Howe, R. and Huber, D. and Korzennik, S. G. and Lebrun, J. C. and Leccia, S. and Martic, M. and Mathur, S. and Mosser, B. and New, R. and Quirion, P. O. and R{\'e}gulo, C. and Roxburgh, I. W. and Salabert, D. and Schou, J. and Sousa, S. G. and Stello, D. and Verner, G. A. and Arentoft, T. and Barban, C. and Belkacem, K. and Benatti, S. and Biazzo, K. and Boumier, P. and Bradley, P. A. and Broomhall, A. M. and Buzasi, D. L. and Claudi, R. U. and Cunha, M. S. and D'Antona, F. and Deheuvels, S. and Derekas, A. and Hernndez, A. Garc{\'i}a and Giampapa, M. S. and Goupil, M. J. and Gruberbauer, M. and Guzik, J. A. and Hale, S. J. and Ireland, M. J. and Kiss, L. L. and Kitiashvili, I. N. and Kolenberg, K. and Korhonen, H. and Kosovichev, A. G. and Kupka, F. and Lebreton, Y. and Leroy, B. and Ludwig, H. G. and Mathis, S. and Michel, E. and Miglio, A. and Montalbn, J. and Moya, A. and Noels, A. and Noyes, R. W. and Pall{\'e}, P. L. and Piau, L. and Preston, H. L. and Cort{\'e}s, T. Roca and Roth, M. and Sato, K. H. and Schmitt, J. and Serenelli, A. M. and Aguirre, V. Silva and Stevens, I. R. and Surez, J. C. and Suran, M. D. and Trampedach, R. and {Turck-Chi{\`e}ze}, S. and Uytterhoeven, K. and Ventura, R. and Wilson, P. A.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  pages = {169--175},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L169},
  abstract = {We present preliminary asteroseismic results from Kepler on three G-type stars. The observations, made at one-minute cadence during the first 33.5days of science operations, reveal high signal-to-noise solar-like oscillation spectra in all three stars: about 20 modes of oscillation may be clearly distinguished in each star. We discuss the appearance of the oscillation spectra, use the frequencies and frequency separations to provide first results on the radii, masses, and ages of the stars, and comment in the light of these results on prospects for inference on other solar-type stars that Kepler will observe. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,Stars: interiors,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/SUK9C2JC/Chaplin et al. - 2010.pdf}
}

@article{Chaplin2011,
  title = {Predicting the Detectability of Oscillations in Solar-Type Stars Observed by {{Kepler}}},
  author = {Chaplin, W J and Kjeldsen, H and Bedding, T R and {Christensen-Dalsgaard}, J and Gilliland, R L and Kawaler, S D and Appourchaux, T and Elsworth, Y and Garc{\'i}a, R A and Houdek, G and Karoff, C and Metcalfe, T S and {Molenda-}, J and P F G Monteiro, M J and Thompson, M J and Verner, G A and Batalha, N and Borucki, W J and Brown, T M and Bryson, S T and Christiansen, J L and Clarke, B D and Jenkins, J M and Klaus, T C and Koch, D and An, D and Ballot, J and Basu, S and Benomar, O and Bonanno, A and Broomhall, A-m and Campante, T L and Gaulme, P and Hale, S J and Handberg, R and Hekker, S and Huber, D and Mathur, S and Mosser, B and New, R and Pinsonneault, M H and Pricopi, D and Quirion, P-o and R{\'e}gulo, C and Roxburgh, I W and Salabert, D and Stello, D and Suran, M D},
  year = {2011},
  journal = {The Astrophysical Journal},
  volume = {732},
  number = {1},
  eprint = {1103.0702v1},
  urldate = {2021-01-16},
  abstract = {Asteroseismology of solar-type stars has an important part to play in the exoplanet program of the NASA Kepler Mission. Precise and accurate inferences on the stellar properties that are made possible by the seismic data allow very tight constraints to be placed on the exoplanetary systems. Here, we outline how to make an estimate of the detectability of solar-like oscillations in any given Kepler target, using rough estimates of the temperature and radius, and the Kepler apparent magnitude.},
  archiveprefix = {arxiv},
  keywords = {interiors-stars,late-type,notion,notion-database,oscillations-stars,stars,stars: interiors,stars: late-type,stars: oscillations,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/9DHREDZF/full-text.pdf;/Users/lbugnet/Zotero/storage/9FWDTKVR/Chaplin et al. - 2011(2).pdf}
}

@article{Chaplin2011,
  title = {Evidence for the Impact of Stellar Activity on the Detectability of Solar-like Oscillations Observed by {{Kepler}}},
  author = {Chaplin, W. J. and Bedding, T. R. and Bonanno, A. and Broomhall, A. M. and Garc{\'i}a, R. A. and Hekker, S. and Huber, D. and Verner, G. A. and Basu, S. and Elsworth, Y. and Houdek, G. and Mathur, S. and Mosser, B. and New, R. and Stevens, I. R. and Appourchaux, T. and Karoff, C. and Metcalfe, T. S. and {Molenda-Zakowicz}, J. and Monteiro, M. J.P.F.G. and Thompson, M. J. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kawaler, S. D. and Kjeldsen, H. and Ballot, J. and Benomar, O. and Corsaro, E. and Campante, T. L. and Gaulme, P. and Hale, S. J. and Handberg, R. and Jarvis, E. and R{\'e}gulo, C. and Roxburgh, I. W. and Salabert, D. and Stello, D. and Mullally, F. and Li, J. and Wohler, W.},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {732},
  number = {1 PART II},
  eprint = {1103.5570},
  issn = {20418213},
  doi = {10.1088/2041-8205/732/1/L5},
  abstract = {We use photometric observations of solar-type stars, made by the NASA Kepler Mission, to conduct a statistical study of the impact of stellar surface activity on the detectability of solar-like oscillations. We find that the number of stars with detected oscillations falls significantly with increasing levels of activity. The results present strong evidence for the impact of magnetic activity on the properties of near-surface convection in the stars, which appears to inhibit the amplitudes of the stochastically excited, intrinsically damped solar-like oscillations. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: activity,stars: interiors,stars: late-type,stars: magnetic field,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/PRVLP9WK/Chaplin et al. - 2011.pdf}
}

@article{Chaplin2011b,
  title = {Ensemble {{Asteroseismology}} of {{Solar-Type Stars}} with The},
  author = {Chaplin, W J and Kjeldsen, H and Basu, S and Miglio, A and Appourchaux, T and Bedding, T R and Elsworth, Y and Garc{\'i}a, R A and Gilliland, R L and Girardi, L and Houdek, G and Karoff, C and Kawaler, S D and Metcalfe, T S and {Molenda-}, J {\.Z} and Monteiro, M J P F G},
  year = {2011},
  volume = {332},
  number = {April},
  pages = {213--217},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BRTEF3U9/Chaplin et al. - 2011(3).pdf}
}

@article{Chaplin2013,
  title = {Asteroseismic Determination of Obliquities of the Exoplanet Systems Kepler-50 and Kepler-65},
  author = {Chaplin, W. J. and {Sanchis-Ojeda}, R. and Campante, T. L. and Handberg, R. and Stello, D. and Winn, J. N. and Basu, S. and {Christensen-Dalsgaard}, J. and Davies, G. R. and Metcalfe, T. S. and Buchhave, L. A. and Fischer, D. A. and Bedding, T. R. and Cochran, W. D. and Elsworth, Y. and Gilliland, R. L. and Hekker, S. and Huber, D. and Isaacson, H. and Karoff, C. and Kawaler, S. D. and Kjeldsen, H. and Latham, D. W. and Lund, M. N. and Lundkvist, M. and Marcy, G. W. and Miglio, A. and Barclay, T. and Lissauer, J. J.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {766},
  number = {2},
  eprint = {1302.3728},
  issn = {15384357},
  doi = {10.1088/0004-637X/766/2/101},
  abstract = {Results on the obliquity of exoplanet host stars - the angle between the stellar spin axis and the planetary orbital axis - provide important diagnostic information for theories describing planetary formation. Here we present the first application of asteroseismology to the problem of stellar obliquity determination in systems with transiting planets and Sun-like host stars. We consider two systems observed by the NASA Kepler mission which have multiple transiting small (super-Earth sized) planets: the previously reported Kepler-50 and a new system, Kepler-65, whose planets we validate in this paper. Both stars show rich spectra of solar-like oscillations. From the asteroseismic analysis we find that each host has its rotation axis nearly perpendicular to the line of sight with the sines of the angles constrained at the 1{$\sigma$} level to lie above 0.97 and 0.91, respectively. We use statistical arguments to show that coplanar orbits are favored in both systems, and that the orientations of the planetary orbits and the stellar rotation axis are correlated. \textcopyright{} 2013. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,planets and satellites: formation,planets and satellites: general,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/UVUN7LWQ/Chaplin et al. - 2013.pdf}
}

@article{Chaplin2013a,
  title = {Asteroseismology of {{Solar-Type}} and {{Red-Giant Stars}}},
  author = {Chaplin, William J. and Miglio, Andrea},
  year = {2013},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {51},
  number = {1},
  eprint = {1303.1957},
  pages = {353--392},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-082812-140938},
  abstract = {We are entering a golden era for stellar physics driven by satellite and telescope observations of unprecedented quality and scope. New insights on stellar evolution and stellar interiors physics are being made possible by asteroseismology, the study of stars by the observation of natural, resonant oscillations. Asteroseismology is proving to be particularly significant for the study of solar-type and red-giant stars. These stars show rich spectra of solar-like oscillations, which are excited and intrinsically damped by turbulence in the outermost layers of the convective envelopes. In this review we discuss the current state of the field, with a particular emphasis on recent advances provided by the Kepler and CoRoT space missions and the wider significance to astronomy of the results from asteroseismology, such as stellar populations studies and exoplanet studies.},
  archiveprefix = {arxiv},
  keywords = {galaxy,late-type,notion,notion-database,oscillations,planet-star interactions,solar-type,stars,stellar content},
  file = {/Users/lbugnet/Zotero/storage/RTCNG598/Chaplin, Miglio - 2013.pdf}
}

@article{Chaplin2014,
  title = {Asteroseismic Fundamental Properties of Solar-Type Stars Observed by the {{NASA Kepler}} Mission},
  author = {Chaplin, W. J. and Basu, S. and Huber, D. and Serenelli, A. and Casagrande, L. and Silva Aguirre, V. and Ball, W. H. and Creevey, O. L. and Gizon, L. and Handberg, R. and Karoff, C. and Lutz, R. and Marques, J. P. and Miglio, A. and Stello, D. and Suran, M. D. and Pricopi, D. and Metcalfe, T. S. and Monteiro, M. J.P.F.G. and {Molenda-Zakowicz}, J. and Appourchaux, T. and {Christensen-Dalsgaard}, J. and Elsworth, Y. and Garc{\'i}a, R. A. and Houdek, G. and Kjeldsen, H. and Bonanno, A. and Campante, T. L. and Corsaro, E. and Gaulme, P. and Hekker, S. and Mathur, S. and Mosser, B. and R{\'e}gulo, C. and Salabert, D.},
  year = {2014},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {210},
  number = {1},
  issn = {00670049},
  doi = {10.1088/0067-0049/210/1/1},
  abstract = {We use asteroseismic data obtained by the NASA Kepler mission to estimate the fundamental properties of more than 500 main-sequence and sub-giant stars. Data obtained during the first 10 months of Kepler science operations were used for this work, when these solar-type targets were observed for one month each in survey mode. Stellar properties have been estimated using two global asteroseismic parameters and complementary photometric and spectroscopic data. Homogeneous sets of effective temperatures, T eff, were available for the entire ensemble from complementary photometry; spectroscopic estimates of T eff and [Fe/H] were available from a homogeneous analysis of ground-based data on a subset of 87 stars. We adopt a grid-based analysis, coupling six pipeline codes to 11 stellar evolutionary grids. Through use of these different grid-pipeline combinations we allow implicitly for the impact on the results of stellar model dependencies from commonly used grids, and differences in adopted pipeline methodologies. By using just two global parameters as the seismic inputs we are able to perform a homogenous analysis of all solar-type stars in the asteroseismic cohort, including many targets for which it would not be possible to provide robust estimates of individual oscillation frequencies (due to a combination of low signal-to-noise ratio and short dataset lengths). The median final quoted uncertainties from consolidation of the grid-based analyses are for the full ensemble (spectroscopic subset) approximately 10.8\% (5.4\%) in mass, 4.4\% (2.2\%) in radius, 0.017 dex (0.010 dex) in log g, and 4.3\% (2.8\%) in mean density. Around 36\% (57\%) of the stars have final age uncertainties smaller than 1 Gyr. These ages will be useful for ensemble studies, but should be treated carefully on a star-by-star basis. Future analyses using individual oscillation frequencies will offer significant improvements on up to 150 stars, in particular for estimates of the ages, where having the individual frequency data is most important. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,stars: fundamental parameters,stars: interiors},
  file = {/Users/lbugnet/Zotero/storage/IWTSTMZQ/Chaplin et al. - 2014.pdf}
}

@article{Chaplin2014a,
  title = {Super-{{Nyquist}} Asteroseismology of Solar-like Oscillators with {{Kepler}} and {{K2}} - Expanding the Asteroseismic Cohort at the Base of the Red Giant Branch},
  author = {Chaplin, W. J. and Elsworth, Y. and Davies, G. R. and Campante, T. L. and Handberg, R. and Miglio, A. and Basu, S.},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {445},
  number = {1},
  pages = {946--954},
  issn = {13652966},
  doi = {10.1093/mnras/stu1811},
  abstract = {We consider the prospects for detecting solar-like oscillations in the 'super-Nyquist' regime of long-cadence (LC) Kepler photometry, i.e. above the associated Nyquist frequency of {$\simeq$} 283 {$\mu$}Hz. Targets of interest are cool, evolved subgiants and stars lying at the base of the red giant branch. These stars would ordinarily be studied using the short-cadence (SC) data, since the associated SC Nyquist frequency lies well above the frequencies of the detectable oscillations. However, the number of available SC target slots is quite limited. This imposes a severe restriction on the size of the ensemble available for SC asteroseismic study.We find that archival Kepler LC data from the nominal mission may be utilized for asteroseismic studies of targets whose dominant oscillation frequencies lie as high as {$\simeq$}500 {$\mu$}Hz, i.e. about 1.75-times the LC Nyquist frequency. The frequency detection threshold for the shorter duration science campaigns of the re-purposed Kepler mission, K2, is lower. The maximum threshold will probably lie somewhere between {$\simeq$}400 and 450 {$\mu$}Hz. The potential to exploit the archival Kepler and K2 LC data in this manner opens the door to increasing significantly the number of subgiant and low-luminosity red giant targets amenable to asteroseismic analysis, overcoming target limitations imposed by the small number of SC slots.We estimate that around 400 such targets are now available for study in the Kepler LC archive. That number could potentially be a lot higher for K2, since there will be a new target list for each of its campaigns.},
  keywords = {asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/CTLR9Y42/Chaplin et al. - 2014(2).pdf}
}

@article{Chaplin2014b,
  title = {Inferences on {{Stellar Activity}} and {{Stellar Cycles}} from {{Asteroseismology}}},
  author = {Chaplin, William J. and Basu, Sarbani},
  year = {2014},
  journal = {Space Science Reviews},
  volume = {186},
  number = {1-4},
  pages = {437--456},
  issn = {15729672},
  doi = {10.1007/s11214-014-0090-2},
  abstract = {The solar activity cycle can be studied using many different types of observations, such as counting sunspots, measuring emission in the Ca~II H\&K lines, magnetograms, radio emissions, etc. One of the more recent ways of studying solar activity is to use the changing properties of solar oscillations. Stellar activity cycles are generally studied using the Ca~II lines, or sometimes using photometry. Asteroseismology is potentially an exciting means of studying these cycles. In this article we examine whether or not asteroseismic data can be used for this purpose, and what the asteroseismic signatures of stellar activity are. We also examine how asteroseismology may help in more indirect ways.},
  keywords = {notion,notion-database,Stars: activity,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/QVK5ZLRS/Chaplin, Basu - 2014.pdf}
}

@article{Chaplin2015a,
  title = {Asteroseismology of {{Solar-Type Stars}} with {{K2}} : {{Detection}} of {{Oscillations}} in {{C1 Data}}},
  author = {Chaplin, W. J. and Lund, M. N. and Handberg, R. and Basu, S. and Buchhave, L. A. and Campante, T. L. and Davies, G. R. and Huber, D. and Latham, D. W. and Latham, C. A. and Serenelli, A. and Antia, H. M. and Appourchaux, T. and Ball, W. H. and Benomar, O. and Casagrande, L. and {Christensen-Dalsgaard}, J. and Coelho, H. R. and Creevey, O. L. and Elsworth, Y. and Garc{\'i}a, R. A. and Gaulme, P. and Hekker, S. and Kallinger, T. and Karoff, C. and Kawaler, S. D. and Kjeldsen, H. and Lundkvist, M. S. and Marcadon, F. and Mathur, S. and Miglio, A. and Mosser, B. and R{\'e}gulo, C. and Roxburgh, I. W. and Silva Aguirre, V. and Stello, D. and Verma, K. and White, T. R. and Bedding, T. R. and Barclay, T. and Buzasi, D. L. and Dehuevels, S. and Gizon, L. and Houdek, G. and Howell, S. B. and Salabert, D. and Soderblom, D. R.},
  year = {2015},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {127},
  number = {956},
  eprint = {1507.01827},
  pages = {1038--1044},
  issn = {00046280},
  doi = {10.1086/683103},
  abstract = {\textcopyright{} 2015, The Astronomical Society of the Pacific. All rights reserved. We present the first detections by the NASA K2 mission of oscillations in solar-type stars, using short-cadence data collected during K2 Campaign 1 (C1). We understand the asteroseismic detection thresholds for C1-like levels of photometric performance, and we can detect oscillations in subgiants having dominant oscillation frequencies around 1000 {$\mu$}Hz. Changes to the operation of the fine-guidance sensors are expected to give significant improvements in the high-frequency performance from C3 onwards. A reduction in the excess high-frequency noise by a factor of 2.5 in amplitude would bring main-sequence stars with dominant oscillation frequencies as high as {$\simeq$}2500 {$\mu$}Hz into play as potential asteroseismic targets for K2.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CKU2R84W/Chaplin et al. - 2015.pdf}
}

@article{Chaplin2020,
  title = {Age Dating of an Early {{Milky Way}} Merger via Asteroseismology of the Naked-Eye Star \$\textbackslash nu\$ {{Indi}}},
  author = {Chaplin, William J. and Serenelli, Aldo M. and Miglio, Andrea and Morel, Thierry and Mackereth, J. Ted and Vincenzo, Fiorenzo and Basu, Hans Kjeldsen Sarbani and Ball, Warrick H. and Stokholm, Amalie and Verma, Kuldeep and Mosumgaard, Jakob R{\o}rsted and Aguirre, Victor Silva and Mazumdar, Anwesh and Ranadive, Pritesh and Antia, H. M. and Lebreton, Yveline and Ong, Joel and Appourchaux, Thierry and Bedding, Timothy R. and {Christensen-Dalsgaard}, J{\o}rgen and Creevey, Orlagh and Garc{\'i}a, Rafael A. and Handberg, Rasmus and Huber, Daniel and Kawaler, Steven D. and Lund, Mikkel N. and Metcalfe, Travis S. and Stassun, Keivan G. and Bazot, Mich{\"a}el and Beck, Paul and Bell, Keaton J. and Bergemann, Maria and Buzasi, Derek L. and Benomar, Othman and Bossini, Diego and Bugnet, Lisa and Campante, Tiago L. and Orhan, Zeynep {\c C}elik and Corsaro, Enrico and {Gonz{\'a}lez-Cuesta}, Luc{\'i}a and Davies, Guy R. and Di Mauro, Maria Pia and Egeland, Ricky and Elsworth, Yvonne P. and Gaulme, Patrick and Ghasemi, Hamed and Guo, Zhao and Hall, Oliver J. and Hasanzadeh, Amir and Hekker, Saskia and Howe, Rachel and Jenkins, Jon M. and Jim{\'e}nez, Antonio and Kiefer, Ren{\'e} and Kuszlewicz, James S. and Kallinger, Thomas and Latham, David W. and Lundkvist, Mia S. and Mathur, Savita and Montalb{\'a}n, Josefina and Mosser, Benoit and Bed{\'o}n, Andres Moya and Nielsen, Martin Bo and {\"O}rtel, Sibel and Rendle, Ben M. and Ricker, George R. and Rodrigues, Tha{\'i}se S. and Roxburgh, Ian W. and Safari, Hossein and Schofield, Mathew and Seager, Sara and Smalley, Barry and Stello, Dennis and Szab{\'o}, R{\'o}bert and Tayar, Jamie and Theme{\ss}l, Nathalie and Thomas, Alexandra E. L. and Vanderspek, Roland K. and {van Rossem}, Walter E. and Vrard, Mathieu and Weiss, Achim and White, Timothy R. and Winn, Joshua N. and Y{\i}ld{\i}z, Mutlu},
  year = {2020},
  month = jan,
  journal = {Nature Astronomy},
  volume = {4},
  eprint = {2001.04653},
  pages = {383--389},
  doi = {10.1038/s41550-019-0975-9},
  urldate = {2020-01-16},
  abstract = {Over the course of its history, the Milky Way has ingested multiple smaller satellite galaxies. While these accreted stellar populations can be forensically identified as kinematically distinct structures within the Galaxy, it is difficult in general to precisely date the age at which any one merger occurred. Recent results have revealed a population of stars that were accreted via the collision of a dwarf galaxy, called \textbackslash textit\{Gaia\}-Enceladus, leading to a substantial pollution of the chemical and dynamical properties of the Milky Way. Here, we identify the very bright, naked-eye star \$\textbackslash nu\$\textbackslash,Indi as a probe of the age of the early in situ population of the Galaxy. We combine asteroseismic, spectroscopic, astrometric, and kinematic observations to show that this metal-poor, alpha-element-rich star was an indigenous member of the halo, and we measure its age to be \$11.0 \textbackslash pm 0.7\$ (stat) \$\textbackslash pm 0.8\$ (sys)\$\textbackslash,\textbackslash rm Gyr\$. The star bears hallmarks consistent with it having been kinematically heated by the \textbackslash textit\{Gaia\}-Enceladus collision. Its age implies that the earliest the merger could have begun was 11.6 and 13.2 Gyr ago at 68 and 95\% confidence, respectively. Input from computations based on hierarchical cosmological models tightens (i.e. reduces) slightly the above limits.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PRRMJPWG/2001.04653.pdf}
}

@article{Chapman1986,
  title = {Solar Irradiance Variations Derived from Magnetograms},
  author = {Chapman, Gary A. and Boyden, J.E.},
  year = {1986},
  journal = {The Astrophysical Journal},
  volume = {302},
  eprint = {1011.1669v3},
  pages = {71--73},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YCN63W7Z/Chapman, Boyden - 1986.pdf}
}

@incollection{Chapter13Matrix,
  title = {Chapter 13: Matrix Elements of Irreductible Tensor Operators},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {2},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WCIJGAWJ/Unknown - Unknown(4).pdf}
}

@incollection{ChapterIrreductibleTensora,
  title = {Chapter 3: {{Irreductible}} Tensora},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SCKDHTJ2/Unknown - Unknown(18).pdf}
}

@incollection{ChapterWIGNERFUNCTIONS,
  title = {Chapter 4 {{WIGNER}} /\^{{FUNCTIONS}} 4.1.},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {5},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YB2SSQPE/Unknown - Unknown(14).pdf}
}

@article{Charbonneau1992,
  title = {Angular Momentum Transport in Magnetized Stellar Radiative Zones. {{I}} - {{Numerical}} Solutions to the Core Spin-up Model Problem},
  author = {Charbonneau, P. and MacGregor, K. B.},
  year = {1992},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {387},
  pages = {639},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/171114},
  urldate = {2020-06-06},
  abstract = {Abstract The present paper investigates the time evolution of the angular momentum and induced toroidal magnetic field distribution in an initially nonrotating radiative stellar envelope containing a large-scale poloidal magnetic field, following the impulsive spin-up ... \textbackslash n},
  keywords = {Angular Momentum,Astrophysics,Computational Astrophysics,Magnetic Diffusion,Magnetic Field Configurations,Magnetohydrodynamics,MAGNETOHYDRODYNAMICS: MHD,METHODS: NUMERICAL,Momentum Transfer,Navier,notion,notion-database,Poloidal Flux,Reynolds Number,STARS: INTERIORS,STARS: MAGNETIC FIELDS,STARS: ROTATION,Stellar Envelopes,Stellar Interiors,Stellar Magnetic Fields,Stellar Rotation,Stokes Equation},
  file = {/Users/lbugnet/Zotero/storage/H9IITF8G/full-text.pdf}
}

@article{Charbonneau1993,
  title = {Spin-Doan of Solar-Type Stars Wiht Internal Magnetic Fields},
  author = {Charbonneau, Paul and MacGregor, Keith B.},
  year = {1993},
  journal = {Inside the stars, IAU Colloquium 137},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YX4IUE5K/Charbonneau, MacGregor - 1993(2).pdf}
}

@article{Charbonneau1993,
  title = {Spin-down of Solar-Type Stars with Internal Magnetic Fields},
  author = {Charbonneau, Paul and MacGregor, Keith B.},
  year = {1993},
  journal = {Inside the stars, IAU Colloquium 137},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/B4VK6C39/Charbonneau, MacGregor - 1993.pdf}
}

@article{Charbonneau2000,
  title = {Detection of {{Planetary Transits Across}} a {{Sun-like Star}}},
  author = {Charbonneau, David and Brown, Timothy M. and Latham, David W. and Mayor, Michel},
  year = {2000},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {529},
  number = {1},
  eprint = {astro-ph/9911436},
  pages = {L45-L48},
  publisher = {{IOP Publishing}},
  issn = {0004637X},
  doi = {10.1086/312457},
  urldate = {2020-07-07},
  abstract = {We report high precision, high cadence photometric measurements of the star HD 209458, which is known from radial velocity measurements to have a planetary mass companion in a close orbit. We detect two separate transit events at times that are consistent with the radial velocity measurements. In both cases, the detailed shape of the transit curve due to both the limb darkening of the star and the finite size of the planet is clearly evident. Assuming stellar parameters of 1.1 R\_Sun and 1.1 M\_Sun, we find that the data are best interpreted as a gas giant with a radius of 1.27 +/- 0.02 R\_Jup in an orbit with an inclination of 87.1 +/- 0.2 degrees. We present values for the planetary surface gravity, escape velocity, and average density, and discuss the numerous observations that are warranted now that a planet is known to transit the disk of its parent star.},
  archiveprefix = {arxiv},
  keywords = {binaries,eclipsing-planetary systems-stars,individual (HD 209458)-techniques,notion,notion-database,photometric-techniques,radial velocities,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/WJ93Q8GQ/full-text.pdf}
}

@article{Charbonneau2001,
  title = {Magnetic {{Fields}} in {{Massive Stars}}. {{I}}. {{Dynamo Models}}},
  author = {Charbonneau, Paul and MacGregor, Keith B.},
  year = {2001},
  month = oct,
  journal = {The Astrophysical Journal},
  volume = {559},
  number = {2},
  pages = {1094--1107},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/322417},
  urldate = {2020-07-02},
  abstract = {ABSTRACT Motivated by mounting evidence for the presence of magnetic fields in the atmospheres of" normal" early-type main-sequence stars, we investigate the various possible modes of dynamo action in their convective core. Working within the framework ... \textbackslash n},
  keywords = {magnetic \DH elds,MHD \`E stars,notion,notion-database,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/JNRQQCVM/full-text.pdf}
}

@techreport{Charbonneau2005,
  title = {Dynamo {{Models}} of the {{Solar Cycle Living Reviews}} in {{Solar Physics}}},
  author = {Charbonneau, Paul},
  year = {2005},
  urldate = {2020-05-14},
  abstract = {This paper reviews recent advances and current debates in modeling the solar cycle as a hydromagnetic dynamo process. Emphasis is placed on (relatively) simple dynamo models that are nonetheless detailed enough to be comparable to solar cycle observations. After a brief overview of the dynamo problem and of key observational constraints, we begin by reviewing the various magnetic field regeneration mechanisms that have been proposed in the solar context. We move on to a presentation and critical discussion of extant solar cycle models based on these mechanisms. We then turn to the origin of fluctuations in these models, including amplitude and parity modulation, chaotic behavior, and intermittency. The paper concludes with a discussion of our current state of ignorance regarding various key questions, the most pressing perhaps being the identification of the physical mechanism(s) responsible for the generation of the Sun's poloidal magnetic field component.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TBR3WHZH/full-text.pdf}
}

@article{Charbonneau2013,
  title = {Modeling the Solar Dynamo},
  author = {Charbonneau, Paul and Smolarkiewicz, Piotr K.},
  year = {2013},
  month = apr,
  journal = {Science},
  volume = {340},
  number = {6128},
  pages = {42--43},
  publisher = {{American Association for the Advancement of Science}},
  issn = {10959203},
  doi = {10.1126/science.1235954},
  urldate = {2020-07-03},
  abstract = {Numerical simulations are changing our views on the dynamo process underlying the solar magnetic activity cycle.},
  keywords = {Astronomy,ASTRONOMY Physics,Computer-Science,notion,notion-database}
}

@article{Charbonneau2014,
  title = {Solar {{Dynamo Theory}}},
  author = {Charbonneau, Paul},
  year = {2014},
  volume = {7},
  pages = {18},
  doi = {10.1146/annurev-astro-081913-040012},
  urldate = {2020-05-13},
  abstract = {The Sun's magnetic field is the engine and energy source driving all phenomena collectively defining solar activity, which in turn structures the whole heliosphere and significantly impacts Earth's atmosphere down at least to the stratosphere. The solar magnetic field is believed to originate through the action of a hydromagnetic dynamo process operating in the Sun's interior , where the strongly turbulent environment of the convection zone leads to flow-field interactions taking place on an extremely wide range of spatial and temporal scales. Following a necessarily brief observational overview of the solar magnetic field and its cycle, this review on solar dynamo theory is structured around three areas in which significant advances have been made in recent years: (a) global magnetohydrodynamical simulations of convection and magnetic cycles, (b) the turbulent electromotive force and the dynamo saturation problem, and (c) flux transport dynamos, and their application to model cycle fluctuations and grand minima and to carry out cycle prediction.},
  keywords = {differential rotation,hydromagnetic dynamo,magnetohydrodynamics,notion,notion-database,solar cycle,Sun,turbulent convection}
}

@article{Charbonnel2013,
  title = {Impact of Internal Gravity Waves on the Rotation Profile inside Pre-Main Sequence Low-Mass Stars},
  author = {Charbonnel, C. and Decressin, T. and Amard, L. and Palacios, A. and Talon, S.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {554},
  pages = {1--14},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321277},
  abstract = {Aims. We study the impact of internal gravity waves (IGW), meridional circulation, shear turbulence, and stellar contraction on the internal rotation profile and surface velocity evolution of solar metallicity low-mass pre-main sequence stars. Methods. We compute a grid of rotating stellar evolution models with masses between 0.6 and 2.0 M{$\odot$} taking these processes into account for the transport of angular momentum, as soon as the radiative core appears and assuming no more disk-locking from that moment on. IGW generation along the PMS is computed taking Reynolds-stress and buoyancy into account in the bulk of the stellar convective envelope and convective core (when present). Redistribution of angular momentum within the radiative layers accounts for damping of prograde and retrograde IGW by thermal diffusivity and viscosity in corotation resonance. Results. Over the whole mass range considered, IGW are found to be efficiently generated by the convective envelope and to slow down the stellar core early on the PMS. In stars more massive than {$\sim$}1.6 M {$\odot$}, IGW produced by the convective core also contribute to angular momentum redistribution close to the ZAMS. Conclusions. Overall, IGW are found to significantly change the internal rotation profile of PMS low-mass stars. \textcopyright{} 2013 ESO.},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: low-mass,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/EDNUWKVM/Charbonnel et al. - 2013.pdf}
}

@article{Charbonnel2017,
  title = {The Magnetic Strip(s) in the Advanced Phases of Stellar Evolution - {{Theoretical}} Convective Turnover Timescale and {{Rossby}} Number for Low- and Intermediate-Mass Stars up to the {{AGB}} at Various Metallicities},
  author = {Charbonnel, C. and Decressin, T. and Lagarde, N. and Gallet, F. and Palacios, A. and Auriere, M. and {Konstantinova-Antova}, R. and Mathis, S. and Anderson, R. I. and Dintrans, B.},
  year = {2017},
  month = mar,
  eprint = {1703.10824},
  doi = {10.1051/0004-6361/201526724},
  urldate = {2020-07-22},
  abstract = {Recent spectropolarimetric observations of otherwise ordinary G, K, and M giants revealed localized magnetic strips in the HRD coincident with the regions where the first dredge-up and core He-burning occur. We seek to understand the origin of magnetic fields in such late-type giant stars. In analogy with late-type dwarf stars, we focus primarily on parameters known to influence the generation of magnetic fields in the outer convective envelope. We compute the classical dynamo parameters along the evolutionary tracks of low- and intermediate-mass stars at various metallicities using stellar models that have been extensively tested by spectroscopic and asteroseismic observations. These include convective turnover timescales and convective Rossby numbers, computed from the PMS to the tip of the RGB or the early AGB. To investigate the effects of the very extended outer convective envelope, we compute these parameters both for the entire convective envelope and locally, that is, at different depths within the envelope. We also compute the turnover timescales and corresponding Rossby numbers for the convective cores of intermediate-mass stars on the main sequence. Our models show that the Rossby number of the convective envelope becomes lower than unity in the well-delimited locations of the Hertzsprung-Russell diagram where magnetic fields have indeed been detected. We show that alpha-omega dynamo processes might not be continuously operating, but that they are favored in the stellar convective envelope at two specific moments along the evolution tracks, that is, during the first dredge-up at the base of the RGB and during central helium burning in the helium-burning phase and early-AGB. This general behavior can explain the so-called magnetic strips recently discovered by dedicated spectropolarimetric surveys of evolved stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{charbonnel2021,
  title = {The Behaviour of Lithium at High Metallicity in the {{Milky Way}}: {{Selection}} Effects in the Samples and the Possible Role of Atomic Diffusion},
  shorttitle = {The Behaviour of Lithium at High Metallicity in the {{Milky Way}}},
  author = {Charbonnel, C. and Borisov, S. and {de Laverny}, P. and Prantzos, N.},
  year = {2021},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {649},
  pages = {L10},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202140873},
  urldate = {2022-07-26},
  abstract = {Aims.               We revisit large spectroscopic data sets for field stars from the literature to derive the upper Li envelope in the high metallicity regime in our Galaxy.                                         Methods.               We take advantage of               Gaia               EDR3 data and state-of-the-art stellar models to precisely determine the position of the sample dwarf stars in the Hertzsprung-Russell diagram.                                         Results.               The highest Li abundances are found in field metal-rich warm dwarfs from the GALAH survey, located on the hot side of the Li-dip. Their mean Li value agrees with what was recently derived for warm dwarfs in metal-rich clusters, pointing towards a continuous increase of Li up to super-solar metallicity. However, if only cool dwarfs are considered in GALAH, as done in the other literature surveys, it is found that the upper Li envelope decreases at super-solar metallicities, blurring the actual Li evolution picture. We confirm the suggestion that field and open cluster surveys that found opposite Li behaviour in the high metallicity regime do not sample the same types of stars: The first ones, with the exception of GALAH, miss warm dwarfs that can potentially preserve their original Li content.                                         Conclusions.               Although we can discard the bending of the Li upper envelope at high metallicity derived from the analysis of cool star samples, we still need to evaluate the effects of atomic diffusion on warm, metal-rich early-F and late-A type dwarfs before deriving the actual Li abundance at high metallicity.},
  file = {/Users/lbugnet/Zotero/storage/UY7BRL9K/Charbonnel et al. - 2021 - The behaviour of lithium at high metallicity in th.pdf}
}

@article{Charpinet1997,
  title = {A {{Driving Mechanism}} for the {{Newly Discovered Class}} of {{Pulsating Subdwarf B Stars}}},
  author = {Charpinet, S. and Fontaine, G. and Brassard, P. and Chayer, P. and Rogers, F. J. and Iglesias, C. A. and Dorman, B.},
  year = {1997},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {483},
  number = {2},
  pages = {L123-L126},
  publisher = {{IOP Publishing}},
  issn = {0004637X},
  doi = {10.1086/310741},
  urldate = {2020-04-09},
  abstract = {We present new calculations that strongly reinforce the idea-originally proposed by Charpinet et al.-that pulsation modes are driven through an opacity bump due to a local enhancement of the iron abundance in the envelopes of sdB stars. Our improved models incorporate nonuniform iron abundance distributions obtained through the condition of diffusive equilibrium between gravitational settling and radiative levitation. They also include special Rosseland opacity tables that take into account the large variations of the iron abundance about the cosmic value that are predicted by equilibrium radiative levitation theory. For representative models with M = 0.48 M {$\odot$} and logg = 5.8, we find strong instabilities for low-order radial and nonradial (p and/) pulsation modes in the range 36,500 K {$\greaterequivlnt$} T eff S 29,000 K. The four pulsating sdB stars currently known all have effective temperatures in that range. In addition, one of our models with T eff = 34,000 K has a band of unstable modes with periods in the range 116-195 s, in excellent agreement with those of the known pulsators. We therefore claim that our proposed iron bump mechanism provides a natural explanation for the instabilities found in the newly discovered class of pulsating sdB stars. \textcopyright{} 1997. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,stars: interior,STARS: INTERIORS,Stars: Oscillations,STARS: OSCILLATIONS,Stars: Subdwarfs,STARS: SUBDWARFS},
  file = {/Users/lbugnet/Zotero/storage/JGVFIJLA/full-text.pdf}
}

@article{Charpinet2000,
  title = {Adiabatic {{Survey}} of {{Subdwarf B Star Oscillations}}. {{I}}. {{Pulsation Properties}} of a {{Representative Evolutionary Model}}},
  author = {Charpinet, S. and Fontaine, G. and Brassard, P. and Dorman, Ben},
  year = {2000},
  month = nov,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {131},
  number = {1},
  pages = {223--247},
  publisher = {{IOP Publishing}},
  issn = {0067-0049},
  doi = {10.1086/317359},
  urldate = {2020-04-09},
  keywords = {notion,notion-database,Stars: Interiors,Stars: Oscillations,Stars: Subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/JZ3KJM7T/full-text.pdf}
}

@article{Charpinet2002,
  title = {Adiabatic {{Survey}} of {{Subdwarf B Star Oscillations}}. {{II}}. {{Effects}} of {{Model Parameters}} on {{Pulsation Modes}}},
  author = {Charpinet, S. and Fontaine, G. and Brassard, P. and Dorman, Ben},
  year = {2002},
  month = apr,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {139},
  number = {2},
  pages = {487--537},
  publisher = {{IOP Publishing}},
  issn = {0067-0049},
  doi = {10.1086/338822},
  urldate = {2020-04-09},
  keywords = {notion,notion-database,Stars: Interiors,Stars: Oscillations,Stars: Subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/DQ6HD97L/full-text.pdf}
}

@article{Charpinet2002a,
  title = {Adiabatic {{Survey}} of {{Subdwarf B Star Oscillations}}. {{III}}. {{Effects}} of {{Extreme Horizontal Branch Stellar Evolution}} on {{Pulsation Modes}}},
  author = {Charpinet, S. and Fontaine, G. and Brassard, P. and Dorman, Ben},
  year = {2002},
  month = jun,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {140},
  number = {2},
  pages = {469--561},
  publisher = {{IOP Publishing}},
  issn = {0067-0049},
  doi = {10.1086/339707},
  urldate = {2020-04-09},
  keywords = {notion,notion-database,Stars: Interiors,Stars: Oscillations,Stars: Subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/SAX49T2G/full-text.pdf}
}

@article{Charpinet2009,
  title = {Seismic Evidence for the Loss of Stellar Angular Momentum before the White-Dwarf Stage},
  author = {Charpinet, S. and Fontaine, G. and Brassard, P.},
  year = {2009},
  month = sep,
  journal = {Nature},
  volume = {461},
  number = {7263},
  pages = {501--503},
  issn = {00280836},
  doi = {10.1038/nature08307},
  urldate = {2020-10-19},
  abstract = {White-dwarf stars represent the final products of the evolution of some 95\% of all stars. If stars were to keep their angular momentum throughout their evolution, their white-dwarf descendants, owing to their compact nature, should all rotate relatively rapidly, with typical periods of the order of a few seconds. Observations of their photospheres show, in contrast, that they rotate much more slowly, with periods ranging from hours to tens of years. It is not known, however, whether a white dwarf could hide some of its original angular momentum below the superficial layers, perhaps spinning much more rapidly inside than at its surface. Here we report a determination of the internal rotation profile of a white dwarf using a method based on asteroseismology. We show that the pulsating white dwarf PG 1159-035 rotates as a solid body (encompassing more than 97.5\% of its mass) with the relatively long period of 33.61 0.59 h. This implies that it has lost essentially all of its angular momentum, thus favouring theories which suggest important angular momentum transfer and loss in evolutionary phases before the white-dwarf stage. \textcopyright{} 2009 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6B6JU6M5/full-text.pdf}
}

@article{Charpinet2013,
  title = {Asteroseismology of Hot {{B}} Subdwarf Stars},
  author = {Charpinet, S. and Van Grootel, V. and Brassard, P. and Fontaine, G. and Green, E.M. and Randall, S.K.},
  editor = {Montalb{\'a}n, J. and Noels, A. and Van Grootel, V.},
  year = {2013},
  journal = {EPJ Web of Conferences},
  volume = {43},
  pages = {04005},
  issn = {2100-014X},
  doi = {10.1051/epjconf/20134304005},
  urldate = {2023-10-02},
  abstract = {Non-radial pulsations in Extreme Horizontal Branch stars (also known as hot B subdwarfs or sdB stars) offer strong opportunities to study, through asteroseismology, the structure and internal dynamics of stars in this intermediate stage of stellar evolution. Most sdB stars directly descend from former red giants and are expected to evolve straight into white dwarfs after core helium exhaustion. They thus represent the most direct link between these two stages. Their properties should therefore reflect both the outcome of the core evolution of red giant stars and the initial state for a fraction of the white dwarfs. We review the status of this field after a decade of efforts to exploit both p-mode and g-mode pulsating sdB stars as asteroseismic laboratories. From the discoveries of these two classes of pulsators in 1997 and 2003, respectively, up to the current epoch of data gathering of unprecedented quality from space, a lot of progress has been made in this area and prospects for future achievements look very promising.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/XMQW7BF8/Charpinet et al. - 2013 - Asteroseismology of hot B subdwarf stars.pdf}
}

@techreport{Charpinet2015,
  title = {Pulsations in Hot Subdwarf Stars: Recent Advances and Prospects for Testing Stellar Physics},
  author = {Charpinet, St{\'e}phane and Van Grootel, V and Fontaine, G and Brassard, P and Randall, S K and Green, E M},
  year = {2015},
  journal = {XXIXth IAU General Assembly},
  volume = {1},
  urldate = {2020-04-09},
  abstract = {The evolved, core helium burning, extreme horizontal branch stars (also known as hot B subdwarfs) host several classes of pulsators showing either p-or g-modes, or both. They offer particularly favorable conditions for probing with asteroseismology their internal structure, thus constituting arguably the most interesting seismic window for this intermediate stage of stellar evolution. G-modes in particular have the power to probe deep inside these stars, down to the convective He-burning core boundary where uncertain physics (convection, overshooting, semi-convection) is at work. Space data recently obtained with CoRoT and Kepler are offering us the possibility to probe these regions in detail and possibly shed new light on how these processes shape the core structure. In this short paper, we present the most recent advances that have taken place in this field and we provide hints of the foreseen future achievements of hot subdwarf asteroseismology.},
  keywords = {notion,notion-database,oscillations,stars,subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/GI7NWWKB/full-text.pdf}
}

@article{Charpinet2017,
  title = {Determining the Core Stratification in White Dwarfs with Asteroseismology},
  author = {Charpinet, S. and Giammichele, N. and Brassard, P. and Fontaine, G.},
  year = {2017},
  month = sep,
  volume = {152},
  pages = {05005},
  doi = {10.1051/epjconf/201715205005},
  urldate = {2023-09-19},
  abstract = {Using the forward modeling approach and a new parameterization for the core chemical stratification in ZZ Ceti stars, we test several situations typical of the usually limited constraints available, such as small numbers of observed independent modes, to carry out asteroseismology of these stars. We find that, even with a limited number of modes, the core chemical stratification (in particular, the location of the steep chemical transitions expected in the oxygen profile) can be determined quite precisely due to the significant sensitivity of some confined modes to partial reflexion (trapping) effects. These effects are similar to the well known trapping induced by the shallower chemical transitions at the edge of the core and at the bottom of the H-rich envelope. We also find that success to unravel the core structure depends on the information content of the available seismic data. In some cases, it may not be possible to isolate a unique, well-defined seismic solution and the problem remains degenerate. Our results establish that constraining the core chemical stratification in white dwarf stars based solely on asteroseismology is possible, an opportunity that we have started to exploit.},
  annotation = {ADS Bibcode: 2017EPJWC.15205005C},
  file = {/Users/lbugnet/Zotero/storage/42Z6DLCP/Charpinet et al. - 2017 - Determining the core stratification in white dwarf.pdf}
}

@article{Charpinet2017a,
  title = {Signature of the {{Core Stratification}} in {{Pulsating White Dwarfs}} and {{Tests}} of {{Seismic Inversion}}},
  author = {Charpinet, S. and Giammichele, N. and Brassard, P. and Fontaine, G.},
  year = {2017},
  month = mar,
  volume = {509},
  pages = {275},
  urldate = {2023-09-19},
  abstract = {We discuss and illustrate how the C/O stratification in the core of white dwarf stars affects their g-mode pulsation spectrum. This effect, mostly occurring through the interplay of partial wave reflection (mode trapping), leaves a subtle but detectable signature, in particular with now available ultra high precision photometry from space, that could be exploited to infer the main structures in this stratification. We provide tests demonstrating that asteroseismology can indeed be used, in some cases, to probe the innermost composition stratification of pulsating white dwarfs. This brings interesting prospects to constrain the core chemical stratification inherited from previous evolutionary phases, which is one of the most uncertain aspect of white dwarf internal structure.},
  annotation = {ADS Bibcode: 2017ASPC..509..275C},
  file = {/Users/lbugnet/Zotero/storage/XSL6K79H/Charpinet et al. - 2017 - Signature of the Core Stratification in Pulsating .pdf}
}

@book{Charpinet2018,
  title = {The Contribution of Asteroseismology to a Better Understanding of Helium-Core-Burning {{sdB}} Stars},
  author = {Charpinet, St{\'e}phane and Brassard, Pierre and Fontaine, Gilles and Van Grootel, Val{\'e}rie and Zong, Weikai and Randall, Suzanna and Green, Elizabeth},
  year = {2018},
  month = sep,
  pages = {26},
  doi = {10.5281/zenodo.1631361},
  urldate = {2023-09-19},
  abstract = {SdB stars are evolved compact objects of about half a solar mass burning helium in their core. Some develop nonradial oscillations driven by a kappa mechanism powered by the accumulation of iron and nickel in their envelope through the selective action of radiative levitation. They come into two main flavors that show rapid p-mode oscillations on a timescale of minutes (the V361 Hya class) or g-modes with periods of 1-4 hours (the V1093 Her class). These pulsations have been particularly propitious to the development of detailed asteroseismic investigations of the internal properties and fundamental parameters of these stars. Here, I review the contibution of asteroseismology to a better understanding of sdB stars, regarding in particular their link to stellar evolution. I also discuss their potential to constrain important processes that occur in the deep interior of helium core burning stars and that ultimately shape the structure of white dwarfs.},
  keywords = {Asteroseismology,Hot subdwarfs,Pulsations,Stars,Zenodo community phost},
  annotation = {ADS Bibcode: 2018phos.confE..26C}
}

@article{Charpinet2018a,
  title = {Rotation in {{sdB}} Stars as Revealed by Stellar Oscillations},
  author = {Charpinet, Stephane and Giammichele, Noemi and Zong, Weikai and Van Grootel, Val{\'e}rie and Brassard, Pierre and Fontaine, Gilles},
  year = {2018},
  month = jul,
  journal = {Open Astronomy},
  volume = {27},
  pages = {112--119},
  doi = {10.1515/astro-2018-0012},
  urldate = {2023-09-19},
  abstract = {An interesting opportunity offered by the detection of stellar oscillations is the possibility to infer the internal rotation rate of a star through the so-called rotational splittings. Such seismic measurements remained rather scarce for hot B subdwarf (sdB) stars until the advent of space observations with the Kepler spacecraft. Nowadays, however, a number of rotation measurements have become available, offering a glimpse on the global rotational properties of sdB stars. Here, we briefly discuss what asteroseismology starts to reveal on the rotation rate of these stars. We also make connections with the internal rotation of red-giant and white-dwarf stars. In particular, we show that the very slow rotation rates derived for single sdB stars, and their similarities with the dynamical properties of the cores of red-clump stars, strongly suggest that they evolved from red-giants rather than merger events.We also point out that no more angular momentum seems to be lost by stellar cores throughout the helium burning phase until the cooling white-dwarf stage, indicating that all the braking occurs before, most likely during red-giant branch evolution.},
  keywords = {stars:evolution,stars:oscillation,stars:rotation,subdwarfs},
  annotation = {ADS Bibcode: 2018OAst...27..112C},
  file = {/Users/lbugnet/Zotero/storage/3K2E94XU/Charpinet et al. - 2018 - Rotation in sdB stars as revealed by stellar oscil.pdf}
}

@inproceedings{Chen2016,
  title = {{{XGBoost}}: {{A Scalable Tree Boosting System}}},
  booktitle = {{{ACM}}},
  author = {Chen, Tianqi and Guestrin, Carlos},
  year = {2016},
  eprint = {1603.02754v3},
  urldate = {2020-04-11},
  abstract = {Tree boosting is a highly effective and widely used machine learning method. In this paper, we describe a scalable end-to-end tree boosting system called XGBoost, which is used widely by data scientists to achieve state-of-the-art results on many machine learning challenges. We propose a novel sparsity-aware algorithm for sparse data and weighted quan-tile sketch for approximate tree learning. More importantly, we provide insights on cache access patterns, data compression and sharding to build a scalable tree boosting system. By combining these insights, XGBoost scales beyond billions of examples using far fewer resources than existing systems.},
  archiveprefix = {arxiv},
  keywords = {Large-scale,Learning,Machine,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XCM7WBX2/full-text.pdf}
}

@article{Chiappini2015,
  title = {Young [{$\alpha$}/{{Fe}}]-Enhanced Stars Discovered by {{CoRoT}} and {{APOGEE}}: {{What}} Is Their Origin?},
  author = {Chiappini, C. and Anders, F. and Rodrigues, T. S. and Miglio, A. and Montalb{\'a}n, J. and Mosser, B. and Girardi, L. and Valentini, M. and Noels, A. and Morel, T. and Minchev, I. and Steinmetz, M. and Santiago, B. X. and Schultheis, M. and Martig, M. and Da Costa, L. N. and Maia, M. A.G. and Allende Prieto, C. and De Assis Peralta, R. and Hekker, S. and Theme{\ss}l, N. and Kallinger, T. and Garc{\'i}a, R. A. and Mathur, S. and Baudin, F. and Beers, T. C. and Cunha, K. and Harding, P. and Holtzman, J. and Majewski, S. and M{\'e}sz{\'a}ros, Sz and Nidever, D. and Pan, K. and Schiavon, R. P. and Shetrone, M. D. and Schneider, D. P. and Stassun, K.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {576},
  pages = {1--7},
  issn = {14320746},
  doi = {10.1051/0004-6361/201525865},
  abstract = {We report the discovery of a group of apparently young CoRoT red-giant stars exhibiting enhanced [{$\alpha$}/Fe] abundance ratios (as determined from APOGEE spectra) with respect to solar values. Their existence is not explained bystandard chemical evolution models of the Milky Way, and shows that the chemical-enrichment history of the Galactic disc is more complex. We find similar stars in previously published samples for which isochrone-ages could be reliably obtained, although in smaller relative numbers. This might explain why these stars have not previously received attention. The young [{$\alpha$}/Fe]-rich stars are much more numerous in the CoRoT-APOGEE (CoRoGEE) inner-field sample than in any other high-resolution sample available at present because only CoRoGEE can explore the inner-disc regions and provide ages for its field stars. The kinematic properties of the young [{$\alpha$}/Fe]-rich stars are not clearly thick-disc like, despite their rather large distances from the Galactic mid-plane. Our tentative interpretation of these and previous intriguing observations in the Milky Way is that these stars were formed close to the end of the Galactic bar, near corotation - a region where gas can be kept inert for longer times than in other regions that are more frequently shocked by the passage of spiral arms. Moreover, this is where the mass return from older inner-disc stellar generations is expected to be highest (according to an inside-out disc-formation scenario), which additionally dilutes the in-situ gas. Other possibilities to explain these observations (e.g., a recent gas-accretion event) are also discussed.},
  keywords = {Asteroseismology,Galaxy: abundances,Galaxy: disk,Galaxy: formation,Galaxy: stellar content,notion,notion-database,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/5A4QWAZX/Chiappini et al. - 2015.pdf}
}

@article{Chowdhury2009,
  title = {Intermediate-Term Periodicities in Sunspot Areas during Solar Cycles 22 and 23},
  author = {Chowdhury, Partha and Khan, Manoranjan and Ray, P. C.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {392},
  number = {3},
  pages = {1159--1180},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2008.14117.x},
  abstract = {In this paper, the data of sunspot areas recorded at the US Air Force National Oceanic and Atmospheric Administration during solar Cycles 22 and 23 (1986 September 1 to 2007 August 31) have been analysed to investigate the midterm periodicities. Power spectral analysis has been performed separately for the data of the whole disc, and the northern and southern hemispheres of the Sun, which provides evidence for a multitude of quasi-periodic oscillations. During Cycle 22, in the high-frequency range, this covers the solar rotation periods, and shows prominent 27-41 d periods in both hemispheres for rising and declining phase of the solar cycle. In the intermediate-frequency range, we have detected a series of significant quasi-periodicities of 87-106, 159-175, 194-219, 292-318 and {$\sim$}389 d in different phases of Cycle 22. This result shows that well-known 'Rieger periodicity' of 150-160 d was present in sunspot activity even in solar cycle 22 but localized mainly in the southern hemisphere. When Cycle 23 is considered, it is found that a short-term periodicity having range of 24-45 d occurred in both rising and descending epochs in all hemispheres. On the other hand, in intermediate range, periods of 69-95, 113-133, 160-187, 245-321, 348-406 d and {$\sim$}1.3 yr were detected. This analysis provides evidence that the Rieger period reappeared in Cycle 23 but is predominant in the southern part of the Sun. Periods near 1.3 yr, which were reported in the rotation rate at the base of convection zone, have been found in the southern hemisphere only during minimum phase of Cycle 23. When time series of combined solar Cycles 22 and 23 were analysed, intermittent periods in the range of 24-43, 50-73, 86-120, 130-180, 240-270 d and quasi-annual period of 330-380 d were detected in all the data sets. Possible explanations of these observed periodicities are delivered on the basis of solar r-mode oscillation. \textcopyright{} 2008 RAS.},
  keywords = {notion,notion-database,Sun: activity,Sun: magnetic field,Sunspots},
  file = {/Users/lbugnet/Zotero/storage/DIMQWJWR/Chowdhury, Khan, Ray - 2009.pdf}
}

@techreport{Christensen-Dalsgaard1984,
  title = {What {{Will Asteroseismology Teach}} Us},
  author = {{Christensen-Dalsgaard}, J.},
  year = {1984},
  journal = {srps},
  pages = {11},
  urldate = {2020-02-28},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Y6E524C8/full-text.pdf}
}

@article{Christensen-Dalsgaard1991a,
  title = {Theory of Solar Oscillations.},
  author = {{Christensen-Dalsgaard}, Jorgen and Berthomieu, Gabrielle},
  year = {1991},
  journal = {IN: Solar interior and atmosphere (A92-36201 14-92). Tucson, AZ, University of Arizona Press},
  pages = {401--478},
  urldate = {2020-06-27},
  keywords = {Asymptotic Methods,Boundary Conditions,Equations Of Motion,Helioseismology,notion,notion-database,Solar Interior,Solar Oscillations,Solar Physics,Stellar Models,Stellar Structure}
}

@article{Christensen-Dalsgaard1992a,
  title = {Solar Oscillations and the Equation of State},
  author = {{Christensen-Dalsgaard}, J{\o}rgen and D{\"a}ppen, Werner},
  year = {1992},
  journal = {The Astronomy and Astrophysics Review},
  volume = {4},
  number = {3},
  pages = {267--361},
  issn = {09354956},
  doi = {10.1007/BF00872687},
  abstract = {Accurate measurements of observed frequencies of solar oscillations are providing a wealth of data on the properties of the solar interior. The frequencies depend on solar structure, and on the properties of the plasma in the Sun. Here we consider in particular the dependence on the thermodynamic state. From an analysis of the equations of stellar structure, and the relevant aspects of the properties of the oscillations, we argue that in the convection zone one can isolate information about the equation of state which is relatively unaffected by other uncertainties in the physics of the solar interior. We review the different treatments that have been used to describe the thermodynamics of stellar plasmas. Through application of several of these to the computation of models of the solar envelope we demonstrate that the sensitivity of the observed frequencies is in fact sufficient to distinguish even quite subtle features of the physics of solar matter. This opens up the possibility of using the Sun as a laboratory for statistical mechanics, under conditions that are out of reach in a terrestrial laboratory. \textcopyright{} 1992 Springer-Verlag.},
  keywords = {Helioseismology,notion,notion-database,Solar oscillations,Solar structure,Thermodynamics of stellar interiors},
  file = {/Users/lbugnet/Zotero/storage/M2W2GY3A/Christensen-Dalsgaard, Däppen - 1992.pdf}
}

@book{Christensen-Dalsgaard2001,
  title = {Stellar Evolution},
  author = {{Christensen-Dalsgaard}, J.},
  year = {2001},
  month = jan,
  journal = {The Encyclopedia of Astronomy and Astrophysics},
  publisher = {{IOP Publishing Ltd}},
  doi = {10.1888/0333750888},
  urldate = {2020-07-11},
  abstract = {We briefly review, at a level appropriate for graduate students and non-specialists, the field of quasar absorption lines (QALs). Emphasis is on the intervening absorbers. We present the anatomy of a quasar spectrum due to various classes of intervening absorption systems, and a brief historical review of each absorber class (Lyman-alpha forest and Lyman limit systems, and metal-line and damped Lyman-alpha absorbers). We also provide several heuristic examples on how the physical properties of both the intergalactic medium and the gaseous environments associated with earlier epoch galaxies can be inferred from QALs. The evolution of these environments from z=4 are discussed.},
  keywords = {notion,notion-database,Stars,Stellar Models and Concepts}
}

@techreport{Christensen-Dalsgaard2002,
  title = {Helioseismology},
  author = {{Christensen-Dalsgaard}, J{\o}rgen},
  year = {2002},
  month = oct,
  volume = {74},
  number = {4},
  pages = {1073--1129},
  issn = {00346861},
  doi = {10.1103/RevModPhys.74.1073},
  urldate = {2020-07-04},
  abstract = {Oscillations detected on the solar surface provide a unique opportunity for investigations of the interior properties of a star. Through major observational efforts, including extensive observations from space, as well as through the development of sophisticated tools for the analysis and interpretation of the data, we have been able to infer the large-scale structure and rotation of the solar interior with substantial accuracy. In addition, information is emerging about the complex subsurface structure and dynamics of sunspot regions, which dominate the magnetic activity in the solar atmosphere and beyond. The results provide a detailed test of the modeling of stellar structure and evolution, and hence of the physical properties of matter assumed in the models. In this way the basis for using stellar modeling in other branches of science is substantially strengthened; an important example is the use of observations of solar neutrinos to constrain the properties of the neutrino.},
  keywords = {26.65.+t,96.40.Fg,96.40.Tv,96.60.Hv,96.60.Jw,96.60.Ly,96.60.Qc,96.60.Vg,Astrophysics,Electric and magnetic fields solar magnetism,Helioseismology pulsations and shock waves,notion,notion-database,Particle emission solar wind,Solar interior,Solar neutrinos},
  annotation = {Reviews of Modern Physics}
}

@article{Christensen-Dalsgaard2004,
  title = {Physics of Solar-like Oscillations},
  author = {{Christensen-Dalsgaard}, J{\o}rgen},
  year = {2004},
  journal = {Solar Physics},
  volume = {220},
  number = {2},
  pages = {137--168},
  issn = {00380938},
  doi = {10.1023/B:SOLA.0000031392.43227.7d},
  abstract = {The physics of solar and stellar oscillations determines their observable properties: frequencies, amplitudes, lifetimes, line asymmetries and phase relations. In the solar case these quantities have been measured, often with high precision, and much has been learned about the properties of the solar interior, and the properties of the oscillations. With recent advances in observational techniques, such seismic investigations are now being extended to solar-like oscillations in distant stars. I provide a brief overview of the basic properties of stellar oscillations, and of the information about stellar properties that may be inferred from them, concentrating mostly on the low-degree modes for which information may be expected for distant stars. In addition, I consider the current state of investigations of solar-like oscillations in other stars, and the prospects for an improved understanding of the physics of such oscillations.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/97G24K2D/Christensen-Dalsgaard - 2004.pdf}
}

@article{Christensen-Dalsgaard2006,
  title = {Rotation of the Solar Convection Zone from Helioseismology},
  author = {{Christensen-Dalsgaard}, J.},
  year = {2006},
  month = oct,
  journal = {Proceedings of the International Astronomical Union},
  volume = {2},
  number = {S239},
  eprint = {astro-ph/0610942},
  pages = {393--404},
  doi = {10.1017/S1743921307000816},
  urldate = {2020-03-08},
  abstract = {Helioseismology has provided very detailed inferences about rotation of the solar interior. Within the convection zone the rotation rate roughly shares the latitudinal variation seen in the surface differential rotation. The transition to the nearly uniformly rotating radiative interior takes place in a narrow tachocline, which is likely important to the operation of the solar magnetic cycle.The convection-zone rotation displays zonal flows, regions of slightly more rapid and slow rotation, extending over much of the depth of the convection zone and converging towards the equator as the solar cycle progresses. In addition, there is some evidence for a quasi-periodic variation in rotation, with a period of around 1.3 yr, at the equator near the bottom of the convection zone.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: interior,Sun: oscillations,Sun: rotation}
}

@article{Christensen-Dalsgaard2008,
  title = {Helio- and Asteroseismology},
  author = {{Christensen-Dalsgaard}, J{\o}rgen},
  year = {2008},
  journal = {Proceedings of the International Astronomical Union},
  volume = {4},
  number = {S252},
  pages = {135--147},
  issn = {17439213},
  doi = {10.1017/S1743921308022679},
  abstract = {Observations of solar and stellar oscillations are providing detailed information about stellar interiors. In the case of the Sun the set of observed frequencies is sufficiently detailed and accurate that the properties of the solar interior, such as sound speed, density and internal rotation, can be inferred with substantial precision and resolution. This allows detailed tests of solar modelling, with interesting and to some extent controversial results. Observations of solar-like oscillations in distant stars have started only recently, owing their very small amplitudes. However, developments in ground-based equipment and observations from space are revolutionizing this field, promising greatly increased insight into the structure and evolution of the stars. \textcopyright{} 2008 International Astronomical Union.},
  keywords = {notion,notion-database,Stars: evolution,Stars: oscillations,Sun: abundances,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/DV5NMRKB/Christensen-Dalsgaard - 2008(2).pdf}
}

@article{Christensen-Dalsgaard2008a,
  title = {{{ADIPLS}} - {{The Aarhus}} Adiabatic Oscillation Package},
  author = {{Christensen-Dalsgaard}, J{\o}rgen},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  eprint = {0710.3106},
  pages = {113--120},
  issn = {0004640X},
  doi = {10.1007/s10509-007-9689-z},
  abstract = {Development of the Aarhus adiabatic pulsation code started around 1978. Although the main features have been stable for more than a decade, development of the code is continuing, concerning numerical properties and output. The code has been provided as a generally available package and has seen substantial use at a number of installations. Further development of the package, including bringing the documentation closer to being up to date, is planned as part of the HELAS Coordination Action. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Numerical methods,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/LSP294E5/Christensen-Dalsgaard - 2008.pdf}
}

@article{Christensen-Dalsgaard2008b,
  title = {The {{Kepler}} Asteroseismic Investigation},
  author = {{Christensen-Dalsgaard}, J. and Arentoft, T. and Brown, T. M. and Gilliland, R. L. and Kjeldsen, H. and Borucki, W. J. and Koch, D.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012039},
  abstract = {The NASA Kepler mission for studies of extra-solar planets, with expected launch early in 2009, will provide a large set of excellent data for asteroseismology. Here we provide a brief presentation of the mission and discuss some aspects of the expected results of the asteroseismic investigations and the organization of the effort in the Kepler Asteroseismic Science Consortium (KASC). \textcopyright{} 2008 IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3DWS95IH/Christensen-Dalsgaard et al. - 2008.pdf}
}

@article{Christensen-Dalsgaard2008c,
  title = {The {{Sun}} as a Fundamental Calibrator of Stellar Evolution},
  author = {{Christensen-Dalsgaard}, J{\o}rgen},
  year = {2008},
  journal = {Proceedings of the International Astronomical Union},
  volume = {4},
  number = {S258},
  eprint = {0904.0358},
  pages = {431--442},
  issn = {1743-9213},
  doi = {10.1017/s1743921309032086},
  abstract = {The Sun is unique amongst stars in having a precisely determined age which does not depend on the modelling of stellar evolution. Furthermore, other global properties of the Sun are known to much higher accuracy than for any other star. Also, helioseismology has provided detailed determination of the solar internal structure and rotation. As a result, the Sun plays a central role in the development and test of stellar modelling. Here I discuss solar modelling and its application to tests of asteroseismic techniques for stellar age determination.},
  archiveprefix = {arxiv},
  keywords = {asteroseismol-,evolution,fundamental parameters,helioseismology,interior,notion,notion-database,oscillations,stars,sun},
  file = {/Users/lbugnet/Zotero/storage/AJIXIKV9/Christensen-Dalsgaard - 2008(4).pdf}
}

@article{Christensen-Dalsgaard2008d,
  title = {{{ASTEC}} - {{The Aarhus STellar Evolution Code}}},
  author = {{Christensen-Dalsgaard}, J{\o}rgen},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  pages = {13--24},
  issn = {0004640X},
  doi = {10.1007/s10509-007-9675-5},
  abstract = {The Aarhus code is the result of a long development, starting in 1974, and still ongoing. A novel feature is the integration of the computation of adiabatic oscillations for specified models as part of the code. It offers substantial flexibility in terms of microphysics and has been carefully tested for the computation of solar models. However, considerable development is still required in the treatment of nuclear reactions, diffusion and convective mixing. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  isbn = {1050900796755},
  keywords = {notion,notion-database,Stars,Stellar evolution,Stellar structure},
  file = {/Users/lbugnet/Zotero/storage/RIAVHEMD/Christensen-Dalsgaard - 2008(3).pdf}
}

@article{Christensen-Dalsgaard2010,
  title = {Seismological Challenges for Stellar Structure},
  author = {{Christensen-Dalsgaard}, J.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  eprint = {1007.1720},
  pages = {866--872},
  issn = {00046337},
  doi = {10.1002/asna.201011416},
  abstract = {Helioseismology has provided very detailed information about the solar interior, and extensive data on a large number of stars, although at less detail, are promised by the ongoing and upcoming asteroseismic projects. In the solar case there remain serious challenges in understanding the inferred solar structure, particularly in the light of the revised determinations of the solar surface composition. Also, a secure understanding of the origins of solar rotation as inferred from helioseismology, both in the radiative interior and in the convection zone, is still missing. In the stellar case challenges are certain to appear as the data allow more detailed inferences of the properties of stellar cores. Large remaining uncertainties in modelling concern the properties of convective cores and other processes that may cause mixing. As a result of developing asteroseismic signatures addressing these and other issues, we can look forward to a highly challenging, and hence exciting, era of stellar astrophysics. \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations,Stars: rotation,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/I4H83XSB/Christensen-Dalsgaard - 2010.pdf}
}

@article{Christensen-Dalsgaard2010a,
  title = {Prospects for Asteroseismology},
  author = {{Christensen-Dalsgaard}, J{\o}rgen and Houdek, G{\"u}nter},
  year = {2010},
  journal = {Astrophysics and Space Science},
  volume = {328},
  number = {1},
  pages = {51--66},
  issn = {0004640X},
  doi = {10.1007/s10509-009-0227-z},
  abstract = {The observational basis for asteroseismology is being dramatically strengthened, through more than two years of data from the CoRoT satellite, the flood of data coming from the Kepler mission and, in the slightly longer term, from dedicated ground-based facilities. Our ability to utilize these data depends on further development of techniques for basic data analysis, as well as on an improved understanding of the relation between the observed frequencies and the underlying properties of the stars. Also, stellar modelling must be further developed, to match the increasing diagnostic potential of the data. Here we discuss some aspects of data interpretation and modelling, focusing on the important case of stars with solar-like oscillations. \textcopyright{} 2009 Springer Science+Business Media B.V.},
  keywords = {Asteroseismology,Helioseismology,notion,notion-database,Solar composition,Stellar evolution,Stellar internal physics,Stellar structure},
  file = {/Users/lbugnet/Zotero/storage/BZG9QQID/Christensen-Dalsgaard, Houdek - 2010.pdf}
}

@article{Christensen-Dalsgaard2010b,
  title = {Asteroseismic Investigation of Known Planet Hosts in the Kepler Field},
  author = {{Christensen-Dalsgaard}, J. and Kjeldsen, H. and Brown, T. M. and Gilliland, R. L. and Arentoft, T. and Frandsen, S. and Quirion, P. O. and Borucki, W. J. and Koch, D. and Jenkins, J. M.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  pages = {164--168},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L164},
  abstract = {In addition to its great potential for characterizing extra-solar planetary systems, the Kepler Mission is providing unique data on stellar oscillations. A key aspect of Kepler asteroseismology is the application to solar-like oscillations of main-sequence stars. As an example, we here consider an initial analysis of data for three stars in the Kepler field for which planetary transits were known from ground-based observations. For one of these, HAT-P-7, we obtain a detailed frequency spectrum and hence strong constraints on the stellar properties. The remaining two stars show definite evidence for solar-like oscillations, yielding a preliminary estimate of their mean densities. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,Planetary systems,Stars: fundamental parameters,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WBQ4VGEJ/Christensen-Dalsgaard et al. - 2010.pdf}
}

@article{Christensen-Dalsgaard2011,
  title = {The Stellar Imager ({{SI}}) - {{A}} Mission to Resolve Stellar Surfaces, Interiors, and Magnetic Activity},
  author = {{Christensen-Dalsgaard}, J{\o}rgen and Carpenter, Kenneth G. and Schrijver, Carolus J. and Karovska, Margarita},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012085},
  abstract = {The Stellar Imager (SI) is a space-based, UV/Optical Interferometer (UVOI) designed to enable 0.1 milli-arcsecond (mas) spectral imaging of stellar surfaces and of the Universe in general. It will also probe via asteroseismology flows and structures in stellar interiors. SI will enable the development and testing of a predictive dynamo model for the Sun, by observing patterns of surface activity and imaging of the structure and differential rotation of stellar interiors in a population study of Sun-like stars to determine the dependence of dynamo action on mass, internal structure and flows, and time. SI's science focuses on the role of magnetism in the Universe and will revolutionize our understanding of the formation of planetary systems, of the habitability and climatology of distant planets, and of many magneto-hydrodynamically controlled processes in the Universe. SI is a "Landmark/Discovery Mission" in the 2005 Heliophysics Roadmap, an implementation of the UVOI in the 2006 Astrophysics Strategic Plan, and a NASA Vision Mission ("NASA Space Science Vision Missions" (2008), ed. M. Allen). We present here the science goals of the SI Mission, a mission architecture that could meet those goals, and the technology development needed to enable this mission. Additional information on SI can be found at: http://hires.gsfc.nasa.gov/si/. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FMKX7ZAR/Christensen-Dalsgaard et al. - 2011.pdf}
}

@inproceedings{Christensen-Dalsgaard2012,
  title = {Advances in {{Helio-}} and {{Asteroseismology}}},
  booktitle = {Proceedings of the 123th {{Symposium}}},
  author = {{Christensen-Dalsgaard}, J.},
  year = {2012},
  urldate = {2020-07-04},
  keywords = {notion,notion-database}
}

@misc{christensen-dalsgaardAsteroseismologyRedGiants2011,
  title = {Asteroseismology of Red Giants},
  author = {{Christensen-Dalsgaard}, J.},
  year = {2011},
  month = jun,
  number = {arXiv:1106.5946},
  eprint = {1106.5946},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-05-19},
  abstract = {Red-giant stars are emerging as one of the most interesting areas of space asteroseismology. Even a relatively basic analysis leads to the determination of the global parameters of the stars, such as their mass and radius, and the very extensive space-based data now available for a large number of stars allow detailed investigation of the deep interiors of red giants, including distinguishing between stars that do and do not have helium fusion in the core, on the basis of periods of gravity waves partially trapped in the core. Here I review the theoretical background for these new developments and provide a simple explanation for the effect on the period spacing of central helium fusion.},
  archiveprefix = {arxiv},
  langid = {english},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/75UCDIHP/Christensen-Dalsgaard - 2011 - Asteroseismology of red giants.pdf}
}

@misc{christensen-dalsgaardKeplerAsteroseismologyRedgiant2011,
  title = {Kepler Asteroseismology of Red-Giant Stars},
  author = {{Christensen-Dalsgaard}, J.},
  year = {2011},
  month = oct,
  number = {arXiv:1110.5012},
  eprint = {1110.5012},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-06-06},
  abstract = {The Kepler mission, launched in March 2009, has revolutionized asteroseismology, providing detailed observations of thousands of stars. This has allowed in-depth analysis of stars ranging from compact hot subdwarfs to red giants, and including the detection of solar-like oscillations in hundreds of stars on or near the main sequence. Here I mainly consider solar-like oscillations in red giants, where Kepler observations are yielding results of a perhaps unexpected richness. In addition to giving a brief overview of the observational and numerical results for these stars, I present a simple analysis which captures some of the properties of the observed frequencies.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/5WPBR828/Christensen-Dalsgaard - 2011 - Kepler asteroseismology of red-giant stars.pdf;/Users/lbugnet/Zotero/storage/6GZSERJV/1110.html}
}

@article{Christensen1976,
  title = {Towards a Heliological Inverse Problem},
  author = {Christensen-Dalsgaard, J{\o}rgen and Gough, D. O.},
  year = {1976},
  journal = {Nature},
  volume = {259},
  pages = {89},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XMGA2FEW/Christensen‐Dalsgaard, Gough - 1976.pdf}
}

@article{Christensen1991,
  title = {The Depth of the Solar Convection Zone},
  author = {Christensen-Dalsgaard, J{\o}rgen and Gough, D. O. and Thompson, M. J.},
  year = {1991},
  journal = {The Astrophysical Journal},
  volume = {378},
  pages = {413--437},
  isbn = {9783540773405},
  keywords = {Acoustic Velocity,Convective Flow,Helioseismology,notion,notion-database,Reynolds Number,Solar Interior,Solar Oscillations,Solar Physics,Sound Propagation,Stellar Composition,SUN: ABUNDANCES,SUN: INTERIOR,SUN: OSCILLATIONS,Temperature Gradients},
  file = {/Users/lbugnet/Zotero/storage/F6GGUGJI/Christensen‐Dalsgaard, Gough, Thompson - 1991.pdf}
}

@article{Christensen1995,
  title = {Modeling {{Solar-like}} Oscillations in Eta Bootis},
  author = {Christensen-Dalsgaard, J{\o}rgen and Bedding, Timothy R. and Kjeldsen, Hans},
  year = {1995},
  journal = {The Astrophysical Journal},
  volume = {443},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/U5DU8PIY/Christensen‐Dalsgaard, Bedding, Kjeldsen - 1995.pdf}
}

@article{Christensen2009,
  title = {Energy Flux Determines Magnetic Field Strength of Planets and Stars},
  author = {Christensen, Ulrich R. and Holzwarth, Volkmar and Reiners, Ansgar},
  year = {2009},
  month = jan,
  journal = {Nature},
  volume = {457},
  number = {7226},
  pages = {167--169},
  publisher = {{Nature Publishing Group}},
  issn = {14764687},
  doi = {10.1038/nature07626},
  urldate = {2020-06-03},
  abstract = {The magnetic fields of Earth and Jupiter, along with those of rapidly rotating, low-mass stars, are generated by convection-driven dynamos that may operate similarly (the slowly rotating Sun generates its field through a different dynamo mechanism). The field strengths of planets and stars vary over three orders of magnitude, but the critical factor causing that variation has hitherto been unclear. Here we report an extension of a scaling law derived from geodynamo models to rapidly rotating stars that have strong density stratification. The unifying principle in the scaling law is that the energy flux available for generating the magnetic field sets the field strength. Our scaling law fits the observed field strengths of Earth, Jupiter, young contracting stars and rapidly rotating low-mass stars, despite vast differences in the physical conditions of the objects. We predict that the field strengths of rapidly rotating brown dwarfs and massive extrasolar planets are high enough to make them observable. \textcopyright 2009 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database}
}

@article{ChristensenDalsgaard1995,
  title = {Helioseismic Estimation of Convective Overshoot in the {{Sun}} - {{NASA}}/{{ADS}}},
  author = {Christensen-Dalsgaard, J{\o}rgen and Monteiro, M{\'a}rio J.P.F.G. and Thompson, Michael J.},
  year = {1995},
  journal = {MNRAS},
  volume = {276},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PNYGRS5E/Christensen‐Dalsgaard, Monteiro, Thompson - 1995.pdf}
}

@article{Christiansen2012,
  title = {The {{Derivation}}, {{Properties}}, and {{Value}} of {{Kepler}}'s {{Combined Differential Photometric Precision}}},
  author = {Christiansen, Jessie L. and Jenkins, Jon M. and Caldwell, Douglas A. and Burke, Christopher J. and Tenenbaum, Peter and Seader, Shawn and Thompson, Susan E. and Barclay, Thomas S. and Clarke, Bruce D. and Li, Jie and Smith, Jeffrey C. and Stumpe, Martin C. and Twicken, Joseph D. and Van Cleve, Jeffrey},
  year = {2012},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {124},
  number = {922},
  eprint = {1208.0595},
  pages = {1279--1287},
  issn = {00046280},
  doi = {10.1086/668847},
  abstract = {The Kepler Mission is searching for Earth-size planets orbiting solar-like stars by simultaneously observing {$>$}160,000 stars to detect sequences of transit events in the photometric light curves. The Combined Differential Photometric Precision (CDPP) is the metric that defines the ease with which these weak terrestrial transit signatures can be detected. An understanding of CDPP is invaluable for evaluating the completeness of the Kepler survey and inferring the underlying planet population. This paper describes how the Kepler CDPP is calculated, and introduces tables of rms CDPP on a per-target basis for 3-, 6-, and 12-hour transit durations, which are now available for all Kepler observations. Quarter 3 is the first typical set of observations at the nominal length and completeness for a quarter, from 2009 September 18 to 2009 December 16, and we examine the properties of the rms CDPP distribution for this data set. Finally, we describe how to employ CDPP to calculate target completeness, an important use case.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ST2KVBAX/Christiansen et al. - 2012.pdf}
}

@article{Christophe2018,
  title = {Deciphering the Oscillation Spectrum of {$\gamma$} {{Doradus}} and {{SPB}} Stars},
  author = {Christophe, S. and Ballot, J. and Ouazzani, R. M. and Antoci, V. and Salmon, S. J.A.J.},
  year = {2018},
  month = oct,
  journal = {Astronomy and Astrophysics},
  volume = {618},
  eprint = {1807.03707},
  pages = {47},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201832782},
  urldate = {2020-11-29},
  abstract = {Context. The space-based Kepler mission provided four years of highly precise and almost uninterrupted photometry for hundreds of {$\gamma$} Doradus stars and tens of slowly pulsating B-Type (SPB) stars, finally allowing us to apply asteroseismology to these gravity mode pulsators. Without rotation, gravity modes are equally spaced in period. This simple structure does not hold in rotating stars for which rotation needs to be taken into account to accurately interpret the oscillation spectrum. Aims. We aim to develop a stellar-model-independent method to analyse and interpret the oscillation spectrum of {$\gamma$} Dor and SPB stars. Methods. Within the traditional approximation of rotation, we highlight the possibility of recovering the equidistance of period spacings by stretching the pulsation periods. The stretching function depends on the degree and azimuthal order of gravity modes and the rotation rate of the star. In this new stretched space, the pulsation modes are regularly spaced by the stellar buoyancy radius. Results. On the basis of this property, we implemented a method to search for these new regularities and simultaneously infer the rotation frequency and buoyancy radius. Tests on synthetic spectra computed with a non-perturbative approach show that we can retrieve these two parameters with reasonable accuracy along with the mode identification. In uniformly rotating models of a typical {$\gamma$} Dor star, and for the most observed prograde dipole modes, we show that the accuracy on the derived parameters is better than 5\% on both the internal rotation rate and the buoyancy radius. Finally, we apply the method to two stars of the Kepler field, a {$\gamma$} Dor and an SPB, and compare our results with those of other existing methods. Conclusions. We provide a stellar-model-independent method to obtain the near-core rotation rate, the buoyancy radius, and the mode identification from gravity-mode spectra of {$\gamma$} Dor and SPB stars.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/7F6MLC6P/full-text.pdf}
}

@article{cifuentesAstronomyAstrophysicsCARMENES2020,
  title = {Astronomy {{Astrophysics CARMENES}} Input Catalogue of {{M}} Dwarfs {{V}}. {{Luminosities}}, Colours, and Spectral Energy Distributions},
  author = {Cifuentes, C and Caballero, J A and {Cort{\'e}s-Contreras}, M and Montes, D and Abell{\'a}n, F J and Dorda, R and Holgado, G and Zapatero Osorio, M R and Morales, J C and Amado, P J and Passegger, V M and Quirrenbach, A and Reiners, A and Ribas, I and {Sanz-Forcada}, J and Schweitzer, A and Seifert, W and Solano, E},
  year = {2020},
  journal = {A\&A},
  volume = {642},
  pages = {115},
  doi = {10.1051/0004-6361/202038295},
  urldate = {2021-08-02},
  abstract = {Context. The relevance of M dwarfs in the search for potentially habitable Earth-sized planets has grown significantly in the last years. Aims. In our ongoing effort to comprehensively and accurately characterise confirmed and potential planet-hosting M dwarfs, in particular for the CARMENES survey, we have carried out a comprehensive multi-band photometric analysis involving spectral energy distributions, luminosities, absolute magnitudes, colours, and spectral types, from which we have derived basic astrophysical parameters. Methods. We have carefully compiled photometry in 20 passbands from the ultraviolet to the mid-infrared, and combined it with the latest parallactic distances and close-multiplicity information, mostly from Gaia DR2, of a sample of 2479 K5 V to L8 stars and ultracool dwarfs, including 2210 nearby, bright M dwarfs. For this, we made extensive use of Virtual Observatory tools. Results. We have homogeneously computed accurate bolometric luminosities and effective temperatures of 1843 single stars, derived their radii and masses, studied the impact of metallicity, and compared our results with the literature. The over 40 000 individually inspected magnitudes, together with the basic data and derived parameters of the stars, individual and averaged by spectral type, have been made public to the astronomical community. In addition, we have reported 40 new close multiple systems and candidates ({$\rho$} {$<$} 3.3 arcsec) and 36 overluminous stars that are assigned to young Galactic populations. Conclusions. In the new era of exoplanet searches around M dwarfs via transit (e.g. TESS, PLATO) and radial velocity (e.g. CARMENES, NIRPS+HARPS), this work is of fundamental importance for stellar and therefore planetary parameter determination.},
  keywords = {astronomical databases,late-type-planetary systems,low-mass-stars,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TMGZZQAI/aa38295-20 (1).pdf}
}

@article{Claudi2005,
  title = {Asteroseismology of Procyon a with Sarg at {{TNG}}},
  author = {Claudi, R. U. and Bonanno, A. and Leccia, S. and Ventura, R. and Desidera, S. and Gratton, R. and Cosentino, R. and Endl, M.},
  year = {2005},
  journal = {European Space Agency, (Special Publication) ESA SP},
  volume = {20},
  number = {560 I},
  pages = {483--486},
  issn = {03796566},
  abstract = {We present the high precision radial velocity measurements on the F5 IV Star {$\alpha$}CMi obtained from the SARG spectrograph at TNG (Telescopio Nazionale Galileo) exploiting the iodine cell technique. The time series of 950 analyzed spectra taken during 6 nights of Procyon observation, shows individual measurement error of 1.3 m/s (very close to the theoretical photon noise limit Brown et al. (1994)). An excess of power between 0.5 and 1.5 mHz, detected also by Martic et al. (2004) is found, but additional structure in the periodogram show up around 2.0 mHz.},
  keywords = {Asterosismology,notion,notion-database,Procyon A,Solar-like oscillations},
  file = {/Users/lbugnet/Zotero/storage/YP5R7DVT/Claudi et al. - 2005.pdf}
}

@article{Claverie1979,
  title = {Solar Structur3e from Global Studies of the 5-Minute Oscillation},
  author = {Claverie, A and Isaak, G R and Mcleod, C P and Raay, H B Van Der and Cortes, T Roca},
  year = {1979},
  volume = {282},
  number = {December},
  pages = {6--9},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9ECTJWUH/Claverie et al. - 1979.pdf}
}

@incollection{Clebsch-gordan,
  title = {Chapter 8: {{Clebsch-gordan}} Coefficients and 3jm Symbols},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {4},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3F5TDWB8/Unknown - Unknown(17).pdf}
}

@article{Colacevich1935,
  title = {On the {{Variable Radial Velocity}} of {$\delta$} {{Scuti}}},
  author = {Colacevich, A.},
  year = {1935},
  month = aug,
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {47},
  number = {278},
  pages = {231},
  publisher = {{IOP Publishing}},
  issn = {0004-6280},
  doi = {10.1086/124599},
  urldate = {2020-03-31},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LU3GEPA9/full-text.pdf}
}

@article{Coleman1976,
  title = {Research Note},
  author = {Coleman, Sandra B.},
  year = {1976},
  journal = {Substance Use and Misuse},
  volume = {11},
  number = {3},
  pages = {551},
  issn = {10826084},
  doi = {10.3109/10826087609056170},
  keywords = {data analysis,helioseismology,methods,notion,notion-database,oscillations,stars,sun},
  file = {/Users/lbugnet/Zotero/storage/IK6Z732W/Coleman - 1976.pdf}
}

@article{Collaboration2016,
  title = {Gaia Data Release 1},
  author = {Gaia, Collaboration and A Brown, A G and Vallenari, A and Prusti, T and {de Bruijne}, J HJ and Mignard, F and Drimmel, R and Babusiaux, C and {Bailer-Jones}, C AL and Bastian, U and Biermann, M and Evans, D W and Eyer, L and Jansen, F and Jordi, C and Katz, D and Klioner, S A and Lammers, U and Lindegren, L and Luri, X and Panem, C and Pourbaix, D and Randich, S and Sartoretti, P and Siddiqui, H I and Soubiran, C and Valette, V and {van Leeuwen}, F and Walton, N A and Aerts, C and Arenou, F and Cropper, M and H{\o}g, E and Lattanzi, M G and Grebel, E K and Holland, A D and Huc, C and Passot, X and Perryman, M and Bramante, L and Cacciari, C and Casta{\~n}eda, J and Chaoul, L and Cheek, N and De Angeli, F and Fabricius, C and Guerra, R and Hern{\'a}ndez, J and {Jean-Antoine-Piccolo}, A and Masana, E and Messineo, R and Mowlavi, N and Nienartowicz, K and {Ord{\'o}{\~n}ez-Blanco}, D and Panuzzo, P and Portell, J and Richards, P J and Riello, M and Seabroke, G M and Tanga, P and Th{\'e}venin, F and Torra, J and Els, S G and {Gracia-Abril}, G and Comoretto, G and {Garcia-Reinaldos}, M and Lock, T and Mercier, E and Altmann, M and Andrae, R and Astraatmadja, T L and {Bellas-Velidis}, I and Benson, K and Berthier, J and Blomme, R and Busso, G and Carry, B and Cellino, A and Clementini, G and Cowell, S and Creevey, O and Cuypers, J and Davidson, M and De Ridder, J and {de Torres}, A and Delchambre, L and Dell, A and Ducourant, C and Fr{\'e}mat, Y and {Garc{\'i}a-Torres}, M and Gosset, E and Halbwachs, J-l and Hambly, N C and Harrison, D L and Hauser, M and Hestroffer, D and Hodgkin, S T and Huckle, H E and Hutton, A and Jasniewicz, G and Jordan, S and Kontizas, M and Korn, A J and Lanzafame, A C and Manteiga, M and Moitinho, A and Muinonen, K and Osinde, J and Pancino, E and Pauwels, T and Petit, J-m and {Recio-Blanco}, A and Robin, A C and Sarro, L M and Siopis, C and Smith, M and Smith, K W and Sozzetti, A and Thuillot, W and {van Reeven}, W and Viala, Y and Abbas, U and Abreu Aramburu, A and Accart, S and Aguado, J J and Allan, P M and Allasia, W and Altavilla, G and {\'A}lvarez, M A and Alves, J and Anderson, R I and Andrei, A H and Anglada Varela, E and Antiche, E and Antoja, T and Ant{\'o}n, S and Arcay, B and Bach, N and Baker, S G and {Balaguer-N{\'u}{\~n}ez}, L and Barache, C and Barata, C and Barbier, A and Barblan, F and Barrado Navascu{\'e}s, D and Barros, M and Barstow, M A and Becciani, U and Bellazzini, M and Bello Garc{\'i}a, A and Belokurov, V and Bendjoya, P and Berihuete, A and Bianchi, L and Bienaym{\'e}, O and Billebaud, F and Blagorodnova, N and {Blanco-Cuaresma}, S and Boch, T and Bombrun, A and Borrachero, R and Bouquillon, S and Bourda, G and Bouy, H and Bragaglia, A and Breddels, M A and Brouillet, N and Br{\"u}semeister, T and Bucciarelli, B and Burgess, P and Burgon, R and Burlacu, A and Busonero, D and Buzzi, R and Caffau, E and Cambras, J and Campbell, H and Cancelliere, R and {Cantat-Gaudin}, T and Carlucci, T and Carrasco, J M and Castellani, M and Charlot, P and Charnas, J and Chiavassa, A and Clotet, M and Cocozza, G and Collins, R S and Costigan, G and Crifo, F and Cross, N JG and Crosta, M and Crowley, C and Dafonte, C and Damerdji, Y and Dapergolas, A and David, P and David, M and De Cat, P and {de Felice}, F and {de Laverny}, P and De Luise, F and De March, R and {de Martino}, D and {de Souza}, R and Debosscher, J and {del Pozo}, E and Delbo, M and Delgado, A and Delgado, H E and Di Matteo, P and Diakite, S and Distefano, E and Dolding, C and Dos Anjos, S and Drazinos, P and Duran, J and Dzigan, Y and Edvardsson, B and Enke, H and Evans, N W and Eynard Bontemps, G and Fabre, C and Fabrizio, M and Faigler, S and Falc{\~a}o, A J and Farr{\`a}s Casas, M and Federici, L and Fedorets, G and {Fern{\'a}ndez-Hern{\'a}ndez}, J and Fernique, P and Fienga, A and Figueras, F and Filippi, F and Findeisen, K and Fonti, A and Fouesneau, M and Fraile, E and Fraser, M and Fuchs, J and Gai, M and Galleti, S and Galluccio, L and Garabato, D and {Garc{\'i}a-Sedano}, F and Garofalo, A and Garralda, N and Gavras, P and Gerssen, J and Geyer, R and Gilmore, G and Girona, S and Giuffrida, G and Gomes, M and {Gonz{\'a}lez-Marcos}, A and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J and {Gonz{\'a}lez-Vidal}, J J and Granvik, M and Guerrier, A and Guillout, P and Guiraud, J and G{\'u}rpide, A and {Guti{\'e}rrez-S{\'a}nchez}, R and Guy, L P and Haigron, R and Hatzidimitriou, D and Haywood, M and Heiter, U and Helmi, A and Hobbs, D and Hofmann, W and Holl, B and Holland, G and Hunt, J AS and Hypki, A and Icardi, V and Irwin, M and {Jevardat de Fombelle}, G and Jofr{\'e}, P and Jonker, P G and Jorissen, A and Julbe, F and Karampelas, A and Kochoska, A and Kohley, R and Kolenberg, K and Kontizas, E and Koposov, S E and Kordopatis, G and Koubsky, P and {Krone-Martins}, A and Kudryashova, M and Kull, I and Bachchan, R K and {Lacoste-Seris}, F and Lanza, A F and Lavigne, J-b and {Le Poncin-Lafitte}, C and Lebreton, Y and Lebzelter, T and Leccia, S and Leclerc, N and {Lecoeur-Taibi}, I and Lemaitre, V and Lenhardt, H and Leroux, F and Liao, S and Licata, E and Lindstr{\o}m, H EP and Lister, T A and Livanou, E and Lobel, A and L{\"o}ffler, W and L{\'o}pez, M and Lorenz, D and MacDonald, I and Magalh{\~a}es Fernandes, T and Managau, S and Mann, R G and Mantelet, G and Marchal, O and Michalik, D and Millar, N R and H Miranda, B M and Molina, D and Molinaro, R and Pentik{\"a}inen, H and Pichon, B and Piersimoni, A M and Pineau, F-x and Plachy, E and Plum, G and Poujoulet, E and Pr{\v s}a, A and Pulone, L and Ragaini, S and Rago, S and Rambaux, N and {Ramos-Lerate}, M and Ranalli, P and Rauw, G and Read, A and Regibo, S and Reyl{\'e}, C and Ribeiro, R A and Rimoldini, L and Ripepi, V and Riva, A and Rixon, G and Roelens, M and {Romero-G{\'o}mez}, M and Rowell, N and Royer, F and {Ruiz-Dern}, L and Sadowski, G and Sagrist{\`a} Sell{\'e}s, T and Sahlmann, J and Salgado, J and Salguero, E and Sarasso, M and Savietto, H and Schultheis, M and Sciacca, E and Segol, M and Segovia, J C and Segransan, D and Shih, I-c and Smareglia, R and Smart, R L and Solano, E and Solitro, F and Sordo, R and Soria Nieto, S and Souchay, J and Spagna, A and Spoto, F and Stampa, U and Steele, I A and Steidelm{\"u}ller, H and Stephenson, C A and Stoev, H and Suess, F F and S{\"u}veges, M and Surdej, J and Szabados, L and {Szegedi-Elek}, E and Tapiador, D and Taris, F and Tauran, G and Taylor, M B and Teixeira, R and Terrett, D and Tingley, B and Trager, S C and Turon, C and Ulla, A and Utrilla, E and Valentini, G and {van Elteren}, A and Van Hemelryck, E and {van Leeuwen}, M and Varadi, M and Vecchiato, A and Veljanoski, J and Via, T and Vicente, D and Vogt, S and Voss, H and Votruba, V and Voutsinas, S and Walmsley, G and Weiler, M and Weingrill, K and Wevers, T and Wyrzykowski, {\L} and Yoldas, A and {\v Z}erjal, M and Zucker, S and Zurbach, C and Zwitter, T and Alecu, A and Allen, M and Allende Prieto, C and Amorim, A and {Anglada-Escud{\'e}}, G and Arsenijevic, V and Azaz, S and Balm, P and Beck, M and Bernstein, H-h and Bigot, L and Bijaoui, A and Blasco, C and Bonfigli, M and Bono, G and Boudreault, S and Bressan, A and Brown, S and Brunet, P-m and Bunclark, P and Buonanno, R and Butkevich, A G and Carret, C and Carrion, C and Chemin, L and Ch{\'e}reau, F and Corcione, L and Darmigny, E and {de Boer}, K S and {de Teodoro}, P and {de Zeeuw}, P T and Delle Luche, C and Domingues, C D and Dubath, P and Fodor, F and Fr{\'e}zouls, B and Fries, A and Fustes, D and Fyfe, D and Gallardo, E and Gallegos, J and Gardiol, D and Gebran, M and Gomboc, A and G{\'o}mez, A and Grux, E and Gueguen, A and Heyrovsky, A and Munari, U and Nguyen, A-t and Nordlander, T and Ocvirk, P and Olias Sanz, A and Ortiz, P and Osorio, J and Oszkiewicz, D and Ouzounis, A and Palmer, M and Park, P and Pasquato, E and Peltzer, C and Peralta, J and P{\'e}turaud, F and Pieniluoma, T and Pigozzi, E and Ziaeepour, H and Zschocke, S},
  year = {2016},
  journal = {I. Serraller Vizcaino},
  volume = {595},
  pages = {68},
  doi = {10.1051/0004-6361/201629512},
  urldate = {2020-03-06},
  abstract = {Context. At about 1000 days after the launch of Gaia we present the first Gaia data release, Gaia DR1, consisting of astrometry and photometry for over 1 billion sources brighter than magnitude 20.7. Aims. A summary of Gaia DR1 is presented along with illustrations of the scientific quality of the data, followed by a discussion of the limitations due to the preliminary nature of this release. Methods. The raw data collected by Gaia during the first 14 months of the mission have been processed by the Gaia Data Processing and Analysis Consortium (DPAC) and turned into an astrometric and photometric catalogue. Results. Gaia DR1 consists of three components: a primary astrometric data set which contains the positions, parallaxes, and mean proper motions for about 2 million of the brightest stars in common with the Hipparcos and Tycho-2 catalogues-a realisation of the Tycho-Gaia Astrometric Solution (TGAS)-and a secondary astrometric data set containing the positions for an additional 1.1 billion sources. The second component is the photometric data set, consisting of mean G-band magnitudes for all sources. The G-band light curves and the characteristics of {$\sim$}3000 Cepheid and RR Lyrae stars, observed at high cadence around the south ecliptic pole, form the third component. For the primary astrometric data set the typical uncertainty is about 0.3 mas for the positions and parallaxes, and about 1 mas yr -1 for the proper motions. A systematic component of {$\sim$}0.3 mas should be added to the parallax uncertainties. For the subset of {$\sim$}94 000 Hipparcos stars in the primary data set, the proper motions are much more precise at about 0.06 mas yr -1. For the secondary astrometric data set, the typical uncertainty of the positions is {$\sim$}10 mas. The median uncertainties on the mean G-band magnitudes range from the mmag level to {$\sim$}0.03 mag over the magnitude range 5 to 20.7. Conclusions. Gaia DR1 is an important milestone ahead of the next Gaia data release, which will feature five-parameter astrometry for all sources. Extensive validation shows that Gaia DR1 represents a major advance in the mapping of the heavens and the availability of basic stellar data that underpin observational astrophysics. Nevertheless, the very preliminary nature of this first Gaia data release does lead to a number of important limitations to the data quality which should be carefully considered before drawing conclusions from the data.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9XUI8GMA/full-text.pdf}
}

@book{Collins2003,
  title = {The Fundamentals of {{Stellar Astrophysics}}},
  author = {Collins, Georges W.},
  year = {2003},
  eprint = {1011.1669v3},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {978-85-7811-079-6},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JIJFHYC7/Collins - 2003.pdf}
}

@article{Colman2017,
  title = {Evidence for Compact Binary Systems around {{Kepler}} Red Giants},
  author = {Colman, Isabel L. and Huber, Daniel and Bedding, Timothy R. and Kuszlewicz, James S. and Yu, Jie and Beck, Paul G. and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Kawaler, Steven D. and Mathur, Savita and Stello, Dennis and White, Timothy R.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {469},
  number = {4},
  pages = {3802--3812},
  issn = {0035-8711},
  doi = {10.1093/mnras/stx1056},
  abstract = {We present an analysis of 168 oscillating red giants from NASA's Kepler mission that ex-hibit anomalous peaks in their Fourier amplitude spectra. These peaks result from ellipsoidal variations that are indicative of binary star systems, at frequencies such that the orbit of any stellar companion would be within the convective envelope of the red giant. Alternatively, the observed phenomenon may be due to a close binary orbiting a red giant in a triple system, or chance alignments of foreground or background binary systems contaminating the target pixel aperture. We identify 87 stars in the sample as chance alignments using a combination of pixel Fourier analysis and difference imaging. We find that in the remaining 81 cases, the anomalous peaks are indistinguishable from the target star to within 4 arcsec, suggesting a physical association. We examine a GALAXIA model of the Kepler field of view to estimate background star counts and find that it is highly unlikely that all targets can be explained by chance alignments. From this, we conclude that these stars may comprise a population of physically associated systems.},
  keywords = {1 i n t,binaries,close,giants,giants has been,notion,notion-database,of oscillating kepler red,oscillations,problem in the study,ro d u c,stars,t i o n,the analysis of red,this paper sets out,to solve a long-standing},
  file = {/Users/lbugnet/Zotero/storage/VR2ZDANV/Colman et al. - 2017.pdf}
}

@article{ConstructionSeismicModel,
  title = {Construction of a {{Seismic Model}} of the {{Sun}} - {{NASA}}/{{ADS}}},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5ESTSTN3/Unknown - Unknown(19).pdf}
}

@article{Corbard,
  title = {{{ABOUT THE ROTATION OF THE SOLAR RADIATIVE INTERIOR The}} Extremely High Quality of Modern Helioseismic Data , and the Large Number of Data Available from a Range of Observations , Is Forcing Us to Revisit and Reassess Those Techniques of Analysis That Are e},
  author = {Corbard, T and Chaplin, W J and Couvidat, S and Korzennik, S G and Ballot, J and Boumier, P and Fossat, E and Henney, C J and Howe, R and Lazrek, M and Lochard, J},
  pages = {269--285},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UVHQG2MK/Corbard et al. - Unknown.pdf}
}

@article{Core2019,
  title = {Session {{F Convection}} and Rotation},
  author = {Core, Cambridge},
  year = {2019},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DFGIAITN/Core - 2019.pdf}
}

@article{Corsaro2012,
  title = {Asteroseismology of the Open Clusters Ngc6791, Ngc6811, and Ngc6819 from 19 Months of Kepler Photometry},
  author = {Corsaro, Enrico and Stello, Dennis and Huber, Daniel and Bedding, Timothy R. and Bonanno, Alfio and Brogaard, Karsten and Kallinger, Thomas and Benomar, Othman and White, Timothy R. and Mosser, Benoit and Basu, Sarbani and Chaplin, William J. and {Christensen-Dalsgaard}, Jorgen and Elsworth, Yvonne P. and Garc{\'i}a, Rafael A. and Hekker, Saskia and Kjeldsen, Hans and Mathur, Savita and Meibom, Soren and Hall, Jennifer R. and Ibrahim, Khadeejah A. and Klaus, Todd C.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {757},
  number = {2},
  eprint = {1205.4023},
  issn = {15384357},
  doi = {10.1088/0004-637X/757/2/190},
  abstract = {We studied solar-like oscillations in 115 red giants in the three open clusters, NGC6791, NGC6811, and NGC6819, based on photometric data covering more than 19 months with NASA's Kepler space telescope. We present the asteroseismic diagrams of the asymptotic parameters {$\delta\nu$}02, {$\delta\nu$}01, and {$\epsilon$}, which show clear correlation with fundamental stellar parameters such as mass and radius. When the stellar populations from the clusters are compared, we see evidence for a difference in mass of the red giant branch stars and possibly a difference in structure of the red clump stars, from our measurements of the small separations {$\delta\nu$}02 and {$\delta\nu$}01. Ensemble \'echelle diagrams and upper limits to the linewidths of {$\mathscr{l}$} = 0 modes as a function of {$\Delta\nu$} of the clusters NGC6791 and NGC6819 are also shown, together with the correlation between the {$\mathscr{l}$} = 0 ridge width and the T eff of the stars. Lastly, we distinguish between red giant branch and red clump stars through the measurement of the period spacing of mixed dipole modes in 53 stars among all the three clusters to verify the stellar classification from the color-magnitude diagram. These seismic results also allow us to identify a number of special cases, including evolved blue stragglers and binaries, as well as stars in late He-core burning phases, which can be potentially interesting targets for detailed theoretical modeling. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,open clusters and associations: individual,stars: evolution,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/LE7JC4H4/Corsaro et al. - 2012.pdf}
}

@article{Corsaro2014,
  title = {{{DIAMONDS}}: {{A}} New {{Bayesian}} Nested Sampling Tool: {{Application}} to Peak Bagging of Solar-like Oscillations},
  author = {Corsaro, E. and De Ridder, J.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {571},
  eprint = {1408.2515},
  pages = {1--22},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424181},
  abstract = {Context. Thanks to the advent of the space-based missions CoRoT and NASA's Kepler, the asteroseismology of solar-like oscillations is now at the base of our understanding about stellar physics. The Kepler spacecraft, especially, is releasing excellent photometric observations of more than three years length in high duty cycle, which contain a large amount of information that has not yet been investigated. Aims. To exploit the full potential of Kepler light curves, sophisticated and robust analysis tools are now required more than ever. Characterizing single stars with an unprecedented level of accuracy and subsequently analyzing stellar populations in detail are fundamental to further constrain stellar structure and evolutionary models. Methods. We developed a new code, termed Diamonds, for Bayesian parameter estimation and model comparison by means of the nested sampling Monte Carlo (NSMC) algorithm, an efficient and powerful method very suitable for high-dimensional and multi-modal problems. A detailed description of the features implemented in the code is given with a focus on the novelties and differences with respect to other existing methods based on NSMC. Diamonds is then tested on the bright F8 V star KIC 9139163, a challenging target for peak-bagging analysis due to its large number of oscillation peaks observed, which are coupled to the blending that occurs between l = 2,0 peaks, and the strong stellar background signal. We further strain the performance of the approach by adopting a 1147.5 days-long Kepler light curve, accounting for more than 840 000 data bins in the power spectrum of the star. Results. The Diamonds code is able to provide robust results for the peak-bagging analysis of KIC 9139163, while preserving a considerable computational efficiency for identifying the solution at the same time. We test the detection of different astrophysical backgrounds in the star and provide a criterion based on the Bayesian evidence for assessing the peak significance of the detected oscillations in detail. We present results for 59 individual oscillation frequencies, amplitudes and linewidths and provide a detailed comparison to the existing values in the literature, from which significant deviations are found when a different background is used. Lastly, we successfully demonstrate an innovative approach to peak bagging that exploits the capability of Diamonds to sample multi-modal distributions, which is of great potential for possible future automatization of the analysis technique.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,Methods: numerical,Methods: statistical,notion,notion-database,Stars: individual: KIC 9139163,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/J8P2T3MW/Corsaro, De Ridder - 2014.pdf}
}

@article{Corsaro2015,
  title = {High-Precision Acoustic Helium Signatures in 18 Low-Mass Low-Luminosity Red Giants},
  author = {Corsaro, E. and De Ridder, J. and Garc{\'i}a, R. A.},
  year = {2015},
  journal = {Astronomy \& Astrophysics},
  volume = {578},
  pages = {A76},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201525922},
  abstract = {High-precision frequencies of acoustic modes in red giant stars are now available thanks to the long observing length and high-quality of the light curves provided by the NASA Kepler mission, thus allowing to probe the interior of evolved cool low-mass stars with unprecedented level of detail. We characterize the acoustic signature of the helium second ionization zone in a sample of 18 low-mass low-luminosity red giants by exploiting new mode frequency measurements derived from more than four years of Kepler observations. We analyze the second frequency differences of radial acoustic modes in all the stars of the sample by using the Bayesian code Diamonds. We find clear acoustic glitches due to the signature of helium second ionization in all the stars of the sample. We measure the acoustic depth and the characteristic width of the acoustic glitches with a precision level on average around \$\textbackslash sim\$2\% and \$\textbackslash sim\$8\%, respectively. We find good agreement with theoretical predictions and existing measurements from the literature. Lastly, we derive the amplitude of the glitch signal at \$\textbackslash nu\_\textbackslash mathrm\{max\}\$ for the second differences and for the frequencies with an average precision of \$\textbackslash sim\$6\%, obtaining values in the range 0.14-0.24 \$\textbackslash mu\$Hz, and 0.08-0.33 \$\textbackslash mu\$Hz, respectively, which can be used to investigate the helium abundance in the stars.},
  keywords = {asteroseismology,data analysis,interiors,late-type,methods,notion,notion-database,oscillations,stars,statistical},
  file = {/Users/lbugnet/Zotero/storage/NT49YZ5U/Corsaro, De Ridder, García - 2015.pdf}
}

@article{Corsaro2015a,
  title = {Bayesian Peak Bagging Analysis of 19 Low-Mass Low-Luminosity Red Giants Observed with {{Kepler}}},
  author = {Corsaro, E. and De Ridder, J. and Garc{\'i}a, R. A.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {579},
  eprint = {1503.08821},
  pages = {1--76},
  issn = {14320746},
  doi = {10.1051/0004-6361/201525895},
  abstract = {Context. Non-radial oscillations, observed in thousands of red giants by the space missions CoRoT and Kepler, allow us to greatly improve our understanding of stellar structure and evolution in cool low-mass stars. The currently available Kepler light curves contain an outstanding amount of information, but a detailed analysis of the individual oscillation modes in the observed power spectra, also known as peak bagging, is computationally demanding and challenging to perform on a large number of targets. Aims. Our intent is to perform for the first time a peak bagging analysis on a sample of 19 low-mass low-luminosity red giants observed by Kepler for more than four years. This allows us to provide high-quality asteroseismic measurements that can be exploited for an intensive testing of the physics used in stellar structure models, stellar evolution, and pulsation codes, as well as for refining existing asteroseismic scaling relations in the red giant branch regime. Methods. For this purpose, powerful and sophisticated analysis tools are needed. We exploit the Bayesian code Diamonds, using an efficient nested sampling Monte Carlo algorithm, to perform both a fast fitting of the individual oscillation modes and a peak detection test based on the Bayesian evidence. Results. We find good agreement for the parameters estimated in the background fitting phase with those given in the literature. We extract and characterize a total of 1618 oscillation modes, providing the largest set of detailed asteroseismic mode measurements ever published. We report on the evidence of a change in regime observed in the relation between linewidths and effective temperatures of the stars occurring at the bottom of the red giant branch. We show the presence of a linewidth depression or plateau around {$\nu<$}inf{$>$}max{$<$}/inf{$>$} for all the red giants of the sample. Lastly, we show a good agreement between our measurements of maximum mode amplitudes and existing maximum amplitudes from global analyses provided in the literature, proving that amplitude scaling relations can be used as empirical tools to improve and simplify the future peak bagging analysis on a larger sample of evolved stars.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,Methods: numerical,Methods: statistical,notion,notion-database,Stars: evolution,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TMMBQ2ZD/Corsaro, De Ridder, García - 2015(2).pdf}
}

@article{Corsaro2017,
  title = {Spin Alignment of Stars in Old Open Clusters},
  author = {Corsaro, Enrico and Lee, Yueh Ning and Garci{\'a}, Rafael A. and Hennebelle, Patrick and Mathur, Savita and Beck, Paul G. and Mathis, Stephane and Stello, Dennis and Bouvier, J{\'e}r{\^o}me},
  year = {2017},
  journal = {Nature Astronomy},
  volume = {1},
  eprint = {1703.05588},
  issn = {23973366},
  doi = {10.1038/s41550-017-0064},
  abstract = {Stellar clusters form by gravitational collapse of turbulent molecular clouds, with up to several thousand stars per cluster 1. They are thought to be the birthplace of most stars and therefore play an important role in our understanding of star formation, a fundamental problem in astrophysics 2,3. The initial conditions of the molecular cloud establish its dynamical history until the stellar cluster is born. However, the evolution of the cloud's angular momentum during cluster formation is not well understood 4. Current observations have suggested that turbulence scrambles the angular momentum of the cluster-forming cloud, preventing spin alignment among stars within a cluster 5. Here we use asteroseismology 6-8 to measure the inclination angles of spin axes in 48 stars from the two old open clusters NGC 6791 and NGC 6819. The stars within each cluster show strong alignment. Three-dimensional hydrodynamical simulations of proto-cluster formation show that at least 50\% of the initial proto-cluster kinetic energy has to be rotational in order to obtain strong stellar-spin alignment within a cluster. Our result indicates that the global angular momentum of the cluster-forming clouds was efficiently transferred to each star and that its imprint has survived several gigayears since the clusters formed.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/T7IHGL2G/Corsaro et al. - 2017(2).pdf}
}

@article{Corsaro2017a,
  title = {Metallicity Effect on Stellar Granulation Detected from Oscillating Red Giants in Open Clusters},
  author = {Corsaro, E. and Mathur, S. and Garci{\'a}, R. A. and Gaulme, P. and Pinsonneault, M. and Stassun, K. and Stello, D. and Tayar, J. and Trampedach, R. and Jiang, C. and Nitschelm, C. and Salabert, D.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {605},
  eprint = {1707.07474},
  issn = {14320746},
  doi = {10.1051/0004-6361/201731094},
  abstract = {The effect of metallicity on the granulation activity in stars, and hence on the convective motions in general, is still poorly understood. Available spectroscopic parameters from the updated APOGEE-Kepler catalog, coupled with high-precision photometric observations from NASA's Kepler mission spanning more than four years of observation, make oscillating red giant stars in open clusters crucial testbeds. Aims. We aim to determine the role of metallicity on the stellar granulation activity by discriminating its effect from that of different stellar properties such as surface gravity, mass, and temperature. We analyze 60 known red giant stars belonging to the open clusters NGC 6791, NGC 6819, and NGC 6811, spanning a metallicity range from [Fe/H] \^a\textperthousand -0.09 to 0.32. The parameters describing the granulation activity of these stars and their frequency of maximum oscillation power, {$\nu$}max, are studied while taking into account different masses, metallicities, and stellar evolutionary stages. We derive new scaling relations for the granulation activity, re-calibrate existing ones, and identify the best scaling relations from the available set of observations. Methods. We adopted the Bayesian code Diamonds for the analysis of the background signal in the Fourier spectra of the stars. We performed a Bayesian parameter estimation and model comparison to test the different model hypotheses proposed in this work and in the literature. Results. Metallicity causes a statistically significant change in the amplitude of the granulation activity, with a dependency stronger than that induced by both stellar mass and surface gravity. We also find that the metallicity has a significant impact on the corresponding time scales of the phenomenon. The effect of metallicity on the time scale is stronger than that of mass. Conclusions. A higher metallicity increases the amplitude of granulation and meso-granulation signals and slows down their characteristic time scales toward longer periods. The trend in amplitude is in qualitative agreement with predictions from existing 3D hydrodynamical simulations of stellar atmospheres from main sequence to red giant stars. We confirm that the granulation activity is not sensitive to changes in the stellar core and that it only depends on the atmospheric parameters of stars.},
  archiveprefix = {arxiv},
  keywords = {Methods: Numerical,Methods: Statistical,notion,notion-database,Open clusters and associations: General,Stars: Fundamental parameters,Stars: Late-type,Stars: Oscillations},
  file = {/Users/lbugnet/Zotero/storage/6LXYGLNE/Corsaro et al. - 2017.pdf}
}

@article{Corsaro2020,
  title = {Fast and {{Automated Peak Bagging}} with {{Diamonds}} ({{FAMED}})},
  author = {Corsaro, E and Mckeever, J M and Kuszlewicz, J S},
  year = {2020},
  journal = {Astronomy \& Astrophysics},
  volume = {640},
  eprint = {2006.08245v1},
  urldate = {2020-09-09},
  abstract = {Stars of low and intermediate mass that exhibit oscillations may show tens of detectable oscillation modes each. Oscillation modes are a powerful to constrain the internal structure and rotational dynamics of the star, hence tool allowing one to obtain an accurate stellar age. The tens of thousands of solar-like oscillators that have been discovered thus far are representative of the large diversity of fundamental stellar properties and evolutionary stages available. Because of the wide range of oscillation features that can be recognized in such stars, it is particularly challenging to properly characterize the oscillation modes in detail, especially in light of large stellar samples. Overcoming this issue requires an automated approach, which has to be fast, reliable, and flexible at the same time. In addition, this approach should not only be capable of extracting the oscillation mode properties of frequency, linewidth, and amplitude from stars in different evolutionary stages, but also able to assign a correct mode identification for each of the modes extracted. Here we present the new freely available pipeline FAMED (Fast and AutoMated pEak bagging with Diamonds), which is capable of performing an automated and detailed asteroseismic analysis in stars ranging from the main sequence up to the core-Helium-burning phase of stellar evolution. This, therefore, includes subgiant stars, stars evolving along the red giant branch (RGB), and stars likely evolving toward the early asymptotic giant branch. In this paper, we additionally show how FAMED can detect rotation from dipolar oscillation modes in main sequence, subgiant, low-luminosity RGB, and core-Helium-burning stars. FAMED can be downloaded from its public GitHub repository (https://github.com/EnricoCorsaro/FAMED).},
  archiveprefix = {arxiv},
  keywords = {asteroseismology-stars,data analysis,late-type-stars,notion,notion-database,numerical-methods,solar-type-methods,statistical-methods},
  file = {/Users/lbugnet/Zotero/storage/LDDUS7IN/full-text.pdf}
}

@techreport{corsaroFastAutomatedOscillation,
  title = {Fast and Automated Oscillation Frequency Extraction Using {{Bayesian}} Multi-Modality},
  author = {Corsaro, Enrico},
  eprint = {1903.09409v1},
  urldate = {2021-02-10},
  abstract = {Since the advent of CoRoT, and NASA Kepler and K2, the number of low-and intermediate-mass stars classified as pulsators has increased very rapidly with time, now accounting for several 10 4 targets. With the recent launch of NASA TESS space mission, we have confirmed our entrance to the era of all-sky observations of oscillating stars. TESS is currently releasing good quality datasets that already allow for the characterization and identification of individual oscillation modes even from single 27-days shots on some stars. When ESA PLATO will become operative by the next decade, we will face the observation of several more hundred thousands stars where identifying individual oscillation modes will be possible. However, estimating the individual frequency, amplitude, and lifetime of the oscillation modes is not an easy task. This is because solar-like oscillations and especially their evolved version, the red giant branch (RGB) oscillations, can vary significantly from one star to another depending on its specific stage of the evolution, mass, effective temperature, metallicity, as well as on its level of rotation and magnetism. In this perspective I will present a novel, fast, and powerful way to derive individual oscillation mode frequencies by building on previous results obtained with DIAMONDS. I will show that the oscillation frequencies obtained with this new approach can reach precisions of about 0.1 \% and accuracies of about 0.01 \% when compared to published literature values for the RGB star KIC 12008916.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,Bayesian,methods: data analysis,methods: numerical,methods: statistical,notion,notion-database,oscillation mode analysis,stars: late-type,stars: oscillations}
}

@article{Corsico2014,
  title = {Pulsating Low-Mass White Dwarfs in the Frame of New Evolutionary Sequences. {{I}}. {{Adiabatic}} Properties},
  author = {C{\'o}rsico, A. H. and Althaus, L. G.},
  year = {2014},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {569},
  pages = {A106},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201424352},
  urldate = {2023-10-02},
  abstract = {Context. Many low-mass white dwarfs with masses M{${_\ast}$}/M{$\odot$} {$\lessequivlnt$} 0.45, including the so-called extremely low-mass white dwarfs (M{${_\ast}$}/M{$\odot$} {$\lessequivlnt$} 0.20 - 0.25), have recently been discovered in the field of our Galaxy through dedicated photometric surveys. The subsequent discovery of pulsations in some of them has opened the unprecedented opportunity of probing the internal structure of these ancient stars. Aims: We present a detailed adiabatic pulsational study of these stars based on full evolutionary sequences derived from binary star evolution computations. The main aim of this study is to provide a detailed theoretical basis of reference for interpreting present and future observations of variable low-mass white dwarfs. Methods: Our pulsational analysis is based on a new set of He-core white-dwarf models with masses ranging from 0.1554 to 0.4352 M{$\odot$} derived by computing the non-conservative evolution of a binary system consisting of an initially 1 M{$\odot$} ZAMS star and a 1.4 M{$\odot$} neutron star. We computed adiabatic radial ({$\mathscr{l}$} = 0) and non-radial ({$\mathscr{l}$} = 1,2) p and g modes to assess the dependence of the pulsational properties of these objects on stellar parameters such as the stellar mass and the effective temperature, as well as the effects of element diffusion. Results: We found that for white dwarf models with masses below \textasciitilde{} 0.18 M{$\odot$}, g modes mainly probe the core regions and p modes the envelope, therefore pulsations offer the opportunity of constraining both the core and envelope chemical structure of these stars via asteroseismology. For models with M{${_\ast}$} {$\greaterequivlnt$} 0.18 M{$\odot$}, on the other hand, g modes are very sensitive to the He/H compositional gradient and therefore can be used as a diagnostic tool for constraining the H envelope thickness. Because both types of objects have not only very distinct evolutionary histories (according to whether the progenitor stars have experienced CNO-flashes or not), but also have strongly different pulsation properties, we propose to define white dwarfs with masses below \textasciitilde{} 0.18 M{$\odot$} as ELM (extremely low-mass) white dwarfs, and white dwarfs with M{${_\ast}$} {$\greaterequivlnt$} 0.18 M{$\odot$} as LM (low-mass) white dwarfs.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations,stars: variables: general,white dwarfs},
  annotation = {ADS Bibcode: 2014A\&A...569A.106C},
  file = {/Users/lbugnet/Zotero/storage/59DCMFNY/Córsico and Althaus - 2014 - Pulsating low-mass white dwarfs in the frame of ne.pdf}
}

@article{Corsico2019,
  title = {Pulsating White Dwarfs: New Insights},
  author = {C{\'o}rsico, Alejandro H. and Althaus, Leandro G. and Bertolami, Marcelo M. Miller and Kepler, S. O.},
  year = {2019},
  month = jun,
  journal = {Astronomy \& Astrophysics Review},
  volume = {27},
  number = {1},
  eprint = {1907.00115},
  publisher = {{Springer Verlag}},
  doi = {10.1007/s00159-019-0118-4},
  urldate = {2020-11-11},
  abstract = {White dwarf stars constitute the final evolutionary stage for more than 95 per cent of all stars. The Galactic population of white dwarfs conveys a wealth of information about several fundamental issues and are of vital importance to study the structure, evolution and chemical enrichment of our Galaxy and its components ---including the star formation history of the Milky Way. In addition, white dwarfs are tracers of the evolution of planetary systems along several phases of stellar evolution. Also, white dwarfs are used as laboratories for astro-particle physics, being their interest focused on physics beyond the standard model. The last decade has witnessed a great progress in the study of white dwarfs. In particular, a wealth of information of these stars from different surveys has allowed us to make meaningful comparison of evolutionary models with observations. While some information like surface chemical composition, temperature and gravity of isolated white dwarfs can be inferred from spectroscopy, and the total mass and radius can be derived as well when they are in binaries, the internal structure of these compact stars can be unveiled only by means of asteroseismology, an approach based on the comparison between the observed pulsation periods of variable stars and the periods predicted by appropriate theoretical models. The asteroseismological techniques allow us to infer details of the internal chemical stratification, the total mass, and even the stellar rotation profile. In this review, we first revise the evolutionary channels currently accepted that lead to the formation of white-dwarf stars, and then, we give a detailed account of the different sub-types of pulsating white dwarfs known so far, emphasizing the recent observational and theoretical advancements in the study of these fascinating variable stars.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stellar evolution,Stellar interiors,Stellar oscillations,White dwarf stars}
}

@article{Corsico2021,
  title = {Pulsating Hydrogen-Deficient White Dwarfs and Pre-White Dwarfs Observed with {{TESS}}. {{I}}. {{Asteroseismology}} of the {{GW Vir}} Stars {{RX J2117}}+3412, {{HS}} 2324+3944, {{NGC}} 6905, {{NGC}} 1501, {{NGC}} 2371, and {{K}} 1-16},
  author = {C{\'o}rsico, A. H. and Uzundag, M. and Kepler, S. O. and Althaus, L. G. and Silvotti, R. and Baran, A. S. and Vu{\v c}kovi{\'c}, M. and Werner, K. and Bell, K. J. and Higgins, M.},
  year = {2021},
  month = jan,
  journal = {Astronomy \& Astrophysics},
  volume = {645},
  pages = {A117},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202039202},
  urldate = {2023-10-09},
  abstract = {Context. The recent arrival of continuous photometric observations of unprecedented quality from space missions has strongly promoted the study of pulsating stars and caused great interest in the stellar astrophysics community. In the particular case of pulsating white dwarfs, the TESS mission is taking asteroseismology of these compact stars to a higher level, emulating or even surpassing the performance of its predecessor, the Kepler mission. Aims: We present a detailed asteroseismological analysis of six GW Vir stars that includes the observations collected by the TESS mission. Methods: We processed and analyzed TESS observations of RX J2117+3412 (TIC 117070953), HS 2324+3944 (TIC 352444061), NGC 6905 (TIC 402913811), NGC 1501 (TIC 084306468), NGC 2371 (TIC 446005482), and K 1-16 (TIC 233689607). We carried out a detailed asteroseismological analysis of these stars on the basis of PG 1159 evolutionary models that take into account the complete evolution of the progenitor stars. We constrained the stellar mass of these stars by comparing the observed period spacing with the average of the computed period spacings, and we employed the individual observed periods to search for a representative seismological model when possible. Results: In total, we extracted 58 periodicities from the TESS light curves of these GW Vir stars using a standard prewhitening procedure to derive the potential pulsation frequencies. All the oscillation frequencies that we found are associated with g-mode pulsations, with periods spanning from {$\sim$}817 s to {$\sim$}2682 s. We find constant period spacings for all but one star (K 1-16), which allowed us to infer their stellar masses and constrain the harmonic degree {$\mathscr{l}$} of the modes. Based on rotational frequency splittings, we derive the rotation period of RX J2117+3412, obtaining a value in agreement with previous determinations. We performed period-to-period fit analyses on five of the six analyzed stars. For four stars (RX J2117+3412, HS 2324+3944, NGC 1501, and NGC 2371), we were able to find an asteroseismological model with masses that agree with the stellar mass values inferred from the period spacings and are generally compatible with the spectroscopic masses. Obtaining seismological models allowed us to estimate the seismological distance and compare it with the precise astrometric distance measured with Gaia. Finally, we find that the period spectrum of K 1-16 exhibits dramatic changes in frequency and amplitude that together with the scarcity of modes prevented us from meaningful seismological modeling of this star. Conclusions: The high-quality data collected by the TESS space mission, considered simultaneously with ground-based observations, provide very valuable input to the asteroseismology of GW Vir stars, similar to the case of other classes of pulsating white dwarf stars. The TESS mission, in conjunction with future space missions and upcoming surveys, will make impressive progress in white dwarf asteroseismology.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,High Energy Physics - Phenomenology,stars: evolution,stars: interiors,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2021A\&A...645A.117C},
  file = {/Users/lbugnet/Zotero/storage/FW3I7FNR/Córsico et al. - 2021 - Pulsating hydrogen-deficient white dwarfs and pre-.pdf}
}

@article{Corsico2022,
  title = {White-Dwarf Asteroseismology with the {{TESS}} Space Telescope},
  author = {C{\'o}rsico, A. H.},
  year = {2022},
  month = jul,
  journal = {Boletin de la Asociacion Argentina de Astronomia La Plata Argentina},
  volume = {63},
  pages = {48--54},
  issn = {0571-3285},
  doi = {10.48550/arXiv.2203.03769},
  urldate = {2023-10-09},
  abstract = {As white-dwarf (WD) stars cool, they go through one or more stages of g(gravity)-mode pulsational instability, becoming multiperiodic variable stars. Stars passing through these instability domains allow astronomers to study their interiors through asteroseismological techniques, as if they could ``look'' at their interiors by analyzing the spectra of pulsation periods. WD asteroseismology has experienced extraordinary advances in recent years thanks to photometric observations of unprecedented quality delivered by space missions such as Kepler and TESS. These advances in the monitoring of variable WDs have been accompanied by the development of new stellar models and techniques for modeling their pulsations. In this article, we review the most outstanding findings -up to early 2022- about these fascinating pulsating stars made possible with the high-sensitivity and continuous observations of the ongoing TESS mission, bearing in mind that there will possibly be many more new results in the immediate future derived from this unique space telescope.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations,white dwarf},
  annotation = {ADS Bibcode: 2022BAAA...63...48C}
}

@article{Couvidat2003,
  title = {The {{Rotation}} of the {{Deep Solar Layers}}},
  author = {Couvidat, S. and Garca, R. A. and {Turck-Chize}, S. and Corbard, T. and Henney, C. J. and {Jimnez-Reyes}, S.},
  year = {2003},
  journal = {The Astrophysical Journal},
  volume = {597},
  number = {1},
  pages = {L77-L79},
  issn = {0004-637X},
  doi = {10.1086/379698},
  abstract = {From the analysis of low-order GOLF+MDI sectoral modes (l{$<$}=3, 6{$<$}=n{$<$}=15, |m|=l) and LOWL data (l{$>$}3), we derive the radial rotation profile by assuming no latitudinal dependence in the solar core. These low-order acoustic modes contain the most statistically significant information about the rotation of the deepest solar layers and should be least influenced by internal variability associated with the solar dynamo. After the correction of the sectoral splittings for their contamination by the rotation of the higher latitudes, we obtain a flat rotation profile down to 0.2 Rsolar.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YLRYEMGG/Couvidat et al. - 2003.pdf}
}

@techreport{Cowling,
  title = {{{THE NON-RADIAL OSCILLATIONS OF POLYTROPIC STARS}}},
  author = {Cowling, T G},
  urldate = {2020-06-22},
  abstract = {1. The problem of the non-radial oscillations of a fluid globe is of interest in the theory of the tidal distortion of binary stars. If the periods of rotation of the components differ from the orbital period, the tidal force produces a periodic disturbance at any point of either component. Provided that the period of this disturbance is long compared with the free periods of the stars, the tidal distortion differs little from that given by equilibrium theory. When, on the other hand, the period of the disturbance is comparable with the free periods, resonance is possible; this leads to an enhanced tidal distortion, resulting, in extreme cases, in the fission of a component. The oscillations of a homogeneous incompressible liquid globe were considered by Kelvin.* The problem for a similar globe in rotation was considered by Bryan f and Love.J This problem is relatively tractable; but when a heterogeneous liquid globe is considered, the mathematical difficulties are much greater. For this reason, we consider here only the oscillations of non-rotating stars. The oscillations of a heterogeneous compressible fluid sphere present a problem which is, in any case, of great mathematical complexity. As Pekeris has recently shown \textsection, the problem is equivalent to the solution of two simultaneous second-order differential equations. Pekeris considered in detail the case of an initially homogeneous sphere of compressible fluid. This is clearly dynamically unstable, since, by transferring material from the outer layers to the centre, a mass of greater central density and smaller gravitational potential energy is obtained; and Pekeris' results indicated this instability. Emden || considered approximately the oscillations of a polytropic gas sphere. His work was, however, vitiated by the approximations made in considering the equation of continuity, which he reduced to the form appropriate to a homogeneous incompressible fluid; the terms neglected and those retained are of the same order of magnitude. He obtained only one free period for oscillations in which the radial displacement is proportional to a surface harmonic of given order; there are, in fact, an infinite number of such periods. In this paper we shall consider a polytropic sphere, whose specific heat may differ from that corresponding to convective equilibrium with the corresponding polytropic index. We shall show that oscillations of indefinitely large period are possible, and consider the bearing of this result on the tidal problem.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3MLW4AET/full-text.pdf}
}

@techreport{Cowling1913,
  title = {{{ON THE SUN}}'{{S GENERAL MAGNETIC FIELD}}},
  author = {Cowling, T G},
  year = {1913},
  volume = {38},
  pages = {237},
  urldate = {2020-05-15},
  abstract = {The time of electromagnetic decay oLthe Sun's general magnetic field is shown to be 10 10 years, suggesting that the field may be a relic from a different primeval state. An alternative hypothesis, ascribing the field to thermal effects-due to convection in the rotating Sun, is shown to give a field of the correct sign, but less than io\textasciitilde{} 7 times the observed field; and a modification of the hypothesis, supposing that the field due to thermal currents is magnified by dynamo action, is shown to demand over 10 18 years for the field to grow to its present size. Other possible explanations of the Sun's field are suggested. In an Appendix, the effect of the Sun's rotation on turbulence in its interior is briefly considered. I. Our knowledge of solar magnetic fields is almost entirely derived from the work of Hale and his collaborators at Mount Wilson. By observations of polarization at the wings of spectral lines, these workers identified a general magnetic field of the Sun, similar in many respects to the Earth's magnetic field.* The field-strength is of order \textasciitilde{} (say) 25 gauss ; the axis of the field is inclined to the axis of rotation of the Sun at about 6\textdegree, and rotates round it in about 31J days. Different spectral lines indicate different intensities for the field; weak lines suggest larger fields than strong lines. Since the latter probably originate at greater heights in the Sun's atmosphere than the former, these results were interpreted as implying that the field falls off rapidly with increasing height. The average observed separation of the Zeeman components is of the same order as the probable error of a single measurement. Because of its smallness, its reality is sometimes doubted. The present author sees no reason to share these doubts. To ensure that personal bias should not colour the results, the original observer measuring the Zeeman displacements was kept in ignorance of the hemisphere and latitude of the observations. Thus if he were prone to imagine a non-existent phenomenon, he would give it sometimes one sign, sometimes the other, and in the aggregate his estimates would cancel out. Since, in spite of this, regular results were obtained, the phenomenon being observed was clearly not imaginary. In fact, though all observers have not been able to identify real Zeeman displacements, all those who have been able to identify them have found effects with the same sign. Moreover, no convincing explanation of the observations has been given, other than the existence of a magnetic field. The phenomenon requiring explanation is a difference in polarization between the two wings of a spectral line. Effects producing a pure displacement or pure broadening of the line cannot explain the polarization; no one has yet suggested a satisfactory alternative to the explanation in terms of a magnetic field. We may, however, doubt whether the field does fall off rapidly with increasing height, as originally suggested. Though all observers have agreed regarding the sign * Hale, Ap.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9BS4N8SJ/full-text.pdf}
}

@article{Cowling1941,
  title = {{{THE NON-RADIAL OSCILLATIONS OF POLYTROPIC STARS}}},
  author = {Cowling, T G and Phil, D.},
  year = {1941},
  journal = {MNRAS},
  volume = {101},
  pages = {367C},
  urldate = {2020-07-14},
  abstract = {1. The problem of the non-radial oscillations of a fluid globe is of interest in the theory of the tidal distortion of binary stars. If the periods of rotation of the components differ from the orbital period, the tidal force produces a periodic disturbance at any point of either component. Provided that the period of this disturbance is long compared with the free periods of the stars, the tidal distortion differs little from that given by equilibrium theory. When, on the other hand, the period of the disturbance is comparable with the free periods, resonance is possible; this leads to an enhanced tidal distortion, resulting, in extreme cases, in the fission of a component. The oscillations of a homogeneous incompressible liquid globe were considered by Kelvin.* The problem for a similar globe in rotation was considered by Bryan f and Love.J This problem is relatively tractable; but when a heterogeneous liquid globe is considered, the mathematical difficulties are much greater. For this reason, we consider here only the oscillations of non-rotating stars. The oscillations of a heterogeneous compressible fluid sphere present a problem which is, in any case, of great mathematical complexity. As Pekeris has recently shown \textsection, the problem is equivalent to the solution of two simultaneous second-order differential equations. Pekeris considered in detail the case of an initially homogeneous sphere of compressible fluid. This is clearly dynamically unstable, since, by transferring material from the outer layers to the centre, a mass of greater central density and smaller gravitational potential energy is obtained; and Pekeris' results indicated this instability. Emden || considered approximately the oscillations of a polytropic gas sphere. His work was, however, vitiated by the approximations made in considering the equation of continuity, which he reduced to the form appropriate to a homogeneous incompressible fluid; the terms neglected and those retained are of the same order of magnitude. He obtained only one free period for oscillations in which the radial displacement is proportional to a surface harmonic of given order; there are, in fact, an infinite number of such periods. In this paper we shall consider a polytropic sphere, whose specific heat may differ from that corresponding to convective equilibrium with the corresponding polytropic index. We shall show that oscillations of indefinitely large period are possible, and consider the bearing of this result on the tidal problem.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/J8WJXXR7/full-text.pdf}
}

@article{Cowling1945,
  title = {{{ON THE SUN}}'{{S GENERAL MAGNETIC FIELD}}},
  author = {Cowling, T G},
  year = {1945},
  journal = {MNRAS},
  volume = {38},
  number = {3},
  pages = {105--166},
  urldate = {2020-05-01},
  abstract = {The time of electromagnetic decay oLthe Sun's general magnetic field is shown to be 10 10 years, suggesting that the field may be a relic from a different primeval state. An alternative hypothesis, ascribing the field to thermal effects-due to convection in the rotating Sun, is shown to give a field of the correct sign, but less than io\textasciitilde{} 7 times the observed field; and a modification of the hypothesis, supposing that the field due to thermal currents is magnified by dynamo action, is shown to demand over 10 18 years for the field to grow to its present size. Other possible explanations of the Sun's field are suggested. In an Appendix, the effect of the Sun's rotation on turbulence in its interior is briefly considered. I. Our knowledge of solar magnetic fields is almost entirely derived from the work of Hale and his collaborators at Mount Wilson. By observations of polarization at the wings of spectral lines, these workers identified a general magnetic field of the Sun, similar in many respects to the Earth's magnetic field.* The field-strength is of order \textasciitilde{} (say) 25 gauss ; the axis of the field is inclined to the axis of rotation of the Sun at about 6\textdegree, and rotates round it in about 31J days. Different spectral lines indicate different intensities for the field; weak lines suggest larger fields than strong lines. Since the latter probably originate at greater heights in the Sun's atmosphere than the former, these results were interpreted as implying that the field falls off rapidly with increasing height. The average observed separation of the Zeeman components is of the same order as the probable error of a single measurement. Because of its smallness, its reality is sometimes doubted. The present author sees no reason to share these doubts. To ensure that personal bias should not colour the results, the original observer measuring the Zeeman displacements was kept in ignorance of the hemisphere and latitude of the observations. Thus if he were prone to imagine a non-existent phenomenon, he would give it sometimes one sign, sometimes the other, and in the aggregate his estimates would cancel out. Since, in spite of this, regular results were obtained, the phenomenon being observed was clearly not imaginary. In fact, though all observers have not been able to identify real Zeeman displacements, all those who have been able to identify them have found effects with the same sign. Moreover, no convincing explanation of the observations has been given, other than the existence of a magnetic field. The phenomenon requiring explanation is a difference in polarization between the two wings of a spectral line. Effects producing a pure displacement or pure broadening of the line cannot explain the polarization; no one has yet suggested a satisfactory alternative to the explanation in terms of a magnetic field. We may, however, doubt whether the field does fall off rapidly with increasing height, as originally suggested. Though all observers have agreed regarding the sign * Hale, Ap.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DHI94G2N/full-text.pdf}
}

@article{Cowling1957,
  title = {Magnetohydrodynamics},
  author = {Cowling, T. G. and Lindsay, R. B.},
  year = {1957},
  month = sep,
  journal = {Physics Today},
  volume = {10},
  number = {9},
  pages = {40--40},
  publisher = {{AIP Publishing}},
  issn = {0031-9228},
  doi = {10.1063/1.3060498},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Cranmer2014,
  title = {Stellar Granulation as the Source of High-Frequency Flicker in Kepler Light Curves},
  author = {Cranmer, Steven R. and Bastien, Fabienne A. and Stassun, Keivan G. and Saar, Steven H.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {781},
  number = {2},
  eprint = {1312.5928},
  issn = {15384357},
  doi = {10.1088/0004-637X/781/2/124},
  abstract = {A large fraction of cool, low-mass stars exhibit brightness fluctuations that arise from a combination of convective granulation, acoustic oscillations, magnetic activity, and stellar rotation. Much of the short-timescale variability takes the form of stochastic noise, whose presence may limit the progress of extrasolar planet detection and characterization. In order to lay the groundwork for extracting useful information from these quasi-random signals, we focus on the origin of the granulation-driven component of the variability. We apply existing theoretical scaling relations to predict the star-integrated variability amplitudes for 508 stars with photometric light curves measured by the Kepler mission. We also derive an empirical correction factor that aims to account for the suppression of convection in F-dwarf stars with magnetic activity and shallow convection zones. So that we can make predictions of specific observational quantities, we performed Monte Carlo simulations of granulation light curves using a Lorentzian power spectrum. These simulations allowed us to reproduce the so-called flicker floor (i.e., a lower bound in the relationship between the full light-curve range and power in short-timescale fluctuations) that was found in the Kepler data. The Monte Carlo model also enabled us to convert the modeled fluctuation variance into a flicker amplitude directly comparable with observations. When the magnetic suppression factor described above is applied, the model reproduces the observed correlation between stellar surface gravity and flicker amplitude. Observationally validated models like these provide new and complementary evidence for a possible impact of magnetic activity on the properties of near-surface convection. \textcopyright{} 2014. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {convection - stars: activity,notion,notion-database,stars: solar-type,starspots,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/A5FDD4JK/Cranmer et al. - 2014.pdf}
}

@article{Creevey2012,
  title = {Fundamental Properties of Five {{Kepler}} Stars Using Global Asteroseismic Quantities and Ground-Based Observations},
  author = {Creevey, O. L. and Do{\v g}an, G. and Frasca, A. and Thygesen, A. O. and Basu, S. and Bhattacharya, J. and Biazzo, K. and Brand{\~a}o, I. M. and Bruntt, H. and Mazumdar, A. and Niemczura, E. and Shrotriya, T. and Sousa, S. G. and Stello, D. and Subramaniam, A. and Campante, T. L. and Handberg, R. and Mathur, S. and Bedding, T. R. and Garc{\'i}a, R. A. and R{\'e}gulo, C. and Salabert, D. and {Molenda-Zakowicz}, J. and Quirion, P. O. and White, T. R. and Bonanno, A. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Christiansen, J. L. and Elsworth, Y. and Fanelli, M. N. and Karoff, C. and Kinemuchi, K. and Kjeldsen, H. and Gai, N. and Monteiro, M. J.P.F.G. and Su{\'a}rez, J. C.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {537},
  pages = {1--17},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117037},
  abstract = {We present an asteroseismic study of the solar-like stars KIC 11395018, KIC 10273246, KIC 10920273, KIC 10339342, and KIC 11234888 using short-cadence time series of more than eight months from the Kepler satellite. For four of these stars, we derive atmospheric parameters from spectra acquired with the Nordic Optical Telescope. The global seismic quantities (average largefrequency separation and frequency of maximum power), combined with the atmospheric parameters, yield the mean density and surface gravity with precisions of 2\% and {$\sim$}0.03 dex, respectively. We also determine the radius, mass, and age with precisions of 2-5\%, 7-11\%, and {$\sim$}35\%, respectively, using grid-based analyses. Coupling the stellar parameters with photometric data yields an asteroseismic distance with a precision better than 10\%. A v sin i measurement provides a rotational period-inclination correlation, and using the rotational periods from the recent literature, we constrain the stellar inclination for three of the stars. An Li abundance analysis yields an independent estimate of the age, but this is inconsistent with the asteroseismically determined age for one of the stars. We assess the performance of five grid-based analysis methods and find them all to provide consistent values of the surface gravity to {$\sim$}0.03 dex when both atmospheric and seismic constraints are at hand. The different grid-based analyses all yield fitted values of radius and mass to within 2.4{$\sigma$}, and taking the mean of these results reduces it to 1.5{$\sigma$}. The absence of a metallicity constraint when the average large frequency separation is measured with a precision of 1\% biases the fitted radius and mass for the stars with non-solar metallicity (metal-rich KIC 11395018 and metal-poor KIC 10273246), while including a metallicity constraint reduces the uncertainties in both of these parameters by almost a factor of two. We found that including the average small frequency separation improves the determination of the age only for KIC 11395018 and KIC 11234888, and for the latter this improvement was due to the lack of strong atmospheric constraints. \textcopyright{} 2012 ESO.},
  keywords = {asteroseismology,notion,notion-database,stars: atmospheres,stars: fundamental parameters,stars: general,stars: oscillations,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/6WFUNH8V/Creevey et al. - 2012.pdf}
}

@article{Creevey2013,
  title = {A Large Sample of Calibration Stars for Gaia: {{Logg}} from Kepler and {{CoRoT}} Fields},
  author = {Creevey, O. L. and Th{\'e}venin, F. and Basu, S. and Chaplin, W. J. and Bigot, L. and Elsworth, Y. and Huber, D. and Monteiro, M. J.P.F.G. and Serenelli, A.},
  year = {2013},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {431},
  number = {3},
  eprint = {1302.7158},
  pages = {2419--2432},
  issn = {00358711},
  doi = {10.1093/mnras/stt336},
  urldate = {2020-03-23},
  abstract = {Asteroseismic data can be used to determine stellar surface gravities with precisions of {$<$}0.05 dex by using the global seismic quantities ({$\delta$}) and {$\nu$}max along with standard atmospheric data such as Teff and metallicity. Surface gravity is also one of the four stellar properties to be derived by automatic analyses for one billion stars from Gaia data (workpackage GSP\_PHOT). In this paper, we explore seismic data from main-sequence F, G, K stars (solar-like stars) observed by the Kepler spacecraft as a potential calibration source for the methods that Gaia will use for object characterization (log g). We calculate log g for some bright nearby stars for which radii and masses are known (e.g. from interferometry or binaries), and using their global seismic quantities in a grid-based method, we determine an asteroseismic log gto within 0.01 dex of the direct calculation, thus validating the accuracy of our method. We also find that errors in adopted atmospheric parameters (mainly [Fe/H]) can, however, cause systematic errors of the order of 0.02 dex.We then apply our method to a list of 40 stars to deliver precise values of surface gravity, i.e. uncertainties of the order of 0.02dex, and we find agreement with recent literature values. Finally, we explore the typical precision that we expect in a sample of more than 400 Kepler stars which have their global seismic quantities measured. We find a mean uncertainty (precision) of the order of better than 0.02 dex in log g over the full explored range 3.8 {$<$} log g {$<$} 4.6, with the mean value varying only with stellar magnitude (0.01-0.02 dex). We study sources of systematic errors in log g and find possiblebiases of the order of 0.04 dex, independent of log g and magnitude, which accounts for errors in the Teff and [Fe/H] measurements, as well as from using a different grid-based method. We conclude that Kepler stars provide a wealth of reliable information that can help to calibrate methods that Gaia will use, in particular, for source characterization with GSP\_PHOT, where excellent precision (small uncertainties) and accuracy in log g is obtained from seismic data. \textcopyright{} 2013 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Galaxy: fundamental parameters,notion,notion-database,Stars: fundamental parameters,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/BWGADPJI/full-text.pdf}
}

@article{Creevey2017,
  title = {Characterizing Solar-Type Stars from Full-Length {{Kepler}} Data Sets Using the {{Asteroseismic Modeling Portal}}},
  author = {Creevey, O. L. and Metcalfe, T. S. and Schultheis, M. and Salabert, D. and Bazot, M. and Th{\'e}venin, F. and Mathur, S. and Xu, H. and Garc{\'i}a, R. A.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {601},
  eprint = {1612.08990},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629496},
  abstract = {The Kepler space telescope yielded unprecedented data for the study of solar-like oscillations in other stars. The large samples of multi-year observations posed an enormous data analysis challenge that has only recently been surmounted. Asteroseismic modeling has become more sophisticated over time, with better methods gradually developing alongside the extended observations and improved data analysis techniques. We apply the latest version of the Asteroseismic Modeling Portal (AMP) to the full-length Kepler data sets for 57 stars, comprising planetary hosts, binaries, solar-analogs, active stars, and for validation purposes, the Sun. From an analysis of the derived stellar properties for the full sample, we identify a variation of the mixing-length parameter with atmospheric properties. We also derive a linear relation between the stellar age and a characteristic frequency separation ratio. In addition, we find that the empirical correction for surface effects suggested by Kjeldsen and coworkers is adequate for solar-type stars that are not much hotter (Teff{$\leq$} 6200 K) or significantly more evolved (log g{$\geq$} 4.2, ( {$\Delta\nu$} ){$\geq$} 80 {$\mu$}Hz) than the Sun. Precise parallaxes from the Gaia mission and future observations from TESS and PLATO promise to improve the reliability of stellar properties derived from asteroseismology.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: numerical,notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/AYCHLJBV/Creevey et al. - 2017.pdf}
}

@article{Croll2006,
  title = {Differential {{Rotation}} of {$\epsilon$} {{Eridani Detected}} by {{MOST}}},
  author = {Croll, Bryce and Walker, Gordon A. H. and Kuschnig, Rainer and Matthews, Jaymie M. and Rowe, Jason F. and Walker, Andrew and Rucinski, Slavek M. and Hatzes, Artie P. and Cochran, William D. and Robb, Russell M. and Guenther, David B. and Moffat, Anthony F. J. and Sasselov, Dimitar and Weiss, Werner W.},
  year = {2006},
  journal = {The Astrophysical Journal},
  volume = {648},
  number = {1},
  pages = {607--613},
  issn = {0004-637X},
  doi = {10.1086/505792},
  abstract = {The Microvariability and Oscillations of STars (MOST) photometric satellite observed three rotations of {$\varepsilon$} Eri continuously in late 2005. We detected two spots ({$\Delta$}m\textasciitilde 0.01) at different latitudes (20.0d, 31.5d) revolving with different periods (11.35 days, 11.55 days), from which we derive a differential rotation coefficient, k=0.11+.03-.02, in agreement with the prediction by Brown and coworkers for a young Sun-like star having roughly twice the solar angular velocity. The light curve was analyzed with the program StarSpotz, a modification of SPOTMODEL by Rib\'arik and coworkers. The best-fitting value for the inclination angle i=30deg+/-3deg is compatible with inclinations already estimated for the disk (\textasciitilde 25\textdegree ) and planetary orbit (26.2d). The inclination also leads to an equatorial rotation speed of 3.42 km s-1 and the photometric value of vsini=1.7 km s-1. When compared with spectroscopically determined values, the photometric vsini allows, in principle, an independent estimate of the macroturbulent velocity. Both spots would have distorted the radial velocity curve \textasciitilde +/-10 m s-1 by the Rossiter-McLaughlin effect, which is similar to the stellar radial velocity ``noise'' detected by others. Details of the StarSpotz model and of the uniqueness tests that we applied in order to arrive at a best solution and realistic estimates of errors in the derived parameters are given. Based on data from the MOST satellite, a Canadian Space Agency mission, jointly operated by Dynacon Inc., the University of Toronto Institute of Aerospace Studies, and the University of British Columbia, with the assistance of the University of Vienna.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5R27QT3Z/Croll et al. - 2006.pdf}
}

@article{Cunha2002,
  title = {A Theoretical Instability Strip for Rapidly Oscillating {{Ap}} Stars},
  author = {Cunha, Margarida S.},
  year = {2002},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {333},
  number = {1},
  pages = {47--54},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2002.05377.x},
  urldate = {2020-03-31},
  abstract = {The mechanism responsible for exciting high-order acoustic oscillations in rapidly oscillating Ap stars is still an open issue. Recently, Balmforth et al. (hereafter BCDGV) proposed a model according to which high-frequency oscillations may be excited in roAp stars if the intensities of the magnetic fields present in these stars are sufficiently large to suppress convection at least in some region of their envelopes. Using models similar to those proposed by BCDGV, we predict the theoretical edges of the instability strip appropriate to roAp stars and compare them with the observations. Moreover, we discuss our results in the light of some of the systematic differences found between roAp stars, noAp stars and Ap stars in general. We suggest that a combination of intrinsic differences between these types of stars and a bias related to the frequencies of the unstable oscillations might hold the explanation to some of the differences observed.},
  keywords = {notion,notion-database,Stars: chemically peculiar,Stars: magnetic fields,Stars: oscillations,Stars: variables: other},
  file = {/Users/lbugnet/Zotero/storage/WZGP7L3C/full-text.pdf}
}

@article{Cunha2005,
  title = {Asteroseismic Theory of Rapidly Oscillating {{Ap}} Stars},
  author = {Cunha, Margarida S.},
  year = {2005},
  journal = {Journal of Astrophysics and Astronomy},
  volume = {26},
  number = {2-3},
  pages = {213--221},
  issn = {02506335},
  doi = {10.1007/BF02702329},
  abstract = {This paper reviews some of the important advances made over the last decade concerning theory of roAp stars.},
  keywords = {Chemically peculiar,Magnetic,notion,notion-database,roAp,Stars: variable},
  file = {/Users/lbugnet/Zotero/storage/HGQ8IY8W/Cunha - 2005.pdf}
}

@article{Cunha2013,
  title = {Testing Excitation Models of Rapidly Oscillating {{Ap}} Stars with Interferometry},
  author = {Cunha, M. S. and Alentiev, D. and Brand{\~a}o, I. M. and Perraut, K.},
  year = {2013},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {436},
  number = {2},
  eprint = {1310.3019},
  doi = {10.1093/mnras/stt1679},
  urldate = {2020-04-09},
  abstract = {Rapidly oscillating Ap stars are unique objects in the potential they offer to study the interplay between a number of important physical phenomena, in particular, pulsations, magnetic fields, diffusion, and convection. Nevertheless, the simple understanding of how the observed pulsations are excited in these stars is still in progress. In this work we perform a test to what is possibly the most widely accepted excitation theory for this class of stellar pulsators. The test is based on the study of a subset of members of this class for which stringent data on the fundamental parameters are available thanks to interferometry. For three out of the four stars considered in this study, we find that linear, non-adiabatic models with envelope convection suppressed around the magnetic poles can reproduce well the frequency region where oscillations are observed. For the fourth star in our sample no agreement is found, indicating that a new excitation mechanism must be considered. For the three stars whose observed frequencies can be explained by the excitation models under discussion, we derive the minimum angular extent of the region where convection must be suppressed. Finally, we find that the frequency regions where modes are expected to be excited in these models is very sensitive to the stellar radius. This opens the interesting possibility of determining this quantity and related ones, such as the effective temperature or luminosity, from comparison between model predictions and observations, in other targets for which these parameters are not well determined.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UH2L7RVQ/full-text.pdf}
}

@article{Cunha2015,
  title = {Oscillations in G-Mode Period Spacings in Red Giants as a Way to Determine Their State of Evolution},
  author = {Cunha, M. S. and Stello, D. and Avelino, P. P. and {Christensen-Dalsgaard}, J.},
  year = {2015},
  journal = {EPJ Web of Conferences},
  volume = {101},
  pages = {1--6},
  issn = {2100014X},
  doi = {10.1051/epjconf/201510101014},
  abstract = {In this work we consider the sensitivity of gravity-mode period spacings to sharp changes in the inner structure of red giant stars, more specifically in the buoyancy frequency inside the g-mode propagation cavity. Based on a comparison between the solutions to the linear pulsation equations in the Cowling approximation for pure g-modes with results obtained with a full oscillation code we identify and correctly interpret the signature of the above-mentioned sharp variations in the period spacings. Two examples, of red giant models in different evolutionary phases, are discussed. Detection of these signatures in CoRoT, Kepler or future PLATO red-giant stars would pin down their evolutionary state in an unprecedented way.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9HXXWIYD/Cunha et al. - 2015.pdf}
}

@article{Cunha2015a,
  title = {Structural Glitches near the Cores of Red Giants Revealed by Oscillations in G-Mode Period Spacings from Stellar Models},
  author = {Cunha, M. S. and Stello, D. and Avelino, P. P. and {Christensen-Dalsgaard}, J. and Townsend, R. H.D.},
  year = {2015},
  month = jun,
  journal = {Astrophysical Journal},
  volume = {805},
  number = {2},
  eprint = {1503.09085},
  pages = {127},
  publisher = {{Institute of Physics Publishing}},
  issn = {15384357},
  doi = {10.1088/0004-637X/805/2/127},
  urldate = {2021-02-22},
  abstract = {With recent advances in asteroseismology it is now possible to peer into the cores of red giants, potentially providing a way to study processes such as nuclear burning and mixing through their imprint as sharp structural variations - glitches - in the stellar cores. Here we show how such core glitches can affect the oscillations we observe in red giants. We derive an analytical expression describing the expected frequency pattern in the presence of a glitch. This formulation also accounts for the coupling between acoustic and gravity waves. From an extensive set of canonical stellar models we find glitch-induced variation in the period spacing and inertia of non-radial modes during several phases of red giant evolution. Significant changes are seen in the appearance of mode amplitude and frequency patterns in asteroseismic diagrams such as the power spectrum and the \'e chelle diagram. Interestingly, along the red giant branch glitch-induced variation occurs only at the luminosity bump, potentially providing a direct seismic indicator of stars in that particular evolution stage. Similarly, we find the variation at only certain post-helium-ignition evolution stages, namely, in the early phases of helium core burning and at the beginning of helium shell burning, signifying the asymptotic giant branch bump. Based on our results, we note that assuming stars to be glitch-free, while they are not, can result in an incorrect estimate of the period spacing. We further note that including diffusion and mixing beyond classical Schwarzschild could affect the characteristics of the glitches, potentially providing a way to study these physical processes.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: evolution,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/V599422G/full-text.pdf}
}

@inproceedings{Cunha2018,
  title = {Theory of Stellar Oscillations},
  booktitle = {Astrophysics and {{Space Science Proceedings}}},
  author = {Cunha, Margarida S.},
  year = {2018},
  volume = {49},
  eprint = {1711.01236},
  issn = {15706605},
  doi = {10.1007/978-3-319-59315-9_2},
  abstract = {In recent years, astronomers have witnessed major progresses in the field of stellar physics. This was made possible thanks to the combination of a solid theoretical understanding of the phenomena of stellar pulsations and the availability of a tremendous amount of exquisite space-based asteroseismic data. In this context, this chapter reviews the basic theory of stellar pulsations, considering small, adiabatic perturbations to a static, spherically symmetric equilibrium. It~starts with a brief discussion of the solar oscillation spectrum, followed by the setting of the theoretical problem, including the presentation of the equations of hydrodynamics, their perturbation, and a discussion of the functional form of the solutions. Emphasis is put on the physical properties of the different types of modes, in particular acoustic (p-) and gravity (g-) modes and their propagation cavities. The surface (f-) mode solutions are also discussed. While not attempting to be comprehensive, it is hoped that the summary presented in this chapter addresses the most important theoretical aspects that are required for a solid start in stellar pulsations research.},
  archiveprefix = {arxiv},
  isbn = {978-3-319-59314-2},
  keywords = {notion,notion-database}
}

@article{Cunha2019,
  title = {Analytical Modelling of Period Spacings across the {{HR}} Diagram},
  author = {Cunha, M. S. and Avelino, P. P. and {Christensen-Dalsgaard}, J. and Stello, D. and Vrard, M. and Jiang, C. and Mosser, B.},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {490},
  number = {1},
  eprint = {1909.04966},
  pages = {909--926},
  issn = {13652966},
  doi = {10.1093/mnras/stz2582},
  abstract = {The characterization of stellar cores may be accomplished through the modelling of asteroseismic data from stars exhibiting either gravity-mode or mixed-mode pulsations, potentially shedding light on the physical processes responsible for the production, mixing, and segregation of chemical elements. In this work, we validate against model data an analytical expression for the period spacing that will facilitate the inference of the properties of stellar cores, including the detection and characterization of buoyancy glitches (strong chemical gradients). This asymptotically based analytical expression is tested both in models with and without buoyancy glitches. It does not assume that glitches are small and, consequently, predicts non-sinusoidal glitch-induced period-spacing variations, as often seen in model and real data. We show that the glitch position and width inferred from the fitting of the analytical expression to model data consisting of pure gravity modes are in close agreement (typically better than 7 per cent relative difference) with the properties measured directly from the stellar models. In the case of fitting mixed-mode model data, the same expression is shown to reproduce well the numerical results, when the glitch properties are known a priori. In addition, the fits performed to mixed-mode model data reveal a frequency dependence of the coupling coefficient, q, for a moderate-luminosity red-giant-branch model star. Finally, we find that fitting the analytical expression to the mixed-mode period spacings may provide a way to infer the frequencies of the pure acoustic dipole modes that would exist if no coupling took place between acoustic and gravity waves.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4B8HJ8Z5/Cunha et al. - 2019.pdf}
}

@article{cunhaAnalyticalModellingPeriod2019,
  title = {Analytical Modelling of Period Spacings across the {{HR}} Diagram},
  author = {Cunha, M. S. and Avelino, P. P. and {Christensen-Dalsgaard}, J. and Stello, D. and Vrard, M. and Jiang, C. and Mosser, B.},
  year = {2019},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {490},
  number = {1},
  eprint = {1909.04966},
  primaryclass = {astro-ph},
  pages = {909--926},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/stz2582},
  urldate = {2023-06-06},
  abstract = {The characterisation of stellar cores may be accomplished through the modelling of asteroseismic data from stars exhibiting either gravity-mode or mixed-mode pulsations, potentially shedding light on the physical processes responsible for the production, mixing, and segregation of chemical elements. In this work we validate against model data an analytical expression for the period spacing that will facilitate the inference of the properties of stellar cores, including the detection and characterisation of buoyancy glitches (strong chemical gradients). This asymptotically-based analytical expression is tested both in models with and without buoyancy glitches. It does not assume that glitches are small and, consequently, predicts non-sinusoidal glitch-induced period-spacing variations, as often seen in model and real data. We show that the glitch position and width inferred from the fitting of the analytical expression to model data consisting of pure gravity modes are in close agreement (typically better than 7\$\textbackslash\%\$ relative difference) with the properties measured directly from the stellar models. In the case of fitting mixed-mode model data, the same expression is shown to reproduce well the numerical results, when the glitch properties are known a priori. In addition, the fits performed to mixed-mode model data reveal a frequency dependence of the coupling coefficient, \$q\$, for a moderate-luminosity red-giant-branch model star. Finally, we find that fitting the analytical expression to the mixed-mode period spacings may provide a way to infer the frequencies of the pure acoustic dipole modes that would exist if no coupling took place between acoustic and gravity waves.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/RAYGXMYU/Cunha et al. - 2019 - Analytical modelling of period spacings across the.pdf;/Users/lbugnet/Zotero/storage/P5Z8P3BV/1909.html}
}

@article{Damiani2015,
  title = {Evolution of Angular-Momentum-Losing Exoplanetary Systems {{Revisiting Darwin}} Stability},
  author = {Damiani, C. and Lanza, A. F.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {574},
  eprint = {1411.3802},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424318},
  abstract = {Aims. We assess the importance of tidal evolution and its interplay with magnetic braking in the population of hot-Jupiter planetary systems. Methods. By minimizing the total mechanical energy of a given system under the constraint of stellar angular momentum loss, we rigorously find the conditions for the existence of dynamical equilibrium states. We estimate their duration, in particular when the wind torque spinning down the star is almost compensated for by the tidal torque spinning it up. We introduce dimensionless variables to characterize the tidal evolution of observed hot Jupiter systems and discuss their spin and orbital states using generalized Darwin diagrams based on our new approach. Results. We show that their orbital properties are related to the effective temperature of their host stars. The long-term evolution of planets orbiting F- and G-type stars is significantly different owing to the combined effect of magnetic braking and tidal dissipation. The existence of a quasi-stationary state, in the case of short-period planets, can significantly delay their tidal evolution that would otherwise bring the planet to fall into its host star. Most of the planets known to orbit F-type stars are presently found to be near this stationary state, probably in a configuration not too far from what they had when their host star settled on the zero-age main sequence. Considering the importance of angular momentum loss in the early stages of stellar evolution, our results indicate that it has to be considered to properly test the migration scenarios of planetary system formation.},
  archiveprefix = {arxiv},
  keywords = {Methods: analytical,notion,notion-database,Planet-star interactions,Planets and satellites: dynamical evolution and st,Stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/9H7J9564/Damiani, Lanza - 2015.pdf}
}

@article{Das2020,
  title = {Sensitivity {{Kernels}} for {{Inferring Lorentz Stresses}} from {{Normal-mode Frequency Splittings}} in the {{Sun}}},
  author = {Das, Srijan Bharati and Chakraborty, Tuneer and Hanasoge, Shravan M. and Tromp, Jeroen},
  year = {2020},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {897},
  pages = {38},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ab8e3a},
  urldate = {2023-06-05},
  abstract = {Departures from standard spherically symmetric solar models, in the form of perturbations such as global and local-scale flows and structural asphericities, result in the splitting of eigenfrequencies in the observed spectrum of solar oscillations. Drawing from prevalent ideas in normal-mode-coupling theory in geophysical literature, we devise a procedure that enables the computation of sensitivity kernels for general Lorentz-stress fields in the Sun. Mode coupling due to any perturbation requires careful consideration of self- and cross coupling of multiplets. Invoking the isolated-multiplet approximation allows for limiting the treatment to purely self coupling, requiring significantly less computational resources. We identify the presence of such isolated multiplets under the effect of Lorentz stresses in the Sun. Currently, solar missions allow for precise measurements of self coupling of multiplets via "a-coefficients" and the cross-spectral correlation signal that enables the estimation of the "structure coefficients". We demonstrate the forward problem for both self coupling (a-coefficients) and cross coupling (structure coefficients). In doing so, we plot the self-coupling kernels and estimate a-coefficients arising from a combination of deep-toroidal and surface-dipolar axisymmetric fields. We also compute the structure coefficients for an arbitrary general magnetic field (real and solenoidal) and plot the corresponding "splitting function", a convenient way to visualize the splitting of multiplets under 3D internal perturbations. The results discussed in this paper pave the way to formally pose an inverse problem and infer solar internal magnetic fields.},
  keywords = {1476,1500,1503,1964,709,73,Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,Helioseismology,Magnetohydrodynamics,Solar interior,Solar magnetic fields,Solar physics},
  annotation = {ADS Bibcode: 2020ApJ...897...38D},
  file = {/Users/lbugnet/Zotero/storage/ZRUYMUMM/Das et al. - 2020 - Sensitivity Kernels for Inferring Lorentz Stresses.pdf}
}

@article{Das2020a,
  title = {Sensitivity {{Kernels}} for {{Inferring Lorentz Stresses}} from {{Normal-mode Frequency Splittings}} in the {{Sun}}},
  author = {Das, Srijan Bharati and Chakraborty, Tuneer and Hanasoge, Shravan M. and Tromp, Jeroen},
  year = {2020},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {897},
  pages = {38},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ab8e3a},
  urldate = {2023-10-09},
  abstract = {Departures from standard spherically symmetric solar models, in the form of perturbations such as global and local-scale flows and structural asphericities, result in the splitting of eigenfrequencies in the observed spectrum of solar oscillations. Drawing from prevalent ideas in normal-mode-coupling theory in geophysical literature, we devise a procedure that enables the computation of sensitivity kernels for general Lorentz-stress fields in the Sun. Mode coupling due to any perturbation requires careful consideration of self- and cross coupling of multiplets. Invoking the isolated-multiplet approximation allows for limiting the treatment to purely self coupling, requiring significantly less computational resources. We identify the presence of such isolated multiplets under the effect of Lorentz stresses in the Sun. Currently, solar missions allow for precise measurements of self coupling of multiplets via "a-coefficients" and the cross-spectral correlation signal that enables the estimation of the "structure coefficients". We demonstrate the forward problem for both self coupling (a-coefficients) and cross coupling (structure coefficients). In doing so, we plot the self-coupling kernels and estimate a-coefficients arising from a combination of deep-toroidal and surface-dipolar axisymmetric fields. We also compute the structure coefficients for an arbitrary general magnetic field (real and solenoidal) and plot the corresponding "splitting function", a convenient way to visualize the splitting of multiplets under 3D internal perturbations. The results discussed in this paper pave the way to formally pose an inverse problem and infer solar internal magnetic fields.},
  keywords = {1476,1500,1503,1964,709,73,Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,Helioseismology,Magnetohydrodynamics,Solar interior,Solar magnetic fields,Solar physics},
  annotation = {ADS Bibcode: 2020ApJ...897...38D},
  file = {/Users/lbugnet/Zotero/storage/9VRTQI3N/Das et al. - 2020 - Sensitivity Kernels for Inferring Lorentz Stresses.pdf}
}

@article{dasSensitivityKernelsInferring2020,
  title = {Sensitivity {{Kernels}} for {{Inferring Lorentz Stresses}} from {{Normal-mode Frequency Splittings}} in the {{Sun}}},
  author = {Das, Srijan Bharati and Chakraborty, Tuneer and Hanasoge, Shravan M. and Tromp, Jeroen},
  year = {2020},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {897},
  pages = {38},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ab8e3a},
  urldate = {2023-05-23},
  abstract = {Departures from standard spherically symmetric solar models, in the form of perturbations such as global and local-scale flows and structural asphericities, result in the splitting of eigenfrequencies in the observed spectrum of solar oscillations. Drawing from prevalent ideas in normal-mode-coupling theory in geophysical literature, we devise a procedure that enables the computation of sensitivity kernels for general Lorentz-stress fields in the Sun. Mode coupling due to any perturbation requires careful consideration of self- and cross coupling of multiplets. Invoking the isolated-multiplet approximation allows for limiting the treatment to purely self coupling, requiring significantly less computational resources. We identify the presence of such isolated multiplets under the effect of Lorentz stresses in the Sun. Currently, solar missions allow for precise measurements of self coupling of multiplets via "a-coefficients" and the cross-spectral correlation signal that enables the estimation of the "structure coefficients". We demonstrate the forward problem for both self coupling (a-coefficients) and cross coupling (structure coefficients). In doing so, we plot the self-coupling kernels and estimate a-coefficients arising from a combination of deep-toroidal and surface-dipolar axisymmetric fields. We also compute the structure coefficients for an arbitrary general magnetic field (real and solenoidal) and plot the corresponding "splitting function", a convenient way to visualize the splitting of multiplets under 3D internal perturbations. The results discussed in this paper pave the way to formally pose an inverse problem and infer solar internal magnetic fields.},
  keywords = {1476,1500,1503,1964,709,73,Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,Helioseismology,Magnetohydrodynamics,Solar interior,Solar magnetic fields,Solar physics},
  annotation = {ADS Bibcode: 2020ApJ...897...38D},
  file = {/Users/lbugnet/Zotero/storage/DWJES5QX/Das et al. - 2020 - Sensitivity Kernels for Inferring Lorentz Stresses.pdf}
}

@article{Datta2015,
  title = {Automated Determination of G-Mode Period Spacing of Red Giant Stars},
  author = {Datta, Abhisek and Mazumdar, Anwesh and Gupta, Umang and Hekker, Saskia},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {447},
  number = {2},
  pages = {1935--1950},
  issn = {13652966},
  doi = {10.1093/mnras/stu2499},
  abstract = {The Kepler satellite has provided photometric timeseries data of unprecedented length, duty cycle and precision. To fully analyse these data for the tens of thousands of stars observed by Kepler, automated methods are a prerequisite. Here, we present an automated procedure to determine the period spacing of gravity modes in red giant stars ascending the red giant branch. The gravity modes reside in a cavity in the deep interior of the stars and provide information on the conditions in the stellar core. However, for red giants the gravity modes are not directly observable on the surface, hence this method is based on the pressure-gravity mixed modes that present observable features in the Fourier power spectrum. The method presented here is based on the vertical alignment and symmetry of these mixed modes in a period echelle diagram. We find that we can obtain reliable results for both model frequencies and observed frequencies. Additionally, we carried out Monte Carlo tests to obtain realistic uncertainties on the period spacings with different set of oscillation modes (for the models) and uncertainties on the frequencies. Furthermore, this method has been used to improve mode detection and identification of the observed frequencies in an iterative manner.},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/BBMGXJDI/Datta et al. - 2015.pdf;/Users/lbugnet/Zotero/storage/T763HJIG/Datta et al. - 2015.pdf}
}

@article{Davies2014,
  title = {{{BISON}} Data Preparation: {{A}} Correction for Differential Extinction and the Weighted Averaging of Contemporaneous Data},
  author = {Davies, G. R. and Chaplin, W. J. and Elsworth, Y. and Haleg, S. J.},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {441},
  number = {4},
  pages = {3009--3017},
  issn = {13652966},
  doi = {10.1093/mnras/stu803},
  abstract = {The Birmingham Solar Oscillations Network (BiSON) has provided high-quality high-cadence observations from as far back in time as 1978. These data must be calibrated from the raw observations into radial velocity and the quality of the calibration has a large impact on the signal-to-noise ratio of the final time series. The aim of this work is to maximize the potential science that can be performed with the BiSON data set by optimizing the calibration procedure. To achieve better levels of signal-to-noise ratio, we perform two key steps in the calibration process: we attempt a correction for terrestrial atmospheric differential extinction; and the resulting improvement in the calibration allows us to perform weighted averaging of contemporaneous data from different BiSON stations. The improvements listed produce significant improvement in the signal-to-noise ratio of the BiSON frequency-power spectrum across all frequency ranges. The reduction of noise in the power spectrum will allow future work to provide greater constraint on changes in the oscillation spectrum with solar activity. In addition, the analysis of the low-frequency region suggests that we have achieved a noise level that may allow us to improve estimates of the upper limit of g-mode amplitudes. \textcopyright{} 2014 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {Data analysis-sun,Helioseismology-sun,Methods,notion,notion-database,Oscillations},
  file = {/Users/lbugnet/Zotero/storage/3FJ65587/Davies et al. - 2014(2).pdf}
}

@article{Davies2014a,
  title = {Low-Frequency, Low-Degree Solar p-Mode Properties from 22 Years of Birmingham Solar Oscillations Network Data},
  author = {Davies, G. R. and Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. and Hale, S. J.},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {439},
  number = {2},
  pages = {2025--2032},
  issn = {13652966},
  doi = {10.1093/mnras/stu080},
  abstract = {The solar low-degree low-frequency modes of oscillation are of particular interest as their frequencies can be measured with very high precision and hence provide good constraints on seismic models. Here we detect and characterize these valuable measures of the solar interior from a 22 yr Birmingham Solar Oscillations Network data set. We report mode frequencies, line widths, heights, amplitudes, and rotational splitting, all with robust uncertainties. The new values of frequency, rotational splitting, amplitude, and line width we provide will help place new constraints on hydrostatic and rotational structure, plus diagnostics of near-surface convection. Further to this, by assuming simple power laws, we extrapolate mode properties to lower frequencies.We demonstrate that the low-l low-frequency p modes have a low signalto-noise ratio and that this cannot be overcome simply by continued observation. It will be necessary to observe the Sun in novel ways to 'beat' the intrinsic granulation noise. \textcopyright{} 2014 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/KW4H3MBI/Davies et al. - 2014.pdf}
}

@article{Davies2015,
  title = {Asteroseismic Inference on Rotation, Gyrochronology and Planetary System Dynamics of 16 {{Cygni}}},
  author = {Davies, G. R. and Chaplin, W. J. and Farr, W. M. and Garc{\'i}a, R. A. and Lund, M. N. and Mathis, S. and Metcalfe, T. S. and Appourchaux, T. and Basu, S. and Benomar, O. and Campante, T. L. and Ceillier, T. and Elsworth, Y. and Handberg, R. and Salabert, D. and Stello, D.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {446},
  number = {3},
  pages = {2959--2966},
  issn = {13652966},
  doi = {10.1093/mnras/stu2331},
  abstract = {The solar analogues 16 Cyg A and B are excellent asteroseismic targets in the Kepler field of view and together with a red dwarf and a Jovian planet form an interesting system. For these more evolved Sun-like stars we cannot detect surface rotation with the current Kepler data but instead use the technique of asteroseimology to determine rotational properties of both 16 Cyg A and B. We find the rotation periods to be 23.8+1.5-1.8 and 23.2+11.5-3.2 d, and the angles of inclination to be 56+6-5 \textdegree{} and 36+17-7 \textdegree, for A and B, respectively. Together with these results we use the published mass and age to suggest that, under the assumption of a solar-like rotation profile, 16 Cyg A could be used when calibrating gyrochronology relations. In addition, we discuss the known 16 Cyg B star-planet eccentricity and measured low obliquity which is consistent with Kozai cycling and tidal theory.},
  keywords = {notion,notion-database,Planet-star interactions,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/XHSIJVJ6/Davies et al. - 2015.pdf}
}

@article{Davies2016b,
  title = {Oscillation Frequencies for 35 {{Kepler}} Solar-Type Planet-Hosting Stars Using {{Bayesian}} Techniques and Machine Learning},
  author = {Davies, G. R. and Silva Aguirre, V. and Bedding, T. R. and Handberg, R. and Lund, M. N. and Chaplin, W. J. and Huber, D. and White, T. R. and Benomar, O. and Hekker, S. and Basu, S. and Campante, T. L. and {Christensen-Dalsgaard}, J. and Elsworth, Y. and Karoff, C. and Kjeldsen, H. and Lundkvist, M. S. and Metcalfe, T. S. and Stello, D.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {456},
  number = {2},
  eprint = {1511.02105},
  pages = {2183--2195},
  issn = {13652966},
  doi = {10.1093/mnras/stv2593},
  abstract = {Kepler has revolutionized our understanding of both exoplanets and their host stars.Asteroseismology is a valuable tool in the characterization of stars and Kepler is an excellent observing facility to perform asteroseismology. Here we select a sample of 35 Kepler solar-type stars which host transiting exoplanets (or planet candidates) with detected solar-like oscillations. Using available Kepler short cadence data up to Quarter 16 we create power spectra optimized for asteroseismology of solar-type stars. We identify modes of oscillation and estimate mode frequencies by 'peak bagging' using a Bayesian Markov Chain Monte Carlo framework. In addition, we expand the methodology of quality assurance using a Bayesian unsupervised machine learning approach. We report the measured frequencies of the modes of oscillation for all 35 stars and frequency ratios commonly used in detailed asteroseismic modelling. Due to the high correlations associated with frequency ratios we report the covariance matrix of all frequencies measured and frequency ratios calculated. These frequencies, frequency ratios, and covariance matrices can be used to obtain tight constraint on the fundamental parameters of these planet-hosting stars.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Planetary systems,Planets and satellites: fundamental parameters,Stars: evolution,Stars: fundamental parameters,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VQJVEFYP/Davies et al. - 2016.pdf}
}

@article{Davies2016c,
  title = {Asteroseismology of Red Giants: {{From}} Analysing Light Curves to Estimating Ages},
  author = {Davies, G. R. and Miglio, A.},
  year = {2016},
  journal = {Astronomische Nachrichten},
  volume = {337},
  number = {8-9},
  eprint = {1601.02802},
  pages = {774--782},
  issn = {15213994},
  doi = {10.1002/asna.201612371},
  abstract = {Asteroseismology has started to provide constraints on stellar properties that will be essential to accurately reconstruct the history of the Milky Way. Here we look at the information content in data sets representing current and future space missions (CoRoT, Kepler, K2, TESS, and PLATO) for red giant stars. We describe techniques for extracting the information in the frequency power spectrum and apply these techniques to Kepler data sets of different observing length to represent the different space missions. We demonstrate that for KIC 12008916, a low-luminosity red giant branch star, we can extract useful information from all data sets, and for all but the shortest data set we obtain good constraint on the g-mode period spacing and core rotation rates. We discuss how the high precision in these parameters will constrain the stellar properties of stellar radius, distance, mass and age. We show that high precision can be achieved in mass and hence age when values of the g-mode period spacing are available. We caution that tests to establish the accuracy of asteroseismic masses and ages are still ``work in progress''.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,stars: fundamental parameters,stars: individual (KIC 12008916),stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/2VBRR22R/Davies, Miglio - 2016.pdf}
}

@article{Davies2017,
  title = {Using Red Clump Stars to Correct the {{Gaia DR1}} Parallaxes},
  author = {Davies, Guy R. and Lund, Mikkel N. and Miglio, Andrea and Elsworth, Yvonne and Kuszlewicz, James S. and North, Thomas S.H. and Rendle, Ben and Chaplin, William J. and Rodrigues, Tha{\'i}se S. and Campante, Tiago L. and Girardi, L{\'e}o and Hale, Steven J. and Hall, Oliver and Jones, Caitlin D. and Kawaler, Steven D. and Roxburgh, Ian and Schofield, Mathew},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {598},
  eprint = {1701.02506},
  pages = {2--6},
  issn = {14320746},
  doi = {10.1051/0004-6361/201630066},
  abstract = {Recent results have suggested that there is tension between the Gaia DR1 TGAS distances and the distances obtained using luminosities determined by eclipsing binaries or asteroseismology on red giant stars. We use the Ks-band luminosities of red clump stars, identified and characterized by asteroseismology, to make independent distance estimates. Our results suggest that Gaia TGAS distances contain a systematic error that decreases with increasing distance. We propose a correction to mitigate this offset as a function of parallax that is valid for the Kepler field and values of parallax that are less than {$\sim$}1.6 mas. For parallaxes greater than this, we find agreement with previously published values. We note that the TGAS distances to the red clump stars of the open cluster M67 show a high level of disagreement that is difficult to correct for.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Parallaxes,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TKV3RPT5/Davies et al. - 2017.pdf}
}

@article{Dawes1864,
  title = {Results of Some Recent {{Observations}} of the {{Solar Surface}}, with {{Remarks}}},
  author = {Dawes, W.R.},
  year = {1864},
  journal = {MNRAS},
  volume = {24},
  urldate = {2020-03-13},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZZLP8DGQ/full-text.pdf}
}

@article{Debosscher2007,
  title = {Automated Supervised Classification of Variable Stars {{I}}. {{Methodology}}},
  author = {Debosscher, J. and Sarro, L. M. and Aerts, C. and Cuypers, J. and Vandenbussche, B. and Garrido, R. and Solano, E.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {475},
  number = {3},
  eprint = {0711.0703},
  pages = {1159--1183},
  issn = {14320746},
  doi = {10.1051/0004-6361:20077638},
  abstract = {Context. The fast classification of new variable stars is an important step in making them available for further research. Selection of science targets from large databases is much more efficient if they have been classified first. Defining the classes in terms of physical parameters is also important to get an unbiased statistical view on the variability mechanisms and the borders of instability strips. Aims. Our goal is twofold: provide an overview of the stellar variability classes that are presently known, in terms of some relevant stellar parameters; use the class descriptions obtained as the basis for an automated "supervised classification" of large databases. Such automated classification will compare and assign new objects to a set of pre-defined variability training classes. Methods. For every variability class, a literature search was performed to find as many well-known member stars as possible, or a considerable subset if too many were present. Next, we searched on-line and private databases for their light curves in the visible band and performed period analysis and harmonic fitting. The derived light curve parameters are used to describe the classes and define the training classifiers. Results. We compared the performance of different classifiers in terms of percentage of correct identification, of confusion among classes and of computation time. We describe how well the classes can be separated using the proposed set of parameters and how future improvements can be made, based on new large databases such as the light curves to be assembled by the CoRoT and Kepler space missions. Conclusions. The derived classifiers' performances are so good in terms of success rate and computational speed that we will evaluate them in practice from the application of our methodology to a large subset of variable stars in the OGLE database and from comparison of the results with published OGLE variable star classifications based on human intervention. These results will be published in a subsequent paper. \textcopyright{} ESO 2007.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Stars: binaries: general,Stars: variables: general,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/ID74HCK8/Debosscher et al. - 2007.pdf}
}

@article{Debosscher2009,
  title = {Automated Supervised Classification of Variable Stars in the {{CoRoT}} Programme: {{Method}} and Application to the First Four Exoplanet Fields},
  author = {Debosscher, J. and Sarro, L. M. and L{\'o}pez, M. and Deleuil, M. and Aerts, C. and Auvergne, M. and Baglin, A. and Baudin, F. and Chadid, M. and Charpinet, S. and Cuypers, J. and De Ridder, J. and Garrido, R. and Hubert, A. M. and {Janot-Pacheco}, E. and Jorda, L. and Kaiser, A. and Kallinger, T. and Kollath, Z. and Maceroni, C. and Mathias, P. and Michel, E. and Moutou, C. and Neiner, C. and Ollivier, M. and Samadi, R. and Solano, E. and Surace, C. and Vandenbussche, B. and Weiss, W. W.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {519--534},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911618},
  abstract = {Aims. In this work, we describe the pipeline for the fast supervised classification of light curves observed by the CoRoT exoplanet CCDs. We present the classification results obtained for the first four measured fields, which represent a one-year in-orbit operation. Methods. The basis of the adopted supervised classification methodology has been described in detail in a previous paper, as is its application to the OGLE database. Here, we present the modifications of the algorithms and of the training set to optimize the performance when applied to the CoRoT data. Results. Classification results are presented for the observed fields IRa01, SRc01, LRc01, and LRa01 of the CoRoT mission. Statistics on the number of variables and the number of objects per class are given and typical light curves of high-probability candidates are shown. We also report on new stellar variability types discovered in the CoRoT data. The full classification results are publicly available.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Stars: binaries: general,Stars: variables: general,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/GCJXSPP2/Debosscher et al. - 2009.pdf}
}

@article{Debosscher2011,
  title = {Global Stellar Variability Study in the Field-of-View of the {{Kepler}} Satellite},
  author = {Debosscher, J. and Blomme, J. and Aerts, C. and De Ridder, J.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {529},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201015647},
  abstract = {Aims. We present the results of an automated variability analysis of the Kepler public data measured in the first quarter (Q1) of the mission. In total, about 150 000 light curves have been analysed to detect stellar variability and to identify new members of known variability classes. We also focus on detecting variables present in eclipsing binary systems, given the strong constraints on stellar fundamental parameters they can provide. Methods. The methodology we use here is based on the automated variability classification pipeline, which was previously developed for and successfully applied to the CoRoT exofield database and to the limited subset of a few thousand Kepler asteroseismology light curves. We use a Fourier decomposition of the light curves to describe their variability behaviour and use the resulting parameters to perform a supervised classification. Several improvements were made, including a separate extractor method to detect the presence of eclipses when other variability is present in the light curves. We also included two new variability classes compared to previous work: variables showing signs of rotational modulation and of activity. Results. Statistics are given on the number of variables and the number of good candidates per class. A comparison is made with results obtained for the CoRoT exoplanet data. We present some special discoveries, including variable stars in eclipsing binary systems. Many new candidate non-radial pulsators are found, mainly {$\delta$} Sct and {$\gamma$} Dor stars. We studied those samples in more detail by using 2MASS colours, and the full classification results are made available as an online catalogue. \textcopyright{} 2011 ESO.},
  keywords = {Binaries: eclipsing,Methods: data analysis,Methods: statistical,notion,notion-database,Stars: statistics,Stars: variables: general,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/C4YPLCXG/Debosscher et al. - 2011.pdf}
}

@article{DeCat2002,
  title = {A Study of Bright Southern Slowly Pulsating {{B}} Stars {{II}}. {{The}} Intrinsic Frequencies},
  author = {De Cat, Peter and Aerts, C.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {393},
  number = {3},
  pages = {965--981},
  publisher = {{EDP Sciences}},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021068},
  urldate = {2020-04-09},
  abstract = {We present the results of detailed frequency analyses of a sample of thirteen confirmed slowly pulsating B stars. Our analysis is based on a combination of elaborate photometric and spectroscopic data-sets. The original sample consists of a mixture of five confirmed slowly pulsating B stars and twelve candidate slowly pulsating B stars discovered thanks to the photometric measurements of the HIPPARCOS satellite. HD 55522 and HD 131120 turn out to be chemically peculiar stars. HD 169978 and HD 69144 are two ellipsoidal variables for which no intrinsic variability is found. At least nine of the thirteen studied slowly pulsating B stars are multi-periodic. For HD 74195, HD 85953, HD 123515 and HD 215573, the observed frequency spacings suggest that we are dealing with frequency multiplets. For the apparent mono-periodic binary HD 24587, it is not clear if the observed variations are induced by stellar pulsation and/or by rotation modulation. We highlight the statistical character of the observed pulsational properties of our sample.},
  keywords = {Binaries: spectroscopic,Line: profiles,notion,notion-database,Stars: early-type,Stars: oscillations,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/WMKBSZJ7/full-text.pdf}
}

@article{Decressin2009,
  title = {Diagnoses to Unravel Secular Hydrodynamical Processes in Rotating Main Sequence Stars},
  author = {Decressin, T and Mathis, S and Palacios, A and Siess, L and Talon, S and Charbonnel, C and Zahn, J.-P},
  year = {2009},
  journal = {Astronomy \& Astrophysics},
  volume = {495},
  eprint = {0812.0363v1},
  pages = {271--286},
  urldate = {2020-07-14},
  abstract = {Context. Recent progresses and constraints brought by helio and asteroseismology call for a better description of stellar interiors and an accurate description of rotation-driven mechanisms in stars. Aims. We present a detailed analysis of the main physical processes responsible for the transport of angular momentum and chemical species in the radiative regions of rotating stars. We focus on cases where meridional circulation and shear-induced turbulence only are included in the simulations (i.e., no internal gravity waves nor magnetic fields). We put special emphasis on analyzing the angular momentum transport loop and on identifying the contribution of each physical process involved. Methods. We develop a variety of diagnostic tools designed to help disentangle the role of the various transport mechanisms. Our analysis is based on a 2-D representation of the secular hydrodynamics, which is treated using expansions in spherical harmonics. By taking appropriate horizontal averages, the problem reduces to one dimension, making it implementable in a 1D stellar evolution code while preserving the advective character of angular momentum transport. We present a full reconstruction of the meridional circulation and of the associated fluctuations of temperature and mean molecular weight along with diagnosis for the transport of angular momentum, heat and chemicals. In the present paper these tools are used to validate the analysis of two main sequence stellar models of 1.5 and 20 M for which the hydrodynamics has been previously extensively studied in the literature. Results. We obtain a clear visualization and a precise estimation of the different terms entering the angular momentum and heat transport equations in radiative zones of rotating stars. This enables us to corroborate the main results obtained over the past decade by Zahn, Maeder, and collaborators concerning the secular hydrodynamics of such objects. We focus on the meridional circulation driven by angular momentum losses and structural readjustements. We confirm quantitatively for the first time through detailed computations and separation of the various components that the advection of entropy by this circulation is very well balanced by the barotropic effects and the thermal relaxation during most of the main sequence evolution. This enables us to derive simplifications for the thermal relaxation on this phase. The meridional currents in turn advect heat and generate temperature fluctuations that induce differential rotation through thermal wind thus closing the transport loop. We plan to make use of our refined diagnosis tools in forthcoming studies of secular (magneto-)hydrodynamics of stars at various evolutionary stages.},
  archiveprefix = {arxiv},
  keywords = {evolution,hydrodynamics-turbulence-stars,notion,notion-database,rotation},
  file = {/Users/lbugnet/Zotero/storage/VFYNCDPV/full-text.pdf}
}

@techreport{Decressin2018,
  title = {Diagnoses to Unravel Secular Hydrodynamical Processes in Rotating Main Sequence Stars},
  author = {Decressin, T and Mathis, S and Palacios, A and Siess, L and Talon, S and Charbonnel, C and Zahn, J.-P},
  year = {2018},
  eprint = {0812.0363v1},
  urldate = {2020-07-13},
  abstract = {Context. Recent progresses and constraints brought by helio and asteroseismology call for a better description of stellar interiors and an accurate description of rotation-driven mechanisms in stars. Aims. We present a detailed analysis of the main physical processes responsible for the transport of angular momentum and chemical species in the radiative regions of rotating stars. We focus on cases where meridional circulation and shear-induced turbulence only are included in the simulations (i.e., no internal gravity waves nor magnetic fields). We put special emphasis on analyzing the angular momentum transport loop and on identifying the contribution of each physical process involved. Methods. We develop a variety of diagnostic tools designed to help disentangle the role of the various transport mechanisms. Our analysis is based on a 2-D representation of the secular hydrodynamics, which is treated using expansions in spherical harmonics. By taking appropriate horizontal averages, the problem reduces to one dimension, making it implementable in a 1D stellar evolution code while preserving the advective character of angular momentum transport. We present a full reconstruction of the meridional circulation and of the associated fluctuations of temperature and mean molecular weight along with diagnosis for the transport of angular momentum, heat and chemicals. In the present paper these tools are used to validate the analysis of two main sequence stellar models of 1.5 and 20 M for which the hydrodynamics has been previously extensively studied in the literature. Results. We obtain a clear visualization and a precise estimation of the different terms entering the angular momentum and heat transport equations in radiative zones of rotating stars. This enables us to corroborate the main results obtained over the past decade by Zahn, Maeder, and collaborators concerning the secular hydrodynamics of such objects. We focus on the meridional circulation driven by angular momentum losses and structural readjustements. We confirm quantitatively for the first time through detailed computations and separation of the various components that the advection of entropy by this circulation is very well balanced by the barotropic effects and the thermal relaxation during most of the main sequence evolution. This enables us to derive simplifications for the thermal relaxation on this phase. The meridional currents in turn advect heat and generate temperature fluctuations that induce differential rotation through thermal wind thus closing the transport loop. We plan to make use of our refined diagnosis tools in forthcoming studies of secular (magneto-)hydrodynamics of stars at various evolutionary stages.},
  archiveprefix = {arxiv},
  keywords = {evolution,hydrodynamics-turbulence-stars,notion,notion-database,rotation},
  file = {/Users/lbugnet/Zotero/storage/ILY6Z8K5/full-text.pdf}
}

@article{Degroote2010,
  title = {Detection of Frequency Spacings in the Young {{O-type}} Binary {{HD}} 46149 from {{CoRoT}} Photometry},
  author = {Degroote, P. and Briquet, M. and Auvergne, M. and {Sim{\'o}n-D{\'i}az}, S. and Aerts, C. and Noels, A. and Rainer, M. and Hareter, M. and Poretti, E. and Mahy, L. and Oreiro, R. and Vu{\v c}kovi{\'c}, M. and Smolders, K. and Baglin, A. and Baudin, F. and Catala, C. and Michel, E. and Samadi, R.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {519},
  number = {3},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/201014543},
  abstract = {Aims. Using the CoRoT space based photometry of the O-type binary HD 46149, stellar atmospheric effects related to rotation can be separated from pulsations, because they leave distinct signatures in the light curve. This offers the possibility of characterising and exploiting any pulsations seismologically. Methods. Combining high-quality space based photometry, multi-wavelength photometry, spectroscopy and constraints imposed by binarity and cluster membership, the detected pulsations in HD 46149 are analyzed and compared with those for a grid of stellar evolutionary models in a proof-of-concept approach. Results. We present evidence of solar-like oscillations in a massive O-type star, and show that the observed frequency range and spacings are compatible with theoretical predictions. Thus, we unlock and confirm the strong potential of this seismically unexplored region in the HR diagram. \textcopyright{} 2010 ESO.},
  keywords = {asteroseismology,binaries: spectroscopic,notion,notion-database,stars: individual: HD46149,stars: massive,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RGPN7B77/Degroote et al. - 2010.pdf}
}

@article{Deheuvels2010,
  title = {Seismic and Spectroscopic Characterization of the Solar-like Pulsating {{CoRoT}} Target {{HD}}},
  author = {Deheuvels, S. and Bruntt, H. and Michel, E. and Barban, C. and Verner, G. and R{\'e}gulo, C. and Mosser, B. and Mathur, S. and Gaulme, P. and Garcia, R. A. and Boumier, P. and Appourchaux, T. and Samadi, R. and Catala, C. and Baudin, F. and Baglin, A. and Auvergne, M. and Roxburgh, I. W. and P{\'e}rez Hern{\'a}ndez, F.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {515},
  number = {9},
  pages = {1--13},
  issn = {14320746},
  doi = {10.1051/0004-6361/200913490},
  abstract = {The star HD 49385 is the first G-type solar-like pulsator observed in the seismology field of the space telescope CoRoT. The satellite collected 137 days of high-precision photometric data on this star, confirming that it presents solar-like oscillations. HD 49385 was also observed in spectroscopy with the NARVAL spectrograph in January 2009. Aims.Our goal is to characterize HD 49385 using both spectroscopic and seismic data. Methods.The fundamental stellar parameters of HD 49385 are derived with the semi-automatic software VWA, and the projected rotational velocity is estimated by fitting synthetic profiles to isolated lines in the observed spectrum. A maximum likelihood estimation is used to determine the parameters of the observed p modes. We perform a global fit, in which modes are fitted simultaneously over nine radial orders, with degrees ranging from = 0 to = 3 (36 individual modes). Results. Precise estimates of the atmospheric parameters (Teff, [M/H], log g) and of the v sin i of HD 49385 are obtained. The seismic analysis of the star leads to a clear identification of the modes for degrees = 0, 1, 2. Around the maximum of the signal (v =1013 {$\mu$}Hz), some peaks are found significant and compatible with the expected characteristics of = 3 modes. Our fit yields robust estimates of the frequencies, linewidths and amplitudes of the modes. We find amplitudes of {$\sim$}5.6 {$\pm$} 0.8 ppm for radial modes at the maximum of the signal. The lifetimes of the modes range from one day (at high frequency) to a bit more than two days (at low frequency). Significant peaks are found outside the identified ridges and are fitted. They are attributed to mixed modes. \textcopyright{} 2010 ESO.},
  keywords = {Methods: data analysis,Methods: observational,Methods: statistical,notion,notion-database,Stars: individual: HD 49385,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/88P5BM4Q/Deheuvels et al. - 2010.pdf}
}

@article{Deheuvels2010a,
  title = {Constraints on the Core {$\mu$}-Gradient of the Solar-like Star {{HD}} 49385 via Low-Degree Mixed Modes},
  author = {Deheuvels, S. and Michel, E.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  eprint = {1006.3178},
  pages = {929--932},
  issn = {00046337},
  doi = {10.1002/asna.201011429},
  abstract = {The existence of an {$\mathscr{l}$} = 1 avoided crossing in the spectrum of the solar-like pulsator CoRoT*-target HD 49385 (*The CoRoT space mission, launched on 2006 December 27, was developed and is operated by the CNES with participation of the Science Programs of ESA; ESA's RSSD, Austria, Belgium, Brazil, Germany, and Spain.) was established by Deheuvels \& Michel (2009). It is the first confirmed detection of such a phenomenon. The authors showed in a preliminary modeling of the star that it was in a post main sequence status. Being a 1.3 M{$\cdot$} -star, HD 49385 has had a convective core during its main sequence phase. The {$\mu$} -gradient left by the withdrawal of this core bears information about the processes of transport at the boundary of the core. We here investigate the constraints that the observed avoided crossing brings on the {$\mu$} -gradient in the core of the star (\textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim) Copyright \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/S6LUCPIT/Deheuvels, Michel - 2010.pdf}
}

@article{Deheuvels2010b,
  title = {Survival of a Convective Core in Low-Mass Solar-like Pulsator {{HD}} 203608},
  author = {Deheuvels, S. and Michel, E. and Goupil, M. J. and Marques, J. P. and Mosser, B. and Dupret, M. A. and Lebreton, Y. and Pichon, B. and Morel, P.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {514},
  number = {2},
  pages = {1--7},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911991},
  abstract = {Context. A 5-night asteroseismic observation of the F8V star HD 203608 was conducted in August 2006 with harps, followed by an analysis of the data, and a preliminary modeling of the star (Mosser et al. 2008). The stellar parameters were significantly constrained, but the behavior of one of the seismic indexes (the small spacing {$\delta$}V01) could not be fitted with the observed one, even with the best considered models. Aims. We study the possibility of improving the agreement between models and observations by changing the physical properties of the inner parts of the star (to which {$\delta$}01 is sensitive). Methods. We show that, in spite of its low mass, it is possible to produce models of HD 203608 with a convective core. No such model was considered in the preliminary modeling. In practice, we obtain these models here by assuming some extra mixing at the edge of the early convective core. We optimized the model parameters using the Levenberg-Marquardt algorithm. Results. The agreement between the new best model with a convective core and the observations is much better than for the models without. All the observational parameters are fitted within 1-{$\sigma$} observational error bars. This is the first observational evidence of a convective core in an old and low-mass star such as HD 203608. In standard models of low-mass stars, the core withdraws shortly after the ZAMS. The survival of the core until the present age of HD 203608 provides very strong constraints on the size of the mixed zone associated to the convective core. Using overshooting as a proxy to model the processes of transport at the edge of the core, we find that to reproduce both global and seismic observations, we must have {$\alpha$} ov = 0.17 {$\pm$} 0.03 Hp for HD 203608. We revisit the process of the extension of the core lifetime due to overshooting in the particular case of HD 203608. \textcopyright{} ESO, 2010.},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/EBBV4CRL/Deheuvels et al. - 2010(2).pdf}
}

@article{Deheuvels2011,
  title = {Constraints on the Structure of the Core of Subgiants via Mixed Modes: {{The}} Case of {{HD}} 49385},
  author = {Deheuvels, S. and Michel, E.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {535},
  eprint = {1109.1191},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117232},
  abstract = {Context. The solar-like pulsator HD 49385 was observed with the CoRoT* satellite over a period of 137 days. The analysis of its oscillation spectrum yielded precise estimates of the mode frequencies over nine radial orders and distinguished some unusual characteristics, such as some modes outside the identified ridges in the \'echelle diagram and that the curvature of the {$\mathscr{l}$} = 1 ridge differs significantly from that of the {$\mathscr{l}$} = 0 ridge. Aims. We search for stellar models that can reproduce the peculiar features of the oscillation spectrum of HD 49385. After showing that they can be accounted for only by a low-frequency {$\mathscr{l}$} = 1 avoided crossing, we investigate the information provided by the mixed modes about the structure of the core of HD 49385. Methods. We propose a toy-model to study the case of avoided crossings with a strong coupling between the p-mode and g-mode cavities in order to establish the presence of mixed modes in the spectrum of HD 49385. We then show that traditional optimization techniques are ill-suited to stars with mixed modes in avoided crossing. We propose a new approach to the computation of grids of models that we apply to HD 49385. Results. The detection of mixed modes leads us to establish the post-main-sequence status of HD 49385. The mixed mode frequencies suggest that there is a strong coupling between the p-mode and g-mode cavities. As a result, we show that the amount of core overshooting in HD 49385 is either very small (0 {$<$} {$\alpha$}ov {$<$} 0.05) or moderate (0.18 {$<$} {$\alpha$}ov {$<$} 0.20). The mixing length parameter is found to be significantly lower than the solar one ({$\alpha$}CGM = 0.55 {$\pm$} 0.04 compared to the solar value {$\alpha\odot$} = 0.64). Finally, we show that the revised solar abundances of Asplund ensure closer agreement with the observations than the classical ones of Grevesse \& Noels. At each step, we investigate the origin and meaning of these seismic diagnostics in terms of the physical structure of the star. Conclusions. The subgiant HD 49385 is the first star for which a thorough modeling has been attempted to reproduce all the properties of an avoided crossing. It has provided the opportunity to show that the study of the coupling between the cavities in these stars can provide valuable insight into open questions such as core overshooting, the efficiency of convection, and the abundances of heavy elements in stars. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual: HD 49385,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/SX7QEW5Z/Deheuvels, Michel - 2011.pdf}
}

@article{Deheuvels2012a,
  title = {Seismic Evidence for a Rapidly Rotating Core in a Lower-Giant-Branch Star Observed with Kepler},
  author = {Deheuvels, S. and Garc{\'i}a, R. A. and Chaplin, W. J. and Basu, S. and Antia, H. M. and Appourchaux, T. and Benomar, O. and Davies, G. R. and Elsworth, Y. and Gizon, L. and Goupil, M. J. and Reese, D. R. and Regulo, C. and Schou, J. and Stahn, T. and Casagrande, L. and {Christensen-Dalsgaard}, J. and Fischer, D. and Hekker, S. and Kjeldsen, H. and Mathur, S. and Mosser, B. and Pinsonneault, M. and Valenti, J. and Christiansen, J. L. and Kinemuchi, K. and Mullally, F.},
  year = {2012},
  journal = {The Astrophysical Journal},
  volume = {756},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/756/1/19},
  abstract = {Rotation is expected to have an important influence on the structure and the evolution of stars. However, the mechanisms of angular momentum transport in stars remain theoretically uncertain and very complex to take into account in stellar models. To achieve a better understanding of these processes, we desperately need observational constraints on the internal rotation of stars, which until very recently was restricted to the Sun. In this paper, we report the detection of mixed modes - i.e., modes that behave both as g modes in the core and as p modes in the envelope - in the spectrum of the early red giant KIC7341231, which was observed during one year with the Kepler spacecraft. By performing an analysis of the oscillation spectrum of the star, we show that its non-radial modes are clearly split by stellar rotation and we are able to determine precisely the rotational splittings of 18 modes. We then find a stellar model that reproduces very well the observed atmospheric and seismic properties of the star. We use this model to perform inversions of the internal rotation profile of the star, which enables us to show that the core of the star is rotating at least five times faster than the envelope. This will shed new light on the processes of transport of angular momentum in stars. In particular, this result can be used to place constraints on the angular momentum coupling between the core and the envelope of early red giants, which could help us discriminate between the theories that have been proposed over the last few decades. \textcopyright{} \textcopyright{} 2012. The American Astronomical Society. All rights reserved..},
  keywords = {notion,notion-database,stars: evolution,stars: individual (KIC 7341231),stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/SYSDZ3XQ/Deheuvels et al. - 2012.pdf}
}

@article{Deheuvels2014a,
  title = {Seismic Constraints on the Radial Dependence of the Internal Rotation Profiles of Six {{Kepler}} Subgiants and Young Red Giants},
  author = {Deheuvels, S. and Do{\v g}an, G. and Goupil, M. J. and Appourchaux, T. and Benomar, O. and Bruntt, H. and Campante, T. L. and Casagrande, L. and Ceillier, T. and Davies, G. R. and De Cat, P. and Fu, J. N. and Garc{\'i}a, R. A. and Lobel, A. and Mosser, B. and Reese, D. R. and Regulo, C. and Schou, J. and Stahn, T. and Thygesen, A. O. and Yang, X. H. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Eggenberger, P. and Gizon, L. and Mathis, S. and {Molenda-Zakowicz}, J. and Pinsonneault, M.},
  year = {2014},
  journal = {Astronomy \& Astrophysics},
  volume = {564},
  issn = {14320746},
  doi = {10.1051/0004-6361/201322779},
  abstract = {Context. We still do not understand which physical mechanisms are responsible for the transport of angular momentum inside stars. The recent detection of mixed modes that contain the clear signature of rotation in the spectra of Kepler subgiants and red giants gives us the opportunity to make progress on this question. Aims. Our aim is to probe the radial dependence of the rotation profiles for a sample of Kepler targets. For this purpose, subgiants and early red giants are particularly interesting targets because their rotational splittings are more sensitive to the rotation outside the deeper core than is the case for their more evolved counterparts. Methods. We first extracted the rotational splittings and frequencies of the modes for six young Kepler red giants. We then performed a seismic modeling of these stars using the evolutionary codes Cesam2k and astec. By using the observed splittings and the rotational kernels of the optimal models, we inverted the internal rotation profiles of the six stars. Results. We obtain estimates of the core rotation rates for these stars, and upper limits to the rotation in their convective envelope. We show that the rotation contrast between the core and the envelope increases during the subgiant branch. Our results also suggest that the core of subgiants spins up with time, while their envelope spins down. For two of the stars, we show that a discontinuous rotation profile with a deep discontinuity reproduces the observed splittings significantly better than a smooth rotation profile. Interestingly, the depths that are found to be most probable for the discontinuities roughly coincide with the location of the H-burning shell, which separates the layers that contract from those that expand. Conclusions. We characterized the differential rotation pattern of six young giants with a range of metallicities, and with both radiative and convective cores on the main sequence. This will bring observational constraints to the scenarios of angular momentum transport in stars. Moreover, if the existence of sharp gradients in the rotation profiles of young red giants is confirmed, it is expected to help in distinguishing between the physical processes that could transport angular momentum in the subgiant and red giant branches. \textcopyright{} 2014 ESO.},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: interiors,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/SMQECNSN/Deheuvels et al. - 2014.pdf}
}

@article{Deheuvels2015,
  title = {Seismic Evidence for a Weak Radial Differential Rotation in Intermediate-Mass Core Helium Burning Stars},
  author = {Deheuvels, S. and Ballot, J. and Beck, P. G. and Mosser, B. and {\O}stensen, R. and Garc{\'i}a, R. A. and Goupil, M. J.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {580},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526449},
  abstract = {Context. The detection of mixed modes that are split by rotation in Kepler red giants has made it possible to probe the internal rotation profiles of these stars, which brings new constraints on the transport of angular momentum in stars. Rotation rates in the central regions of intermediate-mass core helium burning stars (secondary clump stars) have recently been measured. Aims. Our aim is to exploit the rotational splittings of mixed modes to estimate the amount of radial differential rotation in the interior of secondary clump stars using Kepler data in order to place constraints on angular momentum transport in intermediate-mass stars. Methods. We select a subsample of Kepler secondary clump stars with mixed modes that are clearly rotationally split. By applying a thorough statistical analysis, we show that the splittings of gravity-dominated modes (trapped in central regions) and of p-dominated modes (trapped in the envelope) can be measured. We then use these splittings to estimate the amount of differential rotation by using inversion techniques and by applying a simplified approach based on asymptotic theory. Results. We obtain evidence for a weak radial differential rotation for six of the seven targets that were selected, with the central regions rotating from 1.8 {$\pm$} 0.3 to 3.2 {$\pm$} 1.0 times faster than the envelope. The last target is found to be consistent with a solid-body rotation. Conclusions. This demonstrates that an efficient redistribution of angular momentum occurs after the end of the main sequence in the interior of intermediate-mass stars, either during the short-lived subgiant phase or once He-burning has started in the core. In either case, this should bring constraints on the angular momentum transport mechanisms that are at work.},
  keywords = {evolution,notion,notion-database,oscillations-stars,rotation-stars,stars,Stars: evolution,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/DEYHX3KJ/Deheuvels et al. - 2015.pdf}
}

@article{Deheuvels2015a,
  title = {Seismic Evidence for a Weak Radial Differential Rotation in Intermediate-Mass Core Helium Burning Stars},
  author = {Deheuvels, S. and Ballot, J. and Beck, P. G. and Mosser, B. and {\O}stensen, R. and Garc{\'i}a, R. A. and Goupil, M. J.},
  year = {2015},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {580},
  pages = {A96},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201526449},
  urldate = {2023-09-22},
  abstract = {Context. The detection of mixed modes that are split by rotation in Kepler red giants has made it possible to probe the internal rotation profiles of these stars, which brings new constraints on the transport of angular momentum in stars. Rotation rates in the central regions of intermediate-mass core helium burning stars (secondary clump stars) have recently been measured. Aims: Our aim is to exploit the rotational splittings of mixed modes to estimate the amount of radial differential rotation in the interior of secondary clump stars using Kepler data in order to place constraints on angular momentum transport in intermediate-mass stars. Methods: We select a subsample of Kepler secondary clump stars with mixed modes that are clearly rotationally split. By applying a thorough statistical analysis, we show that the splittings of gravity-dominated modes (trapped in central regions) and of p-dominated modes (trapped in the envelope) can be measured. We then use these splittings to estimate the amount of differential rotation by using inversion techniques and by applying a simplified approach based on asymptotic theory. Results: We obtain evidence for a weak radial differential rotation for six of the seven targets that were selected, with the central regions rotating from 1.8 {$\pm$} 0.3 to 3.2 {$\pm$} 1.0 times faster than the envelope. The last target is found to be consistent with a solid-body rotation. Conclusions: This demonstrates that an efficient redistribution of angular momentum occurs after the end of the main sequence in the interior of intermediate-mass stars, either during the short-lived subgiant phase or once He-burning has started in the core. In either case, this should bring constraints on the angular momentum transport mechanisms that are at work.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2015A\&A...580A..96D},
  file = {/Users/lbugnet/Zotero/storage/DZR26E37/Deheuvels et al. - 2015 - Seismic evidence for a weak radial differential ro.pdf}
}

@article{Deheuvels2016,
  title = {Measuring the Extent of Convective Cores in Low-Mass Stars Using {{Kepler}} Data: {{Toward}} a Calibration of Core Overshooting},
  author = {Deheuvels, S. and Brand{\~a}o, I. and Silva Aguirre, V. and Ballot, J. and Michel, E. and Cunha, M. S. and Lebreton, Y. and Appourchaux, T.},
  year = {2016},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {589},
  eprint = {1603.02332},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527967},
  urldate = {2020-06-19},
  abstract = {Context. Our poor understanding of the boundaries of convective cores generates large uncertainties on the extent of these cores and thus on stellar ages. The detection and precise characterization of solar-like oscillations in hundreds of main-sequence stars by CoRoT and Kepler has given the opportunity to revisit this problem. Aims. Our aim is to use asteroseismology to consistently measure the extent of convective cores in a sample of main-sequence stars whose masses lie around the mass limit for having a convective core. Methods. We first tested and validated a seismic diagnostic that was proposed to probe the extent of convective cores in a model-dependent way using the so-called r010 ratios, which are built with l = 0 and l = 1 modes. We applied this procedure to 24 low-mass stars chosen among Kepler targets to optimize the efficiency of this diagnostic. For this purpose, we computed grids of stellar models with both the Cesam2k and mesa evolution codes, where the extensions of convective cores were modeled either by an instantaneous mixing or as a diffusion process. Results. We found that 10 stars in our sample are in fact subgiants. Among the other targets, were able to unambiguously detect convective cores in eight stars, and we obtained seismic measurements of the extent of the mixed core in these targets with a good agreement between the Cesam2k and mesa codes. By performing optimizations using the Levenberg-Marquardt algorithm, we then obtained estimates of the amount of extra mixing beyond the core that is required in Cesam2k to reproduce seismic observations for these eight stars, and we showed that this can be used to propose a calibration of this quantity. This calibration depends on the prescription chosen for the extra mixing, but we found that it should also be valid for the code mesa, provided the same prescription is used. Conclusions. This study constitutes a first step toward calibrating the extension of convective cores in low-mass stars, which will help reduce the uncertainties on the ages of these stars.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,convection,notion,notion-database,stars: evolution,Stars: interiors},
  file = {/Users/lbugnet/Zotero/storage/P3NEN9WH/full-text.pdf}
}

@article{Deheuvels2017,
  title = {Near-Degeneracy Effects on the Frequencies of Rotationally-Split Mixed Modes in Red Giants},
  author = {Deheuvels, S. and Ouazzani, R. M. and Basu, S.},
  year = {2017},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {605},
  eprint = {1705.10326},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201730786},
  urldate = {2020-06-02},
  abstract = {Context. The Kepler space mission has made it possible to measure the rotational splittings of mixed modes in red giants, thereby providing an unprecedented opportunity to probe the internal rotation of these stars. Aims. Asymmetries have been detected in the rotational multiplets of several red giants. This is unexpected since all the red giants whose rotation profiles have been measured thus far are found to rotate slowly, and low rotation, in principle, produces symmetrical multiplets. Our aim here is to explain these asymmetries and find a way of exploiting them to probe the internal rotation of red giants. Methods. We show that in the cases where asymmetrical multiplets were detected, near-degeneracy effects are expected to occur, because of the combined effects of rotation and mode mixing. Such effects have not been taken into account so far. By using both perturbative and non-perturbative approaches, we show that near-degeneracy effects produce multiplet asymmetries that are very similar to the observations. We then propose and validate a method based on the perturbative approach to probe the internal rotation of red giants using multiplet asymmetries. Results. We successfully apply our method to the asymmetrical l = 2 multiplets of the Kepler young red giant KIC 7341231 and obtain precise estimates of its mean rotation in the core and the envelope. The observed asymmetries are reproduced with a good statistical agreement, which confirms that near-degeneracy effects are very likely the cause of the detected multiplet asymmetries. Conclusions. We expect near-degeneracy effects to be important for l = 2 mixed modes all along the red giant branch (RGB). For l = 1 modes, these effects can be neglected only at the base of the RGB. They must therefore be taken into account when interpreting rotational splittings and as shown here, they can bring valuable information about the internal rotation of red giants.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: Evolution,Stars: Individual: KIC 7341231,Stars: Oscillations,Stars: Rotation},
  file = {/Users/lbugnet/Zotero/storage/B54GQYWI/full-text.pdf}
}

@article{Deheuvels2018,
  title = {Seismic Characterization of Red Giants Going through the Helium-Core Flash},
  author = {Deheuvels, S. and Belkacem, K.},
  year = {2018},
  month = dec,
  journal = {Astronomy and Astrophysics},
  volume = {620},
  pages = {A43},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201833409},
  urldate = {2023-09-22},
  abstract = {Context. First-ascent red giants in the approximate mass range 0.7 {$\lessequivlnt$} M/M{$\odot$} {$\lessequivlnt$} 2 ignite helium in their degenerate core as a flash. Stellar evolution codes predict that the He flash consists of a series of consecutive subflashes. Observational evidence of the existence of the He flash and subflashes is lacking. The detection of mixed modes in red giants from space missions CoRoT and Kepler has opened new opportunities to search for such evidence. Aims: During a subflash, the He-burning shell is convective, which splits the cavity of gravity modes in two. We here investigate how this additional cavity modifies the oscillation spectrum of the star. We also address the question of the detectability of the modes, to determine whether they could be used to seismically identify red giants passing through the He flash. Methods: We calculate the asymptotic mode frequencies of stellar models going through a He subflash using the Jeffreys-Wentzel-Kramers-Brillouin (JWKB) approximation. To predict the detectability of the modes, we estimate their expected heights, taking into account the effects of radiative damping in the core. Our results are then compared to the oscillation spectra obtained by numerically calculating the mode frequencies during a He subflash. Results: We show that during a He subflash, the detectable oscillation spectrum mainly consists of modes trapped in the acoustic cavity and in the outer g-mode cavity. The spectrum should thus at first sight resemble that of a core-helium-burning giant. However, we find a list of clear, detectable features that could enable us to identify red giants passing through a He subflash. In particular, during a He subflash, several modes that are trapped in the innermost g-mode cavity are expected to be detectable. We show that these modes could be identified by their frequencies or by their rotational splittings. Other features, such as the measured period spacing of gravity modes or the location of the H-burning shell within the g-mode cavity could also be used to identify stars going through a He subflash. Conclusions: The features derived in this study can now be searched for in the large datasets provided by the CoRoT and Kepler missions.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: oscillations (including pulsations)},
  annotation = {ADS Bibcode: 2018A\&A...620A..43D},
  file = {/Users/lbugnet/Zotero/storage/6LD3GWE4/Deheuvels and Belkacem - 2018 - Seismic characterization of red giants going throu.pdf}
}

@article{Deheuvels2020,
  title = {Astronomy {{Astrophysics Seismic}} Evidence for near Solid-Body Rotation in Two {{Kepler}} Subgiants and Implications for Angular Momentum Transport},
  author = {Deheuvels, S and Ballot, J and Eggenberger, P and Spada, F and Noll, A and Den Hartogh, J W},
  year = {2020},
  journal = {Astronomy \& Astrophysics},
  volume = {641},
  pages = {117},
  doi = {10.1051/0004-6361/202038578},
  urldate = {2021-03-18},
  abstract = {Context. Asteroseismic measurements of the internal rotation of subgiants and red giants all show the need for invoking a more efficient transport of angular momentum than theoretically predicted. Constraints on the core rotation rate are available starting from the base of the red giant branch (RGB) and we are still lacking information on the internal rotation of less evolved subgiants. Aims. We identify two young Kepler subgiants, KIC 8524425 and KIC 5955122, whose mixed modes are clearly split by rotation. We aim to probe their internal rotation profile and assess the efficiency of the angular momentum transport during this phase of the evolution. Methods. Using the full Kepler data set, we extracted the mode frequencies and rotational splittings for the two stars using a Bayesian approach. We then performed a detailed seismic modeling of both targets and used the rotational kernels to invert their internal rotation profiles using the MOLA inversion method. We thus obtained estimates of the average rotation rates in the g-mode cavity ({$\Omega$} g) and in the p-mode cavity ({$\Omega$} p). Results. We found that both stars are rotating nearly as solid bodies, with core-envelope contrasts of {$\Omega$} g /{$\Omega$} p = 0.68 {$\pm$} 0.47 for KIC 8524425 and {$\Omega$} g /{$\Omega$} p = 0.72 {$\pm$} 0.37 for KIC 5955122. This result shows that the internal transport of angular momentum has to occur faster than the timescale at which differential rotation is forced in these stars (between 300 Myr and 600 Myr). By modeling the additional transport of angular momentum as a diffusive process with a constant viscosity {$\nu$} add , we found that values of {$\nu$} add {$>$} 5 \texttimes{} 10 4 cm 2 s -1 are required to account for the internal rotation of KIC 8524425, and {$\nu$} add {$>$} 1.5 \texttimes{} 10 5 cm 2 s -1 for KIC 5955122. These values are lower than or comparable to the efficiency of the core-envelope coupling during the main sequence, as given by the surface rotation of stars in open clusters. On the other hand, they are higher than the viscosity needed to reproduce the rotation of subgiants near the base of the RGB. Conclusions. Our results yield further evidence that the efficiency of the internal redistribution of angular momentum decreases during the subgiant phase. We thus bring new constraints that will need to be accounted for by mechanisms that are proposed as candidates for angular momentum transport in subgiants and red giants.},
  keywords = {asteroseismology-stars,individual,KIC 5955122,KIC 8524425-stars,notion,notion-database,oscillations-stars,rotation-stars},
  file = {/Users/lbugnet/Zotero/storage/8GMKSN42/full-text.pdf}
}

@article{Deheuvels2022,
  title = {Strong Magnetic Fields Detected in the Cores of 11 Red Giant Stars Using Gravity-Mode Period Spacings},
  author = {Deheuvels, S. and Li, G. and Ballot, J. and Ligni{\`e}res, F.},
  year = {2023},
  month = feb,
  journal = {Astronomy \& Astrophysics},
  volume = {670},
  pages = {L16},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202245282},
  urldate = {2023-04-04},
  abstract = {Despite their importance in stellar evolution, little is known about magnetic fields in the interior of stars. The recent seismic detection of magnetic fields in the core of several red giant stars has given measurements of their strength and information on their topology. We revisit the puzzling case of hydrogen-shell burning giants that show deviations from the expected regular period spacing of gravity modes. These stars also tend to have a measured period spacing that is too low compared to their counterparts. In this Letter, we show that these two features are well accounted for by strong magnetic fields in the cores of these stars. For 11 Kepler red giants showing these anomalies, we placed lower limits on the core field strengths ranging from 40 to 610 kG. For one star, the measured field exceeds the critical field above which gravity waves no longer propagate in the core. We find that this star shows mixed mode suppression at low frequency, which further suggests that this phenomenon might be related to strong core magnetic fields.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/48NSQ855/Deheuvels et al. - 2023 - Strong magnetic fields detected in the cores of 11.pdf}
}

@article{Deleuil2008,
  title = {Transiting Exoplanets from the {{CoRoT}} Space Mission},
  author = {Deleuil, M. and Deeg, H. J. and Alonso, R. and Bouchy, F. and Rouan, D. and Auvergne, M. and Baglin, A. and Aigrain, S. and Almenara, J. M. and Barbieri, M. and Barge, P. and Bruntt, H. and Bord{\'e}, P. and Collier Cameron, A. and Csizmadia, {\relax Sz}. and {De la Reza}, R. and Dvorak, R. and Erikson, A. and Fridlund, M. and Gandolfi, D. and Gillon, M. and Guenther, E. and Guillot, T. and Hatzes, A. and H{\'e}brard, G. and Jorda, L. and Lammer, H. and L{\'e}ger, A. and Llebaria, A. and Loeillet, B. and Mayor, M. and Mazeh, T. and Moutou, C. and Ollivier, M. and P{\"a}tzold, M. and Pont, F. and Queloz, D. and Rauer, H. and Schneider, J. and Shporer, A. and Wuchterl, G. and Zucker, S.},
  year = {2008},
  journal = {Astronomy \& Astrophysics},
  volume = {491},
  number = {3},
  pages = {889--897},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:200810625},
  abstract = {Aims.We report the discovery of very shallow ({$\increment$}F/F {$\approx$} 3.4\texttimes 10-4), periodic dips in the light curve of an active V = 11.7G9V star observed bythe CoRoT satellite, which we interpret as caused by a transiting companion.We describe the3-colour CoRoT dataand complementary ground-based observations that support the planetary nature of the companion. Methods.We used CoRoT colours information, good angular resolution ground-based photometric observations in- and out- of transit, adaptive optics imaging, near-infrared spectroscopy, and preliminary results from radial velocity measurements, to test the diluted eclipsing binary scenarios. The parameters of the host star were derived from optical spectra, which were then combined with the CoRoT light curve to derive parameters of the companion. Results.We examined all conceivable cases of false positives carefully, and all the tests support the planetary hypothesis. Blends with separation {$>$}0.40or triple systems are almost excluded with a 8 \texttimes{} 10-4 risk left.We conclude that, inasmuch we have been exhaustive, we have discovered a planetary companion, named CoRoT-7b, for which we derive a period of 0.853 59 {$\pm$}3 \texttimes{} 10-5 day and a radius of Rp = 1.68 {$\pm$}0.09 REarth.Analysis of preliminary radial velocity data yields an upper limit of 21 MEarth for the companion mass, supporting the finding. Conclusions. CoRoT-7b is very likely the first Super-Earth with a measured radius. This object illustrates what will probably become a common situation with missions such as Kepler, namely the need to establish the planetary origin of transits in the absence of a firm radial velocity detection and mass measurement. The composition of CoRoT-7bremains loosely constrained without a precise mass. A veryhighsurface temperature on its irradiated face, {$\approx$}1800\textendash 2600 K at the substellar point, and a very low one, {$\approx$}50 K, on its dark face assuming no atmosphere, have been derived.},
  keywords = {notion,notion-database,photometry,planetary systems,{planetary systems, techniques: photometry, techniq},radial velocity,techniques},
  file = {/Users/lbugnet/Zotero/storage/S7WU62GS/Deleuil et al. - 2008.pdf}
}

@article{DelVecchio2023,
  title = {Rotational {{Splitting}} of {{Pulsating Hot Subdwarfs Observed}} by {{TESS}}},
  author = {Del Vecchio, Gabriana and Barlow, Brad},
  year = {2023},
  month = sep,
  volume = {55},
  pages = {337.06},
  urldate = {2023-10-15},
  abstract = {Hot subdwarf B (sdB) stars are stripped red giants with a helium-fusing core. They are thought to form in binaries through Roche lobe overflow and common envelope interactions. Many hot subdwarfs pulsate with gravity and/or acoustic-mode oscillations, and asteroseismological studies of their vibrations can shed light on their interior structures and fundamental parameters like mass and radius. Stellar rotation can also be observed through a "splitting" of pulsation modes in a Lomb Scargle periodogram. Here we analyze high-cadence TESS photometry of several dozen pulsating hot subdwarfs and look for evidence of rotational splitting.},
  annotation = {ADS Bibcode: 2023AAS...24233706D}
}

@article{Demarque2008,
  title = {{{YREC}}: {{The Yale}} Rotating Stellar Evolution Code: {{Non-rotating}} Version, Seismology Applications},
  author = {Demarque, P. and Guenther, D. B. and Li, L. H. and Mazumdar, A. and Straka, C. W.},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  pages = {31--41},
  issn = {1572946X},
  doi = {10.1007/s10509-007-9698-y},
  abstract = {The stellar evolution code YREC is outlined with emphasis on its applications to helio- and asteroseismology. The procedure for calculating calibrated solar and stellar models is described. Other features of the code such as a non-local treatment of convective core overshoot, and the implementation of a parametrized description of turbulence in stellar models, are considered in some detail. The code has been extensively used for other astrophysical applications, some of which are briefly mentioned at the end of the paper. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  keywords = {Convection,Methods: numerical,notion,notion-database,Stars: evolution,Stars: interior},
  file = {/Users/lbugnet/Zotero/storage/L46D2PJX/Demarque et al. - 2008.pdf}
}

@article{DeMedeiros1996,
  title = {The Distribution of Rotational Velocity for Evolved Stars.},
  author = {{de Medeiros}, J. R. and Da Rocha, C. and Mayor, M.},
  year = {1996},
  journal = {A\&A},
  volume = {314},
  pages = {499--502},
  issn = {0004-6361},
  urldate = {2020-07-13},
  keywords = {notion,notion-database,STARS: FUNDAMENTAL PARAMETERS,STARS: ROTATION,STARS: STATISTICS}
}

@article{denHartogh2019,
  title = {Constraining Transport of Angular Momentum in Stars. {{Combining}} Asteroseismic Observations of Core Helium Burning Stars and White Dwarfs},
  author = {{den Hartogh}, J. W. and Eggenberger, P. and Hirschi, R.},
  year = {2019},
  month = feb,
  journal = {Astronomy \& Astrophysics},
  volume = {622},
  pages = {A187},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201834330},
  urldate = {2023-09-22},
  abstract = {Context. Transport of angular momentum has been a challenging topic within the stellar evolution community, even more since the recent asteroseismic surveys. All published studies on rotation using asteroseismic observations show a discrepancy between the observed and calculated rotation rates, indicating there is an undetermined process of angular momentum transport active in these stars. Aims: We aim to constrain the efficiency of this process by investigating rotation rates of 2.5 M{$\odot$} stars. Methods: First, we investigated whether the Tayler-Spruit dynamo could be responsible for the extra transport of angular momentum for stars with an initial mass of 2.5 M{$\odot$}. Then, by computing rotating models including a constant additional artificial viscosity, we determined the efficiency of the missing process of angular momentum transport by comparing the models to the asteroseismic observations of core helium burning stars. Parameter studies were performed to investigate the effect of the stellar evolution code used, initial mass, and evolutionary stage. We evolved our models into the white dwarf phase, and provide a comparison to white dwarf rotation rates. Results: The Tayler-Spruit dynamo is unable to provide enough transport of angular momentum to reach the observed values of the core helium burning stars investigated in this paper. We find that a value for the additional artificial viscosity {$\nu$}add around 107 cm2 s-1 provides enough transport of angular momentum. However, the rotational period of these models is too high in the white dwarf phase to match the white dwarf observations. From this comparison we infer that the efficiency of the missing process must decrease during the core helium burning phase. When excluding the {$\nu$}add during core helium burning phase, we can match the rotational periods of both the core helium burning stars and white dwarfs.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2019A\&A...622A.187D},
  file = {/Users/lbugnet/Zotero/storage/MAXINXP8/den Hartogh et al. - 2019 - Constraining transport of angular momentum in star.pdf}
}

@article{DenHartogh2020,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum {{III}}. {{Using}} the Rotation Rates of Intermediate-Mass Stars to Test the {{Fuller-formalism}}},
  author = {Den Hartogh, J W and Eggenberger, P and Deheuvels, S},
  year = {2020},
  journal = {Astronomy \& Astrophysics},
  volume = {634},
  doi = {10.1051/0004-6361/202037568},
  abstract = {Context. The internal characteristics of stars, such as their core rotation rates, are obtained via asteroseismic observations. A comparison of core rotation rates found in this way with core rotation rates as predicted by stellar evolution models demonstrate a large discrepancy. This means that there must be a process of angular momentum transport missing in the current theory of stellar evolution. A new formalism was recently proposed to fill in for this missing process, which has the Tayler instability as its starting point (by Fuller et al. 2019, MNRAS, 485, 3661, hereafter referred to as "Fuller-formalism"). Aims. We investigate the effect of the Fuller-formalism on the internal rotation of stellar models with an initial mass of 2.5 M. Methods. Stellar evolution models, including the Fuller-formalism, of intermediate-mass stars were calculated to make a comparison between asteroseismically obtained core rotation rates in the core He burning phase and in the white dwarf phase. Results. Our main results show that models including the Fuller-formalism can match the core rotation rates obtained for the core He burning phases. However, these models are unable to match the rotation rates obtained for white dwarfs. When we exclude the Fuller-formalism at the end of the core He burning phase, the white dwarf rotation rates of the models match the observed rates. Conclusions. We conclude that in the present form, the Fuller-formalism cannot be the sole solution for the missing process of angular momentum transport in intermediate-mass stars.},
  isbn = {3060901201},
  keywords = {evolution-stars,interiors-stars,notion,notion-database,oscillations,rotation-stars,stars},
  file = {/Users/lbugnet/Zotero/storage/WGJQCL6C/full-text.pdf}
}

@article{denHartogh2020,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum. {{III}}. {{Using}} the Rotation Rates of Intermediate-Mass Stars to Test the {{Fuller-formalism}}},
  author = {{den Hartogh}, J. W. and Eggenberger, P. and Deheuvels, S.},
  year = {2020},
  month = feb,
  journal = {Astronomy \& Astrophysics},
  volume = {634},
  pages = {L16},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202037568},
  urldate = {2023-09-22},
  abstract = {Context. The internal characteristics of stars, such as their core rotation rates, are obtained via asteroseismic observations. A comparison of core rotation rates found in this way with core rotation rates as predicted by stellar evolution models demonstrate a large discrepancy. This means that there must be a process of angular momentum transport missing in the current theory of stellar evolution. A new formalism was recently proposed to fill in for this missing process, which has the Tayler instability as its starting point (by Fuller et al. 2019, MNRAS, 485, 3661, hereafter referred to as "Fuller-formalism"). Aims: We investigate the effect of the Fuller-formalism on the internal rotation of stellar models with an initial mass of 2.5 M{$\odot$}. Methods: Stellar evolution models, including the Fuller-formalism, of intermediate-mass stars were calculated to make a comparison between asteroseismically obtained core rotation rates in the core He burning phase and in the white dwarf phase. Results: Our main results show that models including the Fuller-formalism can match the core rotation rates obtained for the core He burning phases. However, these models are unable to match the rotation rates obtained for white dwarfs. When we exclude the Fuller-formalism at the end of the core He burning phase, the white dwarf rotation rates of the models match the observed rates. Conclusions: We conclude that in the present form, the Fuller-formalism cannot be the sole solution for the missing process of angular momentum transport in intermediate-mass stars.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2020A\&A...634L..16D},
  file = {/Users/lbugnet/Zotero/storage/QR6KRCH4/den Hartogh et al. - 2020 - Asteroseismology of evolved stars to constrain the.pdf}
}

@article{Denissenkov2007,
  title = {A {{Revised Prescription}} for the {{Tayler-Spruit Dynamo}}: {{Magnetic Angular Momentum Transport}} in {{Stars}}},
  shorttitle = {A {{Revised Prescription}} for the {{Tayler-Spruit Dynamo}}},
  author = {Denissenkov, Pavel A. and Pinsonneault, Marc},
  year = {2007},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {655},
  pages = {1157--1165},
  issn = {0004-637X},
  doi = {10.1086/510345},
  urldate = {2023-10-09},
  abstract = {Angular momentum transport by internal magnetic fields is an important ingredient for stellar interior models. In this paper we critically examine the basic heuristic assumptions in the model of the Tayler-Spruit dynamo, which describes how a pinch-type instability of a toroidal magnetic field in differentially rotating stellar radiative zones may result in large-scale fluid motion. We agree with prior published work both on the existence of the instability and its nearly horizontal geometry for perturbations. However, the approximations in the original Acheson dispersion relation are valid only for small length scales, and we disagree that the dispersion relation can be extrapolated to horizontal length scales of order the radius of the star. We contend that dynamical effects, in particular, angular momentum conservation, limit the maximum horizontal length scale. We therefore present transport coefficients for chemical mixing and angular momentum redistribution by magnetic torques that are significantly different from previous published values. The new magnetic viscosity is reduced by 2-3 orders of magnitude compared to the old one, and we find that magnetic angular momentum transport by this mechanism is very sensitive to gradients in the mean molecular weight. The revised coefficients are more compatible with empirical constraints on the timescale of core-envelope coupling in young stars than the previous ones. However, solar models including only this mechanism possess a rapidly rotating core, in contradiction with helioseismic data. Previous studies had found strong core-envelope coupling, both for solar models and for the cores of massive evolved stars. We conclude that the Tayler-Spruit mechanism may be important for envelope angular momentum transport but that some other process must be responsible for efficient spin-down of stellar cores.},
  keywords = {Astrophysics,Stars: Interiors,Stars: Magnetic Fields,Sun: Rotation},
  annotation = {ADS Bibcode: 2007ApJ...655.1157D},
  file = {/Users/lbugnet/Zotero/storage/A7LRMEP7/Denissenkov and Pinsonneault - 2007 - A Revised Prescription for the Tayler-Spruit Dynam.pdf}
}

@article{DeRidder2006,
  title = {Discovery of Solar-like Oscillations in the Red Giant {$\epsilon$} {{Ophiuchi}}},
  author = {De Ridder, J. and Barban, C. and Carrier, F. and Mazumdar, A. and Eggenberger, P. and Aerts, C. and Deruyter, S. and Vanautgaerden, J.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {448},
  number = {2},
  pages = {689--695},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053331},
  abstract = {We present the discovery of solar-like oscillations in time-series of the G9.5 red giant e Ophiuchi. The data were obtained with the CORALIE spectrograph at the 1.2 m Swiss telescope in La Silla and the ELODIE spectrograph at the 1.93 m telescope at the Observatoire de Haute Provence. Periodic variations can be observed in the radial velocity time series of individual nights. In the power spectrum of the radial velocity time series there is a clear power excess around 60{$\mu$}Hz, and several individual oscillation frequencies can be distinguished. Our auto-correlation and comb response analysis reveals a large separation of either 4.8 {$\mu$}Hz or (its 11.57 {$\mu$}Hz alias) 6.7 {$\mu$}Hz. We estimate the position of e Oph in the HR diagram, and verify whether CESAM shell hydrogen-burning stellar models exist that can reproduce the observed frequency separation. \textcopyright{} ESO 2006.},
  keywords = {notion,notion-database,Stars: individual: HD 146791,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WM2PIP75/De Ridder et al. - 2006.pdf}
}

@article{DeRidder2009,
  title = {Non-Radial Oscillation Modes with Long Lifetimes in Giant Stars},
  author = {De Ridder, Joris and Barban, Caroline and Baudin, Fr{\'e}d{\'e}ric and Carrier, Fabien and Hatzes, Artie P. and Hekker, Saskia and Kallinger, Thomas and Weiss, Werner W. and Baglin, Annie and Auvergne, Michel and Samadi, R{\'e}za and Barge, Pierre and Deleuil, Magali},
  year = {2009},
  journal = {Nature},
  volume = {459},
  number = {7245},
  pages = {398--400},
  issn = {00280836},
  doi = {10.1038/nature08022},
  abstract = {Towards the end of their lives, stars like the Sun greatly expand to become red giant stars. Such evolved stars could provide stringent tests of stellar theory, as many uncertainties of the internal stellar structure accumulate with age. Important examples are convective overshooting and rotational mixing during the central hydrogen-burning phase, which determine the mass of the helium core, but which are not well understood. In principle, analysis of radial and non-radial stellar oscillations can be used to constrain the mass of the helium core. Although all giants are expected to oscillate, it has hitherto been unclear whether non-radial modes are observable at all in red giants, or whether the oscillation modes have a short or a long mode lifetime, which determines the observational precision of the frequencies. Here we report the presence of radial and non-radial oscillations in more than 300 giant stars. For at least some of the giants, the mode lifetimes are of the order of a month. We observe giant stars with equally spaced frequency peaks in the Fourier spectrum of the time series, as well as giants for which the spectrum seems to be more complex. No satisfactory theoretical explanation currently exists for our observations. \textcopyright{} 2009 Macmillan Publishers Limited.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8CDAN4T8/De Ridder et al. - 2009.pdf}
}

@article{Deubner1984,
  title = {Helioseismology: {{Oscillations}} as a {{Diagnostic}} of the {{Solar Interior}}},
  author = {Deubner, Franz-Ludwig and Gough, Douglas},
  year = {1984},
  month = sep,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {22},
  number = {1},
  pages = {593--619},
  publisher = {{Annual Reviews}},
  issn = {0066-4146},
  doi = {10.1146/annurev.aa.22.090184.003113},
  urldate = {2020-06-26},
  abstract = {Contents: (1) Introduction. (2) Resonant cavities in the Sun. (3) Observational methods. (4) High-degree modes: Solar structure. Subphotospheric velocities. (5) Low-degree modes: High-order p modes. Gravity modes. Solar structure. (6) Five-minute modes of intermediate degree. (7) Limb observations. (8) Problems for the immediate future. Appendix: Classification of stellar oscillations.},
  keywords = {notion,notion-database}
}

@article{deubnerObservationsLowWavenumber1975,
  title = {Observations of Low Wavenumber Nonradial Eigenmodes of the Sun.},
  author = {Deubner, F. -L. and {-L.}, F.},
  year = {1975},
  journal = {A\&A},
  volume = {44},
  number = {2},
  pages = {371--375},
  issn = {0004-6361},
  urldate = {2020-10-19},
  keywords = {Astronomical Models,notion,notion-database,Photoelectric Emission,Photosphere,Solar Atmosphere,Solar Physics,Sound Waves,Spatial Distribution,Standing Waves,Velocity Distribution}
}

@article{Deupree,
  title = {Rotational {{SPlitting}} of {{Pulsation Modes}}},
  author = {Deupree, Robert G. and Beslin, Wilfried},
  keywords = {notion,notion-database,oscillations,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/XVEILKUG/Deupree, Beslin - Unknown.pdf}
}

@article{Dhouib2021a,
  title = {The Traditional Approximation of Rotation for Rapidly Rotating Stars and Planets. {{I}}. {{The}} Impact of Strong Deformation},
  author = {Dhouib, H. and Prat, V. and Van Reeth, T. and Mathis, S.},
  year = {2021},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {652},
  pages = {A154},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202140615},
  urldate = {2023-06-05},
  abstract = {Context. The traditional approximation of rotation (TAR) is a treatment of the hydrodynamic equations of rotating and stably stratified fluids in which the action of the Coriolis acceleration along the direction of the entropy and chemical stratifications is neglected because it is weak in comparison with the buoyancy Archimedean force. This leads to the neglect of the horizontal projection of the rotation vector in the equations for the dynamics of gravito-inertial waves (GIWs). The dependent variables in those equations then become separable into radial and horizontal parts as in the non-rotating case. The TAR is built on the assumptions that the star is spherical (i.e., its centrifugal deformation is neglected) and uniformly rotating. However, it has recently been generalised to include the effects of a moderate centrifugal deformation using a perturbative approach. Aims: We study the feasibility of carrying out a new generalisation to account for the centrifugal acceleration in the case of strongly deformed uniformly and rapidly rotating stars (and planets), and to identify the validity domain of this approximation. Methods: We built a complete formalism analytically that allows the study of the dynamics of GIWs in spheroidal coordinates which take the flattening of uniformly and rapidly rotating stars into account by assuming the hierarchies of frequencies adopted within the TAR in the spherical case. Results: Using 2D stellar models, we determine the validity domain of the generalised TAR as a function of the rotation rate of the star normalised by its critical angular velocity and its pseudo-radius. Assuming the anelastic and the two-dimensional Jeffreys-Wentzel-Kramers-Brillouin approximations, we derive a generalised Laplace tidal equation for the horizontal eigenfunctions of the GIWs and their asymptotic wave periods, which can be used to probe the structure and dynamics of rotating deformed stars with asteroseismology. The generalised TAR where the centrifugal deformation of a star (or planet) is taken into account non-perturbatively allows us to identify, within the framework of 2D Evolution STEllaire en Rotation models, the validity domain of this approximation which is reduced by increasing the rate of rotation. We can affirm with a level of confidence of 90\% that the TAR remains applicable in all the space domain of deformed stars rotating at a rotation rate lower than 20\% of the critical rotation rate. Conclusions: A new generalisation of the TAR, which takes the centrifugal acceleration into account in a non-perturbative way, is derived. This generalisation allows us to study the detectability and the signature of the centrifugal effects on GIWs in rapidly rotating deformed stars (and planets). We found that the effects of the centrifugal acceleration in rapidly rotating early-type stars on GIWs are theoretically detectable in modern space photometry using observations from Kepler. We found also, by comparing the period spacing pattern computed with the standard and the generalised TAR, that the centrifugal acceleration affects the period spacing by increasing its values for low radial orders and by decreasing them slightly for high radial orders.},
  keywords = {Astrophysics - Earth and Planetary Astrophysics,Astrophysics - Solar and Stellar Astrophysics,hydrodynamics,methods: analytical,methods: numerical,Physics - Atmospheric and Oceanic Physics,Physics - Fluid Dynamics,stars: oscillations,stars: rotation,waves},
  annotation = {ADS Bibcode: 2021A\&A...652A.154D},
  file = {/Users/lbugnet/Zotero/storage/D5SEZ282/Dhouib et al. - 2021 - The traditional approximation of rotation for rapi.pdf}
}

@article{Dhouib2021b,
  title = {The Traditional Approximation of Rotation for Rapidly Rotating Stars and Planets. {{II}}. {{Deformation}} and Differential Rotation},
  author = {Dhouib, H. and Prat, V. and Van Reeth, T. and Mathis, S.},
  year = {2021},
  month = dec,
  journal = {Astronomy and Astrophysics},
  volume = {656},
  pages = {A122},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202141152},
  urldate = {2023-06-05},
  abstract = {Context. We examine the dynamics of low-frequency gravito-inertial waves (GIWs) in differentially rotating deformed radiation zones in stars and planets by generalising the traditional approximation of rotation (TAR). The TAR treatment was built on the assumptions that the star is spherical (i.e. its centrifugal deformation is neglected) and uniformly rotating. However, it has been generalised in our previous work by including the effects of the centrifugal deformation using a non-perturbative approach. In the meantime, TAR has been generalised in spherical geometry to take the differential rotation into account. Aims: We aim to carry out a new generalisation of the TAR treatment to account for the differential rotation and the strong centrifugal deformation simultaneously. Methods: We generalise our previous work by taking into account the differential rotation in the derivation of our complete analytical formalism that allows the study of the dynamics of GIWs in differentially and rapidly rotating stars. Results: We derived the complete set of equations that generalises the TAR, simultaneously taking the full centrifugal acceleration and the differential rotation into account. Within the validity domain of the TAR, we derived a generalised Laplace tidal equation for the horizontal eigenfunctions and asymptotic wave periods of the GIWs, which can be used to probe the structure and dynamics of differentially rotating deformed stars with asteroseismology. Conclusions: A new generalisation of the TAR, which simultaneously takes into account the differential rotation and the centrifugal acceleration in a non-perturbative way, was derived. This generalisation allowed us to study the detectability and the signature of the differential rotation on GIWs in rapidly rotating deformed stars and planets. We found that the effects of the differential rotation in early-type deformed stars on GIWs is theoretically largely detectable in modern space photometry using observations from Kepler and TESS.},
  keywords = {Astrophysics - Earth and Planetary Astrophysics,Astrophysics - Solar and Stellar Astrophysics,hydrodynamics,methods: analytical,methods: numerical,Physics - Atmospheric and Oceanic Physics,Physics - Fluid Dynamics,stars: oscillations,stars: rotation,waves},
  annotation = {ADS Bibcode: 2021A\&A...656A.122D},
  file = {/Users/lbugnet/Zotero/storage/CHU3LWBN/Dhouib et al. - 2021 - The traditional approximation of rotation for rapi.pdf}
}

@article{Dhouib2022,
  title = {Detecting Deep Axisymmetric Toroidal Magnetic Fields in Stars. {{The}} Traditional Approximation of Rotation for Differentially Rotating Deep Spherical Shells with a General Azimuthal Magnetic Field},
  author = {Dhouib, H. and Mathis, S. and Bugnet, L. and Van Reeth, T. and Aerts, C.},
  year = {2022},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {661},
  pages = {A133},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202142956},
  urldate = {2023-10-09},
  abstract = {Context. Asteroseismology has revealed small core-to-surface rotation contrasts in stars in the whole Hertzsprung-Russell diagram. This is the signature of strong transport of angular momentum (AM) in stellar interiors. One of the plausible candidates to efficiently carry AM is magnetic fields with various topologies that could be present in stellar radiative zones. Among them, strong axisymmetric azimuthal (toroidal) magnetic fields have received a lot of interest. Indeed, if they are subject to the so-called Tayler instability, the accompanying triggered Maxwell stresses can transport AM efficiently. In addition, the electromotive force induced by the fluctuations of magnetic and velocity fields could potentially sustain a dynamo action that leads to the regeneration of the initial strong axisymmetric azimuthal magnetic field. Aims: The key question we aim to answer is whether we can detect signatures of these deep strong azimuthal magnetic fields. The only way to answer this question is asteroseismology, and the best laboratories of study are intermediate-mass and massive stars with external radiative envelopes. Most of these are rapid rotators during their main sequence. Therefore, we have to study stellar pulsations propagating in stably stratified, rotating, and potentially strongly magnetised radiative zones, namely magneto-gravito-inertial (MGI) waves. Methods: We generalise the traditional approximation of rotation (TAR) by simultaneously taking general axisymmetric differential rotation and azimuthal magnetic fields into account. Both the Coriolis acceleration and the Lorentz force are therefore treated in a non-perturbative way. Using this new formalism, we derive the asymptotic properties of MGI waves and their period spacings. Results: We find that toroidal magnetic fields induce a shift in the period spacings of gravity (g) and Rossby (r) modes. An equatorial azimuthal magnetic field with an amplitude of the order of 105 G leads to signatures that are detectable in period spacings for high-radial-order g and r modes in {$\gamma$} Doradus ({$\gamma$} Dor) and slowly pulsating B (SPB) stars. More complex hemispheric configurations are more difficult to observe, particularly when they are localised out of the propagation region of MGI modes, which can be localised in an equatorial belt. Conclusions: The magnetic TAR, which takes into account toroidal magnetic fields in a non-perturbative way, is derived. This new formalism allows us to assess the effects of the magnetic field in {$\gamma$} Dor and SPB stars on g and r modes. We find that these effects should be detectable for equatorial fields thanks to modern space photometry using observations from Kepler, TESS CVZ, and PLATO.},
  keywords = {Astrophysics - High Energy Astrophysical Phenomena,Astrophysics - Solar and Stellar Astrophysics,magnetohydrodynamics (MHD),methods: analytical,Physics - Atmospheric and Oceanic Physics,Physics - Fluid Dynamics,stars: magnetic field,stars: oscillations,stars: rotation,waves},
  annotation = {ADS Bibcode: 2022A\&A...661A.133D},
  file = {/Users/lbugnet/Zotero/storage/AYBI4WK8/Dhouib et al. - 2022 - Detecting deep axisymmetric toroidal magnetic fiel.pdf}
}

@article{Diaz-Merced2011,
  title = {Sonification of Astronomical Data},
  author = {{Diaz-Merced}, Wanda L. and Candey, Robert M. and Brickhouse, Nancy and Schneps, Matthew and Mannone, John C. and Brewster, Stephen and Kolenberg, Katrien},
  year = {2011},
  journal = {Proceedings of the International Astronomical Union},
  volume = {7},
  number = {S285},
  pages = {133--136},
  issn = {17439213},
  doi = {10.1017/S1743921312000440},
  abstract = {This document presents Java-based software called xSonify that uses a sonification technique (the adaptation of sound to convey information) to promote discovery in astronomical data. The prototype is designed to analyze two-dimensional data, such as time-series data. We demonstrate the utility of the sonification technique with examples applied to X-ray astronomy and solar data. We have identified frequencies in the Chandra X-Ray observations of EX Hya, a cataclysmic variable of the intermediate polar type. In another example we study the impact of a major solar flare, with its associated coronal mass ejection (CME), on the solar wind plasma (in particular the solar wind between the Sun and the Earth), and the Earth's magnetosphere. \textcopyright{} 2012 International Astronomical Union.},
  isbn = {9781107019850},
  keywords = {notion,notion-database,Solar Wind,Sonification,Variable Stars,xSonify},
  file = {/Users/lbugnet/Zotero/storage/5YGJ7XAB/Diaz-Merced et al. - 2011.pdf}
}

@article{Dikpati1999,
  title = {Joint {{Instability}} of {{Latitudinal Differential Rotation}} and {{Concentrated Toroidal Fields}} below the {{Solar Convection Zone}}},
  author = {Dikpati, Mausumi and Gilman, Peter A.},
  year = {1999},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {512},
  number = {1},
  pages = {417--441},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/306748},
  urldate = {2020-05-14},
  abstract = {Motivated by observations of sunspot and active-region latitudes that suggest that the subsurface toroidal field in the Sun occurs in narrow latitude belts, we analyze the joint instability of solar latitudinal differential rotation and the concentrated toroidal field below the base of the convection zone, extending the work of Gilman \& Fox (hereafter GF). We represent the profile of the toroidal field by Gaussian functions whose width is a variable parameter and solve the two-dimensional perturbation equations of GF by relaxation methods. We reproduce the results of GF for broad profiles, and we find instability for a wide range of amplitudes of differential rotation and toroidal fields (103-106 G fields at the base of the solar convection zone), as well as a wide range of toroidal-field bandwidths. We show that the combination of concentrated toroidal fields and solar-type latitudinal differential rotation is again unstable, not only to longitudinal wavenumber m=1 as in GF, but also to m{$>$}1 for sufficiently narrow toroidal-field profiles. For a fixed peak field strength, the growth rate first increases as the toroidal-field band is narrowed, reaching a peak for bandwidths between 10\textdegree{} and 20\textdegree{} in latitude, depending on the peak field strength, and then decreases to a cut-off in the instability for toroidal field bands of 3\textdegree -4\textdegree. Irrespective of bandwidth, the differential rotation is the primary energy source for the instability for weak fields, and the toroidal field is the primary source for strong fields. The weaker (stronger) the peak toroidal field is, the narrower (broader) is the bandwidth for which the toroidal field becomes the primary energy source. The Reynolds, Maxwell, and mixed stresses required to extract energy from the differential rotation and toroidal field are most active in the neighborhood of the singular or turning points of the perturbation equations. This first study focuses on toroidal fields that peak near 45\textdegree{} latitude, as in GF; later papers will place the toroidal-field peak at a wide variety of latitudes, as we might expect to occur at different phases of a sunspot cycle.},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/K8IDPEU5/full-text.pdf}
}

@article{Dikpati1999a,
  title = {A {{Babcock}}-{{Leighton Flux Transport Dynamo}} with {{Solar}}-like {{Differential Rotation}}},
  author = {Dikpati, Mausumi and Charbonneau, Paul},
  year = {1999},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {518},
  number = {1},
  pages = {508--520},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/307269},
  urldate = {2020-05-14},
  abstract = {We investigate the properties of a kinematic flux transport solar dynamo model. The model is characterized by a solar-like internal differential rotation profile, a single-cell meridional flow in the convective envelope that is directed poleward at the surface, and a magnetic diffusivity that is constant within the envelope but decreases sharply at the core-envelope interface. As in earlier flux transport models of the Babcock-Leighton type, we assume that the poloidal field is regenerated as a consequence of the emergence at the surface, and subsequent decay, of bipolar active regions exhibiting a systematic tilt with respect to the east-west direction. Inspired by recent simulations of the rise of toroidal magnetic flux ropes across the solar convective envelope, we model this poloidal field regeneration mechanism as a nonlocal source term formulated in such a way as to account for some of the properties of rising flux ropes revealed by the simulations. For a broad range of parameter values the model leads to solar cycle-like oscillatory solutions. Because of the solar-like internal differential rotation profile used in the model, solutions tend to be characterized by time-latitude (butterfly) diagrams that exhibit both poleward- and equatorward-propagating branches. We demonstrate that the latitudinal shear in the envelope, often omitted in other flux transport models previously published in the literature, actually has a dominant effect on the global morphology and period of the solutions, while the radial shear near the core-envelope interface leads to further intensification of the toroidal field. On the basis of an extensive parameter space study, we establish a scaling law between the time period of the cycle and the primary parameters of the model, namely the meridional flow speed, source coefficient, and turbulent diffusion coefficient. In the parameter regime expected to characterize the Sun, we show that the time period of the cycle is most significantly influenced by the circulation flow speed and, unlike for conventional mean field alphaOmega dynamos, is little affected by the magnitude of the source coefficient. Finally, we present one specific solution that exhibits features that compare advantageously with the observed properties of the solar cycle.},
  keywords = {Diffusion,DIFFUSION,notion,notion-database,Sun: Interior,SUN: INTERIOR,Sun: Magnetic Fields,SUN: MAGNETIC FIELDS,Sun: Rotation,SUN: ROTATION},
  file = {/Users/lbugnet/Zotero/storage/H9AUTHIW/full-text.pdf}
}

@article{Dikpati2001,
  title = {Flux-{{Transport Dynamos}} with {$\alpha$}-{{Effect}} from {{Global Instability}} of {{Tachocline Differential Rotation}}: {{A Solution}} for {{Magnetic Parity Selection}} in the {{Sun}}},
  author = {Dikpati, Mausumi and Gilman, Peter A.},
  year = {2001},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {559},
  number = {1},
  pages = {428--442},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/322410},
  urldate = {2020-05-14},
  abstract = {We propose an {$\alpha\Omega$} flux-transport dynamo for the Sun that is driven by a tachocline {$\alpha$}-effect. This {$\alpha$}-effect comes from the global hydrodynamic instability of latitudinal differential rotation in the tachocline, as calculated using a shallow-water model. Growing, unstable shallow-water modes propagating longitudinally in the tachocline create vortices that correlate with radial motion in the layer to produce a longitude-averaged net kinetic helicity and, hence, an {$\alpha$}-effect. We show that such a dynamo is equally successful as a Babcock-Leighton-type flux-transport dynamo in reproducing many large-scale solar cycle features. The success of both dynamo types depends on the inclusion of meridional circulation of a sign and magnitude similar to that seen on the Sun. Both {$\alpha$}-effects (the Babcock-Leighton-type and tachocline {$\alpha$}-effect) are likely to exist in the Sun, but it is hard to estimate their relative magnitudes. By extending the simulation to a full spherical shell, we show that the flux-transport dynamo driven by the tachocline {$\alpha$}-effect selects a toroidal field that is antisymmetric about the equator, while the Babcock-Leighton flux-transport dynamo selects a symmetric toroidal field. Since our present Sun selects antisymmetric fields, we argue that the tachocline {$\alpha$}-effect must be more important than the Babcock-Leighton {$\alpha$}-effect.},
  keywords = {Magnetohydrodynamics: MHD,notion,notion-database,Sun: Magnetic Fields},
  file = {/Users/lbugnet/Zotero/storage/HB6YXWY3/full-text.pdf}
}

@article{Dikpati2005,
  title = {Solar Magnetic Fields and the Dynamo Theory},
  author = {Dikpati, M.},
  year = {2005},
  journal = {Advances in Space Research},
  volume = {35},
  number = {3},
  pages = {322--328},
  issn = {02731177},
  doi = {10.1016/j.asr.2005.04.061},
  abstract = {Unlike Earth's dipolar magnetic fields, solar magnetic fields consist of wide ranges of length-scales and strengths, and interestingly, they evolve in a cyclic fashion with a 22-year periodicity. A magnetohydrodynamic dynamo operating in the Sun is most likely responsible for producing the solar magnetic activity cycle. While the first solar dynamo models were built half a century ago, recent views differ significantly from those models. According to widely accepted present concepts, the large-scale solar dynamo is of flux-transport type, which involves three basic processes: (i) generation of toroidal fields by shearing the pre-existing poloidal fields by differential rotation (the {$\Omega$}-effect); (ii) re-generation of poloidal fields by lifting and twisting the toroidal fluxtubes (the {$\alpha$}-effect); (iii) flux transport by meridional circulation. This class of dynamos has been successful in explaining many large-scale solar cycle features, including a particularly difficult one - the correct phase relationship between the equatorward-migrating sunspot belt and the poleward drifting large-scale, diffuse fields. The dynamo cycle period in such models is primarily governed by the meridional flow speed near the bottom of the convection zone. After briefly reviewing the historical background, we will present the successes of flux-transport dynamos, including their predictive capability. For example, we will demonstrate how the meridional circulation plays a key role in governing the Sun's memory about its own magnetic field, and how a flux-transport dynamo-based predictive tool can explain the cause of the very slow polar reversal in the so-called "peculiar" cycle 23 compared to those in cycles 20, 21 and 22. We will close by presenting explanations for certain long-term variability using these models, such as, what may have maintained the observed cyclic variation in slow solar wind flow during Maunder minima, in the presence of near zero solar activity. \textcopyright{} 2005 COSPAR. Published by Elsevier Ltd. All rights reserved.},
  keywords = {Activity cycle,Cycle prediction,Dynamo theory,notion,notion-database,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/UMPJ47EE/Dikpati - 2005.pdf}
}

@article{Dikpati2005a,
  title = {Constraints on the {{Applicability}} of an {{Interface Dynamo}} to the {{Sun}}},
  author = {Dikpati, Mausumi and Gilman, Peter A. and MacGregor, Keith B.},
  year = {2005},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {631},
  number = {1},
  pages = {647--652},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/432436},
  urldate = {2020-05-14},
  keywords = {notion,notion-database,Sun: Activity,Sun: Interior,Sun: Magnetic Fields},
  file = {/Users/lbugnet/Zotero/storage/8KBHPD9Q/full-text.pdf}
}

@article{Dikpati2006,
  title = {Penetration of {{Dynamo}}-generated {{Magnetic Fields}} into the {{Sun}}'s {{Radiative Interior}}},
  author = {Dikpati, Mausumi and Gilman, Peter A. and MacGregor, Keith B.},
  year = {2006},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {638},
  number = {1},
  pages = {564--575},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/498682},
  urldate = {2020-05-14},
  abstract = {Any large-scale magnetic fields present in solar/stellar radiative interiors have so far been thought to be primordial or residuals from extinct dynamos. We show that a regular cyclic dynamo can also be the origin of strong magnetic fields in the solar radiative tachocline and interior below. By exploiting a kinematic, mean-field flux-transport dynamo, we show that for a wide range of core-diffusivity values, from 109 cm2 s-1 down to a molecular diffusivity of 103 cm2 s-1, oscillatory dynamo fields penetrate below the tachocline. Amplitudes of these fields are in the range of \textasciitilde 1 kG to 3\texttimes 103 kG, depending on core diffusivity value, when the dynamo produces \textasciitilde 100 kG peak toroidal fields in the overshoot tachocline. For a low enough core diffusivity ({$<\sptilde$}107 cm2 s-1), there is also a steady (nonreversing) dynamo in the radiative tachocline and below, which generates strong toroidal field of amplitude \textasciitilde 1 kG to 3\texttimes 103 kG or more there. The key elements in this dynamo are the low diffusivity, the differential rotation near the bottom of the tachocline, and an assumed tachocline {$\alpha$}-effect. The Lorentz force feedback may limit oscillatory dynamo fields to \textasciitilde 30 kG, for which the mean nonreversing toroidal fields is still \textasciitilde 300 kG, for the lowest core diffusivity value. The presence of strong oscillatory and steady toroidal fields in the radiative tachocline implies that there cannot be a slow tachocline; the dynamics should always be fast there, dominated by MHD. These results are obtained using solar parameters, but they should also apply generally to stars with convecting shells and perhaps also with convective cores.},
  keywords = {notion,notion-database,Sun: Interior,Sun: Magnetic Fields},
  file = {/Users/lbugnet/Zotero/storage/TPWJQM4I/full-text.pdf}
}

@article{DiMauro2011,
  title = {Solar-like Oscillations from the Depths of the Red-Giant Star {{KIC4351319}} Observed with {{Kepler}}},
  author = {{di Mauro}, M. P. and Cardini, D. and Catanzaro, G. and Ventura, R. and Barban, C. and Bedding, T. R. and {Christensen-Dalsgaard}, J. and {de Ridder}, J. and Hekker, S. and Huber, D. and Kallinger, T. and Miglio, A. and Montalban, J. and Mosser, B. and Stello, D. and Uytterhoeven, K. and Kinemuchi, K. and Kjeldsen, H. and Mullally, F. and Still, M.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {415},
  number = {4},
  eprint = {1105.1076},
  pages = {3783--3797},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.18996.x},
  abstract = {We present the results of the asteroseismic analysis of the red-giant star KIC 4351319 (TYC 3124-914-1), observed for 30d in short-cadence mode with theKeplersatellite. The analysis has allowed us to determine the large and small frequency separations, Hz and Hz, respectively, and the frequency of maximum oscillation power, Hz. The high signal-to-noise ratio of the observations allowed us to identify 25 independent pulsation modes whose frequencies range approximately from 300 to Hz. The observed oscillation frequencies together with the accurate determination of the atmospheric parameters (effective temperature, gravity and metallicity), provided by additional ground-based spectroscopic observations, enabled us to theoretically interpret the observed oscillation spectrum. KIC 4351319 appears to oscillate with a well-defined solar-type p-mode pattern due to radial acoustic modes and non-radial nearly pure p modes. In addition, several non-radial mixed modes have been identified. Theoretical models well reproduce the observed oscillation frequencies and indicate that this star, located at the base of the ascending red-giant branch, is in the hydrogen-shell-burning phase, with a mass of \textasciitilde 1.3M{$\odot$}, a radius of and an age of \textasciitilde 5.6 Gyr. The main parameters of this star have been determined with an unprecedented level of precision for a red-giant star, with uncertainties of 2 per cent for mass, 7 per cent for age, 1 per cent for radius and 4 per cent for luminosity. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: AGB and post-AGB,Stars: evolution,Stars: fundamental parameters,Stars: individual: KIC 4351319,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/WV7SUIYQ/di Mauro et al. - 2011.pdf}
}

@article{DiMauro2013,
  title = {Internal Rotation of Red Giants by Asteroseismology},
  author = {Di Mauro, M. P. and Cardini, D. and Ventura, R. and Stello, D. and Beck, P. G. and Davies, G. and Elsworth, Y. and Garc{\'i}a, R. A. and Hekker, S. and Mosser, B. and {Christensen-Dalsgaard}, J. and Bloemen, S. and Catanzaro, G. and De Smedt, K. and Tkachenko, A.},
  year = {2013},
  journal = {EPJ Web of Conferences},
  volume = {43},
  eprint = {1212.4758},
  pages = {0--3},
  issn = {21016275},
  doi = {10.1051/epjconf/20134303012},
  abstract = {We present an asteroseismic approach to study the dynamics of the stellar interior in red giant stars by asteroseismic inversion of the splittings induced by the stellar rotation on the oscillation frequencies. We show preliminary results obtained for the red giant KIC4448777 observed by the space mission Kepler. \textcopyright{} 2013 Owned by the authors, published by EDP Sciences.},
  archiveprefix = {arxiv},
  isbn = {9782759809691},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SXHKAMRI/Di Mauro et al. - 2013.pdf}
}

@inproceedings{DiMauro2016a,
  title = {A Review on {{Asteroseismology}}},
  booktitle = {Proceedings of {{Science}}},
  author = {Di Mauro, M. P.},
  year = {2016},
  volume = {2016-May},
  eprint = {1703.07604},
  issn = {18248039},
  doi = {10.22323/1.269.0029},
  abstract = {Over the last decade, thanks to the successful space missions launched to detect stellar pulsations, Asteroseismology has produced an extraordinary revolution in astrophysics, unveiling a wealth of results on structural properties of stars over a large part of the H-R diagram. Particularly impressive has been the development of Asteroseismology for stars showing solar-like oscillations, which are excited and intrinsically damped in stars with convective envelopes. Here I will review on the modern era of Asteroseismology with emphasis on results obtained for solar-likefile:///Users/lbugnet/Downloads/1703.07604.pdf stars and discuss its potential for the advancement of stellar physics.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/X6J57MW2/Di Mauro - 2016.pdf}
}

@article{DiMauro2016b,
  title = {Internal {{Rotation}} of the {{Red-Giant Star Kic}} 4448777 {{By Means}} of {{Asteroseismic Inversion}}},
  author = {Di Mauro, M. P. and Ventura, R. and Cardini, D. and Stello, D. and {Christensen-Dalsgaard}, J. and Dziembowski, W. A. and Patern{\`o}, L. and Beck, P. G. and Bloemen, S. and Davies, G. R. and De Smedt, K. and Elsworth, Y. and Garc{\'i}a, R. A. and Hekker, S. and Mosser, B. and Tkachenko, A.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {817},
  number = {1},
  pages = {65},
  doi = {10.3847/0004-637x/817/1/65},
  abstract = {In this paper we study the dynamics of the stellar interior of the early red-giant star KIC 4448777 by asteroseismic inversion of 14 splittings of the dipole mixed modes obtained from \{\textbackslash it Kepler\} observations. In order to overcome the complexity of the oscillation pattern typical of red-giant stars, we present a procedure which involves a combination of different methods to extract the rotational splittings from the power spectrum. We find not only that the core rotates faster than the surface, confirming previous inversion results generated for other red giants (Deheuvels et al. 2012,2014), but we also estimate the variation of the angular velocity within the helium core with a spatial resolution of \$\textbackslash Delta r=0.001R\$ and verify the hypothesis of a sharp discontinuity in the inner stellar rotation (Deheuvels et al. 2014). The results show that the entire core rotates rigidly with an angular velocity of about \$\textbackslash langle\textbackslash Omega\_c/2\textbackslash pi\textbackslash rangle=748\textbackslash pm18\$\textasciitilde nHz and provide evidence for an angular velocity decrease through a region between the helium core and part of the hydrogen burning shell; however we do not succeed to characterize the rotational slope, due to the intrinsic limits of the applied techniques. The angular velocity, from the edge of the core and through the hydrogen burning shell, appears to decrease with increasing distance from the center, reaching an average value in the convective envelope of \$\textbackslash langle\textbackslash Omega\_s/2\textbackslash pi\textbackslash rangle=68\textbackslash pm22\$\textasciitilde nHz. Hence, the core in KIC\textasciitilde 4448777 is rotating from a minimum of 8 to a maximum of 17 times faster than the envelope. We conclude that a set of data which includes only dipolar modes is sufficient to infer quite accurately the rotation of a red giant not only in the dense core but also, with a lower level of confidence, in part of the radiative region and in the convective envelope.},
  keywords = {agb and post-agb,individual,interiors,kic 4448777,notion,notion-database,oscillations,rotation,solar-type,stars},
  file = {/Users/lbugnet/Zotero/storage/2A4E6KNL/Di Mauro et al. - 2016.pdf}
}

@article{Dintrans2005a,
  title = {Spectrum and Amplitudes of Internal Gravity Waves Excited by Penetrative Convection in Solar-Type Stars},
  author = {Dintrans, B. and Brandenburg, A. and Nordlund, {\AA} and Stein, R. F.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {438},
  number = {1},
  pages = {365--376},
  issn = {00046361},
  doi = {10.1051/0004-6361:20052831},
  abstract = {The excitation of internal gravity waves by penetrative convective plumes is investigated using 2-D direct simulations of compressible convection. The wave generation is quantitatively studied from the linear response of the radiative zone to the plumes penetration, using projections onto the g-modes solutions of the associated linear eigenvalue problem for the perturbations. This allows an accurate determination of both the spectrum and amplitudes of the stochastically excited modes. Using time-frequency diagrams of the mode amplitudes, we then show that the lifetime of a mode is around twice its period and that during times of significant excitation up to 40\% of the total kinetic energy may be contained into g-modes. \textcopyright{} ESO 2005.},
  keywords = {Convection,Hydrodynamics,Methods: numerical,notion,notion-database,Stars: oscillations,Waves},
  file = {/Users/lbugnet/Zotero/storage/NIFKKIKI/Dintrans et al. - 2005.pdf}
}

@techreport{Djorgovski2013,
  title = {Sky {{Surveys}}},
  author = {Djorgovski, S G and Mahabal, Aa and Drake, Aj and Graham, {\relax MJ} and Donalek, C},
  year = {2013},
  pages = {1898--1974},
  urldate = {2020-04-11},
  abstract = {Sky surveys represent a fundamental data basis for astronomy. We use them to map in a systematic way the universe and its constituents, and to discover new types of objects or phenomena. We review the subject, with an emphasis on the wide-field, imaging surveys, placing them in a broader scientific and historical context. Surveys are now the largest data generators in astronomy, propelled by the advances in information and computation technology, and have transformed the ways in which astronomy is done. This trend is bound to continue, especially with the new generation of synoptic sky surveys that cover wide areas of the sky repeatedly, and open a new time domain of discovery. We describe the variety and the general properties of surveys, illustrated by a number of examples, the ways in which they may be quantified and compared, and offer some figures of merit that can be used to compare their scientific discovery potential. Surveys enable a very wide range of science, and that is perhaps their key unifying characteristic. As new domains of the observable parameter space open up thanks to the advances in technology, surveys are often the initial step in their exploration. Some science can be done with the survey data alone (or a combination of data from different surveys), and some requires a targeted follow-up of potentially interesting sources selected from surveys. Surveys can be used to generate large, statistical samples of objects that can be studied as populations, or as tracers of larger structures to which they belong. They can be also used to discover or generate samples of rare or unusual objects, and may lead to discoveries of some previously unknown types. We discuss a general framework of parameter spaces that can be used for an assessment and comparison of different surveys, and the strategies for their scientific exploration. As we are moving into the Petascale regime and beyond, an effective processing and scientific exploitation of such large data sets and data streams poses many challenges, some of which are specific to any given survey, and some of which may be addressed in the framework of Virtual Observatory and Astroinformatics. The exponential growth of data volumes and complexity makes a broader application of data mining and knowledge discovery technologies critical in order to take a full advantage of this wealth of information. Finally, we discuss some outstanding challenges and prospects for the future. * We dedicate this chapter to the memory of three pioneers of sky surveys},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RK844MUS/full-text.pdf}
}

@article{DoCao2011,
  title = {Effects of Turbulent Pumping on Stellar Activity Cycles},
  author = {Do Cao, Olivier and Brun, Allan Sacha},
  year = {2011},
  month = dec,
  journal = {Astronomische Nachrichten},
  volume = {332},
  number = {9-10},
  eprint = {1112.1321},
  pages = {907--917},
  doi = {10.1002/asna.201111623},
  urldate = {2020-07-13},
  abstract = {Stellar magnetic activity of solar like stars is thought to be due to an internal dynamo. While the Sun has been the subject of intense research for refining dynamo models, observations of magnetic cyclic activity in solar type stars have become more and more available, opening a new path to understand the underlying physics behind stellar cycles. For instance, it is key to understand how stellar rotation rate influences magnetic cycle period \$\textbackslash Pcyc\$. Recent numerical simulations of advection-dominated Babcock Leighton models have demonstrated that it is difficult to explain this observed trend given a) the strong influence of the cycle period to the meridional circulation amplitude and b) the fact that 3D models indicate that meridional flows become weaker as the rotation rate increases. In this paper, we introduce the turbulent pumping mechanism as another advective process capable also of transporting the magnetic fields. We found that this model is now able to reproduce the observations under the assumption that this effect increases as \$\textbackslash Omega\^2\$. The turbulent pumping becomes indeed another major player able to circumvent the meridional circulation. However, for high rotation rates (\$\textbackslash Omega \textbackslash simeq 5 \textbackslash Omega\_\textbackslash odot\$), its effects dominate those of the meridional circulation, entering a new class of regime dominated by the advection of turbulent pumping and thus leading to a cyclic activity qualitatively different from that of the sun.},
  archiveprefix = {arxiv},
  keywords = {Methods: numerical,notion,notion-database,Stars: activity,Stars: interiors,Stars: magnetic fields,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/ELPPP9EY/full-text.pdf}
}

@article{Dogan2013,
  title = {Characterizing {{Two Solar-Type Kepler Subgiants}} with {{Asteroseismology}}: {{KIC}} 10920273 and {{KIC}} 11395018},
  author = {Do{\v g}an, G. and Metcalfe, T. S. and Deheuvels, S. and Di Mauro, M. P. and Eggenberger, P. and Creevey, O. L. and Monteiro, M. J.P.F.G. and Pinsonneault, M. and Frasca, A. and Karoff, C. and Mathur, S. and Sousa, S. G. and Brand{\~a}o, I. M. and Campante, T. L. and Handberg, R. and Thygesen, A. O. and Biazzo, K. and Bruntt, H. and Niemczura, E. and Bedding, T. R. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Garc{\'i}a, R. A. and {Molenda-Zakowicz}, J. and Stello, D. and Van Saders, J. L. and Kjeldsen, H. and Still, M. and Thompson, S. E. and Van Cleve, J.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {763},
  number = {1},
  eprint = {1211.6650},
  issn = {15384357},
  doi = {10.1088/0004-637X/763/1/49},
  abstract = {Determining fundamental properties of stars through stellar modeling has improved substantially due to recent advances in asteroseismology. Thanks to the unprecedented data quality obtained by space missions, particularly CoRoT and Kepler, invaluable information is extracted from the high-precision stellar oscillation frequencies, which provide very strong constraints on possible stellar models for a given set of classical observations. In this work, we have characterized two relatively faint stars, KIC 10920273 and KIC 11395018, using oscillation data from Kepler photometry and atmospheric constraints from ground-based spectroscopy. Both stars have very similar atmospheric properties; however, using the individual frequencies extracted from the Kepler data, we have determined quite distinct global properties, with increased precision compared to that of earlier results. We found that both stars have left the main sequence and characterized them as follows: KIC 10920273 is a one-solar-mass star (M = 1.00 {$\pm$} 0.04 M{$\odot$}), but much older than our Sun (t = 7.12 {$\pm$} 0.47 Gyr), while KIC 11395018 is significantly more massive than the Sun (M = 1.27 {$\pm$} 0.04 M{$\odot$}) with an age close to that of the Sun (t = 4.57 {$\pm$} 0.23 Gyr). We confirm that the high lithium abundance reported for these stars should not be considered to represent young ages, as we precisely determined them to be evolved subgiants. We discuss the use of surface lithium abundance, rotation, and activity relations as potential age diagnostics. \textcopyright{} 2013 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,stars: evolution,stars: fundamental parameters,{stars: individual (KIC 10920273, KIC 11395018)},stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/GDLVN68C/Doǧan et al. - 2013.pdf}
}

@article{Dogel1990,
  title = {Differential Rotation and Stellar Convection},
  author = {Dogel', V. A.},
  year = {1990},
  month = may,
  journal = {Soviet Physics - Uspekhi},
  volume = {33},
  number = {5},
  pages = {392},
  publisher = {{IOP Publishing}},
  issn = {21695296},
  doi = {10.1070/PU1990v033n05ABEH002591},
  urldate = {2020-03-15},
  keywords = {notion,notion-database}
}

@article{Domingo1995,
  title = {The {{SOHO}} Mission: {{An}} Overview},
  author = {Domingo, V. and Fleck, B. and Poland, A. I.},
  year = {1995},
  month = dec,
  journal = {Solar Physics},
  volume = {162},
  number = {1-2},
  pages = {1--37},
  publisher = {{Kluwer Academic Publishers}},
  issn = {00380938},
  doi = {10.1007/BF00733425},
  urldate = {2020-07-04},
  abstract = {The Solar and Heliospheric Observatory (SOHO) is a space mission that forms part of the Solar-Terrestrial Science Program (STSP), developed in a collaborative effort by the European Space Agency (ESA) and the National Aeronautics and Space Administration (NASA). The STSP constitutes the first "cornerstone" of ESA's long-term programme known as "Space Science - Horizon 2000". The principal scientific objectives of the SOHO mission are a) to reach a better understanding of the structure and dynamics of the solar interior using techniques of helioseismology, and b) to gain better insight into the physical processes that form and heat the Sun's corona, maintain it and give rise to its acceleration into the solar wind. To achieve these goals, SOHO carries a payload consisting of 12 sets of complementary instruments. SOHO is a three-axis stabilized spacecraft with a total mass of 1850 kg; 1150 W of power will be provided by the solar panels. The payload weighs about 640 kg and will consume 450 W in orbit. SOHO will be launched by an ATLAS II-AS and will be placed in a halo orbit around the Sun-Earth L1 Lagrangian point where it will be continuously pointing to Sun centre with an accuracy of 10 arcsec. Pointing stability will be better than 1 arcsec over 15 min intervals. The SOHO payload produces a continuous science data stream of 40 kbits/s which will be increased by 160 kbits/s whenever the solar oscillations imaging instrument is operated in its highrate mode. Telemetry will be received by NASA's Deep Space Network (DSN). Planning, coordination and operation of the spacecraft and the scientific payload will be conducted from the Experiment Operations Facility (EOF) at NASA's Goddard Space Flight Center (GSFC). \textcopyright{} 1995 Kluwer Academic Publishers.},
  keywords = {notion,notion-database,SOHO,solar corona,solar interior,solar wind}
}

@article{Donahue1996,
  title = {A Relationship between Mean Rotation Period in Lower Main-Sequence Stars and Its Observed Range},
  author = {Donahue, R. A. and Saar, Steven H. and Baliunas, Sallie L.},
  year = {1996},
  journal = {The Astrophysical Journal},
  pages = {384--391},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HV8I32DE/Donahue, Saar, Baliunas - 1996.pdf}
}

@article{DoNascimento2012a,
  title = {Rotational Periods and Evolutionary Models for Subgiant Stars Observed by {{CoRoT}}},
  author = {Do Nascimento, J. D. and Da Costa, J. S. and Castro, M.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {548},
  pages = {1--8},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219791},
  abstract = {Context. We present rotation period measurements for subgiants observed by CoRoT. Interpreting the modulation of stellar light that is caused by star-spots on the time scale of the rotational period depends on knowing the fundamental stellar parameters. Aims. Constraints on the angular momentum distribution can be extracted from the true stellar rotational period. By using models with an internal angular momentum distribution and comparing these with measurements of rotation periods of subgiant stars we investigate the agreement between theoretical predictions and observational results. With this comparison we can also reduce the global stellar parameter space compatible with the rotational period measurements from subgiant light curves. We can prove that an evolution assuming solid body rotation is incompatible with the direct measurement of the rotational periods of subgiant stars. Methods. Measuring the rotation periods relies on two different periodogram procedures, the Lomb-Scargle algorithm and the Plavchan periodogram. Angular momentum evolution models were computed to give us the expected rotation periods for subgiants, which we compared with measured rotational periods. Results. We find evidence of a sinusoidal signal that is compatible in terms of both phase and amplitude with rotational modulation. Rotation periods were directly measured from light curves for 30 subgiant stars and indicate a range of 30 to 100 d for their rotational periods. Conclusions. Our models reproduce the rotational periods obtained from CoRoT light curves. These new measurements of rotation periods and stellar models probe the non-rigid rotation of subgiant stars. \textcopyright{} ESO, 2012.},
  keywords = {notion,notion-database,Stars: interiors,Stars: late-type,Stars: rotation,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/IB2MUXNC/Do Nascimento, Da Costa, Castro - 2012.pdf}
}

@article{DoNascimento2014,
  title = {Rotation Periods and Ages of Solar Analogs and Solar Twins Revealed by the Kepler Mission},
  author = {Do Nascimento, J. D. and Garc{\'i}a, R. A. and Mathur, S. and Anthony, F. and Barnes, S. A. and Meibom, S. and Da Costa, J. S. and Castro, M. and Salabert, D. and Ceillier, T.},
  year = {2014},
  journal = {Astrophysical Journal Letters},
  volume = {790},
  number = {2},
  issn = {20418213},
  doi = {10.1088/2041-8205/790/2/L23},
  abstract = {A new sample of solar analogs and twin candidates has been constructed and studied, paying particular attention to their light curves from NASA's Kepler mission. This Letter aims to assess their evolutionary status, derive their rotation and ages, and identify those which are solar analogs or solar twin candidates. We separate out the subgiants that compose a large fraction of the asteroseismic sample, and which show an increase in the average rotation period as the stars ascend the subgiant branch. The rotation periods of the dwarfs, ranging from 6 to 30 days and averaging 19 days, allow us to assess their individual evolutionary states on the main sequence and to derive their ages using gyrochronology. These ages are found to be in agreement with a correlation coefficient of r = 0.79 with independent asteroseismic ages, where available. As a result of this investigation, we are able to identify 34 stars as solar analogs and 22 of them as solar twin candidates. \textcopyright{} 2014. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,stars: evolution,stars: fundamental parameters,stars: rotation,stars: solar-type,Sun: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/LX9ETAQI/Do Nascimento et al. - 2014.pdf}
}

@article{Donati1997,
  title = {Spectropolarimetric Observations of Active Stars},
  author = {Donati, J.-F and Semel, M and Carter, B D and Rees, D E and Cameron, A C},
  year = {1997},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {291},
  pages = {658--682},
  urldate = {2020-06-07},
  abstract = {This paper reports the results of five years (five runs, 23 nights) of spectropolarimetric observations of active stars with the VCL Echelle Spectrograph of the Anglo-Australian Telescope. 225 circularly (and four linearly) polarized spectra were recorded on 28 objects (21 active stars and seven calibration standards) using the new technique of Zeeman-Doppler imaging. To extract polarization echelle spectra from raw frames, we developed a new dedicated automatic software package (called ESpRIT, which utilizes optimal extraction techniques) whose detailed description is given in the paper. For each recorded spectrum, we extract 'mean' polarized and unpolarized profiles using 'least-squares deconvolution', a technique similar to cross-correlation, which can enhance enormously the sensitivity of Zeeman-Doppler imaging, by up to 7.5 mag in flux with respect to a single average line analysis or by 4.5 mag compared with the older technique of Donati et al. in the particular case of a K1 star. Magnetic field is detected unambiguously on 14 objects, namely the weak-line T Tauri star V410 Tau, the pre-main-sequence binary HD 155555, the ZAMS stars AB Dor and LQ Hya, the dwarf flare star CC Eri, the RS CVn systems HR 1099, EI Eri, TY Pyx, CF Thc, SZ Psc, II Peg, 1M Peg and IL Hya, and the FK Com star YY Men. Marginal field detections are also obtained for the weak-line T Tauri star HD 283572 and the Herbig Ae star HD 104237. Except on HR 1099 and II Peg, our results represent the first direct field detections ever reported on these objects, and in particular the first direct field detection on as young a star as V410 Tau. Most of the magnetic signatures we detect on cool stars show several sign reversals throughout. the line profile, indicating that the parent field structure is rather complex and must feature (as expected) many small-scale magnetic regions of different polarities. For all stars on which Zeeman detections are recorded with sufficient accuracy (namely LQ Hya, CC Eri, HR 1099, EI Eri, II Peg, IL Hya and YY Men), differential least-squares deconvolution from both the blue and the red parts of the spectral domain indicates that the magnetic regions we detect are mostly 500 to 1000 K cooler than, and sometimes at the same temperature as, but never warmer than the surrounding photosphere. Serendipitous results include the first detection (i) of small-amplitude radial velocity variations (1.3 kIn S-1 peak to peak) of the Herbig Ae star HD 104237 with small enough a period (37.5 {$\pm$} 1 min) that they must be due to stellar pulsations and (ii) of the solar-like secondary component of the RS CVn system IL Hya.},
  keywords = {activity-stars,atmospheres-stars,late-type-stars,line,magnetic fields *,notion,notion-database,profiles-polarization-stars}
}

@article{Donati2006,
  title = {The Surprising Magnetic Topology of {$\tau$} {{Sco}}: {{Fossil}} Remnant or Dynamo Output?},
  author = {Donati, J. F. and Howarth, I. D. and Jardine, M. M. and Petit, P. and Catala, C. and Landstreet, J. D. and Bouret, J. C. and Alecian, E. and Barnes, J. R. and Forveille, T. and Paletou, F. and Manset, N.},
  year = {2006},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {370},
  number = {2},
  pages = {629--644},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2006.10558.x},
  urldate = {2020-07-02},
  abstract = {We report the discovery of a medium-strength ({$\sim$}0.5 kG) magnetic field on the young, massive star {$\tau$} Sco (B0.2 V), which becomes the third-hottest magnetic star known. Circularly polarized Zeeman signatures are clearly detected in observations collected mostly with the ESPaDOnS spectropolarimeter, recently installed on the 3.6-m Canada-France-Hawaii Telescope; temporal variability is also clearly established in the polarimetry, and can be unambiguously attributed to rotational modulation with a period close to 41 d. Archival ultraviolet (UV) spectra confirm that this modulation repeats over time-scales of decades, and refine the rotation period to 41.033 {$\pm$} 0.002 d. Despite the slow rotation rate of {$\tau$} Sco, we none the less succeed in reconstructing the large-scale structure of its magnetic topology. We find that the magnetic structure is unusually complex for a hot star, with significant power in spherical-harmonic modes of degree up to 5. The surface topology is dominated by a potential field, although a moderate toroidal component is probably present. We fail to detect intrinsic temporal variability of the magnetic structure over the 1.5-yr period of our spectropolarimetric observations (in agreement with the stable temporal variations of the UV spectra), and infer that any differential surface rotation must be very small. The topology of the extended magnetic field that we derive from the photospheric magnetic maps is also more complex than a global dipole, and features in particular a significantly warped torus of closed magnetic loops encircling the star (tilted at about 90\textdegree{} to the rotation axis), with additional, smaller, networks of closed-field lines. This topology appears to be consistent with the exceptional X-ray properties of {$\tau$} Sco and also provides a natural explanation of the variability observed in wind-formed UV lines. Although we cannot completely rule out the possibility that the field is produced through dynamo processes of an exotic kind, we conclude that its magnetic field is most probably a fossil remnant from the star formation stage. \textcopyright{} 2006 RAS.},
  keywords = {notion,notion-database,Stars: early-type,Stars: individual: {$\tau$} Sco,Stars: magnetic fields,Stars: rotation,{Stars: winds, outflows},Techniques: polarimetric},
  file = {/Users/lbugnet/Zotero/storage/SWZCKYKL/full-text.pdf}
}

@article{Donati2009,
  title = {Magnetic {{Fields}} of {{Nondegenerate Stars}}},
  author = {Donati, J.-F. and Landstreet, J.D.},
  year = {2009},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {47},
  number = {1},
  eprint = {0904.1938},
  pages = {333--370},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-082708-101833},
  abstract = {Magnetic fields are present in a wide variety of stars throughout the HR diagram and play a role at basically all evolutionary stages, from very-low-mass dwarfs to very massive stars, and from young star-forming molecular clouds and protostellar accretion discs to evolved giants/supergiants and magnetic white dwarfs/neutron stars. These fields range from a few microG (e.g., in molecular clouds) to TeraG and more (e.g., in magnetic neutron stars); in non-degenerate stars in particular, they feature large-scale topologies varying from simple nearly-axisymmetric dipoles to complex non-axsymmetric structures, and from mainly poloidal to mainly toroidal topology. After recalling the main techniques of detecting and modelling stellar magnetic fields, we review the existing properties of magnetic fields reported in cool, hot and young non-degenerate stars and protostars, and discuss our understanding of the origin of these fields and their impact on the birth and life of stars.},
  archiveprefix = {arxiv},
  keywords = {abundances,activity,early-type,formation,late-type,magnetic fields,mass-loss,notion,notion-database,polarimetry,rotation,rotation; techniques: polarimetry,spectroscopy,stars,stars: activity,techniques},
  file = {/Users/lbugnet/Zotero/storage/CJ3ER3QJ/full-text.pdf;/Users/lbugnet/Zotero/storage/DJ7ILYHY/Donati, Landstreet - 2009.pdf}
}

@article{Donati2009a,
  title = {Magnetic {{Fields}} of {{Nondegenerate Stars}}},
  author = {Donati, J. -F. and Landstreet, J. D.},
  year = {2009},
  month = sep,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {47},
  pages = {333--370},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-082708-101833},
  urldate = {2023-10-05},
  abstract = {Magnetic fields are present in a wide variety of stars throughout the HR diagram and play a role at basically all evolutionary stages, from very-low-mass dwarfs to very massive stars, and from young star-forming molecular clouds and protostellar accretion discs to evolved giants/supergiants and magnetic white dwarfs/neutron stars. These fields range from a few {$\mu$}G (e.g., in molecular clouds) to TG and more (e.g., in magnetic neutron stars); in nondegenerate stars in particular, they feature large-scale topologies varying from simple nearly axisymmetric dipoles to complex nonaxsymmetric structures, and from mainly poloidal to mainly toroidal topologies. After recalling the main techniques of detecting and modeling stellar magnetic fields, we review the existing properties of magnetic fields reported in cool, hot, and young nondegenerate stars and protostars, and discuss our understanding of the origin of these fields and their impact on the birth and life of stars.},
  keywords = {Astrophysics - Instrumentation and Methods for Astrophysics,Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2009ARA\&A..47..333D},
  file = {/Users/lbugnet/Zotero/storage/SJMPAUBP/Donati and Landstreet - 2009 - Magnetic Fields of Nondegenerate Stars.pdf}
}

@article{Dorren1987,
  title = {A New Formulation of the Starspot Model, and the Consequences of Starspot Structure},
  author = {Dorren, J.D.},
  year = {1987},
  journal = {The Astrophysical Journal},
  volume = {320},
  pages = {756--767},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/L7M5FS9E/Dorren - 1987.pdf}
}

@article{Doyle2014,
  title = {Determining Stellar Macroturbulence Using Asteroseismic Rotational Velocities from {{Kepler}}},
  author = {Doyle, Amanda P. and Davies, Guy R. and Smalley, Barry and Chaplin, William J. and Elsworth, Yvonne},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {444},
  number = {4},
  eprint = {1408.3988},
  pages = {3592--3602},
  issn = {13652966},
  doi = {10.1093/mnras/stu1692},
  abstract = {The Rossiter-McLaughlin effect observed for transiting exoplanets often requires prior knowledge of the stellar projected equatorial rotational velocity (v sin i). This is usually provided by measuring the broadening of spectral lines, however this method has uncertainties as lines are also broadened by velocity fields in the stellar photosphere known as macroturbulence (v{$<$}inf{$>$}mac{$<$}/inf{$>$}). We have estimated accurate v sin i values from asteroseismic analyses of main-sequence stars observed by Kepler. The rotational frequency splittings of the detected solar-like oscillations of these stars are determined largely by the near-surface rotation. These estimates have been used to infer the v{$<$}inf{$>$}mac{$<$}/inf{$>$} values for 28 Kepler stars. Out of this sample, 26 stars were used along with the Sun to obtain a new calibration between v{$<$}inf{$>$}mac{$<$}/inf{$>$}, effective temperature and surface gravity. The new calibration is valid for the temperature range 5200 to 6400 K and the gravity range 4.0 to 4.6 dex. A comparison is also provided with previous v{$<$}inf{$>$}mac{$<$}/inf{$>$} calibrations. As a result of this work, v{$<$}inf{$>$}mac{$<$}/inf{$>$}, and thus v sin i, can now be determined with confidence for stars that do not have asteroseismic data available. We present new spectroscopic v sin i values for the WASP planet host stars, using high-resolution HARPS spectra.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Line: profiles,notion,notion-database,Planets and satellites: fundamental parameters,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/3VMP3SY8/Doyle et al. - 2014.pdf}
}

@article{Dressing2013,
  title = {The Occurrence Rate of Small Planets around Small Stars},
  author = {Dressing, Courtney D. and Charbonneau, David},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {767},
  number = {1},
  eprint = {1302.1647},
  issn = {15384357},
  doi = {10.1088/0004-637X/767/1/95},
  abstract = {We use the optical and near-infrared photometry from the Kepler Input Catalog to provide improved estimates of the stellar characteristics of the smallest stars in the Kepler target list. We find 3897 dwarfs with temperatures below 4000 K, including 64 planet candidate host stars orbited by 95 transiting planet candidates. We refit the transit events in the Kepler light curves for these planet candidates and combine the revised planet/star radius ratios with our improved stellar radii to revise the radii of the planet candidates orbiting the cool target stars. We then compare the number of observed planet candidates to the number of stars around which such planets could have been detected in order to estimate the planet occurrence rate around cool stars. We find that the occurrence rate of 0.5-4 R {$\oplus$} planets with orbital periods shorter than 50 days is planets per star. The occurrence rate of Earth-size (0.5-1.4 R {$\oplus$}) planets is constant across the temperature range of our sample at Earth-size planets per star, but the occurrence of 1.4-4 R {$\oplus$} planets decreases significantly at cooler temperatures. Our sample includes two Earth-size planet candidates in the habitable zone, allowing us to estimate that the mean number of Earth-size planets in the habitable zone is planets per cool star. Our 95\% confidence lower limit on the occurrence rate of Earth-size planets in the habitable zones of cool stars is 0.04 planets per star. With 95\% confidence, the nearest transiting Earth-size planet in the habitable zone of a cool star is within 21 pc. Moreover, the nearest non-transiting planet in the habitable zone is within 5 pc with 95\% confidence. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {catalogs,methods: data analysis,notion,notion-database,planetary systems,stars: low-mass,surveys,techniques:photometric},
  file = {/Users/lbugnet/Zotero/storage/AI68KMNH/Dressing, Charbonneau - 2013.pdf;/Users/lbugnet/Zotero/storage/CHJ67ZNJ/Dressing, Charbonneau - 2013.pdf}
}

@article{Drobyshevski1974,
  title = {Topological Pumping of Magnetic Flux by Three-Dimensional Convection},
  author = {Drobyshevski, E. M. and Yuferev, V. S.},
  year = {1974},
  month = jan,
  journal = {Journal of Fluid Mechanics},
  volume = {65},
  pages = {33--44},
  issn = {0022-1120},
  doi = {10.1017/S0022112074001236},
  urldate = {2023-10-18},
  annotation = {ADS Bibcode: 1974JFM....65...33D}
}

@article{Drury,
  title = {{{KIC2569073}}, {{A}} Second {{Cepheid}} in the {{Kepler FOV}}},
  author = {Drury, Jason A and Kuehn, Charles A and Bellamy, Beau R and Stello, Dennis and Bedding, Timothy R},
  doi = {10.1051/C},
  urldate = {2020-03-27},
  abstract = {One particularly interesting new variable discovered via Kepler's 200x200 pixel superstamp images is KIC2569073. With a period of 14.66 days and 0.04mag variability it is only the second Cepheid in the Kepler field, or a rotationally modulated variable. We discuss its classification as a Type II W Virginis Class Cepheid, and present the cycle-to-cycle period variations of this star, as well as the first direct observations of granulation noise within a Cepheid.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/54QXXW2L/full-text.pdf}
}

@article{Drury2015,
  title = {{{KIC2569073}}, {{A}} Second {{Cepheid}} in the {{Kepler FOV}}},
  author = {Drury, Jason A. and Kuehn, Charles A. and Bellamy, Beau R. and Stello, Dennis and Bedding, Timothy R.},
  year = {2015},
  journal = {EPJWC},
  volume = {101},
  pages = {06024},
  doi = {10.1051/EPJCONF/201510106024},
  urldate = {2020-04-14},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XF9PDZXE/full-text.pdf}
}

@article{Du2019,
  title = {Mode {{Angular Degree Identification}} in {{Subgiant Stars}} with {{Convolutional Neural Networks}} Based on {{Power Spectrum}}},
  author = {Du, Minghao and Bi, Shaolan and Zhang, Xianfei and Li, Yaguang and Li, Tanda and Shi, Ruijie},
  year = {2019},
  journal = {MNRAS},
  volume = {accepted},
  eprint = {2012.13120v1},
  urldate = {2021-01-13},
  abstract = {Identifying the angular degrees \'i \textmu\'i{$\pm$} of oscillation modes is essential for asteroseismology and depends on visual tagging before fitting power spectra in a so-called peakbagging analysis. In oscillating subgiants, radial (\'i \textmu\'i{$\pm$} = 0) mode frequencies distributed linearly in frequency, while non-radial (\'i \textmu\'i{$\pm$} {$\geq$} 1) modes are p-g mixed modes that having a complex distribution in frequency, which increased the difficulty of identifying \'i \textmu\'i{$\pm$}. In this study, we trained a 1D convolutional neural network to perform this task using smoothed oscillation spectra. By training simulation data and fine-tuning the pre-trained network, we achieved a 95 per cent accuracy on Kepler data.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology-methods,data analysis-techniques,image processing-stars,notion,notion-database,statistics},
  file = {/Users/lbugnet/Zotero/storage/EVW6HH3Y/full-text.pdf}
}

@article{Duc2004,
  title = {Astrophysics {{A}} Top-down Scenario for the Formation},
  author = {Duc, P and Bournaud, F and Masset, F},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {814},
  eprint = {astro-ph/0408524},
  pages = {803--814},
  issn = {0004-6361},
  doi = {10.1051/0004-6361},
  abstract = {Among those objects formed out of collisional debris during galaxy mergers, the prominent gaseous accumulations observed near the tip of some long tidal tails are the most likely to survive long enough to form genuine recycled galaxies. Using simple numerical models, Bournaud et al. (2003) claimed that tidal objects as massive as 109 M  could only form, in these simulations, within extended dark matter (DM) haloes. We present here a new set of simulations of galaxy collisions to further investigate the structure of tidal tails. First of all, we checked that massive objects are still produced in full N-body codes that include feedback and a large number of particles. Using a simpler N-body code with rigid haloes, we noticed that dissipation and self-gravity in the tails, although important, are not the key factors. Exploiting toy models, we found that, for truncated DM haloes, material is stretched along the tail, while, within extended haloes, the tidal field can efficiently carry away from the disk a large fraction of the gas, while maintaining its surface density to a high value. This creates a density enhancement near the tip of the tail. Only later-on, self-gravity takes over; the gas clouds collapse and start forming stars. Thus, such objects were fundamentally formed following a kinematical process, according to a top-down scenario, contrary to the less massive Super Star Clusters that are also present around mergers. This conclusion leads us to introduce a restrictive definition for Tidal Dwarf Galaxies (TDGs) and their progenitors, considering only the most massive ones, initially mostly made of gas, that were able to pile up in the tidal tails. More simulations will be necessary to precisely determine the fate of these proto\textendash TDGs and estimate their number.},
  archiveprefix = {arxiv},
  keywords = {abundances,accretion,accretion disks,Activit\'e stellaire,Champ intense,Champ magn\'etique,cosmology,dark matter,dwarf,Espectropolarimetr\'ia,Etoile magn\'etique,Etoile type RR Lyrae,formation,galaxies,halos,High field,hydrodynamics,interactions,Magnetic fields,Magnetic stars,Mod\`ele,Modelo,Models,notion,notion-database,planetary systems,pre-main sequence,rotation,RR Lyr,RR Lyrae stars,Spectropolarim\'etrie,Spectropolarimetry,stars,stars: individual: RR Lyrae,stars: magnetic fields,stars: oscillations,stars: variables: RR Lyr,Stellar activity,{techniques: spectroscopic, polarimetric}},
  file = {/Users/lbugnet/Zotero/storage/5V3GV2LZ/Bouvier - 2008.pdf;/Users/lbugnet/Zotero/storage/5WGX9MSJ/Duc, Bournaud, Masset - 2004(5).pdf;/Users/lbugnet/Zotero/storage/C2Y4CVPR/Duc, Bournaud, Masset - 2004(3).pdf;/Users/lbugnet/Zotero/storage/DMMJJR9L/full-text.pdf;/Users/lbugnet/Zotero/storage/EIU6GJMC/Duc, Bournaud, Masset - 2004(7).pdf;/Users/lbugnet/Zotero/storage/ITKZG9IG/full-text.pdf;/Users/lbugnet/Zotero/storage/JHP28M8M/full-text.pdf;/Users/lbugnet/Zotero/storage/KT3LZIWJ/full-text.pdf;/Users/lbugnet/Zotero/storage/LCCVG5TG/Duc, Bournaud, Masset - 2004(6).pdf;/Users/lbugnet/Zotero/storage/NQA9J689/full-text.pdf;/Users/lbugnet/Zotero/storage/PL7BGS82/Duc, Bournaud, Masset - 2004.pdf;/Users/lbugnet/Zotero/storage/PRTFJDCI/Duc, Bournaud, Masset - 2004(4).pdf;/Users/lbugnet/Zotero/storage/V3QPGFKQ/Duc, Bournaud, Masset - 2004(2).pdf}
}

@article{Duchene2013,
  title = {Stellar Multiplicity},
  author = {Duch{\^e}ne, Gaspard and Kraus, Adam},
  year = {2013},
  month = aug,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {51},
  number = {1},
  eprint = {1303.3028},
  pages = {269--310},
  issn = {00664146},
  doi = {10.1146/annurev-astro-081710-102602},
  urldate = {2020-08-31},
  abstract = {Stellar multiplicity is a ubiquitous outcome of the star-formation process. The frequency and main characteristics of multiple systems, and their dependence on primary mass and environment, are powerful tools to probe this process. Although early attempts were fraught with selection biases and limited completeness, instrumentation breakthroughs in the past two decades now enable robust statistical analyses. In this review, we summarize current empirical knowledge of stellar multiplicity for main sequence stars and brown dwarfs, as well as among populations of pre-main-sequence stars and embedded protostars. Among field objects, the multiplicity rate and breadth of the orbital period distribution are steep functions of the primary mass, whereas the mass ratio distribution is essentially flat for most populations other than the lowest mass objects. The time-variation of the frequency of visual companions follows two parallel, constant tracks corresponding to loose and dense stellar populations, although current observations do not yet distinguish whether initial multiplicity properties are universal or dependent on the physical conditions of the parent cloud. Nonetheless, these quantitative trends provide a rich comparison basis for numerical and analytical models of star formation. Copyright \textcopyright 2013 by Annual Reviews. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Main-sequence stars,notion,notion-database,Pre-main-sequence stars,Protostars,Star formation}
}

@phdthesis{Duez2009,
  title = {Par {{Mod\'elisation}} Des {{Champs Magn\'etiques}} de {{Grandes \'Echelles}} Dans Les {{Int\'erieurs Stellaires Application}} Aux \'Etoiles de Type Solaire et Aux \'Etoiles {{Ap}}},
  author = {Duez, Vincent},
  year = {2009},
  keywords = {notion,notion-database}
}

@article{Duez2010,
  title = {Relaxed Equilibrium Configurations to Model Fossil Fields: {{I}}. {{A}} First Family},
  author = {Duez, V. and Mathis, S.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {517},
  number = {8},
  pages = {1--13},
  issn = {14320746},
  doi = {10.1051/0004-6361/200913496},
  abstract = {Context. The understanding of fossil fields' origin, topology, and stability is one of the corner stones of the stellar magnetism theory. On one hand, since they survive on secular time scales, they may modify the structure and the evolution of their host stars. On the other hand, they must have a complex stable structure since it has been demonstrated that the simplest purely poloidal or toroidal fields are unstable on dynamical time scales. In this context, the only stable configuration found today is the one resulting from a numerical simulation by Braithwaite and collaborators who studied the evolution of an initial stochastic magnetic field, which is found to relax on a mixed stable configuration (poloidal and toroidal) that seems to be in equilibrium and then diffuses. Aims. We investigate an equilibrium field in a semi-analytical way. In this first article, we study the barotropic magnetohydrostatic equilibrium states. Methods. The problem reduces to a Grad-Shafranov-like equation with arbitrary functions. These functions are constrained by deriving the lowest-energy equilibrium states for given invariants of the considered axisymmetric problem, in particular for a given helicity known to be one of the causes of such problems. These theoretical results were applied to realistic stellar cases, the solar radiative core and the envelope of an Ap star, and discussed. In both cases we assumed that the field is initially confined in the stellar radiation zone. Results. The generalization of the force-free Taylor's relaxation states studied in laboratory experiments (in spheromaks) that become non force-free in the self-gravitating stellar case are obtained. The case of general baroclinic equilibrium states will be studied in Paper II. \textcopyright{} 2010 ESO.},
  keywords = {magnetic field,Magnetic fields,Magnetohydrodynamics (MHD),notion,notion-database,Plasmas,Stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/3PNX83SM/Duez, Mathis - 2010.pdf}
}

@article{Duez2010a,
  title = {On the Stability of Non-Force-Free Magnetic Equilibria in Stars},
  author = {Duez, V. and Braithwaite, J. and Mathis, S.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {724},
  number = {1 PART 2},
  pages = {34--38},
  issn = {20418213},
  doi = {10.1088/2041-8205/724/1/L34},
  abstract = {The existence of stable magnetic configurations in white dwarfs, neutron stars, and various non-convective stellar regions is now well recognized. It has recently been shown numerically that various families of equilibria, including axisymmetric mixed poloidal-toroidal configurations, are stable. Here we test the stability of an analytically derived non-force-free magnetic equilibrium resulting from an initial relaxation (self-organization) process, using threedimensional magnetohydrodynamic simulations: the obtained mixed configuration is compared with the dynamical evolution of its purely poloidal and purely toroidal components, both known to be unstable. The mixed equilibrium shows no sign of instability under white noise perturbations. This configuration therefore provides a good description of magnetic equilibrium topology inside non-convective stellar objects and will be useful to initialize magneto-rotational transport in stellar evolution codes and in multi-dimensional magnetohydrodynamic simulations. \textcopyright{} 2010 The American Astronomical Society. All rights reserved.},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Stars: interiors,Stars: magnetic field,Stars: neutron,Sun: magnetic topology,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/QSA7GRGN/Duez, Braithwaite, Mathis - 2010.pdf}
}

@article{Duez2010b,
  title = {Effect of a Fossil Magnetic Field on the Structure of a Young {{Sun}}},
  author = {Duez, V. and Mathis, S. and {Turck-Chi{\`e}ze}, S.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {402},
  number = {1},
  pages = {271--281},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.15955.x},
  abstract = {We study the impact of a fossil magnetic field on the physical quantities which describe the structure of a young Sun of 500 Myr. We consider for the first time a non-force-free field composed of a mixture of poloidal and toroidal magnetic fields and propose a specific configuration to illustrate our purpose. In this paper, we estimate the relative role of the different terms which appear in the modified stellar structure equations. We note that the Lorentz tension plays a non-negligible role in addition to the magnetic pressure. This is interesting because most of the previous stellar evolution codes ignored that term and the geometry of the field. The solar structure perturbations are, as already known, small and consequently we have been able to estimate each term semi-analytically. We develop a general treatment to calculate the global modification of the structure and of the energetic balance. We also estimate the gravitational multipolar moments associated with the presence of a fossil large-scale magnetic field in radiative zone. The values given for the young Sun help the future implementation in stellar evolution codes. This work can be repeated for any other field configuration and prepares the achievement of a solar magnetohydrodynamic model where we will follow the transport of such field on secular time-scales and the associated transport of momentum and chemicals. The described method will be applied at the present Sun and the results will be compared with the coming balloon or space measurements. \textcopyright{} 2009 The Authors. Journal compilation \textcopyright{} 2009 RAS.},
  keywords = {Magnetic fields,MHD,notion,notion-database,Sun: interior,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/6KSVFX79/Duez, Mathis, Turck-Chièze - 2010.pdf}
}

@article{Duez2011,
  title = {Numerical Simulations of Magnetic Relaxation in Rotating Stellar Radiation Zones},
  author = {Duez, V.},
  year = {2011},
  month = dec,
  journal = {Astronomische Nachrichten},
  volume = {332},
  number = {9-10},
  pages = {983--987},
  issn = {00046337},
  doi = {10.1002/asna.201111610},
  urldate = {2020-07-02},
  abstract = {I detail the results of simulations of magnetic relaxation, as is assumed to happen in stellar radiation zones: starting from an initially stochastically organized magnetic field, this one self-organizes towards a large-scale, mainly dipolar configuration with both poloidal and toroidal components. While previous studies focused on the description of static equilibria, I include here the rotation in the numerical setup which substantially modifies the outcome of the simulations. In particular, magnetic equilibria are found, whose configuration remain stable over diffusive timescales (in general of the order of the main-sequence lifetime) rather than dynamic ones, as would be the case in presence of MHD instability. Their privileged axis are inclined with respect to the rotation axis, as observed in early-type, magnetic main sequence stars. The stationary internal flows and the dependence of the final equilibrium state on the rotation rate are described. Implications on stellar evolution are discussed. \textcopyright{} 2011 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {Magnetohydrodynamics (MHD),Methods: numerical,notion,notion-database,Stars: magnetic fields,Stars: rotation}
}

@article{Dufour2008,
  title = {{{SDSS J142625}}.71+575218.3: {{The First Pulsating White Dwarf}} with a {{Large Detectable Magnetic Field}}},
  shorttitle = {{{SDSS J142625}}.71+575218.3},
  author = {Dufour, P. and Fontaine, G. and Liebert, James and Williams, Kurtis and Lai, David K.},
  year = {2008},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {683},
  pages = {L167},
  issn = {0004-637X},
  doi = {10.1086/591672},
  urldate = {2023-10-19},
  abstract = {We report the discovery of a strong magnetic field in the unique pulsating carbon-atmosphere white dwarf SDSS J142625.71+575218.3. From spectra gathered at the MMT and Keck telescopes, we infer a surface field of Bssimeq 1.2 MG, based on obvious Zeeman components seen in several carbon lines. We also detect the presence of a Zeeman-splitted He I {$\lambda$}4471 line, which is an indicator of the presence of a nonnegligible amount of helium in the atmosphere of this "hot DQ" star. This is important for understanding its pulsations, as nonadabatic theory reveals that some helium must be present in the envelope mixture for pulsation modes to be excited in the range of effective temperature where the target star is found. Out of nearly 200 pulsating white dwarfs known today, this is the first example of a star with a large detectable magnetic field. We suggest that SDSS J142625.71+575218.3 is the white dwarf equivalent of a rapidly oscillating Ap star.},
  keywords = {Astrophysics,stars: abundances,stars: atmospheres,stars: individual: SDSS J1426\&plus5752,stars: magnetic fields},
  annotation = {ADS Bibcode: 2008ApJ...683L.167D},
  file = {/Users/lbugnet/Zotero/storage/ARJ8Q7YQ/Dufour et al. - 2008 - SDSS J142625.71+575218.3 The First Pulsating Whit.pdf}
}

@article{Dumusque2011,
  title = {Astronomy \& {{Astrophysics Planetary}} Detection Limits Taking into Account Stellar Noise {{I}}. {{Observational}} Strategies to Reduce Stellar Oscillation and Granulation Effects},
  author = {Dumusque, X and Udry, S and Lovis, C and Santos, N C and Monteiro, M J P F G},
  year = {2011},
  journal = {A\&A},
  volume = {525},
  pages = {140},
  doi = {10.1051/0004-6361/201014097},
  urldate = {2020-03-15},
  abstract = {Context. Stellar noise produced by oscillations, granulation phenomena (granulation, mesogranulation, and supergranulation), and activity affects radial velocity measurements. The signature of the corresponding effect in radial velocity is small, around the meter-per-second, but already too large for the detection of Earth-mass planets in habitable zones. Aims. We address the important role played by observational strategies in averaging out the radial velocity signature of stellar noise. We also derive the planetary mass detection limits expected in the presence of stellar noise. Methods. We start with HARPS asteroseismology measurements for four stars ({$\beta$} Hyi, {$\alpha$} Cen A, {$\mu$} Ara, and {$\tau$} Ceti) available in the ESO archive and very precise measurements of {$\alpha$} Cen B. This sample covers different spectral types from G2 to K1 and different evolutionary stages, from subgiant to dwarf stars. Since data span between 5 and 8 days, only stellar noise sources with timescales shorter than this time span will be extracted from these observations. Therefore, we are able to study oscillation modes and granulation phenomena without being significantly affected by activity noise present on longer timescales. For those five stars, we generate synthetic radial velocity measurements after fitting the corresponding models of stellar noise in Fourier space. These measurements allow us to study the radial velocity variation due to stellar noise for different observational strategies as well as the corresponding planetary mass detection limits. Results. Applying three measurements per night of 10 min exposure each, 2 h apart, seems to most efficiently average out the stellar noise considered. For quiet K1V stars such as {$\alpha$} Cen B, this strategy allows us to detect planets of about three times the mass of Earth with an orbital period of 200 days, corresponding to the habitable zone of the star. Moreover, our simulations suggest that planets smaller than typically 5 M {$\oplus$} can be detected with HARPS over a wide range of separations around most non-active solar-type dwarfs. Since activity is not yet included in our simulation, these detection limits correspond to a case, which exists, where the host star has few magnetic features and stellar noise is dominated by oscillation modes and granulation phenomena. For our star sample, a trend between spectral type and surface gravity and the level of radial velocity variation is also identified by our simulations.},
  keywords = {notion,notion-database,oscillations,oscillations-techniques,planetary systems,planetary systems-stars,radial velocities,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/HAXS94LX/full-text.pdf}
}

@article{Dumusque2011a,
  title = {Planetary Detection Limits Taking into Account Stellar Noise: {{II}}. {{Effect}} of Stellar Spot Groups on Radial-Velocities},
  author = {Dumusque, X. and Santos, N. C. and Udry, S. and Lovis, C. and Bonfils, X.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {527},
  number = {10},
  issn = {00046361},
  doi = {10.1051/0004-6361/201015877},
  abstract = {Context. The detection of small mass planets with the radial-velocity technique is now confronted with the interference of stellar noise. HARPS can now reach a precision below the meter-per-second, which corresponds to the amplitudes of different stellar perturbations, such as oscillation, granulation, and activity. Aims. Solar spot groups induced by activity produce a radial-velocity noise of a few meter-per-second. The aim of this paper is to simulate this activity and calculate detection limits according to different observational strategies. Methods. Based on Sun observations, we reproduce the evolution of spot groups on the surface of a rotating star. We then calculate the radial-velocity effect induced by these spot groups as a function of time. Taking into account oscillation, granulation, activity, and a HARPS instrumental error of 80-1, we simulate the effect of different observational strategies in order to efficiently reduce all sources of noise. Results. Applying three measurements per night of 10 min every three days, 10 nights a month seems the best tested strategy. Depending on the level of activity considered, from log R{${'}$}HK = - 5 to - 4.75, this strategy would allow us to find planets of 2.5 to 3.5 M{$\oplus$} in the habitable zone of a K1V dwarf. Using Bern's model of planetary formation, we estimate that for the same range of activity level, 15 to 35\% of the planets between 1 and 5 M{$\oplus$} and with a period between 100 and 200 days should be found with HARPS. A comparison between the performance of HARPS and ESPRESSO is also emphasized by our simulations. Using the same optimized strategy, ESPRESSO could find 1.3 M{$\oplus$} planets in the habitable zone of K dwarfs. In addition, 80\% of planets with mass between 1 and 5 M{$\oplus$} and with a period between 100 and 200 days could be detected. \textcopyright{} 2011 ESO.},
  keywords = {notion,notion-database,planetary systems,stars: activity,stars: individual: \'a CenB,Sun: activity,sunspots,techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/EFLPEWK2/Dumusque et al. - 2011.pdf}
}

@article{Dumusque2014,
  title = {The Kepler-10 Planetary System Revisited by Harps-n: {{A}} Hot Rocky World and a Solid Neptune-Mass Planet},
  author = {Dumusque, Xavier and Bonomo, Aldo S. and Haywood, Rapha{\"e}lle D. and Malavolta, Luca and S{\'e}gransan, Damien and Buchhave, Lars A. and Cameron, Andrew Collier and Latham, David W. and Molinari, Emilio and Pepe, Francesco and Udry, St{\'e}phane and Charbonneau, David and Cosentino, Rosario and Dressing, Courtney D. and Figueira, Pedro and Fiorenzano, Aldo F.M. and Gettel, Sara and Harutyunyan, Avet and Horne, Keith and {Lopez-Morales}, Mercedes and Lovis, Christophe and Mayor, Michel and Micela, Giusi and Motalebi, Fatemeh and Nascimbeni, Valerio and Phillips, David F. and Piotto, Giampaolo and Pollacco, Don and Queloz, Didier and Rice, Ken and Sasselov, Dimitar and Sozzetti, Alessandro and Szentgyorgyi, Andrew and Watson, Chris},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {789},
  number = {2},
  issn = {15384357},
  doi = {10.1088/0004-637X/789/2/154},
  abstract = {Kepler-10b was the first rocky planet detected by the Kepler satellite and confirmed with radial velocity follow-up observations from Keck-HIRES. The mass of the planet was measured with a precision of around 30\%, which was insufficient to constrain models of its internal structure and composition in detail. In addition to Kepler-10b, a second planet transiting the same star with a period of 45 days was statistically validated, but the radial velocities were only good enough to set an upper limit of 20 M {$\oplus$} for the mass of Kepler-10c. To improve the precision on the mass for planet b, the HARPS-N Collaboration decided to observe Kepler-10 intensively with the HARPS-N spectrograph on the Telescopio Nazionale Galileo on La Palma. In total, 148 high-quality radial-velocity measurements were obtained over two observing seasons. These new data allow us to improve the precision of the mass determination for Kepler-10b to 15\%. With a mass of 3.33 {$\pm$} 0.49 M {$\oplus$} and an updated radius of R {$\oplus$}, Kepler-10b has a density of 5.8 {$\pm$} 0.8 g cm-3, very close to the value predicted by models with the same internal structure and composition as the Earth. We were also able to determine a mass for the 45-day period planet Kepler-10c, with an even better precision of 11\%. With a mass of 17.2 {$\pm$} 1.9 M {$\oplus$} and radius of R {$\oplus$}, Kepler-10c has a density of 7.1 {$\pm$} 1.0 g cm-3. Kepler-10c appears to be the first strong evidence of a class of more massive solid planets with longer orbital periods. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  keywords = {notion,notion-database,planetary systems,stars: individual (Kepler-10 KOI-072 KIC 11904151),stars: statistics,techniques: photometric,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/6FPSWKCK/Dumusque et al. - 2014.pdf}
}

@article{Dupret2005,
  title = {Convection-Pulsation Coupling. {{II}}. {{Excitation}} and Stabilization Mechanisms in {$\delta$} {{Sct}} and {$\gamma$} {{Dor}} Stars},
  author = {Dupret, M. A. and Grigahc{\`e}ne, A. and Garrido, R. and Gabriel, M. and Scuflaire, R.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {435},
  number = {3},
  pages = {927--939},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041817},
  abstract = {We apply here the Time Dependent Convection (TDC) treatment presented in our earlier paper in this series to the study of {$\delta$} Sct and {$\gamma$} Dor pulsating stars. Stabilization of the {$\delta$} Set p-modes at the red edge of the Instability Strip (IS) and the driving of the {$\gamma$} Dor g-modes are explained by our models. Theoretical IS obtained with different values of the Mixing Length (ML) parameter {$\alpha$} are compared to observations and a good agreement is obtained for {$\alpha$} between 1.8 and 2. The influence of each term of our TDC treatment (perturbation of convective flux, turbulent pressure, and turbulent kinetic energy dissipation) on the eigenfrequencies and on the driving and damping mechanisms is investigated. Finally, we show that our TDC models predict the likely existence of hybrid stars with both {$\delta$} Set p-modes and {$\gamma$} Dor g-modes oscillations. \textcopyright{} ESO 2005.},
  keywords = {Convection,notion,notion-database,Stars: interiors,Stars: oscillations,Stars: variables: 6 Set,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/TT56BE4F/Dupret et al. - 2005.pdf}
}

@article{Dupret2009,
  title = {Theoretical Amplitudes and Lifetimes of Non-Radial Solar-like Oscillations in Red Giants},
  author = {Dupret, M. A. and Belkacem, K. and Samadi, R. and Montalban, J. and Moreira, O. and Miglio, A. and Godart, M. and Ventura, P. and Ludwig, H. G. and Grigahc{\`e}ne, A. and Goupil, M. J. and Noels, A. and Caffau, E.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {57--67},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911713},
  abstract = {Context. Solar-like oscillations have been observed in numerous red giants from ground and from space. An important question arises: could we expect to detect non-radial modes probing the internal structure of these stars? Aims. We investigate under what physical circumstances non-radial modes could be observable in red giants; what would be their amplitudes, lifetimes and heights in the power spectrum (PS)? Methods. Using a non-radial non-adiabatic pulsation code including a non-local time-dependent treatment of convection, we compute the theoretical lifetimes of radial and non-radial modes in several red giant models. Next, using a stochastic excitation model, we compute the amplitudes of these modes and their heights in the PS. Results. Distinct cases appear. Case A corresponds to subgiants and stars at the bottom of the ascending giant branch. Our results show that the lifetimes of the modes are mainly proportional to the inertia I, which is modulated by the mode trapping. The predicted amplitudes are lower for non-radial modes. But the height of the peaks in the PS are of the same order for radial and non-radial modes as long as they can be resolved. The resulting frequency spectrum is complex. Case B corresponds to intermediate models in the red giant branch. In these models, the radiative damping becomes high enough to destroy the non-radial modes trapped in the core. Hence, only modes trapped in the envelope have significant heights in the PS and could be observed. The resulting frequency spectrum of detectable modes is regular for {$\mathscr{l}$} = 0 and 2, but a little more complex for {$\mathscr{l}$} = 1 modes because of less efficient trapping. Case C corresponds to models of even higher luminosity. In these models the radiative damping of non-radial modes is even larger than in the previous case and only radial and non-radial modes completely trapped in the envelope could be observed. The frequency pattern is very regular for these stars. The comparison between the predictions for radial and non-radial modes is very different if we consider the heights in the PS instead of the amplitudes. This is important as the heights (not the amplitudes) are used as detection criterion.},
  keywords = {Convection,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/NL7YYEFR/Dupret et al. - 2009.pdf}
}

@article{Durney1971,
  title = {Differential {{Rotation}}, {{Meridional Velocities}}, and {{Pole-Equator Difference}} in {{Temperature}} of a {{Rotating Convective Spherical Shell}}},
  author = {Durney, B.},
  year = {1971},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {163},
  pages = {353},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/150775},
  urldate = {2020-03-09},
  keywords = {notion,notion-database}
}

@article{Duvall1983,
  title = {Observations of Solar Oscillations of Low and Intermediate Degree},
  author = {Duvall, T. L. and Harvey, J. W.},
  year = {1983},
  journal = {Nature},
  volume = {302},
  number = {5903},
  pages = {24--27},
  issn = {00280836},
  doi = {10.1038/302024a0},
  abstract = {Measurements are presented of solar velocity oscillations with spherical harmonic degree 1-139 and angular order {$\sim$}0. With an amplitude sensitivity of {$\sim$}2 cm s -1, trapped acoustic wave modes of radial orders 2-26 are observed at frequencies between 1.7 and 5.5 mHz. The radial order identifications of low-degree modes previously inferred from theory are confirmed. Only marginal evidence of long-period, gravity-mode oscillations is found \textcopyright{} 1983 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/X7F3SN28/Duvall, Harvey - 1983.pdf}
}

@article{Duvall1984,
  title = {Internal Rotation of the {{Sun}}},
  author = {Duvall, T. L. and Dziembowski, W. A. and Goode, P. R. and Gough, D. O. and Harvey, J. W. and Leibacher, J. W.},
  year = {1984},
  journal = {Nature},
  volume = {310},
  number = {5972},
  pages = {22--25},
  issn = {00280836},
  doi = {10.1038/310022a0},
  urldate = {2020-03-02},
  abstract = {The frequency difference between prograde and retrograde sectoral solar oscillations is analysed to determine the rotation rate of the solar interior, assuming no latitudinal dependence. Much of the solar interior rotates slightly less rapidly than the surface, while the innermost part apparently rotates more rapidly. The resulting solar gravitational quadrupole moment is J2 = (1.7{$\pm$}0.4) \texttimes{} 10-7 and provides a negligible contribution to current planetary tests of Einstein's theory of general relativity. \textcopyright{} 1984 Nature Publishing Group.},
  keywords = {Convection,notion,notion-database,Quadrupoles,Relativity,Solar Interior,Solar Oscillations,Solar Physics,Solar Rotation,Stellar Cores,Stellar Spectra},
  file = {/Users/lbugnet/Zotero/storage/E44RMRCN/full-text.pdf}
}

@article{Duvall1991,
  title = {Measurements of High-Frequency Solar Oscillation Modes},
  author = {Duvall, T. L. {\relax Jr}. and Harvey, J. W. and Jefferies, S. M. and Pomerantz, M. A.},
  year = {1991},
  journal = {The Astrophysical Journal},
  volume = {373},
  eprint = {1011.1669v3},
  pages = {308--316},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YN7843PG/Duvall et al. - 1991.pdf}
}

@article{Dziembowski1984,
  title = {Simple {{Asymptotic Estimates}} of the {{Fine Structure}} in the {{Spectrum}} of {{Solar Oscillations}} Due to {{Rotation}} and {{Magnetism}}},
  author = {Dziembowski, W. A. and Goode, P. R.},
  year = {1984},
  journal = {Mem. S.A. It.},
  volume = {55},
  number = {1-2},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DIM3NZN2/Dziembowski, Goode - 1984.pdf}
}

@article{Dziembowski1985,
  title = {Frequency Splitting in {{Ap}} Stars},
  author = {Dziembowski, W. A. and Goode, P. R.},
  year = {1985},
  journal = {The Astrophysical Journal},
  volume = {296},
  eprint = {1011.1669v3},
  pages = {27--30},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RHKU5E2N/Dziembowski, Goode - 1985.pdf}
}

@article{Dziembowski1989,
  title = {The Toroidal Magnetic Fiels inside the Sun},
  author = {Dziembowski, W. A. and Goode, P. R.},
  year = {1989},
  journal = {The Astrophysical Journal},
  volume = {347},
  eprint = {1011.1669v3},
  pages = {540--550},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KV2GC3I7/Dziembowski, Goode - 1989.pdf}
}

@article{Dziembowski1989a,
  title = {The Raidal Gradient in the Sun's Rotation},
  author = {Dziembowski, W. A. and Goode, P. R. and Libbrecht, K G},
  year = {1989},
  journal = {The Astrophysical Journal of Chemical Information and Modeling},
  volume = {337},
  eprint = {1011.1669v3},
  pages = {53--57},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9XG46ZUS/Dziembowski, Goode, Libbrecht - 1989.pdf}
}

@article{Dziembowski1992,
  title = {Effects of Differential Rotation on Stellar Oscillations - {{A}} Second-Order Theory},
  author = {Dziembowski, W. A. and Goode, Philip R.},
  year = {1992},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {394},
  pages = {670},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/171621},
  urldate = {2020-06-03},
  abstract = {A complete formalism, valid through second order in differential rotation, is developed and applied to calculate the frequencies of stellar oscillations. We improved the derivation and generalized the asymptotic formulae for g-mode splittings. In application to solar oscillations, we find that the second-order effects are dominated by distortion for l  {$<$}  500. Further, these effects are sufficiently large that they must be accounted for in any effort to seismically determine the Sun's internal magnetic field. In the solar oscillation spectrum, accidental degeneracies happen but cannot lead to large frequency shifts. For evolved {$\delta$} Scuti stars, calculated spectra are dense, and, under the perturbing effect of rotation, members of neighboring multiplets may overlap. The seismic potential of modes of mixed p-mode and g-mode character is emphasized for these stars.},
  keywords = {Astronomy,Cepheid Variables,Computational Astrophysics,notion,notion-database,Solar Magnetic Field,Solar Oscillations,STARS: OSCILLATIONS,STARS: ROTATION,Stellar Evolution,Stellar Models,Stellar Oscillations,Stellar Rotation,Stellar Spectra,SUN: OSCILLATIONS}
}

@article{Dziembowski1993,
  title = {The Opacity Mechanism in {{B-type}} Stars-1. {{Unstable}} Modes in \ss{} {{Cephei}} Star Models},
  author = {Dziembowski, W A and Pamyatnykh, A A},
  year = {1993},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {262},
  pages = {204--212},
  urldate = {2020-04-09},
  abstract = {An improved version of the opal opacities, with the metal abundance parameter Z having values of 0.02 and 0.03, has been used in a stability survey for models of 7-to 16-M 0 stars in the main-sequence (MS) and early post-MS evolutionary phases. All \ss{} Cep stars lie within the domain of the HR diagram where pulsational instability is caused by the opacity mechanism acting in the metal opacity bump at r\guillemotleft 2xl0 5 K. For most of the objects, a value of Z = 0.02 suffices to account for the pulsation. The positions of \ss{} Cep stars in the HR diagram correspond to models in an advanced phase of core hydrogen burning, constructed without allowing for effects of the convective overshooting. The fundamental radial mode \{pj is unstable in all sequences of stellar models considered, except the one with M=7 M 0 and Z = 0.02. Instability of the overtones, up to p 3 for Z = 0.03, appears with mass increase. Non-radial modes of low degrees are unstable in a wider frequency range encompassing low-order g-modes. All of these modes may be associated with the \ss{} Cep phenomenon. In addition, for higher spherical harmonic degrees (/\^ 6), there is a domain of high-order g-mode instability. Excitation of such modes may be responsible for long-period variability of line profiles observed in some B-type stars.\vphantom\}},
  keywords = {early-type-stars,instabilities-stars,interiors-stars,notion,notion-database,oscillations},
  file = {/Users/lbugnet/Zotero/storage/FDK6T25S/full-text.pdf}
}

@article{Dziembowski1996,
  title = {Magnetic {{Effects}} on {{Oscillations}} in {{roAp Stars}}},
  author = {Dziembowski, W. A. and Goode, Phillip R.},
  year = {1996},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {458},
  pages = {338},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/176816},
  urldate = {2020-06-29},
  abstract = {We calculate the effect of a simple dipole magnetic field on high-order p-mode oscillations. The stellar models, oscillation modes, and range of field intensity were selected to correspond to the data on roAp stars. We did not account for the field in the static models. Some of the modes we calculate exhibit a strong driving due to the {$\kappa$}-mechanism acting in the hydrogen ionization zone. This driving is only somewhat smaller than the radiative damping occurring beneath. We argue that the situation is likely to reverse after needed improvements are made in model calculations. The effect of the field is very significant. At KG photospheric intensity, the mode frequencies are shifted by about 10-20 {$\mu$}Hz from their nonmagnetic values. Such shifts are comparable to the small separations. Damping rates due to Alfv\'enic wave losses are in the 2-10 {$\mu$}Hz range and are comparable to nonadiabatic damping rates. Surface amplitudes significantly depart from pure, single spherical harmonic dependence, which severely complicates mode identification and observational determination of large separations. Thus, taking into account the effects of the magnetic field is a prerequisite to any meaningful roAp star asteroseismology and to understanding mode selection in these objects. \textcopyright{} 1996. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database}
}

@article{Dziembowski2001,
  title = {Oscillations of {$\alpha$} {{UMa}} and Other Red Giants},
  author = {Dziembowski, W. A. and Gough, D. O. and Houdek, G. and Sienkiewicz, R.},
  year = {2001},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {328},
  number = {2},
  pages = {601--610},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2001.04894.x},
  abstract = {There is growing observational evidence that the variability of red giants could be caused by self-excitation of global modes of oscillation. The most recent evidence of such oscillations was reported for {$\alpha$} UMa by Buzasi et al. who analysed space photometric data from the WIRE satellite. Little is understood concerning the oscillation properties in red giants. In this paper we address the question as to whether excited radial and non-radial modes can explain the observed variability in red giants. In particular, we present the results of numerical computations of oscillation properties of a model of {$\alpha$} UMa and of several models of a 2-M{$\odot$} star in the red giant phase. The red giant stars that we have studied have two cavities that can support oscillations: the inner core that supports gravity (g) waves and the outer one that supports acoustic (p) waves. Most of the modes in the p-mode frequency range are g modes confined in the core; those modes with frequencies close to a corresponding characteristic frequency of a p mode in the outer cavity are of mixed character and have substantial amplitudes in the outer cavity. We have shown that such modes of low degree, {$\mathscr{l}$} = 1 and 2, together with the radial (p) modes, can be unstable. The linear growth rates of these non-radial modes are similar to those of corresponding radial modes. In the model of {$\alpha$} UMa and in the 2-M{$\odot$} models in the lower regions of the giant branch, high amplitudes in the p-mode cavity arise only for modes with {$\mathscr{l}$} = 2. We have been unable to explain the observed oscillation properties of {$\alpha$} UMa, either in terms of mode instability or in terms of stochastic excitation by turbulent convection. The modes with the lowest frequencies, which exhibit the largest amplitudes and may correspond to the first three radial modes, are computed to be unstable if all of the effects of convection are neglected in the stability analyses. However, if the Lagrangian perturbations of the turbulent fluxes (heat and momentum) are taken into account in the pulsation calculation, only modes with higher frequencies are found to be unstable. The observed frequency dependence of amplitudes reported by Buzasi et al. does not agree with what one expects from stochastic excitation. This mechanism predicts an amplitude of the fundamental mode about two orders of magnitude smaller than the amplitudes of modes with orders n {$\geq$} 5, which is in stark disagreement with the observations.},
  keywords = {Convection,notion,notion-database,Stars: individual: {$\alpha$} Uma,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/PPN92AD3/Dziembowski et al. - 2001.pdf}
}

@article{Dziembowski2004a,
  title = {Helioseismic {{Probing}} of {{Solar Variability}}: {{The Formalism}} and {{Simple Assessments}}},
  author = {Dziembowski, W. A. and Goode, P. R.},
  year = {2004},
  journal = {The Astrophysical Journal},
  volume = {600},
  number = {1},
  eprint = {astro-ph/0310095},
  pages = {464--479},
  issn = {0004-637X},
  doi = {10.1086/379708},
  abstract = {We derive formulae connecting the frequency variations in the spectrum of solar oscillations to the dynamical quantities that are expected to change over the solar activity cycle. This is done for both centroids and the asymmetric part of the fine structure (so-called even-a coefficients). We consider the near-surface, small-scale magnetic and turbulent velocity fields, as well as horizontal magnetic fields buried near the base of the convective zone. For the centroids we also discuss the effect of temperature variation. We demonstrate that there is a full, one-to-one correspondence between the expansion coefficients of the fine structure and those of both the averaged small-scale velocity and magnetic fields. Measured changes in the centroid frequencies and the even-a coefficients over the rising phase solar cycle may be accounted for by a decrease in the turbulent velocity of order 1\%. We show that the mean temperature decrease associated with the net decrease in the efficiency of convective transport may also significantly contribute to the increase of the centroid frequencies. Alternatively, the increase may be accounted for by an increase of the small-scale magnetic field of order 100 G, if the growing field is predominantly radial. We also show that global seismology can be used to detect a field at the level of a few times 10 5  G, if such a field were present and confined to a thin layer near the base of the convective envelope.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2Z2BUEFY/Dziembowski, Goode - 2004.pdf}
}

@article{Dziembowski2005a,
  title = {Sources of {{Oscillation Frequency Increase}} with {{Rising Solar Activity}}},
  author = {Dziembowski, W. A. and Goode, P. R.},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {625},
  number = {1},
  eprint = {astro-ph/0503266},
  pages = {548--555},
  issn = {0004-637X},
  doi = {10.1086/429712},
  abstract = {We analyze and interpret SOHO/MDI data on oscillation frequency changes between 1996 and 2004 focusing on differences between activity minimum and maximum of solar cycle 23. We study only the behavior of the centroid frequencies, which reflect changes averaged over spherical surfaces. Both the f-mode and p-mode frequencies are correlated with general measures of the sun's magnetic activity. However, the physics behind each of the two correlations is quite different. We show that for the f-modes the dominant cause of the frequency increase is the dynamical effect of the rising magnetic field. The relevant rise must occur in subphotospheric layers reaching to some 0.5 - 0.7 kG at a depth of about 5 Mm. However, the implied constraints also require the field change in the atmosphere to be so small that it has only a tiny dynamical effect on p-mode frequencies. For p-modes, the most plausible explanation of the frequency increase is a less than 2 percent decrease in the radial component of the turbulent velocity in the outer layers. Lower velocity implies a lower efficiency of the convective transport, hence lower temperature, which also contributes to the p-mode frequency increase.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Y82G5UVS/Dziembowski, Goode - 2005.pdf}
}

@article{Dziembowski2012a,
  title = {Dipolar Modes in Luminous Red Giants},
  author = {Dziembowski, W. A.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {539},
  pages = {1--10},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117733},
  abstract = {Context. Lots of information on solar-like oscillations in red giants has been obtained thanks to observations with CoRoT and Kepler space telescopes. Data on dipolar modes appear most interesting. Aims. We study properties of dipolar oscillations in luminous red giants to explain mechanism of mode trapping in the convective envelope and to assess what may be learned from the new data. Methods. Equations for adiabatic oscillations are solved by numerical integration down to the bottom of convective envelope, where the boundary condition is applied. The condition is based on asymptotic decomposition of the fourth order system into components describing a running wave and a nearly uniform shift of radiative core. Results. If the luminosity of a red giant is sufficiently high (L 100 Lo at M = 2 Mo), the dipolar modes become effectively trapped in the acoustic cavity, which covers the outer part of convective envelope. Energy loss caused by gravity wave emission at the envelope base is a secondary or negligible source of damping. Frequencies are insensitive to structure of the deep interior. \textcopyright{} ESO, 2012.},
  keywords = {Diffusion,Methods: analytical,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/L6HBWGYC/Dziembowski - 2012.pdf}
}

@article{Dziewonski1981,
  title = {Preliminary Reference {{Earth}} Model *},
  author = {Dziewonski, Adam M and Anderson, Don L},
  year = {1981},
  journal = {Preliminary reference Earth modeL Phys. Earth Planet. Inter},
  volume = {25},
  pages = {297--356},
  urldate = {2020-05-21},
  abstract = {A large data set consisting of about 1000 normal mode periods, 500 summary travel time observations, 100 normal mode Q values, mass and moment of inertia have been inverted to obtain the radial distribution of elastic properties, Q values and density in the Earth's interior. The data set was supplemented with a special study of 12 years of ISC phase data which yielded an additional 1.75 X 106 travel time observations for P and S waves. In order to obtain satisfactory agreement with the entire data set we were required to take into account anelastic dispersion. The introduction of transverse isotropy into the outer 220 km of the mantle was required in order to satisfy the shorter penod fundamental toroidal and spheroidal modet This anisotropy also improved the fit of the larger data set. The horizontal and vertical velocities in the upper mantle differ by 2-4\%, both for P and S waves. The mantle below 220 km is not required to be anisotropic. Mantle Rayleigh waves are surprisingly sensitive to compressional velocity in the upper mantle. High S\textasciitilde{} velocities, low P\textasciitilde velocities and a pronounced low-velocity zone are features of most global inversion models that are stqipressed when anisotropy is allowed for in the inversion. The Preliminary Reference Earth Model, PREM, and auxiliary tables showing fits to the data are presented. Preamble and his models A and B were employed extensively. The study of precession and nutation in astron-Seismological studies of the structure of the omy and geodesy, and of Earth tides and free Earth have developed rapidly since 1950, much oscillations in geophysics, need knowledge of the aided by the fast improvement in computer tech-internal structure of the Earth. The importance of niques. free and forced nutations, for instance, polar mo-Expansion in the utilization of computers made tion, Chandler and annual components, and di-it possible to construct many types of Earth mod-urnal motion of the Earth, in different fields of els. The consequent proliferation of Earth models science, emphasizes the value of the contribution had two consequences: of seismology for these researches. (I) There was a difficulty of choice of an ade-It was very difficult to set up models of the quate Earth model for researchers that depend on Earth's structure before the advent of computers; the structure of the Earth, such as those listed in the more important ones were set up by Bullen, the first paragraph. (2) Several researchers adopted some properties \textbullet{} With a preamble by the Standard Earth Committee of the from one model and other properties from a sec-I.U.G.G. Followed by "A note on the calculation of travel ond model, with the consequence that their models times in a transversely isotropic Earth model" by L\textasciitilde{} were not self-compatible. Woodhouse (this issue, pp. 357-359). These difficulties were pointed out, at a Sym},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5567VICS/full-text.pdf}
}

@article{Eastman2010,
  title = {Achieving {{Better Than}} 1~{{Minute Accuracy}} in the {{Heliocentric}} and {{Barycentric Julian Dates}}},
  author = {Eastman, Jason and Siverd, Robert and Gaudi, B. Scott},
  year = {2010},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {122},
  number = {894},
  eprint = {1005.4415},
  pages = {935--946},
  issn = {0004-6280},
  doi = {10.1086/655938},
  abstract = {As the quality and quantity of astrophysical data continue to improve, the precision with which certain astrophysical events can be timed becomes limited not by the data themselves, but by the manner, standard, and uniformity with which time itself is referenced. While some areas of astronomy (most notably pulsar studies) have required absolute time stamps with precisions of considerably better than 1 minute for many decades, recently new areas have crossed into this regime. In particular, in the exoplanet community, we have found that the (typically unspecified) time standards adopted by various groups can differ by as much as a minute. Left uncorrected, this ambiguity may be mistaken for transit timing variations and bias eccentricity measurements. We argue that, since the commonly-used Julian Date, as well as its heliocentric and barycentric counterparts, can be specified in several time standards, it is imperative that their time standards always be reported when accuracies of 1 minute are required. We summarize the rationale behind our recommendation to quote the site arrival time, in addition to using BJD\_TDB, the Barycentric Julian Date in the Barycentric Dynamical Time standard for any astrophysical event. The BJD\_TDB is the most practical absolute time stamp for extra-terrestrial phenomena, and is ultimately limited by the properties of the target system. We compile a general summary of factors that must be considered in order to achieve timing precisions ranging from 15 minutes to 1 microsecond. Finally, we provide software tools that, in principal, allow one to calculate BJD\_TDB to a precision of 1 microsecond for any target from anywhere on Earth or from any spacecraft.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/U2P22BSG/Eastman, Siverd, Gaudi - 2010.pdf}
}

@article{Eckart1960,
  title = {Variation {{Principles}} of {{Hydrodynamics}}},
  author = {Eckart, Carl},
  year = {1960},
  month = may,
  journal = {Physics of Fluids},
  volume = {3},
  pages = {421--427},
  issn = {0899-82131070-6631},
  doi = {10.1063/1.1706053},
  urldate = {2023-06-05},
  abstract = {It is shown that the Lagrangian equations for the motion of both incompressible and compressible fluids can be derived from variation principles. As has been pointed out by C. C. Lin, an important feature of these principles is the boundary condition: The coordinates of each particle (and not merely the normal component of its velocity) must be specified. A systematic application of known results from the calculus of variations reveals new interrelations between such hydrodynamic results as Bernoulli's principle and the circulation theorem. Their derivation is both simplified and systematized. Clebsch's transformation is found to have an important relation to the problem of integrating the vorticity equation. The general solution of this problem for nonbarotropic flow is obtained. This reduces the second-order Lagrange equations to a set of first-order equations, in which the potential of the irrotational component replaces the pressure. The entropy gradients and a remarkable quantity, defined as the time-integral of the temperature of a particle of the fluid, also appear.},
  annotation = {ADS Bibcode: 1960PhFl....3..421E}
}

@article{Eddington1924,
  title = {The {{Relation}} between the {{Masses}} and {{Luminosities}} of the {{Stars}}. {{A THEORY}} of the Physical Conditions in The},
  author = {Eddington, A. S.},
  year = {1924},
  journal = {Nature},
  volume = {113},
  pages = {786--788},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CB8KFFI2/113786a0.pdf}
}

@article{Eff-Darwich2010,
  title = {Advances in Solar Rotation Rate Inferences: {{Unstructured}} Grid Inversions and Improved Rotational Splittings},
  author = {{Eff-Darwich}, A. and Korzennik, S. and Garc{\'i}a, R.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  pages = {890--895},
  issn = {00046337},
  doi = {10.1002/asna.201011420},
  abstract = {We present a new inversion methodology that adapts the inversion grid in both radius and co-latitude to the data set and solves the inversion problem through an iterative procedure. This method was tested on state-of-the-art global mode frequency splittings to assess the solar interior rotation rate and its temporal variation. We also explore the influence of different data sets on the interpretation of the dynamics of the solar interior, particularly the spatial extend of the torsional oscillations \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: interior,Sun: oscillations,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/RR2FFRQH/Eff-Darwich, Korzennik, García - 2010.pdf}
}

@article{Eff-Darwich2013,
  title = {The {{Dynamics}} of the {{Solar Radiative Zone}}},
  author = {{Eff-Darwich}, A. and Korzennik, S. G.},
  year = {2013},
  journal = {Solar Physics},
  volume = {287},
  number = {1-2},
  eprint = {1205.3143},
  pages = {43--56},
  issn = {00380938},
  doi = {10.1007/s11207-012-0048-z},
  abstract = {The dynamics of the solar radiative interior are still poorly constrained by comparison to the convective zone. This disparity is even more marked when we attempt to derive meaningful temporal variations. Many data sets contain a small number of modes that are sensitive to the inner layers of the Sun, but we found that the estimates of their uncertainties are often inaccurate. As a result, these data sets allow us to obtain, at best, a low-resolution estimate of the solar-core rotation rate down to approximately 0.2R {$\odot$}. We present inferences based on mode determination resulting from an alternate peak-fitting methodology aimed at increasing the amount of observed modes that are sensitive to the radiative zone, while special care was taken in the determination of their uncertainties. This methodology has been applied to MDI and GONG data, for the whole Solar Cycle 23, and to the newly available HMI data. The numerical inversions of all these data sets result in the best inferences to date of the rotation in the radiative region. These results and the method used to obtain them are discussed. The resulting profiles are shown and analyzed, and the significance of the detected changes is discussed. \textcopyright{} 2012 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {Helioseismology,Interior,Inverse modeling,notion,notion-database,Observations,Radiative zone},
  file = {/Users/lbugnet/Zotero/storage/ZD495KCE/Eff-Darwich, Korzennik - 2013.pdf}
}

@article{EffDarwich2008,
  title = {Analysis of the {{Sensitivity}} of {{Solar Rotation}} to {{Helioseismic Data}} from {{GONG}}, {{GOLF}}, and {{MDI Observations}}},
  author = {Eff-Darwich, A. and Korzennik, S. G. and Jim{\'e}nez-Reyes, S. J. and Garc{\'i}a, R. A.},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {679},
  number = {2},
  eprint = {0802.3604},
  pages = {1636--1643},
  issn = {0004-637X},
  doi = {10.1086/586724},
  abstract = {Accurate determination of the rotation rate in the radiative zone of the\textbackslash nSun from helioseismic observations requires rotational frequency\textbackslash nsplittings of exceptional quality as well as reliable inversion\textbackslash ntechniques. Here we present inferences based on mode parameters\textbackslash ncalculated from 2088 day MDI, GONG, and GOLF time series that were\textbackslash nfitted to estimate very low frequency rotational splittings (v {$<$} 1.7\textbackslash nmHz). These low-frequency modes provide data of exceptional quality,\textbackslash nsince the width of the mode peaks is much smaller than the rotational\textbackslash nsplitting, and hence it is much easier to separate the rotational\textbackslash nsplittings from the effects caused by the finite lifetime and the\textbackslash nstochastic excitation of the modes. We have also implemented a new\textbackslash ninversion methodology that allows us to infer the rotation rate of the\textbackslash nradiative interior from mode sets that span l = 1 to 25. Our results are\textbackslash ncompatible with the Sun rotating like a rigid solid in most of the\textbackslash nradiative zone, and slowing down in the core (r/R-circle dot {$<$} 0.2). A\textbackslash nresolution analysis of the inversion was carried out for the solar\textbackslash nrotation inverse problem. This analysis effectively establishes a direct\textbackslash nrelationship between the mode set included in the inversion and the\textbackslash nsensitivity and information content of the resulting inferences. We show\textbackslash nthat such an approach allows us to determine the effect of adding\textbackslash nlow-frequency and low-degree p-modes, high-frequency and low-degree\textbackslash np-modes, and some g-modes on the derived rotation rate in the solar\textbackslash nradiative zone, and in particular the solar core. We conclude that the\textbackslash nlevel of uncertainty that is needed to infer the dynamical conditions in\textbackslash nthe core when only p-modes are included is unlikely to be reached in the\textbackslash nnear future, and hence sustained efforts are needed toward the detection\textbackslash nand characterization of g-modes.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZQRFBX6R/Eff‐Darwich et al. - 2008.pdf}
}

@article{Egeland2015,
  title = {{{SUN-LIKE MAGNETIC CYCLES}} in the {{RAPIDLY ROTATING YOUNG SOLAR ANALOG HD}} 30495},
  author = {Egeland, Ricky and Metcalfe, Travis S. and Hall, Jeffrey C. and Henry, Gregory W.},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {812},
  number = {1},
  pages = {12},
  publisher = {{IOP Publishing}},
  issn = {15384357},
  doi = {10.1088/0004-637X/812/1/12},
  abstract = {A growing body of evidence suggests that multiple dynamo mechanisms can drive magnetic variability on different timescales, not only in the Sun but also in other stars. Many solar activity proxies exhibit a quasi-biennial ({$\sim$}2 year) variation, which is superimposed upon the dominant 11 year cycle. A well-characterized stellar sample suggests at least two different relationships between rotation period and cycle period, with some stars exhibiting long and short cycles simultaneously. Within this sample, the solar cycle periods are typical of a more rapidly rotating star, implying that the Sun might be in a transitional state or that it has an unusual evolutionary history. In this work, we present new and archival observations of dual magnetic cycles in the young solar analog HD 30495, a {$\sim$}1 Gyr old G1.5 V star with a rotation period near 11 days. This star falls squarely on the relationships established by the broader stellar sample, with short-period variations at {$\sim$}1.7 years and a long cycle of {$\sim$}12 years. We measure three individual long-period cycles and find durations ranging from 9.6 to 15.5 years. We find the short-term variability to be intermittent, but present throughout the majority of the time series, though its occurrence and amplitude are uncorrelated with the longer cycle. These essentially solar-like variations occur in a Sun-like star with more rapid rotation, though surface differential rotation measurements leave open the possibility of a solar equivalence.},
  keywords = {dynamo,notion,notion-database,stars: activity,stars: individual (HD 30495),stars: rotation,stars: solar-type Supporting material: machine-rea},
  file = {/Users/lbugnet/Zotero/storage/4LCFBVBC/Egeland et al. - 2015.pdf}
}

@article{Egeland2016,
  title = {Dynamo {{Sensitivity}} in {{Solar Analogs}} with 50 {{Years}} of {{Ca II H}} \& {{K Activity}}},
  author = {Egeland, Ricky and Soon, Willie and Baliunas, Sallie and Hall, Jeffrey C. and Pevtsov, Alexei A. and Henry, Gregory W.},
  year = {2016},
  eprint = {1609.04756},
  pages = {1--5},
  doi = {10.5281/zenodo.154118},
  abstract = {The Sun has a steady 11-year cycle in magnetic activity most well-known by the rising and falling in the occurrence of dark sunspots on the solar disk in visible bandpasses. The 11-year cycle is also manifest in the variations of emission in the Ca II H \& K line cores, due to non-thermal (i.e. magnetic) heating in the lower chromosphere. The large variation in Ca II H \& K emission allows for study of the patterns of long-term variability in other stars thanks to synoptic monitoring with the Mount Wilson Observatory HK photometers (1966-2003) and Lowell Observatory Solar-Stellar Spectrograph (1994-present). Overlapping measurements for a set of 27 nearby solar-analog (spectral types G0-G5) stars were used to calibrate the two instruments and construct time series of magnetic activity up to 50 years in length. Precise properties of fundamental importance to the dynamo are available from Hipparcos, the Geneva-Copenhagen Survey, and CHARA interferometry. Using these long time series and measurements of fundamental properties, we do a comparative study of stellar "twins" to explore the sensitivity of the stellar dynamo to small changes to structure, rotation, and composition. We also compare this sample to the Sun and find hints that the regular periodic variability of the solar cycle may be rare among its nearest neighbors in parameter space.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,Long,notion,notion-database,Solar Analogs,Solar and Stellar Astrophysics,Stellar Activity,Stellar Rotation,Sun,Term Variability,Zenodo community cs19},
  file = {/Users/lbugnet/Zotero/storage/8ZQJ6VSP/Egeland et al. - 2016.pdf}
}

@article{Egeland2017,
  title = {The {{Mount Wilson Observatory S}} -{{Index}} of the {{Sun}}},
  author = {Egeland, Ricky and Soon, Willie and Baliunas, Sallie and Hall, Jeffrey C. and Pevtsov, Alexei A. and Bertello, Luca},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {835},
  number = {1},
  eprint = {1611.04540},
  pages = {25},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/835/1/25},
  abstract = {The most commonly used index of stellar magnetic activity is the instrumental flux scale of singly-ionized calcium H \& K line core emission, S, developed by the Mount Wilson Observatory (MWO) HK Project, or the derivative index R'\_HK. Accurately placing the Sun on the S scale is important for comparing solar activity to that of the Sun-like stars. We present previously unpublished measurements of the reflected sunlight from the Moon using the second-generation MWO HK photometer during solar cycle 23 and determine cycle minimum S\_min,23 = 0.1634 +/- 0.0008, amplitude Delta S\_23 = 0.0143 +/- 0.0012, and mean {$<$}S\_23{$>$} = 0.1701 +/- 0.0005. By establishing a proxy relationship with the closely related National Solar Observatory Sacramento Peak calcium K emission index, itself well-correlated with the Kodaikanal Observatory plage index, we extend the MWO S time series to cover cycles 15-24 and find on average {$<$}S\_min{$>$} = 0.1621 +/- 0.0008, {$<$}Delta S\_cyc{$>$} = 0.0145 +/- 0.0012, {$<$}S\_cyc{$>$} = 0.1694 +/- 0.0005. Our measurements represent an improvement over previous estimates which relied on stellar measurements or solar proxies with non-overlapping time series. We find good agreement from these results with measurements by the Solar-Stellar Spectrograph at Lowell Observatory, an independently calibrated instrument, which gives us additional confidence that we have accurately placed the Sun on the S-index flux scale.},
  archiveprefix = {arxiv},
  keywords = {activity,chromosphere,machine-readable table,notion,notion-database,stars,stars: activity,sun,Sun: activity,Sun: chromosphere,supporting material},
  file = {/Users/lbugnet/Zotero/storage/DDUZ52Z4/Egeland et al. - 2017.pdf}
}

@article{Eggenberger2004,
  title = {Solar-like Oscillations in {{Procyon A}}},
  author = {Eggenberger, P. and Carrier, F. and Bouchy, F. and Blecha, A.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {422},
  number = {1},
  pages = {247--252},
  issn = {00046361},
  doi = {10.1051/0004-6361:20040148},
  abstract = {The F5 subgiant Procyon A ({$\alpha$}a CMi, HR 2943) was observed with the CORALIE fiber-fed echelle spectrograph on the 1.2-m Swiss telescope at La Silla in February 1999. The resulting 908 high-accuracy radial velocities exhibit a mean noise level in the amplitude spectrum of 0.11 ms-1 at high frequency. These measurements show significant excess in the power spectrum between 0.6-1.6 mHz with 0.60 m s-1 peak amplitude. An average large spacing of 55.5 {$\mu$}Hz has been determined and twenty-three individual frequencies have been identified.},
  keywords = {notion,notion-database,Stars: individual: {$\alpha$} Canis Minoris,Stars: oscillations,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/H8XFI3PK/Eggenberger et al. - 2004.pdf}
}

@article{Eggenberger2005,
  title = {Stellar {{Evolution}} with {{Rotation}} and {{Magnetic Fields IV}}: {{The Solar Rotation Profile}}},
  author = {Eggenberger, P. and Maeder, A. and Meynet, G.},
  year = {2005},
  month = aug,
  journal = {Astronomy \& Astrophysics},
  volume = {440},
  number = {1},
  eprint = {astro-ph/0508455},
  pages = {9--12},
  doi = {10.1051/0004-6361:200500156},
  urldate = {2020-07-13},
  abstract = {We examine the generation of a magnetic field in a solar-like star and its effects on the internal distribution of the angular velocity. We suggest that the evolution of a rotating star with magnetic fields leads to an equilibrium value of the differential rotation. This equilibrium is determined by the magnetic coupling, which favours a constant rotation profile, and meridional circulation which tends to build differential rotation. The global equilibrium stage is close to solid body rotation between about 0.7 and 0.2 R\_sun, in good agreement with helioseismic measurements.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: magnetic fields,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/LFVQSAJX/full-text.pdf}
}

@article{Eggenberger2008,
  title = {Modelling Solar-like Oscillators},
  author = {Eggenberger, P. and Carrier, F. and Mathis, S. and Miglio, A.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012021},
  abstract = {The computation of models of stars for which solar-like oscillations have been observed is discussed. After a brief intoduction on the observations of solar-like oscillations, the modelling of isolated stars and of stars belonging to a binary system is presented with specific examples of recent theoretical calibrations. Finally the input physics introduced in stellar evolution codes for the computation of solar-type stars is discussed with a peculiar emphasis on the modelling of rotation for these stars. \textcopyright{} 2008 IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UH55IZ3W/Eggenberger et al. - 2008.pdf}
}

@article{Eggenberger2008a,
  title = {The {{Geneva}} Stellar Evolution Code},
  author = {Eggenberger, P. and Meynet, G. and Maeder, A. and Hirschi, R. and Charbonnel, C. and Talon, S. and Ekstr{\"o}m, S.},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  pages = {43--54},
  issn = {0004640X},
  doi = {10.1007/s10509-007-9511-y},
  abstract = {This paper presents the Geneva stellar evolution code with special emphasis on the modeling of solar-type stars. The basic input physics used in the Geneva code as well as the modeling of atomic diffusion is first discussed. The physical description of rotation is then presented. Finally, the modeling of magnetic instabilities and transport of angular momentum by internal gravity waves is briefly summarized. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  keywords = {notion,notion-database,Stars: evolution},
  file = {/Users/lbugnet/Zotero/storage/A57CHS8H/Eggenberger et al. - 2008(2).pdf}
}

@article{Eggenberger2010,
  title = {Effects of Rotation and Magnetic Fields on the Lithium Abundance and Asteroseismic Properties of Exoplanet-Host Stars},
  author = {Eggenberger, P. and Maeder, A. and Meynet, G.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {519},
  number = {1},
  pages = {1--9},
  issn = {00046361},
  doi = {10.1051/0004-6361/201014939},
  abstract = {Context. Recent spectroscopic observations indicate lower lithium abundances of exoplanet-host stars compared to solar-type stars without detected exoplanets. Moreover, studies based on the distribution of rotational periods of solar-type stars suggest a possible link between lithium depletion and the rotational history of exoplanet-host stars. Aims. The effects of rotation and magnetic fields on the surface abundances of solar-type stars are studied in order to investigate whether the reported difference in lithium content of exoplanet-host stars can be related to their rotational history. Moreover, the asteroseismic properties predicted for stars with and without exoplanets are compared to determine how such a scenario, which relates the lithium abundances and the rotational history of the star, can be further challenged by observations of solar-like oscillations. Methods. Based on observations of rotational periods of solar-type stars, slow rotators on the zero age main sequence (ZAMS) are modelled with a comprehensive treatment of only the shellular rotation, while fast rotators are modelled including both shellular rotation and magnetic fields. Assuming a possible link between low rotation rates on the ZAMS and the presence of planets as a result of a longer disc-locking phase during the pre-main sequence (PMS), we compare the surface abundances and asteroseismic properties of slow and fast rotating models, which correspond to exoplanet-host stars and stars without detected planets, respectively. Results. We confirm previous suggestions that the difference in the lithium content of stars with and without detected planets can be related to their different rotational history. The larger efficiency of rotational mixing predicted in exoplanet-host stars explains their lithium depletion and also leads to changes in the structure and chemical composition of the central stellar layers. Asteroseismic observations can reveal these changes and can help us distinguish between different possible explanations for the lower lithium content of exoplanet-host stars. \textcopyright{} 2010 ESO.},
  keywords = {notion,notion-database,Stars: abundances,Stars: magnetic field,Stars: oscillations,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/YD5898W8/Eggenberger, Maeder, Meynet - 2010.pdf}
}

@article{Eggenberger2010a,
  title = {Effects of Rotational Mixing on the Asteroseismic Properties of Solar-Type Stars},
  author = {Eggenberger, P. and Meynet, G. and Maeder, A. and Miglio, A. and Montalban, J. and Carrier, F. and Mathis, S. and Charbonnel, C. and Talon, S.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {519},
  number = {13},
  eprint = {1009.4541},
  pages = {1--10},
  issn = {00046361},
  doi = {10.1051/0004-6361/201014713},
  abstract = {Context. Observations of solar-like oscillations obtained either from the ground or from space stimulated the study of the effects of various physical processes on the modelling of solar-type stars. Aims. The influence of rotational mixing on the evolution and asteroseismic properties of solar-type stars is studied. Methods. Global and asteroseismic properties of models of solar-type stars computed with and without a comprehensive treatment of shellular rotation are compared. The effects of internal magnetic fields are also discussed in the framework of the Tayler-Spruit dynamo. Results. Rotational mixing changes the global properties of a solar-type star with a significant increase of the effective temperature resulting in a shift of the evolutionary track to the blue part of the HR diagram. These differences observed in the HR diagram are related to changes of the chemical composition, because rotational mixing counteracts the effects of atomic diffusion leading to larger helium surface abundances for rotating models than for non-rotating ones. Higher values of the large frequency separation are then found for rotating models than for non-rotating ones at the same evolutionary stage, because the increase of the effective temperature leads to a smaller radius and hence to an increase of the stellar mean density. In addition to changing the global properties of solar-type stars, rotational mixing also has a considerable impact on the structure and chemical composition of the central stellar layers by bringing fresh hydrogen fuel to the central stellar core, thereby enhancing the main-sequence lifetime. The increase of the central hydrogen abundance together with the change of the chemical profiles in the central layers result in a significant increase of the values of the small frequency separations and of the ratio of the small to large separations for models including shellular rotation. This increase is clearly seen for models with the same age sharing the same initial parameters except for the inclusion of rotation as well as for models with the same global stellar parameters and in particular the same location in the HR diagram. By computing rotating models of solar-type stars including the effects of a dynamo that possibly occurs in the radiative zone, we find that the efficiency of rotational mixing is strongly reduced when the effects of magnetic fields are taken into account, in contrast to what happens in massive stars. \textcopyright{} ESO, 2010.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: interiors,Stars: magnetic field,Stars: oscillations,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/FQB47MQU/Eggenberger et al. - 2010.pdf}
}

@article{Eggenberger2012,
  title = {Impact of Rotation and Disc Lifetime on Pre-Main Sequence Lithium Depletion of Solar-Type Stars},
  author = {Eggenberger, P. and Haemmerl{\'e}, L. and Meynet, G. and Maeder, A.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {539},
  pages = {1--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201118432},
  abstract = {Aims. We study the influence of rotation and disc lifetime on lithium depletion of pre-main sequence (PMS) solar-type stars. Methods. The impact of rotational mixing and of the hydrostatic effects of rotation on lithium abundances are investigated by computing non-rotating and rotating PMS models that include a comprehensive treatment of shellular rotation. The influence of the disc lifetime is then studied by comparing the lithium content of PMS rotating models experiencing different durations of the disc-locking phase between 3 and 9Myr. Results. The surface lithium abundance at the end of the PMS is decreased when rotational effects are included. During the beginning of the lithium depletion phase, only hydrostatic effects of rotation are at work. This results in a decrease in the lithium depletion rate for rotating models compared to non-rotating ones. When the convective envelope recedes from the stellar centre, rotational mixing begins to play an important role due to differential rotation near the bottom of the convective envelope. This mixing results in a decrease in the surface lithium abundance with a limited contribution from hydrostatic effects of rotation, which favours lithium depletion during the second part of the PMS evolution. The impact of rotation on PMS lithium depletion is also found to be sensitive to the duration of the disc-locking phase. When the disc lifetime increases, the PMS lithium abundance of a solar-type star decreases owing to the higher efficiency of rotational mixing in the radiative zone. A relationship between the surface rotation and lithium abundance at the end of the PMS is then obtained: slow rotators on the zero-age main sequence are predicted to be more lithium-depleted than fast rotators due to the increase in the disc lifetime. \textcopyright{} ESO, 2012.},
  keywords = {notion,notion-database,Stars: abundances,Stars: pre-main sequence,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/E36L5268/Eggenberger et al. - 2012.pdf}
}

@article{Eggenberger2012abis,
  title = {Angular Momentum Transport in Stellar Interiors Constrained by Rotational Splittings of Mixed Modes in Red Giants},
  author = {Eggenberger, P. and Montalb{\'a}n, J. and Miglio, A.},
  year = {2012},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {544},
  eprint = {1207.1023},
  doi = {10.1051/0004-6361/201219729},
  urldate = {2020-03-08},
  abstract = {Context: Recent asteroseismic observations have led to the determination of rotational frequency splittings for l=1 mixed modes in red giants. Aims: We investigate how these observed splittings can constrain the modelling of the physical processes transporting angular momentum in stellar interiors. Methods: We first compare models including a comprehensive treatment of shellular rotation only, with the rotational splittings observed for the red giant KIC 8366239. We then study how these asteroseismic constraints can give us information about the efficiency of an additional mechanism for the internal transport of angular momentum. This is done by computing rotating models of KIC 8366239 that include a constant viscosity corresponding to this physical process, in addition to the treatment of shellular rotation. Results: We find that models of red giant stars including shellular rotation only predict steep rotation profiles, which are incompatible with the measurements of rotational splittings in the red giant KIC 8366239. Meridional circulation and shear mixing alone are found to produce an insufficient internal coupling so that an additional mechanism for the internal transport of angular momentum is needed during the post-main sequence evolution. We show that the viscosity nu\_add corresponding to this mechanism is strongly constrained to be nu\_add=3x10\^4 cm\^2 s\^-1 thanks to the observed ratio of the splittings for modes in the wings to those at the centre of the dipole forests. Such a value of viscosity may suggest that the same unknown physical process is at work during the main sequence and the post-main sequence evolution.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G33RCMW3/full-text.pdf}
}

@article{Eggenberger2015,
  title = {Effects of Rotation on Stellar Evolution and Asteroseismology of Red Giants},
  author = {Eggenberger, Patrick},
  year = {2015},
  journal = {Astrophysics and Space Science Proceedings},
  volume = {39},
  pages = {33--41},
  issn = {15706605},
  doi = {10.1007/978-3-319-10993-0_4},
  abstract = {The impact of rotation on the properties of low-mass stars at different evolutionary stages is first described by discussing the properties of stellar models computed with shellular rotation. The observational constraints that are currently available to progress in our understanding of these dynamical processes are then presented, with a peculiar focus on asteroseismic measurements of red-giant stars.},
  isbn = {9783319109923},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LCEPVJEF/Eggenberger - 2015.pdf}
}

@article{Eggenberger2017bis,
  title = {Constraining the Efficiency of Angular Momentum Transport with Asteroseismology of Red Giants: {{The}} Effect of Stellar Mass},
  author = {Eggenberger, P. and Lagarde, N. and Miglio, A. and Montalb{\'a}n, J. and Ekstr{\"o}m, S. and Georgy, C. and Meynet, G. and Salmon, S. and Ceillier, T. and Garci{\'a}, R. A. and Mathis, S. and Deheuvels, S. and Maeder, A. and Den Hartogh, J. W. and Hirschi, R.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {599},
  pages = {1--12},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629459},
  abstract = {Context. Constraints on the internal rotation of red giants are now available thanks to asteroseismic observations. Preliminary comparisons with rotating stellar models indicate that an undetermined additional process for the internal transport of angular momentum is required in addition to purely hydrodynamic processes. Aims. We investigate how asteroseismic measurements of red giants can help us characterize the additional transport mechanism. Methods. We first determine the efficiency of the missing transport mechanism for the low-mass red giant KIC 7341231 by computing rotating models that include an additional viscosity corresponding to this process. We then discuss the change in the efficiency of this transport of angular momentum with the mass, metallicity, and evolutionary stage in the light of the corresponding viscosity determined for the more massive red giant KIC 8366239. Results. In the case of the low-mass red giant KIC 7341231, we find that the viscosity corresponding to the additional mechanism is constrained to the range {$\nu$}add = 1 \texttimes{} 103-1.3 \texttimes{} 104 cm2 s-1. This constraint on the efficiency of the unknown additional transport mechanism during the post-main sequence is obtained independently of any specific assumption about the modeling of rotational effects during the pre-main sequence and the main sequence (in particular, the braking of the surface by magnetized winds and the efficiency of the internal transport of angular momentum before the post-main-sequence phase). When we assume that the additional transport mechanism is at work during the whole evolution of the star together with a solar-calibrated braking of the surface by magnetized winds, the range of {$\nu$}add is reduced to 1-4 \texttimes{} 103 cm2 s-1. In addition to being sensitive to the evolutionary stage of the star, the efficiency of the unknown process for internal transport of angular momentum increases with the stellar mass.},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/N7A8NSV8/Eggenberger et al. - 2017.pdf}
}

@article{Eggenberger2019a,
  title = {Rotation Rate of the Solar Core as a Key Constraint to Magnetic Angular Momentum Transport in Stellar Interiors},
  author = {Eggenberger, P. and Buldgen, G. and Salmon, S. J. A. J.},
  year = {2019},
  journal = {Astronomy \& Astrophysics},
  volume = {626},
  number = {1998},
  eprint = {1911.06343},
  pages = {L1},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201935509},
  abstract = {Context . The internal rotation of the Sun constitutes a fundamental constraint when modelling angular momentum transport in stellar interiors. In addition to the more external regions of the solar radiative zone probed by pressure modes, measurements of rotational splittings of gravity modes would offer an invaluable constraint on the rotation of the solar core.  Aims . We study the constraints that a measurement of the core rotation rate of the Sun could bring on magnetic angular momentum transport in stellar radiative zones.  Methods . Solar models accounting for angular momentum transport by hydrodynamic and magnetic instabilities were computed for different initial velocities and disc lifetimes on the pre-main sequence to reproduce the surface rotation velocities observed for solar-type stars in open clusters. The internal rotation of these solar models was then compared to helioseismic measurements.  Results . We first show that models computed with angular momentum transport by magnetic instabilities and a recent prescription for the braking of the stellar surface by magnetized winds can reproduce the observations of surface velocities of stars in open clusters. These solar models predict both a flat rotation profile in the external part of the solar radiative zone probed by pressure modes and an increase in the rotation rate in the solar core, where the stabilizing effect of chemical gradients plays a key role. A rapid rotation of the core of the Sun, as suggested by reported detections of gravity modes, is thus found to be compatible with angular momentum transport by magnetic instabilities. Moreover, we show that the efficiency of magnetic angular momentum transport in regions of strong chemical gradients can be calibrated by the solar core rotation rate independently from the unknown rotational history of the Sun. In particular, we find that a recent revised prescription for the transport of angular momentum by the Tayler instability can be easily distinguished from the original Tayler\textendash Spruit dynamo, with a faster rotating solar core supporting the original prescription.  Conclusions . By calibrating the efficiency of magnetic angular momentum transport in regions of strong chemical gradients, a determination of the solar core rotation rate through gravity modes is of prime relevance not only for the Sun, but for stars in general, since radial differential rotation precisely develops in these regions during the more advanced stages of evolution.},
  archiveprefix = {arxiv},
  keywords = {interiors,magnetic field,notion,notion-database,oscillations,rotation,stars,sun},
  file = {/Users/lbugnet/Zotero/storage/9RDENQIH/Eggenberger, Buldgen, Salmon - 2019.pdf}
}

@article{Eggenberger2019b,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum},
  author = {Eggenberger, P. and Deheuvels, S. and Miglio, A. and Ekstr{\"o}m, S. and Georgy, C. and Meynet, G. and Lagarde, N. and Salmon, S. and Buldgen, G. and Montalb{\'a}n, J. and Spada, F. and Ballot, J.},
  year = {2019},
  journal = {Astronomy \& Astrophysics},
  volume = {621},
  pages = {A66},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201833447},
  abstract = {Context. The observations of solar-like oscillations in evolved stars have brought important constraints on their internal rotation rates. To correctly reproduce these data, an efficient transport mechanism is needed in addition to the transport of angular momentum by meridional circulation and shear instability. The efficiency of this undetermined process is found to increase both with the mass and the evolutionary stage during the red giant phase.Aims. We study the efficiency of the transport of angular momentum during the subgiant phase.Methods. The efficiency of the unknown transport mechanism is determined during the subgiant phase by comparing rotating models computed with an additional corresponding viscosity to the asteroseismic measurements of both core and surface-rotation rates for six subgiants observed by the Kepler spacecraft. We then investigate the change in the efficiency of this transport of angular momentum with stellar mass and evolution during the subgiant phase.Results. The precise asteroseismic measurements of both core and surface-rotation rates available for the six Kepler targets enable a precise determination of the efficiency of the transport of angular momentum needed for each of these subgiants. These results are found to be insensitive to all the uncertainties related to the modelling of rotational effects before the post-main sequence (poMS) phase. An interesting exception in this context is the case of young subgiants (typical values of log(g) close to 4), because their rotational properties are sensitive to the degree of radial differential rotation on the main sequence (MS). These young subgiants constitute therefore perfect targets to constrain the transport of angular momentum on the MS from asteroseismic observations of evolved stars. As for red giants, we find that the efficiency of the additional transport process increases with the mass of the star during the subgiant phase. However, the efficiency of this undetermined mechanism decreases with evolution during the subgiant phase, contrary to what is found for red giants. Consequently, a transport process with an efficiency that increases with the degree of radial differential rotation cannot account for the core-rotation rates of subgiants, while it correctly reproduces the rotation rates of red giant stars. This suggests that the physical nature of the additional mechanism needed for the internal transport of angular momentum may be different in subgiant and red giant stars.},
  keywords = {interiors,notion,notion-database,oscillations,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/4ATPE6HH/Eggenberger et al. - 2019.pdf}
}

@article{Eggenberger2020,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum {{II}}. {{Test}} of a Revised Prescription for Transport by the {{Tayler}} Instability},
  author = {Eggenberger, P. and den Hartogh, J. W. and Buldgen, G. and Meynet, G. and Salmon, S. J. A. J. and Deheuvels, S.},
  year = {2019},
  month = jan,
  journal = {Astronomy and Astrophysics},
  volume = {631},
  number = {L6},
  eprint = {2001.11525},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201936348},
  urldate = {2020-07-17},
  abstract = {Context: Asteroseismic measurements reveal that an unknown efficient angular momentum (AM) transport mechanism is needed for subgiant and red giant stars. A revised prescription for AM transport by the magnetic Tayler instability has been recently proposed as a possible candidate for such a missing mechanism. Results: The revised prescription for the transport by the Tayler instability leads to low core rotation rates after the main sequence that are in better global agreement with asteroseismic measurements than those predicted by models with purely hydrodynamic processes or with the original Tayler-Spruit dynamo. A detailed comparison with asteroseismic data shows that the rotational properties of at most two of the six subgiants can be correctly reproduced by models accounting for this revised magnetic transport process. This result is obtained independently of the value adopted for the calibration parameter in this prescription. We also find that this transport by the Tayler instability faces difficulties in simultaneously reproducing asteroseismic measurements available for subgiant and red giant stars. The low values of the calibration parameter needed to correctly reproduce the rotational properties of two of the six subgiants lead to core rotation rates during the red giant phase that are too high. Inversely, the higher values of this parameter needed to reproduce the core rotation rates of red giants lead to a very low degree of radial differential rotation before the red giant phase, which is in contradiction with the internal rotation of subgiant stars. Conclusions: In its present form, the revised prescription for the transport by the Tayler instability does not provide a complete solution to the missing AM transport revealed by asteroseismology of evolved stars.},
  archiveprefix = {arxiv},
  keywords = {interiors,magnetic field-Stars,notion,notion-database,oscillations-Stars,rotation-Stars,Stars},
  file = {/Users/lbugnet/Zotero/storage/7F9ZRP56/full-text.pdf}
}

@article{Eggenberger2021,
  title = {Grids of Stellar Models with Rotation. {{VI}}. {{Models}} from 0.8 to 120 {{M}}{$\odot$} at a Metallicity {{Z}} = 0.006},
  author = {Eggenberger, Patrick and Ekstr{\"o}m, Sylvia and Georgy, Cyril and Martinet, S{\'e}bastien and Pezzotti, Camilla and Nandal, Devesh and Meynet, Georges and Buldgen, Ga{\"e}l and Salmon, S{\'e}bastien and Haemmerl{\'e}, Lionel and Maeder, Andr{\'e} and Hirschi, Raphael and Yusof, Norhasliza and Groh, Jos{\'e} and Farrell, Eoin and Murphy, Laura and Choplin, Arthur},
  year = {2021},
  month = aug,
  journal = {Astronomy \& Astrophysics},
  volume = {652},
  pages = {A137},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202141222},
  urldate = {2023-10-18},
  abstract = {Context. Grids of stellar models, computed with the same physical ingredients, allow one to study the impact of a given physics on a broad range of initial conditions and they are a key ingredient for modeling the evolution of galaxies. Aims: We present here a grid of single star models for masses between 0.8 and 120 M{$\odot$}, with and without rotation for a mass fraction of heavy element Z = 0.006, representative of the Large Magellanic Cloud (LMC). Methods: We used the GENeva stellar Evolution Code. The evolution was computed until the end of the central carbon-burning phase, the early asymptotic giant branch phase, or the core helium-flash for massive, intermediate, and low mass stars, respectively. Results: The outputs of the present stellar models are well framed by the outputs of the two grids obtained by our group for metallicities above and below the one considered here. The models of the present work provide a good fit to the nitrogen surface enrichments observed during the main sequence for stars in the LMC with initial masses around 15 M{$\odot$}. They also reproduce the slope of the luminosity function of red supergiants of the LMC well, which is a feature that is sensitive to the time-averaged mass loss rate over the red supergiant phase. The most massive black hole that can be formed from the present models at Z = 0.006 is around 55 M{$\odot$}. No model in the range of mass considered will enter into the pair-instability supernova regime, while the minimal mass to enter the region of pair pulsation instability is around 60 M{$\odot$} for the rotating models and 85 M{$\odot$} for the nonrotating ones. Conclusions: The present models are of particular interest for comparisons with observations in the LMC and also in the outer regions of the Milky Way. We provide public access to numerical tables that can be used for computing interpolated tracks and for population synthesis studies. The numerical data of the present grid are directly accessible on the web page at https://www.unige.ch/sciences/astro/evolution/fr/base-de-donnees/.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,stars: abundances,stars: evolution,stars: rotation},
  annotation = {ADS Bibcode: 2021A\&A...652A.137E},
  file = {/Users/lbugnet/Zotero/storage/B8KVKNGZ/Eggenberger et al. - 2021 - Grids of stellar models with rotation. VI. Models .pdf}
}

@article{Eggenberger2022,
  title = {Rotation in Stellar Interiors: {{General}} Formulation and an Asteroseismic-Calibrated Transport by the {{Tayler}} Instability},
  shorttitle = {Rotation in Stellar Interiors},
  author = {Eggenberger, P. and Moyano, F. D. and {den Hartogh}, J. W.},
  year = {2022},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {664},
  pages = {L16},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202243781},
  urldate = {2023-10-11},
  abstract = {Context. Asteroseismic measurements of the internal rotation of evolved stars indicate that at least one unknown efficient angular momentum (AM) transport mechanism is needed in stellar radiative zones in addition to hydrodynamic transport processes. Aims: We investigate the impact of AM transport by the magnetic Tayler instability as a possible candidate for such a missing physical mechanism. Methods: We derived general equations for AM transport by the Tayler instability to be able to test different versions of the Tayler-Spruit (TS) dynamo by comparing rotational properties of these models with asteroseismic constraints available for sub-giant and red giant stars. Results: These general equations highlight, in a simple way, the key role played by the adopted damping timescale of the azimuthal magnetic field on the efficiency of the resulting AM transport. Using this framework, we first show that the original TS dynamo provides an insufficient coupling in low-mass red giants that have a radiative core during the main sequence (MS), as was found previously for more massive stars that develop a convective core during the MS. We find that the core rotation rates of red giant branch (RGB) stars predicted by models computed with various prescriptions for the TS dynamo are nearly insensitive to the adopted initial rotation velocity. We then derived a new calibrated version of the original TS dynamo and find that the damping timescale adopted for the azimuthal field in the original TS dynamo has to be increased by a factor of about 200 to correctly reproduce the core rotation rates of stars on the RGB. This calibrated version predicts no correlation of the core rotation rates with the stellar mass for RGB stars in good agreement with asteroseismic observations. Moreover, it correctly reproduces the core rotation rates of clump stars similarly to a revised prescription proposed recently. Interestingly, this new calibrated version of the TS dynamo is found to be in slightly better agreement with the core rotation rates of sub-giant stars, while simultaneously better accounting for the evolution of the core rotation rates along the RGB compared to the revised dynamo version. These results were obtained with both the Geneva and the MESA stellar evolution codes.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: interiors,stars: magnetic field,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2022A\&A...664L..16E},
  file = {/Users/lbugnet/Zotero/storage/8EVCVEFL/Eggenberger et al. - 2022 - Rotation in stellar interiors General formulation.pdf}
}

@article{Ellien2021,
  title = {{{DAWIS}}: {{A}} Detection Algorithm with Wavelets for Intracluster Light Studies},
  author = {Ellien, A. and Slezak, E. and Martinet, N. and Durret, F. and Adami, C. and Gavazzi, R. and Raba{\c c}a, C. R. and Da Rocha, C. and Epit{\'a}cio Pereira, D. N.},
  year = {2021},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {649},
  eprint = {2101.03835},
  pages = {A38},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/202038419},
  urldate = {2022-01-08},
  abstract = {Context. Large numbers of deep optical images will be available in the near future, allowing statistically significant studies of low surface brightness structures such as intracluster light (ICL) in galaxy clusters. The detection of these structures requires efficient algorithms dedicated to this task, which traditional methods find difficult to solve. Aims. We present our new detection algorithm with wavelets for intracluster light studies (DAWIS), which we developed and optimized for the detection of low surface brightness sources in images, in particular (but not limited to) ICL. Methods. DAWIS follows a multiresolution vision based on wavelet representation to detect sources. It is embedded in an iterative procedure called synthesis-by-analysis approach to restore the unmasked light distribution of these sources with very good quality. The algorithm is built so that sources can be classified based on criteria depending on the analysis goal. We present the case of ICL detection and the measurement of ICL fractions. We test the efficiency of DAWIS on 270 mock images of galaxy clusters with various ICL profiles and compare its efficiency to more traditional ICL detection methods such as the surface brightness threshold method. We also run DAWIS on a real galaxy cluster image, and compare the output to results obtained with previous multiscale analysis algorithms. Results. We find in simulations that DAWIS is on average able to separate galaxy light from ICL more efficiently, and to detect a greater quantity of ICL flux because of the way sky background noise is treated. We also show that the ICL fraction, a metric used on a regular basis to characterize ICL, is subject to several measurement biases on galaxies and ICL fluxes. In the real galaxy cluster image, DAWIS detects a faint and extended source with an absolute magnitude two orders brighter than previous multiscale methods.},
  archiveprefix = {arxiv},
  keywords = {Galaxies: clusters: general,Methods: data analysis,notion,notion-database,Techniques: image processing},
  file = {/Users/lbugnet/Zotero/storage/8NL5PC37/full-text.pdf;/Users/lbugnet/Zotero/storage/Q7GTFYVG/abstract.html}
}

@article{ellienComplexCaseMACS2019,
  title = {The Complex Case of {{MACS J0717}}.5+3745 and Its Extended Filament: Intra-Cluster Light, Galaxy Luminosity Function, and Galaxy Orientations},
  shorttitle = {The Complex Case of {{MACS J0717}}.5+3745 and Its Extended Filament},
  author = {Ellien, A. and Durret, F. and Adami, C. and Martinet, N. and Lobo, C. and Jauzac, M.},
  year = {2019},
  month = aug,
  journal = {Astronomy \&amp; Astrophysics, Volume 628, id.A34, {$<$}NUMPAGES{$>$}18{$<$}/NUMPAGES{$>$} pp.},
  volume = {628},
  pages = {A34},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201935673},
  urldate = {2022-07-18},
  abstract = {Context. The properties of galaxies are known to be affected by their environment, but although galaxies in clusters and groups have been quite thoroughly investigated, little is known about galaxies belonging to filaments of the cosmic web, or about the properties of the filaments themselves. {$<$}BR /{$>$} Aims: Here we investigate the properties of the rich cluster MACS J0717.5+3745 and its extended filament by analyzing the distribution and fractions of intra-cluster light (ICL) in its core and by trying to detect intra-filament light (IFL) in the filament. We analyze the galaxy luminosity function (GLF) of the cluster core and of the filament. We also study the orientations of galaxies in the filament to better constrain the filament properties. {$<$}BR /{$>$} Methods: This work is based on Hubble Space Telescope (HST) archive data, both from the Hubble Frontier Fields in the F435W, F606W, F814W, and F105W bands, and from a mosaic of images in the F606W and F814W bands. The spatial distribution of the ICL was determined with our new wavelet-based software, DAWIS. The GLFs were extracted in the F606W and F814W bands, with a statistical subtraction of the background, and fit with Schechter functions. The galaxy orientations in the filaments were estimated with SExtractor after correction for the point spread function. {$<$}BR /{$>$} Results: We detect a large amount of ICL in the cluster core, but no IFL in the cosmic filament. The fraction of ICL in the core peaks in the F606W filter before decreasing with wavelength. Though relatively noisy, the GLFs in the filament are notably different from those of field galaxies, with a flatter faint end slope and an excess of bright galaxies. We do not detect a significant alignment of the galaxies in the filament region analyzed.},
  langid = {english},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5DC3BHC7/Ellien et al. - 2019 - The complex case of MACS J0717.5+3745 and its exte.pdf;/Users/lbugnet/Zotero/storage/TS9HH2MP/abstract.html}
}

@article{Elsworth1990,
  title = {Evidence from Solar Seismology against Non-Standard Solar-Core Models},
  author = {Elsworth, Y. and Howe, R. and Isaak, G. R. and McLeod, C. P. and New, R.},
  year = {1990},
  journal = {Nature},
  volume = {347},
  number = {6293},
  pages = {536--539},
  issn = {00280836},
  doi = {10.1038/347536a0},
  abstract = {GLOBAL oscillations of the Sun1 have been used to test solar models2, but modelling the oscillation frequencies to their measured accuracies of a few microhertz has proved difficult, mostly owing to ignorance of the structure of the Sun's outer layers3. The frequency separation between closely spaced modes in the acoustic spectrum is expected to depend more on core properties4, however, and thus to provide constraints on models of the solar core. Our observations combine data from a global network of observing stations, which reduces the masking effect of daily sidebands in the spectral analysis. Here we present precision measurements of fine structure and its variation with frequency. Our results agree with standard solar models5-7, and seem to remove the need for significant mixing8,9 or weakly interacting massive particles (WIMPS)10,11 in the core, both of which have been advanced to explain the low measured flux of solar neutrinos12,13. This suggests that the solar neutrino problem must be resolved within neutrino physics, not solar physics; neutrino oscillations and a finite neutrino mass form a possible explanation. \textcopyright{} 1990 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6BAAZ37C/Elsworth et al. - 1990.pdf}
}

@article{Elsworth1995,
  title = {Slow Rotation of the Sun's Interior},
  author = {Elsworth, Y. and Howe, R. and Isaak, G. R. and McLeod, C. P. and Miller, B. A. and New, R. and Wheeler, S. J. and Gough, D. O.},
  year = {1995},
  journal = {Nature},
  volume = {376},
  number = {6542},
  pages = {669--672},
  issn = {00280836},
  doi = {10.1038/376669a0},
  abstract = {THE rotation of the Sun is not that of a rigid body; at its surface, the gas near the poles has a lower angular velocity than that near the equator1. This latitudinal variation persists to the base of the convection zone, below which the angular velocity becomes approximately uniform2,3. Any variations of angular velocity at much greater depths are. however, poorly constrained4-10. Obser-vations of solar oscillation modes have been used to probe densityvariations in the Sun; rotational splitting of degenerate modes, although difficult to resolve, provides important constraints on the dynamical structure11. Here we report observations of rotationallysplit modes made over a three-year period with the Birmingham Solar Oscillations Network. Our results indicate that there is a substantial region inside the Sun that is rotating more slowly thanthe surface. This situation seems likely to be transient-the mini-mum-energy state would have all the deeper regions rotating with the same angular velocity-and is at variance with our currentideas about the rotational evolution of main-sequence stars12. Wehave no solution to he dynamical problem this poses. \textcopyright{} 1995, Nature Publishing Group. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DKGZ4B2H/Elsworth et al. - 1995.pdf}
}

@article{Elsworth2004,
  title = {Asteroseismology of {{Sun-like}} Stars},
  author = {Elsworth, Yvonne P. and Thompson, Michael J.},
  year = {2004},
  journal = {Astronomy and Geophysics},
  volume = {45},
  number = {5},
  issn = {13668781},
  doi = {10.1046/j.1468-4004.2003.45514.x},
  abstract = {Seismology has become a powerful tool for analysis of the interior of the Sun; it has great potential for the study of oscillations in solar-like stars. Asteroseimology could provide direct information about detailed properties of stellar interiors, bringing the potential for testing theories of stellar evolution and structure. Current stellar models are simple with few direct observational constraints; consequences such as age estimates are uncertain to a factor of two. A recent attempt at asteroseismology on Procyon, a likely candidate star, found no detectable oscillations. In this paper we discuss the asteroseismology of solar-like stars in the context of studies of the Sun and then indicate possible reasons for the Procyon results.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G8T3D5RH/Elsworth, Thompson - 2004.pdf}
}

@book{Elsworth2015,
  title = {The {{Importance}} of {{Long-Term Synoptic Observations}} and {{Data Sets}} for {{Solar Physics}} and {{Helioseismology}}},
  author = {Elsworth, Yvonne and Broomhall, Anne Marie and Gosain, Sanjay and Roth, Markus and Jefferies, Stuart M. and Hill, Frank},
  year = {2015},
  month = dec,
  journal = {Space Science Reviews},
  volume = {196},
  publisher = {{Springer Netherlands}},
  issn = {15729672},
  doi = {10.1007/s11214-015-0212-5},
  urldate = {2020-03-08},
  abstract = {A casual single glance at the Sun would not lead an observer to conclude that it varies. The discovery of the 11-year sunspot cycle was only made possible through systematic daily observations of the Sun over 150 years and even today historic sunspot drawings are used to study the behavior of past solar cycles. The origin of solar activity is still poorly understood as shown by the number of different models that give widely different predictions for the strength and timing of future cycles. Our understanding of the rapid transient phenomena related to solar activity, such as flares and coronal mass ejections (CMEs) is also insufficient and making reliable predictions of these events, which can adversely impact technology, remains elusive. There is thus still much to learn about the Sun and its activity that requires observations over many solar cycles. In particular, modern helioseismic observations of the solar interior currently span only 1.5 cycles, which is far too short to adequately sample the characteristics of the plasma flows that govern the dynamo mechanism underlying solar activity. In this paper, we review some of the long-term solar and helioseismic observations and outline some future directions.},
  keywords = {Helioseismology,notion,notion-database,Observations,Sun}
}

@article{Elsworth2017,
  title = {A New Method for the Asteroseismic Determination of the Evolutionary State of Red-Giant Stars},
  author = {Elsworth, Yvonne and Hekker, Saskia and Basu, Sarbani and Davies, Guy R.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {466},
  number = {3},
  eprint = {1612.04751},
  pages = {3344--3352},
  issn = {13652966},
  doi = {10.1093/mnras/stw3288},
  abstract = {Determining the ages of red-giant stars is a key problem in stellar astrophysics. One of the difficulties in this determination is to know the evolutionary state of the individual stars - i.e. have they started to burn Helium in their cores? That is the topic of this paper. Asteroseismic data provide a route to achieving this information. What we present here is a highly autonomous way of determining the evolutionary state from an analysis of the power spectrum of the light curve. The method is fast and efficient and can provide results for a large number of stars. It uses the structure of the dipole-mode oscillations, which have a mixed character in red-giant stars, to determine some measures that are used in the categorization. It does not require that all the individual components of any given mode be separately characterized. Some 6604 redgiant stars have been classified. Of these, 3566 are determined to be on the red-giant branch, 2077 are red-clump and 439 are secondary-clump stars. We do not specifically identify the low-metallicity, horizontal-branch stars. The difference between red-clump and secondaryclump stars is dependent on the manner in which Helium burning is first initiated. We discuss that the way the boundary between these classifications is set may lead to mis-categorization in a small number of stars. The remaining 522 stars were not classified either because they lacked sufficient power in the dipole modes (so-called depressed dipole modes) or because of conflicting values in the parameters.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: low-mass,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/EMIV6RVG/Elsworth et al. - 2017.pdf}
}

@article{Emeriau-Viard2017,
  title = {Origin and Evolution of Magnetic Fields in {{PMS}} Stars : Influence of Rotation and Structural Changes},
  author = {{Emeriau-Viard}, Constance and Brun, Allan Sacha},
  year = {2017},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {846},
  number = {1},
  eprint = {1709.04667},
  doi = {10.3847/1538-4357/aa7b33},
  urldate = {2020-06-19},
  abstract = {During stellar evolution, especially in the PMS, stellar structure and rotation evolve significantly causing major changes in the dynamics and global flows of the star. We wish to assess the consequences of these changes on stellar dynamo, internal magnetic field topology and activity level. To do so, we have performed a series of 3D HD and MHD simulations with the ASH code. We choose five different models characterized by the radius of their radiative zone following an evolutionary track computed by a 1D stellar evolution code. These models characterized stellar evolution from 1 Myr to 50 Myr. By introducing a seed magnetic field in the fully convective model and spreading its evolved state through all four remaining cases, we observe systematic variations in the dynamical properties and magnetic field amplitude and topology of the models. The five MHD simulations develop strong dynamo field that can reach equipartition state between the kinetic and magnetic energy and even super- equipartition levels in the faster rotating cases. We find that the magnetic field amplitude increases as it evolves toward the ZAMS. Moreover the magnetic field topology becomes more complex, with a decreasing axisymmetric component and a non-axisymmetric one becoming predominant. The dipolar components decrease as the rotation rate and the size of the radiative core increase. The magnetic fields possess a mixed poloidal-toroidal topology with no obvious dominant component. Moreover the relaxation of the vestige dynamo magnetic field within the radiative core is found to satisfy MHD stability criteria. Hence it does not experience a global reconfiguration but slowly relaxes by retaining its mixed stable poloidal-toroidal topology.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3MM5I4EV/full-text.pdf}
}

@article{Emeriau-Viard2017a,
  title = {Origin and {{Evolution}} of {{Magnetic Field}} in {{PMS Stars}}: {{Influence}} of {{Rotation}} and {{Structural Changes}}},
  shorttitle = {Origin and {{Evolution}} of {{Magnetic Field}} in {{PMS Stars}}},
  author = {{Emeriau-Viard}, Constance and Brun, Allan Sacha},
  year = {2017},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {846},
  pages = {8},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/aa7b33},
  urldate = {2023-10-11},
  abstract = {During stellar evolution, especially in the pre-main-sequence phase, stellar structure and rotation evolve significantly, causing major changes in the dynamics and global flows of the star. We wish to assess the consequences of these changes on stellar dynamo, internal magnetic field topology, and activity level. To do so, we have performed a series of 3D HD and MHD simulations with the ASH code. We choose five different models characterized by the radius of their radiative zone following an evolutionary track computed by a 1D stellar evolution code. These models characterized stellar evolution from 1 to 50 Myr. By introducing a seed magnetic field in the fully convective model and spreading its evolved state through all four remaining cases, we observe systematic variations in the dynamical properties and magnetic field amplitude and topology of the models. The five MHD simulations develop a strong dynamo field that can reach an equipartition state between the kinetic and magnetic energies and even superequipartition levels in the faster-rotating cases. We find that the magnetic field amplitude increases as it evolves toward the zero-age main sequence. Moreover, the magnetic field topology becomes more complex, with a decreasing axisymmetric component and a nonaxisymmetric one becoming predominant. The dipolar components decrease as the rotation rate and the size of the radiative core increase. The magnetic fields possess a mixed poloidal-toroidal topology with no obvious dominant component. Moreover, the relaxation of the vestige dynamo magnetic field within the radiative core is found to satisfy MHD stability criteria. Hence, it does not experience a global reconfiguration but slowly relaxes by retaining its mixed stable poloidal-toroidal topology.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,convection,dynamo,magnetohydrodynamics: MHD,stars: interiors,stars: magnetic field},
  annotation = {ADS Bibcode: 2017ApJ...846....8E},
  file = {/Users/lbugnet/Zotero/storage/LMK8YZV7/Emeriau-Viard and Brun - 2017 - Origin and Evolution of Magnetic Field in PMS Star.pdf}
}

@techreport{Emeriau2014,
  title = {Impact of Rotation on the Geometrical Configurations of Fossil Magnetic Fields},
  author = {Emeriau, C and Mathis, S},
  year = {2014},
  eprint = {1408.4279v1},
  urldate = {2020-06-19},
  abstract = {The MiMeS project demonstrated that a small fraction of massive stars (around 7\%) presents large-scale, stable, generally dipolar magnetic fields at their surface. They are supposed to be fossil remnants of initial phases of stellar evolution. In fact, they result from the relaxation to MHD equilibrium states during the formation of stable radiation zones of initial fields generated by a previous convective phase. In contrast with the case of magnetic fields built by dynamo mechanisms, the geometry of fossil fields at the surface of early-type stars seems to be independent of rotation: dipolar fields are observed both in slowly-and rapidly-rotating stars. In this work, we present new theoretical results, where we generalized previous studies by taking rotation into account. The properties of relaxed fossil fields are compared to those obtained when rotation is ignored. Consequences for magnetic fields in the radiative envelope of rotating early-type stars are discussed.},
  archiveprefix = {arxiv},
  keywords = {magnetic fields,MHD,notion,notion-database,stars: interiors,stars: magnetic fields,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/MFI5SG67/full-text.pdf}
}

@phdthesis{Emeriau2017,
  title = {\'Etoiles et Les {{Turbulence}} Plasma Dans Les e Tokamaks : Magn \textasciiacute},
  author = {Emeriau, C.},
  year = {2017},
  keywords = {notion,notion-database}
}

@article{Endal1978,
  title = {The Evolution of Rotating Stars. {{II}}. {{Calculations}} with Time-Dependent Redistribution of Angular Momentum for 7 and 10 {{M}} Sun Stars.},
  author = {Endal, A. S. and Sofia, S.},
  year = {1978},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {220},
  pages = {279--290},
  issn = {0004-637X},
  doi = {10.1086/155904},
  urldate = {2023-10-28},
  abstract = {Calculations have been performed for the evolution of rotating stars with realistic time-dependent redistribution of angular momentum and chemical composition due to gas-dynamical instabilities. Convection and Eddington circulation are found to be the most important mechanisms for changing the angular-momentum distribution, while the dynamical shear and Solberg-Hoiland instabilities produce chemical mixing in regions which remain unmixed in nonrotating calculations. The calculations indicate that ignoring the finite time scales associated with angular-momentum redistribution is a poor and often misleading approximation. The primary results are: (1) evolved stellar cores develop nonaxisymmetric instabilities corresponding to the bifurcation of the Maclaurin sequence before they reach critical (Keplerian) rotational velocities; (2) for the 7-solar-mass star, the instability point is reached prior to carbon ignition, indicating that catastrophic carbon detonation may be avoided by rotating stars; and (3) the hydrodynamic events associated with violent stellar death will generally involve rapidly rotating, triaxial, or fissioning cores. In addition to radically altering the nature of these events, this indicates that stellar collapse may be a strong source of gravitational-wave radiation.},
  keywords = {Angular Momentum,Angular Velocity,Astrophysics,Carbon,Chemical Composition,Convection,Eddington Approximation,Evolution:Rotating Stars,Gravitational Collapse,Main Sequence Stars,Momentum Transfer,Radial Velocity,Secular Variations,Stellar Evolution,Stellar Models,Stellar Rotation,Thermal Instability,Time Dependence},
  annotation = {ADS Bibcode: 1978ApJ...220..279E},
  file = {/Users/lbugnet/Zotero/storage/EQ76NKFQ/Endal and Sofia - 1978 - The evolution of rotating stars. II. Calculations .pdf}
}

@article{Epstein2014,
  title = {Testing the Asteroseismic Mass Scale Using Metal-Poor Stars Characterized with {{APOGEE}} and {{Kepler}}},
  author = {Epstein, Courtney R. and Elsworth, Yvonne P. and Johnson, Jennifer A. and Shetrone, Matthew and Mosser, Beno{\^i}t and Hekker, Saskia and Tayar, Jamie and Harding, Paul and Pinsonneault, Marc and Silva Aguirre, V{\'i}ctor and Basu, Sarbani and Beers, Timothy C. and Bizyaev, Dmitry and Bedding, Timothy R. and Chaplin, William J. and Frinchaboy, Peter M. and Garc{\'i}a, Rafael A. and P{\'e}rez, Ana E.Garc{\'i}a and Hearty, Fred R. and Huber, Daniel and Ivans, Inese I. and Majewski, Steven R. and Mathur, Savita and Nidever, David and Serenelli, Aldo and Schiavon, Ricardo P. and Schneider, Donald P. and Sch{\"o}nrich, Ralph and Sobeck, Jennifer S. and Stassun, Keivan G. and Stello, Dennis and Zasowski, Gail},
  year = {2014},
  journal = {Astrophysical Journal Letters},
  volume = {785},
  number = {2},
  eprint = {1403.1872},
  issn = {20418213},
  doi = {10.1088/2041-8205/785/2/L28},
  abstract = {Fundamental stellar properties, such as mass, radius, and age, can be inferred using asteroseismology. Cool stars with convective envelopes have turbulent motions that can stochastically drive and damp pulsations. The properties of the oscillation frequency power spectrum can be tied to mass and radius through solar-scaled asteroseismic relations. Stellar properties derived using these scaling relations need verification over a range of metallicities. Because the age and mass of halo stars are well-constrained by astrophysical priors, they provide an independent, empirical check on asteroseismic mass estimates in the low-metallicity regime. We identify nine metal-poor red giants (including six stars that are kinematically associated with the halo) from a sample observed by both the Kepler space telescope and the Sloan Digital Sky Survey-III APOGEE spectroscopic survey. We compare masses inferred using asteroseismology to those expected for halo and thick-disk stars. Although our sample is small, standard scaling relations, combined with asteroseismic parameters from the APOKASC Catalog, produce masses that are systematically higher ({$<\Delta$}M {$>$} =0.17 {$\pm$} 0.05 M{$\odot$}) than astrophysical expectations. The magnitude of the mass discrepancy is reduced by known theoretical corrections to the measured large frequency separation scaling relationship. Using alternative methods for measuring asteroseismic parameters induces systematic shifts at the 0.04 M{$\odot$} level. We also compare published asteroseismic analyses with scaling relationship masses to examine the impact of using the frequency of maximum power as a constraint. Upcoming APOKASC observations will provide a larger sample of 100 metal-poor stars, important for detailed asteroseismic characterization of Galactic stellar populations. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,Galaxy: halo,notion,notion-database,stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/UPVABJ93/Epstein et al. - 2014.pdf}
}

@article{Epstein2014a,
  title = {How Good a Clock Is Rotation? The Stellar Rotation-Mass-Age Relationship for Old Field Stars},
  author = {Epstein, Courtney R. and Pinsonneault, Marc H.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {780},
  number = {2},
  eprint = {1203.1618},
  issn = {15384357},
  doi = {10.1088/0004-637X/780/2/159},
  abstract = {The rotation-mass-age relationship offers a promising avenue for measuring the ages of field stars, assuming the attendant uncertainties to this technique can be well characterized. We model stellar angular momentum evolution starting with a rotation distribution from open cluster M37. Our predicted rotation-mass-age relationship shows significant zero-point offsets compared to an alternative angular momentum loss law and published gyrochronology relations. Systematic errors at the 30\% level are permitted by current data, highlighting the need for empirical guidance. We identify two fundamental sources of uncertainty that limit the precision of rotation-based ages and quantify their impact. Stars are born with a range of rotation rates, which leads to an age range at fixed rotation period. We find that the inherent ambiguity from the initial conditions is important for all young stars, and remains large for old stars below 0.6 M{$\odot$}. Latitudinal surface differential rotation also introduces a minimum uncertainty into rotation period measurements and, by extension, rotation-based ages. Both models and the data from binary star systems 61 Cyg and {$\alpha$} Cen demonstrate that latitudinal differential rotation is the limiting factor for rotation-based age precision among old field stars, inducing uncertainties at the {$\sim$}2 Gyr level. We also examine the relationship between variability amplitude, rotation period, and age. Existing ground-based surveys can detect field populations with ages as old as 1-2 Gyr, while space missions can detect stars as old as the Galactic disk. In comparison with other techniques for measuring the ages of lower main sequence stars, including geometric parallax and asteroseismology, rotation-based ages have the potential to be the most precise chronometer for 0.6-1.0 M stars. \textcopyright{} 2014. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: evolution,stars: late-type,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/24TU54U6/Epstein, Pinsonneault - 2014.pdf}
}

@book{Erdelyi1956,
  title = {Asymptotic {{Expansions}}},
  author = {Erd{\'e}lyi, A},
  year = {1956},
  urldate = {2020-07-19},
  keywords = {notion,notion-database}
}

@book{Erdelyi1965,
  title = {Asymptotic {{Expansions}}},
  author = {Erd{\'e}lyi, A.},
  year = {1965},
  urldate = {2020-06-26},
  keywords = {notion,notion-database}
}

@techreport{europeanspaceagencyPLATORevealingHabitable2017,
  title = {{{PLATO Revealing}} Habitable Worlds around Solar-like Stars {{Definition Study Report European Space Agency}}},
  author = {{European Space Agency}},
  year = {2017},
  urldate = {2020-12-24},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2THX6JZQ/full-text.pdf}
}

@article{Evans1962a,
  title = {Observational {{Study}} of {{Macroscopic Inhomogeneities}} in the {{Solar Atmosphere}}. {{III}}. {{Vertical Oscillatory Motions}} in the {{Solar Photosphere}}.},
  author = {Evans, J. W. and Michard, R.},
  year = {1962},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {136},
  pages = {493},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/147403},
  urldate = {2020-03-08},
  abstract = {We have studied the Doppler displacements in two time sequences of spectrograms, one showing Fe I 5171.61, Mgi 5172.70 (b2), and Tii 5173.75 at the center of the solar disk, the other showing Fei 5324.19 at the limb. At the center we find that the velocity field consists mainly of short-lived oscillations of small elements of the solar atmosphere. The r.m.s. velocity amplitudes are 0.42 and 0.81 km/sec at low and high levels, respectively. The periods of the vertical oscillations cover roughly the range seconds, with a mean value around 242 sec. The periods seem to decrease with height in the atmosphere. An autocorrelation study shows also that the vertical velocity field is dominated by periodic oscillations, the time-correlation function having a strong positive peak at 300 seconds from the origin. The study of the time lags of oscillations between strong and faint lines suggests that they are of a type intermediate between progressive sonic waves (for the shorter periods) and standing waves (for the longer periods). Gradual transition from the first type to the second seems to occur during the life of a given oscillation. There is an indication that the individual oscillations are associated with individual granules. Near the limb, the observed horizontal motions consist of slowly changing velocities of the order of 0.5 km/sec in large surface elements, on which are superposed smaller random velocities of short duration. Oscillations rapidly disappear away from the center of the disk. The horizontal and vertical observable motions appear to be physically independent.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/H78MQFV3/J.W., Michard - 1962.pdf}
}

@book{Fallis2009,
  title = {The {{Rotation}} of {{Sun}} and {{Stars}}},
  author = {Fallis, A.G},
  year = {2009},
  journal = {Journal of Chemical Information and Modeling},
  volume = {765},
  eprint = {1011.1669v3},
  issn = {1098-6596},
  doi = {10.1007/978-3-540-87831-5},
  abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein-protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-{$\alpha$}-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD {$\leq$} 2.0 \AA{} for the interface backbone atoms) increased from 21\% with default Glide SP settings to 58\% with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63\% success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40\% of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
  archiveprefix = {arxiv},
  isbn = {978-3-540-87830-8},
  pmid = {25246403},
  keywords = {icle,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KXLHTYJ2/Fallis - 2009.pdf}
}

@article{Fallis2009a,
  title = {The {{Rotation}} of {{Sun}} and {{Stars}}},
  author = {Fallis, A.G},
  year = {2009},
  journal = {Journal of Chemical Information and Modeling},
  volume = {765},
  number = {9},
  eprint = {1011.1669v3},
  pages = {1689--1699},
  issn = {1098-6596},
  doi = {10.1007/978-3-540-87831-5},
  abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein-protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-{$\alpha$}-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD {$\leq$} 2.0 \AA{} for the interface backbone atoms) increased from 21\% with default Glide SP settings to 58\% with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63\% success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40\% of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
  archiveprefix = {arxiv},
  isbn = {978-3-540-87830-8},
  pmid = {25246403},
  keywords = {icle,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Y889QKR7/Fallis - 2009(2).pdf}
}

@article{Fan2004,
  title = {Magnetic Fields in the Solar Convection Zone},
  author = {Fan, Yuhong},
  year = {2004},
  journal = {Living Reviews in Solar Physics},
  volume = {1},
  number = {1},
  pages = {1--74},
  issn = {16144961},
  doi = {10.12942/lrsp-2004-1},
  urldate = {2020-05-14},
  abstract = {Recent studies of the dynamic evolution of magnetic flux tubes in the solar convection zone are reviewed with focus on emerging flux tubes responsible for the formation of solar active regions. The current prevailing picture is that active regions on the solar surface originate from strong toroidal magnetic fields generated by the solar dynamo mechanism at the thin tachocline layer at the base of the solar convection zone. Thus the magnetic fields need to traverse the entire convection zone before they reach the photosphere to form the observed solar active regions. This review discusses results with regard to the following major topics: 1. the equilibrium properties of the toroidal magnetic fields stored in the stable overshoot region at the base of the convection zone, 2. the buoyancy instability associated with the toroidal magnetic fields and the formation of buoyant magnetic flux tubes, 3. the rise of emerging flux loops through the solar convective envelope as modeled by the thin flux tube calculations which infer that the field strength of the toroidal magnetic fields at the base of the solar convection zone is significantly higher than the value in equipartition with convection, 4. the observed hemispheric trend of the twist of the magnetic field in solar active regions and its origin, 5. the minimum twist needed for maintaining cohesion of the rising flux tubes, 6. the rise of highly twisted kink unstable flux tubes as a possible origin of {$\delta$}-sunspots, 7. the evolution of buoyant magnetic flux tubes in 3D stratified convection, 8. turbulent pumping of magnetic flux by penetrative compressible convection, 9. an alternative mechanism for intensifying toroidal magnetic fields to significantly superequipartition field strengths by conversion of the potential energy associated with the superadiabatic stratification of the solar convection zone, and finally 10. a brief overview of our current understanding of flux emergence at the surface and postemergence evolution of the subsurface magnetic fields.},
  keywords = {Convection Zone,Flux Tube,Magnetic Flux Tube,notion,notion-database,Solar Active Region,Toroidal Magnetic Field},
  file = {/Users/lbugnet/Zotero/storage/Q5UUFTRM/full-text.pdf}
}

@article{Fares2009,
  title = {Magnetic Cycles of the Planet-Hosting Star {$\tau$} {{Bootis}} - {{II}}. {{A}} Second Magnetic Polarity Reversal},
  author = {Fares, R. and Donati, J. F. and Moutou, C. and Bohlender, D. and Catala, C. and Deleuil, M. and Shkolnik, E. and Cameron, A. C. and Jardine, M. M. and Walker, G. A.H.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {398},
  number = {3},
  eprint = {0906.4515},
  pages = {1383--1391},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.15303.x},
  abstract = {In this paper, we present new spectropolarimetric observations of the planet-hosting star {$\tau$} Bootis, using ESPaDOnS and Narval spectropolarimeters at Canada-France-Hawaii Telescope and Telescope Bernard Lyot, respectively. We detected the magnetic field of the star at three epochs in 2008. It has a weak magnetic field of only a few gauss, oscillating between a predominant toroidal component in January and a dominant poloidal component in June and July. A magnetic polarity reversal was observed relative to the magnetic topology in 2007 June. This is the second such reversal observed in 2 years on this star, suggesting that {$\tau$} Boo has a magnetic cycle of about 2 years. This is the first detection of a magnetic cycle for a star other than the Sun. The role of the close-in massive planet in the short activity cycle of the star is questioned. {$\tau$} Boo has a strong differential rotation, a common trend for stars with shallow convective envelope. At latitude 40\textdegree, the surface layer of the star rotates in 3.31 d, equal to the orbital period. Synchronization suggests that the tidal effects induced by the planet may be strong enough to force at least the thin convective envelope into corotation. {$\tau$} Boo shows variability in the Ca ii H \& K and H{$\alpha$} throughout the night and on a night-to-night time-scale. We do not detect enhancement in the activity of the star that may be related to the conjunction of the planet. Further data are needed to conclude about the activity enhancement due to the planet. \textcopyright{} 2009 RAS.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: activity,Stars: individual: {$\tau$} Boo,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/86SFUHNZ/Fares et al. - 2009.pdf}
}

@article{Fares2012,
  title = {Magnetic Field, Differential Rotation and Activity of the Hot-{{Jupiter-hosting}} Star {{HD}} 179949},
  author = {Fares, R. and Donati, J. F. and Moutou, C. and Jardine, M. and Cameron, A. C. and Lanza, A. F. and Bohlender, D. and Dieters, S. and Mart{\'i}nez Fiorenzano, A. F. and Maggio, A. and Pagano, I. and Shkolnik, E. L.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {423},
  number = {2},
  pages = {1006--1017},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.20780.x},
  abstract = {HD 179949 is an F8V star, orbited by a giant planet at {$\sim$}8R \{black star\} every 3.092514 d. The system was reported to undergo episodes of stellar activity enhancement modulated by the orbital period, interpreted as caused by star-planet interactions (SPIs). One possible cause of SPIs is the large-scale magnetic field of the host star in which the close-in giant planet orbits. In this paper we present spectropolarimetric observations of HD 179949 during two observing campaigns (2009 September and 2007 June). We detect a weak large-scale magnetic field of a few gauss at the surface of the star. The field configuration is mainly poloidal at both observing epochs. The star is found to rotate differentially, with a surface rotation shear of d{$\Omega$}= 0.216 {$\pm$} 0.061radd -1, corresponding to equatorial and polar rotation periods of 7.62 {$\pm$} 0.07 and 10.3 {$\pm$} 0.8d, respectively. The coronal field estimated by extrapolating the surface maps resembles a dipole tilted at {$\sim$}70\textdegree. We also find that the chromospheric activity of HD 179949 is mainly modulated by the rotation of the star, with two clear maxima per rotation period as expected from a highly tilted magnetosphere. In 2009 September, we find that the activity of HD 179949 shows hints of low-amplitude fluctuations with a period close to the beat period of the system. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {notion,notion-database,Planet-star interactions,Stars: activity,Stars: individual: HD 179949,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/G3WIPE3U/Fares et al. - 2012.pdf}
}

@article{Farihi2023,
  title = {Discovery of Dipolar Chromospheres in Two White Dwarfs},
  author = {Farihi, J. and Hermes, J. J. and Littlefair, S. P. and Howarth, I. D. and Walters, N. and Parsons, S. G.},
  year = {2023},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {525},
  pages = {1097--1105},
  issn = {0035-8711},
  doi = {10.1093/mnras/stad2184},
  urldate = {2023-10-05},
  abstract = {This paper reports the ULTRACAM discovery of dipolar surface spots in two cool magnetic white dwarfs with Balmer emission lines, while a third system exhibits a single spot, similar to the prototype GD 356. The light curves are modelled with simple, circular, isothermal dark spots, yielding relatively large regions with minimum angular radii of 20\textdegree. For those stars with two light-curve minima, the dual spots are likely observed at high inclination (or colatitude); however, identical and antipodal spots cannot simultaneously reproduce both the distinct minima depths and the phases of the light-curve maxima. The amplitudes of the multiband photometric variability reported here are all several times larger than that observed in the prototype GD 356; nevertheless, all DAHe stars with available data appear to have light-curve amplitudes that increase towards the blue in correlated ratios. This behaviour is consistent with cool spots that produce higher contrasts at shorter wavelengths, with remarkably similar spectral properties given the diversity of magnetic field strengths and rotation rates. These findings support the interpretation that some magnetic white dwarfs generate intrinsic chromospheres as they cool, and that no external source is responsible for the observed temperature inversion. Spectroscopic time-series data for DAHe stars is paramount for further characterization, where it is important to obtain well-sampled data, and consider wavelength shifts, equivalent widths, and spectropolarimetry.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: magnetic field,white dwarfs},
  annotation = {ADS Bibcode: 2023MNRAS.525.1097F},
  file = {/Users/lbugnet/Zotero/storage/A5L286E6/Farihi et al. - 2023 - Discovery of dipolar chromospheres in two white dw.pdf}
}

@article{Fath1935,
  title = {The {{Variability}} of {$\delta$} {{Scuti}}},
  author = {Fath, E. A.},
  year = {1935},
  month = aug,
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {47},
  number = {278},
  pages = {232},
  publisher = {{IOP Publishing}},
  issn = {0004-6280},
  doi = {10.1086/124600},
  urldate = {2020-03-31},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/S56DE84S/full-text.pdf}
}

@article{Favata2008,
  title = {The {{X-ray}} Cycle in the Solar-Type Star {{HD}} 81809},
  author = {Favata, F. and Micela, G. and Orlando, S. and Schmitt, J. H.M.M. and Sciortino, S. and Hall, J.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {490},
  number = {3},
  pages = {1121--1126},
  issn = {14320746},
  doi = {10.1051/0004-6361:200809694},
  abstract = {Context. The 11-yr cycle is the best known manifestation of the Sun's activity. While chromospheric cycles have been studied in a number of solar-like stars, very little is known about how these are reflected in the cyclical behavior of the coronal X-ray emission in stars other than the Sun. Aims. Our long-term XMM-Newtonprogram of long-term monitoring of a solar-like star with a well-studied chromospheric cycle, HD 81809, aims to study whether an X-ray cycle is present, along with studying its characteristics and its relation to the chromospheric cycle. Methods. Regular observations of HD 81809 were performed with XMM-Newton, spaced by 6 months from 2001 to 2007. We studied the variations in the resulting coronal luminosity and temperature, and compared them with the chromospheric Ca ii variations. We also modeled the observations in terms of a mixture of active regions, using a methodology originally developed to study the solar corona. Results. Our observations show a well-defined cycle with an amplitude exceeding 1 dex and an average luminosity approximately one order of magnitude higher than in the Sun. The behavior of the corona of HD 81809 can be modeled well in terms of varying coverage of solar-like active regions, with a larger coverage than for the Sun, showing it to be compatible with a simple extension of the solar case. \textcopyright{} 2008 ESO.},
  keywords = {notion,notion-database,Stars: activity,Stars: coronae,Stars: late-type,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/EFD7TTHI/Favata et al. - 2008.pdf}
}

@article{Fawzy2012a,
  title = {Atmospheric Oscillations in Late-Type Stars - {{I}}. {{Non-linear}} Response to Excitation by Acoustic Wave Energy Spectra},
  author = {Fawzy, Diaa E. and Musielak, Z. E.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {421},
  number = {1},
  pages = {159--168},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.20285.x},
  abstract = {The main aim of this paper is to perform first self-consistent numerical computation of the response of stellar atmospheres to the propagation of acoustic waves specified by realistic acoustic wave energy spectra. In the numerical approach, stellar atmospheres are stratified, non-isothermal and plane-parallel, and only their magnetic-free regions are considered. The resulting atmospheric heating is calculated and the time sequence of atmospheric velocities computed by a time-dependent hydrodynamic numerical code is analysed. All computations are done adiabatically and Fourier analysis is used in order to determine the oscillatory properties of stellar atmospheres. The numerical approach is supplemented by an analytical treatment in which three different local acoustic cut-off frequencies are selected from the literature; their values in the stellar atmospheric models are calculated and compared to the numerical results. The theoretical results obtained clearly show that atmospheric oscillations do exist in late-type stars and that their origin and physical properties are similar to those observed in the solar atmosphere. The oscillation frequency of stellar atmospheric oscillations ranges from 7.5mHz for F5V stars to 16.0mHz for M0V stars. The relevance of this theoretically predicted range of stellar oscillation in solar-like stars to the recent data obtained by the NASA space mission Kepler is discussed. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {Methods: numerical,notion,notion-database,Shock waves,Stars: atmospheres,Stars: late-type,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/TCK5HH9Q/Fawzy, Musielak - 2012.pdf}
}

@article{Featherstone2007,
  title = {Magnetic {{Dynamo Action In The Convective Cores Of A-type Stars In The Presence Of Fossil Fields}}},
  author = {Featherstone, Nicholas and Browning, M. K. and Brun, A. S. and Toomre, J.},
  year = {2007},
  journal = {AAS},
  volume = {210},
  pages = {17.02},
  urldate = {2020-05-14},
  keywords = {notion,notion-database}
}

@article{Featherstone2009,
  title = {Effects of Fossil Magnetic Fields on Convective Core Dynamos in A-{{Type}} Stars},
  author = {Featherstone, Nicholas A. and Browning, Matthew K. and Brun, Allan Sacha and Toomre, Juri},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {705},
  number = {1},
  pages = {1000--1018},
  issn = {15384357},
  doi = {10.1088/0004-637X/705/1/1000},
  abstract = {The vigorous magnetic dynamo action achieved within the convective cores of A-Type stars may be influenced by fossil magnetic fields within their radiative envelopes.We study such effects through three-dimensional simulations that model the inner 30\% by radius of a 2M A-Type star, capturing the convective core and a portion of the overlying radiative envelope within our computational domain.We employ the three-dimensional anelastic spherical harmonic code to model turbulent dynamics within a deep rotating spherical shell. The interaction between a fossil field and the core dynamo is examined by introducing a large-scale magnetic field into the radiative envelope of a mature A star dynamo simulation. We find that the inclusion of a twisted toroidal fossil field can lead to a remarkable transition in the core dynamo behavior. Namely, a super-equipartition state can be realized in which the magnetic energy built by dynamo action is 10-fold greater than the kinetic energy of the convection itself. Such strongfield states may suggest that the resulting Lorentz forces should seek to quench the flows, yet we have achieved super-equipartition dynamo action that persists for multiple diffusion times. This is achieved by the relative coalignment of the flows and magnetic fields in much of the domain, along with some lateral displacements of the fastest flows from the strongest fields. Convection in the presence of such strong magnetic fields typically manifests as 4-6 cylindrical rolls aligned with the rotation axis, each possessing central axial flows that imbue the rolls with a helical nature. The roll system also possesses core-crossing flows that couple distant regions of the core. We find that the magnetic fields exhibit a comparable global topology with broad, continuous swathes of magnetic field linking opposite sides of the convective core. We have explored several poloidal and toroidal fossil field geometries, finding that a poloidal component is essential for a transition to super-equipartition to occur.},
  keywords = {convection,Convection,Evolution,Magnetic fields,MHD,notion,notion-database,Stars,stars: evolution,stars: interiors,Stars: interiors,stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/SII44PPF/Featherstone et al. - 2009.pdf}
}

@article{Featherstone2023,
  title = {The {{Puzzling Structure}} of {{Solar Convection}}: {{Window}} into the {{Dynamo}}},
  shorttitle = {The {{Puzzling Structure}} of {{Solar Convection}}},
  author = {Featherstone, Nicholas and Anders, Evan H. and Augustson, Kyle C. and Aurnou, Jonathan and Blume, Catherine and Brown, Benjamin P. and Brummell, Nicholas and Burns, Keaton J. and Calkins, Michael A. and Camisassa, Maria and Dikpati, Mausumi and Fan, Yuhong and Fuentes, J. R. and Guerrero, Gustavo and Hindman, Bradley W. and Julien, Keith and Kitiashvili, Irina N. and Korre, Lydia and Lecoanet, Daniel and Manek, Bhishek and Matilsky, Loren and Nelson, Nicholas J. and Oishi, Jeffrey S. and Powers, Whitney T. and Rempel, Matthias and Soderlund, Krista and Vasil, Geoffrey M. and Stejko, Andrey M. and Miesch, Mark},
  year = {2023},
  month = jul,
  volume = {55},
  pages = {105},
  address = {{eprint: arXiv:2305.08823}},
  doi = {10.3847/25c2cfeb.240cbaca},
  urldate = {2023-10-18},
  abstract = {The operation of the solar dynamo remains an outstanding problem of solar physics owing to continuing uncertainty in the speed and structure of deep-seated convective flows. We discuss the relationship between this aspect of convection and the dynamo. We suggest that observations of the solar poles, coupled with theory and simulation are vital to attain new perspectives on the dynamo.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2023BAAS...55c.105F},
  file = {/Users/lbugnet/Zotero/storage/JCWUNCJA/Featherstone et al. - 2023 - The Puzzling Structure of Solar Convection Window.pdf}
}

@article{Fellay2021,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum. {{IV}}. {{Internal}} Rotation of {{Kepler-56}} from an {{MCMC}} Analysis of the Rotational Splittings},
  author = {Fellay, L. and Buldgen, G. and Eggenberger, P. and Khan, S. and Salmon, S. J. A. J. and Miglio, A. and Montalb{\'a}n, J.},
  year = {2021},
  month = oct,
  journal = {Astronomy and Astrophysics},
  volume = {654},
  pages = {A133},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202140518},
  urldate = {2023-09-22},
  abstract = {Context. The observations of global stellar oscillations of post-main-sequence stars by space-based photometry missions have allowed us to directly determine their internal rotation. These constraints have pointed towards the existence of angular momentum transport processes not accounted for in theoretical models. Constraining the properties of their internal rotation thus appears to be the golden path to determine the physical nature of these missing dynamical processes. Aims: Our aim is to determine the robustness of a new approach to study the internal rotation of post-main-sequence stars, using parametric rotation profiles coupled to a global optimization technique. Methods: We tested our methodology on Kepler-56, a red giant observed by the Kepler mission. First, we carried out an extensive modelling of the star using global and local minimizations techniques, and seismic inversions. Then, using our best model, we study in details its internal rotation profile, we adopted a Bayesian approach to constrain stellar parametric predetermined rotation profiles using a Markov chain Monte Carlo analysis of the rotational splittings of mixed modes. Results: Our Markov chain Monte Carlo analysis of the rotational splittings allows us to determine the core and envelope rotation of Kepler-56 and gives us hints about the location of the transition between the slowly rotating envelope and the fast-rotating core. We are able to discard a rigid rotation profile in the radiative regions followed by a power law in the convective zone, and we show that the data favours a transition located in the radiative region, as predicted by processes originating from a turbulent nature such as for example magnetic instabilities. Conclusions: Our new approach to studying the internal rotation of red giants constitutes a viable option to analyse Kepler targets and allows us to put stringent constraints on the properties of the missing angular momentum transport process acting in post-main-sequence stars. Our analysis of Kepler-56 indicates that turbulent processes whose transport efficiency is reduced by chemical gradients are favoured, while large-scale fossil magnetic fields are disfavoured as a solution to the missing angular momentum transport.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: individual: KIC 6448890,stars: interiors,stars: rotation},
  annotation = {ADS Bibcode: 2021A\&A...654A.133F},
  file = {/Users/lbugnet/Zotero/storage/5J9BGCL8/Fellay et al. - 2021 - Asteroseismology of evolved stars to constrain the.pdf}
}

@article{Ferguson2005,
  title = {Low-{{Temperature Opacities}}},
  author = {Ferguson, Jason W. and Alexander, David R. and Allard, France and Barman, Travis and Bodnarik, Julia G. and Hauschildt, Peter H. and Heffner-Wong, Amanda and Tamanai, Akemi},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {623},
  number = {1},
  eprint = {astro-ph/0502045},
  pages = {585--596},
  issn = {0004-637X},
  doi = {10.1086/428642},
  abstract = {Previous computations of low temperature Rosseland and Planck mean opacities from Alexander \& Ferguson (1994) are updated and expanded. The new computations include a more complete equation of state with more grain species and updated optical constants. Grains are now explicitly included in thermal equilibrium in the equation of state calculation, which allows for a much wider range of grain compositions to be accurately included than was previously the case. The inclusion of high temperature condensates such as Al\$\_2\$O\$\_3\$ and CaTiO\$\_3\$ significantly affects the total opacity over a narrow range of temperatures before the appearance of the first silicate grains. The new opacity tables are tabulated for temperatures ranging from 30000 K to 500 K with gas densities from 10\$\^\{-4\}\$ g cm\$\^\{-3\}\$ to 10\$\^\{-19\}\$ g cm\$\^\{-3\}\$. Comparisons with previous Rosseland mean opacity calculations are discussed. At high temperatures, the agreement with OPAL and Opacity Project is quite good. Comparisons at lower temperatures are more divergent as a result of differences in molecular and grain physics included in different calculations. The computation of Planck mean opacities performed with the opacity sampling method are shown to require a very large number of opacity sampling wavelength points; previously published results obtained with fewer wavelength points are shown to be significantly in error. Methods for requesting or obtaining the new tables are provided.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TL2AVBKP/Ferguson et al. - 2005.pdf}
}

@article{Ferrario2005,
  title = {Magnetic Fields and Rotation in White Dwarfs and Neutron Stars},
  author = {Ferrario, Lilia and Wickramasinghe, D. T.},
  year = {2005},
  month = jan,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {356},
  number = {2},
  pages = {615--620},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2004.08474.x},
  urldate = {2020-03-09},
  abstract = {Recent spectropolarimetric observations of Ap and Bp stars with improved sensitivity have suggested that most Ap and Bp stars are magnetic with dipolar fields of at least a few hundred gauss. These new estimates suggest that the range of magnetic fluxes found for the majority of magnetic white dwarfs is similar to that of main-sequence Ap-Bp stars, thus strengthening the empirical evidence for an evolutionary link between magnetism on the main sequence and magnetism in white dwarfs. We draw parallels between the magnetic white dwarfs and the magnetic neutron stars and argue that the observed range of magnetic fields in isolated neutron stars (Bp{$\sim$} {$\sim$} 10 11-1015 G) could also be explained if their mainly O-type progenitors have effective dipolar fields in the range of a few gauss to a few kilogauss, assuming approximate magnetic flux conservation with the upper limit being consistent with the recent measurement of a field of Bp {$\sim$} 1100 G for \texttheta{} Orion C. In the magnetic field-rotation diagram, the magnetic white dwarfs can be divided into three groups of different origin: a significant group of strongly magnetized slow rotators (Prot {$\sim$} 50-100 yr) that have originated from single-star evolution, a group of strongly magnetized fast rotators (Prot {$\sim$} 700 s), typified by EUVE J0317-853, that have originated from a merger, and a group of modest rotators (Prot {$\sim$} hours-days) of mixed origin (single-star and CV-type binary evolution). We propose that the neutron stars may similarly divide into distinct classes at birth, and suggest that the magnetars may be the counterparts of the slowly rotating high-field magnetic white dwarfs.},
  keywords = {notion,notion-database,Stars: Magnetic fields,Stars: Neutron,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/KUGE8222/full-text.pdf}
}

@inproceedings{Ferrario2007,
  title = {High {{Field Magnetic White Dwarfs}}, {{Pulsars}}, {{Magnetars}}, and Their {{Main Sequence Progenitors}}},
  booktitle = {15th {{European Workshop}} on {{White Dwarfs}}, {{ASP}} Conference {{Series}}},
  author = {Ferrario, Lilia and Wickramasinghe, D T},
  year = {2007},
  volume = {372},
  urldate = {2020-03-09},
  abstract = {Super-strong magnetic fields are observed in both white dwarfs and neutron stars. In this paper, we present calculations that highlight the commonality of their properties and the implications for their main sequence progenitors.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Q95ETU2E/full-text.pdf}
}

@article{Ferrario2015,
  title = {Magnetic {{Field Generation}} in {{Stars}}},
  author = {Ferrario, Lilia and Melatos, Andrew and Zrake, Jonathan},
  year = {2015},
  journal = {Space Science Reviews},
  volume = {191},
  number = {1-4},
  eprint = {1504.08074},
  pages = {77--109},
  publisher = {{Springer Science+Business Media Dordrecht}},
  issn = {15729672},
  doi = {10.1007/s11214-015-0138-y},
  abstract = {Enormous progress has been made on observing stellar magnetism in stars from the main sequence (particularly thanks to the MiMeS, MAGORI and BOB surveys) through to compact objects. Recent data have thrown into sharper relief the vexed question of the origin of stellar magnetic fields, which remains one of the main unanswered questions in astrophysics. In this chapter we review recent work in this area of research. In particular, we look at the fossil field hypothesis which links magnetism in compact stars to magnetism in main sequence and pre-main sequence stars and we consider why its feasibility has now been questioned particularly in the context of highly magnetic white dwarfs. We also review the fossil versus dynamo debate in the context of neutron stars and the roles played by key physical processes such as buoyancy, helicity, and superfluid turbulence, in the generation and stability of neutron star fields. Independent information on the internal magnetic field of neutron stars will come from future gravitational wave detections. Coherent searches for the Crab pulsar with the Laser Interferometer Gravitational Wave Observatory (LIGO) have already constrained its gravitational wave luminosity to be {$\lessequivlnt$}2~\% of the observed spin-down luminosity, thus placing a limit of {$\lessequivlnt$}1016 G on the internal field. Indirect spin-down limits inferred from recycled pulsars also yield interesting gravitational-wave-related constraints. Thus we may be at the dawn of a new era of exciting discoveries in compact star magnetism driven by the opening of a new, non-electromagnetic observational window. We also review recent advances in the theory and computation of magnetohydrodynamic turbulence as it applies to stellar magnetism and dynamo theory. These advances offer insight into the action of stellar dynamos as well as processes which control the diffusive magnetic flux transport in stars.},
  archiveprefix = {arxiv},
  keywords = {Magnetic fields,Main sequence stars,Neutron stars,notion,notion-database,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/UTB4366E/Ferrario, Melatos, Zrake - 2015.pdf}
}

@article{Ferrario2015a,
  title = {Magnetic {{White Dwarfs}}},
  author = {Ferrario, Lilia and {de Martino}, Domitilla and G{\"a}nsicke, Boris T.},
  year = {2015},
  month = oct,
  journal = {Space Science Reviews},
  volume = {191},
  pages = {111--169},
  issn = {0038-6308},
  doi = {10.1007/s11214-015-0152-0},
  urldate = {2023-10-05},
  abstract = {In this paper we review the current status of research on the observational and theoretical characteristics of isolated and binary magnetic white dwarfs (MWDs).},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,Binary systems,Magnetic cataclysmic variables,Magnetic fields,Magnetic white dwarfs},
  annotation = {ADS Bibcode: 2015SSRv..191..111F},
  file = {/Users/lbugnet/Zotero/storage/9JNRFKJJ/Ferrario et al. - 2015 - Magnetic White Dwarfs.pdf}
}

@article{Ferrario2019,
  title = {Magnetic Fields in Isolated and Interacting White Dwarfs},
  author = {Ferrario, Lilia and Wickramasinghe, Dayal and Kawka, Adela},
  year = {2019},
  journal = {Advances in Space Research},
  eprint = {2001.10147},
  publisher = {{Elsevier Ltd}},
  issn = {18791948},
  doi = {10.1016/j.asr.2019.11.012},
  urldate = {2020-05-14},
  abstract = {The magnetic white dwarfs (MWDs) are found either isolated or in interacting binaries. The isolated MWDs divide into two groups: a high field group (105\textendash 109 G) comprising some 13{$\pm$}4\% of all white dwarfs (WDs), and a low field group (B{$<$}105 G) whose incidence is currently under investigation. The situation may be similar in magnetic binaries because the bright accretion discs in low field systems hide the photosphere of their WDs thus preventing the study of their magnetic fields' strength and structure. Considerable research has been devoted to the vexed question on the origin of magnetic fields. One hypothesis is that WD magnetic fields are of fossil origin, that is, their progenitors are the magnetic main-sequence Ap/Bp stars and magnetic flux is conserved during their evolution. The other hypothesis is that magnetic fields arise from binary interaction, through differential rotation, during common envelope evolution. If the two stars merge the end product is a single high field MWD. If close binaries survive and the primary develops a strong field, they may later evolve into the magnetic cataclysmic variables (MCVs). The recently discovered population of hot, carbon-rich WDs exhibiting an incidence of magnetism of up to about 70\% and a variability from a few minutes to a couple of days may support the merging binary hypothesis. The fields in the low field MWDs may instead arise from a dynamo mechanism taking place in convective zones during post main-sequence evolution. Should this be the case, there may be a field strength below which all WDs are magnetic and thus fields are expected to always play a role in accretion processes in close binaries. Several studies have raised the possibility of the detection of planets around MWDs. Rocky planets may be discovered by the detection of anomalous atmospheric heating of the MWD when the unipolar inductor mechanism operates whilst large gaseous planets may reveal themselves through cyclotron emission from wind-driven accretion onto the MWD. Planetary remains have recently revealed themselves in the atmospheres of about 25\% of WDs that are polluted by elements such as Ca, Si, and often also Mg, Fe, Na. This pollution has been explained by ongoing accretion of planetary debris. Interestingly, the incidence of magnetism is approximately 50\% in cool, hydrogen-rich, polluted WDs, suggesting that these fields may be related to differential rotation induced by some super-Jupiter bodies that have plunged into the WD. The study of isolated and accreting MWDs is likely to continue to yield exciting discoveries for many years to come.},
  archiveprefix = {arxiv},
  keywords = {Accretion processes,Binary systems,Magnetic cataclysmic variables,Magnetic white dwarfs,notion,notion-database,Planetary systems,Zeeman and cyclotron modelling}
}

@article{Ferrario2020,
  title = {Magnetic Fields in Isolated and Interacting White Dwarfs},
  author = {Ferrario, Lilia and Wickramasinghe, Dayal and Kawka, Adela},
  year = {2020},
  month = sep,
  journal = {Advances in Space Research},
  volume = {66},
  pages = {1025--1056},
  issn = {0273-1177},
  doi = {10.1016/j.asr.2019.11.012},
  urldate = {2023-10-05},
  abstract = {The magnetic white dwarfs (MWDs) are found either isolated or in interacting binaries. The isolated MWDs divide into two groups: a high field group (105 -109 G) comprising some 13 {$\pm$} 4 \% of all white dwarfs (WDs), and a low field group (B {$<$}105 G) whose incidence is currently under investigation. The situation may be similar in magnetic binaries because the bright accretion discs in low field systems hide the photosphere of their WDs thus preventing the study of their magnetic fields' strength and structure. Considerable research has been devoted to the vexed question on the origin of magnetic fields. One hypothesis is that WD magnetic fields are of fossil origin, that is, their progenitors are the magnetic main-sequence Ap/Bp stars and magnetic flux is conserved during their evolution. The other hypothesis is that magnetic fields arise from binary interaction, through differential rotation, during common envelope evolution. If the two stars merge the end product is a single high field MWD. If close binaries survive and the primary develops a strong field, they may later evolve into the magnetic cataclysmic variables (MCVs). The recently discovered population of hot, carbon-rich WDs exhibiting an incidence of magnetism of up to about 70\% and a variability from a few minutes to a couple of days may support the merging binary hypothesis. The fields in the low field MWDs may instead arise from a dynamo mechanism taking place in convective zones during post main-sequence evolution. Should this be the case, there may be a field strength below which all WDs are magnetic and thus fields are expected to always play a role in accretion processes in close binaries. Several studies have raised the possibility of the detection of planets around MWDs. Rocky planets may be discovered by the detection of anomalous atmospheric heating of the MWD when the unipolar inductor mechanism operates whilst large gaseous planets may reveal themselves through cyclotron emission from wind-driven accretion onto the MWD. Planetary remains have recently revealed themselves in the atmospheres of about 25\% of WDs that are polluted by elements such as Ca, Si, and often also Mg, Fe, Na. This pollution has been explained by ongoing accretion of planetary debris. Interestingly, the incidence of magnetism is approximately 50\% in cool, hydrogen-rich, polluted WDs, suggesting that these fields may be related to differential rotation induced by some super-Jupiter bodies that have plunged into the WD. The study of isolated and accreting MWDs is likely to continue to yield exciting discoveries for many years to come.},
  keywords = {Accretion processes,Astrophysics - Solar and Stellar Astrophysics,Binary systems,Magnetic cataclysmic variables,Magnetic white dwarfs,Planetary systems,Zeeman and cyclotron modelling},
  annotation = {ADS Bibcode: 2020AdSpR..66.1025F},
  file = {/Users/lbugnet/Zotero/storage/CB5ET8ES/Ferrario et al. - 2020 - Magnetic fields in isolated and interacting white .pdf}
}

@article{Ferraro1937,
  title = {{{THE NON-UNIFORM ROTATION OF THE SUN AND ITS MAGNETIC FIELD}}},
  author = {Ferraro, V C A},
  year = {1937},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {97},
  number = {6},
  pages = {458--472},
  urldate = {2020-06-14},
  keywords = {notion,notion-database}
}

@inproceedings{Ferriere2015,
  title = {Interstellar {{Magnetic}} Fields: From {{Galactic}} Scales to the Edge of the Heliosphere},
  booktitle = {13th {{Annual Internationnal Astrophysics Conference}}: {{Voyager}}, {{IBEX}} and the {{Interstellar Medium}}},
  author = {Ferri{\`e}re, K.},
  year = {2015},
  doi = {10.1088/1742-6596/577/1/012008},
  urldate = {2020-07-03},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RSFA9ZXA/full-text.pdf}
}

@article{Fisher1991,
  title = {The {{Stretching}} of {{Magnetic Flux Tubes}} in the {{Convective Overshoot Region}}},
  author = {Fisher, George H. and McClymont, Alexander N. and Chou, Dean-Yi},
  year = {1991},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {374},
  pages = {766},
  issn = {0004-637X},
  doi = {10.1086/170161},
  urldate = {2023-10-18},
  abstract = {The present study examines the fate of a magnetic flux tube initially lying at the bottom of the solar convective overshoot region. Stretching of the flux tube, e.g., by differential rotation, reduces its density, causing it to rise quasi-statically (a process referred to as vertical flux drift) until it reaches the top of the overshoot region and enters the buoyantly unstable convection region, from which a portion of it may ultimately protrude to form an active region on the surface. It is suggested that vertical flux drift and flux destabilization are inevitable consequences of field amplification, and it is surmised that these phenomena should be considered in self-consistent models of solar and stellar dynamos operating in the overshoot region.},
  keywords = {Astronomical Models,Astrophysics,Boundary Layer Flow,Convective Heat Transfer,Magnetic Field Configurations,Magnetic Flux,Solar Activity,Solar Cycles,STARS: INTERIORS,Stellar Interiors,SUN: ACTIVITY,SUN: INTERIOR},
  annotation = {ADS Bibcode: 1991ApJ...374..766F},
  file = {/Users/lbugnet/Zotero/storage/8MXC46JS/Fisher et al. - 1991 - The Stretching of Magnetic Flux Tubes in the Conve.pdf}
}

@article{Fletcher2006a,
  title = {Frequency, Splitting, Linewidth and Amplitude Estimates of Low-{$\mathscr{l}$} p Modes of {$\alpha$} {{Cen A}}: {{Analysis}} of Wide-Field Infrared Explorer Photometry},
  author = {Fletcher, S. T. and Chaplin, W. J. and Elsworth, Y. and Schou, J. and Buzasi, D.},
  year = {2006},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {371},
  number = {2},
  pages = {935--944},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2006.10727.x},
  abstract = {We present results of fitting the 50-d time series of photometry of {$\alpha$} Cen A taken by the Wide-Field Infrared Explorer (WIRE) satellite in 1999. Both power spectrum and autocovariance function (ACF) fitting techniques were used in an attempt to determine mode frequencies, rotational splittings, lifetimes and amplitudes of low-{$\mathscr{l}$} p modes. In all, using both techniques, we managed to fit 18 modes (seven {$\mathscr{l}$} = 0, eight {$\mathscr{l}$} = 1 and three {$\mathscr{l}$} = 2) with frequencies determined to within 1-2 {$\mu$}Hz. These estimates are shown to be 0.6 {$\pm$} 0.3 {$\mu$}Hz lower, on average, than the frequencies determined from two other more recent studies, which used data gathered about 19 months after the WIRE observations. This could be indicative of an activity cycle, although due to the large uncertainty, more data would be needed to confirm this. Over a range of 1700-2650 {$\mu$}Hz, we were also able to use the ACF fitting to determine an average lifetime of 3.9 {$\pm$} 1.4 d, and an average rotational splitting of 0.54 {$\pm$} 0.22 {$\mu$}Hz, which is the first ever reliable estimate of this parameter. In contrast to the ACF, the power spectrum fitting was shown to return significantly biased results for these parameters. \textcopyright{} 2006 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/JE94TXEW/Fletcher et al. - 2006.pdf}
}

@article{Fletcher2008,
  title = {A Modified Peak-Bagging Technique for Fitting Low-{$\mathscr{l}$} Solar p-Modes},
  author = {Fletcher, S. T. and Chaplin, W. J. and Elsworth, Y. and New, R.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  pages = {447--452},
  issn = {00046337},
  doi = {10.1002/asna.200710978},
  abstract = {We introduce a modified version of a standard power spectrum 'peak-bagging' technique which is designed to gain some of the advantages that fitting the entire low-degree p-mode power spectrum simultaneously would bring, but without the problems involved in fitting a model incorporating many hundreds of parameters. Employing Monte-Carlo simulations we show that by using this modified fitting code it is possible to determine the true background level in the vicinity of the p-mode peaks. In addition to this we show how small biases in other mode parameters, which are related to inaccurate estimates of the true background, are also consequently removed. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {Methods: Data analysis,notion,notion-database,Sun: Helioseismology},
  file = {/Users/lbugnet/Zotero/storage/LIQGJ9HL/Fletcher et al. - 2008.pdf}
}

@article{Fletcher2009,
  title = {Efficient Pseudo-Global Fitting for Helioseismic Data},
  author = {Fletcher, S. T. and Chaplin, W. J. and Elsworth, Y. and New, Roger},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {694},
  number = {1},
  pages = {144--150},
  issn = {15384357},
  doi = {10.1088/0004-637X/694/1/144},
  abstract = {Mode fitting or "peak bagging" is an important procedure in helioseismology allowing one to determine the various mode parameters of solar oscillations. Here we describe a way of reducing the systematic bias in the fits of certain mode parameters that are seen when using "local" fitting techniques to analyze the Sun-as-a-star p-mode power spectrum. To do this we have developed a new "pseudo-global" fitting algorithm designed to gain the advantages of fitting the entire power spectrum, but without the problems involved in fitting a model incorporating many hundreds of parameters. We have performed a comparative analysis between the local and pseudo-global peak-bagging techniques by fitting the "limit" profiles of simulated helioseismic data. Results show that for asymmetric modes the traditional fitting technique returns systematically biased estimates of the central frequency parameter. This bias is significantly reduced when employing the pseudo-global routine. Similarly, we show that estimates of the background returned from the pseudo-global routine match the input values much more closely than the estimates from the local fitting method. We have also used the two fitting techniques to analyze a set of real solar data collected by the Global Oscillations at Low Frequencies instrument on board the ESA/NASA Solar and Heliospheric Observatory spacecraft. Similar differences between the estimated frequencies returned by the two techniques are seen when fitting both the real and simulated data. We show that the background fits returned by the pseudo-global routine more closely match the estimate of the background one can infer from interpolating between fits to the high and low frequency ends of the p-mode power spectrum. \textcopyright{} 2009. The American Astronomical Society.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/AWBE67XY/Fletcher et al. - 2009.pdf}
}

@article{Fletcher2010,
  title = {A Seismic Signature of a Second Dynamo?},
  author = {Fletcher, Stephen T. and Broomhall, Anne Marie and Salabert, David and Basu, Sarbani and Chaplin, William J. and Elsworth, Yvonne and Garcia, Rafael A. and New, Roger},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {718},
  number = {1 PART 2},
  pages = {19--22},
  issn = {20418213},
  doi = {10.1088/2041-8205/718/1/L19},
  abstract = {The Sun is a variable star whose magnetic activity varies most perceptibly on a timescale of approximately 11 years. However, significant variation is also observed on much shorter timescales. We observe a quasi-biennial (2 year) signal in the natural oscillation frequencies of the Sun. The oscillation frequencies are sensitive probes of the solar interior and so by studying them we can gain information about conditions beneath the solar surface. Our results strongly point to the 2 year signal being distinct and separate from, but nevertheless susceptible to the influence of, the main 11 year solar cycle. \textcopyright{} 2010. The American Astronomical Society. All rights reserved..},
  keywords = {methods: data analysis,notion,notion-database,Sun: activity,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4KQ9DGVQ/Fletcher et al. - 2010.pdf}
}

@article{Floranes2005a,
  title = {The Use of Frequency-Separation Ratios for Asteroseismology},
  author = {Floranes, H. Ot{\'i} and {Christensen-Dalsgaard}, J. and Thompson, M. J.},
  year = {2005},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {356},
  number = {2},
  pages = {671--679},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2004.08487.x},
  abstract = {The systematic patterns of separations between frequencies of modes of different degree and order are a characteristic of p-mode oscillations of stars. The frequency separations depend on the internal structure of the star and so measuring them in the observed oscillation spectra of variable stars gives valuable diagnostics of the interior of a star. Roxburgh \& Vorontsov proposed using the ratio of the so-called small frequency separation to the large frequency separation as a diagnostic of the stellar interior, and demonstrated that this ratio was less sensitive than the individual frequency separations themselves to uncertain details of the nearsurface structure. Here we derive kernels relating the frequency separation ratio to structure, and show why the ratio is relatively insensitive to the near-surface structure in terms of the very small amplitude of the kernels in the near-surface layers. We also investigate the behaviour of the separation ratio for stars of different masses and ages, and demonstrate the usefulness of the ratio in the so-called asteroseismic Hertzsprung-Russell diagram.},
  keywords = {notion,notion-database,Stars: interiors,Stars: variables: other,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WPYVHQDY/Floranes, Christensen-Dalsgaard, Thompson - 2005.pdf}
}

@article{Flowers1977,
  title = {Evolution of Pulsar Magnetic Fields},
  author = {Flowers, E. and Ruderman, M. A.},
  year = {1977},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {215},
  pages = {302},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/155359},
  urldate = {2020-07-03},
  abstract = {Theoretical considerations of neutron star matter and magnetic fields suggest a picture of the evolution of pulsar dipole moments. At birth the spin axis and magnetic dipole are argued to be roughly aligned. Subsequently the magnetic dipole greatly diminishes in strength and changes its direction until it ultimately makes a large angle with the spin axis. This view is supported by observations of pulsar subpulse drifting and the relation of pulsar periods to spin-down rates.},
  keywords = {Astrophysics,Dipole Moments,Magnetic Effects,Magnetic Field Configurations,Magnetic Flux,Neutron Stars,notion,notion-database,Pulsars,Stellar Evolution,Stellar Magnetic Fields,Stellar Rotation}
}

@article{Foing2021,
  title = {{{CHARACTERIZING EXOPLANET TRANSITS AND STELLAR ACTIVITY IN KEPLER LIGHTCURVES WITH SCALABLE GAUSSIAN PROCESSES}}},
  author = {Foing, V and Heras, A M and Foing, B},
  year = {2021},
  journal = {52nd Lunar and Planetary Science Conference 2021},
  doi = {10.5281/zenodo.1998447},
  urldate = {2022-01-09},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WNDYJVYN/full-text.pdf}
}

@article{Folsom2016,
  title = {The Evolution of Surface Magnetic Fields in Young Solar-Type Stars - {{I}}. {{The}} First 250 {{Myr}}},
  author = {Folsom, C. P. and Petit, P. and Bouvier, J. and L{\`e}bre, A. and Amard, L. and Palacios, A. and Morin, J. and Donati, J. F. and Jeffers, S. V. and Marsden, S. C. and Vidotto, A. A.},
  year = {2016},
  month = jan,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {457},
  number = {1},
  eprint = {1601.00684},
  pages = {580--607},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stv2924},
  urldate = {2020-07-13},
  abstract = {The surface rotation rates of young solar-type stars vary rapidly with age from the end of the pre-main sequence through the early main sequence. Important changes in the dynamos operating in these stars may result from this evolution, which should be observable in their surface magnetic fields. Here we present a study aimed at observing the evolution of these magnetic fields through this critical time period.We observed stars in open clusters and stellar associations of known ages, and used Zeeman Doppler imaging to characterize their complex magnetic large-scale fields. Presented here are results for 15 stars, from five associations, with ages from 20 to 250 Myr, masses from 0.7 to 1.2M{$\odot$}, and rotation periods from 0.4 to 6 d. We find complex large-scale magnetic field geometries, with global average strengths from 14 to 140 G. There is a clear trend towards decreasing average large-scale magnetic field strength with age, and a tight correlation between magnetic field strength and Rossby number. Comparing the magnetic properties of our zero-age main-sequence sample to those of both younger and older stars, it appears that the magnetic evolution of solar-type stars during the pre-main sequence is primarily driven by structural changes, while it closely follows the stars' rotational evolution on the main sequence.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: formation,Stars: imaging,Stars: magnetic field,Stars: rotation,Stars: solar-type,Techniques: polarimetric},
  file = {/Users/lbugnet/Zotero/storage/5Y2U2AVK/full-text.pdf}
}

@article{Folsom2018,
  title = {The Evolution of Surface Magnetic Fields in Young Solar-Type Stars {{II}}: {{The}} Early Main Sequence (250-650 {{Myr}})},
  author = {Folsom, C. P. and Bouvier, J. and Petit, P. and L{\`e}bre, A. and Amard, L. and Palacios, A. and Morin, J. and Donati, J. F. and Vidotto, A. A.},
  year = {2018},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {474},
  number = {4},
  eprint = {1711.08636},
  pages = {4956--4987},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stx3021},
  urldate = {2020-07-13},
  abstract = {There is a large change in surface rotation rates of sun-like stars on the pre-main sequence and early main sequence. Since these stars have dynamo-driven magnetic fields, this implies a strong evolution of their magnetic properties over this time period. The spin-down of these stars is controlled by interactions between stellar and magnetic fields, thus magnetic evolution in turn plays an important role in rotational evolution. We present here the second part of a study investigating the evolution of large-scale surface magnetic fields in this critical time period. We observed stars in open clusters and stellar associations with known ages between 120 and 650 Myr, and used spectropolarimetry and Zeeman Doppler Imaging to characterize their large-scale magnetic field strength and geometry. We report 15 stars with magnetic detections here. These stars have masses from 0.8 to 0.95 M{$\odot$}, rotation periods from 0.326 to 10.6 d, and we find large-scale magnetic field strengths from 8.5 to 195G with a wide range of geometries. We find a clear trend towards decreasing magnetic field strength with age, and a power law decrease in magnetic field strength with Rossby number. There is some tentative evidence for saturation of the large-scale magnetic field strength at Rossby numbers below 0.1, although the saturation point is not yet well defined. Comparing to younger classical T Tauri stars, we support the hypothesis that differences in internal structure produce large differences in observed magnetic fields, however for weak-lined T Tauri stars this is less clear.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: formation,Stars: imaging,Stars: magnetic fields,Stars: rotation,Stars: solar-type,Techniques: polarimetric}
}

@article{Fontaine2003,
  title = {A {{Driving Mechanism}} for the {{Newly Discovered Long}}-{{Period Pulsating Subdwarf B Stars}}},
  author = {Fontaine, G. and Brassard, P. and Charpinet, S. and Green, E. M. and Chayer, P. and Billeres, M. and Randall, S. K.},
  year = {2003},
  month = nov,
  journal = {The Astrophysical Journal},
  volume = {597},
  number = {1},
  pages = {518--534},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/378270},
  urldate = {2020-04-09},
  abstract = {We present the results of a stability survey carried out for a sequence of representative models of subdwarf B stars spanning the range of effective temperature 22; 000 K T eff 38; 000 K. We show that long-period, high-order g-modes are excited in the cooler models through the same -mechanism that successfully explains the presence of short-period, low-order p-modes in the hotter EC 14026 pulsators. This is analogous to the case of the Cep/slowly pulsating B stars on the main sequence. We stress that radiative levitation is needed to boost the iron abundance in the driving region for both types of pulsating subdwarf B stars. And indeed, we find that pulsation modes cannot be excited in B subdwarf models if the metallicity is assumed to be uniform and solar. On the basis of our current models, we propose that the pulsation modes detected in long-period pulsating subdwarf B stars have values of the degree index l {$\frac{1}{4}$} 3 and/or 4, not the canonical values l {$\frac{1}{4}$} 1; 2, a suggestion that is, in principle, testable through multicolor photometry or time-resolved spectros-copy. In this way, we are able to explain quite well, at least at the qualitative level, the main observed characteristics of these pulsators. On the first account, the excited high-order g-modes with l {$\frac{1}{4}$} 3 and 4 in our models have periods that overlap with the range of quasi-periods observed in these stars. On the second account, if the observable modes in these pulsators have indeed such '' high '' values of l as we suggest, we find a natural explanation for the fact that their amplitudes are distinctly and systematically smaller than the amplitudes observed in EC 14026 stars. Finally, our results are also consistent with the observed fact that the long-period pulsators appear systematically cooler than the short-period EC 14026 stars. We point out, however, that our analysis suggests effective temperatures for the long-period B subdwarf pulsators that are somewhat lower than current spectroscopic estimates. The solution to this problem may come from future improvements in the models, the establishment of an effective temperature scale for subdwarf B stars that is free of systematic effects, or both.},
  keywords = {Branch,notion,notion-database,Stars: Horizontal,Stars: Interiors,Stars: Oscillations,Stars: Subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/YLVLBPTF/full-text.pdf}
}

@article{Fontaine2013,
  title = {An Overview of White Dwarf Stars},
  author = {Fontaine, G. and Brassard, P. and Charpinet, S. and Randall, S.K. and Van Grootel, V.},
  editor = {Montalb{\'a}n, J. and Noels, A. and Van Grootel, V.},
  year = {2013},
  journal = {EPJ Web of Conferences},
  volume = {43},
  pages = {05001},
  issn = {2100-014X},
  doi = {10.1051/epjconf/20134305001},
  urldate = {2023-10-02},
  abstract = {We present a brief summary of what is currently known about white dwarf stars, with an emphasis on their evolutionary and internal properties. As is well known, white dwarfs represent the end products of stellar evolution for the vast majority of stars and, as such, bear the signatures of past events (such as mass loss, mixing phases, loss and redistribution of angular momentum, and thermonuclear burning) that are of essential importance in the evolution of stars in general. In addition, white dwarf stars represent ideal testbeds for our understanding of matter under extreme conditions, and work on their constitutive physics (neutrino production rates, conductive and radiative opacities, interior liquid/solid equations of state, partially ionized and partially degenerate envelope equations of state, diffusion coefficients, line broadening mechanisms) is still being actively pursued. Given a set of constitutive physics, cooling white dwarfs can be used advantageously as cosmochronometers. Moreover, the field has been blessed by the existence of four distinct families of pulsating white dwarfs, each mapping a different evolutionary phase, and this allows the application of the asteroseismological method to probe and test their internal structure and evolutionary state. We set the stage for the reviews that follow on cooling white dwarfs as cosmochronometers and physics laboratories, as well as on the properties of pulsating white dwarfs and the asteroseismological results that can be inferred.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/PIURL4NU/Fontaine et al. - 2013 - An overview of white dwarf stars.pdf}
}

@article{Foreman-Mackey2013,
  title = {Emcee : {{The MCMC Hammer}}},
  author = {{Foreman-Mackey}, Daniel and Hogg, David W. and Lang, Dustin and Goodman, Jonathan},
  year = {2013},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {125},
  number = {925},
  eprint = {1202.3665},
  pages = {306--312},
  issn = {00046280},
  doi = {10.1086/670067},
  abstract = {We introduce a stable, well tested Python implementation of the affine-invariant ensemble sampler for Markov chain Monte Carlo (MCMC) proposed by Goodman \& Weare (2010). The code is open source and has already been used in several published projects in the astrophysics literature. The algorithm behind emcee has several advantages over traditional MCMC sampling methods and it has excellent performance as measured by the autocorrelation time (or function calls per independent sample). One major advantage of the algorithm is that it requires hand-tuning of only 1 or 2 parameters compared to \$\textbackslash sim N\^2\$ for a traditional algorithm in an N-dimensional parameter space. In this document, we describe the algorithm and the details of our implementation and API. Exploiting the parallelism of the ensemble method, emcee permits any user to take advantage of multiple CPU cores without extra effort. The code is available online at http://dan.iel.fm/emcee under the MIT License.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YX2HA7PG/Foreman-Mackey et al. - 2013.pdf}
}

@article{ForemanMackey2019,
  title = {Emcee v3: {{A Python}} Ensemble Sampling Toolkit for Affine-Invariant {{MCMC}}},
  author = {{Foreman-Mackey}, Daniel and Farr, Will and Sinha, Manodeep and Archibald, Anne and Hogg, David and Sanders, Jeremy and Zuntz, Joe and Williams, Peter and Nelson, Andrew and {de Val-Borro}, Miguel and Erhardt, Tobias and Pashchenko, Ilya and Pla, Oriol},
  year = {2019},
  month = nov,
  journal = {Journal of Open Source Software},
  volume = {4},
  number = {43},
  eprint = {1911.07688},
  pages = {1864},
  publisher = {{The Open Journal}},
  issn = {2475-9066},
  doi = {10.21105/joss.01864},
  urldate = {2021-12-22},
  abstract = {emcee is a Python library implementing a class of affine-invariant ensemble samplers for Markov chain Monte Carlo (MCMC). This package has been widely applied to probabilistic modeling problems in astrophysics where it was originally published, with some applications in other fields. When it was first released in 2012, the interface implemented in emcee was fundamentally different from the MCMC libraries that were popular at the time, such as PyMC, because it was specifically designed to work with "black box" models instead of structured graphical models. This has been a popular interface for applications in astrophysics because it is often non-trivial to implement realistic physics within the modeling frameworks required by other libraries. Since emcee's release, other libraries have been developed with similar interfaces, such as dynesty (Speagle 2019). The version 3.0 release of emcee is the first major release of the library in about 6 years and it includes a full re-write of the computational backend, several commonly requested features, and a set of new "move" implementations.},
  archiveprefix = {arxiv},
  keywords = {astronomy,Astrophysics,Computation,Instrumentation and Methods for Astrophysics,notion,notion-database,Python,Statistics},
  file = {/Users/lbugnet/Zotero/storage/743YHUHA/full-text.pdf}
}

@article{ForemanMackey2019,
  title = {Exoplanet: {{Probabilistic}} Modeling of Transit or Radial Velocity Observations of Exoplanets},
  author = {{Foreman-Mackey}, Dan and {Foreman-Mackey} and {Dan}},
  year = {2019},
  journal = {ascl},
  pages = {ascl:1910.005},
  urldate = {2022-01-09},
  keywords = {notion,notion-database,Software}
}

@article{Fossat1991,
  title = {The {{IRIS}} Network for Full Disk Helioseismology: {{Present}} Status of the Programme},
  author = {Fossat, Eric},
  year = {1991},
  journal = {Solar Physics},
  volume = {133},
  number = {1},
  pages = {1--12},
  issn = {00380938},
  doi = {10.1007/BF00149818},
  abstract = {IRIS (International Research on the Interior of the Sun) is the name of a worldwide network of 8 observing stations for full disk helioseismology. The IRIS scientific community is organizing a yearly workshop in one of the 8 sites. This paper is the introduction to the proceedings of the second IRIS workshop, held at Tashkent, Uzbekistan SSR. It presents a brief history, the structure of the international cooperation, the membership rule, the list of sites and members, the scientific working teams additional structure and, as an appendix, the report of the first meeting of the IRIS Scientific Committee. \textcopyright{} 1991 Kluwer Academic Publishers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Z7M8G2MT/Fossat - 1991.pdf}
}

@article{Fossat2017a,
  title = {Asymptotic g Modes: {{Evidence}} for a Rapid Rotation of the Solar Core},
  author = {Fossat, E. and Boumier, P. and Corbard, T. and Provost, J. and Salabert, D. and Schmider, F. X. and Gabriel, A. H. and Grec, G. and Renaud, C. and Robillot, J. M. and {Roca-Cort{\'e}s}, T. and {Turck-Chi{\`e}ze}, S. and Ulrich, R. K. and Lazrek, M.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {604},
  eprint = {1708.00259},
  issn = {14320746},
  doi = {10.1051/0004-6361/201730460},
  abstract = {Context. Over the past 40 years, helioseismology has been enormously successful in the study of the solar interior. A shortcoming has been the lack of a convincing detection of the solar g modes, which are oscillations driven by gravity and are hidden in the deepest part of the solar body - its hydrogen-burning core. The detection of g modes is expected to dramatically improve our ability to model this core, the rotational characteristics of which have, until now, remained unknown. Aims. We present the identification of very low frequency g modes in the asymptotic regime and two important parameters that have long been waited for: the core rotation rate, and the asymptotic equidistant period spacing of these g modes. Methods. The GOLF instrument on board the SOHO space observatory has provided two decades of full-disk helioseismic data. The search for g modes in GOLF measurements has been extremely difficult because of solar and instrumental noise. In the present study, the p modes of the GOLF signal are analyzed differently: we search for possible collective frequency modulations that are produced by periodic changes in the deep solar structure. Such modulations provide access to only very low frequency g modes, thus allowing statistical methods to take advantage of their asymptotic properties. Results. For oscillatory periods in the range between 9 and nearly 48 h, almost 100 g modes of spherical harmonic degree 1 and more than 100 g modes of degree 2 are predicted. They are not observed individually, but when combined, they unambiguously provide their asymptotic period equidistance and rotational splittings, in excellent agreement with the requirements of the asymptotic approximations. When the period equidistance has been measured, all of the individual frequencies of each mode can be determined. Previously, p-mode helioseismology allowed the g-mode period equidistance parameter P0 to be bracketed inside a narrow range, between approximately 34 and 35 min. Here, P0 is measured to be 34 min 01 s, with a 1 s uncertainty. The previously unknown g-mode splittings have now been measured from a non-synodic reference with very high accuracy, and they imply a mean weighted rotation of 1277 {$\pm$} 10 nHz (9-day period) of their kernels, resulting in a rapid rotation frequency of 1644 {$\pm$} 23 nHz (period of one week) of the solar core itself, which is a factor 3.8 {$\pm$} 0.1 faster than the rotation of the radiative envelope. Conclusions. The g modes are known to be the keys to a better understanding of the structure and dynamics of the solar core. Their detection with these precise parameters will certainly stimulate a new era of research in this field.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Fossat2018,
  title = {Astronomy {{More}} about Solar g Modes},
  author = {Fossat, E and Schmider, F X},
  year = {2018},
  journal = {Astronomy \& Astrophysics},
  volume = {612},
  pages = {1},
  doi = {10.1051/0004-6361/201832626},
  urldate = {2020-07-29},
  abstract = {Context. The detection of asymptotic solar g-mode parameters was the main goal of the GOLF instrument onboard the SOHO space observatory. This detection has recently been reported and has identified a rapid mean rotation of the solar core, with a one-week period, nearly four times faster than all the rest of the solar body, from the surface to the bottom of the radiative zone. Aims. We present here the detection of more g modes of higher degree, and a more precise estimation of all their parameters, which will have to be exploited as additional constraints in modeling the solar core. Methods. Having identified the period equidistance and the splitting of a large number of asymptotic g modes of degrees 1 and 2, we test a model of frequencies of these modes by a cross-correlation with the power spectrum from which they have been detected. It shows a high correlation peak at lag zero, showing that the model is hidden but present in the real spectrum. The model parameters can then be adjusted to optimize the position (at exactly zero lag) and the height of this correlation peak. The same method is then extended to the search for modes of degrees 3 and 4, which were not detected in the previous analysis. Results. g-mode parameters are optimally measured in similar-frequency bandwidths, ranging from 7 to 8 \textmu Hz at one end and all close to 30 \textmu Hz at the other end, for the degrees 1 to 4. They include the four asymptotic period equidistances, the slight departure from equidistance of the detected periods for l = 1 and l = 2, the measured amplitudes, functions of the degree and the tesseral order, and the splittings that will possibly constrain the estimated sharpness of the transition between the one-week mean rotation of the core and the almost four-week rotation of the radiative envelope. The g-mode periods themselves are crucial inputs in the solar core structure helioseismic investigation.},
  keywords = {helioseismology-Sun,interior-Sun,notion,notion-database,oscillations,rotation-Sun,Sun},
  file = {/Users/lbugnet/Zotero/storage/WT5MVDJ3/full-text.pdf}
}

@article{Frandsen2002,
  title = {Detection of Solar-like Oscillations in the {{G7}} Giant Star {$\xi$} {{Hya}}},
  author = {Frandsen, S. and Carrier, F. and Aerts, C. and Stello, D. and Maas, T. and Burnet, M. and Bruntt, H. and Teixeira, T. C. and De Medeiros, J. R. and Bouchy, F. and Kjeldsen, H. and Pijpers, F. and {Christensen-Dalsgaard}, J.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {394},
  number = {1},
  pages = {8--11},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021281},
  abstract = {We report the firm discovery of solar-like oscillations in a giant star. We monitored the star {$\xi$} Hya (G7III) continuously during one month with the CORALIE spectrograph attached to the 1.2 m Swiss Euler telescope. The 433 high-precision radial-velocity measurements clearly reveal multiple oscillation frequencies in the range 50-130 {$\mu$}Hz, corresponding to periods between 2.0 and 5.5 hours. The amplitudes of the strongest modes are slightly smaller than 2 m s-1. Current model calculations are compatible with the detected modes.},
  keywords = {Asteroseismology,Giant stars,notion,notion-database,Solar type oscillations},
  file = {/Users/lbugnet/Zotero/storage/4A38HT6U/Frandsen et al. - 2002.pdf}
}

@article{Frankowski2007,
  title = {Proper-Motion Binaries in the {{Hipparcos}} Catalogue: {{Comparison}} with Radial Velocity Data},
  author = {Frankowski, A. and Jancart, S. and Jorissen, A.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {464},
  number = {1},
  pages = {377--392},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065526},
  abstract = {Context. This paper is the last in a series devoted to the analysis of the binary content of the Hipparcos Catalogue. Aims. The comparison of the proper motions constructed from positions spanning a short (Hipparcos) or long time (Tycho-2) makes it possible to uncover binaries with periods of the order of or somewhat larger than the short time span (in this case, the 3 yr duration of the Hipparcos mission), since the unrecognised orbital motion will then add to the proper motion. Methods. A list of candidate proper motion binaries is constructed from a carefully designed {$\chi$}2 test evaluating the statistical significance of the difference between the Tycho-2 and Hipparcos proper motions for 103 134 stars in common between the two catalogues (excluding components of visual systems). Since similar lists of proper-motion binaries have already been constructed, the present paper focuses on the evaluation of the detection efficiency of proper-motion binaries, using different kinds of control data (mostly radial velocities). The detection rate for entries from the Ninth Catalogue of Spectroscopic Binary Orbits (SB9) is evaluated, as well as for stars like barium stars, which are known to be all binaries, and finally for spectroscopic binaries identified from radial velocity data in the Geneva-Copenhagen survey of F and G dwarfs in the solar neighbourhood. Results. Proper motion binaries are efficiently detected for systems with parallaxes in excess of {$\sim$}20 mas, and periods in the range 1000-30 000 d. The shortest periods in this range (1000-2000 d, i.e., once to twice the duration of the Hipparcos mission) may appear only as DMSA/G binaries (accelerated proper motion in the Hipparcos Double and Multiple System Annex). Proper motion binaries detected among SB9 systems having periods shorter than about 400 d hint at triple systems, the proper-motion binary involving a component with a longer orbital period. A list of 19 candidate triple systems is provided. Binaries suspected of having low-mass (brown-dwarf-like) companions are listed as well. Among the 37 barium stars with parallaxes larger than 5 mas, only 7 exhibit no evidence for duplicity whatsoever (be it spectroscopic or astrometric). Finally, the fraction of proper-motion binaries shows no significant variation among the various (regular) spectral classes, when due account is taken for the detection biases. \textcopyright{} ESO 2007.},
  keywords = {Astrometry,Binaries: general,Binaries: spectroscopic,Binaries: visual,Catalogs,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6MH9REVG/Frankowski, Jancart, Jorissen - 2007.pdf}
}

@article{Frasca2011,
  title = {Magnetic Activity and Differential Rotation in the Very Young Star {{KIC}} 8429280},
  author = {Frasca, A. and Fr{\"o}hlich, H. E. and Bonanno, A. and Catanzaro, G. and Biazzo, K. and {Molenda-Zakowicz}, J.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {532},
  pages = {1--12},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116980},
  abstract = {Aims. We present a spectroscopic and photometric analysis of the rapid rotator KIC 8429280, discovered by ourselves as a very young star and observed by the NASA Kepler mission, designed to determine its activity level, spot distribution, and differential rotation. Methods. We use ground-based data, such as high-resolution spectroscopy and multicolor broad-band photometry, to derive stellar parameters (vsini, spectral type, T eff , log g, and [Fe/H]), and we adopt a spectral subtraction technique to highlight the strong chromospheric emission in the cores of hydrogen H{$\alpha$} and Ca ii H\&K and infrared triplet (IRT) lines. We then fit a robust spot model to the high-precision Kepler photometry spanning 138 days. Model selection and parameter estimation is performed in a Bayesian manner using a Markov chain Monte Carlo method. Results. We find that KIC 8429280 is a cool (K2 V) star with an age of about 50 Myr, based on its lithium content, that has passed its T Tau phase and is spinning up approaching the ZAMS on its radiative track. Its high level of chromospheric activity is clearly indicated by the strong radiative losses in Ca ii H\&K and IRT, H{$\alpha$}, and H{$\beta$} lines. Furthermore, its Balmer decrement and the flux ratio of Ca ii IRT lines imply that these lines are mainly formed in optically-thick regions similar to solar plages. The analysis of the Kepler data uncovers evidence of at least seven enduring spots. Since the star's inclination is rather high-nearly 70\textdegree -the assignment of the spots to either the northern or southern hemisphere is not unambiguous. We find at least three solutions with nearly the same level of residuals. Even in the case of seven spots, the fit is far from being perfect. Owing to the exceptional precision of the Kepler photometry, it is not possible to reach the noise floor without strongly enhancing the degrees of freedom and, consequently, the non-uniqueness of the solution. The distribution of the active regions is such that the spots are located around three latitude belts, i.e. around the star's equator and around {$\pm$} (50\textdegree -60\textdegree ), with the high-latitude spots rotating slower than the low-latitude ones. The equator-to-pole differential rotation d{$\Omega$} \^a\textperthousand{} 0.27 rad d -1 is at variance with some recent mean-field models of differential rotation in rapidly rotating main-sequence stars, which predict a much smaller latitudinal shear. Our results are consistent with the scenario of a higher differential rotation, which changes along the magnetic cycle, as proposed by other models. \textcopyright{} 2011 ESO.},
  keywords = {notion,notion-database,stars: activity,stars: chromospheres,stars: individual: KIC 8429280,stars: rotation,starspots,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/KG4DHYSA/Frasca et al. - 2011.pdf}
}

@article{Frasca2016,
  title = {Activity Indicators and Stellar Parameters of the {{Kepler}} Targets: {{An}} Application of the {{ROTFIT}} Pipeline to {{LAMOST-Kepler}} Stellar Spectra},
  author = {Frasca, A. and {Molenda-Zakowicz}, J. and De Cat, P. and Catanzaro, G. and Fu, J. N. and Ren, A. B. and Luo, A. L. and Shi, J. R. and Wu, Y. and Zhang, H. T.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {594},
  eprint = {1606.09149},
  pages = {1--31},
  issn = {14320746},
  doi = {10.1051/0004-6361/201628337},
  abstract = {Aims. A comprehensive and homogeneous determination of stellar parameters for the stars observed by the Kepler space telescope is necessary for statistical studies of their properties. As a result of the large number of stars monitored by Kepler, the largest and more complete databases of stellar parameters published to date are multiband photometric surveys. The LAMOST-Kepler survey, whose spectra are analyzed in the present paper, was the first large spectroscopic project, which started in 2011 and aimed at filling that gap. In this work we present the results of our analysis, which is focused on selecting spectra with emission lines and chromospherically active stars by means of the spectral subtraction of inactive templates. The spectroscopic determination of the atmospheric parameters for a large number of stars is a by-product of our analysis. Methods. We have used a purposely developed version of the code ROTFIT for the determination of the stellar parameters by exploiting a wide and homogeneous collection of real star spectra, namely the Indo US library. We provide a catalog with the atmospheric parameters (Teff, log g, and [Fe/H]), radial velocity (RV), and an estimate of the projected rotation velocity (v sin i). For cool stars (Teff {$\leq$} 6000 K), we also calculated the H and Ca ii-IRT fluxes, which are important proxies of chromospheric activity. Results. We have derived the RV and atmospheric parameters for 61 753 spectra of 51 385 stars. The average uncertainties, which we estimate from the stars observed more than once, are about 12 km s-1, 1.3\%, 0.05 dex, and 0.06 dex for RV, Teff, log g, and [Fe/H], respectively, although they are larger for the spectra with a very low signal-to-noise ratio. Literature data for a few hundred stars (mainly from high-resolution spectroscopy) were used to peform quality control of our results. The final accuracy of the RV is about 14 km s-1. The accuracy of the Teff, log g, and [Fe/H] measurements is about 3.5\%, 0.3 dex, and 0.2 dex, respectively. However, while the Te values are in very good agreement with the literature, we noted some issues with the determination of [Fe/H] of metal poor stars and the tendency, for log g, to cluster around the values typical for main-sequence and red giant stars.We propose correction relations based on these comparisons and we show that this does not have a significant effect on the determination of the chromospheric fluxes. The RV distribution is asymmetric and shows an excess of stars with negative RVs that are larger at low metallicities. Despite the rather low LAMOST resolution, we were able to identify interesting and peculiar objects, such as stars with variable RV, ultrafast rotators, and emission-line objects. Based on the H and Ca ii-IRT fluxes, we found 442 chromospherically active stars, one of which is a likely accreting object. The availability of precise rotation periods from the Kepler photometry allowed us to study the dependency of these chromospheric fluxes on the rotation rate for a very large sample of field stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: chromospheres,Stars: fundamental parameters,Stars: kinematics and dynamics,Surveys,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/UGCUQVEC/Frasca et al. - 2016.pdf}
}

@article{Fraser2022,
  title = {Characterizing {{Observed Extra Mixing Trends}} in {{Red Giants}} Using the {{Reduced Density Ratio}} from {{Thermohaline Models}}},
  author = {Fraser, Adrian E. and Joyce, Meridith and Anders, Evan H. and Tayar, Jamie and Cantiello, Matteo},
  year = {2022},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {941},
  pages = {164},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/aca024},
  urldate = {2023-10-18},
  abstract = {Observations show an almost ubiquitous presence of extra mixing in low-mass upper giant branch stars. The most commonly invoked explanation for this is thermohaline mixing. One-dimensional stellar evolution models include various prescriptions for thermohaline mixing, but the use of observational data directly to discriminate between thermohaline prescriptions has thus far been limited. Here, we propose a new framework to facilitate direct comparison: using carbon-to-nitrogen measurements from the Sloan Digital Sky Survey-IV APOGEE survey as a probe of mixing and a fluid parameter known as the reduced density ratio from one-dimensional stellar evolution programs, we compare the observed amount of extra mixing on the upper giant branch to predicted trends from three-dimensional fluid dynamics simulations. Using this method, we are able to empirically constrain how mixing efficiency should vary with the reduced density ratio. We find the observed amount of extra mixing is strongly correlated with the reduced density ratio and that trends between reduced density ratio and fundamental stellar parameters are robust across choices for modeling prescription. We show that stars with available mixing data tend to have relatively low density ratios, which should inform the regimes selected for future simulation efforts. Finally, we show that there is increased mixing at low reduced density ratios, which is consistent with current hydrodynamical models of thermohaline mixing. The introduction of this framework sets a new standard for theoretical modeling efforts, as validation for not only the amount of extra mixing, but trends between the degree of extra mixing and fundamental stellar parameters is now possible.},
  keywords = {101,11,1368,1369,1577,1599,1606,1963,409,Abundance ratios,Astrophysical fluid dynamics,Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,Dredge-up,Hydrodynamics,Physics - Plasma Physics,Red giant branch,Red giant bump,Stellar abundances,Stellar evolution,Stellar interiors},
  annotation = {ADS Bibcode: 2022ApJ...941..164F},
  file = {/Users/lbugnet/Zotero/storage/X6GXDLQ8/Fraser et al. - 2022 - Characterizing Observed Extra Mixing Trends in Red.pdf}
}

@article{Freeman2002,
  title = {The {{New Galaxy}}: {{Signatures}} of {{Its Formation}}},
  author = {Freeman, Ken and {Bland-Hawthorn}, Joss},
  year = {2002},
  month = sep,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {40},
  number = {1},
  eprint = {astro-ph/0208106},
  pages = {487--537},
  publisher = {{Annual Reviews}},
  issn = {0066-4146},
  doi = {10.1146/annurev.astro.40.060401.093840},
  urldate = {2020-03-06},
  abstract = {The formation and evolution of galaxies is one of the great outstanding problems of astrophysics. Within the broad context of hierachical structure formation, we have only a crude picture of how galaxies like our own came into existence. A detailed physical picture where individual stellar populations can be associated with (tagged to) elements of the protocloud is far beyond our current understanding. Important clues have begun to emerge from both the Galaxy (near-field cosmology) and the high redshift universe (far-field cosmology). Here we focus on the fossil evidence provided by the Galaxy. Detailed studies of the Galaxy lie at the core of understanding the complex processes involved in baryon dissipation. This is a necessary first step towards achieving a successful theory of galaxy formation.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,local group,notion,notion-database,osmology,stellar kinematics,stellar populations}
}

@inproceedings{Freytag1997,
  title = {On the {{Scale}} of {{Photospheric Convection}}},
  booktitle = {Science with the {{VLT Interferometer}} : Proceedings of the {{ESO}} Workshop Held at {{Garching}}, {{Germany}}, 18-21 {{June}} 1996},
  author = {Freytag, B. and Holweger, H. and Steffen, M. and Ludwig, H. -G.},
  year = {1997},
  pages = {316},
  publisher = {{Springer}},
  urldate = {2020-03-16},
  isbn = {3-540-63264-6},
  keywords = {notion,notion-database}
}

@article{Friedman2001,
  title = {Greedy Function Approximation: {{A}} Gradient Boosting Machine.},
  author = {Friedman, Jerome H.},
  year = {2001},
  journal = {The Annals of Statistics},
  volume = {29},
  number = {5},
  pages = {1189--1232},
  publisher = {{Institute of Mathematical Statistics}},
  issn = {0090-5364},
  doi = {10.1214/AOS/1013203451},
  urldate = {2020-04-11},
  keywords = {boosting,decision trees,Function estimation,notion,notion-database,robust nonparametric regression}
}

@article{Friedman2002,
  title = {Stochastic Gradient Boosting},
  author = {Friedman, Jerome H.},
  year = {2002},
  month = feb,
  journal = {Computational Statistics and Data Analysis},
  volume = {38},
  number = {4},
  pages = {367--378},
  issn = {01679473},
  doi = {10.1016/S0167-9473(01)00065-2},
  urldate = {2020-04-11},
  abstract = {Gradient boosting constructs additive regression models by sequentially fitting a simple parameterized function (base learner) to current "pseudo" -residuals by least squares at each iteration. The pseudo-residuals are the gradient of the loss functional being minimized, with respect to the model values at each training data point evaluated at the current step. It is shown that both the approximation accuracy and execution speed of gradient boosting can be substantially improved by incorporating randomization into the procedure. Specifically, at each iteration a subsample of the training data is drawn at random (without replacement) from the full training data set. This randomly selected subsample is then used in place of the full sample to fit the base learner and compute the model update for the current iteration. This randomized approach also increases robustness against overcapacity of the base learner. \textcopyright{} 2002 Elsevier Science B.V. All rights reserved.},
  keywords = {notion,notion-database}
}

@article{Frohlich1995,
  title = {{{VIRGO}}: {{Experiment}} for Helioseismology and Solar Irradiance Monitoring},
  author = {Fr{\"o}hlich, Claus and Romero, Jos{\'e} and Roth, Hansj{\"o}rg and Wehrli, Christoph and Andersen, Bo N. and Appourchaux, Thierry and Domingo, Vicente and Telljohann, Udo and Berthomieu, Gabrielle and Delache, Philippe and Provost, Janine and Toutain, Thierry and Crommelynck, Dominique A. and Chevalier, Andr{\'e} and Fichot, Alain and D{\"a}ppen, Werner and Gough, Douglas and Hoeksema, Todd and Jim{\'e}nez, Antonio and G{\'o}mez, Maria F. and Herreros, Jos{\'e} M. and Cort{\'e}s, Teodoro Roca and Jones, Andrew R. and Pap, Judit M. and Willson, Richard C.},
  year = {1995},
  month = dec,
  journal = {Solar Physics},
  volume = {162},
  number = {1-2},
  pages = {101--128},
  publisher = {{Kluwer Academic Publishers}},
  issn = {00380938},
  doi = {10.1007/BF00733428},
  urldate = {2020-07-14},
  abstract = {The scientific objective of the VIRGO experiment (Variability of solar IRradiance and Gravity Oscillations) is to determine the characteristics of pressure and internal gravity oscillations by observing irradiance and radiance variations, to measure the solar total and spectral irradiance and to quantify their variability over periods of days to the duration of the mission. With these data helioseismological methods can be used to probe the solar interior. Certain characteristics of convection and its interaction with magnetic fields, related to, for example, activity, will be studied from the results of the irradiance monitoring and from the comparison of amplitudes and phases of the oscillations as manifest in brightness from VIRGO, in velocity from GOLF, and in both velocity and continuum intensity from SOI/MDI. The VIRGO experiment contains two different active-cavity radiometers for monitoring the solar 'constant', two three-channel sunphotometers (SPM) for the measurement of the spectral irradiance at 402, 500 and 862 nm, and a low-resolution imager (LOI) with 12 pixels, for the measurement of the radiance distribution over the solar disk at 500 um. In this paper the scientific objectives of VIRGO are presented, the instruments and the data acquisition and control system are described in detail, and their measured performance is given. \textcopyright{} 1995 Kluwer Academic Publishers.},
  keywords = {Helioseismology,Low-Resolution Solar Radiance,notion,notion-database,SOHO Mission,Spectral Solar Irradiance,Total Solar Irradiance}
}

@article{Frohlich1997a,
  title = {In-Flight Performance of the {{VIRGO}} Solar Irradiance Instruments on {{SOHO}}},
  author = {Fr{\"o}hlich, Claus and Crommelynck, Dominique A. and Wehrli, Christoph and Anklin, Martin and Dewitte, Steven and Fichot, Alain and Finsterle, Wolfgang and Jim{\'e}nez, Antonio and Chevalier, Andr{\'e} and Roth, Hansj{\"o}rg},
  year = {1997},
  journal = {Solar Physics},
  volume = {175},
  number = {2},
  pages = {267--286},
  issn = {00380938},
  doi = {10.1023/A:1004929108864},
  abstract = {The in-flight performance of the total and spectral irradiance instruments within VIRGO (Variability of solar IRradiance and Gravity Oscillations) on the ESA/NASA Mission SOHO (SOlar and Heliospheric Observatory) is in most aspects better than expected. The behaviour during the first year of operation of the two types of radiometers and the sunphotometers together with a description of their data evaluation procedures is presented.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2DYD7BF4/Fröhlich et al. - 1997.pdf}
}

@article{Frohlich2012,
  title = {Magnetic Activity and Differential Rotation in the Young {{Sun-like}} Stars {{KIC}} 7985370 and {{KIC}} 7765135},
  author = {Fr{\"o}hlich, H. E. and Frasca, A. and Catanzaro, G. and Bonanno, A. and Corsaro, E. and {Molenda-Zakowicz}, J. and Klutsch, A. and Montes, D.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {543},
  pages = {1--16},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219167},
  abstract = {Aims. We present a detailed study of the two Sun-like stars KIC 7985370 and KIC 7765135, to determine their activity level, spot distribution, and differential rotation. Both stars were previously discovered by us to be young stars and were observed by the NASA Kepler mission. Methods. The fundamental stellar parameters (vsini, spectral type, T eff, log g, and [Fe/H]) were derived from optical spectroscopy by comparison with both standard-star and synthetic spectra. The spectra of the targets allowed us to study the chromospheric activity based on the emission in the core of hydrogen H{$\alpha$} and Ca ii infrared triplet (IRT) lines, which was revealed by the subtraction of inactive templates. The high-precision Kepler photometric data spanning over 229 days were then fitted with a robust spot model. Model selection and parameter estimation were performed in a Bayesian manner, using a Markov chain Monte Carlo method. Results. We find that both stars are Sun-like (of G1.5 V spectral type) and have an age of about 100-200 Myr, based on their lithium content and kinematics. Their youth is confirmed by their high level of chromospheric activity, which is comparable to that displayed by the early G-type stars in the Pleiades cluster. The Balmer decrement and flux ratio of their Ca ii-IRT lines suggest that the formation of the core of these lines occurs mainly in optically thick regions that are analogous to solar plages. The spot model applied to the Kepler photometry requires at least seven persistent spots in the case of KIC 7985370 and nine spots in the case of KIC 7765135 to provide a satisfactory fit to the data. The assumption of the longevity of the star spots, whose area is allowed to evolve with time, is at the heart of our spot-modelling approach. On both stars, the surface differential rotation is Sun-like, with the high-latitude spots rotating slower than the low-latitude ones. We found, for both stars, a rather high value of the equator-to-pole differential rotation (d{$\Omega$} {$\approx$} 0.18 rad d -1), which disagrees with the predictions of some mean-field models of differential rotation for rapidly rotating stars. Our results agree instead with previous works on solar-type stars and other models that predict a higher latitudinal shear, increasing with equatorial angular velocity, that can vary during the magnetic cycle. \textcopyright{} 2012 ESO.},
  keywords = {notion,notion-database,Stars: activity,Stars: chromospheres,Stars: individual: KIC 7765135,Stars: individual: KIC 7985370,Stars: rotation,Starspots},
  file = {/Users/lbugnet/Zotero/storage/6JIP8VJ7/Fröhlich et al. - 2012.pdf}
}

@book{Froman2005,
  title = {Physical Problems Solved by the Phase-Integral Method},
  author = {Froman, Nanny and Froman, Per Olof},
  year = {2005},
  journal = {ppsp},
  publisher = {{ppsp}},
  urldate = {2020-06-20},
  abstract = {Title from publisher's bibliographic system (viewed on 05 Oct 2015). This book provides a thorough introduction to one of the most efficient approximation methods for the analysis and solution of problems in theoretical physics and applied mathematics. It is written with practical needs in mind and contains a discussion of 50 problems with solutions, of varying degrees of difficulty. The problems are taken from quantum mechanics, but the method has important applications in any field of science involving second order ordinary differential equations. The power of the asymptotic solution of second order differential equations is demonstrated, and in each case the authors clearly indicate which concepts and results of the general theory are needed to solve a particular problem. This book will be ideal as a manual for users of the phase-integral method, as well as a valuable reference text for experienced research workers and graduate students. 1. Historical survey -- 1.1. Development from 1817 to 1926 -- 1.2. Development after 1926 -- 2. Description of the phase-integral method -- 2.1. Form of the wave function and the q-equation -- 2.2. Phase-integral approximation generated from an unspecified base function -- 2.3. F-matrix method -- 2.4. F-matrix connecting points on opposite sides of a well-isolated turning point, and expressions for the wave function in these regions -- 2.5. Phase-integral connection formulas for a real, smooth, single-hump potential barrier -- 3. Problems with solutions -- 3.1. Base function for the radial Schrodinger equation when the physical potential has at the most a Coulomb singularity at the origin -- 3.2. Base function and wave function close to the origin when the physical potential is repulsive and strongly singular at the origin -- 3.3. Reflectionless potential -- 3.4. Stokes and anti-Stokes lines -- 3.5. Properties of the phase-integral approximation along an anti-Stokes line 3.6. Properties of the phase-integral approximation along a path on which the absolute value of exp[iw(z)] is monotonic in the strict sense, in particular along a Stokes line -- 3.7. Determination of the Stokes constants associated with the three anti-Stokes lines that emerge from a well isolated, simple transition zero -- 3.8. Connection formula for tracing a phase-integral wave function from a Stokes line emerging from a simple transition zero t to the anti-Stokes line emerging from t in the opposite direction -- 3.9. Connection formula for tracing a phase-integral wave function from an anti-Stokes line emerging from a simple transition zero t to the Stokes line emerging from t in the opposite direction -- 3.10. Connection formula for tracing a phase-integral wave function from a classically forbidden to a classically allowed region 3.11. One-directional nature of the connection formula for tracing a phase-integral wave function from a classically forbidden to a classically allowed region -- 3.12. Connection formulas for tracing a phase-integral wave function from a classically allowed to a classically forbidden region -- 3.13. One-directional nature of the connection formulas for tracing a phase-integral wave function from a classically allowed to a classically forbidden region -- 3.14. Value at the turning point of the wave function associated with the connection formula for tracing a phase-integral wave function from the classically forbidden to the classically allowed region -- 3.15. Value at the turning point of the wave function associated with a connection formula for tracing the phase-integral wave function from the classically allowed to the classically forbidden region -- 3.16. Illustration of the accuracy of the approximate formulas for the value of the wave function at a turning point 3.17. Expression for the a-coefficients associated with the Airy functions -- 3.18. Expressions for the parameters [alpha], [beta] and [gamma] when Q[superscript 2](z) = R(z) = -z -- 3.19. Solutions of the Airy differential equation that at a fixed point on one side of the turning point are represented by a single, pure phase-integral function, and their representation on the other side of the turning point -- 3.20. Connection formulas and their one-directional nature demonstrated for the Airy differential equation -- 3.21. Dependence of the phase of the wave function in a classically allowed region on the value of the logarithmic derivative of the wave function at a fixed point X[subscript 1] in an adjacent classically forbidden region -- 3.22. Phase of the wave function in the classically allowed regions adjacent to a real, symmetric potential barrier, when the logarithmic derivative of the wave function is given at the centre of the barrier 3.23. Eigenvalue problem for a quantal particle in a broad, symmetric potential well between two symmetric potential barriers of equal shape, with boundary conditions imposed in the middle of each barrier -- 3.24. Dependence of the phase of the wave function in a classically allowed region on the position of the point [chi][subscript 1] in an adjacent classically forbidden region where the boundary condition [psi][chi][subscript 1]) = 0 is imposed -- 3.25. Phase-shift formula -- 3.26. Distance between near-lying energy levels in different types of physical systems, expressed either in terms of the frequency of classical oscillations in a potential well or in terms of the derivative of the energy with respect to a quantum number -- 3.27. Arbitrary-order quantization condition for a particle in a single-well potential, derived on the assumption that the classically allowed region is broad enough to allow the use of a connection formula 3.28. Arbitrary-order quantization condition for a particle in a single-well potential, derived without the assumption that the classically allowed region is broad -- 3.29. Displacement of the energy levels due to compression of an atom (simple treatment) -- 3.30. Displacement of the energy levels due to compression of an atom (alternative treatment) -- 3.31. Quantization condition for a particle in a smooth potential well, limited on one side by an impenetrable wall and on the other side by a smooth, infinitely thick potential barrier, and in particular for a particle in a uniform gravitational field limited from below by an impenetrable plane surface -- 3.32. Energy spectrum of a non-relativistic particle in a potential proportional to cot[superscript 2]([chi]/a[subscript 0]), where 0 {$<$}[chi]/a[subscript 0] {$<$}[pi] and a[subscript 0] is a quantity with the dimension of length, e.g. the Bohr radius 3.33. Determination of a one-dimensional, smooth, single-well potential from the energy spectrum of the bound states -- 3.34. Determination of a radical, smooth, single-well potential from the energy spectrum of the bound states -- 3.35. Determination of the radial, single-well potential, when the energy eigenvalues are -mZ[superscript 2]e[superscript 4]/[2[actual symbol not reproducible][superscript 2]([iota]+s+1)[superscript 2]], where [iota] is the angular momentum quantum number, and s is the radial quantum number -- 3.36. Exact formula for the normalization integral for the wave function pertaining to a bound state of a particle in a radial potential -- 3.37. Phase-integral formula for the normalized radial wave function pertaining to a bound state of a particle in a radial single-well potential 3.38. Radial wave function [psi](z) for as s-electron in a classically allowed region containing the origin, when the potential near the origin is dominated by a strong, attractive Coulomb singularity, and the normalization factor is chosen such that, when the radial variable z is dimensionless, [psi](z)/z tends to unity as z tends to zero -- 3.39. Quantization condition, and value of the normalized wave function at the origin expressed in terms of the level density, for as s-electron in a single-well potential with a strong attractive Coulomb singularity at the origin -- 3.40. Expectation value of an unspecified function f(z) for a non-relativistic particle in a bound state -- 3.41. Some cases in which the phase-integral expectation value formula yields the expectation value exactly in the first-order approximation -- 3.42. Expectation value of the kinetic energy of a non-relativistic particle in a bound state. Verification of the virial theorem 3.43. Phase-integral calculation of quantal matrix elements -- 3.44. Connection formula for a complex potential barrier -- 3.45. Connection formula for a real, single-hump potential barrier -- 3.46. Energy levels of a particle in a smooth double-well potential, when no symmetry requirement is imposed -- 3.47. Energy levels of a particle in a smooth, symmetric, double-well potential -- 3.48. Determination of the quasi-stationary energy levels of a particle in a radial potential with a thick single-hump barrier -- 3.49. Transmission coefficient for a particle penetrating a real single-hump potential barrier -- 3.50. Transmission coefficient for a particle penetrating a real, symmetric, superdense double-hump potential barrier.},
  isbn = {0-521-67576-6},
  keywords = {notion,notion-database}
}

@article{Fromang2004,
  title = {Evolution of Self-Gravitating Magnetized Disks. {{II- Interaction}} between {{MHD}} Turbulence and Gravitational Instabilities},
  author = {Fromang, Sebastien and Balbus, Steven A. and Terquem, Caroline and De Villiers, Jean-Pierre},
  year = {2004},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {616},
  number = {1},
  eprint = {astro-ph/0409404},
  pages = {364--375},
  publisher = {{IOP Publishing}},
  doi = {10.1086/424829},
  urldate = {2020-07-02},
  abstract = {We present 3D magnetohydrodynamic (MHD) numerical simulations of the evolution of self--gravitating and weakly magnetized disks with an adiabatic equation of state. Such disks are subject to the development of both the magnetorotational and gravitational instabilities, which transport angular momentum outward. As in previous studies, our hydrodynamical simulations show the growth of strong m=2 spiral structure. This spiral disturbance drives matter toward the central object and disappears when the Toomre parameter Q has increased well above unity. When a weak magnetic field is present as well, the magnetorotational instability grows and leads to turbulence. In that case, the strength of the gravitational stress tensor is lowered by a factor of about\textasciitilde 2 compared to the hydrodynamical run and oscillates periodically, reaching very small values at its minimum. We attribute this behavior to the presence of a second spiral mode with higher pattern speed than the one which dominates in the hydrodynamical simulations. It is apparently excited by the high frequency motions associated with MHD turbulence. The nonlinear coupling between these two spiral modes gives rise to a stress tensor that oscillates with a frequency which is a combination of the frequencies of each of the modes. This interaction between MHD turbulence and gravitational instabilities therefore results in a smaller mass accretion rate onto the central object.},
  archiveprefix = {arxiv},
  keywords = {accretion,accretion disks-instabilities-MHD-turbulence,notion,notion-database,Subject headingg s},
  file = {/Users/lbugnet/Zotero/storage/WPGRMZPU/full-text.pdf}
}

@article{Fromang2006,
  title = {Evolution Des Disques d'accretion Protoplanetaires},
  author = {Fromang, Sebastien},
  year = {2006},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/38XJNP67/Fromang - 2006.pdf}
}

@article{Fuentes2017,
  title = {Stellar Halo Hierarchical Density Structure Identification Using ({{F}}){{OPTICS}}},
  author = {Sans Fuentes, S. A. and De Ridder, J. and Debosscher, J.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {599},
  pages = {143},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629719},
  urldate = {2020-04-13},
  abstract = {Context. The stellar halo holds some of the best preserved fossils of Galactic formation history that can be detected as overdensities. The detection and analysis of merger by-products within the halo enables the reconstruction of the accretion history of the Milky Way. Upcoming large-scale all-sky surveys such as Gaia and The Large Synoptic Survey Telescope (LSST) will provide a huge and rich data set, which at the same time poses challenges for automated halo debris detection. Aims. We investigate the overdensity detection algorithm Ordering Points To Identify the Clustering Structure (OPTICS) as a method to identify tidal debris in the Galactic halo with large-scale surveys, as well as the variant FOPTICS which is capable of handling data sets with multi-dimensional uncertainty ellipsoids. Methods. We applied OPTICS to the a simulated Galactic stellar Halo to assess the detection performance. Additionally, we tested the performance of FOPTICS is tested by introducing uncertainty ellipsoids to the 6D phase space of two test cases. We present the Jaccard index as an alternative way to test the stability of halo debris overdensity detections without the need for a local background density estimate. Results. We optimized the OPTICS overdensity detection algorithm so that it has a slightly superlinear run-time complexity, making the method suitable for large-scale surveys. Our test on a mock galactic halo in 6D phase space shows an excellent capability to not only detect the compact dense clusters, but also the larger streams that cover a significant part of the sky. The output of OPTICS, the so-called 2D reachability diagram, proved to be a very useful tool to grasp the size, density, and substructure of the overdensities without needing to resort to complex projections of the 6D phase space. Using FOPTICS, we show the effects of introducing uncertainty ellipsoids in the 6D phase space on the retrieved tidal streams, and how the detectability of a cluster depends on whether its size and density is sufficiently large to overcome the effects of the uncertainties on the attributes.},
  keywords = {Galaxy: halo,Galaxy: structure,Methods: numerical,notion,notion-database,Techniques: miscellaneous}
}

@article{Fuhrmann2004,
  title = {Nearby Stars of the {{Galactic}} Disk and Halo. {{III}}},
  author = {Fuhrmann, K.},
  year = {2004},
  journal = {Astronomische Nachrichten},
  volume = {325},
  number = {1},
  pages = {3--80},
  publisher = {{Wiley-VCH Verlag}},
  issn = {00046337},
  doi = {10.1002/asna.200310173},
  urldate = {2020-07-08},
  abstract = {High-resolution spectroscopic observations of about 150 nearby stars or star systems are presented and discussed. The study of these and another 100 objects of the previous papers of this series implies that the Galaxy became reality 13 or 14 Gyr ago with the implementation of a massive, rotationally-supported population of thick-disk stars. The very high star formation rate in that phase gave rise to a rapid metal enrichment and an expulsion of gas in supernovae-driven Galactic winds, but was followed by a star formation gap for no less than three billion years at the Sun's galactocentric distance. In a second phase, then, the thin disk - our "familiar Milky Way" - came on stage. Nowadays it traces the bright side of the Galaxy, but it is also embedded in a huge coffin of dead thick-disk stars that account for a large amount of baryonic dark matter. As opposed to this, cold-dark-matter-dominated cosmologies that suggest a more gradual hierarchical buildup through mergers of minor structures, though popular, are a poor description for the Milky Way Galaxy - and by inference many other spirals as well - if, as the sample implies, the fossil records of its long-lived stars do not stick to this paradigm. Apart from this general picture that emerges with reference to the entire sample stars, a good deal of the present work is however also concerned with detailed discussions of many individual objects. Among the most interesting we mention the blue straggler or merger candidates HD 165401 and HD 137763/HD 137778, the likely accretion of a giant planet or brown dwarf on 59 Vir in its recent history, and HD 63433 that proves to be a young solar analog at {$\tau$} {$\sim$} 200 Myr. Likewise, the secondary to HR 4867, formerly suspected non-single from the Hipparcos astrometry, is directly detectable in the high-resolution spectroscopic tracings, whereas the visual binary {$\chi$} Cet is instead at least triple, and presumably even quadruple. With respect to the nearby young stars a complete account of the Ursa Major Association is presented, and we provide as well plain evidence for another, the "Hercules-Lyra Association", the likely existence of which was only realized in recent years. On account of its rotation, chemistry, and age we do confirm that the Sun is very typical among its G-type neighbors; as to its kinematics, it appears however not unlikely that the Sun's known low peculiar space velocity could indeed be the cause for the weak paleontological record of mass extinctions and major impact events on our parent planet during the most recent Galactic plane passage of the solar system. Although the significance of this correlation certainly remains a matter of debate for years to come, we point in this context to the principal importance of the thick disk for a complete census with respect to the local surface and volume densities. Other important effects that can be ascribed to this dark stellar population comprise (i) the observed plateau in the shape of the luminosity function of the local FGK stars, (ii) a small though systematic effect on the basic solar motion, (iii) a reassessment of the term "asymmetrical drift velocity" for the remainder (i.e. the thin disk) of the stellar objects, (iv) its ability to account for the bulk of the recently discovered high-velocity blue white dwarfs, (v) its major contribution to the Sun's {$\sim$} 220 km s-1 rotational velocity around the Galactic center, and (vi) the significant flattening that it imposes on the Milky Way's rotation curve. Finally we note a high multiplicity fraction in the small but volume-complete local sample of stars of this ancient population. This in turn is highly suggestive for a star formation scenario wherein the few existing single stellar objects might only arise from either late mergers or the dynamical ejection of former triple or higher level star systems. \textcopyright 2004 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {Galaxy: evolution,Galaxy: formation,Galaxy: stellar content,notion,notion-database,Stars: fundamental parameters}
}

@article{Fuller,
  title = {A {{Solution}} to the {{Slow Spins}} of {{Stellar Cores The Spin}} of {{Stellar Cores}}},
  author = {Fuller, Jim},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YNINCIKR/Fuller - Unknown.pdf}
}

@article{Fuller2008,
  title = {Asteroseismology Can Reveal Strong Internal Magnetic Fields in Red Giant Stars},
  author = {Fuller, Jim and Garcia, Rafael A and Bildsten, Lars},
  year = {2008},
  volume = {2412},
  number = {1985},
  pages = {2520--2523},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BZ2GBY2V/Fuller, Garcia, Bildsten - 2008.pdf}
}

@article{Fuller2014,
  title = {Angular Momentum Transport via Internal Gravity Waves in Evolving Stars},
  author = {Fuller, Jim and Lecoanet, Daniel and Cantiello, Matteo and Brown, Ben},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {796},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/796/1/17},
  abstract = {Recent asteroseismic advances have allowed for direct measurements of the internal rotation rates of many subgiant and red giant stars. Unlike the nearly rigidly rotating Sun, these evolved stars contain radiative cores that spin faster than their overlying convective envelopes, but slower than they would in the absence of internal angular momentum transport. We investigate the role of internal gravity waves in angular momentum transport in evolving low-mass stars. In agreement with previous results, we find that convectively excited gravity waves can prevent the development of strong differential rotation in the radiative cores of Sun-like stars. As stars evolve into subgiants, however, low-frequency gravity waves become strongly attenuated and cannot propagate below the hydrogen-burning shell, allowing the spin of the core to decouple from the convective envelope. This decoupling occurs at the base of the subgiant branch when stars have surface temperatures of T {$\approx$} 5500 K. However, gravity waves can still spin down the upper radiative region, implying that the observed differential rotation is likely confined to the deep core near the hydrogen-burning shell. The torque on the upper radiative region may also prevent the core from accreting high angular momentum material and slow the rate of core spin-up. The observed spin-down of cores on the red giant branch cannot be totally attributed to gravity waves, but the waves may enhance shear within the radiative region and thus increase the efficacy of viscous/magnetic torques.},
  keywords = {asteroseismology,hydrodynamics,notion,notion-database,stars: evolution,stars: interiors,stars: oscillations,Sun: helioseismology,Sun: rotation,turbulence,waves},
  file = {/Users/lbugnet/Zotero/storage/9J6GA77D/Fuller et al. - 2014.pdf}
}

@article{Fuller2014a,
  title = {Saturn Ring Seismology: {{Evidence}} for Stable Stratification in the Deep Interior of {{Saturn}}},
  author = {Fuller, Jim},
  year = {2014},
  month = dec,
  journal = {Icarus},
  volume = {242},
  eprint = {1406.3343},
  pages = {283--296},
  publisher = {{Academic Press Inc.}},
  issn = {10902643},
  doi = {10.1016/j.icarus.2014.08.006},
  urldate = {2020-05-21},
  abstract = {Seismology allows for direct observational constraints on the interior structures of stars and planets. Recent observations of Saturn's ring system have revealed the presence of density waves within the rings excited by oscillation modes within Saturn, allowing for precise measurements of a limited set of the planet's mode frequencies. We construct interior structure models of Saturn, compute the corresponding mode frequencies, and compare them with the observed mode frequencies. The fundamental mode frequencies of our models match the observed frequencies (of the largest amplitude waves) to an accuracy of \textasciitilde 1\%, confirming that these waves are indeed excited by Saturn's f-modes. The presence of the lower amplitude waves (finely split in frequency from the f-modes) can only be reproduced in models containing gravity modes that propagate in a stably stratified region of the planet. The stable stratification must exist deep within the planet near the large density gradients between the core and envelope. Our models cannot easily reproduce the observed fine splitting of the m=. -. 3 modes, suggesting that additional effects (e.g., significant latitudinal differential rotation) may be important.},
  archiveprefix = {arxiv},
  keywords = {Interiors,notion,notion-database,{Resonances, rings},Saturn,{Saturn, interior},{Saturn, rings}}
}

@article{Fuller2015,
  title = {Asteroseismology Can Reveal Strong Internal Magnetic Fields in Red Giant Stars},
  author = {Fuller, Jim and Cantiello, Matteo and Stello, Dennis and Garcia, Rafael A. and Bildsten, Lars},
  year = {2015},
  journal = {Science},
  volume = {350},
  number = {6259},
  eprint = {1510.06960},
  pages = {423--426},
  issn = {10959203},
  doi = {10.1126/science.aac6933},
  abstract = {Internal stellar magnetic fields are inaccessible to direct observations, and little is known about their amplitude, geometry, and evolution. We demonstrate that strong magnetic fields in the cores of red giant stars can be identified with asteroseismology. The fields can manifest themselves via depressed dipole stellar oscillation modes, arising from a magnetic greenhouse effect that scatters and traps oscillation-mode energy within the core of the star. The Kepler satellite has observed a few dozen red giants with depressed dipole modes, which we interpret as stars with strongly magnetized cores. We find that field strengths larger than {$\sim$}105 gauss may produce the observed depression, and in one case we infer a minimum core field strength of {$\approx$}107 gauss.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UH9K8RBQ/Fuller et al. - 2015.pdf}
}

@article{Fuller2019,
  title = {Slowing the Spins of Stellar Cores},
  author = {Fuller, Jim and Piro, Anthony L. and Jermyn, Adam S.},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {485},
  number = {3},
  eprint = {1902.08227},
  pages = {3661--3680},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stz514},
  abstract = {The angular momentum (AM) evolution of stellar interiors, along with the resulting rotation rates of stellar remnants, remains poorly understood. Asteroseismic measurements of red giant stars reveal that their cores rotate much faster than their surfaces, but much slower than theoretically predicted, indicating an unidentified source of AM transport operates in their radiative cores. Motivated by this, we investigate the magnetic Tayler instability and argue that it saturates when turbulent dissipation of the perturbed magnetic field energy is equal to magnetic energy generation via winding. This leads to larger magnetic field amplitudes, more efficient AM transport, and smaller shears than predicted by the classic Tayler\textendash Spruit dynamo. We provide prescriptions for the effective AM diffusivity and incorporate them into numerical stellar models, finding they largely reproduce (1) the nearly rigid rotation of the Sun and main sequence stars, (2) the core rotation rates of low-mass red giants during hydrogen shell and helium burning, and (3) the rotation rates of white dwarfs. We discuss implications for stellar rotational evolution, internal rotation profiles, rotational mixing, and the spins of compact objects.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology \textendash{} instabilities \textendash{} MHD \textendash{} stars,Evolution \textendash{} stars,Interiors \textendash{} stars,notion,notion-database,Rotation},
  file = {/Users/lbugnet/Zotero/storage/QTJVE4GU/Fuller, Piro, Jermyn - 2019.pdf}
}

@article{Gabriel1995,
  title = {Global {{Oscillations}} at {{Low Frequency}} from the {{SOHO}} Mission ({{GOLF}})},
  author = {Gabriel, A. H. and Grec, G. and Charra, J. and Robillot, J. M. and Roca Cort{\'e}s, T. and {Turck-Chi{\`e}ze}, S. and Bocchia, R. and Boumier, P. and Cantin, M. and Cesp{\'e}des, E. and Cougrand, B. and Cr{\'e}tolle, J. and Dam{\'e}, L. and Decaudin, M. and Delache, P. and Denis, N. and Duc, R. and Dzitko, H. and Fossat, E. and Fourmond, J. J. and Garc{\'i}a, R. A. and Gough, D. and Grivel, C. and Herreros, J. M. and Lagard{\`e}re, H. and Moalic, J. P. and Pall{\'e}, P. L. and P{\'e}trou, N. and Sanchez, M. and Ulrich, R. and {van der Raay}, H. B.},
  year = {1995},
  journal = {Solar Physics},
  volume = {162},
  number = {1-2},
  pages = {61--99},
  publisher = {{Kluwer Academic Publishers}},
  issn = {1573093X},
  doi = {10.1007/BF00733427},
  urldate = {2020-07-14},
  abstract = {The GOLF experiment on the SOHO mission aims to study the internal structure of the sun by measuring the spectrum of global oscillations in the frequency range 10-7 to 10-2 Hz. Both p and g mode oscillations will be investigated, with the emphasis on the low order long period waves which penetrate the solar core. The instrument employs an extension to space of the proven ground-based technique for measuring the mean line-of-sight velocity of the viewed solar surface. By avoiding the atmospheric disturbances experienced from the ground, and choosing a non-eclipsing orbit, GOLF aims to improve the instrumental sensitivity limit by an order of magnitude to 1 mm s-1 over 20 days for frequencies higher than 2.10-4 Hz. A sodium vapour resonance cell is used in a longitudinal magnetic field to sample the two wings of the solar absorption line. The addition of a small modulating field component enables the slope of the wings to be measured. This provides not only an internal calibration of the instrument sensitivity, but also offers a further possibility to recognise, and correct for, the solar background signal produced by the effects of solar magnetically active regions. The use of an additional rotating polariser enables measurement of the mean solar line-of-sight magnetic field, as a secondary objective. \textcopyright{} 1995 Kluwer Academic Publishers.},
  keywords = {helioseismology,notion,notion-database,sun}
}

@article{Gabriel1997a,
  title = {Performance and Early Results from the Golf Instrument Flown on the {{SOHO}} Mission},
  author = {Gabriel, A. H. and Charra, J. and Grec, G. and Robillot, J. M. and Roca Cort{\'e}s, T. and {Turck-Chi{\`e}ze}, S. and Ulrich, R. and Basu, S. and Baudin, F. and Bertello, L. and Boumier, P. and Charra, M. and {Christensen-Dalsgaard}, J. and Decaudin, M. and Dzitko, H. and Foglizzo, T. and Fossat, E. and Garc{\'i}a, R. A. and Herreros, J. M. and Lazrek, M. and Pall{\'e}, P. L. and P{\'e}trou, N. and Renaud, C. and R{\'e}gulo, C.},
  year = {1997},
  journal = {Solar Physics},
  volume = {175},
  number = {2},
  pages = {207--226},
  issn = {00380938},
  doi = {10.1023/A:1004911408285},
  abstract = {GOLF in-flight commissioning and calibration was carried out during the first four months, most of which represented the cruise phase of SOHO towards its final L.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9WHYP24B/Gabriel et al. - 1997.pdf}
}

@article{Gabriel2002,
  title = {A Search for Solar g Modes in the {{GOLF}} Data},
  author = {Gabriel, A. H. and Baudin, F. and Boumier, P. and Garc{\'i}a, R. A. and {Turck-Chi{\`e}ze}, S. and Appourchaux, T. and Bertello, L. and Berthomieu, G. and Charra, J. and Gough, D. O. and Pall{\'e}, P. L. and Provost, J. and Renaud, C. and Robillot, J. M. and Roca Cort{\'e}s, T. and Thiery, S. and Ulrich, R. K.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {390},
  number = {3},
  pages = {1119--1131},
  issn = {00046361},
  doi = {10.1051/0004-6361:20020695},
  abstract = {With over 5 years of GOLF data having some 90\% continuity, a new attempt has been made to search for possible solar g modes. Statistical methods are used, based on the minimum of assumptions regarding the solar physics; namely that mode line-widths are small compared with the inverse of the observing time, and that modes are sought in the frequency interval 150 to 400 {$\mu$}Hz. A number of simulations are carried out in order to understand the expected behaviour of a system consisting principally of a solar noise continuum overlaid with some weak sharp resonances. The method adopted is based on the FFT analysis of a time series with zero-padding by a factor of 5. One prominent at 284.666 {$\mu$}Hz coincides with a previous tentative assignment as one member of an n = 1, l = 1, p-mode multiplet. Components of two multiplets, previously tentatively identified as possible g-mode candidates from the GOLF data in 1998, continue to be found, although their statistical significance is shown to be insufficient, within the present assumption regarding the nature of the signal. An upper limit to the amplitude of any g mode present is calculated using two different statistical approaches, according to either the assumed absence (H0 hypothesis) or the assumed presence (H1 hypothesis) of a signal. The former yields a slightly lower limit of around 6 mm/s.},
  keywords = {Helioseismology,notion,notion-database,Sun},
  file = {/Users/lbugnet/Zotero/storage/3C35WY4E/Gabriel et al. - 2002.pdf}
}

@article{GaiaCollaboration2018,
  title = {Gaia {{Data Release}} 2. {{Summary}} of the Contents and Survey Properties},
  author = {{Gaia Collaboration} and Brown, A. G. A. and Vallenari, A. and Prusti, T. and {de Bruijne}, J. H. J. and Babusiaux, C. and {Bailer-Jones}, C. A. L.},
  year = {2018},
  month = apr,
  journal = {Astronomy \& Astrophysics},
  volume = {616},
  number = {A1},
  eprint = {1804.09365},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201833051},
  urldate = {2020-07-07},
  abstract = {We present the second Gaia data release, Gaia DR2, consisting of astrometry, photometry, radial velocities, and information on astrophysical parameters and variability, for sources brighter than magnitude 21. In addition epoch astrometry and photometry are provided for a modest sample of minor planets in the solar system. A summary of the contents of Gaia DR2 is presented, accompanied by a discussion on the differences with respect to Gaia DR1 and an overview of the main limitations which are still present in the survey. Recommendations are made on the responsible use of Gaia DR2 results. Gaia DR2 contains celestial positions and the apparent brightness in G for approximately 1.7 billion sources. For 1.3 billion of those sources, parallaxes and proper motions are in addition available. The sample of sources for which variability information is provided is expanded to 0.5 million stars. This data release contains four new elements: broad-band colour information in the form of the apparent brightness in the \$G\_\textbackslash mathrm\{BP\}\$ (330--680 nm) and \$G\_\textbackslash mathrm\{RP\}\$ (630--1050 nm) bands is available for 1.4 billion sources; median radial velocities for some 7 million sources are presented; for between 77 and 161 million sources estimates are provided of the stellar effective temperature, extinction, reddening, and radius and luminosity; and for a pre-selected list of 14000 minor planets in the solar system epoch astrometry and photometry are presented. Finally, Gaia DR2 also represents a new materialisation of the celestial reference frame in the optical, the Gaia-CRF2, which is the first optical reference frame based solely on extragalactic sources. There are notable changes in the photometric system and the catalogue source list with respect to Gaia DR1, and we stress the need to consider the two data releases as independent.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Gallet2013,
  title = {Improved Angular Momentum Evolution Model for Solar-like Stars},
  author = {Gallet, F. and Bouvier, J.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {556},
  eprint = {1306.2130},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321302},
  urldate = {2020-07-17},
  abstract = {Context. Understanding the origin and evolution of stellar angular momentum is one of the major challenges of stellar physics. Aims. We present new models for the rotational evolution of solar-like stars between 1 Myr and 10 Gyr with the aim of reproducing the distributions of rotational periods observed for star forming regions and young open clusters within this age range. Methods. The models include a new wind braking law based on recent numerical simulations of magnetized stellar winds and specific dynamo and mass-loss prescriptions are adopted to tie angular momentum loss to angular velocity. The models additionally assume constant angular velocity during the disk accretion phase and allow for decoupling between the radiative core and the convective envelope as soon as the former develops. Results. We have developed rotational evolution models for slow, median, and fast rotators with initial periods of 10, 7, and 1.4 d, respectively. The models reproduce reasonably well the rotational behavior of solar-type stars between 1 Myr and 4.5 Gyr, including pre-main sequence (PMS) to zero-age main sequence (ZAMS) spin up, prompt ZAMS spin down, and the early-main sequence (MS) convergence of surface rotation rates. We find the model parameters accounting for the slow and median rotators are very similar to each other, with a disk lifetime of 5 Myr and a core-envelope coupling timescale of 28-30 Myr. In contrast, fast rotators have both shorter disk lifetimes (2.5 Myr) and core-envelope coupling timescales (12 Myr). We show that a large amount of angular momentum is hidden in the radiative core for as long as 1 Gyr in these models and we discuss the implications for internal differential rotation and lithium depletion. We emphasize that these results are highly dependent on the adopted braking law. We also report a tentative correlation between the initial rotational period and disk lifetime, which suggests that protostellar spin down by massive disks in the embedded phase is at the origin of the initial dispersion of rotation rates in young stars. Conclusions. We conclude that this class of semi-empirical models successfully grasp the main trends of the rotational behavior of solar-type stars as they evolve and make specific predictions that may serve as a guide for further development. \textcopyright{} ESO, 2013.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: magnetic field,Stars: mass-loss,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/9LZV4MEA/full-text.pdf}
}

@article{Gallet2013a,
  title = {Improved Angular Momentum Evolution Model for Solar-like Stars},
  author = {Gallet, F. and Bouvier, J.},
  year = {2013},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {556},
  pages = {A36},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201321302},
  urldate = {2023-10-26},
  abstract = {Context. Understanding the origin and evolution of stellar angular momentum is one of the major challenges of stellar physics. Aims: We present new models for the rotational evolution of solar-like stars between 1 Myr and 10 Gyr with the aim of reproducing the distributions of rotational periods observed for star forming regions and young open clusters within this age range. Methods: The models include a new wind braking law based on recent numerical simulations of magnetized stellar winds and specific dynamo and mass-loss prescriptions are adopted to tie angular momentum loss to angular velocity. The models additionally assume constant angular velocity during the disk accretion phase and allow for decoupling between the radiative core and the convective envelope as soon as the former develops. Results: We have developed rotational evolution models for slow, median, and fast rotators with initial periods of 10, 7, and 1.4 d, respectively. The models reproduce reasonably well the rotational behavior of solar-type stars between 1 Myr and 4.5 Gyr, including pre-main sequence (PMS) to zero-age main sequence (ZAMS) spin up, prompt ZAMS spin down, and the early-main sequence (MS) convergence of surface rotation rates. We find the model parameters accounting for the slow and median rotators are very similar to each other, with a disk lifetime of 5 Myr and a core-envelope coupling timescale of 28-30 Myr. In contrast, fast rotators have both shorter disk lifetimes (2.5 Myr) and core-envelope coupling timescales (12 Myr). We show that a large amount of angular momentum is hidden in the radiative core for as long as 1 Gyr in these models and we discuss the implications for internal differential rotation and lithium depletion. We emphasize that these results are highly dependent on the adopted braking law. We also report a tentative correlation between the initial rotational period and disk lifetime, which suggests that protostellar spin down by massive disks in the embedded phase is at the origin of the initial dispersion of rotation rates in young stars. Conclusions: We conclude that this class of semi-empirical models successfully grasp the main trends of the rotational behavior of solar-type stars as they evolve and make specific predictions that may serve as a guide for further development. Appendix A is available in electronic form at http://www.aanda.org},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: magnetic field,stars: mass-loss,stars: rotation,stars: solar-type},
  annotation = {ADS Bibcode: 2013A\&A...556A..36G},
  file = {/Users/lbugnet/Zotero/storage/GYJZC9UY/Gallet and Bouvier - 2013 - Improved angular momentum evolution model for sola.pdf}
}

@article{Gallet2015,
  title = {Improved Angular Momentum Evolution Model for Solar-like Stars {{II}}. {{Exploring}} the Mass Dependence},
  author = {Gallet, Florian and Bouvier, J{\'e}r{\^o}me},
  year = {2015},
  month = feb,
  journal = {Astronomy \& Astrophysics},
  volume = {577},
  number = {A98},
  eprint = {1502.05801},
  doi = {10.1051/0004-6361/201525660},
  urldate = {2020-07-17},
  abstract = {We developed angular momentum evolution models for 0.5 and 0.8 \$M\_\{\textbackslash odot\}\$ stars. The parametric models include a new wind braking law based on recent numerical simulations of magnetised stellar winds, specific dynamo and mass-loss rate prescriptions, as well as core/envelope decoupling. We compare model predictions to the distributions of rotational periods measured for low mass stars belonging to star forming regions and young open clusters. Furthermore, we explore the mass dependence of model parameters by comparing these new models to the solar-mass models we developed earlier. Rotational evolution models are computed for slow, median, and fast rotators at each stellar mass. The models reproduce reasonably well the rotational behaviour of low-mass stars between 1 Myr and 8-10 Gyr, including pre-main sequence to zero-age main sequence spin up, prompt zero-age main sequence spin down, and early-main sequence convergence of the surface rotation rates. Fast rotators are found to have systematically shorter disk lifetimes than moderate and slow rotators, thus enabling dramatic pre-main sequence spin up. They also have shorter core-envelope coupling timescales, i.e., more uniform internal rotation. As to the mass dependence, lower mass stars require significantly longer core-envelope coupling timescale than solar-type ones, which results in strong differential rotation developing in the stellar interior on the early main sequence. Lower mass stars also require a weaker braking torque to account for their longer spin down timescale on the early main sequence, while they ultimately converge towards lower rotational velocities than solar-type stars on the longer term due to their reduced moment of inertia. We also find evidence that the mass-dependence of the wind braking efficiency may be related to a change of the magnetic topology in lower mass stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Gandolfi2018,
  title = {{{TESS}} ' s First Planet {{A}} Super-{{Earth}} Transiting the Naked-Eye Star {$\pi$} {{Mensae}}},
  author = {Gandolfi, D and Livingston, J H and Fridlund, M and Justesen, A B and Redfield, S and Fossati, L and Mathur, S and Grziwa, S and Cabrera, J and Persson, C M and Eylen, V Van and Hatzes, A P and Hidalgo, D and Albrecht, S and Bugnet, L and Cochran, W D and Deeg, H and Endl, M and Erikson, A and Esposito, M and Guenther, E and Korth, J and Luque, R and Nespral, D and Nowak, G},
  year = {2018},
  journal = {Astronomy and Astrophysics Letter to the editor},
  volume = {10},
  pages = {1--10},
  isbn = {4623036865373},
  keywords = {detection,fundamental parameters,notion,notion-database,planetary systems,planets and satellites,stars,terrestrial planets},
  file = {/Users/lbugnet/Zotero/storage/EP3KUSLL/Gandolfi et al. - 2018.pdf}
}

@article{Garaud1999,
  title = {Propagation of a Dynamo Field in the Radiative Interior of the {{Sun}}},
  author = {Garaud, P.},
  year = {1999},
  month = apr,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {304},
  number = {3},
  pages = {583--588},
  publisher = {{Blackwell Publishing Ltd}},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.1999.02338.x},
  urldate = {2020-05-14},
  abstract = {Large-scale magnetic fields are believed to play an important role in the radiative zone of the Sun, in particular in the dynamical processes in the transition region between the convective and radiative zones (the tachoclme). Also, they are probably responsible for the observed uniform rotation of the radiative zone. In that respect, since it has been suggested that the solar dynamo may lie near the outer edge of the tachocline, it is important to assess the question of how deep the dynamo field can penetrate, and whether it can influence significantly the dynamics of the solar interior. The magnetic cycle of the Sun is not strictly periodic, but undergoes random fluctuations in amplitude and phase. It is shown how the random fluctuations in the poloidal field diffuse into the radiative zone. An explicit solution for this diffusion process is given under certain simplifying assumptions. The result is then used together with some assumptions about the solar dynamo field to suggest that a field of order of 10-1 G should be expected near the outer edge of the radiative zone, dropping rapidly to 10-6G beneath r = 0.3 R{$\odot$}. This confirms the expectation that the dynamo field has a negligible effect on the dynamical processes taking place both in the tachocline and deeper in the radiative zone.},
  keywords = {notion,notion-database,Sun: interior,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/TSTSBDW3/full-text.pdf}
}

@article{Garaud2002,
  title = {Dynamics of the Solar Tachocline - {{I}}. {{An}} Incompressible Study},
  author = {Garaud, Pascale},
  year = {2002},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {329},
  pages = {1--17},
  keywords = {interior - sun,magnetic fields - mhd,magnetic fields - sun,notion,notion-database,rotation,sun},
  file = {/Users/lbugnet/Zotero/storage/FSG5YQP9/Garaud - 2002.pdf}
}

@article{Garaud2007,
  title = {Magnetic Confinement of the Solar Tachocline},
  author = {Garaud, Pascale},
  year = {2007},
  journal = {The Solar Tachocline},
  volume = {9780521861},
  pages = {147--182},
  doi = {10.1017/CBO9780511536243.008},
  abstract = {Two distinct classes of magnetic confinement models exist for the solar tachocline. The 'slow tachocline' models are associated with a large-scale primordial field embedded in the radiative zone. The 'fast tachocline' models are associated with an overlying dynamo field. I describe the results obtained in each case, their pros and cons, and compare them with existing solar observations. I conclude by discussing new lines of investigation that should be pursued, as well as some means by which these models could be unified or reconciled. Introduction Magnetic fields in the tachocline Two distinct possible origins for solar magnetic fields in the tachocline region can be identified. The Ohmic decay timescale of a large-scale dipolar field embedded in the radiative interior is much larger than the estimated age of the Sun (Cowling 1945; Garaud 1999), so that a fraction of the magnetic flux initially frozen within the accreting protostellar gas is likely to persist today. In parallel, according to the standard dynamo field theory, small-scale magnetic fields are thought to be constantly generated by fluid motions within the solar interior. Optimal conditions for the generation of large-scale fields require the combination of large-scale azimuthal shear and small-scale helical motion, which are both naturally found in the region of the tachocline (Parker 1993; Ossendrijver 2003; Tobias 2005).},
  isbn = {9780511536243},
  keywords = {evolution,magnetohydrodynamics,mhd,notion,notion-database,rotation,stars,sun,turbulence},
  file = {/Users/lbugnet/Zotero/storage/QJ9K8ARJ/Garaud - 2007.pdf}
}

@article{Garaud2008,
  title = {Dynamics of the Solar Tachocline - {{II}}. the Stratified Case},
  author = {Garaud, P. and Garaud, J. D.},
  year = {2008},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {391},
  number = {3},
  eprint = {0806.2551},
  pages = {1239--1258},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2008.13930.x},
  abstract = {We present a detailed numerical study of the Gough \& McIntyre model for the solar tachocline. This model explains the uniformity of the rotation profile observed in the bulk of the radiative zone by the presence of a large-scale primordial magnetic field, confined below the tachocline by flows originating from within the convection zone. We attribute the failure of previous numerical attempts at reproducing even qualitatively Gough \& McIntyre's idea to the use of inappropriate boundary conditions at the radiative-convective interface. We emphasize the key role of flows downwelling from the convection zone in confining the assumed internal field. We carefully select the range of parameters used in the simulations to guarantee a faithful representation of the hierarchy of expected length-scales. We then present, for the first time, a fully non-linear and self-consistent numerical solution of the Gough \& McIntyre model which qualitatively satisfies the following set of observational constraints: (i) the quenching of the large-scale differential rotation below the tachocline - including in the polar regions - as seen by helioseismology (ii) the confinement of the large-scale meridional flows to the uppermost layers of the radiative zone as required by observed light element abundances and suggested by helioseismic sound-speed data. \textcopyright{} 2008 RAS.},
  archiveprefix = {arxiv},
  keywords = {MHD,notion,notion-database,Sun: interior,Sun: magnetic fields,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/KQ8TWCR2/Garaud, Garaud - 2008.pdf}
}

@article{Garcia2005,
  title = {Global Solar {{Doppler}} Velocity Determination with the {{GOLF}}/{{SoHO}} Instrument},
  author = {Garc{\'i}a, R. A. and {Turck-Chi{\`e}ze}, S. and Boumier, P. and Robillot, J. M. and Bertello, L. and Charra, J. and Dzitko, H. and Gabriel, A. H. and {Jim{\'e}nez-Reyes}, S. J. and Pall{\'e}, P. L. and Renaud, C. and {Roca Cort\'es} and Ulrich, R. K.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {442},
  number = {1},
  pages = {385--395},
  issn = {00046361},
  doi = {10.1051/0004-6361:20052779},
  abstract = {The Global Oscillation at Low Frequencies (GOLF) experiment is a resonant scattering spectrophotometer on board the Solar and Heliospheric Observatory (SoHO) mission, originally designed to measure the disk-integrated solar oscillations of the Sun. This instrument was designed in a relative photometric mode involving both wings of the neutral sodium doublet (D1 at {$\lambda$} 5896 and D2 at {$\lambda$} 5890 \AA ). However, a "one-wing" photometric mode has been selected to ensure 100\% continuity in the measurements after a problem in the polarization mechanisms. Thus the velocity is obtained from only two points on the same wing of the lines. This operating configuration imposes tighter constraints on the stability of the instrument with a higher sensitivity to instrumental variations. In this paper we discuss the evolution of the instrument during the last 8 years in space and the corrections applied to the measured counting rates due to known instrumental effects. We also describe a scaling procedure to obtain the variation of the Doppler velocity based on our knowledge of the sodium profile slope and we compare it to previous velocity estimations. \textcopyright{} ESO 2005.},
  keywords = {Instrumentation: detectors,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/BXUHFFCA/García et al. - 2005.pdf}
}

@article{Garcia2007a,
  title = {Tracking {{Solar Gravity Modes}}: {{The Dynamics}} of the {{Solar Core}}},
  shorttitle = {Tracking {{Solar Gravity Modes}}},
  author = {Garc{\'i}a, Rafael A. and {Turck-Chi{\`e}ze}, Sylvaine and {Jim{\'e}nez-Reyes}, Sebastian J. and Ballot, J{\'e}r{\^o}me and Pall{\'e}, Pere L. and {Eff-Darwich}, Antonio and Mathur, Savita and Provost, Janine},
  year = {2007},
  month = jun,
  journal = {Science},
  volume = {316},
  pages = {1591},
  issn = {0036-8075},
  doi = {10.1126/science.1140598},
  urldate = {2023-11-07},
  abstract = {Solar gravity modes have been actively sought because they directly probe the solar core (below 0.2 solar radius), but they have not been conclusively detected in the Sun because of their small surface amplitudes. Using data from the Global Oscillation at Low Frequency instrument, we detected a periodic structure in agreement with the period separation predicted by the theory for gravity dipole modes. When studied in relation to simulations including the best physics of the Sun determined through the acoustic modes, such a structure favors a faster rotation rate in the core than in the rest of the radiative zone.},
  keywords = {ASTRONOMY},
  annotation = {ADS Bibcode: 2007Sci...316.1591G}
}

@article{Garcia2008,
  title = {Low-Degree Modes},
  author = {Garc{\'i}a, Rafael A.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012026},
  abstract = {We review some of the works done during the last year and some of the challenges we have to face today in the study of low-degree acoustic and gravity modes and their implications in the study of the solar internal structure and dynamics. \textcopyright{} 2008 IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CEWU3VBS/García - 2008.pdf}
}

@article{Garcia2008a,
  title = {Influence of Low-Degree High-Order p-Mode Splittings on the Solar Rotation Profile},
  author = {Garc{\'i}a, R. A. and Mathur, S. and Ballot, J. and {Eff-Darwich}, A. and {Jim{\'e}nez-Reyes}, S. J. and Korzennik, S. G.},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  pages = {119--133},
  issn = {00380938},
  doi = {10.1007/s11207-008-9144-5},
  abstract = {The solar rotation profile is well constrained down to about 0.25R {$\odot$} thanks to the study of acoustic modes. Since the radius of the inner turning point of a resonant acoustic mode is inversely proportional to the ratio of its frequency to its degree, only the low-degree p modes reach the core. The higher the order of these modes, the deeper they penetrate into the Sun and thus they carry more diagnostic information on the inner regions. Unfortunately, the estimates of frequency splittings at high frequency from Sun-as-a-star measurements have higher observational errors because of mode blending, resulting in weaker constraints on the rotation profile in the inner core. Therefore inversions for the solar internal rotation use only modes below 2.4 mHz for {$\mathscr{l}$} {$\leq$}3. In the work presented here, we used an 11.5-year-long time series to compute the rotational frequency splittings for modes {$\mathscr{l}$} {$\leq$}3 using velocities measured with the GOLF instrument. We carried out a theoretical study of the influence of the low-degree modes in the region from 2 to 3.5 mHz on the inferred rotation profile as a function of their error bars. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  isbn = {1120700891445},
  keywords = {Core,Helioseismology,Interior,Inverse modeling,notion,notion-database,Observations,Radiative zone,Rotation},
  file = {/Users/lbugnet/Zotero/storage/RST9M64S/García et al. - 2008.pdf}
}

@article{Garcia2008b,
  title = {Update on G-Mode Research},
  author = {Garc{\'i}a, R. A. and Jim{\'e}nez, A. and Mathur, S. and Ballot, J. and {Eff-Darwich}, A. and {Jim{\'e}nez-Reyes}, S. J. and Pall{\'e}, P. L. and Provost, J. and {Turck-Ch{\`i}eze}, S.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  pages = {476--484},
  issn = {00046337},
  doi = {10.1002/asna.200710980},
  abstract = {Since the beginning of this century we have attended a blooming of the gravity-mode research thanks to the unprecedented quality of the data available, either from space with SoHO, or from the ground-based networks as BiSON or GONG. From the first upper limit of the gravity-mode amplitudes fixed at 10 mm/s at 200 {$\mu$}Hz given by Appourchaux et al. (2000), on one hand, a peak was supposed to be a component of the {$\mathscr{l}$} = 1, n = 1 mixed mode (Garc\'ia et al. 2001a, 2001b; Gabriel et al. 2002) and, on the other hand, a couple of patterns - multiplets - were attributed to gravity modes (Turck-Chi\`eze et al. 2004; Mathur et al. 2007). One of these patterns, found around 220 {$\mu$}Hz, could be labeled as the {$\mathscr{l}$} = 2, n = -3 g mode, which is expected to be the one with the highest surface amplitude (Cox \& Guzik 2004). Finally, in 2007, Garc\`ia et al. were able to measure the fingertips of the dipole gravity modes looking for their asymptotic properties. In the present paper we present an update of the recent developments on this subject with special attention to the 220 {$\mu$}Hz region, the dipole asymptotic properties and the impact of the incoming g-mode observations on the knowledge of the solar structure and rotation profile. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: interior,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4S43967S/García et al. - 2008(2).pdf}
}

@article{Garcia2008d,
  title = {Can We Constrain Solar Interior Physics by Studying the Gravity-Mode Asymptotic Signature?},
  author = {Garc{\'i}a, R. A. and Mathur, S. and Ballot, J.},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  pages = {135--147},
  issn = {00380938},
  doi = {10.1007/s11207-008-9159-y},
  abstract = {Gravity modes are the best probes to infer the properties of the solar radiative zone, which represents 98\% of the Sun's total mass. It is usually assumed that high-frequency g modes give information about the structure of the solar interior whereas low-frequency g modes are more sensitive to the solar dynamics (the internal rotation). In this work, we develop a new methodology, based on the analysis of the almost constant separation of the dipole gravity modes, to introduce new constraints on the solar models. To validate this analysis procedure, several solar models - including different physical processes and either old or new chemical abundances (from, respectively, Grevesse and Noels (Origin and Evolution of the Elements 199, Cambridge University Press, Cambridge, 15, 1993) and Asplund, Grevesse, and Sauval (Cosmic Abundances as Records of Stellar Evolution and Nucleosynthesis CS-336, Astron. Soc. Pac., San Francisco, 25-38, 2005)) - have been compared to another model used as a reference. The analysis clearly shows that this methodology has enough sensitivity to distinguish among some of the models, in particular, among those with different compositions. The comparison of the models with the g-mode asymptotic signature detected in GOLF data favors the ones with old abundances. Therefore, the physics of the core - obtained through the analysis of the g-mode properties - is in agreement with the results obtained in the previous studies based on the acoustic modes, which are mostly sensitive to more external layers of the Sun. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  keywords = {Helioseismology: Observations,{Interior: Radiative zone, core},notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SYA8WGQ5/García, Mathur, Ballot - 2008.pdf}
}

@article{Garcia2009,
  title = {Detecting Individual Gravity Modes in the {{Sun}}: {{Chimera}} or Reality?},
  author = {Garc{\'i}a, Rafael A.},
  year = {2009},
  journal = {Proceedings of the International Astronomical Union},
  volume = {5},
  number = {H15},
  eprint = {0910.0848},
  pages = {345--346},
  issn = {1743-9213},
  doi = {10.1017/s1743921310009695},
  abstract = {Over the past 15 years, our knowledge of the interior of the Sun has tremendously progressed by the use of helioseismic measurements. However, to go further in our understanding of the solar core, we need to measure gravity (g) modes. Thanks to the high quality of the Doppler-velocity signal measured by GOLF/SoHO, it has been possible to unveil the signature of the asymptotic properties of the solar g modes, thus obtaining a hint of the rotation rate in the core (Garc\'ia et al . 2007, 2008a). However, the quest for the detection of individual g modes is not yet over. In this work, we apply the latest theoretical developments to guide our research using GOLF velocity time series. In contrary to what was thought till now, we are maybe starting to identify individual low-frequency g modes.~.~.},
  archiveprefix = {arxiv},
  isbn = {1743921310009},
  keywords = {1,2009,basu et al,e,g,garc,gravity modes are very,helioseismology,interior,notion,notion-database,observations and analysis,oscillations,rotation,sensitive to the structure,sun},
  file = {/Users/lbugnet/Zotero/storage/EESQW26Y/García - 2009.pdf}
}

@article{Garcia2009a,
  title = {Solar-like Oscillations with Low Amplitude in the {{CoRoT}} Target {{HD}} 181906},
  author = {Garc{\'i}a, R. A. and R{\'e}gulo, C. and Samadi, R. and Ballot, J. and Barban, C. and Benomar, O. and Chaplin, W. J. and Gaulme, P. and Appourchaux, T. and Mathur, S. and Mosser, B. and Toutain, T. and Verner, G. A. and Auvergne, M. and Baglin, A. and Baudin, F. and Boumier, P. and Bruntt, H. and Catala, C. and Deheuvels, S. and Elsworth, Y. and {Jim{\'e}nez-Reyes}, S. J. and Michel, E. and P{\'e}rez Hern{\'a}ndez, F. and Roxburgh, I. W. and Salabert, D.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {41--50},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911910},
  abstract = {Context. The F8 star HD 181906 (effective temperature {$\sim$}6300 K) was observed for 156 days by the CoRoT satellite during the first long run in the direction of the galactic centre. Analysis of the data reveals a spectrum of solar-like acoustic oscillations. However, the faintness of the target (m{$\nu$} = 7.65) means the signal-to-noise (S/N) in the acoustic modes is quite low, and this low S/N leads to complications in the analysis. Aims. We extract global variables of the star, as well as key parameters of the p modes observed in the power spectrum of the lightcurve. Methods. The power spectrum of the lightcurve, a wavelet transform and spot fitting were used to obtain the average rotation rate of the star and its inclination angle. Then, the autocorrelation of the power spectrum and the power spectrum of the power spectrum were used to properly determine the large separation. Finally, estimations of the mode parameters were done by maximizing the likelihood of a global fit, where several modes were fit simultaneously. Results. We have been able to infer the mean surface rotation rate of the star ({$\sim$}4 {$\mu$}Hz) with indications of the presence of surface differential rotation, the large separation of the p modes ({$\sim$}87 {$\mu$}Hz), hence also the "ridges" corresponding to overtones of the acoustic modes.},
  keywords = {Methods: observational,Methods: statistical,notion,notion-database,Stars: individual: HD 181906,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WUGYBS9I/García et al. - 2009.pdf}
}

@article{Garcia2010,
  title = {{{CoRoT}} Reveals a Magnetic Activity Cycle in a Sun-like Star},
  author = {Garc{\'i}a, Rafael A. and Mathur, Savita and Salabert, David and Ballot, J{\'e}r{\^o}me and R{\'e}gulo, Clara and Metcalfe, Travis S. and Baglin, Annie},
  year = {2010},
  journal = {Science},
  volume = {329},
  number = {5995},
  pages = {1032},
  issn = {10959203},
  doi = {10.1126/science.1191064},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2H2BYEH8/García et al. - 2010.pdf}
}

@article{Garcia2011,
  title = {The Acoustic Low-Degree Modes of the {{Sun}} Measured with 14 Years of Continuous {{GOLF}} \& {{VIRGO}} Measurements},
  author = {Garc{\'i}a, R. A. and Salabert, D. and Ballot, J. and Sato, K. and Mathur, S. and Jim{\'e}nez, A.},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012049},
  abstract = {The helioseismic Global Oscillation at Low Frequency (GOLF) and the Variability of solar Irradiance and Gravity Oscillations (VIRGO) instruments onboard SoHO, have been observing the Sun continuously for the last 14 years. In this preliminary work, we characterize the acoustic modes over the entire p-mode range in both, Doppler velocity and luminosity, with a special care for the low-frequency modes taking advantage of the stability and the high duty cycle of space observations. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/B5YX7CWZ/García et al. - 2011.pdf}
}

@article{Garcia2011a,
  title = {New Insights on the Solar Core},
  author = {Garc{\'i}a, R. A. and Salabert, D. and Ballot, J. and {Eff-Darwich}, A. and Garrido, R. and Jim{\'e}nez, A. and Mathis, S. and Mathur, S. and Moya, A. and Pall{\'e}, P. L. and R{\'e}gulo, C. and Sato, K. and Surez, J. C. and {Turck-Chi{\`e}ze}, S.},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012046},
  abstract = {Since the detection of the asymptotic properties of the dipole gravity modes in the Sun, the quest to find individual gravity modes has continued. An extensive and deeper analysis of 14 years of continuous GOLF/SoHO observational data, unveils the presence of a pattern of peaks that could be interpreted as individual dipole gravity modes in the frequency range between 60 and 140 microHz, with amplitudes compatible with the latest theoretical predictions. By collapsing the power spectrum we have obtained a quite constant splitting for these patterns in comparison to regions where no g modes were expected. Moreover, the same technique applied to simultaneous VIRGO/SoHO data unveils some common signals between the power spectra of both instruments. Thus, we are able to identify and characterize individual g modes with their central frequencies, amplitudes and splittings allowing to do seismic inversions of the rotation profile inside the solar core. These results open a new ligh t on the physics and dynamics of the solar deep core. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SDLD5XPE/García et al. - 2011(2).pdf}
}

@article{Garcia2011b,
  title = {Preparation of {{Kepler}} Light Curves for Asteroseismic Analyses},
  author = {Garc{\'i}a, R. A. and Hekker, S. and Stello, D. and {Guti{\'e}rrez-Soto}, J. and Handberg, R. and Huber, D. and Karoff, C. and Uytterhoeven, K. and Appourchaux, T. and Chaplin, W. J. and Elsworth, Y. and Mathur, S. and Ballot, J. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Houdek, G. and Jenkins, J. M. and Kjeldsen, H. and McCauliff, S. and Metcalfe, T. and Middour, C. K. and {Molenda-Zakowicz}, J. and Monteiro, M. J.P.F.G. and Smith, J. C. and Thompson, M. J.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {414},
  number = {1},
  eprint = {1103.0382},
  pages = {6--10},
  issn = {17453933},
  doi = {10.1111/j.1745-3933.2011.01042.x},
  abstract = {The Kepler mission is providing photometric data of exquisite quality for the asteroseismic study of different classes of pulsating stars. These analyses place particular demands on the pre-processing of the data, over a range of time-scales from minutes to months. Here, we describe processing procedures developed by the Kepler Asteroseismic Science Consortium to prepare light curves that are optimized for the asteroseismic study of solar-like oscillating stars in which outliers, jumps and drifts are corrected. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society. \textcopyright{} 2011 RAS.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JCTRIAWW/García et al. - 2011(3).pdf}
}

@article{Garcia2013,
  title = {Towards Solar Activity Maximum 24 as Seen by {{GOLF}} and {{VIRGO}}/{{SPM}} Instruments},
  author = {Garc{\'i}a, R. A. and Salabert, D. and Mathur, S. and R{\'e}gulo, C. and Ballot, J. and Davies, G. R. and Jim{\'e}nez, A. and Simoniello, R.},
  year = {2013},
  journal = {Journal of Physics: Conference Series},
  volume = {440},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/440/1/012020},
  abstract = {All p-mode parameters vary with time as a response to the changes induced by the cyclic behavior of solar magnetic activity. After the unusual long solar-activity minimum between cycles 23 and 24 -where the p-mode parameters have shown a different behavior than the surface magnetic proxies- we analyze the temporal variation of low-degree p-mode parameters measured by GOLF (in velocity) and VIRGO (in intensity) Sun-as-a-star instruments on board SoHO. We compare our results with other activity proxies. \textcopyright{} 2013 Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LEL7EZQT/García et al. - 2013.pdf}
}

@article{Garcia2013a,
  title = {The {{Sun-as-a-star}} Observations: {{GOLF}} \& {{VIRGO}} on {{SoHO}}, and {{BiSON}} Network},
  author = {Garc{\'i}a, R. A. and Davies, G. R. and Jim{\'e}nez, A. and Ballot, J. and Mathur, S. and Salabert, D. and Chaplin, W. J. and Elsworth, Y. and R{\'e}gulo, C. and {Turck-Chi{\`e}ze}, S.},
  year = {2013},
  journal = {Journal of Physics: Conference Series},
  volume = {440},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/440/1/012040},
  abstract = {Sun-as-a-star observations are very important for the study of the conditions within the Sun and in particular for the deep interior where higher degree modes do not penetrate. They are also of significance in this era of dramatic advances in stellar asteroseismology as they are comparable to those measured in other stars by asteroseismic missions such as CoRoT, Kepler, and MOST. More than 17 years of continuous measurements of SoHO and more than 30 years of BiSON observations provide very long data sets of uninterrupted helioseismic observations. In this work, we discuss the present status of all these facilities that continue to provide state-of-the-art measurements and invaluable data to improve our knowledge of the deepest layers of the Sun and its structural changes during the activity cycle. \textcopyright{} 2013 Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/227T6CVB/García et al. - 2013(2).pdf}
}

@article{Garcia2014,
  title = {Impact on Asteroseismic Analyses of Regular Gaps in {{Kepler}} Data},
  author = {Garc{\'i}a, R. A. and Mathur, S. and Pires, S. and R{\'e}gulo, C. and Bellamy, B. and Pall{\'e}, P. L. and Ballot, J. and Barcel{\'o} Forteza, S. and Beck, P. G. and Bedding, T. R. and Ceillier, T. and Roca Cort{\'e}s, T. and Salabert, D. and Stello, D.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {568},
  pages = {1--8},
  issn = {14320746},
  doi = {10.1051/0004-6361/201323326},
  abstract = {Context. The NASA Kepler mission has observed more than 190 000 stars in the constellations of Cygnus and Lyra. Around 4 years of almost continuous ultra high-precision photometry have been obtained reaching a duty cycle higher than 90\% for many of these stars. However, almost regular gaps due to nominal operations are present in the light curves on different time scales. Aims. In this paper we want to highlight the impact of those regular gaps in asteroseismic analyses, and we try to find a method that minimizes their effect on the frequency domain. Methods. To do so, we isolate the two main time scales of quasi regular gaps in the data. We then interpolate the gaps and compare the power density spectra of four different stars: two red giants at different stages of their evolution, a young F-type star, and a classical pulsator in the instability strip. Results. The spectra obtained after filling the gaps in the selected solar-like stars show a net reduction in the overall background level, as well as a change in the background parameters. The inferred convective properties could change as much as \textasciitilde 200\% in the selected example, introducing a bias in the p-mode frequency of maximum power. When asteroseismic scaling relations are used, this bias can lead to a variation in the surface gravity of 0.05 dex. Finally, the oscillation spectrum in the classical pulsator is cleaner than the original one. \textcopyright{} ESO, 2014.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/3NJ2HXAV/García et al. - 2014.pdf}
}

@article{Garcia2014a,
  title = {Rotation and Magnetism of {{Kepler}} Pulsating Solar-like Stars: {{Towards}} Asteroseismically Calibrated Age-Rotation Relations},
  author = {Garc{\'i}a, R. A. and Ceillier, T. and Salabert, D. and Mathur, S. and Van Saders, J. L. and Pinsonneault, M. and Ballot, J. and Beck, P. G. and Bloemen, S. and Campante, T. L. and Davies, G. R. and Do Nascimento, J. D. and Mathis, S. and Metcalfe, T. S. and Nielsen, M. B. and Su{\'a}rez, J. C. and Chaplin, W. J. and Jim{\'e}nez, A. and Karoff, C.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {572},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201423888},
  abstract = {Kepler ultra-high precision photometry of long and continuous observations provides a unique dataset in which surface rotation and variability can be studied for thousands of stars. Because many of these old field stars also have independently measured asteroseismic ages, measurements of rotation and activity are particularly interesting in the context of age-rotation-activity relations. In particular, age-rotation relations generally lack good calibrators at old ages, a problem that this Kepler sample of old-field stars is uniquely suited to address. We study the surface rotation and photometric magnetic activity of a subset of 540 solar-like stars on the main-sequence and the subgiant branch for which stellar pulsations have been measured. The rotation period was determined by comparing the results from two different analysis methods: i) the projection onto the frequency domain of the time-period analysis, and ii) the autocorrelation function of the light curves. Reliable surface rotation rates were then extracted by comparing the results from two different sets of calibrated data and from the two complementary analyses. General photometric levels of magnetic activity in this sample of stars were also extracted by using a photometric activity index, which takes into account the rotation period of the stars. We report rotation periods for 310 out of 540 targets (excluding known binaries and candidate planet-host stars); our measurements span a range of 1 to 100 days. The photometric magnetic activity levels of these stars were computed, and for 61.5\% of the dwarfs, this level is similar to the range, from minimum to maximum, of the solar magnetic activity. We demonstrate that hot dwarfs, cool dwarfs, and subgiants have very different rotation-age relationships, highlighting the importance of separating out distinct populations when interpreting stellar rotation periods. Our sample of cool dwarf stars with age and metallicity data of the highest quality is consistent with gyrochronology relations reported in the literature.},
  keywords = {Asteroseismology,notion,notion-database,Stars: activity,Stars: evolution,Stars: oscillations,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/H2I3GZQW/García et al. - 2014(2).pdf}
}

@article{Garcia2014b,
  title = {Study of {{KIC}} 8561221 Observed by {{Kepler}}: {{An}} Early Red Giant Showing Depressed Dipolar Modes},
  author = {Garc{\'i}a, R. A. and P{\'e}rez Hern{\'a}ndez, F. and Benomar, O. and Silva Aguirre, V. and Ballot, J. and Davies, G. R. and Do{\v g}an, G. and Stello, D. and {Christensen-Dalsgaard}, J. and Houdek, G. and Ligni{\`e}res, F. and Mathur, S. and Takata, M. and Ceillier, T. and Chaplin, W. J. and Mathis, S. and Mosser, B. and Ouazzani, R. M. and Pinsonneault, M. H. and Reese, D. R. and R{\'e}gulo, C. and Salabert, D. and Thompson, M. J. and Van Saders, J. L. and Neiner, C. and De Ridder, J.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {563},
  pages = {1--17},
  issn = {14320746},
  doi = {10.1051/0004-6361/201322823},
  abstract = {Context. The continuous high-precision photometric observations provided by the CoRoT and Kepler space missions have allowed us to understand the structure and dynamics of red giants better using asteroseismic techniques. A small fraction of these stars show dipole modes with unexpectedly low amplitudes. The reduction in amplitude is more pronounced for stars with a higher frequency of maximum power, {$\nu$}max. Aims. In this work we want to characterise KIC 8561221 in order to confirm that it is currently the least evolved star among this peculiar subset and to discuss several hypotheses that could help explain the reduction of the dipole mode amplitudes. Methods. We used Kepler short-and long-cadence data combined with spectroscopic observations to infer the stellar structure and dynamics of KIC 8561221. We then discussed different scenarios that could contribute to reducing the dipole amplitudes, such as a fast-rotating interior or the effect of a magnetic field on the properties of the modes. We also performed a detailed study of the inertia and damping of the modes. Results. We have been able to characterise 36 oscillations modes, in particular, a few dipole modes above {$\nu$}max that exhibit nearly normal amplitudes. The frequencies of all the measured modes were used to determine the overall properties and the internal structure of the star. We have inferred a surface rotation period of \textasciitilde 91 days and uncovered a variation in the surface magnetic activity during the last 4 years. The analysis of the convective background did not reveal any difference compared to "normal" red giants. As expected, the internal regions of the star probed by the {$\mathscr{l}$} = 2 and 3 modes spin 4 to 8 times faster than the surface. Conclusions. With our grid of standard models we are able to properly fit the observed frequencies. Our model calculation of mode inertia and damping give no explanation for the depressed dipole modes. A fast-rotating core is also ruled out as a possible explanation. Finally, we do not have any observational evidence of a strong deep magnetic field inside the star. \textcopyright{} 2014 ESO.},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual: KIC 8561221,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/N39JKBD5/García et al. - 2014(3).pdf}
}

@article{Garcia2015,
  title = {Observational Techniques to Measure Solar and Stellar Oscillations},
  author = {Garc{\'i}a, R. A.},
  year = {2015},
  journal = {EAS Publications Series},
  volume = {73--74},
  number = {2015},
  eprint = {1510.02651},
  pages = {193--259},
  issn = {16381963},
  doi = {10.1051/eas/1573004},
  abstract = {As said by Sir A. Eddington in 1925: "Our telescopes may probe farther and farther into the depths of space. At first sight it would seem that the deep interior of the sun and stars is less accessible to scientific investigation than any other region of the universe. What appliance can pierce through the outer layers of a star and test the conditions within?" Eddington (1926). Nowadays, asteroseismology has proven its ability to pierce below stellar photospheres and allow us to "see" inside the interior of thousands of stars down to the stellar cores, answering the question asked by Eddington ninety years ago. In this chapter we review the general properties of the spectral analysis which is the base of any asteroseismic investigation. After describing the stellar power spectrum, we will describe in details the characterization of the modal spectrum. This chapter will end by a brief description of the instrumentation in both helio and asteroseismology.},
  archiveprefix = {arxiv},
  isbn = {9782759817351},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/C55YN5JH/García - 2015.pdf}
}

@article{Garcia2019,
  title = {Asteroseismology of Solar-Type Stars},
  author = {Garc{\'i}a, Rafael A. and Ballot, J{\'e}r{\^o}me},
  year = {2019},
  month = dec,
  journal = {Living Reviews in Solar Physics},
  volume = {16},
  number = {1},
  eprint = {1906.12262},
  pages = {4},
  publisher = {{Springer}},
  issn = {16144961},
  doi = {10.1007/s41116-019-0020-1},
  urldate = {2021-02-01},
  abstract = {Until the last few decades, investigations of stellar interiors had been restricted to theoretical studies only constrained by observations of their global properties and external characteristics. However, in the last 30 years the field has been revolutionized by the ability to perform seismic investigations of stellar interiors. This revolution begun with the Sun, where helioseismology has been yielding information competing with what can be inferred about the Earth's interior from geoseismology. The last two decades have witnessed the advent of asteroseismology of solar-like stars, thanks to a dramatic development of new observing facilities providing the first reliable results on the interiors of distant stars. The coming years will see a huge development in this field. In this review we focus on solar-type stars, i.e., cool main-sequence stars where oscillations are stochastically excited by surface convection. After a short introduction and a historical overview of the discipline, we review the observational techniques generally used, and we describe the theory behind stellar oscillations in cool main-sequence stars. We continue with a complete description of the normal mode analyses through which it is possible to extract the physical information about the structure and dynamics of the stars. We then summarize the lessons that we have learned and discuss unsolved issues and questions that are still unanswered.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Solar analogs,Stellar oscillations},
  file = {/Users/lbugnet/Zotero/storage/QTCEZBY4/full-text.pdf}
}

@article{GarciaPerez2016,
  title = {Aspcap: The {{Apogee Stellar Parameter}} and {{Chemical Abundances Pipeline}}},
  author = {Garc{\'i}a P{\'e}rez, Ana E. and Prieto, Carlos Allende and Holtzman, Jon A. and Shetrone, Matthew and M{\'e}sz{\'a}ros, Szabolcs and Bizyaev, Dmitry and Carrera, Ricardo and Cunha, Katia and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Johnson, Jennifer A. and Majewski, Steven R. and Nidever, David L. and Schiavon, Ricardo P. and Shane, Neville and Smith, Verne V. and Sobeck, Jennifer and Troup, Nicholas and Zamora, Olga and Weinberg, David H. and Bovy, Jo and Eisenstein, Daniel J. and Feuillet, Diane and Frinchaboy, Peter M. and Hayden, Michael R. and Hearty, Fred R. and Nguyen, Duy C. and O'Connell, Robert W. and Pinsonneault, Marc H. and Wilson, John C. and Zasowski, Gail},
  year = {2016},
  journal = {The Astronomical Journal},
  volume = {151},
  number = {6},
  eprint = {1510.07635},
  pages = {144},
  publisher = {{IOP Publishing}},
  issn = {0004-6256},
  doi = {10.3847/0004-6256/151/6/144},
  abstract = {The Apache Point Observatory Galactic Evolution Experiment (APOGEE) has built the largest moderately high-resolution (R=22, 500) spectroscopic map of the stars across the Milky Way, and including dust-obscured areas. The APOGEE Stellar Parameter and Chemical Abundances Pipeline (ASPCAP) is the software developed for the automated analysis of these spectra. ASPCAP determines atmospheric parameters and chemical abundances from observed spectra by comparing observed spectra to libraries of theoretical spectra, using chi-2 minimization in a multidimensional parameter space. The package consists of a fortran90 code that does the actual minimization, and a wrapper IDL code for book-keeping and data handling. This paper explains in detail the ASPCAP components and functionality, and presents results from a number of tests designed to check its performance. ASPCAP provides stellar effective temperatures, surface gravities, and metallicities precise to 2\%, 0.1 dex, and 0.05 dex, respectively, for most APOGEE stars, which are predominantly giants. It also provides abundances for up to 15 chemical elements with various levels of precision, typically under 0.1 dex. The final data release (DR12) of the Sloan Digital Sky Survey III contains an APOGEE database of more than 150,000 stars. ASPCAP development continues in the SDSS-IV APOGEE-2 survey.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: center,Galaxy: structure,methods: data analysis,notion,notion-database,stars: abundances,stars: atmospheres},
  file = {/Users/lbugnet/Zotero/storage/WNUS92EA/García Pérez et al. - 2016.pdf}
}

@article{Garrido1990,
  title = {{{PHASE SHIFTS BETWEEN COLOURS IN PULSATING STARS}} ** {{Abstract}} . {{Observational}} Evidence Is Presented Showing That the Time of Maximum Light for Pulsating Stars Depends on Observed Wavelength . {{This}} Fact Is Well Explained by Assuming That Starlight Variations},
  author = {Garrido, R and Guez, Rodr and Peg, D Y and Aqr, C Y and Lyn, T V and Cam, U Y and Cmi, A D},
  year = {1990},
  pages = {205--209},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/P2MY9ZF3/Garrido et al. - 1990.pdf}
}

@article{Gaulme2008,
  title = {{{SYMPA}}, a Dedicated Instrument for {{Jovian}} Seismology {{II}}. {{Real}} Performance and First Results},
  author = {Gaulme, P. and Schmider, F. X. and Gay, J. and Jacob, C. and Alvarez, M. and {Reyes-Ruiz}, M. and Belmonte, J. A. and Fossat, E. and Jeanneaux, F. and Valtier, J. C.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {490},
  number = {2},
  pages = {859--871},
  issn = {00046361},
  doi = {10.1051/0004-6361:200809512},
  abstract = {Aims. SYMPA is the first instrument dedicated to the observation of free oscillations of Jupiter. Its principles and theoretical performance have been presented in Paper I. This second paper describes the data processing method, the real instrumental performance and presents the first results of a Jovian observation run, lead in 2005 at Teide Observatory. Methods. SYMPA is a Fourier transform spectrometer which works at a fixed optical path difference. It produces Doppler shift maps of the observed object. The velocity amplitude of Jupiter's oscillations is expected to be below 60 cm s-1. Results. Despite light technical defects, the instrument was demonstrated to work correctly, being limited only by photon noise. A noise level of about 12 cm s-1 was reached on a 10-night observation run, with 21\% duty cycle, which is 5 time better than similar previous observations. However, no signal from Jupiter is clearly highlighted. \textcopyright{} ESO 2008.},
  keywords = {Instrumentation: interferometers,Methods: observational,notion,notion-database,Planets and satellites: formation,Planets and satellites: individual: Jupiter,Sun: helioseismology,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/UDPUWFFE/Gaulme et al. - 2008.pdf}
}

@article{Gaulme2009a,
  title = {Mode Width Fitting with a Simple {{Bayesian}} Approach: {{Application}} to {{CoRoT}} Targets {{HD}} 181420 and {{HD}} 49933},
  author = {Gaulme, P. and Appourchaux, T. and Boumier, P.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {7--14},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911920},
  abstract = {Aims. We investigate the asteroseismology of two solar-like targets as observed with the CoRoT satellite, with particular attention paid to the mode fitting. HD 181420 and HD 49933 are typical CoRoT solar-like targets (156 and 60-day runs). The low signal-to-noise ratio (SNR) of about 3-10 prevents us from unambiguously identifying the individual oscillation modes. In particular, convergence problems appear at the edges of the oscillation spectrum. Methods. We apply a Bayesian approach to the analysis of these data. We compare the global fitting of the power spectra obtained by the classical maximum likelihood (MLE) and the maximum a posteriori (MAP) estimators. Results. We examine the impact of the choice of the priors upon the fitted parameters. We also propose to reduce the number of free parameters in the fitting, by replacing the individual estimate of mode height associated with each overtone by a continuous function of frequency (Gaussian profile). Conclusions. The MAP appears as a powerful tool to constrain the global fits, but it must be used carefully and only with reliable priors. The mode width of the stars increases with the frequency over all the oscillation spectrum.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/5LI82PKK/Gaulme, Appourchaux, Boumier - 2009.pdf}
}

@article{Gaulme2010,
  title = {{{HD}} 46375: {{Seismic}} and Spectropolarimetric Analysis of a Young {{Sun}} Hosting a {{Saturn-like}} Planet},
  author = {Gaulme, P. and Deheuvels, S. and Weiss, W. W. and Mosser, B. and Moutou, C. and Bruntt, H. and Donati, J. F. and Vannier, M. and Guillot, T. and Appourchaux, T. and Michel, E. and Auvergne, M. and Samadi, R. and Baudin, F. and Catala, C. and Baglin, A.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {524},
  number = {2},
  issn = {00046361},
  doi = {10.1051/0004-6361/201014142},
  abstract = {Context. HD 46375 is known to host a Saturn-like exoplanet orbiting at 0.04 AU from its host star. Stellar light reflected by the planet was tentatively identified in the 34-day CoRoT run acquired in October-November 2008. Aims. We constrain the properties of the magnetic field of HD 46375 based on spectropolarimetric observations with the NARVAL spectrograph at the Pic du Midi observatory. In addition, we use a high-resolution NARVAL flux spectrum to contrain the atmospheric parameters. With these constraints, we perform an asteroseismic analysis and modelling of HD 46375 using the frequencies extracted from the CoRoT light curve. Methods. We used Zeeman Doppler imaging to reconstruct the magnetic map of the stellar surface. In the spectroscopic analysis we fitted isolated lines using 1D LTE atmosphere models. This analysis was used to constrain the effective temperature, surface gravity, and chemical composition of the star. To extract information about the p-mode oscillations, we used a technique based on the envelope autocorrelation function (EACF). Results. From the Zeeman Doppler imaging observations, we observe a magnetic field of {$\approx$} 5 Gauss. From the spectral analysis, HD 46375 is inferred to be an unevolved K0 type star with high metallicity [Fe/H] = +0.39. Owing to the relative faintness of the star (mhip = 8.05), the signal-to-noise ratio is too low to identify individual modes. However, we measure the p-mode excess power and large separation {$\Delta\nu$}0 = 153.0{$\pm$}0.7 {$\mu$}Hz. Conclusions. We are able do constrain the fundamental parameters of the star thanks to spectrometric and seismic analyses. We conclude that HD 46375 is similar to a young version of {$\alpha$} Cen B. This work is of special interest because of its combination of exoplanetary science and asteroseismology, which are the subjects of the current Kepler mission and the proposed Plato mission. \textcopyright{} 2010 ESO.},
  keywords = {methods: data analysis,methods: observational,notion,notion-database,planetary systems,stars: individual: HD 46375,stars: magnetic field,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/R9TNC826/Gaulme et al. - 2010.pdf}
}

@article{Gaulme2010a,
  title = {Possible Detection of Phase Changes from the Non-Transiting Planet {{HD}} 46375b by {{CoRoT}}},
  author = {Gaulme, P. and Vannier, M. and Guillot, T. and Mosser, B. and Mary, D. and Weiss, W. W. and Schmider, F. X. and Bourguignon, S. and Deeg, H. J. and R{\'e}gulo, C. and Aigrain, S. and Schneider, J. and Bruntt, H. and Deheuvels, S. and Donati, J. F. and Appourchaux, T. and Auvergne, M. and Baglin, A. and Baudin, F. and Catala, C. and Michel, E. and Samadi, R.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {518},
  number = {22},
  pages = {1--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201014303},
  abstract = {Context. The present work deals with the detection of phase changes in an exoplanetary system. HD 46375 is a solar analog known to host a non-transiting Saturn-mass exoplanet with a 3.0236 day period. It was observed by the CoRoT satellite for 34 days during the fall of 2008. Aims. We attempt to identify at optical wavelengths, the changing phases of the planet as it orbits its star. We then try to improve the star model by means of a seismic analysis of the same light curve and the use of ground-based spectropolarimetric observations. Methods. The data analysis relies on the Fourier spectrum and the folding of the time series. Results. We find evidence of a sinusoidal signal compatible in terms of both amplitude and phase with light reflected by the planet. Its relative amplitude is {$\Delta$} Fp/F* = [13.0, 26.8] ppm, implying an albedo A = [0.16, 0.33] or a dayside visible brightness temperature Tb [1880, 2030] K by assuming a radius R = 1.1 R Jup and an inclination i = 45\textdegree. Its orbital phase differs from that of the radial-velocity signal by at most 2 {$\sigma$}RV. However, the tiny planetary signal is strongly blended by another signal, which we attribute to a telluric signal with a 1 day period. We show that this signal is suppressed, but not eliminated, when using the time series for HD 46179 from the same CoRoT run as a reference. Conclusions. This detection of reflected light from a non-transiting planet should be confirmable with a longer CoRoT observation of the same field. In any case, it demonstrates that non-transiting planets can be characterized using ultra-precise photometric lightcurves with present-day observations by CoRoT and Kepler. The combined detection of solar-type oscillations on the same targets (Gaulme et al. 2010a) highlights the overlap between exoplanetary science and asteroseismology and shows the high potential of a mission such as Plato. \textcopyright{} 2010 ESO.},
  keywords = {Methods: data analysis,notion,notion-database,Planetary systems,Stars: individual: HD 46375,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/IN5Q488C/Gaulme et al. - 2010(2).pdf}
}

@article{Gaulme2011,
  title = {Detection of {{Jovian}} Seismic Waves: {{A}} New Probe of Its Interior Structure},
  author = {Gaulme, P. and Schmider, F. X. and Gay, J. and Guillot, T. and Jacob, C.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {531},
  number = {January},
  pages = {1--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116903},
  abstract = {Knowledge of Jupiter's deep interior would provide unique constraints on the formation of the Solar System. Measurement of its core mass and global composition would shed light on whether the planet formed by accretion or by direct gravitational collapse. At present, the inner structure of Jupiter is poorly constrained and seismology, which consists of identifying acoustic eigenmodes, offers a way to directly measure its deep sound speed profile, and thus its physical properties. Seismology of Jupiter has been considered since the mid 1970s, but hitherto the various attempts to detect global modes have led, at best, to ambiguous results. We report the detection of global modes of Jupiter, based on radial velocity measurements performed with the SYMPA Fourier spectro-imager. The global seismic parameters that we measure include the frequency of maximum amplitude 1213 {$\pm$} 50 {$\mu$}Hz, the mean large frequency spacing between radial harmonics 155.3 {$\pm$} 2.2 {$\mu$}Hz, and the mode maximum amplitude 49-10+8 cm s-1, all values that are consistent with current models of Jupiter. This result opens the way to the investigation of the inner structure of the Solar System's giant planets based on seismology techniques. \textcopyright{} 2011 ESO.},
  keywords = {Asteroseismology,data analysis-asteroseismology,individual,interiors-waves-techniques,Jupiter-planets and satellites,Methods: data analysis,notion,notion-database,planets and satellites,Planets and satellites: individual: Jupiter,Planets and satellites: interiors,radial velocities-methods,Techniques: radial velocities,Waves},
  file = {/Users/lbugnet/Zotero/storage/RRMDIU2C/Gaulme et al. - 2011.pdf}
}

@article{Gaulme2013a,
  title = {Red Giants in Eclipsing Binary and Multiple-Star Systems: {{Modeling}} and Asteroseismic Analysis of 70 Candidates from {{Kepler}} Data},
  author = {Gaulme, P. and McKeever, J. and Rawls, M. L. and Jackiewicz, J. and Mosser, B. and Guzik, J. A.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {767},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/767/1/82},
  abstract = {Red giant stars are proving to be an incredible source of information for testing models of stellar evolution, as asteroseismology has opened up a window into their interiors. Such insights are a direct result of the unprecedented data from space missions CoRoT and Kepler as well as recent theoretical advances. Eclipsing binaries are also fundamental astrophysical objects, and when coupled with asteroseismology, binaries provide two independent methods to obtain masses and radii and exciting opportunities to develop highly constrained stellar models. The possibility of discovering pulsating red giants in eclipsing binary systems is therefore an important goal that could potentially offer very robust characterization of these systems. Until recently, only one case has been discovered with Kepler. We cross-correlate the detected red giant and eclipsing-binary catalogs from Kepler data to find possible candidate systems. Light-curve modeling and mean properties measured from asteroseismology are combined to yield specific measurements of periods, masses, radii, temperatures, eclipse timing variations, core rotation rates, and red giant evolutionary state. After using three different techniques to eliminate false positives, out of the 70 systems common to the red giant and eclipsing-binary catalogs we find 13 strong candidates (12 previously unknown) to be eclipsing binaries, one to be a non-eclipsing binary with tidally induced oscillations, and 10 more to be hierarchical triple systems, all of which include a pulsating red giant. The systems span a range of orbital eccentricities, periods, and spectral types F, G, K, and M for the companion of the red giant. One case even suggests an eclipsing binary composed of two red giant stars and another of a red giant with a {$\delta$}-Scuti star. The discovery of multiple pulsating red giants in eclipsing binaries provides an exciting test bed for precise astrophysical modeling, and follow-up spectroscopic observations of many of the candidate systems are encouraged. The resulting highly constrained stellar parameters will allow, for example, the exploration of how binary tidal interactions affect pulsations when compared to the single-star case. \textcopyright{} 2013. The American Astronomical Society. All rights reserved..},
  keywords = {binaries: eclipsing,methods: data analysis,notion,notion-database,stars: AGB and post-AGB,stars: interiors,stars: oscillations (including pulsations),techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/R2GM7WE3/Gaulme et al. - 2013.pdf}
}

@article{Gaulme2014,
  title = {Surface Activity and Oscillation Amplitudes of Red Giants in Eclipsing Binaries},
  author = {Gaulme, P. and Jackiewicz, J. and Appourchaux, T. and Mosser, B.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {785},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/785/1/5},
  abstract = {Among the 19 red-giant stars belonging to eclipsing binary systems that have been identified in Kepler data, 15 display solar-like oscillations. We study whether the absence of mode detection in the remaining 4 is an observational bias or possibly evidence of mode damping that originates from tidal interactions. A careful analysis of the corresponding Kepler light curves shows that modes with amplitudes that are usually observed in red giants would have been detected if they were present. We observe that mode depletion is strongly associated with short-period systems, in which stellar radii account for 16\%-24\% of the semi-major axis, and where red-giant surface activity is detected. We suggest that when the rotational and orbital periods synchronize in close binaries, the red-giant component is spun up, so that a dynamo mechanism starts and generates a magnetic field, leading to observable stellar activity. Pressure modes would then be damped as acoustic waves dissipate in these fields. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  keywords = {binaries: eclipsing,notion,notion-database,stars: evolution,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/YMQZSWRK/Gaulme et al. - 2014.pdf}
}

@article{Gaulme2014a,
  title = {Seismology of {{Giant Planets}}},
  author = {Gaulme, Patrick and Mosser, Benoit and Schmider, Francois-Xavier and Guillot, Tristan and Jackiewicz, Jason},
  year = {2014},
  month = nov,
  journal = {Extraterrestrial Seismology},
  eprint = {1411.1740},
  pages = {189--202},
  publisher = {{Cambridge University Press}},
  doi = {10.1017/CBO9781107300668.017},
  urldate = {2020-05-21},
  abstract = {Seismology applied to giant planets could drastically change our understanding of their deep interiors, as it has happened with the Earth, the Sun, and many main-sequence and evolved stars. The study of giant planets' composition is important for understanding both the mechanisms enabling their formation and the origins of planetary systems, in particular our own. Unfortunately, its determination is complicated by the fact that their interior is thought not to be homogeneous, so that spectroscopic determinations of atmospheric abundances are probably not representative of the planet as a whole. Instead, the determination of their composition and structure must rely on indirect measurements and interior models. Giant planets are mostly fluid and convective, which makes their seismology much closer to that of solar-like stars than that of terrestrial planets. Hence, helioseismology techniques naturally transfer to giant planets. In addition, two alternative methods can be used: photometry of the solar light reflected by planetary atmospheres, and ring seismology in the specific case of Saturn. The current decade has been promising thanks to the detection of Jupiter's acoustic oscillations with the ground-based imaging-spectrometer SYMPA and indirect detection of Saturn's f-modes in its rings by the NASA Cassini orbiter. This has motivated new projects of ground-based and space-borne instruments that are under development. The purpose of this paper is to support the chapter Seismology of Giant Planets which will appear in May 2015 in the book Extraterrestrial Seismology, published in Cambridge University Press. Here, we review the key questions about jovian interiors as well as the most recent observational results, and refer the reader to the book chapter above-mentioned for further details.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZPJNJC6E/full-text.pdf}
}

@article{Gaulme2016,
  title = {A {{Distant Mirror}}: {{Solar Oscillations Observed}} on {{Neptune By}} the {{Kepler K}} 2 {{Mission}}},
  author = {Gaulme, P. and Rowe, J. F. and Bedding, T. R. and Benomar, O. and Corsaro, E. and Davies, G. R. and Hale, S. J. and Howe, R. and Garcia, R. A. and Huber, D. and Jim{\'e}nez, A. and Mathur, S. and Mosser, B. and Appourchaux, T. and Boumier, P. and Jackiewicz, J. and Leibacher, J. and Schmider, F.-X. and Hammel, H. B. and Lissauer, J. J. and Marley, M. S. and Simon, A. A. and Chaplin, W. J. and Elsworth, Y. and Guzik, J. A. and Murphy, N. and Aguirre, V. Silva},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {833},
  number = {1},
  eprint = {1612.04287},
  pages = {L13},
  publisher = {{IOP Publishing}},
  issn = {2041-8213},
  doi = {10.3847/2041-8213/833/1/l13},
  abstract = {Starting in December 2014, Kepler K2 observed Neptune continuously for 49 days at a 1-minute cadence. The goals consisted of studying its atmospheric dynamics (Simon et al. 2016), detecting its global acoustic oscillations (Rowe et al., submitted), and those of the Sun, which we report on here. We present the first indirect detection of solar oscillations in intensity measurements. Beyond the remarkable technical performance, it indicates how Kepler would see a star like the Sun. The result from the global asteroseismic approach, which consists of measuring the oscillation frequency at maximum amplitude "nu\_max" and the mean frequency separation between mode overtones "Delta nu", is surprising as the nu\_max measured from Neptune photometry is larger than the accepted value. Compared to the usual reference nu\_max\_sun = 3100 muHz, the asteroseismic scaling relations therefore make the solar mass and radius appear larger by 13.8 +/- 5.8 \% and 4.3 +/- 1.9 \% respectively. The higher nu\_max is caused by a combination of the value of nu\_max\_sun, being larger at the time of observations than the usual reference from SOHO/VIRGO/SPM data (3160 +/- 10 muHz), and the noise level of the K2 time series, being ten times larger than VIRGO's. The peak-bagging method provides more consistent results: despite a low signal-to-noise ratio (SNR), we model ten overtones for degrees l=0,1,2. We compare the K2 data with simultaneous SOHO/VIRGO/SPM photometry and BiSON velocity measurements. The individual frequencies, widths, and amplitudes mostly match those from VIRGO and BiSON within 1 sigma, except for the few peaks with lowest SNR.},
  archiveprefix = {arxiv},
  keywords = {1,helioseismology,including pulsations,individual,it is well known,neptune,notion,notion-database,oscillations,oscillations on a 5,photometric,planets and satellites,planets and satellites: individual (Neptune),solar modes,stars,stars: oscillations (including pulsations),sun,Sun: helioseismology,techniques,techniques: photometric,that the sun exhibits,the importance of reflected},
  file = {/Users/lbugnet/Zotero/storage/28PHQHNW/Gaulme et al. - 2016.pdf}
}

@article{Gaulme2020,
  title = {Active Red Giants: {{Close}} Binaries versus Single Rapid Rotators},
  author = {Gaulme, P. and Jackiewicz, J. and Spada, F. and Chojnowski, D. and Mosser, B. and McKeever, J. and Hedlund, A. and Vrard, M. and Benbakoura, M. and Damiani, C.},
  year = {2020},
  month = jun,
  journal = {Astronomy and Astrophysics},
  eprint = {2004.13792},
  publisher = {{EDP Sciences}},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202037781},
  urldate = {2020-07-21},
  abstract = {The objective of this work is to determine what fraction of red-giant (RG) stars shows photometric rotational modulation, and understand its origin. One of the underlying questions is the role of close binarity in this population, standing upon the fact that RGs in short-period binary systems ({$<$}150 days or so) have been observed to display strong rotational modulation. We select a sample of about 4500 relatively bright RGs observed by Kepler, and show that 370 of them (8\%) display rotational modulation. Almost all have oscillation amplitudes below the median of the sample, while 30 of them are not oscillating at all. Of the 85 of these RGs with rotational modulation chosen for follow-up radial-velocity observation and analysis, 34 show clear evidence of spectroscopic binarity. Surprisingly, 26 of the 30 non-oscillators are in this group of binaries. To the contrary, about 85\% of the active RGs with detectable oscillations are not part of close binaries. With the help of stellar masses and evolutionary states computed from the oscillation properties, it appears that low-mass red-giant branch stars tend to be magnetically inactive, while intermediate-mass ones tend to be highly active. The opposite trends are true for helium-core burning (red clump) stars, whereby the lower-mass clump stars are comparatively more active and the higher-mass ones less so. In other words, we find that low-mass red-giant branch stars gain angular momentum as they evolve to clump stars, while higher-mass ones lose angular momentum. The trend observed with low-mass stars leads to possible scenarios of planet engulfment or other merging events during the shell-burning phase. Regarding intermediate-mass stars, the rotation periods are long with respect to theoretical expectations reported in the literature, which reinforces the existence of an unidentified sink of angular momentum after the main sequence.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6TJ656EM/full-text.pdf}
}

@article{Gaurat2015,
  title = {Evolution of a Magnetic Field in a Differentially Rotating Radiative Zone},
  author = {Gaurat, M. and Jouve, L. and Ligni{\`e}res, F. and Gastine, T.},
  year = {2015},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {580},
  eprint = {1507.01508},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526125},
  urldate = {2020-06-19},
  abstract = {Context. Recent spectropolarimetric surveys of main-sequence intermediate-mass stars have exhibited a dichotomy in the distribution of the observed magnetic field between the kG dipoles of Ap/Bp stars and the sub-Gauss magnetism of Vega and Sirius. Aims. We would like to test whether this dichotomy is linked to the stability versus instability of large-scale magnetic configurations in differentially rotating radiative zones. Methods. We computed the axisymmetric magnetic field obtained from the evolution of a dipolar field threading a differentially rotating shell. A full parameter study including various density profiles and initial and boundary conditions was performed with a 2D numerical code. We then focused on the ratio between the toroidal and poloidal components of the magnetic field and discuss the stability of the configurations dominated by the toroidal component using local stability criteria and insights from recent 3D numerical simulations. Results. The numerical results and a simple model show that the ratio between the toroidal and the poloidal magnetic fields is highest after an Alfv\'en crossing time of the initial poloidal field. For high density contrasts, this ratio converges towards an asymptotic value that can thus be extrapolated to realistic stellar cases. We then consider the stability of the magnetic configurations to non-axisymmetric perturbations and find that configurations dominated by the toroidal component are likely to be unstable if the shear strength is significantly higher than the poloidal Alfv\'en frequency. An expression for the critical poloidal field below which magnetic fields are likely to be unstable is found and is compared to the lower bound of Ap/Bp magnetic fields.},
  archiveprefix = {arxiv},
  keywords = {Magnetohydrodynamics (MHD),Methods: numerical,notion,notion-database,Stars: interiors,Stars: magnetic field,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/WCYVEXZS/full-text.pdf}
}

@article{Gautschy1993,
  title = {Pulsating Post-Asymptotic Giant Branch Stars},
  author = {Gautschy, Alfred},
  year = {1993},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {265},
  pages = {340--346},
  urldate = {2020-04-09},
  abstract = {Numerical stability analyses of envelopes of post-asymptotic giant branch stars show instabilities towards radial pulsations over a broad range of effective temperatures , although only stars with sufficiently high luminosity-to-mass ratios and high enough iron abundances are excited. Particular choices for the concentrations of the remaining chemical elements in the stellar envelopes appear to be of minor importance for destabilization. The instabilities turn out to be generated or at least strongly influenced by the enhanced iron bump apparent in the opal opacity tables. The pulsations of the central star of the young planetary nebula IC418 can be modelled by adopting stellar parameters constrained by observations.},
  keywords = {abundances-stars,AGB and post-AGB-stars,IC 418,individual,instabilities-methods,notion,notion-database,numerical-stars,oscillations-planetary nebulae},
  file = {/Users/lbugnet/Zotero/storage/P2RJ7MKP/full-text.pdf}
}

@article{Ge2006,
  title = {The {{First Extrasolar Planet Discovered}} with a {{New Generation High Throughput Doppler Instrument}}},
  author = {Ge, Jian and {van Eyken}, Julian and Mahadevan, Suvrath and DeWitt, Curtis and Kane, Stephen R. and Cohen, Roger and Heuvel, Andrew Vanden and Fleming, Scott W. and Guo, Pengcheng and Henry, Gregory W. and Schneider, Donald P. and Ramsey, Lawrence W. and Wittenmyer, Robert A. and Endl, Michael and Cochran, William D. and Ford, Eric B. and Martin, Eduardo L. and Israelian, Garik and Valenti, Jeff and Montes, David},
  year = {2006},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {648},
  number = {1},
  eprint = {astro-ph/0605247},
  pages = {683--695},
  publisher = {{IOP Publishing}},
  doi = {10.1086/505699},
  urldate = {2020-07-13},
  abstract = {We report the detection of the first extrasolar planet, ET-1 (HD 102195b), using the Exoplanet Tracker (ET), a new generation Doppler instrument. The planet orbits HD 102195, a young star with solar metallicity that may be part of the local association. The planet imparts radial velocity variability to the star with a semiamplitude of \$63.4\textbackslash pm2.0\$ m s\$\^\{-1\}\$ and a period of 4.11 days. The planetary minimum mass (\$m \textbackslash sin i\$) is \$0.488\textbackslash pm0.015\$ \$M\_J\$.},
  archiveprefix = {arxiv},
  keywords = {individual ( HD 102195)-techniques,instrumentation,interferometers-instrumentation,notion,notion-database,radial velocities,spectrographs-planetary systems-stars,Subject headingg s},
  file = {/Users/lbugnet/Zotero/storage/6K9INFH8/full-text.pdf}
}

@article{Gehan2018,
  title = {Core Rotation Braking on the Red Giant Branch for Various Mass Ranges},
  author = {Gehan, C. and Mosser, B. and Michel, E. and Samadi, R. and Kallinger, T.},
  year = {2018},
  journal = {Astronomy and Astrophysics},
  volume = {616},
  eprint = {1802.04558},
  pages = {1--12},
  issn = {14320746},
  doi = {10.1051/0004-6361/201832822},
  abstract = {Context. Asteroseismology allows us to probe stellar interiors. In the case of red giant stars, conditions in the stellar interior are such as to allow for the existence of mixed modes, consisting in a coupling between gravity waves in the radiative interior and pressure waves in the convective envelope. Mixed modes can thus be used to probe the physical conditions in red giant cores. However, we still need to identify the physical mechanisms that transport angular momentum inside red giants, leading to the slow-down observed for red giant core rotation. Thus large-scale measurements of red giant core rotation are of prime importance to obtain tighter constraints on the efficiency of the internal angular momentum transport, and to study how this efficiency changes with stellar parameters. Aims. This work aims at identifying the components of the rotational multiplets for dipole mixed modes in a large number of red giant oscillation spectra observed by Kepler. Such identification provides us with a direct measurement of the red giant mean core rotation. Methods. We compute stretched spectra that mimic the regular pattern of pure dipole gravity modes. Mixed modes with the same azimuthal order are expected to be almost equally spaced in stretched period, with a spacing equal to the pure dipole gravity mode period spacing. The departure from this regular pattern allows us to disentangle the various rotational components and therefore to determine the mean core rotation rates of red giants. Results. We automatically identify the rotational multiplet components of 1183 stars on the red giant branch with a success rate of 69\% with respect to our initial sample. As no information on the internal rotation can be deduced for stars seen pole-on, we obtain mean core rotation measurements for 875 red giant branch stars. This large sample includes stars with a mass as large as 2.5 M{${_\ast}$}, allowing us to test the dependence of the core slow-down rate on the stellar mass. Conclusions. Disentangling rotational splittings from mixed modes is now possible in an automated way for stars on the red giant branch, even for the most complicated cases, where the rotational splittings exceed half the mixed-mode spacing. This work on a large sample allows us to refine previous measurements of the evolution of the mean core rotation on the red giant branch. Rather than a slight slow-down, our results suggest rotation is constant along the red giant branch, with values independent of the mass.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: interiors,Stars: oscillations,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/GDYI77WH/Gehan et al. - 2018.pdf}
}

@techreport{Gehan2018a,
  title = {Core Rotation Braking on the Red Giant Branch for Various Mass Ranges},
  author = {Gehan, C and Mosser, B and Michel, E and Samadi, R and Kallinger, T},
  year = {2018},
  eprint = {1802.04558v1},
  urldate = {2020-05-03},
  abstract = {Context. Asteroseismology allows us to probe stellar interiors. In the case of red giant stars, conditions in the stellar interior are such to allow for the existence of mixed modes, consisting in a coupling between gravity waves in the radiative interior and pressure waves in the convective envelope. Mixed modes can thus be used to probe the physical conditions in red giant cores. However, we still need to identify the physical mechanisms that transport angular momentum inside red giants, leading to the slowdown observed for the red giant core rotation. Thus large-scale measurements of the red giant core rotation are of prime importance to obtain tighter constraints on the efficiency of the internal angular momentum transport, and to study how this efficiency changes with stellar parameters. Aims. This work aims at identifying the components of the rotational multiplets for dipole mixed modes in a large number of red giant oscillation spectra observed by Kepler. Such identification provides us with a direct measurement of the red giant mean core rotation. Methods. We compute stretched spectra that mimic the regular pattern of pure dipole gravity modes. Mixed modes with same azimuthal order are expected to be almost equally spaced in stretched period, with a spacing equals to the pure dipole gravity mode period spacing. The departure from this regular pattern allows us to disentangle the various rotational components and therefore to determine the mean core rotation rates of red giants. Results. We automatically identify the rotational multiplet components of 1183 stars on the red giant branch with a success rate of 69\% with respect to our initial sample. As no information on the internal rotation can be deduced for stars seen pole-on, we obtain mean core rotation measurements for 875 red giant branch stars. This large sample includes stars with a mass as large as 2.5 M, allowing us to test the dependence of the core slowdown rate on the stellar mass. Conclusions. Disentangling rotational splittings from mixed modes is now possible in an automated way for stars on the red giant branch, even for the most complicated cases, where the rotational splittings exceed half the mixed-mode period spacing. This work on a large sample allows us to refine previous measurements of the evolution of the mean core rotation on the red giant branch. Rather than a slight slow down, our results suggest rotation to be constant along the red giant branch, with values independent on the mass.},
  archiveprefix = {arxiv},
  keywords = {evolution-Stars,interior-Stars,notion,notion-database,oscillations-Stars,rotation,Stars},
  file = {/Users/lbugnet/Zotero/storage/7TX9IU9Y/full-text.pdf}
}

@phdthesis{Gehan2019,
  title = {\'Evolution de La Rotation Du C\oe ur Des \'Etoiles Sur La Branche Des G\'eantes Rouges : Des Mesures \`a Grande \'Echelle Vers Une Caract\'erisation Du Transport de Moment Cin\'etique {{To}} Cite This Version : {{HAL Id}} : Tel-02128409 de l ' {{Universit\'e}} de Recherche {{Paris Scien}}},
  author = {Gehan, Charlotte},
  year = {2019},
  keywords = {notion,notion-database}
}

@article{Gehan2021,
  title = {Automated Approach to Measure Stellar Inclinations: Validation through Large-Scale Measurements on the Red Giant Branch},
  author = {Gehan, C and Mosser, B and Michel, E and Cunha, M S},
  year = {2020},
  eprint = {2011.02502v2},
  urldate = {2021-10-22},
  abstract = {Context. Measuring stellar inclinations is fundamental to understanding planetary formation and dynamics as well as the physical conditions during star formation. Oscillation spectra of red giant stars exhibit mixed modes that have both a gravity component from the radiative interior and a pressure component from the convective envelope. Gravity-dominated (g-m) mixed modes split by rotation are well separated inside frequency spectra, allowing accurate measurement of stellar inclinations. Aims. We aim to develop an automated and general approach to measuring stellar inclinations that can be applied to any solar-type pulsator for which oscillation modes are identified. We also aim to validate this approach using red giant branch stars observed by Kepler. Methods. Stellar inclination impacts the visibility of oscillation modes with azimuthal orders m = \{-1, 0, +1\}. We used the mean height-to-background ratio of dipole mixed modes with different azimuthal orders to measure stellar inclinations. We recovered the underlying statistical distribution of inclinations in an unbiased way using a probability density function for the stellar inclination angle. Results. We derive stellar inclination measurements for 1139 stars on the red giant branch for which Gehan et al. (2018) identified the azimuthal order of dipole g-m mixed modes. Raw measured inclinations exhibit strong deviation with respect to isotropy which is expected for random inclinations over the sky. When taking uncertainties into account, the reconstructed distribution of inclinations actually follows the expected isotropic distribution of the rotational axis. Conclusions. This work highlights the biases that affect inclination measurements and provides a way to infer their underlying statistical distribution. When a star is seen either pole on or equator on, measurements are challenging and result in a biased distribution. Correcting biases that appear in low-and high-inclination regimes allows us to recover the underlying inclination distribution.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Asteroseismology-Methods,data analysis-Techniques,interiors-Stars,low-mass-Stars,Methods: data analysis,notion,notion-database,photometric-Stars,solar-type,Stars: interiors,Stars: low-mass,Stars: solar-type,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/NEVZMKD3/full-text.pdf}
}

@article{Geier2013,
  title = {Hot Subdwarf Stars in Close-up View - {{III}}. {{Metal}} Abundances of Subdwarf {{B}} Stars},
  author = {Geier, S.},
  year = {2013},
  month = jan,
  journal = {Astronomy \& Astrophysics},
  volume = {549},
  eprint = {1211.2689},
  primaryclass = {astro-ph},
  pages = {A110},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201220549},
  urldate = {2023-10-02},
  abstract = {Context: Hot subdwarf B stars (sdBs) are considered to be core helium-burning stars with very thin hydrogen envelopes situated on or near the extreme horizontal branch (EHB). The formation of sdBs is still unclear as well as the chemical composition of their atmospheres. The observed helium depletion is attributed to atmospheric diffusion. Metal abundances have been determined for about a dozen sdBs only resulting in puzzling patterns with enrichment of heavy metals and depletion of lighter ones. Aims: In this paper we present a detailed metal abundance analysis of 106 sdBs. Methods: From high resolution spectra we measured elemental abundances of up to 24 different ions per star. A semi-automatic analysis pipeline was developed to calculate and fit LTE models to a standard set of spectral lines. Results: A general trend of enrichment was found with increasing temperature for most of the heavier elements. The lighter elements like carbon, oxygen and nitrogen are depleted and less affected by temperature. Although there is considerable scatter from star to star, the general abundance patterns in most sdBs are similar. State-of-the-art diffusion models predict such patterns and are in qualitative agreement with our results. However, the highest enrichments measured cannot not be explained with these models. Peculiar line shapes of the strongest metal lines in some stars indicate vertical stratification to be present in the atmospheres. Such effects are not accounted for in current diffusion models and may be responsible for some of the yet unexplained abundance anomalies.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/TJGSTW4A/Geier - 2013 - Hot subdwarf stars in close-up view - III. Metal a.pdf;/Users/lbugnet/Zotero/storage/7665YGKM/1211.html}
}

@article{Gelly2002a,
  title = {Solar P-Modes from 1979 Days of the {{GOLF}} Experiment},
  author = {Gelly, B. and Lazrek, M. and Grec, G. and Ayad, A. and Schmider, F. X. and Renaud, C. and Salabert, D. and Fossat, E.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {394},
  number = {1},
  pages = {285--297},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021106},
  abstract = {With the GOLF instrument onboard the SoHO observatory, 1979 days of full-disc Doppler velocity observations have been compiled into a study of p-mode properties. We develop a multi-step iterative method (MSIM) algorithm to access all p-mode parameters while minimizing any perturbating effect or cross-talk between parameters during their determination. We present frequency and splitting tables, amplitudes, linewidths, line asymmetries, pseudo-modes, and background noise determinations. We have a first look at the changes induced by the transition from the low-activity to the high-activity part of solar cycle 23: we have recorded frequency shifts with a downturn at 3.7 mHz followed by a possible higher upturn, and linewidth changes to a good accuracy. We detect an effect on the noise background at 3 mHz possibly related to an interaction between noise and the modes and connected to the asymmetry of the profiles.},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/UF6XWGZZ/Gelly et al. - 2002.pdf}
}

@techreport{Genuer,
  title = {Random {{Forests}}: Some Methodological Insights},
  author = {Genuer, Robin and Poggi, Jean-Michel and Tuleau, Christine},
  urldate = {2020-03-23},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3GBLR6HW/full-text.pdf}
}

@phdthesis{Genuer2008,
  title = {Random {{Forests}}: Some Methodological Insights},
  author = {Genuer, Robin and Poggi, Jean-Michel and Tuleau, Christine},
  year = {2008},
  month = nov,
  eprint = {0811.3619},
  urldate = {2020-07-07},
  abstract = {This paper examines from an experimental perspective random forests, the increasingly used statistical method for classification and regression problems introduced by Leo Breiman in 2001. It first aims at confirming, known but sparse, advice for using random forests and at proposing some complementary remarks for both standard problems as well as high dimensional ones for which the number of variables hugely exceeds the sample size. But the main contribution of this paper is twofold: to provide some insights about the behavior of the variable importance index based on random forests and in addition, to propose to investigate two classical issues of variable selection. The first one is to find important variables for interpretation and the second one is more restrictive and try to design a good prediction model. The strategy involves a ranking of explanatory variables using the random forests score of importance and a stepwise ascending variable introduction strategy.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/88P22MMN/full-text.pdf}
}

@phdthesis{Genuer2017,
  title = {Arbres {{CART}} et {{For\^ets}} Al\'eatoires, {{Importance}} et S\'election de Variables {{Arbres CART}} et {{For\^ets}} Al\'eatoires {{Importance}} et S\'election de Variables},
  author = {Genuer, Robin and Poggi, Jean-Michel},
  year = {2017},
  urldate = {2020-03-20},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JMU28BT5/full-text.pdf}
}

@article{Ghezzi2010,
  title = {Stellar {{Parameters}} and {{Metallicities}} of {{Stars Hosting Jovian}} and {{Neptunian Mass Planets}}: {{A Possible Dependence}} of {{Planetary Mass}} on {{Metallicity}}},
  author = {Ghezzi, L. and Cunha, K. and Smith, V. V. and {de Ara{\'u}jo}, F. X. and Schuler, S. C. and {de la Reza}, R.},
  year = {2010},
  month = jul,
  journal = {ApJ},
  volume = {720},
  number = {2},
  eprint = {1007.2681},
  pages = {1290--1302},
  doi = {10.1088/0004-637X/720/2/1290},
  urldate = {2020-03-16},
  abstract = {The metal content of planet hosting stars is an important ingredient which may affect the formation and evolution of planetary systems. Accurate stellar abundances require the determinations of reliable physical parameters, namely the effective temperature, surface gravity, microturbulent velocity, and metallicity. This work presents the homogeneous derivation of such parameters for a large sample of stars hosting planets (N=117), as well as a control sample of disk stars not known to harbor giant, closely orbiting planets (N=145). Stellar parameters and iron abundances are derived from an automated analysis technique developed for this work. As previously found in the literature, the results in this study indicate that the metallicity distribution of planet hosting stars is more metal-rich by \textasciitilde 0.15 dex when compared to the control sample stars. A segregation of the sample according to planet mass indicates that the metallicity distribution of stars hosting only Neptunian-mass planets (with no Jovian-mass planets) tends to be more metal-poor in comparison with that obtained for stars hosting a closely orbiting Jovian planet. The significance of this difference in metallicity arises from a homogeneous analysis of samples of FGK dwarfs which do not include the cooler and more problematic M dwarfs. This result would indicate that there is a possible link between planet mass and metallicity such that metallicity plays a role in setting the mass of the most massive planet. Further confirmation, however, must await larger samples.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,planetary systems,planets and satellites: formation,Solar and Stellar Astrophysics,stars: abundances,stars: atmospheres,stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/VM436WHJ/full-text.pdf}
}

@article{Ghirlanda2010,
  title = {Astrophysics {{L}} Etter to the {{E}} Ditor {{The}} Onset of the {{GeV}} Afterglow of {{GRB}} 090510},
  author = {Ghirlanda, G and Ghisellini, G and Nava, L},
  year = {2010},
  volume = {7},
  pages = {1--4},
  keywords = {gamma-ray burst,general,non-thermal,notion,notion-database,radiation mechanisms,rays,x},
  file = {/Users/lbugnet/Zotero/storage/69YL52YT/Ghirlanda, Ghisellini, Nava - 2010.pdf}
}

@article{Giammichele2017,
  title = {The Potential of Asteroseismology for Probing the Core Chemical Stratification in White Dwarf Stars},
  author = {Giammichele, N. and Charpinet, S. and Brassard, P. and Fontaine, G.},
  year = {2017},
  month = feb,
  journal = {Astronomy and Astrophysics},
  volume = {598},
  pages = {A109},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201629935},
  urldate = {2023-09-19},
  abstract = {Context. The details of the C/O core structure in white dwarf stars has mostly remained inaccessible to the technique of asteroseismology, despite several attempts carried out in the past. Aims: We aim to re-assess the potential of asteroseismology for probing the chemical stratification in white dwarf cores, in light of new highly efficient tools recently developed for that purpose. Methods: Using the forward modeling approach and a new parameterization for the core chemical stratification in ZZ Ceti stars, we tested several situations typical of the usually limited constraints available, such as small numbers of observed independent modes, to carry out asteroseismology of these stars. Results: We find that, even with a limited number of modes, the core chemical stratification (in particular, the location of the steep chemical transitions expected in the oxygen profile) can be determined quite precisely due to the significant sensitivity of some confined modes to partial reflexion (trapping) effects. These effects are similar to the well known trapping induced by the shallower chemical transitions at the edge of the core and at the bottom of the H-rich envelope. We also find that success to unravel the core structure depends on the information content of the available seismic data. In some cases, it may not be possible to isolate a unique, well-defined seismic solution and the problem remains degenerate. Conclusions: Our results establish that constraining the core chemical stratification in white dwarf stars based solely on asteroseismology is possible, an opportunity that we have begun to exploit.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: interiors,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2017A\&A...598A.109G},
  file = {/Users/lbugnet/Zotero/storage/UZQ8YABA/Giammichele et al. - 2017 - The potential of asteroseismology for probing the .pdf}
}

@misc{Giammichele2021,
  title = {Asteroseismic Cartography of Hydrogen-Deficient White Dwarfs},
  author = {Giammichele, N. and Charpinet, S. and Fontaine, G. and Brassard, P. and Bergeron, P. and Reindl, N. and Baran, A. S.},
  year = {2021},
  month = jun,
  number = {arXiv:2106.15701},
  eprint = {2106.15701},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-09-19},
  abstract = {We present the results of the asteroseismic analysis of the hydrogen-deficient white dwarf PG 0112+104 from the \$Kepler\$-2 field. Our seismic procedure using the forward method based on physically sound, static models, includes the new core parameterization leading us to reproduce the periods of this star near the precision of the observations. This new fit outperforms current state-of-the-art standards by order of magnitudes. We precisely establish the internal structure and unravel the inner C/O stratification of its core. This opens up interesting perspectives on better constraining key processes in stellar physics such as nuclear burning, convection, and mixing, that shape this stratification over time.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/IC9F5B3W/Giammichele et al. - 2021 - Asteroseismic cartography of hydrogen-deficient wh.pdf;/Users/lbugnet/Zotero/storage/XG2C3NLX/2106.html}
}

@article{Giampapa2006,
  title = {A {{Survey}} of {{Chromospheric Activity}} in the {{Solar}}-{{Type Stars}} in the {{Open Cluster M67}}},
  author = {Giampapa, Mark S. and Hall, Jeffrey C. and Radick, Richard R. and Baliunas, Sallie L.},
  year = {2006},
  journal = {The Astrophysical Journal},
  volume = {651},
  number = {1},
  eprint = {astro-ph/0607313},
  pages = {444--461},
  issn = {0004-637X},
  doi = {10.1086/507624},
  abstract = {We present the results of a spectroscopic survey of the Ca II H \& K core strengths in a sample of 60 solar-type stars that are members of the solar-age and solar-metallicity open cluster M67. We adopt the HK index, defined as the summed H+K core strengths in 0.1 nm bandpasses centered on the H and K lines, respectively, as a measure of the chromospheric activity that is present. We compare the distribution of mean HK index values for the M67 solar-type stars with the variation of this index as measured for the Sun during the contemporary solar cycle. We find that the stellar distribution in our HK index is broader than that for the solar cycle. Approximately 17\% of the M67 sun-like stars exhibit average HK indices that are less than solar minimum. About 7\%-12\% are characterized by relatively high activity in excess of solar maximum values while 72\%-80\% of the solar analogs exhibit Ca II H+K strengths within the range of the modern solar cycle. The ranges given reflect uncertainties in the most representative value of the maximum in the HK index to adopt for the solar cycle variations observed during the period A.D. 1976--2004. Thus, \textasciitilde{} 20\% - 30\% of our homogeneous sample of sun-like stars have mean chromospheric H+K strengths that are outside the range of the contemporary solar cycle. Any cycle-like variability that is present in the M67 solar-type stars appears to be characterized by periods greater than \textasciitilde{} 6 years. Finally, we estimate a mean chromospheric age for M67 in the range of 3.8--4.3 Gyr.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YGPC9M9S/Giampapa et al. - 2006.pdf}
}

@article{Gianninas2016,
  title = {Discovery of {{Three Pulsating}}, {{Mixed-atmosphere}}, {{Extremely Low-mass White Dwarf Precursors}}},
  author = {Gianninas, A. and Curd, Brandon and Fontaine, G. and Brown, Warren R. and Kilic, Mukremin},
  year = {2016},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {822},
  pages = {L27},
  issn = {0004-637X},
  doi = {10.3847/2041-8205/822/2/L27},
  urldate = {2023-10-09},
  abstract = {We report the discovery of pulsations in three mixed-atmosphere, extremely low-mass white dwarf (ELM WD, M {$\leq$}slant 0.3 M {$\odot$}) precursors. Following the recent discoveries of pulsations in both ELM and pre-ELM WDs, we targeted pre-ELM WDs with mixed H/He atmospheres with high-speed photometry. We find significant optical variability in all three observed targets with periods in the range 320-590 s, consistent in timescale with theoretical predictions of p-mode pulsations in mixed-atmosphere {$\approx$}0.18 M {$\odot$} He-core pre-ELM WDs. This represents the first empirical evidence that pulsations in pre-ELM WDs can only occur if a significant amount of He is present in the atmosphere. Future, more extensive, timeseries photometry of the brightest of the three new pulsators offers an excellent opportunity to constrain the thickness of the surface H layer, which regulates the cooling timescales for ELM WDs. Based on observations obtained at the Gemini Observatory, which is operated by the Association of Universities for Research in Astronomy, Inc., under a cooperative agreement with the NSF on behalf of the Gemini partnership: the National Science Foundation (United States), the National Research Council (Canada), CONICYT (Chile), Ministerio de Ciencia, Tecnolog\'ia e Innovaci\'on Productiva (Argentina), and Minist\'erio da Ci\^encia, Tecnologia e Inova\c{c}\~ao (Brazil).},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,SDSS J114155.56+385003.0,SDSS J115734.46+054645.6,stars: individual: SDSS J075610.71+670424.7,techniques: photometric,white dwarfs},
  annotation = {ADS Bibcode: 2016ApJ...822L..27G},
  file = {/Users/lbugnet/Zotero/storage/F4SYCF2B/Gianninas et al. - 2016 - Discovery of Three Pulsating, Mixed-atmosphere, Ex.pdf}
}

@article{Giardini2020,
  title = {The {{Seismicity}} of {{Mars}}},
  author = {Giardini, D. and Lognonn{\'e}, P. and Banerdt, W. and Pike, W. and Christensen, U. and Ceylan, S. and Clinton, J. and van Driel, M. and St{\"a}hler, S. and B{\"o}se, M. and Garcia, R. and Khan, A. and Panning, M. and Perrin, Cl{\'e}ment and Banfield, D. and Beucler, E. and Charalambous, C. and Euchner, F. and Horleston, A. and Jacob, A. and Kawamura, T. and Kedar, S. and Mainsant, G. and Scholz, J.-R. and Smrekar, S. and Spiga, A. and Agard, C. and Antonangeli, D. and Barkaoui, S. and Barrett, E. and Combes, P. and Conejero, V. and Daubar, I. and Drilleau, M. and Ferrier, C. and Gabsi, T. and Gudkova, T. and Hurst, K. and Karakostas, F. and King, S. and Knapmeyer, M. and {Knapmeyer-Endrun}, B. and {Ljorca-Cejudo}, R. and Lucas, A. and Luno, L. and Margerin, L. and McClean, J. and Mimoun, D. and Murdoch, N. and Nimmo, F. and Nonon, M. and Pardo, C. and Rivoldini, A. and Manfredi, J. A. Rodriguez and Samuel, H. and Schimmel, M. and Stott, A. E. and Stutzman, E. and Teanby, N. and Warren, T. and Weber, R. and Wieczorek, M. and Yana., C.},
  year = {2020},
  month = feb,
  journal = {Nature Geoscience},
  volume = {in press},
  number = {3},
  pages = {205--212},
  publisher = {{Nature Publishing Group}},
  doi = {10.1038/s41561-020-0539-8},
  urldate = {2020-03-07},
  abstract = {The InSight (Interior Exploration using Seismic Investigations, Geodesy and Heat Transport) mission landed in Elysium Planitia on Mars on 26 November 2018 and fully deployed its seismometer by the end of February 2019. The mission aims to detect, characterize and locate seismic activity on Mars, and to further constrain the internal structure, composition and dynamics of the planet. Here, we present seismometer data recorded until 30 September 2019, which reveal that Mars is seismically active. We identify 174 marsquakes, comprising two distinct populations: 150 small-magnitude, high-frequency events with waves propagating at crustal depths and 24 low-frequency, subcrustal events of magnitude Mw 3\textendash 4 with waves propagating at various depths in the mantle. These marsquakes have spectral characteristics similar to the seismicity observed on the Earth and Moon. We determine that two of the largest detected marsquakes were located near the Cerberus Fossae fracture system. From the recorded seismicity, we constrain attenuation in the crust and mantle, and find indications of a potential low-S-wave-velocity layer in the upper mantle. Mars is seismically active: 24 subcrustal magnitude 3\textendash 4 marsquakes and 150 smaller events have been identified up to 30 September 2019, by an analysis of seismometer data from the InSight lander.},
  keywords = {Inner planets,notion,notion-database,Seismology}
}

@article{Gilliland2008,
  title = {Photometric Oscillations of Low-Luminosity Red Giant Stars},
  author = {Gilliland, Ronald L.},
  year = {2008},
  journal = {Astronomical Journal},
  volume = {136},
  number = {2},
  eprint = {0806.1497},
  pages = {566--579},
  issn = {00046256},
  doi = {10.1088/0004-6256/136/2/566},
  abstract = {I present details of the variations of several hundred red giant stars on timescales of a few hours to a few days from Hubble Space Telescope (HST) observations of a low-extinction galactic bulge sample from an intensive seven-day campaign. Variations in the red giants are shown to be a strong function of position within the color-magnitude diagram (CMD) in accord with general expectations from theory. Amplitudes are greater for stars with larger radii, whether this results from higher luminosity at the same effective temperature or lower temperature at a fixed apparent magnitude. Likewise, characteristic timescales for the variations increase to the upper right in a CMD as does the ratio of amplitudes measured at 606 nm compared to 814 nm. Characteristic variation timescales are well matched by low-order radial pulsation modes. The effective sample discussed here extends from about two magnitudes above the bulge turnoff at which red giant radii are 7 R/R at 5000 K with typical amplitudes of 0.5 mmag to 40 R/R at 4000 K with amplitudes of 3.5 mmag. Variability characteristics are quite similar at any given position in the CMD, and at levels in the CMD where oscillations are easily detected nearly all red giants show such. If these variations represent oscillations with sufficient lifetimes to derive accurate mode frequencies, more extensive observations, e.g., as should soon be provided by the Kepler Mission, would provide a rich asteroseismic return. \textcopyright{} 2008. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: late-type,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/A84T4MHC/Gilliland - 2008.pdf}
}

@article{Gilliland2010,
  title = {Kepler {{Asteroseismology Program}}: {{Introduction}} and {{First Results}}},
  author = {Gilliland, Ronald L. and Brown, Timothy M. and {Christensen-Dalsgaard}, J{\o}rgen and Kjeldsen, Hans and Aerts, Conny and Appourchaux, Thierry and Basu, Sarbani and Bedding, Timothy R. and Chaplin, William J. and Cunha, Margarida S. and De Cat, Peter and De Ridder, Joris and Guzik, Joyce A. and Handler, Gerald and Kawaler, Steven and Kiss, L{\'a}szl{\'o} and Kolenberg, Katrien and Kurtz, Donald W. and Metcalfe, Travis S. and Monteiro, Mario J. P. F. G. and Szab{\'o}, Robert and Arentoft, Torben and Balona, Luis and Debosscher, Jonas and Elsworth, Yvonne P. and Quirion, Pierre-Olivier and Stello, Dennis and Su{\'a}rez, Juan Carlos and Borucki, William J. and Jenkins, Jon M. and Koch, David and Kondo, Yoji and Latham, David W. and Rowe, Jason F. and Steffen, Jason H.},
  year = {2010},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {122},
  number = {888},
  pages = {131--143},
  issn = {0004-6280},
  doi = {10.1086/650399},
  abstract = {Asteroseismology involves probing the interiors of stars and quantifying their global properties, such as radius and age, through observations of normal modes of oscillation. The technical requirements for conducting asteroseismology include ultrahigh precision measured in photometry in parts per million, as well as nearly continuous time series over weeks to years, and cadences rapid enough to sample oscillations with periods as short as a few minutes. We report on results from the first 43 days of observations, in which the unique capabilities of Kepler in providing a revolutionary advance in asteroseismology are already well in evidence. The Kepler asteroseismology program holds intrinsic importance in supporting the core planetary search program through greatly enhanced knowledge of host star properties, and extends well beyond this to rich applications in stellar astrophysics.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BCTL7C87/Gilliland et al. - 2010(2).pdf}
}

@article{Gilliland2010b,
  title = {Initial Characteristics of Kepler Short Cadence Data},
  author = {Gilliland, Ronald L. and Jenkins, Jon M. and Borucki, William J. and Bryson, Stephen T. and Caldwell, Douglas A. and Clarke, Bruce D. and Dotson, Jessie L. and Haas, Michael R. and Hall, Jennifer and Klaus, Todd and Koch, David and McCauliff, Sean and Quintana, Elisa V. and Twicken, Joseph D. and Van Cleve, Jeffrey E.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0142},
  pages = {160--163},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L160},
  abstract = {The Kepler Mission offers two options for observations - either long cadence (LC) used for the bulk of core mission science, or short cadence (SC) which is used for applications such as asteroseismology of solar-like stars and transit timing measurements of exoplanets where the 1minute sampling is critical. We discuss the characteristics of SC data obtained in the 33.5 day long Quarter 1 observations with Kepler which completed on 2009 June 15. The truly excellent time series precisions are nearly Poisson limited at 11th magnitude providing per-point measurement errors of 200 parts-per-million per minute. For extremely saturated stars near seventh magnitude precisions of 40ppm are reached, while for background limited measurements at 17th magnitude precisions of 7 mmag are maintained. We note the presence of two additive artifacts, one that generates regularly spaced peaks in frequency, and one that involves additive offsets in the time domain inversely proportional to stellar brightness. The difference between LC and SC sampling is illustrated for transit observations of TrES-2. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/G64DXJFY/Gilliland et al. - 2010.pdf}
}

@article{Gilliland2011a,
  title = {Kepler Mission Stellar and Instrument Noise Properties},
  author = {Gilliland, Ronald L. and Chaplin, William J. and Dunham, Edward W. and Argabright, Vic S. and Borucki, William J. and Basri, Gibor and Bryson, Stephen T. and Buzasi, Derek L. and Caldwell, Douglas A. and Elsworth, Yvonne P. and Jenkins, Jon M. and Koch, David G. and Kolodziejczak, Jeffrey and Miglio, Andrea and Van Cleve, Jeffrey and Walkowicz, Lucianne M. and Welsh, William F.},
  year = {2011},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {197},
  number = {1},
  eprint = {1107.5207},
  issn = {00670049},
  doi = {10.1088/0067-0049/197/1/6},
  abstract = {Kepler mission results are rapidly contributing to fundamentally new discoveries in both the exoplanet and asteroseismology fields. The data returned from Kepler are unique in terms of the number of stars observed, precision of photometry for time series observations, and the temporal extent of high duty cycle observations. As the first mission to provide extensive time series measurements on thousands of stars over months to years at a level hitherto possible only for the Sun, the results from Kepler will vastly increase our knowledge of stellar variability for quiet solar-type stars. Here, we report on the stellar noise inferred on the timescale of a few hours of most interest for detection of exoplanets via transits. By design the data from moderately bright Kepler stars are expected to have roughly comparable levels of noise intrinsic to the stars and arising from a combination of fundamental limitations such as Poisson statistics and any instrument noise. The noise levels attained by Kepler on-orbit exceed by some 50\% the target levels for solar-type, quiet stars. We provide a decomposition of observed noise for an ensemble of 12th magnitude stars arising from fundamental terms (Poisson and readout noise), added noise due to the instrument and that intrinsic to the stars. The largest factor in the modestly higher than anticipated noise follows from intrinsic stellar noise. We show that using stellar parameters from galactic stellar synthesis models, and projections to stellar rotation, activity, and hence noise levels reproduce the primary intrinsic stellar noise features. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {methods: observational,notion,notion-database,stars: activity,stars: late-type,stars: oscillations,stars: statistics,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/SJI8QCUG/Gilliland et al. - 2011.pdf}
}

@article{Gillon2010a,
  title = {Transiting Exoplanets from the {{CoRoT}} Space Mission},
  author = {Gillon, M. and Hatzes, A. and Csizmadia, {\relax Sz}. and Fridlund, M. and Deleuil, M. and Aigrain, S. and Alonso, R. and Auvergne, M. and Baglin, A. and Barge, P. and Barnes, S. I. and Bonomo, A. S. and Bord{\'e}, P. and Bouchy, F. and Bruntt, H. and Cabrera, J. and Carone, L. and Carpano, S. and Cochran, W. D. and Deeg, H. J. and Dvorak, R. and Endl, M. and Erikson, A. and {Ferraz-Mello}, S. and Gandolfi, D. and Gazzano, J. C. and Guenther, E. and Guillot, T. and Havel, M. and H{\'e}brard, G. and Jorda, L. and L{\'e}ger, A. and Llebaria, A. and Lammer, H. and Lovis, C. and Mayor, M. and Mazeh, T. and Montalb{\'a}n, J. and Moutou, C. and Ofir, A. and Ollivier, M. and P{\"a}tzold, M. and Pepe, F. and Queloz, D. and Rauer, H. and Rouan, D. and Samuel, B. and Santerne, A. and Schneider, J. and Tingley, B. and Udry, S. and Weingrill, J. and Wuchterl, G.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {520},
  pages = {A97},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201014981},
  abstract = {\emph{Aims. {$<$}i/{$>$}We report the discovery of very shallow (\$\textbackslash Delta F/F \textbackslash approx 3.4\textbackslash times 10\^\{-4\}\$), periodic dips in the light curve of an active \$V = 11.7\$~G9V star observed by the CoRoT\, satellite, which we interpret as caused by a transiting companion. We describe the 3-colour CoRoT data and complementary ground-based observations that support the planetary nature of the companion.\emph{Methods. {$<$}i/{$>$}We used CoRoT\, colours information, good angular resolution ground-based photometric observations in- and out- of transit, adaptive optics imaging, near-infrared spectroscopy, and preliminary results from radial velocity measurements, to test the diluted eclipsing binary scenarios. The parameters of the host star were derived from optical spectra, which were then combined with the CoRoT\, light curve to derive parameters of the companion.\emph{Results. {$<$}i/{$>$}We examined all conceivable cases of false positives carefully, and all the tests support the planetary hypothesis. Blends with separation {$>$}0.40\textasciiacute\textasciiacute or triple systems are almost excluded with a \$8 \textbackslash times 10\^\{-4\}\$~risk left. We conclude that, inasmuch we have been exhaustive, we have discovered a planetary companion, named CoRoT-7b, for which we derive a period of 0.853 \$59 \textbackslash pm 3 \textbackslash times 10\^\{-5\}\$ day and a radius of \$R\_\{\textbackslash rm p\} = 1.68 \textbackslash pm 0.09\$~\emph{R{$<$}i/{$>$}\textsubscript{Earth{$<$}sub/{$>$}. Analysis of preliminary radial velocity data yields an upper limit of 21~\emph{M{$<$}i/{$>$}\textsubscript{Earth{$<$}sub/{$>$}\, for the companion mass, supporting the finding.\emph{Conclusions. {$<$}i/{$>$}CoRoT-7b\, is very likely the first Super-Earth with a measured radius. This object illustrates what will probably become a common situation with missions such as Kepler, namely the need to establish the planetary origin of transits in the absence of a firm radial velocity detection and mass measurement. The composition of CoRoT-7b\, remains loosely constrained without a precise mass. A very high surface temperature on its irradiated face, \emph{{$\approx<$}i/{$>$}1800\textendash 2600~K at the substellar point, and a very low one, \emph{{$\approx<$}i/{$>$}50~K, on its dark face assuming no atmosphere, have been derived.}}}}}}}}}}},
  keywords = {2006,austria,by cnes,developed and is operated,has been,high angular resolution,launched on 27 december,notion,notion-database,photometric,planetary systems,radial velocities,spectroscopic,techniques,{techniques: photometric, techniques: spectroscopic},the corot space mission,with the contribution of},
  file = {/Users/lbugnet/Zotero/storage/4HYIX7QK/Gillon et al. - 2010.pdf}
}

@article{Gillon2017,
  title = {Seven Temperate Terrestrial Planets around the Nearby Ultracool Dwarf Star {{TRAPPIST-1}}},
  author = {Gillon, Micha{\"e}l and Triaud, Amaury H.M.J. and Demory, Brice Olivier and Jehin, Emmanu{\"e}l and Agol, Eric and Deck, Katherine M. and Lederer, Susan M. and De Wit, Julien and Burdanov, Artem and Ingalls, James G. and Bolmont, Emeline and Leconte, Jeremy and Raymond, Sean N. and Selsis, Franck and Turbet, Martin and Barkaoui, Khalid and Burgasser, Adam and Burleigh, Matthew R. and Carey, Sean J. and Chaushev, Aleksander and Copperwheat, Chris M. and Delrez, Laetitia and Fernandes, Catarina S. and Holdsworth, Daniel L. and Kotze, Enrico J. and Van Grootel, Val{\'e}rie and Almleaky, Yaseen and Benkhaldoun, Zouhair and Magain, Pierre and Queloz, Didier},
  year = {2017},
  journal = {Nature},
  volume = {542},
  number = {7642},
  pages = {456--460},
  publisher = {{Nature Publishing Group}},
  issn = {14764687},
  doi = {10.1038/nature21360},
  abstract = {One aim of modern astronomy is to detect temperate, Earth-like exoplanets that are well suited for atmospheric characterization. Recently, three Earth-sized planets were detected that transit (that is, pass in front of) a star with a mass just eight per cent that of the Sun, located 12 parsecs away. The transiting configuration of these planets, combined with the Jupiter-like size of their host star - named TRAPPIST-1 - makes possible in-depth studies of their atmospheric properties with present-day and future astronomical facilities. Here we report the results of a photometric monitoring campaign of that star from the ground and space. Our observations reveal that at least seven planets with sizes and masses similar to those of Earth revolve around TRAPPIST-1. The six inner planets form a near-resonant chain, such that their orbital periods (1.51, 2.42, 4.04, 6.06, 9.1 and 12.35 days) are near-ratios of small integers. This architecture suggests that the planets formed farther from the star and migrated inwards. Moreover, the seven planets have equilibrium temperatures low enough to make possible the presence of liquid water on their surfaces.},
  keywords = {Astrophysics,Earth and Planetary Astrophysics,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G78EKUL3/full-text.pdf;/Users/lbugnet/Zotero/storage/HJQB6LY9/Gillon et al. - 2017.pdf}
}

@article{Gilman1989,
  title = {Angular Momentum Transport and Dynamo Action in the Sun - {{Implications}} of Recent Oscillation Measurements},
  author = {Gilman, Peter A. and Morrow, Cherilynn A. and Deluca, Edward E.},
  year = {1989},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {338},
  pages = {528},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/167215},
  urldate = {2020-07-02},
  abstract = {The implications of a newly proposed picture of the sun's internal  rotation (Brown et al., 1989; Morrow, 1988) for the distribution and  transport of angular momentum and for the solar dynamo are considered.  The new results, derived from an analysis of solar acoustic  oscillations, affect understanding of how momentum is cycled in the sun  and provide clues as to how and where the solar dynamo is driven. The  data imply that the only significant radial gradient of angular velocity  exists in a transitional region between the bottom of the convection  zone, which is rotating like the solar surface, and the top of the deep  interior, which is rotating rigidly at a rate intermediate between the  equatorial and polar rates at the surface. Thus the radial gradient must  change sign at the latitude where the angular velocity of the surface  matches that of the interior. These inferences suggest that the cycle of  angular momentum that produces the observed latitudinal differential  rotation in the convection zone may be coupled to layers of the interior  beneath the convection zone.},
  keywords = {Angular Momentum,Dynamo Theory,HYDROMAGNETICS,hydromagnetics-Sun,interior-Sun,Magnetohydrodynamics,Momentum Transfer,notion,notion-database,oscillations-Sun,rotation,Solar Interior,Solar Oscillations,Solar Physics,Solar Rotation,Solar Velocity,Subject headings,SUN: INTERIOR,SUN: OSCILLATIONS,SUN: ROTATION},
  file = {/Users/lbugnet/Zotero/storage/IWA4VL73/full-text.pdf}
}

@article{Gilman1997,
  title = {Joint {{Instability}} of {{Latitudinal Differential Rotation}} and {{Toroidal Magnetic Fields}} below the {{Solar Convection Zone}}},
  author = {Gilman, Peter A. and Fox, Peter A.},
  year = {1997},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {484},
  number = {1},
  pages = {439--454},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/304330},
  urldate = {2020-05-14},
  abstract = {Below the convection zone, where the stratification is radiatively controlled, large-scale motions should be mainly horizontal, i.e., in spherical shells due to the stabilizing effect of negative buoyancy on radial displacements. Watson showed that the observed surface solar differential rotation is at the threshold for instability to horizontal disturbances. Therefore, since helioseismology tells us the latitudinal differential rotation below the convection zone is less than the surface value, the profile should be stable too. We show that in the presence of a broad, nonuniform toroidal field the solar differential rotation is unstable. This is true for a wide range of kinetic and magnetic energies of the unperturbed state, from well below equipartition to well above it. We find instability for essentially all values of differential rotation and toroidal fields for which we are able to find converged solutions. The instability appears to occur only for longitudinal wave number 1. Disturbance symmetries about the equator and profiles in latitude depend on the amplitude of the toroidal field. Peak e-folding times are a few months. The primary energy source for the instability is differential rotation for low field strengths and the toroidal field for high field strengths. The mechanism of energy release from the differential rotation is the poleward transport of angular momentum, by the Maxwell stress rather than the Reynolds stress. For the profiles studied, the Reynolds stress is almost always trying to rebuild differential rotation, the exact opposite of the nonmagnetic case. Second-order perturbation theory predicts that the unstable modes produce zonal jets and fine structure in the toroidal field, the latitude of which migrates toward the equator with increasing magnetic field strength. The instability we have found may play a role in the solar dynamo, although being two-dimensional, it cannot produce a dynamo by itself. Mixing of angular momentum caused by the instability could allow achievement of equilibrium of the solar tachocline hypothesized by Spiegel \& Zahn.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NWPP2ZBT/full-text.pdf}
}

@article{Girardi2000,
  title = {Evolutionary Tracks and Isochrones for Low- and Intermediate-Mass Stars: {{From}} 0.15 to 7 {{M}}{$\odot$}, and from {{Z}} = 0.0004 to 0.03},
  author = {Girardi, L. and Bressan, A. and Bertelli, G. and Chiosi, C.},
  year = {2000},
  month = feb,
  journal = {Astronomy and Astrophysics Supplement Series},
  volume = {141},
  number = {3},
  eprint = {astro-ph/9910164},
  pages = {371--383},
  publisher = {{EDP Sciences}},
  issn = {03650138},
  doi = {10.1051/aas:2000126},
  urldate = {2020-07-07},
  abstract = {We present a large grid of stellar evolutionary tracks, which are suitable to modelling star clusters and galaxies by means of population synthesis. The tracks are presented for the initial chemical compositions [Z = 0.0004, Y = 0.23], [Z = 0.001, Y = 0.23], [Z = 0.004, Y = 0.24], [Z = 0.008, Y = 0.25], [Z = 0.019, Y = 0.273] (solar composition), and [Z = 0.03, Y = 0.30]. They are computed with updated opacities and equation of state, and a moderate amount of convective overshoot. The range of initial masses goes from 0.15 M{$\odot$} to 7 M{$\odot$}, and the evolutionary phases extend from the zero age main sequence (ZAMS) till either the thermally pulsing AGB regime or carbon ignition. We also present an additional set of models with solar composition, computed using the classical Schwarzschild criterion for convective boundaries. From all these tracks, we derive the theoretical isochrones in the Johnson-Cousins UBVRIJHK broad-band photometric system.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: Hertzsprung-Russell (HR) diagram,Stars: interiors,Stars: low-mass},
  file = {/Users/lbugnet/Zotero/storage/26YBHT63/full-text.pdf}
}

@article{Girardi2005,
  title = {Star Counts in the Galaxy Simulating from Very Deep to Very Shallow Photometric Surveys with the {{TRILEGAL}} Code},
  author = {Girardi, L. and Groenewegen, M. A.T. and Hatziminaoglou, E. and Da Costa, L.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {436},
  number = {3},
  eprint = {astro-ph/0504047},
  pages = {895--915},
  issn = {00046361},
  doi = {10.1051/0004-6361:20042352},
  abstract = {We describe TRILEGAL, a new populations synthesis code for simulating the stellar photometry of any Galaxy field. The code attempts to improve upon several technical aspects of star count models, by: dealing with very complete input libraries of evolutionary tracks; using a stellar spectral library to simulate the photometry in virtually any broad-band system; being very versatile allowing easy changes in the input libraries and in the description of all of its ingredients - like the star formation rate, age-metallicity relation, initial mass function, and geometry of Galaxy components. In a previous paper (Groenewegen et al. 2002, Paper I), the code was first applied to describe the very deep star counts of the CDFS stellar catalogue. Here, we briefly describe its initial calibration using EIS-deep and DMS star counts, which, as we show, are adequate samples to probe both the halo and the disc components of largest scale heights (oldest ages). We then present the changes in the calibration that were necessary to cope with some improvements in the model input data, and the use of more extensive photometry datasets: now the code is shown to successfully simulate also the relatively shallower 2MASS catalogue, which probes mostly the disc at intermediate ages, and the immediate solar neighbourhood as sampled by Hipparcos - in particular its absolute magnitude versus colour diagram -, which contains a somewhat larger fraction of younger stars than deeper surveys. Remarkably, the same model calibration can reproduce well the star counts in all the above-mentioned data sets, that span from the very deep magnitudes of CDFS (16 {$<$} R {$<$} 23) to the very shallow ones of Hipparcos (V {$<$} 8). Significant deviations (above 50 percent in number counts) are found just for fields close to the Galactic Center (since no bulge component was included) and Plane, and for a single set of South Galactic Pole data. The TRILEGAL code is ready to use for the variety of wide-angle surveys in the optical/infrared that will become available in the coming years. \textcopyright{} ESO 2005.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: Stellar content,Galaxy: Structure,M diagrams,notion,notion-database,Russell (HR) C,Stars: Hertzsprung,{Stars: Luminosity function, mass function},Surveys},
  file = {/Users/lbugnet/Zotero/storage/UGDE3S5P/Girardi et al. - 2005.pdf}
}

@article{Girardi2016,
  title = {Red {{Clump Stars}}},
  author = {Girardi, L{\'e}o},
  year = {2016},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {54},
  number = {1},
  pages = {95--133},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-081915-023354},
  abstract = {\textcopyright{} 2016 by Annual Reviews. Low-mass stars in their core-helium-burning stage define the sharpest feature present in the color-magnitude diagrams of nearby galaxy systems: the red clump (RC). This feature has given rise to a series of methods aimed at measuring the distributions of stellar distances and extinctions, especially in the Magellanic Clouds and Milky Way Bulge. Because the RC is easily recognizable within the data of large spectroscopic and asteroseismic surveys, it is a useful probe of stellar densities, kinematics, and chemical abundances across the Milky Way disk; it can be applied up to larger distances than that allowed by dwarfs; and it has better accuracy than is possible with other kinds of giants. Here, we discuss the reasons for the RC narrowness in several sets of observational data, its fine structure, and the presence of systematic changes in the RC properties as regards age, metallicity, and the observed passband. These factors set the limits on the validity and accuracy of several RC methods defined in the literature.},
  keywords = {diagrams,evolution,galaxy,hertzsprung-russell and color-magnitude,low mass,notion,notion-database,stars,stellar content,surveys},
  file = {/Users/lbugnet/Zotero/storage/B24ANRPI/Girardi - 2016.pdf}
}

@article{Girardi2016a,
  title = {Red {{Clump Stars}}},
  author = {Girardi, L{\'e}o},
  year = {2016},
  month = sep,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {54},
  pages = {95--133},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-081915-023354},
  urldate = {2023-09-20},
  abstract = {Low-mass stars in their core-helium-burning stage define the sharpest feature present in the color-magnitude diagrams of nearby galaxy systems: the red clump (RC). This feature has given rise to a series of methods aimed at measuring the distributions of stellar distances and extinctions, especially in the Magellanic Clouds and Milky Way Bulge. Because the RC is easily recognizable within the data of large spectroscopic and asteroseismic surveys, it is a useful probe of stellar densities, kinematics, and chemical abundances across the Milky Way disk; it can be applied up to larger distances than that allowed by dwarfs; and it has better accuracy than is possible with other kinds of giants. Here, we discuss the reasons for the RC narrowness in several sets of observational data, its fine structure, and the presence of systematic changes in the RC properties as regards age, metallicity, and the observed passband. These factors set the limits on the validity and accuracy of several RC methods defined in the literature.},
  annotation = {ADS Bibcode: 2016ARA\&A..54...95G},
  file = {/Users/lbugnet/Zotero/storage/552YG5XU/Girardi - 2016 - Red Clump Stars.pdf}
}

@article{Gizon2003,
  title = {Determining the {{Inclination}} of the {{Rotation Axis}} of a {{Sun}}-like {{Star}}},
  author = {Gizon, L. and Solanki, S. K.},
  year = {2003},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {589},
  number = {2},
  pages = {1009--1019},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/374715},
  urldate = {2020-06-27},
  abstract = {Asteroseismology provides us with the possibility of determining the angle, i, between the direction of the rotation axis of a pulsating Sun-like star and the line of sight. A knowledge of i is important not just for obtaining improved stellar parameters, but also in order to determine the true masses of extrasolar planets detected from the radial velocity shifts of their central stars. By means of Monte Carlo simulations, we estimate the precision of the measurement of i and other stellar parameters. We find that the inclination angle can be retrieved accurately when i\&gt;\textasciitilde 30deg for stars that rotate at least twice as fast as the Sun.},
  keywords = {notion,notion-database,Stars: Fundamental Parameters,Stars: Oscillations,Stars: Planetary Systems,Stars: Rotation},
  file = {/Users/lbugnet/Zotero/storage/QNPGD5K6/full-text.pdf}
}

@article{Gizon2005,
  title = {Local {{Helioseismology}}},
  author = {Gizon, Laurent and Birch, Aaron C.},
  year = {2005},
  journal = {Living Reviews in Solar Physics},
  volume = {2},
  number = {1},
  pages = {6},
  issn = {1614-4961},
  doi = {10.12942/lrsp-2005-6},
  urldate = {2020-03-07},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8YHK52P6/full-text.pdf}
}

@article{Gizon2010,
  title = {Local {{Helioseismology}}: {{Three Dimensional Imaging}} of the {{Solar Interior}}},
  author = {Gizon, L. and Birch, A. C. and Spruit, H. C.},
  year = {2010},
  month = jan,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {48},
  number = {1},
  eprint = {1001.0930},
  pages = {289--338},
  publisher = {{Annual Reviews}},
  doi = {10.1146/annurev-astro-082708-101722},
  urldate = {2020-03-07},
  abstract = {The Sun supports a rich spectrum of internal waves that are continuously excited by turbulent convection. The GONG network and the MDI/SOHO space instrument provide an exceptional data base of spatially-resolved observations of solar oscillations, covering an entire sunspot cycle (11 years). Local helioseismology is a set of tools for probing the solar interior in three dimensions using measurements of wave travel times and local mode frequencies. Local helioseismology has discovered (i) near-surface vector flows associated with convection (ii) 250 m/s subsurface horizontal outflows around sunspots (iii) \textasciitilde 50 m/s extended horizontal flows around active regions (converging near the surface and diverging below), (iv) the effect of the Coriolis force on convective flows and active region flows (v) the subsurface signature of the 15 m/s poleward meridional flow, (vi) a +/-5 m/s time-varying depth-dependent component of the meridional circulation around the mean latitude of activity, and (vii) magnetic activity on the far side of the Sun.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,solar convection,solar cycle,solar magnetism,solar oscillations,sunspots},
  file = {/Users/lbugnet/Zotero/storage/AMHMRR8R/Gizon, Birch, Spruit - 2010.pdf;/Users/lbugnet/Zotero/storage/IH87784B/full-text.pdf}
}

@article{Gizon2013,
  title = {Seismic Constraints on Rotation of {{Sun-like}} Star and Mass of Exoplanet},
  author = {Gizon, Laurent and Ballot, J{\'e}rome and Michel, Eric and Stahn, Thorsten and Vauclair, G{\'e}rard and Bruntt, Hans and Quirion, Pierre Olivier and Benomar, Othman and Vauclair, Sylvie and Appourchaux, Thierry and Auvergne, Michel and Baglin, Annie and Barban, Caroline and Baudin, Fr{\'e}deric and Bazot, Micha{\"e}l and Campante, Tiago and Catala, Claude and Chaplin, William and Creevey, Orlagh and Deheuvels, S{\'e}bastien and Dolez, No{\"e}l and Elsworth, Yvonne and Garc{\'i}a, Rafael and Gaulme, Patrick and Mathis, St{\'e}phane and Mathur, Savita and Mosser, Beno{\^i}t and R{\'e}gulo, Clara and Roxburgh, Ian and Salabert, David and Samadi, R{\'e}za and Sato, Kumiko and Verner, Graham and Hanasoge, Shravan and Sreenivasan, Katepalli R.},
  year = {2013},
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  volume = {110},
  number = {33},
  pages = {13267--13271},
  issn = {00278424},
  doi = {10.1073/pnas.1303291110},
  abstract = {Rotation is thought to drive cyclic magnetic activity in the Sun and Sun-like stars. Stellar dynamos, however, are poorly understood owing to the scarcity of observations of rotation and magnetic fields in stars. Here, inferences are drawn on the internal rotation of a distant Sun-like star by studying its global modes of oscillation. We report asteroseismic constraints imposed on the rotation rate and the inclination of the spin axis of the Sun-like star HD 52265, a principal target observed by the CoRoT satellite that is known to host a planetary companion. These seismic inferences are remarkably consistent with an independent spectroscopic observation (rotational line broadening) and with the observed rotation period of star spots. Furthermore, asteroseismology constrains the mass of exoplanet HD 52265b. Under the standard assumption that the stellar spin axis and the axis of the planetary orbit coincide, the minimum spectroscopic mass of the planet can be converted into a true mass of 1:85+0:52 -0:42MJupiter, which implies that it is a planet, not a brown dwarf.},
  keywords = {Extrasolar planets,notion,notion-database,Stellar oscillations,Stellar rotation},
  file = {/Users/lbugnet/Zotero/storage/NUM6Y9SR/Gizon et al. - 2013.pdf}
}

@article{Gizon2021,
  title = {Solar Inertial Modes: {{Observations}}, Identification, and Diagnostic Promise},
  author = {Gizon, Laurent and Cameron, Robert H. and Bekki, Yuto and Birch, Aaron C. and Bogart, Richard S. and Sacha Brun, Allan and Damiani, Cilia and Fournier, Damien and Hyest, Laura and Jain, Kiran and Lekshmi, B. and Liang, Zhi Chao and Proxauf, Bastian},
  year = {2021},
  month = aug,
  journal = {A\&A},
  volume = {652},
  eprint = {2107.09499},
  pages = {L6},
  publisher = {{EDP Sciences}},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202141462},
  urldate = {2022-04-05},
  abstract = {The oscillations of a slowly rotating star have long been classified into spheroidal and toroidal modes. The spheroidal modes include the well-known 5-min acoustic modes used in helioseismology. Here we report observations of the Sun's toroidal modes, for which the restoring force is the Coriolis force and whose periods are on the order of the solar rotation period. By comparing the observations with the normal modes of a differentially rotating spherical shell, we are able to identify many of the observed modes. These are the high-latitude inertial modes, the critical-latitude inertial modes, and the equatorial Rossby modes. In the model, the high-latitude and critical-latitude modes have maximum kinetic energy density at the base of the convection zone, and the high-latitude modes are baroclinically unstable due to the latitudinal entropy gradient. As a first application of inertial-mode helioseismology, we constrain the superadiabaticity and the turbulent viscosity in the deep convection zone.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics,Sun: general,Sun: helioseismology,Sun: interior,Sun: oscillations,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/8PBI24RI/full-text.pdf}
}

@article{Goldrei,
  title = {Excitation of Solar P-Modes},
  author = {Goldreich, P. and Murray, N. and Kumar, Pawan},
  year = {1994},
  journal = {The Astrophysical Journal},
  volume = {424},
  pages = {466--479},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NZ3EZMPW/Goldreich, Murray, Kumar - 1994.pdf}
}

@article{Goldreich1977,
  title = {Solar Seismology. {{II}} - {{The}} Stochastic Excitation of the Solar p-Modes by Turbulent Convection},
  author = {Goldreich, P. and Keeley, D. A.},
  year = {1977},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {212},
  pages = {243},
  publisher = {{American Astronomical Society}},
  issn = {0004-637X},
  doi = {10.1086/155043},
  urldate = {2022-01-26},
  abstract = {We test the hypothesis that the solar p-modes are stabilized by damping due to turbulent viscosity in the convective zone. Starting from the assumption that the modes are stable, we calculate expectation values for the modal energies. We find that the interaction between a p-mode and the turbulent convection is such that the modal energy tends toward equipartition with the kinetic energy of turbulent eddies whose lifetimes are comparable to the modal period. From the calculated values of the modal energies, we compute rms surface velocity amplitudes. Our predicted rms surface velocities range from 0.01 cm/sec for the fundamental radial mode to 0.6 cm/sec for the radial mode whose period is approximately 5 minutes. The predicted surface velocities for the low order p-modes are much smaller than the velocities inferred from recent observations.},
  keywords = {notion,notion-database}
}

@article{Goldreich1990,
  title = {Wave {{Generation}} by {{Turbulent Convection}}},
  author = {Goldreich, Peter and Kumar, Pawan and Goldreich, Peter and Kumar, Pawan},
  year = {1990},
  month = nov,
  journal = {ApJ},
  volume = {363},
  pages = {694},
  publisher = {{American Astronomical Society}},
  issn = {0004-637X},
  doi = {10.1086/169376},
  urldate = {2022-01-26},
  abstract = {Wave generation by turbulent convection in a plane parallel, stratified atmosphere lying in a gravitational field is studied. The turbulent spectrum is related to the convective energy flux via the Kolmogorov scaling and the mixing length hypothesis. Efficiencies for the conversion of the convective energy flux into both trapped and propagating waves are estimated.},
  keywords = {Acoustic Emission,Astrophysics,Convection,CONVECTION,Gravitational Fields,Magnetohydrodynamic Turbulence,Magnetohydrodynamic Waves,notion,notion-database,Solar Atmosphere,Sound Waves,SUN: ATMOSPHERE,SUN: OSCILLATIONS,TURBULENCE,Wave Generation,WAVE MOTIONS}
}

@article{Gomes2020,
  title = {Core Magnetic Field Imprint in the Non-Radial Oscillations of Red Giant Stars},
  author = {Gomes, Pedro and Lopes, Il{\'i}dio},
  year = {2020},
  month = jul,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {496},
  pages = {620--628},
  issn = {0035-8711},
  doi = {10.1093/mnras/staa1585},
  urldate = {2023-07-27},
  abstract = {Magnetic fields in red giant stars remain a poorly understood topic, particularly in what concerns their intensity in regions far below the surface. In this work, we propose that gravity-dominated mixed modes of high absolute radial order and low angular degree can be used to probe the magnetic field in their radiative cores. Using two poloidal, axisymmetric configurations for the field in the core and the classical perturbative approach, we derive an analytical expression for the magnetic frequency splitting of these oscillation modes. Considering three distinct red giant models, with masses of 1.3, 1.6, and 2.0 M{$\odot$}, we find that a field strength of 105 G is necessary in the core of these stars to induce a frequency splitting of the order of a {$\mu$}Hz in dipole and quadrupole oscillation modes. Moreover, taking into account observational limits, we estimate that magnetic fields in the cores of red giants that do not present observable magnetic splittings cannot exceed 104 G. Given the general absence of observable splittings in the oscillation spectra of these stars, and assuming that present mode suppression mechanisms are not biased towards certain azimuthal orders and retain all peaks in each multiplet, our results lead us to conclude that internal fields with the considered configurations and strengths above 104 G are not prevalent in red giants.},
  keywords = {Asteroseismology,Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,stars: interiors,stars: low-mass,stars: magnetic field,stars: oscillations},
  annotation = {ADS Bibcode: 2020MNRAS.496..620G},
  file = {/Users/lbugnet/Zotero/storage/RRX83JT4/Gomes and Lopes - 2020 - Core magnetic field imprint in the non-radial osci.pdf}
}

@article{Gonczi1998,
  title = {{{SOLAR SOUND SPEED INFERRED FROM SoHO HELIOSEISMIC DATA}}},
  author = {Gonczi, G. and Berthomieu, G. and Corbard, T. and Provost, J. and Morel, P. and {GOLF team}},
  year = {1998},
  journal = {ESASP},
  volume = {418},
  urldate = {2020-03-02},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VB8AB9YH/full-text.pdf}
}

@article{Gondoin2009a,
  title = {Differential Rotation on Active Late-Type Stars Observed with {{Corot}}},
  author = {Gondoin, P. and Fridlund, M. and Gandolfi, D. and G{\"u}enter, E.},
  year = {2009},
  journal = {Proceedings of the International Astronomical Union},
  volume = {5},
  number = {S264},
  pages = {60--62},
  issn = {1743-9213},
  doi = {10.1017/s1743921309992365},
  abstract = {One major topic in studying stellar activity is to explain how phenomena seen on the Sun and stars, and specially magnetic phenomena, depend on stellar properties such as rotation and age. Differential rotation is an important physical process in theories of stellar magnetic field generation. The solar surface differential rotation was initially discovered via the simple method of tracking the rotation rates of individual starspots at different latitudes. Adopting a similar principle, high accuracy light curves of active stars observed with the CoRoT satellite are analyzed using a model based on the rotational modulation of the visibility of active regions.},
  keywords = {activity,late-type,notion,notion-database,rotation,spots,stars},
  file = {/Users/lbugnet/Zotero/storage/XVSC8YG5/Gondoin et al. - 2009.pdf}
}

@article{Gondoin2012,
  title = {A Time Evolution Model of {{X-ray}} Activity on the Main Sequence},
  author = {Gondoin, P},
  year = {2012},
  journal = {A\&A},
  volume = {546},
  pages = {117},
  doi = {10.1051/0004-6361/201219823},
  urldate = {2020-07-02},
  abstract = {Context. The X-ray emission from late-type stars in open clusters exhibits two kinds of dependences on stellar rotation. While fast ro-tators have a relatively constant X-ray emission level, slower rotators show a decline of their X-ray emission with decreasing rotation rate. The physical significance of the transition between these two X-ray emission regimes is a matter of debate. During the {$\sim$}500 Myr period of stellar evolution that separates the Pleiades from the Hyades, late-type stars such as those present in the M 34 open cluster undergo significant changes in their rotation rates. These could affect the dynamo processes in their interiors, possibly altering their surface magnetic fluxes. Aims. The purpose of the present study is to look for the X-ray signatures of such possible modifications, to search for correlations with rotation and stellar parameters, and to propose a parameterization of the X-ray activity evolution on the main sequence. The aim is to provide observational constraints on the time evolution of dynamo processes in the interiors of late-type stars. Methods. The distributions of stellar X-ray luminosities vs. rotation periods and Rossby numbers of a sample of M 34 late-type stars are compared with rotation-activity relationships established in a large sample of cluster members and field stars. A model of X-ray activity evolution is developed by combining an X-ray activity-rotation relationship with a recent model of stellar rotation evolution on the main sequence. The distribution of stellar X-ray luminosities in M 34 is compared with this model. Results. A correlation is observed between the saturated and non-saturated regime of X-ray emission and the C-and I-rotational sequences that have been observed in M 34 from extensive rotational periods surveys. M 34 sample stars show a steep transition in X-ray to bolometric luminosity ratio between the C-sequence and gap stars that emit close to the 10 -3 saturation level, and the I-sequence stars, whose L X /L bol ratio is significantly lower for similar values of the Rossby number. A comparison between X-ray emission vs. mass distribution in M 34 and the X-ray luminosity evolution model suggests that the transition between the saturated and non-saturated regime of X-ray emission occurs in M 34 cluster members depending on their convective turnover time and period of rotation. Conclusions. I argue that the drop of (L X /L bol) by one order of magnitude observed in M 34 around a Rossby number of 0.3 is indicative of a change in dynamo efficiency. I conclude that the transition from the saturated to the non-saturated regime of X-ray emission among main-sequence stars is the result of a dynamo regime transition, possibly between a turbulent dynamo and an interface-type dynamo.},
  keywords = {activity-stars,atmospheres-stars,individual,late-type-stars,M 34-stars,magnetic field-stars,notion,notion-database,open clusters and associations,rotation}
}

@article{Gondoin2012a,
  title = {From {{CoRoT}} 102899501 to the {{Sun}}. {{A}} Time Evolution Model of Chromospheric Activity on the Main Sequence},
  author = {Gondoin, P. and Gandolfi, D. and Fridlund, M. and Frasca, A. and Guenther, E. W. and Hatzes, A. and Deeg, H. J. and Parviainen, H. and Eigmueller, P. and Deleuil, M.},
  year = {2012},
  month = oct,
  eprint = {1210.3221},
  doi = {10.1051/0004-6361/201219101},
  urldate = {2020-07-04},
  abstract = {Using a model based on the rotational modulation of the visibility of active regions, we analyse the high-accuracy CoRoT lightcurve of the active young star CoRoT102899501. Spectroscopic follow-up observations are used to derive its fundamental parameters. We compare its chromospheric activity level with a model of chrosmospheric activity evolution established by combining relationships between the R'HK index and the Rossby number with a recent model of stellar rotation evolution on the main sequence. We measure the spot coverage of the stellar surface as a function of time, and find evidence for a tentative increase from 5-14\% at the beginning of the observing run to 13-29\% 35 days later. A high level of magnetic activity on CoRoT102899501 is corroborated by a strong emission in the Balmer and Ca II HK lines (logR'HK \textasciitilde{} -4). The starspots used as tracers of the star rotation constrain the rotation period to 1.625+/-0.002 days and do not show evidence for differential rotation. The effective temperature (Teff=5180+/-80 K), surface gravity (logg=4.35+/-0.1), and metallicity ([M/H]=0.05+/-0.07 dex) indicate that the object is located near the evolutionary track of a 1.09+/-0.12 M\_Sun pre-main sequence star at an age of 23+/-10 Myrs. This value is consistent with the "gyro-age" of about 8-25 Myrs, inferred using a parameterization of the stellar rotation period as a function of colour index and time established for the I-sequence of stars in stellar clusters. We conclude that the high magnetic activity level and fast rotation of CoRoT102899501 are manifestations of its stellar youth consistent with its estimated evolutionary status and with the detection of a strong Li I 6707.8 A absorption line in its spectrum. We argue that a magnetic activity level comparable to that observed on CoRoT102899501 could have been present on the Sun at the time of planet formation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AFAZ6UIR/full-text.pdf}
}

@article{Gontcharov2018,
  title = {Isochrone Fitting of {{Galactic}} Globular Clusters - {{I}}. {{NGC}} 5904},
  author = {Gontcharov, George A. and Mosenkov, Aleksandr V. and Khovritchev, Maxim Yu.},
  year = {2018},
  month = dec,
  eprint = {1812.06433},
  doi = {10.1093/mnras/sty3439},
  abstract = {We present new isochrone fits to colour-magnitude diagrams of the Galactic globular cluster NGC 5904 (M5). We utilise 29 photometric bands from the ultraviolet to mid-infrared by use of the data from the \{\textbackslash it Hubble Space Telescope\}, \{\textbackslash it Gaia\} DR2, \{\textbackslash it Wide-field Infrared Survey Explorer\}, Sloan Digital Sky Survey (SDSS), and other photometric data. In our isochrone fitting we use the PAdova and TRieste Stellar Evolution Code, the MESA Isochrones and Stellar Tracks, the Dartmouth Stellar Evolution Program, and a Bag of Stellar Tracks and Isochrones both for the solar-scaled and enhanced He and \$\textbackslash alpha\$ abundances with a metallicity about [Fe/H]\$=-1.33\$ adopted from the literature. All tools provide us with estimates of the distance, age, and extinction law to the cluster. The best-fit distance, true distance modulus, and age are \$7.4\textbackslash pm0.3\$ kpc, \$14.34\textbackslash pm0.09\$ mag, and \$12.15\textbackslash pm1.00\$ Gyr, respectively. The derived distance agrees with the literature, including the \{\textbackslash it Gaia\} DR2 parallax with its known global zero-point correction. All the data and models, except some UV and SDSS data, agree with the extinction law of Cardelli-Clayton-Mathis with \$R\_\textbackslash mathrm\{V\}=3.60\textbackslash pm0.05\$ and \$A\_\textbackslash mathrm\{V\}=0.20\textbackslash pm0.02\$ mag. This extinction is twice as high as generally accepted due to a rather high extinction between 625 and 2000 nm. An offset of the model colours instead of the high extinction in this range is a less likely, yet possible explanation of the discovered large deviations of the isochrones from the data.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/H7QTKERM/1812.06433.pdf}
}

@article{Gonzalez2016,
  title = {Variability among Stars in the {{M}} 67 Field from {{Kepler}}/{{K2-Campaign-5}} Light Curves},
  author = {Gonzalez, Guillermo},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {459},
  number = {1},
  pages = {1060--1068},
  issn = {13652966},
  doi = {10.1093/mnras/stw700},
  abstract = {We examine the photometric variability of stars in the M 67 field using Kepler/K2-Campaign-5 light curves. Variabilities and periods were determined for 639 stars. The mean photometric period of 28 single Sun-like members stars in M 67 is 23.4 {$\pm$} 1.2 d. This corresponds to a gyro-age of 3.7 {$\pm$} 0.3 Gyr, assuming the periods can be associated with rotation. The intrinsic variabilities of the solar analogues are greater than the Sun's variability, as measure from VIRGO fluxes. We also find evidence that the single cluster members have a different distribution of variability than the binary members.},
  keywords = {notion,notion-database,Open clusters and associations: individual: M 67,Stars: rotation,Stars: variables: general,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/E2ESXDJA/Gonzalez - 2016.pdf}
}

@article{GonzlezHernndez2010a,
  title = {Meridional Circulation during the Extended Solar Minimum: {{Another}} Component of the Torsional Oscillation?},
  author = {Gonzlez Hernndez, I. and Howe, R. and Komm, R. and Hill, F.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {1 PART 2},
  pages = {16--20},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/1/L16},
  abstract = {We show here a component of the meridional circulation developing at medium-high latitudes (40\textdegree -50\textdegree ) before the new solar cycle starts. Like the torsional oscillation of the zonal flows, this extra circulation seems to precede the onset of magnetic activity at the solar surface and moves slowly toward lower latitudes. However, the behavior of this component differs from that of the torsional oscillation regarding location and convergence toward the equator at the end of the cycle. The observation of this component before the magnetic regions appear at the solar surface has only been possible due to the prolonged solar minimum. The results could settle the discussion as to whether the extra component of the meridional circulation around the activity belts, which has been known for some time, is or is not an effect of material motions around the active regions. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: interior,Sun: surface magnetism},
  file = {/Users/lbugnet/Zotero/storage/JDHESXLY/Gonzlez Hernndez et al. - 2010.pdf}
}

@article{Goode1992,
  title = {The Effect of an Inlcined Magnetic Field on Solar Oscillation Frequencies},
  author = {Goode, P. R. and Thompson, Michael J.},
  year = {1992},
  journal = {The Astrophysical Journal},
  volume = {395},
  eprint = {1011.1669v3},
  pages = {307--315},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G8GIMKE6/Goode, Thompson - 1992.pdf}
}

@article{Goodricke1784,
  title = {On the {{Periods}} of the {{Changes}} of {{Light}} in the {{Star Algol}}. {{In}} a {{Letter}} from {{John Goodricke}}, {{Esq}}. to the {{Rev}}. {{Anthony Shepherd}}, {{D}}. {{D}}. {{F}}. {{R}}. {{S}}. {{Professor}} of {{Astronomy}} at {{Cambridge}}},
  author = {Goodricke, John and {John}},
  year = {1784},
  journal = {RSPT},
  volume = {74},
  pages = {287--292},
  urldate = {2020-03-07},
  keywords = {notion,notion-database}
}

@article{gotbergImpactStarsStripped2019,
  title = {The Impact of Stars Stripped in Binaries on the Integrated Spectra of Stellar Populations},
  author = {G{\"o}tberg, Y. and {de Mink}, S. E. and Groh, J. H. and Leitherer, C. and Norman, C.},
  year = {2019},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {629},
  pages = {A134},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201834525},
  urldate = {2022-08-08},
  abstract = {Stars stripped of their envelopes from interaction with a binary companion emit a significant fraction of their radiation as ionizing photons. They are potentially important stellar sources of ionizing radiation, however, they are still often neglected in spectral synthesis simulations or simulations of stellar feedback. In anticipating the large datasets of galaxy spectra from the upcoming James Webb Space Telescope, we modeled the radiative contribution from stripped stars by using detailed evolutionary and spectral models. We estimated their impact on the integrated spectra and specifically on the emission rates of H i-, He i-, and He ii-ionizing photons from stellar populations. We find that stripped stars have the largest impact on the ionizing spectrum of a population in which star formation halted several Myr ago. In such stellar populations, stripped stars dominate the emission of ionizing photons, mimicking a younger stellar population in which massive stars are still present. Our models also suggest that stripped stars have harder ionizing spectra than massive stars. The additional ionizing radiation, with which stripped stars contribute affects observable properties that are related to the emission of ionizing photons from stellar populations. In co-eval stellar populations, the ionizing radiation from stripped stars increases the ionization parameter and the production efficiency of hydrogen ionizing photons. They also cause high values for these parameters for about ten times longer than what is predicted for massive stars. The effect on properties related to non-ionizing wavelengths is less pronounced, such as on the ultraviolet continuum slope or stellar contribution to emission lines. However, the hard ionizing radiation from stripped stars likely introduces a characteristic ionization structure of the nebula, which leads to the emission of highly ionized elements such as O2+ and C3+. We, therefore, expect that the presence of stripped stars affects the location in the BPT diagram and the diagnostic ratio of O iii to O ii nebular emission lines. Our models are publicly available through CDS database and on the Starburst99 website.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/757BZ86T/Götberg et al. - 2019 - The impact of stars stripped in binaries on the in.pdf}
}

@article{gotbergStarsStrippedBinaries2020,
  title = {Stars {{Stripped}} in {{Binaries}}: {{The Living Gravitational-wave Sources}}},
  shorttitle = {Stars {{Stripped}} in {{Binaries}}},
  author = {G{\"o}tberg, Y. and Korol, V. and Lamberts, A. and Kupfer, T. and Breivik, K. and Ludwig, B. and Drout, M. R.},
  year = {2020},
  month = nov,
  journal = {The Astrophysical Journal},
  volume = {904},
  number = {1},
  pages = {56},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/abbda5},
  urldate = {2022-08-08},
  abstract = {Binary interaction can cause stellar envelopes to be stripped, which significantly reduces the radius of the star. The orbit of a binary composed of a stripped star and a compact object can therefore be so tight that the gravitational radiation the system produces reaches frequencies accessible to the Laser Interferometer Space Antenna (LISA). Two such stripped stars in tight orbits with white dwarfs are known so far (ZTF J2130+4420 and CD-30\textdegree 11223), but many more are expected to exist. These binaries provide important constraints for binary evolution models and may be used as LISA verification sources. We develop a Monte Carlo code that uses detailed evolutionary models to simulate the Galactic population of stripped stars in tight orbits with either neutron star or white dwarf companions. We predict 0\textendash 100 stripped star + white dwarf binaries and 0\textendash 4 stripped star + neutron star binaries with a signal-to-noise ratio {$>$}5 after 10 yr of observations with LISA. More than 90\% of these binaries are expected to show large radial velocity shifts of 200 km s-1, which are spectroscopically detectable. Photometric variability due to tidal deformation of the stripped star is also expected and has been observed in ZTF J2130+4420 and CD-30\textdegree 11223.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/8UCQEGLW/Götberg et al. - 2020 - Stars Stripped in Binaries The Living Gravitation.pdf}
}

@article{Gough1977,
  title = {Mixing Length Theory for Pulsating Stars},
  author = {Gough, D. O.},
  year = {2019},
  journal = {The Astrophysical Journal},
  volume = {214},
  eprint = {1011.1669v3},
  pages = {196--213},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KF4VYTNR/Gough - 2019.pdf}
}

@article{Gough1984,
  title = {Influence of Rotation and Magnetic Fields on Stellar Oscillation Eigenfrequencies},
  author = {Gough, D. O. and Taylor, P.P.},
  year = {1984},
  journal = {Mem. S.A. It.},
  volume = {55},
  pages = {215},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/THJTT5QA/Gough, Taylor - 1984.pdf}
}

@article{Gough1984,
  title = {Helioseismology},
  author = {Gough, Douglas},
  year = {1984},
  journal = {Interdisciplinary Science Reviews},
  volume = {9},
  number = {3},
  pages = {240--251},
  issn = {17432790},
  doi = {10.1179/isr.1984.9.3.240},
  abstract = {Sound waves generated in the solar convection zone propagate through the Sun and cause it to vibrate. Resonant vibrations are detected by measuring wavelike motion that they produce on the solar surface; by analyzing them we can learn about conditions in the solar interior. At present we have only limited data but already we have drawn an important conclusion. We have inferred that outside the core of the Sun, and beneath the subsurface convection zone, the abundance of helium is about 25\% by mass. It is generally believed that the intermediate region in the Sun is uncontaminated by the products of the nuclear reactions in the core and by material that might have fallen into the Sun from interstellar space. If that is indeed the case, we have measured the helium abundance of the gas cloud from which the Sun condensed some 4.7 thousand million years ago. This information is relevant to our understanding of the early stages of the evolution of the Universe. It is exciting that there are hints in the vibration data that might even enable us to determine whether the Sun really has remained unmixed, and hence whether we have a faithful record of the primordial mixture. There is also evidence in the data concerning the Sun's internal rotation. It appears that the core of the Sun rotate faster than the surface, but by how much is a subject of some controversy. It is very important to settle the matter, because the result is an essential step in one of the most important tests of Einstein's General Theory of Relativity. What evidence we have at present does not contradict Einstein's theory. \textcopyright{} 1984 Maney Publishing.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/V3NZ5MIV/Gough - 1984.pdf}
}

@book{Gough1986,
  title = {Book-{{Review}} - {{Seismology}} of the {{Sun}} and the {{Distant Stars}} - {{NASA}}/{{ADS}}},
  author = {Gough, D.O.},
  year = {1986},
  volume = {72},
  urldate = {2020-04-09},
  keywords = {notion,notion-database}
}

@article{Gough1990a,
  title = {The Effect of Rotation and a Burried Magnetic Field on Stellar Oscillations},
  author = {Gough, D. O. and Thompson, M. J.},
  year = {1990},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {242},
  pages = {25--55},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2RCW6RJI/Gough, Thompson - 1990.pdf}
}

@inproceedings{Gough1993,
  title = {Linear Adiabatic Stellar Pulsation.},
  booktitle = {47. Session de l'{{Ecole}} d'{{Et\'e}} de {{Physique Th\'eorique}}: {{Astrophysical}} Fluid Dynamics - {{Les Houches}}},
  author = {Gough, D. O.},
  year = {1993},
  pages = {399--560},
  urldate = {2020-06-26},
  keywords = {Nonradial Pulsations: Stellar Models,notion,notion-database,Pulsation Theory: Stars,Solar Oscillations,Stellar Oscillations}
}

@article{Gough1995,
  title = {Constrained Estimates of Low-Degree Mode Frequencies and the Determination of the Interior Structure of the {{Sun}}},
  author = {Gough, D. O. and Kosovichev, A. G. and Toutain, T.},
  year = {1995},
  journal = {Solar Physics},
  volume = {157},
  number = {1-2},
  pages = {1--15},
  issn = {00380938},
  doi = {10.1007/BF00680605},
  abstract = {Low-degree p-modes penetrate to the solar centre and provide direct information about the core. However, the high observational accuracy that is required to resolve the details of the structure of the core is difficult to achieve because the oscillation power spectrum is significantly distorted by stochastic forcing of the oscillations, which appears as multiplicative noise. Here, an attempt is reported to reduce uncertainties of spectral parameter estimation by incorporating constraints imposed by smooth behaviour of some of the parameters (e.g., linewidths, background noise, rotational splitting) over a group of lines. Instead of estimating these parameters independently for each line, we determine them as smooth functions of frequency. It is expected that this procedure gives more accurate estimates of the average frequencies of any multiplet in the power spectrum, to which we have applied no constraints. We give some examples of the procedure for whole-disk measurements by the IPHIR space experiment. It is shown that the additional constraints do not result in significant changes in the frequency estimates, except for one mode whose peak in the power spectrum has the lowest signal-to-noise ratio. However, the uncertainty in the frequency of that mode does not influence substantially the results of the structure inversion in the core. Inversions of the IPHIR datasets are compared with corresponding inversions of data from the Birmingham Solar Oscillation Network (BISON). The IPHIR data indicate a sharp increase towards the centre of the deviation of the squared sound speed of the sun from that of a standard solar model, whereas the BISON data show a decrease. The difference between the IPHIR and BISON inversions is significant, preventing any definite conclusion about the deviation of the structure of the solar core from that of the model. \textcopyright{} 1995 Kluwer Academic Publishers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SME3LCDH/Gough, Kosovichev, Toutain - 1995.pdf}
}

@article{Gough1996,
  title = {The Seismic Structure of the Sun},
  author = {Gough, D. O. and Kosovichev, A. G. and Toomre, J. and Anderson, E. and Antia, H. M. and Basu, S. and Chaboyer, B. and Chitre, S. M. and {Christensen-Dalsgaard}, J. and Dziembowski, W. A. and {Eff-Darwich}, A. and Elliott, J. R. and Giles, P. M. and Goode, P. R. and Guzik, J. A. and Harvey, J. W. and Hill, F. and Leibacher, J. W. and Monteiro, M. J.P.F.G. and Richard, O. and Sekii, T. and Shibahashi, H. and Takata, M. and Thompson, M. J. and Vauclair, S. and Vorontsov, S. V.},
  year = {1996},
  journal = {Science},
  volume = {272},
  number = {5266},
  pages = {1296--1300},
  issn = {00368075},
  doi = {10.1126/science.272.5266.1296},
  abstract = {Global Oscillation Network Group data reveal that the internal structure of the sun can be well represented by a calibrated standard model. However, immediately beneath the convection zone and at the edge of the energy-generating core, the sound-speed variation is somewhat smoother in the sun than it is in the model. This could be a consequence of chemical inhomogeneity that is too severe in the model, perhaps owing to inaccurate modeling of gravitational settling or to neglected macroscopic motion that may be present in the sun. Accurate knowledge of the sun's structure enables inferences to be made about the physics that controls the sun; for example, through the opacity, the equation of state, or wave motion. Those inferences can then be used elsewhere in astrophysics.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NP8TUJQ6/Gough et al. - 1996.pdf}
}

@article{Gough1998,
  title = {Inevitability of a Magnetic Field in the Sun's Radiative Interior},
  author = {Gough, D. O. and McIntyre, M. E.},
  year = {1998},
  month = aug,
  journal = {Nature},
  volume = {394},
  number = {6695},
  pages = {755--757},
  issn = {00280836},
  doi = {10.1038/29472},
  urldate = {2020-06-06},
  abstract = {The gas in the convective outer layers of the Sun rotates faster at the equator than in the polar regions, yet deeper inside (in the radiative zone) the gas rotates almost uniformly. There is a thin transition layer between these zones, called the tachocline. This structure has been measured seismologically, but no purely fluid-dynamical mechanism can explain its existence. Here we argue that a self-consistent model requires a large-scale magnetic field in the Sun's interior, as well as consideration of the Coriolis effects in the convection zone and in the tachocline. Turbulent stresses in the convection zone induce (through Coriolis effects) a meridional circulation, causing the gas from the convection zone to burrow downwards, thereby generating the horizontal and vertical shear that characterizes the tachocline. The interior magnetic field stops the burrowing, and confines the shear, as demanded by the observed structure of the tacholine. We outline a dynamical theory of the flow, from which we estimate a field strength of about 10-4 tesla just beneath the tachocline. An important test of this picture, after numerical refinement, will be quantitative consistency between the predicted and observed interior angular velocities.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/X2QXKZV5/Gough, McIntyre - 1998.pdf}
}

@article{Gough2003,
  title = {Solar {{Neutrino Production}}},
  author = {Gough, Douglas},
  year = {2003},
  journal = {Annales Henri Poincare},
  volume = {4},
  number = {SUPPL. 1},
  pages = {303--317},
  issn = {14240637},
  doi = {10.1007/s00023-003-0924-z},
  abstract = {It is commonly and quite plausibly presumed that neutrino flavour transitions are responsible for essentially all of the discrepancy between the observed flux of neutrinos from the Sun and the theoretically calculated neutrino production rate. Indeed, the comparison between the detection rates by SuperKamiokande and by the Sudbury Neutrino Observatory are consistent with this presumption. Helio-seismological analysis has set quite tight constraints on the conditions in the Sun's core, where the neutrino-emitting nuclear reactions take place. These constraints have been obtained subject to certain assumptions which need to be investigated before secure precise conclusions concerning neutrino production can be drawn.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YBGZJIVV/Gough - 2003.pdf}
}

@article{Gough2004,
  title = {What We Need to Know about the {{Sun}}},
  author = {Gough, Douglas},
  year = {2004},
  journal = {Proceedings of the International Astronomical Union},
  volume = {2004},
  number = {IAUS223},
  pages = {723},
  issn = {1743-9213},
  doi = {10.1017/s1743921304007434},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JJK6WFDR/Gough - 2004.pdf}
}

@article{Gough2007a,
  title = {Discussion on Solar-like Oscillators and {$\gamma$} {{Doradus}} Stars},
  author = {Gough, D. O.},
  year = {2007},
  journal = {Communications in Asteroseismology},
  volume = {150},
  pages = {155--158},
  issn = {1021-2043},
  doi = {10.1553/cia150s155},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/75JFVPIB/Gough - 2007.pdf}
}

@article{Gough2008,
  title = {The Current State of Stellar Mixing-Length Theory},
  author = {Gough, Douglas},
  year = {2008},
  journal = {Problems of Stellar Convection},
  pages = {15--56},
  doi = {10.1007/3-540-08532-7_31},
  abstract = {The physical model, assumptions, uncertainties, and degree of contact with reality involved in mixing-length theory as applied to stellar convection are reviewed. Attention is given to the ideas behind mixing-length theories, equations of motion, local mixing-length formalisms for a stationary envelope, the assumed structure of the convective flow, and the dynamics of convective eddies. A specific mixing-length model is considered in which the flow is represented by a conglomerate of cells or eddies that form, grow, and subsequently break up. The growth of convective eddies is examined along with the eddy convection rate, initial conditions, an eddy-annihilation hypothesis, and turbulent fluxes. The choice of a mixing length and the calibration of the heat-flux formula are discussed, Reynolds stress is analyzed, and transport of heat and momentum by small-scale turbulence is incorporated into the dynamics. Additional refinements and generalizations are described.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XDUH823K/Gough - 2008.pdf}
}

@article{Gouhier2022,
  title = {Angular Momentum Transport in a Contracting Stellar Radiative Zone Embedded in a Large-Scale Magnetic Field},
  author = {Gouhier, B. and Jouve, L. and Ligni{\`e}res, F.},
  year = {2022},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {661},
  pages = {A119},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202141613},
  urldate = {2023-08-07},
  abstract = {Methods. We performed axisymmetric Boussinesq and anelastic numerical simulations in which a portion of the radiative zone was modelled by a rotating spherical layer, stably stratified and embedded in a large-scale (either dipolar or quadrupolar) magnetic field. This layer is subject to a mass-conserving radial velocity field mimicking contraction. The quasi-steady flows were studied in strongly or weakly stably stratified regimes relevant for pre-main sequence stars and for the cores of subgiant and red giant stars. The parametric study consists in varying the amplitude of the contraction velocity and of the initial magnetic field. The other parameters were fixed with the guidance of a previous study. Results. After an unsteady phase during which the toroidal field grew linearly and then back-reacted on the flow, a quasi-steady configuration was reached, characterised by the presence of two magnetically decoupled regions. In one of them, magnetic tension imposes solid-body rotation. In the other, called the dead zone, the main force balance in the angular momentum equation does not involve the Lorentz force and a differential rotation exists. In the strongly stably stratified regime, when the initial magnetic field is quadrupolar, a magnetorotational instability is found to develop in the dead zones. The large-scale structure is eventually destroyed and the differential rotation is able to build up in the whole radiative zone. In the weakly stably stratified regime, the instability is not observed in our simulations, but we argue that it may be present in stars. Conclusions. We propose a scenario that may account for the post-main sequence evolution of solar-like stars, in which quasi-solid rotation can be maintained by a large-scale magnetic field during a contraction timescale. Then, an axisymmetric instability would destroy this large-scale structure and this enables the differential rotation to set in. Such a contraction-driven instability could also be at the origin of the observed dichotomy between strongly and weakly magnetic intermediate-mass stars.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/GMGCJ5QI/Gouhier et al. - 2022 - Angular momentum transport in a contracting stella.pdf}
}

@article{Goupil2011,
  title = {Open Issues in Probing Interiors of Solar-like Oscillating Main Sequence Stars 1. from the {{Sun}} to Nearly Suns},
  author = {Goupil, M. J. and Lebreton, Y. and Marques, J. P. and Samadi, R. and Baudin, F.},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  eprint = {1102.0247},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012031},
  abstract = {We review some major, open issues in the current modelling of low and intermediate mass, main sequence stars based on seismological studies. In the present paper, the solar case is discussed together with current problems that are common to the Sun and stars with a structure similar to that of the Sun. Several additional issues specific to main sequence stars other than the Sun are reviewed and illustrated with a few stars observed with CoRoT in a companion paper. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/J249Q2W2/Goupil et al. - 2011.pdf;/Users/lbugnet/Zotero/storage/MIFVPTZP/Goupil et al. - 2011(2).pdf}
}

@article{Goupil2013,
  title = {Seismic Diagnostics for Transport of Angular Momentum in Stars : {{II}}. {{Interpreting}} Observed Rotational Splittings of Slowly Rotating Red Giant Stars},
  author = {Goupil, M. J. and Mosser, B. and Marques, J. P. and Ouazzani, R. M. and Belkacem, K. and Lebreton, Y. and Samadi, R.},
  year = {2013},
  journal = {Astronomy \& Astrophysics},
  volume = {549},
  eprint = {1211.1546},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220266},
  urldate = {2020-04-20},
  abstract = {Asteroseismology based on observations from the space-borne missions CoRoT and Kepler provides a powerful means of testing the modeling of transport processes in stars. Rotational splittings are currently measured for a large number of red giant stars and can provide stringent constraints on the rotation profiles. The aim of this paper is to obtain a theoretical framework for understanding the properties of the observed rotational splittings of red giant stars with slowly rotating cores. This allows us to establish appropriate seismic diagnostics for the rotation of these evolved stars. Rotational splittings were computed for stochastically excited dipolar modes by adopting a first-order perturbative approach for two 1.3 M{$\cdot$} benchmark models that assume slowly rotating cores. For red giant stars with slowly rotating cores, we show that the variation in the rotational splittings of {$\mathscr{l}$}= 1 modes with frequency depends only on the large frequency separation, the g-mode period spacing, and the ratio of the average envelope to core rotation rates (R). This led us to propose a way to infer directly \^a., from the observations. This method is validated using the Kepler red giant star KIC 5356201. Finally, we provide theoretical support for using a Lorentzian profile to measure the observed splittings for red giant stars. \textcopyright{} 2012 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/9UJW95VC/full-text.pdf}
}

@article{Goupil2014,
  title = {Transport of Angular Momentum in Solar-like Oscillating Stars},
  author = {Goupil, Mariejo and Deheuvels, S{\'e}bastien and Marques, Joao and Lebreton, Yveline and Mosser, Benoit and Garc{\'i}a, Rafa and Belkacem, Kevin and Mathis, St{\'e}phane},
  year = {2014},
  journal = {Proceedings of the International Astronomical Union},
  volume = {9},
  number = {S301},
  pages = {161--168},
  issn = {17439213},
  doi = {10.1017/S1743921313014269},
  abstract = {Our current understanding and modeling of angular momentum transport in low-mass stars are briefly reviewed. Emphasis is set on single stars slightly younger that the Sun and on subgiants and red giants observed by the space missions CoRoT and Kepler. Copyright \textcopyright{} International Astronomical Union 2014.},
  isbn = {9781107045170},
  keywords = {notion,notion-database,stars: evolution,stars: interiors,stars: oscillations,stars: rotation,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/78NX85D8/Goupil et al. - 2014.pdf}
}

@incollection{Grad1958,
  title = {Principles of the {{Kinetic Theory}} of {{Gases}}},
  booktitle = {{{HDP}}},
  author = {Grad, Harold},
  year = {1958},
  volume = {3},
  pages = {205--294},
  doi = {10.1007/978-3-642-45892-7_3},
  urldate = {2020-07-02},
  abstract = {For the purposes of this article, the subject of the kinetic theory of gases is considered to be coextensive with the theory of the \{Boltzmann\} equation. We consider only the original equation of Maxwell and of \{Boltzmann\} for classical point molecules and short range forces, putting aside the equally interesting but distinct questions which arise from the inclusion of internal degrees of freedom, quantum interactions, inverse square forces, and imperfect gases. The special case of a Knudsen gas of freely streaming particles is only touched on, mainly for purposes of comparison.},
  keywords = {notion,notion-database}
}

@article{Green2003,
  title = {Discovery of {{A New Class}} of {{Pulsating Stars}}: {{Gravity-Mode Pulsators}} among {{Subdwarf B Stars}}},
  author = {Green, E. M. and Fontaine, G. and Reed, M. D. and Callerame, K. and Seitenzahl, I. R. and White, B. A. and Hyde, E. A. and {\O}stensen, R. and Cordes, O. and Brassard, P. and Falter, S. and Jeffery, E. J. and Dreizler, S. and Schuh, S. L. and Giovanni, M. and Edelmann, H. and Rigby, J. and Bronowska, A.},
  year = {2003},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {583},
  number = {1},
  pages = {L31-L34},
  publisher = {{IOP Publishing}},
  issn = {0004637X},
  doi = {10.1086/367929},
  urldate = {2020-04-09},
  abstract = {During the course of an ongoing CCD monitoring program to investigate low-level light variations in subdwarf B (sdB) stars, we have serendipitously discovered a new class of low-amplitude, multimode sdB pulsators with periods of the order of an hour. These periods are more than a factor of 10 longer than those of previously known multimode sdB pulsators (EC 14026 stars), implying that they are due to gravity modes rather than pressure modes. The longer period pulsators are found only among cooler sdB stars, where they are surprisingly common. The iron opacity instability that drives the short-period EC 14026 stars is effective only in hot sdB stars, leaving the driving mechanism for the deeper gravity modes in cool sdB stars currently unknown. We present the first observational results for our newly identified sdB variables and discuss possible implications.},
  keywords = {Branch,notion,notion-database,Stars: Horizontal,Stars: Individual: Alphanumeric: PG 1716+426,Stars: Oscillations,Stars: Subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/EV5D9NZP/full-text.pdf}
}

@article{Griffiths2022,
  title = {The Magneto-Rotational Instability in Massive Stars},
  author = {Griffiths, Adam and Eggenberger, Patrick and Meynet, Georges and Moyano, Facundo and Aloy, Miguel-{\'A}.},
  year = {2022},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {665},
  pages = {A147},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202243599},
  urldate = {2023-10-18},
  abstract = {Context. The magneto-rotational instability (MRI) has been proposed as a mechanism to transport angular momentum (AM) and chemical elements in theoretical stellar models. Aims: Using as a prototype a massive star of 15 M{$\odot$} with solar metallicity, we explore the effects of the MRI on the evolution of massive stars. Methods: We used the Geneva Stellar Evolution Code to simulate the evolution of various models, up to the end of oxygen burning, including the MRI through effective, one-dimensional, diffusion coefficients. We consider different trigger conditions (depending on the weighting of chemical gradients through an arbitrary but commonly used factor) and different treatments of meridional circulation as either advective or diffusive. We also compare the MRI with the Tayler-Spruit (TS) dynamo in models that included both instabilities. Results: The MRI triggers throughout stellar evolution. Its activation is highly sensitive to the treatment of meridional circulation and the existence of chemical gradients. The MRI is very efficient at transporting both matter and AM, leading to noticeable differences in rotation rates and chemical structure, which may be observable in young main sequence stars. While the TS dynamo is the dominant mechanism for transferring AM, the MRI remains relevant in models where both instabilities are included. Extrapolation of our results suggests that models that include the MRI tend to develop more compact cores, which likely produce failed explosions and black holes, than models where only the TS dynamo is included (where explosions and neutron stars may be more frequent). Conclusions: The MRI can be an important factor in massive star evolution but is very sensitive to the implementation of other processes in the model. The transport of AM and chemical elements due to the MRI alters the rotation rates and the chemical makeup of the star from the core to the surface and may change the explodability properties of massive stars.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,instabilities,stars: abundances,stars: evolution,stars: magnetic field,stars: rotation},
  annotation = {ADS Bibcode: 2022A\&A...665A.147G},
  file = {/Users/lbugnet/Zotero/storage/PHJGFEC5/Griffiths et al. - 2022 - The magneto-rotational instability in massive star.pdf}
}

@article{Grigahcène2005,
  title = {Convection-Pulsation Coupling. {{I}}. {{A}} Mixing-Length Perturbative Theory},
  author = {Grigahc{\`e}ne, A. and Dupret, M. A. and Gabriel, M. and Garrido, R. and Scuflaire, R.},
  year = {2005},
  month = may,
  journal = {A\&A},
  volume = {434},
  number = {3},
  pages = {1055--1062},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20041816},
  urldate = {2022-01-26},
  abstract = {We present in details a time-dependent convection treatment in the frame of the Mixing-Length Theory (MLT). Following the original ideas by Unno (1967, PASJ, 19, 140), this theory has been developed by Gabriel et al. (1974, Bull. Ac. Roy. Belgique, Classe des Sciences, 60, 866) and Gabriel (1996, Bull. Astron. Soc. India, 24, 233). In this paper, we present it in a united form, we detail the basic derivations and approximations and give final improvements. A new perturbation of the energy closure equation is proposed for the first time, making it possible to avoid the occurrence of short wavelength spatial oscillations of the thermal eigenfunctions. This theory accounts for the perturbation of the corrective flux, the turbulent Reynolds stress and the turbulent kinetic energy dissipation. It has been numerically implemented in a non-radial non-adiabatic pulsation code and the first results published in a Letter by Dupret et al. (2004a, A\&A, 414, L17) indicate that the theory predicts the observed red border of the lower end of the instability strip and the driving mechanism of the recently discovered {$\gamma$} Dor stars. \textcopyright ESO 2005.},
  keywords = {convection,notion,notion-database,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/SGMTNVBJ/full-text.pdf}
}

@article{Grigahcene2010,
  title = {Hybrid {{$\gamma$dORADUS-$\delta$Scuti Pulsators}}: {{New}} Insights into the Physics of the Oscillations from Kepler Observations},
  author = {Grigahc{\`e}ne, A. and Antoci, V. and Balona, L. and Catanzaro, G. and {Daszy{\'n}ska-Daszkiewicz}, J. and Guzik, J. A. and Handler, G. and Houdek, G. and Kurtz, D. W. and Marconi, M. and Monteiro, M. J.P.F.G. and Moya, A. and Ripepi, V. and Surez, J. C. and Uytterhoeven, K. and Borucki, W. J. and Brown, T. M. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Jenkins, J. M. and Kjeldsen, H. and Koch, D. and Bernabei, S. and Bradley, P. and Breger, M. and Criscienzo, M. Di and Dupret, M. A. and Garc{\'i}a, R. A. and Hernndez, A. Garc{\'i}a and Jackiewicz, J. and Kaiser, A. and Lehmann, H. and {Mart{\'i}n-Ruiz}, S. and Mathias, P. and {Molenda-Akowicz}, J. and Nemec, J. M. and Nuspl, J. and Papar{\'o}, M. and Roth, M. and Szab{\'o}, R. and Suran, M. D. and Ventura, R.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0747},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L192},
  abstract = {Observations of the pulsations of stars can be used to infer their interior structure and test theoretical models. The main-sequence {$\gamma$}Doradus (Dor) and {$\delta$}Scuti (Sct) stars with masses 1.2-2.5M are particularly useful for these studies. The {$\gamma$}Dor stars pulsate in high-order g-modes with periods of order 1day, driven by convective blocking at the base of their envelope convection zone. The {$\delta$}Sct stars pulsate in low-order g- and p-modes with periods of order 2 hr, driven by the {$\kappa$} mechanism operating in the He II ionization zone. Theory predicts an overlap region in the Hertzsprung-Russell diagram between instability regions, where "hybrid" stars pulsating in both types of modes should exist. The two types of modes with properties governed by different portions of the stellar interior provide complementary model constraints. Among the known {$\gamma$}Dor and {$\delta$}Sct stars, only four have been confirmed as hybrids. Now, analysis of combined Quarter 0 and Quarter 1 Kepler data for hundreds of variable stars shows that the frequency spectra are so rich that there are practically no pure {$\delta$}Sct or {$\gamma$}Dor pulsators, i.e., essentially all of the stars show frequencies in both the {$\delta$}Sct and the {$\gamma$}Dor frequency range. A new observational classification scheme is proposed that takes into account the amplitude as well as the frequency and is applied to categorize 234 stars as {$\delta$}Sct, {$\gamma$}Dor, {$\delta$}Sct/{$\gamma$}Dor or {$\gamma$}Dor/{$\delta$}Sct hybrids. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Space vehicles: instruments,Stars: variables: delta Scuti},
  file = {/Users/lbugnet/Zotero/storage/ZJ23FGTP/Grigahcène et al. - 2010.pdf}
}

@article{Grigahcene2010b,
  title = {Kepler Observations: {{Light}} Shed on the Hybrid {$\gamma$} {{Doradus}} - {$\delta$} {{Scuti}} Pulsation Phenomenon},
  author = {Grigahc{\`e}ne, A. and Uytterhoeven, K. and Antoci, V. and Balona, L. and Catanzaro, G. and {Daszy{\'n}ska-Daszkiewicz}, J. and Guzik, J. A. and Handler, G. and Houdek, G. and Kurtz, D. W. and Marconi, M. and Monteiro, M. J.P.F.G. and Moya, A. and Ripepi, V. and Su{\'a}rez, J. C. and Borucki, W. J. and Brown, T. M. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Jenkins, J. M. and Kjeldsen, H. and Koch, D. and Bernabei, S. and Bradley, P. and Breger, M. and Di Criscienzo, M. and Dupret, M. A. and Garc{\'i}a, R. A. and Garc{\'i}a Hern{\'a}ndez, A. and Jackiewicz, J. and Kaiser, A. and Lehmann, H. and {Mart{\'i}n-Ruiz}, S. and Mathias, P. and {Molenda-Zakowicz}, J. and Nemec, J. M. and Nuspl, J. and Papar{\'o}, M. and Roth, M. and Szab{\'o}, R. and Suran, M. D. and Ventura, R.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  pages = {989--992},
  issn = {15213994},
  doi = {10.1002/asna.201011443},
  abstract = {Through the observational study of stellar pulsations, the internal structure of stars can be probed and theoretical models can be tested. The main sequence -{$\gamma$} Doradus (Dor) and {$\delta$} Scuti (Sct) stars with masses 1.2-2.5 M{$\odot$} are particularly interesting for asteroseismic study. The -{$\gamma$} Dor stars pulsate in high-order gravity (g) modes, with pulsational periods of order of one day. The {$\delta$} Sct stars, on the other hand, show low-order g and pressure (p) modes with periods of order of 2 hours. Theory predicts the existence of 'hybrid' stars, i.e. stars pulsating in both types of modes, in an overlap region between the instability strips of -{$\gamma$} Dor and {$\delta$} Sct stars in the Hertzsprung-Russell diagram. Hybrid stars are particularly interesting as the two types of modes probe different regions of the stellar interior and hence provide complementary model constraints. Before the advent of Kepler, only a few hybrid stars had been confirmed. The Kepler satellite is providing a true revolution in the study of and search for hybrid stars. Analysis of the first 50 days of Kepler data of hundreds of -{$\gamma$} Dor and {$\delta$} Sct candidates reveals extremely rich frequency spectra, with most stars showing frequencies in both the {$\delta$} Sct and -{$\gamma$} Dor frequency range. As these results show that there are practically no pure {$\delta$} Sct or -{$\gamma$} Dor pulsators, a new observational classification scheme is proposed by Grigahc\`ene et al. (2010). We present their results and characterize 234 stars in terms of {$\delta$} Sct, -{$\gamma$} Dor, {$\delta$} Sct/-{$\gamma$} Dor or -{$\gamma$} Dor/{$\delta$} Sct hybrids (\textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim) Copyright \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {Delta Scuti stars,Gamma Doradus stars,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/MIRQJHRK/Grigahcène et al. - 2010(2).pdf}
}

@article{Gruberbauer2013a,
  title = {Bayesian Asteroseismology of 23 Solar-like Kepler Targets},
  author = {Gruberbauer, M. and Guenther, D. B. and MacLeod, K. and Kallinger, T.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {435},
  number = {1},
  pages = {242--254},
  issn = {00358711},
  doi = {10.1093/mnras/stt1289},
  abstract = {We study 23 previously published Kepler targets to perform a consistent grid-based Bayesian asteroseismic analysis and compare our results to those obtained via the Asteroseismic Modelling Portal. We find differences in the derived stellar parameters of many targets and their uncertainties. While some of these differences can be attributed to systematic effects between stellar evolutionary models, we show that the different methodologies deliver incompatible uncertainties for some parameters. Using non-adiabatic models and our capability to measure surface effects, we also investigate the dependency of these surface effects on the stellar parameters. Our results suggest a dependence of the magnitude of the surface effect on the mixing length parameter which also, but only minimally, affects the determination of stellar parameters. While some stars in our sample show no surface effect at all, the most significant surface effects are found for stars that are close to the Sun's position in the Hertzsprung-Russell diagram. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {Methods: statistical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VRGQSD6T/Gruberbauer et al. - 2013.pdf}
}

@article{Gruberbauer2013c,
  title = {Bayesian Seismology of the {{Sun}}},
  author = {Gruberbauer, M. and Guenther, D. B.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {432},
  number = {1},
  eprint = {1303.3824},
  pages = {417--429},
  issn = {00358711},
  doi = {10.1093/mnras/stt477},
  abstract = {We perform a Bayesian grid-based analysis of the solar l = 0, 1, 2 and 3 p modes obtained viaBiSON in order to deliver the first Bayesian asteroseismic analysis of the solar compositionproblem. We do not find decisive evidence to prefer either of the contending chemical compositions,although the revised solar abundances (AGSS09) are more probable in general. Wedo find indications for systematic problems in standard stellar evolution models, unrelated tothe consequences of inadequate modelling of the outer layers on the higher order modes. Theseismic observables are best fitted by solar models that are several hundred million years olderthan the meteoritic age of the Sun. Similarly, meteoritic age calibrated models do not adequatelyreproduce the observed seismic observables. Our results suggest that these problemswill affect any asteroseismic inference that relies on a calibration to the Sun. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: abundances,Sun: fundamental parameters,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/IZF9H392/Gruberbauer, Guenther - 2013.pdf}
}

@article{Grundahl2008,
  title = {Stellar {{Oscillations Network Group}} - {{SONG}}},
  author = {Grundahl, F. and Arentoft, T. and {Christensen-Dalsgaard}, J. and Frandsen, S. and Kjeldsen, H. and Rasmussen, P. K.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012041},
  abstract = {The Stellar Oscillations Network Group (SONG) is an initiative which aims at designing and building a ground-based network of 1 m telescopes dedicated to the study of phenomena occurring in the time domain. In particular the study of stellar oscillations and the search for and characterisation of extra-solar planets. There will be eight identical nodes in the network, located at existing sites. Each node will have two instruments: 1) a high-resolution spectrograph for obtaining high precision radial velocities using an iodine cell as velocity reference - this will be the main instrument for asteroseismology because solar-like oscillations are much easier to detect in velocity than intensity; and 2) an optical imager which will be used for photometry and guiding. Detailed design of the network prototype node will begin in 2008, and a fully functioning and tested prototype will be ready by the end of 2011, with the goal of achieving a fully operational network around 2014. \textcopyright{} 2008 IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CJT64VMC/Grundahl et al. - 2008.pdf}
}

@article{Grundahl2011a,
  title = {{{SONG}} - {{Getting}} Ready for the Prototype},
  author = {Grundahl, F. and {Christensen-Dalsgaard}, J. and J{\o}rgensen, U. Gr{\aa}e and Frandsen, S. and Kjeldsen, H. and Rasmussen, P. Kj{\ae}rgaard},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012083},
  abstract = {The Stellar Observations Network Group, SONG, is a project which aims at building a network of eight identical telescopes distributed geographically around the globe to allow long-term, high-duty-cycle observations of stellar oscillations and to search for exoplanets via the microlensing technique. At each of the network nodes a 1 m telescope with a high-resolution spectrograph and two lucky-imaging cameras is placed. The instruments and telescope, for the prototype node, are currently being built and installation at Observatorio del Teide, Tenerife, Spain is foreseen for early 2011. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KP2QSJME/Grundahl et al. - 2011.pdf}
}

@article{guanDeepConvolutionalNeural2019,
  title = {Deep Convolutional Neural Network {{Inception-v3}} Model for Differential Diagnosing of Lymph Node in Cytological Images: A Pilot Study},
  author = {Guan, Qing and Wan, Xiaochun and Lu, Hongtao and Ping, Bo and Li, Duanshu and Wang, Li and Zhu, Yongxue and Wang, Yunjun and Xiang, Jun},
  year = {2019},
  month = jul,
  journal = {Annals of Translational Medicine},
  volume = {7},
  number = {14},
  pages = {307--307},
  publisher = {{AME Publishing Company}},
  issn = {23055839},
  doi = {10.21037/atm.2019.06.29},
  urldate = {2021-01-10},
  abstract = {Background: In this study, we exploited the Inception-v3 deep convolutional neural network (DCNN) model to differentiate cervical lymphadenopathy using cytological images. Method(s): A dataset of 80 cases was collected through the fine-needle aspiration (FNA) of enlarged cervical lymph nodes, which consisted of 20 cases of reactive lymphoid hyperplasia, 24 cases of non-Hodgkin's lymphoma (NHL), 16 cases of squamous cell carcinoma (SCC), and 20 cases of adenocarcinoma. The images were cropped into fragmented images and divided into a training dataset and a test dataset. Inception-v3 was trained to make differential diagnoses and then tested. The features of misdiagnosed images were further analysed to discover the features that may influence the diagnostic efficiency of such a DCNN. Result(s): A total of 742 original images were derived from the cases, from which a total of 7,934 fragmented images were cropped. The classification accuracies for the original images of reactive lymphoid hyperplasia, NHL, SCC and adenocarcinoma were 88.46\%, 80.77\%, 89.29\% and 100\%, respectively. The total accuracy on the test dataset was 89.62\%. Three fragmented images of reactive lymphoid hyperplasia and three fragmented images of SCC were misclassified as NHL. Three fragmented images of NHL were misclassified as reactive lymphoid hyperplasia, one was misclassified as SCC, and one was misclassified as adenocarcinoma. Conclusion(s): In summary, after training with a large dataset, the Inception-v3 DCNN model showed great potential in facilitating the diagnosis of cervical lymphadenopathy using cytological images. Analysis of the misdiagnosed cases revealed that NHL was the most challenging cytology type for DCNN to differentiate.Copyright \textcopyright{} Annals of Translational Medicine. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/F3TIMDBP/full-text.pdf}
}

@article{Guenther1993,
  title = {Evolution and Seismology of {{Procyon}}},
  author = {Guenther, David B. and Demarque, Pierre},
  year = {1993},
  journal = {The Astrophysical Journal},
  volume = {405},
  pages = {298--306},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4I3LKQU4/Guenther, Demarque - 1993.pdf}
}

@article{Guenther2007,
  title = {Searching for P-Modes in n {{Bo\"otis}} \& {{Procyon}} Using {{MOST}} Satellite Data},
  author = {Guenther, D. B.},
  year = {2007},
  journal = {Communications in Asteroseismology},
  volume = {151},
  pages = {5--25},
  issn = {1021-2043},
  doi = {10.1553/cia151s5},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TG6F7TCC/Guenther - 2007.pdf}
}

@article{Guerrero2019,
  title = {Global Simulations of {{Tayler}} Instability in Stellar Interiors: {{The}} Stabilizing Effect of Gravity},
  author = {Guerrero, G and Del Sordo, F and Bonanno, A and Smolarkiewicz, P K},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  eprint = {1909.02897},
  pages = {1--11},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz2849},
  abstract = {Unveiling the evolution of toroidal field instability, known as Tayler instability, is essential to understand the strength and topology of the magnetic fields observed in early-type stars, in the core of the red giants, or in any stellar radiative zone. We want to study the non-linear evolution of the instability of a toroidal field stored in a stably stratified layer, in spherical symmetry and in the absence of rotation. In particular, we intend to quantify the suppression of the instability as a function of the Brunt-V\~A\textcurrency is\~A\textcurrency la ({$\omega$}BV) and the Alfv\~A\textcopyright n ({$\omega$}A) frequencies. We use the MHD equations as implemented in the anelastic approximation in the EULAG-MHD code and perform a large series of numerical simulations of the instability exploring the parameter space for the {$\omega$}BV and {$\omega$}A. We show that beyond a critical value gravity strongly suppress the instability, in agreement with the linear analysis. The intensity of the initial field also plays an important role: weaker fields show much slower growth rates. Moreover, in the case of very low gravity, the fastest growing modes have a large characteristic radial scale, at variance with the case of strong gravity, where the instability is characterized by horizontal displacements. Our results illustrate that the anelastic approximation can efficiently describe the evolution of toroidal field instability in stellar interiors. The suppression of the instability as a consequence of increasing values of {$\omega$}BV might play a role to explain the magnetic desert in Ap/Bp stars, since weak fields are only marginally unstable in the case of strong gravity.},
  archiveprefix = {arxiv},
  keywords = {magnetic fields,notion,notion-database,numerical simulations,stellar evolution},
  file = {/Users/lbugnet/Zotero/storage/ZTY7FC27/Guerrero et al. - 2019.pdf}
}

@article{Guggenberger2012a,
  title = {The Complex Case of {{V445 Lyr}} Observed with {{Kepler}}: {{Two Blazhko}} Modulations, a Non-Radial Mode, Possible Triple Mode {{RR Lyrae}} Pulsation, and More},
  author = {Guggenberger, E. and Kolenberg, K. and Nemec, J. M. and Smolec, R. and Benko, J. M. and Ngeow, C. C. and Cohen, J. G. and Sesar, B. and Szab{\'o}, R. and Catelan, M. and Moskalik, P. and Kinemuchi, K. and Seader, S. E. and Smith, J. C. and Tenenbaum, P. and Kjeldsen, H.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {424},
  number = {1},
  eprint = {1205.1344},
  pages = {649--665},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.21244.x},
  abstract = {Rapid and strong changes in the Blazhko modulation of RR Lyrae stars, as have recently been detected in high-precision satellite data, have become a crucial topic in finding an explanation of the long-standing mystery of the Blazhko effect. We present here an analysis of the most extreme case detected so far, the RRab star V445 Lyr (KIC 6186029) which was observed with the Kepler space mission. V445 Lyr shows very strong cycle-to-cycle changes in its Blazhko modulation, which are caused by both a secondary long-term modulation period and irregular variations. In addition to the complex Blazhko modulation, V445 Lyr also shows a rich spectrum of additional peaks in the frequency range between the fundamental pulsation and the first harmonic. Among those peaks, the second radial overtone could be identified, which, combined with a metallicity estimate of [Fe/H] =-2.0 dex from spectroscopy, allowed us to constrain the mass (0.55-0.65 M {$\odot$}) and luminosity (40-50 L {$\odot$}) of V445 Lyr through theoretical Petersen diagrams. A non-radial mode and possibly the first overtone are also excited. Furthermore, V445 Lyr shows signs of the period-doubling phenomenon and a long-term period change. A detailed Fourier analysis along with a study of the O - C variation of V445 Lyr is presented, and the origin of the additional peaks and possible causes of the changes in the Blazhko modulation are discussed. The results are then put into context with those of the only other star with a variable Blazhko effect for which a long enough set of high-precision continuous satellite data has been published so far, the CoRoT star 105288363. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: individual: CoRoT 105288363,Stars: individual: KIC 6186029 (V445 Lyr),Stars: variables: RR Lyrae,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/GLV82FNK/Guggenberger et al. - 2012.pdf}
}

@article{Guggenberger2016a,
  title = {Significantly Improving Stellar Mass and Radius Estimates: {{A}} New Reference Function for the {{$\Delta\nu$}} Scaling Relation},
  author = {Guggenberger, Elisabeth and Hekker, Saskia and Basu, Sarbani and Bellinger, Earl},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {460},
  number = {4},
  eprint = {1606.01917},
  pages = {4277--4281},
  issn = {13652966},
  doi = {10.1093/mnras/stw1326},
  abstract = {The scaling relations between global asteroseismic observables and stellar properties are widely used to estimate masses and radii of stars exhibiting solar-like oscillations. Since the mass and radius of the Sun are known independently, the Sun is commonly used as a reference to scale to. However, the validity of the scaling relations depends on the homology between the star under study and the reference star. Solar-like oscillators span a wide range of masses and metallicities, as well as evolutionary phases. Most of these stars are therefore not homologous to the Sun. This leads to errors of up to 10 per cent (5 per cent) in mass (radius) when using the asteroseismic scaling relations with the Sun as the reference. In this paper, we derive a reference function to replace the solar-reference value used in the large-frequency separation scaling relation. Our function is the first that depends on both effective temperature and metallicity, and is applicable from the end of the main sequence to just above the bump on the red giant branch. This reference function improves the estimates of masses and radii determined through scaling relations by a factor of 2, i.e. allows masses and radii to be recovered with an accuracy of 5 per cent and 2 per cent, respectively.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: fundamental parameters,Stars: general,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/GW96JIPL/Guggenberger et al. - 2016.pdf}
}

@article{Guillot2002,
  title = {Evolution of "51 {{Pegasus}} b-like" Planets},
  author = {Guillot, T. and Showman, A. P.},
  year = {2002},
  month = apr,
  journal = {Astronomy and Astrophysics},
  volume = {385},
  number = {1},
  eprint = {astro-ph/0202234},
  pages = {156--165},
  publisher = {{EDP Sciences}},
  issn = {00046361},
  doi = {10.1051/0004-6361:20011624},
  urldate = {2020-03-23},
  abstract = {About one-quarter of the extrasolar giant planets discovered so far have orbital distances smaller than 0.1 AU. These "51 Peg b-like" planets can now be directly characterized, as shown by the planet transiting in front the star HD 209458. We review the processes that affect their evolution. We apply our work to the case of HD 209458b, whose radius has been recently measured. We argue that its radius can be reproduced only when the deep atmosphere is assumed to be unrealistically hot. When using more realistic atmospheric temperatures, an energy source appears to be missing in order to explain HD 209458b's large size. The most likely source of energy available is not in the planet's spin or orbit, but in the intense radiation received from the parent star. We show that the radius of HD 209458b can be reproduced if a small fraction ({$\sim$}1\%) of the stellar flux is transformed into kinetic energy in the planetary atmosphere and subsequently converted to thermal energy by dynamical processes at pressures of tens of bars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planets and satellites: general,{Stars: individual: 51 Peg, HD 209458},Stars: planetary systems},
  file = {/Users/lbugnet/Zotero/storage/XCS2JMJU/full-text.pdf}
}

@article{Guillot2005,
  title = {{{THE INTERIORS OF GIANT PLANETS}}: {{Models}} and {{Outstanding Questions}}},
  author = {Guillot, Tristan},
  year = {2005},
  month = may,
  journal = {Annual Review of Earth and Planetary Sciences},
  volume = {33},
  number = {1},
  eprint = {astro-ph/0502068},
  pages = {493--530},
  publisher = {{Annual Reviews}},
  issn = {0084-6597},
  doi = {10.1146/annurev.earth.32.101802.120325},
  urldate = {2020-03-23},
  abstract = {We know that giant planets played a crucial role in the making of our Solar System. The discovery of giant planets orbiting other stars is a formidable opportunity to learn more about these objects, what is their composition, how various processes influence their structure and evolution, and most importantly how they form. Jupiter, Saturn, Uranus and Neptune can be studied in detail, mostly from close spacecraft flybys. We can infer that they are all enriched in heavy elements compared to the Sun, with the relative global enrichments increasing with distance to the Sun. We can also infer that they possess dense cores of varied masses. The intercomparison of presently caracterised extrasolar giant planets show that they are also mainly made of hydrogen and helium, but that they either have significantly different amounts of heavy elements, or have had different orbital evolutions, or both. Hence, many questions remain and are to be answered for significant progresses on the origins of planets.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database}
}

@article{Guzik2000,
  title = {Driving the {{Gravity-Mode Pulsations}} in {$\gamma$} {{Doradus Variables}}},
  author = {Guzik, Joyce A. and Kaye, Anthony B. and Bradley, Paul A. and Cox, Arthur N. and Neuforge, Corinne},
  year = {2000},
  month = oct,
  journal = {The Astrophysical Journal},
  volume = {542},
  number = {1},
  pages = {L57-L60},
  publisher = {{American Astronomical Society}},
  issn = {0004637X},
  doi = {10.1086/312908},
  urldate = {2020-11-29},
  abstract = {The {$\gamma$} Doradus stars are a newly discovered class of gravity-mode pulsators that lie just at or beyond the red edge of the {$\delta$} Scuti instability strip. We present the results of calculations that the predict pulsation instability of high-order g-modes with periods between 0.4 and 3 days, as observed in these stars. The pulsations are driven by the modulation of the radiative flux by convection at the base of a deep envelope convection zone. Pulsation instability is predicted only for models with temperatures at the convection zone base between {$\sim$}200,000 and {$\sim$}480,000 K. The estimated shear dissipation that is due to turbulent viscosity within the convection zone or in an overshoot region below the convection zone can be comparable to or even exceed the predicted driving and is likely to reduce the number of unstable modes or possibly quench the instability. Additional refinements in the pulsation modeling are required to determine the outcome. At least one {$\gamma$} Doradus star has been observed that also pulsates in {$\delta$} Scuti-type p-modes, and others have been identified as chemically peculiar. Since our calculated driving region is relatively deep, {$\gamma$} Doradus pulsations are not necessarily incompatible with surface abundance peculiarities or with {$\delta$} Scuti p-mode pulsations driven by the H and He ionization {$\kappa$}-effect. Such stars will provide useful observational constraints on the proposed {$\gamma$} Doradus pulsation mechanism.},
  keywords = {notion,notion-database,oscillations-stars,other,stars,Subject headings,variables},
  file = {/Users/lbugnet/Zotero/storage/INDNMJJN/full-text.pdf}
}

@article{Guzik2005a,
  title = {Can {{Enhanced Diffusion Improve Helioseismic Agreement}} for {{Solar Models}} with {{Revised Abundances}}?},
  author = {Guzik, Joyce A. and Watson, L. Scott and Cox, Arthur N.},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {627},
  number = {2},
  pages = {1049--1056},
  issn = {0004-637X},
  doi = {10.1086/430438},
  abstract = {Recent solar photospheric abundance analyses (by Asplund et al. and Lodders) revise the C, N, O, Ne, and Ar abundances downward by 0.15-0.2 dex compared to previous determinations by Grevesse \& Sauval. The abundances of Fe and other elements are reduced by smaller amounts, 0.05-0.1 dex. With these revisions, the photospheric Z / X decreases to 0.0165 (or 0.0177, according to Lodders), and Z decreases to \textasciitilde 0.0122 (or 0.0133, according to Lodders). A number of papers (by, e.g., Basu \& Antia, Montalban et al., Bahcall \& Pinsonneault, Turck-Chi{$\surd\circledR$}ze et al., and Antia \& Basu) report that solar models evolved with standard opacities and diffusion treatment using these new abundances give poor agreement with helioseismic inferences for sound-speed and density profile, convection-zone helium abundance, and convection-zone depth. These authors also considered a limited set of models with increased opacities, enhanced diffusion, or abundance variations to improve agreement, finding no entirely satisfactory solution. Here we explore evolved solar models with varying diffusion treatments, including enhanced diffusion with separate multipliers for helium and other elements, to reduce the photospheric abundances, while keeping the interior abundances about the same as earlier standard models. While enhanced diffusion improves agreement with some helioseismic constraints compared to a solar model evolved with the new abundances using nominal input physics, the required increases in thermal diffusion rates are unphysically large, and none of the variations tried completely restores the good agreement attained using the earlier abundances. A combination of modest opacity increases, diffusion enhancements, and abundance increases near the level of the uncertainties, while somewhat contrived, remains the most physically plausible means to restore agreement with helioseismology. The case for enhanced diffusion would be improved if the inferred convection-zone helium abundance could be reduced; we recommend reconsidering this derivation in light of new equations of state with modified abundances and other improvements. We also recommend considering, as a last resort, diluting the convection zone, which contains only 2.5\% of the Sun's mass, by accretion of material depleted in the more volatile elements C, N, O, Ne, and Ar after the Sun arrived on the main sequence.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4NMY2YNA/Guzik, Watson, Cox - 2005.pdf}
}

@article{Guzik2016a,
  title = {Detection of {{Solar-Like Oscillations}}, {{Observational Constraints}}, and {{Stellar Models}} for {{$\Theta$ Cyg}}, the {{Brightest Star Observed By}} the {{Kepler Mission}}},
  author = {Guzik, J. A. and Houdek, G. and Chaplin, W. J. and Smalley, B. and Kurtz, D. W. and Gilliland, R. L. and Mullally, F. and Rowe, J. F. and Bryson, S. T. and Still, M. D. and Antoci, V. and Appourchaux, T. and Basu, S. and Bedding, T. R. and Benomar, O. and Garcia, R. A. and Huber, D. and Kjeldsen, H. and Latham, D. W. and Metcalfe, T. S. and P{\'a}pics, P. I. and White, T. R. and Aerts, C. and Ballot, J. and Boyajian, T. S. and Briquet, M. and Bruntt, H. and Buchhave, L. A. and Campante, T. L. and Catanzaro, G. and {Christensen-Dalsgaard}, J. and Davies, G. R. and Do{\u g}an, G. and Dragomir, D. and Doyle, A. P. and Elsworth, Y. and Frasca, A. and Gaulme, P. and Gruberbauer, M. and Handberg, R. and Hekker, S. and Karoff, C. and Lehmann, H. and Mathias, P. and Mathur, S. and Miglio, A. and {Molenda-{\.Z}akowicz}, J. and Mosser, B. and Murphy, S. J. and R{\'e}gulo, C. and Ripepi, V. and Salabert, D. and Sousa, S. G. and Stello, D. and Uytterhoeven, K.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {831},
  number = {1},
  pages = {17},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/831/1/17},
  abstract = {\textcopyright{} 2016. The American Astronomical Society. All rights reserved.. \texttheta{} Cygni is an F3 spectral type magnitude V = 4.48 main-sequence star that was the brightest star observed by the original Kepler spacecraft mission. Short-cadence (58.8 s) photometric data using a custom aperture were first obtained during Quarter 6 (2010 June-September) and subsequently in Quarters 8 and 12-17. We present analyses of solar-like oscillations based on Q6 and Q8 data, identifying angular degree l = 0, 1, and 2 modes with frequencies of 1000-2700 {$\mu$}Hz, a large frequency separation of 83.9 {$\pm$} 0.4 {$\mu$}Hz, and maximum oscillation amplitude at frequency {$\nu$} max = 1829 {$\pm$} 54 {$\mu$}Hz. We also present analyses of new ground-based spectroscopic observations, which, combined with interferometric angular diameter measurements, give T eff = 6697 {$\pm$} 78 K, radius 1.49 {$\pm$} 0.03 R o , [Fe/H] = -0.02 {$\pm$} 0.06 dex, and log g = 4.23 {$\pm$} 0.03. We calculate stellar models matching these constraints using the Yale Rotating Evolution Code and the Asteroseismic Modeling Portal. The best-fit models have masses of 1.35-1.39 M o and ages of 1.0-1.6 Gyr. \texttheta{} Cyg's T eff and log g place it cooler than the red edge of the {$\gamma$} Doradus instability region established from pre-Kepler ground-based observations, but just at the red edge derived from pulsation modeling . The pulsation models show {$\gamma$} Dor gravity modes driven by the convective blocking mechanism, with frequencies of 1-3 cycles per day (11 to 33 {$\mu$}Hz). However, gravity modes were not seen in Kepler data; one signal at 1.776 cycles per day (20.56 {$\mu$}Hz) may be attributable to a faint, possibly background, binary.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/7JLM28ZV/Guzik et al. - 2016.pdf}
}

@article{Haas2010a,
  title = {Kepler Science Operations},
  author = {Haas, Michael R. and Batalha, Natalie M. and Bryson, Steve T. and Caldwell, Douglas A. and Dotson, Jessie L. and Hall, Jennifer and Jenkins, Jon M. and Klaus, Todd C. and Koch, David G. and Kolodziejczak, Jeffrey and Middour, Chris and Smith, Marcie and Sobeck, Charles K. and Stober, Jeremy and Thompson, Richard S. and Van Cleve, Jeffrey E.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  pages = {1--10},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L115},
  abstract = {Kepler's mission design includes a comprehensive plan for commissioning and science operations. The commissioning phase completed all critical tasks and accomplished all mission objectives within a week of the pre-launch plan. Since the start of science data collection, the nominal timeline has been interrupted by two safe-mode events, several losses of fine point, and some small pointing adjustments. The most important anomalies are understood and mitigated, so Kepler's technical performance has improved significantly over this period, and the prognosis for mission success is excellent. The Kepler data archive is established and hosting data for the science team, guest observers, and the public. The first data to become publicly available include the monthly full-frame images and the light curves for targets that are dropped from the exoplanet program or released after publication. Data are placed in the archive on a quarterly basis; the Kepler Results Catalog will be released annually starting in 2011. \textcopyright{} 2010. The American Astronomical Society.},
  keywords = {notion,notion-database,Space vehicles: instruments,Telescopes},
  file = {/Users/lbugnet/Zotero/storage/THGUBYQU/Haas et al. - 2010.pdf}
}

@article{Hale2016,
  title = {Performance of the {{Birmingham Solar-Oscillations Network}} ({{BiSON}})},
  author = {Hale, S. J. and Howe, R. and Chaplin, W. J. and Davies, G. R. and Elsworth, Y. P.},
  year = {2016},
  journal = {Solar Physics},
  volume = {291},
  number = {1},
  pages = {1--28},
  publisher = {{The Author(s)}},
  issn = {1573093X},
  doi = {10.1007/s11207-015-0810-0},
  abstract = {The Birmingham Solar-Oscillations Network (BiSON) has been operating with a full complement of six stations since 1992. Over 20 years later, we look back on the network history. The meta-data from the sites have been analysed to assess performance in terms of site insolation, with a brief look at the challenges that have been encountered over the years. We explain how the international community can gain easy access to the ever-growing dataset produced by the network, and finally look to the future of the network and the potential impact of nearly 25 years of technology miniaturisation.},
  keywords = {{Helioseismology, observations},notion,notion-database,{Oscillations, solar}},
  file = {/Users/lbugnet/Zotero/storage/QXZHWUUQ/Hale et al. - 2016.pdf}
}

@article{Hall2005,
  title = {Stellar Chromospheric Activity},
  author = {Hall, Jeffrey C.},
  year = {2005},
  journal = {Living Reviews in Solar Physics},
  volume = {5},
  number = {1},
  pages = {2},
  issn = {16144961},
  doi = {10.12942/lrsp-2008-2},
  urldate = {2020-07-02},
  abstract = {The Sun, stars similar to it, and many rather dissimilar to it, have chromospheres, regions classically viewed as lying above the brilliant photosphere and characterized by a positive temperature gradient and a marked departure from radiative equilibrium. Stellar chromospheres exhibit a wide range of phenomena collectively called activity, stemming largely from the time evolution of their magnetic fields and the mass flux and transfer of radiation through the complex magnetic topology and the increasingly optically thin plasma of the outer stellar atmosphere. In this review, I will (1) outline the development of our understanding of chromospheric structure from 1960 to the present, (2) discuss the major observational programs and theoretical lines of inquiry, (3) review the origin and nature of both solar and stellar chromospheric activity and its relationship to, and effect on, stellar parameters including total energy output, and (4) summarize the outstanding problems today.},
  keywords = {notion,notion-database,Stars: chromospheres,Sun},
  file = {/Users/lbugnet/Zotero/storage/TGZ538QB/full-text.pdf}
}

@article{Hambleton2013a,
  title = {{{KIC}} 4544587: {{An}} Eccentric, Short-Period Binary System with {$\delta$} {{Sct}} Pulsations and Tidally Excited Modes},
  author = {Hambleton, K. M. and Kurtz, D. W. and Pr{\v s}a, A. and Guzik, J. A. and Pavlovski, K. and Bloemen, S. and Southworth, J. and Conroy, K. and Littlefair, S. P. and Fuller, J.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {434},
  number = {2},
  pages = {925--940},
  issn = {00358711},
  doi = {10.1093/mnras/stt886},
  abstract = {We present Kepler photometry and ground-based spectroscopy of KIC 4544587, a short-period eccentric eclipsing binary system with self-excited pressure and gravity modes, tidally excited modes, tidally influenced p modes and rapid apsidal motion of 182 yr per cycle. The primary and secondary components of KIC 4544587 reside within the d Scuti and {$\gamma$} Dor instability region of the Hertzsprung-Russell diagram, respectively. By applying the binary modelling software PHOEBE to prewhitenedKepler photometric data and radial velocity data obtained using the William Herschel Telescope and 4-m Mayall telescope at Kitt Peak Northern Observatory (KPNO), the fundamental parameters of this important system have been determined, including the stellarmasses, 1.98{$\pm$}0.07 and 1.60{$\pm$}0.06 M{$\odot$}, and radii, 1.76{$\pm$}0.03 and 1.42{$\pm$}0.02R{$\odot$}, for the primary and secondary components, respectively. Frequency analysis of the residual data revealed 31 modes, 14 in the gravity mode region and 17 in the pressure mode region. Of the 14 gravity modes, 8 are orbital harmonics: a signature of tidal resonance. While the measured amplitude of these modes may be partially attributed to residual signal from binary model subtraction, we demonstrate through consideration of the folded light curve that these frequencies do in fact correspond to tidally excited pulsations. Furthermore, we present an echelle diagram of the pressure mode frequency region (modulo the orbital frequency) and demonstrate that the tides are also influencing the p modes. A first look at asteroseismology hints that the secondary component is responsible for the p modes, which is contrary to our expectation that the hotter star should pulsate in higher radial overtone, higher frequency p modes. \textcopyright 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {Binaries:eclipsing,notion,notion-database,Stars: individual: KIC 4544587,Stars: oscillations,Stars: variables: d Scuti.},
  file = {/Users/lbugnet/Zotero/storage/TW598FIN/Hambleton et al. - 2013.pdf}
}

@article{Han2002,
  title = {The Origin of Subdwarf {{B}} Stars - {{I}}. {{The}} Formation Channels},
  author = {Han, Z. and Podsiadlowski, {\relax Ph}. and Maxted, P. F. L. and Marsh, T. R. and Ivanova, N.},
  year = {2002},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {336},
  pages = {449--466},
  issn = {0035-8711},
  doi = {10.1046/j.1365-8711.2002.05752.x},
  urldate = {2023-10-02},
  abstract = {Subdwarf B (sdB) stars (and related sdO/sdOB stars) are believed to be helium-core-burning objects with very thin hydrogen-rich envelopes. In recent years it has become increasingly clear from observational surveys that a large fraction of these objects are members of binary systems. To understand their formation better, we present the results of a detailed investigation of the three main binary evolution channels that can lead to the formation of sdB stars: the common-envelope (CE) ejection channel, the stable Roche lobe overflow (RLOF) channel, and the double helium white dwarfs (WDs) merger channel. The CE ejection channel leads to the formation of sdB stars in short-period binaries with typical orbital periods between 0.1 and 10 d, very thin hydrogen-rich envelopes and a mass distribution sharply peaked around {$\sim$}0.46 M{$\odot$}. On the other hand, under the assumption that all mass transferred is soon lost, the stable RLOF channel produces sdB stars with similar masses but long orbital periods (400-1500 d) and with rather thick hydrogen-rich envelopes. The merger channel gives rise to single sdB stars whose hydrogen-rich envelopes are extremely thin but which have a fairly wide distribution of masses (0.4-0.65 M{$\odot$}). We obtained the conditions for the formation of sdB stars from each of these channels using detailed stellar and binary evolution calculations where we modelled the detailed evolution of sdB stars and carried out simplified binary population synthesis simulations. The observed period distribution of sdB stars in compact binaries strongly constrains the CE ejection parameters. The best fits to the observations are obtained for very efficient CE ejection where the envelope ionization energy is included, consistent with previous results. We also present the distribution of sdB stars in the Teff-log g diagram, the Hertzsprung-Russell diagram and the distribution of mass functions.},
  keywords = {Astrophysics},
  annotation = {ADS Bibcode: 2002MNRAS.336..449H},
  file = {/Users/lbugnet/Zotero/storage/FEP2FX9X/Han et al. - 2002 - The origin of subdwarf B stars - I. The formation .pdf}
}

@article{Handberg2011a,
  title = {Bayesian Peak-Bagging of Solar-like Oscillators Using {{MCMC}}: {{A}} Comprehensive Guide},
  author = {Handberg, R. and Campante, T. L.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {527},
  number = {7},
  pages = {1--12},
  issn = {00046361},
  doi = {10.1051/0004-6361/201015451},
  abstract = {Context. Asteroseismology has entered a new era with the advent of the NASA Kepler mission. Long and continuous photometric observations of unprecedented quality are now available which have stimulated the development of a number of suites of innovative analysis tools. Aims. The power spectra of solar-like oscillations are an inexhaustible source of information on stellar structure and evolution. Robust methods are hence needed in order to infer both individual oscillation mode parameters and parameters describing non-resonant features, thus making a seismic interpretation possible. Methods. We present a comprehensive guide to the implementation of a Bayesian peak-bagging tool that employs a Markov chain Monte Carlo (MCMC). Besides making it possible to incorporate relevant prior information through Bayes' theorem, this tool also allows one to obtain the marginal probability density function for each of the fitted parameters. We apply this tool to a couple of recent asteroseismic data sets, namely, to CoRoT observations of HD 49933 and to ground-based observations made during a campaign devoted to Procyon. Results. The developed method performs remarkably well at constraining not only in the traditional case of extracting oscillation frequencies, but also when pushing the limit where traditional methods have difficulties. Moreover it provides an rigorous way of comparing competing models, such as the ridge identifications, against the asteroseismic data. \textcopyright{} 2011 ESO.},
  keywords = {methods: data analysis,methods: statistical,notion,notion-database,stars: late-type,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ELIL9RFF/Handberg, Campante - 2011.pdf}
}

@article{Handberg2014a,
  title = {Automated Preparation of {{Kepler}} Time Series of Planet Hosts for Asteroseismic Analysis},
  author = {Handberg, R. and Lund, M. N.},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {445},
  number = {3},
  pages = {2698--2709},
  issn = {13652966},
  doi = {10.1093/mnras/stu1823},
  abstract = {One of the tasks of the Kepler Asteroseismic Science Operations Center (KASOC) is to provide asteroseismic analyses on Kepler Objects of Interest. However, asteroseismic analysis of planetary host stars presents some unique complications with respect to data pre-processing, compared to pure asteroseismic targets. If not accounted for, the presence of planetary transits in the photometric time series often greatly complicates or even hinders these asteroseismic analyses. This drives the need for specialized methods of pre-processing data to make them suitable for asteroseismic analysis. In this paper, we present the KASOC filter, which is used to automatically prepare data from the Kepler/K2 mission for asteroseismic analyses of solar-like planet host stars. The methods are very effective at removing unwanted signals of both instrumental and planetary origins and produce significantly cleaner photometric time series than the original data. The methods are automated and can therefore easily be applied to a large number of stars. The application of the filter is not restricted to planetary hosts, but can be applied to any solar-like or red giant stars observed by Kepler/K2.},
  keywords = {Methods: data analysis,notion,notion-database,Planetary systems,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/PNS9TGC5/Handberg, Lund - 2014.pdf}
}

@article{Handberg2017,
  title = {{{NGC6819}}: {{Testing}} the Asteroseismic Mass Scale, Mass Loss and Evidence for Products of Non-Standard Evolution},
  author = {Handberg, R. and Brogaard, K. and Miglio, A. and Bossini, D. and Elsworth, Y. and Slumstrup, D. and Davies, G. R. and Chaplin, W. J.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {472},
  number = {1},
  eprint = {1707.08223},
  issn = {13652966},
  doi = {10.1093/MNRAS/STX1929},
  abstract = {We present an extensive peakbagging effort on Kepler data of \textasciitilde 50 red giant stars in the open star cluster NGC6819. By employing sophisticated pre-processing of the time series and Markov chain Monte Carlo techniques we extracted individual frequencies, heights and line widths for hundreds of oscillation modes.We show that the 'average' asteroseismic parameter {$\delta$}v02, derived from these, can be used to distinguish the stellar evolutionary state between the red giant branch (RGB) stars and red clump (RC) stars. Masses and radii are estimated using asteroseismic scaling relations, both empirically corrected to obtain self-consistency and agreement with independent measures of distance, and using updated theoretical corrections. Remarkable agreement is found, allowing the evolutionary state of the giants to be determined exclusively from the empirical correction to the scaling relations. We find a mean mass of the RGB stars and RC stars in NGC6819 to be 1.61 {$\pm$} 0.02 and 1.64 {$\pm$} 0.02M{$\odot$}, respectively. The difference {$\Delta$}M=-0.03 {$\pm$} 0.01M{$\odot$} is almost insensitive to systematics, suggesting very little RGB mass loss, if any. Stars that are outliers relative to the ensemble reveal overmassive members that likely evolved via mass transfer in a blue straggler phase. We suggest that KIC 4937011, a low-mass Li-rich giant, is a cluster member in the RC phase that experienced very high mass loss during its evolution. Such over- and undermassive stars need to be considered when studying field giants, since the true age of such stars cannot be known and there is currently no way to distinguish them from normal stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Handler2012a,
  title = {A Multisite Photometric Study of Two Unusual {$\beta$} {{Cep}} Stars: {{The}} Magnetic {{V2052 Oph}} and the Massive Rapid Rotator {{V986 Oph}}},
  author = {Handler, G. and Shobbrook, R. R. and Uytterhoeven, K. and Briquet, M. and Neiner, C. and Tshenye, T. and Ngwato, B. and {van Winckel}, H. and Guggenberger, E. and Raskin, G. and Rodr{\'i}guez, E. and Mazumdar, A. and Barban, C. and Lorenz, D. and Vandenbussche, B. and {\c S}ahin, T. and Medupe, R. and Aerts, C.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {424},
  number = {3},
  pages = {2380--2391},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.21414.x},
  abstract = {We report a multisite photometric campaign for the {$\beta$} Cep stars V2052 Oph and V986 Oph. 670h of high-quality differential photoelectric Str\"omgren, Johnson and Geneva time-series photometry was obtained with eight telescopes on five continents during 182 nights. Frequency analyses of the V2052 Oph data enabled the detection of three pulsation frequencies, the first harmonic of the strongest signal, and the rotation frequency with its first harmonic. Pulsational mode identification from analysing the colour amplitude ratios confirms the dominant mode as being radial, whereas the other two oscillations are most likely l = 4. Combining seismic constraints on the inclination of the rotation axis with published magnetic field analyses we conclude that the radial mode must be the fundamental mode. The rotational light modulation is in phase with published spectroscopic variability, and consistent with an oblique rotator for which both magnetic poles pass through the line of sight. The inclination of the rotation axis is 54\textdegree{} {$<$} i {$<$} 58\textdegree{} and the magnetic obliquity 58\textdegree{} {$<$} {$\beta$} {$<$} 66\textdegree. The possibility that V2052 Oph has a magnetically confined wind is discussed. The photometric amplitudes of the single oscillation of V986 Oph are most consistent with an l = 3 mode, but this identification is uncertain. Additional intrinsic, apparently temporally incoherent light variations of V986 Oph are reported. Different interpretations thereof cannot be distinguished at this point, but this kind of variability appears to be present in many OB stars. The prospects of obtaining asteroseismic information for more rapidly rotating {$\beta$} Cep stars, which appear to prefer modes of higher l, are briefly discussed. \textcopyright{} 2012 The Authors. Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {notion,notion-database,Stars: early-type,Stars: individual: V2052 Oph,Stars: individual: V986 Oph,Stars: magnetic field,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/MAK4UNGU/Handler et al. - 2012.pdf}
}

@article{Hanson2022,
  title = {Discovery of High-Frequency Retrograde Vorticity Waves in the {{Sun}}},
  author = {Hanson, Chris S. and Hanasoge, Shravan and Sreenivasan, Katepalli R.},
  year = {2022},
  journal = {Nature Astronomy},
  keywords = {notion,notion-database}
}

@incollection{Harmonics2012a,
  title = {Chapter 5: {{Spherical}} Harmonics},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  year = {2012},
  number = {October},
  pages = {3--5},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5KM6D3Z6/Unknown - 2012.pdf}
}

@inproceedings{Harper2018,
  title = {Science with an {{ngVLA}}: {{Stellar Activity}} on {{Red Giant}} and {{Supergiant Stars}}: {{Mass Loss}} and the {{Evolution}} of the {{Stellar Dynamo}}},
  booktitle = {{{ASP Conference Series}}},
  author = {Harper, Graham M},
  year = {2018},
  eprint = {1810.09353v1},
  urldate = {2020-05-22},
  abstract = {In this Chapter we examine the role of the ngVLA to further our understanding of the different manifestations of convective or turbulence-driven stellar activity on red giant and supergiant stars. The combination of high spatial resolution and high sensitivity will enable the ngVLA to significantly improve our understanding of the processes that dissipate energy in the extended atmospheres of cool evolved stars, and drive ubiquitous stellar outflows. The high spatial resolution will enable us to image the surfaces of nearby red supergiants, and to measure the atmospheric extent of red giants. Multi-frequency observations will permit thermal continuum tomography on the largest angular diameter stars, providing key empirical data to test theoretical models. The complementary frequencies and similar spatial resolutions of the ngVLA and ALMA will be a powerful synergy. 1. Context Cool stars have vigorous sub-photospheric convection zones that lead to turbulent motions in their photospheres, and in the layers above. The interaction of surface magnetic fields (e.g., Auri\'ere et al. 2015) and dynamic ionized plasma leads to complex phenomena including starspots, active regions, chromospheres, and stellar outflows. These manifestations of Stellar Activity (Schrijver \& Zwaan 2000) are not well understood but have important astrophysical consequences, ranging from the effects of mass loss on galactic structure and chemical evolution, the nature of space-weather for exo-planets orbiting red giants, to the effects of cool supergiant mass-loss history on the interpretation of early-time supernovae spectra (e.g., Dessart et al. 2017). Theoretical models have not been able to reproduce observational signatures of stellar activity, and progress is being led by state-of-the-art observations made at the highest spatial resolution and with the greatest sensitivity. Thermal radio continuum observations are powerful diagnostics in this context because the atomic cross-sections are very accurately known (Hummer 1988) and the emission source term is the Planck function, which is linear in electron temperature. For example, resolved VLA images provided a ground breaking discovery and new insights into red supergiant (RSG) outflows with the finding by Lim et al. (1998) that Betel-geuse's extended atmosphere is cooler and much less ionized than predicted by leading theoretical and semi-empirical models of the time (see Hartmann \& Avrett 1984; Harper et al. 2001).},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/P64QVMNN/full-text.pdf}
}

@article{Hart1954,
  title = {{{MOTIONS IN THE SUN AT THE PHOTO SPHERIC LEVEL IV}}. {{The}} Equatorial Rotation and Possible Velocity Fields {{IN THE PHOTOSPHERE}}},
  author = {Hart, A B},
  year = {1954},
  journal = {MNRAS},
  volume = {114},
  urldate = {2020-03-15},
  abstract = {From spectra of the equatorial photosphere taken near the limb of the Sun between 1950 October and 1952 June, 480 determinations of line-of-sight velocity are made. A careful investigation shows, contrary to an earlier suggestion, that the effect on velocities, of light scattered in the Earth's atmosphere and in the telescope, is negligible. In order that each day on which observations are made should carry equal weight in the final solution, only 334 of the determinations are used to find the mean equatorial velocity. After the elimination of limb effect, the velocity due to solar rotation is found to be 1*91 km sec-1 for the mean epoch 1951*5. The individual determinations have a large dispersion about this mean and a statistical discussion shows that the chance is less than one in a thousand that the dispersion is due to errors of measurement. It is therefore highly probable that the velocity varies from point to point in the photosphere. The extreme range in measured velocity is approximately 0*3 km sec-1 and successive maxima or minima of velocity appear to be separated by a distance of the order of 75 000 km. Some evidence is found for bands of constant velocity occurring perpendicular to the solar equator, but this is less certain. The existence of such velocity changes may account for the discrepant rates of rotation found by earlier observers. Introduction.-From visual measures of Doppler displacements, Dun\'er (5) in 1888 made the first spectroscopic determination of solar rotation. The potential accuracy of the method and its applicability to all solar latitudes gave grounds for the belief that the determination of rotation by sunspots would soon be superseded. Discrepant results were, however, obtained by photographic spectroscopy between 1906 and 1913, and since 1915 investigations have been restricted to a determination of equatorial velocity in the hope of elucidating the causes of these discrepancies. Adams (2) at Mt. Wilson between 1906 and 1908 made the first photographic measures and laid the foundations of a method used by many later investigators. Working in the wavelength region 4250 A with a solar image 170 mm in diameter and a dispersion of 0*71 or 0-56 A mm-1 , he used two small prisms to bring light from opposite limbs of the Sun into juxtaposition on the slit of the spectroscope. Half the displacement between the same spectral line on the two limbs gave the value of the rotation. The spectra were measured with an ordinary cross-wire micrometer. This procedure was improved by J. S. Plaskett (19), at Ottawa in 1911, who used a triple-prism system. It produced spectra arranged so that the spectrum},
  keywords = {notion,notion-database}
}

@article{Hartman2008,
  title = {Deep {{MMT Transit Survey}} of the {{Open Cluster M37}}. {{I}}. {{Observations}} and {{Cluster Parameters}}},
  author = {Hartman, J. D. and Gaudi, B. S. and Holman, M. J. and McLeod, B. A. and Stanek, K. Z. and Barranco, J. A. and Pinsonneault, M. H. and Meibom, S. and Kalirai, J. S.},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {675},
  number = {2},
  eprint = {0709.3484},
  pages = {1233--1253},
  issn = {0004-637X},
  doi = {10.1086/527465},
  abstract = {We have conducted a deep (15 {$\lessequivlnt$} r {$\lessequivlnt$} 23), 20 night survey for transiting planets in the intermediate-age open cluster M37 (NGC 2099) using the Megacam wide-field mosaic CCD camera on the 6.5 m MMT. In this paper we describe the observations and data reduction procedures for the survey and analyze the stellar content and dynamical state of the cluster. By combining high-resolution spectroscopy with existing BVICKS and new gri color-magnitude diagrams, we determine the fundamental cluster parameters: t = 485 {$\pm$} 28 Myr without overshooting (t = 550 {$\pm$} 30 Myr with overshooting), E( B- V) = 0.227 {$\pm$} 0.038, (m - M)V = 11.57 {$\pm$} 0.13, and [M/H] = +0.045 {$\pm$} 0.044, which are in good agreement with, although more precise than, previous measurements. We determine the mass function down to 0.3 M{$\odot$} and use this to estimate the total cluster mass of 3640 {$\pm$} 170 M{$\odot$}. \textcopyright{} 2008. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/44UPKIJ3/Hartman et al. - 2008.pdf}
}

@inproceedings{Harvey1985,
  title = {{{HIGH-RESOLUTION HELIOSEISMOLOGY}}},
  booktitle = {{{ESA Workshop}} on {{Future Mission}} in {{SOlar}}, {{Heliospheric}} \& {{Space Plasma Physics}}},
  author = {Harvey, J.},
  year = {1985},
  urldate = {2020-03-14},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/E4D5YXEX/full-text.pdf}
}

@article{Hasan2005a,
  title = {Probing the Internal Magnetic Field of Slowly Pulsating {{B-stars}} through g Modes},
  author = {Hasan, S. S. and Zahn, J. P. and {Christensen-Dalsgaard}, J.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {444},
  number = {2},
  pages = {29--32},
  issn = {00046361},
  doi = {10.1051/0004-6361:200500203},
  abstract = {We suggest that high-order g modes can be used as a probe of the internal magnetic field of SPB (slowly pulsating B) stars. The idea is based on earlier work by the authors hich analytically investigated the effect of a vertical magnetic field on p and g modes in a plane-parallel isothermal stratified atmosphere. It was found that even a weak field can significantly shift the g-mode frequencies - the effect increases with mode order. Methods. In the present study we adopt the classical perturbative approach to estimate the internal field of a 4 solar mass SPB star by looking at its effect on a low-degree (l = 1) and high-order (n = 20) g mode with a period of about 1.5 d. Results. We find that a polar field strength of about 110 kG on the edge of the convective core is required to produce a frequency shift of 1\%. Frequency splittings of that order have been observed in several SPB variables, in some cases clearly too small to be ascribed to rotation. We suggest that they may be due to a poloidal field with a strength of order 100 kG, buried in the deep interior of the star. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Stars: magnetic fields,Stars: oscillations,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/EW5PZGKW/Hasan, Zahn, Christensen-Dalsgaard - 2005.pdf}
}

@misc{Hatami2017,
  title = {Classification of {{Time-Series Images Using Deep Convolutional Neural Networks}}},
  author = {Hatami, Nima and Gavet, Yann and Debayle, Johan},
  year = {2017},
  month = oct,
  number = {arXiv:1710.00886},
  eprint = {1710.00886},
  primaryclass = {cs},
  publisher = {{arXiv}},
  doi = {10.48550/arXiv.1710.00886},
  urldate = {2023-05-16},
  abstract = {Convolutional Neural Networks (CNN) has achieved a great success in image recognition task by automatically learning a hierarchical feature representation from raw data. While the majority of Time-Series Classification (TSC) literature is focused on 1D signals, this paper uses Recurrence Plots (RP) to transform time-series into 2D texture images and then take advantage of the deep CNN classifier. Image representation of time-series introduces different feature types that are not available for 1D signals, and therefore TSC can be treated as texture image recognition task. CNN model also allows learning different levels of representations together with a classifier, jointly and automatically. Therefore, using RP and CNN in a unified framework is expected to boost the recognition rate of TSC. Experimental results on the UCR time-series classification archive demonstrate competitive accuracy of the proposed approach, compared not only to the existing deep architectures, but also to the state-of-the art TSC algorithms.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Computer Vision and Pattern Recognition},
  file = {/Users/lbugnet/Zotero/storage/HKEZ7S25/Hatami et al. - 2017 - Classification of Time-Series Images Using Deep Co.pdf;/Users/lbugnet/Zotero/storage/X8DWJDVM/1710.html}
}

@article{Hathaway2010,
  title = {The {{Solar Cycle}}},
  author = {Hathaway, David H.},
  year = {2010},
  month = dec,
  journal = {Living Reviews in Solar Physics},
  volume = {7},
  number = {1},
  pages = {1},
  issn = {2367-3648},
  doi = {10.12942/lrsp-2010-1},
  urldate = {2020-05-22},
  keywords = {Geomagnetic Activity,notion,notion-database,Polar Field,Solar activity,Solar Activity,Solar cycle,Solar Cycle,Solar cycle prediction,Sunspot Number,Sunspots}
}

@article{Hawley1996,
  title = {Local {{Three-dimensional Simulations}} of an {{Accretion Disk Hydromagnetic Dynamo}}},
  author = {Hawley, John F. and Gammie, Charles F. and Balbus, Steven A.},
  year = {1996},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {464},
  pages = {690},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/177356},
  urldate = {2020-07-02},
  abstract = {Using three-dimensional numerical simulations, we have found that the weak-field magnetorotational instability constitutes a hydromagnetic dynamo in astrophysical disks. The field amplification mechanism lies outside the scope of kinematic dynamo theory and implies that kinematic dynamo theory is not applicable to accretion disk systems. We begin with simulations of isotropic, homogeneous turbulence to demonstrate the ability of our finite-difference code to reproduce known dynamos. To calibrate our code, we measure magnetic field rates when the turbulent velocity field is not sustained through external forcing. When the turbulence is maintained with imposed velocity fields, a magnetic dynamo can be produced. Two cases are considered: velocity fields with and without net helicity. Both the helical and the nonhelical velocity fields amplify and sustain magnetic fields despite substantial turbulent dissipation. The nonhelical dynamo increases the magnetic field energy by an order of magnitude. The helical dynamo produces greater amplification (a factor of 30 in energy) and a more ordered field. Lorentz forces eventually limit the growth of the magnetic field in both cases. We next carry out simulations in the local shearing box model of an accretion disk. The initial magnetic field has a mean field value of zero over the computational domain and is weak in the sense that the initial Alfv\'en speed is much less than the sound speed. The magnetorotational instability rapidly generates turbulence within the disk. The turbulence is anisotropic, producing significant Maxwell and Reynolds stresses that transport angular momentum outward. Both the stresses and magnetic energy density remain subthermal and do not approach equipartition. The magnetic energy is amplified by a factor of 20 and maintained for over 200 orbits of time, far longer than the magnetic decay time in the absence of an amplification mechanism. A parameter survey indicates the final turbulent state does not depend on the initial average field strength; some dependence on the computational domain size, magnetic Prandtl number, and numerical resolution is observed. Finally, we demonstrate explicitly that more than shear and turbulence are required to produce dynamo amplification of magnetic fields.},
  keywords = {ACCRETION,ACCRETION DISKS,HYDRODYNAMICS,MAGNETOHYDRODYNAMICS: MHD,notion,notion-database,TURBULENCE}
}

@article{He2016a,
  title = {Activity {{Analyses}} for {{Solar-Type Stars Observed With Kepler}}. {{I}}. {{Proxies}} of {{Magnetic Activity}}},
  author = {He, Han and Wang, Huaning and Yun, Duo},
  year = {2016},
  eprint = {1602.02233},
  doi = {10.1088/0067-0049/221/1/18},
  abstract = {Light curves of solar-type stars often show gradual fluctuations due to rotational modulation by magnetic features (starspots and faculae) on stellar surfaces. Two quantitative measures of modulated light curves are employed as the proxies of magnetic activity for solar-type stars observed with Kepler telescope. The first is named autocorrelation index \$i\_\{AC\}\$, which describes the degree of periodicity of the light curve, the second is the effective fluctuation range of the light curve \$R\_\{eff\}\$, which reflects the depth of rotational modulation. The two measures are complementary and depict different aspects of magnetic activities on solar-type stars. By using the two proxies \$i\_\{AC\}\$ and \$R\_\{eff\}\$, we analyzed activity properties of two carefully selected solar-type stars observed with Kepler (Kepler ID: 9766237 and 10864581), which have distinct rotational periods (14.7 vs. 6.0 days). We also applied the two measures to the Sun for a comparative study. The result shows that both the measures can reveal cyclic activity variations (referred to as \$i\_\{AC\}\$-cycle and \$R\_\{eff\}\$-cycle) on the two Kepler stars and the Sun. For the Kepler star with the faster rotation rate, \$i\_\{AC\}\$-cycle and \$R\_\{eff\}\$-cycle are in the same phase, while for the Sun (slower rotator), they are in the opposite phase. By comparing the solar light curve with simultaneous photospheric magnetograms, it is identified that the magnetic feature that causes the periodic light curve during solar minima is the faculae of the enhanced network region, which can also be a candidate of magnetic features that dominate the periodic light curves on the two Kepler stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/C77YK9PC/He, Wang, Yun - 2016.pdf}
}

@article{He2019,
  title = {Learning to Predict the Cosmological Structure Formation},
  author = {He, Siyu and Li, Yin and Feng, Yu and Ho, Shirley and Ravanbakhsh, Siamak and Chen, Wei and P{\'o}czos, Barnab{\'a}s},
  year = {2019},
  month = jul,
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  volume = {116},
  number = {28},
  eprint = {1811.06533},
  pages = {13825--13832},
  publisher = {{National Academy of Sciences}},
  issn = {10916490},
  doi = {10.1073/pnas.1821458116},
  urldate = {2021-01-06},
  abstract = {Matter evolved under the influence of gravity from minuscule density fluctuations. Nonperturbative structure formed hierarchically over all scales and developed non-Gaussian features in the Universe, known as the cosmic web. To fully understand the structure formation of the Universe is one of the holy grails of modern astrophysics. Astrophysicists survey large volumes of the Universe and use a large ensemble of computer simulations to compare with the observed data to extract the full information of our own Universe. However, to evolve billions of particles over billions of years, even with the simplest physics, is a daunting task. We build a deep neural network, the Deep Density Displacement Model (D3M), which learns from a set of prerun numerical simulations, to predict the nonlinear large-scale structure of the Universe with the Zel'dovich Approximation (ZA), an analytical approximation based on perturbation theory, as the input. Our extensive analysis demonstrates that D3M outperforms the second-order perturbation theory (2LPT), the commonly used fast-approximate simulation method, in predicting cosmic structure in the nonlinear regime. We also show that D3M is able to accurately extrapolate far beyond its training data and predict structure formation for significantly different cosmological parameters. Our study proves that deep learning is a practical and accurate alternative to approximate 3D simulations of the gravitational structure formation of the Universe.},
  archiveprefix = {arxiv},
  pmid = {31235606},
  keywords = {Cosmology,Deep learning,notion,notion-database,Simulation},
  file = {/Users/lbugnet/Zotero/storage/Q8APCBIY/full-text.pdf}
}

@article{Heger2000,
  title = {Presupernova {{Evolution}} of {{Rotating Massive Stars}}. {{I}}. {{Numerical Method}} and {{Evolution}} of the {{Internal Stellar Structure}}},
  author = {Heger, A. and Langer, N. and Woosley, S. E.},
  year = {2000},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {528},
  pages = {368--396},
  issn = {0004-637X},
  doi = {10.1086/308158},
  urldate = {2023-11-01},
  abstract = {The evolution of rotating stars with zero-age main-sequence (ZAMS) masses in the range 8-25 Msolar is followed through all stages of stable evolution. The initial angular momentum is chosen such that the star's equatorial rotational velocity on the ZAMS ranges from zero to \textasciitilde 70\% of breakup. The stars rotate rigidly on the ZAMS as a consequence of angular momentum redistribution during the pre-main-sequence evolution. Redistribution of angular momentum and chemical species are then followed as a consequence of Eddington-Sweet circulation, Solberg-H\o iland instability, the Goldreich-Schubert-Fricke instability, and secular and dynamic shear instability. The effects of the centrifugal force on the stellar structure are included. Convectively unstable zones are assumed to tend toward rigid rotation, and uncertain mixing efficiencies are gauged by observations. We find, as noted in previous work, that rotation increases the helium core masses and enriches the stellar envelopes with products of hydrogen burning. We determine, for the first time, the angular momentum distribution in typical presupernova stars along with their detailed chemical structure. Angular momentum loss due to (nonmagnetic) stellar winds and the redistribution of angular momentum during core hydrogen burning are of crucial importance for the specific angular momentum of the core. Neglecting magnetic fields, we find angular momentum transport from the core to the envelope to be unimportant after core helium burning. We obtain specific angular momenta for the iron core and overlying material of 1016-1017 cm2 s-1. These values are insensitive to the initial angular momentum and to uncertainties in the efficiencies of rotational mixing. They are small enough to avoid triaxial deformations of the iron core before it collapses, but could lead to neutron stars which rotate close to breakup. They are also in the range required for the collapsar model of gamma-ray bursts. The apparent discrepancy with the measured rotation rates of young pulsars is discussed.},
  keywords = {Astrophysics,Hydrodynamics,HYDRODYNAMICS,Methods: Numerical,METHODS: NUMERICAL,stars early-type,STARS EARLY-TYPE,stars rotation,STARS ROTATION,Stars: Evolution,STARS: EVOLUTION,Stars: Interiors,STARS: INTERIORS},
  annotation = {ADS Bibcode: 2000ApJ...528..368H},
  file = {/Users/lbugnet/Zotero/storage/JRFPPDVC/Heger et al. - 2000 - Presupernova Evolution of Rotating Massive Stars. .pdf}
}

@article{Heger2005,
  title = {Presupernova {{Evolution}} of {{Differentially Rotating Massive Stars Including Magnetic Fields}}},
  author = {Heger, A. and Woosley, S. E. and Spruit, H. C.},
  year = {2005},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {626},
  number = {1},
  eprint = {astro-ph/0409422},
  pages = {350--363},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/429868},
  urldate = {2020-07-13},
  abstract = {As a massive star evolves through multiple stages of nuclear burning on its way to becoming a supernova, a complex, differentially rotating structure is set up. Angular momentum is transported by a variety of classic instabilities, and also by magnetic torques from fields generated by the differential rotation. We present the first stellar evolution calculations to follow the evolution of rotating massive stars including, at least approximately, all these effects, magnetic and non-magnetic, from the zero-age main sequence until the onset of iron-core collapse. The evolution and action of the magnetic fields is as described by Spruit 2002 and a range of uncertain parameters is explored. In general, we find that magnetic torques decrease the final rotation rate of the collapsing iron core by about a factor of 30 to 50 when compared with the non-magnetic counterparts. Angular momentum in that part of the presupernova star destined to become a neutron star is an increasing function of main sequence mass. That is, pulsars derived from more massive stars will rotate faster and rotation will play a more dominant role in the star's explosion. The final angular momentum of the core is determined - to within a factor of two - by the time the star ignites carbon burning. For the lighter stars studied, around 15 solar masses, we predict pulsar periods at birth near 15 ms, though a factor of two range is easily tolerated by the uncertainties. Several mechanisms for additional braking in a young neutron star, especially by fall back, are also explored.},
  archiveprefix = {arxiv},
  keywords = {evolution-stars,general-stars,magnetic fields-stars,notion,notion-database,pulsars,rotation,Subject headingg s},
  file = {/Users/lbugnet/Zotero/storage/36E25TR7/full-text.pdf}
}

@article{Hekker2006,
  title = {Pulsations Detected in the Line Profile Variations of Red Giants {{Modelling}} of Line Moments, Line Bisector and Line Shape},
  author = {Hekker, S. and Aerts, C. and De Ridder, J. and Carrier, F.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {458},
  number = {3},
  pages = {931--940},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065755},
  abstract = {Context. So far, red giant oscillations have been studied from radial velocity and/or light curve variations, which reveal frequencies of the oscillation modes. To characterise radial and non-radial oscillations, line profile variations are a valuable diagnostic. Here we present for the first time a line profile analysis of pulsating red giants, taking into account the small line profile variations and the predicted short damping and re-excitation times. We do so by modelling the time variations in the cross correlation profiles in terms of oscillation theory. Aims. The performance of existing diagnostics for mode identification is investigated for known oscillating giants which have very small line profile variations. We modify these diagnostics, perform simulations, and characterise the radial and non-radial modes detected in the cross correlation profiles. Methods. Moments and line bisectors are computed and analysed for four giants. The robustness of the discriminant of the moments against small oscillations with finite lifetimes is investigated. In addition, line profiles are simulated with short damping and re-excitation times and their line shapes are compared with the observations. Results. For three stars, we find evidence for the presence of non-radial pulsation modes, while for f Hydrae perhaps only radial modes are present. Furthermore the line bisectors are not able to distinguish between different pulsation modes and are an insufficient diagnostic to discriminate small line profile variations due to oscillations from exoplanet motion. \textcopyright{} ESO 2006.},
  keywords = {Line: profiles,notion,notion-database,Stars: general,Stars: oscillations,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/HT9RKE6E/Hekker et al. - 2006.pdf}
}

@article{Hekker2008,
  title = {Oscillations in {{Procyon A}}: {{First}} Results from a Multi-Site Campaign},
  author = {Hekker, S. and Arentoft, T. and Kjeldsen, H. and Bedding, T. R. and {Christensen-Dalsgaard}, J. and Reffert, S. and Bruntt, H. and Butler, R. P. and Kiss, L. L. and O'Toole, S. J. and Kambe, E. and Ando, H. and Izumiura, H. and Sato, B. and Hartmann, M. and Hatzes, A. P. and Appourchaux, T. and Barban, C. and Berthomieu, G. and Bouchy, F. and Garc{\'i}a, R. A. and Lebrun, J. C. and Marti{\'c}, M. and Michel, E. and Mosser, B. and Nghiem, P. A.P. and Provost, J. and Samadi, R. and Th{\'e}venin, F. and {Turck-Chi{\`e}ze}, S. and Bonanno, S. A. and Benatti, S. and Claudi, R. U. and Cosentino, R. and Leccia, S. and Frandsen, S. and Brogaard, K. and Grundahl, F. and Stempels, H. C. and Bazot, M. and Dall, T. H. and Karoff, C. and Carrier, F. and Eggenberger, P. and Sosnowska, D. and Wittenmyer, R. A. and Endl, M. and Metcalfe, T. S.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  eprint = {0710.3772},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012059},
  abstract = {Procyon A is a bright F5IV star in a binary system. Although the distance, mass and angular diameter of this star are all known with high precision, the exact evolutionary state is still unclear. Evolutionary tracks with different ages and different mass fractions of hydrogen in the core pass, within the errors, through the observed position of Procyon A in the Hertzsprung-Russell diagram. For more than15 years several different groups have studied the solar-like oscillations in Procyon A to determine its evolutionary state. Although several studies independently detected power excess in the periodogram, there is no agreement on the actual oscillation frequencies yet. This is probably due to either insufficient high-quality data (i.e., aliasing) or due to intrinsic properties of the star (i.e., short mode lifetimes). Now a spectroscopic multi-site campaign using 10 telescopes world-wide (minimizing aliasing effects) with a total time span of nearly 4 weeks (increase the frequency resolution) is performed to identify frequencies in this star and finally determine its properties and evolutionary state. \textcopyright{} 2008 IOP Publishing Ltd.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G46WM4U9/Hekker et al. - 2008.pdf}
}

@article{Hekker2009,
  title = {Characteristics of Solar-like Oscillations in Red Giants Observed in the {{CoRoT}} Exoplanet Field},
  author = {Hekker, S. and Kallinger, T. and Baudin, F. and De Ridder, J. and Barban, C. and Carrier, F. and Hatzes, A. P. and Weiss, W. W. and Baglin, A.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {465--469},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911858},
  abstract = {Context. Observations during the first long run ({$\sim$}150 days) in the exo-planet field of CoRoT increase the number of G-K giant stars for which solar-like oscillations are observed by a factor of 100. This opens the possibility to study the characteristics of their oscillations in a statistical sense. Aims. We aim to understand the statistical distribution of the frequencies of maximum oscillation power ({$\nu$}max) in red giants and to search for a possible correlation between {$\nu$}max and the large separation ({$\Delta\nu$}). Methods. Red giants with detectable solar-like oscillations are identified using both semi-automatic and manual procedures. For these stars, we determine {$\nu$}max as the centre of a Gaussian fit to the oscillation power excess. For the determination of {$\Delta\nu$}, we use the autocorrelation of the Fourier spectra, the comb response function and the power spectrum of the power spectrum. Results. The resulting {$\nu$}max distribution shows a pronounced peak between 20.40 {$\mu$}Hz. For about half of the stars we obtain {$\Delta\nu$} with at least two methods. The correlation between {$\nu$}max and {$\Delta\nu$} follows the same scaling relation as inferred for solar-like stars. Conclusions. The shape of the {$\nu$}max distribution can partly be explained by granulation at low frequencies and by white noise at high frequencies, but the population density of the observed stars turns out to be also an important factor. From the fact that the correlation between {$\Delta\nu$} and {$\nu$}max for red giants follows the same scaling relation as obtained for sun-like stars, we conclude that the sound travel time over the pressure scale height of the atmosphere scales with the sound travel time through the whole star irrespective of evolution. The fraction of stars for which we determine {$\Delta\nu$} does not correlate with {$\nu$}max in the investigated frequency range, which confirms theoretical predictions.},
  keywords = {Methods: observational,notion,notion-database,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/2AYR4I9I/Hekker et al. - 2009.pdf}
}

@article{Hekker2010a,
  title = {Oscillation Mode Lifetimes of Red Giants Observed during the Initial and First Anticentre Long Run of {{CoRoT}}},
  author = {Hekker, S. and Barban, C. and Baudin, F. and De Ridder, J. and Kallinger, T. and Morel, T. and Chaplin, W. J. and Elsworth, Y.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {520},
  number = {9},
  pages = {1--11},
  issn = {00046361},
  doi = {10.1051/0004-6361/201014944},
  abstract = {Context. Long timeseries of data increase the frequency resolution in the power spectrum. This allows for resolving stochastically excited modes with long mode lifetimes, as well as features that are close together in frequency. The CoRoT fields observed during the initial run and second long run partly overlap, and stars in this overlapping field observed in both runs are used to create timeseries with a longer timespan than available from the individual runs. Aims. We aim to measure the mode lifetimes of red giants and compare them with theoretical predictions. We also investigate the dependence of the mode lifetimes on frequency and the degree of the oscillation modes. Methods. We perform simulations to investigate the influence of the gap in the data between the initial and second long run, the total length of the run and the signal-to-noise ratio on the measured mode lifetime. This provides us with a correction factor to apply to the mode lifetimes measured from a maximum likelihood fit to the oscillation frequencies. Results. We find that the length of the timeseries, the signal-to-noise ratio and possible gaps do have a non-negligible effect on the measurements of the mode lifetime of stochastically excited oscillation modes, but we can correct for it. For the four stars for which we can perform a fit of the oscillation frequencies, we find that the mode lifetimes depend on frequency and on degree of the mode, which quantitatively agrees with theoretical predictions. \textcopyright{} 2010 ESO.},
  keywords = {methods: observational,notion,notion-database,stars: late-type,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/2P8UEPJG/Hekker et al. - 2010.pdf}
}

@article{Hekker2010b,
  title = {The {{Octave}} ({{Birmingham-Sheffield Hallam}}) Automated Pipeline for Extracting Oscillation Parameters of Solar-like Main-Sequence Stars},
  author = {Hekker, S. and Broomhall, A. M. and Chaplin, W. J. and Elsworth, Y. P. and Fletcher, S. T. and New, R. and Arentoft, T. and Quirion, P. O. and Kjeldsen, H.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {402},
  number = {3},
  pages = {2049--2059},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.16030.x},
  abstract = {The number of main-sequence stars for which we can observe solar-like oscillations is expected to increase considerably with the short-cadence high-precision photometric observations from the NASA Kepler satellite. Because of this increase in the number of stars, automated tools are needed to analyse these data in a reasonable amount of time. In the framework of the asteroFLAG consortium, we present an automated pipeline which extracts frequencies and other parameters of solar-like oscillations in main-sequence and subgiant stars. The pipeline uses only the time series data as input and does not require any other input information. Tests on 353 artificial stars reveal that we can obtain accurate frequencies and oscillation parameters for about three quarters of the stars. We conclude that our methods are well suited for the analysis of main-sequence stars, which show mainly p-mode oscillations. \textcopyright{} 2009 The Authors. Journal compilation \textcopyright{} 2009 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/9LVIJ5QT/Hekker et al. - 2010(2).pdf}
}

@article{Hekker2011a,
  title = {Solar-like Oscillations in Red Giants Observed with {{Kepler}} : Comparison of Global Oscillation Parameters from Different Methods},
  author = {Hekker, S. and Elsworth, Y. and De Ridder, J. and Mosser, B. and Garc{\'i}a, R. A. and Kallinger, T. and Mathur, S. and Huber, D. and Buzasi, D. L. and Preston, H. L. and Hale, S. J. and Ballot, J. and Chaplin, W. J. and R{\'e}gulo, C. and Bedding, T. R. and Stello, D. and Borucki, W. J. and Koch, D. G. and Jenkins, J. and Allen, C. and Gilliland, R. L. and Kjeldsen, H. and {Christensen-Dalsgaard}, J.},
  year = {2011},
  journal = {Astronomy \& Astrophysics},
  volume = {525},
  pages = {A131},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201015185},
  abstract = {Context. The large number of stars for which uninterrupted high-precision photometric timeseries data are being collected with Kepler and CoRoT initiated the development of automated methods to analyse the stochastically excited oscillations in main-sequence, subgiant and red-giant stars. Aims: We investigate the differences in results for global oscillation parameters of G and K red-giant stars due to different methods and definitions. We also investigate uncertainties originating from the stochastic nature of the oscillations. Methods: For this investigation we use Kepler data obtained during the first four months of operation. These data have been analysed by different groups using already published methods and the results are compared. We also performed simulations to investigate the uncertainty on the resulting parameters due to different realizations of the stochastic signal. Results: We obtain results for the frequency of maximum oscillation power ({$\nu\_$}max) and the mean large separation ({$<\Delta\nu>$}) from different methods for over one thousand red-giant stars. The results for these parameters agree within a few percent and seem therefore robust to the different analysis methods and definitions used here. The uncertainties for {$\nu\_$}max and {$<\Delta\nu>$} due to differences in realization noise are not negligible and should be taken into account when using these results for stellar modelling. Table 7 is only available in electronic form at http://www.aanda.org},
  keywords = {asteroseismology,late-type,methods,notion,notion-database,observational,photometric,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/UMVKULWW/Hekker et al. - 2011.pdf}
}

@article{Hekker2011b,
  title = {Asteroseismic Inferences on Red Giants in Open Clusters {{NGC}} 6791, {{NGC}} 6819, and {{NGC}} 6811 Using {{Kepler}}},
  author = {Hekker, S. and Basu, S. and Stello, D. and Kallinger, T. and Grundahl, F. and Mathur, S. and Garc{\'i}a, R. A. and Mosser, B. and Huber, D. and Bedding, T. R. and Szab{\'o}, R. and De Ridder, J. and Chaplin, W. J. and Elsworth, Y. and Hale, S. J. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Still, M. and McCauliff, S. and Quintana, E. V.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {530},
  pages = {1--9},
  issn = {00046361},
  doi = {10.1051/0004-6361/201016303},
  abstract = {Context. Four open clusters are present in the Kepler field of view and timeseries of nearly a year in length are now available. These timeseries allow us to derive asteroseismic global oscillation parameters of red-giant stars in the three open clusters NGC 6791, NGC 6819 and NGC 6811. From these parameters and effective temperatures, we derive masses, radii and luminosities for the clusters as well as field red giants. Aims. We study the influence of evolution and metallicity on the observed red-giant populations. Methods. The global oscillation parameters are derived using different published methods and the effective temperatures are derived from 2MASS colours. The observational results are compared with BaSTI evolution models. Results. We find that the mass has significant influence on the asteroseismic quantities {$\Delta\nu$} vs. {$\nu$}max relation, while the influence of metallicity is negligible, under the assumption that the metallicity does not affect the excitation/damping of the oscillations. The positions of the stars in the H-R diagram depend on both mass and metallicity. Furthermore, the stellar masses derived for the field stars are bracketed by those of the cluster stars. Conclusions. Both the mass and metallicity contribute to the observed difference in locations in the H-R diagram of the old metal-rich cluster NGC 6791 and the middle-aged solar-metallicity cluster NGC 6819. For the young cluster NGC 6811, the explanation of the position of the stars in the H-R diagram challenges the assumption of solar metallicity, and this open cluster might have significantly lower metallicity [Fe/H] in the range - 0.3 to - 0.7 dex. Also, nearly all the observed field stars seem to be older than NGC 6811 and younger than NGC 6791. \textcopyright{} 2011 ESO.},
  keywords = {Asteroseismology,Methods: observational,notion,notion-database,Open clusters and associations: general,Stars: late-type,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/R7KPLR5G/Hekker et al. - 2011(2).pdf}
}

@article{Hekker2011c,
  title = {Characterization of Red Giant Stars in the Public {{Kepler}} Data},
  author = {Hekker, S. and Gilliland, R. L. and Elsworth, Y. and Chaplin, W. J. and {de Ridder}, J. and Stello, D. and Kallinger, T. and Ibrahim, K. A. and Klaus, T. C. and Li, J.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {414},
  number = {3},
  pages = {2594--2601},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.18574.x},
  abstract = {The first public release of long-cadence stellar photometric data collected by the NASA Kepler mission has now been made available. In this paper, we characterize the red giant (G-K) stars in this large sample in terms of their solar-like oscillations. We use published methods and well-known scaling relations in the analysis. Just over 70 per cent of the red giants in the sample show detectable solar-like oscillations, and from these oscillations we are able to estimate the fundamental properties of the stars. This asteroseismic analysis reveals different populations: low-luminosity H-shell burning red giant branch stars, cool high-luminosity red giants on the red giant branch and He-core burning clump and secondary-clump giants. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {Methods: observational,notion,notion-database,Stars: late type,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/THQRNRVS/Hekker et al. - 2011(3).pdf}
}

@article{Hekker2012,
  title = {Solar-like Oscillations in Red Giants Observed with {{Kepler}}: {{Influence}} of Increased Timespan on Global Oscillation Parameters},
  author = {Hekker, S. and Elsworth, Y. and Mosser, B. and Kallinger, T. and Chaplin, W. J. and De Ridder, J. and Garc{\'i}a, R. A. and Stello, D. and Clarke, B. D. and Hall, J. R. and Ibrahim, K. A.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {544},
  pages = {1--11},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219328},
  abstract = {Context. The length of the asteroseismic timeseries obtained from the Kepler satellite analysed here span 19 months. Kepler provides the longest continuous timeseries currently available, which calls for a study of the influence of the increased timespan on the accuracy and precision of the obtained results. Aims. We aim to investigate how the increased timespan influences the detectability of the oscillation modes, and the absolute values and uncertainties of the global oscillation parameters, i.e., frequency of maximum oscillation power, {$\nu$} max, and large frequency separation between modes of the same degree and consecutive orders, ({$\Delta\nu$}). Methods. We use published methods to derive {$\nu$} max and ({$\Delta\nu$}) for timeseries ranging from 50 to 600 days and compare these results as a function of method, timespan and ({$\Delta\nu$}). Results. We find that in general a minimum of the order of 400 day long timeseries are necessary to obtain reliable results for the global oscillation parameters in more than 95\% of the stars, but this does depend on ({$\Delta\nu$}). In a statistical sense the quoted uncertainties seem to provide a reasonable indication of the precision of the obtained results in short (50-day) runs, they do however seem to be overestimated for results of longer runs. Furthermore, the different definitions of the global parameters used in the different methods have non-negligible effects on the obtained values. Additionally, we show that there is a correlation between {$\nu$} max and the flux variance. Conclusions. We conclude that longer timeseries improve the likelihood to detect oscillations with automated codes (from \textasciitilde 60\% in 50 day runs to {$>$}95\% in 400 day runs with a slight method dependence) and the precision of the obtained global oscillation parameters. The trends suggest that the improvement will continue for even longer timeseries than the 600 days considered here, with a reduction in the median absolute deviation of more than a factor of 10 for an increase in timespan from 50 to 2000 days (the currently foreseen length of the mission). This work shows that global parameters determined with high precision-thus from long datasets-using different definitions can be used to identify the evolutionary state of the stars. \textcopyright{} 2012 ESO.},
  keywords = {notion,notion-database,Stars: interiors,Stars: late-type,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/8C5C9TAJ/Hekker et al. - 2012.pdf}
}

@article{Hekker2013,
  title = {Asteroseismic Surface Gravity for Evolved Stars},
  author = {Hekker, S. and Elsworth, Y. and Mosser, B. and Kallinger, T. and Basu, Sarbani and Chaplin, W. J. and Stello, D.},
  year = {2013},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {556},
  number = {A59},
  eprint = {1305.6586},
  doi = {10.1051/0004-6361/201321630},
  urldate = {2020-03-23},
  abstract = {Context: Asteroseismic surface gravity values can be of importance in determining spectroscopic stellar parameters. The independent log(g) value from asteroseismology can be used as a fixed value in the spectroscopic analysis to reduce uncertainties due to the fact that log(g) and effective temperature can not be determined independently from spectra. Since 2012, a combined analysis of seismically and spectroscopically derived stellar properties is ongoing for a large survey with SDSS/APOGEE and Kepler. Therefore, knowledge of any potential biases and uncertainties in asteroseismic log(g) values is now becoming important. Aims: The seismic parameter needed to derive log(g) is the frequency of maximum oscillation power (nu\_max). Here, we investigate the influence of nu\_max derived with different methods on the derived log(g) values. The large frequency separation between modes of the same degree and consecutive radial orders (Dnu) is often used as an additional constraint for the determination of log(g). Additionally, we checked the influence of small corrections applied to Dnu on the derived values of log(g). Methods We use methods extensively described in the literature to determine nu\_max and Dnu together with seismic scaling relations and grid-based modeling to derive log(g). Results: We find that different approaches to derive oscillation parameters give results for log(g) with small, but different, biases for red-clump and red-giant-branch stars. These biases are well within the quoted uncertainties of \textasciitilde 0.01 dex (cgs). Corrections suggested in the literature to the Dnu scaling relation have no significant effect on log(g). However somewhat unexpectedly, method specific solar reference values induce biases of the order of the uncertainties, which is not the case when canonical solar reference values are used.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/D6GGMQB2/full-text.pdf}
}

@article{Hekker2014a,
  title = {Grid-Based Seismic Modelling at High and Low Signal-to-Noise Ratios: {{HD}} 181420 and {{HD}} 175272},
  author = {Hekker, S. and Ball, W. H.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {564},
  pages = {1--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201323121},
  abstract = {Context. Recently, the CoRoT target HD 175272 (F5V), which shows a weak signal of solar-like oscillations, was modelled by a differential asteroseismic analysis (Ozel et al. 2013, A\&A, 558, A79) relative to a seismically similar star, HD 181420 (F2V), for which there is a clear signature of solar-like oscillations. The results provided by Ozel et al. indicate the possibility of HD 175272 having subsolar mass, while being of the order of 1000 K hotter than the Sun. This seems unphysical-standard stellar evolution theory generally does not predict solar-metallicity stars of subsolar mass to be hotter than about 6000 K-and calls for a reanalysis of this star. Aims. We aim to compare the performance of differential asteroseismic analysis with that of grid-based modelling. Methods. We use two sets of stellar model grids and two grid-fitting methods to model HD 175272 and HD 181420 using their effective temperatures, metallicities, large frequency separations ({$\Delta\nu$}), and frequencies of maximum oscillation power ({$\nu$}max) as observational constraints. Results. We find that we are able to model both stars with parameters that are both mutually compatible and comparable with other modelling efforts. Hence, with modest spectroscopic and asteroseismic inputs, we obtain reasonable estimates of stellar parameters. In the case of HD 175272, the uncertainties of the stellar parameters from our grid-based modelling are smaller, and hence more physical, than those reported in the differential analysis. For both stars, the models have significantly lower values of {$\nu$}max than the reported observed values. Furthermore, when using the asymptotic large frequency separation as opposed to the scaling relation to compute {$\Delta\nu$}, we find that our modelling results are significantly more self-consistent when {$\nu$}max is ignored. Conclusions. Grid-based modelling is a useful tool even in cases of weak solar-like oscillations. It provides more precise and more realistic results than obtained with differential seismology. The difference in the observed and modelled values of {$\nu$}max indicates that the four observational constraints are not fully consistent with the stellar models used here, with {$\nu$}max most likely to be the inconsistent constraint for these two stars. \textcopyright{} 2014 ESO.},
  keywords = {Asteroseismology,notion,notion-database,Stars: individual: HD 175272,Stars: individual: HD 181420},
  file = {/Users/lbugnet/Zotero/storage/CYN4IJBT/Hekker, Ball - 2014.pdf}
}

@inproceedings{Hekker2017,
  title = {Evolutionary States of Red-Giant Stars from Grid-Based Modelling},
  booktitle = {{{EPJ Web}} of {{Conferences}}},
  author = {Hekker, Saskia and Elsworth, Yvonne and Basu, Sarbani and Bellinger, Earl},
  year = {2017},
  volume = {160},
  eprint = {1705.05879},
  issn = {2100014X},
  doi = {10.1051/epjconf/201716004006},
  abstract = {From its surface properties it can be difficult to determine whether a red-giant star is in its heliumcore-burning phase or only burning hydrogen in a shell around an inert helium core. Stars in either of these stages can have similar effective temperatures, radii and hence luminosities, i.e. they can be located at the same position in the Hertzsprung-Russell diagram. Asteroseismology - the study of the internal structure of stars through their global oscillations - can provide the necessary additional constraints to determine the evolutionary states of red-giant stars. Here, we present a method that uses grid-based modelling based on global asteroseismic properties (vmax, frequency of maximum oscillation power; and {$\Delta$}v, frequency spacing between modes of the same degree and consecutive radial orders) as well as effective temperature and metallicity to determine the evolutionary phases. This method is applicable even to timeseries data of limited length, although with a small fraction of miss-classifications.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Hekker2017a,
  title = {Giant Star Seismology},
  author = {Hekker, S and {Christensen-Dalsgaard}, J},
  year = {2017},
  journal = {The Astronomy and Astrophysics Review},
  volume = {25},
  number = {1},
  eprint = {1609.07487v3},
  urldate = {2020-04-20},
  abstract = {The internal properties of stars in the red-giant phase undergo significant changes on relatively short timescales. Long near-uninterrupted high-precision pho-tometric timeseries observations from dedicated space missions such as CoRoT and Kepler have provided seismic inferences of the global and internal properties of a large number of evolved stars, including red giants. These inferences are confronted with predictions from theoretical models to improve our understanding of stellar structure and evolution. Our knowledge and understanding of red giants have indeed increased tremendously using these seismic inferences, and we anticipate that more information is still hidden in the data. Unraveling this will further improve our understanding of stellar evolution. This will also have significant impact on our knowledge of the Milky Way Galaxy as well as on exo-planet host stars. The latter is important for our understanding of the formation and structure of planetary systems.},
  archiveprefix = {arxiv},
  keywords = {(),notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QTAEC26I/full-text.pdf}
}

@misc{hekkerLowperiodSpacingCorehelium2023,
  title = {Low-Period Spacing Core-Helium Burning Giants: `hot Subdwarf Analogues'?},
  shorttitle = {Low-Period Spacing Core-Helium Burning Giants},
  author = {Hekker, S. and Elsworth, Y. and Braun, T. A. M. and Basu, S.},
  year = {2023},
  month = may,
  number = {arXiv:2305.10578},
  eprint = {2305.10578},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-06-06},
  abstract = {Global stellar oscillations probe the internal structure of stars. In low- to intermediate-mass red giants, these oscillations provide signatures from both the outer regions of the star as well as from the core. These signatures are imprinted in e.g. the frequency of maximum oscillation power, and in the differences in periods of non-radial oscillations (period spacings), respectively. In core helium burning giants with masses below about 1.7 solar masses, i.e. stars that have gone through a helium flash, the asymptotic period spacings take values of about 220 -350 s at frequency of maximum oscillation power of \$\textbackslash sim\$30-50 \$\textbackslash mu\$Hz. A set of stars with asymptotic period spacings lower than about 200 s at similar frequencies separations has recently been discovered by Elsworth and collaborators. In this work, we present a hypothesis for the formation scenario of these stars. We find that these stars can be the result of a mass-loss event at the end of the red-giant branch phase of stars massive enough to not have a degenerate core, i.e. one of the scenarios to form hot subdwarf stars. Therefore, these stars can be classified as `hot subdwarf analogues'. Interestingly, if mass loss continues gradually during the core helium burning phase, these stars turn hotter and denser, and could, therefore, be hot subdwarf progenitors as they shed more of their envelope.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/8I3UNWU4/Hekker et al. - 2023 - Low-period spacing core-helium burning giants `ho.pdf;/Users/lbugnet/Zotero/storage/ZHBMC663/2305.html}
}

@article{Hempelmann2003,
  title = {Wavelet Analysis of Stellar Differential Rotation: {{III}}. {{The}} Sun in White Light},
  author = {Hempelmann, A.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {399},
  number = {2},
  pages = {717--721},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021758},
  abstract = {Future space projects like KEPLER will deliver a vast quantity of high precision light curves of stars. This paper describes a test concerning the observability of rotation and even differential rotation of slowly rotating stars from such data. Two published light curves of solar total irradiance measures are investigated: the Nimbus-7 Earth Radiation Budget (ERB) observations between 1978 and 1993 and the Active Cavity Radiometer Irradiance Monitor I (ACRIM I) measurements between 1980 and 1989. Light curve analysis show that oscillations on time-scales comparable to solar rotation but of a complex pattern are visible. Neither Fourier analysis nor time-frequency Wavelet analysis yield the true rotation period during the more active phases of the solar cycle. The true rotation period dominates only for a short time during solar minimum. In the light of this study even space-born broad band photometry may turn out an inappropriate instrument to study stellar butterfly diagrams of stars rotating as slow as the Sun. However, it was shown in Papers I and II of this series that chromospheric tracers like Lyman {$\alpha$}, Mg II h+k and CaII H+K are appropriate instruments to perform this task.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: rotation,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/FFK44UGU/Hempelmann - 2003.pdf}
}

@article{Heng2009,
  title = {Magnetohydrodynamic Shallow Water Waves: {{Linear}} Analysis},
  author = {Heng, Kevin and Spitkovsky, Anatoly},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {703},
  number = {2},
  eprint = {0908.0946},
  pages = {1819--1831},
  publisher = {{Institute of Physics Publishing}},
  issn = {15384357},
  doi = {10.1088/0004-637X/703/2/1819},
  urldate = {2020-11-29},
  abstract = {We present a linear analysis of inviscid, incompressible, magnetohydrodynamic (MHD) shallow water systems. In spherical geometry, a generic property of such systems is the existence of five wave modes. Three of them (two magneto-Poincar\'e modes and one magneto-Rossby mode) are previously known. The other two wave modes are strongly influenced by the magnetic field and rotation, and have substantially lower angular frequencies; as such, we term them "magnetostrophic modes." We obtain analytical functions for the velocity, height, and magnetic field perturbations in the limit that the magnitude of the MHD analogue of Lamb's parameter is large. On a sphere, the magnetostrophic modes reside near the poles, while the other modes are equatorially confined. Magnetostrophic modes may be an ingredient in explaining the frequency drifts observed in Type I X-ray bursts from neutron stars. \textcopyright{} 2009. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {MHD,notion,notion-database,Stars: neutron,Waves,X-rays: bursts},
  file = {/Users/lbugnet/Zotero/storage/2IE9P84L/full-text.pdf}
}

@article{Hennebelle2013,
  title = {Observational Studies of Stellar Rotation},
  author = {Hennebelle, P. and Charbonnel, C. and Bouvier, J.},
  year = {2013},
  journal = {EAS Publications Series},
  volume = {62},
  eprint = {1307.2891},
  pages = {143--168},
  issn = {16381963},
  doi = {10.1051/eas/1362005},
  abstract = {This course reviews the rotational properties of non-degenerate stars as observed from the protostellar stage to the end of the main sequence. It includes an introduction to the various observational techniques used to measure stellar rotation. Angular momentum evolution models developed over the mass range from the substellar domain to high-mass stars are briefly discussed. \textcopyright{} EAS, EDP Sciences, 2013.},
  archiveprefix = {arxiv},
  isbn = {9782759810734},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MFPADTKI/Hennebelle, Charbonnel, Bouvier - 2013.pdf}
}

@article{Henneco2021,
  title = {The Effect of the Centrifugal Acceleration on Period Spacings of Gravito-Inertial Modes in Intermediate-Mass Stars},
  author = {Henneco, J. and Van Reeth, T. and Prat, V. and Mathis, S. and Mombarg, J. S. G. and Aerts, C.},
  year = {2021},
  month = apr,
  journal = {Astronomy and Astrophysics},
  volume = {648},
  pages = {A97},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202039464},
  urldate = {2023-06-05},
  abstract = {Context. The Kepler and Transiting Exoplanet Survey Satellite (TESS) space telescopes delivered high-precision, long-duration photometric time series for hundreds of main-sequence stars, revealing their numerous gravito-inertial (g) pulsation modes. This high precision allows us to evaluate increasingly detailed theoretical stellar models. Recent theoretical work extended the traditional approximation of rotation, a framework to evaluate the effect of the Coriolis acceleration on g modes, to include the effects of the centrifugal acceleration in the approximation of slightly deformed stars, which so far have mostly been neglected in asteroseismology. This extension of the traditional approximation was conceived by re-deriving the traditional approximation in a centrifugally-deformed, spheroidal coordinate system. Aims: We explore the effect of the centrifugal acceleration on g modes and assess its detectability in space-based photometric observations. Methods: We implemented the new theoretical framework to calculate the centrifugal deformation of pre-computed 1D spherical stellar structure models and computed the corresponding g-mode frequencies, assuming uniform rotation. The framework was evaluated for a grid of stellar structure models covering a relevant parameter space for observed g-mode pulsators. Results: The centrifugal acceleration modifies the effect of the Coriolis acceleration on g modes, narrowing the equatorial band in which they are trapped. Furthermore, the centrifugal acceleration causes the pulsation periods and period spacings of the most common g modes (prograde dipole modes and r modes) to increase with values similar to the observational uncertainties of the measured period spacing values in Kepler and TESS data. Conclusions: The effect of the centrifugal acceleration on g modes is formally detectable in modern space photometry. The implementation of the used theoretical framework in stellar structure and pulsation codes will allow for more precise asteroseismic modelling of centrifugally deformed stars in order to assess its effect on mode excitation, trapping, and damping.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,hydrodynamics,stars: interiors,stars: oscillations,stars: rotation,waves},
  annotation = {ADS Bibcode: 2021A\&A...648A..97H},
  file = {/Users/lbugnet/Zotero/storage/TDNFJSLH/Henneco et al. - 2021 - The effect of the centrifugal acceleration on peri.pdf}
}

@article{Henry2000,
  title = {A {{Transiting}} ``51 {{Peg}}\textendash like'' {{Planet}}},
  author = {Henry, Gregory W. and Marcy, Geoffrey W. and Butler, R. Paul and Vogt, Steven S.},
  year = {2000},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {529},
  number = {1},
  pages = {L41-L44},
  publisher = {{IOP Publishing}},
  issn = {0004637X},
  doi = {10.1086/312458},
  urldate = {2020-07-07},
  abstract = {Doppler measurements from Keck exhibit a sinusoidal periodicity in the velocities of the G0 dwarf HD 209458, having a semiamplitude of 81 m s-1 and a period of 3.5239 days, which is indicative of a ``51 Peg-like'' planet with a minimum mass (Msini) of 0.62 MJup and a semimajor axis of 0.046 AU. Follow-up photometry reveals a drop of 0.017 mag at the predicted time (within the errors) of transit by the companion based on the velocities. This is the first extrasolar planet observed to transit its star. The radius of the planet derived from the magnitude of the dimming is 1.42 RJup, which is consistent with models of irradiated Jupiter-mass planets. The transit implies that sini{$>$}0.993, leading to a true mass of 0.62 MJup for the planet. The resulting mean density of 0.27 g cm-3 implies that the companion is a gas giant. Based on observations obtained at the W. M. Keck Observatory, which is operated jointly by the University of California and the California Institute of Technology, and the automatic photoelectric telescopes at Fairborn Observatory in the Patagonia Mountains of southern Arizona.},
  keywords = {individual (HD 209458),notion,notion-database,planetary systems-stars,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/ZMP6DEYD/full-text.pdf}
}

@article{Hermes2012,
  title = {{{SDSS J184037}}.78+642312.3: {{The First Pulsating Extremely Low Mass White Dwarf}}},
  shorttitle = {{{SDSS J184037}}.78+642312.3},
  author = {Hermes, J. J. and Montgomery, M. H. and Winget, D. E. and Brown, Warren R. and Kilic, Mukremin and Kenyon, Scott J.},
  year = {2012},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {750},
  pages = {L28},
  issn = {0004-637X},
  doi = {10.1088/2041-8205/750/2/L28},
  urldate = {2023-10-09},
  abstract = {We report the discovery of the first pulsating extremely low mass (ELM) white dwarf (WD), SDSS J184037.78+642312.3 (hereafter J1840). This DA (hydrogen-atmosphere) WD is by far the coolest and the lowest-mass pulsating WD, with T eff = 9100 {$\pm$} 170 K and log g = 6.22 {$\pm$} 0.06, which corresponds to a mass of \textasciitilde 0.17 M {$\odot$}. This low-mass pulsating WD greatly extends the DAV (or ZZ Ceti) instability strip, effectively bridging the log g gap between WDs and main-sequence stars. We detect high-amplitude variability in J1840 on timescales exceeding 4000 s, with a non-sinusoidal pulse shape. Our observations also suggest that the variability is multi-periodic. The star is in a 4.6 hr binary with another compact object, most likely another WD. Future, more extensive time-series photometry of this ELM WD offers the first opportunity to probe the interior of a low-mass, presumably He-core WD using the tools of asteroseismology.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,binaries: close,Galaxy: stellar content,stars: individual: SDSS J184037.78+642312.3,stars: variables: general,white dwarfs},
  annotation = {ADS Bibcode: 2012ApJ...750L..28H},
  file = {/Users/lbugnet/Zotero/storage/XCTLBB85/Hermes et al. - 2012 - SDSS J184037.78+642312.3 The First Pulsating Extr.pdf}
}

@article{Hermes2013,
  title = {A New Class of Pulsating White Dwarf of Extremely Low Mass: The Fourth and Fifth Members},
  shorttitle = {A New Class of Pulsating White Dwarf of Extremely Low Mass},
  author = {Hermes, J. J. and Montgomery, M. H. and Gianninas, A. and Winget, D. E. and Brown, Warren R. and Harrold, Samuel T. and Bell, Keaton J. and Kenyon, Scott J. and Kilic, Mukremin and Castanheira, Barbara G.},
  year = {2013},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {436},
  pages = {3573--3580},
  issn = {0035-8711},
  doi = {10.1093/mnras/stt1835},
  urldate = {2023-10-09},
  abstract = {We report the discovery of two new pulsating extremely low-mass (ELM) white dwarfs (WDs), SDSS J161431.28+191219.4 (hereafter J1614) and SDSS J222859.93+362359.6 (hereafter J2228). Both WDs have masses {$<$}0.25 M{$\odot$} and thus likely harbour helium cores. Spectral fits indicate these are the two coolest pulsating WDs ever found. J1614 has Teff = 8880 {$\pm$} 170 K and log g = 6.66 {$\pm$} 0.14, which corresponds to a {$\sim$}0.19 M{$\odot$} WD. J2228 is considerably cooler, with a Teff = 7870 {$\pm$} 120 K and log g = 6.03 {$\pm$} 0.08, which corresponds to an {$\sim$}0.16 M{$\odot$} WD, making it the coolest and lowest mass pulsating WD known. There are multiple ELM WDs with effective temperatures between the warmest and coolest known ELM pulsators that do not pulsate to observable amplitudes, which questions the purity of the instability strip for low-mass WDs. In contrast to the CO-core ZZ Ceti stars, which are believed to represent a stage in the evolution of all such WDs, ELM WDs may not all evolve as a simple cooling sequence through an instability strip. Both stars exhibit long-period variability (1184-6235 s) consistent with non-radial g-mode pulsations. Although ELM WDs are preferentially found in close binary systems, both J1614 and J2228 do not exhibit significant radial-velocity variability, and are perhaps in low-inclination systems or have low-mass companions. These are the fourth and fifth pulsating ELM WDs known, all of which have hydrogen-dominated atmospheres, establishing these objects as a new class of pulsating WD.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,Galaxy: stellar content,Stars: individual: SDSS J161431.28+191219.4,Stars: individual: SDSS J222859.93+362359.6,Stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2013MNRAS.436.3573H},
  file = {/Users/lbugnet/Zotero/storage/288KZ4UW/Hermes et al. - 2013 - A new class of pulsating white dwarf of extremely .pdf}
}

@article{Hermes2013a,
  title = {Discovery of {{Pulsations}}, {{Including Possible Pressure Modes}}, in {{Two New Extremely Low Mass}}, {{He-core White Dwarfs}}},
  author = {Hermes, J. J. and Montgomery, M. H. and Winget, D. E. and Brown, Warren R. and Gianninas, A. and Kilic, Mukremin and Kenyon, Scott J. and Bell, Keaton J. and Harrold, Samuel T.},
  year = {2013},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {765},
  pages = {102},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/765/2/102},
  urldate = {2023-10-09},
  abstract = {We report the discovery of the second and third pulsating extremely low mass (ELM) white dwarfs (WDs), SDSS J111215.82+111745.0 (hereafter J1112) and SDSS J151826.68+065813.2 (hereafter J1518). Both have masses {$<$} 0.25 M {$\odot$} and effective temperatures below 10, 000 K, establishing these putatively He-core WDs as a cooler class of pulsating hydrogen-atmosphere WDs (DAVs, or ZZ Ceti stars). The short-period pulsations evidenced in the light curve of J1112 may also represent the first observation of acoustic (p-mode) pulsations in any WD, which provide an exciting opportunity to probe this WD in a complimentary way compared to the long-period g-modes that are also present. J1112 is a T eff =9590 {$\pm$} 140 K and log g =6.36 {$\pm$} 0.06 WD. The star displays sinusoidal variability at five distinct periodicities between 1792 and 2855 s. In this star, we also see short-period variability, strongest at 134.3 s, well short of the expected g-modes for such a low-mass WD. The other new pulsating WD, J1518, is a T eff =9900 {$\pm$} 140 K and log g =6.80 {$\pm$} 0.05 WD. The light curve of J1518 is highly non-sinusoidal, with at least seven significant periods between 1335 and 3848 s. Consistent with the expectation that ELM WDs must be formed in binaries, these two new pulsating He-core WDs, in addition to the prototype SDSS J184037.78+642312.3, have close companions. However, the observed variability is inconsistent with tidally induced pulsations and is so far best explained by the same hydrogen partial-ionization driving mechanism at work in classic C/O-core ZZ Ceti stars.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: close,Galaxy: stellar content,stars: individual: SDSS J111215.82+111745.0 SDSS J151826.68+065813.2,stars: variables: general,white dwarfs},
  annotation = {ADS Bibcode: 2013ApJ...765..102H},
  file = {/Users/lbugnet/Zotero/storage/L497YTC6/Hermes et al. - 2013 - Discovery of Pulsations, Including Possible Pressu.pdf}
}

@article{Hermes2017,
  title = {White {{Dwarf Rotation}} as a {{Function}} of {{Mass}} and a {{Dichotomy}} of {{Mode Line Widths}}: {{Kepler Observations}} of 27 {{Pulsating DA White Dwarfs}} through {{K2 Campaign}} 8},
  author = {Hermes, J. J. and G{\"a}nsicke, B. T. and Kawaler, Steven D. and Greiss, S. and Tremblay, P.-E. and Fusillo, N. P. Gentile and Raddi, R. and Fanale, S. M. and Bell, Keaton J. and Dennihy, E. and Fuchs, J. T. and Dunlap, B. H. and Clemens, J. C. and Montgomery, M. H. and Winget, D. E. and Chote, P. and Marsh, T. R. and Redfield, S.},
  year = {2017},
  month = oct,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {232},
  number = {2},
  eprint = {1709.07004},
  pages = {23},
  publisher = {{American Astronomical Society}},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/aa8bb5},
  urldate = {2020-03-09},
  abstract = {We present photometry and spectroscopy for 27 pulsating hydrogen-atmosphere white dwarfs (DAVs, a.k.a. ZZ Ceti stars) observed by the Kepler space telescope up to K2 Campaign 8, an extensive compilation of observations with unprecedented duration ({$>$}75 days) and duty cycle ({$>$}90\%). The space-based photometry reveals pulsation properties previously inaccessible to ground-based observations. We observe a sharp dichotomy in oscillation mode linewidths at roughly 800 s, such that white dwarf pulsations with periods exceeding 800 s have substantially broader mode linewidths, more reminiscent of a damped harmonic oscillator than a heat-driven pulsator. Extended Kepler coverage also permits extensive mode identification: We identify the spherical degree of 61 out of 154 unique radial orders, providing direct constraints of the rotation period for 20 of these 27 DAVs, more than doubling the number of white dwarfs with rotation periods determined via asteroseismology. We also obtain spectroscopy from 4m-class telescopes for all DAVs with Kepler photometry. Using these homogeneously analyzed spectra we estimate the overall mass of all 27 DAVs, which allows us to measure white dwarf rotation as a function of mass, constraining the endpoints of angular momentum in low- and intermediate-mass stars. We find that 0.51-to-0.73-solar-mass white dwarfs, which evolved from 1.7-to-3.0-solar-mass ZAMS progenitors, have a mean rotation period of 35 hr with a standard deviation of 28 hr, with notable exceptions for higher-mass white dwarfs. Finally, we announce an online repository for our Kepler data and follow-up spectroscopy, which we collect at http://www.k2wd.org.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6YFP7TQP/full-text.pdf;/Users/lbugnet/Zotero/storage/9VDLGWFB/Hermes_2017_ApJS_232_23.pdf}
}

@article{Hermes2017a,
  title = {A {{Deep Test}} of {{Radial Differential Rotation}} in a {{Helium-atmosphere White Dwarf}}. {{I}}. {{Discovery}} of {{Pulsations}} in {{PG}} 0112+104},
  author = {Hermes, J J and Kawaler, Steven D and {Bischoff-Kim}, A and Provencal, J L and Dunlap, B H and Clemens, J C},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {835},
  doi = {10.3847/1538-4357/835/2/277},
  urldate = {2020-03-10},
  abstract = {We present the detection of non-radial oscillations in a hot, helium-atmosphere white dwarf using 78.7 days of nearly uninterrupted photometry from the Kepler space telescope. With an effective temperature {$>$}30,000 K, PG 0112+104 becomes the hottest helium-atmosphere white dwarf known to pulsate. The rich oscillation spectrum of low-order g-modes includes clear patterns of rotational splittings from consecutive sequences of dipole and quadrupole modes, which can be used to probe the rotation rate with depth in this highly evolved stellar remnant. We also measure a surface rotation rate of 10.17404 hr from an apparent spot modulation in the K2 data. With two independent measures of rotation, PG 0112+104 provides a remarkable test of asteroseismic inference.},
  keywords = {notion,notion-database,stars: individual (PG 0112+104),stars: oscillations (including pulsations),stars: variables: general,white dwarfs},
  file = {/Users/lbugnet/Zotero/storage/M5ZARWYV/full-text.pdf}
}

@article{Hernandez2016,
  title = {Asteroseismology of 19 Low-Luminosity Red Giant Stars from {{Kepler}}},
  author = {Hern{\'a}ndez, F. P{\'e}rez and Garc{\'i}a, R. A. and Corsaro, E. and Triana, S. A. and De Ridder, J.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {591},
  eprint = {1605.01567},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/201628311},
  abstract = {Context. Frequencies of acoustic and mixed modes in red giant stars are now determined with high precision thanks to the long continuous observations provided by the NASA's Keplermission. Here we consider the eigenfrequencies of nineteen low-luminosity red giant stars selected in a recent publication for a detailed peak-bagging analysis. Aims. Our objective is to obtain stellar parameters by using individual mode frequencies and spectroscopic information. Methods. We use a forward modelling technique based on a minimization procedure combining the frequencies of the p-modes, the period spacing of the dipolar modes, and the spectroscopic data. Results. Consistent results between the forward modelling technique and values derived from the seismic scaling relations are found but the errors derived using the former technique are lower. The average error for log g is 0.002 dex, compared to 0.011 dex from the frequency of maximum power, {$\nu$}max, and 0.10 dex from the spectroscopic analysis. Relative errors in the masses and radii are on average 2\% and 0.5\% respectively, compared to 3\% and 2\% derived from the scaling relations. No reliable determination of the initial helium abundances and the mixing length parameters could be made. Finally, for our grid of models with given input physics, we found that low-mass stars require higher values of the overshooting parameter.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: general,Stars: interiors},
  file = {/Users/lbugnet/Zotero/storage/G4UDYPRG/Hernández et al. - 2016.pdf}
}

@article{Herschel1801,
  title = {Observations {{Tending}} to {{Investigate}} the {{Nature}} of the {{Sun}}, in {{Order}} to {{Find}} the {{Causes}} or {{Symptoms}} of {{Its Variable Emission}} of {{Light}} and {{Heat}}; {{With Remarks}} on the {{Use That May Possibly Be Drawn}} from {{Solar Observations}}},
  author = {Herschel, William and {William}},
  year = {1801},
  journal = {RSPT},
  volume = {91},
  pages = {265--318},
  urldate = {2020-03-13},
  keywords = {notion,notion-database}
}

@article{Herwig2005,
  title = {Evolution of {{Asymptotic Giant Branch Stars}}},
  author = {Herwig, Falk},
  year = {2005},
  month = sep,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {43},
  pages = {435--479},
  issn = {0066-4146},
  doi = {10.1146/annurev.astro.43.072103.150600},
  urldate = {2023-09-20},
  abstract = {The current status of modeling the evolution and nucleosynthesis of asymptotic giant branch (AGB) stars is reviewed. The principles of AGB evolution have been investigated in recent years leading to improved and refined models, for example with regard to hot-bottom burning or the third dredge-up. The postprocessing s-process model yields quantitative results that reproduce many observations. However, these and most other processes in AGB stars are intimately related to the physics of stellar mixing. Mixing in AGB stars is currently not well-enough understood for accurate yield predictions. Several constraints and methods are available to improve the models. Some regimes of AGB evolution have not yet been studied in sufficient detail. These include the super-AGB stars and AGB stars at extremely low or ultra low metallicity.},
  annotation = {ADS Bibcode: 2005ARA\&A..43..435H},
  file = {/Users/lbugnet/Zotero/storage/XT3YKKUJ/Herwig - 2005 - Evolution of Asymptotic Giant Branch Stars.pdf}
}

@article{Hill1994,
  title = {The Global Oscillation Network Group Site Survey - {{I}}. {{Data}} Collection and Analysis Methods},
  author = {Hill, Frank and Fischer, George and Grier, Jennifer and Leibacher, John W. and Jones, Harrison B. and Jones, Patricia P. and Kupke, Renate and Stebbins, Robin T.},
  year = {1994},
  month = jul,
  journal = {Solar Physics},
  volume = {152},
  number = {2},
  pages = {321--349},
  publisher = {{Kluwer Academic Publishers}},
  issn = {00380938},
  doi = {10.1007/BF00680443},
  urldate = {2020-03-08},
  abstract = {The Global Oscillation Network Group (GONG) Project is planning to place a set of instruments around the world to observe solar oscillations as continuously as possible for at last three years. The Project has now chosen the sites that will comprise the network. This paper describes the methods of data collection and analysis that were used to make this decision. Solar irradiance data were collected with a one-minute cadence at fifteen sites around the world and analyzed to produce statistics of cloud cover, atmospheric extinction, and transparency power spectra at the individual sites. Nearly 200 reasonable six-site networks were assembled from the individual stations, and a set of statistical measures of the performance of the networks was analyzed using a principal component analysis. An accompanying paper presents the results of the survey. \textcopyright{} 1994 Kluwer Academic Publishers.},
  keywords = {Astronomy,Atmospheric Optics,Cloud Cover,Correlation Coefficients,Extinction,Helioseismology,Irradiance,Least Squares Method,Magnetohydrodynamic Waves,Michelson Interferometers,Monte Carlo Method,notion,notion-database,Performance Prediction,Principal Components Analysis,Pyranometers,Signal To Noise Ratios,Solar Interior,Solar Oscillations,Solar Rotation,Statistical Analysis,Statistical Correlation}
}

@misc{Hoffleit1997,
  title = {History of the {{Discovery}} of {{Mira Stars}} - {{NASA}}/{{ADS}}},
  author = {{Hoffleit}},
  year = {1997},
  urldate = {2020-03-07},
  howpublished = {https://ui.adsabs.harvard.edu/abs/1997JAVSO..25..115H/abstract},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ER9CQUWX/1997JAVSO__25__115H.pdf}
}

@article{Holdsworth2014,
  title = {{{KIC}} 7582608: {{A}} New {{Kepler roAp}} Star with Frequency Variability},
  author = {Holdsworth, Daniel L. and Smalley, Barry and Kurtz, Donald W. and Southworth, John and Cunha, Margarida S. and Clubb, Kelsey I.},
  year = {2014},
  month = jun,
  eprint = {1406.7680},
  doi = {10.1093/mnras/stu1303},
  urldate = {2020-04-09},
  abstract = {We analyse the fifth roAp star reported in the Kepler field, KIC 7582608, discovered with the SuperWASP project. The object shows a high frequency pulsation at 181.7324 d\$\^\{-1\}\$ (P=7.9 min) with an amplitude of 1.45 mmag, and low frequency rotational modulation corresponding to a period of 20.4339 d with an amplitude of 7.64 mmag. Spectral analysis confirms the Ap nature of the target, with characteristic lines of Eu II, Nd III and Pr III present. The spectra are not greatly affected by broadening, which is consistent with the long rotational period found from photometry. From our spectral observations we derive a lower limit on the mean magnetic field modulus of \textbf{ = 3.05\$\textbackslash pm\$0.23 kG. Long Cadence Kepler observations show a frequency quintuplet split by the rotational period of the star, typical for an oblique pulsator. We suggest the star is a quadrupole pulsator with a geometry such that \$i\textbackslash sim66\^\textbackslash circ\$ and \$\textbackslash beta\textbackslash sim33\^\textbackslash circ\$. We detect frequency variations of the pulsation in both the WASP and Kepler data sets on many time scales. Linear, non-adiabatic stability modelling allows us to constrain a region on the HR diagram where the pulsations are unstable, an area consistent with observations.}},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Holman2010,
  title = {Kepler-9: {{A}} System of Multiple Planets Transiting a Sun-like Star, Confirmed by Timing Variations},
  author = {Holman, Matthew J. and Fabrycky, Daniel C. and Ragozzine, Darin and Ford, Eric B. and Steffen, Jason H. and Welsh, William F. and Lissauer, Jack J. and Latham, David W. and Marcy, Geoffrey W. and Walkowicz, Lucianne M. and Batalha, Natalie M. and Jenkins, Jon M. and Rowe, Jason F. and Cochran, William D. and Fressin, Francois and Torres, Guillermo and Buchhave, Lars A. and Sasselov, Dimitar D. and Borucki, William J. and Koch, David G. and Basri, Gibor and Brown, Timothy M. and Caldwell, Douglas A. and Charbonneau, David and Dunham, Edward W. and Gautier, Thomas N. and Geary, John C. and Gilliland, Ronald L. and Haas, Michael R. and Howell, Steve B. and Ciardi, David R. and Endl, Michael and Fischer, Debra and F{\"u}r{\'e}sz, G{\'a}bor and Hartman, Joel D. and Isaacson, Howard and Johnson, John A. and MacQueen, Phillip J. and Moorhead, Althea V. and Morehead, Robert C. and Orosz, Jerome A.},
  year = {2010},
  journal = {Science},
  volume = {330},
  number = {6000},
  pages = {51--54},
  issn = {00368075},
  doi = {10.1126/science.1195778},
  abstract = {The Kepler spacecraft is monitoring more than 150,000 stars for evidence of planets transiting those stars. We report the detection of two Saturn-size planets that transit the same Sun-like star, based on 7 months of Kepler observations. Their 19.2- and 38.9-day periods are presently increasing and decreasing at respective average rates of 4 and 39 minutes per orbit; in addition, the transit times of the inner body display an alternating variation of smaller amplitude. These signatures are characteristic of gravitational interaction of two planets near a 2:1 orbital resonance. Six radial-velocity observations show that these two planets are the most massive objects orbiting close to the star and substantially improve the estimates of their masses. After removing the signal of the two confirmed giant planets, we identified an additional transiting super-Earth-size planet candidate with a period of 1.6 days.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/V9ZV3NW9/Holman et al. - 2010.pdf}
}

@article{Holmberg2007,
  title = {The {{Geneva-Copenhagen}} Survey of the {{Solar}} Neighbourhood {{II New}} Uvby Calibrations and Rediscussion of Stellar Ages, the {{G}} Dwarf Problem, Age-Metallicity Diagram, and Heating Mechanisms of the Disk},
  author = {Holmberg, J. and Nordstr{\"o}m, B. and Andersen, J.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {475},
  number = {2},
  pages = {519--537},
  issn = {00046361},
  doi = {10.1051/0004-6361:20077221},
  abstract = {Context. Ages, metallicities, space velocities, and Galactic orbits of stars in the Solar neighbourhood are fundamental observational constraints on models of galactic disk evolution. Understanding and minimising systematic errors and sample selection biases in the data is crucial for their interpretation. Aims. We aim to consolidate the calibrations of uvby\ss{} photometry into Teff, [Fe/H], distance, and age for F and G stars and rediscuss the results of the Geneva-Copenhagen Survey (Nordstr\"om et al. 2004; GCS) in terms of the evolution of the disk. Methods. We use recent V - K photometry, angular diameters, high-resolution spectroscopy, Hipparcos parallaxes, and extensive numerical simulations to re-examine and verify the temperature, metallicity, distance, and reddening calibrations for the uvby\ss{} system. We also highlight the selection effects inherent in the apparent-magnitude limited GCS sample. Results. We substantially improve the Teff and [Fe/H] calibrations for early F stars, where spectroscopic temperatures have large systematic errors. A slight offset of the GCS photometry and the non-standard helium abundance of the Hyades invalidate its use for checking metallicity or age scales; however, the distances, reddenings, metallicities, and age scale for GCS field stars require minor corrections only. Our recomputed ages are in excellent agreement with the independent determinations by Takeda et al. (2007), indicating that isochrone ages can now be reliably determined. Conclusions. The revised G-dwarf metallicity distribution remains incompatible with closed-box models, and the age-metallicity relation for the thin disk remains almost flat, with large and real scatter at all ages ({$\sigma$}intrinsic = 0.20 dex). Dynamical heating of the thin disk continues throughout its life; specific in-plane dynamical effects dominate the evolution of the U and V velocities, while the W velocities remain random at all ages. When assigning thick and thin-disk membership for stars from kinematic criteria, parameters for the oldest stars should be used to characterise the thin disk. \textcopyright{} ESO 2007.},
  keywords = {Galaxy: disk,Galaxy: evolution,Galaxy: kinematics and dynamics,Galaxy: solar neighbourhood,Galaxy: stellar content,notion,notion-database,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/H7MEIDQZ/Holmberg, Nordström, Andersen - 2007.pdf}
}

@article{Hon2017,
  title = {Deep Learning Classification in Asteroseismology},
  author = {Hon, Marc and Stello, Dennis and Yu, Jie},
  year = {2017},
  journal = {MNRAS},
  volume = {469},
  pages = {4578--4583},
  doi = {10.1093/mnras/stx1174},
  urldate = {2021-01-02},
  abstract = {In the power spectra of oscillating red giants, there are visually distinct features defining stars ascending the red giant branch from those that have commenced helium core burning. We train a 1D convolutional neural network by supervised learning to automatically learn these visual features from images of folded oscillation spectra. By training and testing on Kepler red giants, we achieve an accuracy of up to 99 per cent in separating helium-burning red giants from those ascending the red giant branch. The convolutional neural network additionally shows capability in accurately predicting the evolutionary states of 5379 previously unclassified Kepler red giants, by which we now have greatly increased the number of classified stars.},
  keywords = {asteroseismology-methods,data analysis-techniques,image processing-stars,notion,notion-database,oscillations-stars,statistics},
  file = {/Users/lbugnet/Zotero/storage/9MBY9KDD/stx1174.pdf}
}

@article{Hon2018b,
  title = {Detecting {{Solar-like Oscillations}} in {{Red Giants}} with {{Deep Learning}}},
  author = {Hon, Marc and Stello, Dennis and Zinn, Joel C.},
  year = {2018},
  journal = {The Astrophysical Journal},
  volume = {859},
  number = {1},
  eprint = {1804.07495},
  pages = {64},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aabfdb},
  abstract = {Time-resolved photometry of tens of thousands of red giant stars from space missions like Kepler and K2 has created the need for automated asteroseismic analysis methods. The first and most fundamental step in such analysis, is to identify which stars show oscillations. It is critical that this step can be performed with no, or little, detection bias, particularly when performing subsequent ensemble analyses that aim to compare properties of observed stellar populations with those from galactic models. Yet, an efficient, automated solution to this initial detection step has still not been found, meaning that expert visual inspection of data from each star is required to obtain the highest level of detections. Hence, to mimic how an expert eye analyses the data, we use supervised deep learning to not only detect oscillations in red giants, but also predict the location of the frequency at maximum power, \$\textbackslash nu\_\{\textbackslash mathrm\{max\}\}\$, by observing features in 2D images of power spectra. By training on Kepler data, we benchmark our deep learning classifier against K2 data that are given detections by the expert eye, achieving a detection accuracy of 98\% on K2 Campaign 6 stars and a detection accuracy of 99\% on K2 Campaign 3 stars. We further find that the estimated uncertainty of our deep learning-based \$\textbackslash nu\_\{\textbackslash mathrm\{max\}\}\$ predictions is about 5\%. This is comparable to human-level performance using visual inspection. When examining outliers we find that the deep learning results are more likely to provide robust \$\textbackslash nu\_\{\textbackslash mathrm\{max\}\}\$ estimates than the classical model-fitting method.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,{asteroseismology,methods: data analysis,stars: osc},data analysis,including pulsations,methods,notion,notion-database,oscillations,stars,statistics},
  file = {/Users/lbugnet/Zotero/storage/M3RQRWL3/Hon, Stello, Zinn - 2018.pdf}
}

@article{Hon2018c,
  title = {Deep Learning Classification in Asteroseismology Using an Improved Neural Network: {{Results}} on 15 000 {{Kepler}} Red Giants and Applications to {{K2}} and {{TESS}} Data},
  author = {Hon, Marc and Stello, Dennis and Yu, Jie},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {476},
  number = {3},
  eprint = {1802.07260},
  pages = {3233--3244},
  issn = {13652966},
  doi = {10.1093/MNRAS/STY483},
  abstract = {Deep learning in the form of 1D convolutional neural networks have previously been shown to be capable of efficiently classifying the evolutionary state of oscillating red giants into red giant branch stars and helium-core burning stars by recognizing visual features in their asteroseismic frequency spectra. We elaborate further on the deep learning method by developing an improved convolutional neural network classifier. To make our method useful for current and future space missions such as K2, TESS, and PLATO, we train classifiers that are able to classify the evolutionary states of lower frequency resolution spectra expected from these missions. Additionally, we provide new classifications for 8633 Kepler red giants, out of which 426 have previously not been classified using asteroseismology. This brings the total to 14983 Kepler red giants classified with our new neural network. We also verify that our classifiers are remarkably robust to suboptimal data, including low signal-to-noise and incorrect training truth labels.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: evolution,Stars: oscillations,Stars: statistics},
  file = {/Users/lbugnet/Zotero/storage/2BXA3LRT/Hon, Stello, Yu - 2018.pdf}
}

@article{Hon2019,
  title = {A Search for Red Giant Solar-like Oscillations in All {{Kepler}} Data},
  author = {Hon, Marc and Stello, Dennis and Garc{\'i}a, Rafael A and Mathur, Savita and Sharma, Sanjib and Colman, Isabel L and Bugnet, Lisa},
  year = {2019},
  journal = {MNRAS},
  volume = {485},
  pages = {5616--5630},
  doi = {10.1093/mnras/stz622},
  urldate = {2020-01-16},
  abstract = {The recently published Kepler mission Data Release 25 (DR25) reported on {$\sim$}197 000 targets observed during the mission. Despite this, no wide search for red giants showing solar-like oscillations have been made across all stars observed in Kepler's long-cadence mode. In this work, we perform this task using custom apertures on the Kepler pixel files and detect oscillations in 21 914 stars, representing the largest sample of solar-like oscillating stars to date. We measure their frequency at maximum power, {$\nu$} max , down to {$\nu$} max 4 {$\mu$}Hz and obtain log (g) estimates with a typical uncertainty below 0.05 dex, which is superior to typical measurements from spectroscopy. Additionally, the {$\nu$} max distribution of our detections show good agreement with results from a simulated model of the Milky Way, with a ratio of observed to predicted stars of 0.992 for stars with 10 {$<$} {$\nu$} max {$<$} 270 {$\mu$}Hz. Among our red giant detections, we find 909 to be dwarf/subgiant stars whose flux signal is polluted by a neighbouring giant as a result of using larger photometric apertures than those used by the NASA Kepler science processing pipeline. We further find that only 293 of the polluting giants are known Kepler targets. The remainder comprises over 600 newly identified oscillating red giants, with many expected to belong to the Galactic halo, serendipitously falling within the Kepler pixel files of targeted stars.},
  keywords = {asteroseismology-methods,data analysis-techniques,image processing-stars,notion,notion-database,oscillations-stars,statistics},
  file = {/Users/lbugnet/Zotero/storage/9QU4NBHK/full-text.pdf}
}

@misc{honSearchRedGiant2019,
  title = {A Search for Red Giant Solar-like Oscillations in All Kepler Data},
  author = {Hon, M. and Stello, D. and Garc{\'i}a, R.A. and Mathur, S. and Sharma, S. and Colman, I.L. and Bugnet, L.},
  year = {2019},
  journal = {arXiv},
  abstract = {Copyright \textcopyright{} 2019, arXiv, All rights reserved. The recently published Kepler mission Data Release 25 (DR25) reported on {$\sim$}197, 000 targets observed during the mission. Despite this, no wide search for red giants showing solar-like oscillations have been made across all stars observed in Kepler's long-cadence mode. In this work, we perform this task using custom apertures on the Kepler pixel files and detect oscillations in 21, 914 stars, representing the largest sample of solar-like oscillating stars to date. We measure their frequency at maximum power, vmax, down to vmax{$\simeq$} 4{$\mu$}Hz and obtain log(g) estimates with a typical uncertainty below 0.05 dex, which is superior to typical measurements from spectroscopy. Additionally, the vmaxdistribution of our detections show good agreement with results from a simulated model of the Milky Way, with a ratio of observed to predicted stars of 0.992 for stars with 10{$\mu$}Hz {$<$} vmax{$<$} 270{$\mu$}Hz. Among our red giant detections, we find 909 to be dwarf/subgiant stars whose flux signal is polluted by a neighbouring giant as a result of using larger photometric apertures than those used by the NASA Kepler Science Processing Pipeline. We further find that only 293 of the polluting giants are known Kepler targets. The remainder comprises over 600 newly identified oscillating red giants, with many expected to belong to the galactic halo, serendipitously falling within the Kepler pixel files of targeted stars.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations,Stars: statistics,Techniques: image processing}
}

@article{Horch2014,
  title = {{{MOST}} Sub-Arcsecond Companions of {{Kepler}} Exoplanet Candidate Host Stars Are Gravitationally Bound},
  author = {Horch, Elliott P. and Howell, Steve B. and Everett, Mark E. and Ciardi, David R.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {795},
  number = {1},
  eprint = {1409.1249},
  pages = {1--23},
  issn = {15384357},
  doi = {10.1088/0004-637X/795/1/60},
  abstract = {Using the known detection limits for high-resolution imaging observations and the statistical properties of true binary and line-of-sight companions, we estimate the binary fraction of Kepler exoplanet host stars. Our speckle imaging programs at the WIYN 3.5 m and Gemini North 8.1 m telescopes have observed over 600 Kepler objects of interest and detected 49 stellar companions within 1 arcsec. Assuming binary stars follow a log-normal period distribution for an effective temperature range of 3000-10,000 K, then the model predicts that the vast majority of detected sub-arcsecond companions are long period (P {$>$} 50 yr), gravitationally bound companions. In comparing the model predictions to the number of real detections in both observational programs, we conclude that the overall binary fraction of host stars is similar to the 40\%-50\% rate observed for field stars.},
  archiveprefix = {arxiv},
  keywords = {Binaries: visual,notion,notion-database,Planetary systems,Stars: solar-type,Techniques: high angular resolution,Techniques: interferometric,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/XSQNTN6T/Horch et al. - 2014.pdf}
}

@article{Hotta2017,
  title = {Solar Overshoot Region and Small-Scale Dynamo with Realistic Energy Flux},
  author = {Hotta, H.},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {843},
  number = {1},
  eprint = {1706.06413},
  pages = {52},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/aa784b},
  abstract = {We carry out high resolution calculations of the solar overshoot region with unprecedentedly realistic parameters, especially the small energy flux compared with {$\rho$}c3s, where {$\rho$} and cs are density and speed of sound. Our main purpose is to investigate behavior of the overshoot and the small-scale dynamo with parameters as close as possible to thoes of the Sun. Our calculations show that the bottom part of the convection zone becomes subadiabatic, which efficiently suppresses downflows. As a result we see a steep transition from the CZ to the RZ whose width is estimated 0.4\% of the local pressure scale height. This result is consistent with a semi-analytic convection/overshoot model. We also find that the small-scale dynamo becomes efficient with a smaller energy flux. The sudden suppression of the downflows around the base of the convection zone increases the efficiency of the small-scale dynamo.},
  archiveprefix = {arxiv},
  keywords = {animation,dynamo,interior,interiors,notion,notion-database,stars,stars: interiors,sun,Sun: interior,supporting material,turbulence},
  file = {/Users/lbugnet/Zotero/storage/LJJKW5PF/Hotta_2017_The%20Astrophysical%20Journal_Solar%20Overshoot%20Region%20and%20Small-scale%20Dynamo%20with%20Realistic%20Energy%20Flux.pdf}
}

@article{Houdek2001,
  title = {Changes in Convective Properties over the Solar Cycle: {{Effect}} on p-Mode Damping Rates},
  author = {Houdek, G. and Chaplin, W. J. and Appourchaux, T. and {Christensen-Dalsgaard}, J. and D{\"a}ppen, W. and Elsworth, Y. and Gough, D. O. and Isaak, G. R. and New, R. and {Rabello-Soares}, M. C.},
  year = {2001},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {327},
  number = {2},
  pages = {483--487},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2001.04749.x},
  abstract = {Measurements of both solar irradiance and p-mode oscillation frequencies indicate that the structure of the Sun changes with the solar cycle. Balmforth, Gough \& Merryfield investigated the effect of symmetrical thermal disturbances on the solar structure and the resulting pulsation frequency changes. They concluded that thermal perturbations alone cannot account for the variations in both irradiance and p-mode frequencies, and that the presence of a magnetic field affecting acoustical propagation is the most likely explanation of the frequency change, in the manner suggested earlier by Gough \& Thompson and by Goldreich et al. Numerical simulations of Boussinesq convection in a magnetic field have shown that at high Rayleigh number the magnetic field can modify the preferred horizontal length scale of the convective flow. Here, we investigate the effect of changing the horizontal length scale of convective eddies on the linewidths of the acoustic resonant mode peaks observed in helioseismic power spectra. The turbulent fluxes in these model computations are obtained from a time-dependent, non-local generalization of the mixing-length formalism. The modelled variations are compared with p-mode linewidth changes revealed by the analysis of helioseismic data collected by the Birmingham Solar-Oscillations Network (BiSON); these low-degree (low-l) observations cover the complete falling phase of solar activity cycle 22. The results are also discussed in the light of observations of solar-cycle variations of the horizontal size of granules and with results from 2D simulations by Steffen of convective granules.},
  keywords = {Convection,notion,notion-database,Sun: activity,Sun: granulation,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/BHMJCDN3/Houdek et al. - 2001.pdf}
}

@article{Houdek2002,
  title = {Modelling Pulsation Amplitudes of {$\xi$} {{Hydrae}} 2 {{M O D E L C O M P U TAT I O N S}}},
  author = {Houdek, G and Gough, D O},
  year = {2002},
  volume = {69},
  keywords = {convection,individual,notion,notion-database,oscillations,stars,{$\xi$} hya},
  file = {/Users/lbugnet/Zotero/storage/EZL4SLMS/Houdek, Gough - 2002.pdf}
}

@article{Houdek2011,
  title = {On the Seismic Age and Heavy-Element Abundance of the {{Sun}}},
  author = {Houdek, G. and Gough, D. O.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {418},
  number = {2},
  pages = {1217--1230},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.19572.x},
  abstract = {We estimate the main-sequence age and heavy-element abundance of the Sun by means of an asteroseismic calibration of theoretical solar models using only low-degree acoustic modes from the BiSON. The method can therefore be applied also to other solar-type stars, such as those observed by the NASA satellite Kepler and the planned ground-based Danish-led Stellar Observations Network Group (SONG). The age, 4.60 {$\pm$} 0.04 Gyr, obtained with this new seismic method, is similar to, although somewhat greater than, today's commonly adopted values, and the surface heavy-element abundance by mass, Zs= 0.0142 {$\pm$} 0.0005, lies between the values quoted recently by Asplund et al. and by Caffau et al. We stress that our best-fitting model is not a seismic model, but a theoretically evolved model of the Sun constructed with 'standard' physics and calibrated against helioseismic data. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations,Sun: abundances,Sun: fundamental parameters,Sun: interior,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/FTLJH5YA/Houdek, Gough - 2011.pdf}
}

@article{Houdek2015a,
  title = {Interaction between Convection and Pulsation},
  author = {Houdek, G{\"u}nter and Dupret, Marc Antoine},
  year = {2015},
  journal = {Living Reviews in Solar Physics},
  volume = {12},
  number = {1},
  eprint = {1601.03913},
  issn = {16144961},
  doi = {10.1007/lrsp-2015-8},
  abstract = {This article reviews our current understanding of modelling convection dynamics in stars. Several semi-analytical time-dependent convection models have been proposed for pulsating one-dimensional stellar structures with different formulations for how the convective turbulent velocity field couples with the global stellar oscillations. In this review we put emphasis on two, widely used, time-dependent convection formulations for estimating pulsation properties in one-dimensional stellar models. Applications to pulsating stars are presented with results for oscillation properties, such as the effects of convection dynamics on the oscillation frequencies, or the stability of pulsation modes, in classical pulsators and in stars supporting solar-type oscillations.},
  archiveprefix = {arxiv},
  keywords = {Mode physics,notion,notion-database,Stellar convection,Time-dependent convection},
  file = {/Users/lbugnet/Zotero/storage/RDWYB5DB/Houdek, Dupret - 2015.pdf}
}

@article{Hough1898,
  title = {V. {{On}} the Application of Harmonic Analysis to the Dynamical Theory of the Tides.\textemdash{{Part II}}. {{On}} the General Integration of {{Laplace}}'s Dynamical Equations},
  author = {{Hough}},
  year = {1898},
  month = dec,
  journal = {Philosophical Transactions of the Royal Society of London. Series A, Containing Papers of a Mathematical or Physical Character},
  volume = {191},
  pages = {139--185},
  publisher = {{The Royal Society London}},
  issn = {0264-3952},
  doi = {10.1098/RSTA.1898.0005},
  urldate = {2021-12-22},
  abstract = {In the former paper on this subject I have dealt with the formation of Laplace's dynamical equation for the tides, and the integration of it, subject to the limitation that the solutions obtained s...},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CQEVZHYT/full-text.pdf}
}

@article{Howe2009,
  title = {A Note on the Torsional Oscillation at Solar Minimum},
  author = {Howe, R. and {Christensen-Dalsgaard}, J. and Hill, F. and Komm, R. and Schou, J. and Thompson, M. J.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {701},
  number = {2 PART 2},
  eprint = {0907.2965},
  pages = {1--10},
  issn = {15384357},
  doi = {10.1088/0004-637X/701/2/L87},
  abstract = {We examine the evolution of the zonal flow pattern in the upper solar convection zone during the current extended solar minimum, and compare it with that during the previous minimum. The results suggest that a configuration matching that at the previous minimum was reached during 2008, but that the flow band corresponding to the new cycle has been moving more slowly toward the equator than was observed in the previous cycle, resulting in a gradual increase in the apparent length of the cycle during the 2007-2008 period. The current position of the lower-latitude fast-rotating belt corresponds to that seen around the onset of activity in the previous cycle. \textcopyright{} 2009. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/I4CK3HNN/Howe et al. - 2009.pdf}
}

@article{Howe2013,
  title = {Low-Degree Multi-Spectral p-Mode Fitting},
  author = {Howe, Rachel and Broomhall, Anne Marie and Chaplin, William James and Elsworth, Yvonne and Jain, Kiran},
  year = {2013},
  journal = {Journal of Physics: Conference Series},
  volume = {440},
  number = {012011},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SSPBTI3X/Howe et al. - 2013.pdf}
}

@article{Howe2015a,
  title = {Validation of Solar-Cycle Changes in Low-Degree Helioseismic Parameters from the {{Birmingham Solar-Oscillations Network}}},
  author = {Howe, R. and Davies, G. R. and Chaplin, W. J. and Elsworth, Y. P. and Hale, S. J.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {454},
  number = {4},
  pages = {4120--4141},
  issn = {13652966},
  doi = {10.1093/mnras/stv2210},
  abstract = {We present a new and up-to-date analysis of the solar low-degree p-mode parameter shifts from the Birmingham Solar-Oscillations Network over the past 22 years, up to the end of 2014. We aim to demonstrate that they are not dominated by changes in the asymmetry of the resonant peak profiles of the modes and that the previously published results on the solarcycle variations of mode parameters are reliable. We compare the results obtained using a conventional maximum-likelihood estimation algorithm and a new one based on the Markov ChainMonte Carlo (MCMC) technique, both taking into account mode asymmetry.We assess the reliability of the solar-cycle trends seen in the data by applying the same analysis to artificially generated spectra. We find that the two methods are in good agreement. Both methods accurately reproduce the input frequency shifts in the artificial data and underestimate the amplitude and width changes by a small amount, around 10 per cent. We confirm earlier findings that the frequency and line width are positively correlated, and the mode amplitude anticorrelated, with the level of solar activity, with the energy supplied to the modes remaining essentially unchanged. For the mode asymmetry the correlation with activity is marginal, but the MCMC algorithm gives more robust results than the MLE (Maximum-Likelihood Estimate). The magnitude of the parameter shifts is consistent with earlier work. There is no evidence that the frequency changes we see arise from changes in the asymmetry, which would need to be much larger than those observed in order to give the observed frequency shift.},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VJQ27JJP/Howe et al. - 2015.pdf}
}

@article{Howell2012,
  title = {{{KEPLER-21b}}: {{A}} 1.6 {{REarth}} Planet Transiting the Bright Oscillating {{F}} Subgiant Star {{HD179070}}},
  author = {Howell, Steve B. and Rowe, Jason F. and Bryson, Stephen T. and Quinn, Samuel N. and Marcy, Geoffrey W. and Isaacson, Howard and Ciardi, David R. and Chaplin, William J. and Metcalfe, Travis S. and Monteiro, Mario J.P.F.G. and Appourchaux, Thierry and Basu, Sarbani and Creevey, Orlagh L. and Gilliland, Ronald L. and Quirion, Pierre Olivier and Stello, Denis and Kjeldsen, Hans and {Christensen-Dalsgaard}, J{\"o}rgen and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Houdek, G{\"u}nter and Karoff, Christoffer and {Molenda-Akowicz}, Joanna and Thompson, Michael J. and Verner, Graham A. and Torres, Guillermo and Fressin, Francois and Crepp, Justin R. and Adams, Elisabeth and Dupree, Andrea and Sasselov, Dimitar D. and Dressing, Courtney D. and Borucki, William J. and Koch, David G. and Lissauer, Jack J. and Latham, David W. and Buchhave, Lars A. and Gautier, Thomas N. and Everett, Mark and Horch, Elliott and Batalha, Natalie M. and Dunham, Edward W. and Szkody, Paula and Silva, David R. and Mighell, Ken and Holberg, Jay and Ballot, Jerme and Bedding, Timothy R. and Bruntt, Hans and Campante, Tiago L. and Handberg, Rasmus and Hekker, Saskia and Huber, Daniel and Mathur, Savita and Mosser, Benoit and R{\'e}gulo, Clara and White, Timothy R. and Christiansen, Jessie L. and Middour, Christopher K. and Haas, Michael R. and Hall, Jennifer R. and Jenkins, Jon M. and McCaulif, Sean and Fanelli, Michael N. and Kulesa, Craig and McCarthy, Don and Henze, Christopher E.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {746},
  number = {2},
  issn = {15384357},
  doi = {10.1088/0004-637X/746/2/123},
  abstract = {We present Kepler observations of the bright (V = 8.3), oscillating star HD179070. The observations show transit-like events which reveal that the star is orbited every 2.8days by a small, 1.6 R Earth object. Seismic studies of HD179070 using short cadence Kepler observations show that HD179070 has a frequency-power spectrum consistent with solar-like oscillations that are acoustic p-modes. Asteroseismic analysis provides robust values for the mass and radius of HD179070, 1.34 {$\pm$} 0.06 M {$\odot$} and 1.86 {$\pm$} 0.04 R {$\odot$}, respectively, as well as yielding an age of 2.84 {$\pm$} 0.34Gyr for this F5 subgiant. Together with ground-based follow-up observations, analysis of the Kepler light curves and image data, and blend scenario models, we conservatively show at the {$>$}99.7\% confidence level (3{$\sigma$}) that the transit event is caused by a 1.64 0.04 R Earth exoplanet in a 2.785755 {$\pm$} 0.000032day orbit. The exoplanet is only 0.04 AU away from the star and our spectroscopic observations provide an upper limit to its mass of {$\sim$}10 M Earth (2{$\sigma$}). HD179070 is the brightest exoplanet host star yet discovered by Kepler. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,planetary systems,stars: activity,stars: individual (HD 179070: KIC 3632418),stars: interiors,stars: late-type,stars: magnetic field,stars: oscillations (including pulsations),techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/DPN5AJHP/Howell et al. - 2012.pdf}
}

@article{Howell2014a,
  title = {The {{K2 Mission}}: {{Characterization}} and {{Early Results}}},
  author = {Howell, Steve B. and Sobeck, Charlie and Haas, Michael and Still, Martin and Barclay, Thomas and Mullally, Fergal and Troeltzsch, John and Aigrain, Suzanne and Bryson, Stephen T. and Caldwell, Doug and Chaplin, William J. and Cochran, William D. and Huber, Daniel and Marcy, Geoffrey W. and Miglio, Andrea and Najita, Joan R. and Smith, Marcie and Twicken, J. D. and Fortney, Jonathan J.},
  year = {2014},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {126},
  number = {938},
  eprint = {1402.5163},
  pages = {398--408},
  issn = {00046280},
  doi = {10.1086/676406},
  abstract = {The K2 mission will make use of the Kepler spacecraft and its assets to expand upon Kepler's groundbreaking discoveries in the fields of exoplanets and astrophysics through new and exciting observations. K2 will use an innovative way of operating the spacecraft to observe target fields along the ecliptic for the next 2-3 years. Early science commissioning observations have shown an estimated photometric precision near 400 ppm in a single 30 minute observation, and a 6-hour photometric precision of 80 ppm (both at V=12). The K2 mission offers long-term, simultaneous optical observation of thousands of objects at a precision far better than is achievable from ground-based telescopes. Ecliptic fields will be observed for approximately 75-days enabling a unique exoplanet survey which fills the gaps in duration and sensitivity between the Kepler and TESS missions, and offers pre-launch exoplanet target identification for JWST transit spectroscopy. Astrophysics observations with K2 will include studies of young open clusters, bright stars, galaxies, supernovae, and asteroseismology.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SV5X8F8D/Howell et al. - 2014.pdf}
}

@article{Huber2010a,
  title = {Asteroseismology of Red Giants from the First Four Months of {{Kepler}} Data: {{Global}} Oscillation Parameters for 800 Stars},
  author = {Huber, D. and Bedding, T. R. and Stello, D. and Mosser, B. and Mathur, S. and Kallinger, T. and Hekker, S. and Elsworth, Y. P. and Buzasi, D. L. and De Ridder, J. and Gilliland, R. L. and Kjeldsen, H. and Chaplin, W. J. and Garc{\'i}a, R. A. and Hale, S. J. and Preston, H. L. and White, T. R. and Borucki, W. J. and {Christensen-Dalsgaard}, J. and Clarke, B. D. and Jenkins, J. M. and Koch, D.},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {723},
  number = {2},
  eprint = {1010.4566},
  pages = {1607--1617},
  issn = {15384357},
  doi = {10.1088/0004-637X/723/2/1607},
  abstract = {We have studied solar-like oscillations in {$\sim$}800 red giant stars using Kepler long-cadence photometry. The sample includes stars ranging in evolution from the lower part of the red giant branch to the helium main sequence. We investigate the relation between the large frequency separation ({$\Delta\nu$}) and the frequency of maximum power ({$\nu$}max) and show that it is different for red giants than for main-sequence stars, which is consistent with evolutionary models and scaling relations. The distributions of {$\nu$}max and {$\Delta\nu$} are in qualitative agreement with a simple stellar population model of the Kepler field, including the first evidence for a secondary clump population characterized by M {$\greaterequivlnt$} 2M{$\odot$} and {$\nu$}max {$\simeq$} 40-110 {$\mu$}Hz. We measured the small frequency separations {$\delta\nu$}02 and {$\delta\nu$}01 in over 400 stars and {$\delta\nu$}03 in over 40. We present C-D diagrams for l = 1,2, and 3 and show that the frequency separation ratios {$\delta\nu$} 02/{$\Delta\nu$} and {$\delta\nu$}01/{$\Delta\nu$} have opposite trends as a function of {$\Delta\nu$}. The data show a narrowing of the l=1 ridge toward lower {$\nu$}max, in agreement with models predicting more efficient mode trapping in stars with higher luminosity. We investigate the offset {$\in$} in the asymptotic relation and find a clear correlation with {$\Delta\nu$}, demonstrating that it is related to fundamental stellar parameters. Finally, we present the first amplitude-vmax relation for Kepler red giants. We observe a lack of low-amplitude stars for {$\nu$}max {$\greaterequivlnt$} 110 {$\mu$}Hz and find that, for a given {$\nu$}max between 40 and 110 {$\nu$}Hz, stars with lower {$\Delta\nu$} (and consequently higher mass) tend to show lower amplitudes than stars with higher {$\Delta\nu$}. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/663R9XQV/Huber et al. - 2010(2).pdf;/Users/lbugnet/Zotero/storage/M5AHL96Y/Huber et al. - 2010.pdf}
}

@article{Huber2011,
  title = {Solar-like Oscillations and Activity in {{Procyon}}: {{A}} Comparison of the 2007 Most and Ground-Based Radial Velocity Campaigns},
  author = {Huber, Daniel and Bedding, Timothy R. and Arentoft, Torben and Gruberbauer, Michael and Guenther, David B. and Houdek, G{\"u}nter and Kallinger, Thomas and Kjeldsen, Hans and Matthews, Jaymie M. and Stello, Dennis and Weiss, Werner W.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {731},
  number = {2},
  eprint = {1102.2894},
  issn = {15384357},
  doi = {10.1088/0004-637X/731/2/94},
  abstract = {We compare the simultaneous 2007 space-based MOST photometry and ground-based radial velocity (RV) observations of the F5 star Procyon. We identify slow variations in the MOST data that are similar to those reported in the RV time series and confirm by comparison with the Sun that these variations are likely the signature of stellar activity. The MOST power spectrum yields clear evidence for individual oscillation frequencies that match those found in the RV data by Bedding etal. We identify the same ridges due to modes of different spherical degree in both data sets, but are not able to confirm a definite ridge identification using the MOST data. We measure the luminosity amplitude per radial mode A l=0,phot = 9.1 {$\pm$} 0.5ppm. Combined with the estimate for the RV data by Arentoft etal., this gives a mean amplitude ratio of A l=0,phot/A l=0,RV = 0.24 {$\pm$} 0.02ppm cm-1s, considerably higher than expected from scaling relations but in reasonable agreement with theoretical models by Houdek. We also compare the amplitude ratio as a function of frequency and find that the maximum of the oscillation envelope is shifted to higher frequencies in photometry than in velocity. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: activity,stars: individual (Procyon),stars: oscillations,stars: rotation,techniques: photometric,techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/RX4PNL3G/Huber et al. - 2011.pdf}
}

@article{Huber2011b,
  title = {Testing Scaling Relations for Solar-like Oscillations from the Main Sequence to Red Giants Using Kepler Data},
  author = {Huber, D. and Bedding, T. R. and Stello, D. and Hekker, S. and Mathur, S. and Mosser, B. and Verner, G. A. and Bonanno, A. and Buzasi, D. L. and Campante, T. L. and Elsworth, Y. P. and Hale, S. J. and Kallinger, T. and Silva Aguirre, V. and Chaplin, W. J. and De Ridder, J. and Garc{\'i}a, R. A. and Appourchaux, T. and Frandsen, S. and Houdek, G. and {Molenda-Zakowicz}, J. and Monteiro, M. J.P.F.G. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kawaler, S. D. and Kjeldsen, H. and Broomhall, A. M. and Corsaro, E. and Salabert, D. and Sanderfer, D. T. and Seader, S. E. and Smith, J. C.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {743},
  number = {2},
  eprint = {1109.3460},
  issn = {15384357},
  doi = {10.1088/0004-637X/743/2/143},
  abstract = {We have analyzed solar-like oscillations in 1700 stars observed by the Kepler Mission, spanning from the main sequence to the red clump. Using evolutionary models, we test asteroseismic scaling relations for the frequency of maximum power ({$\nu$}max), the large frequency separation ({$\Delta\nu$}), and oscillation amplitudes. We show that the difference of the {$\Delta\nu$}-{$\nu$}max relation for unevolved and evolved stars can be explained by different distributions in effective temperature and stellar mass, in agreement with what is expected from scaling relations. For oscillation amplitudes, we show that neither (L/M)s scaling nor the revised scaling relation by Kjeldsen \& Bedding is accurate for red-giant stars, and demonstrate that a revised scaling relation with a separate luminosity-mass dependence can be used to calculate amplitudes from the main sequence to red giants to a precision of 25\%. The residuals show an offset particularly for unevolved stars, suggesting that an additional physical dependency is necessary to fully reproduce the observed amplitudes. We investigate correlations between amplitudes and stellar activity, and find evidence that the effect of amplitude suppression is most pronounced for subgiant stars. Finally, we test the location of the cool edge of the instability strip in the Hertzsprung-Russell diagram using solar-like oscillations and find the detections in the hottest stars compatible with a domain of hybrid stochastically excited and opacity driven pulsation. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: late-type,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/PKAMYUGI/Huber et al. - 2011(2).pdf}
}

@article{Huber2012a,
  title = {Fundamental Properties of Stars Using Asteroseismology from {{Kepler}} and {{CoRoT}} and Interferometry from the {{CHARA Array}}},
  author = {Huber, D. and Ireland, M. J. and Bedding, T. R. and Brand{\~a}o, I. M. and Piau, L. and Maestro, V. and White, T. R. and Bruntt, H. and Casagrande, L. and {Molenda-Zakowicz}, J. and Silva Aguirre, V. and Sousa, S. G. and Barclay, T. and Burke, C. J. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Cunha, M. S. and De Ridder, J. and Farrington, C. D. and Frasca, A. and Garc{\'i}a, R. A. and Gilliland, R. L. and Goldfinger, P. J. and Hekker, S. and Kawaler, S. D. and Kjeldsen, H. and McAlister, H. A. and Metcalfe, T. S. and Miglio, A. and Monteiro, M. J.P.F.G. and Pinsonneault, M. H. and Schaefer, G. H. and Stello, D. and Stumpe, M. C. and Sturmann, J. and Sturmann, L. and Ten Brummelaar, T. A. and Thompson, M. J. and Turner, N. and Uytterhoeven, K.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {760},
  number = {1},
  eprint = {1210.0012},
  issn = {15384357},
  doi = {10.1088/0004-637X/760/1/32},
  abstract = {We present results of a long-baseline interferometry campaign using the PAVO beam combiner at the CHARA Array to measure the angular sizes of five main-sequence stars, one subgiant and four red giant stars for which solar-like oscillations have been detected by either Kepler or CoRoT. By combining interferometric angular diameters, Hipparcos parallaxes, asteroseismic densities, bolometric fluxes, and high-resolution spectroscopy, we derive a full set of near-model-independent fundamental properties for the sample. We first use these properties to test asteroseismic scaling relations for the frequency of maximum power ({$\nu$}max) and the large frequency separation ({$\Delta\nu$}). We find excellent agreement within the observational uncertainties, and empirically show that simple estimates of asteroseismic radii for main-sequence stars are accurate to {$\lessequivlnt$} 4\%. We furthermore find good agreement of our measured effective temperatures with spectroscopic and photometric estimates with mean deviations for stars between T eff = 4600-6200 K of -22 {$\pm$} 32 K (with a scatter of 97K) and -58 {$\pm$} 31 K (with a scatter of 93K), respectively. Finally, we present a first comparison with evolutionary models, and find differences between observed and theoretical properties for the metal-rich main-sequence star HD173701. We conclude that the constraints presented in this study will have strong potential for testing stellar model physics, in particular when combined with detailed modeling of individual oscillation frequencies. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: late-type,stars: oscillations (including pulsations),techniques: interferometric,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/Y393DRNA/Huber et al. - 2012.pdf}
}

@article{Huber2013a,
  title = {Stellar Spin-Orbit Misalignment in a Multiplanet System},
  author = {Huber, Daniel and Carter, Joshua A. and Barbieri, Mauro and Miglio, Andrea and Deck, Katherine M. and Fabrycky, Daniel C. and Montet, Benjamin T. and Buchhave, Lars A. and Chaplin, William J. and Hekker, Saskia and Montalb{\'a}n, Josefina and {Sanchis-Ojeda}, Roberto and Basu, Sarbani and Bedding, Timothy R. and Campante, Tiago L. and {Christensen-Dalsgaard}, J{\o}rgen and Elsworth, Yvonne P. and Stello, Dennis and Arentoft, Torben and Ford, Eric B. and Gilliland, Ronald L. and Handberg, Rasmus and Howard, Andrew W. and Isaacson, Howard and Johnson, John Asher and Karoff, Christoffer and Kawaler, Steven D. and Kjeldsen, Hans and Latham, David W. and Lund, Mikkel N. and Lundkvist, Mia and Marcy, Geoffrey W. and Metcalfe, Travis S. and Aguirre, Victor Silva and Winn, Joshua N.},
  year = {2013},
  journal = {Science},
  volume = {342},
  number = {6156},
  eprint = {1310.4503},
  pages = {331--334},
  issn = {10959203},
  doi = {10.1126/science.1242066},
  abstract = {Stars hosting hot Jupiters are often observed to have high obliquities, whereas stars with multiple coplanar planets have been seen to have low obliquities. This has been interpreted as evidence that hot-Jupiter formation is linked to dynamical disruption, as opposed to planet migration through a protoplanetary disk. We used asteroseismology to measure a large obliquity for Kepler-56, a red giant star hosting two transiting coplanar planets. These observations show that spin-orbit misalignments are not confined to hot-Jupiter systems. Misalignments in a broader class of systems had been predicted as a consequence of torques from wide-orbiting companions, and indeed radial velocity measurements revealed a third companion in a wide orbit in the Kepler-56 system.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KVVG4V8U/Huber et al. - 2013.pdf}
}

@article{Huber2013c,
  title = {Fundamental Properties of Kepler Planet-Candidate Host Stars Using Asteroseismology},
  author = {Huber, Daniel and Chaplin, William J. and {Christensen-Dalsgaard}, J{\o}rgen and Gilliland, Ronald L. and Kjeldsen, Hans and Buchhave, Lars A. and Fischer, Debra A. and Lissauer, Jack J. and Rowe, Jason F. and {Sanchis-Ojeda}, Roberto and Basu, Sarbani and Handberg, Rasmus and Hekker, Saskia and Howard, Andrew W. and Isaacson, Howard and Karoff, Christoffer and Latham, David W. and Lund, Mikkel N. and Lundkvist, Mia and Marcy, Geoffrey W. and Miglio, Andrea and Silva Aguirre, Victor and Stello, Dennis and Arentoft, Torben and Barclay, Thomas and Bedding, Timothy R. and Burke, Christopher J. and Christiansen, Jessie L. and Elsworth, Yvonne P. and Haas, Michael R. and Kawaler, Steven D. and Metcalfe, Travis S. and Mullally, Fergal and Thompson, Susan E.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {767},
  number = {2},
  eprint = {1302.2624},
  issn = {15384357},
  doi = {10.1088/0004-637X/767/2/127},
  abstract = {We have used asteroseismology to determine fundamental properties for 66 Kepler planet-candidate host stars, with typical uncertainties of 3\% and 7\% in radius and mass, respectively. The results include new asteroseismic solutions for four host stars with confirmed planets (Kepler-4, Kepler-14, Kepler-23 and Kepler-25) and increase the total number of Kepler host stars with asteroseismic solutions to 77. A comparison with stellar properties in the planet-candidate catalog by Batalha et al. shows that radii for subgiants and giants obtained from spectroscopic follow-up are systematically too low by up to a factor of 1.5, while the properties for unevolved stars are in good agreement. We furthermore apply asteroseismology to confirm that a large majority of cool main-sequence hosts are indeed dwarfs and not misclassified giants. Using the revised stellar properties, we recalculate the radii for 107 planet candidates in our sample, and comment on candidates for which the radii change from a previously giant-planet/brown-dwarf/stellar regime to a sub-Jupiter size or vice versa. A comparison of stellar densities from asteroseismology with densities derived from transit models in Batalha et al. assuming circular orbits shows significant disagreement for more than half of the sample due to systematics in the modeled impact parameters or due to planet candidates that may be in eccentric orbits. Finally, we investigate tentative correlations between host-star masses and planet-candidate radii, orbital periods, and multiplicity, but caution that these results may be influenced by the small sample size and detection biases. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,planetary systems,stars: late-type,stars: oscillations,techniques: photometric,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/RABF5YNM/Huber et al. - 2013(2).pdf}
}

@article{Huber2014,
  title = {{{REVISED STELLAR PROPERTIES OF KEPLER TARGETS FOR THE QUARTER}} 1-16 {{TRANSIT DETECTION RUN}}},
  author = {Huber, Daniel and Aguirre, Victor Silva and Matthews, Jaymie M and Pinsonneault, Marc H and Gaidos, Eric and Garc{\'i}a, Rafael A and Hekker, Saskia and Mathur, Savita and Mosser, Beno{\textasciicircum}{\i}t and Torres, Guillermo and Bastien, Fabienne A and Basu, Sarbani and Bedding, Timothy R and Chaplin, William J and Demory, Brice-Olivier and Fleming, Scott W and Guo, Zhao and Mann, Andrew W and Rowe, Jason F and Serenelli, Aldo M and Smith, Myron A and Stello, Dennis},
  year = {2014},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {211},
  number = {2},
  doi = {10.1088/0067-0049/211/1/2},
  urldate = {2020-03-23},
  abstract = {We present revised properties for 196,468 stars observed by the NASA Kepler mission and used in the analysis of Quarter 1-16 (Q1-Q16) data to detect and characterize transiting planets. The catalog is based on a compilation of literature values for atmospheric properties (temperature, surface gravity, and metallicity) derived from different observational techniques (photometry, spectroscopy, asteroseismology, and exoplanet transits), which were then homogeneously fitted to a grid of Dartmouth stellar isochrones. We use broadband photometry and asteroseismology to characterize 11,532 Kepler targets which were previously unclassified in the Kepler Input Catalog (KIC). We report the detection of oscillations in 2762 of these targets, classifying them as giant stars and increasing the number of known oscillating giant stars observed by Kepler by {$\sim$}20\% to a total of {$\sim$}15,500 stars. Typical uncertainties in derived radii and masses are {$\sim$}40\% and {$\sim$}20\%, respectively, for stars with photometric constraints only, and 5\%-15\% and {$\sim$}10\% for stars based on spectroscopy and/or asteroseismology, although these uncertainties vary strongly with spectral type and luminosity class. A comparison with the Q1-Q12 catalog shows a systematic decrease in radii of M dwarfs, while radii for K dwarfs decrease or increase depending on the Q1-Q12 provenance (KIC or Yonsei-Yale isochrones). Radii of F-G dwarfs are on average unchanged, with the exception of newly identified giants. The Q1-Q16 star properties catalog is a first step toward an improved characterization of all Kepler targets to support planet-occurrence studies.},
  keywords = {catalogs-planetary systems,catalogs-planetary systems-stars,fundamental parameters-stars,notion,notion-database,oscillations-techniques,photometric,stars: fundamental parameters,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/CYJXM7YR/full-text.pdf}
}

@article{Huber2016,
  title = {{{THE K2 ECLIPTIC PLANE INPUT CATALOG}} ({{EPIC}}) {{AND STELLAR CLASSIFICATIONS OF}} 138,600 {{TARGETS IN CAMPAIGNS}} 1\textendash 8},
  author = {Huber, Daniel and Bryson, Stephen T. and Haas, Michael R. and Barclay, Thomas and Barentsen, Geert and Howell, Steve B. and Sharma, Sanjib and Stello, Dennis and Thompson, Susan E.},
  year = {2016},
  month = may,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {224},
  number = {1},
  eprint = {1512.02643},
  pages = {2},
  publisher = {{American Astronomical Society}},
  issn = {0067-0049},
  doi = {10.3847/0067-0049/224/1/2},
  urldate = {2020-04-13},
  abstract = {The K2 Mission uses the Kepler spacecraft to obtain high-precision photometry over \textasciitilde 80 day campaigns in the ecliptic plane. The Ecliptic Plane Input Catalog (EPIC) provides coordinates, photometry and kinematics based on a federation of all-sky catalogs to support target selection and target management for the K2 mission. We describe the construction of the EPIC, as well as modifications and shortcomings of the catalog. Kepler magnitudes (Kp) are shown to be accurate to \textasciitilde 0.1 mag for the Kepler field, and the EPIC is typically complete to Kp\textasciitilde 17 (Kp\textasciitilde 19 for campaigns covered by SDSS). We furthermore classify 138,600 targets in Campaigns 1-8 (\textasciitilde 88\% of the full target sample) using colors, proper motions, spectroscopy, parallaxes, and galactic population synthesis models, with typical uncertainties for G-type stars of \textasciitilde 3\% in Teff, \textasciitilde 0.3 dex in log(g), \textasciitilde 40\% in radius, \textasciitilde 10\% in mass, and \textasciitilde 40\% in distance. Our results show that stars targeted by K2 are dominated by K-M dwarfs (\textasciitilde 41\% of all selected targets), F-G dwarfs (\textasciitilde 36\%) and K giants (\textasciitilde 21\%), consistent with key K2 science programs to search for transiting exoplanets and galactic archeology studies using oscillating red giants. However, we find a significant variation of the fraction of cool dwarfs with galactic latitude, indicating a target selection bias due to interstellar reddening and the increased contamination by giant stars near the galactic plane. We discuss possible systematic errors in the derived stellar properties, and differences to published classifications for K2 exoplanet host stars. The EPIC is hosted at the Mikulski Archive for Space Telescopes (MAST): http://archive.stsci.edu/k2/epic/search.php.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,catalogs,Earth and Planetary Astrophysics,notion,notion-database,planetary systems,proper motions,Solar and Stellar Astrophysics,stars: fundamental parameters,stars: late,techniques: photometric,type},
  file = {/Users/lbugnet/Zotero/storage/J5S2F64S/full-text.pdf}
}

@techreport{Huber2017,
  title = {Synergies between {{Asteroseismology}} and {{Exoplanetary Science}}},
  author = {Huber, Daniel},
  year = {2017},
  eprint = {1711.01281v1},
  urldate = {2020-07-04},
  abstract = {Over the past decade asteroseismology has become a powerful method to systematically characterize host stars and dynamical architectures of exoplanet systems. In this contribution I review current key synergies between asteroseismol-ogy and exoplanetary science such as the precise determination of planet radii and ages, the measurement of orbital eccentricities, stellar obliquities and their impact on hot Jupiter formation theories, and the importance of asteroseismology on spec-troscopic analyses of exoplanet hosts. I also give an outlook on future synergies such as the characterization of sub-Neptune-size planets orbiting solar-type stars, the study of planet populations orbiting evolved stars, and the determination of ages of intermediate-mass stars hosting directly imaged planets.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/EW6EZ8KY/full-text.pdf}
}

@article{Huber2017a,
  title = {Asteroseismology and {{Gaia}} : {{Testing Scaling Relations Using}} 2200 {{Kepler Stars}} with {{TGAS Parallaxes}}},
  author = {Huber, Daniel and Zinn, Joel and {Bojsen-Hansen}, Mathias and Pinsonneault, Marc and Sahlholdt, Christian and Serenelli, Aldo and Aguirre, Victor Silva and Stassun, Keivan and Stello, Dennis and Tayar, Jamie and Bastien, Fabienne and Bedding, Timothy R. and Buchhave, Lars A. and Chaplin, William J. and Davies, Guy R. and Garc{\'i}a, Rafael A. and Latham, David W. and Mathur, Savita and Mosser, Benoit and Sharma, Sanjib},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {844},
  number = {2},
  eprint = {1705.04697},
  pages = {102},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aa75ca},
  abstract = {We present a comparison of parallaxes and radii from asteroseismology and Gaia DR1 (TGAS) for 2200 Kepler stars spanning from the main sequence to the red giant branch. We show that previously identified offsets between TGAS parallaxes and distances derived from asteroseismology and eclipsing binaries have likely been overestimated for parallaxes {$<\sptilde$} 5-10 mas (\textasciitilde{} 90-98\% of the TGAS sample). The observed differences in our sample can furthermore be partially compensated by adopting a hotter Teff scale (such as the infrared flux method) instead of spectroscopic temperatures for dwarfs and subgiants. Residual systematic differences are at the \textasciitilde{} 2\% level in parallax across three orders of magnitude. We use TGAS parallaxes to empirically demonstrate that asteroseismic radii are accurate to \textasciitilde{} 5\% or better for stars between \textasciitilde{} 0.8-8 Rsun. We find no significant offset for main-sequence ({$<\sptilde$} 1.5 Rsun) and low-luminosity RGB stars (\textasciitilde{} 3-8 Rsun), but seismic radii appear to be systematically underestimated by \textasciitilde 5\% for subgiants (\textasciitilde{} 1.5-3 Rsun). We find no systematic errors as a function of metallicity between [Fe/H] \textasciitilde{} -0.8 to +0.4 dex, and show tentative evidence that corrections to the scaling relation for the large frequency separation (Dnu) improve the agreement with TGAS for RGB stars. Finally, we demonstrate that beyond \textasciitilde{} 3 kpc asteroseismology will provide more precise distances than end-of-mission Gaia data, highlighting the synergy and complementary nature of Gaia and asteroseismology for studying galactic stellar populations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,{parallaxes,stars: distances,stars: fundamental par}},
  file = {/Users/lbugnet/Zotero/storage/R2WD5IYX/Huber et al. - 2017.pdf}
}

@article{Huber2019a,
  title = {A {{Hot Saturn Orbiting}} an {{Oscillating Late Subgiant Discovered}} by {{TESS}}},
  author = {Huber, D. and Chaplin, W.J. and Chontos, A. and Kjeldsen, H. and {Christensen-Dalsgaard}, J. and Bedding, T.R. and Ball, W. and Brahm, R. and Espinoza, N. and Henning, T. and Jord{\'a}n, A. and Sarkis, P. and Knudstrup, E. and Albrecht, S. and Grundahl, F. and Andersen, M.F. and Pall{\'e}, P.L. and Crossfield, I. and Fulton, B. and Howard, A.W. and Isaacson, H.T. and Weiss, L.M. and Handberg, R. and Lund, M.N. and Serenelli, A.M. and R{\o}rsted Mosumgaard, J. and Stokholm, A. and Bieryla, A. and Buchhave, L.A. and Latham, D.W. and Quinn, S.N. and Gaidos, E. and Hirano, T. and Ricker, G.R. and Vanderspek, R.K. and Seager, S. and Jenkins, J.M. and Winn, J.N. and Antia, H.M. and Appourchaux, T. and Basu, S. and Bell, K.J. and Benomar, O. and Bonanno, A. and Buzasi, D.L. and Campante, T.L. and {\c C}elik Orhan, Z. and Corsaro, E. and Cunha, M.S. and Davies, G.R. and Deheuvels, S. and Grunblatt, S.K. and Hasanzadeh, A. and Di Mauro, M.P. and A. Garc{\'i}a, R. and Gaulme, P. and Girardi, L. and Guzik, J.A. and Hon, M. and Jiang, C. and Kallinger, T. and Kawaler, S.D. and Kuszlewicz, J.S. and Lebreton, Y. and Li, T. and Lucas, M. and Lundkvist, M.S. and Mann, A.W. and Mathis, S. and Mathur, S. and Mazumdar, A. and Metcalfe, T.S. and Miglio, A. and F. G. Monteiro, M.J.P. and Mosser, B. and Noll, A. and Nsamba, B. and Joel Ong, J.M. and {\"O}rtel, S. and Pereira, F. and Ranadive, P. and R{\'e}gulo, C. and Rodrigues, T.S. and Roxburgh, I.W. and Aguirre, V.S. and Smalley, B. and Schofield, M. and Sousa, S.G. and Stassun, K.G. and Stello, D. and Tayar, J. and White, T.R. and Verma, K. and Vrard, M. and Yildiz, M. and Baker, D. and Bazot, M. and Beichmann, C. and Bergmann, C. and Bugnet, L. and Cale, B. and Carlino, R. and Cartwright, S.M. and Christiansen, J.L. and Ciardi, D.R. and Creevey, O. and Dittmann, J.A. and Nascimento, J.-D.D. and Eylen, V.V. and F{\"u}r{\'e}sz, G. and Gagn{\'e}, J. and Gao, P. and Gazeas, K. and Giddens, F. and Hall, O.J. and Hekker, S. and Ireland, M.J. and Latouf, N. and Lebrun, D. and Levine, A.M. and Matzko, W. and Natinsky, E. and Page, E. and Plavchan, P. and {Mansouri-Samani}, M. and McCauliff, S. and Mullally, S.E. and Orenstein, B. and Soto, A.G. and Paegert, M. and Van Saders, J.L. and Schnaible, C. and Soderblom, D.R. and Szab{\'o}, R. and Tanner, A. and Tinney, C.G. and Teske, J. and Thomas, A. and Trampedach, R. and Wright, D. and Yuan, T.T. and Zohrabi, F.},
  year = {2019},
  journal = {Astronomical Journal},
  volume = {157},
  number = {6},
  eprint = {1901.01643},
  issn = {00046256},
  doi = {10.3847/1538-3881/ab1488},
  abstract = {\textcopyright{} 2019. The American Astronomical Society. All rights reserved.. We present the discovery of HD 221416 b, the first transiting planet identified by the Transiting Exoplanet Survey Satellite (TESS) for which asteroseismology of the host star is possible. HD 221416 b (HIP 116158, TOI-197) is a bright (V = 8.2 mag), spectroscopically classified subgiant that oscillates with an average frequency of about 430 {$\mu$}Hz and displays a clear signature of mixed modes. The oscillation amplitude confirms that the redder TESS bandpass compared to Kepler has a small effect on the oscillations, supporting the expected yield of thousands of solar-like oscillators with TESS 2 minute cadence observations. Asteroseismic modeling yields a robust determination of the host star radius (R{${_\ast}$} = 2.943 {$\pm$} 0.064 Ro), mass (M{${_\ast}$} = 1.212 {$\pm$} 0.074 Mo), and age (4.9 {$\pm$} 1.1 Gyr), and demonstrates that it has just started ascending the red-giant branch. Combining asteroseismology with transit modeling and radial-velocity observations, we show that the planet is a "hot Saturn" (Rp = 9.17 {$\pm$} 0.33 R{$\oplus$}) with an orbital period of {$\sim$}14.3 days, irradiance of F = 343 {$\pm$} 24 F{$\oplus$}, and moderate mass (Mp = 60.5 {$\pm$} 5.7 M{$\oplus$}) and density ({$\rho$}p = 0.431 {$\pm$} 0.062 g cm-3). The properties of HD 221416 b show that the host-star metallicity-planet mass correlation found in sub-Saturns (4-8 R{$\oplus$}) does not extend to larger radii, indicating that planets in the transition between sub-Saturns and Jupiters follow a relatively narrow range of densities. With a density measured to {$\sim$}15\%, HD 221416 b is one of the best characterized Saturn-size planets to date, augmenting the small number of known transiting planets around evolved stars and demonstrating the power of TESS to characterize exoplanets and their host stars using asteroseismology.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,planets and satellites: fundamental parameters,planets and satellites: individual (HD 221416 b),stars: fundamental parameters,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/BKUUBYRL/Huber et al. - 2019.pdf}
}

@article{huberAutomatedExtractionOscillation2009,
  title = {Automated Extraction of Oscillation Parameters for {{Kepler}} Observations of Solar-Type Stars},
  author = {Huber, D. and Stello, D. and Bedding, T.R. and Chaplin, W.J. and Arentoft, T. and Quirion, P-O. and Kjeldsen, H.},
  year = {2009},
  month = oct,
  journal = {Communication in Asteroseismology},
  volume = {160},
  urldate = {2021-05-26},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4WUW65I4/m-api-41be2274-cac3-4e07-288e-276b3781100a.pdf}
}

@article{Hubrig2023,
  title = {Searching for Magnetic Fields in Pulsating {{A-type}} Stars: The Discovery of a Strong Field in the Probable {$\delta$} {{Sct}} Star {{HD}} 340577 and a Null Result for the {$\gamma$} {{Dor}} Star {{HR}} 8799},
  shorttitle = {Searching for Magnetic Fields in Pulsating {{A-type}} Stars},
  author = {Hubrig, S. and J{\"a}rvinen, S. P. and {Alvarado-G{\'o}mez}, J. D. and Ilyin, I. and Sch{\"o}ller, M.},
  year = {2023},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {526},
  pages = {L83-L87},
  issn = {0035-8711},
  doi = {10.1093/mnrasl/slad116},
  urldate = {2023-10-17},
  abstract = {Numerous {$\delta$} Sct and {$\gamma$} Dor pulsators are identified in the region of the Hertzsprung-Russell diagram that is occupied by chemically peculiar magnetic Ap stars. The connection between {$\delta$} Sct and {$\gamma$} Dor pulsations and the magnetic field in Ap stars is however not clear: theory suggests for magnetic Ap stars some critical field strengths for pulsation mode suppression by computing the magnetic damping effect for selected p and g modes. To test these theoretical considerations, we obtained PEPSI spectropolarimetric snapshots of the typical Ap star HD 340577, for which {$\delta$} Sct-like pulsations were recently detected in Transiting Exoplanet Survey Satellite data, and the {$\gamma$} Dor pulsator HR 8799, which is a remarkable system with multiple planets and two debris discs. Our measurements reveal the presence of a magnetic field with a strength of several hundred Gauss in HD 340577. The measured mean longitudinal field would be the strongest field measured so far in a {$\delta$} Sct star if the pulsational character of HD 340577 is confirmed spectroscopically. No magnetic field is detected in HR 8799.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,HR 8799,stars: chemically peculiar,stars: individual: HD 340577,stars: magnetic field,stars: oscillations,techniques: polarimetric,techniques: spectroscopic},
  annotation = {ADS Bibcode: 2023MNRAS.526L..83H},
  file = {/Users/lbugnet/Zotero/storage/4J9NFPR3/Hubrig et al. - 2023 - Searching for magnetic fields in pulsating A-type .pdf}
}

@article{Hufbauer2006,
  title = {Stellar Structure and Evolution, 1924-1939},
  author = {Hufbauer, Karl},
  year = {2006},
  journal = {Journal for the History of Astronomy},
  volume = {37},
  number = {2},
  pages = {203--227},
  issn = {00218286},
  doi = {10.1177/002182860603700205},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/C5KKUHG9/Hufbauer - 2006.pdf}
}

@techreport{hussainRoleMagneticFields2013,
  title = {The Role of Magnetic Fields in Pre-Main Sequence Stars},
  author = {Hussain, Gaitee A J and Alecian, Evelyne},
  year = {2013},
  journal = {IAUS},
  volume = {302},
  eprint = {1402.7130v1},
  urldate = {2021-02-14},
  abstract = {Strong, kilo-Gauss, magnetic fields are required to explain a range of observational properties in young, accreting pre-main sequence (PMS) systems. We review the techniques used to detect magnetic fields in PMS stars. Key results from a long running campaign aimed at characterising the large scale magnetic fields in accreting T Tauri stars are presented. Maps of surface magnetic flux in these systems can be used to build 3-D models exploring the role of magnetic fields and the efficiency with which magnetic fields can channel accretion from circumstellar disks on to young stars. Long-term variability in T Tauri star magnetic fields strongly point to a dynamo origin of the magnetic fields. Studies are underway to quantify how changes in magnetic fields affect their accretion properties. We also present the first results from a new programme that investigates the evolution of magnetic fields in intermediate mass (1.5-3 M) pre-main sequence stars as they evolve from being convective T Tauri stars to fully radiative Herbig AeBe stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: accreting,stars: activity,stars: circumstellar matter,stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/2SGADLLY/full-text.pdf}
}

@article{Icarus1985,
  title = {Provided That the Velocity Distribution Drops off Sufficiently Rapidly. {{We}} Have Shown That a Thermal Spike Velocity Distribution (Equation (2)) Produces Such a Peak Whereas Distributions That Fall off as v- 3 or Less Do Not Create the Required Peak. (2)},
  author = {Icarus, L A},
  year = {1985},
  number = {2},
  pages = {1--5},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QEV54ID9/Icarus - 1985.pdf}
}

@article{Isern2022,
  title = {White Dwarfs as {{Physics}} Laboratories: Lights and Shadows},
  shorttitle = {White Dwarfs as {{Physics}} Laboratories},
  author = {Isern, J. and Torres, S. and {Rebassa-Mansergas}, A.},
  year = {2022},
  month = jan,
  journal = {Frontiers in Astronomy and Space Sciences},
  volume = {9},
  pages = {6},
  doi = {10.3389/fspas.2022.815517},
  urldate = {2023-09-19},
  abstract = {The evolution of white dwarfs is just a simple process of cooling in which the basic ingredients for predicting their evolution are well identified, although not always well understood. There are two independent ways to test the cooling rate. One is the luminosity function of the white dwarf population, and another is the secular drift of the period of pulsation of those individuals that experience variations. Both scenarios are sensitive to the cooling or heating time scales, for which reason, the inclusion of any additional source or sink of energy will modify these properties and will allow to set bounds to these perturbations. These studies also require complete and statistical significant samples for which current large data surveys are providing an unprecedented wealth of information. In this paper we review how these techniques are applied to several cases like the secular drift of the Newton gravitational constant, neutrino magnetic moments, axions and weakly interacting massive particles (WIMPS).},
  keywords = {(stars) white dwarfs,Asteroseismology,astroparticle physics,Astrophysics - High Energy Astrophysical Phenomena,Gravitation,High Energy Physics - Phenomenology,mass function,Stars: luminosity function,stars: oscillations (including pulsations},
  annotation = {ADS Bibcode: 2022FrASS...9....6I},
  file = {/Users/lbugnet/Zotero/storage/54I7TDRJ/Isern et al. - 2022 - White dwarfs as Physics laboratories lights and s.pdf}
}

@article{Israelian2009,
  title = {Enhanced Lithium Depletion in {{Sun-like}} Stars with Orbiting Planets},
  author = {Israelian, Garik and Mena, Elisa Delgado and Santos, Nuno C. and Sousa, Sergio G. and Mayor, Michel and Udry, Stephane and Cerd{\~e}a, Carolina Dom{\'i}nguez and Rebolo, Rafael and Randich, Sofia},
  year = {2009},
  journal = {Nature},
  volume = {462},
  number = {7270},
  pages = {189--191},
  issn = {00280836},
  doi = {10.1038/nature08483},
  abstract = {The surface abundance of lithium on the Sun is 140 times less than the protosolar value, yet the temperature at the base of the surface convective zone is not hot enough to burnand hence depleteLi (refs 2, 3). A large range of Li abundances is observed in solar-type stars of the same age, mass and metallicity as the Sun, but such a range is theoretically difficult to understand. An earlier suggestion that Li is more depleted in stars with planets was weakened by the lack of a proper comparison sample of stars without detected planets. Here we report Li abundances for an unbiased sample of solar-analogue stars with and without detected planets. We find that the planet-bearing stars have less than one per cent of the primordial Li abundance, while about 50 per cent of the solar analogues without detected planets have on average ten times more Li. The presence of planets may increase the amount of mixing and deepen the convective zone to such an extent that the Li can be burned. \textcopyright{} 2009 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XTJL3XZW/Israelian et al. - 2009.pdf}
}

@article{Israelian2009a,
  title = {Lithium in Stars with Exoplanets},
  author = {Israelian, Garik},
  year = {2009},
  journal = {Proceedings of the International Astronomical Union},
  volume = {5},
  number = {S268},
  pages = {285--290},
  issn = {17439221},
  doi = {10.1017/S1743921310004254},
  abstract = {Our recent study of solar-type stars from the HARPS GTO sample provides highly accurate information with regard to Lithium abundances in stars with and without detected planets (Israelian et al. 2009) . When the Li abundances of planet bearing stars are compared with the "single" stars, we find an excess of Li depletion in planet hosts with effective temperatures in the range 5700-5850 K. We also found that small amounts of Li have survived in the atmospheres of some planet-host solar analogs. Enhanced Li depletion in planet host stars puts constraints on mixing processes responsible for this phenomenon. We show that neither age nor metallicity are responsible for this observational fact.},
  keywords = {Late-type,notion,notion-database,Planetary systems,Stars: abundances},
  file = {/Users/lbugnet/Zotero/storage/EGVACQK8/Israelian - 2009.pdf}
}

@article{Jain2009,
  title = {Solar Activity Phases and Intermediate-Degree Mode Frequencies},
  author = {Jain, Kiran and Tripathy, S. C. and Hill, F.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {695},
  number = {2},
  eprint = {0902.1557},
  pages = {1567--1576},
  issn = {15384357},
  doi = {10.1088/0004-637X/695/2/1567},
  abstract = {We analyze intermediate-degree p-mode eigenfrequencies measured by Global Oscillation Network Group and Michelson Doppler Imager/Solar and Heliospheric Observatory over a solar cycle to study the source of their variability. We carry out a correlation analysis between the change in frequencies and several measures of the Sun's magnetic activity that are sensitive to changes at different levels in the solar atmosphere. The observations span a period of about 12 years starting from mid-1996 (the minimum of cycle 23) to early-2008 (near minimum of cycle 24), corresponding to a nearly complete solar activity cycle. We demonstrate that the frequencies do vary in phase with the solar activity indices, however, the degree of correlation differs from phase to phase of the cycle. During the rising and declining phases, the mode frequency shifts are strongly correlated with the activity proxies whereas during the high-activity period, the shifts have significantly lower correlation with all activity proxies, except for the 10.7 cm radio flux. In particular, the proxies that are only influenced by the variation of the strong component of the magnetic field in the photosphere have a much lower correlation at the high-activity period. On the other hand, the shifts are better correlated with the proxies sensitive to changes in the weak component of the magnetic field. Our correlation analysis suggests that more than 90\% of the variation in the oscillation frequencies in all activity phases can be explained by changes in both components of the magnetic field. Further, the slopes obtained from the linear regression analysis also differ from phase to phase and show a strong correlation with the correlation coefficients between frequency shifts and solar activity.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: magnetic fields,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/Y2IB85YE/Jain, Tripathy, Hill - 2009.pdf}
}

@article{Janson2008,
  title = {A Comprehensive Examination of the {{Eps Eri}} System -- {{Verification}} of a 4 Micron Narrow-Band High-Contrast Imaging Approach for Planet Searches},
  author = {Janson, Markus and Reffert, Sabine and Brandner, Wolfgang and Henning, Thomas and Lenzen, Rainer and Hippler, Stefan},
  year = {2008},
  month = jul,
  journal = {Astronomy and Astrophysics},
  volume = {488},
  number = {2},
  eprint = {0807.0301},
  pages = {771--780},
  doi = {10.1051/0004-6361:200809984},
  urldate = {2020-07-13},
  abstract = {Due to its proximity, youth, and solar-like characteristics with a spectral type of K2V, Eps Eri is one of the most extensively studied systems in an extrasolar planet context. Based on radial velocity, astrometry, and studies of the structure of its circumstellar debris disk, at least two planetary companion candidates to Eps Eri have been inferred in the literature (Eps Eri b, Eps Eri c). Some of these methods also hint at additional companions residing in the system. Here we present a new adaptive optics assisted high-contrast imaging approach that takes advantage of the favourable planet spectral energy distribution at 4 microns, using narrow-band angular differential imaging to provide an improved contrast at small and intermediate separations from the star. We use this method to search for planets at orbits intermediate between Eps Eri b (3.4 AU) and Eps Eri c (40 AU). The method is described in detail, and important issues related to the detectability of planets such as the age of Eps Eri and constraints from indirect measurements are discussed. The non-detection of companion candidates provides stringent upper limits for the masses of additional planets. Using a combination of the existing dynamic and imaging data, we exclude the presence of any planetary companion more massive than 3 Mjup anywhere in the Eps Eri system. Specifically, with regards to the possible residual linear radial velocity trend, we find that it is unlikely to correspond to a real physical companion if the system is as young as 200 Myr, whereas if it is as old as 800 Myr, there is an allowed semi-major axis range between about 8.5 and 25 AU.},
  archiveprefix = {arxiv},
  keywords = {Instrumentation: adaptive optics,Instrumentation: high angular resolution,notion,notion-database,Planetary systems,Stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/BSZ28P2H/full-text.pdf}
}

@article{Javaraiah2003,
  title = {Long-Term Variations in the Solar Differential Rotation},
  author = {Javaraiah, J.},
  year = {2003},
  journal = {Solar Physics},
  volume = {212},
  number = {1},
  pages = {23--49},
  issn = {00380938},
  doi = {10.1023/A:1022912430585},
  abstract = {Using Greenwich data (1879-1976) and SOON/NOAA data (1977-2002) on sunspot groups we found the following results: (i) The Sun's mean (over all the concerned cycles during 1879-1975) equatorial rotation rate (A) is significantly larger ({$\approx$} 0.1\%) in the odd-numbered sunspot cycles (ONSCs) than in the even-numbered sunspot cycles (ENSCs). The mean rotation is significantly ({$\approx$} 10\%) more differential in the ONSCs than in the ENSCs. North-south difference in the mean equatorial rotation rate is larger in the ONSCs than in the ENSCs. North-south difference in the mean latitude gradient of the rotation is significant in the ENSCs and insignificant in the ONSCs. (ii) The known very large decrease in A from cycle 13 to cycle 14 is confirmed. The amount of this decrease in the mean A was about 0.017 {$\mu$}rad s-1. Also, we find that A decreased from cycle 17 to cycle 18 by about 0.008 {$\mu$}rad s-1and from cycle 21 to cycle 22 by about 0.016 {$\mu$}rad s-1. From cycle 13 to cycle 14 the decrease in A was more in the northern hemisphere than in the southern hemisphere, it is opposite in the later two epochs. The time gap between the consecutive drops in A is about 44 years, suggesting the existence of a '44-yr' cycle or 'double Hale cycle' in A. The time gap between the two large drops, viz., from cycle 13 to cycle 14 and from cycle 21 to cycle 22, is about 90 years (Gleissberg cycle). We predict that the next drop (moderate) in A will be occurring from cycle 25 to cycle 26 and will be followed by a relatively large-amplitude 'double Hale cycle' of sunspot activity, (iii) Existence of a 90-yr cycle is seen in the cycle-to-cycle variation of the latitude gradient (B). A weak 22-yr modulation in B seems to be superposed on the relatively strong 90-yr modulation. (iv) The coefficient A varies significantly only during ONSCs and the variation has maximum amplitude in the order of 0.01 {$\mu$}rad s-1around activity minima. (v) There exists a good anticorrelation between the mean variation of B during the ONSCs and that during the ENSCs, suggesting the existence of a '22-yr' periodicity in B. The maximum amplitude of the variation of B is of the order of 0.05 {$\mu$}rad s-1around the activity minima. (vi) It seems that the well-known Gnevyshev and Ohl rule of solar activity is applicable also to the cycle-to-cycle amplitude modulation of B from cycle 13 to cycle 20, but the cycles 12 (in the northern hemisphere, Greenwich data) and 21 (in both hemispheres, SOON/NOAA data) seem to violate this rule in B. And (vii) All the aforesaid statistically significant variations in A and B seem to be related to the approximate 179-yr cycle, 1811-1989, of variation in the Sun's motion about the center of mass of the solar system.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TZU39LQX/Javaraiah - 2003.pdf}
}

@article{Jefferies1994,
  title = {Us Eof Acoustic Wave Travel-Time Measurements to Probe the near-Surface Layers of the Sun},
  author = {Jefferies, S. M. and Osaki, Y. and Shibahashi, Hiromoto and Duvall, T. L. and Harvey, J. W. and Pomerantz, M. A.},
  year = {1994},
  journal = {The Astrophysical Journal},
  volume = {434},
  pages = {795--800},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8J6LHNFI/Jefferies et al. - 1994.pdf}
}

@article{Jeffery2016,
  title = {Radial Pulsation as a Function of Hydrogen Abundance},
  author = {Jeffery, C. S. and Saio, H.},
  year = {2016},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {458},
  number = {2},
  pages = {1352--1373},
  issn = {0035-8711},
  doi = {10.1093/mnras/stw388},
  urldate = {2023-10-15},
  abstract = {Using linear non-adiabatic pulsation analysis, we explore the radial-mode (p-mode) stability of stars across a wide range of mass (\$0.2 \textbackslash le M \textbackslash le 50\{\textbackslash,\textbackslash rm M\_\{\{\textbackslash odot \}\}\}\$), composition (0 {$\leq$} X {$\leq$} 0.7, Z = 0.001, 0.02), effective temperature (3000 {$\leq$} Teff {$\leq$} 40\,000~K), and luminosity (0.01 {$\leq$} L/M {$\leq$} 100\,000 solar units). We identify the instability boundaries associated with low- to high-order radial oscillations (0 {$\leq$} n {$\leq$} 16). The instability boundaries are a strong function of both composition and radial order (n). With decreasing hydrogen abundance we find that (i) the classical blue edge of the Cepheid instability strip shifts to higher effective temperature and luminosity, and (ii) high-order modes are more easily excited and small islands of high radial-order instability develop, some of which correspond with real stars. Driving in all cases is by the classical {$\kappa$}-mechanism and/or strange modes. We identify regions of parameter space where new classes of pulsating variable may, in future, be discovered. The majority of these are associated with reduced hydrogen abundance in the envelope; one has not been identified previously.},
  file = {/Users/lbugnet/Zotero/storage/H76HL7KN/Jeffery and Saio - 2016 - Radial pulsation as a function of hydrogen abundan.pdf;/Users/lbugnet/Zotero/storage/TE2SLS7W/2589083.html}
}

@article{Jenkins2010,
  title = {Initial Characteristics of Kepler Long Cadence Data for Detecting Transiting Planets},
  author = {Jenkins, Jon M. and Caldwell, Douglas A. and Chandrasekaran, Hema and Twicken, Joseph D. and Bryson, Stephen T. and Quintana, Elisa V. and Clarke, Bruce D. and Li, Jie and Allen, Christopher and Tenenbaum, Peter and Wu, Hayley and Klaus, Todd C. and Van Cleve, Jeffrey and Dotson, Jessie A. and Haas, Michael R. and Gilliland, Ronald L. and Koch, David G. and Borucki, William J.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0256},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L120},
  abstract = {The Kepler Mission seeks to detect Earth-size planets transiting solar-like stars in its {$\sim$}115deg2 field of view over the course of its 3.5 year primary mission by monitoring the brightness of each of {$\sim$}156,000 Long Cadence stellar targets with a time resolution of 29.4 minutes. We discuss the photometric precision achieved on timescales relevant to transit detection for data obtained in the 33.5 day long Quarter 1 (Q1) observations that ended 2009 June 15. The lower envelope of the photometric precision obtained at various timescales is consistent with expected random noise sources, indicating that Kepler has the capability to fulfill its mission. The Kepler light curves exhibit high precision over a large dynamic range, which will surely permit their use for a large variety of investigations in addition to finding and characterizing planets. We discuss the temporal characteristics of both the raw flux time series and the systematic error-corrected flux time series produced by the Kepler Science Pipeline, and give examples illustrating Kepler's large dynamic range and the variety of light curves obtained from the Q1 observations. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/TIP2MYSW/Jenkins et al. - 2010.pdf}
}

@article{Jenkins2010a,
  title = {Overview of the Kepler Science Processing Pipeline},
  author = {Jenkins, Jon M. and Caldwell, Douglas A. and Chandrasekaran, Hema and Twicken, Joseph D. and Bryson, Stephen T. and Quintana, Elisa V. and Clarke, Bruce D. and Li, Jie and Allen, Christopher and Tenenbaum, Peter and Wu, Hayley and Klaus, Todd C. and Middour, Christopher K. and Cote, Miles T. and McCauliff, Sean and Girouard, Forrest R. and Gunter, Jay P. and Wohler, Bill and Sommers, Jeneen and Hall, Jennifer R. and Uddin, Akm K. and Wu, Michael S. and Bhavsar, Paresh A. and Van Cleve, Jeffrey and Pletcher, Davidl and Dotson, Jessie A. and Haas, Michael R. and Gilliland, Ronald L. and Koch, David G. and Borucki, Williamj},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0258},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L87},
  abstract = {The Kepler Mission Science Operations Center (SOC) performs several critical functions including managing the {$\sim$}156,000 target stars, associated target tables, science data compression tables and parameters, as well as processing the raw photometric data downlinked from the spacecraft each month. The raw data are first calibrated at the pixel level to correct for bias, smear induced by a shutterless readout, and other detector and electronic effects. A background sky flux is estimated from {$\sim$}4500 pixels on each of the 84 CCD readout channels, and simple aperture photometry is performed on an optimal aperture for each star. Ancillary engineering data and diagnostic information extracted from the science data are used to remove systematic errors in the flux time series that are correlated with these data prior to searching for signatures of transiting planets with a wavelet-based, adaptive matched filter. Stars with signatures exceeding 7.1{$\sigma$} are subjected to a suite of statistical tests including an examination of each star's centroid motion to reject false positives caused by background eclipsing binaries. Physical parameters for each planetary candidate are fitted to the transit signature, and signatures of additional transiting planets are sought in the residual light curve. The pipeline is operational, finding planetary signatures and providing robust eliminations of false positives. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/6RQN2R32/Jenkins et al. - 2010(2).pdf}
}

@article{Jenkins2011a,
  title = {Chromospheric Activities and Kinematics for Solar Type Dwarfs and Subgiants: {{Analysis}} of the Activity Distribution and the {{AVR}}},
  author = {Jenkins, J. S. and Murgas, F. and Rojo, P. and Jones, H. R.A. and {Day-Jones}, A. C. and Jones, M. I. and Clarke, J. R.A. and Ruiz, M. T. and Pinfield, D. J.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {531},
  issn = {00046361},
  doi = {10.1051/0004-6361/201016333},
  abstract = {Aims. In this work we present chromospheric activity indices, kinematics, radial-velocities, and rotational velocities for more than 850 FGK-type dwarfs and subgiant stars in the southern hemisphere and test how best to calibrate and measure S-indices from echelle spectra. Methods. We measured our parameters using the high-resolution and high-S/N FEROS echelle spectra acquired for this purpose. Results. We confirm the bimodal distribution of chromospheric activities for such stars and highlight the role that the more active K-dwarfs play in biasing the number of active stars. We show that the age-activity relationship does appear to continue to ages older than the Sun if we simply compare main sequence stars and subgiant stars with an offset of around 2.5 Gyr between the peaks of both distributions. Also we show evidence of an increased spin-down timescale for cool K dwarfs compared with earlier F and G type stars. We highlight that activities drawn from low-resolution spectra (R {$<$} 2500) significantly increase the rms scatter when calibrating onto common systems of measurements like the Mt. Wilson system. Also we show that older and widely used catalogues of activities in the south appear to be offset compared to more recent works at the {$\sim$}0.1 dex level in RHK through calibrator drift. In addition, we show how kinematics can be used to preselect inactive stars for future planet search projects. We see the well known trend between projected rotational velocity and activity, however we also find a correlation between kinematic space velocity and chromospheric activity. It appears that after the Vaughan-Preston gap there is a quick step function in the kinematic space motion towards a significantly broader spread in velocities. We speculate on reasons for this correlation and provide some model scenarios to describe the bimodal activity distribution through magnetic saturation, residual low level gas accretion, or accretion by the star of planets or planetesimals. Finally, we provide a new empirical measurement for the disk-heating law, using the latest age-activity relationships to reconstruct the age-velocity distribution for local disk stars. We find a value of 0.337 {$\pm$} 0.045 for the exponent of this power law (i.e. {$\sigma$}tot t0.337), in excellent agreement with those found using isochrone fitting methods and with theoretical disk-heating models. \textcopyright{} 2011 ESO.},
  keywords = {notion,notion-database,planetary systems,stars: activity,stars: atmospheres,stars: fundamental parameters,stars: kinematics and dynamics,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/H874XI6H/Jenkins et al. - 2011.pdf}
}

@article{Jermyn2020,
  title = {The {{Origin}} of the {{Bimodal Distribution}} of {{Magnetic Fields}} in {{Early-type Stars}}},
  author = {Jermyn, Adam S. and Cantiello, Matteo},
  year = {2020},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {900},
  pages = {113},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ab9e70},
  urldate = {2023-10-10},
  abstract = {In early-type stars a fossil magnetic field may be generated during the star formation process or be the result of a stellar merger event. Surface magnetic fields are thought to be erased by (sub)surface convection layers, which typically leave behind weak disordered fields. However, if the fossil field is strong enough it can prevent the onset of (sub)surface convection and so be preserved onto the main sequence. We calculate the critical field strength at which this occurs, and find that it corresponds well with the lower limit amplitude of observed fields in strongly magnetized Ap/Bp stars ({$\approx$}300 G). The critical field strength is predicted to increase slightly during the main-sequence evolution, which could also explain the observed decline in the fraction of magnetic stars. This supports the conclusion that the bimodal distribution of observed magnetic fields in early-type stars reflects two different field origin stories: strongly magnetic fields are fossils fields inherited from star formation or a merger event, and weak fields are the product of ongoing dynamo action.},
  keywords = {1599,1606,994,995,Astrophysics - Solar and Stellar Astrophysics,Magnetic fields,Magnetic stars,Stellar evolution,Stellar interiors},
  annotation = {ADS Bibcode: 2020ApJ...900..113J},
  file = {/Users/lbugnet/Zotero/storage/UXEIVDJF/Jermyn and Cantiello - 2020 - The Origin of the Bimodal Distribution of Magnetic.pdf}
}

@article{Jermyn2021,
  title = {Magnetic {{Archaeology}} of {{Early-type Stellar Dynamos}}},
  author = {Jermyn, Adam S. and Cantiello, Matteo},
  year = {2021},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {923},
  pages = {104},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac2d2a},
  urldate = {2023-10-10},
  abstract = {Early-type stars show a bimodal distribution of magnetic field strengths, with some showing very strong fields ({$\greaterequivlnt$}1 kG) and others very weak fields ({$\lessequivlnt$}10 G). Recently, we proposed that this reflects the processing or lack thereof of fossil fields by subsurface convection zones. Stars with weak fossil fields process these at the surface into even weaker dynamo-generated fields, while in stars with stronger fossil fields magnetism inhibits convection, allowing the fossil field to remain as is. We now expand on this theory and explore the timescales involved in the evolution of near-surface magnetic fields. We find that mass loss strips near-surface regions faster than magnetic fields can diffuse through them. As a result, observations of surface magnetism directly probe the frozen-in remains of the convective dynamo. This explains the slow evolution of magnetism in stars with very weak fields: these dynamo-generated magnetic fields evolve on the timescale of the mass loss, not that of the dynamo.},
  keywords = {1606,1610,Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2021ApJ...923..104J},
  file = {/Users/lbugnet/Zotero/storage/HT59WZPS/Jermyn and Cantiello - 2021 - Magnetic Archaeology of Early-type Stellar Dynamos.pdf}
}

@article{Jermyn2022,
  title = {An {{Atlas}} of {{Convection}} in {{Main-sequence Stars}}},
  author = {Jermyn, Adam S. and Anders, Evan H. and Lecoanet, Daniel and Cantiello, Matteo},
  year = {2022},
  month = sep,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {262},
  pages = {19},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/ac7cee},
  urldate = {2023-10-18},
  abstract = {Convection is ubiquitous in stars and occurs under many different conditions. Here we explore convection in main-sequence stars through two lenses: dimensionless parameters arising from stellar structure and parameters that emerge from the application of mixing length theory. We first define each quantity in terms familiar to both the 1D stellar evolution community and the hydrodynamics community. We then explore the variation of these quantities across different convection zones, different masses, and different stages of main-sequence evolution. We find immense diversity across stellar convection zones. Convection occurs in thin shells, deep envelopes, and nearly spherical cores; it can be efficient or inefficient, rotationally constrained or not, transsonic or deeply subsonic. This atlas serves as a guide for future theoretical and observational investigations by indicating which regimes of convection are active in a given star, and by describing appropriate model assumptions for numerical simulations.},
  keywords = {1621,2046,301,Astrophysics - Solar and Stellar Astrophysics,Physics - Fluid Dynamics,Stellar convective zones,Stellar evolutionary models,Stellar physics},
  annotation = {ADS Bibcode: 2022ApJS..262...19J},
  file = {/Users/lbugnet/Zotero/storage/GEQ9R79N/Jermyn et al. - 2022 - An Atlas of Convection in Main-sequence Stars.pdf}
}

@article{jermynConvectiveDifferentialRotation2020,
  title = {Convective Differential Rotation in Stars and Planets-{{I}}. {{Theory}}},
  author = {Jermyn, Adam S and Chitre, Shashikumar M and Lesaffre, Pierre and Tout, Christopher A},
  year = {2020},
  journal = {MNRAS},
  volume = {498},
  pages = {3758--3781},
  doi = {10.1093/mnras/staa2323},
  urldate = {2021-05-10},
  abstract = {We derive the scaling of differential rotation in both slowly and rapidly rotating convection zones using order of magnitude methods. Our calculations apply across stars and fluid planets and all rotation rates, as well as to both magnetized and purely hydrodynamic systems. We find shear |R{$\nabla$}| of order the angular frequency for slowly rotating systems with |N|, where N is the Br\"unt-V\"ais\"al\"a frequency, and find that it declines as a power law in for rapidly rotating systems with |N|. We further calculate the meridional circulation rate and baroclinicity and examine the magnetic field strength in the rapidly rotating limit. Our results are in general agreement with simulations and observations and we perform a detailed comparison with those in a companion paper.},
  keywords = {convection-Sun,evolution-stars,interiors-stars,notion,notion-database,rotation,rotation-stars},
  file = {/Users/lbugnet/Zotero/storage/DIN2HLIJ/full-text.pdf}
}

@article{Jiang2020,
  title = {Variations of the Mixing Character of Dipolar Mixed Modes in Red Giant Stars},
  author = {Jiang, C and Cunha, M and {Christensen-Dalsgaard}, J and Zhang, {\relax QS}},
  year = {2020},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  eprint = {2005.01464},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/staa1285},
  urldate = {2020-06-02},
  abstract = {Thanks to the high quality data of space missions, the detection of mixed modes has become possible in numerous stars. In this work, we investigate how the mixing character of dipolar mixed modes changes with stellar evolution, as well as with frequency within each stellar model. This is achieved by monitoring the variations in the coupling strength and the period spacing of dipolar mixed modes in red-giant models. These parameters are measured by fitting the asymptotic expansion of mixed modes to the model frequencies of a grid of red-giant models with masses between 1.0 and 2.0~M{$\bigodot$} and three different chemical abundances. The coupling strength and the period spacing decrease with stellar evolution. We find that the slopes of their decreasing trends depend on the radial order of the pressure mode component. A non-negligible increase of the coupling strength with frequency by up to around 40\% is found in the observable frequency range for a set of red-giant models. On the contrary, no significant changes of the period spacing with frequency are found. The changes in the mixing character of the modes are in most cases affected by the model mass and metallicity. Buoyancy glitches also have an impact on the mixing character. Significant fluctuations in the estimated coupling strength and period spacing are found for models approaching the luminosity bump, if the glitch impact of the frequencies is not considered in the applied asymptotic expansion.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Jimen,
  title = {The Rotation of the Solar Core},
  author = {Jimenez, A. and Hern{\'a}ndez, F. P{\'e}rez and Claret, A. and Pall{\'e}, Pere L. and Regulo, C. and Cort{\'e}s, Teodoro Roca},
  year = {1994},
  journal = {The Astrophysical Journal},
  volume = {435},
  pages = {874--880},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/7PQULNK6/Jimenez et al. - 1994.pdf}
}

@article{Jimenez-Reyes2008a,
  title = {{{SolarFLAG}} Hare and Hounds: {{Estimation}} of p-Mode Frequencies from {{Sun-as-star}} Helioseismology Data},
  author = {{Jim{\'e}nez-Reyes}, S. J. and Chaplin, W. J. and Garc{\'i}a, R. A. and Appourchaux, T. and Baudin, F. and Boumier, P. and Elsworth, Y. and Fletcher, S. T. and Lazrek, M. and Leibacher, J. W. and Lochard, J. and New, R. and R{\'e}gulo, C. and Salabert, D. and Toutain, T. and Verner, G. A. and Wachter, R.},
  year = {2008},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {389},
  number = {4},
  pages = {1780--1790},
  issn = {13652966},
  doi = {10.1111/j.1365-2966.2008.13668.x},
  abstract = {We report on the results of the latest solarFLAG hare-and-hounds exercise, which was concerned with testing methods for extraction of frequencies of low-degree solar p modes from data collected by Sun-as-a-star observations. We have used the new solarFLAG simulator, which includes the effects of correlated mode excitation and correlations with background noise, to make artificial time-series data that mimic Doppler velocity observations of the Sun-as-a-star. The correlations give rise to asymmetry of mode peaks in the frequency power spectrum. 10 members of the group (the hounds) applied their 'peak-bagging' codes to a 3456-d data set, and the estimated mode frequencies were returned to the hare (who was WJC) for comparison. Analysis of the results reveals a systematic bias in the estimated frequencies of modes above {$\approx$}1.8 mHz. The bias is negative, meaning the estimated frequencies systematically underestimate the input frequencies. We identify two sources that are the dominant contributions to the frequency bias. Both sources involve failure to model accurately subtle aspects of the observed power spectral density in the part (window) of the frequency power spectrum that is being fitted. One source of bias arises from a failure to account for the power spectral density coming from all those modes whose frequencies lie outside the fitting windows. The other source arises from a failure to account for the power spectral density of the weak l = 4 and 5 modes, which are often ignored in Sun-as-a-star analysis. The Sun-as-a-star peak-bagging codes need to allow for both sources, otherwise the frequencies are likely to be biased. \textcopyright{} 2008 RAS.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/V5Z83THN/Jiménez-Reyes et al. - 2008.pdf}
}

@article{Jimenez2009,
  title = {On the Solar Origin of the Signal at 220.7 {$M$}hz: {{A}} Possible Component of a g-{{Mode}}?},
  author = {Jim{\'e}nez, A. and Garc{\'i}a, R. A.},
  year = {2009},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {184},
  number = {2},
  eprint = {0908.0562},
  pages = {288--297},
  issn = {00670049},
  doi = {10.1088/0067-0049/184/2/288},
  abstract = {Gravity modes in the Sun have been the object of a long and difficult search in recent decades. Thanks to the data accumulated with the last generation of instruments (BiSON, GONG, and three helioseismic instruments aboard the Solar and Heliospheric Observatory (SOHO)), scientists have been able to find signatures of their presence. However, the individual detection of such modes remains evasive. In this article, we study the signal at 220.7 {$\mu$}Hz which is a peak that is present in most of the helioseismic data of the last 10 years. This signal has already been identified as being a component of a g-mode candidate detected in the GOLF Doppler velocity signal. The nature of this peak is studied in particular using the VIRGO/SPM instrument aboard SOHO. First we analyze all the available instrumental data of VIRGO and SOHO (housekeeping) to reject any possible instrumental origin. No relation was found, implying that the signal has a solar origin. Using Monte Carlo simulations, we find, with more than 99\% confidence level, that the signal found in VIRGO/SPM is very unlikely to be due to pure noise. \textcopyright{} 2009. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/B6GVJMFL/Jiménez, García - 2009.pdf}
}

@article{Jimenez2011a,
  title = {The Acoustic Cutoff Frequency of the Sun and the Solar Magnetic Activity Cycle},
  author = {Jim{\'e}nez, A. and Garc{\'i}a, R. A. and Pall{\'e}, P. L.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {743},
  number = {2},
  eprint = {1109.3326},
  pages = {1--26},
  issn = {15384357},
  doi = {10.1088/0004-637X/743/2/99},
  abstract = {The acoustic cutoff frequency - the highest frequency for acoustic solar eigenmodes - is an important parameter of the solar atmosphere as it determines the upper boundary of the p-mode resonant cavities. At frequencies beyond this value, acoustic disturbances are no longer trapped but are traveling waves. Interference among them gives rise to higher-frequency peaks - the pseudomodes - in the solar acoustic spectrum. The pseudomodes are shifted slightly in frequency with respect to p-modes, making possible the use of pseudomodes to determine the acoustic cutoff frequency. Using data from the GOLF and VIRGO instruments on board the Solar and Heliospheric Observatory spacecraft, we calculate the acoustic cutoff frequency using the coherence function between both the velocity and intensity sets of data. By using data gathered by these instruments during the entire lifetime of the mission (1996 until the present), a variation in the acoustic cutoff frequency with the solar magnetic activity cycle is found. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/NZGRTJF9/Jiménez, García, Pallé - 2011.pdf}
}

@article{Jimenez2015,
  title = {Analysis of the Acoustic Cut-off Frequency and High-Frequency Peaks in Six {{Kepler}} Stars with Stochastically Excited Pulsations},
  author = {Jim{\'e}nez, A. and Garc{\'i}a, R. A. and P{\'e}rez Hern{\'a}ndez, F. and Mathur, S.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {583},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526469},
  abstract = {Gravito-acoustic modes in the Sun and other stars propagate in resonant cavities with a frequency below a given limit known as the cut-off frequency. At higher frequencies, waves are no longer trapped in the stellar interior and become traveller waves. In this article, we study six pulsating solar-like stars at different evolutionary stages observed by the NASA Kepler mission. These high signal-to-noise targets show a peak structure that extends at very high frequencies and are good candidates for studying the transition region between the modes and interference peaks or pseudo-modes. Following the same methodology successfully applied on Sun-as-a-star measurements, we uncover the existence of pseudo-modes in these stars with one or two dominant interference patterns depending on the evolutionary stage of the star. We also infer their cut-off frequency as the midpoint between the last eigenmode and the first peak of the interference patterns. Using ray theory we show that, while the period of one of the interference patterns is very close to half the large separation, the period of the other interference pattern depends on the time phase of mixed waves, thus carrying additional information on the stellar structure and evolution.},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/UWPIFQUN/Jiménez et al. - 2015.pdf}
}

@article{Johns2018,
  title = {Revised {{Exoplanet Radii}} and {{Habitability Using Gaia Data Release}} 2},
  author = {Johns, Daniel and Marti, Connor and Huff, Madison and McCann, Jacob and Wittenmyer, Robert A. and Horner, Jonathan and Wright, Duncan J.},
  year = {2018},
  month = nov,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {239},
  number = {1},
  eprint = {1808.04533},
  pages = {14},
  publisher = {{American Astronomical Society}},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/aae5fb},
  urldate = {2020-03-07},
  abstract = {Accurate stellar properties are crucial for determining exoplanet characteristics. Gaia DR2 presents revised distances, luminosities, and radii for 1.6 billion stars. Here, we report the calculation of revised radii and densities for 320 exoplanets using this data and present updated calculations of the incident flux received by 690 known exoplanets. This allows the likelihood that those planets orbit in the habitable zone of their host stars to be reassessed. As a result of this analysis, three planets can be added to the catalogue of potentially habitable worlds: HIP\textasciitilde 67537\textasciitilde b, HD\textasciitilde 148156\textasciitilde b, and HD\textasciitilde 106720\textasciitilde b. In addition, the changed parameterisation of BD\textasciitilde +49\textasciitilde 898 means that its planet, BD\textasciitilde +49\textasciitilde 898\textasciitilde b, now receives an incident flux that places it outside the optimistic habitable zone region, as defined by \textbackslash citep\{Kopparapu2013,Kopparapu2014\}. We find that use of the new \textbackslash textit\{Gaia\} data results in a mean increase in calculated exoplanet radius of 3.76\textbackslash\%. Previously, CoRoT-3 b had been reported as having the highest density of all known exoplanets. Here, we use updated information to revise the calculated density of CoRoT-3\textasciitilde b from 26.4\$g\textbackslash :cm\^\{-3\}\$ to 17.3\$\textbackslash pm2.9g\textbackslash :cm\^\{-3\}\$. We also report the densest exoplanet in our dataset, KELT-1\textasciitilde b, with a density of 23.7\$\textbackslash pm4.0g\textbackslash :cm\^\{-3\}\$. Overall, our results highlight the importance of ensuring the the parameterisation of known exoplanets be revisited whenever significant improvements are made to the precision of the stellar parameters upon which they are based.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6BQ554PF/full-text.pdf}
}

@article{Jorgensen2005,
  title = {Determination of Stellar Ages from Isochrones: {{Bayesian}} Estimation versus Isochrone Fitting},
  author = {J{\o}rgensen, B. R. and Lindegren, L.},
  year = {2005},
  month = jun,
  journal = {Astronomy and Astrophysics},
  volume = {436},
  number = {1},
  pages = {127--143},
  issn = {00046361},
  doi = {10.1051/0004-6361:20042185},
  urldate = {2020-07-08},
  abstract = {We present a new method, using Bayesian estimation, to determine stellar ages and their uncertainties from observational data and theoretical isochrones. The result for an individual star is obtained as the relative posterior probability density as function of the age ("G function"). From this can be derived the most probable age and confidence intervals. The convoluted morphology of isochrones and strong non-linearities make the age determination by any method difficult and susceptible to statistical biases, and as a result age uncertainties havee often been underestimated in the literature. From simulations we find that the G functions provide a general, robust and reliable way to quantify age information. Resulting age estimates are at least as accurate as those obtained with conventional isochrone fitting methods, and in some cases much better, especially when the observational uncertainties are large. We also find that undetected binaries, on the whole, have a surprisingly small effect on the age determinations. For a stellar sample, the individual G functions can be combined to derive the star formation history of the population; this will be developed in a forthcoming paper. For a coeval population the combination simplifies to computing the product of the individual G functions, and we apply that method to estimate the ages of the two open clusters IC 4651 and M 67, using Padova isochrones and photometric data from the literature. For IC 4651 we find an estimated age of 1.56{$\pm$}0.03 Gyr, assuming a true distance modulus of 9.80. For M 67 we find 4.05{$\pm$}0.05 Gyr for true distance modulus 9.48. The small formal errors of these age estimates do not include the (much larger) uncertainties from calibration and model errors, but illustrate the statistical power of combining G functions. Our statistical approach to the age determination problem is well suited for the mass treatment of data resulting from large-scale surveys such as the Gaia mission. \textcopyright{} ESO 2005.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Solar neighbourhood,Stars: evolution,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/YHK3PSV9/full-text.pdf}
}

@article{Jouve2007,
  title = {On the Role of Meridional Flows in Flux Transport Dynamo Models},
  author = {Jouve, L. and Brun, A. S.},
  year = {2007},
  month = dec,
  journal = {Astronomy and Astrophysics},
  volume = {474},
  number = {1},
  eprint = {0712.3200},
  pages = {239--250},
  doi = {10.1051/0004-6361:20077070},
  urldate = {2020-07-13},
  abstract = {The Sun is a magnetic star whose magnetism and cyclic activity is linked to the existence of an internal dynamo. We aim to understand the establishment of the solar magnetic 22-yr cycle, its associated butterfly diagram and field parity selection through numerical simulations of the solar global dynamo. Inspired by recent observations and 3D simulations that both exhibit multicellular flows in the solar convection zone, we seek to characterise the influence of various profiles of circulation on the behaviour of solar mean-field dynamo models. We are using 2-D mean field flux transport Babcock-Leighton numerical models in which we test several types of meridional flows: 1 large single cell, 2 cells in radius and 4 cells per hemisphere. We confirm that adding cells in latitude tends to speed up the dynamo cycle whereas adding cells in radius more than triples the period. We find that the cycle period in the four cells model is less sensitive to the flow speed than in the other simpler meridional circulation profiles studied. Moreover, our studies show that adding cells in radius or in latitude seems to favour the parity switching to a quadrupolar solution. According to our numerical models, the observed 22-yr cycle and dipolar parity is easily reproduced by models including multicellular meridional flows. On the contrary, the resulting butterfly diagram and phase relationship between the toroidal and poloidal fields are affected to a point where it is unlikely that such multicellular meridional flows persist for a long period of time inside the Sun, without having to reconsider the model itself.},
  archiveprefix = {arxiv},
  keywords = {Methods: numerical,notion,notion-database,Sun: activity,Sun: interior,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/MEGZ9R8R/full-text.pdf}
}

@article{Jouve2010a,
  title = {Exploring the {{Pcyc}} vs. {{Prot}} Relation with Flux Transport Dynamo Models of Solar-like Stars},
  author = {Jouve, L. and Brown, B. P. and Brun, A. S.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {509},
  number = {1},
  pages = {1--11},
  issn = {14320746},
  doi = {10.1051/0004-6361/200913103},
  abstract = {Aims: Understand stellar magnetism and test the validity of the Babcock-Leighton flux transport mean field dynamo models with stellar activity observations Methods: 2-D mean field dynamo models at various rotation rates are computed with the STELEM code to study the sensitivity of the activity cycle period and butterfly diagram to parameter changes and are compared to observational data. The novelty is that these 2-D mean field dynamo models incorporate scaling laws deduced from 3-D hydrodynamical simulations for the influence of rotation rate on the amplitude and profile of the meridional circulation. These models make also use of observational scaling laws for the variation of differential rotation with rotation rate. Results: We find that Babcock-Leighton flux transport dynamo models are able to reproduce the change in topology of the magnetic field (i.e. toward being more toroidal with increasing rotation rate) but seem to have difficulty reproducing the cycle period vs activity period correlation observed in solar-like stars if a monolithic single cell meridional flow is assumed. It may however be possible to recover the Pcyc vs. Prot relation with more complex meridional flows, if the profile changes in a particular assumed manner with rotation rate. Conclusions: The Babcock-Leighton flux transport dynamo model based on single cell meridional circulation does not reproduce the Pcyc vs. Prot relation unless the amplitude of the meridional circulation is assumed to increase with rotation rate which seems to be in contradiction with recent results obtained with 3-D global simulations. \textcopyright{} 2010 ESO.},
  keywords = {Activity - Methods,Activity - Stars,Magnetic fields - Sun,Magnetohydrodynamics - Stars,notion,notion-database,Numerical},
  file = {/Users/lbugnet/Zotero/storage/BGVPF55R/Jouve, Brown, Brun - 2010.pdf}
}

@article{Jouve2015,
  title = {{{3D}} Evolution of Magnetic Fields in a Differentially Rotating Stellar Radiative Zone},
  author = {Jouve, Laur{\`e}ne and Gastine, Thomas and Ligni{\`e}res, Fran{\c c}ois},
  year = {2015},
  month = dec,
  journal = {Astronomy \& Astrophysics},
  volume = {575},
  eprint = {1412.2900},
  doi = {10.1051/0004-6361/201425240},
  urldate = {2020-07-17},
  abstract = {The question of the origin and evolution of magnetic fields in stars possessing a radiative envelope, like the A-type stars, is still regarded as a challenge for stellar physics. Those zones are likely to be differentially rotating, which suggests that strong interactions between differential rotation and magnetic fields could be at play. We numerically compute the joint evolution of the magnetic and velocity fields in a 3D spherical shell starting from an initial profile for the poloidal magnetic field and differential rotation. The poloidal magnetic field is initially wound-up by the differential rotation to produce a toroidal field which becomes unstable. In the particular setup studied here where the differential rotation is dominant, the magneto-rotational instability is triggered. The growth rate of the instability depends mainly on the initial rotation rate, while the background state typically oscillates over a poloidal Alfv\textbackslash 'en time. We thus find that the axisymmetric magnetic configuration is strongly modified by the instability only if the ratio between the poloidal Alfv\textbackslash 'en frequency and the rotation rate is sufficiently small. An enhanced transport of angular momentum is found in the most unstable cases: the typical time to flatten the rotation profile is then much faster than the diffusion time scale. We conclude that the magneto-rotational instability is always favored (over the Tayler instability) in unstratified spherical shells when an initial poloidal field is sheared by a sufficiently strong cylindrical differential rotation. A possible application to the magnetic desert observed among A stars is given. We argue that the dichotomy between stars exhibiting strong axisymmetric fields (Ap stars) and those harboring a sub-Gauss magnetism could be linked to the threshold for the instability.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/EF6DDW5U/full-text.pdf;/Users/lbugnet/Zotero/storage/MS6BCU6G/1412.2900.pdf}
}

@article{Jouve2020,
  title = {Astrophysics {{Interplay}} between Magnetic Fields and Differential Rotation in a Stably Stratified Stellar Radiative Zone},
  author = {Jouve, L and Ligni{\`e}res, F and Gaurat, M},
  year = {2020},
  journal = {A\&A},
  volume = {641},
  pages = {13},
  doi = {10.1051/0004-6361/202037828},
  abstract = {Context. The interactions between magnetic fields and differential rotation in stellar radiative interiors could play a major role in achieving an understanding of the magnetism of intermediate-mass and massive stars and of the differential rotation profile observed in red-giant stars. Aims. The present study is aimed at studying the flow and field produced by a stellar radiative zone which is initially made to rotate differentially in the presence of a large-scale poloidal magnetic field threading the whole domain. We focus both on the axisymmetric configurations produced by the initial winding-up of the magnetic field lines and on the possible instabilities of those configurations. We investigate in detail the effects of the stable stratification and thermal diffusion and we aim, in particular, to assess the role of the stratification at stabilising the system. Methods. We performed 2D and 3D global Boussinesq numerical simulations started from an initial radial or cylindrical differential rotation and a large-scale poloidal magnetic field. Under the conditions of a large rotation frequency compared to the Alfv\'en frequency, we built a magnetic configuration strongly dominated by its toroidal component. We then perturbed this configuration to observe the development of non-axisymmetric instabilities. Results. The parameters of the simulations were chosen to respect the ordering of time scales of a typical stellar radiative zone. In this framework, the axisymmetric evolution is studied by varying the relative effects of the thermal diffusion, the Brunt-V\"ais\"al\"a frequency, the rotation, and the initial poloidal field strength. After a transient time and using a suitable adimensionalisation, we find that the axisymmetric state only depends on t es /t Ap the ratio between the Eddington-Sweet circulation time scale and the Alfv\'en time scale. A scale analysis of the Boussinesq magnetohydrodynamical equations allows us to recover this result. In the cylindrical case, a magneto-rotational instability develops when the thermal diffusivity is sufficiently high to enable the favored wavenumbers to be insensitive to the effects of the stable stratification. In the radial case, the magneto-rotational instability is driven by the latitudinal shear created by the back-reaction of the Lorentz force on the flow. Increasing the level of stratification then leaves the growth rate of the instability mainly unaffected while its horizontal length scale grows. Conclusions. Non-axisymmetric instabilities are likely to exist in stellar radiative zones despite the stable stratification. They could be at the origin of the magnetic dichotomy observed in intermediate-mass and massive stars. They are also unavoidable candidates for the transport of angular momentum in red giant stars.},
  keywords = {instabilities-magnetohydrodynamics (MHD)-methods,interiors,magnetic field-stars,notion,notion-database,numerical-stars,rotation-stars},
  file = {/Users/lbugnet/Zotero/storage/H9HIA67D/full-text.pdf}
}

@article{Joy1945,
  title = {T {{Tauri Variable Stars}}.},
  author = {Joy, Alfred H.},
  year = {1945},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {102},
  pages = {168},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/144749},
  urldate = {2020-07-12},
  abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein-protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-{$\alpha$}-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD {$\leq$} 2.0 \AA{} for the interface backbone atoms) increased from 21\% with default Glide SP settings to 58\% with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63\% success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40\% of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
  keywords = {notion,notion-database}
}

@article{Juckett2008,
  title = {Evidence for Long-Term Retrograde Motions of Sunspot Patterns and Indications of Coupled g-Mode Rotation Rates},
  author = {Juckett, David A. and Wolff, Charles L.},
  year = {2008},
  journal = {Solar Physics},
  volume = {252},
  number = {2},
  pages = {247--266},
  issn = {00380938},
  doi = {10.1007/s11207-008-9265-x},
  abstract = {Solar g-modes are global oscillations that would exist primarily in the radiative zone (RZ) and would be excited by either convective overshoot or nuclear burning in the core. Wolff and O'Donovan (Astrophys. J. 661, 568, 2007) proposed a non-linear coupling of g-modes into groups that share the same harmonic degree {$\mathscr{l}$}. Each group (denoted set({$\mathscr{l}$}) exhibits a unique retrograde rotation rate with respect to the RZ that depends mainly on {$\mathscr{l}$}. The coupling yields a standing wave (nearly stationary in longitude) that has two angularly defined hot spots offset from the equator on opposite sides of the Sun that would deposit energy asymmetrically in the lower convective envelope (CE). It is anticipated that when two or more groups overlap in longitude, an increase in local heating would influence the distribution of sunspots. In this paper, we scanned a multitude of rotational reference frames for sunspot clustering to test for frames that are concordant with the rotation of these g-modes sets. To achieve this, spherical harmonic filtering of sunspot synoptic maps was used to extract patterns consistent with coalesced g-modes. The latitude band, with minimal differential rotation, was sampled from each filtered synoptic map and layered into a stackplot. This was progressively shifted, line-by-line, into different rotational reference frames. We have detected long-lived longitudinal alignments, spanning 90 years of solar cycles, which are consistent with the rotation rate of the deep solar interior as well as other rotational frames predicted by the coupled g-mode model. Their sidereal rotation rates of 370.0, 398.8, 412.7, 418.3, 421.0, 424.2 and 430.0 nHz correspond, respectively, to coupled g-modes for {$\mathscr{l}$} = 2 through 7 and G, where G is a set with high {$\mathscr{l}$} values or a group of such sets (unresolved) that rotate almost as fast as the RZ. While the clustering in these reference frames offers new approaches for studying the longitudinal behavior of solar activity, it tentatively leads to the more profound conclusion that a portion of the driving force for sunspot occurrence is linked to energy extracted from the solar core and deposited at the top of the RZ by solar g-modes. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  isbn = {1120700892},
  keywords = {G-modes,notion,notion-database,Rotation,Solar activity,Solar cycle,Solar interior,Spherical harmonics,Stackplots,Sunspots},
  file = {/Users/lbugnet/Zotero/storage/WJ7VMKTC/Juckett, Wolff - 2008.pdf}
}

@article{Judge2011,
  title = {Solar and Stellar Activity: {{Diagnostics}} and Indices},
  author = {Judge, Philip G. and Thompson, Michael J.},
  year = {2011},
  journal = {Proceedings of the International Astronomical Union},
  volume = {7},
  number = {S286},
  eprint = {1201.4625},
  pages = {15--26},
  issn = {17439213},
  doi = {10.1017/S1743921312004589},
  abstract = {We summarize the fifty-year concerted effort to place the "activity" of the Sun in the context of the stars. As a working definition of solar activity in the context of stars, we adopt those globally-observable variations on time scales below thermal time scales, of {$\sim$}10 5 yr for the convection zone. So defined, activity is dominated by magnetic-field evolution, including the 22-year Hale cycle, the typical time it takes for the quasi-periodic reversal in which the global magnetic-field takes place. This is accompanied by sunspot variations with 11 year periods, known since the time of Schwabe, as well as faster variations due to rotation of active regions and flaring. "Diagnostics and indices" are terms given to the indirect signatures of varying magnetic-fields, including the photometric (broad-band) variations associated with the sunspot cycle, and variations of the accompanying heated plasma in higher layers of stellar atmospheres seen at special optical wavelengths, and UV and X-ray wavelengths. Our attention is also focussed on the theme of the Symposium by examining evidence for deep and extended minima of stars, and placing the 70-year long solar Maunder Minimum into a stellar context. \textcopyright{} 2012 International Astronomical Union.},
  archiveprefix = {arxiv},
  isbn = {9781107019867},
  keywords = {notion,notion-database,stars: activity,stars: evolution,Sun: chromosphere,Sun: helioseismology,Sun: magnetic fields,Sun: UV radiation,techniques: photometric,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/V97DNWLJ/Judge, Thompson - 2011.pdf}
}

@article{Jurcsik1996,
  title = {Determination of [{{Fe}}/{{H}}] from the Light Curves of {{RR Lyrae}} Stars},
  author = {Jurcsik, Kovacs, G., J.},
  year = {1996},
  journal = {A\&A},
  pages = {111--120},
  urldate = {2020-04-09},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/V7R2CKY2/full-text.pdf}
}

@article{Jurcsik2009,
  title = {The {{Konkoly Blazhko Survey}}: {{Is}} Light-Curve Modulation a Common Property of {{RRab}} Stars?},
  author = {Jurcsik, J. and S{\'o}dor, A and Szeidl, B. and Hurta, Zs and V{\'a}radi, M. and Posztob{\'a}nyi, K. and Vida, K. and Hajdu, G. and Kov{\'a}ri, Zs and Nagy, I. and Moln{\'a}r, L. and Belucz, B.},
  year = {2009},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {400},
  number = {2},
  eprint = {0908.1015},
  pages = {1006--1018},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.15515.x},
  urldate = {2020-04-11},
  abstract = {A systematic survey to establish the true incidence rate of Blazhko modulation among short-period, fundamental-mode, Galactic field RR Lyrae stars has been carried out. The Konkoly Blazhko Survey (KBS) was initiated in 2004. Since then, more than 750 nights of observation have been devoted to this project. A sample of 30 RRab stars was extensively observed, and light-curve modulation was detected in 14 cases. The 47 per cent occurrence rate of the modulation is much larger than any previous estimate. The significant increase of the detected incidence rate is mostly a result of the discovery of small-amplitude modulation. Half of the Blazhko variables in our sample show the modulation with such a small amplitude that they would definitely have been missed in previous surveys. We have found that the modulation can be very unstable in some cases; for example, RY Com showed regular modulation during only one part of the observations, and had a stable light curve with abrupt, small changes in the pulsation amplitude during two observing seasons. This type of light-curve variability is hard to detect in the data from other surveys. The higher frequency of the light-curve modulation of RRab stars makes it even more important to find an explanation for the Blazhko phenomenon. The validity of the [Fe/H](P, {$\varphi$}31) relationship using the mean light curves of Blazhko variables is checked in our sample. We found that the formula gives accurate result for small-modulation-amplitude Blazhko stars, and this is also the case for large-modulation-amplitude stars if the light curve has complete phase coverage. However, if the data for large-modulation-amplitude Blazhko stars are not extended enough (e.g. fewer than 500 data points from fewer than 15 nights), the formula may give false result owing to the distorted shape of the mean light curve used. \textcopyright{} 2009 RAS.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: horizontal branch,Stars: oscillations,Stars: variables: other,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/B86N6I4X/full-text.pdf}
}

@article{Kaiser2008a,
  title = {The {{STEREO}} Mission: {{An}} Introduction},
  author = {Kaiser, M. L. and Kucera, T. A. and Davila, J. M. and Cyr, O. C.St and Guhathakurta, M. and Christian, E.},
  year = {2008},
  journal = {Space Science Reviews},
  volume = {136},
  number = {1-4},
  pages = {5--16},
  issn = {00386308},
  doi = {10.1007/s11214-007-9277-0},
  abstract = {The twin STEREO spacecraft were launched on October 26, 2006, at 00:52 UT from Kennedy Space Center aboard a Delta 7925 launch vehicle. After a series of highly eccentric Earth orbits with apogees beyond the moon, each spacecraft used close flybys of the moon to escape into orbits about the Sun near 1 AU. Once in heliospheric orbit, one spacecraft trails Earth while the other leads. As viewed from the Sun, the two spacecraft separate at approximately 44 to 45 degrees per year. The purposes of the STEREO Mission are to understand the causes and mechanisms of coronal mass ejection (CME) initiation and to follow the propagation of CMEs through the inner heliosphere to Earth. Researchers will use STEREO measurements to study the mechanisms and sites of energetic particle acceleration and to develop three-dimensional (3-D) time-dependent models of the magnetic topology, temperature, density and velocity of the solar wind between the Sun and Earth. To accomplish these goals, each STEREO spacecraft is equipped with an almost identical set of optical, radio and in situ particles and fields instruments provided by U.S. and European investigators. The SECCHI suite of instruments includes two white light coronagraphs, an extreme ultraviolet imager and two heliospheric white light imagers which track CMEs out to 1 AU. The IMPACT suite of instruments measures in situ solar wind electrons, energetic electrons, protons and heavier ions. IMPACT also includes a magnetometer to measure the in situ magnetic field strength and direction. The PLASTIC instrument measures the composition of heavy ions in the ambient plasma as well as protons and alpha particles. The S/WAVES instrument uses radio waves to track the location of CME-driven shocks and the 3-D topology of open field lines along which flow particles produced by solar flares. Each of the four instrument packages produce a small real-time stream of selected data for purposes of predicting space weather events at Earth. NOAA forecasters at the Space Environment Center and others will use these data in their space weather forecasting and their resultant products will be widely used throughout the world. In addition to the four instrument teams, there is substantial participation by modeling and theory oriented teams. All STEREO data are freely available through individual Web sites at the four Principal Investigator institutions as well as at the STEREO Science Center located at NASA Goddard Space Flight Center. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  keywords = {CME,notion,notion-database,Solar,Three-dimensional},
  file = {/Users/lbugnet/Zotero/storage/XC5F2YN2/Kaiser et al. - 2008.pdf}
}

@article{Kallinger2008,
  title = {{{MOST}} Found Evidence for Solar-Type Oscillations in the {{K2}} Giant Star {{HD20884}}},
  author = {Kallinger, T.},
  year = {2008},
  journal = {Communications in Asteroseismology},
  volume = {153},
  pages = {84--102},
  issn = {1021-2043},
  doi = {10.1553/cia_153s84},
  abstract = {We found evidence for radial p-modes and nonradial mixed modes in the oscillation spectrum of the K giant HD 20884 based on 20.6 days of nearly continuous high-precision photometry obtained by the Canadian microsatellite MOST Oscillation frequencies range from 5-31 {$\mu$}Hz (periods of about 2.3 d - 9 hr) with luminosity amplitudes between about 300 and 950 ppm and mode lifetimes exceeding 10 days are indicated. The mode identifications are based on searches of a large grid of models for a best fit to the frequencies and temperature of HD 20884. The latter is better constrained now by spectroscopy obtained at the David Dunlap Observatory as part of this work. Based on data from the MOST (Microvariability \{\&\} Oscillation of STars) satellite, a Canadian Space Agency mission jointly operated by Dynacon, Inc., the University of Toronto Institute of Aerospace Studies, and the University of British Columbia, with assistance from the University of Vienna, Austria.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/N5V8A4NS/Kallinger - 2008.pdf}
}

@article{Kallinger2010,
  title = {Oscillating Red Giants in the {{CoRoT}} Exofield: {{Asteroseismic}} Mass and Radius Determination},
  author = {Kallinger, T. and Weiss, W. W. and Barban, C. and Baudin, F. and Cameron, C. and Carrier, F. and De Ridder, J. and Goupil, M. J. and Gruberbauer, M. and Hatzes, A. and Hekker, S. and Samadi, R. and Deleuil, M.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {509},
  number = {1},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/200811437},
  abstract = {Context: Observations and analysis of solar-type oscillations in red-giant stars is an emerging aspect of asteroseismic analysis with a number of open questions yet to be explored. Although stochastic oscillations have previously been detected in red giants from both radial velocity and photometric measurements, those data were either too short or had sampling that was not complete enough to perform a detailed data analysis of the variability. The quality and quantity of photometric data as provided by the CoRoT satellite is necessary to provide a breakthrough in observing p-mode oscillations in red giants. We have analyzed continuous photometric time-series of about 11 400 relatively faint stars obtained in the exofield of CoRoT during the first 150 days long-run campaign from May to October 2007. We find several hundred stars showing a clear power excess in a frequency and amplitude range expected for red-giant pulsators. In this paper we present first results on a sub-sample of these stars. Aims: Knowing reliable fundamental parameters like mass and radius is essential for detailed asteroseismic studies of red-giant stars. As the CoRoT exofield targets are relatively faint (11-16 mag) there are no (or only weak) constraints on the stars' location in the H-R diagram. We therefore aim to extract information about such fundamental parameters solely from the available time series. Methods: We model the convective background noise and the power excess hump due to pulsation with a global model fit and deduce reliable estimates for the stellar mass and radius from scaling relations for the frequency of maximum oscillation power and the characteristic frequency separation. Results: We provide a simple method to estimate stellar masses and radii for stars exhibiting solar-type oscillations. Our method is tested on a number of known solar-type pulsators. \textcopyright{} 2010 ESO.},
  keywords = {Fundamental parameters - Techniques,notion,notion-database,Oscillations - Stars,Photometric,Stars},
  file = {/Users/lbugnet/Zotero/storage/3VFWCRQX/Kallinger et al. - 2010.pdf}
}

@article{Kallinger2010a,
  title = {Evidence for Granulation in Early {{A-type}} Stars},
  author = {Kallinger, Thomas and Matthews, Jaymie M.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {711},
  number = {1 PART 2},
  eprint = {1001.4879},
  pages = {1--8},
  issn = {20418213},
  doi = {10.1088/2041-8205/711/1/L35},
  abstract = {Stars with spectral types earlier than about F0 on (or close) to the main sequence have long been believed to lack observable surface convection, although evolutionary models of A-type stars do predict very thin surface convective zones. We present evidence for granulation in two {$\delta$}Scuti stars of spectral type A2: HD174936 and HD50844. Recent analyses of space-based CoRoT data revealed up to some 1000 frequencies in the photometry of these stars. The frequencies were interpreted as individual pulsation modes. If true, there must be large numbers of nonradial modes of very high degree l which should suffer cancellation effects in disk-integrated photometry (even of high space-based precision). The p-mode interpretation of all the frequencies in HD174936 and HD50844 depends on the assumption of white (frequency-independent) noise. Our independent analyses of the data provide an alternative explanation: most of the peaks in the Fourier spectra are the signature of non-white granulation background noise, and less than about 100 of the frequencies are actual stellar p-modes in each star. We find granulation timescales which are consistent with scaling relations that describe cooler stars with known surface convection. If the granulation interpretation is correct, the hundreds of low-amplitude Fourier peaks reported in recent studies are falsely interpreted as independent pulsation modes and a significantly lower number of frequencies are associated with pulsation, consistent with only modes of low degree. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,{Stars: individual (HD50844, HD 174936)},Stars: oscillations,Stars: variables: delta Scuti},
  file = {/Users/lbugnet/Zotero/storage/GP3UXRCE/Kallinger, Matthews - 2010.pdf}
}

@article{Kallinger2010c,
  title = {The Nature of P-Modes and Granulation in {{HD49933}} Observed by {{CoRoT}}},
  author = {Kallinger, T. and Gruberbauer, M. and Guenther, D. B. and Fossati, L. and Weiss, W. W.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {510},
  number = {1},
  pages = {1--9},
  issn = {00046361},
  doi = {10.1051/0004-6361/200811438},
  abstract = {Context: Recent observations of HD49933 by the space-photometric mission CoRoT provide photometric evidence of solar type oscillations in a star other than our Sun. The first published reduction, analysis, and interpretation of the CoRoT data yielded a spectrum of p-modes with l = 0, 1, and 2. Aims: We present our own analysis of the CoRoT data in an attempt to compare the detected pulsation modes with eigenfrequencies of models that are consistent with the observed luminosity and surface temperature. Methods: We used the Gruberbauer et al. frequency set derived based on a more conservative Bayesian analysis with ignorance priors and fit models from a dense grid of model spectra.We also introduce a Bayesian approach to searching and quantifying the best model fits to the observed oscillation spectra. Results: We identify 26 frequencies as radial and dipolar modes. Our best fitting model has solar composition and coincides within the error box with the spectroscopically determined position of HD49933 in the H-R diagram. We also show that lower-than-solar Z models have a lower probability of matching the observations than the solar metallicity models. To quantify the effect of the deficiencies in modeling the stellar surface layers in our analysis, we compare adiabatic and nonadiabatic model fits and find that the latter reproduces the observed frequencies better. \textcopyright{} 2010 ESO.},
  keywords = {notion,notion-database,Stars: fundamental parameters,Stars: individual: HD 49933,Stars: late-type,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/43BTSQ2B/Kallinger et al. - 2010(2).pdf}
}

@article{Kallinger2012a,
  title = {Evolutionary Influences on the Structure of Red-Giant Acoustic Oscillation Spectra from 600d of {{Kepler}} Observations},
  author = {Kallinger, T. and Hekker, S. and Mosser, B. and De Ridder, J. and Bedding, T. R. and Elsworth, Y. P. and Gruberbauer, M. and Guenther, D. B. and Stello, D. and Basu, S. and Garc{\'i}a, R. A. and Chaplin, W. J. and Mullally, F. and Still, M. and Thompson, S. E.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {541},
  issn = {00046361},
  doi = {10.1051/0004-6361/201218854},
  abstract = {Context. It was recently discovered that the period spacings of mixed pressure/gravity dipole modes in red giants permit a distinction between the otherwise unknown evolutionary stage of these stars. The Kepler space mission is reaching continuous observing times long enough to also start studying the fine structure of the observed pressure-mode spectra. Aims. In this paper, we aim to study the signature of stellar evolution on the radial and pressure-dominated l = 2 modes in an ensemble of red giants that show solar-type oscillations. Methods. We use established methods to automatically identify the mode degree of l = 0 and 2 modes and measure the large ({$\Delta\nu$} c) and small ({$\delta\nu$} 02) frequency separation around the central radial mode. We then determine the phase shift {$\in$} c of the central radial mode, i.e. the linear offset in the asymptotic fit to the acoustic modes. Furthermore we measure the individual frequencies of radial modes and investigate their average curvature. Results. We find that {$\in$} c is significantly different for red giants at a given {$\Delta\nu$} c but which burn only H in a shell (RGB) than those that have already ignited core He burning. Even though not directly probing the stellar core the pair of local seismic observables ({$\Delta\nu$} c, {$\in$} c) can be used as an evolutionary stage discriminator that turned out to be as reliable as the period spacing of the mixed dipole modes. We find a tight correlation between {$\in$} c and {$\Delta\nu$} c for RGB stars and unlike less evolved stars we find no indication that {$\in$} c depends on other properties of the star. It appears that the difference in {$\in$} c between the two populations becomes smaller and eventually indistinguishable if we use an average of several radial orders, instead of a local, i.e. only around the central radial mode, large separation to determine the phase shift. This indicates that the information on the evolutionary stage is encoded locally, more precisely in the shape of the radial mode sequence. This shape turns out to be approximately symmetric around the central radial mode for RGB stars but asymmetric for core He burning stars. We computed radial mode frequencies for a sequence of red-giant models and find them to qualitatively confirm our findings. We also find that, at least in our models, the local {$\Delta\nu$} is an at least as good and mostly better proxy for both the asymptotic spacing and the large separation scaled from the model density than the average {$\Delta\nu$}. Finally, we investigate the signature of the evolutionary stage on {$\delta\nu$} 02 and quantify the mass dependency of this seismic parameter. \textcopyright{} 2012 ESO.},
  keywords = {notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/SLR9TIGC/Kallinger et al. - 2012.pdf}
}

@article{Kallinger2014,
  title = {The Connection between Stellar Granulation and Oscillation as Seen by the {{Kepler}} Mission},
  author = {Kallinger, T. and De Ridder, J. and Hekker, S. and Mathur, S. and Mosser, B. and Gruberbauer, M. and Garc{\'i}a, R. A. and Karoff, C. and Ballot, J.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {570},
  eprint = {1408.0817},
  pages = {1--17},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424313},
  abstract = {Context. The long and almost continuous observations by Kepler show clear evidence of a granulation background signal in a large sample of stars, which is interpreted as the surface manifestation of convection. It has been shown that its characteristic timescale and rms intensity fluctuation scale with the peak frequency ({$\nu$}max) of the solar-like oscillations. Various attempts have been made to quantify the observed signal, to determine scaling relations for its characteristic parameters, and to compare them to theoretical predictions. Even though they are consistent on a global scale, large systematic differences of an unknown origin remain between different methods, as well as between the observations and simulations. Aims. We aim to study different approaches to quantifying the signature of stellar granulation and to search for a unified model that reproduces the observed signal best in a wide variety of stars. We then aim to define empirical scaling relations between the granulation properties and {$\nu$}max and various other stellar parameters. Methods. We use a probabilistic method to compare different approaches to extracting the granulation signal. We fit the power density spectra of a large set of Kepler targets, determine the granulation and global oscillation parameter, and quantify scaling relations between them. Results. We establish that a depression in power at about {$\nu$}max/2, known from the Sun and a few other main-sequence stars, is also statistically significant in red giants and that a super-Lorentzian function with two components is best suited to reproducing the granulation signal in the broader vicinity of the pulsation power excess. We also establish that the specific choice of the background model can affect the determination of {$\nu$}max, introducing systematic uncertainties that can significantly exceed the random uncertainties. We find the characteristic frequency (i.e., inverse timescale) and amplitude of both background components to tightly scale with {$\nu$}max for a wide variety of stars (about 2-2000\^a\textperthousand{} {$\mu$}Hz in {$\nu$}max), and quantify a mass dependency of the latter. To enable comparison with theoretical predictions (which do not include the observed power depression), we computed effective timescales and bolometric intensity fluctuations and found them to approximately scale as {$\tau$}effg-0.85T-0.4 and Agran(g2M)-1/4 (or more conveniently R/M3/4), respectively. Similarly, the bolometric pulsation amplitude scales approximately as Apuls(g2M)-1/3 (or R4/3/M), which implicitly verifies a separate mass and luminosity dependence of Apuls. We have also checked our scaling relations with solar reference values and find them in good agreement. Conclusions. We provide a thorough analysis of the granulation background signal in a large sample of stars, from which we establish a unified model that allows us to accurately extract the granulation and global oscillation parameter. The resulting scaling relations allow a simple estimate of the overall spectral shape of any solar-type oscillator and might serve as a starting point for future large-sample studies or as a reference for theoretical modelling of granulation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: fundamental parameters,Stars: late-type,Stars: oscillations (including pulsations),Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/HI9DTJ5P/Kallinger et al. - 2014.pdf}
}

@article{Kallinger2016,
  title = {Precise Stellar Surface Gravities from the Time Scales of Convectively Driven Brightness Variations},
  author = {Kallinger, Thomas and Hekker, Saskia and Garc{\'i}a, Rafael A. and Huber, Daniel and Matthews, Jaymie M.},
  year = {2016},
  month = jan,
  journal = {Science Advances},
  volume = {2},
  number = {1},
  pages = {1500654},
  publisher = {{American Association for the Advancement of Science}},
  issn = {23752548},
  doi = {10.1126/sciadv.1500654},
  urldate = {2020-07-08},
  abstract = {A significant part of the intrinsic brightness variations in cool stars of low and intermediate mass arises from surface convection (seen as granulation) and acoustic oscillations (p-mode pulsations). The characteristics of these phenomena are largely determined by the stars' surface gravity g.Detailed photometricmeasurements of either signal can yield an accurate value of g. However, even with ultraprecise photometry from NASA's Kepler mission, many stars are too faint for current methods or onlymoderate accuracy can be achieved in a limited range of stellar evolutionary stages. This means thatmany of the stars in the Kepler sample, including exoplanet hosts, are not sufficiently characterized to fully describe the sample and exoplanet properties.We present a novel way tomeasure surface gravities with accuracies of about 4\%.Our technique exploits the tight relation between g and the characteristic timescale of the combined granulation and p-mode oscillation signal. It is applicable to all stars with a convective envelope, including active stars. It canmeasure g in stars for which no other analysis is now possible. Because it depends on the time scale (and no other properties) of the signal, our technique is largely independent of the type of measurement (for example, photometry or radial velocity measurements) and the calibration of the instrumentation used. However, the oscillation signal must be temporally resolved; thus, it cannot be applied to dwarf stars observed by Kepler in its long-cadence mode.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ADH6BK6E/full-text.pdf}
}

@article{Kallinger2017,
  title = {Triple System {{HD}} 201433 with a {{SPB}} Star Component Seen by {{BRITE}} - {{Constellation}}: {{Pulsation}}, Differential Rotation, and Angular Momentum Transfer},
  shorttitle = {Triple System {{HD}} 201433 with a {{SPB}} Star Component Seen by {{BRITE}} - {{Constellation}}},
  author = {Kallinger, T. and Weiss, W. W. and Beck, P. G. and Pigulski, A. and Kuschnig, R. and Tkachenko, A. and Pakhomov, Y. and Ryabchikova, T. and L{\"u}ftinger, T. and Palle, P. L. and Semenko, E. and Handler, G. and Koudelka, O. and Matthews, J. M. and Moffat, A. F. J. and Pablo, H. and Popowicz, A. and Rucinski, S. and Wade, G. A. and Zwintz, K.},
  year = {2017},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {603},
  pages = {A13},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201730625},
  urldate = {2023-10-28},
  abstract = {Context. Stellar rotation affects the transport of chemical elements and angular momentum and is therefore a key process during stellar evolution, which is still not fully understood. This is especially true for massive OB-type stars, which are important for the chemical enrichment of the Universe. It is therefore important to constrain the physical parameters and internal angular momentum distribution of massive OB-type stars to calibrate stellar structure and evolution models. Stellar internal rotation can be probed through asteroseismic studies of rotationally split non radial oscillations but such results are still quite rare, especially for stars more massive than the Sun. The slowly pulsating B9V star HD 201433 is known to be part of a single-lined spectroscopic triple system, with two low-mass companions orbiting with periods of about 3.3 and 154 days. Aims: Our goal is to measure the internal rotation profile of HD 201433 and investigate the tidal interaction with the close companion. Methods: We used probabilistic methods to analyse the BRITE - Constellation photometry and radial velocity measurements, to identify a representative stellar model, and to determine the internal rotation profile of the star. Results: Our results are based on photometric observations made by BRITE - Constellation and the Solar Mass Ejection Imager on board the Coriolis satellite, high-resolution spectroscopy, and more than 96 yr of radial velocity measurements. We identify a sequence of nine frequency doublets in the photometric time series, consistent with rotationally split dipole modes with a period spacing of about 5030 s. We establish that HD 201433 is in principle a solid-body rotator with a very slow rotation period of 297 {$\pm$} 76 days. Tidal interaction with the inner companion has, however, significantly accelerated the spin of the surface layers by a factor of approximately one hundred. The angular momentum transfer onto the surface of HD 201433 is also reflected by the statistically significant decrease of the orbital period of about 0.9 s during the last 96 yr. Conclusions: Combining the asteroseismic inferences with the spectroscopic measurements and the orbital analysis of the inner binary system, we conclude that tidal interactions between the central SPB star and its inner companion have almost circularised the orbit. They have, however, not yet aligned all spins of the system and have just begun to synchronise rotation. Based on data collected by the BRITE - Constellation satellite mission, built, launched and operated thanks to support from the Austrian Aeronautics and Space Agency and the University of Vienna, the Canadian Space Agency (CSA), and the Foundation for Polish Science \& Technology (FNiTP MNiSW) and National Science Centre (NCN), the Hermes spectrograph mounted on the 1.2 m Mercator Telescope at the Spanish Observatorio del Roque de los Muchachos of the Instituto de Astrof\'isica de Canarias, and the Solar Mass Ejection Imager, which is a joint project of the University of California San Diego, Boston College, the University of Birmingham (UK), and the Air Force Research Laboratory.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,binaries: general,stars: individual: HD 201433,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2017A\&A...603A..13K},
  file = {/Users/lbugnet/Zotero/storage/WT9IFUSD/Kallinger et al. - 2017 - Triple system HD 201433 with a SPB star component .pdf}
}

@article{Kallinger2018,
  title = {Nonlinear Seismic Scaling Relations},
  author = {Kallinger, T. and Beck, P. G. and Stello, D. and Garcia, R. A.},
  year = {2018},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {616},
  eprint = {1805.06249},
  doi = {10.1051/0004-6361/201832831},
  urldate = {2020-07-23},
  abstract = {In recent years the global seismic scaling relations for the frequency of maximum power and for the large frequency separation have caught the attention of various fields of astrophysics. With the exquisite photometry of \textbackslash textit\{Kepler\}, the uncertainties in the seismic observables are small enough to estimate masses and radii with a precision of only a few per cent. Even though this seems to work quite well for main-sequence stars, there is empirical evidence, mainly from studies of eclipsing binary systems, that the seismic scaling relations overestimate the mass and radius of red giants by about 15 and 5\textbackslash\%, respectively. Model-based corrections of the \$\textbackslash Delta\textbackslash nu -\$scaling reduce the problem but do not solve it. We re-examine the global oscillation parameters of the giants in the binary systems in order to determine their seismic fundamental parameters and find them to agree with the dynamic parameters from the literature if we adopt nonlinear scalings. We note that a curvature and glitch corrected \$\textbackslash Delta\textbackslash nu\_\textbackslash mathrm\{cor\}\$ should be preferred over a local or average values. We then compare the observed seismic parameters of the cluster giants to those scaled from independent measurements and find the same nonlinear behaviour as for the eclipsing binaries. Our final proposed scaling relations are based on both samples and cover a broad range of evolutionary stages from RGB to RC stars: \$g/\textbackslash sqrt\{T\_\textbackslash mathrm\{eff\}\} = (\textbackslash nu\_\textbackslash mathrm\{max\}/\textbackslash nu\_\textbackslash mathrm\{max,\textbackslash odot\})\^\{1.0075\textbackslash pm0.0021\}\$ and \$\textbackslash sqrt\{\textbackslash bar\textbackslash rho\} = (\textbackslash Delta\textbackslash nu\_\textbackslash mathrm\{cor\}/\textbackslash Delta\textbackslash nu\_\textbackslash mathrm\{cor,\textbackslash odot\})[\textbackslash eta - (0.0085\textbackslash pm0.0025) \textbackslash log\^2 (\textbackslash Delta\textbackslash nu\_\textbackslash mathrm\{cor\}/\textbackslash Delta\textbackslash nu\_\textbackslash mathrm\{cor,\textbackslash odot\})]\^\{-1\}\$, where \$g\$, \$T\_\textbackslash mathrm\{eff\}\$, and \$\textbackslash bar\textbackslash rho\$ are in solar units, \$\textbackslash nu\_\textbackslash mathrm\{max,\textbackslash odot\}=3140\textbackslash pm5\textbackslash mu\$Hz and \$\textbackslash Delta\textbackslash nu\_\textbackslash mathrm\{cor,\textbackslash odot\}=135.08\textbackslash pm0.02\textbackslash mu\$Hz , and \$\textbackslash eta\$ is equal to one in case of RGB stars and \$1.04\textbackslash pm0.01\$ for RC stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/INRCI49J/full-text.pdf}
}

@article{Kamchatnov1982,
  title = {Topological Solitons in Magnetohydrodynamics},
  author = {Kamchatnov, A M},
  year = {1982},
  journal = {Sov JETP},
  volume = {82},
  urldate = {2020-07-02},
  abstract = {We use the Hopf mapping to construct a magnetic configuration consisting of closed field lines, each of which is linked with all the other ones. We obtain in this way a solution of the equations of magnetohydrodynamics of an ideal incompressible fluid with infinite conductivity, which describes a localized topological soliton.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZN729R2I/full-text.pdf}
}

@article{kantelhardtFractalMultifractalTime2008,
  title = {Fractal and {{Multifractal Time Series}}},
  author = {Kantelhardt, Jan W.},
  year = {2008},
  month = apr,
  journal = {Encyclopedia of Complexity and Systems Science},
  eprint = {0804.0747},
  pages = {1--37},
  publisher = {{Springer Berlin Heidelberg}},
  urldate = {2021-01-25},
  abstract = {Data series generated by complex systems exhibit fluctuations on many time scales and/or broad distributions of the values. In both equilibrium and non-equilibrium situations, the natural fluctuations are often found to follow a scaling relation over several orders of magnitude, allowing for a characterisation of the data and the generating complex system by fractal (or multifractal) scaling exponents. In addition, fractal and multifractal approaches can be used for modelling time series and deriving predictions regarding extreme events. This review article describes and exemplifies several methods originating from Statistical Physics and Applied Mathematics, which have been used for fractal and multifractal time series analysis.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4PE64YUS/full-text.pdf}
}

@article{Karoff2007a,
  title = {High-Frequency Modes in Solar-like Stars},
  author = {Karoff, C.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {381},
  number = {3},
  pages = {1001--1008},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.12340.x},
  abstract = {p-mode oscillations in solar-like stars are excited by the outer convection zone in these stars and reflected close to the surface. The p modes are trapped inside an acoustic cavity, but the modes only stay trapped up to a given frequency [known as the acoustic cut-off frequency ({$\nu$}ac)] as modes with larger frequencies are generally not reflected at the surface. This means that modes with frequency larger than the acoustic cut-off frequency must be travelling waves. The high-frequency modes may provide information about the physics in the outer layers of the stars and the excitation source and are therefore highly interesting as it is the estimation of these two phenomena that cause some of the largest uncertainties when calculating stellar oscillations. High-frequency modes have been detected in the Sun, in {$\beta$} Hydri and in {$\alpha$} Cen A and {$\alpha$} Cen B by smoothing the so-called echelle diagram and the large frequency separation as a function of frequency has been estimated. The large frequency separation has been compared with a simple model of the acoustic cavity which suggests that the reflectivity of the photosphere is larger at high frequency than predicted by standard models of the solar atmosphere and that the depth of the excitation source is larger than what has been estimated by other models and might depend on the order n and degree l of the modes. \textcopyright{} 2007 RAS.},
  keywords = {notion,notion-database,Stars: individual: {$\alpha$} Cen A,Stars: individual: {$\alpha$} Cen B,Stars: individual: {$\beta$} Hydri,Stars: oscillations,Sun: atmosphere,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/5W4BNLNU/Karoff - 2007.pdf}
}

@article{Karoff2007b,
  title = {Detection of P-Mode Oscillations in {$\beta$} {{Hydri}} from Photometric Observations with {{WIRE}}},
  author = {Karoff, C.},
  year = {2007},
  journal = {Communications in Asteroseismology},
  volume = {150},
  number = {2004},
  pages = {147--148},
  issn = {1021-2043},
  doi = {10.1553/cia150s147},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ELHKM84W/Karoff - 2007(2).pdf}
}

@article{Karoff2008,
  title = {Evidence {{That Solar Flares Drive Global Oscillations}} in the {{Sun}}},
  author = {Karoff, C. and Kjeldsen, H.},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {678},
  number = {1},
  eprint = {0803.3137},
  pages = {L73-L76},
  issn = {0004-637X},
  doi = {10.1086/588466},
  abstract = {Solar flares are large explosions on the Sun's surface caused by a sudden release of magnetic energy. They are known to cause local short-lived oscillations travelling away from the explosion like water rings. Here we show that the energy in the solar acoustic spectrum is correlated with flares. This means that the flares drive global oscillations in the Sun in the same way that the entire Earth is set ringing for several weeks after a major earthquake like the December 2004 Sumatra-Andaman Earthquake. The correlation between flares and energy in the acoustic spectrum of disk-integrated sunlight is stronger for high-frequency waves than for ordinary p-modes which are excited by the turbulence in the near surface convection zone immediately beneath the photosphere.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/65D3EBK7/Karoff, Kjeldsen - 2008.pdf}
}

@article{Karoff2009a,
  title = {Sounding Stellar Cycles with {{Kepler}} - {{I}}. {{Strategy}} for Selecting Targets},
  author = {Karoff, C. and Metcalfe, T. S. and Chaplin, W. J. and Elsworth, Y. and Kjeldsen, H. and Arentoft, T. and Buzasi, D.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {399},
  number = {2},
  pages = {914--923},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.15323.x},
  abstract = {The long-term monitoring and high photometric precision of the Kepler satellite will provide a unique opportunity to sound the stellar cycles of many solar-type stars using asteroseismology. This can be achieved by studying periodic changes in the amplitudes and frequencies of the oscillation modes observed in these stars. By comparing these measurements with conventional ground-based chromospheric activity indices, we can improve our understanding of the relationship between chromospheric changes and those taking place deep in the interior throughout the stellar activity cycle. In addition, asteroseismic measurements of the convection zone depth and differential rotation may help us determine whether stellar cycles are driven at the top or at the base of the convection zone. In this paper, we analyse the precision that will be possible using Kepler to measure stellar cycles, convection zone depths and differential rotation. Based on this analysis, we describe a strategy for selecting specific targets to be observed by the Kepler Asteroseismic Investigation for the full length of the mission, to optimize their suitability for probing stellar cycles in a wide variety of solar-type stars. \textcopyright{} 2009 RAS.},
  keywords = {notion,notion-database,Stars: activity,Stars: oscillations,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/CB8YRZ27/Karoff et al. - 2009.pdf}
}

@article{Karoff2010a,
  title = {Asteroseismology of Solar-Type Stars with {{Kepler I}}: {{Data}} Analysis},
  author = {Karoff, C. and Chaplin, W. J. and Appourchaux, T. and Elsworth, Y. and Garcia, R. A. and Houdek, G. and Metcalfe, T. S. and {Molenda-ZAkowicz}, J. and Monteiro, M. J.P.F.G. and Thompson, M. J. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kjeldsen, H. and Basu, S. and Bedding, T. R. and Campante, T. L. and Eggenberger, P. and Fletcher, S. T. and Gaulme, P. and Handberg, R. and Hekker, S. and Martic, M. and Mathur, S. and Mosser, B. and Regulo, C. and Roxburgh, I. W. and Salabert, D. and Stello, D. and Verner, G. A. and Belkacem, K. and Biazzo, K. and Cunha, M. S. and Gruberbauer, M. and Guzik, J. A. and Kupka, F. and Leroy, B. and Ludwig, H. G. and Mathis, S. and Noels, A. and Noyes, R. W. and Roca Cortes, T. and Roth, M. and Sato, K. H. and Schmitt, J. and Suran, M. D. and Trampedach, R. and Uytterhoeven, K. and Ventura, R. and Wilson, P. A.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  eprint = {1005.0507},
  pages = {972--976},
  issn = {00046337},
  doi = {10.1002/asna.201011438},
  abstract = {We report on the first asteroseismic analysis of solar-type stars observed by Kepler. Observations of three G-type stars, made at one-minute cadence during the first 33.5 days of science operations, reveal high signal-to-noise solar-like oscillation spectra in all three stars: About 20 modes of oscillation can clearly be distinguished in each star. We discuss the appearance of the oscillation spectra, including the presence of a possible signature of faculae, and the presence of mixed modes in one of the three stars (\textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim) Copyright \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: interiors,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/XPWZYU7H/Karoff et al. - 2010.pdf}
}

@article{Karoff2013,
  title = {Sounding Stellar Cycles with {{Kepler}} - {{II}}. Ground-Based Observations},
  author = {Karoff, C. and Metcalfe, T. S. and Chaplin, W. J. and Frandsen, S. and Grundahl, F. and Kjeldsen, H. and {Christensen-Dalsgaard}, J. and Nielsen, M. B. and Frimann, S. and Thygesen, A. O. and Arentoft, T. and Amby, T. M. and Sousa, S. G. and Buzasi, D. L.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {433},
  number = {4},
  pages = {3227--3238},
  issn = {13652966},
  doi = {10.1093/mnras/stt964},
  abstract = {We have monitored 20 Sun-like stars in the Kepler field-of-view for excess flux with the Fibrefed Echelle Spectrograph on the Nordic Optical Telescope since the launch ofKepler spacecraft in 2009. These 20 stars were selected based on their asteroseismic properties to sample the parameter space (effective temperature, surface gravity, activity level, etc.) around the Sun. Though the ultimate goal is to improve stellar dynamo models, we focus the present paper on the combination of space-based and ground-based observations that can be used to test the age- rotation-activity relations. In this paper we describe the considerations behind the selection of these 20 Sun-like stars and present an initial asteroseismic analysis, which includes stellar age estimates. We also describe the observations from the Nordic Optical Telescope and present mean values of measured excess fluxes. These measurements are combined with estimates of the rotation periods obtained from a simple analysis of the modulation in photometric observations from Kepler caused by starspots, and asteroseismic determinations of stellar ages, to test relations between age, rotation and activity. \textcopyright{} 2013 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {notion,notion-database,Stars: activity,Stars: oscillations,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/8MLN5DQH/Karoff et al. - 2013.pdf}
}

@article{Karoff2018,
  title = {The {{Influence}} of {{Metallicity}} on {{Stellar Differential Rotation}} and {{Magnetic Activity}}},
  author = {Karoff, Christoffer and Metcalfe, Travis S. and Santos, {\^A}ngela R. G. and Montet, Benjamin T. and Isaacson, Howard and Witzke, Veronika and Shapiro, Alexander I. and Mathur, Savita and Davies, Guy R. and Lund, Mikkel N. and Garcia, Rafael A. and Brun, Allan S. and Salabert, David and Avelino, Pedro P. and van Saders, Jennifer and Egeland, Ricky and Cunha, Margarida S. and Campante, Tiago L. and Chaplin, William J. and Krivova, Natalie and Solanki, Sami K. and Stritzinger, Maximilian and Knudsen, Mads F.},
  year = {2018},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {852},
  number = {1},
  eprint = {1711.07716},
  pages = {46},
  publisher = {{American Astronomical Society}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aaa026},
  abstract = {Observations of Sun-like stars over the last half-century have improved our understanding of how magnetic dynamos, like that responsible for the 11-year solar cycle, change with rotation, mass and age. Here we show for the first time how metallicity can affect a stellar dynamo. Using the most complete set of observations of a stellar cycle ever obtained for a Sun-like star, we show how the solar analog HD 173701 exhibits solar-like differential rotation and a 7.4-year activity cycle. While the duration of the cycle is comparable to that generated by the solar dynamo, the amplitude of the brightness variability is substantially stronger. The only significant difference between HD 173701 and the Sun is its metallicity, which is twice the solar value. Therefore, this provides a unique opportunity to study the effect of the higher metallicity on the dynamo acting in this star and to obtain a comprehensive understanding of the physical mechanisms responsible for the observed photometric variability. The observations can be explained by the higher metallicity of the star, which is predicted to foster a deeper outer convection zone and a higher facular contrast, resulting in stronger variability.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8BZNB7DD/Karoff_2018_ApJ_852_46.pdf}
}

@article{Kasting1993,
  title = {Habitable {{Zones}} around {{Main Sequence Stars}}},
  author = {Kasting, James F. and Whitmire, Daniel P. and Reynolds, Ray T.},
  year = {1993},
  month = jan,
  journal = {Icarus},
  volume = {101},
  number = {1},
  pages = {108--128},
  publisher = {{Academic Press}},
  issn = {10902643},
  doi = {10.1006/icar.1993.1010},
  urldate = {2020-03-07},
  abstract = {A one-dimensional climate model is used to estimate the width of the habitable zone (HZ) around our Sun and around other main sequence stars. Our basic premise is that we are dealing with Earth-like planets with CO2/H2O/N2 atmospheres and that habitability requires the presence of liquid water on the planet's surface. The inner edge of the HZ is determined in our model by loss of water via photolysis and hydrogen escape. The outer edge of the HZ is determined by the formation of CO2 clouds, which cool a planet's surface by increasing its albedo and by lowering the convective lapse rate. Conservative estimates for these distances in our own Solar System are 0.95 and 1.37 AU, respectively; the actual width of the present HZ could be much greater. Between these two limits, climate stability is ensured by a feedback mechanism in which atmospheric CO2 concentrations vary inversely with planetary surface temperature. The width of the HZ is slightly greater for planets that are larger than Earth and for planets which have higher N2 partial pressures. The HZ evolves outward in time because the Sun increases in luminosity as it ages. A conservative estimate for the width of the 4.6-Gyr continuously habitable zone (CHZ) is 0.95 to 1.15 AU. Stars later than F0 have main sequence lifetimes exceeding 2 Gyr and, so, are also potential candidates for harboring habitable planets. The HZ around an F star is larger and occurs farther out than for our Sun; the HZ around K and M stars is smaller and occurs farther in. Nevertheless, the widths of all of these HZs are approximately the same if distance is expressed on a logarithmic scale. A log distance scale is probably the appropriate scale for this problem because the planets in our own Solar System are spaced logarithmically and because the distance at which another star would be expected to form planets should be related to the star's mass. The width of the CHZ around other stars depends on the time that a planet is required to remain habitable and on whether a planet that is initially frozen can be thawed by modest increases in stellar luminosity. For a specified period of habitability, CHZs around K and M stars are wider (in log distance) than for our Sun because these stars evolve more slowly. Planets orbiting late K stars and M stars may not be habitable, however, because they can become trapped in synchronous rotation as a consequence of tidal damping. F stars have narrower (log distance) CHZ's than our Sun because they evolve more rapidly. Our results suggest that mid-to-early K stars should be considered along with G stars as optimal candidates in the search for extraterrestrial life. \textcopyright{} 1993 by Academic Press, Inc.},
  keywords = {notion,notion-database}
}

@article{Kaufman2022,
  title = {The Stability of {{Prendergast}} Magnetic Fields},
  author = {Kaufman, Emma and Lecoanet, Daniel and Anders, Evan H. and Brown, Benjamin P. and Vasil, Geoffrey M. and Oishi, Jeffrey S. and Burns, Keaton J.},
  year = {2022},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {517},
  pages = {3332--3340},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac2707},
  urldate = {2023-04-18},
  abstract = {Convection in massive main-sequence stars generates large-scale magnetic fields in their cores that persists as they evolve up the red giant branch. The remnants of these fields may take the form of the Prendergast magnetic field, a combination of poloidal and toroidal field components that are expected to stabilize each other. Previous analytic and numerical calculations did not find any evidence for instability of the Prendergast field over short time-scales. In this paper, we present numerical simulations which show a long time-scale, linear instability of this magnetic field. We find the instability to be robust to changes in boundary conditions and it is not stabilized by strong stable stratification. The instability is a resistive instability, and the growth rate has a power-law dependence on the resistivity, in which the growth rate decreases as the resistivity decreases. We estimate the growth rate of the instability in stars by extrapolating this power law to stellar values of the resistivity. The instability is sufficiently rapid to destabilize the magnetic field on time-scales shorter than the stellar evolution time-scale, indicating that the Prendergast field is not a good model to use in studies of magnetic fields in stars.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,instabilities,MHD,stars: magnetic field},
  annotation = {ADS Bibcode: 2022MNRAS.517.3332K},
  file = {/Users/lbugnet/Zotero/storage/7FVFHPXL/Kaufman et al. - 2022 - The stability of Prendergast magnetic fields.pdf}
}

@article{Kawaler1988,
  title = {Angular Momentum Loss in Low-Mass Stars},
  author = {Kawaler, Steven D.},
  year = {1988},
  journal = {The Astrophysical Journal},
  volume = {333},
  eprint = {1011.1669v3},
  pages = {236--247},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MHIDXB8Y/Kawaler - 1988.pdf}
}

@article{Kawaler1989,
  title = {Rotational Dating of Middle-Aged Stars},
  author = {Kawaler, Steven D.},
  year = {1989},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {343},
  pages = {L65},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/185512},
  urldate = {2020-10-19},
  abstract = {By the age of about 100 million years, the rotational velocity of solar mass stars becomes independent of the initial rotation rate on the main sequence, due to the strong dependence of the angular momentum loss rate on the rotation rate; once this common value is reached, the rotation velocity depends only on time and the mass of the star. Thus, the measured rotation rate of a low-mass star provides an estimate of its age when its mass is known. The observed rotation periods of low-mass stars in the Hyades are used to test this conclusion and to check the validity of the theoretical angular momentum loss rates. Adapting the magnetic braking model of Kawaler (1988), the angular momentum loss rate is integrated to derive a relation between rotation period and age, and this relation is converted to a period-age-color relation using simple stellar models. Using this method, a mean rotational age for the Hyades is obtained which is in close agreement with the age determined by isochrone fitting.},
  keywords = {Angular Momentum,Astrophysics,Calibrating,CLUSTERS: OPEN,Main Sequence Stars,notion,notion-database,Open Clusters,STARS: EVOLUTION,STARS: ROTATION,Stellar Evolution,Stellar Mass,Stellar Models,Stellar Rotation,Stellar Winds}
}

@article{Kawaler1999a,
  title = {Prospects for {{Measuring Differential Rotation}} in {{White Dwarfs}} through {{Asteroseismology}}},
  author = {Kawaler, Steven D. and Sekii, Takashi and Gough, Douglas},
  year = {1999},
  journal = {The Astrophysical Journal},
  volume = {516},
  number = {1},
  pages = {349--365},
  issn = {0004-637X},
  doi = {10.1086/307087},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MLEQ22GY/Kawaler, Sekii, Gough - 1999.pdf}
}

@article{Kawka2004,
  title = {Observations of {{White Dwarfs}} in the {{Solar Neighborhood}}},
  author = {Kawka, Adela and Vennes, Stphane and Thorstensen, John R.},
  year = {2004},
  month = mar,
  journal = {The Astronomical Journal},
  volume = {127},
  number = {3},
  pages = {1702--1711},
  publisher = {{IOP Publishing}},
  issn = {0004-6256},
  doi = {10.1086/382110},
  urldate = {2020-03-09},
  abstract = {High proper motion surveys are still adding much to our understanding of the local white dwarf population and, possibly, to the Galactic halo membership of some objects. As part of our study of white dwarfs in the solar neighborhood we have observed seven white dwarfs from the revised New Luyten Two Tenths (NLTT) catalog of Salim \& Gould. We found four DA white dwarfs (NLTT 529, 49985, 53468, 55932), one DZ white dwarf (NLTT 40607) that shows a close resemblance to the unusual DZ white dwarf G165-7, and two DC white dwarfs (NLTT 19138, NLTT 52404). The white dwarf candidates were chosen using the V-J reduced proper-motion diagram of Salim \& Gould and an optical-infrared diagram (V-J vs. J-H). We also observed five stars from the list of local white dwarfs by Holberg, Oswalt, \& Sion, that required confirmation of their spectral classification. We confirm that GD 1212 and WD 1717-345 are white dwarfs but that BPM 17113 (WD 0311-543), KUV 05097+1649, and BPM 19929 (WD 1013-559) are main-sequence F stars rather than white dwarfs. An analysis of a color-selected sample of white dwarf candidates extracted from the rNLTT catalog could contribute more than 200 new white dwarfs, most belonging to the thin disk, with a few (N{$<$}15) kinematically selected members of an older population (thick disk or halo).},
  keywords = {Galaxy: Disk,Galaxy: Solar Neighborhood,notion,notion-database,Stars: White Dwarfs},
  file = {/Users/lbugnet/Zotero/storage/MDCBHKZ9/full-text.pdf}
}

@article{Keen2015,
  title = {{{KIC}} 10080943: A Binary Star with Two {$\gamma$} {{Doradus}}/{$\delta$} {{Scuti}} Hybrid Pulsators. {{Analysis}} of the g Modes},
  author = {Keen, M A and Bedding, T R and Murphy, S J and Schmid, V S and Aerts, C and Tkachenko, A and Ouazzani, R.-M and Kurtz, D W},
  year = {2015},
  journal = {MNRAS},
  volume = {454},
  pages = {1792--1797},
  doi = {10.1093/mnras/stv2107},
  urldate = {2020-03-24},
  abstract = {We use 4 yr of Kepler photometry to study the non-eclipsing spectroscopic binary KIC 10080943. We find both components to be {$\gamma$} Doradus/{$\delta$} Scuti hybrids, which pulsate in both p and g modes. We present an analysis of the g modes, which is complicated by the fact that the two sets of = 1 modes partially overlap in the frequency spectrum. Nevertheless, it is possible to disentangle them by identifying rotationally split doublets from one component and triplets from the other. The identification is helped by the presence of additive combination frequencies in the spectrum that involve the doublets but not the triplets. The rotational splittings of the multiplets imply core rotation periods of about 11 and 7 d in the two stars. One of the stars also shows evidence of = 2 modes.},
  keywords = {asteroseismology-binaries,general,individual,KIC 10080943-stars,notion,notion-database,oscillations-stars,spectroscopic-stars,variables,{$\delta$} Scuti-stars},
  file = {/Users/lbugnet/Zotero/storage/UEDQYPWE/full-text.pdf}
}

@article{Keenan1938,
  title = {Dimensions of the {{Solar Granules}}.},
  author = {Keenan, Philip C.},
  year = {1938},
  month = oct,
  journal = {The Astrophysical Journal},
  volume = {88},
  pages = {360},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/143991},
  urldate = {2020-03-13},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/D4R2DI9C/full-text.pdf}
}

@article{Kepler1995,
  title = {Structure and {{Evolution}} of {{White}} Dwarfs},
  author = {Kepler, S.O. and Bradley, P.A.},
  year = {1995},
  journal = {Baltic Astronomy},
  volume = {4},
  pages = {166--220},
  urldate = {2020-11-10},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/C7QXYDL7/m-api-1831cd0e-3a0f-ea0f-599f-272ce2c6faae.pdf}
}

@article{Kepler2017,
  title = {White {{Dwarf Mass Distribution}}},
  author = {Kepler, S. O. and Koester, D. and Romero, A. D. and Ourique, G. and Pelisoli, I.},
  year = {2017},
  month = mar,
  volume = {509},
  pages = {421},
  address = {{eprint: arXiv:1610.00371}},
  doi = {10.48550/arXiv.1610.00371},
  urldate = {2023-10-09},
  abstract = {We present the mass distribution for all S/N {$\geq$} 15 DA white dwarfs detected in the Sloan Digital Sky Survey up to Data Release 12 in 2015, fitted with Koester models for ML2/{$\alpha$}=0.8 (Teff{$\geq$} 10000 K), and for DBs with S/N {$\geq$} 10, fitted with ML2/{$\alpha$}=1.25, for Teff {$>$}16 000 K. These mass distributions are for logg{$\geq$}6.5 stars, i.e., excluding the Extremely Low Mass white dwarfs. We also present the mass distributions corrected by volume with the 1/Vmax approach, for stars brighter than g=19. Both distributions have a maximum at M=0.624 M {$\odot$} but very distinct shapes.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2017ASPC..509..421K},
  file = {/Users/lbugnet/Zotero/storage/7US643XV/Kepler et al. - 2017 - White Dwarf Mass Distribution.pdf}
}

@article{Kepler2019,
  title = {White Dwarf and Subdwarf Stars in the {{Sloan Digital Sky Survey Data Release}} 14},
  author = {Kepler, S. O. and Pelisoli, Ingrid and Koester, Detlev and Reindl, Nicole and Geier, Stephan and Romero, Alejandra D. and Ourique, Gustavo and Oliveira, Cristiane de Paula and Amaral, Larissa A.},
  year = {2019},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {486},
  pages = {2169--2183},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz960},
  urldate = {2023-10-09},
  abstract = {White dwarfs carry information on the structure and evolution of the Galaxy, especially through their luminosity function and initial-to-final mass relation. Very cool white dwarfs provide insight into the early ages of each population. Examining the spectra of all stars with 3{$\sigma$} proper motion in the Sloan Digital Sky Survey Data Release 14, we report the classification for 20 088 spectroscopically confirmed white dwarfs, plus 415 hot subdwarfs, and 311 cataclysmic variables. We obtain Teff, log g, and mass for hydrogen atmosphere white dwarf stars (DAs), warm helium atmosphere white dwarfs (DBs), hot subdwarfs (sdBs and sdOs), and estimate photometric Teff for white dwarf stars with continuum spectra (DCs). We find 15 793 sdAs and 447 dCs between the white dwarf cooling sequence and the main sequence, especially below T\_eff{$\sim$}eq 10 000 K; most are likely low-mass metal-poor main-sequence stars, but some could be the result of interacting binary evolution.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,cataclysmic variables,catalogues,stars: fundamental parameters,subdwarfs,white dwarfs},
  annotation = {ADS Bibcode: 2019MNRAS.486.2169K},
  file = {/Users/lbugnet/Zotero/storage/VLQANEJX/Kepler et al. - 2019 - White dwarf and subdwarf stars in the Sloan Digita.pdf}
}

@article{Keszthelyi2021,
  title = {The Effects of Surface Fossil Magnetic Fields on Massive Star Evolution \textendash{} {{III}}. {{The}} Case of {$\tau$} {{Sco}}},
  author = {Keszthelyi, Z and Meynet, G and Martins, F and {de~Koter}, A and {David-Uraz}, A},
  year = {2021},
  month = apr,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {504},
  number = {2},
  pages = {2474--2492},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/stab893},
  urldate = {2023-10-11},
  abstract = {ABSTRACT             {$\tau$} Sco, a well-studied magnetic B-type star in the Upper Sco association, has a number of surprising characteristics. It rotates very slowly and shows nitrogen excess. Its surface magnetic field is much more complex than a purely dipolar configuration which is unusual for a magnetic massive star. We employ the cmfgen radiative transfer code to determine the fundamental parameters and surface CNO and helium abundances. Then, we employ mesa and genec stellar evolution models accounting for the effects of surface magnetic fields. To reconcile {$\tau~$}Sco's properties with single-star models, an increase is necessary in the efficiency of rotational mixing by a factor of 3\textendash 10 and in the efficiency of magnetic braking by a factor of 10. The spin-down could be explained by assuming a magnetic field decay scenario. However, the simultaneous chemical enrichment challenges the single-star scenario. Previous works indeed suggested a stellar merger origin for {$\tau~$}Sco. However, the merger scenario also faces similar challenges as our magnetic single-star models to explain {$\tau~$}Sco's simultaneous slow rotation and nitrogen excess. In conclusion, the single-star channel seems less likely and versatile to explain these discrepancies, while the merger scenario and other potential binary-evolution channels still require further assessment as to whether they may self-consistently explain the observables of {$\tau~$}Sco.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/QCJE7BD3/Keszthelyi et al. - 2021 - The effects of surface fossil magnetic fields on m.pdf}
}

@article{Keszthelyi2022,
  title = {The Effects of Surface Fossil Magnetic Fields on Massive Star Evolution: {{IV}}. {{Grids}} of Models at {{Solar}}, {{LMC}}, and {{SMC}} Metallicities},
  shorttitle = {The Effects of Surface Fossil Magnetic Fields on Massive Star Evolution},
  author = {Keszthelyi, Z. and {de Koter}, A. and G{\"o}tberg, Y. and Meynet, G. and Brands, S. A. and Petit, V. and Carrington, M. and {David-Uraz}, A. and Geen, S. T. and Georgy, C. and Hirschi, R. and Puls, J. and Ramalatswa, K. J. and Shultz, M. E. and {ud-Doula}, A.},
  year = {2022},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {517},
  pages = {2028--2055},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac2598},
  urldate = {2023-09-22},
  abstract = {Magnetic fields can drastically change predictions of evolutionary models of massive stars via mass-loss quenching, magnetic braking, and efficient angular momentum transport, which we aim to quantify in this work. We use the MESA software instrument to compute an extensive main-sequence grid of stellar structure and evolution models, as well as isochrones, accounting for the effects attributed to a surface fossil magnetic field. The grid is densely populated in initial mass (3-60 M{$\odot$}), surface equatorial magnetic field strength (0-50 kG), and metallicity (representative of the Solar neighbourhood and the Magellanic Clouds). We use two magnetic braking and two chemical mixing schemes and compare the model predictions for slowly rotating, nitrogen-enriched ('Group 2') stars with observations in the Large Magellanic Cloud. We quantify a range of initial field strengths that allow for producing Group 2 stars and find that typical values (up to a few kG) lead to solutions. Between the subgrids, we find notable departures in surface abundances and evolutionary paths. In our magnetic models, chemical mixing is always less efficient compared to non-magnetic models due to the rapid spin-down. We identify that quasi-chemically homogeneous main sequence evolution by efficient mixing could be prevented by fossil magnetic fields. We recommend comparing this grid of evolutionary models with spectropolarimetric and spectroscopic observations with the goals of (i) revisiting the derived stellar parameters of known magnetic stars, and (ii) observationally constraining the uncertain magnetic braking and chemical mixing schemes.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,stars: abundances,stars: evolution,stars: magnetic field,stars: massive,stars: rotation},
  annotation = {ADS Bibcode: 2022MNRAS.517.2028K},
  file = {/Users/lbugnet/Zotero/storage/V87PDMAY/Keszthelyi et al. - 2022 - The effects of surface fossil magnetic fields on m.pdf}
}

@article{Keszthelyi2022a,
  title = {The Effects of Surface Fossil Magnetic Fields on Massive Star Evolution: {{IV}}. {{Grids}} of Models at {{Solar}}, {{LMC}}, and {{SMC}} Metallicities},
  shorttitle = {The Effects of Surface Fossil Magnetic Fields on Massive Star Evolution},
  author = {Keszthelyi, Z and {de~Koter}, A and G{\"o}tberg, Y and Meynet, G and Brands, S A and Petit, V and Carrington, M and {David-Uraz}, A and Geen, S T and Georgy, C and Hirschi, R and Puls, J and Ramalatswa, K J and Shultz, M E and {ud-Doula}, A},
  year = {2022},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {517},
  number = {2},
  pages = {2028--2055},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/stac2598},
  urldate = {2023-10-25},
  abstract = {ABSTRACT             Magnetic fields can drastically change predictions of evolutionary models of massive stars via mass-loss quenching, magnetic braking, and efficient angular momentum transport, which we aim to quantify in this work. We use the mesa software instrument to compute an extensive main-sequence grid of stellar structure and evolution models, as well as isochrones, accounting for the effects attributed to a surface fossil magnetic field. The grid is densely populated in initial mass (3\textendash 60~M{$\odot$}), surface equatorial magnetic field strength (0\textendash 50~kG), and metallicity (representative of the Solar neighbourhood and the Magellanic Clouds). We use two magnetic braking and two chemical mixing schemes and compare the model predictions for slowly rotating, nitrogen-enriched (`Group~2') stars with observations in the Large Magellanic Cloud. We quantify a range of initial field strengths that allow for producing Group~2 stars and find that typical values (up to a few kG) lead to solutions. Between the subgrids, we find notable departures in surface abundances and evolutionary paths. In our magnetic models, chemical mixing is always less efficient compared to non-magnetic models due to the rapid spin-down. We identify that quasi-chemically homogeneous main sequence evolution by efficient mixing could be prevented by fossil magnetic fields. We recommend comparing this grid of evolutionary models with spectropolarimetric and spectroscopic observations with the goals of (i) revisiting the derived stellar parameters of known magnetic stars, and (ii) observationally constraining the uncertain magnetic braking and chemical mixing schemes.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/GNRSLX4D/Keszthelyi et al. - 2022 - The effects of surface fossil magnetic fields on m.pdf}
}

@article{Kgoadi2019,
  title = {General Classification of Light Curves Using Extreme Boosting},
  author = {Kgoadi, Refilwe and Engelbrecht, Chris and Whittingham, Ian and Tkachenko, Andrew},
  year = {2019},
  volume = {14},
  number = {June},
  eprint = {1906.06628},
  pages = {1--14},
  abstract = {A significant degree of misclassification of variable stars through the application of machine learning methods to survey data motivates a search for more reliable and accurate machine learning procedures, especially in light of the very large data cubes that will be generated by future surveys and the need for immediate production of accurate, formalised catalogues of variable behaviour to enable science to proceed. In this study, the efficiency of an ensemble machine learning procedure utilising extreme boosting was determined by application to a large sample of data from the OGLE III and IV surveys and from the \textbackslash textit\{Kepler\} mission. Through recursive training of classifiers, the study developed a variable star classification workflow which produced an average efficiency determined with the average precision of the model (0.81 for \textbackslash textit\{Kepler\} and 0.91 for OGLE) and the \$f-score\$ of predictions on the test sets. This suggests that extreme boosting can be presented as one of the favourable shallow learning methods in developing a variable star classifier for future large survey projects.},
  archiveprefix = {arxiv},
  keywords = {astro-,data analysis,methods,miscellaneous,nomical data bases,notion,notion-database,stars,statistical,variables},
  file = {/Users/lbugnet/Zotero/storage/GQWN4XQU/Kgoadi et al. - 2019.pdf}
}

@article{Khan2019,
  title = {New Light on the {{Gaia DR2}} Parallax Zero-Point: {{Influence}} of the Asteroseismic Approach, in and beyond the {{Kepler}} Field},
  author = {Khan, S. and Miglio, A. and Mosser, B. and Arenou, F. and Belkacem, K. and Brown, A. G.A. and Katz, D. and Casagrande, L. and Chaplin, W. J. and Davies, G. R. and Rendle, B. M. and Rodrigues, T. S. and Bossini, D. and {Cantat-Gaudin}, T. and Elsworth, Y. P. and Girardi, L. and North, T. S.H. and Vallenari, A.},
  year = {2019},
  journal = {Astronomy and Astrophysics},
  volume = {628},
  eprint = {1904.05676},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201935304},
  abstract = {The importance of studying the Gaia DR2 parallax zero-point by external means was underlined by the articles that accompanied the release, and initiated by several works making use of Cepheids, eclipsing binaries, and asteroseismology. Despite a very efficient elimination of basic-angle variations, a small fluctuation remains and shows up as a small offset in the Gaia DR2 parallaxes. By combining astrometric, asteroseismic, spectroscopic, and photometric constraints, we undertake a new analysis of the Gaia parallax offset for nearly 3000 red-giant branch (RGB) and 2200 red clump (RC) stars observed by Kepler, as well as about 500 and 700 red giants (all either in the RGB or RC phase) selected by the K2 Galactic Archaeology Program in campaigns 3 and 6. Engaging in a thorough comparison of the astrometric and asteroseismic parallaxes, we are able to highlight the influence of the asteroseismic method, and measure parallax offsets in the Kepler field that are compatible with independent estimates from literature and open clusters. Moreover, adding the K2 fields to our investigation allows us to retrieve a clear illustration of the positional dependence of the zero-point, in general agreement with the information provided by quasars. Lastly, we initiate a two-step methodology to make progress in the simultaneous calibration of the asteroseismic scaling relations and of the Gaia DR2 parallax offset, which will greatly benefit from the gain in precision with the third data release of Gaia.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Astrometry,notion,notion-database,Parallaxes,Stars: Low-mass},
  file = {/Users/lbugnet/Zotero/storage/378K2N4C/Khan et al. - 2019.pdf}
}

@article{Kholikov2008,
  title = {Acoustic Radius Measurements from {{MDI}} and {{GONG}}},
  author = {Kholikov, S. and Hill, F.},
  year = {2008},
  journal = {Solar Physics},
  volume = {251},
  number = {1-2},
  pages = {157--161},
  issn = {00380938},
  doi = {10.1007/s11207-008-9205-9},
  abstract = {We study the temporal autocorrelation function (ACF) of global solar oscillations. It is well known that the "large frequency separation" is proportional to the solar acoustic radius. We analyze the ACF of MDI and GONG spherical-harmonic-coefficient time series for degrees {$\mathscr{l}$}=0-3. Acoustic radius measurements obtained from the first dominant peak locations of the ACF show a significant anticorrelation with solar cycle. This technique can be a useful tool to search for stellar activity. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  isbn = {1120700892},
  keywords = {notion,notion-database,Oscillations,Solar radius,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/EDB86AT6/Kholikov, Hill - 2008.pdf}
}

@article{Kiefer2017,
  title = {Stellar Magnetic Activity and Variability of Oscillation Parameters: {{An}} Investigation of 24 Solar-like Stars Observed by {{Kepler}}},
  author = {Kiefer, Ren{\'e} and Schad, Ariane and Davies, Guy and Roth, Markus},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {598},
  pages = {1--26},
  issn = {14320746},
  doi = {10.1051/0004-6361/201628469},
  abstract = {Context. The Sun and solar-like stars undergo activity cycles for which the underlying mechanisms are not well understood. The oscillations of the Sun are known to vary with its activity cycle and these changes provide diagnostics on the conditions below the photosphere. Kepler has detected solar-like oscillations in hundreds of stars but as of yet, no widespread detection of signatures of magnetic activity cycles in the oscillation parameters of these stars have been reported. Aims. We analysed the photometric short cadence Kepler time series of a set of 24 solar-like stars, which were observed for at least 960 d each, with the aim to find signatures of stellar magnetic activity in the oscillation parameters. Methods. We analyse the temporal evolution of oscillation parameters by measuring mode frequency shifts, changes in the height of the p-mode envelope, as well as granulation timescales. Results. For 23 of the 24 investigated stars, we find significant frequency shifts in time. We present evidence for magnetic activity in six of these stars. We find that the amplitude of the frequency shifts decreases with stellar age and rotation period. For KIC 8006161 (the most prominent example), we find that frequency shifts are smallest for the lowest and largest for the highest p-mode frequencies, as they are for the Sun. Conclusions. These findings show that magnetic activity can be routinely observed in the oscillation parameters for solar-like stars, which opens up the possibility of placing the solar activity cycle in the context of other stars by asteroseismology.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: activity,Stars: magnetic field,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/8BEMFPCV/Kiefer et al. - 2017.pdf}
}

@article{Kiefer2017a,
  title = {The {{Direct Effect}} of {{Toroidal Magnetic Fields}} on {{Stellar Oscillations}}: {{An Analytical Expression}} for the {{General Matrix Element}}},
  author = {Kiefer, Ren{\'e} and Schad, Ariane and Roth, Markus},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {846},
  number = {2},
  eprint = {1709.02454},
  pages = {162},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aa8634},
  abstract = {Where is the solar dynamo located and what is its modus operandi? These are still open questions in solar physics. Helio- and asteroseismology can help answer them by enabling us to study solar and stellar internal structures through global oscillations. The properties of solar and stellar acoustic modes are changing with the level of magnetic activity. However, until now, the inference on subsurface magnetic fields with seismic measures has been very limited. The aim of this paper is to develop a formalism to calculate the effect of large-scale toroidal magnetic fields on solar and stellar global oscillation eigenfunctions and eigenfrequencies. If the Lorentz force is added to the equilibrium equation of motion, stellar eigenmodes can couple. In quasi-degenerate perturbation theory, this coupling, also known as the direct effect, can be quantified by the general matrix element. We present the analytical expression of the matrix element for a superposition of subsurface zonal toroidal magnetic field configurations. The matrix element is important for forward calculations of perturbed solar and stellar eigenfunctions and frequency perturbations. The results presented here will help to ascertain solar and stellar large-scale subsurface magnetic fields, and their geometric configuration, strength, and their change over the course of activity cycles.},
  archiveprefix = {arxiv},
  keywords = {analytical,asteroseismology,{asteroseismology,dynamo,magnetic fields,methods: a},dynamo,interiors,magnetic fi elds,methods,notion,notion-database,stars,sun},
  file = {/Users/lbugnet/Zotero/storage/SXW9L7I4/Kiefer, Schad, Roth - 2017(2).pdf}
}

@article{Kiefer2018,
  title = {The {{Effect}} of {{Toroidal Magnetic Fields}} on {{Solar Oscillation Frequencies}}},
  author = {Kiefer, Ren{\'e} and Roth, Markus},
  year = {2018},
  journal = {The Astrophysical Journal},
  volume = {854},
  number = {1},
  eprint = {1801.07932},
  pages = {74},
  publisher = {{IOP Publishing}},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aaa3f7},
  abstract = {Solar oscillation frequencies change with the level of magnetic activity. Localizing subsurface magnetic field concentrations in the Sun with helioseismology will help us to understand the solar dynamo. Because the magnetic fields are not considered in standard solar models, adding them to the basic equations of stellar structure changes the eigenfunctions and eigenfrequencies. We use quasi-degenerate perturbation theory to calculate the effect of toroidal magnetic fields on solar oscillation mean multiplet frequencies for six field configurations. In our calculations, we consider both the direct effect of the magnetic field, which describes the coupling of modes, and the indirect effect, which accounts for changes in stellar structure due to the magnetic field. We limit our calculations to self-coupling of modes. We find that the magnetic field affects the multiplet frequencies in a way that depends on the location and the geometry of the field inside the Sun. Comparing our theoretical results with observed shifts, we find that strong tachocline fields cannot be responsible for the observed frequency shifts of p modes over the solar cycle. We also find that part of the surface effect in helioseismic oscillation frequencies might be attributed to magnetic fields in the outer layers of the Sun. The theory presented here is also applicable to models of solar-like stars and their oscillation frequencies.},
  archiveprefix = {arxiv},
  keywords = {analytical,asteroseismology,{asteroseismology,dynamo,methods: analytical,method},dynamo,helioseismology,methods,notion,notion-database,numerical,sun},
  file = {/Users/lbugnet/Zotero/storage/YLFCG7SH/Kiefer, Roth - 2018.pdf}
}

@article{Kilic2018,
  title = {Gaia Reveals Evidence for Merged White Dwarfs},
  author = {Kilic, Mukremin and Hambly, N. C. and Bergeron, P. and {Genest-Beaulieu}, C. and Rowell, N.},
  year = {2018},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {479},
  pages = {L113-L117},
  issn = {0035-8711},
  doi = {10.1093/mnrasl/sly110},
  urldate = {2023-10-09},
  abstract = {We use Gaia Data Release 2 to identify 13 928 white dwarfs (WDs) within 100 pc of the Sun. The exquisite astrometry from Gaia reveals for the first time a bifurcation in the observed WD sequence in both Gaia and the Sloan Digital Sky Survey (SDSS) passbands. The latter is easily explained by a helium atmosphere WD fraction of 36 per cent. However, the bifurcation in the Gaia colour-magnitude diagram depends on both the atmospheric composition and the mass distribution. We simulate theoretical colour-magnitude diagrams for single and binary WDs using a population synthesis approach and demonstrate that there is a significant contribution from relatively massive WDs that likely formed through mergers. These include WD remnants of main-sequence (blue stragglers) and post-main-sequence mergers. The mass distribution of the SDSS subsample, including the spectroscopically confirmed WDs, also shows this massive bump. This is the first direct detection of such a population in a volume-limited sample.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,Galaxy: disc,Galaxy: stellar content,Hertzsprung-Russell and colour-magnitude diagrams,stars: evolution,stars: fundamental parameters,white dwarfs},
  annotation = {ADS Bibcode: 2018MNRAS.479L.113K},
  file = {/Users/lbugnet/Zotero/storage/P5RA5QD3/Kilic et al. - 2018 - Gaia reveals evidence for merged white dwarfs.pdf}
}

@article{Kilkenny1997,
  title = {A New Class of Rapidly Pulsating Star - {{I}}. {{EC}} 14026-2647, the Class Prototype},
  author = {Kilkenny, D. and Koen, C. and O'Donoghue, D. and Stobie, R. S.},
  year = {1997},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {285},
  pages = {640--644},
  issn = {0035-8711},
  doi = {10.1093/mnras/285.3.640},
  urldate = {2023-10-09},
  abstract = {We report the discovery of small-amplitude, very rapid light variations in the sdB binary, EC 14026-2647. The variations, probably due to pulsation of the sdB star, have an apparently stable main period near 144s with a semi- amplitude of \textasciitilde 0.012 mag. There is good evidence for a period near 134s with a semi-amplitude of \textasciitilde 0.004 mag; the latter might be variable. We regard this star as the prototype for a new class of variable which we refer to as EC 14026 stars.},
  keywords = {BINARIES: GENERAL,STARS: INDIVIDUAL: EC 14026-2647,STARS: OSCILLATIONS,STARS: VARIABLES: OTHER},
  annotation = {ADS Bibcode: 1997MNRAS.285..640K},
  file = {/Users/lbugnet/Zotero/storage/RYWMRQ3E/Kilkenny et al. - 1997 - A new class of rapidly pulsating star - I. EC 1402.pdf}
}

@article{Kim1996,
  title = {The Teoretical {{Calculation}} of the Rossby Number and the "Nonlocal" Convective Overturn Time for Pre-Main-Sequence and Early Post-Main Sequence Stars},
  author = {Kim, Yong Cheol and Demarque, Pierre},
  year = {1996},
  journal = {The Astrophysical Journal},
  volume = {457},
  pages = {340--347},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NL39FEVX/Kim, Demarque - 1996.pdf}
}

@article{Kippenhahn1963,
  title = {Differential {{Rotation}} in {{Stars}} with {{Convective Envelopes}}.},
  author = {Kippenhahn, Rudolf},
  year = {1963},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {137},
  pages = {664},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/147539},
  urldate = {2020-03-09},
  abstract = {Abstract image available at: http://adsabs.harvard.edu/abs/1963ApJ...137..664K},
  keywords = {notion,notion-database}
}

@book{Kippenhahn1990,
  title = {Stellar {{Structure}} and {{Evolution}}},
  author = {Kippenhahn, R. and Weigert, A.},
  year = {1990},
  urldate = {2020-06-22},
  keywords = {notion,notion-database}
}

@book{Kippenhahn2012,
  title = {Stellar {{Structure}} and {{Evolution}}},
  author = {Kippenhahn, Rudolf and Weigert, Alfred and Weiss, Achim},
  year = {2012},
  journal = {sse},
  publisher = {{Springer Berlin Heidelberg}},
  address = {{Berlin, Heidelberg}},
  doi = {10.1007/978-3-642-30304-3},
  urldate = {2020-07-12},
  isbn = {978-3-642-30255-8},
  keywords = {notion,notion-database,Physics}
}

@article{Kirk2016,
  title = {Kepler {{Eclipsing Binary Stars}}. {{Vii}}. the {{Catalog}} of {{Eclipsing Binaries Found}} in the {{Entire Kepler Data Set}}},
  author = {Kirk, Brian and Conroy, Kyle and Pr{\v s}a, Andrej and {Abdul-Masih}, Michael and Kochoska, Angela and Matijevi{\v c}, Gal and Hambleton, Kelly and Barclay, Thomas and Bloemen, Steven and Boyajian, Tabetha and Doyle, Laurance R. and Fulton, B. J. and Hoekstra, Abe Johannes and Jek, Kian and Kane, Stephen R. and Kostov, Veselin and Latham, David and Mazeh, Tsevi and Orosz, Jerome A. and Pepper, Joshua and Quarles, Billy and Ragozzine, Darin and Shporer, Avi and Southworth, John and Stassun, Keivan and Thompson, Susan E. and Welsh, William F. and Agol, Eric and Derekas, Aliz and Devor, Jonathan and Fischer, Debra and Green, Gregory and Gropp, Jeff and Jacobs, Tom and Johnston, Cole and LaCourse, Daryll Matthew and Saetre, Kristian and Schwengeler, Hans and Toczyski, Jacek and Werner, Griffin and Garrett, Matthew and Gore, Joanna and Martinez, Arturo O. and Spitzer, Isaac and Stevick, Justin and Thomadis, Pantelis C. and Vrijmoet, Eliot Halley and Yenawine, Mitchell and Batalha, Natalie and Borucki, William},
  year = {2016},
  journal = {The Astronomical Journal},
  volume = {151},
  number = {3},
  pages = {68},
  issn = {0004-6256},
  doi = {10.3847/0004-6256/151/3/68},
  abstract = {\textcopyright{} 2016. The American Astronomical Society. All rights reserved..The primary Kepler Mission provided nearly continuous monitoring of {$\sim$}200,000 objects with unprecedented photometric precision. We present the final catalog of eclipsing binary systems within the 105 deg2 Kepler field of view. This release incorporates the full extent of the data from the primary mission (Q0-Q17 Data Release). As a result, new systems have been added, additional false positives have been removed, ephemerides and principal parameters have been recomputed, classifications have been revised to rely on analytical models, and eclipse timing variations have been computed for each system. We identify several classes of systems including those that exhibit tertiary eclipse events, systems that show clear evidence of additional bodies, heartbeat systems, systems with changing eclipse depths, and systems exhibiting only one eclipse event over the duration of the mission. We have updated the period and galactic latitude distribution diagrams and included a catalog completeness evaluation. The total number of identified eclipsing and ellipsoidal binary systems in the Kepler field of view has increased to 2878, 1.3\% of all observed Kepler targets. An online version of this catalog with downloadable content and visualization tools is maintained at http://keplerEBs.villanova.edu.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HS8W4HKJ/Kirk et al. - 2016.pdf}
}

@article{Kissin2015,
  title = {{{ROTATION OF GIANT STARS}}},
  author = {Kissin, Yevgeni and Thompson, Christopher},
  year = {2015},
  journal = {The Astrophysical Journal},
  volume = {808},
  eprint = {1501.07217v3},
  urldate = {2020-07-05},
  abstract = {The internal rotation of post-main sequence stars is investigated, in response to the convective pumping of angular momentum toward the stellar core, combined with a tight magnetic coupling between core and envelope. The spin evolution is calculated using model stars of initial mass 1, 1.5 and 5 M {$\odot$} , taking into account mass loss on the giant branches. We also include the deposition of orbital angular momentum from a sub-stellar companion, as influenced by tidal drag along with the excitation of orbital eccentricity by a fluctuating gravitational quadrupole moment. A range of angular velocity profiles {$\Omega$}(r) is considered in the envelope, extending from solid rotation to constant specific angular momentum. We focus on the backreaction of the Coriolis force, and the threshold for dynamo action in the inner envelope. Quantitative agreement with measurements of core rotation in subgiants and post-He core flash stars by Kepler is obtained with a two-layer angular velocity profile: uniform specific angular momentum where the Coriolis parameter Co {$\equiv$} {$\Omega\tau$} con 1 (here {$\tau$} con is the convective time); and {$\Omega$}(r) {$\propto$} r -1 where Co 1. The inner profile is interpreted in terms of a balance between the Coriolis force and angular pressure gradients driven by radially extended convective plumes. Inward angular momentum pumping reduces the surface rotation of subgiants, and the need for a rejuvenated magnetic wind torque. The co-evolution of internal magnetic fields and rotation is considered in Kissin \& Thompson, along with the breaking of the rotational coupling between core and envelope due to heavy mass loss.},
  archiveprefix = {arxiv},
  keywords = {giants-stars,notion,notion-database,rotation-magnetic fields,stars,Subject headings,white dwarfs-stars},
  file = {/Users/lbugnet/Zotero/storage/IDTKXNVI/full-text.pdf}
}

@article{Kissin2015a,
  title = {Spin and {{Magnetism}} of {{White Dwarfs}}},
  author = {Kissin, Yevgeni and Thompson, Christopher},
  year = {2015},
  month = jan,
  journal = {ApJ},
  volume = {809},
  number = {2},
  eprint = {1501.07197},
  pages = {108},
  doi = {10.1088/0004-637X/809/2/108},
  urldate = {2020-07-05},
  abstract = {The magnetism and rotation of white dwarf (WD) stars are investigated in relation to a hydromagnetic dynamo operating in the progenitor during shell burning phases. The downward pumping of angular momentum in the convective envelope, in combination with the absorption of a planet or tidal spin-up from a binary companion, can trigger strong dynamo action near the core-envelope boundary. Several arguments point to the outer core as the source for a magnetic field in the WD remnant: the outer third of a \$\textbackslash sim 0.55\textbackslash,M\_\textbackslash odot\$ WD is processed during the shell burning phase(s) of the progenitor; the escape of magnetic helicity through the envelope mediates the growth of (compensating) helicity in the core, as is needed to maintain a stable magnetic field in the remnant; and the intense radiation flux at the core boundary facilitates magnetic buoyancy within a relatively thick tachocline layer. The helicity flux into the growing core is driven by a dynamical imbalance with a latitude-dependent rotational stress. The magnetic field deposited in an isolated massive WD is concentrated in an outer shell of mass \$\textbackslash lesssim 0.1\textbackslash,M\_\textbackslash odot\$ and can reach \$\textbackslash sim 10\textbackslash,\$MG. A buried toroidal field experiences moderate ohmic decay above an age \$\textbackslash sim 0.3\$ Gyr, which may lead to growth or decay of the external magnetic field. The final WD spin period is related to a critical spin rate below which magnetic activity shuts off, and core and envelope decouple; it generally sits in the range of hours to days. WD periods ranging up to a year are possible if the envelope re-expands following a late thermal pulse.},
  archiveprefix = {arxiv},
  keywords = {magnetic fields,notion,notion-database,planet\textendash star interactions,stars: AGB and post-AGB,stars: rotation,white dwarfs},
  file = {/Users/lbugnet/Zotero/storage/6RA8TYJ5/full-text.pdf}
}

@article{Kitchatinov2006,
  title = {Differential Rotation of a Star Induced by Meridional Circulation},
  author = {Kitchatinov, L. L.},
  year = {2006},
  month = jun,
  journal = {Astronomy Reports},
  volume = {50},
  number = {6},
  pages = {512--516},
  issn = {10637729},
  doi = {10.1134/S1063772906060102},
  urldate = {2020-03-09},
  abstract = {Global meridional flows in stars transport angular momentum, thus giving rise to nonuniform rotation. The pattern of differential rotation associated with slow meridional circulation depends on the direction of this circulation. A flow directed from the poles to the equator at the surface and from the equator to the poles in deep layers results in relatively fast rotation of the equatorial zone. If the circulation is directed oppositely, the angular velocity increases from the equator to the poles. Relatively fast rotation at the poles may also result from fast circulation, irrespective of its direction. A simple illustrative explanation is given here to these results. Analytical estimates are supported by numerical calculations. The time variations in the meridional flow observed on the Sun should contribute to torsional oscillations. \textcopyright{} Pleiades Publishing; Inc., 2006.},
  keywords = {97.10.K,notion,notion-database,PACS numbers 97.10.K}
}

@article{Kitchatinov2016,
  title = {Meridional Circulation in the {{Sun}} and Stars},
  author = {Kitchatinov, L L},
  year = {2016},
  journal = {Geomagnetism and Aeronomy},
  volume = {56},
  number = {8},
  eprint = {1603.07852v3},
  urldate = {2020-05-21},
  abstract = {Mean-field hydrodynamics advanced to clear explanations for the origin and properties of the global meridional flow in stellar convection zones. Qualitative arguments and analysis of basic equations both show that the meridional circulation is driven by non-conservative centrifugal and buoyancy forces and results from a slight disbalance between these two drivers. The deviations from the thermal wind balance are relatively large near the boundaries of convection zones. Accordingly, the meridional flow attains its largest velocities in the boundary layers and decreases inside the convection zone. This picture, however, is neither supported nor dismissed by the conflicting results of recent helioseismic soundings or 3D numerical experiments. The relevant physics of the differential temperature and its possible relation to the solar oblateness are briefly discussed.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/G25WBHIJ/full-text.pdf}
}

@article{Kitchatinov2019a,
  title = {Modelling Differential Rotation of Red Giants: The Case of the Evolved Sun},
  author = {Kitchatinov, Leonid and Nepomnyashchikh, Alexander},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {490},
  number = {1},
  eprint = {1909.11928},
  pages = {L71-L75},
  publisher = {{Oxford University Press}},
  issn = {1745-3925},
  doi = {10.1093/mnrasl/slz150},
  abstract = {Asteroseismology has revealed that cores of red giants rotate about one order of magnitude faster than their convective envelopes. This paper attempts an explanation for this rotational state in terms of the theory of angular momentum transport in stellar convection zones. A differential rotation model based on the theory is applied to a sequence of evolutionary states of a red giant of one solar mass. The model computations show a rotation of about ten times faster in the cores compared to the stellar surface. This rotational state is caused by the non-diffusive downward convective transport of angular momentum. The contrast in rotational rates between core and envelope increases with the radius (age) of the star. Seismologically detected scaling for the spin-down of the giants' cores is also reproduced.},
  archiveprefix = {arxiv},
  keywords = {1 i n t,2012,analysed the,asteroseismology of red giants,beck et al,evolution,has revealed a strong,hydrodynamics,in the rotation of,inhomogeneity,interiors,notion,notion-database,ro d u c,rotation,stars,sun,t i o n,their interiors},
  file = {/Users/lbugnet/Zotero/storage/F39DQE8R/Kitchatinov, Nepomnyashchikh - 2019.pdf}
}

@article{Kjeldsen1994,
  title = {Solar-like Oscillations in Eta {{Boo}}},
  author = {Kjeldsen, Hans and Bedding, Timothy R and Viskum, M. and Frandsen, S{\o}ren},
  year = {1994},
  journal = {The Astronomical Journal},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/D6L638UG/Kjeldsen et al. - 1994.pdf}
}

@article{Kjeldsen2008,
  title = {The {{Amplitude}} of {{Solar Oscillations Using Stellar Techniques}}},
  author = {Kjeldsen, Hans and Bedding, Timothy R. and Arentoft, Torben and Butler, R. Paul and Dall, Thomas H. and Karoff, Christoffer and Kiss, L{\'a}szl{\'o} L. and Tinney, C. G. and Chaplin, William J.},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {682},
  number = {2},
  eprint = {0804.1182},
  pages = {1370--1375},
  issn = {0004-637X},
  doi = {10.1086/589142},
  abstract = {The amplitudes of solar-like oscillations depend on the excitation and damping, both of which are controlled by convection. Comparing observations with theory should therefore improve our understanding of the underlying physics. However, theoretical models invariably compute oscillation amplitudes relative to the Sun, and it is therefore vital to have a good calibration of the solar amplitude using stellar techniques. We have used daytime spectra of the Sun, obtained with HARPS and UCLES, to measure the solar oscillations and made a detailed comparison with observations using the BiSON helioseismology instrument. We find that the mean solar amplitude measured using stellar techniques, averaged over one full solar cycle, is 18.7 +/- 0.7 cm/s for the strongest radial modes (l=0) and 25.2 +/- 0.9 cm/s for l=1. In addition, we use simulations to establish an equation that estimates the uncertainty of amplitude measurements that are made of other stars, given that the mode lifetime is known. Finally, we also give amplitudes of solar-like oscillations for three stars that we measured from a series of short observations with HARPS (gamma Ser, beta Aql and alpha For), together with revised amplitudes for five other stars for which we have previously published results (alpha Cen A, alpha Cen B, beta Hyi, nu Ind and delta Pav).},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4K4H5UR6/Kjeldsen et al. - 2008.pdf}
}

@article{Kjeldsen2008b,
  title = {Correcting {{Stellar Oscillation Frequencies}} for {{Near-Surface Effects}}},
  author = {Kjeldsen, Hans and Bedding, Timothy R. and {Christensen-Dalsgaard}, J{\o}rgen},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {683},
  number = {2},
  eprint = {0807.1769},
  pages = {L175-L178},
  issn = {0004-637X},
  doi = {10.1086/591667},
  abstract = {In helioseismology, there is a well-known offset between observed and computed oscillation frequencies. This offset is known to arise from improper modeling of the near-surface layers of the Sun, and a similar effect must occur for models of other stars. Such an effect impedes progress in asteroseismology, which involves comparing observed oscillation frequencies with those calculated from theoretical models. Here, we use data for the Sun to derive an empirical correction for the near-surface offset, which we then apply three other stars (alpha Cen A, alpha Cen B and beta Hyi). The method appears to give good results, in particular providing an accurate estimate of the mean density of each star.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/66VRVI8S/Kjeldsen, Bedding, Christensen-Dalsgaard - 2008.pdf}
}

@article{Kjeldsen2010a,
  title = {The {{Kepler Asteroseismic Investigation}}: {{Scientific}} Goals and First Results},
  author = {Kjeldsen, H. and {Christensen-Dalsgaard}, J. and Handberg, R. and Brown, T. M. and Gilliland, R. L. and Borucki, W. J. and Koch, D.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  pages = {966--971},
  issn = {00046337},
  doi = {10.1002/asna.201011437},
  abstract = {Kepler is a NASA mission designed to detect exoplanets and characterize the properties of exoplanetary systems. Kepler also includes an asteroseismic programme which is being conducted through the Kepler Asteroseismic Science Consortium (KASC), whose 400 members are organized into 13 working groups by type of variable star. So far data have been available from the first 7 month of the mission containing a total of 2937 targets observed at a 1-min cadence for periods between 10 days and 7 months. The goals of the asteroseismic part of the Kepler project is to perform detailed studies of stellar interiors. The first results of the asteroseismic analysis are orders of magnitude better than seen before, and this bodes well for how the future analysis of Kepler data for many types of stars will impact our general understanding of stellar structure and evolution. \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {notion,notion-database,Planetary systems,Space vehicles,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/655W9KTR/Kjeldsen et al. - 2010.pdf}
}

@article{Kjeldsen2011,
  title = {Amplitudes of Solar-like Oscillations: {{A}} New Scaling Relation},
  author = {Kjeldsen, H. and Bedding, T. R.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {529},
  eprint = {1104.1659},
  pages = {2--5},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116789},
  abstract = {Solar-like oscillations are excited by near-surface convection and are being observed in growing numbers of stars using ground- and space-based telescopes. We have previously suggested an empirical scaling relation to predict their amplitudes. This relation has found widespread use but it predicts amplitudes in F-type stars that are higher than observed. Here we present a new scaling relation that is based on the postulate that the power in velocity fluctuations due to p-mode oscillations scales with stellar parameters in the same way as the power in velocity fluctuations due to granulation. The new relation includes a dependence on the damping rate via the mode lifetime and should be testable using observations from the CoRoT and Kepler missions. We also suggest scaling relations for the properties of the background power due to granulation and argue that both these and the amplitude relations should be applicable to red giant stars. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: general,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/YZN9DBHX/Kjeldsen, Bedding - 2011.pdf}
}

@article{Kleinman2013,
  title = {{{SDSS DR7 White Dwarf Catalog}}},
  author = {Kleinman, S. J. and Kepler, S. O. and Koester, D. and Pelisoli, Ingrid and Pe{\c c}anha, Viviane and Nitta, A. and Costa, J. E. S. and Krzesinski, J. and Dufour, P. and Lachapelle, F. -R. and Bergeron, P. and Yip, Ching-Wa and Harris, Hugh C. and Eisenstein, Daniel J. and Althaus, L. and C{\'o}rsico, A.},
  year = {2013},
  month = jan,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {204},
  pages = {5},
  issn = {0067-0049},
  doi = {10.1088/0067-0049/204/1/5},
  urldate = {2023-10-09},
  abstract = {We present a new catalog of spectroscopically confirmed white dwarf stars from the Sloan Digital Sky Survey (SDSS) Data Release 7 spectroscopic catalog. We find 20,407 white dwarf spectra, representing 19,712 stars, and provide atmospheric model fits to 14,120 DA and 1011 DB white dwarf spectra from 12,843 and 923 stars, respectively. These numbers represent more than a factor of two increase in the total number of white dwarf stars from the previous SDSS white dwarf catalogs based on DR4 data. Our distribution of subtypes varies from previous catalogs due to our more conservative, manual classifications of each star in our catalog, supplementing our automatic fits. In particular, we find a large number of magnetic white dwarf stars whose small Zeeman splittings mimic increased Stark broadening that would otherwise result in an overestimated log g if fit as a non-magnetic white dwarf. We calculate mean DA and DB masses for our clean, non-magnetic sample and find the DB mean mass is statistically larger than that for the DAs.},
  keywords = {Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,catalogs,magnetic fields,mass function,stars: luminosity function,surveys,white dwarfs},
  annotation = {ADS Bibcode: 2013ApJS..204....5K},
  file = {/Users/lbugnet/Zotero/storage/2JAS5AIA/Kleinman et al. - 2013 - SDSS DR7 White Dwarf Catalog.pdf}
}

@article{Koch2010,
  title = {Kepler Mission Design, Realized Photometric Performance, and Early Science},
  author = {Koch, David G. and Borucki, William J. and Basri, Gibor and Batalha, Natalie M. and Brown, Timothy M. and Caldwell, Douglas and {Christensen-Dalsgaard}, J{\o}rgen and Cochran, William D. and Devore, Edna and Dunham, Edward W. and Gautier, Thomas N. and Geary, John C. and Gilliland, Ronald L. and Gould, Alan and Jenkins, Jon and Kondo, Yoji and Latham, David W. and Lissauer, Jack J. and Marcy, Geoffrey and Monet, David and Sasselov, Dimitar and Boss, Alan and Brownlee, Donald and Caldwell, John and Dupree, Andrea K. and Howell, Steve B. and Kjeldsen, Hans and Meibom, S{\o}ren and Morrison, David and Owen, Tobias and Reitsema, Harold and Tarter, Jill and Bryson, Stephen T. and Dotson, Jessie L. and Gazis, Paul and Haas, Michael R. and Kolodziejczak, Jeffrey and Rowe, Jason F. and Van Cleve, Jeffrey E. and Allen, Christopher and Chandrasekaran, Hema and Clarke, Bruce D. and Li, Jie and Quintana, Elisa V. and Tenenbaum, Peter and Twicken, Joseph D. and Wu, Hayley},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L79},
  abstract = {The Kepler Mission, launched on 2009 March 6, was designed with the explicit capability to detect Earth-size planets in the habitable zone of solar-like stars using the transit photometry method. Results from just 43days of data along with ground-based follow-up observations have identified five new transiting planets with measurements of their masses, radii, and orbital periods. Many aspects of stellar astrophysics also benefit from the unique, precise, extended, and nearly continuous data set for a large number and variety of stars. Early results for classical variables and eclipsing stars show great promise. To fully understand the methodology, processes, and eventually the results from the mission, we present the underlying rationale that ultimately led to the flight and ground system designs used to achieve the exquisite photometric performance. As an example of the initial photometric results, we present variability measurements that can be used to distinguish dwarf stars from red giants. \textcopyright{} 2010. The American Astronomical Society. All rights reserved..},
  keywords = {general,instrumentation,instruments,notion,notion-database,photometers,photometric,planetary systems,space vehicles,stars,statistics,techniques,variables},
  file = {/Users/lbugnet/Zotero/storage/EKKSYACI/Koch et al. - 2010.pdf}
}

@article{Kochukhov2010,
  title = {Least-Squares Deconvolution of the Stellar Intensity and Polarization Spectra},
  author = {Kochukhov, O. and Makaganiuk, V. and Piskunov, N.},
  year = {2010},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {524},
  number = {1},
  eprint = {1008.5115},
  issn = {00046361},
  doi = {10.1051/0004-6361/201015429},
  urldate = {2020-07-02},
  abstract = {Context. Least-squares deconvolution (LSD) is a powerful method of extracting high-precision average line profiles from the stellar intensity and polarization spectra. This technique is widely used for detection, characterization, and detailed mapping of the temperature, magnetic, and chemical abundance structures on the surfaces of stars. Aims. Despite its common usage, the LSD method is poorly documented and has never been tested with realistic synthetic spectra. In this study we revisit the key assumptions of the LSD technique, clarify its numerical implementation, discuss possible improvements and give recommendations of how to make LSD results understandable and reproducible. We also address the problem of interpretation of the moments and shapes of the LSD profiles in terms of physical parameters. Methods. We have developed an improved, multiprofile version of LSD (iLSD) and have extended the deconvolution procedure to linear polarization analysis taking into account anomalous Zeeman splitting of spectral lines. The iLSD method is applied to the theoretical Stokes parameter spectra computed for a wide wavelength interval containing all relevant spectral lines. We test various methods of interpreting the mean profiles, investigating how coarse approximations of the multiline technique translate into errors of the derived parameters. Results. We find that, generally, the Stokes parameter LSD profiles do not behave as a real spectral line with respect to the variation of magnetic field and elemental abundance. This problem is especially prominent for the Stokes I (intensity) variation with abundance and Stokes Q (linear polarization) variation with magnetic field. At the same time, the Stokes V (circular polarization) LSD spectra closely resemble the profile of a properly chosen synthetic line for the magnetic field strength up to 1 kG. The longitudinal field estimated from the Stokes V LSD profile is accurate to within 10\% for the field strength below 5 kG and to within a few percent for the fields weaker than 1 kG. Our iLSD technique offers clear advantages over the standard LSD method in the individual analysis of different chemical elements. Conclusions. We conclude that the usual method of interpreting the LSD profiles by assuming that they are equivalent to a real spectral line gives satisfactory results only in a limited parameter range and thus should be applied with caution. A more trustworthy approach is to abandon the single-line approximation of the average profiles and apply LSD consistently to observations and synthetic spectra. \textcopyright{} ESO, 2010.},
  archiveprefix = {arxiv},
  keywords = {Line: formation,Magnetic fields,Methods: data analysis,Methods: numerical,notion,notion-database,Polarization,Stars: atmospheres},
  file = {/Users/lbugnet/Zotero/storage/KES69YZN/full-text.pdf}
}

@article{Kohonen1990,
  title = {Cortical Maps [10]},
  author = {Kohonen, T.},
  year = {1990},
  journal = {Nature},
  volume = {346},
  number = {6279},
  pages = {24},
  publisher = {{Nature Publishing Group}},
  issn = {00280836},
  doi = {10.1038/346024b0},
  urldate = {2020-04-11},
  keywords = {Humanities and Social Sciences,multidisciplinary,notion,notion-database,Science}
}

@article{Kolenberg2010,
  title = {First Kepler Results on Rrlyrae Stars},
  author = {Kolenberg, K. and Szab{\'o}, R. and Kurtz, D. W. and Gilliland, R. L. and {Christensen-Dalsgaard}, J. and Kjeldsen, H. and Brown, T. M. and Benk{\~o}, J. M. and Chadid, M. and Derekas, A. and Criscienzo, M. Di and Guggenberger, E. and Kinemuchi, K. and Kunder, A. and Koll{\'a}th, Z. and Kopacki, G. and Moskalik, P. and Nemec, J. M. and Nuspl, J. and Silvotti, R. and Suran, M. D. and Borucki, W. J. and Koch, D. and Jenkins, J. M.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  eprint = {1001.0417},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L198},
  abstract = {We present the first results of our analyses of selected RRLyrae stars for which data have been obtained by the Kepler Mission. As expected, we find a significant fraction of the RRab stars to show the Blazhko effect, a still unexplained phenomenon that manifests itself as periodic amplitude and phase modulations of the light curve, on timescales of typically tens to hundreds of days. The long time span of the Kepler Mission of 3.5yr and the unprecedentedly high precision of its data provide a unique opportunity for the study of RRLyrae stars. Using data of a modulated star observed in the first roll as a showcase, we discuss the data, our analyses, findings, and their implications for our understanding of RRLyrae stars and the Blazhko effect. With at least 40\% of the RR Lyrae stars in our sample showing modulation, we confirm the high incidence rate that was only found in recent high-precision studies. Moreover, we report the occurrence of additional frequencies, beyond the main pulsation mode and its modulation components. Their half-integer ratio to the main frequency is reminiscent of a period doubling effect caused by resonances, observed for the first time in RRLyrae stars. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,{Stars: individual: (KIC5559631 (V783 Cyg), KIC3733},Stars: oscillations,Stars: variables: RR Lyrae},
  file = {/Users/lbugnet/Zotero/storage/CINDLW7R/Kolenberg et al. - 2010.pdf}
}

@article{Kolotkov2015,
  title = {Hilbert-{{Huang}} Transform Analysis of Periodicities in the Last Two Solar Activity Cycles},
  author = {Kolotkov, D. Y. and Broomhall, A. M. and Nakariakov, V. M.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {451},
  number = {4},
  pages = {4360--4367},
  issn = {13652966},
  doi = {10.1093/mnras/stv1253},
  abstract = {We investigated periodicities associated with the last two-and-a-half solar activity cycles with the novel Hilbert-Huang transform (HHT) method. Raw data signals of five different observational proxies: the 10.7 cm radio flux intensity, the helioseismic frequency shift, and the sunspot area signals recorded from the whole solar disc, and separately from the Northern and Southern hemispheres, were expanded into a set of intrinsic modes with the ensemble empirical mode decomposition technique. Instant and mean periods of each empirical mode were obtained with the use of the Hilbert transform applied independently to each separate mode. The periodicities were allocated to three distinct groups: short-term variations (with periods shorter than 0.5 yr), quasi-biennial oscillations (with typical periods from 0.5 yr to 3.9 yr), and longer periodicities, e.g. such as the 11 yr cycle. All periodicities detected in the examined solar cycles 22-24 are consistent with the well-known results found in the earlier solar epochs. We have demonstrated that the HHT method is a good tool for characterizing periodicities in the helioseismic data, which are necessarily relatively limited in terms of their time resolution. Periodicities obtained using the helioseismic data are, nevertheless, consistent with those found in other proxies. Since helioseismic oscillations are sensitive to the solar interior, this indicates that the behaviour of surface and atmospheric magnetic activity reflects that of the Sun's internal magnetic field. All identified intrinsic modes are seen to have clear amplitude modulation highly correlated with the 11 yr cycle. This amplitude modulation is most pronounced in the short-period modes. The short-term periodicities were found to be multiples of the shortest period, of 25 d. This ordering of the short-term periodicities is consistent with the previous findings. Signatures of the north-south asymmetry were detected in the individual hemisphere sunspot area indices. Furthermore, evidence of the last 'extended' solar minimum was detected too.},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/24REHNGI/Kolotkov, Broomhall, Nakariakov - 2015.pdf}
}

@article{Komm2000,
  title = {{{SOLAR-CYCLE CHANGES IN GONG}} p-{{MODE WIDTHS AND AMPLITUDES 1995\`E1998}}},
  author = {Komm, R W and Howe, R and Hill, F},
  year = {2000},
  journal = {THE ASTROPHYSICAL JOURNAL},
  volume = {531},
  pages = {1094--1108},
  urldate = {2022-01-26},
  abstract = {We search for a solar-cycle variation in mode widths and amplitudes derived from 3 month GONG time series. The variation of mode width and amplitude observed in GONG data are the combined e \textdagger ects of \DH ll factor, temporal variation, and measurement uncertainties. The largest variation is caused by the \DH ll factor resulting in modes with increased width and reduced amplitude when \DH ll is lower. We assume that the solar-cycle variation is the only other systematic variation beside the temporal window function e \textdagger ect. We correct all currently available data sets for the \DH ll factor and simultaneously derive the solar-cycle variation. We \DH nd an increase of about 3\% on average in mode width from the previous minimum to October 1998 and a decrease of about 7\% and 6\% in mode amplitude and mode area (width ] amplitude). We \DH nd no l dependence of the solar-cycle changes. As a function of frequency, these changes show a maximum between 2.7 and 3.3 mHz with about 47\% higher than average values for mode width and about 29\% and 36\% higher ones for mode amplitude and area. We estimate the signi\DH cance of these rather small changes by a prewhitening method and \DH nd that the results are signi\DH -cant at or above the 99.9\% level, with mode area showing the highest level of signi\DH cance and mode width the lowest. The variation in background amplitude is most likely not signi\DH cant and is consistent with a zero change.},
  keywords = {activity \`E Sun,evolution \`E Sun,notion,notion-database,oscillations,Subject headings,Sun},
  file = {/Users/lbugnet/Zotero/storage/UMJQU9IC/full-text.pdf}
}

@article{Komm2013,
  title = {Subsurface {{Meridional Flow}} from {{HMI Using}} the {{Ring-Diagram Pipeline}}},
  author = {Komm, R. and Gonz{\'a}lez~Hern{\'a}ndez, I. and Hill, F. and Bogart, R. and {Rabello-Soares}, M. C. and Haber, D.},
  year = {2013},
  journal = {Solar Physics},
  volume = {287},
  number = {1-2},
  pages = {85--106},
  issn = {1573093X},
  doi = {10.1007/s11207-012-0073-y},
  abstract = {We have determined the meridional flows in subsurface layers for 18 Carrington rotations (CR 2097 to 2114) analyzing high-resolution Dopplergrams obtained with the Helioseismic and Magnetic Imager (HMI) instrument onboard the Solar Dynamics Observatory (SDO). We are especially interested in flows at high latitudes up to 75\textdegree{} in order to address the question whether the meridional flow remains poleward or reverses direction (so-called counter cells). The flows have been determined in depth from near-surface layers to about 16 Mm using the HMI ring-diagram pipeline. The measured meridional flows show systematic effects, such as a variation with the B 0 -angle and a variation with central meridian distance (CMD). These variations have been taken into account to lead to more reliable flow estimates at high latitudes. The corrected average meridional flow is poleward at most depths and latitudes with a maximum amplitude of about 20 ms -1 near 37.5\textdegree{} latitude. The flows are more poleward on the equatorward side of the mean latitude of magnetic activity at 22\textdegree{} and less poleward on the poleward side, which can be interpreted as convergent flows near the mean latitude of activity. The corrected meridional flow is poleward at all depths within {$\pm$} 67.5\textdegree{} latitude. The corrected flow is equatorward only at 75\textdegree{} latitude in the southern hemisphere at depths between about 4 and 8 Mm and at 75\textdegree{} latitude in the northern hemisphere only when the B 0 angle is barely large enough to measure flows at this latitude. These counter cells are most likely the remains of an insufficiently corrected B 0 -angle variation and not of solar origin. Flow measurements and B 0 -angle corrections are difficult at the highest latitude because these flows are only determined during limited periods when the B 0 angle is sufficiently large. \textcopyright{} 2012 Springer Science+Business Media B.V.},
  keywords = {{Helioseismology, observations},notion,notion-database,{Velocity fields, interior}},
  file = {/Users/lbugnet/Zotero/storage/778NA7WW/Komm et al. - 2013.pdf}
}

@article{Korre2021,
  title = {On the Dynamical Interaction between Overshooting Convection and an Underlying Dipole Magnetic Field - {{I}}. {{The}} Non-Dynamo Regime},
  author = {Korre, L. and Brummell, {\relax NH} and Garaud, P. and Guervilly, C.},
  year = {2021},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {503},
  pages = {362--375},
  issn = {0035-8711},
  doi = {10.1093/mnras/stab477},
  urldate = {2023-10-11},
  abstract = {Motivated by the dynamics in the deep interiors of many stars, we study the interaction between overshooting convection and the large-scale poloidal fields residing in radiative zones. We have run a suite of 3D Boussinesq numerical calculations in a spherical shell that consists of a convection zone with an underlying stable region that initially compactly contains a dipole field. By varying the strength of the convective driving, we find that, in the less turbulent regime, convection acts as turbulent diffusion that removes the field faster than solely molecular diffusion would do. However, in the more turbulent regime, turbulent pumping becomes more efficient and partially counteracts turbulent diffusion, leading to a local accumulation of the field below the overshoot region. These simulations suggest that dipole fields might be confined in underlying stable regions by highly turbulent convective motions at stellar parameters. The confinement is of large-scale field in an average sense and we show that it is reasonably modelled by mean-field ideas. Our findings are particularly interesting for certain models of the Sun, which require a large-scale, poloidal magnetic field to be confined in the solar radiative zone in order to explain simultaneously the uniform rotation of the latter and the thinness of the solar tachocline.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,convection,MHD,Physics - Fluid Dynamics,stars: interiors,Sun: interior},
  annotation = {ADS Bibcode: 2021MNRAS.503..362K},
  file = {/Users/lbugnet/Zotero/storage/6UJBJ7Z7/Korre et al. - 2021 - On the dynamical interaction between overshooting .pdf}
}

@article{Korre2021a,
  title = {On the Dynamical Interaction between Overshooting Convection and an Underlying Dipole Magnetic Field - {{I}}. {{The}} Non-Dynamo Regime},
  author = {Korre, L. and Brummell, N. H. and Garaud, P. and Guervilly, C.},
  year = {2021},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {503},
  number = {1},
  pages = {362--375},
  issn = {0035-8711},
  doi = {10.1093/mnras/stab477},
  urldate = {2023-10-12},
  abstract = {Motivated by the dynamics in the deep interiors of many stars, we study the interaction between overshooting convection and the large-scale poloidal fields residing in radiative zones. We have run a suite of 3D Boussinesq numerical calculations in a spherical shell that consists of a convection zone with an underlying stable region that initially compactly contains a dipole field. By varying the strength of the convective driving, we find that, in the less turbulent regime, convection acts as turbulent diffusion that removes the field faster than solely molecular diffusion would do. However, in the more turbulent regime, turbulent pumping becomes more efficient and partially counteracts turbulent diffusion, leading to a local accumulation of the field below the overshoot region. These simulations suggest that dipole fields might be confined in underlying stable regions by highly turbulent convective motions at stellar parameters. The confinement is of large-scale field in an average sense and we show that it is reasonably modelled by mean-field ideas. Our findings are particularly interesting for certain models of the Sun, which require a large-scale, poloidal magnetic field to be confined in the solar radiative zone in order to explain simultaneously the uniform rotation of the latter and the thinness of the solar tachocline.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/KFDSISJG/Korre et al. - 2021 - On the dynamical interaction between overshooting .pdf}
}

@article{Korzennik2005,
  title = {A {{Mode}}-{{Fitting Methodology Optimized}} for {{Very Long Helioseismic Time Series}}},
  author = {Korzennik, S. G.},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {626},
  number = {1},
  eprint = {astro-ph/0406470},
  pages = {585--615},
  issn = {0004-637X},
  doi = {10.1086/429748},
  abstract = {I describe and present the results of a newly developed fitting methodology optimized for very long time series. The development of this new methodology was motivated by the fact that we now have more than half a decade of nearly uninterrupted observations by the Global Oscillation Network Group (GONG) and the Michelson Doppler Imager (MDI), with fill factors as high as 82.2\% and 89.8\%, respectively. It was recently prompted by the availability of a 2088 day long time series of spherical harmonic coefficients produced by the MDI team. The fitting procedure uses an optimal sine multitaper spectral estimator, with the number of tapers based on the mode line width, the complete leakage matrix (i.e., horizontal as well as vertical components), and an asymmetric mode profile to fit simultaneously all the azimuthal orders with individually parameterized profiles. This method was applied to 2088 day long time series of MDI and GONG observations, as well as 728 day long subsets, and for spherical harmonic degrees between 1 and 25. The values resulting from these fits are intercompared (MDI vs. GONG) and compared to equivalent estimates from the MDI team and the GONG project. I also compare the results from fitting the 728 day subsets to the result of the 2088 day time series. This comparison shows the well-known change of frequencies with solar activity and how it scales with a nearly constant pattern in frequency and m/l. This comparison also shows some changes in the mode line width and the constancy of the mode asymmetry. Subject headingg s: methods: statistical-Sun: oscillations Online material: color figures, machine-readable table 1. MOTIVATION Several methodologies for the precise measurements of p-mode frequencies have been developed over the years (see, among others, These techniques have evolved as the quality of the observations has improved over the years. More recently, such methods have produced frequency and rotational frequency splitting tables-typically based on 108 day long and 72 day long time series for Global Oscillation Network Group (GONG) and Michelson Doppler Imager (MDI) data, respectively-that have been the basis for countless inferences of the structure and dynamics of the solar interior. Some 8 years after the deployment of the GONG network and the launch of the Solar and Heliospheric Observatory (SOHO), we now have access to more than half a decade of nearly uninterrupted times series of solar observations. The MDI team has recently produced a 2088 day long time series of spherical harmonic coefficients at a 1 minute sampling interval, namely a time series in excess of 3 million points. For low-degree and low-frequency modes the availability of such a very long time series provides a unique opportunity to develop a mode-fitting methodology that exploits the properties of such an exquisite data set. I present here a new methodology that I have developed to fit modes using very long time series. This methodology includes an optimal sine multitaper spectral estimator, the complete leakage matrix (i.e., horizontal as well as vertical components), an asymmetric profile, and the simultaneous fitting of individual profiles at all the azimuthal orders (m) for a given (n, l) mode. The contamination by nearby modes (n 0 , l 0) within the fitting range is also included. Since simultaneous fitting on these contaminants is impractical, the fitting procedure is iterated; i.e., the characteristics of the contaminants used in the fitting correspond to the values fitted at the previous iteration. The primary goal of this work was to extend the mode fitting to low-order and low-degree modes. The low-degree modes carry information on the structure and dynamics of the deep interior, while the low-order low-degree modes are long lived (i.e., show very narrow peaks) and can thus be measured with very high precision. Since their amplitude is small, they will emerge above the background noise only for very long time series. The secondary goal was to fit simultaneously all the modes instead of using the traditional polynomial expansion in m/l, while using the complete leakage matrix and including the well-known mode-profile asymmetry. I describe the data sets I used in x 2 and present the details of the methodology in x 3. In x 4 I present the results of fitting both MDI and GONG 2088 day long coeval time series. These results are compared to equivalent estimates from the MDI team and the GONG project. I also present the results of fitting 2 yr long subsets of that time series for both data sets and show how the fitted parameters change with epoch and hence with solar activity. 2. DATA SETS USED The work presented here is based on times series of spherical harmonic coefficients computed from full-disk observations by the MDI and GONG instruments and limited to l 25. The MDI 2088 day long time series was used to develop the methodology. It was then applied to the coeval GONG data set. Both data sets were also subdivided into five 728 day long overlapping segments (actually 1,048,576 minute long segments, i.e., 1024 2), each offset by some 364 days (i.e., 524,288 minutes) from the previous one. The last 728 day segment was completed by augmenting the 2088 day time series by an extra 97 days (i.e., 139,008 minutes) to fill it completely. The respective ranges of A 585},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/M2MT9Y8G/Korzennik - 2005.pdf}
}

@article{Korzennik2008a,
  title = {Current Status of Asteroseismology},
  author = {Korzennik, Sylvain G.},
  year = {2008},
  journal = {Advances in Space Research},
  volume = {41},
  number = {6},
  pages = {897--906},
  issn = {02731177},
  doi = {10.1016/j.asr.2007.01.029},
  abstract = {Asteroseismology, the extension of helioseismology to stars - solar-alike or not - has been an exciting and active field of research for about two decades. While over that period helioseismology has had great success in revealing the solar structure and its dynamics, progress in asteroseismology has been hampered by the observational challenge to carry out, primarily from the ground, high precision measurements on unresolved objects with a substantially lower flux. Over the past years, the field has seen a new golden age, primarily driven by observational advances and opportunities. With the June 2003 launch of the MOST spacecraft and the highly anticipated December 2006 launch of the COROT mission, we have truly entered the space-based observational era of asteroseismology. The ambitious vision mission like the Stellar Imager might even one day allow us to spatially resolve oscillations on not too distant stars. At the same time ground-based observations have recently seen a quantum leap in precision thanks to the synergy between asteroseismology and exo-planet detection which both rely primarily on precise radial velocity techniques. The diagnostic potential of asteroseismology is clearly demonstrated by the wealth of inferences collected from helioseismology. Nevertheless the current status of observations, their interpretations and their implications for our models remain hotly debated subjects. I review the status of the field, with an emphasis on solar-like targets, while incorporating my own healthy scepticism and observational bias. \textcopyright{} 2007 COSPAR.},
  keywords = {Asteroseismology,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BVIV2RSY/Korzennik - 2008.pdf}
}

@article{Kosovichev1988,
  title = {The {{Internal Rotation}} of the {{Sun}} from {{Helioseismological Data}}},
  author = {Kosovichev, A. G. and G., A.},
  year = {1988},
  journal = {SvAL},
  volume = {14},
  pages = {145},
  urldate = {2020-03-08},
  keywords = {notion,notion-database}
}

@article{Kosovichev1998,
  title = {X-Ray Flare Sparks Quake inside Sun [5]},
  author = {Kosovichev, A. G. and Zharkova, V. V.},
  year = {1998},
  journal = {Nature},
  volume = {393},
  number = {6683},
  pages = {317--318},
  issn = {00280836},
  doi = {10.1038/30629},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/H9BK3CCB/Kosovichev, Zharkova - 1998.pdf}
}

@article{Kosovichev2008,
  title = {Special Feature {{L}} Etter to the {{E}} Ditor {{Properties}} of High-Degree Oscillation Modes of the {{Sun}} Observed with {{Hinode}} / {{SOT}}},
  author = {Kosovichev, A G and Sekii, T},
  year = {2008},
  volume = {4},
  pages = {1--4},
  keywords = {atmosphere,granulation,helioseismology,notion,notion-database,oscillations,sun,{Sun: atmosphere, Sun: granulation, Sun: helioseism}},
  file = {/Users/lbugnet/Zotero/storage/Q92Q55RF/Kosovichev, Sekii - 2008.pdf}
}

@article{Kosovichev2009a,
  title = {Solar Oscillations},
  author = {Kosovichev, A. G.},
  year = {2009},
  journal = {AIP Conference Proceedings},
  volume = {1170},
  pages = {547--559},
  issn = {0094243X},
  doi = {10.1063/1.3246561},
  abstract = {In recent years solar oscillations have been studied in great detail, both observationally and theoretically; so, perhaps, the Sun currently is the best understood pulsating star. The observational studies include long, almost uninterrupted series of oscillation data from the SOHO spacecraft and ground-based networks, GONG and BiSON, and more recently, extremely high-resolution observations from the Hinode mission. These observational data cover the whole oscillation spectrum, and have been extensively used for helioseismology studies, providing frequencies and travel times for diagnostics of the internal stratification, differential rotation, zonal and meridional flows, subsurface convection and sunspots. Together with realistic numerical simulations, they lead to better understanding of the excitation mechanism and interactions of the oscillations with turbulence and magnetic fields. However, many problems remain unsolved. In particular, the precision of the helioseismology measurements is still insufficient for detecting the dynamo zone and deep routes of sunspots. Our knowledge of the oscillation physics in strong magnetic field regions is inadequate for interpretation of MHD waves in sunspots and for sunspot seismology. A new significant progress in studying the solar oscillations is expected from the Solar Dynamics Observatory scheduled for launch in 2009.\textcopyright{} 2009 American Institute of Physics.},
  isbn = {9780735407077},
  keywords = {Helioseismology,notion,notion-database,Solar interior,Solar oscillations},
  file = {/Users/lbugnet/Zotero/storage/YWZKV9GT/Kosovichev - 2009(2).pdf;/Users/lbugnet/Zotero/storage/ZLARMM8G/Kosovichev - 2009.pdf}
}

@article{Kotov1983a,
  title = {Quality {{Diagrams}} for {{Processes}} in {{Nonlinear Automatic Systems}}.},
  author = {Kotov, Ye A. and Popov, Ye P.},
  year = {1983},
  journal = {Engineering cybernetics},
  volume = {21},
  number = {4},
  pages = {49--54},
  issn = {0013788X},
  abstract = {A new approach is proposed for the solution of harmonically linearized equations defining the transition processes in nonlinear systems. This approach is based on preliminary transformation of the original equations to bilinear form and it can be applied to nonlinear automatic control systems whose block diagram is put in a form with an arbitrary singled-out nonlinearity and an arbitrary reduced linear part. The algorithms are described in detail for solving harmonically linearized equations in the study of systems with various kinds of nonlinearities.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VQ8RAAVQ/Kotov, Popov - 1983.pdf}
}

@article{Kovari2014,
  title = {Observing {{Dynamos}} in {{Cool Stars}}},
  author = {K{\H o}v{\'a}ri, Z. and Ol{\'a}h, K.},
  year = {2014},
  journal = {Space Science Reviews},
  volume = {186},
  number = {1-4},
  pages = {457--489},
  issn = {15729672},
  doi = {10.1007/s11214-014-0092-0},
  abstract = {The main aim of this paper is to introduce the most important observables that help us to investigate stellar dynamos and compare those to the modeling results. We give an overview of the available observational methods and data processing techniques that are suitable for such purposes, with touching upon examples of inadequate interpretations as well. Stellar observations are compared to the solar data in such a way, which ensures that the measurements are comparable in dimension, wavelength, and timescale. A brief outlook is given to the future plans and possibilities. A~thorough review of this topic was published nearly a decade ago (Berdyugina in Living Rev. Sol. Phys. 2:8, 2005), now we focus on the experiences that have been gathered since that time.},
  keywords = {Active stars,Activity cycle,Differential rotation,Magnetic activity,Meridional flow,notion,notion-database,Stellar dynamo},
  file = {/Users/lbugnet/Zotero/storage/R8745NQG/Kővári, Oláh - 2014.pdf}
}

@techreport{Krizhevsky,
  title = {{{ImageNet Classification}} with {{Deep Convolutional Neural Networks}}},
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  urldate = {2020-06-19},
  abstract = {We trained a large, deep convolutional neural network to classify the 1.2 million high-resolution images in the ImageNet LSVRC-2010 contest into the 1000 different classes. On the test data, we achieved top-1 and top-5 error rates of 37.5\% and 17.0\% which is considerably better than the previous state-of-the-art. The neural network, which has 60 million parameters and 650,000 neurons, consists of five convolutional layers, some of which are followed by max-pooling layers, and three fully-connected layers with a final 1000-way softmax. To make training faster, we used non-saturating neurons and a very efficient GPU implementation of the convolution operation. To reduce overfitting in the fully-connected layers we employed a recently-developed regularization method called "dropout" that proved to be very effective. We also entered a variant of this model in the ILSVRC-2012 competition and achieved a winning top-5 test error rate of 15.3\%, compared to 26.2\% achieved by the second-best entry.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/7RSWCHH8/full-text.pdf}
}

@techreport{Krizhevsky2012,
  title = {{{ImageNet Classification}} with {{Deep Convolutional Neural Networks}}},
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  year = {2012},
  urldate = {2020-07-20},
  abstract = {We trained a large, deep convolutional neural network to classify the 1.2 million high-resolution images in the ImageNet LSVRC-2010 contest into the 1000 different classes. On the test data, we achieved top-1 and top-5 error rates of 37.5\% and 17.0\% which is considerably better than the previous state-of-the-art. The neural network, which has 60 million parameters and 650,000 neurons, consists of five convolutional layers, some of which are followed by max-pooling layers, and three fully-connected layers with a final 1000-way softmax. To make training faster, we used non-saturating neurons and a very efficient GPU implementation of the convolution operation. To reduce overfitting in the fully-connected layers we employed a recently-developed regularization method called "dropout" that proved to be very effective. We also entered a variant of this model in the ILSVRC-2012 competition and achieved a winning top-5 test error rate of 15.3\%, compared to 26.2\% achieved by the second-best entry.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Y9QK3R72/full-text.pdf}
}

@article{Kuhn2012,
  title = {The Precise Solar Shape and Its Variability},
  author = {Kuhn, J. R. and Bush, R. and Emilio, M. and Scholl, I. F.},
  year = {2012},
  journal = {Science},
  volume = {337},
  number = {6102},
  pages = {1638--1640},
  issn = {10959203},
  doi = {10.1126/science.1223231},
  abstract = {The precise shape of the Sun has not been convincingly determined, despite half a century of modern photoelectric observations. The expected deviation of the solar-limb shape from a perfect circle is very small, but such asphericity is sensitive to the Sun's otherwise invisible interior conditions, as well as the solar atmosphere. We use evidence from a long-running experiment based in space to show that, when analyzed with sufficiently high spatial resolution, the Sun's oblate shape is distinctly constant and almost completely unaffected by the solar-cycle variability seen on its surface. The solar oblateness is significantly lower than theoretical expectations by an amount that could be explained by a slower differential rotation in the outer few percent of the Sun.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GP29UBDH/Kuhn et al. - 2012.pdf}
}

@article{Kumar1996,
  title = {Observational {{Searches}} for {{Solar}} [{{ITAL}}]g[/{{ITAL}}]-{{Modes}}: {{Some Theoretical Considerations}}},
  author = {Kumar, Pawan and Quataert, Eliot J. and Bahcall, John N.},
  year = {1996},
  journal = {The Astrophysical Journal},
  volume = {458},
  number = {2},
  pages = {1--9},
  issn = {0004637X},
  doi = {10.1086/309926},
  abstract = {We argue that the solar g-modes are unlikely to have caused the discrete peaks in the power spectrum of the solar wind flux observed by Thomson et al (1995). The lower limit to the energy of individual g-modes, using the amplitudes},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DMJX9DVH/Kumar, Quataert, Bahcall - 1996.pdf}
}

@article{Kumar2008a,
  title = {What Are the Observed High-Frequency Solar Acoustic Modes?},
  author = {Kumar, P. and Duvall, T. L. and Harvey, J. W. and Jefferies, S. M. and Pomerantz, M. A. and Thompson, M. J.},
  year = {2008},
  journal = {Progress of Seismology of the Sun and Stars},
  pages = {87--92},
  doi = {10.1007/3-540-53091-6_68},
  abstract = {Jefferies et al. (1988) observe discrete peaks up to 7mHz in the power spectra of their intermediate degree solar intensity oscillation data obtained at South Pole. This is perhaps surprising since waves with frequency greater than the acoustic cut-off frequency at the temperature minimum ( 5.5mHz), unlike their lower frequency counterparts, are not trapped in the solar interior. We propose that the observed peaks are associated with what are principally progressive waves emanating from a broad-band acoustic source. The geometrical effect of projecting observations of these progressive waves onto spherical harmonics then gives rise to peaks in the power spectra. The frequencies and amplitudes of the peaks will depend on the spatial characteristics of the source. Partial reflections in the solar atmosphere modify the power spectra, but in this picture they are not the primary reason for the appearance of the peaks. We estimate the frequency and power which would be expected from this model and compare it with the observations. We argue that these high frequency mock-modes are not overstable, and that they are excited by acoustic emission from turbulent convection.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BYEW37S7/Kumar et al. - 2008.pdf}
}

@article{Kumar2010,
  title = {On the Flare Induced High-Frequency Global Waves in the Sun},
  author = {Kumar, Brajesh and Mathur, Savita and Garc{\'i}a, R. A. and Venkatakrishnan, P.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {711},
  number = {1 PART 2},
  eprint = {1001.4331},
  issn = {20418213},
  doi = {10.1088/2041-8205/711/1/L12},
  abstract = {Recently, Karoff \& Kjeldsen presented evidence of strong correlation between the energy in the high-frequency part (5.3 {$<$} {$\nu$} {$<$} 8.3mHz) of the acoustic spectrum of the Sun and the solar X-ray flux. They have used disk-integrated intensity observations of the Sun obtained from the Variability of solar IRradiance and Gravity Oscillations instrument on board Solar and Heliospheric Observatory (SOHO) spacecraft. Similar signature of flares in velocity observations has not been confirmed till now. The study of low-degree high-frequency waves in the Sun is important for our understanding of the dynamics of the deeper solar layers. In this Letter, we present the analysis of the velocity observations of the Sun obtained from the Michelson and Doppler Imager (MDI) and the Global Oscillations at Low Frequencies (GOLF) instruments on board SOHO for some major flare events of the solar cycle 23. Application of wavelet techniques to the time series of disk-integrated velocity signals from the solar surface using the full-disk Dopplergrams obtained from the MDI clearly indicates that there is enhancement of high-frequency global waves in the Sun during the flares. This signature of flares is also visible in the Fourier Power Spectrum of these velocity oscillations. On the other hand, the analysis of disk-integrated velocity observations obtained from the GOLF shows only marginal evidence of effects of flares on high-frequency oscillations. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: atmosphere,Sun: flares,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4JQ3ME33/Kumar et al. - 2010.pdf}
}

@article{Kumar2011,
  title = {On the Flare-Induced Seismicity in the Active Region {{NOAA}} 10930 and Related Enhancement of Global Waves in the {{Sun}}},
  author = {Kumar, Brajesh and Venkatakrishnan, P. and Mathur, Savita and Tiwari, Sanjiv Kumar and Garc{\'i}a, R. A.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {743},
  number = {1},
  eprint = {1110.6309},
  issn = {15384357},
  doi = {10.1088/0004-637X/743/1/29},
  abstract = {A major flare (of class X3.4) occurred on 2006 December 13 in the active region NOAA 10930. This flare event has remained interesting to solar researchers for studies related to particle acceleration during the flare process and the reconfiguration of magnetic fields as well as fine-scale features in the active region. The energy released during flares is also known to induce acoustic oscillations in the Sun. Here, we analyze the line-of-sight velocity patterns in this active region during the X3.4 flare using the Dopplergrams obtained by the Global Oscillation Network Group (GONG) instrument. We have also analyzed the disk-integrated velocity observations of the Sun obtained by the Global Oscillation at Low Frequency (GOLF) instrument on board the Solar and Heliospheric Observatory spacecraft as well as full-disk collapsed velocity signals from GONG observations during this flare to study any possible connection between the flare-related changes seen in the local and global velocity oscillations in the Sun. We apply wavelet transform to the time series of the localized velocity oscillations as well as the global velocity oscillations in the Sun spanning the flare event. The line-of-sight velocity shows significant enhancement in some localized regions of the penumbra of this active region during the flare. The affected region is seen to be away from the locations of the flare ribbons and the hard X-ray footpoints. The sudden enhancement of this velocity seems to be caused by the Lorentz force driven by the "magnetic jerk" in the localized penumbral region. Application of wavelet analysis to these flare-induced localized seismic signals shows significant enhancement in the high-frequency domain (5 {$<\nu$} {$<$} 8mHz) and a feeble enhancement in the p-mode oscillations (2 {$<\nu$} {$<$} 5mHz) during the flare. On the other hand, the wavelet analysis of GOLF velocity data and the full-disk collapsed GONG velocity data spanning the flare event indicates significant post-flare enhancements in the high-frequency global velocity oscillations in the Sun, as evident from the wavelet power spectrum and the corresponding scale-average variance. The present observations of the flare-induced seismic signals in the active region in context of the driving force are different as compared to previous reports on such cases. We also find indications of a connection between flare-induced localized seismic signals and the excitation of global high-frequency oscillations in the Sun. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: chromosphere,Sun: flares,Sun: oscillations,Sun: photosphere,sunspots},
  file = {/Users/lbugnet/Zotero/storage/C45V3H5I/Kumar et al. - 2011.pdf}
}

@article{Kunder2017a,
  title = {The {{Radial Velocity Experiment}} ({{Rave}}): {{Fifth Data Release}}},
  author = {Kunder, Andrea and Kordopatis, Georges and Steinmetz, Matthias and Zwitter, Toma{\v z} and McMillan, Paul J. and Casagrande, Luca and Enke, Harry and Wojno, Jennifer and Valentini, Marica and Chiappini, Cristina and Matijevi{\v c}, Gal and Siviero, Alessandro and {de Laverny}, Patrick and {Recio-Blanco}, Alejandra and Bijaoui, Albert and Wyse, Rosemary F. G. and Binney, James and Grebel, E. K. and Helmi, Amina and Jofre, Paula and Antoja, Teresa and Gilmore, Gerard and Siebert, Arnaud and Famaey, Benoit and Bienaym{\'e}, Olivier and Gibson, Brad K. and Freeman, Kenneth C. and Navarro, Julio F. and Munari, Ulisse and Seabroke, George and Anguiano, Borja and {\v Z}erjal, Maru{\v s}a and Minchev, Ivan and Reid, Warren and {Bland-Hawthorn}, Joss and Kos, Janez and Sharma, Sanjib and Watson, Fred and Parker, Quentin A. and Scholz, Ralf-Dieter and Burton, Donna and Cass, Paul and Hartley, Malcolm and Fiegert, Kristin and Stupar, Milorad and Ritter, Andreas and Hawkins, Keith and Gerhard, Ortwin and Chaplin, W. J. and Davies, G. R. and Elsworth, Y. P. and Lund, M. N. and Miglio, A. and Mosser, B.},
  year = {2017},
  journal = {The Astronomical Journal},
  volume = {153},
  number = {2},
  eprint = {1609.03210},
  pages = {75},
  issn = {0004-6256},
  doi = {10.3847/1538-3881/153/2/75},
  abstract = {Data Release 5 (DR5) of the Radial Velocity Experiment (RAVE) is the fifth data release from a magnitude-limited (9{$<$} I {$<$} 12) survey of stars randomly selected in the southern hemisphere. The RAVE medium-resolution spectra (\$R\textbackslash sim7500\$) covering the Ca-triplet region (8410-8795\textbackslash AA) span the complete time frame from the start of RAVE observations in 2003 to their completion in 2013. Radial velocities from 520,781 spectra of 457,588 unique stars are presented, of which 255,922 stellar observations have parallaxes and proper motions from the Tycho-Gaia astrometric solution (TGAS) in Gaia DR1. For our main DR5 catalog, stellar parameters (effective temperature, surface gravity, and overall metallicity) are computed using the RAVE DR4 stellar pipeline, but calibrated using recent K2 Campaign 1 seismic gravities and Gaia benchmark stars, as well as results obtained from high-resolution studies. Also included are temperatures from the Infrared Flux Method, and we provide a catalogue of red giant stars in the dereddened color \$(J-Ks)\_0\$ interval (0.50,0.85) for which the gravities were calibrated based only on seismology. Further data products for sub-samples of the RAVE stars include individual abundances for Mg, Al, Si, Ca, Ti, Fe, and Ni, and distances found using isochrones. Each RAVE spectrum is complemented by an error spectrum, which has been used to determine uncertainties on the parameters. The data can be accessed via the RAVE Web site or the Vizier database.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AYDWWACH/Kunder et al. - 2017.pdf}
}

@article{Kunitomo2017,
  title = {Astrophysics {{Revisiting}} the Pre-Main-Sequence Evolution of Stars {{I}}. {{Importance}} of Accretion Efficiency and Deuterium Abundance},
  author = {Kunitomo, Masanobu and Guillot, Tristan and Takeuchi, Taku and Ida, Shigeru},
  year = {2017},
  journal = {A\&A},
  volume = {599},
  pages = {49},
  doi = {10.1051/0004-6361/201628260},
  urldate = {2021-02-14},
  abstract = {Context. Protostars grow from the first formation of a small seed and subsequent accretion of material. Recent theoretical work has shown that the pre-main-sequence (PMS) evolution of stars is much more complex than previously envisioned. Instead of the traditional steady, one-dimensional solution, accretion may be episodic and not necessarily symmetrical, thereby affecting the energy deposited inside the star and its interior structure. Aims. Given this new framework, we want to understand what controls the evolution of accreting stars. Methods. We use the MESA stellar evolution code with various sets of conditions. In particular, we account for the (unknown) efficiency of accretion in burying gravitational energy into the protostar through a parameter, {$\xi$}, and we vary the amount of deuterium present. Results. We confirm the findings of previous works that, in terms of evolutionary tracks on an Hertzprung-Russell (H-R) diagram, the evolution changes significantly with the amount of energy that is lost during accretion. We find that deuterium burning also regulates the PMS evolution. In the low-entropy accretion scenario, the evolutionary tracks in the H-R diagram are significantly different from the classical tracks and are sensitive to the deuterium content. A comparison of theoretical evolutionary tracks and observations allows us to exclude some cold accretion models ({$\xi$} {$\sim$} 0) with low deuterium abundances. Conclusions. We confirm that the luminosity spread seen in clusters can be explained by models with a somewhat inefficient injection of accretion heat. The resulting evolutionary tracks then become sensitive to the accretion heat efficiency, initial core entropy, and deuterium content. In this context, we predict that clusters with a higher D/H ratio should have less scatter in luminosity than clusters with a smaller D/H. Future work on this issue should include radiation-hydrodynamic simulations to determine the efficiency of accretion heating and further observations to investigate the deuterium content in star-forming regions.},
  keywords = {accretion disks-stars,evolution-Hertzsprung-Russell and C-M diagrams,formation-stars,low-mass-accretion,notion,notion-database,pre-main sequence-stars,stars}
}

@article{Kunstler2015,
  title = {Spot Evolution on the Red Giant Star {{XX Triangulum}}: {{A}} Starspot-Decay Analysis Based on Time-Series {{Doppler}} Imaging},
  author = {K{\"u}nstler, A. and Carroll, T. A. and Strassmeier, K. G.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {578},
  pages = {1--25},
  issn = {14320746},
  doi = {10.1051/0004-6361/201525687},
  abstract = {Context. Solar spots appear to decay linearly proportional to their size. The decay rate of solar spots is directly related to magnetic diffusivity, which itself is a key quantity for the length of a magnetic-activity cycle. Is a linear spot decay also seen on other stars, and is this in agreement with the large range of solar and stellar activity cycle lengths? Aims. We investigate the evolution of starspots on the rapidly-rotating (Prot{$\approx$} 24 d) K0 giant XX Tri, using consecutive time-series Doppler images. Our aim is to obtain a well-sampled movie of the stellar surface over many years, and thereby detect and quantify a starspot decay law for further comparison with the Sun. Methods. We obtained continuous high-resolution and phase-resolved spectroscopy with the 1.2-m robotic STELLA telescope on Tenerife over six years, and these observations are ongoing. For each observing season, we obtained between 5 to 7 independent Doppler images, one per stellar rotation, making up a total of 36 maps. All images were reconstructed with our line-profile inversion code iMap. A wavelet analysis was implemented for denoising the line profiles. To quantify starspot area decay and growth, we match the observed images with simplified spot models based on a Monte Carlo approach. Results. It is shown that the surface of XX Tri is covered with large high-latitude and even polar spots and with occasional small equatorial spots. Just over the course of six years, we see a systematically changing spot distribution with various timescales and morphology, such as spot fragmentation and spot merging as well as spot decay and formation. An average linear decay of D = -0.022 {$\pm$} 0.002 SH/day is inferred. We found evidence of an active longitude in phase toward the (unseen) companion star. Furthermore, we detect a weak solar-like differential rotation with a surface shear of {$\alpha$} = 0.016 {$\pm$} 0.003. From the decay rate, we determine a turbulent diffusivity of {$\eta$}T = (6.3 {$\pm$} 0.5) \texttimes{} 1014 cm2/s and predict a magnetic activity cycle of {$\approx$} 26 {$\pm$} 6 yr. Finally, we present a short movie of the spatially resolved surface of XX Tri.},
  keywords = {notion,notion-database,Stars activity,Stars individual XX Tri,Stars late-type,Starspots,Techniques spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/IDJ3799Z/Künstler, Carroll, Strassmeier - 2015.pdf}
}

@article{Kurtz1982,
  title = {Rapidly Oscillating {{Ap}} Stars | {{Monthly Notices}} of the {{Royal Astronomical Society}} | {{Oxford Academic}}},
  author = {Kurtz, D.W.},
  year = {1982},
  journal = {MNRAS},
  volume = {200},
  number = {3},
  pages = {807--859},
  urldate = {2020-06-29},
  keywords = {notion,notion-database}
}

@article{Kurtz1990,
  title = {Rapidly {{Oscillating Ap Stars}}},
  author = {Kurtz, D. W.},
  year = {1990},
  month = sep,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {28},
  number = {1},
  pages = {607--655},
  publisher = {{Annual Reviews}},
  issn = {0066-4146},
  doi = {10.1146/annurev.aa.28.090190.003135},
  urldate = {2020-04-09},
  abstract = {After a discussion of the general properties of Ap stars, the paper examines HR 3831 (HD 83368) in the framework of the oblique pulsator model. Attention is also given to astroseismology in connection with HR 1217 (HD 24712); the spotted pulsator model; HD 60435 and the lifetimes of the pulsation modes in roAp stars; period changes in roAp stars; and excitation mechanisms; mode and identification; and the search for roAp stars.},
  keywords = {A Stars,Astrophysics,Magnetic Stars,Metallicity,notion,notion-database,Starquakes,Stellar Interiors,Stellar Magnetic Fields,Stellar Mass,Stellar Oscillations,Stellar Rotation}
}

@article{Kurtz2014,
  title = {Asteroseismic Measurement of Surface-to-Core Rotation in a Main-Sequence {{A}} Star, {{KIC}} 11145123},
  author = {Kurtz, Donald W and Saio, Hideyuki and Takata, Masao and Shibahashi, Hiromoto and Murphy, Simon J and Sekii, Takashi},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {444},
  pages = {102--116},
  doi = {10.1093/mnras/stu1329},
  urldate = {2020-03-10},
  abstract = {We have discovered rotationally split core g-mode triplets and surface p-mode triplets and quintuplets in a terminal age main-sequence A star, KIC 11145123, that shows both {$\delta$} Sct p-mode pulsations and {$\gamma$} Dor g-mode pulsations. This gives the first robust determination of the rotation of the deep core and surface of a main-sequence star, essentially model independently. We find its rotation to be nearly uniform with a period near 100 d, but we show with high confidence that the surface rotates slightly faster than the core. A strong angular momentum transfer mechanism must be operating to produce the nearly rigid rotation, and a mechanism other than viscosity must be operating to produce a more rapidly rotating surface than core. Our asteroseismic result, along with previous asteroseismic constraints on internal rotation in some B stars, and measurements of internal rotation in some subgiant, giant and white dwarf stars, has made angular momentum transport in stars throughout their lifetimes an observational science.},
  keywords = {asteroseismology-stars,individual,interiors-stars,KIC 11145123-stars,notion,notion-database,oscillations-stars,rotation-stars,variables,{$\delta$} Scuti}
}

@article{Kurtz2015,
  title = {A Unifying Explanation of Complex Frequency Spectra of {$\gamma$} {{Dor}}, {{SPB}} and {{Be}} Stars: {{Combination}} Frequencies and Highly Non-Sinusoidal Light Curves},
  author = {Kurtz, Donald W. and Shibahashi, Hiromoto and Murphy, Simon J. and Bedding, Timothy R. and Bowman, Dominic M.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {450},
  number = {3},
  eprint = {1504.04245},
  pages = {3015--3029},
  issn = {13652966},
  doi = {10.1093/mnras/stv868},
  abstract = {There are many Slowly Pulsating B (SPB) stars and {$\gamma$} Dor stars in the Kepler mission data set. The light curves of these pulsating stars have been classified phenomenologically into starswith symmetric light curves and with asymmetric light curves. In the same effective temperature ranges as the {$\gamma$} Dor and SPB stars, there are variable stars with downward light curves that have been conjectured to be caused by spots. Among these phenomenological classes of stars, some show 'frequency groups' in their amplitude spectra that have not previously been understood. While it has been recognized that non-linear pulsation gives rise to combination frequencies in a Fourier description of the light curves of these stars, such combination frequencies have been considered to be a only a minor constituent of the amplitude spectra. In this paper, we unify the Fourier description of the light curves of these groups of stars, showing that many of them can be understood in terms of only a few base frequencies, which we attribute to g-mode pulsations, and combination frequencies, where sometimes a very large number of combination frequencies dominate the amplitude spectra. The frequency groups seen in these stars are thus tremendously simplified. We show observationally that the combination frequencies can have amplitudes greater than the base frequency amplitudes, and we show theoretically how this arises. Thus for some {$\gamma$} Dor and SPB stars, combination frequencies can have the highest observed amplitudes. Among the B stars are pulsating Be stars that show emission lines in their spectra from occasional ejection of material into a circumstellar disc. Our analysis gives strong support to the understanding of these pulsating Be stars as rapidly rotating SPB stars, explained entirely by g-mode pulsations.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,{Stars: emission-line, be},Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VKG35U4X/Kurtz et al. - 2015.pdf}
}

@article{Kurtz2022,
  title = {Asteroseismology {{Across}} the {{Hertzsprung-Russell Diagram}}},
  author = {Kurtz, Donald W.},
  year = {2022},
  month = aug,
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {60},
  pages = {31--71},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-052920-094232},
  urldate = {2023-09-19},
  abstract = {Asteroseismology has grown from its beginnings three decades ago to a mature field teeming with discoveries and applications. This phenomenal growth has been enabled by space photometry with precision 10-100 times better than ground-based observations, with nearly continuous light curves for durations of weeks to years, and by large-scale ground-based surveys spanning years designed to detect all time-variable phenomena. The new high-precision data are full of surprises, deepening our understanding of the physics of stars. This review explores asteroseismic developments from the past decade primarily as a result of light curves from the Kepler and Transiting Exoplanet Survey Satellite space missions for massive upper main sequence OBAF stars, pre-main-sequence stars, peculiar stars, classical pulsators, white dwarfs and subdwarfs, and tidally interacting close binaries. The space missions have increased the numbers of pulsators in many classes by an order of magnitude. Asteroseismology measures fundamental stellar parameters and stellar interior physics-mass, radius, age, metallicity, luminosity, distance, magnetic fields, interior rotation, angular momentum transfer, convective overshoot, core-burning stage-supporting disparate fields such as galactic archeology, exoplanet host stars, supernovae progenitors, gamma-ray and gravitational wave precursors, close binary star origins and evolution, and standard candles. Stars are the luminous tracers of the Universe. Asteroseismology significantly improves models of stellar structure and evolution on which all inference from stars depends.},
  annotation = {ADS Bibcode: 2022ARA\&A..60...31K},
  file = {/Users/lbugnet/Zotero/storage/XVNXEP28/Kurtz - 2022 - Asteroseismology Across the Hertzsprung-Russell Di.pdf}
}

@article{Kuszlewicz2018,
  title = {Bayesian Hierarchical Inference of Asteroseismic Inclination Angles},
  author = {Kuszlewicz, James S and Chaplin, William J and North, Thomas S H and Farr, Will M and Bell, Keaton J and Davies, Guy R and Campante, Tiago L and Hekker, Saskia},
  year = {2019},
  journal = {MNRAS},
  volume = {488},
  pages = {572--589},
  doi = {10.1093/mnras/stz1689},
  urldate = {2021-09-03},
  abstract = {The stellar inclination angle-the angle between the rotation axis of a star and our line of sight-provides valuable information in many different areas, from the characterization of the geometry of exoplanetary and eclipsing binary systems to the formation and evolution of those systems. We propose a method based on asteroseismology and a Bayesian hierarchical scheme for extracting the inclination angle of a single star. This hierarchical method therefore provides a means to both accurately and robustly extract inclination angles from red giant stars. We successfully apply this technique to an artificial data set with an underlying isotropic inclination angle distribution to verify the method. We also apply this technique to 123 red giant stars observed with Kepler. We also show the need for a selection function to account for possible population-level biases, which are not present in individual star-by-star cases, in order to extend the hierarchical method towards inferring underlying population inclination angle distributions.},
  keywords = {asteroseismology-methods,data analysis-methods,notion,notion-database,statistical}
}

@article{Kuszlewicz2020,
  title = {Clumpiness: Time-Domain Classification of Red Giant Evolutionary States},
  author = {Kuszlewicz, James S and Hekker, Saskia and Bell, Keaton J},
  year = {2020},
  journal = {MNRAS},
  volume = {497},
  pages = {4843--4856},
  doi = {10.1093/mnras/staa2155},
  urldate = {2022-01-08},
  abstract = {Long, high-quality time-series data provided by previous space missions such as CoRoT and Kepler have made it possible to derive the evolutionary state of red giant stars, i.e. whether the stars are hydrogen-shell burning around an inert helium core or helium-core burning, from their individual oscillation modes. We utilize data from the Kepler mission to develop a tool to classify the evolutionary state for the large number of stars being observed in the current era of K2, TESS, and for the future PLATO mission. These missions provide new challenges for evolutionary state classification given the large number of stars being observed and the shorter observing duration of the data. We propose a new method, Clumpiness, based upon a supervised classification scheme that uses 'summary statistics' of the time series, combined with distance information from the Gaia mission to predict the evolutionary state. Applying this to red giants in the APOKASC catalogue, we obtain a classification accuracy of {$\sim$} 91 per cent for the full 4 yr of Kepler data, for those stars that are either only hydrogen-shell burning or also helium-core burning. We also applied the method to shorter Kepler data sets, mimicking CoRoT, K2, and TESS achieving an accuracy {$>$} 91 per cent even for the 27 d time series. This work paves the way towards fast, reliable classification of vast amounts of relatively short-time-span data with a few, well-engineered features.},
  keywords = {asteroseismology-methods,data analysis-methods,notion,notion-database,statistical}
}

@misc{Kuszlewicz2023,
  title = {Mixed-Mode {{Ensemble Asteroseismology}} of {{Low-Luminosity Kepler Red Giants}}},
  author = {Kuszlewicz, James S. and Hon, Marc and Huber, Daniel},
  year = {2023},
  month = jul,
  journal = {arXiv e-prints},
  doi = {10.48550/arXiv.2307.06482},
  urldate = {2023-07-27},
  abstract = {We present measurements of the dipole mode asymptotic period spacing (\$\textbackslash Delta\textbackslash Pi\_1\$), the coupling factor between p- and g- modes (\$q\$), the g-mode phase offset (\$\textbackslash epsilon\_g\$), and the mixed-mode frequency rotational splitting (\$\textbackslash delta\textbackslash nu\_\{\textbackslash mathrm\{rot\}\}\$) for 1,074 low-luminosity red giants from the Kepler mission. Using oscillation mode frequencies extracted from each star, we apply Bayesian optimization to estimate \$\textbackslash Delta\textbackslash Pi\_1\$ from the power spectrum of the stretched period spectrum and to perform the subsequent forward modelling of the mixed-mode frequencies. With our measurements, we show that the mode coupling factor \$q\$ shows significant anti-correlation with both stellar mass and metallicity, and can reveal highly metal-poor stars. We present the evolution of \$\textbackslash epsilon\_g\$ up the lower giant branch up to before the luminosity bump, and find no significant trends in \$\textbackslash epsilon\_g\$ or \$\textbackslash delta\textbackslash nu\_\{\textbackslash mathrm\{rot\}\}\$ with stellar mass and metallicity in our sample. Additionally, we identify six new red giants showing anomalous distortions in their g-mode pattern. Our data products, code, and results are provided in a public repository.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2023arXiv230706482K},
  file = {/Users/lbugnet/Zotero/storage/BK896FS2/Kuszlewicz et al. - 2023 - Mixed-mode Ensemble Asteroseismology of Low-Lumino.pdf}
}

@article{Kuzuhara2013a,
  title = {Direct Imaging of a Cold Jovian Exoplanet in Orbit around the Sun-like Star {{GJ}} 504},
  author = {Kuzuhara, M. and Tamura, M. and Kudo, T. and Janson, M. and Kandori, R. and Brandt, T. D. and Thalmann, C. and Spiegel, D. and Biller, B. and Carson, J. and Hori, Y. and Suzuki, R. and Burrows, A. and Henning, T. and Turner, E. L. and McElwain, M. W. and {Moro-Mart{\'i}n}, A. and Suenaga, T. and Takahashi, Y. H. and Kwon, J. and Lucas, P. and Abe, L. and Brandner, W. and Egner, S. and Feldt, M. and Fujiwara, H. and Goto, M. and Grady, C. A. and Guyon, O. and Hashimoto, J. and Hayano, Y. and Hayashi, M. and Hayashi, S. S. and Hodapp, K. W. and Ishii, M. and Iye, M. and Knapp, G. R. and Matsuo, T. and Mayama, S. and Miyama, S. and Morino, J. I. and Nishikawa, J. and Nishimura, T. and Kotani, T. and Kusakabe, N. and Pyo, T. S. and Serabyn, E. and Suto, H. and Takami, M. and Takato, N. and Terada, H. and Tomono, D. and Watanabe, M. and Wisniewski, J. P. and Yamada, T. and Takami, H. and Usuda, T.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {774},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/774/1/11},
  abstract = {Several exoplanets have recently been imaged at wide separations of {$>$}10 AU from their parent stars. These span a limited range of ages ({$<$}50 Myr) and atmospheric properties, with temperatures of 800-1800 K and very red colors (J-H {$>$} 0.5 mag), implying thick cloud covers. Furthermore, substantial model uncertainties exist at these young ages due to the unknown initial conditions at formation, which can lead to an order of magnitude of uncertainty in the modeled planet mass. Here, we report the direct-imaging discovery of a Jovian exoplanet around the Sun-like star GJ 504, detected as part of the SEEDS survey. The system is older than all other known directly imaged planets; as a result, its estimated mass remains in the planetary regime independent of uncertainties related to choices of initial conditions in the exoplanet modeling. Using the most common exoplanet cooling model, and given the system age of 160 Myr, GJ 504b has an estimated mass of 4 Jupiter masses, among the lowest of directly imaged planets. Its projected separation of 43.5 AU exceeds the typical outer boundary of {$\sim$}30 AU predicted for the core accretion mechanism. GJ 504b is also significantly cooler (510 K) and has a bluer color (J-H = -0.23 mag) than previously imaged exoplanets, suggesting a largely cloud-free atmosphere accessible to spectroscopic characterization. Thus, it has the potential of providing novel insights into the origins of giant planets as well as their atmospheric properties. \textcopyright{} 2013. The American Astronomical Society. All rights reserved..},
  keywords = {notion,notion-database,planetary systems,stars: formation,stars: individual (GJ 504)},
  file = {/Users/lbugnet/Zotero/storage/H3AEQU75/Kuzuhara et al. - 2013.pdf}
}

@article{Lagarde2015,
  title = {Astrophysics {{Models}} of Red Giants in the {{CoRoT}} Asteroseismology Fields Combining Asteroseismic and Spectroscopic Constraints},
  author = {Lagarde, N and Miglio, A and Eggenberger, P and Morel, T and Montalb{\'a}n, J and Mosser, B and Rodrigues, T S and Girardi, L and Rainer, M and Poretti, E and Barban, C and Hekker, S and Kallinger, T and Valentini, M and Carrier, F and Hareter, M and Mantegazza, L and Elsworth, Y and Michel, E and Baglin, A},
  year = {2015},
  journal = {A\&A},
  volume = {580},
  pages = {141},
  doi = {10.1051/0004-6361/201525856},
  urldate = {2021-03-15},
  abstract = {Context. The availability of asteroseismic constraints for a large sample of red giant stars from the CoRoT and Kepler missions paves the way for various statistical studies of the seismic properties of stellar populations. Aims. We use a detailed spectroscopic study of 19 CoRoT red giant stars to compare theoretical stellar evolution models to observations of the open cluster NGC 6633 and field stars. Methods. In order to explore the effects of rotation-induced mixing and thermohaline instability, we compare surface abundances of carbon isotopic ratio and lithium with stellar evolution predictions. These chemicals are sensitive to extra-mixing on the red giant branch. Results. We estimate mass, radius, and distance for each star using the seismic constraints. We note that the Hipparcos and seismic distances are different. However, the uncertainties are such that this may not be significant. Although the seismic distances for the cluster members are self consistent they are somewhat larger than the Hipparcos distance. This is an issue that should be considered elsewhere. Models including thermohaline instability and rotation-induced mixing, together with the seismically determined masses can explain the chemical properties of red giant targets. However, with this sample of stars we cannot perform stringent tests of the current stellar models. Tighter constraints on the physics of the models would require the measurement of the core and surface rotation rates, and of the period spacing of gravity-dominated mixed modes. A larger number of stars with longer times series, as provided by Kepler or expected with Plato, would help ensemble asteroseismology.},
  keywords = {abundances-stars,asteroseismology-stars,evolution-stars,interiors,notion,notion-database,rotation-stars}
}

@article{Lagarde2016,
  title = {Testing the Cores of First Ascent Red Giant Stars Using the Period Spacing of g Modes},
  author = {Lagarde, N. and Bossini, D. and Miglio, A. and Vrard, M. and Mosser, B.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {457},
  number = {1},
  eprint = {1512.03656},
  pages = {L59-L63},
  issn = {17453933},
  doi = {10.1093/mnrasl/slv201},
  abstract = {In the context of the determination of stellar properties using asteroseismology, we study the influence of rotation and convective-core overshooting on the properties of red giant stars. We used models in order to investigate the effects of these mechanisms on the asymptotic period spacing of gravity modes ({$\Delta\Pi$}1) of red-giant stars that ignite He burning in degenerate conditions (M {$\leq$} 2.0 M{$\odot$}). We also compare the predictions of these models with Kepler observations. For a given {$\Delta$}v, {$\Delta\Pi$}1 depends not only on the stellar mass, but also on mixing processes that can affect the structure of the core. We find that in the case of more evolved red-giant-branch stars and regardless of the transport processes occurring in their interiors, the observed {$\Delta\Pi$}1 can provide information as to their stellar luminosity, within \textasciitilde 10-20 per cent. In general, the trends of {$\Delta\Pi$}1 with respect to mass and metallicity that are observed in Kepler red-giant stars are well reproduced by the models.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: interiors,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/SRYGULGS/Lagarde et al. - 2016.pdf}
}

@article{Lagarde2017,
  title = {Population Synthesis to Constrain {{Galactic}} and Stellar Physics: {{I}}. {{Determining}} Age and Mass of Thin-Disc Red-Giant Stars},
  author = {Lagarde, N. and Robin, A. C. and Reyl{\'e}, C. and Nasello, G.},
  year = {2017},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {601},
  eprint = {1702.01769},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201630253},
  urldate = {2020-07-03},
  abstract = {Context. The cornerstone mission of the European Space Agency, Gaia, together with forthcoming complementary surveys (CoRoT, Kepler, K2, APOGEE, and Gaia-ESO), will revolutionize our understanding of the formation and history of our Galaxy, providing accurate stellar masses, radii, ages, distances, as well as chemical properties for a very large sample of stars across different Galactic stellar populations. Aims. Using an improved population synthesis approach and new stellar evolution models we attempt to evaluate the possibility of deriving ages and masses of clump stars from their chemical properties. Methods. A new version of the Besan\c{c}on Galaxy models (BGM) is used in which new stellar evolutionary tracks are computed from the stellar evolution code STAREVOL. These provide global, chemical, and seismic properties of stars from the pre-main sequence to the early-AGB. For the first time, the BGM can explore the effects of an extra-mixing occurring in red-giant stars. In particular we focus on the effects of thermohaline instability on chemical properties as well as on the determination of stellar ages and masses using the surface [C/N] abundance ratio. Results. The impact of extra-mixing on 3He, 12C/13C, nitrogen, and [C/N] abundances along the giant branch is quantified. We underline the crucial contribution of asteroseismology to discriminate between evolutionary states of field giants belonging to the Galactic disc. The inclusion of thermohaline instability has a significant impact on 12C/13C, 3He as well as on the [C/N] values. We clearly show the efficiency of thermohaline mixing at different metallicities and its influence on the determined stellar mass and age from the observed [C/N] ratio. We then propose simple relations to determine ages and masses from chemical abundances according to these models. Conclusions. We emphasize the usefulness of population synthesis tools to test stellar models and transport processes inside stars. We show that transport processes occurring in red-giant stars should be taken into account in the determination of ages for future Galactic archaeology studies.},
  archiveprefix = {arxiv},
  keywords = {abundances,Asteroseismology,evolution,Galaxy,notion,notion-database,Stars,stellar content},
  file = {/Users/lbugnet/Zotero/storage/IHI23Q7E/full-text.pdf}
}

@book{Lamb1932,
  title = {Hydrodynamics},
  author = {Lamb, H.},
  year = {1932},
  urldate = {2020-06-26},
  keywords = {notion,notion-database}
}

@article{Lambert2006a,
  title = {Curvelet Analysis of Asteroseismic Data},
  author = {Lambert, P. and Pires, S. and Ballot, J. and Garc{\'i}a, R. A. and Starck, J.-L. and {Turck-Chi{\`e}ze}, S.},
  year = {2006},
  journal = {Astronomy \& Astrophysics},
  volume = {454},
  number = {3},
  pages = {1021--1027},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20054541},
  abstract = {\emph{Context.{$<$}i/{$>$}The detection and identification of oscillation modes (in terms of their~,~\emph{m{$<$}i/{$>$}, and successive~\emph{n{$<$}i/{$>$}) is a great challenge for present and future asteroseismic space missions. ``Peak tagging" is an important step in the analysis of these data to provide estimations of stellar oscillation mode parameters, i.e., frequencies, rotation rates, and further studies on the stellar structure. \emph{Aims.{$<$}i/{$>$}Our goal is to increase the signal-to-noise ratio of the asteroseismic spectra computed from the time series that are representative of MOST and CoRoT observations (30- and 150-day observations). \emph{Methods.{$<$}i/{$>$}We apply the curvelet transform \textendash{} a recent image processing technique that looks for curved patterns \textendash{} to echelle diagrams built using asteroseismic power spectra. In the resulting diagram, the eigenfrequencies appear as smooth continuous ridges. To test the method, we use Monte-Carlo simulations of several sun-like stars with different combinations of rotation rates, rotation-axis inclination, and signal-to-noise ratios. \emph{Results.{$<$}i/{$>$}The filtered diagrams enhance the contrast between the ridges of the modes and the background, allowing a better tagging of the modes and a better extraction of some stellar parameters. Monte-Carlo simulations have also shown that the region where modes can be detected is enlarged at lower and higher frequencies compared to the raw spectra. In addition, the extraction of the mean rotational splitting from modes at low frequency can be done more easily using the filtered spectra rather than the raw spectra.}}}}}}},
  keywords = {data analysis,image processing,methods,notion,notion-database,oscillations,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/62CPPYSY/Lambert et al. - 2006.pdf}
}

@article{Landstreet1992,
  title = {Magnetic Fields at the Surfaces of Stars},
  author = {Landstreet, J. D.},
  year = {1992},
  month = mar,
  journal = {The Astronomy and Astrophysics Review},
  volume = {4},
  number = {1},
  pages = {35--77},
  publisher = {{Springer-Verlag}},
  issn = {09354956},
  doi = {10.1007/BF00873569},
  urldate = {2020-06-18},
  abstract = {Magnetic fields have now been detected in stars in several parts of the Hertzsprung-Russell diagram. Roughly dipolar fields ranging in strength between 3\texttimes{} 102 and 3\texttimes 104 G are found in many chemically peculiar A and B main sequence stars. Dipolar fields are also found in some 2-3\% of white dwarfs, but with strengths between 1\texttimes 106 and 5\texttimes 108 G. In both these types of stars, the observed fields vary as the underlying star turns, but do not change in a secular manner. In solartype stars, structurally complex fields of a few kG are found with filling factors of the order of 0.1 to 0.8. Further indirect evidence of fields in cool main sequence stars is provided by detection of visible and ultraviolet line emission (chromospheric activity), x radiation (coronal matter), and giant starspots. In this review, we survey the observations of stellar magnetism in all these types of stars, as well as efforts to model the observed magnetic fields and associated photospheric peculiarities and activity. \textcopyright{} 1992 Springer-Verlag.},
  keywords = {activity of - Stars,magnetic field - Stars,Magnetic field - Stars,notion,notion-database,peculiar A - Stars,white dwarf}
}

@article{Landstreet2000,
  title = {Magnetic Models of Slowly Rotating Magnetic {{Ap}} Stars: Aligned Magnetic and Rotation Axes},
  author = {Landstreet, J. D. and Mathys, G.},
  year = {2000},
  journal = {A\&A},
  volume = {359},
  pages = {213--226},
  issn = {0004-6361},
  urldate = {2022-01-07},
  keywords = {notion,notion-database,STARS: CHEMICALLY PECULIAR,STARS: FUNDAMENTAL PARAMETERS,STARS: MAGNETIC FIELDS,STARS: STATISTICS}
}

@inproceedings{Landstreet2009,
  title = {Evolution of {{Global Magnetic Fields}} in {{Main Sequence A}} and {{B Stars}}},
  booktitle = {In {{Honor}} of {{Jan Stenflo ASP Conference Series}}},
  author = {Landstreet, J. D. and Bagnulo, S. and Andretta, V. and Fossati, L. and Mason, E. and Silaj, J. and Wade, G. A.},
  year = {2009},
  volume = {405},
  pages = {505},
  issn = {1050-3390},
  urldate = {2020-11-29},
  keywords = {notion,notion-database}
}

@article{Lanza2008,
  title = {Magnetic Activity in the Photosphere of {{CoRoT-Exo-2a}}. {{Active}} Longitudes and Short-Term Spot Cycle in a Young {{Sun-like}} Star},
  author = {Lanza, A. F. and Pagano, I. and Leto, G. and Messina, S. and Aigrain, S. and Alonso, R. and Auvergne, M. and Baglin, A. and Barge, P. and Bonomo, A. S. and Boumier, P. and Cameron, A. Collier and Comparato, M. and Cutispoto, G. and De Medeiros, J. R. and Foing, B. and Kaiser, A. and Moutou, C. and Parihar, P. S. and Silva, A. V. R. and Weiss, W. W.},
  year = {2008},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {493},
  number = {1},
  eprint = {0811.0461},
  pages = {193--200},
  doi = {10.1051/0004-6361:200810591},
  urldate = {2020-07-04},
  abstract = {The space experiment CoRoT has recently detected transits by a hot Jupiter across the disc of an active G7V star (CoRoT-Exo-2a) that can be considered as a good proxy for the Sun at an age of approximately 0.5 Gyr. We present a spot modelling of the optical variability of the star during 142 days of uninterrupted observations performed by CoRoT with unprecedented photometric precision. We apply spot modelling approaches previously tested in the case of the Sun by modelling total solar irradiance variations. To model the light curve of CoRoT-Exo-2a, we take into account both the photometric effects of cool spots as well as those of solar-like faculae, adopting solar analogy. Two active longitudes initially on opposite hemispheres are found on the photosphere of CoRoT-Exo-2a with a rotation period of 4.522 \$\textbackslash pm\$ 0.024 days. Their separation changes by approximately 80 degrees during the time span of the observations. From this variation, a relative amplitude of the surface differential rotation lower than about 1 percent is estimated. Individual spots form within the active longitudes and show an angular velocity about 1 percent smaller than that of the longitude pattern. The total spotted area shows a cyclic oscillation with a period of 28.9 \$\textbackslash pm\$ 4.3 days, which is close to 10 times the synodic period of the planet as seen by the rotating active longitudes. The implications of such results for the internal rotation of CoRoT-Exo-2a are discussed on the basis of solar analogy. A possible magnetic star-planet interaction is suggested by the cyclic variation of the spotted area. Alternatively, the 28.9-d cycle may be related to Rossby-type waves propagating in the subphotospheric layers of the star.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: activity,Stars: individual: CoRoT-Exo-2a,Stars: late-type,Stars: magnetic fields,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/9EX7ZYQX/full-text.pdf}
}

@article{Lanza2009a,
  title = {Stellar Magnetic Cycles},
  author = {Lanza, A. F.},
  year = {2009},
  journal = {Proceedings of the International Astronomical Union},
  volume = {5},
  number = {S264},
  pages = {120--129},
  issn = {1743-9213},
  doi = {10.1017/s1743921309992523},
  abstract = {The solar activity cycle is a manifestation of the hydromagnetic dynamo working inside our star. The detection of activity cycles in solar-like stars and the study of their properties allow us to put the solar dynamo in perspective, investigating how dynamo action depends on stellar parameters and stellar structure. Nevertheless, the lack of spatial resolution and the limited time extension of stellar data pose limitations to our understanding of stellar cycles and the possibility to constrain dynamo models. I briefly review some results obtained from disc-integrated proxies of stellar magnetic fields and discuss the new opportunities opened by space-borne photometry made available by MOST, CoRoT, Kepler, and GAIA, and by new ground-based spectroscopic or spectropolarimetric observations. Stellar cycles have a significant impact on the energetic output and circumstellar magnetic fields of late-type active stars which affects the interaction between stars and their planets. On the other hand, a close-in massive planet could affect the activity of its host star. Recent observations provide circumstantial evidence of such an interaction with possible consequences for stellar activity cycles.},
  keywords = {activity,late-type,magnetic fields,notion,notion-database,planetary,stars,sun},
  file = {/Users/lbugnet/Zotero/storage/XP2PBSSD/Lanza - 2009.pdf}
}

@article{Lanza2010,
  title = {Photospheric Activity, Rotation, and Radial Velocity Variations of the Planet-Hosting Star {{CoRoT-7}}},
  author = {Lanza, A. F. and Bonomo, A. S. and Moutou, C. and Pagano, I. and Messina, S. and Leto, G. and Cutispoto, G. and Aigrain, S. and Alonso, R. and Barge, P. and Deleuil, M. and Auvergne, M. and Baglin, A. and Collier Cameron, A.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {520},
  number = {9},
  eprint = {1005.3602},
  pages = {1--13},
  issn = {14320746},
  doi = {10.1051/0004-6361/201014403},
  abstract = {Context. The CoRoT satellite has recently discovered the transits of an Earth-like planet across the disc of a late-type magnetically active star dubbed CoRoT-7, while a second planet was detected after filtering out the radial velocity (hereafter RV) variations due to stellar activity. Aims. We investigate the magnetic activity of CoRoT-7 and use the results for a better understanding of the impact of magnetic activity on stellar RV variations. Methods. We derived the longitudinal distribution of active regions on CoRoT-7 from a maximum entropy spot model of the CoRoT lightcurve. Assuming that each active region consists of dark spots and bright faculae in a fixed proportion, we synthesized the expected RV variations. Results. Active regions are mainly located at three active longitudes that appear to migrate at different rates, probably as a consequence of surface differential rotation, for which a lower limit of {$\Delta\Omega$}/{$\Omega$} = 0.058 {$\pm$} 0.017 is found. The synthesized activity-induced RV variations reproduce the amplitude of the observed RV curve and are used to study the impact of stellar activity on planetary detection. Conclusions. In spite of the non-simultaneous CoRoT and HARPS observations, our study confirms the validity of the method previously adopted to filter out RV variations induced by stellar activity. We find a false-alarm probability {$<$}10-4 that the RV oscillations attributed to CoRoT-7b and CoRoT-7c are spurious effects of noise and activity. Additionally, our model suggests that other periodicities found in the observed RV curve of CoRoT-7 could be explained by active regions whose visibility is modulated by a differential stellar rotation with periods ranging from 23.6 to 27.6 days. \textcopyright{} 2010 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,planetary systems,stars: activity,stars: individual: CoRoT-7,stars: late-type,stars: magnetic field,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/8KZRY8EG/Lanza et al. - 2010.pdf}
}

@article{Lanza2013a,
  title = {Current State of the Modelling of Photospheric Activity},
  author = {Lanza, A. F.},
  year = {2013},
  journal = {Astrophysics and Space Science Proceedings},
  volume = {31},
  number = {2013},
  pages = {215--220},
  issn = {15706605},
  doi = {10.1007/978-3-642-29630-7_40},
  abstract = {I briefly review the current state of the modelling of photospheric activity based on the high-precision optical light curves obtained with MOST, CoRoT, and Kepler. These models can be used to search for active longitudes where activity is preferentially concentrated, estimate the amplitude of stellar differential rotation, and look for short-term activity cycles as, e.g., in the case of CoRoT-2. In the case of a late-type star accompanied by a transiting hot Jupiter, the small light modulations observed during transits when a dark spot is occulted by the disc of the planet are also briefly considered. They can be used to derive information on individual active regions as well as on stellar rotation and the spin\textendash orbit alignment of the system.},
  isbn = {9783642296291},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NWGLJXSI/Lanza - 2013.pdf}
}

@article{Lanza2014a,
  title = {Measuring Stellar Differential Rotation with High-Precision Space-Borne Photometry},
  author = {Lanza, A. F. and Das Chagas, M. L. and De Medeiros, J. R.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {564},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201323172},
  abstract = {Context. Stellar differential rotation is important for understanding hydromagnetic stellar dynamos, instabilities, and transport processes in stellar interiors, as well as for a better treatment of tides in close binary and star-planet systems. Aims. We introduce a method of measuring a lower limit to the amplitude of surface differential rotation from high-precision, evenly sampled photometric time series, such as those obtained by space-borne telescopes. It is designed to be applied to main-sequence late-type stars whose optical flux modulation is dominated by starspots. Methods. An autocorrelation of the time series was used to select stars that allow an accurate determination of starspot rotation periods. A simple two-spot model was applied together with a Bayesian information criterion to preliminarily select intervals of the time series showing evidence of differential rotation with starspots of almost constant area. Finally, the significance of the differential rotation detection and a measurement of its amplitude and uncertainty were obtained by an a posteriori Bayesian analysis based on a Monte Carlo Markov chain approach. We applied our method to the Sun and eight other stars for which previous spot modelling had been performed to compare our results with previous ones. Results. We find that autocorrelation is a simple method for selecting stars with a coherent rotational signal that is a prerequisite for successfully measuring differential rotation through spot modelling. For a proper Monte Carlo Markov chain analysis, it is necessary to take the strong correlations among different parameters that exist in spot modelling into account. For the planet-hosting star Kepler-30, we derive a lower limit to the relative amplitude of the differential rotation of {$\Delta$}P/P = 0.0523 {$\pm$} 0.0016. We confirm that the Sun as a star in the optical passband is not suitable for measuring differential rotation owing to the rapid evolution of its photospheric active regions. In general, our method performs well in comparison to more sophisticated and time-consuming approaches. \textcopyright{} 2014 ESO.},
  keywords = {notion,notion-database,Stars: late-type,Stars: rotation,Starspots,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/HWLVK4JW/Lanza, Das Chagas, De Medeiros - 2014.pdf}
}

@article{Lanzafame2015,
  title = {Rotational Evolution of Slow-Rotator Sequence Stars},
  author = {Lanzafame, A. C. and Spada, F.},
  year = {2015},
  month = dec,
  journal = {Astronomy \& Astrophysics},
  volume = {584},
  pages = {A30},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201526770},
  urldate = {2023-10-28},
  abstract = {Context. The observed relationship between mass, age and rotation in open clusters shows the progressive development of a slow-rotator sequence among stars possessing a radiative interior and a convective envelope during their pre-main sequence and main-sequence evolution. After 0.6 Gyr, most cluster members of this type have settled on this sequence. Aims: The observed clustering on this sequence suggests that it corresponds to some equilibrium or asymptotic condition that still lacks a complete theoretical interpretation, and which is crucial to our understanding of the stellar angular momentum evolution. Methods: We couple a rotational evolution model, which takes internal differential rotation into account, with classical and new proposals for the wind braking law, and fit models to the data using a Monte Carlo Markov chain (MCMC) method tailored to the problem at hand. We explore to what extent these models are able to reproduce the mass and time dependence of the stellar rotational evolution on the slow-rotator sequence. Results: The description of the evolution of the slow-rotator sequence requires taking the transfer of angular momentum from the radiative core to the convective envelope into account. We find that, in the mass range 0.85-1.10 M{$\odot$}, the core-envelope coupling timescale for stars in the slow-rotator sequence scales as M-7.28. Quasi-solid body rotation is achieved only after 1-2 Gyr, depending on stellar mass, which implies that observing small deviations from the Skumanich law (P {$\propto$} {$\surd\lbrace$}t\vphantom\{\}) would require period data of older open clusters than is available to date. The observed evolution in the 0.1-2.5 Gyr age range and in the 0.85-1.10 M{$\odot$} mass range is best reproduced by assuming an empirical mass dependence of the wind angular momentum loss proportional to the convective turnover timescale and to the stellar moment of inertia. Period isochrones based on our MCMC fit provide a tool for inferring stellar ages of solar-like main-sequence stars from their mass and rotation period that is largely independent of the wind braking model adopted. These effectively represent gyro-chronology relationships that take the physics of the two-zone model for the stellar angular momentum evolution into account.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,open clusters and associations: general,stars: evolution,stars: late-type,stars: rotation},
  annotation = {ADS Bibcode: 2015A\&A...584A..30L},
  file = {/Users/lbugnet/Zotero/storage/M3HZQYA8/Lanzafame and Spada - 2015 - Rotational evolution of slow-rotator sequence star.pdf}
}

@article{Lanzafame2018,
  title = {Gaia {{Data Release}} 2: {{Rotational}} Modulation in Late-Type Dwarfs},
  author = {Lanzafame, A. C. and Distefano, E. and Messina, S. and Pagano, I. and Lanza, A. F. and Eyer, L. and Guy, L. P. and Rimoldini, L. and {Lecoeur-Taibi}, I. and Holl, B. and Audard, M. and De Fombelle, G. J. and Nienartowicz, K. and Marchal, O. and Mowlavi, N.},
  year = {2018},
  month = aug,
  journal = {Astronomy \& Astrophysics},
  volume = {616},
  eprint = {1805.00421},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201833334},
  urldate = {2020-07-02},
  abstract = {Context. Amongst the 5 \texttimes{} 105 sources identified as variable stars in Gaia Data Release 2 (DR2), 26\% are rotational modulation variable candidates of the BY Dra class. Gaia DR2 provides their multi-band (G, GBP, and GRP) photometric time series collected by the European Space Agency spacecraft Gaia during the first 22 months of operations as well as the essential parameters related to their flux modulation induced by surface inhomogeneities and rotation. Aims. We developed methods to identify the BY Dra variable candidates and to infer their variability parameters. Methods. BY Dra candidates were pre-selected from their position in the Hertzsprung-Russel diagram, built from Gaia parallaxes, G magnitudes, and (GBP-GRP) colours. Since the time evolution of the stellar active region can disrupt the coherence of the signal, segments not much longer than their expected evolution timescale were extracted from the entire photometric time series, and period search algorithms were applied to each segment. For the Gaia DR2, we selected sources with similar periods in at least two segments as candidate BY Dra variables. Results were further filtered considering the time-series phase coverage and the expected approximate light-curve shape. Results. Gaia DR2 includes rotational periods and modulation amplitudes of 147 535 BY Dra candidates. The data unveil the existence of two populations with distinctive period and amplitude distributions. The sample covers 38\% of the whole sky when divided into bins (HEALPix) of 0.84 square degrees, and we estimate that this represents 0.7-5\% of all BY Dra stars potentially detectable with Gaia. Conclusions. The preliminary data contained in Gaia DR2 illustrate the vast and unique information that the mission is going to provide on stellar rotation and magnetic activity. This information, complemented by the exquisite Gaia parallaxes, proper motions, and astrophysical parameters, is opening new and unique perspectives for our understanding of the evolution of stellar angular momentum and dynamo action.},
  archiveprefix = {arxiv},
  keywords = {Catalogs,Galaxy: stellar content,notion,notion-database,Stars: magnetic field,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/Q3U7246W/full-text.pdf}
}

@article{Larson1978,
  title = {Star Formation Rates in Normal and Peculiar Galaxies},
  author = {Larson, R. B. and Tinsley, B. M.},
  year = {1978},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {219},
  pages = {46},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/155753},
  urldate = {2020-03-07},
  abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein-protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-{$\alpha$}-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD {$\leq$} 2.0 \AA{} for the interface backbone atoms) increased from 21\% with default Glide SP settings to 58\% with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63\% success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40\% of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
  keywords = {Astronomical Models,Astrophysics,Galactic Structure,Galaxies:Star Formation,Gravitational Effects,notion,notion-database,Peculiar Galaxies,Star Distribution,Star Formation,Star Formation Rate,Tides,Ubv Spectra}
}

@article{Laskar2012a,
  title = {Tidal Dissipation in Multi-Planet Systems and Constraints on Orbit Fitting},
  author = {Laskar, J. and Bou{\'e}, G. and Correia, A. C.M.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {538},
  pages = {1--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116643},
  abstract = {We present here in full detail the linear secular theory with tidal damping that was used to constrain the fit to the HD 10180 planetary system in Lovis et al. (2011, A\&A, 528, A112). The theory is very general and can provide some intuitive understanding of the final state of a planetary system when one or more planets are close to their central star. We globally recover the results of Mardling (2007, MNRAS, 382, 1768). However, for the HD 209458 planetary system, we show that the consideration of the tides raised by the central star on the planet leads one to believe that the eccentricity of HD 209458b is most probably much smaller than 0.01. \textcopyright{} 2012 ESO.},
  keywords = {celestial mechanics,methods: analytical,notion,notion-database,planets and satellites: general},
  file = {/Users/lbugnet/Zotero/storage/RMXERX9N/Laskar, Boué, Correia - 2012.pdf}
}

@article{Lasky2012a,
  title = {Gravitational {{Waves}} and {{Hydromagnetic Instabilities}} in {{Rotating Magnetized Neutron Stars}}},
  author = {Lasky, Paul D and Zink, Burkhard and Kokkotas, Kostas D},
  year = {2012},
  eprint = {1203.3590v1},
  abstract = {We perform nonlinear general relativistic ideal magnetohydrodynamic simulations of poloidal magnetic fields in rotating polytropic neutron stars. We have three primary goals: i) to understand the nature of magnetohydrodynamic instabilities inherent to poloidal magnetic fields in non-rotating and rotating neutron stars, ii) to explore the possible space of stable equilibrium configurations and iii) to understand gravitational wave emissions caused by the catastrophic reconfiguration of magnetic fields associated with giant magnetar flares. Our key physical contributions can be summarized as follows: i) gravitational waves from f-modes caused by magnetar flares are unlikely to be detected in the current or near-future generation of gravitational waves observatories, ii) gravitational waves from Alfven waves propagating inside the neutron star are more likely candidates, although this interpretation relies on the unknown damping time of these modes, iii) any magnetic field equilibria derived from our simulations are characterized as non-axisymmetric, with approximately 65\% of their magnetic energy in the poloidal field, iv) rotation acts to separate the timescales of different instabilities in our system, with the varicose mode playing a more major role due to a delayed kink instability and v) despite the slowing growth rate of the kink mode, it is always present in our simulations, even for models where the rotational period is of the same order as the Alfven timescale.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2CIDXNJM/Lasky, Zink, Kokkotas - 2012.pdf}
}

@article{Lasky2013a,
  title = {Tilted Torus Magnetic Fields in Neutron Stars and Their Gravitational Wave Signatures},
  author = {Lasky, Paul D. and Melatos, Andrew},
  year = {2013},
  journal = {Physical Review D - Particles, Fields, Gravitation and Cosmology},
  volume = {88},
  number = {10},
  eprint = {1310.7633},
  issn = {15507998},
  doi = {10.1103/PhysRevD.88.103005},
  abstract = {Gravitational-wave diagnostics are developed for discriminating between varieties of mixed poloidal-toroidal magnetic fields in neutron stars, with particular emphasis on differentially rotating protoneutron stars. It is shown that tilted torus magnetic fields, defined as the sum of an internal/external poloidal component, whose axis of symmetry is tilted with respect to the rotation axis, and an internal toroidal component, whose axis of symmetry is aligned with the rotation axis, deform the star triaxially, unlike twisted torus fields, which deform the star biaxially. Utilizing an analytic tilted torus example, we show that these two topologies can be distinguished by their gravitational wave spectrum and polarization phase portraits. For example, the relative amplitudes and frequencies of the spectral peaks allow one to infer the relative strengths of the toroidal and poloidal components of the field, and the magnetic inclination angle. Finally, we show how a tilted torus field arises naturally from magnetohydrodynamic simulations of differentially rotating neutron stars, and how the gravitational wave spectrum evolves as the internal toroidal field winds up. These results point to the sorts of experiments that may become possible once gravitational wave interferometers detect core-collapse supernovae routinely. \textcopyright{} 2013 American Physical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/W4I4IIB4/Lasky, Melatos - 2013.pdf}
}

@article{Latham1969,
  title = {The {{Apollo}} Passive Seismic Experiment},
  author = {Latham, G. and Ewing, M. and Press, F. and Sutton, G.},
  year = {1969},
  journal = {Science},
  volume = {165},
  number = {3890},
  pages = {241--250},
  doi = {10.1126/science.165.3890.241},
  urldate = {2020-03-07},
  keywords = {notion,notion-database}
}

@article{Laundal2017,
  title = {Magnetic {{Coordinate Systems}}},
  author = {Laundal, K. M. and Richmond, A. D.},
  year = {2017},
  journal = {Space Science Reviews},
  volume = {206},
  number = {1-4},
  pages = {27--59},
  publisher = {{The Author(s)}},
  issn = {15729672},
  doi = {10.1007/s11214-016-0275-y},
  abstract = {Geospace phenomena such as the aurora, plasma motion, ionospheric currents and associated magnetic field disturbances are highly organized by Earth's main magnetic field. This is due to the fact that the charged particles that comprise space plasma can move almost freely along magnetic field lines, but not across them. For this reason it is sensible to present such phenomena relative to Earth's magnetic field. A large variety of magnetic coordinate systems exist, designed for different purposes and regions, ranging from the magnetopause to the ionosphere. In this paper we review the most common magnetic coordinate systems and describe how they are defined, where they are used, and how to convert between them. The definitions are presented based on the spherical harmonic expansion coefficients of the International Geomagnetic Reference Field (IGRF) and, in some of the coordinate systems, the position of the Sun which we show how to calculate from the time and date. The most detailed coordinate systems take the full IGRF into account and define magnetic latitude and longitude such that they are constant along field lines. These coordinate systems, which are useful at ionospheric altitudes, are non-orthogonal. We show how to handle vectors and vector calculus in such coordinates, and discuss how systematic errors may appear if this is not done correctly.},
  keywords = {Ionospheric electrodynamics,Magnetic coordinates,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5MKPE69P/Laundal, Richmond - 2017.pdf}
}

@article{Lazrek1997a,
  title = {First Results on p Modes from {{GOLF}} Experiment},
  author = {Lazrek, M. and Baudin, F. and Bertello, L. and Boumier, P. and Charra, J. and {Fierry-Fraillon}, D. and Fossat, E. and Gabriel, A. H. and Garc{\'i}a, R. A. and Gelly, B. and Gouiffes, C. and Grec, G. and Pall{\'e}, P. L. and P{\'e}rez Hern{\'a}ndez, F. and R{\'e}gulo, C. and Renaud, C. and Robillot, J. M. and Roca Cort{\'e}s, T. and {Turck-Chi{\`e}ze}, S. and Ulrich, R. K.},
  year = {1997},
  journal = {Solar Physics},
  volume = {175},
  number = {2},
  pages = {227--246},
  issn = {00380938},
  doi = {10.1023/A:1004942929956},
  abstract = {The GOLF experiment on the SOHO mission aims to study the internal structure of the Sun by measuring the spectrum of global oscillations in the frequency range 10-7 to 10-2 Hz. Here we present the results of the analysis of the first 8 months of data. Special emphasis is put into the frequency determination of the p modes, as well as the splitting in the multiplets due to rotation. For both, we show that the improvement in S/N level with respect to the ground-based networks and other experiments is essential in achieving a very low-degree frequency table with small errors ({$\sim$} 2 parts in 105). On the other hand, the splitting found seems to favour a solar core which does not rotate slower than its surface. The line widths do agree with theoretical expectations and other observations.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XZNZITQG/Lazrek et al. - 1997.pdf}
}

@article{Lebreton2008,
  title = {Stellar Ages from Asteroseismology},
  author = {Lebreton, Yveline and Montalb{\'a}n, Josefina},
  year = {2008},
  month = oct,
  journal = {Proceedings of the International Astronomical Union},
  volume = {4},
  number = {S258},
  eprint = {0811.2908},
  pages = {419--430},
  publisher = {{Cambridge University Press (CUP)}},
  issn = {1743-9213},
  doi = {10.1017/s1743921309032074},
  urldate = {2020-03-03},
  abstract = {Asteroseismology has been recognized for a long time as a very powerful mean to probe stellar interiors. The oscillations frequencies are closely related to stellar internal structure properties via the density and the sound speed profiles. Since these properties are in turn tightly linked with the mass and evolutionary state, we can expect to determine the age and mass of a star from the comparison of its oscillation spectrum with the predictions of stellar models. Such a comparison will of course suffer both from the problems we face when modeling a particular star (for instance the uncertainties on its global parameters and chemical composition) and from our general misunderstanding of the physical processes at work in stellar interiors (for instance the various transport processes that may lead to core mixing and affect the ages predicted by models). However for stars where observations have provided very precise and numerous oscillation frequencies together with accurate global parameters and additional information (as the radius or the mass of the star if it is member of a binary system, the radius if it observable in interferometry or the mean density if the star is an exoplanet host), we can also expect to better constrain the physical description of the stellar structure and transport processes and to finally get a more reliable age estimation.After a brief survey of stellar pulsations, we present some general seismic diagnostics that can be used to infer the age of a pulsating star as well as their limitations. We then illustrate the ability of asteroseismology to scrutinize stellar interiors on the basis of a few examples. In the years to come, extended very precise asteroseismic observations are expected, either in photometry or in spectroscopy, from present and future ground-based (HARPS, CORALIE, ELODIE, UVES, UCLES, SIAMOIS, SONG) or spatial devices (MOST, CoRoT, WIRE, Kepler, PLATO). This will considerably enlarge the sample of stars eligible to asteroseismic age determination and should allow to estimate the age of individual stars with a 10-20\% accuracy.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,evolution,fundamental parameters,interiors,notion,notion-database,oscillations,stars: atmospheres,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/GGJ759QF/2009IAUS__258__419L.pdf}
}

@article{Lebreton2008a,
  title = {The {{CoRoT}} Evolution and Seismic Tools Activity: {{Goals}} and Tasks},
  author = {Lebreton, Y. and Monteiro, M. J.P.F.G. and Montalb{\'a}n, J. and Moya, A. and Baglin, A. and {Christensen-Dalsgaard}, J. and Goupil, M. J. and Michel, E. and Provost, J. and Roxburgh, I. W. and Scuflaire, R.},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  pages = {1--12},
  issn = {0004640X},
  doi = {10.1007/s10509-008-9771-1},
  abstract = {The forthcoming data expected from space missions such as CoRoT require the capacity of the available tools to provide accurate models whose numerical precision is well above the expected observational errors. In order to secure that these tools meet the specifications, a team has been established to test and, when necessary, to improve the codes available in the community. The CoRoT Evolution and Seismic Tool Activity (ESTA) has been set up with this mission. Several groups have been involved. The present paper describes the motivation and the organisation of this activity, providing the context and the basis for the presentation of the results that have been achieved so far. This is not a finished task as future even better data will continue to demand more precise and complete tools for asteroseismology. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  isbn = {1050900897711},
  keywords = {Methods: numerical,notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/MIFHUQ5G/Lebreton et al. - 2008.pdf}
}

@article{Lebreton2012a,
  title = {Seismic Signature of Envelope Penetrative Convection: {{The CoRoT}} Star {{HD}} 52265},
  author = {Lebreton, Y. and Goupil, M. J.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {544},
  pages = {4--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220000},
  abstract = {Aims. We aim at characterizing the inward transition from convective to radiative energy transport at the base of the convective envelope of the solar-like oscillator HD 52265 recently observed by the CoRoT satellite. Methods. We investigated the origin of one specific feature found in the HD 52265 frequency spectrum. We modelled the star to derive the internal structure and the oscillation frequencies that best match the observations and used a seismic indicator sensitive to the properties of the base of the envelope convection zone. Results. The seismic indicators clearly reveal that to best represent the observed properties of HD 52265, models must include penetrative convection below the outer convective envelope. The penetrative distance is estimated to be {$\sim$}0.95H P, which corresponds to an extent over a distance representing 6.0 per cents of the total stellar radius, significantly larger than what is found for the Sun. The inner boundary of the extra-mixing region is found at 0.800 {$\pm$} 0.004 R where R = 1.3 R {$\odot$} is the stellar radius. Conclusions. These results contribute to the tachocline characterization in stars other than the Sun. \textcopyright{} 2012 ESO.},
  keywords = {Asteroseismology,notion,notion-database,Stars: individual: HD 52265,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/52Q2RIUM/Lebreton, Goupil - 2012.pdf}
}

@inproceedings{Lebreton2014,
  title = {How Accurate Are Stellar Ages Based on Stellar Models?: {{II}}. {{The}} Impact of Asteroseismology},
  booktitle = {{{EAS Publications Series}}},
  author = {Lebreton, Y. and Goupil, M. J. and Montalb{\'a}n, J.},
  year = {2014},
  month = nov,
  volume = {65},
  eprint = {1410.5337},
  pages = {177--223},
  publisher = {{EDP Sciences}},
  issn = {16381963},
  doi = {10.1051/eas/1465005},
  urldate = {2020-03-05},
  abstract = {Accurate and precise stellar ages are best determined for stars which are strongly observationally constrained, that is which are intrinsically oscillating. We review here the seismic diagnostics which are sensitive to stellar ages and provide some illustrating examples of seismically age-dated stars.},
  archiveprefix = {arxiv},
  isbn = {978-2-7598-1684-2},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/A4EE43NS/full-text.pdf}
}

@inproceedings{Lebreton2014a,
  title = {How Accurate Are Stellar Ages Based on Stellar Models?: {{I}}. {{The}} Impact of Stellar Models Uncertainties},
  booktitle = {{{EAS Publications Series}}},
  author = {Lebreton, Y. and Goupil, M. J. and Montalb{\'a}n, J.},
  year = {2014},
  month = nov,
  volume = {65},
  eprint = {1410.5336},
  pages = {99--176},
  publisher = {{EDP Sciences}},
  issn = {16381963},
  doi = {10.1051/eas/1465004},
  urldate = {2020-03-05},
  abstract = {Among the various methods used to age-date stars, methods based on stellar model predictions are widely used, for nearly all kind of stars in large ranges of masses, chemical compositions and evolutionary stages. The precision and accuracy on the age determination depend on both the precision and number of observational constraints, and on our ability to correctly describe the stellar interior and evolution. The imperfect input physics of stellar models as well as the uncertainties on the initial chemical composition of stars are responsible for uncertainties in the age determination. We present an overview of the calculation of stellar models and discuss the impact on age of their numerous inputs.},
  archiveprefix = {arxiv},
  isbn = {978-2-7598-1684-2},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LF6LZB95/full-text.pdf}
}

@article{Lebreton2014c,
  title = {Asteroseismology for ``\`a La Carte'' Stellar Age-Dating and Weighing},
  author = {Lebreton, Y. and Goupil, M. J.},
  year = {2014},
  journal = {Astronomy \& Astrophysics},
  volume = {569},
  pages = {A21},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201423797},
  abstract = {In the context of CoRoT, Kepler, Gaia, TESS, and PLATO, precise and accurate stellar ages, masses and radii are of paramount importance. They are crucial to constrain scenarii of planetary formation and evolution.We aim at quantifying how detailed stellar modeling improves the accuracy and precision on age and mass of individual stars. We adopt a multifaceted approach where we examine how the number of observational constraints as well as the uncertainties on observations and on model input physics impact the age-dating and weighing. We modelled the exoplanet host-star HD52265, a MS, solar-like oscillator observed by CoRoT. We considered different sets of observational constraints (HR data, metallicity, seismic constraints). For each case, we determined the age, mass, and properties of HD52265 inferred from models, and quantified the impact of the models inputs. Our seismic analysis provides an age A=2.10-2.54 Gyr, a mass M=1.14-1.32 Msun, and a radius R=1.30-1.34 Rsun, which corresponds to uncertainties of 10, 7, and 1.5\% respectively. Our seismic study provides constraints on surface convection, through the mixing-length found to be 12-15\% smaller than the solar one. Because of helium-mass degeneracy, the initial He abundance is determined modulo the mass. The seismic mass of the exoplanet is found to be Mp sin i=1.17-1.26 MJup, much more precise than what can be derived by HR diagram inversion. We demonstrate that asteroseismology allows to improve the age accuracy compared to other methods. We emphasize that the knowledge of the mean properties of oscillations -as the large frequency separation- is not enough for deriving accurate ages. We need precise individual frequencies to narrow the age scatter due to model uncertainties. This strengthen the case for precise classical stellar parameters and frequencies as will be obtained by Gaia and PLATO.},
  keywords = {asteroseismology,evolution,fundamental parameters,hd 52265,individual,interiors,notion,notion-database,planets and satellites,stars},
  file = {/Users/lbugnet/Zotero/storage/VTKHQVCG/Lebreton, Goupil - 2014.pdf}
}

@article{Lecoanet2017b,
  title = {Conversion of Internal Gravity Waves into Magnetic Waves},
  author = {Lecoanet, D. and Vasil, G. M. and Fuller, J. and Cantiello, M. and Burns, K. J.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {466},
  number = {2},
  eprint = {1610.08506},
  pages = {2181--2193},
  issn = {0035-8711},
  doi = {10.1093/mnras/stw3273},
  abstract = {Asteroseismology probes the interiors of stars by studying oscillation modes at a star's surface. Although pulsation spectra are well understood for solar-like oscillators, a substantial fraction of red giant stars observed by Kepler exhibit abnormally low-amplitude dipole oscillation modes. Fuller et al. (2015) suggests this effect is produced by strong core magnetic fields that scatter dipole internal gravity waves (IGWs) into higher multipole IGWs or magnetic waves. In this paper, we study the interaction of IGWs with a magnetic field to test this mechanism. We consider two background stellar structures: one with a uniform magnetic field, and another with a magnetic field that varies both horizontally and vertically. We derive analytic solutions to the wave propagation problem and validate them with numerical simulations. In both cases, we find perfect conversion from IGWs into magnetic waves when the IGWs propagate into a region exceeding a critical magnetic field strength. Downward propagating IGWs cannot reflect into upward propagating IGWs because their vertical wavenumber never approaches zero. Instead, they are converted into upward propagating slow (Alfvenic) waves, and we show they will likely dissipate as they propagate back into weakly magnetized regions. Therefore, strong internal magnetic fields can produce dipole mode suppression in red giants, and gravity modes will likely be totally absent from the pulsation spectra of sufficiently magnetized stars.},
  archiveprefix = {arxiv},
  keywords = {1 i n t,asteroseismology,clues to prior phases,harbour strong magnetic fields,lutionary processes and yield,magnetic field,many types of stars,notion,notion-database,of evolution,ro d u c,scattering,stars,t i o n,that drive evo-,waves},
  file = {/Users/lbugnet/Zotero/storage/6RV8VFFE/Lecoanet et al. - 2017(2).pdf}
}

@article{Lecoanet2022,
  title = {Asteroseismic Inference of the Near-Core Magnetic Field Strength in the Main Sequence {{B}} Star {{HD}} 43317},
  author = {Lecoanet, Daniel and Bowman, Dominic M. and Van Reeth, Timothy},
  year = {2022},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {512},
  number = {1},
  eprint = {2202.03440},
  primaryclass = {astro-ph},
  pages = {L16-L20},
  issn = {1745-3925, 1745-3933},
  doi = {10.1093/mnrasl/slac013},
  urldate = {2023-05-09},
  abstract = {About 10 per cent of intermediate- and high-mass dwarf stars are observed to host a strong large-scale magnetic field at their surface, which is thought to be of fossil field origin. However, there are few inferences as to the magnetic field strength and geometry within the deep interiors of stars. Considering that massive stars harbour a convective core whilst on the main sequence, asteroseismology of gravity (g) modes is able to provide constraints on their core masses, yet it has so far not been used to probe the strength of their interior magnetic fields. Here we use asteroseismology to constrain an upper limit for the magnetic field strength in the near-core region of the pulsating and magnetic B star HD 43317, based on the expected interaction of a magnetic field and its g modes. We find a magnetic field strength of order \$5 \textbackslash times 10\^5\$ G is sufficient to suppress high-radial order g modes and reproduce the observed frequency spectrum of HD 43317, which contains only high-frequency g modes. This result is the first inference of the magnetic field strength inside a main-sequence star.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/SADYQICH/Lecoanet et al. - 2022 - Asteroseismic inference of the near-core magnetic .pdf;/Users/lbugnet/Zotero/storage/2RRRL5WH/2202.html}
}

@article{Lee1997,
  title = {Low-{{Frequency Nonradial Oscillations}} in {{Rotating Stars}}. {{I}}. {{Angular Dependence}}},
  author = {Lee, Umin and Saio, Hideyuki},
  year = {1997},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {491},
  number = {2},
  pages = {839--845},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/304980},
  urldate = {2020-05-28},
  abstract = {We obtain the \texttheta -dependence of the displacement vector of rotationally modulated low-frequency nonradial oscillations by numerically integrating Laplace's tidal equation as an eigenvalue problem with a relaxation method. This method of calculation is more tractable than our previous method in which the \texttheta -dependence was represented by a truncated series of associated Legendre functions. Laplace's tidal equation has two families of eigenvalues. In one of these families, an eigenvalue {$\lambda$} coincides with l(l + 1) when rotation is absent, where l is the latitudinal degree of the associated Legendre function, Pml(cos \texttheta ). The value of {$\lambda$} changes as a function of {$\nu$} {$\equiv$} 2{$\Omega$}/{$\omega$}, where {$\Omega$} and {$\omega$} are the angular frequencies of rotation and of oscillation (seen in the corotating frame), respectively. These eigenvalues correspond to rotationally modulated g-mode oscillations. In the domain of | {$\nu$} | \&gt; 1, another family of eigenvalues exists. Eigenvalues belonging to this family have negative values for prograde oscillations, while they change signs from negative to positive for retrograde oscillations as | {$\nu$} | increases. Negative {$\lambda$}'s correspond to oscillatory convective modes. The solution associated with a {$\lambda$} that has a small positive value after changing its sign is identified as an r-mode (global Rossby wave) oscillation. Amplitudes of g-mode oscillations tend to be confined to the equatorial region as | {$\nu$} | increases. This tendency is stronger for larger {$\lambda$}. On the other hand, amplitudes of oscillatory convective modes are small near the equator.},
  keywords = {Methods: Numerical,notion,notion-database,oscillations \`E stars,rotation,Stars: Oscillations,Stars: Rotation},
  file = {/Users/lbugnet/Zotero/storage/GHWYHT8A/full-text.pdf;/Users/lbugnet/Zotero/storage/TUW85L93/full-text.pdf}
}

@misc{leeProbingCosmicBirefringence2022,
  title = {Probing {{Cosmic Birefringence}} with {{Polarized Sunyaev Zel}}'dovich {{Tomography}}},
  author = {Lee, Nanoom and Hotinli, Selim C. and Kamionkowski, Marc},
  year = {2022},
  month = jul,
  journal = {arXiv e-prints},
  urldate = {2022-07-18},
  abstract = {If the physics behind dark energy and/or dark matter violates the parity symmetry assumed in the standard cosmological paradigm, the linear polarization of the cosmic microwave background (CMB) photons can rotate due to their coupling to the dark sector. Recent 3\$\textbackslash sigma\$ hints of this 'cosmic birefringence' in the EB spectrum of the CMB polarization motivates us to pursue new directions to independently validate and characterize the signal. Here, we explore the prospects to probe cosmic birefringence from small-scale fluctuations in the CMB using polarized Sunyaev Zel'dovich (pSZ) tomography. We find that pSZ can be used to infer the redshift dependence of cosmic birefringence and also help calibrate the instrumental polarization orientation. To illustrate the prospects, we show that pSZ tomography may probe an axion-like dark energy model with masses \$m\_\textbackslash phi \textbackslash lesssim 10\^\{-32\}\$eV with \$\textbackslash mathcal\{O\}(0.1)\$ degrees of rotation between reionization and recombination.},
  keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics,High Energy Physics - Phenomenology,notion,notion-database},
  annotation = {ADS Bibcode: 2022arXiv220705687L},
  file = {/Users/lbugnet/Zotero/storage/U8DKCUD2/Lee et al. - 2022 - Probing Cosmic Birefringence with Polarized Sunyae.pdf}
}

@article{Lefebvre2008,
  title = {Variations of the Solar Granulation Motions with Height Using the {{GOLF}}/{{SoHO}} Experiment},
  author = {Lefebvre, S. and Garc{\'i}a, R. A. and {Jim{\'e}nez-Reyes}, S. J. and {Turck-Chi{\`e}ze}, S. and Mathur, S.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {490},
  number = {3},
  pages = {1143--1149},
  issn = {00046361},
  doi = {10.1051/0004-6361:200810344},
  abstract = {Context. Below 1 mHz, the power spectrum of helioseismic velocity measurements is dominated by the spectrum of convective motions (granulation and supergranulation) and it is difficult to detect the low-order acoustic modes and gravity modes.Aims. We attempt to understand more clearly the behavior of solar granulation as a function of observing height in the solar atmosphere and with magnetic activity during solar cycle 23.Methods. We analyze the Power Spectral Density (PSD) of eleven years of GOLF/SOHO velocity time series data using a Harvey-type model to characterize the properties of the convective motions in the solar oscillation power spectrum. We study the evolution of the granulation with both altitude in the solar atmosphere and solar activity.Results. We first demonstrate that the traditional use of a Lorentzian profile to describe the envelope of the modes is unsuitable for GOLF data. To model properly the solar spectrum, we must instead adopt a second Lorentzian profile. Secondly, we show that the granulation clearly evolves with height in the photosphere but does not present any significant variation with the activity cycle.. \textcopyright{} 2008 ESO.},
  keywords = {notion,notion-database,Sun: activity,Sun: chromosphere,Sun: granulation,Sun: helioseismology,Sun: oscillations,Sun: photosphere},
  file = {/Users/lbugnet/Zotero/storage/QURDB23Q/Lefebvre et al. - 2008.pdf}
}

@article{Lehmann1936,
  title = {Selektive {{Beeinflussung}} Fr\"uhembryonaler {{Entwicklungsvorg\"ange}} Bei {{Wirbeltieren}}},
  author = {Lehmann, F. E.},
  year = {1936},
  month = jun,
  journal = {Die Naturwissenschaften},
  volume = {24},
  number = {26},
  pages = {401--407},
  publisher = {{Springer-Verlag}},
  issn = {00281042},
  doi = {10.1007/BF01473929},
  urldate = {2020-07-04},
  keywords = {notion,notion-database}
}

@article{Leibacher,
  title = {A {{New Description}} of the {{Solar Five-Minute Oscillation}} - {{NASA}}/{{ADS}}},
  author = {Leibacher, John W. and Stein, R. F.},
  year = {1971},
  journal = {Astrophysical Letters},
  urldate = {2020-03-08},
  keywords = {notion,notion-database}
}

@article{Leibacher1971,
  title = {A {{New Description}} of the {{Solar Five-Minute Oscillation}}},
  author = {Leibacher, J. W. and Stein, R. F.},
  year = {1971},
  journal = {ApL},
  volume = {7},
  pages = {191--192},
  issn = {0004-6388},
  urldate = {2020-07-04},
  keywords = {GLOBAL MODES,JOHN LEIBACHER,notion,notion-database,THEORY}
}

@article{Leighton1962,
  title = {Velocity {{Fields}} in the {{Solar Atmosphere}}. {{I}}. {{Preliminary Report}}.},
  author = {Leighton, Robert B. and Noyes, Robert W. and Simon, George W.},
  year = {1962},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {135},
  pages = {474},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/147285},
  urldate = {2020-02-28},
  abstract = {applicability for this approach.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YHEGH5HI/full-text.pdf}
}

@article{Leighton1969,
  title = {A {{Magneto-Kinematic Model}} of the {{Solar Cycle}}},
  author = {Leighton, Robert B.},
  year = {1969},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {156},
  pages = {1},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/149943},
  urldate = {2020-05-14},
  abstract = {Abstract image available at: http://adsabs.harvard.edu/abs/1969ApJ...156....1L},
  keywords = {notion,notion-database}
}

@article{Lenain2007a,
  title = {The {{$E$-mechanism}} in {{PMS}} and {{MS}} {$\delta$} {{Scuti}} Stars},
  author = {Lenain, G.},
  year = {2007},
  journal = {Communications in Asteroseismology},
  volume = {147},
  pages = {93--96},
  issn = {1021-2043},
  doi = {10.1553/cia147s93},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QW2ELFQR/Lenain - 2007.pdf}
}

@article{Leone2007,
  title = {Measuring Stellar Magnetic Fields with the Low Resolution Spectropolarimeter of the {{William Herschel Telescope}}},
  author = {Leone, F.},
  year = {2007},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {382},
  number = {4},
  eprint = {0709.2106},
  pages = {1690--1696},
  doi = {10.1111/j.1365-2966.2007.12457.x},
  urldate = {2020-07-04},
  abstract = {Despite the influence of magnetic fields on the structure and evolution of stars is largely demonstrated from the theoretical point of view, their observational evidence in non-degenerated stars is still rather scanty and mainly circumscribed to bright objects (V{$<$}10). Stellar magnetic fields are commonly measured on the basis of circular spectropolarimetry at high/middle resolution across the profile of metal lines. The present sensitivity of telescopes and spectrographs makes this still an almost prohibitive method for faint stars. In principle, stellar magnetic fields can be also measured on the basis of low resolution spectropolarimetry, with very important results obtained at the 8 m ESO telescopes with FORS1. The trade off between S/N and spectral resolution in measuring stellar magnetic fields justify an attempt, here presented, to perform these measurements at the 4.5 m William Herschel Telescope. HD3360, one of the stars with the weakest known magnetic field, and the magnetic chemically peculiar stars HD10783, HD74521 and HD201601 have been observed with the spectropolarimeter ISIS in the 3785-4480 A range. Measured stellar magnetic fields, from Stokes I and V spectra with S/N {$>$} 600, show an internal error of {$<$}50 G selecting the whole interval and {$<$}200 G within a Balmer line. Ripples in the Stokes V spectra of HD3360 result in an instrumental positive magnetic field certainly not larger than 80 G.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: individual: HD 10783,Stars: individual: HD 201601,Stars: individual: HD 74521,Stars: magnetic fields,Techniques: polarimetric,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/STCCQW23/full-text.pdf}
}

@article{Leone2014,
  title = {A Search for Magnetic Fields on Central Stars in Planetary Nebulae},
  author = {Leone, F. and Corradi, R. L. M. and Mart{\'i}nez Gonz{\'a}lez, M. J. and Asensio Ramos, A. and Manso Sainz, R.},
  year = {2014},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {563},
  pages = {A43},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201322753},
  urldate = {2023-10-09},
  abstract = {Context. One of the possible mechanisms responsible for the panoply of shapes in planetary nebulae is the presence of magnetic fields that drive the ejection of ionized material during the proto-planetary nebula phase. Aims: Therefore, detecting magnetic fields in such objects is of key importance for understanding their dynamics. Still, magnetic fields have not been detected using polarimetry in the central stars of planetary nebulae. Methods: Circularly polarized light spectra have been obtained with the Focal Reducer and Low Dispersion Spectrograph at the Very Large Telescope of the European Southern Observatory and the Intermediate dispersion Spectrograph and Imaging System at the William Herschel Telescope. Twentythree planetary nebulae that span very different morphology and evolutionary stages have been selected. Most of central stars have been observed at different rotation phases to point out evidence of magnetic variability. Results: In this paper, we present the result of two observational campaigns aimed to detect and measure the magnetic field in the central stars of planetary nebulae on the basis of low resolution spectropolarimetry. In the limit of the adopted method, we can state that large scale fields of kG order are not hosted on the central star of planetary nebulae.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,planetary nebulae: general,stars: magnetic field,techniques: polarimetric},
  annotation = {ADS Bibcode: 2014A\&A...563A..43L},
  file = {/Users/lbugnet/Zotero/storage/QWXXUIT3/Leone et al. - 2014 - A search for magnetic fields on central stars in p.pdf}
}

@article{LePennec2015a,
  title = {First New Solar Models with Opas Opacity Tables},
  author = {Le Pennec, M. and {Turck-Chi{\`e}ze}, S. and Salmon, S. and Blancard, C. and Coss{\'e}, P. and Faussurier, G. and Mondet, G.},
  year = {2015},
  journal = {Astrophysical Journal Letters},
  volume = {813},
  number = {2},
  pages = {L42},
  publisher = {{IOP Publishing}},
  issn = {20418213},
  doi = {10.1088/2041-8205/813/2/L42},
  abstract = {Stellar seismology appears more and more as a powerful tool for a better determination of the fundamental properties of solar-type stars. However, the particular case of the Sun is still challenging. For about a decade now, the helioseismic sound-speed determination has continued to disagree with the standard solar model (SSM) prediction, questioning the reliability of this model. One of the sources of uncertainty could be in the treatment of the transport of radiation from the solar core to the surface. In this Letter, we use the new OPAS opacity tables, recently available for solar modeling, to address this issue. We discuss first the peculiarities of these tables, then we quantify their impact on the solar sound-speed and density profiles using the reduced OPAS tables taken on the grids of the OPAL ones. We use the two evolution codes, Modules for Experiments in Stellar Astrophysics and Code Li\'egeois d'Evolution Stellaire, that led to similar conclusions in the solar radiative zone. In comparison to commonly used OPAL opacity tables, the new solar models are computed for the most recent photospheric composition with OPAS tables and present improvements to the location of the base of the convective zone and to the description of the solar radiative zone in comparison to the helioseismic observations, even if the differences in the Rosseland mean opacity do not exceed 6\%. We finally carry out a comparison to a solar model computed with the OP opacity tables.},
  keywords = {Atomic Processes,notion,notion-database,opacity,plasmas,stars: evolution,stars: interiors},
  file = {/Users/lbugnet/Zotero/storage/MXKIZS9R/Le Pennec et al. - 2015.pdf}
}

@article{Levrard2009a,
  title = {Falling Transiting Extrasolar Giant Planets},
  author = {Levrard, B. and Winisdoerffer, C. and Chabrier, G.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {692},
  number = {1},
  eprint = {0901.2048},
  pages = {1--6},
  issn = {15384357},
  doi = {10.1088/0004-637X/692/1/L9},
  abstract = {We revisit the tidal stability of extrasolar systems harboring a transiting planet and demonstrate that, independently of any tidal model, none, but one (HAT-P-2b) of these planets has a tidal equilibrium state, which implies ultimately a collision of these objects with their host star. Consequently, conventional circularization and synchronization timescales cannot be defined because the corresponding states do not represent the endpoint of the tidal evolution. Using numerical simulations of the coupled tidal equations for the spin and orbital parameters of each transiting planetary system, we confirm these predictions and show that the orbital eccentricity and the stellar obliquity do not follow the usually assumed exponential relaxation but instead decrease significantly, eventually reaching a zero value only during the final runaway merging of the planet with the star. The only characteristic evolution timescale of all rotational and orbital parameters is the lifetime of the system, which crucially depends on the magnitude of tidal dissipation within the star. These results imply that the nearly circular orbits of transiting planets and the alignment between the stellar spin axis and the planetary orbit are unlikely to be due to tidal dissipation. Other dissipative mechanisms, for instance interactions with the protoplanetary disk, must be invoked to explain these properties. \textcopyright{} 2009. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {Celestial mechanics,notion,notion-database,Planetary systems: formation,Planetary systems: protoplanetary disks},
  file = {/Users/lbugnet/Zotero/storage/JJWSG5MF/Levrard, Winisdoerffer, Chabrier - 2009.pdf}
}

@article{Li2015,
  title = {Asteroseismology of the {{ZZ Ceti}} Star {{KUV}} 08368+4026},
  author = {Li, C. and Fu, J.-N. and Vauclair, G. and Dolez, N. and {Fox-Machedo}, L. and Michel, R. and Chavez, M. and Bertone, E.},
  year = {2015},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {449},
  number = {4},
  eprint = {1709.09206},
  primaryclass = {astro-ph},
  pages = {3360--3369},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/stv481},
  urldate = {2023-10-14},
  abstract = {Asteroseismology is a unique tool to explore the internal structure of stars through both observational and theoretical research. The internal structure of pulsating hydrogen shell white dwarfs (ZZ Ceti stars) detected by asteroseismology is regarded as the representative of all DA white dwarfs. Observations for KUV\textasciitilde 08368+4026, which locates in the middle of the ZZ Ceti instability strip, have been carried out in 1999 and from 2009 to 2012 with either single-site runs or multisite campaigns. Time-series photometric data of about 300 hours were collected in total. Through data reduction and analysis, 30 frequencies were extracted, including four triplets, two doublets, one single mode and further signals. The independent modes are identified as either l=1 or l=2 modes. Hence, a rotation period of \$5.52\textbackslash pm 0.22\$ days was deduced from the period spacing in the multiplets. Theoretical static models were built and a best fit model for KUV\textasciitilde 08368+4026 was obtained with \$0.692\textbackslash pm0.002\$ solar mass, \$(2.92\textbackslash pm0.02)\textbackslash times 10\^\{-3\}\$ solar luminosity and the hydrogen mass fraction of \$10\^\{-4\}\$ stellar mass.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/MIPE9GPY/Li et al. - 2015 - Asteroseismology of the ZZ Ceti star KUV 08368+402.pdf;/Users/lbugnet/Zotero/storage/AC8ZGZIT/1709.html}
}

@article{Li2018,
  title = {Modelling Kepler Red Giants in Eclipsing Binaries: {{Calibrating}} the Mixing-Length Parameter with Asteroseismology},
  author = {Li, Tanda and Bedding, Timothy R. and Huber, Daniel and Ball, Warrick H. and Stello, Dennis and Murphy, Simon J. and {Bland-Hawthorn}, Joss},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {475},
  number = {1},
  eprint = {1712.01424},
  issn = {13652966},
  doi = {10.1093/mnras/stx3079},
  abstract = {Stellar models rely on a number of free parameters. High-quality observations of eclipsing binary stars observed by Kepler offer a great opportunity to calibrate model parameters for evolved stars. Our study focuses on six Kepler red giants with the goal of calibrating the mixing-length parameter of convection as well as the asteroseismic surface term in models. We introduce a new method to improve the identification of oscillation modes that exploits theoretical frequencies to guide the mode identification ('peak-bagging') stage of the data analysis. Our results indicate that the convective mixing-length parameter ({$\alpha$}) is {$\approx$}14 per cent larger for red giants than for the Sun, in agreement with recent results from modelling the APOGEE stars.We found that the asteroseismic surface term (i.e. the frequency offset between the observed and predicted modes) correlates with stellar parameters (Teff, log g) and the mixing-length parameter. This frequency offset generally decreases as giants evolve. The two coefficients a-1 and a3 for the inverse and cubic terms that have been used to describe the surface term correction are found to correlate linearly. The effect of the surface term is also seen in the p-g mixed modes; however, established methods for correcting the effect are not able to properly correct the g-dominated modes in late evolved stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Li2019,
  title = {Period Spacings of {$\gamma$} {{Doradus}} Pulsators in the {{Kepler}} Field: {{Rossby}} and Gravity Modes in 82 Stars},
  shorttitle = {Period Spacings of {$\gamma$} {{Doradus}} Pulsators in the {{Kepler}} Field},
  author = {Li, Gang and Van Reeth, Timothy and Bedding, Timothy R. and Murphy, Simon J. and Antoci, Victoria},
  year = {2019},
  month = jul,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {487},
  pages = {782--800},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz1171},
  urldate = {2023-07-27},
  abstract = {Rossby modes are the oscillations in a rotating fluid, whose restoring force is the Coriolis force. They provide an additional diagnostic to understand the rotation of stars, which complicates asteroseismic modelling. We report 82 {$\gamma$} Doradus stars for which clear period spacing patterns of both gravity and Rossby modes have been detected. The period spacings of both show a quasi-linear relation with the pulsation period, but the slope is negative for the gravity modes and positive for the Rossby modes. Most Rossby modes have k = -2, m = -1. For only one star, a series of k = -1, m = -1 modes is seen. For each pattern, the mean pulsation period, the mean period spacing, and the slope are measured. We find that the slope correlates with the mean period for Rossby mode patterns. The traditional approximation of rotation is used to measure the near-core rotation rate, assuming the star rotates rigidly. We report the near-core rotation rates, the asymptotic period spacings, and the radial orders of excited modes of these 82 main-sequence stars. The near-core rotation rates lie between 0.6 and 2.3 d\^\{-1\}. Six stars show surface rotation modulations, among which only KIC 3341457 shows differential rotation, whilst the other five stars have uniform rotations. The radial orders of excited modes show different distributions for the dipole and quadrupole gravity modes versus the Rossby modes.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: oscillations,stars: rotation,stars: variables},
  annotation = {ADS Bibcode: 2019MNRAS.487..782L},
  file = {/Users/lbugnet/Zotero/storage/HJPF3XRU/Li et al. - 2019 - Period spacings of γ Doradus pulsators in the Kepl.pdf}
}

@article{Li2019a,
  title = {Period Spacings of {$\gamma$} {{Doradus}} Pulsators in the {{Kepler}} Field: {{Detection}} Methods and Application to 22 Slow Rotators},
  author = {Li, Gang and Bedding, Timothy R. and Murphy, Simon J. and Reeth, Timothy Van and Antoci, Victoria and Ouazzani, Rhita Maria},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {482},
  number = {2},
  eprint = {1810.03362},
  pages = {1757--1785},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/sty2743},
  abstract = {In {$\gamma$} Doradus ({$\gamma$} Dor) stars, the g-mode period spacing shows an approximately linear relation with period. The slope is a new asteroseismic diagnostic, related to the rotation rate and the azimuthal orderm.We report two automated methods, the 'moving-windowFourier transform' and the 'cross-correlation', to detect and measure the period spacings based on 4-yr light curves from the Kepler satellite. The results show that the cross-correlation method performs better at detecting the period spacings and their slopes. In this paper, we apply our method to 22 {$\gamma$} Dor stars with g-mode multiplets split by rotation. The rotation periods are similar to the g-mode period spacings, causing the multiplets to overlap. To clarify the overlapping patterns, we use the \'echelle diagram and introduce a 'copy-shift' diagram to discern and measure the splittings. The first observational relation between slopes and splittings is shown. The slope deviates from zero when the splitting increases, as the theory predicts. We found that what appears to be rotational splittings in two stars is in fact caused by two nearly identical overlapping patterns from binaries.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: rotation,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/CTUKHBIU/Li et al. - 2019.pdf}
}

@article{Li2020,
  title = {Gravity-Mode Period Spacings and near-Core Rotation Rates of 611 {$\gamma$} {{Doradus}} Stars with {{Kepler}}},
  author = {Li, Gang and Van Reeth, Timothy and Bedding, Timothy R. and Murphy, Simon J. and Antoci, Victoria and Ouazzani, Rhita-Maria and Barbara, Nicholas H.},
  year = {2020},
  month = jan,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {491},
  pages = {3586--3605},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz2906},
  urldate = {2023-11-07},
  abstract = {We report our survey of {$\gamma$} Dor stars from the 4-yr Kepler mission. These stars pulsate mainly in g modes and r modes, showing period-spacing patterns in the amplitude spectra. The period-spacing patterns are sensitive to the chemical composition gradients and the near-core rotation, hence they are essential for understanding the stellar interior. We identified period-spacing patterns in 611 {$\gamma$} Dor stars. Almost every star pulsates in dipole g modes, while about 30 per cent of stars also show clear patterns for quadrupole g modes and 16 per cent of stars present r-mode patterns. We measure periods, period spacings, and the gradient of the period spacings. These three observables guide the mode identifications and can be used to estimate the near-core rotation rate. We find many stars are hotter and show longer period-spacing patterns than theory. Using the traditional approximation of rotation (TAR), we inferred the asymptotic spacings, the near-core rotation rates, and the radial orders of the g and r modes. Most stars have a near-core rotation rate around 1 d-1 and an asymptotic spacing around 4000 s. We also find that many stars rotate more slowly than predicted by theory for unclear reasons. 11 stars show rotational splittings with fast rotation rates. We compared the observed slope-rotation relation with the theory and find a large spread. We detected rotational modulations in 58 stars and used them to derive the core-to-surface rotation ratios. The interiors rotate faster than the cores in most stars, but by no more than 5 per cent.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2020MNRAS.491.3586L},
  file = {/Users/lbugnet/Zotero/storage/FIH4WDJZ/Li et al. - 2020 - Gravity-mode period spacings and near-core rotatio.pdf}
}

@article{Li2022,
  title = {Magnetic Fields of 30 to 100 {{kG}} in the Cores of Red Giant Stars},
  author = {Li, Gang and Deheuvels, S{\'e}bastien and Ballot, J{\'e}r{\^o}me and Ligni{\`e}res, Fran{\c c}ois},
  year = {2022},
  month = oct,
  journal = {Nature},
  volume = {610},
  pages = {43--46},
  issn = {0028-0836},
  doi = {10.1038/s41586-022-05176-0},
  urldate = {2023-05-09},
  abstract = {A red giant star is an evolved low- or intermediate-mass star that has exhausted its central hydrogen content, leaving a helium core and a hydrogen-burning shell. Oscillations of stars can be observed as periodic dimmings and brightenings in the optical light curves. In red giant stars, non-radial acoustic waves couple to gravity waves and give rise to mixed modes, which behave as pressure modes in the envelope and gravity modes in the core. These modes have previously been used to measure the internal rotation of red giants1,2, leading to the conclusion that purely hydrodynamical processes of angular momentum transport from the core are too inefficient3. Magnetic fields could produce the additional required transport4-6. However, owing to the lack of direct measurements of magnetic fields in stellar interiors, little is currently known about their properties. Asteroseismology can provide direct detection of magnetic fields because, like rotation, the fields induce shifts in the oscillation mode frequencies7-12. Here we report the measurement of magnetic fields in the cores of three red giant stars observed with the Kepler13 satellite. The fields induce shifts that break the symmetry of dipole mode multiplets. We thus measure field strengths ranging from about 30 kilogauss to about 100 kilogauss in the vicinity of the hydrogen-burning shell and place constraints on the field topology.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2022Natur.610...43L},
  file = {/Users/lbugnet/Zotero/storage/TAXPI7BS/Li et al. - 2022 - Magnetic fields of 30 to 100 kG in the cores of re.pdf}
}

@article{Li2023,
  title = {Internal Magnetic Fields in 13 Red Giants Detected by Asteroseismology},
  author = {Li, G. and Deheuvels, S. and Li, T. and Ballot, J. and Lignieres, F.},
  year = {2023},
  month = oct,
  journal = {Astronomy \& Astrophysics},
  publisher = {{EDP Sciences}},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202347260},
  urldate = {2023-10-09},
  abstract = {Astronomy \& Astrophysics (A\&A) is an international journal which publishes papers on all aspects of astronomy and astrophysics},
  copyright = {\textcopyright{} 2023, ESO},
  langid = {english}
}

@article{Libbrecht1989,
  title = {Solar P-Mode Frequency Splittings},
  author = {Libbrecht, K G},
  year = {1989},
  volume = {336},
  number = {336},
  pages = {1092--1097},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/7PJNGXEI/Libbrecht - 1989.pdf}
}

@article{Libbrecht1990,
  title = {Solar-Cycle Effects on Solar Oscillation Frequencies},
  author = {Libbrecht, K G and Woodard, M F},
  year = {1990},
  volume = {345},
  number = {June},
  pages = {779--782},
  isbn = {1111111111},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UZNI2Y72/Libbrecht, Woodard - 1990.pdf}
}

@article{libbrecht1992,
  title = {On the Ultime Accuracy of Solar Oscillation Frequency Measurements},
  author = {Libbrecht, K G},
  year = {1992},
  journal = {The Astrophysical Journal},
  volume = {387},
  number = {2},
  pages = {712--714},
  doi = {10.20595/jjbf.19.0_3},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4EETLGR7/Libbrecht - 1992.pdf}
}

@article{Liebert2002,
  title = {The {{True Incidence}} of {{Magnetism}} among {{Field White Dwarfs}}},
  author = {Liebert, James and Bergeron, P. and Holberg, J. B.},
  year = {2002},
  month = oct,
  journal = {The Astronomical Journal},
  volume = {125},
  number = {1},
  eprint = {astro-ph/0210319},
  pages = {348--353},
  publisher = {{IOP Publishing}},
  doi = {10.1086/345573},
  urldate = {2020-03-09},
  abstract = {We study the incidence of magnetism in white dwarfs from three large and well-observed samples of hot, cool, and nearby white dwarfs in order to test whether the fraction of magnetic degenerates is biased, and whether it varies with effective temperature, cooling age, or distance. The magnetic fraction is considerably higher for the cool sample of Bergeron, Ruiz, and Leggett, and the Holberg, Oswalt, and Sion sample of local white dwarfs that it is for the generally-hotter white dwarfs of the Palomar Green Survey. We show that the mean mass of magnetic white dwarfs in this survey is 0.93 solar masses or more, so there may be a strong bias against their selection in the magnitude-limited Palomar Green Survey. We argue that this bias is not as important in the samples of cool and nearby white dwarfs. However, this bias may not account for all of the difference in the magnetic fractions of these samples. It is not clear that the magnetic white dwarfs in the cool and local samples are drawn from the same population as the hotter PG stars. In particular, two or threee of the cool sample are low-mass white dwarfs in unresolved binary systems. Moreover, there is a suggestion from the local sample that the fractional incidence may increase with decreasing temperature, luminosity, and/or cooling age. Overall, the true incidence of magnetism at the level of 2 megagauss or greater is at least 10\%, and could be higher. Limited studies capable of detecting lower field strengths down to 10 kilogauss suggest by implication that the total fraction may be substantially higher than 10\%.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Stars: Magnetic Fields,Stars: Statistics,Stars: White Dwarfs},
  file = {/Users/lbugnet/Zotero/storage/YW455W5R/full-text.pdf}
}

@article{Lim1998,
  title = {Large Convection Cells as the Source of {{Betelgeuse}}'s Extended Atmosphere},
  author = {Lim, Jeremy and Carilli, Chris L. and White, Stephen M. and Beasley, Anthony J. and Marson, Ralph G.},
  year = {1998},
  month = apr,
  journal = {Nature},
  volume = {392},
  number = {6676},
  pages = {575--577},
  issn = {00280836},
  doi = {10.1038/33352},
  urldate = {2020-03-14},
  abstract = {Supergiant stars such as Betelgeuse have very extended atmospheres, the properties of which are poorly understood. Alfven waves, acoustic waves and radial pulsations have all been suggested as likely mechanisms for elevating these atmospheres and driving the massive outflows of gas seen in these stars: such mechanisms would heat the atmosphere from below, and there are indeed observations showing that Betelgeuse's extended atmosphere is hotter than the underlying photosphere. Here we report radio observations of Betelgeuse that reveal the temperature structure of the extended atmosphere from two to seven times the photospheric radius. Close to the star, we find that the atmosphere has an irregular structure, and a temperature (3,450 {$\pm$} 850 K) consistent with the photospheric temperature but much lower than that of gas in the same region probed by optical and ultraviolet observations. This cooler gas decreases steadily in temperature with radius, reaching 1,370 {$\pm$} 330 K by seven stellar radii. The cool gas coexists with the hot chromospheric gas, but must be much more abundant as it dominates the radio emission. Our results suggest that a few inhomogeneously distributed large convective cells (which are widely believed to be present in such stars) are responsible for lifting the cooler photospheric gas into the atmosphere; radiation pressure on dust grains that condense from this gas may then drive Betelgeuse's outflow.},
  keywords = {notion,notion-database}
}

@article{Lin2007,
  title = {Seismic {{Study}} of the {{Chemical Composition}} of the {{Solar Convection Zone}}},
  author = {Lin, Chia-Hsien and Antia, H. M. and Basu, Sarbani},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {668},
  number = {1},
  eprint = {0706.3046},
  pages = {603--610},
  issn = {0004-637X},
  doi = {10.1086/520916},
  abstract = {Recent downward revision of solar heavy-element abundances using a\textbackslash r\textbackslash nthree-dimensional atmospheric model has introduced serious discrepancies\textbackslash r\textbackslash nbetween standard solar models and helioseismic inferences about solar\textbackslash r\textbackslash nstructure. In this paper we investigate the possibility of determining\textbackslash r\textbackslash nthe heavy-element abundances using helioseismic inversion techniques\textbackslash r\textbackslash nwith the hope of providing an independent estimate. We use the adiabatic\textbackslash r\textbackslash nindex {$\Gamma$}1{$\equiv$}({$\partial$}lnP/{$\partial$}ln{$\rho$})s as\textbackslash r\textbackslash na probe to examine the effects of the total heavy-element abundance, as\textbackslash r\textbackslash nwell as the effects due to the abundance of individual elements. Our\textbackslash r\textbackslash ninversion results show that the new, lower, abundance increases the\textbackslash r\textbackslash ndiscrepancy between the Sun and the solar models.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KMYYQLHK/Lin, Antia, Basu - 2007.pdf}
}

@article{Lindsey2005,
  title = {The {{Acoustic Showerglass}}. {{I}}. {{Seismic Diagnostics}} of {{Photospheric Magnetic Fields}}},
  author = {Lindsey, Charles and Braun, D. C.},
  year = {2005},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {620},
  number = {2},
  pages = {1107--1117},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/426065},
  urldate = {2020-07-04},
  abstract = {A problem of major interest in the helioseismology of active regions is the acoustics of magnetic photospheres and shallow subphotospheres. Magnetic fields suppress the photospheric signatures of acoustic waves impinging onto them from the underlying solar interior and shift their phases. The phase shifts function as a sort of acoustic showerglass that impairs the coherence of seismic waves arriving from below, degrading images of subsurface anomalies derived by mechanical reconstruction of phase-coherent waves. The purpose of this study is to characterize the ``acoustic showerglass'' in general optical terms and make a rough practical assessment of its impact on local seismic diagnostics of the shallow subphotospheres of active regions. We compile statistics comparing the acoustic field in magnetic photospheres with holographic projections of waves arriving from distant surrounding pupils. These ``local control correlations'' are consistent with an acoustic anomaly in the shallow subphotosphere of the active region that is strong but predominantly superficial; we call this the ``acoustic Wilson depression.'' The local control correlations also exhibit a phenomenon we call the ``penumbral acoustic anomaly,'' characterized by a conspicuous phase shift in regions of inclined magnetic field. This appears to be consistent with a fairly straightforward hydromechanical interpretation of the interaction of acoustic waves with photospheric magnetic forces. Detailed numerical simulations of the interaction of acoustic waves with magnetic forces can greatly facilitate our understanding of the acoustic showerglass and the thermal structure of the top few hundred kilometers of active region subphotospheres.},
  keywords = {activity-Sun,helioseismology-sunspots,notion,notion-database,Subject headings,Sun},
  file = {/Users/lbugnet/Zotero/storage/AFPUK8PK/full-text.pdf}
}

@article{Line2015,
  title = {Uniform {{Atmospheric Retrieval Analysis}} of {{Ultracool Dwarfs I}}: {{Characterizing Benchmarks}}, {{Gl570D}} and {{HD3651B}}},
  author = {Line, Michael R. and Teske, Johanna and Burningham, Ben and Fortney, Jonathan and Marley, Mark},
  year = {2015},
  month = apr,
  journal = {ApJ},
  volume = {807},
  number = {2},
  eprint = {1504.06670},
  pages = {183},
  doi = {10.1088/0004-637X/807/2/183},
  urldate = {2020-07-13},
  abstract = {Interpreting the spectra of brown dwarfs is key to determining the fundamental physical and chemical processes occurring in their atmospheres. Powerful Bayesian atmospheric retrieval tools have recently been applied to both exoplanet and brown dwarf spectra to tease out the thermal structures and molecular abundances to understand those processes. In this manuscript we develop a significantly upgraded retrieval method and apply it to the SpeX spectral library data of two benchmark late T-dwarfs, Gl570D and HD3651B, to establish the validity of our upgraded forward model parameterization and Bayesian estimator. Our retrieved metallicities, gravities, and effective temperature are consistent with the metallicity and presumed ages of the systems. We add the carbon-to-oxygen ratio as a new dimension to benchmark systems and find good agreement between carbon-to-oxygens ratio derived in the brown dwarfs and the host stars. Furthermore, we have for the first time unambiguously determined the presence of ammonia in the low-resolution spectra of these two late T-dwarfs. We also show that the retrieved results are not significantly impacted by the possible presence of clouds, though some quantities are significantly impacted by uncertainties in photometry. This investigation represents a watershed study in establishing the utility of atmospheric retrieval approaches on brown dwarf spectra.},
  archiveprefix = {arxiv},
  keywords = {brown dwarfs,HD 3651),notion,notion-database,radiative transfer,stars: abundances,stars: atmospheres,stars: individual (Gl 570},
  file = {/Users/lbugnet/Zotero/storage/KY3KUW99/full-text.pdf}
}

@article{Linsky2019,
  title = {Star-Planet Interactions},
  author = {Linsky, Jeffrey},
  year = {2019},
  journal = {Lecture Notes in Physics},
  volume = {955},
  eprint = {1408.6049},
  pages = {257--270},
  issn = {00758450},
  doi = {10.1007/978-3-030-11452-7_14},
  abstract = {In Chaps. 10 and 11, I surveyed the various ways in which a host star's radiation and wind can erode an exoplanet's atmosphere, change its chemistry, and thereby determine whether the exoplanet could be habitable. I now turn to the question of whether an exoplanet can change the properties of its host star, in particular, its rotation rate, UV and X-ray radiation, and the properties of its wind. The study of this feedback of an exoplanet on its host star is usually called star-planet interactions (SPI), although a more accurate term would be planet-star interactions.},
  archiveprefix = {arxiv},
  keywords = {low-mass,notion,notion-database,planet-star interactions,planetary systems,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/XGVFSZHH/Linsky - 2019.pdf}
}

@article{Lissauer2011a,
  title = {A Closely Packed System of Low-Mass, Low-Density Planets Transiting {{Kepler-11}}},
  author = {Lissauer, Jack J. and Fabrycky, Daniel C. and Ford, Eric B. and Borucki, William J. and Fressin, Francois and Marcy, Geoffrey W. and Orosz, Jerome A. and Rowe, Jason F. and Torres, Guillermo and Welsh, William F. and Batalha, Natalie M. and Bryson, Stephen T. and Buchhave, Lars A. and Caldwell, Douglas A. and Carter, Joshua A. and Charbonneau, David and Christiansen, Jessie L. and Cochran, William D. and Desert, Jean Michel and Dunham, Edward W. and Fanelli, Michael N. and Fortney, Jonathan J. and Gautier, Thomas N. and Geary, John C. and Gilliland, Ronald L. and Haas, Michael R. and Hall, Jennifer R. and Holman, Matthew J. and Koch, David G. and Latham, David W. and Lopez, Eric and McCauliff, Sean and Miller, Neil and Morehead, Robert C. and Quintana, Elisa V. and Ragozzine, Darin and Sasselov, Dimitar and Short, Donald R. and Steffen, Jason H.},
  year = {2011},
  journal = {Nature},
  volume = {470},
  number = {7332},
  pages = {53--58},
  publisher = {{Nature Publishing Group}},
  issn = {00280836},
  doi = {10.1038/nature09760},
  abstract = {When an extrasolar planet passes in front of (transits) its star, its radius can be measured from the decrease in starlight and its orbital period from the time between transits. Multiple planets transiting the same star reveal much more: period ratios determine stability and dynamics, mutual gravitational interactions reflect planet masses and orbital shapes, and the fraction of transiting planets observed as multiples has implications for the planarity of planetary systems. But few stars have more than one known transiting planet, and none has more than three. Here we report Kepler spacecraft observations of a single Sun-like star, which we call Kepler-11, that reveal six transiting planets, five with orbital periods between 10 and 47days and a sixth planet with a longer period. The five inner planets are among the smallest for which mass and size have both been measured, and these measurements imply substantial envelopes of light gases. The degree of coplanarity and proximity of the planetary orbits imply energy dissipation near the end of planet formation. \textcopyright{} 2011 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TIYUZGCB/Lissauer et al. - 2011.pdf}
}

@article{Lockwood2007a,
  title = {Patterns of {{Photometric}} and {{Chromospheric Variation}} among {{Sun}}-like {{Stars}}: {{A}} 20 {{Year Perspective}}},
  author = {Lockwood, G. W. and Skiff, B. A. and Henry, Gregory W. and Henry, Stephen and Radick, R. R. and Baliunas, S. L. and Donahue, R. A. and Soon, W.},
  year = {2007},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {171},
  number = {1},
  pages = {260--303},
  issn = {0067-0049},
  doi = {10.1086/516752},
  abstract = {We examine patterns of variation of 32 primarily main-sequence Sun-like stars [selected at project onset as stars on or near the main sequence and color index 0.42 {$\leq$} (B - V) {$\leq$} 1.4], extending our previous 7-12 yr time series to 13-20 yr by combining Str\"omgren b, y photometry from Lowell Observatory with similar data from Fairborn Observatory. Parallel chromospheric Ca II H and K emission data from the Mount Wilson Observatory span the entire interval. The extended data strengthen the relationship between chromospheric and brightness variability at visible wavelengths derived previously. We show that the full range of photometric variation has probably now been observed for a majority of the program stars. Twenty-seven stars are deemed variable according to an objective statistical criterion. On a year-to-year timescale, young active stars become fainter when their Ca n emission increases, while older less active stars such as the Sun become brighter when their Ca .emission increases. The Sun's total irradiance variation, scaled to the b and y stellar filter photometry, still appears to be somewhat smaller than stars in our limited sample with similar mean chromospheric activity, but we now regard this discrepancy as probably due mainly to our limited stellar sample. \textcopyright{} 2007. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/55XDTH8W/Lockwood et al. - 2007.pdf}
}

@article{Lognonne2014,
  title = {{{SEIS}}/{{INSIGHT}} and {{Mars}} Seismology: {{Development}} Status and Focus on the {{Impact}} Detection},
  author = {Lognonne, Philippe and Banerdt, William and Pike, Tom and Giardini, Domenico and Christensen, Ulli and Banfield, Don and Mimoun, David and Laudet, Philippe and {de Raucourt}, Sebastien and Bierwirth, Marco and Zweifel, Peter and Calcutt, Simon and Hurst, Ken and Bruce, Carl},
  year = {2014},
  journal = {EGUGA},
  pages = {12183},
  urldate = {2020-03-07},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/45WQYP59/full-text.pdf}
}

@article{Lognonne2019,
  title = {{{SEIS}}: {{Insight}}'s {{Seismic Experiment}} for {{Internal Structure}} of {{Mars}}},
  author = {Lognonn{\'e}, P. and Banerdt, W. B. and Giardini, D. and Pike, W. T. and Christensen, U. and Laudet, P. and {de Raucourt}, S. and Zweifel, P. and Calcutt, S. and Bierwirth, M. and Hurst, K. J. and Ijpelaan, F. and Umland, J. W. and {Llorca-Cejudo}, R. and Larson, S. A. and Garcia, R. F. and Kedar, S. and {Knapmeyer-Endrun}, B. and Mimoun, D. and Mocquet, A. and Panning, M. P. and Weber, R. C. and {Sylvestre-Baron}, A. and Pont, G. and Verdier, N. and Kerjean, L. and Facto, L. J. and Gharakanian, V. and Feldman, J. E. and Hoffman, T. L. and Klein, D. B. and Klein, K. and Onufer, N. P. and {Paredes-Garcia}, J. and Petkov, M. P. and Willis, J. R. and Smrekar, S. E. and Drilleau, M. and Gabsi, T. and Nebut, T. and Robert, O. and Tillier, S. and Moreau, C. and Parise, M. and Aveni, G. and Ben Charef, S. and Bennour, Y. and Camus, T. and Dandonneau, P. A. and Desfoux, C. and Lecomte, B. and Pot, O. and Revuz, P. and Mance, D. and TenPierick, J. and Bowles, N. E. and Charalambous, C. and Delahunty, A. K. and Hurley, J. and Irshad, R. and Liu, Huafeng and Mukherjee, A. G. and Standley, I. M. and Stott, A. E. and Temple, J. and Warren, T. and Eberhardt, M. and Kramer, A. and K{\"u}hne, W. and Miettinen, E. P. and Monecke, M. and Aicardi, C. and Andr{\'e}, M. and Baroukh, J. and Borrien, A. and Bouisset, A. and Boutte, P. and Brethom{\'e}, K. and Brysbaert, C. and Carlier, T. and Deleuze, M. and Desmarres, J. M. and Dilhan, D. and Doucet, C. and Faye, D. and {Faye-Refalo}, N. and Gonzalez, R. and Imbert, C. and Larigauderie, C. and Locatelli, E. and Luno, L. and Meyer, J. R. and Mialhe, F. and Mouret, J. M. and Nonon, M. and Pahn, Y. and Paillet, A. and Pasquier, P. and Perez, G. and Perez, R. and Perrin, L. and Pouilloux, B. and Rosak, A. and {Savin de Larclause}, I. and Sicre, J. and Sodki, M. and Toulemont, N. and Vella, B. and Yana, C. and Alibay, F. and Avalos, O. M. and Balzer, M. A. and Bhandari, P. and Blanco, E. and Bone, B. D. and Bousman, J. C. and Bruneau, P. and Calef, F. J. and Calvet, R. J. and D'Agostino, S. A. and {de los Santos}, G. and Deen, R. G. and Denise, R. W. and Ervin, J. and Ferraro, N. W. and Gengl, H. E. and Grinblat, F. and Hernandez, D. and Hetzel, M. and Johnson, M. E. and Khachikyan, L. and Lin, J. Y. and Madzunkov, S. M. and Marshall, S. L. and Mikellides, I. G. and Miller, E. A. and Raff, W. and Singer, J. E. and Sunday, C. M. and Villalvazo, J. F. and Wallace, M. C. and Banfield, D. and {Rodriguez-Manfredi}, J. A. and Russell, C. T. and {Trebi-Ollennu}, A. and Maki, J. N. and Beucler, E. and B{\"o}se, M. and Bonjour, C. and Berenguer, J. L. and Ceylan, S. and Clinton, J. and Conejero, V. and Daubar, I. and Dehant, V. and Delage, P. and Euchner, F. and Est{\`e}ve, I. and Fayon, L. and Ferraioli, L. and Johnson, C. L. and {Gagnepain-Beyneix}, J. and Golombek, M. and Khan, A. and Kawamura, T. and Kenda, B. and Labrot, P. and Murdoch, N. and Pardo, C. and Perrin, C. and Pou, L. and Sauron, A. and Savoie, D. and St{\"a}hler, S. and Stutzmann, E. and Teanby, N. A. and Tromp, J. and {van Driel}, M. and Wieczorek, M. and {Widmer-Schnidrig}, R. and Wookey, J.},
  year = {2019},
  month = jan,
  journal = {Space Science Reviews},
  volume = {215},
  number = {1},
  pages = {12},
  publisher = {{Springer Netherlands}},
  issn = {15729672},
  doi = {10.1007/s11214-018-0574-6},
  urldate = {2020-03-07},
  abstract = {By the end of 2018, 42 years after the landing of the two Viking seismometers on Mars, InSight will deploy onto Mars' surface the SEIS (Seismic Experiment for Internal Structure) instrument; a six-axes seismometer equipped with both a long-period three-axes Very Broad Band (VBB) instrument and a three-axes short-period (SP) instrument. These six sensors will cover a broad range of the seismic bandwidth, from 0.01 Hz to 50 Hz, with possible extension to longer periods. Data will be transmitted in the form of three continuous VBB components at 2 sample per second (sps), an estimation of the short period energy content from the SP at 1 sps and a continuous compound VBB/SP vertical axis at 10 sps. The continuous streams will be augmented by requested event data with sample rates from 20 to 100 sps. SEIS will improve upon the existing resolution of Viking's Mars seismic monitoring by a factor of {$\sim$} 2500 at 1 Hz and {$\sim$}200000 at 0.1 Hz. An additional major improvement is that, contrary to Viking, the seismometers will be deployed via a robotic arm directly onto Mars' surface and will be protected against temperature and wind by highly efficient thermal and wind shielding. Based on existing knowledge of Mars, it is reasonable to infer a moment magnitude detection threshold of M w {$\sim$} 3 at 40 {$\circ$} epicentral distance and a potential to detect several tens of quakes and about five impacts per year. In this paper, we first describe the science goals of the experiment and the rationale used to define its requirements. We then provide a detailed description of the hardware, from the sensors to the deployment system and associated performance, including transfer functions of the seismic sensors and temperature sensors. We conclude by describing the experiment ground segment, including data processing services, outreach and education networks and provide a description of the format to be used for future data distribution.},
  keywords = {InSight,Mars seismology,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NEU7GNM4/full-text.pdf}
}

@article{Loi2017,
  title = {Torsional {{Alfv\'en}} Resonances as an Efficient Damping Mechanism for Non-Radial Oscillations in Red Giant Stars},
  author = {Loi, Shyeh Tjing and Papaloizou, John C. B.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {3225},
  eprint = {1701.08771},
  pages = {3212--3225},
  issn = {0035-8711},
  doi = {10.1093/mnras/stx281},
  abstract = {Stars are self-gravitating fluids in which pressure, buoyancy, rotation and magnetic fields provide the restoring forces for global modes of oscillation. Pressure and buoyancy energetically dominate, while rotation and magnetism are generally assumed to be weak perturbations and often ignored. However, observations of anomalously weak dipole mode amplitudes in red giant stars suggest that a substantial fraction of these are subject to an additional source of damping localised to their core region, with indirect evidence pointing to the role of a deeply buried magnetic field. It is also known that in many instances the gravity-mode character of affected modes is preserved, but so far no effective damping mechanism has been proposed that accommodates this aspect. Here we present such a mechanism, which damps the oscillations of stars harbouring magnetised cores via resonant interactions with standing Alfv\textbackslash 'en modes of high harmonic index. The damping rates produced by this mechanism are quantitatively on par with those associated with turbulent convection, and in the range required to explain observations, for realistic stellar models and magnetic field strengths. Our results suggest that magnetic fields can provide an efficient means of damping stellar oscillations without needing to disrupt the internal structure of the modes, and lay the groundwork for an extension of the theory of global stellar oscillations that incorporates these effects.},
  archiveprefix = {arxiv},
  keywords = {analytical,interiors,magnetic field,methods,mhd,notion,notion-database,stars},
  file = {/Users/lbugnet/Zotero/storage/K9JRC9XN/Loi, Papaloizou - 2017.pdf}
}

@article{Loi2018,
  title = {Effects of a Strong Magnetic Field on Internal Gravity Waves: Trapping, Phase Mixing, Reflection, and Dynamical Chaos},
  author = {Loi, Shyeh Tjing and Papaloizou, John C B},
  year = {2018},
  month = jul,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {477},
  number = {4},
  eprint = {1804.03664},
  pages = {5338--5357},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/sty917},
  urldate = {2020-06-06},
  abstract = {The spectrum of oscillation modes of a star provides information not only about its material properties (e.g. mean density), but also its symmetries. Spherical symmetry can be broken by rotation and/or magnetic fields. It has been postulated that strong magnetic fields in the cores of some red giants are responsible for their anomalously weak dipole mode amplitudes (the "dipole dichotomy" problem), but a detailed understanding of how gravity waves interact with strong fields is thus far lacking. In this work, we attack the problem through a variety of analytical and numerical techniques, applied to a localised region centred on a null line of a confined axisymmetric magnetic field which is approximated as being cylindrically symmetric. We uncover a rich variety of phenomena that manifest when the field strength exceeds a critical value, beyond which the symmetry is drastically broken by the Lorentz force. When this threshold is reached, the spatial structure of the g-modes becomes heavily altered. The dynamics of wave packet propagation transitions from regular to chaotic, which is expected to fundamentally change the organisation of the mode spectrum. In addition, depending on their frequency and the orientation of field lines with respect to the stratification, waves impinging on different parts of the magnetised region are found to undergo either reflection or trapping. Trapping regions provide an avenue for energy loss through Alfven wave phase mixing. Our results may find application in various astrophysical contexts, including the dipole dichotomy problem, the solar interior, and compact star oscillations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/EGYCU38T/Loi, Papaloizou - 2018.pdf}
}

@article{Loi2019,
  title = {Low-Degree Mixed Modes in Red Giant Stars with Moderate Core Magnetic Fields},
  author = {Loi, Shyeh Tjing and Papaloizou, John C B},
  year = {2020},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {491},
  number = {1},
  eprint = {1910.09940v1},
  pages = {1--18},
  urldate = {2020-01-24},
  abstract = {Observations of pressure-gravity mixed modes, combined with a theoretical framework for understanding mode formation, can yield a wealth of information about deep stellar interiors. In this paper, we seek to develop a formalism for treating the effects of deeply buried core magnetic fields on mixed modes in evolved stars, where the fields are moderate, i.e. not strong enough to disrupt wave propagation, but where they may be too strong for non-degenerate first-order perturbation theory to be applied. The magnetic field is incorporated in a way that avoids having to use this. Inclusion of the Lorentz force term is shown to yield a system of differential equations that allows for the magnetically-affected eigenfunctions to be computed from scratch, rather than following the approach of first-order perturbation theory. For sufficiently weak fields, coupling between different spherical harmonics can be neglected, allowing for reduction to a second-order system of ordinary differential equations akin to the usual oscillation equations that can be solved analogously. We derive expressions for (i) the mixed-mode quantisation condition in the presence of a field and (ii) the frequency shift associated with the magnetic field. In addition, for modes of low degree we uncover an extra offset term in the quantisation condition that is sensitive to properties of the evanescent zone. These expressions may be inverted to extract information about the stellar structure and magnetic field from observational data.},
  archiveprefix = {arxiv},
  keywords = {analytical-stars,interiors-stars,magnetic field-stars,MHD-methods,notion,notion-database,oscillations},
  file = {/Users/lbugnet/Zotero/storage/6GWXGILA/full-text.pdf}
}

@article{Loi2020,
  title = {Effect of a Strong Magnetic Field on Gravity-Mode Period Spacings in Red Giant Stars},
  author = {Loi, Shyeh Tjing},
  year = {2020},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {496},
  number = {3},
  eprint = {2006.08635},
  pages = {3829--3840},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/MNRAS/STAA1823},
  urldate = {2022-01-06},
  abstract = {When a star evolves into a red giant, the enhanced coupling between core-based gravity modes and envelope-based pressure modes forms mixed modes, allowing its deep interior to be probed by asteroseismology. The ability to obtain information about stellar interiors is important for constraining theories of stellar structure and evolution, for which the origin of various discrepancies between prediction and observation is still under debate. Ongoing speculation surrounds the possibility that some red giant starsmay harbour strong (dynamically significant) magnetic fields in their cores, but interpretation of the observational data remains controversial. In part, this is tied to shortfalls in our understanding of the effects of strong fields on the seismic properties of gravity modes, which lies beyond the regime of standard perturbative methods. Here, we seek to investigate the effect of a strong magnetic field on the asymptotic period spacings of gravity modes. We use a Hamiltonian ray approach to measure the volume of phase space occupied by mode-forming rays, this being roughly proportional to the average density of modes (number of modes per unit frequency interval). A strong field appears to systematically increase this by about 10 per cent, which predicts a {$\sim$}10 per cent smaller period spacing. Evidence of near integrability in the ray dynamics hints that the gravity-mode spectrum may still exhibit pseudo-regularities under a strong field.},
  archiveprefix = {arxiv},
  keywords = {Methods: Numerical,Mhd-waves,notion,notion-database,Stars: Interiors,Stars: Magnetic field},
  file = {/Users/lbugnet/Zotero/storage/YDN7S48K/2006.08635.pdf}
}

@article{Loi2021,
  title = {Topology and Obliquity of Core Magnetic Fields in Shaping Seismic Properties of Slowly Rotating Evolved Stars},
  author = {Loi, Shyeh Tjing},
  year = {2021},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {504},
  pages = {3711--3729},
  doi = {10.1093/mnras/stab991},
  urldate = {2021-10-20},
  abstract = {It is thought that magnetic fields must be present in the interiors of stars to resolve certain discrepancies between theory and observation (e.g. angular momentum transport), but such fields are difficult to detect and characterize. Asteroseismology is a powerful technique for inferring the internal structures of stars by measuring their oscillation frequencies, and succeeds particularly with evolved stars, owing to their mixed modes, which are sensitive to the deep interior. The goal of this work is to present a phenomenological study of the combined effects of rotation and magnetism in evolved stars, where both are assumed weak enough that first-order perturbation theory applies, and we focus on the regime where Coriolis and Lorentz forces are comparable. Axisymmetric 'twisted-torus' field configurations are used, which are confined to the core and allowed to be misaligned with respect to the rotation axis. Factors such as the field radius, topology and obliquity are examined. We observe that fields with finer-scale radial structure and/or smaller radial extent produce smaller contributions to the frequency shift. The interplay of rotation and magnetism is shown to be complex: we demonstrate that it is possible for nearly symmetric multiplets of apparently low multiplicity to arise even under a substantial field, which might falsely appear to rule out its presence. Our results suggest that proper modelling of rotation and magnetism, in a simultaneous fashion, may be required to draw robust conclusions about the existence/non-existence of a core magnetic field in any given object.},
  keywords = {(magnetohydrodynamics) MHD-methods,interiors-stars,magnetic field,magnetic field-waves,MHD-methods,notion,notion-database,numerical-stars,numerical-waves-stars},
  file = {/Users/lbugnet/Zotero/storage/IJWI45LG/full-text.pdf;/Users/lbugnet/Zotero/storage/ZL9NEYT8/stab991.pdf}
}

@article{Lomb1976,
  title = {Least-Squares Frequency Analysis of Unequally Spaced Data},
  author = {Lomb, N. R.},
  year = {1976},
  month = feb,
  journal = {Astrophysics and Space Science},
  volume = {39},
  number = {2},
  pages = {447--462},
  publisher = {{Kluwer Academic Publishers}},
  issn = {0004640X},
  doi = {10.1007/BF00648343},
  urldate = {2020-04-09},
  abstract = {The statistical properties of least-squares frequency analysis of unequally spaced data are examined. It is shown that, in the least-squares spectrum of gaussian noise, the reduction in the sum of squares at a particular frequency is a X22 variable. The reductions at different frequencies are not independent, as there is a correlation between the height of the spectrum at any two frequencies, f1 and f2, which is equal to the mean height of the spectrum due to a sinusoidal signal of frequency f1, at the frequency f2. These correlations reduce the distortion in the spectrum of a signal affected by noise. Some numerical illustrations of the properties of least-squares frequency spectra are also given. \textcopyright{} 1976 D. Reidel Publishing Company.},
  keywords = {Astronomy,Background Noise,Data Reduction,Least Squares Method,notion,notion-database,Power Spectra,Sine Waves,Spectrum Analysis,Statistical Analysis,Variable Stars}
}

@article{Lopes2010,
  title = {Probing the Existence of a Dark Matter Isothermal Core Using Gravity Modes},
  author = {Lopes, Il{\'i}dio and Silk, Joseph},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {722},
  number = {1 PART 2},
  eprint = {1009.5122},
  issn = {20418213},
  doi = {10.1088/2041-8205/722/1/L95},
  abstract = {Although helioseismology has been used as an effective tool for studying the physical mechanisms acting in most of the solar interior, the microscopic level and the dynamics of the deep core are still not well understood. Helioseismological anomalies may be partially resolved if the Sun captures light, non-annihilating dark matter particles, a currently discussed dark matter candidate that is motivated by recent direct detection limits. Once trapped, such particles (4-10 GeV) naturally fill the solar core.With the use of a well-defined stellar evolution code that takes into account an accurate description of the capture of dark matter particles by the Sun, we investigate the impact of such particles in its inner core. Even a relatively small amount of dark matter particles in the solar core will leave an imprint on the absolute frequency values of gravity modes as well as the equidistant spacing between modes of the same degree. The period separation for gravity modes could reveal changes of up to 3\% for annihilating dark matter and of up to 20\% for non-annihilating dark matter. This effect is most pronounced in the case of the gravity dipole (l = 1) modes. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Dark matter,Elementary particles,notion,notion-database,Stars: evolution,Stars: interiors,Sun: helioseismology,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/ML8SRFAA/Lopes, Silk - 2010.pdf}
}

@article{Lopes2010b,
  title = {Neutrino Spectroscopy Can Probe the Dark Matter Content in the Sun},
  author = {Lopes, Il{\'i}dio and Silk, Joseph},
  year = {2010},
  journal = {Science},
  volume = {330},
  number = {6003},
  pages = {462},
  issn = {00368075},
  doi = {10.1126/science.1196564},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/44RKZVJ3/Lopes, Silk - 2010(2).pdf}
}

@article{Lopez-Santiago2010a,
  title = {A High-Resolution Spectroscopic Survey of Late-Type Stars: {{Chromospheric}} Activity, Rotation, Kinematics, and Age},
  author = {{L{\'o}pez-Santiago}, J. and Montes, D. and {G{\'a}lvez-Ortiz}, M. C. and {Crespo-Chac{\'o}n}, I. and {Mart{\'i}nez-Arn{\'a}iz}, R. M. and {Fern{\'a}ndez-Figueroa}, M. J. and De Castro, E. and Cornide, M.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {514},
  number = {14},
  issn = {14320746},
  doi = {10.1051/0004-6361/200913437},
  abstract = {Aims. We present a compilation of spectroscopic data from a survey of 144 chromospherically active young stars in the solar neighborhood, which may be used to investigate different aspects of its formation and evolution in terms of kinematics and stellar formation history. The data have already been used by us in several studies. With this paper, we make all these data accessible to the scientific community for future studies on different topics. Methods. We performed spectroscopic observations with echelle spectrographs to cover the entirety of the optical spectral range simultaneously. Standard data reduction was performed with the IRAF echelle package. We applied the spectral subtraction technique to reveal chromospheric emission in the stars of the sample. The equivalent width of chromospheric emission lines was measured in the subtracted spectra and then converted to fluxes using equivalent width-flux relationships. Radial and rotational velocities were determined by the cross-correlation technique. Kinematics, equivalent widths of the lithium line {$\lambda$}6707.8 \AA{} and spectral types were also determined. Results. A catalog of spectroscopic data is compiled: radial and rotational velocities, space motion, equivalent widths of optical chromospheric activity indicators from Ca II H \& K to the calcium infrared triplet and the lithium line in {$\lambda$}6708 \AA. Fluxes in the chromospheric emission lines and RHK are also determined for each observation of a star in the sample. We used these data to investigate the emission levels of our stars. The study of the H{$\alpha$} emission line revealed two different populations of chromospheric emitters in the sample, clearly separated in the logFH\textbackslash alpha/Fbol-(V-J) diagram. The dichotomy may be associated with the age of the stars. \textcopyright{} ESO, 2010.},
  keywords = {Galaxy: stellar content,notion,notion-database,Solar neighborhood,Stars: activity,Stars: chromospheres,Stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/RW88NLTW/López-Santiago et al. - 2010.pdf}
}

@article{Lopez2021,
  title = {Discovery, {{TESS Characterization}}, and {{Modeling}} of {{Pulsations}} in the {{Extremely Low-mass White Dwarf GD}} 278},
  author = {Lopez, Isaac D. and Hermes, J. J. and Calcaferro, Leila M. and Bell, Keaton J. and Samuels, Adam and Vanderbosch, Zachary P. and C{\'o}rsico, Alejandro H. and Istrate, Alina G.},
  year = {2021},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {922},
  pages = {220},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac2d28},
  urldate = {2023-10-02},
  abstract = {We report the discovery of pulsations in the extremely low-mass (ELM), likely helium-core white dwarf GD 278 via ground- and space-based photometry. GD 278 was observed by the Transiting Exoplanet Survey Satellite (TESS) in Sector 18 at a 2 minute cadence for roughly 24 days. The TESS data reveal at least 19 significant periodicities between 2447 and 6729 s, one of which is the longest pulsation period ever detected in a white dwarf. Previous spectroscopy found that this white dwarf is in a 4.61 hr orbit with an unseen {$>$}0.4 M {$\odot$} companion and has T eff = 9230 {$\pm$} 100 K and \$\textbackslash mathrm\{log\}g=6.627\textbackslash pm 0.056\$ , which corresponds to a mass of 0.191 {$\pm$} 0.013 M {$\odot$}. Patterns in the TESS pulsation frequencies from rotational splittings appear to reveal a stellar rotation period of roughly 10 hr, making GD 278 the first ELM white dwarf with a measured rotation rate. The patterns inform our mode identification for asteroseismic fits, which, unfortunately, do not reveal a global best-fit solution. Asteroseismology reveals two main solutions roughly consistent with the spectroscopic parameters of this ELM white dwarf, but with vastly different hydrogen-layer masses; future seismic fits could be further improved by using the stellar parallax. GD 278 is now the tenth known pulsating ELM white dwarf; it is only the fifth known to be in a short-period binary, but is the first with extended, space-based photometry.},
  keywords = {1625,1799,1847,73,Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2021ApJ...922..220L},
  file = {/Users/lbugnet/Zotero/storage/8H9THMI2/Lopez et al. - 2021 - Discovery, TESS Characterization, and Modeling of .pdf}
}

@article{Lopez2021a,
  title = {Discovery, {{TESS Characterization}}, and {{Modeling}} of {{Pulsations}} in the {{Extremely Low-mass White Dwarf GD}} 278},
  author = {Lopez, Isaac D. and Hermes, J. J. and Calcaferro, Leila M. and Bell, Keaton J. and Samuels, Adam and Vanderbosch, Zachary P. and C{\'o}rsico, Alejandro H. and Istrate, Alina G.},
  year = {2021},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {922},
  pages = {220},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac2d28},
  urldate = {2023-10-09},
  abstract = {We report the discovery of pulsations in the extremely low-mass (ELM), likely helium-core white dwarf GD 278 via ground- and space-based photometry. GD 278 was observed by the Transiting Exoplanet Survey Satellite (TESS) in Sector 18 at a 2 minute cadence for roughly 24 days. The TESS data reveal at least 19 significant periodicities between 2447 and 6729 s, one of which is the longest pulsation period ever detected in a white dwarf. Previous spectroscopy found that this white dwarf is in a 4.61 hr orbit with an unseen {$>$}0.4 M {$\odot$} companion and has T eff = 9230 {$\pm$} 100 K and \$\textbackslash mathrm\{log\}g=6.627\textbackslash pm 0.056\$ , which corresponds to a mass of 0.191 {$\pm$} 0.013 M {$\odot$}. Patterns in the TESS pulsation frequencies from rotational splittings appear to reveal a stellar rotation period of roughly 10 hr, making GD 278 the first ELM white dwarf with a measured rotation rate. The patterns inform our mode identification for asteroseismic fits, which, unfortunately, do not reveal a global best-fit solution. Asteroseismology reveals two main solutions roughly consistent with the spectroscopic parameters of this ELM white dwarf, but with vastly different hydrogen-layer masses; future seismic fits could be further improved by using the stellar parallax. GD 278 is now the tenth known pulsating ELM white dwarf; it is only the fifth known to be in a short-period binary, but is the first with extended, space-based photometry.},
  keywords = {1625,1799,1847,73,Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2021ApJ...922..220L},
  file = {/Users/lbugnet/Zotero/storage/67CYG2GE/Lopez et al. - 2021 - Discovery, TESS Characterization, and Modeling of .pdf}
}

@article{Loptien2018,
  title = {Global-Scale Equatorial {{Rossby}} Waves as an Essential Component of Solar Internal Dynamics},
  author = {L{\"o}ptien, Bj{\"o}rn and Gizon, Laurent and Birch, Aaron C. and Schou, Jesper and Proxauf, Bastian and Duvall, Thomas L. and Bogart, Richard S. and Christensen, Ulrich R.},
  year = {2018},
  month = jul,
  journal = {Nature Astronomy},
  volume = {2},
  number = {7},
  eprint = {1805.07244},
  pages = {568--573},
  publisher = {{Nature Publishing Group}},
  issn = {23973366},
  doi = {10.1038/s41550-018-0460-x},
  urldate = {2022-04-05},
  abstract = {The Sun's complex dynamics is controlled by buoyancy and rotation in the convection zone. Large-scale flows are dominated by vortical motions and appear to be weaker than expected in the solar interior. One possibility is that waves of vorticity due to the Coriolis force, known as Rossby waves or r modes, remove energy from convection at the largest scales. However, the presence of these waves in the Sun is still debated. Here, we unambiguously discover and characterize retrograde-propagating vorticity waves in the shallow subsurface layers of the Sun at azimuthal wavenumbers below 15, with the dispersion relation of textbook sectoral Rossby waves. The waves have lifetimes of several months, well-defined mode frequencies below twice the solar rotational frequency, and eigenfunctions of vorticity that peak at the equator. Rossby waves have nearly as much vorticity as the convection at the same scales, thus they are an essential component of solar dynamics. We observe a transition from turbulence-like to wave-like dynamics around the Rhines scale of angular wavenumber of approximately 20. This transition might provide an explanation for the puzzling deficit of kinetic energy at the largest spatial scales.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics}
}

@article{Luan2018,
  title = {{{DAVs}}: {{Red Edge}} and {{Outbursts}}},
  shorttitle = {{{DAVs}}},
  author = {Luan, Jing and Goldreich, Peter},
  year = {2018},
  month = aug,
  journal = {The Astrophysical Journal},
  volume = {863},
  pages = {82},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/aad0f4},
  urldate = {2023-10-14},
  abstract = {As established by photometric surveys, white dwarfs with hydrogen atmospheres and surface gravity, log(g) {$\approx$} 8.0 pulsate as they cool across the temperature range of 12,500 K {$\greaterequivlnt$} T eff {$\greaterequivlnt$} 10,800 K. Known as DAVs or ZZ Ceti stars, their oscillations are attributed to gravity modes excited by convective driving. Overstability requires convective driving to exceed radiative damping. Previous works have demonstrated that {$\omega$} {$\greaterequivlnt$} max({$\tau$} c -1, L {$\mathscr{l}$},b ) is a necessary and sufficient condition for overstability. Here {$\tau$} c and L {$\mathscr{l}$},b are the effective thermal timescale and Lamb frequency at the base of the surface convection zone. Below the observational red edge, L {$\mathscr{l}$},b {$\gg$} {$\tau$} c -1, so overstable modes all have {$\omega\tau$} c {$\gg$} 1. Consequently, their photometric amplitudes are reduced by that large factor rendering them difficult to detect. Although proposed previously, the condition {$\omega$} {$\greaterequivlnt$} L {$\mathscr{l}$},b has not been clearly interpreted. We show that modes with {$\omega$} {$<$} L {$\mathscr{l}$},b suffer enhanced radiative damping that exceeds convective driving rendering them damped. A quasi-adiabatic analysis is adequate to account for this enhancement. Although this approximation is only marginally valid at the red edge, it becomes increasingly accurate toward both higher and lower \{T\}eff\vphantom\{\}. Recently, Kepler discovered a number of cool DAVs that exhibit sporadic flux outbursts. Typical outbursts last several hours, are separated by days, and release {$\sim$}1033-1034 erg. We attribute outbursts to limit cycles arising from sufficiently resonant 3-mode couplings between overstable parent modes and pairs of radiatively damped daughter modes. Limit cycles account for the durations and energies of outbursts and their prevalence near the red edge of the DAV instability strip.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,instabilities,stars: activity,stars: oscillations,white dwarfs},
  annotation = {ADS Bibcode: 2018ApJ...863...82L},
  file = {/Users/lbugnet/Zotero/storage/2Z3ZY55D/Luan and Goldreich - 2018 - DAVs Red Edge and Outbursts.pdf}
}

@article{Ludwig2009,
  title = {Special Feature {{Hydrodynamical}} Simulations of Convection-Related Stellar},
  author = {Ludwig, H},
  year = {2009},
  volume = {173},
  pages = {167--173},
  keywords = {atmospheres,convection,hd 49933,hydrodynamics,individual,late-type,methods,notion,notion-database,numerical,stars},
  file = {/Users/lbugnet/Zotero/storage/3DWF92IV/Ludwig - 2009.pdf}
}

@article{Ludwig2009a,
  title = {Hydrodynamical Simulations of Convection-Related Stellar Micro-Variability. {{II}}. {{The}} Enigmatic Granulation Background of the {{COROT}} Target {{HD49933}}},
  author = {Ludwig, H. -G. and Samadi, R. and Steffen, M. and Appourchaux, T. and Baudin, F. and Belkacem, K. and Boumier, P. and Goupil, M. -J. and Michel, E.},
  year = {2009},
  month = may,
  eprint = {0905.2695},
  doi = {10.1051/0004-6361/200911930},
  urldate = {2020-03-15},
  abstract = {Local-box hydrodynamical model atmospheres provide statistical information about a star's emergent radiation field which allows one to predict the level of its granulation-related micro-variability. Space-based photometry is now sufficiently accurate to test model predictions. We aim to model the photometric granulation background of HD49933 as well as the Sun, and compare the predictions to the measurements obtained by the COROT and SOHO satellite missions. We construct hydrodynamical model atmospheres representing HD49933 and the Sun, and use a previously developed scaling technique to obtain the observable disk-integrated brightness fluctuations. We further performed exploratory magneto-hydrodynamical simulations to gauge the impact of small scale magnetic fields on the synthetic light-curves. We find that the granulation-related brightness fluctuations depend on metallicity. We obtain a satisfactory correspondence between prediction and observation for the Sun, validating our approach. For HD49933, we arrive at a significant over-estimation by a factor of two to three in total power. Locally generated magnetic fields are unlikely to be responsible, otherwise existing fields would need to be rather strong to sufficiently suppress the granulation signal. Presently suggested updates on the fundamental stellar parameters do not improve the correspondence; however, an ad-hoc increase of the HD49933 surface gravity by about 0.2dex would eliminate most of the discrepancy. We diagnose a puzzling discrepancy between the predicted and observed granulation background in HD49933, with only rather ad-hoc ideas for remedies at hand.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SHH9NFGU/full-text.pdf}
}

@article{Luger2016,
  title = {{{EVEREST}}: {{Pixel Level Decorrelation}} of {{K2 Light}} Curves},
  author = {Luger, Rodrigo and Agol, Eric and Kruse, Ethan and Barnes, Rory and Becker, Andrew and {Foreman-Mackey}, Daniel and Deming, Drake},
  year = {2016},
  month = jul,
  journal = {AJ},
  volume = {152},
  number = {4},
  eprint = {1607.00524},
  pages = {100},
  doi = {10.3847/0004-6256/152/4/100},
  urldate = {2020-07-21},
  abstract = {We present EVEREST, an open-source pipeline for removing instrumental noise from K2 light curves. EVEREST employs a variant of pixel level decorrelation (PLD) to remove systematics introduced by the spacecraft's pointing error and a Gaussian process (GP) to capture astrophysical variability. We apply EVEREST to all K2 targets in campaigns 0-7, yielding light curves with precision comparable to that of the original Kepler mission for stars brighter than \$K\_p \textbackslash approx 13\$, and within a factor of two of the Kepler precision for fainter targets. We perform cross-validation and transit injection and recovery tests to validate the pipeline, and compare our light curves to the other de-trended light curves available for download at the MAST High Level Science Products archive. We find that EVEREST achieves the highest average precision of any of these pipelines for unsaturated K2 stars. The improved precision of these light curves will aid in exoplanet detection and characterization, investigations of stellar variability, asteroseismology, and other photometric studies. The EVEREST pipeline can also easily be applied to future surveys, such as the TESS mission, to correct for instrumental systematics and enable the detection of low signal-to-noise transiting exoplanets. The EVEREST light curves and the source code used to generate them are freely available online.},
  archiveprefix = {arxiv},
  keywords = {catalogs,notion,notion-database,planets and satellites: detection,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/3S53DRY6/full-text.pdf}
}

@article{Lund2012,
  title = {A New Method to Detect Solar-like Oscillations at Very Low {{S}}/{{N}} Using Statistical Significance Testing},
  author = {Lund, Mikkel N. and Chaplin, William J. and Kjeldsen, Hans},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {427},
  number = {2},
  pages = {1784--1792},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.22098.x},
  abstract = {We introduce a new method to detect solar-like oscillations in frequency power spectra of stellar observations, under conditions of very low signal-to-noise ratio. The Moving-Windowed-Power-Search (MWPS) searches the power spectrum for signatures of excess power, over and above slowly varying (in frequency) background contributions from stellar granulation and shot or instrumental noise. We adopt a false-alarm approach to ascertain whether flagged excess power, which is consistent with the excess expected from solar-like oscillations, is hard to explain by chance alone (and hence a candidate detection). We apply the method to solar photometry data, whose quality was systematically degraded to test the performance of the MWPS at low signal-to-noise ratios. We also compare the performance of the MWPS against the frequently applied power-spectrum-of-power-spectrum (PS{$\otimes$}PS) detection method. The MWPS is found to outperform the PS{$\otimes$}PS method. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/TB5CIWHY/Lund, Chaplin, Kjeldsen - 2012.pdf}
}

@article{Lund2014,
  title = {Detection of {$\mathscr{l}$} = 4 and {$\mathscr{l}$} = 5 Modes in 12 Years of Solar Virgo-Spm Data - {{Tests}} on Kepler Observations of 16 {{Cyg A}} and {{B}}},
  author = {Lund, Mikkel N{\o}rup and Kjeldsen, Hans and {Christensen-Dalsgaard}, J{\o}rgen and Handberg, Rasmus and Aguirre, Victor Silva},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {782},
  number = {1},
  eprint = {1401.7003},
  issn = {15384357},
  doi = {10.1088/0004-637X/782/1/2},
  abstract = {We present the detection of {$\mathscr{l}$} = 4 and {$\mathscr{l}$} = 5 modes in power spectra of the Sun, constructed from 12 yr full-disk VIRGO-SPM data sets. A method for enhancing the detectability of these modes in asteroseismic targets is presented and applied to Kepler data of the two solar analogues 16 Cyg A and B. For these targets, we see indications of a signal from {$\mathscr{l}$} = 4 modes, while nothing is yet seen for {$\mathscr{l}$} = 5 modes. We further simulate the power spectra of these stars and from this we estimate that it should indeed be possible to see such indications of {$\mathscr{l}$} = 4 modes at the present length of the data sets. In the simulation process, we briefly look into the apparent misfit between observed and calculated mode visibilities. We predict that firm detections of at least {$\mathscr{l}$} = 4 should be possible in any case at the end of the Kepler mission. For {$\mathscr{l}$} = 5, we do not predict any firm detections from Kepler data. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,{stars: individual (16Cyg A, 16 CygB)},stars: oscillations,stars: solar-type,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TAWYJABB/Lund et al. - 2014.pdf}
}

@article{Lund2014b,
  title = {Differential Rotation in Main-Sequence Solar-like Stars: {{Qualitative}} Inference from Asteroseismic Data},
  author = {Lund, Mikkel N. and Miesch, Mark S. and {Christensen-Dalsgaard}, J{\o}rgen},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {790},
  number = {2},
  eprint = {1406.7873},
  issn = {15384357},
  doi = {10.1088/0004-637X/790/2/121},
  abstract = {Understanding differential rotation of Sun-like stars is of great importance for insight into the angular momentum transport in these stars. One means of gaining such information is that of asteroseismology. By a forward modeling approach we analyze in a qualitative manner the impact of different differential rotation profiles on the splittings of p-mode oscillation frequencies. The optimum modes for inference on differential rotation are identified along with the best value of the stellar inclination angle. We find that in general it is not likely that asteroseismology can be used to make an unambiguous distinction between a rotation profile such as a conical Sun-like profile and a cylindrical profile. In addition, it seems unlikely that asteroseismology of Sun-like stars will result in inferences on the radial profile of the differential rotation, such as can be done for red giants. At best, one could possibly obtain the sign of the radial differential rotation gradient. Measurements of the extent of the latitudinal differential from frequency splitting are, however, more promising. One very interesting aspect that could likely be tested from frequency splittings is whether the differential rotation is solar-like or anti-solar-like in nature, in the sense that a solar-like profile has an equator rotating faster than the poles. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {analytical - stars,asteroseismology - methods,notion,notion-database,oscillations - stars,rotation - stars,solar-type},
  file = {/Users/lbugnet/Zotero/storage/IAYQY8KW/Lund, Miesch, Christensen-Dalsgaard - 2014.pdf}
}

@article{Lund2015,
  title = {{{K2P2}} - {{A PHOTOMETRY PIPELINE}} for the {{K2 MISSION}}},
  author = {Lund, Mikkel N. and Handberg, Rasmus and Davies, Guy R. and Chaplin, William J. and Jones, Caitlin D.},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {806},
  number = {1},
  eprint = {1504.05199},
  issn = {15384357},
  doi = {10.1088/0004-637X/806/1/30},
  abstract = {With the loss of a second reaction wheel, resulting in the inability to point continuously and stably at the same field of view, the NASA Kepler satellite recently entered a new mode of observation known as the K2 mission. The data from this redesigned mission present a specific challenge; the targets systematically drift in position on an {$\sim$}6 hr timescale, inducing a significant instrumental signal in the photometric time series - this greatly impacts the ability to detect planetary signals and perform asteroseismic analysis. Here we detail our version of a reduction pipeline for K2 target pixel data, which automaticallydefines masks for all targets in a given frame; extracts the target's fluxand position time series; corrects the time series based on the apparent movement on the CCD (either in 1D or 2D), combined with the correction of instrumental and/or planetary signals via the Kepler Asteroseismic Science Operations Center (KASOC) filter, thus rendering the time series ready for asteroseismic analysis; computes power spectra for all targets;and identifies potential contaminations between targets. From a test of our pipeline on a sample of targets from the K2 campaign 0, the recovery of data for multiple targets increases the amount of potential light curves by a factor of . Our pipeline could be applied to the upcoming TESS and PLATO 2.0 missions.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,stars: solar-type,techniques: image processing,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/D2H6HQ4E/Lund et al. - 2015.pdf}
}

@article{Lund2016a,
  title = {Asteroseismology of the Hyades with {{K2}}: {{First}} Detection of Main-Sequence Solar-like Oscillations in an Open Cluster},
  author = {Lund, Mikkel N. and Basu, Sarbani and Aguirre, V{\'i}ctor Silva and Chaplin, William J. and Serenelli, Aldo M. and Garcia, Rafael A. and Latham, David W. and Casagrande, Luca and Bieryla, Allyson and Davies, Guy R. and Viani, Lucas S. and Buchhave, Lars A. and Miglio, Andrea and Soderblom, David R. and Valenti, Jeff A. and Stefanik, Robert P. and Handberg, Rasmus},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {463},
  number = {3},
  eprint = {1608.07290},
  pages = {2600--2611},
  issn = {13652966},
  doi = {10.1093/mnras/stw2160},
  abstract = {The Hyades open cluster was targeted during Campaign 4 (C4) of the NASA K2 mission, and short-cadence data were collected on a number of cool main-sequence stars. Here, we report results on two F-type stars that show detectable oscillations of a quality that allows asteroseismic analyses to be performed. These are the first ever detections of solar-like oscillations in main-sequence stars in an open cluster.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Galaxies: star clusters: individual: hyades,Methods: data analysis,notion,notion-database,{Stars: individual: ePIC 210444167 (HIP 20357, vB 3},{Stars: individual: ePIC 210499243 (HIP 19877, vB 2},Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/EPNUYS9Y/Lund et al. - 2016.pdf}
}

@article{Lund2016c,
  title = {Asteroseismic Properties of Solar-Type Stars Observed with the {{NASA K2}} Mission: {{Results}} from Campaigns 1-3 and Prospects for Future Observations},
  author = {Lund, Mikkel N. and Chaplin, William J. and Casagrande, Luca and Aguirre, V{\'i}ctor Silva and Basu, Sarbani and Bieryla, Allyson and {Christensen-Dalsgaard}, J{\o}rgen and Latham, David W. and White, Timothy R. and Davies, Guy R. and Huber, Daniel and Buchhave, Lars A. and Handberg, Rasmus},
  year = {2016},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {128},
  number = {970},
  eprint = {1608.07292},
  issn = {00046280},
  doi = {10.1088/1538-3873/128/970/124204},
  abstract = {We present an asteroseismic analysis of 33 solar-type stars observed in short cadence (SC) during Campaigns (C) 1-3 of the NASA K2 mission. We were able to extract both average seismic parameters and individual mode frequencies for stars with dominant frequencies up to {$\sim$}3300 {$\mu$}Hz, and we find that data for some targets are good enough to allow for a measurement of the rotational splitting. Modeling of the extracted parameters is performed by using grid-based methods using average parameters and individual frequencies together with spectroscopic parameters. For the target selection in C3, stars were chosen as in C1 and C2 to cover a wide range in parameter space to better understand the performance and noise characteristics. For C3 we still detected oscillations in 73\% of the observed stars that we proposed. Future K2 campaigns hold great promise for the study of nearby clusters and the chemical evolution and age-metallicity relation of nearby field stars in the solar neighborhood. We expect oscillations to be detected in {$\sim$}388 SC targets if the K2 mission continues until C18, which will greatly complement the {$\sim$}500 detections of solar-like oscillations made for SC targets during the nominal Kepler mission. For {$\sim$}30-40 of these, including several members of the Hyades open cluster, we furthermore expect that inference from interferometry should be possible.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology-methods,Data analysis-stars,Distances-stars,Fundamental parameters-stars,notion,notion-database,Oscillations,Stars-solar-type},
  file = {/Users/lbugnet/Zotero/storage/XNDCX43M/Lund et al. - 2016(2).pdf}
}

@article{Lund2017,
  title = {Standing on the {{Shoulders}} of {{Dwarfs}}: The {{Kepler Asteroseismic LEGACY Sample}}. {{I}}. {{Oscillation Mode Parameters}}},
  author = {Lund, Mikkel N. and Aguirre, V{\'i}ctor Silva and Davies, Guy R. and Chaplin, William J. and {Christensen-Dalsgaard}, J{\o}rgen and Houdek, G{\"u}nter and White, Timothy R. and Bedding, Timothy R. and Ball, Warrick H. and Huber, Daniel and Antia, H. M. and Lebreton, Yveline and Latham, David W. and Handberg, Rasmus and Verma, Kuldeep and Basu, Sarbani and Casagrande, Luca and Justesen, Anders B. and Kjeldsen, Hans and Mosumgaard, Jakob R.},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {835},
  number = {2},
  eprint = {1612.00436},
  pages = {172},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/835/2/172},
  abstract = {\textcopyright{} 2017. The American Astronomical Society. All rights reserved. The advent of space-based missions like Kepler has revolutionized the study of solar-type stars, particularly through the measurement and modeling of their resonant modes of oscillation. Here we analyze a sample of 66 Kepler main-sequence stars showing solar-like oscillations as part of the Kepler seismic LEGACY project. We use Kepler short-cadence data, of which each star has at least 12 months, to create frequency-power spectra optimized for asteroseismology. For each star, we identify its modes of oscillation and extract parameters such as frequency, amplitude, and line width using a Bayesian Markov chain Monte Carlo "peak-bagging" approach. We report the extracted mode parameters for all 66 stars, as well as derived quantities such as frequency difference ratios, the large and small separations and the behavior of line widths with frequency and line widths at with , for which we derive parametrizations; and behavior of mode visibilities. These average properties can be applied in future peak-bagging exercises to better constrain the parameters of the stellar oscillation spectra. The frequencies and frequency ratios can tightly constrain the fundamental parameters of these solar-type stars, and mode line widths and amplitudes can test models of mode damping and excitation.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,evolution,fundamental parameters,notion,notion-database,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/6WRPIWLP/Lund et al. - 2017(2).pdf}
}

@article{Lund2017a,
  title = {Data Preparation for Asteroseismology with {{TESS}}},
  author = {Lund, Mikkel N. and Handberg, Rasmus and Kjeldsen, Hans and Chaplin, William J. and {Christensen-Dalsgaard}, J{\o}rgen},
  year = {2017},
  journal = {EPJ Web of Conferences},
  volume = {160},
  eprint = {1610.02702},
  issn = {2100014X},
  doi = {10.1051/epjconf/201716001005},
  abstract = {The Transiting Exoplanet Survey Satellite (TESS) is a NASA Astrophysics Explorer mission. Following its scheduled launch in 2017, TESS will focus on detecting exoplanets around the nearest and brightest stars in the sky, for which detailed follow-up observations are possible. TESS will, as the NASA Kepler mission, include a asteroseismic program that will be organized within the TESS Asteroseismic Science Consortium (TASC), building on the success of the Kepler Asteroseismic Science Consortium (KASC). Within TASC data for asteroseismic analysis will be prepared by the TASC Working Group 0 (WG-0), who will facilitate data to the community via the TESS Asteroseismic Science Operations Center (TASOC), again building on the success of the corresponding KASOC platform for Kepler. Here, we give an overview of the steps being taken within WG-0 to prepare for the upcoming TESS mission.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LMCDJ5PY/Lund et al. - 2017.pdf}
}

@article{Lund2018,
  title = {Tutorial: {{Asteroseismic}} Stellar Modelling with {{AIMS}}},
  author = {Lund, Mikkel N. and Reese, Daniel R.},
  year = {2018},
  journal = {Astrophysics and Space Science Proceedings},
  volume = {49},
  eprint = {1711.01896},
  pages = {149--161},
  issn = {15706605},
  doi = {10.1007/978-3-319-59315-9_8},
  abstract = {The goal of aims (Asteroseismic Inference on a Massive Scale) is to estimate stellar parameters and credible intervals/error bars in a Bayesian manner from a set of asteroseismic frequency data and so-called classical constraints. To achieve reliable parameter estimates and computational efficiency, it searches through a grid of pre-computed models using an MCMC algorithm\textemdash interpolation within the grid of models is performed by first tessellating the grid using a Delaunay triangulation and then doing a linear barycentric interpolation on matching simplexes. Inputs for the modelling consist of individual frequencies from peak-bagging, which can be complemented with classical spectroscopic constraints. aims is mostly written in Python with a modular structure to facilitate contributions from the community. Only a few computationally intensive parts have been rewritten in Fortran in order to speed up calculations.},
  archiveprefix = {arxiv},
  isbn = {9783319593142},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/95QQSVCU/Lund, Reese - 2018.pdf}
}

@inproceedings{Lundberg2017,
  title = {A {{Unified Approach}} to {{Interpreting Model Predictions}}},
  booktitle = {T {{Conference}} on {{Neural Information Processing Systems}}},
  author = {Lundberg, Scott M and Allen, Paul G and Lee, Su-In},
  year = {2017},
  urldate = {2020-04-14},
  abstract = {Understanding why a model makes a certain prediction can be as crucial as the prediction's accuracy in many applications. However, the highest accuracy for large modern datasets is often achieved by complex models that even experts struggle to interpret, such as ensemble or deep learning models, creating a tension between accuracy and interpretability. In response, various methods have recently been proposed to help users interpret the predictions of complex models, but it is often unclear how these methods are related and when one method is preferable over another. To address this problem, we present a unified framework for interpreting predictions, SHAP (SHapley Additive exPlanations). SHAP assigns each feature an importance value for a particular prediction. Its novel components include: (1) the identification of a new class of additive feature importance measures, and (2) theoretical results showing there is a unique solution in this class with a set of desirable properties. The new class unifies six existing methods, notable because several recent methods in the class lack the proposed desirable properties. Based on insights from this unification, we present new methods that show improved computational performance and/or better consistency with human intuition than previous approaches.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZLSWNFJV/full-text.pdf}
}

@article{Lutz2008,
  title = {Light {{Curve Analysis}} of the {{Hybrid SdB PulsatorsHS}} 0702+6043 and {{HS}} 2201+2610},
  author = {Lutz, R. and Schuh, S. and Silvotti, R. and Dreizler, S. and Green, E. M. and Fontaine, G. and Stahn, T. and H{\"u}gelmeyer, S. D. and Husser, T. -O.},
  year = {2008},
  month = jan,
  journal = {Hot Subdwarf Stars and Related Objects ASP Conference Series},
  volume = {392},
  pages = {339},
  address = {{eprint: arXiv:0710.4871}},
  doi = {10.48550/arXiv.0710.4871},
  urldate = {2023-10-09},
  abstract = {We present the detection of low-amplitude, long-period g-modes in two individual sdBV stars which are known to be p-mode pulsators. Only few of these hybrid objects, showing both p- and g-modes, are known today. We resolve the g-mode domain in HS 0702+6043 and add HS 2201+2610 to the list of hybrid pulsators. To discover the low-amplitude g-modes, a filtering algorithm based on wavelet transformations was applied to denoise observational data.},
  keywords = {Astrophysics},
  annotation = {ADS Bibcode: 2008ASPC..392..339L},
  file = {/Users/lbugnet/Zotero/storage/IFGMK2BI/Lutz et al. - 2008 - Light Curve Analysis of the Hybrid SdB PulsatorsHS.pdf}
}

@article{Ma2019,
  title = {Angular Momentum Transport in Massive Stars and Natal Neutron Star Rotation Rates},
  author = {Ma, Linhao and Fuller, Jim},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {488},
  number = {3},
  eprint = {1907.03713},
  pages = {4338--4355},
  publisher = {{Oxford University Press}},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz2009},
  abstract = {The internal rotational dynamics of massive stars are poorly understood. If angular momentum (AM) transport between the core and the envelope is inefficient, the large core AM upon core-collapse will produce rapidly rotating neutron stars (NSs). However, observations of low-mass stars suggest an efficient AM transport mechanism is at work, which could drastically reduce NS spin rates. Here, we study the effects of the baroclinic instability and the magnetic Tayler instability in differentially rotating radiative zones. Although the baroclinic instability may occur, the Tayler instability is likely to be more effective for AM transport. We implement Tayler torques as prescribed by Fuller, Piro,~and Jermyn into models of massive stars, finding they remove the vast majority of the core's AM as it contracts between the main-sequence and helium-burning phases of evolution. If core AM is conserved during core-collapse, we predict natal NS rotation periods of \$P\_\{\textbackslash rm NS\} \textbackslash approx 50\textbackslash!-\textbackslash!200 \textbackslash, \{\textbackslash rm ms\}\$, suggesting these torques help explain the relatively slow rotation rates of most young NSs, and the rarity of rapidly rotating engine-driven supernovae. Stochastic spin-up via waves just before core-collapse, asymmetric explosions, and various binary evolution scenarios may increase the initial rotation rates of many NSs.},
  archiveprefix = {arxiv},
  keywords = {1 i n t,constrained and,evolution,instabilities,internal rotation rates of,magnetic field,massive,massive stars are weakly,neu-,notion,notion-database,ro d u c,rotation,stars,t i o n,tron},
  file = {/Users/lbugnet/Zotero/storage/4A99Z28L/Ma, Fuller - 2019(2).pdf}
}

@article{MacGregor1991,
  title = {Rotational {{Evolution}} of {{Solar-Type Stars}}. {{I}}. {{Main-Sequence Evolution}}},
  author = {MacGregor, K. B. and Brenner, M.},
  year = {1991},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {376},
  pages = {204},
  issn = {0004-637X},
  doi = {10.1086/170269},
  urldate = {2023-10-10},
  abstract = {A simple, parameterized model for the redistribution of angular momentum within the interiors of solar-type stars is presented. By incorporating it with a description of angular momentum loss through the action of a magnetically coupled wind, tracing the rotational histories of low-mass dwarf stars for a variety of initial conditions and parameter specifications is accomplished. The results of calculations are discussed for the rotational evolution of a 1 solar mass star, from the time of its arrival on the zero-age main sequence to the age of the present-day sun. Best agreement is with observational constraints for (1) a surface magnetic field strength which is largely independent of surface angular velocity omega for rapid rotation, and approximately linearly dependent on omega for approximately solar values, and (2), a time scale for angular momentum transfer from the core to the convection zone which remains essentially constant throughout the evolution, with magnitude of a about 10 million yr. This value is approximately equal to the initial wind braking time. These results are discussed in the context of a qualitative description of angluar momentum redistribution by magnetic fields in the radiative interiors of solar-type stars.},
  keywords = {Angular Momentum,Angular Velocity,Astrophysics,Magnetic Stars,Main Sequence Stars,Momentum Transfer,STARS: EVOLUTION,STARS: INTERIORS,STARS: MAGNETIC,STARS: ROTATION,STARS: WINDS,Stellar Evolution,Stellar Interiors,Stellar Magnetic Fields,Stellar Models,Stellar Rotation,Stellar Winds},
  annotation = {ADS Bibcode: 1991ApJ...376..204M},
  file = {/Users/lbugnet/Zotero/storage/8GVMJDL3/MacGregor and Brenner - 1991 - Rotational Evolution of Solar-Type Stars. I. Main-.pdf}
}

@article{MacGregor1999,
  title = {Angular {{Momentum Transport}} in {{Magnetized Stellar Radiative Zones}}. {{IV}}. {{Ferraro}}'s {{Theorem}} and the {{Solar Tachocline}}},
  author = {MacGregor, K. B. and Charbonneau, P.},
  year = {1999},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {519},
  number = {2},
  pages = {911--917},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/307389},
  urldate = {2020-07-03},
  abstract = {We consider the circumstances under which the latitudinal di erential rotation of the solar convective envelope can (or cannot) be imprinted on the underlying radiative core through the agency of a hypo-thetical weak, large-scale poloidal magnetic \DH eld threading the solar radiative interior. We do so by con-structing steady, two-dimensional axisymmetric solutions to the coupled momentum and induction equations under the assumption of a purely zonal \~Now and time-independent poloidal magnetic \DH eld. Our results show that the structure of the interior solutions is entirely determined by the boundary con-ditions imposed at the core-envelope interface. Speci\DH cally, in the high Reynolds number regime a poloi-dal \DH eld having a nonzero component normal to the core-envelope interface can lead to the transmission of signi\DH cant di erential rotation into the radiative interior. In contrast, for a poloidal \DH eld that is con-tained entirely within the radiative core, any di erential rotation is con\DH ned to a thin magnetoviscous boundary layer located immediately beneath the interface, as well as along the rotation/magnetic axis. We argue that a magnetically decoupled con\DH guration is more likely to be realized in the solar interior. Consequently, the helioseismically inferred lack of di erential rotation in the radiative core does not nec-essarily preclude the existence of a weak, large-scale poloidal \DH eld therein. We suggest that such a \DH eld may well be dynamically signi\DH cant in determining the structure of the solar tachocline. Subject headings : Sun : interior \`E Sun : oscillations \`E Sun : rotation 1. INTRODUCTION Measurements of solar p-mode oscillation frequencies have been used to infer the angular velocity of rotation)(r, h) throughout much of the Sun\"Is interior. Numerous analyses of helioseismic observations reveal that the photo-spheric dependence of) on h also describes the variation of the internal rotation rate with latitude at any radius r within the convective envelope, R CE (B 0.713 R \_) {$^1$} r {$^1$} (Brown et al. 1989 ; Tomczyk, Schou, \& Thompson R \_ 1995). Somewhat below the base of the convection zone, there exists a thin shear layer (called the tachocline by Spiegel \& Zahn 1992), within which the surface-like rota-tion of the convection zone changes to near-uniform rota-tion in the radiative interior. The central radius of the tachocline appears to lie within the range 0.695\`E0.705 R \_ , and its thickness is estimated to be (Kosovichev [0.05 R \_ 1996 ; Basu 1997 ; Charbonneau et al. 1998a ; Corbard et al. 1999). In the radiative layers beneath the tachocline,) is almost independent of both r and h ; in fact, the region 0.1 seems to rotate nearly rigidly at a rate like R \_ [ r [ 0.7 R \_ that of the solar surface at a latitude of about 30\textexclamdown{} (Charbonneau et al. 1998b). The apparent absence of signi\DH cant di erential rotation in the radiative core of the Sun represents a stringent con-straint on potential mechanisms for internal angular momentum redistribution. Evidently, the process(es) at work in this region must be able to counteract the e ects of the shearing stress exerted by the convective envelope on the stable layers just beneath it. Models for the solar rota-tional evolution in which the internal transport of angular},
  keywords = {notion,notion-database,Sun: Interior,SUN: INTERIOR,Sun: Oscillations,SUN: OSCILLATIONS,Sun: Rotation,SUN: ROTATION},
  file = {/Users/lbugnet/Zotero/storage/GWT8D5A4/full-text.pdf}
}

@article{MacGregor2002,
  title = {Magnetic {{Fields}} in {{Massive Stars}}. {{II}}. {{The Buoyant Rise}} of {{Magnetic Flux Tubes Through}} the {{Radiative Interior}}},
  author = {MacGregor, K. B. and Cassinelli, J. P.},
  year = {2003},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {586},
  number = {1},
  eprint = {astro-ph/0212224},
  pages = {480--494},
  publisher = {{IOP Publishing}},
  doi = {10.1086/346257},
  urldate = {2020-07-02},
  abstract = {We present results from an investigation of the dynamical behavior of buoyant magnetic flux rings in the radiative interior of a uniformly rotating early-type star. Our physical model describes a thin, axisymmetric, toroidal flux tube that is released from the outer boundary of the convective core, and is acted upon by buoyant, centrifugal, Coriolis, magnetic tension, and aerodynamic drag forces. We find that rings emitted in the equatorial plane can attain a stationary equilibrium state that is stable with respect to small displacements in radius, but is unstable when perturbed in the meridional direction. Rings emitted at other latitudes travel toward the surface along trajectories that largely parallel the rotation axis of the star. Over much of the ascent, the instantaneous rise speed is determined by the rate of heating by the absorption of radiation that diffuses into the tube from the external medium. Since the time scale for this heating varies like the square of the tube cross-sectional radius, for the same field strength, thin rings rise more rapidly than do thick rings. For a reasonable range of assumed ring sizes and field strengths, our results suggest that buoyancy is a viable mechanism for bringing magnetic flux from the core to the surface, being capable of accomplishing this transport in a time that is generally much less than the stellar main sequence lifetime.},
  archiveprefix = {arxiv},
  keywords = {atmospheres-stars,convection-stars,early-type-stars,interiors-stars,magnetic fields,notion,notion-database,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/GKSEXYK7/full-text.pdf}
}

@article{Maeder1996,
  title = {Diffusive Mixing by Shears in Rotating Stars.},
  author = {Maeder, A. and Meynet, G.},
  year = {1996},
  journal = {A\&A},
  volume = {313},
  pages = {140--144},
  issn = {0004-6361},
  urldate = {2020-07-17},
  keywords = {DIFFUSION,INTERIORS,notion,notion-database,ROTATION,STARS: EVOLUTION}
}

@article{Maeder1998,
  title = {Stellar Evolution with Rotation. {{III}}. {{Meridional}} Circulation with {{MU}} -Gradients and Non-Stationarity},
  author = {Maeder, Andre and Zahn, Jean-Paul},
  year = {1998},
  journal = {A\&A},
  volume = {334},
  pages = {1000--1006},
  issn = {0004-6361},
  urldate = {2020-07-04},
  keywords = {notion,notion-database,STARS: EARLY,STARS: INTERIOR,STARS: ROTATION,TYPE}
}

@article{Maeder2003,
  title = {Stellar Evolution with Rotation and Magnetic Fields {{I}}. {{The}} Relative Importance of Rotational and Magnetic Effects},
  author = {Maeder, A. and Meynet, G.},
  year = {2003},
  month = dec,
  journal = {Astronomy \& Astrophysics},
  volume = {411},
  number = {3},
  eprint = {astro-ph/0309672},
  pages = {543--552},
  issn = {00046361},
  doi = {10.1051/0004-6361:20031491},
  urldate = {2020-07-13},
  abstract = {We compare the current effects of rotation in stellar evolution to those of the magnetic field created by the Tayler instability. In stellar regions, where a magnetic field can be generated by the dynamo due to differential rotation (Spruit 2002), we find that the growth rate of the magnetic instability is much faster than for the thermal instability. Thus, meridional circulation is small with respect to the magnetic fields, both for the transport of angular momentum and of chemical elements. Also, the horizontal coupling by the magnetic field, which reaches values of a few 105 G, is much more important than the effects of the horizontal turbulence. The field, however, is not sufficient to distort the shape of the equipotentials. We impose the condition that the energy of the magnetic field created by the Tayler-Spruit dynamo cannot be larger than the energy excess present in the differential rotation. This leads to a criterion for the existence of the magnetic field in stellar interiors. Numerical tests are made in a rotating star model of 15 M{$\odot$} rotating with an initial velocity of 300 km s-1. We find that the coefficients of diffusion for the transport of angular momentum by the magnetic field are several orders of magnitude larger than the transport coefficients for meridional circulation and shear mixing. The same applies to the diffusion coefficients for the chemical elements: however, very close to the core, the strong {$\mu$}-gradient reduces the mixing by the magnetic instability to values not too different from the case without magnetic field. We also find that magnetic instability is present throughout the radiative envelope, with the exception of the very outer layers, where differential rotation is insufficient to build the field, a fact consistent with the lack of evidence of strong fields at the surface of massive stars. However, the equilibrium situation reached by a rotating star with magnetic field and rotation is still to be ascertained.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: magnetic field,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/RGDUMD7V/full-text.pdf}
}

@article{Maeder2004,
  title = {Stellar Evolution with Rotation and Magnetic Fields. {{II}}. {{General}} Equations for the Transport by {{Tayler-Spruit}} Dynamo},
  author = {Maeder, A. and Meynet, G.},
  year = {2004},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {422},
  pages = {225--237},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20034583},
  urldate = {2023-10-09},
  abstract = {We further develop the Tayler-Spruit dynamo theory, based on the most efficient instability for generating magnetic fields in radiative layers of differentially rotating stars. We avoid the simplifying assumptions that either the {$\mu$}- or the T-gradient dominates, but we treat the general case and we also account for the nonadiabatic effects, which favour the growth of the magnetic field. The general equation leads to the same analytical solutions in the limiting cases considered by Spruit (\textbackslash cite\{Spruit02\}). Numerical models of a 15 M{$\odot$} star with a magnetic field are performed. The differences between the asymptotic solutions and the general solution demonstrate the need to use the general solution. Stars with a magnetic field rotate almost as a solid body. Several of their properties (size of the core, MS lifetimes, tracks, abundances) are closer to those of models without rotation than with rotation only. In particular, the observed N/C or N/H excesses in OB stars are better explained by our previous models with rotation only than by the present models with magnetic fields that predict no nitrogen excesses. We show that there is a complex feedback loop between the magnetic instability and the thermal instability driving meridional circulation. Equilibrium of the loop, with a small amount of differential rotation, can be reached when the velocity Umagn of the growth of the magnetic instability is of the same order as the velocity Ucirc of the meridional circulation. This opens the possibility for further magnetic models, but at this stage we do not know the relative importance of the magnetic fields due to the Tayler instability in stellar interiors.},
  keywords = {Astrophysics,stars: evolution,stars: magnetic fields,stars: rotation},
  annotation = {ADS Bibcode: 2004A\&A...422..225M},
  file = {/Users/lbugnet/Zotero/storage/Z7UC6PN5/Maeder and Meynet - 2004 - Stellar evolution with rotation and magnetic field.pdf}
}

@article{Maeder2005,
  title = {Stellar Evolution with Rotation and Magnetic Fields {{III}}. {{The}} Interplay of Circulation and Dynamo},
  author = {Maeder, A. and Meynet, G.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {440},
  number = {3},
  pages = {1041--1049},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053261},
  abstract = {We examine the effects of the magnetic field created by the Tayler-Spruit dynamo in differentially rotating stars. Magnetic fields of the order of a few 104 G are present through most of the stellar envelope, with the exception of the outer layers. The diffusion coefficient for the transport of angular momentum is very large and it imposes nearly solid body rotation during the MS phase. In turn, solid body rotation drives meridional circulation currents which are much faster than usual and leads to much larger diffusion coefficients than the magnetic diffusivity for the chemical species. The consequence is that the interplay of the thermal and magnetic instabilities favours the chemical transport of elements, while there would be no transport in models with magnetic field only. We also discuss the effects on the stellar interior, lifetimes and HR diagram. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Stars: evolution,Stars: magnetic fields,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/WR2HP43C/Maeder, Meynet - 2005.pdf}
}

@article{Maeder2009a,
  title = {Physics, {{Formation}} and {{Evolution}} of {{Rotating Stars}}},
  author = {Maeder, A.},
  year = {2009},
  journal = {Springer},
  pages = {520},
  issn = {0941-7834},
  doi = {10.1007/978-3-540-76949-1},
  abstract = {Rotation is ubiquitous at each step of stellar evolution, from star formation to the final stages, and it affects the course of evolution, the timescales and nucleosynthesis. Stellar rotation is also an essential prerequisite for the occurrence of Gamma-Ray Bursts. In this book the author thoroughly examines the basic mechanical and thermal effects of rotation, their influence on mass loss by stellar winds, the effects of differential rotation and its associated instabilities, the relation with magnetic fields and the evolution of the internal and surface rotation. Further, he discusses the numerous observational signatures of rotational effects obtained from spectroscopy and interferometric observations, as well as from chemical abundance determinations, helioseismology and asteroseismology, etc. On an introductory level, this book presents in a didactical way the basic concepts of stellar structure and evolution in "track 1" chapters. The other more specialized chapters form an advanced course on the graduate level and will further serve as a valuable reference work for professional astrophysicists.},
  isbn = {978-3-540-76948-4},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/I6AVY8Q6/Maeder - 2009.pdf}
}

@article{Maeder2012a,
  title = {Rotating Massive Stars: {{From}} First Stars to Gamma Ray Bursts},
  author = {Maeder, Andr{\'e} and Meynet, Georges},
  year = {2012},
  journal = {Reviews of Modern Physics},
  volume = {84},
  number = {1},
  pages = {25--63},
  issn = {00346861},
  doi = {10.1103/RevModPhys.84.25},
  abstract = {This article first reviews the basic physics of rotating stars and their evolution. The changes of the mechanical and thermal equilibrium of rotating stars are examined. An important, predicted and observed, effect is that rotating stars are hotter at the poles and cooler at the equator. The mass loss by stellar winds, which are influenced by the anisotropic temperature distribution, is discussed. These anisotropies in the interior are also driving circulation currents, which transports the chemical elements and the angular momentum in stars. Internal differential rotation, if present, creates instabilities and mixing, in particular, the shear mixing, the horizontal turbulence and their interactions. A major check of the model predictions concerns the changes of the surface abundances, which are modified by mass loss in the very massive stars and by rotational mixing in O-type and B-type stars. The observations are shown to confirm the existence of rotational mixing, with much larger effects at lower metallicities. The predictions of stellar models concerning the evolution of the surface velocities, the evolutionary tracks in the Hertzsprung-Russell diagram and lifetimes, the populations of blue, red supergiants and Wolf-Rayet stars, and the progenitors of type Ibc supernovae are discussed. In many aspects, rotating models are shown to provide a much better fit than nonrotating ones. Using the same physical ingredients as those which fit the best observations of stars at near solar metallicities, the consequences of rotating models for the status of Be stars, the progenitors of gamma ray bursts, the evolution of Pop III stars and of very metal-poor stars, the early chemical evolution of galaxies, the origin of the C-enhanced metal poor stars and of the chemical anomalies in globular clusters are explored. Rotation together with mass loss are two key physical ingredients shaping the evolution of massive stars during the whole cosmic history. \textcopyright{} 2012 American Physical Society.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BWSHYIVH/Maeder, Meynet - 2012.pdf}
}

@article{Maeder2014,
  title = {Magnetic Braking of Stellar Cores in Red Giants and Supergiants},
  author = {Maeder, Andr{\'e} and Meynet, Georges},
  year = {2014},
  journal = {Astrophysical Journal},
  eprint = {1408.1192},
  issn = {15384357},
  doi = {10.1088/0004-637X/793/2/123},
  abstract = {Magnetic configurations, stable on the long term, appear to exist in various evolutionary phases, from main-sequence stars to white dwarfs and neutron stars. The large-scale ordered nature of these fields, often approximately dipolar, and their scaling according to the flux conservation scenario favor a fossil field model. We make some first estimates of the magnetic coupling between the stellar cores and the outer layers in red giants and supergiants. Analytical expressions of the truncation radius of the field coupling are established for a convective envelope and for a rotating radiative zone with horizontal turbulence. The timescales of the internal exchanges of angular momentum are considered. Numerical estimates are made on the basis of recent model grids. The direct magnetic coupling of the core to the extended convective envelope of red giants and supergiants appears unlikely. However, we find that the intermediate radiative zone is fully coupled to the core during the He-burning and later phases. This coupling is able to produce a strong spin down of the core of red giants and supergiants, also leading to relatively slowly rotating stellar remnants such as white dwarfs and pulsars. Some angular momentum is also transferred to the outer convective envelope of red giants and supergiants during the He-burning phase and later.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: magnetic field,stars: rotation}
}

@article{Maeder2014a,
  title = {Magnetic {{Braking}} of {{Stellar Cores}} in {{Red Giants}} and {{Supergiants}}},
  author = {Maeder, Andr{\'e} and Meynet, Georges},
  year = {2014},
  month = oct,
  journal = {The Astrophysical Journal},
  volume = {793},
  pages = {123},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/793/2/123},
  urldate = {2023-10-11},
  abstract = {Magnetic configurations, stable on the long term, appear to exist in various evolutionary phases, from main-sequence stars to white dwarfs and neutron stars. The large-scale ordered nature of these fields, often approximately dipolar, and their scaling according to the flux conservation scenario favor a fossil field model. We make some first estimates of the magnetic coupling between the stellar cores and the outer layers in red giants and supergiants. Analytical expressions of the truncation radius of the field coupling are established for a convective envelope and for a rotating radiative zone with horizontal turbulence. The timescales of the internal exchanges of angular momentum are considered. Numerical estimates are made on the basis of recent model grids. The direct magnetic coupling of the core to the extended convective envelope of red giants and supergiants appears unlikely. However, we find that the intermediate radiative zone is fully coupled to the core during the He-burning and later phases. This coupling is able to produce a strong spin down of the core of red giants and supergiants, also leading to relatively slowly rotating stellar remnants such as white dwarfs and pulsars. Some angular momentum is also transferred to the outer convective envelope of red giants and supergiants during the He-burning phase and later.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: magnetic field,stars: rotation},
  annotation = {ADS Bibcode: 2014ApJ...793..123M},
  file = {/Users/lbugnet/Zotero/storage/YZXEJ84Y/Maeder and Meynet - 2014 - Magnetic Braking of Stellar Cores in Red Giants an.pdf}
}

@article{Mag2018,
  title = {{{ERC Advanced Grant}} 2018 {{Research}} Proposal - {{EPISWITCH}} [ {{Part B2}} ]},
  author = {{Meynet G.}},
  year = {2018},
  pages = {1--18},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AUMJD2ZE/Meynet G. - 2018.pdf}
}

@article{magauddaFirstEROSITAStudy2021,
  title = {First {{eROSITA}} Study of Nearby {{M}} Dwarfs and the Rotation-Activity Relation in Combination with {{TESS}}},
  author = {Magaudda, E. and B., Stelzer and Raetz, {\relax St}. and A, Klutsch},
  year = {2021},
  month = jun,
  eprint = {2106.14548},
  urldate = {2021-08-01},
  abstract = {We present the first study of nearby M dwarfs with the ROentgen Survey with an Imaging Telescope Array (eROSITA) on board the Russian Spektrum-Roentgen-Gamma mission (SRG). To this end we extracted the Gaia DR2 data for the \textasciitilde 9000 nearby M dwarfs in the superblink proper motion catalog and calculated their stellar parameters from empirical relations with optical-IR colors. We cross-matched this catalog with the eROSITA Final Equatorial Depth Survey (eFEDS) and the first eROSITA all-sky survey (eRASS1). Our sample consists of 704 stars (SpT = K5-M7). This unprecedented data base for X-ray emitting M dwarfs allowed to quantitatively constrain the mass dependence of the X-ray luminosity, and to determine the change in the activity level with respect to pre-main-sequence stars. We also combined these data with the Transiting Exoplanet Survey Satellite (TESS) observations that are available for 501 of 704 X-ray detected M dwarfs and determined the rotation period for 180 of them. With the joint eROSITA-TESS sample, and combining it with our historical X-ray and rotation data for M dwarfs, we examined the mass dependence in the saturated regime of the rotation-activity relation. A first comparison of eROSITA hardness ratios and spectra shows that 65\% of our X-ray detected M dwarfs have coronal temperatures of \$\textbackslash sim 0.5\$ keV. We investigated their long-term X-ray variability by comparing the eRASS1 and ROSAT all-sky survey (RASS) measurements. Evidence for X-ray flares is found in various parts of our analysis: directly from inspection of the eFEDS light curves, in the relation between RASS and eRASS1 X-ray luminosities, and in stars displaying X-ray emission hotter than the bulk of the sample according to the hardness ratios. Finally, we point out the need of X-ray spectroscopy for more M dwarfs to study the coronal temperature-luminosity relation, not well constrained by our eFEDS results.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Majaess2010,
  title = {Anchoring the {{Universal Distance Scale}} via a {{Wesenheit Template}}},
  author = {Majaess, Daniel J. and Turner, David G. and Lane, David J. and Henden, Arne and Krajci, Tom},
  year = {2010},
  month = jul,
  journal = {JAVSO},
  volume = {25},
  number = {2},
  eprint = {1007.2300},
  pages = {115--136},
  issn = {0271-9053},
  urldate = {2020-03-07},
  abstract = {A VI Wesenheit diagram featuring SX Phoenicis, delta Scuti, RR Lyrae, type II and classical Cepheid variables is calibrated by means of geometric-based distances inferred from HST, Hipparcos, and VLBA observations (n=30). The distance to a target population follows from the offset between the observed Wesenheit magnitudes and the calibrated template. The method is evaluated by ascertaining the distance moduli for the LMC (mu\_0=18.43+-0.03 se) and the globular clusters omega Cen, M54, M13, M3, and M15. The results agree with estimates cited in the literature, although a nearer distance to M13 is favoured (pending confirmation of the data's photometric zero-point) and observations of variables near the core of M15 suffer from photometric contamination. The calibrated LMC data is subsequently added to the Wesenheit template since that galaxy exhibits precise OGLE photometry for innumerable variables of differing classes, that includes recent observations for delta Scuti variables indicating the stars follow a steeper VI Wesenheit function than classical Cepheids pulsating in the fundamental mode. VI photometry for the calibrators is tabulated to facilitate further research, and includes new observations acquired via the AAVSO's robotic telescope network (e.g., VY Pyx: {$<$}V{$>$}=7.25 and {$<$}V{$>$}-\emph{=0.67). The approach outlined here supersedes the lead author's prior first-order effort to unify variables of the instability strip in order to establish reliable distances.}},
  archiveprefix = {arxiv},
  keywords = {Mira,Mira Variables,notion,notion-database,Variable Stars},
  file = {/Users/lbugnet/Zotero/storage/J7RQ36GI/full-text.pdf}
}

@article{Majewski2016,
  title = {The {{Apache Point Observatory Galactic EVolution Experiment}} ({{APOGEE}}) and Its Successor, {{APOGEE-2}}},
  author = {Majewski, S R and Team, Apogee- and Team, Apogee-2},
  year = {2016},
  journal = {Astronomische Nachrichten},
  volume = {337},
  pages = {863--870},
  keywords = {abundances,evolution,galaxy,kinematics and dynamics,notion,notion-database,stellar content},
  file = {/Users/lbugnet/Zotero/storage/YKC5VNJN/Majewski, Team, Team - 2016.pdf}
}

@article{maldonadoStellarParametersEarly2015,
  title = {Stellar Parameters of Early {{M}} Dwarfs from Ratios of Spectral Features at Optical Wavelengths {$\star$},{$\star\star$}},
  author = {Maldonado, J and Affer, L and Micela, G and Scandariato, G and Damasso, M and Stelzer, B and Barbieri, M and Bedin, L R and Biazzo, K and Bignamini, A and Borsa, F and Claudi, R U and Covino, E and Desidera, S and Esposito, M and Gratton, R and Gonz{\'a}lez Hern{\'a}ndez, J I and Lanza, A F and Maggio, A and Molinari, E and Pagano, I and Perger, M and Pillitteri, I and Piotto, G and Poretti, E and Prisinzano, L and Rebolo, R and Ribas, I and Shkolnik, E and Southworth, J and Sozzetti, A and Mascare{\~n}o, A Su{\'a}rez},
  year = {2015},
  eprint = {1503.03010v1},
  urldate = {2021-08-01},
  abstract = {Context. Low-mass stars have been recognised as promising targets in the search for rocky, small planets with the potential of supporting life. As a consequence, Doppler search programmes using high-resolution spectrographs like HARPS or HARPS-N are providing huge quantities of optical spectra of M dwarfs. However, determining the stellar parameters of M dwarfs using optical spectra has proven to be challenging. Aims. We aim to calibrate empirical relationships to determine accurate stellar parameters for early M dwarfs (spectral types M0-M4.5) using the same spectra that are used for the radial velocity determinations, without the necessity of acquiring IR spectra or relying on atmospheric models and/or photometric calibrations. Methods. Our methodology consists in the use of ratios of pseudo equivalent widths of spectral features as a temperature diagnostic, a technique largely used in solar-type stars. Stars with effective temperatures obtained from interferometric estimates of their radii are used as calibrators. Empirical calibrations for the spectral type are also provided. Combinations of features and ratios of features are used to derive calibrations for the stellar metallicity. Our methods are then applied to a large sample of M dwarfs that are currently being observed in the framework of the HARPS GTO search for extrasolar planets. The derived temperatures and metallicities are used together with photometric estimates of mass, radius, and surface gravity to calibrate empirical relationships for these parameters. Results. A large list of spectral features in the optical spectra of early M dwarfs was identified. From this list the pseudo equivalent width of roughly 43\% of the features shows a strong anticorrelation with the effective temperature. The correlation with the stellar metallicity is weaker. A total of 112 temperature sensitive ratios have been identified and calibrated over the range 3100-3950 K, providing effective temperatures with typical uncertainties of the order of 70 K. Eighty-two ratios of pseudo equivalent widths of features were calibrated to derive spectral types within 0.5 subtypes for stars with spectral types between K7V and M4.5V. Regarding stellar metallicity, 696 combinations of pseudo equivalent widths of individual features and temperature-sensitive ratios have been calibrated, over the metallicity range from-0.54 to +0.24 dex, with estimated uncertainties in the range of 0.07-0.10 dex. We provide our own empirical calibrations for stellar mass, radius, and surface gravity. These parameters are found to show a dependence on the stellar metallicity. For a given effective temperature, lower metallicities predict lower masses and radii, as well as larger gravities. Conclusions.},
  archiveprefix = {arxiv},
  keywords = {fundamental parameters,late-type-stars,low-mass-stars,notion,notion-database,spectroscopic-stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/UHYWXXZ9/full-text.pdf}
}

@article{Mallat1989,
  title = {A Theory for Multiresolution Signal Decomposition - {{The}} Wavelet Representation},
  author = {Mallat, Stephane G. and {Mallat} and G., Stephane},
  year = {1989},
  journal = {ITPAM},
  volume = {11},
  pages = {674--693},
  issn = {0162-8828},
  urldate = {2022-01-08},
  keywords = {Communications and Radar,Computer Vision,Fourier Transformation,Fractals,Image Processing,Image Reconstruction,Mathematical Models,notion,notion-database,Orthonormal Functions,Pixels,Signal Processing,Wave Functions}
}

@article{Mamajek2008,
  title = {Improved {{Age Estimation}} for {{Solar}}-{{Type Dwarfs Using Activity}}-{{Rotation Diagnostics}}},
  author = {Mamajek, Eric E. and Hillenbrand, Lynne A.},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {687},
  number = {2},
  eprint = {0807.1686},
  pages = {1264--1293},
  issn = {0004-637X},
  doi = {10.1086/591785},
  abstract = {While the strong anti-correlation between chromospheric activity and age has led to the common use of the Ca II H \& K emission index (R'\_HK = L\_HK/L\_bol) as an empirical age estimator for solar type dwarfs, existing activity-age relations produce implausible ages at both high and low activity levels. We have compiled R'\_HK data from the literature for young stellar clusters, richly populating for the first time the young end of the activity-age relation. Combining the cluster activity data with modern cluster age estimates, and analyzing the color-dependence of the chromospheric activity age index, we derive an improved activity-age calibration for F7-K2 dwarfs (0.5 {$<$} B-V {$<$} 0.9 mag). We also present a more fundamentally motivated activity-age calibration that relies on conversion of R'\_HK values through the Rossby number to rotation periods, and then makes use of improved gyrochronology relations. We demonstrate that our new activity-age calibration has typical age precision of \textasciitilde 0.2 dex for normal solar-type dwarfs aged between the Hyades and the Sun (\textasciitilde 0.6-4.5 Gyr). Inferring ages through activity-rotation-age relations accounts for some color-dependent effects, and systematically improves the age estimates (albeit only slightly). We demonstrate that coronal activity as measured through the fractional X-ray luminosity (R\_X = L\_X/L\_bol) has nearly the same age- and rotation-inferring capability as chromospheric activity measured through R'\_HK. As a first application of our calibrations, we provide new activity-derived age estimates for the nearest 100 solar-type field dwarfs (d {$<$} 15 pc).},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LI89ZEZ6/Mamajek, Hillenbrand - 2008.pdf}
}

@incollection{Management1996,
  title = {Chapter 9 . {{Multiple Resolution}} in {{Data Storage}}},
  year = {1996},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/W2JLSVDC/Unknown - 1996.pdf}
}

@article{Mankovich2019,
  title = {Cassini {{Ring Seismology}} as a {{Probe}} of {{Saturn}}'s {{Interior}}. {{I}}. {{Rigid Rotation}}},
  author = {Mankovich, Christopher and Marley, Mark S and Fortney, Jonathan J and Movshovitz, Naor},
  year = {2019},
  journal = {The Astrophysical Journal},
  volume = {871},
  pages = {1},
  doi = {10.3847/1538-4357/aaf798},
  urldate = {2020-05-21},
  abstract = {Seismology of the gas giants holds the potential to resolve long-standing questions about their internal structure and rotation state. We construct a family of Saturn interior models constrained by the gravity field and compute their adiabatic mode eigenfrequencies and corresponding Lindblad and vertical resonances in Saturn's C ring, where more than 20 waves with pattern speeds faster than the ring mean motion have been detected and characterized using high-resolution Cassini Visual and Infrared Mapping Spectrometer stellar occultation data. We present identifications of the fundamental modes of Saturn that appear to be the origin of these observed ring waves, and we use their observed pattern speeds and azimuthal wavenumbers to estimate the bulk rotation period of Saturn's interior to be-+ 10 33 38s h m 1m19s 1m52s (median and 5\%/95\% quantiles), significantly faster than Voyager and Cassini measurements of periods in Saturn's kilometric radiation, the traditional proxy for Saturn's bulk rotation period. The global fit does not exhibit any clear systematics indicating strong differential rotation in Saturn's outer envelope.},
  keywords = {notion,notion-database,planets and satellites: individual (Saturn),planets and satellites: interiors,planets and satellites: rings},
  file = {/Users/lbugnet/Zotero/storage/IJSEQCM7/full-text.pdf}
}

@article{mannApJAcceptedHOW,
  title = {{{ApJ}} Accepted {{HOW TO CONSTRAIN YOUR M DWARF}}: {{MEASURING EFFECTIVE TEMPERATURE}}, {{BOLOMETRIC LUMINOSITY}}, {{MASS}}, {{AND RADIUS}}},
  author = {Mann, Andrew W and Feiden, Gregory A and Gaidos, Eric and Boyajian, Tabetha and Von Braun, Kaspar},
  eprint = {1501.01635v3},
  urldate = {2021-08-01},
  abstract = {Precise and accurate parameters for late-type (late K and M) dwarf stars are important for characterization of any orbiting planets, but such determinations have been hampered by these stars' complex spectra and dissimilarity to the Sun. We exploit an empirically calibrated method to estimate spectroscopic effective temperature (T eff) and the Stefan-Boltzmann law to determine radii of 183 nearby K7-M7 single stars with a precision of 2-5\%. Our improved stellar parameters enable us to develop model-independent relations between T eff or absolute magnitude and radius, as well as between color and T eff. The derived T eff-radius relation depends strongly on [Fe/H], as predicted by theory. The relation between absolute K S magnitude and radius can predict radii accurate to 3\%. We derive bolometric corrections to the V R C I C grizJHK S and Gaia passbands as a function of color, accurate to 1-3\%. We confront the reliability of predictions from Dartmouth stellar evolution models using a Markov Chain Monte Carlo to find the values of unobservable model parameters (mass, age) that best reproduce the observed effective temperature and bolometric flux while satisfying constraints on distance and metallicity as Bayesian priors. With the inferred masses we derive a semi-empirical mass-absolute magnitude relation with a scatter of 2\% in mass. The best-agreement models over-predict stellar T eff s by an average of 2.2\% and under-predict stellar radii by 4.6\%, similar to differences with values from low-mass eclipsing binaries. These differences are not correlated with metallicity, mass, or indicators of activity, suggesting issues with the underlying model assumptions e.g., opacities or convective mixing length.},
  archiveprefix = {arxiv},
  keywords = {abundances-stars,fundamental parameters-stars,late-type-stars,low-mass-stars,notion,notion-database,planetary systems,stars,statistics-stars,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/TSAVGUND/full-text.pdf}
}

@inproceedings{Manset2003,
  title = {{{ESPaDOnS}}; an {{Echelle}} Spectropolarimetric Device for the Observation of Stars},
  booktitle = {Polarimetry in {{Astronomy}}},
  author = {Manset, Nadine and Donati, Jean-Francois},
  year = {2003},
  month = feb,
  volume = {4843},
  pages = {425},
  publisher = {{SPIE}},
  issn = {0277786X},
  doi = {10.1117/12.458230},
  urldate = {2020-05-21},
  keywords = {notion,notion-database}
}

@article{Marchant2010,
  title = {Revisiting the {{Flowers-Ruderman}} Instability of Magnetic Stars},
  author = {Marchant, Pablo and Reisenegger, Andreas and Akg{\"u}n, Taner},
  year = {2010},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {415},
  number = {3},
  eprint = {1011.0661},
  pages = {2426--2438},
  doi = {10.1111/j.1365-2966.2011.18874.x},
  urldate = {2020-07-03},
  abstract = {In 1977, Flowers and Ruderman described a perturbation that destabilises a purely dipolar magnetic field in a fluid star. They considered the effect of cutting the star in half along a plane containing the symmetry axis and rotating each half by \$90\textbackslash degr\$ in opposite directions, which would cause the energy of the magnetic field in the exterior of the star to be greatly reduced, just as it happens with a pair of aligned magnets. We formally solve for the energy of the external magnetic field and check that it decreases monotonously along the entire rotation. We also describe the instability using perturbation theory, and see that it happens due to the work done by the interaction of the magnetic field with surface currents. Finally, we consider the stabilising effect of adding a toroidal field by studying the potential energy perturbation when the rotation is not done along a sharp cut, but with a continuous displacement field that switches the direction of rotation across a region of small but finite width. Using these results, we estimate the relative strengths of the toroidal and poloidal field needed to make the star stable to this displacement and see that the energy of the toroidal field required for stabilisation is much smaller than the energy of the poloidal field. We also show that, contrary to a common argument, the Flowers-Ruderman instability cannot be applied many times in a row to reduce the external magnetic energy indefinitely.},
  archiveprefix = {arxiv},
  keywords = {Magnetic fields,MHD,notion,notion-database,Stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/L7ZN2RMZ/full-text.pdf}
}

@techreport{marchioriInflightPhotometryExtraction,
  title = {In-Flight Photometry Extraction of {{PLATO}} Targets {{Optimal}} Apertures for Detecting Extrasolar Planets},
  author = {Marchiori, V and Samadi, R and Fialho, F and Paproth, C and Santerne, A and Pertenais, M and B{\"o}rner, A and Cabrera, J and Monsky, A and Kutrowski, N},
  eprint = {1906.00892v1},
  urldate = {2021-04-11},
  abstract = {Context. The ESA PLATO space mission is devoted to unveiling and characterizing new extrasolar planets and their host stars. This mission will encompass a very large ({$>$}2,100 deg 2) field of view, granting it the potential to survey up to one million stars depending on the final observation strategy. The telemetry budget of the spacecraft cannot handle transmitting individual images for such a huge stellar sample at the right cadence, so the development of an appropriate strategy to perform on-board data reduction is mandatory. Aims. We employ mask-based (aperture) photometry to produce stellar light curves in flight. Our aim is thus to find the mask model that optimizes the scientific performance of the reduced data. Methods. We considered three distinct aperture models: binary mask, weighted Gaussian mask, and weighted gradient mask giving lowest noise-to-signal ratio, computed through a novel direct method. Each model was tested on synthetic images generated for 50,000 potential PLATO targets. We extracted the stellar population from the Gaia DR2 catalogue. An innovative criterion was adopted for choosing between different mask models. We designated as optimal the model providing the best compromise between sensitivity to detect true and false planet transits. We determined the optimal model based on simulated noise-to-signal ratio and frequency of threshold crossing events. Results. Our results show that, although the binary mask statistically presents a few percent higher noise-to-signal ratio compared to weighted masks, both strategies have very similar efficiency in detecting legitimate planet transits. When it comes to avoiding spurious signals from contaminant stars however the binary mask statistically collects considerably less contaminant flux than weighted masks, thereby allowing the former to deliver up to {$\sim$}30\% less false transit signatures at 7.1{$\sigma$} detection threshold. Conclusions. Our proposed approach for choosing apertures has been proven to be decisive for the determination of a mask model capable to provide near maximum planet yield and substantially reduced occurrence of false positives for the PLATO mission. Overall, this work constitutes an important step in the design of both on-board and on-ground science data processing pipelines.},
  archiveprefix = {arxiv},
  keywords = {detection-techniques,instrumentation,notion,notion-database,numerical-catalogs-zodiacal dust,photometers-planets and satellites,photometric-methods},
  file = {/Users/lbugnet/Zotero/storage/WIVWHANA/full-text.pdf}
}

@article{marchioriOptimalAperturesDetecting2019,
  title = {Optimal Apertures for Detecting Extrasolar Planets},
  author = {Marchiori, V and Samadi, R and Fialho, F and Paproth, C and Santerne, A and Pertenais, M and B{\"o}rner, A and Cabrera, J and Monsky, A and Kutrowski, N},
  year = {2019},
  journal = {A\&A},
  volume = {627},
  pages = {71},
  doi = {10.1051/0004-6361/201935269},
  urldate = {2021-04-06},
  abstract = {Context. The ESA PLATO space mission is devoted to unveiling and characterizing new extrasolar planets and their host stars. This mission will encompass a very large ({$>$}2100 deg 2) field of view, granting it the potential to survey up to one million stars depending on the final observation strategy. The telemetry budget of the spacecraft cannot handle transmitting individual images for such a huge stellar sample at the right cadence, so the development of an appropriate strategy to perform on-board data reduction is mandatory. Aims. We employ mask-based (aperture) photometry to produce stellar light curves in flight. Our aim is thus to find the mask model that optimizes the scientific performance of the reduced data. Methods. We considered three distinct aperture models: binary mask, weighted Gaussian mask, and weighted gradient mask giving lowest noise-to-signal ratio, computed through a novel direct method. Each model was tested on synthetic images generated for 50 000 potential PLATO targets. We extracted the stellar population from the Gaia DR2 catalogue. An innovative criterion was adopted for choosing between different mask models. We designated as optimal the model providing the best compromise between sensitivity to detect true and false planet transits. We determined the optimal model based on simulated noise-to-signal ratio and frequency of threshold crossing events. Results. Our results show that, although the binary mask statistically presents a few percent higher noise-to-signal ratio compared to weighted masks, both strategies have very similar efficiency in detecting legitimate planet transits. When it comes to avoiding spurious signals from contaminant stars however the binary mask statistically collects considerably less contaminant flux than weighted masks, thereby allowing the former to deliver up to {$\sim$}30\% less false transit signatures at 7.1{$\sigma$} detection threshold. Conclusions. Our proposed approach for choosing apertures has been proven to be decisive for the determination of a mask model capable to provide near maximum planet yield and substantially reduced occurrence of false positives for the PLATO mission. Overall, this work constitutes an important step in the design of both on-board and on-ground science data processing pipelines.},
  keywords = {detection-techniques,instrumentation,notion,notion-database,numerical-catalogs-zodiacal dust,photometers-planets and satellites,photometric-methods}
}

@phdthesis{Marie-Christine,
  title = {Du Transport de Moment Cin\'etique Par Les Ondes Internes de Gravit\'e \`a l'heure de La Sismologie Stellaire},
  author = {Pin{\c c}on, C.},
  abstract = {Pr\'epar\'ee au LESIA-Observatoire de Paris Du transport de moment cin\'etique par les ondes internes de gravit\'e \`a l'heure de la sismologie stellaire \'Ecole doctorale n o 127},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PQUWKMDB/82096_PINCON_2017_archivage.pdf}
}

@article{Marigo2008a,
  title = {Evolution of Asymptotic Giant Branch Stars: {{II}}. {{Optical}} to Far-Infrared Isochrones with Improved {{TP-AGB}} Models},
  author = {Marigo, P. and Girardi, L. and Bressan, A. and Groenewegen, M. A.T. and Silva, L. and Granato, G. L.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {482},
  number = {3},
  pages = {883--905},
  issn = {00046361},
  doi = {10.1051/0004-6361:20078467},
  abstract = {We present a large set of theoretical isochrones, whose distinctive features mostly reside on the greatly-improved treatment of the thermally-pulsing asymptotic giant branch (TP-AGB) phase. Essentially, we have coupled the TP-AGB tracks described in Paper I, at their stages of pre-flash quiescent H-shell burning, with the evolutionary tracks for the previous evolutionary phases from Girardi et al. (2000, A\&AS, 141, 371). Theoretical isochrones for any intermediate value of age and metallicity are then derived by interpolation in the grids. We take care that the isochrones keep, to a good level of detail, the several peculiarities present in these TP-AGB tracks - e.g., the cool tails of C-type stars owing to the use of proper molecular opacities as convective dredge-up occurs along the TP-AGB; the bell-shaped sequences in the Hertzsprung-Russell (HR) diagram for stars with hot-bottom burning; the changes of pulsation mode between fundamental and first overtone; the sudden changes of mean mass-loss rates as the surface chemistry changes from M- to C-type; etc. Theoretical isochrones are then converted to about 20 different photometric systems - including traditional ground-based systems, and those of recent major wide-field surveys such as SDSS, OGLE, DENIS, 2MASS, UKIDSS, etc., - by means of synthetic photometry applied to an updated library of stellar spectra, suitably extended to include C-type stars. Finally, we correct the predicted photometry for the effect of circumstellar dust during the mass-losing stages of the AGB evolution, which allows us to improve the results for the optical-to-infrared systems, and to simulate mid- and far-IR systems such as those of Spitzer and AKARI. We illustrate the most striking properties of these isochrones by means of basic comparisons with observational data for the Milky Way disc and the Magellanic Clouds. Access to the data is provided both via a web repository of static tables (http://stev.oapd.inaf.it/dustyAGB07 and CDS), and via an interactive web interface (http://stev.oapd.inaf.it/cmd), which provides tables for any intermediate value of age and metallicity, for several photometric systems, and for different choices of dust properties. \textcopyright{} 2008 ESO.},
  keywords = {Astronomical data bases: miscellaneous,Galaxies: Magellanic Clouds,notion,notion-database,Stars: AGB and post-AGB,Stars: carbon,Stars: evolution,Stars: Hertzsprung-Russell (HR) and C-M diagrams},
  file = {/Users/lbugnet/Zotero/storage/ZKQD6KQS/Marigo et al. - 2008.pdf}
}

@article{Markey1973,
  title = {The Adiabatic Stability of Stars Containing Magnetic Fields {{II}} Poloidal Fields},
  author = {Markey, P. and Tayler, R.J.},
  year = {1973},
  journal = {Monthly Notices of the Royal Astronomical Society},
  number = {63},
  pages = {77--91},
  urldate = {2020-05-01},
  abstract = {It is shown that, if a star contains a poloidal magnetic field with field lines closed within the star, it is almost certain to suffer from hydromagnetic instabilities with a growth time very much shorter than the thermal time scale of the star. The motions driven by these instabilities are almost entirely parallel to surfaces of constant gravitational potential. The ultimate result of the instabilities is unclear. In the first instance they are likely to become oscillations of finite amplitude. If their wavelengths are short enough they may be damped by resistivity and this could lead to a substantial reduction of magnetic flux in the star. This simple result will be affected by rotation and the presence of a toroidal component of magnetic field. Neither of these factors is considered in detail in the present paper but it is made plausible that the instabilities might be suppressed if the toroidal magnetic field is comparable in strength with the poloidal field.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/32KRUDN6/full-text.pdf}
}

@article{Markey1974,
  title = {{{THE ADIABATIC STABILITY OF STARS CONTAINING MAGNETIC FIELDS-III Additional Results}} for {{Poloidal Fields}}},
  author = {Markey, P and Tayler, R J},
  year = {1974},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {168},
  number = {3},
  pages = {505--514},
  urldate = {2020-07-02},
  abstract = {In a previous paper it has been shown that a particular poloidal magnetic field configuration, with closed magnetic field lines inside a star, is unstable and that the instabilities grow in a short time compared with time scales important in stellar evolution. In that paper it was suggested that the results obtained depended only on the field topology and not on its precise structure. In the present paper three further types of poloidal field configuration are studied and they are all shown to be unstable. It thus appears very probable that all poloidal configurations with closed field lines are unstable.},
  keywords = {notion,notion-database}
}

@article{Marques2013a,
  title = {Seismic Diagnostics for Transport of Angular Momentum in Stars: {{I}}. {{Rotational}} Splittings from the Pre-Main Sequence to the Red-Giant Branch},
  author = {Marques, J. P. and Goupil, M. J. and Lebreton, Y. and Talon, S. and Palacios, A. and Belkacem, K. and Ouazzani, R. M. and Mosser, B. and Moya, A. and Morel, P. and Pichon, B. and Mathis, S. and Zahn, J. P. and {Turck-Chi{\`e}ze}, S. and Nghiem, P. A.P.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {549},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220211},
  abstract = {Context. Rotational splittings are currently measured for several main sequence stars and a large number of red giants with the space mission Kepler. This will provide stringent constraints on rotation profiles. Aims. Our aim is to obtain seismic constraints on the internal transport and surface loss of the angular momentum of oscillating solar-like stars. To this end, we study the evolution of rotational splittings from the pre-main sequence to the red-giant branch for stochastically excited oscillation modes. Methods. We modified the evolutionary code CESAM2K to take rotationally induced transport in radiative zones into account. Linear rotational splittings were computed for a sequence of 1.3 M{$\cdot$} models. Rotation profiles were derived from our evolutionary models and eigenfunctions from linear adiabatic oscillation calculations. Results. We find that transport by meridional circulation and shear turbulence yields far too high a core rotation rate for red-giant models compared with recent seismic observations. We discuss several uncertainties in the physical description of stars that could have an impact on the rotation profiles. For instance, we find that the Goldreich-Schubert-Fricke instability does not extract enough angular momentum from the core to account for the discrepancy. In contrast, an increase of the horizontal turbulent viscosity by 2 orders of magnitude is able to significantly decrease the central rotation rate on the red-giant branch. Conclusions. Our results indicate that it is possible that the prescription for the horizontal turbulent viscosity largely underestimates its actual value or else a mechanism not included in current stellar models of low mass stars is needed to slow down the rotation in the radiative core of red-giant stars. \textcopyright{} 2012 ESO.},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/XVHRR8BG/Marques et al. - 2013.pdf}
}

@article{Marsden2014,
  title = {A {{BCool}} Magnetic Snapshot Survey of Solar-Type Stars},
  author = {Marsden, S. C. and Petit, P. and Jeffers, S. V. and Morin, J. and Fares, R. and Reiners, A. and Do Nascimento, J. D. and Auri{\`e}re, M. and Bouvier, J. and Carter, B. D. and Catala, C. and Dintrans, B. and Donati, J. F. and Gastine, T. and Jardine, M. and {Konstantinova-Antova}, R. and Lanoux, J. and Ligni{\`e}res, F. and Morgenthaler, A. and {Ram{\'i}rez-V{\'e}lez}, J. C. and Th{\'e}ado, S. and Van Grootel, V.},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {444},
  number = {4},
  eprint = {1311.3374},
  pages = {3517--3536},
  issn = {13652966},
  doi = {10.1093/mnras/stu1663},
  abstract = {We present the results of a major high-resolution spectropolarimetric BCool project magnetic survey of 170 solar-type stars. Surface magnetic fields were detected on 67 stars, with 21 classified as mature solar-type stars, a result that increases by a factor of 4 the number of mature solar-type stars on which magnetic fields have been observed. In addition, a magnetic fieldwas detected for 3 out of 18 of the subgiant stars surveyed. For the population of K-dwarfs, the mean value of |B{$<$}inf{$>$}l{$<$}/inf{$>$}| (|B{$<$}inf{$>$}l{$<$}/inf{$>$}|mean) was also found to be higher (5.7 G) than |Bl|mean measured for the G-dwarfs (3.2 G) and the F-dwarfs (3.3 G). For the sample as a whole, |B{$<$}inf{$>$}l{$<$}/inf{$>$}|mean increases with rotation rate and decreases with age, and the upper envelope for |B{$<$}inf{$>$}l{$<$}/inf{$>$}| correlates well with the observed chromospheric emission. Stars with a chromospheric S-index greater than about 0.2 show a high magnetic field detection rate and so offer optimal targets for future studies. This survey constitutes the most extensive spectropolarimetric survey of cool stars undertaken to date, and suggests that it is feasible to pursue magnetic mapping of a wide range of moderately active solar-type stars to improve our understanding of their surface fields and dynamos.},
  archiveprefix = {arxiv},
  keywords = {Line: profiles,Magnetic fields,notion,notion-database,Stars: activity},
  file = {/Users/lbugnet/Zotero/storage/3MJAVT2W/Marsden et al. - 2014.pdf}
}

@article{Marsh1995,
  title = {Low-{{Mass White Dwarfs Need Friends}} - {{Five New Double-Degenerate Close Binary Stars}}},
  author = {Marsh, T. R. and Dhillon, V. S. and Duck, S. R.},
  year = {1995},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {275},
  pages = {828},
  issn = {0035-8711},
  doi = {10.1093/mnras/275.3.828},
  urldate = {2023-10-09},
  abstract = {We have discovered five detached close binary stars out of seven white dwarfs chosen for their low mass ({$<$}0.45 Msun). The high success rate of our observations supports the notion that evolution within a binary star is needed to obtain white dwarfs with masses below 0.45 Msun. We have measured the orbital period and radial velocity amplitude of four of our discoveries. No late-type features are seen in any of our targets at a level which forces the mass of any main-sequence companion to be less than 0.1 Msun. This, together with our measured mass functions, implies that the companion stars are in fact white dwarfs. Our observations raise the number of detached, double-degenerate close binaries with known orbital periods from two to six. All of the orbits are circular, a consequence of past interaction. We find periods of 1.1, 3.3 and 4.8 d for 1713+332, 1241-010 and 1317+453. 2331+290 has a very short period, most likely 4h, but with the 1 cycle d-1 alias at 4.8 h also a possibility. Gravitational radiation will cause this star to merge within about 2 \texttimes{} 109 yr. Close double-degenerates go through one or more stages during which the two stars orbit inside a common envelope. The long orbital periods of 1241-010 and 1317+453 suggest that the ejection of the envelope during the common-envelope phase is very efficient. The spectrum of the companion is directly detectable in 1713+332 but in none of the other systems.},
  keywords = {binaries: close - binaries: spectroscopic - white dwarfs},
  annotation = {ADS Bibcode: 1995MNRAS.275..828M},
  file = {/Users/lbugnet/Zotero/storage/SFJMLC5Q/Marsh et al. - 1995 - Low-Mass White Dwarfs Need Friends - Five New Doub.pdf}
}

@article{Marti2004,
  title = {P -Mode Frequencies in Solar-like Stars},
  author = {Marti, M and Lebrun, J and Appourchaux, T},
  year = {2004},
  volume = {303},
  pages = {295--303},
  keywords = {including pulsations,individual,notion,notion-database,oscillations,procyon a,radial velocities,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/PUES8Q94/Marti, Lebrun, Appourchaux - 2004.pdf}
}

@article{Martic1999,
  title = {Evidence for Global Pressure Oscillations on {{Procyon}}},
  author = {Martic, M and Schmitt, J and Lebrun, J.-C and Barban, C and Connes, P and Bouchy, F and Michel, E and Baglin, A and Appourchaux, T and Bertaux, J.-L},
  year = {1999},
  journal = {Astron. Astrophys},
  volume = {351},
  pages = {993--1002},
  urldate = {2020-03-08},
  abstract = {Precise Doppler measurements of the star Procyon ({$\alpha$} CMi, HR 2943) have been obtained with the ELODIE fiber-fed cross-dispersed echelle spectrograph on the 1.93 m telescope at Observatoire de Haute Provence. Here, we present the analysis of data from 10 days observing run carried out in November 1998. We detect significant excess in the power between 0.5-1.5 mHz in the periodograms of the time series of mean Doppler shifts. Observations of {$\eta$} Cas made with the same instrument during the same time interval and in almost identical night conditions show a flat spectrum in this frequency range, indicating that the excess of Doppler signal seen on Pro-cyon is of stellar origin. When data from the whole run are jointly analyzed, a period analysis places an upper limit of 0.50-0.60 ms -1 for the amplitude of oscillations, while the frequency cutoff is around 1.5 mHz. The power evidently drops near 0.55 and 1.5 mHz on the average of unfiltered power spectra of individual nights, which is consistent with the expected p-mode oscillation properties for Procyon. Several equispaced peaks in frequency are recurrent in the power spectra of two independent segments of 4 and 3 contiguous nights; the most probable frequency spacing seems to be 55 \textmu Hz. In conclusion, we now have an instrument setup which is sufficiently stable and fast to be used for a multi-site campaign involving instruments with comparable velocity precisions, to detect the oscillation modes of sun-like stars.},
  keywords = {individual,notion,notion-database,oscillations-stars,Procyon-techniques,spectroscopic,stars},
  file = {/Users/lbugnet/Zotero/storage/45CNJZNS/full-text.pdf}
}

@article{Martig2015,
  title = {Young {$\alpha$}-Enriched Giant Stars in the Solar Neighbourhood},
  author = {Martig, Marie and Rix, Hans Walter and Aguirre, Victor Silva and Hekker, Saskia and Mosser, Benoit and Elsworth, Yvonne and Bovy, Jo and Stello, Dennis and Anders, Friedrich and Garc{\'i}a, Rafael A. and Tayar, Jamie and Rodrigues, Tha{\'i}se S. and Basu, Sarbani and Carrera, Ricardo and Ceillier, Tugdual and Chaplin, William J. and Chiappini, Cristina and Frinchaboy, Peter M. and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Hearty, Fred R. and Holtzman, Jon and Johnson, Jennifer A. and Majewski, Steven R. and Mathur, Savita and M{\'e}sz{\'a}ros, Szabolcs and Miglio, Andrea and Nidever, David and Pan, Kaike and Pinsonneault, Marc and Schiavon, Ricardo P. and Schneider, Donald P. and Serenelli, Aldo and Shetrone, Matthew and Zamora, Olga},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {451},
  number = {2},
  eprint = {1412.3453},
  pages = {2230--2243},
  issn = {13652966},
  doi = {10.1093/mnras/stv1071},
  abstract = {We derive age constraints for 1639 red giants in the APOKASC sample for which seismic parameters from Kepler, as well as effective temperatures, metallicities and [{$\alpha$}/Fe] values from APOGEE DR12 (Apache Point Observatory Galactic Evolution Experiment Data Release 12) are available.We investigate the relation between age and chemical abundances for these stars, using a simple and robust approach to obtain ages.We first derive stellarmasses using standard seismic scaling relations, then determine the maximum possible age for each star as function of its mass and metallicity, independently of its evolutionary stage. While the overall trend between maximum age and chemical abundances is a declining fraction of young stars with increasing [{$\alpha$}/Fe], at least 14 out of 241 stars with [{$\alpha$}/Fe] {$>$}0.13 are younger than 6 Gyr. Five stars with [{$\alpha$}/Fe] {$\geq$}0.2 have ages below 4 Gyr. We examine the effect of modifications in the standard seismic scaling relations, as well as the effect of very low helium fractions, but these changes are not enough to make these stars as old as usually expected for {$\alpha$}-rich stars (i.e. ages greater than 8-9 Gyr). Such unusual {$\alpha$}-rich young stars have also been detected by other surveys, but defy simple explanations in a galaxy evolution context.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: abundances,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/7GE4Z2WY/Martig et al. - 2015.pdf}
}

@article{Martin2007,
  title = {A Turbulent Wake as a Tracer of 30,000 Years of {{Mira}}'s Mass Loss History},
  author = {Martin, D. Christopher and Seibert, Mark and Neill, James D. and Schiminovich, David and Forster, Karl and Rich, R. Michael and Welsh, Barry Y. and Madore, Barry F. and Wheatley, Jonathan M. and Morrissey, Patrick and Barlow, Tom A.},
  year = {2007},
  journal = {Nature},
  volume = {448},
  number = {7155},
  pages = {780--783},
  issn = {14764687},
  doi = {10.1038/nature06003},
  abstract = {Mira is one of the first variable stars ever discovered and it is the prototype (and also the nearest example) of a class of low-to-intermediate-mass stars in the late stages of stellar evolution. These stars are relatively common and they return a large fraction of their original mass to the interstellar medium (ISM) (ref. 2) through a processed, dusty, molecular wind. Thus stars in Mira's stage of evolution have a direct impact on subsequent star and planet formation in their host galaxy. Previously, the only direct observation of the interaction between Mira-type stellar winds and the ISM was in the infrared. Here we report the discovery of an ultraviolet-emitting bow shock and turbulent wake extending over 2 degrees on the sky, arising from Mira's large space velocity and the interaction between its wind and the ISM. The wake is visible only in the far ultraviolet and is consistent with an unusual emission mechanism whereby molecular hydrogen is excited by turbulent mixing of cool molecular gas and shock-heated gas. This wind wake is a tracer of the past 30,000 years of Mira's mass-loss history and provides an excellent laboratory for studying turbulent stellar wind-ISM interactions. \textcopyright 2007 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VDGMGUVJ/Martin et al. - 2007.pdf}
}

@article{martinSURFACEGRAVITIES228,
  title = {{{SURFACE GRAVITIES FOR}} 228 {{M}}, {{L}}, {{AND T DWARFS IN THE NIRSPEC BROWN DWARF SPECTROSCOPIC SURVEY}} *},
  author = {Martin, Emily C and Mace, Gregory N and Mclean, Ian S and Logsdon, Sarah E and Rice, Emily L and Kirkpatrick, J Davy and Burgasser, Adam J and Mcgovern, Mark R and Prato, Lisa},
  eprint = {1703.03811v1},
  urldate = {2021-08-01},
  abstract = {We combine 131 new medium-resolution (R {$\sim$} 2000) J-band spectra of M, L, and T dwarfs from the Keck NIRSPEC Brown Dwarf Spectroscopic Survey (BDSS) with 97 previously published BDSS spectra to study surface-gravity-sensitive indices for 228 low-mass stars and brown dwarfs spanning spectral types M5-T9. Specifically, we use an established set of spectral indices to determine surface gravity classifications for all M6-L7 objects in our sample by measuring equivalent widths (EW) of the K I lines at 1.1692, 1.1778, 1.2529 \textmu m, and the 1.2 \textmu m FeH J absorption index. Our results are consistent with previous surface gravity measurements, showing a distinct double peak-at {$\sim$} L5 and T5-in K I EW as a function of spectral type. We analyze K I EWs of 73 objects of known ages and find a linear trend between log(Age) and EW. From this relationship, we assign age ranges to the very low gravity, intermediate gravity, and field gravity designations for spectral types M6-L0. Interestingly, the ages probed by these designations remain broad, change with spectral type, and depend on the gravity sensitive index used. Gravity designations are useful indicators of the possibility of youth, but current datasets cannot be used to provide a precise age estimate.},
  archiveprefix = {arxiv},
  keywords = {atmospheres-stars,brown dwarfs-infrared,low-mass-surveys,notion,notion-database,stars-stars},
  file = {/Users/lbugnet/Zotero/storage/F75PJ62G/full-text.pdf}
}

@article{martinSurfaceGravities2282017,
  title = {Surface {{Gravities}} for 228 {{M}}, {{L}}, and {{T Dwarfs}} in the {{NIRSPEC Brown Dwarf Spectroscopic Survey}} *},
  author = {Martin, Emily C and Mace, Gregory N and Mclean, Ian S and Logsdon, Sarah E and Rice, Emily L and Kirkpatrick, J Davy and Burgasser, Adam J and Mcgovern, Mark R and Prato, Lisa},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {838},
  pages = {73},
  doi = {10.3847/1538-4357/aa6338},
  urldate = {2021-08-01},
  abstract = {We combine 131 new medium-resolution (R {$\sim$} 2000) J-band spectra of M, L, and T dwarfs from the Keck NIRSPEC Brown Dwarf Spectroscopic Survey (BDSS) with 97 previously published BDSS spectra to study surface-gravity-sensitive indices for 228 low-mass stars and brown dwarfs spanning spectral types M5-T9. Specifically, we use an established set of spectral indices to determine surface gravity classifications for all of the M6-L7 objects in our sample by measuring the equivalent widths (EW) of the K I lines at 1.1692, 1.1778, and 1.2529 {$\mu$}m, and the 1.2 {$\mu$}m FeH J absorption index. Our results are consistent with previous surface gravity measurements, showing a distinct double peak-at {$\sim$}L5 and T5-in K I EW as a function of spectral type. We analyze the K I EWs of 73 objects of known ages and find a linear trend between log(Age) and EW. From this relationship, we assign age ranges to the very low gravity, intermediate gravity, and field gravity designations for spectral types M6-L0. Interestingly, the ages probed by these designations remain broad, change with spectral type, and depend on the gravity-sensitive index used. Gravity designations are useful indicators of the possibility of youth, but current data sets cannot be used to provide a precise age estimate.},
  keywords = {brown dwarfs,infrared: stars,notion,notion-database,stars: atmospheres,stars: low-mass,surveys}
}

@article{Masana2006a,
  title = {Effective Temperature Scale and Bolometric Corrections from {{2MASS}} Photometry},
  author = {Masana, E. and Jordi, C. and Ribas, I.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {450},
  number = {2},
  pages = {735--746},
  issn = {00046361},
  doi = {10.1051/0004-6361:20054021},
  abstract = {We present a method to determine effective temperatures, angular semi-diameters and bolometric corrections for population I and II FGK type stars based on V and 2MASS IR photometry. Accurate calibration is accomplished by using a sample of solar analogues, whose average temperature is assumed to be equal to the solar effective temperature of 5777 K. By taking into account all possible sources of error we estimate associated uncertainties to better than 1 \% in effective temperature and in the range 1.0-2.5\% in angular semi-diameter for unreddened stars. Comparison of our new temperatures with other determinations extracted from the literature indicates, in general, remarkably good agreement. These results suggest that the effective temperaure scale of FGK stars is currently established with an accuracy better than 0.5\%-1\%. The application of the method to a sample of 10999 dwarfs in the Hipparcos catalogue allows us to define temperature and bolometric correction (K band) calibrations as a function of (V - K), [m/H] and log g. Bolometric corrections in the V and K bands as a function of T eff, [m/H] and log g are also given. We provide effective temperatures, angular semi-diameters, radii and bolometric corrections in the V and K bands for the 10999 FGK stars in our sample with the corresponding uncertainties. \textcopyright{} ESO 2006.},
  keywords = {Infrared: stars,Methods: analytical,notion,notion-database,Stars: fundamental parameters,Stars: late-type,Stars: sub-dwarfs,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/TG8JDQ92/Masana, Jordi, Ribas - 2006.pdf}
}

@article{Massarotti2008,
  title = {{{STELLAR ROTATION AND PLANET INGESTION IN GIANTS}}},
  author = {Massarotti, Alessandro},
  year = {2008},
  journal = {The Astronomical Journal},
  volume = {135},
  number = {6},
  pages = {2287--2290},
  doi = {10.1088/0004-6256/135/6/2287},
  urldate = {2020-07-13},
  abstract = {We investigate the expected increase in the rotation rate of post-main-sequence stars as they expand and ingest orbiting planets. This phenomenon is expected to occur when the stellar radius becomes larger than the planet's periastron distance. We calculate the expected frequency of planet ingestion during the red giant, horizontal branch (HB), and early asymptotic giant branch phases for planets of mass m p 1M J. We also calculate the probability of observing anomalous rotation rates in a population of solar metallicity giants as a function of stellar mass and evolutionary stage. Planet ingestion is most easily detectable in a solar mass HB star, with a probability of about 1\% for solar-neighborhood metallicity. Our analysis is based on the observed distribution of mass, eccentricity, semimajor axis for extrasolar planets around solar-type main-sequence stars, on stellar evolution models, and on the typical observed rotation rates observed in a sample of solar-neighborhood giants.},
  keywords = {AGB and post-AGB-stars,evolution-stars,horizontal-branch-stars,notion,notion-database,rotation-planetary systems-techniques,spectroscopic,stars}
}

@article{Mathis2004,
  title = {Transport and Mixing in the Radiation Zones of Rotating Stars: {{I}}. {{Hydrodynamical}} Processes},
  author = {Mathis, S. and Zahn, J. P.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {425},
  number = {1},
  eprint = {astro-ph/0406418},
  pages = {229--242},
  issn = {00046361},
  doi = {10.1051/0004-6361:20040278},
  abstract = {The purpose of this paper is to improve the modelization of the rotational mixing which occurs in stellar radiation zones, through the combined action of the thermally driven meridional circulation and of the turbulence generated by the shear of differential rotation. The turbulence is assumed to be anisotropic, due to the stratification, with stronger transport in the horizontal directions than in the vertical. The main difference with the former treatments by Zahn (1992, A\&A, 265, 115) and Maeder \& Zahn (1998, A\&A, 334, 1000) is that we expand here the departures from spherical symmetry to higher order, and include explicitly the differential rotation in latitude, to first order. This allows us to treat simultaneously the bulk of a radiation zone and its tachocline(s). Moreover, we take fully into account the non-stationarity of the problem, which will enable us to tackle the rapid phases of evolution. The system of partial differential equations, which govern the transport of angular momentum, heat and chemical elements, is written in a form which makes it ready to implement in a stellar evolution code. Here the effect of a magnetic field is deliberately ignored; it will be included in forthcoming papers.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/EPSBS7A9/Mathis, Zahn - 2004.pdf}
}

@article{Mathis2004b,
  title = {On Shear-Induced Turbulence in Rotating Stars},
  author = {Mathis, S. and Palacios, A. and Zahn, J. -P.},
  year = {2004},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {425},
  number = {1},
  eprint = {astro-ph/0403580},
  pages = {243--247},
  doi = {10.1051/0004-6361:20040279},
  urldate = {2020-07-04},
  abstract = {We review various prescriptions which have been proposed for the turbulent transport of matter and angular momentum in differentially rotating stellar radiation zones. A new prescription is presented for the horizontal transport associated with the anisotropic shear turbulence which is produced by the differential rotation in latitude; this `beta-viscosity' is drawn from torque measurements in the classical Couette-Taylor experiment (Richard \& Zahn 1999). Its implementation in a stellar evolution code leads to enhanced mixing, as illustrated by models of a rotating main-sequence star of 1.5 solar mass.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/IK6ATEWE/full-text.pdf}
}

@article{Mathis2005,
  title = {Transport and Mixing in the Radiation Zones of Rotating Stars {{II}}. {{Axisymmetric}} Magnetic Field},
  author = {Mathis, S. and Zahn, J. P.},
  year = {2005},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {440},
  number = {2},
  eprint = {astro-ph/0506105},
  pages = {653--666},
  issn = {00046361},
  doi = {10.1051/0004-6361:20052640},
  urldate = {2020-06-19},
  abstract = {The purpose of this paper is to improve the modeling of the mixing of chemical elements that occurs in stellar radiation zones. In addition to the classical rotational mixing considered in our previous paper, which results of the combined action of the thermally-driven meridional circulation and of the turbulence generated by the shear of differential rotation, we include here the effect of an axisymmetric magnetic field in a self-consistent way. We treat the advection of the field by the meridional circulation, its Ohmic diffusion, and the production of its toroidal component through the shear of differential rotation. The Lorentz force is assumed not to exceed the centrifugal force; it acts on the baroclinic balance and therefore on the meridional flow, and it has a strong impact on the transport of angular momentum. All variables and governing equations are expanded in spherical or spherical vectorial functions, to arbitrary order: this yields a system of partial differential equations in time and in the radial coordinate, which is ready to be implemented in a stellar structure code. \textcopyright{} ESO 2005.},
  archiveprefix = {arxiv},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Stars: evolution,Stars: magnetic fields,Stars: rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/YTGNCYX2/full-text.pdf}
}

@article{Mathis2010,
  title = {The Interior of the {{Sun}} in 3-{{D}}: {{Beyond}} the Spherical {{Sun}} Picture},
  author = {Mathis, S.},
  year = {2010},
  month = dec,
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  pages = {883--889},
  issn = {00046337},
  doi = {10.1002/asna.201011419},
  urldate = {2020-06-19},
  abstract = {With all the results now obtained by global helioseismology, it is clear that we have to go beyond the classical spherical modelling of the Sun. In this way, it is now necessary to draw a picture that takes into account internal dynamical processes such as rotation, magnetic field, and waves from the core to the surface. This is a challenging task since such mechanisms involve length and time-scales that differ from several orders of magnitude and impact on the solar behaviour both on dynamical and secular times. In this review, I will thus describe the present state of the art in the modelling of the internal dynamics of the Sun \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Sun: evolution,Sun: helioseismology,Sun: interior,Sun: magnetic fields,Sun: rotation}
}

@inproceedings{Mathis2010a,
  title = {Mhd Relaxation of Fossil Magnetic Fields in Stellar Interiors},
  booktitle = {Proceedings of the {{International Astronomical Union}}},
  author = {Mathis, Stephane and Duez, Vincent and Braithwaite, Jonathan},
  year = {2010},
  month = jun,
  volume = {6},
  pages = {270--278},
  issn = {17439213},
  doi = {10.1017/S1743921311017698},
  urldate = {2020-07-17},
  abstract = {The understanding of fossil fields origin, topology, and stability is one of the corner stones of the stellar magnetism theory. On one hand, since they survive on secular time scales, they may modify the structure and the evolution of their host stars. On the other hand, they must have a complex stable structure since it has been demonstrated that the simplest purely poloidal or toroidal fields are unstable on dynamical time scales. In this context, the only stable stellar configurations found today are those resulting from numerical simulations by Braithwaite and collaborators who studied the evolution of an initial stochastic magnetic field, which relaxes with a selective decay of magnetic helicity and energy, on mixed stable configurations (poloidal and toroidal) that seem to be in equilibrium and then diffuse. In this talk, we report the semianalytical investigation of such an equilibrium field in the axisymmetric case. We use variational methods, which describe selective decay of magnetic helicity and energy during MHD relaxation, and we identify a supplementary invariant due to the stable stratification of stellar radiation zones. This leads to states that generalize force-free Taylor's relaxation states studied in plasma laboratory experiments that become non force-free in the stellar case. Moreover, astrophysical applications are presented and the stability of obtained configurations is studied. \textcopyright{} International Astronomical Union 2011.},
  isbn = {978-0-521-19739-7},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Plasmas,Stars: magnetic field}
}

@article{Mathis2010b,
  title = {{{MHD}} Relaxation of Fossil Magnetic Fields in Stellar Interiors},
  author = {Mathis, St{\'e}phane and Duez, Vincent and Braithwaite, Jonathan},
  year = {2010},
  journal = {International Astronomical Union},
  number = {271},
  doi = {10.1017/S1743921311017698},
  urldate = {2020-08-11},
  abstract = {The understanding of fossil fields origin, topology, and stability is one of the corner stones of the stellar magnetism theory. On one hand, since they survive on secular time scales, they may modify the structure and the evolution of their host stars. On the other hand, they must have a complex stable structure since it has been demonstrated that the simplest purely poloidal or toroidal fields are unstable on dynamical time scales. In this context, the only stable stellar configurations found today are those resulting from numerical simulations by Braithwaite and collaborators who studied the evolution of an initial stochastic magnetic field, which relaxes with a selective decay of magnetic helicity and energy, on mixed stable configurations (poloidal and toroidal) that seem to be in equilibrium and then diffuse. In this talk, we report the semi-analytical investigation of such an equilibrium field in the axisymmetric case. We use variational methods, which describe selective decay of magnetic helicity and energy during MHD relaxation, and we identify a supplementary invariant due to the stable stratification of stellar radiation zones. This leads to states that generalize force-free Taylor's relaxation states studied in plasma laboratory experiments that become non force-free in the stellar case. Moreover, astrophysical applications are presented and the stability of obtained configurations is studied.},
  keywords = {magnetohydrodynamics (MHD),notion,notion-database,plasmas,stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/GEUW5ZBX/full-text.pdf}
}

@article{Mathis2011a,
  title = {Low-Frequency Internal Waves in Magnetized Rotating Stellar Radiation Zones: {{I}}. {{Wave}} Structure Modification by a Toroidal Field},
  author = {Mathis, S. and De Brye, N.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {526},
  number = {8},
  pages = {1--12},
  issn = {00046361},
  doi = {10.1051/0004-6361/201015571},
  abstract = {Context. The study of helioseismology, asteroseismology, and powerful ground-based instrumentation dedicated to stellar physics is developing strongly (cf. CoRoT, KEPLER, and ESPaDOnS). This generates tight constraints on the stellar internal structure and dynamical processes. In this context, it is thus necessary to go beyond the non-rotating and the non-magnetic picture of stellar interiors, particularly for large-scale transport mechanisms and waves. Aims. We focus on low-frequency internal waves in magnetic, rotating, stably stratified stellar radiation zones. For frequencies, which can be close to the Alfv\'en and the inertial frequencies, we go beyond the non-magnetic and non-rotating description of wave dynamics with taking the Coriolis acceleration and the Lorentz force into account. Then, we have to couple wave dynamics with fossil magnetic fields, which must have mixed configurations (both poloidal and toroidal) to survive in stellar radiation zones. Methods. We chose to study such coupling step by step, first with purely toroidal fields and then with purely poloidal fields, to unravel their modification by each corresponding component of a realistic mixed-field. Thus, we analytically built a complete formalism, which describes both effects of the Coriolis acceleration and of the Lorentz force in a non-perturbative way in the case of an axisymmetric toroidal field. We consider here the case where both Alfv\'en frequency and angular velocity are chosen to be uniform, to isolate wave properties. Results. The different approximations possible for low-frequency internal waves in this model are examined and discussed. In this way, the traditional approximation used to describe the dynamics of low-frequency regular elliptic gravito-inertial waves in the purely hydrodynamical case is generalized to the magnetic one. The complete structure of internal waves, which become magneto-gravito-inertial waves, is then derived and compared to the non-magnetic case. The asymptotic behaviour of such waves is obtained. Conclusions. A global study of magneto-gravito-inertial waves in stellar radiation zones is achieved in the case of an axisymmetric toroidal magnetic field. In the near future, consequences for angular momentum transport and the case of general differential rotation and azimuthal magnetic field have to be studied. Moreover, the same methodology must be applied to the case of poloidal fields, and the hyperbolic regime has to be carefully studied. \textcopyright{} 2010 ESO.},
  keywords = {magnetohydrodynamics (MHD),methods: analytical,notion,notion-database,stars: magnetic field,stars: oscillations,stars: rotation,waves},
  file = {/Users/lbugnet/Zotero/storage/MYP74UFB/Mathis, De Brye - 2011.pdf}
}

@article{Mathis2012a,
  title = {Low-Frequency Internal Waves in Magnetized Rotating Stellar Radiation Zones: {{II}}. {{Angular}} Momentum Transport with a Toroidal Field},
  author = {Mathis, S. and De Brye, N.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {540},
  issn = {00046361},
  doi = {10.1051/0004-6361/201118322},
  abstract = {Context. With the progress of observational constraints on dynamical processes in stars, it becomes necessary to understand the angular momentum and the rotation profile history. In this context, internal waves constitute an efficient transport mechanism over long distances in stellar radiation zones. Indeed, they could be one of the mechanisms responsible for the quasi-flat rotation profile of the solar radiative region up to 0.2 R {$\odot$}. Aims. Angular momentum transport induced by internal waves depends on the properties of their excitation regions and of their dissipation during propagation. Then, the bottom of convective envelopes (the top of convective cores, respectively) are differentially rotating magnetic layers while radiation zones may host fossil magnetic fields. It is therefore necessary to understand the modification of internal wave mechanisms by both rotation and magnetic fields. Methods. We continue our previous work by proceeding step by step. We analytically built a complete formalism that treats the angular momentum transport by internal waves while taking into account both the Coriolis acceleration and the Lorentz force in a non-perturbative way for an axisymmetric toroidal field. We assumed a uniform Alfv\'en frequency and a weak differential rotation to isolate the transport properties as a function of the Rossby and Elsasser numbers. Results. We examined the different possible approximations to describe low-frequency internal waves modified by the Coriolis acceleration and the Lorentz force in a deep spherical shell. The complete structure of these waves, which become magneto-gravito-inertial waves, is given assuming the quasi-linear approximation first in the adiabatic case and then in the dissipative one. Vertical and equatorial trapping phenomena appear that favor retrograde waves. The efficiency of the induced transport as a function of the Rossby and Elsasser numbers is then obtained. Conclusions. A complete study of the transport of angular momentum induced by magneto-gravito-inertial waves in stellar radiative regions is achieved for an axisymmetric toroidal magnetic field for a uniform Alfv\'en frequency and a weak differential rotation. General differential rotation, complex azimuthal magnetic fields, and poloidal and mixed fields will be examined in follow-up studies. \textcopyright{} 2012 ESO.},
  keywords = {magnetohydrodynamics (MHD),methods: analytical,notion,notion-database,stars: evolution,stars: magnetic field,stars: rotation,waves},
  file = {/Users/lbugnet/Zotero/storage/JPFZ2HHN/Mathis, De Brye - 2012.pdf}
}

@article{Mathis2013,
  title = {Angular Momentum Transport by Internal Waves in Stellar Interiors},
  author = {Mathis, S.},
  year = {2013},
  journal = {EAS Publications Series},
  volume = {63},
  pages = {269--284},
  issn = {16381963},
  doi = {10.1051/eas/1363031},
  abstract = {Internal gravity waves are excited in stellar interiors thanks to turbulent convective regions, to opacity bumps and to tides when there is a close stellar or planetary companion. Then, they propagate in stably stratified stellar radiation zones where they deposit/extract angular momentum by damping processes and corotation resonances. This modifies the rotational evolution as well as the internal mixing in stars. In this review, we will present the state of the art for modelling such transport mechanisms with a peculiar focus on the most recent advances taking into account the influence of rotation, shear, and magnetic fields on internal gravity waves. Next, we will discuss consequences for stars dynamical evolution and what can be learnt from stellar seismology.},
  keywords = {asteroseismology,evolution,including pulsations,interiors,notion,notion-database,oscillations,rotation,stars,waves},
  file = {/Users/lbugnet/Zotero/storage/7MG5GBZT/Mathis - 2013.pdf}
}

@article{Mathis2013a,
  title = {Diagnoses to Unravel Secular Hydrodynamical Processes in Rotating Main Sequence Stars: {{II}}. the Actions of Internal Gravity Waves},
  author = {Mathis, S. and Decressin, T. and Eggenberger, P. and Charbonnel, C.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {558},
  pages = {271--286},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321934},
  abstract = {Context. With the progress of observational constraints on stellar rotation and on the angular velocity profile in stars, it is necessary to understand how angular momentum is transported in stellar interiors during their whole evolution. In this context, more highly refined dynamical stellar evolution models have been built that take into account transport mechanisms. Aims. Internal gravity waves (IGWs) excited by convective regions constitute an efficient transport mechanism over long distances in stellar radiation zones. They are one of the mechanisms that are suspected of being responsible for the quasi-flat rotation profile of the solar radiative region up to 0.2 R \^a\v{S}\texttrademark. Therefore, we include them in our detailed analysis started in Paper I of the main physical processes responsible for the transport of angular momentum and chemical species in stellar radiation zones. Here, we focus on the complete interaction between differential rotation, meridional circulation, shear-induced turbulence, and IGWs during the main sequence. Methods. We improved the diagnosis tools designed in Paper I to unravel angular momentum transport and chemical mixing in rotating stars by taking into account IGWs. The star's secular hydrodynamics is treated using projection on axisymmetric spherical harmonics and appropriate horizontal averages that allow the problem to be reduced to one dimension while preserving the non-diffusive character of angular momentum transport by the meridional circulation and IGWs. Wave excitation by convective zones is computed at each time-step of the evolution track. We choose here to analyse the evolution of a 1.1 M\^a\v{S}\texttrademark, Z\^a\v{S}\texttrademark{} star in which IGWs are known to be efficient. Results. We quantify the relative importance of the physical mechanisms that sustain meridional currents and that drive the transport of angular momentum, heat, and chemicals when IGWs are taken into account. First, angular momentum extraction, Reynolds stresses caused by IGWs, and viscous stresses sustain a large-scale multi-cellular meridional circulation. This circulation in turn advects entropy, which generates temperature fluctuations and a new rotation profile because of thermal wind. Conclusions. We have refined our diagnosis of secular transport processes in stellar interiors. We confirm that meridional circulation is sustained by applied torques, internal stresses, and structural readjustments, rather than by thermal imbalance, and we detail the impact of IGWs. These large-scale flows then modify the thermal structure of stars, their internal rotation profile, and their chemical stratification. The tools we developed in Paper I and generalised for the present analysis will be used in the near future to study secular hydrodynamics of rotating stars taking into account IGWs in the whole Hertzsprung-Russell diagram. \textcopyright{} ESO, 2013.},
  keywords = {Hydrodynamics,notion,notion-database,Stars: evolution,Stars: rotation,Turbulence,Waves},
  file = {/Users/lbugnet/Zotero/storage/UBVVFJM9/Mathis et al. - 2013.pdf}
}

@incollection{Mathis2013b,
  title = {Transport {{Processes}} in {{Stellar Interiors}}},
  booktitle = {{{LNP}}},
  author = {Mathis, St{\'e}phane},
  year = {2013},
  volume = {865},
  pages = {23--47},
  doi = {10.1007/978-3-642-33380-4_2},
  urldate = {2020-07-02},
  keywords = {notion,notion-database,Physics}
}

@article{Mathis2014,
  title = {Impact of Rotation on Stochastic Excitation of Gravity and Gravito-Inertial Waves in Stars},
  author = {Mathis, S and Neiner, C and Tran, N},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {565},
  number = {A47},
  eprint = {1403.6373v1},
  urldate = {2020-12-22},
  abstract = {Context. Gravity waves (or their signatures) are detected in stars thanks to helio-and asteroseismology and they may play an important role in the evolution of stellar angular momentum. Moreover, the observational study of the CoRoT target HD 51452 by Neiner and collaborators demonstrated the potential strong impact of rotation on the stochastic excitation of gravito-inertial waves in stellar interiors. Aims. Our goal is to explore and unravel the action of rotation on the stochastic excitation of gravity and gravito-inertial waves in stars. Methods. The dynamics of gravito-inertial waves in stellar interiors, both in radiation and in convection zones, is described with a local non-traditional f-plane model. Their couplings with convective turbulent flows leading to their stochastic excitation is studied in this framework. Results. First, we find that, in the super-inertial regime in which the wave frequency is over twice the rotation frequency ({$\sigma$} {$>$} 2{$\Omega$}), the evanescence of gravito-inertial waves in convective regions decreases with decreasing wave frequency. Next, in the sub-inertial regime ({$\sigma$} {$<$} 2{$\Omega$}), gravito-inertial waves become purely propagative inertial waves in convection zones. Simultaneously, turbulence in convective regions is modified by rotation. Indeed, the turbulent energy cascade towards small scales is slowed down and in the case of rapid rotation, strongly anisotropic turbulent flows are obtained that can be understood as complex non-linear triadic interactions of propagative inertial waves. These different behaviours, due to the action of the Coriolis acceleration, strongly modify the wave couplings with turbulent flows. On one hand, turbulence weakly influenced by rotation is coupled with evanescent gravito-inertial waves. On the other hand, rapidly rotating turbulence is intrinsically and strongly coupled with sub-inertial waves. Finally, to study these mechanisms, the traditional approximation cannot be assumed because it does not properly treat the couplings between gravity and inertial waves in the sub-inertial regime. Conclusions. Our results demonstrate the action of rotation on stochastic excitation of gravity waves thanks to the Coriolis acceleration which modifies their dynamics in rapidly rotating stars and turbulent flows. As the ratio 2{$\Omega$}/{$\sigma$} increases, the couplings and thus the amplitude of stochastic gravity waves are amplified.},
  archiveprefix = {arxiv},
  keywords = {evolution,hydrodynamics-waves-turbulence-stars,notion,notion-database,rotation-stars},
  file = {/Users/lbugnet/Zotero/storage/KV64HDT7/full-text.pdf}
}

@article{Mathis2016,
  title = {The Impact of Rotation on Turbulent Tidal Friction in Stellar and Planetary Convective Regions},
  author = {Mathis, St{\'e}phane and {Auclair-Desrotour}, Pierre and Guenel, Mathieu and Gallet, Florian and {Poncin-Lafitte}, Christophe Le},
  year = {2016},
  month = apr,
  eprint = {1604.08570},
  doi = {10.1051/0004-6361/201527545},
  urldate = {2020-07-13},
  abstract = {Turbulent friction in convective regions in stars and planets is one of the key physical mechanisms that drive the dissipation of the kinetic energy of tidal flows in their interiors and the evolution of their systems. This friction acts both on the equilibrium/non-wave like tide and on tidal inertial waves in these layers. It is thus necessary to obtain a robust prescription for this friction. In the current state-of-the-art, it is modeled by a turbulent eddy-viscosity coefficient, based on mixing-length theory, applied on velocities of tides. However, none of the current prescriptions take into account the action of rotation that can strongly affects turbulent convection. Therefore, we use theoretical scaling laws for convective velocities and characteristic lengthscales in rotating stars and planets that have been recently confirmed by 3-D high-resolution nonlinear Cartesian numerical simulations to derive a new prescription. A corresponding local model of tidal waves is used to understand the consequences for the linear tidal dissipation. Finally, new grids of rotating stellar models and published values of planetary convective Rossby numbers are used to discuss astrophysical consequences. The action of rotation on convection deeply modifies the turbulent friction applied on tides. In the regime of rapid rotation (with a convective Rossby number below 0.25), the eddy-viscosity may be decreased by several ordres of magnitude. It may lead to a loss of efficiency of the viscous dissipation of the equilibrium tide and to a more efficient complex and resonant dissipation of tidal inertial waves in the bulk of convective regions. Therefore, it is necessary to have a completely coupled treatment of the tidal/rotational evolution of star-planet systems and multiple stars with a coherent treatment of the variations of tidal flows and of their dissipation as a function of rotation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FRBGVM5U/full-text.pdf}
}

@article{Mathis2018a,
  title = {Anisotropic Turbulent Transport in Stably Stratified Rotating Stellar Radiation Zones},
  author = {Mathis, S. and Prat, V. and Amard, L. and Charbonnel, C. and Palacios, A. and Lagarde, N. and Eggenberger, P.},
  year = {2018},
  journal = {Astronomy and Astrophysics},
  volume = {620},
  pages = {1--16},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629187},
  abstract = {Context. Rotation is one of the key physical mechanisms that deeply impact the evolution of stars. Helio- A nd asteroseismology reveal a strong extraction of angular momentum from stellar radiation zones over the whole Hertzsprung-Russell diagram. Aims. Turbulent transport in differentially rotating, stably stratified stellar radiation zones should be carefully modelled and its strength evaluated. Stratification and rotation imply that this turbulent transport is anisotropic. So far only phenomenological prescriptions have been proposed for the transport in the horizontal direction. This, however, constitutes a cornerstone in current theoretical formalisms for stellar hydrodynamics in evolution codes. We aim to improve its modelling. Methods. We derived a new theoretical prescription for the anisotropy of the turbulent transport in radiation zones using a spectral formalism for turbulence that takes simultaneously stable stratification, rotation, and a radial shear into account. Then, the horizontal turbulent transport resulting from 3D turbulent motions sustained by the instability of the radial differential rotation is derived. We implemented this framework in the stellar evolution code STAREVOL and quantified its impact on the rotational and structural evolution of solar metallicity low-mass stars from the pre-main-sequence to the red giant branch. Results. The anisotropy of the turbulent transport scales as N4{$\tau$}2/(2{$\Omega$}2), N and {$\Omega$} being the buoyancy and rotation frequencies respectively and {$\tau$} a time characterizing the source of turbulence. This leads to a horizontal turbulent transport of similar strength in average that those obtained with previously proposed prescriptions even if it can be locally larger below the convective envelope. Hence the models computed with the new formalism still build up too steep internal rotation gradients compared to helioseismic and asteroseismic constraints. As a consequence, a complementary transport mechanism such as internal gravity waves or magnetic fields is still needed to explain the observed strong transport of angular momentum along stellar evolution. Conclusions. The new prescription links for the first time the anisotropy of the turbulent transport in radiation zones to their stratification and rotation. This constitutes important theoretical progress and demonstrates how turbulent closure models should be improved to get firm conclusions on the potential importance of other processes that transport angular momentum and chemicals inside stars along their evolution.},
  keywords = {Hydrodynamics,notion,notion-database,Stars: Evolution,Stars: Rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/V7FT9CQ7/Mathis et al. - 2018.pdf}
}

@article{Mathis2019a,
  title = {Tidal Dissipation in Stars and Giant Planets: {{Jean-Paul}} Zahn's Pioneering Work and Legacy},
  author = {Mathis, S.},
  year = {2019},
  journal = {EAS Publications Series},
  volume = {82},
  pages = {5--33},
  publisher = {{EDP Sciences}},
  issn = {16381963},
  doi = {10.1051/eas/1982002},
  urldate = {2020-11-29},
  abstract = {In this lecture opening the session focused on tides in stellar and planetary systems, I will review the Jean-Paul Zahn's key contributions to the theory of tidal dissipation in stars and fluid planetary layers. I will first recall the general principles of tidal friction in celestial bodies. Then, I will focus on the theories of the stellar equilibrium and dynamical tides founded by Jean-Paul and their predictions for the evolution of binary stars. I will underline their essential legacy for ongoing studies of tidal dissipation in stars hosting planets and in fluid planetary regions. I will also discuss his pioneering work on the turbulent friction applied on tidal flows by stellar convection and the corresponding still unsolved challenging problems. Next, I will present the results we obtained on tidal dissipation in the potential dense rocky/icy core of gaseous giant planets such as Jupiter and Saturn within the Encelade international team. This mechanism provides important keys to interpret the high-precision astrometric measurements of the rates of tidal orbital migration of the moons of these planets, which are found to be larger than expected. This corresponds to a Jovian and Saturnian tidal frictions which are higher by one order of magnitude than the usually used values calibrated on formation scenarios. Finally, I will review the work done by Jean-Paul and Michel Rieutord on potential Ekman boundary layers associated to tidal flows. As a consequence, a coherent physical modeling of tides is now mandatory to understand the properties and the evolution of stellar and planetary systems. To progress on this forefront research subject, we are walking on the path first drawn by Jean-Paul.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/U2HPK8J6/full-text.pdf}
}

@article{Mathis2019a,
  title = {The Traditional Approximation of Rotation, Including the Centrifugal Acceleration for Slightly Deformed Stars},
  author = {Mathis, S. and Prat, V.},
  year = {2019},
  journal = {Astronomy \& Astrophysics},
  volume = {631},
  eprint = {1908.06521},
  pages = {A26},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201935639},
  abstract = {Context. The traditional approximation of rotation (TAR) is a treatment of the dynamical equations of rotating and stably stratified fluids in which the action of the Coriolis acceleration along the direction of the entropy (and chemicals) stratification is neglected, while assuming that the fluid motions are mostly horizontal because of their inhibition in the vertical direction by the buoyancy force. This leads to the neglect of the horizontal projection of the rotation vector in the equations for the dynamics of gravito-inertial waves (GIWs) that become separable, such as in the non-rotating case, while they are not separable in the case in which the full Coriolis acceleration is taken into account. This approximation, first introduced in geophysical fluid dynamics for thin atmospheres and oceans, has been broadly applied in stellar (and planetary) astrophysics to study low-frequency GIWs that have short vertical wavelengths. The appoximation is now being tested thanks to direct 2D oscillation codes, which constrain its domain of validity. The mathematical flexibility of this treatment allows us to explore broad parameter spaces and to perform detailed seismic modelling of stars.  Aims. The TAR treatment is built on the assumptions that the star is spherical (i.e. its centrifugal deformation is neglected) and uniformly rotating while an adiabatic treatment of the dynamics of the waves is adopted. In addition, their induced gravitational potential fluctuations is neglected. However, it has been recently generalised with including the effects of a differential rotation. We aim to carry out a new generalisation that takes into account the centrifugal acceleration in the case of deformed stars that are moderately and uniformly rotating.  Methods. We construct an analytical expansion of the equations for the dynamics of GIWs in a spheroidal coordinates system by assuming the hierarchies of frequencies and amplitudes of the velocity components adopted within TAR in the spherical case.  Results. We derive the complete set of equations that generalises TAR by taking the centrifugal acceleration into account. As in the case of a differentially rotating spherical star, the problem becomes 2D but can be treated analytically if we assume the anelastic and JWKB approximations, which are relevant for low-frequency GIWs. This allows us to derive a generalised Laplace tidal equation for the horizontal eigenfunctions and asymptotic wave periods, which can be used to probe the structure and dynamics of rotating deformed stars thanks to asteroseismology. A first numerical exploration of its eigenvalues and horizontal eigenfunctions shows their variation as a function of the pseudo-radius for different rotation rates and frequencies and the development of avoided crossings.},
  archiveprefix = {arxiv},
  keywords = {analytical,hydrodynamics,including pulsations,interiors,methods,notion,notion-database,oscillations,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/UR347C5C/Mathis, Prat - 2019.pdf}
}

@article{Mathis2021,
  title = {Probing the Internal Magnetism of Stars Using Asymptotic Magneto-Asteroseismology},
  author = {Mathis, St{\'e}phane and Bugnet, Lisa and Prat, Vincent and Augustson, Kyle and Mathur, Savita and Garcia, Rafael A.},
  year = {2021},
  month = dec,
  journal = {Astronomy and Astrophysics},
  volume = {647},
  number = {A122},
  eprint = {2012.11050},
  urldate = {2021-01-03},
  abstract = {Our knowledge of the dynamics of stars has undergone a revolution thanks to the simultaneous large amount of high-quality photometric observations collected by space-based asteroseismology and ground-based high-precision spectropolarimetry. They allowed us to probe the internal rotation of stars and their surface magnetism in the whole Hertzsprung-Russell diagram. However, new methods should still be developed to probe the deep magnetic fields in those stars. Our goal is to provide seismic diagnoses that allow us to sound the internal magnetism of stars. Here, we focus on asymptotic low-frequency gravity modes and high-frequency acoustic modes. Using a first-order perturbative theory, we derive magnetic splittings of their frequencies as explicit functions of stellar parameters. As in the case of rotation, we show how asymptotic gravity and acoustic modes can allow us to probe the different components of the magnetic field in the cavities where they propagate. This demonstrates again the high potential of using mixed-modes when this is possible.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: Analytical,notion,notion-database,Stars: Magnetic field,Stars: Oscillations (including pulsations),Waves},
  file = {/Users/lbugnet/Zotero/storage/SNDT7NI9/full-text.pdf}
}

@article{Mathis2023,
  title = {Asymmetries of Frequency Splittings of Dipolar Mixed Modes: {{A}} Window on the Topology of Deep Magnetic Fields},
  shorttitle = {Asymmetries of Frequency Splittings of Dipolar Mixed Modes},
  author = {Mathis, S. and Bugnet, L.},
  year = {2023},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {676},
  pages = {L9},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202346832},
  urldate = {2023-10-09},
  abstract = {Context. Space asteroseismology is revolutionizing our knowledge of the internal structure and dynamics of stars. A breakthrough is ongoing with the recent discoveries of signatures of strong magnetic fields in the core of red giant stars. The key signature for such a detection is the asymmetry these fields induce in the frequency splittings of observed dipolar mixed gravito-acoustic modes. Aims: We investigate the ability of the observed asymmetries of the frequency splittings of dipolar mixed modes to constrain the geometrical properties of deep magnetic fields. Methods: We used the powerful analytical Racah-Wigner algebra used in quantum mechanics to characterize the geometrical couplings of dipolar mixed oscillation modes with various realistically plausible topologies of fossil magnetic fields. We also computed the induced perturbation of their frequencies. Results: First, in the case of an oblique magnetic dipole, we provide the exact analytical expression of the asymmetry as a function of the angle between the rotation and magnetic axes. Its value provides a direct measure of this angle. Second, considering a combination of axisymmetric dipolar and quadrupolar fields, we show how the asymmetry is blind to the unraveling of the relative strength and sign of each component. Finally, in the case of a given multipole, we show that a negative asymmetry is a signature of non-axisymmetric topologies. Conclusions: Asymmetries of dipolar mixed modes provide a key bit of information on the geometrical topology of deep fossil magnetic fields, but this is insufficient on its own. Asteroseismic constraints should therefore be combined with spectropolarimetric observations and numerical simulations, which aim to predict the more probable stable large-scale geometries.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,methods: analytical,stars: magnetic field,stars: oscillations},
  annotation = {ADS Bibcode: 2023A\&A...676L...9M},
  file = {/Users/lbugnet/Zotero/storage/26YFZRMZ/Mathis and Bugnet - 2023 - Asymmetries of frequency splittings of dipolar mix.pdf}
}

@article{Mathur2008,
  title = {Sensitivity of Helioseismic Gravity Modes to the Dynamics of the Solar Core},
  author = {Mathur, S. and {Eff-Darwich}, A. and Garc{\'i}a, R. A. and {Turck-Chi{\`e}ze}, S.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {484},
  number = {2},
  pages = {517--522},
  issn = {00046361},
  doi = {10.1051/0004-6361:20078839},
  abstract = {Context: The dynamics of the solar core cannot be properly constrained through the analysis of acoustic oscillation modes. Gravity modes (g modes) are necessary to understand the structure and dynamics of the deepest layers of the Sun. Through recent progress on the observation of these modes - both individually and collectively - new information is available to contribute to inferring the rotation profile inside the nuclear burning core. Aims: We aim to see the sensitivity of gravity modes to the rotation of the solar core. We analyze the influence of adding the splitting of one and several g modes to the data sets used in helioseismic numerical inversions. We look for constraints on the uncertainties required in the observations to improve the derived core rotation profile. Methods: We compute three artificial sets of splittings derived for three rotation profiles: a rigid profile taken as a reference; a step-like profile and a smoother profile with higher rates in the core. We compute inversions based on regularized least-squares methodology (RLS) for both artificial data with real error bars and real data. Several sets of data are used: first, we invert only acoustic modes (p modes), then we add one and several g modes to which different values of observational uncertainties (75 and 7.5 nHz) are attributed. For the real data, we include g-mode candidate, , with several splittings and associated uncertainties. Results: We show that the introduction of one g mode in artificial data improves the rate in the solar core and gives an idea of the tendency of the rotation profile. The addition of more g modes lends greater accuracy to the inversions and stabilizes them. The inversion of real data with the g-mode candidate gives a rotation profile that remains unchanged down to 0.2 , whatever value of splitting we attribute to the g mode. \textcopyright{} 2008 ESO.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/ZURJKX4C/Mathur et al. - 2008.pdf}
}

@article{Mathur2010a,
  title = {Determining Global Parameters of the Oscillations of Solar-like Stars},
  author = {Mathur, S. and Garc{\'i}a, R. A. and R{\'e}gulo, C. and Creevey, O. L. and Ballot, J. and Salabert, D. and Arentoft, T. and Quirion, P. O. and Chaplin, W. J. and Kjeldsen, H.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {511},
  number = {1},
  eprint = {0912.3367},
  pages = {1--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/200913266},
  abstract = {Context: Helioseismology has enabled us to better understand the solar interior, while also allowing us to better constrain solar models. But now is a tremendous epoch for asteroseismology as space missions dedicated to studying stellar oscillations have been launched within the last years (MOST and CoRoT). CoRoT has already proved valuable results for many types of stars, while Kepler, which was launched in March 2009, will provide us with a huge number of seismic data very soon. This is an opportunity to better constrain stellar models and to finally understand stellar structure and evolution. Aims: The goal of this research work is to estimate the global parameters of any solar-like oscillating target in an automatic manner. We want to determine the global parameters of the acoustic modes (large separation, range of excited pressure modes, maximum amplitude, and its corresponding frequency), retrieve the surface rotation period of the star and use these results to estimate the global parameters of the star (radius and mass). Methods: To prepare for the arrival and the analysis of hundreds of solar-like oscillating stars, we have developed a robust and automatic pipeline, which was partially adapted from helioseismic methods. The pipeline consists of data analysis techniques, such as Fast Fourier Transform, wavelets, autocorrelation, as well as the application of minimisation algorithms for stellar-modelling. Results: We apply our pipeline to some simulated lightcurves from the asteroFLAG team and the Aarhus-asteroFLAG simulator, and obtain results that are consistent with the input data to the simulations. Our strategy gives correct results for stars with magnitudes below 11 with only a few 10\% of bad determinations among the reliable results. We then apply the pipeline to the Sun and three CoRoT targets. In particular we determine the large separation and radius of the Sun, HD49933, HD181906, and HD181420. \textcopyright{} 2010 ESO.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/MJ5T2MDY/Mathur et al. - 2010.pdf}
}

@article{Mathur2010b,
  title = {The Solar-like {{CoRoT}} Target {{HD}} 170987 : Spectroscopic},
  author = {Mathur, S and Garc{\'i}a, R A and Catala, C and Bruntt, H and Mosser, B and Appourchaux, T and Ballot, J and Creevey, O L},
  year = {2010},
  journal = {Astronomy \& Astrophysics},
  volume = {518},
  pages = {1--11},
  keywords = {asteroseismology,data analysis,hd 170987,individual,methods,notion,notion-database,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/6JL9JWJF/Mathur et al. - 2010(2).pdf}
}

@article{Mathur2011,
  title = {Solar-like Oscillations in {{KIC}} 11395018 and {{KIC}} 11234888 from 8 Months of {{Kepler}} Data},
  author = {Mathur, S. and Handberg, R. and Campante, T. L. and Garc{\'i}a, R. A. and Appourchaux, T. and Bedding, T. R. and Mosser, B. and Chaplin, W. J. and Ballot, J. and Benomar, O. and Bonanno, A. and Corsaro, E. and Gaulme, P. and Hekker, S. and R{\'e}gulo, C. and Salabert, D. and Verner, G. and White, T. R. and Brand{\~a}o, I. M. and Creevey, O. L. and Do{\v g}an, G. and Elsworth, Y. and Huber, D. and Hale, S. J. and Houdek, G. and Karoff, C. and Metcalfe, T. S. and {Molenda-Zakowicz}, J. and Monteiro, M. J.P.F.G. and Thompson, M. J. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kawaler, S. D. and Kjeldsen, H. and Quintana, E. V. and Sanderfer, D. T. and Seader, S. E.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {733},
  number = {2},
  eprint = {1103.4085},
  pages = {1--39},
  issn = {15384357},
  doi = {10.1088/0004-637X/733/2/95},
  abstract = {We analyze the photometric short-cadence data obtained with the Kepler mission during the first 8 months of observations of two solar-type stars of spectral types G and F: KIC 11395018 and KIC 11234888, respectively, the latter having a lower signal-to-noise ratio (S/N) compared with the former. We estimate global parameters of the acoustic (p) modes such as the average large and small frequency separations, the frequency of the maximum of the p-mode envelope, and the average line width of the acoustic modes. We were able to identify and to measure 22 p-mode frequencies for the first star and 16 for the second one even though the S/N of these stars are rather low. We also derive some information about the stellar rotation periods from the analyses of the low-frequency parts of the power spectral densities. A model-independent estimation of the mean density, mass, and radius is obtained using the scaling laws. We emphasize the importance of continued observations for the stars with low S/N for an improved characterization of the oscillation modes. Our results offer a preview of what will be possible for many stars with the long data sets obtained during the remainder of the mission. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,methods: data analysis,notion,notion-database,{stars: individual (KIC 11395018, KIC 11234888)},stars: oscillations,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/PPU26M62/Mathur et al. - 2011.pdf}
}

@article{Mathur2011a,
  title = {Granulation in Red Giants: {{Observations}} by the {{Kepler}} Mission and Three-Dimensional Convection Simulations},
  author = {Mathur, S. and Hekker, S. and Trampedach, R. and Ballot, J. and Kallinger, T. and Buzasi, D. and Garc{\'i}a, R. A. and Huber, D. and Jim{\'e}nez, A. and Mosser, B. and Bedding, T. R. and Elsworth, Y. and R{\'e}gulo, C. and Stello, D. and Chaplin, W. J. and De Ridder, J. and Hale, S. J. and Kinemuchi, K. and Kjeldsen, H. and Mullally, F. and Thompson, S. E.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {741},
  number = {2},
  eprint = {1109.1194},
  pages = {1--43},
  issn = {15384357},
  doi = {10.1088/0004-637X/741/2/119},
  abstract = {The granulation pattern that we observe on the surface of the Sun is due to hot plasma rising to the photosphere where it cools down and descends back into the interior at the edges of granules. This is the visible manifestation of convection taking place in the outer part of the solar convection zone. Because red giants have deeper convection zones than the Sun, we cannot a priori assume that their granulation is a scaled version of solar granulation. Until now, neither observations nor one-dimensional analytical convection models could put constraints on granulation in red giants. With asteroseismology, this study can now be performed. We analyze {$\sim$}1000 red giants that have been observed by Kepler during 13 months. We fit the power spectra with Harvey-like profiles to retrieve the characteristics of the granulation (timescale {$\tau$}gran and power P gran). We search for a correlation between these parameters and the global acoustic-mode parameter (the position of maximum power, {$\nu$}max) as well as with stellar parameters (mass, radius, surface gravity (log g), and effective temperature (T eff)). We show that {$\tau$}eff{$\omega\nu$}-0.89max and P gran{$\omega\nu$}-1.90max, which is consistent with the theoretical predictions. We find that the granulation timescales of stars that belong to the red clump have similar values while the timescales of stars in the red giant branch are spread in a wider range. Finally, we show that realistic three-dimensional simulations of the surface convection in stars, spanning the (T eff, log g) range of our sample of red giants, match the Kepler observations well in terms of trends. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {methods: data analysis,notion,notion-database,stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/5W6VNYWH/Mathur et al. - 2011(2).pdf;/Users/lbugnet/Zotero/storage/LQI7M8HY/full-text.pdf}
}

@article{Mathur2012,
  title = {Study of {{HD 169392A}} Observed by {{CoRoT}} and {{HARPS}}},
  author = {Mathur, S. and Bruntt, H. and Catala, C. and Benomar, O. and Davies, G. R. and Garc{\'i}a, R. A. and Salabert, D. and Ballot, J. and Mosser, B. and R{\'e}gulo, C. and Chaplin, W. J. and Elsworth, Y. and Handberg, R. and Hekker, S. and Mantegazza, L. and Michel, E. and Poretti, E. and Rainer, M. and Roxburgh, I. W. and Samadi, R. and St{\c e}licki, M. and Uytterhoeven, K. and Verner, G. A. and Auvergne, M. and Baglin, A. and Barcel{\'o} Forteza, S. and Baudin, F. and Roca Cort{\'e}s, T.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {549},
  pages = {1--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219678},
  abstract = {Context. The results obtained by asteroseismology with data from space missions such as CoRoT and Kepler are providing new insights into stellar evolution. After five years of observations, CoRoT is continuing to provide high-quality data and we here present an analysis of the CoRoT observations of the double star HD 169392, complemented by ground-based spectroscopic observations. Aims. This work aims at characterising the fundamental parameters of the two stars, their chemical composition, the acoustic-mode global parameters including their individual frequencies, and their dynamics. Methods. We analysed HARPS observations of the two stars to derive their chemical compositions. Several methods were used and compared to determine the global properties of stars' acoustic modes and their individual frequencies from the photometric data of CoRoT. Results. The new spectroscopic observations and archival astrometric values suggest that HD 169392 is a weakly bound wide binary system. We obtained spectroscopic parameters for both components which suggest that they originate from the same interstellar cloud. However, only the signature of oscillation modes of HD 169392 A was measured; the signal-to-noise ratio of the modes in HD 169392B is too low to allow any confident detection. For HD 169392 A we were able to extract parameters of modes for = 0, 1, 2, and 3. The analysis of splittings and inclination angle gives two possible solutions: one with with splittings and inclination angles of 0.4-1.0 {$\mu$}Hz and 20-40\textdegree, the other with 0.2-0.5 {$\mu$}Hz and 55-86\textdegree. Modelling this star using the Asteroseismic Modeling Portal (AMP) gives a mass of 1.15 {$\pm$} 0.01 M{$\cdot$}, a radius of 1.88 {$\pm$} 0.02 R{$\cdot$}, and an age of 4.33 {$\pm$} 0.12 Gyr. The uncertainties come from estimated errors on the observables but do not include uncertainties on the surface layer correction or the physics of stellar models. \textcopyright{} 2012 ESO.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: individual: HD 169392,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/XMMIRL67/Mathur et al. - 2012.pdf}
}

@article{Mathur2012a,
  title = {A Uniform Asteroseismic Analysis of 22 Solar-Type Stars Observed by {{Kepler}}},
  author = {Mathur, S. and Metcalfe, T. S. and Woitaszek, M. and Bruntt, H. and Verner, G. A. and {Christensen-Dalsgaard}, J. and Creevey, O. L. and Dogan, G. and Basu, S. and Karoff, C. and Stello, D. and Appourchaux, T. and Campante, T. L. and Chaplin, W. J. and Garc{\'i}a, R. A. and Bedding, T. R. and Benomar, O. and Bonanno, A. and Deheuvels, S. and Elsworth, Y. and Gaulme, P. and Guzik, J. A. and Handberg, R. and Hekker, S. and Herzberg, W. and Monteiro, M. J.P.F.G. and Piau, L. and Quirion, P. O. and R{\'e}gulo, C. and Roth, M. and Salabert, D. and Serenelli, A. and Thompson, M. J. and Trampedach, R. and White, T. R. and Ballot, J. and Brand{\~a}o, I. M. and {Molenda-Zakowicz}, J. and Kjeldsen, H. and Twicken, J. D. and Uddin, K. and Wohler, B.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {749},
  number = {2},
  eprint = {1202.2844},
  issn = {15384357},
  doi = {10.1088/0004-637X/749/2/152},
  abstract = {Asteroseismology with the Kepler space telescope is providing not only an improved characterization of exoplanets and their hoststars, but also a new window on stellar structure and evolution for the large sample of solar-typestars in the field. We perform a uniform analysis of 22 of the brightest asteroseismic targets with the highest signal-to-noise ratio observed for 1 month each during the first year of the mission, and we quantify the precision and relative accuracy of asteroseismic determinations of the stellar radius, mass, and age that are possible using various methods. We present the properties of each star in the sample derived from an automated analysis of the individual oscillation frequencies and other observational constraints using the Asteroseismic Modeling Portal (AMP), and we compare them to the results of model-grid-based methods that fit the global oscillation properties. We find that fitting the individual frequencies typically yields asteroseismic radii and masses to {$\sim$}1\% precision, and ages to {$\sim$}2.5\% precision (respectively, 2, 5, and 8 times better than fitting the global oscillation properties). The absolute level of agreement between the results from different approaches is also encouraging, with model-grid-based methods yielding slightly smaller estimates of the radius and mass and slightly older values for the stellar age relative to AMP, which computes a large number of dedicated models for each star. The sample of targets for which this type of analysis is possible will grow as longer data sets are obtained during the remainder of the mission. \textcopyright{} 2012 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {methods: numerical,notion,notion-database,stars: evolution,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VLYFYXUH/Mathur et al. - 2012(2).pdf}
}

@article{Mathur2013,
  title = {Constraining Magnetic-Activity Modulations in Three Solar-like Stars Observed by {{CoRoT}} and {{NARVAL}}},
  author = {Mathur, S. and Garc{\'i}a, R. A. and Morgenthaler, A. and Salabert, D. and Petit, P. and Ballot, J. and R{\'e}gulo, C. and Catala, C.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {550},
  pages = {1--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117913},
  abstract = {Context. Stellar activity cycles are the manifestation of dynamo process running in the stellar interiors. They have been observed from years to decades thanks to the measurement of stellar magnetic proxies on the surface of the stars, such as the chromospheric and X-ray emissions, and to the measurement of the magnetic field with spectropolarimetry. However, all of these measurements rely on external features that cannot be visible during, for example, a Maunder-type minimum. With the advent of long observations provided by space asteroseismic missions, it has been possible to penetrate the stars and study their properties. Moreover, the acoustic-mode properties are also perturbed by the presence of these dynamos. Aims. We track the temporal variations of the amplitudes and frequencies of acoustic modes allowing us to search for signature of magnetic activity cycles, as has already been done in the Sun and in the CoRoT target HD 49933. Methods. We used asteroseimic tools and more classical spectroscopic measurements performed with the NARVAL spectropolarimeter to check that there are hints of any activity cycle in three solar-like stars observed continuously for more than 117 days by the CoRoT satellite: HD 49385, HD 181420, and HD 52265. To consider that we have found a hint of magnetic activity in a star we require finding a change in the amplitude of the p modes that should be anti-correlated with a change in their frequency shifts, as well as a change in the spectroscopic observations in the same direction as the asteroseismic data. Results. Our analysis gives very small variation in the seismic parameters preventing us from detecting any magnetic modulation. However, we are able to provide a lower limit of any magnetic-activity change in the three stars that should be longer than 120 days, which is the length of the time series. Moreover we computed the upper limit for the line-of-sight magnetic field component being 1, 3, and 0.6 G for HD 49385, HD 181420, and HD 52265, respectively. More seismic and spectroscopic data would be required to have a firm detection in these stars. \textcopyright{} 2013 ESO.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: activity,Stars: general,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/Z6VYSVD2/Mathur et al. - 2013.pdf}
}

@article{Mathur2014,
  title = {Magnetic Activity of {{F}} Stars Observed by {{Kepler}}},
  author = {Mathur, S. and Garc{\'i}a, R. A. and Ballot, J. and Ceillier, T. and Salabert, D. and Metcalfe, T. S. and R{\'e}gulo, C. and Jim{\'e}nez, A. and Bloemen, S.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {562},
  pages = {1--24},
  issn = {00046361},
  doi = {10.1051/0004-6361/201322707},
  abstract = {Context. The study of stellar activity is important because it can provide new constraints for dynamo models when combined with surface rotation rates and the depth of the convection zone. We know that the dynamo mechanism, which is believed to be the main process that rules the magnetic cycle of solar-like stars, results from the interaction between (differential) rotation, convection, and magnetic field. The Kepler mission has already been collecting data for a large number of stars during four years allowing us to investigate magnetic stellar cycles. Aims. We investigated the Kepler light curves to look for magnetic activity or even hints of magnetic activity cycles. Based on the photometric data we also looked for new magnetic indexes to characterise the magnetic activity of the stars. Methods. We selected a sample of 22 solar-like F stars that have a rotation period shorter than 12 days. We performed a time-frequency analysis using the Morlet wavelet yielding a magnetic proxy for our sample of stars. We computed the magnetic index Sph as the standard deviation of the whole time series and the index \^aY\"\" Sph \textcopyright, which is the mean of standard deviations measured in subseries of length five times the rotation period of the star. We defined new indicators, such as the contrast between high and low activity, to take into account the fact that complete magnetic cycles are not observed for all the stars. We also inferred the Rossby number of the stars and studied their stellar background. Results. This analysis shows different types of behaviour in the 22 F stars. Two stars show behaviour very similar to magnetic activity cycles. Five stars show long-lived spots or active regions suggesting the existence of active longitudes. Two stars in our sample seem to have a decreasing or increasing trend in the temporal variation of the magnetic proxies. Finally, the last group of stars shows magnetic activity (with the presence of spots) but no sign of cycle. \textcopyright{} 2014 ESO.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: activity,Stars: general,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/JBX9KQ8M/Mathur et al. - 2014.pdf}
}

@article{Mathur2014a,
  title = {Photometric Magnetic-Activity Metrics Tested with the {{Sun}}: {{Application}} to {{Kepler M}} Dwarfs},
  author = {Mathur, Savita and Salabert, David and Garc{\'i}a, Rafael A. and Ceillier, Tugdual},
  year = {2014},
  journal = {Journal of Space Weather and Space Climate},
  volume = {4},
  eprint = {1404.3076},
  issn = {21157251},
  doi = {10.1051/swsc/2014011},
  abstract = {The Kepler mission has been providing high-quality photometric data leading to many breakthroughs in the exoplanet search and in stellar physics. Stellar magnetic activity results from the interaction between rotation, convection, and magnetic field. Constraining these processes is important if we want to better understand stellar magnetic activity. Using the Sun, we want to test a magnetic activity index based on the analysis of the photometric response and then apply it to a sample of M dwarfs observed by Kepler. We estimate a global stellar magnetic activity index by measuring the standard deviation of the whole time series, Sph. Because stellar variability can be related to convection, pulsations or magnetism, we need to ensure that this index mostly takes into account magnetic effects. We define another stellar magnetic activity index as the average of the standard deviation of shorter subseries which lengths are determined by the rotation period of the star. This way we can ensure that the measured photometric variability is related to starspots crossing the visible stellar disc. This new index combined with a time-frequency analysis based on the Morlet wavelets allows us to determine the existence of magnetic activity cycles. We measure magnetic indexes for the Sun and for 34 M dwarfs observed by Kepler. As expected, we obtain that the sample of M dwarfs studied in this work is much more active than the Sun. Moreover, we find a small correlation between the rotation period and the magnetic index. Finally, by combining a time-frequency analysis with phase diagrams, we discover the presence of long-lived features suggesting the existence of active longitudes on the surface of these stars. \textcopyright{} 2014 S. Mathur et al., Published by EDP Sciences.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,M dwarfs,notion,notion-database,Solar activity,Stellar activity},
  file = {/Users/lbugnet/Zotero/storage/YMZKXZDJ/Mathur et al. - 2014(2).pdf}
}

@article{Mathur2016,
  title = {Probing the {{Deep End}} of the {{Milky Way With Kepler}} : {{Asteroseismic Analysis}} of 854 {{Faint Red Giants Misclassified As Cool Dwarfs}}},
  author = {Mathur, S. and Garc{\'i}a, R. A. and Huber, D. and Regulo, C. and Stello, D. and Beck, P. G. and Houmani, K. and Salabert, D.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {827},
  number = {1},
  eprint = {1605.03675},
  pages = {50},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/827/1/50},
  abstract = {Asteroseismology has proven to be an excellent tool to determine not only the global stellar properties with a good precision but also to infer stellar structure, dynamics, and evolution for a large sample of Kepler stars. Prior to the launch of the mission the properties of Kepler targets were inferred from broadband photometry, leading to the Input Catalog (KIC Brown et al. 2011). The KIC was later revised in the Kepler Star Properties Catalog (Huber et al. 2014), based on literature values and an asteroseismic analysis of stars which were unclassified in the KIC. Here we present an asteroseismic analysis of 45,400 stars which were classified as dwarfs in the Kepler Star Properties Catalog. We found that around 2\% of the sample shows acoustic modes in the typical frequency range that put them in the red-giant category rather than cool dwarfs. We analyse the asteroseismic properties of these stars, derive their surface gravities, masses, and radii and present updated effective temperatures and distances. We show that the sample is significantly fainter than the previously known oscillating giants in the Kepler field, with the faintest stars reaching down to a Kepler magnitude, Kp\textasciitilde 16. We demonstrate that 404 stars are at distances beyond 5 kpc and that the stars are significantly less massive than for the original Kepler red-giant sample, consistent with a population of distant halo giants. A comparison with a galactic population model shows that up to 40 stars might be genuine halo giants, which would increase the number of known asteroseismic halo stars by a factor of 4. The detections presented here will provide a valuable sample for galactic archeology studies.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HJXQVSSL/Mathur et al. - 2016.pdf}
}

@article{Mathur2017,
  title = {Revised {{Stellar Properties}} of {{Kepler Targets}} for the {{Q1-17}} ({{DR25}}) {{Transit Detection Run}}},
  author = {Mathur, Savita and Huber, Daniel and Batalha, Natalie M. and Ciardi, David R. and Bastien, Fabienne A. and Bieryla, Allyson and Buchhave, Lars A. and Cochran, William D. and Endl, Michael and Esquerdo, Gilbert A. and Furlan, Elise and Howard, Andrew and Howell, Steve B. and Isaacson, Howard and Latham, David W. and MacQueen, Phillip J. and Silva, David R.},
  year = {2017},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {229},
  number = {2},
  eprint = {1609.04128},
  pages = {30},
  publisher = {{IOP Publishing}},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/229/2/30},
  abstract = {The determination of exoplanet properties and occurrence rates using Kepler data critically depends on our knowledge of the fundamental properties (such as temperature, radius and mass) of the observed stars. We present revised stellar properties for 197,096 Kepler targets observed between Quarters 1-17 (Q1-17), which were used for the final transiting planet search run by the Kepler Mission (Data Release 25, DR25). Similar to the Q1--16 catalog by Huber et al. the classifications are based on conditioning published atmospheric parameters on a grid of Dartmouth isochrones, with significant improvements in the adopted methodology and over 29,000 new sources for temperatures, surface gravities or metallicities. In addition to fundamental stellar properties the new catalog also includes distances and extinctions, and we provide posterior samples for each stellar parameter of each star. Typical uncertainties are \textasciitilde 27\% in radius, \textasciitilde 17\% in mass, and \textasciitilde 51\% in density, which is somewhat smaller than previous catalogs due to the larger number of improved logg constraints and the inclusion of isochrone weighting when deriving stellar posterior distributions. On average, the catalog includes a significantly larger number of evolved solar-type stars, with an increase of 43.5\% in the number of subgiants. We discuss the overall changes of radii and masses of Kepler targets as a function of spectral type, with particular focus on exoplanet host stars.},
  archiveprefix = {arxiv},
  keywords = {catalogs,{catalogs,planetary systems,stars: distances,stars:},distances,evolution,fundamental parameters,machine-readable tables,notion,notion-database,planetary systems,stars,supporting material},
  file = {/Users/lbugnet/Zotero/storage/259SPP2E/Mathur et al. - 2017.pdf}
}

@article{Mathur2019,
  title = {Revisiting the {{Impact}} of {{Stellar Magnetic Activity}} on the {{Detectability}} of {{Solar-Like Oscillations}} by {{Kepler}}},
  author = {Mathur, Savita and Garc{\'i}a, Rafael A. and Bugnet, Lisa and Santos, {\^A}ngela R.G. and Santiago, Netsha and Beck, Paul G.},
  year = {2019},
  month = jul,
  journal = {Frontiers in Astronomy and Space Sciences},
  volume = {6},
  issn = {2296-987X},
  doi = {10.3389/fspas.2019.00046},
  urldate = {2020-01-16},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9BPU25CW/fspas-06-00046.pdf}
}

@misc{mathurRevisitingImpactStellar2019,
  title = {Revisiting the Impact of Stellar Magnetic Activity on the Detectability of Solar-like Oscillations by {{Kepler}}},
  author = {Mathur, S. and Garc{\'i}a, R.A. and Bugnet, L. and Santos, {\^A}.R.G. and Santiago, N. and Beck, P.G.},
  year = {2019},
  journal = {arXiv},
  abstract = {Copyright \textcopyright{} 2019, arXiv, All rights reserved. Over 2,000 stars were observed for one month with a high enough cadence in order to look for acoustic modes during the survey phase of the Kepler mission. Solar-like oscillations have been detected in about 540 stars. The question of why no oscillations were detected in the remaining stars is still open. Previous works explained the non-detection of modes with the high level of magnetic activity of the stars. However, the sample of stars studied contained some classical pulsators and red giants that could have biased the results. In this work, we revisit this analysis on a cleaner sample of main-sequence solar-like stars that consists of 1,014 stars. First we compute the predicted amplitude of the modes of that sample and for the stars with detected oscillation and compare it to the noise at high frequency in the power spectrum. We find that the stars with detected modes have an amplitude to noise ratio larger than 0.94. We measure reliable rotation periods and the associated photometric magnetic index for 684 stars out of the full sample and in particular for 323 stars where the amplitude of the modes is predicted to be high enough to be detected. We find that among these 323 stars 32\% of them have a level of magnetic activity larger than the Sun during its maximum activity, explaining the non-detection of acoustic modes. Interestingly, magnetic activity cannot be the primary reason responsible for the absence of detectable modes in the remaining 68\% of the stars without acoustic modes detected and with reliable rotation periods. Thus, we investigate metallicity, inclination angle of the rotation axis, and binarity as possible causes of low mode amplitudes. Using spectroscopic observations for a subsample, we find that a low metallicity could be the reason for suppressed modes. No clear correlation with binarity nor inclination is found. We also derive the lower limit for our photometric activity index (of 20-30 ppm) below which rotation and magnetic activity are not detected. Finally, with our analysis we conclude that stars with a photometric activity index larger than 2,000 ppm have 98.3\% probability of not having oscillations detected.},
  keywords = {Asteroseismology,Magnetic Activity,Main-sequence stars,notion,notion-database,Solar-like oscillations,Stellar Rotation}
}

@article{Mathys2012,
  title = {A Search for Magnetic Fields in Cool {{sdB}} Stars},
  author = {Mathys, G. and Hubrig, S. and Mason, E. and Michaud, G. and Sch{\"o}ller, M. and Wesemael, F.},
  year = {2012},
  month = jan,
  journal = {Astronomische Nachrichten},
  volume = {333},
  pages = {30},
  issn = {0004-6337},
  doi = {10.1002/asna.201111618},
  urldate = {2023-10-09},
  abstract = {Hot cluster horizontal branch (HB) stars and field subdwarf B (sdB) stars are core helium burning stars that exhibit abundance anomalies that are believed to be due to atomic diffusion. Diffusion can be effective in these stars because they are slowly rotating. In particular, the slow rotation of the hot HB stars (T\_eff {$>$} 11 000 K), which show abundance anomalies, contrasts with the fast rotation of the cool HB stars, where the observed abundances are consistent with those of red giants belonging to the same cluster. The reason why sdB stars and hot HB stars are rotating slowly is unknown. In order to assess the possible role of magnetic fields on abundances and rotation, we investigated the occurrence of such fields in sdB stars with T\_eff {$<$} 30 000 K, whose temperatures overlap with those of the hot HB stars. We conclude that large-scale organised magnetic fields of kG order are not generally present in these stars but at the achieved accuracy, the possibility that they have fields of a few hundred Gauss remains open. We report the marginal detection of such a field in SB 290; further observations are needed to confirm it. Based on observations obtained at the European Southern Observatory, Paranal, Chile (ESO programmes 083.D-0007(A) and 087.D-0049(A)).},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: horizontal-branch,stars: individual (Feige 86),stars: magnetic fields,techniques: polarimetric},
  annotation = {ADS Bibcode: 2012AN....333...30M},
  file = {/Users/lbugnet/Zotero/storage/T3T53DTR/Mathys et al. - 2012 - A search for magnetic fields in cool sdB stars.pdf}
}

@article{Matson2019,
  title = {Detecting {{Unresolved Binaries}} in {{TESS Data}} with {{Speckle Imaging}}},
  author = {Matson, Rachel A. and Howell, Steve B. and Ciardi, David R.},
  year = {2019},
  journal = {The Astronomical Journal},
  volume = {157},
  number = {5},
  eprint = {1811.02108},
  pages = {211},
  publisher = {{IOP Publishing}},
  issn = {0004-6256},
  doi = {10.3847/1538-3881/ab1755},
  abstract = {The Transiting Exoplanet Survey Satellite (TESS) is conducting a two-year wide-field survey searching for transiting exoplanets around nearby bright stars that will be ideal for follow-up characterization. To facilitate studies of planet compositions and atmospheric properties, accurate and precise planetary radii need to be derived from the transit light curves. Since 40 - 50\% of exoplanet host stars are in multiple star systems, however, the observed transit depth may be diluted by the flux of a companion star, causing the radius of the planet to be underestimated. High angular resolution imaging can detect companion stars that are not resolved in the TESS Input Catalog, or by seeing-limited photometry, to validate exoplanet candidates and derive accurate planetary radii. We examine the population of stellar companions that will be detectable around TESS planet candidate host stars, and those that will remain undetected, by applying the detection limits of speckle imaging to the simulated host star populations of Sullivan et al. (2015) and Barclay et al. (2018). By detecting companions with contrasts of delta m {$<$} 7 - 9 and separations of \textasciitilde 0.02 - 1.2'', speckle imaging can detect companion stars as faint as early M stars around A - F stars and stars as faint as mid-M around G - M stars, as well as up to 99\% of the expected binary star distribution for systems located within a few hundred parsecs.},
  archiveprefix = {arxiv},
  keywords = {binaries,{binaries: general,binaries: visual,planetary syste},general,high angular resolution,machine-readable table,notion,notion-database,planetary systems,supporting material,techniques,visual},
  file = {/Users/lbugnet/Zotero/storage/T82PRJAI/Matson, Howell, Ciardi - 2019.pdf}
}

@article{Matt2012,
  title = {Magnetic Braking Formulation for Sun-like Stars: {{Dependence}} on Dipole Field Strength and Rotation Rate},
  author = {Matt, Sean P. and MacGregor, Keith B. and Pinsonneault, Marc H. and Greene, Thomas P.},
  year = {2012},
  journal = {Astrophysical Journal Letters},
  volume = {754},
  number = {2},
  issn = {20418205},
  doi = {10.1088/2041-8205/754/2/L26},
  abstract = {We use two-dimensional axisymmetric magnetohydrodynamic simulations to compute steady-state solutions for solar-like stellar winds from rotating stars with dipolar magnetic fields. Our parameter study includes 50 simulations covering a wide range of relative magnetic field strengths and rotation rates, extending from the slow- and approaching the fast-magnetic-rotator regimes. Using the simulations to compute the angular momentum loss, we derive a semi-analytic formulation for the external torque on the star that fits all of the simulations to a precision of a few percent. This formula provides a simple method for computing the magnetic braking of Sun-like stars due to magnetized stellar winds, which properly includes the dependence on the strength of the magnetic field, mass loss rate, stellar radius, surface gravity, and spin rate, and which is valid for both slow and fast rotators. \textcopyright{} 2012. The American Astronomical Society. All rights reserved..},
  keywords = {magnetohydrodynamics (MHD),notion,notion-database,stars: magnetic field,stars: rotation,stars: solar-type,{stars: winds, outflows}},
  file = {/Users/lbugnet/Zotero/storage/K3ENZHFJ/Matt et al. - 2012.pdf}
}

@article{Matt2015,
  title = {The Mass-Dependence of Angular Momentum Evolution in Sun-like Stars},
  author = {Matt, Sean P. and Brun, A. Sacha and Baraffe, Isabelle and Bouvier, J{\'e}r{\^o}me and Chabrier, Gilles},
  year = {2015},
  journal = {Astrophysical Journal Letters},
  volume = {799},
  number = {2},
  eprint = {1412.4786},
  pages = {1--6},
  issn = {20418213},
  doi = {10.1088/2041-8205/799/2/L23},
  abstract = {To better understand the observed distributions of the rotation rate and magnetic activity of Sun-like and low-mass stars, we derive a physically motivated scaling for the dependence of the stellar wind torque on the Rossby number. The torque also contains an empirically derived scaling with stellar mass (and radius), which provides new insight into the mass-dependence of stellar magnetic and wind properties. We demonstrate that this new formulation explains why the lowest mass stars are observed to maintain rapid rotation for much longer than solar-mass stars, and simultaneously why older populations exhibit a sequence of slowly rotating stars, in which the low-mass stars rotate more slowly than solar-mass stars. The model also reproduces some previously unexplained features in the period-mass diagram for the Kepler field, notably: the particular shape of the "upper envelope" of the distribution, suggesting that {$\sim$}95\% of Kepler field stars with measured rotation periods are younger than {$\sim$}4 Gyr; and the shape of the "lower envelope," corresponding to the location where stars transition between magnetically saturated and unsaturated regimes.},
  archiveprefix = {arxiv},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Outflows,Stars: evolution,Stars: late-type,Stars: magnetic field,Stars: rotation,Stars: winds},
  file = {/Users/lbugnet/Zotero/storage/FYA6LIXX/Matt et al. - 2015.pdf}
}

@incollection{Matteucci2010,
  title = {Chemical {{Enrichment}} in {{Galaxies}}: {{Constraints}} on {{Nucleogenesis}} and {{Galaxy Evolution}}},
  booktitle = {Galaxies and Their {{Masks}}},
  author = {Matteucci, Francesca},
  year = {2010},
  pages = {261--276},
  publisher = {{Springer New York}},
  doi = {10.1007/978-1-4419-7317-7_22},
  urldate = {2020-03-06},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/F7K6ICI2/full-text.pdf}
}

@article{Matteuzzi2023,
  title = {Red Horizontal Branch Stars: {{An}} Asteroseismic Perspective},
  shorttitle = {Red Horizontal Branch Stars},
  author = {Matteuzzi, Massimiliano and Montalb{\'a}n, Josefina and Miglio, Andrea and Vrard, Mathieu and Casali, Giada and Stokholm, Amalie and Tailo, Marco and Ball, Warrick H. and {van Rossem}, Walter E. and Valentini, Marica},
  year = {2023},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {671},
  pages = {A53},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202245746},
  urldate = {2023-08-01},
  abstract = {Robust age estimates of red giant stars are now possible thanks to the precise inference of their mass based on asteroseismic constraints. However, there are cases where such age estimates can be highly precise yet very inaccurate. An example is giants that have undergone mass loss or mass transfer events that have significantly altered their mass. In this context, stars with `apparent' ages significantly higher than the age of the Universe are candidates for stripped stars, or stars that have lost more mass than expected, most likely via interactions with a companion star or because of the poorly understood mass-loss mechanism along the red-giant branch. In this work we identify examples of such objects among red giants observed by Kepler, both at low ([Fe/H] {$\lessequivlnt$} -0.5) and solar metallicity. By modelling their structure and pulsation spectra, we find a consistent picture that confirms that they are indeed low-mass objects consisting of a He core of {$\approx$}0.5 M{$\odot$} and an envelope of {$\approx$}0.1 - 0.2 M{$\odot$}. Moreover, we find that these stars are characterised by a rather extreme coupling (q {$\greaterequivlnt$} 0.4) between the pressure-mode and gravity-mode cavities, one that is much higher than the typical value for red clump stars, thus providing a direct seismic signature of their peculiar structure. The complex pulsation spectra of these objects, if observed with sufficient frequency resolution, hold detailed information about the structural properties of likely products of mass stripping and can hence potentially shed light on their formation mechanism. On the other hand, our tests highlight the difficulties associated with reliably measuring the large frequency separation, especially in shorter datasets, which impacts the reliability of the inferred masses and ages of low-mass red clump stars with, for example, K2 or TESS data.},
  keywords = {asteroseismology,Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: fundamental parameters,stars: horizontal-branch,stars: interiors,stars: mass-loss},
  annotation = {ADS Bibcode: 2023A\&A...671A..53M},
  file = {/Users/lbugnet/Zotero/storage/6MSYLGMN/Matteuzzi et al. - 2023 - Red horizontal branch stars An asteroseismic pers.pdf}
}

@article{matteuzziRedHorizontalBranch2023,
  title = {Red Horizontal Branch Stars: {{An}} Asteroseismic Perspective},
  shorttitle = {Red Horizontal Branch Stars},
  author = {Matteuzzi, Massimiliano and Montalb{\'a}n, Josefina and Miglio, Andrea and Vrard, Mathieu and Casali, Giada and Stokholm, Amalie and Tailo, Marco and Ball, Warrick H. and {van Rossem}, Walter E. and Valentini, Marica},
  year = {2023},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {671},
  pages = {A53},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202245746},
  urldate = {2023-05-28},
  abstract = {Robust age estimates of red giant stars are now possible thanks to the precise inference of their mass based on asteroseismic constraints. However, there are cases where such age estimates can be highly precise yet very inaccurate. An example is giants that have undergone mass loss or mass transfer events that have significantly altered their mass. In this context, stars with `apparent' ages significantly higher than the age of the Universe are candidates for stripped stars, or stars that have lost more mass than expected, most likely via interactions with a companion star or because of the poorly understood mass-loss mechanism along the red-giant branch. In this work we identify examples of such objects among red giants observed by Kepler, both at low ([Fe/H] {$\lessequivlnt$} -0.5) and solar metallicity. By modelling their structure and pulsation spectra, we find a consistent picture that confirms that they are indeed low-mass objects consisting of a He core of {$\approx$}0.5 M{$\odot$} and an envelope of {$\approx$}0.1 - 0.2 M{$\odot$}. Moreover, we find that these stars are characterised by a rather extreme coupling (q {$\greaterequivlnt$} 0.4) between the pressure-mode and gravity-mode cavities, one that is much higher than the typical value for red clump stars, thus providing a direct seismic signature of their peculiar structure. The complex pulsation spectra of these objects, if observed with sufficient frequency resolution, hold detailed information about the structural properties of likely products of mass stripping and can hence potentially shed light on their formation mechanism. On the other hand, our tests highlight the difficulties associated with reliably measuring the large frequency separation, especially in shorter datasets, which impacts the reliability of the inferred masses and ages of low-mass red clump stars with, for example, K2 or TESS data.},
  keywords = {asteroseismology,Astrophysics - Astrophysics of Galaxies,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: fundamental parameters,stars: horizontal-branch,stars: interiors,stars: mass-loss},
  annotation = {ADS Bibcode: 2023A\&A...671A..53M},
  file = {/Users/lbugnet/Zotero/storage/LBADFW2F/Matteuzzi et al. - 2023 - Red horizontal branch stars An asteroseismic pers.pdf}
}

@article{Matthews2004,
  title = {Erratum: {{No}} Stellar p-Mode Oscillations in Space-Based Photometry of Procyon ({{Nature}} (2004) 430 (51-53))},
  author = {Matthews, Jaymie M. and Kuschnig, Rainer and Guenther, David B. and Walker, Gordon A.H. and Moffat, Anthony F.J. and Rucinski, Slavek M. and Sasselov, Dimitar and Weiss, Werner W.},
  year = {2004},
  journal = {Nature},
  volume = {430},
  number = {7002},
  pages = {921},
  issn = {00280836},
  doi = {10.1038/nature02812},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/T5Z2EWW8/Matthews et al. - 2004.pdf}
}

@article{Mattis2006,
  title = {Quantum {{Theory}} of {{Angular Momentum}}},
  author = {Mattis, Daniel C},
  year = {2006},
  journal = {The Theory of Magnetism Made Simple},
  pages = {70--103},
  doi = {10.1142/9789812774842_0003},
  abstract = {1. Vectors, Basis Vectors cartesian basis vectors (p. 4) polar basis vectors (p. 5) covariant spherical basis vectors (p. 6) contravariant spherical basis vectors (p. 6) cartesian components of vector A (p. 12) polar components of vector A (p. 12) covariant spherical ...},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZZBBUC3N/Mattis - 2006.pdf}
}

@article{Maxted2013,
  title = {Multi-Periodic Pulsations of a Stripped Red-Giant Star in an Eclipsing Binary System},
  author = {Maxted, Pierre F. L. and Serenelli, Aldo M. and Miglio, Andrea and Marsh, Thomas R. and Heber, Ulrich and Dhillon, Vikram S. and Littlefair, Stuart and Copperwheat, Chris and Smalley, Barry and Breedt, Elm{\'e} and Schaffenroth, Veronika},
  year = {2013},
  month = jun,
  journal = {Nature},
  volume = {498},
  pages = {463--465},
  issn = {0028-0836},
  doi = {10.1038/nature12192},
  urldate = {2023-10-09},
  abstract = {Low-mass white-dwarf stars are the remnants of disrupted red-giant stars in binary millisecond pulsars and other exotic binary star systems. Some low-mass white dwarfs cool rapidly, whereas others stay bright for millions of years because of stable fusion in thick surface hydrogen layers. This dichotomy is not well understood, so the potential use of low-mass white dwarfs as independent clocks with which to test the spin-down ages of pulsars or as probes of the extreme environments in which low-mass white dwarfs form cannot fully be exploited. Here we report precise mass and radius measurements for the precursor to a low-mass white dwarf. We find that only models in which this disrupted red-giant star has a thick hydrogen envelope can match the strong constraints provided by our data. Very cool low-mass white dwarfs must therefore have lost their thick hydrogen envelopes by irradiation from pulsar companions or by episodes of unstable hydrogen fusion (shell flashes). We also find that this low-mass white-dwarf precursor is a type of pulsating star not hitherto seen. The observed pulsation frequencies are sensitive to internal processes that determine whether this star will undergo shell flashes.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2013Natur.498..463M},
  file = {/Users/lbugnet/Zotero/storage/4WSH8ZXA/Maxted et al. - 2013 - Multi-periodic pulsations of a stripped red-giant .pdf}
}

@article{Maxted2014,
  title = {{{EL CVn-type}} Binaries - Discovery of 17 Helium White Dwarf Precursors in Bright Eclipsing Binary Star Systems},
  author = {Maxted, P. F. L. and Bloemen, S. and Heber, U. and Geier, S. and Wheatley, P. J. and Marsh, T. R. and Breedt, E. and Sebastian, D. and Faillace, G. and Owen, C. and Pulley, D. and Smith, D. and Kolb, U. and Haswell, C. A. and Southworth, J. and Anderson, D. R. and Smalley, B. and Collier Cameron, A. and Hebb, L. and Simpson, E. K. and West, R. G. and Bochinski, J. and Busuttil, R. and Hadigal, S.},
  year = {2014},
  month = jan,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {437},
  pages = {1681--1697},
  issn = {0035-8711},
  doi = {10.1093/mnras/stt2007},
  urldate = {2023-10-09},
  abstract = {The star 1SWASP J024743.37-251549.2 was recently discovered to be a binary star in which an A-type dwarf star eclipses the remnant of a disrupted red giant star (WASP 0247-25 B). The remnant is in a rarely observed state evolving to higher effective temperatures at nearly constant luminosity prior to becoming a very low mass white dwarf composed almost entirely of helium, i.e. it is a pre-helium white dwarf (pre-He-WD). We have used the photometric database from the Wide Angle Search for Planets (WASP) to find 17 eclipsing binary stars with orbital periods P = 0.7-2.2 d with similar light curves to 1SWASP J024743.37-251549.2. The only star in this group previously identified as a variable star is the brightest one, EL CVn, which we adopt as the prototype for this class of eclipsing binary star. The characteristic light curves of EL CVn-type stars show a total eclipse by an A-type dwarf star of a smaller, hotter star and a secondary eclipse of comparable depth to the primary eclipse. We have used new spectroscopic observations for six of these systems to confirm that the companions to the A-type stars in these binaries have very low masses (\{{$\approx$} \} 0.2\{ M\_\{{$\odot\rbrace\rbrace$}). This includes the companion to EL CVn which was not previously known to be a pre-He-WD. EL CVn-type binary star systems will enable us to study the formation of very low mass white dwarfs in great detail, particularly in those cases where the pre-He-WD star shows non-radial pulsations similar to those recently discovered in WASP0247-25 B.\vphantom{\}\}}},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: close,binaries: eclipsing,binaries: spectroscopic,stars: individual: 1SWASP J024743.37-251549.2,stars: individual: EL CVn},
  annotation = {ADS Bibcode: 2014MNRAS.437.1681M},
  file = {/Users/lbugnet/Zotero/storage/ZHLMXM2E/Maxted et al. - 2014 - EL CVn-type binaries - discovery of 17 helium whit.pdf}
}

@article{Mayor1995,
  title = {A Jupiter-Mass Companion to a Solar-Type Star},
  author = {Mayor, Michel and Queloz, Didier},
  year = {1995},
  month = nov,
  journal = {Nature},
  volume = {378},
  number = {6555},
  pages = {355--359},
  issn = {00280836},
  doi = {10.1038/378355a0},
  urldate = {2020-03-08},
  abstract = {The presence of a Jupiter-mass companion to the star 51 Pegasi is inferred from observations of periodic variations in the star's radial velocity. The companion lies only about eight million kilometres from the star, which would be well inside the orbit of Mercury in our Solar System. This object might be a gas-giant planet that has migrated to this location through orbital evolution, or from the radiative stripping of a brown dwarf. \textcopyright{} 1995 Nature Publishing Group. All rights reserved.},
  keywords = {notion,notion-database}
}

@article{Mazumdar2012,
  title = {Acoustic Glitches in Solar-Type Stars from {{Kepler}}},
  author = {Mazumdar, A. and Monteiro, M. J.P.F.G. and Ballot, J. and Antia, H. M. and Basu, S. and Houdek, G. and Mathur, S. and Cunha, M. S. and Silva Aguirre, V. and Garc{\'i}a, R. A. and Salabert, D. and Verner, G. A. and {Christensen-Dalsgaard}, J. and Metcalfe, T. S. and Chaplin, W. J.},
  year = {2012},
  journal = {Astronomische Nachrichten},
  volume = {333},
  number = {10},
  pages = {1040--1043},
  issn = {00046337},
  doi = {10.1002/asna.201211825},
  abstract = {We report the measurement of the acoustic locations of layers of sharp variation in sound speed in the interiors of 19 solar-type stars observed by the Kepler mission. The oscillatory signal in the frequencies arising due to the acoustic glitches at the base of the convection zone and the second helium ionisation zone was utilised to determine their location by four independent methods. Despite the significantly different methods of analysis, remarkable agreement was found between the results of these four methods. Further, the extracted locations of these layers were found to be consistent with representative models of the stars. \textcopyright{} 2012 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WU5FH8CB/Mazumdar et al. - 2012(2).pdf}
}

@article{Mazumdar2012a,
  title = {Seismic Detection of Acoustic Sharp Features in the {{CoRoT}} Target {{HD}} 49933},
  author = {Mazumdar, A. and Michel, E. and Antia, H. M. and Deheuvels, S.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {540},
  pages = {2--5},
  issn = {00046361},
  doi = {10.1051/0004-6361/201118495},
  abstract = {The technique of determining the acoustic location of layers of sharp changes in the sound speed inside a star from the oscillatory signal in its frequencies is applied to a solar-type star, the CoRoT target, HD 49933. We are able to determine the acoustic depth of the second helium ionisation zone of HD 49933 to be 794 -68+55 s. The acoustic depth of the base of the convective zone is found to be 1855 -412+173 s where the large error bars reflect the ambiguity in the result, which is difficult to determine with present precision on the frequencies because of the intrinsically weak nature of the signal. The positions of both these layers are consistent with those in a representative stellar model of HD 49933. \textcopyright{} 2012 ESO.},
  keywords = {notion,notion-database,stars: fundamental parameters,stars: individual: HD 49933,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/7WJHIK97/Mazumdar et al. - 2012.pdf}
}

@article{Mazumdar2014,
  title = {Measurement of Acoustic Glitches in Solar-Type Stars from Oscillation Frequencies Observed by Kepler},
  author = {Mazumdar, A. and Monteiro, M. J.P.F.G. and Ballot, J. and Antia, H. M. and Basu, S. and Houdek, G. and Mathur, S. and Cunha, M. S. and Silva Aguirre, V. and Garc{\'i}a, R. A. and Salabert, D. and Verner, G. A. and {Christensen-Dalsgaard}, J. and Metcalfe, T. S. and Sanderfer, D. T. and Seader, S. E. and Smith, J. C. and Chaplin, W. J.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {782},
  number = {1},
  eprint = {1312.4907},
  issn = {15384357},
  doi = {10.1088/0004-637X/782/1/18},
  abstract = {For the very best and brightest asteroseismic solar-type targets observed by Kepler, the frequency precision is sufficient to determine the acoustic depths of the surface convective layer and the helium ionization zone. Such sharp features inside the acoustic cavity of the star, which we call acoustic glitches, create small oscillatory deviations from the uniform spacing of frequencies in a sequence of oscillation modes with the same spherical harmonic degree. We use these oscillatory signals to determine the acoustic locations of such features in 19 solar-type stars observed by the Kepler mission. Four independent groups of researchers utilized the oscillation frequencies themselves, the second differences of the frequencies and the ratio of the small and large separation to locate the base of the convection zone and the second helium ionization zone. Despite the significantly different methods of analysis, good agreement was found between the results of these four groups, barring a few cases. These results also agree reasonably well with the locations of these layers in representative models of the stars. These results firmly establish the presence of the oscillatory signals in the asteroseismic data and the viability of several techniques to determine the location of acoustic glitches inside stars. \textcopyright{} 2014. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/7BQ8U36I/Mazumdar et al. - 2014.pdf}
}

@article{McLean2000a,
  title = {Probing the Internal Structure of Nanowires},
  author = {McLean, A. B. and Hill, I. G.},
  year = {2000},
  journal = {Applied Surface Science},
  volume = {162},
  pages = {620--624},
  issn = {01694332},
  doi = {10.1016/S0169-4332(00)00260-9},
  abstract = {Si(111)-In(4\texttimes 1) is a fascinating quasi-1D system that contains a repeated nanowire motif. The nanowires contain only two rows of In atoms. We demonstrate that it is possible to infer the spacing between the rows from a study of the dispersion of the image state band, measured using inverse photoemission. Our analysis suggest that the rows of In atoms are separated by 4{$\pm$}0.5 angstroms. This value is in excellent agreement with estimates of the spacing by both STM and surface X-ray diffraction.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4X7Q6UTL/McLean, Hill - 2000.pdf}
}

@article{McNamara2012,
  title = {The Classification of {{Kepler B-star}} Variables},
  author = {McNamara, Bernard J. and Jackiewicz, Jason and McKeever, Jean},
  year = {2012},
  journal = {Astronomical Journal},
  volume = {143},
  number = {4},
  eprint = {1202.2329},
  issn = {00046256},
  doi = {10.1088/0004-6256/143/4/101},
  abstract = {The light curves of 252 B-star candidates in the Kepler database are analyzed in a similar fashion to that done by Balona et al. to further characterize B-star variability, increase the sample of variable B stars for future study, and to identify stars whose power spectra include particularly interesting features such as frequency groupings. Stars are classified as either constant light emitters, {$\beta$}Cep stars, slowly pulsating B stars (SPBs), hybrid pulsators, binaries or stars whose light curves are dominated by rotation (Bin/Rot), hot subdwarfs, or white dwarfs. One-hundred stars in our sample were found to be either light constants or to be variable at a level of less than 0.02mmag. We increase the number of candidate B-star variables found in the Kepler database by Balona et al. in the following fashion: {$\beta$}Cep stars from 0 to 10, SPBs from eight to 54, hybrid pulsators from seven to 21, and Bin/Rot stars from 23 to 82. For comparison purposes, approximately 51 SPBs and six hybrids had been known prior to 2007. The number of {$\beta$}Cep stars known prior to 2004 was 93. A secondary result of this study is the identification of an additional 11 pulsating white dwarf candidates, four of which possess frequency groupings. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: early-type,stars: oscillations,stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/7LDUH3F4/McNamara, Jackiewicz, McKeever - 2012.pdf}
}

@article{McQuillan2012,
  title = {Statistics of Stellar Variability from {{Kepler}}},
  author = {McQuillan, A. and Aigrain, S. and Roberts, S.},
  year = {2012},
  journal = {Astronomy \& Astrophysics},
  volume = {539},
  pages = {A137},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201016148},
  abstract = {We investigate the variability properties of main sequence stars in the first month of Kepler data, using a new astrophysically robust systematics correction, and find that 60\% of stars are more variable then the active Sun. We define low and high variability samples, with a cut corresponding to twice the variability level of the active Sun, and compare the properties of the stars belonging to each sample. We show tentative evidence that the more active stars have lower proper motions and may be located closer to the galactic plane. We also investigate the frequency content of the variability, finding clear evidence for periodic or quasi-periodic behaviour in 16\% of stars, and showing that there exist significant differences in the nature of variability between spectral types. Of the periodic objects, most A and F stars have short periods ({$<$} 2 days) and highly sinusoidal variability, suggestive of pulsations, whilst G, K and M stars tend to have longer periods ({$>$} 5 days, with a trend towards longer periods at later spectral types) and show a mixture of periodic and stochastic variability, indicative of activity. Finally, we use auto-regressive models to characterise the stochastic component of the variability, and show that its typical amplitude and time-scale both increase towards later spectral types, which we interpret as a corresponding increase in the characteristic size and life-time of active regions.},
  keywords = {activity,galaxy,notion,notion-database,photometric,rotation,stars,statistics,structure,techniques},
  file = {/Users/lbugnet/Zotero/storage/4TYQAZMG/McQuillan, Aigrain, Roberts - 2012.pdf}
}

@article{McQuillan2013,
  title = {Stellar Rotation Periods of the {{Kepler}} Objects of Interest: {{A}} Dearth of Close-in Planets around Fast Rotators},
  author = {McQuillan, A. and Mazeh, T. and Aigrain, S.},
  year = {2013},
  journal = {Astrophysical Journal Letters},
  volume = {775},
  number = {1},
  eprint = {1308.1845},
  pages = {1--5},
  issn = {20418205},
  doi = {10.1088/2041-8205/775/1/L11},
  abstract = {We present a large sample of stellar rotation periods for Kepler Objects of Interest, based on three years of public Kepler data. These were measured by detecting periodic photometric modulation caused by star spots, using an algorithm based on the autocorrelation function of the light curve, developed recently by McQuillan, Aigrain \& Mazeh (2013). Of the 1919 main-sequence exoplanet hosts analyzed, robust rotation periods were detected for 737. Comparing the detected stellar periods to the orbital periods of the innermost planet in each system reveals a notable lack of close-in planets around rapid rotators. It appears that only slowly spinning stars with rotation periods longer than 5-10 days host planets on orbits shorter than 2 or 3 days, although the mechanism(s) that lead(s) to this is not clear. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {methods: observational,notion,notion-database,planets and satellites: dynamical evolution and st,planetstar interactions,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/39D72FBD/McQuillan, Mazeh, Aigrain - 2013.pdf}
}

@article{McQuillan2013a,
  title = {Measuring the Rotation Period Distribution of Field {{M}} Dwarfs with Kepler},
  author = {McQuillan, A. and Aigrain, S. and Mazeh, T.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {432},
  number = {2},
  eprint = {1303.6787},
  pages = {1203--1216},
  issn = {00358711},
  doi = {10.1093/mnras/stt536},
  abstract = {We have analysed 10 months of public data from the Kepler space mission to measure rotation periods of main-sequence stars with masses between 0.3 and 0.55M{\.o}. To derive the rotational period, we introduce the autocorrelation function and show that it is robust against phase and amplitude modulation and residual instrumental systematics. Of the 2483 stars examined, we detected rotation periods in 1570 (63.2 per cent), representing an increase of a factor of \textasciitilde 30 in the number of rotation period determination for field M dwarfs. The periods range from 0.37 to 69.7 d, with amplitudes ranging from 1.0 to 140.8 mmag.The rotation period distribution is clearly bimodal, with peaks at\textasciitilde 19 and\textasciitilde 33 d, hinting at two distinct waves of star formation, a hypothesis that is supported by the fact that slower rotators tend to have larger proper motions. The two peaks of the rotation period distribution form two distinct sequences in period- temperature space, with the period decreasing with increasing temperature, reminiscent of the Vaughan-Preston gap. The period-mass distribution of our sample shows no evidence of a transition at the fully convectiveboundary. On the other hand, the slope of the upper envelope of the period-mass relation changes sign around 0.55 M{\.o}, below which period rises with decreasing mass. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: evolution,Stars: low-mass,Stars: magnetic field,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/DEEQ3SJL/McQuillan, Aigrain, Mazeh - 2013.pdf}
}

@article{McQuillan2014,
  title = {Rotation Periods of 34,030 {{Kepler}} Main-Sequence Stars: {{The}} Full Autocorrelation Sample},
  author = {McQuillan, A. and Mazeh, T. and Aigrain, S.},
  year = {2014},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {211},
  number = {2},
  eprint = {1402.5694},
  issn = {00670049},
  doi = {10.1088/0067-0049/211/2/24},
  abstract = {We analyzed three years of data from the Kepler space mission to derive rotation periods of main-sequence stars below 6500 K. Our automated autocorrelation-based method detected rotation periods between 0.2 and 70 days for 34,030 (25.6\%) of the 133,030 main-sequence Kepler targets (excluding known eclipsing binaries and Kepler Objects of Interest), making this the largest sample of stellar rotation periods to date. In this paper we consider the detailed features of the now well-populated period-temperature distribution and demonstrate that the period bimodality, first seen by McQuillan et al. in the M-dwarf sample, persists to higher masses, becoming less visible above 0.6 M{$\odot$}. We show that these results are globally consistent with the existing ground-based rotation-period data and find that the upper envelope of the period distribution is broadly consistent with a gyrochronological age of 4.5 Gyr, based on the isochrones of Barnes, Mamajek, \& Hillenbrand and Meibom et al. We also performed a detailed comparison of our results to those of Reinhold et al. and Nielsen et al., who measured rotation periods of field stars observed by Kepler. We examined the amplitude of periodic variability for the stars with detection rotation periods, and found a typical range between 950 ppm (5th percentile) and 22,700 ppm (95th percentile), with a median of 5600 ppm. We found typically higher amplitudes for shorter periods and lower effective temperatures, with an excess of low-amplitude stars above 5400 K. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {catalogs methods,data analysis methods,low-mass stars,notion,notion-database,observational stars: activity stars,photometric,rotation techniques},
  file = {/Users/lbugnet/Zotero/storage/A32GUXTW/McQuillan, Mazeh, Aigrain - 2014.pdf}
}

@misc{Meeting843960440002,
  title = {Meeting-84396044000-2},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MAGPFAH3/meeting-84396044000-2.ics}
}

@article{meetingPLATOInstrumentPerformance2015,
  title = {{{PLATO}} : Instrument Performance {{PLATO}} : Instrument Performance},
  author = {Meeting, Stellar Science},
  year = {2015},
  number = {April},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MCJ8HLMZ/RS_TA.pdf}
}

@article{Mehrabi2017,
  title = {Magnetic {{Activity Analysis}} for a {{Sample}} of {{G-Type Main Sequence Kepler Targets}}},
  author = {Mehrabi, Ahmad and He, Han and Khosroshahi, Habib},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {834},
  number = {2},
  eprint = {1611.07262},
  pages = {207},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/834/2/207},
  abstract = {The variation of a stellar light curve owing to the rotational modulation by the magnetic features (starspots and faculae) on the star's surface can be used to investigate the magnetic properties of the host star. In this paper, we use the periodicity and magnitude of the light-curve variation, as two proxies, suggested by (He et al. 2015), to study the stellar magnetic properties for a large sample of G-type main sequence \textbackslash emph\{Kepler\} targets, for which the rotation periods recently determined by (McQuillan et al. 2014). By analyzing the correlation between the two magnetic proxies, it is found that: (1) The two proxies are positively correlated for most of the stars in our sample, and the percentages of negative, zero, and positive correlation are \$4.27\textbackslash\%\$, \$6.81\textbackslash\%\$, and \$88.91\textbackslash\%\$, respectively; (2) Negative correlation stars cannot have large magnitude of light-curve variation; (3) with the increase of rotation period, the relative number of positive correlation stars decreases and the negative correlation one increases. These results indicate that the stars with shorter rotation period tend to have positive correlation between the two proxies, and a good portion of the positive correlation stars have larger magnitude of light-curve variation (and hence more intense magnetic activities) than the negative correlation stars.},
  archiveprefix = {arxiv},
  keywords = {activity,magnetic field,notion,notion-database,rotation,solar-type,stars},
  file = {/Users/lbugnet/Zotero/storage/ITCX8EJC/Mehrabi, He, Khosroshahi - 2017.pdf}
}

@misc{Meibom2009,
  title = {Stellar {{Rotation}} in {{M35 Mass-Period Relations}}, {{Sp}}},
  author = {Meibom, S{\o}ren},
  year = {2009},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3WDJ64LU/Meibom - 2009.pdf}
}

@article{Meibom2009a,
  title = {Stellar Rotation in M35: {{Mass-period}} Relations, Spin-down Rates, and Gyrochronology},
  author = {Meibom, S{\o}ren and Mathieu, Robert D. and Stassun, Keivan G.},
  year = {2009},
  month = apr,
  journal = {Astrophysical Journal},
  volume = {695},
  number = {1},
  eprint = {0805.1040},
  pages = {679--694},
  publisher = {{Institute of Physics Publishing}},
  issn = {15384357},
  doi = {10.1088/0004-637X/695/1/679},
  abstract = {We present the results of a five month photometric time-series survey for stellar rotation over a 40 \texttimes{} 40 field centered on the 150 Myr open cluster M35. We report rotation periods for 441 stars within this field and determine their cluster membership and binarity based on a decade-long radial velocity survey, proper-motion measurements, and multiband photometric observations. We find that 310 of the stars with measured rotation periods are late-Type members of M35. The distribution of rotation periods for cluster members span more than 2 orders of magnitude from {$\sim$}0.1 to 15 days, not constrained by the sampling frequency and the timespan of the survey. With an age between the zero-Age main sequence and the Hyades, and with {$\sim$}6 times more rotation periods than measured in the Pleiades, M35 permit detailed studies of early rotational evolution of late-Type stars. Nearly 80\% of the 310 rotators lie on two distinct sequences in the color-period plane, and define clear relations between stellar rotation period and color (mass). The M35 color-period diagram enables us to determine timescales for the transition between the two rotational states, of {$\sim$}60 Myr and {$\sim$}140 Myr for G and K dwarfs, respectively. These timescales are inversely related to the mass of the convective envelope, and offer constraints on the rates of internal and external angular momentum transport and of the evolution of stellar dynamos. A comparison to the Hyades, confirm the Skumanich spin-down dependence for G dwarfs on one rotational state, but suggest that K dwarfs spin down more slowly. The locations of the rotational sequences in the M35 color-period diagram support the use of rotational isochrones to determine ages for coeval stellar populations.We use such gyrochronology to determine "gyro-Ages" for M35 from 134 Myr to 161 Myr. We use the M35 data to evaluate new color dependences for the rotational isochrones.},
  archiveprefix = {arxiv},
  keywords = {Color figures,Evolution,Extended figure,Machine-readable table,notion,notion-database,Open clusters and associations: individual (M35),Rotation online-only material,Stars,Stars: late-Type}
}

@article{Meibom2011,
  title = {The {{Kepler}} Cluster Study: {{Stellar}} Rotation in {{NGC6811}}},
  author = {Meibom, S{\o}ren and Barnes, Sydney A. and Latham, David W. and Batalha, Natalie and Borucki, William J. and Koch, David G. and Basri, Gibor and Walkowicz, Lucianne M. and Janes, Kenneth A. and Jenkins, Jon and Van Cleve, Jeffrey and Haas, Michael R. and Bryson, Stephen T. and Dupree, Andrea K. and Furesz, Gabor and Szentgyorgyi, Andrew H. and Buchhave, Lars A. and Clarke, Bruced and Twicken, Joseph D. and Quintana, Elisa V.},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {733},
  number = {1 PART 2},
  eprint = {1104.2912},
  pages = {1--14},
  issn = {20418205},
  doi = {10.1088/2041-8205/733/1/L9},
  abstract = {We present rotation periods for 71 single dwarf members of the open cluster NGC6811 determined using photometry from NASA's Kepler mission. The results are the first from The Kepler Cluster Study, which combines Kepler's photometry with ground-based spectroscopy for cluster membership and binarity. The rotation periods delineate a tight sequence in the NGC6811 color-period diagram from 1day at mid-F to 11days at early-K spectral type. This result extends to 1Gyr similar prior results in the 600Myr Hyades and Praesepe clusters, suggesting that rotation periods for cool dwarf stars delineate a well-defined surface in the three-dimensional space of color (mass), rotation, and age. It implies that reliable ages can be derived for field dwarf stars with measured colors and rotation periods, and it promises to enable further understanding of various aspects of stellar rotation and activity for cool stars. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,open clusters and associations: individual (NGC 68,stars: activity,stars: late-type,stars: rotation,starspots},
  file = {/Users/lbugnet/Zotero/storage/RRGHN3K7/Meibom et al. - 2011.pdf}
}

@article{Meibom2011a,
  title = {The Color-Period Diagram and Stellar Rotational Evolution - {{New}} Rotation Period Measurements in the Open Cluster {{M34}}},
  author = {Meibom, S{\o}ren and Mathieu, Robert D. and Stassun, Keivan G. and Liebesny, Paul and Saar, Steven H.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {733},
  number = {2},
  eprint = {1103.5171},
  issn = {15384357},
  doi = {10.1088/0004-637X/733/2/115},
  abstract = {We present the results of a 5 month photometric time-series survey for stellar rotation periods combined with a 4 year radial-velocity survey for membership and binarity in the 220Myr open cluster M34. We report surface rotation periods for 120 stars, 83 of which are kinematic and photometric late-type cluster members. A comparison to previous work serves to illustrate the importance of high-cadence long baseline photometric observations and membership information. The new M34 periods are less biased against slow rotation and cleaned for non-members. The rotation periods of the cluster members span over more than an order of magnitude from 0.5 days up to 11.5days, and trace two distinct rotational sequences - fast (C) and moderate-to-slow (I) - in the color-period diagram. The sequences represent two different states (fast and slow) in the rotational evolution of the late-type cluster members. We use the color-period diagrams for M34 and for younger and older clusters to estimate the timescale for the transition from the C to the I sequence and find {$\lessequivlnt$}150Myr, {$\sim$}150-300Myr, and 300-600Myr for G, early-mid K, and late K dwarfs, respectively. The small number of stars in the gap between C and I suggests a quick transition. We estimate a lower limit on the maximum spin-down rate (dP/dt) during this transition to be 0.06daysMyr-1 and 0.08daysMyr-1 for early and late K dwarfs, respectively. We compare the I sequence rotation periods in M34 and the Hyades for G and K dwarfs and find that K dwarfs spin down slower than the Skumanich {$\surd$}t rate. We determine a gyrochronology age of 240Myr for M34. The gyro-age has a small formal uncertainty of 2\% which reflects the tight I sequence in the M34 color-period diagram. We measure the effect of cluster age uncertainties on the gyrochronology age for M34 and find the resulting error on the gyro-age to be consistent with the 15\% error estimate for the technique in general. We use the M34 I sequence to redetermine the coefficients in the expression for rotational dependence on color used in gyrochronology. Finally, we propose that stability in the phase, shape, and amplitude of the photometric variability for the 120 rotators over the 5 month duration of our survey is due to spot generation at active stellar longitudes. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,open clusters and associations: individual (M34),stars: activity,stars: late-type,stars: rotation,starspots},
  file = {/Users/lbugnet/Zotero/storage/2J7FKTKX/Meibom et al. - 2011(2).pdf}
}

@article{Meibom2015,
  title = {A Spin-down Clock for Cool Stars from Observations of a 2.5-Billion-Year-Old Cluster},
  author = {Meibom, S{\o}ren and Barnes, Sydney A. and Platais, Imants and Gilliland, Ronald L. and Latham, David W. and Mathieu, Robert D.},
  year = {2015},
  journal = {Nature},
  volume = {517},
  number = {7536},
  pages = {589--591},
  publisher = {{Nature Publishing Group}},
  issn = {14764687},
  doi = {10.1038/nature14118},
  abstract = {The ages of the most common stars - low-mass (cool) stars like the Sun, and smaller - are difficult to derive because traditional dating methods use stellar properties that either change little as the stars age or are hard to measure. The rotation rates of all cool stars decrease substantially with time as the stars steadily lose their angular momenta. If properly calibrated, rotation therefore can act as a reliable determinant of their ages based on the method of gyrochronology. To calibrate gyrochronology, the relationship between rotation period and age must be determined for cool stars of different masses, which is best accomplished with rotation period measurements for stars in clusters with well-known ages. Hitherto, such measurements have been possible only in clusters with ages of less than about one billion years, and gyrochronology ages for older stars have been inferred from model predictions. Here we report rotation period measurements for 30 cool stars in the 2.5-billion-year-old cluster NGC 6819. The periods reveal a well-defined relationship between rotation period and stellar mass at the cluster age, suggesting that ages with a precision of order 10 per cent can be derived for large numbers of cool Galactic field stars.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VAIGXNZA/Meibom et al. - 2015.pdf}
}

@article{Mestel1937,
  title = {{{ROTATION AND STELLAR EVOLUTION}}},
  author = {Mestel, L},
  year = {1953},
  journal = {MNRAS},
  volume = {113},
  number = {713M},
  urldate = {2020-06-19},
  abstract = {Sweet's discussion (1) of rotational currents in a Cowling model star is reviewed. It is shown that the non-spherical distribution of matter set up by the currents themselves tends to choke back the motion, so that no rotationally stable star can suffer any considerable mixing between core and envelope, if the angular velocity is nearly constant throughout the star. If, however, the rotation rate increases substantially inwards, enough mixing can occur to influence seriously the evolution of the star.},
  keywords = {notion,notion-database}
}

@article{Mestel1953,
  title = {Rotation and Stellar Evolution - {{NASA}}/{{ADS}}},
  author = {Mestel, L.},
  year = {1953},
  journal = {MNRAS},
  volume = {113},
  pages = {716},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Mestel1987,
  title = {Magnetic Fields and Non-Uniform Rotation in Stellar Radiative Zones},
  author = {Mestel, L. and Weiss, 0},
  year = {1987},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {226},
  pages = {123--135},
  urldate = {2020-06-19},
  abstract = {This paper examines the effects of dynamical and resistive instabilities on magnetic redistribution of angular momentum within a star. It is tentatively concluded that if significant differential rotation survives in a stably stratified radiative zone over a stellar evolution time, then the poloidal field, cannot exceed an upper limit of order 3x 10" 2 G and is probably less than 10" 3 G. In the radiative core of the Sun B p is estimated to be at least of order 5xlO \_2 G and probably 100 G or more. Values greater than 0.1 G cannot easily be reconciled with the rotational shear inferred from frequency splitting of solar oscillations.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XZV9V4Y2/full-text.pdf}
}

@article{Mestel1988,
  title = {The Mutual Interaction of Magnetism, Rotation and Meridian Circulation in Stellar Radiative Zones},
  author = {Mestel, L. and Moss, D. and Tayler, R.J.},
  year = {1988},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {231},
  pages = {873--885},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4JZR9UH4/Mestel, Moss, Tayler - 1988.pdf}
}

@article{Mestel1990,
  title = {The Rotation of Early-Type Magnetic Stars},
  author = {Mestel, L and Tayler, J},
  year = {1990},
  journal = {OMNRAS.245. .550M Mon. Not. R. astr. Soc},
  volume = {19},
  pages = {550--558},
  abstract = {In a star with a magnetic field that is strictly symmetrical about the rotation axis, direct magnetic transport of angular momentum in a radiative envelope occurs along but not across field Unes. Significant mutual coupling of different field lines will, however, occur if there is some penetration of the field into the outer regions of the strongly viscous convective core. Some numerical examples show how an initially arbitrary rotation field can thus be converted into one of near-uniform rotation. If the field distribution is non-axisymmetric, as in the oblique rotator, non-uniform rotation generates magnetic torques which in general do interchange angular momentum between different flux tubes. Calculations for a cylindrical model with quite small dissipative coefficients illustrate how a moderately strong field will again quickly establish near-uniform rotation.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YRUUJLGS/1990MNRAS_245__550M.pdf}
}

@article{Metcalfe2003,
  title = {Stellar Structure Modeling Using a Parallel Genetic Algorithm for Objective Global Optimization},
  author = {Metcalfe, Travis S. and Charbonneau, Paul},
  year = {2003},
  journal = {Journal of Computational Physics},
  volume = {185},
  number = {1},
  pages = {176--193},
  issn = {00219991},
  doi = {10.1016/S0021-9991(02)00053-0},
  abstract = {Genetic algorithms are a class of heuristic search techniques that apply basic evolutionary operators in a computational setting. We have designed a fully parallel and distributed hardware/software implementation of the generalized optimization subroutine PIKAIA, which utilizes a genetic algorithm to provide an objective determination of the globally optimal parameters for a given model against an observational data set. We have used this modeling tool in the context of white dwarf asteroseismology, i.e., the art and science of extracting physical and structural information about these stars from observations of their oscillation frequencies. The efficient, parallel exploration of parameter-space made possible by genetic-algorithm-based numerical optimization led us to a number of interesting physical results: (1) resolution of a hitherto puzzling discrepancy between stellar evolution models and prior asteroseismic inferences of the surface helium layer mass for a DBV white dwarf; (2) precise determination of the central oxygen mass fraction in a white dwarf star; and (3) a preliminary estimate of the astrophysically important but experimentally uncertain rate for the 12C({$\alpha$}, {$\gamma$})16O nuclear reaction. These successes suggest that a broad class of computationally intensive modeling applications could also benefit from this approach. \textcopyright{} 2002 Elsevier Science B.V. All rights reserved.},
  keywords = {notion,notion-database,Optimization,Parallel computation,Stellar structure},
  file = {/Users/lbugnet/Zotero/storage/BEBAWBBI/Metcalfe, Charbonneau - 2003.pdf}
}

@article{Metcalfe2007,
  title = {Asteroseismic Signatures of Stellar Magnetic Activity Cycles},
  author = {Metcalfe, T. S. and Dziembowski, W. A. and Judge, P. G. and Snow, M.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {379},
  number = {1},
  pages = {16--20},
  issn = {17453933},
  doi = {10.1111/j.1745-3933.2007.00325.x},
  abstract = {Observations of stellar activity cycles provide an opportunity to study magnetic dynamos under many different physical conditions. Space-based asteroseismology missions will soon yield useful constraints on the interior conditions that nurture such magnetic cycles, and will be sensitive enough to detect shifts in the oscillation frequencies due to the magnetic variations. We derive a method for predicting these shifts from changes in the Mg II activity index by scaling from solar data. We demonstrate this technique on the solar-type subgiant {$\beta$} Hyi, using archival International Ultraviolet Explorer spectra and two epochs of ground-based asteroseismic observations. We find qualitative evidence of the expected frequency shifts and predict the optimal timing for future asteroseismic observations of this star. \textcopyright{} 2007 The Authors. Journal compilation \textcopyright{} 2007 RAS.},
  keywords = {notion,notion-database,Stars: activity,Stars: individual: {$\beta$} hyi,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/63NNEWPN/Metcalfe et al. - 2007.pdf}
}

@article{Metcalfe2010,
  title = {A Precise Asteroseismic Age and Radius for the Evolved Sun-like Star {{KIC}} 11026764},
  author = {Metcalfe, T. S. and Monteiro, M. J.P.F.G. and Thompson, M. J. and {Molenda-Zakowicz}, J. and Appourchaux, T. and Chaplin, W. J. and Do{\v g}an, G. and Eggenberger, P. and Bedding, T. R. and Bruntt, H. and Creevey, O. L. and Quirion, P. O. and Stello, D. and Bonanno, A. and Silva Aguirre, V. and Basu, S. and Esch, L. and Gai, N. and Di Mauro, M. P. and Kosovichev, A. G. and Kitiashvili, I. N. and Su{\'a}rez, J. C. and Moya, A. and Piau, L. and Garc{\'i}a, R. A. and Marques, J. P. and Frasca, A. and Biazzo, K. and Sousa, S. G. and Dreizler, S. and Bazot, M. and Karoff, C. and Frandsen, S. and Wilson, P. A. and Brown, T. M. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kjeldsen, H. and Campante, T. L. and Fletcher, S. T. and Handberg, R. and R{\'e}gulo, C. and Salabert, D. and Schou, J. and Verner, G. A. and Ballot, J. and Broomhall, A. M. and Elsworth, Y. and Hekker, S. and Huber, D. and Mathur, S. and New, R. and Roxburgh, I. W. and Sato, K. H. and White, T. R. and Borucki, W. J. and Koch, D. G. and Jenkins, J. M.},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {723},
  number = {2},
  eprint = {1010.4329},
  pages = {1583--1598},
  issn = {15384357},
  doi = {10.1088/0004-637X/723/2/1583},
  abstract = {The primary science goal of the Kepler Mission is to provide a census of exoplanets in the solar neighborhood, including the identification and characterization of habitable Earth-like planets. The asteroseismic capabilities of the mission are being used to determine precise radii and ages for the target stars from their solar-like oscillations. Chaplin et al. published observations of three bright G-type stars, which were monitored during the first 33.5 days of science operations. One of these stars, the subgiant KIC 11026764, exhibits a characteristic pattern of oscillation frequencies suggesting that it has evolved significantly. We have derived asteroseismic estimates of the properties of KIC 11026764 from Kepler photometry combined with ground-based spectroscopic data. We present the results of detailed modeling for this star, employing a variety of independent codes and analyses that attempt to match the asteroseismic and spectroscopic constraints simultaneously. We determine both the radius and the age of KIC 11026764 with a precision near 1\%, and an accuracy near 2\% for the radius and 15\% for the age. Continued observations of this star promise to reveal additional oscillation frequencies that will further improve the determination of its fundamental properties. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual (KIC 11026764),Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/36AHE2PM/Metcalfe et al. - 2010.pdf}
}

@article{Metcalfe2010a,
  title = {Discovery of a 1.6 Year Magnetic Activity Cycle in the Exoplanet Host Star {$\iota$} {{Horologii}}},
  author = {Metcalfe, T. S. and Basu, S. and Henry, T. J. and Soderblom, D. R. and Judge, P. G. and Kn{\"o}lker, M. and Mathur, S. and Rempel, M.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {723},
  number = {2 PART 2},
  eprint = {1009.5399},
  pages = {1--5},
  issn = {20418213},
  doi = {10.1088/2041-8205/723/2/L213},
  abstract = {The Mount Wilson Ca HK survey revealed magnetic activity variations in a large sample of solar-type stars with timescales ranging from 2.5 to 25 years. This broad range of cycle periods is thought to reflect differences in the rotational properties and the depths of the surface convection zones for stars with various masses and ages. In 2007, we initiated a long-term monitoring campaign of Ca ii H and K emission for a sample of 57 southern solar-type stars to measure their magnetic activity cycles and their rotational properties when possible. We report the discovery of a 1.6 year magnetic activity cycle in the exoplanet host star {$\iota$} Horologii and obtain an estimate of the rotation period that is consistent with Hyades membership. This is the shortest activity cycle so far measured for a solar-type star and may be related to the short-timescale magnetic variations recently identified in the Sun and HD 49933 from helioseismic and asteroseismic measurements. Future asteroseismic observations of {$\iota$} Hor can be compared to those obtained near the magnetic minimum in 2006 to search for cycle-induced shifts in the oscillation frequencies. If such short activity cycles are common in F stars, then NASA's Kepler mission should observe their effects in many of its long-term asteroseismic targets. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: chromospheres,{Stars: individual (HD 17051, HR 810)},Surveys},
  file = {/Users/lbugnet/Zotero/storage/ZDLJ8PMA/Metcalfe et al. - 2010(2).pdf}
}

@article{Metcalfe2012,
  title = {Asteroseismology of the Solar Analogs 16 {{Cyg A}} and {{B}} from {{Kepler}} Observations},
  author = {Metcalfe, T. S. and Chaplin, W. J. and Appourchaux, T. and Garc{\'i}a, R. A. and Basu, S. and Brand{\~a}o, I. and Creevey, O. L. and Deheuvels, S. and Doan, G. and Eggenberger, P. and Karoff, C. and Miglio, A. and Stello, D. and Yildiz, M. and Elik, Z. and Antia, H. M. and Benomar, O. and Howe, R. and R{\'e}gulo, C. and Salabert, D. and Stahn, T. and Bedding, T. R. and Davies, G. R. and Elsworth, Y. and Gizon, L. and Hekker, S. and Mathur, S. and Mosser, B. and Bryson, S. T. and Still, M. D. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kawaler, S. D. and Kjeldsen, H. and Ibrahim, K. A. and Klaus, T. C. and Li, J.},
  year = {2012},
  journal = {Astrophysical Journal Letters},
  volume = {748},
  number = {1},
  issn = {20418205},
  doi = {10.1088/2041-8205/748/1/L10},
  abstract = {The evolved solar-type stars 16 Cyg A and B have long been studied as solar analogs, yielding a glimpse into the future of our own Sun. The orbital period of the binary system is too long to provide meaningful dynamical constraints on the stellar properties, but asteroseismology can help because the stars are among the brightest in the Kepler field. We present an analysis of three months of nearly uninterrupted photometry of 16 Cyg A and B from the Kepler space telescope. We extract a total of 46 and 41 oscillation frequencies for the two components, respectively, including a clear detection of octupole (l = 3) modes in both stars. We derive the properties of each star independently using the Asteroseismic Modeling Portal, fitting the individual oscillation frequencies and other observational constraints simultaneously. We evaluate the systematic uncertainties from an ensemble of results generated by a variety of stellar evolution codes and fitting methods. The optimal models derived by fitting each component individually yield a common age (t = 6.8 {$\pm$} 0.4Gyr) and initial composition (Z i = 0.024 {$\pm$} 0.002, Y i = 0.25 {$\pm$} 0.01) within the uncertainties, as expected for the components of a binary system, bolstering our confidence in the reliability of asteroseismic techniques. The longer data sets that will ultimately become available will allow future studies of differential rotation, convection zone depths, and long-term changes due to stellar activity cycles. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,stars: fundamental parameters,{stars: individual (HD 186408, HD 186427)},stars: interiors,stars: oscillations,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/8BYPKSES/Metcalfe et al. - 2012.pdf}
}

@article{Metcalfe2013,
  title = {Magnetic Activity Cycles in the Exoplanet Host Star {$\epsilon$} Eridani},
  author = {Metcalfe, T. S. and Buccino, A. P. and Brown, B. P. and Mathur, S. and Soderblom, D. R. and Henry, T. J. and Mauas, P. J.D. and Petrucci, R. and Hall, J. C. and Basu, S.},
  year = {2013},
  journal = {Astrophysical Journal Letters},
  volume = {763},
  number = {2},
  eprint = {1212.4425},
  issn = {20418205},
  doi = {10.1088/2041-8205/763/2/L26},
  abstract = {The active K2 dwarf {$\epsilon$} Eri has been extensively characterized both as a young solar analog and more recently as an exoplanet host star. As one of the nearest and brightest stars in the sky, it provides an unparalleled opportunity to constrain stellar dynamo theory beyond the Sun. We confirm and document the 3-year magnetic activity cycle in {$\epsilon$} Eri originally reported by Hatzes and coworkers, and we examine the archival data from previous observations spanning 45 years. The data show coexisting 3-year and 13-year periods leading into a broad activity minimum that resembles a Maunder minimum-like state, followed by the resurgence of a coherent 3-year cycle. The nearly continuous activity record suggests the simultaneous operation of two stellar dynamos with cycle periods of 2.95 {$\pm$} 0.03 years and 12.7 {$\pm$} 0.3 years, which, by analogy with the solar case, suggests a revised identification of the dynamo mechanisms that are responsible for the so-called "active" and "inactive" sequences as proposed by B\"ohm-Vitense. Finally, based on the observed properties of {$\epsilon$} Eri, we argue that the rotational history of the Sun is what makes it an outlier in the context of magnetic cycles observed in other stars (as also suggested by its Li depletion), and that a Jovian-mass companion cannot be the universal explanation for the solar peculiarities. \textcopyright{} 2013. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: activity,stars: chromospheres,stars: individual (HD 22049),surveys},
  file = {/Users/lbugnet/Zotero/storage/PHCCW4V5/Metcalfe et al. - 2013.pdf}
}

@article{Metcalfe2014,
  title = {Properties of 42 Solar-Type {{Kepler}} Targets from the Asteroseismic Modeling Portal},
  author = {Metcalfe, T. S. and Creevey, O. L. and Do{$\Elztrnt$}an, G. and Mathur, S. and Xu, H. and Bedding, T. R. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Karoff, C. and Trampedach, R. and Benomar, O. and Brown, B. P. and Buzasi, D. L. and Campante, T. L. and {\c C}elik, Z. and Cunha, M. S. and Davies, G. R. and Deheuvels, S. and Derekas, A. and Mauro, M. P.Di and Garc{\'i}a, R. A. and Guzik, J. A. and Howe, R. and Macgregor, K. B. and Mazumdar, A. and Montalb{\'a}n, J. and Monteiro, M. J.P.F.G. and Salabert, D. and Serenelli, A. and Stello, D. and St{\k{e}}{\"s}licki, M. and Suran, M. D. and Yildiz, M. and Aksoy, C. and Elsworth, Y. and Gruberbauer, M. and Guenther, D. B. and Lebreton, Y. and Molaverdikhani, K. and Pricopi, D. and Simoniello, R. and White, T. R.},
  year = {2014},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {214},
  number = {2},
  eprint = {1402.3614},
  issn = {00670049},
  doi = {10.1088/0067-0049/214/2/27},
  abstract = {Recently the number of main-sequence and subgiant stars exhibiting solar-like oscillations that are resolved into individual mode frequencies has increased dramatically. While only a few such data sets were available for detailed modeling just a decade ago, the Kepler mission has produced suitable observations for hundreds of new targets. This rapid expansion in observational capacity has been accompanied by a shift in analysis and modeling strategies to yield uniform sets of derived stellar properties more quickly and easily. We use previously published asteroseismic and spectroscopic data sets to provide a uniform analysis of 42 solar-type Kepler targets from the Asteroseismic Modeling Portal. We find that fitting the individual frequencies typically doubles the precision of the asteroseismic radius, mass, and age compared to grid-based modeling of the global oscillation properties, and improves the precision of the radius and mass by about a factor of three over empirical scaling relations. We demonstrate the utility of the derived properties with several applications.},
  archiveprefix = {arxiv},
  keywords = {methods: numerical,notion,notion-database,stars: evolution,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/3BE48QGT/Metcalfe et al. - 2014.pdf}
}

@article{Metcalfe2016,
  title = {Stellar {{Evidence That}} the {{Solar Dynamo May Be}} in {{Transition}}},
  author = {Metcalfe, Travis S. and Egeland, Ricky and {van Saders}, Jennifer},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {826},
  number = {1},
  eprint = {1606.01926},
  pages = {L2},
  issn = {2041-8213},
  doi = {10.3847/2041-8205/826/1/l2},
  abstract = {Precise photometry from the Kepler space telescope allows not only the measurement of rotation in solar-type field stars, but also the determination of reliable masses and ages from asteroseismology. These critical data have recently provided the first opportunity to calibrate rotation-age relations for stars older than the Sun. The evolutionary picture that emerges is surprising: beyond middle-age the efficiency of magnetic braking is dramatically reduced, implying a fundamental change in angular momentum loss beyond a critical Rossby number (Ro\textasciitilde 2). We compile published chromospheric activity measurements for the sample of Kepler asteroseismic targets that were used to establish the new rotation-age relations. We use these data along with a sample of well characterized solar analogs from the Mount Wilson HK survey to develop a qualitative scenario connecting the evolution of chromospheric activity to a fundamental shift in the character of differential rotation. We conclude that the Sun may be in a transitional evolutionary phase, and that its magnetic cycle might represent a special case of stellar dynamo theory.},
  archiveprefix = {arxiv},
  keywords = {activity,evolution,magnetic field,notion,notion-database,rotation,solar-type,stars},
  file = {/Users/lbugnet/Zotero/storage/XGEXPTSP/Metcalfe, Egeland, van Saders - 2016.pdf}
}

@article{Metcalfe2017,
  title = {Magnetic {{Evolution}} and the {{Disappearance}} of {{Sun-Like Activity Cycles}}},
  author = {Metcalfe, Travis S. and {van Saders}, Jennifer},
  year = {2017},
  journal = {Solar Physics},
  volume = {292},
  number = {9},
  eprint = {1705.09668},
  pages = {1--12},
  publisher = {{Springer Science+Business Media B.V.}},
  issn = {1573093X},
  doi = {10.1007/s11207-017-1157-5},
  abstract = {After decades of effort, the solar activity cycle is exceptionally well characterized, but it remains poorly understood. Pioneering work at the Mount Wilson Observatory demonstrated that other Sun-like stars also show regular activity cycles, and suggested two possible relationships between the rotation rate and the length of the cycle. Neither of these relationships correctly describes the properties of the Sun, a peculiarity that demands explanation. Recent discoveries have started to shed light on this issue, suggesting that the Sun's rotation rate and magnetic field are currently in a transitional phase that occurs in all middle-aged stars. Motivated by these developments, we identify the manifestation of this magnetic transition in the best available data on stellar cycles. We propose a reinterpretation of previously published observations to suggest that the solar cycle may be growing longer on stellar evolutionary timescales, and that the cycle might disappear sometime in the next 0.8 \textendash{} 2.4~Gyr. Future tests of this hypothesis will come from ground-based activity monitoring of Kepler targets that span the magnetic transition, and from asteroseismology with the Transiting Exoplanet Survey Satellite (TESS) mission to determine precise masses and ages for bright stars with known cycles.},
  archiveprefix = {arxiv},
  isbn = {1120701711575},
  keywords = {{Magnetic fields, chromosphere},notion,notion-database,Rotation,{Solar cycle, observations}},
  file = {/Users/lbugnet/Zotero/storage/3CKSXVUG/Metcalfe, van Saders - 2017.pdf}
}

@misc{Meynet2018,
  title = {{{STARs}} at the {{EXtreme E R C Advanced B1}}},
  author = {Meynet, G.},
  year = {2018},
  pages = {1--13},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QWTSCYZC/Meynet - 2018.pdf}
}

@article{Michel2008,
  title = {{{CoRoT}} Measures Solar-like Oscillations and Granulation in Stars Hotter than the {{Sun}}},
  author = {Michel, Eric and Baglin, Annie and Auvergne, Michel and Catala, Claude and Samadi, Reza and Baudin, Fr{\'e}d{\'e}ric and Appourchaux, Thierry and Barban, Caroline and Weiss, Werner W. and Berthomieu, Gabrielle and Boumier, Patrick and Dupret, Marc Antoine and Garcia, Rafael A. and Fridlund, Malcolm and Garrido, Rafael and Goupil, Marie Jo and Kjeldsen, Hans and Lebreton, Yveline and Mosser, Beno{\^i}t and {Grotsch-Noels}, Arlette and {Janot-Pacheco}, Eduardo and Provost, Janine and Roxburgh, Ian W. and Thoul, Anne and Toutain, Thierry and Tiph{\`e}ne, Didier and {Turck-Chieze}, Sylvaine and Vauclair, Sylvie D. and Vauclair, G{\'e}rard P. and Aerts, Conny and Alecian, Georges and Ballot, J{\'e}r{\^o}me and Charpinet, St{\'e}phane and Hubert, Anne Marie and Ligni{\`e}res, Fran{\c c}ois and Mathias, Philippe and Monteiro, Mario J.P.F.G. and Neiner, Coralie and Poretti, Ennio and De Medeiros, Jos{\'e} Renan and Ribas, Ignasi and Rieutord, Michel L. and Cort{\'e}s, Teodoro Roca and Zwintz, Konstanze},
  year = {2008},
  month = oct,
  journal = {Science},
  volume = {322},
  number = {5901},
  pages = {558--560},
  issn = {00368075},
  doi = {10.1126/science.1163004},
  urldate = {2020-06-19},
  abstract = {Oscillations of the Sun have been used to understand its interior structure. The extension of similar studies to more distant stars has raised many difficulties despite the strong efforts of the international community over the past decades. The CoRoT (Convection Rotation and Planetary Transits) satellite, launched in December 2006, has now measured oscillations and the stellar granulation signature in three main sequence stars that are noticeably hotter than the sun. The oscillation amplitudes are about 1.5 times as large as those in the Sun; the stellar granulation is up to three times as high. The stellar amplitudes are about 25\% below the theoretic values, providing a measurement of the nonadiabaticity of the process ruling the oscillations in the outer layers of the stars.},
  keywords = {Astrophysics,notion,notion-database}
}

@article{Michel2009,
  title = {Intrinsic Photometric Characterisation of Stellar Oscillations and Granulation {{Solar}} Reference Values and {{CoRoT}} Response Functions},
  author = {Michel, E. and Samadi, R. and Baudin, F. and Barban, C. and Appourchaux, T. and Auvergne, M.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {495},
  number = {3},
  eprint = {0809.1078},
  pages = {979--987},
  issn = {00046361},
  doi = {10.1051/0004-6361:200810353},
  abstract = {Context. Measuring amplitudes of solar-like oscillations and the granulation power spectral density constitute two promising sources of information to improve our understanding and description of the convection in outer layers of stars. However, different instruments, using different techniques and different bandpasses, give measurements that cannot be directly compared to each other or to theoretical values. Aims. In this work, we define simple response functions to derive intrinsic oscillation amplitudes and granulation power densities, from photometry measurements obtained with a specific instrument on a specific star. Methods. We test this method on different photometry data sets obtained on the Sun with two different instruments in three different bandpasses. Results. We show that the results are in good agreement and we establish reference intrinsic values for the Sun with photometry. We also compute the response functions of the CoRoT instrument for a range of parameters representative of the Main Sequence solar-like pulsators to be observed with CoRoT. We show that these response functions can be conveniently described by simple analytic functions of the effective temperature of the target star. \textcopyright{} ESO 2009.},
  archiveprefix = {arxiv},
  keywords = {Convection,notion,notion-database,Stars: Oscillations,Sun: Granulation,Sun: Oscillations,Techniques: Photometric},
  file = {/Users/lbugnet/Zotero/storage/EMEKU7RE/Michel et al. - 2009.pdf}
}

@article{Michielsen2021,
  title = {Probing the Temperature Gradient in the Core Boundary Layer of Stars with Gravito-Inertial Modes. {{The}} Case of {{KIC}} 7760680},
  author = {Michielsen, M. and Aerts, C. and Bowman, D. M.},
  year = {2021},
  month = jun,
  journal = {Astronomy and Astrophysics},
  volume = {650},
  pages = {A175},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202039926},
  urldate = {2023-06-05},
  abstract = {Aims: We investigated the thermal and chemical structure in the near-core region of stars with a convective core by means of gravito-inertial modes. We determined the probing power of different asteroseismic observables and fitting methodologies. We focus on the case of the B-type star KIC 7760680, rotating at a quarter of its critical rotation velocity. Methods: We computed grids of 1D stellar structure and evolution models for two different prescriptions of the temperature gradient and mixing profile in the near-core region. We determined which of these prescriptions is preferred according to the prograde dipole modes detected in 4 yr Kepler photometry of KIC 7760680. We considered different sets of asteroseismic observables and compared the outcomes of the regression problem for a {$\chi$}2 and a Mahalanobis distance merit function, where the latter takes into account realistic uncertainties for the theoretical predictions and the former does not. Results: Period spacings of modes with consecutive radial order offer a better diagnostic than mode periods or mode frequencies for asteroseismic modelling of stars revealing only high-order gravito-inertial modes. We find KIC 7760680 to reveal a radiative temperature gradient in models with convective boundary mixing, but less complex models without such mixing are statistically preferred for this rotating star, revealing extremely low vertical envelope mixing. Conclusions: Our results strongly suggest the use of measured individual period spacing values for modes of consecutive radial order as an asteroseismic diagnostic for stellar modelling of B-type pulsators with gravito-inertial modes.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,convection,methods: statistical,stars: interiors,stars: oscillations,techniques: photometric},
  annotation = {ADS Bibcode: 2021A\&A...650A.175M},
  file = {/Users/lbugnet/Zotero/storage/CBP2PY4E/Michielsen et al. - 2021 - Probing the temperature gradient in the core bound.pdf}
}

@misc{Michielsen2023,
  title = {Probing the Physics in the Core Boundary Layers of the Double-Lined {{B-type}} Binary {{KIC4930889}} from Its Gravito-Inertial Modes},
  author = {Michielsen, Mathias and Van Reeth, Timothy and Tkachenko, Andrew and Aerts, Conny},
  year = {2023},
  month = sep,
  journal = {arXiv e-prints},
  doi = {10.48550/arXiv.2309.13123},
  urldate = {2023-10-17},
  abstract = {Stellar evolution models of B-type stars are still uncertain in terms of internal mixing properties, notably in the area between the convective core and the radiative envelope. This impacts age determination of such stars in addition to the computation of chemical yields produced at the end of their life. We investigated the thermal and chemical structure and rotation rate in the near-core boundary layer of the double-lined B-type binary KIC4930889 from its four-year Kepler light curve, ground-based spectroscopy, and Gaia astrometry. We computed grids of 1D stellar structure and evolution models for different mixing profiles and prescriptions of the temperature gradient in the near-core region. We examined the preferred prescription and the near-core rotation rate using 22 prograde dipole modes detected by Kepler photometry. We employed a Mahalanobis distance merit function and considered various nested stellar model grids, rewarding goodness of fit but penalising model complexity. Furthermore, we found a preference for either an exponentially decaying mixing profile in the near-core region or absence of additional near-core mixing, but found no preference for the temperature gradient in this region. The frequency (co)variances of our theoretical predictions are much larger than the errors on the observed frequencies. This forms the main limitation on further constraining the individual parameters of our models. Additionally, non-adiabatic pulsation computations of our best models indicate a need for opacity enhancements to accurately reproduce the observed mode excitation. The eccentric close binary system KIC4930889 proves to be a promising target to investigate additional physics in close binaries by developing new modelling methods with the capacity to include the effect of tidal interactions for full exploitation of all detected oscillation modes.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2023arXiv230913123M},
  file = {/Users/lbugnet/Zotero/storage/TT5SPGN8/Michielsen et al. - 2023 - Probing the physics in the core boundary layers of.pdf}
}

@article{Miglio2008,
  title = {Gravity Modes and Mixed Modes as Probes of Stellar Cores in Main-Sequence Stars: {{From}} Solar-like to {$\beta$} {{Cep}} Stars},
  author = {Miglio, A. and Montalb{\'a}n, J. and Eggenberger, P. and Noels, A.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  eprint = {0712.3479},
  pages = {529--534},
  issn = {00046337},
  doi = {10.1002/asna.200710991},
  abstract = {We investigate how the frequencies of gravity modes depend on the detailed properties of the chemical composition gradient that develops near the core of main-sequence stars and, therefore, on the transport processes that are able to modify the {$\mu$} profile in the central regions. We show that in main-sequence models, similarly to the case of white dwarfs, the periods of high-order gravity modes are accurately described by a uniform period spacing superposed to an oscillatory component. The periodicity and amplitude of such a component are related, respectively, to the location and sharpness of the {$\mu$} gradient. We briefly discuss and interpret, by means of this simple approximation, the effect of turbulent mixing near the core on the periods of both high-order and low-order g modes, as well as of modes of mixed pressure-gravity character. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/EKL9SNQL/Miglio et al. - 2008.pdf}
}

@article{Miglio2009,
  title = {Probing Populations of Red Giants in the Galactic Disk with {{CoRoT}}},
  author = {Miglio, A. and Montalb{\'a}n, J. and Baudin, F. and Eggenberger, P. and Noels, A. and Hekker, S. and De Ridder, J. and Weiss, W. and Baglin, A.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {503},
  number = {3},
  pages = {21--24},
  issn = {00046361},
  doi = {10.1051/0004-6361/200912822},
  abstract = {Context. The detection with CoRoT of solar-like oscillations in nearly 800 red giants in the first 150-days long observational run paves the way for detailed studies of populations of galactic-disk red giants. Aims. We investigate which information on the observed population can be recovered by the distribution of the observed seismic constraints: the frequency of maximum oscillation power ({$\nu$}max) and the large frequency separation ({$\Delta\nu$}). Methods. We propose to use the observed distribution of {$\nu$}max and of {$\Delta\nu$} as a tool for investigating the properties of galactic red-giant stars through comparison with simulated distributions based on synthetic stellar populations. Results. We can clearly identify the bulk of the red giants observed by CoRoT as red-clump stars, i.e. post-flash core-He-burning stars. The distribution of {$\nu$}max and of {$\Delta\nu$} gives us access to the distribution of the stellar radius and mass, and thus represent a most promising probe of the age and star formation rate of the disk, and of the mass-loss rate during the red-giant branch. Conclusions. CoRoT observations are supplying seismic constraints for the most populated class of He-burning stars in the galactic disk. This opens a new access gate to probing the properties of red-giant stars that, coupled with classical observations, promises to extend our knowledge of these advanced phases of stellar evolution and to add relevant constraints to models of composite stellar populations in the Galaxy. \textcopyright{} ESO 2009.},
  keywords = {Galaxy: disk,Galaxy: stellar content,notion,notion-database,Stars: fundamental parameters,Stars: horizontal-branch,Stars: mass-loss,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ICUU3DM8/Miglio et al. - 2009.pdf}
}

@article{Miglio2010,
  title = {Evidence for a Sharp Structure Variation inside a Red-Giant Star},
  author = {Miglio, A. and Montalb{\'a}n, J. and Carrier, F. and De Ridder, J. and Mosser, B. and Eggenberger, P. and Scuflaire, R. and Ventura, P. and D'Antona, F. and Noels, A. and Baglin, A.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {520},
  number = {20},
  pages = {1--4},
  issn = {00046361},
  doi = {10.1051/0004-6361/201015442},
  abstract = {Context. The availability of precisely determined frequencies of radial and non-radial oscillation modes in red giants is finally paving the way for detailed studies of the internal structure of these stars. Aims. We look for the seismic signature of regions of sharp structure variation in the internal structure of the CoRoT target HR 7349. Methods. We analyse the frequency dependence of the large frequency separation and second frequency differences, as well as the behaviour of the large frequency separation obtained with the envelope auto-correlation function. Results. We find evidence for a periodic component in the oscillation frequencies, i.e. the seismic signature of a sharp structure variation in HR 7349. In a comparison with stellar models we interpret this feature as caused by a local depression of the sound speed that occurs in the helium second-ionization region. Using solely seismic constraints this allows us to estimate the mass (M = 1.2-0.4+0.6 M{$\odot$}) and radius (R = 12.2-1.8+2.1 R{$\odot$}) of HR 7349, which agrees with the location of the star in an HR diagram. \textcopyright{} 2010 ESO.},
  keywords = {asteroseismology,notion,notion-database,stars: fundamental parameters,stars: individual: HR 7349,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/XNPD8385/Miglio et al. - 2010.pdf}
}

@article{Miglio2012,
  title = {Solar-like Pulsating Stars as Distance Indicators: {{G-K}} Giants in the {{CoRoT}} and {{Kepler}} Fields},
  author = {Miglio, A. and Morel, T. and Barbieri, M. and Mosser, B. and Girardi, L. and Montalb{\'a}n, J. and Valentini, M.},
  year = {2012},
  journal = {EPJ Web of Conferences},
  volume = {19},
  pages = {0--2},
  issn = {21016275},
  doi = {10.1051/epjconf/20121905012},
  abstract = {The detection of radial and non-radial solar-like oscillations in thousands of G-K giants with CoRoT and Kepler is paving the road for detailed studies of stellar populations in the Galaxy. The available average seismic constraints allow a precise and largely model-independent determination of stellar radii (hence distances) and masses. We here briefly report on the distance determination of thousands of giants in the CoRoT and Kepler fields of view. \textcopyright{} Owned by the authors, published by EDP Sciences, 2012.},
  isbn = {9782759807185},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TZJSQIXP/Miglio et al. - 2012.pdf}
}

@article{Miglio2012a,
  title = {Asteroseismology of Old Open Clusters with {{Kepler}}: {{Direct}} Estimate of the Integrated Red Giant Branch Mass-Loss in {{NGC}} 6791 and 6819},
  author = {Miglio, A. and Brogaard, K. and Stello, D. and Chaplin, W. J. and D'Antona, F. and Montalb{\'a}n, J. and Basu, S. and Bressan, A. and Grundahl, F. and Pinsonneault, M. and Serenelli, A. M. and Elsworth, Y. and Hekker, S. and Kallinger, T. and Mosser, B. and Ventura, P. and Bonanno, A. and Noels, A. and Silva Aguirre, V. and Szabo, R. and Li, J. and McCauliff, S. and Middour, C. K. and Kjeldsen, H.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {419},
  number = {3},
  pages = {2077--2088},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.19859.x},
  abstract = {Mass-loss of red giant branch (RGB) stars is still poorly determined, despite its crucial role in the chemical enrichment of galaxies. Thanks to the recent detection of solar-like oscillations in G-K giants in open clusters with Kepler, we can now directly determine stellar masses for a statistically significant sample of stars in the old open clusters NGC 6791 and 6819. The aim of this work is to constrain the integrated RGB mass-loss by comparing the average mass of stars in the red clump (RC) with that of stars in the low-luminosity portion of the RGB [i.e. stars with L{$\lessequivlnt$}L(RC)]. Stellar masses were determined by combining the available seismic parameters {$\nu$} max and {$\Delta\nu$} with additional photometric constraints and with independent distance estimates. We measured the masses of 40 stars on the RGB and 19 in the RC of the old metal-rich cluster NGC 6791. We find that the difference between the average mass of RGB and RC stars is small, but significant [(random) {$\pm$}0.04 (systematic) M {$\odot$}]. Interestingly, such a small does not support scenarios of an extreme mass-loss for this metal-rich cluster. If we describe the mass-loss rate with Reimers prescription, a first comparison with isochrones suggests that the observed is compatible with a mass-loss efficiency parameter in the range 0.1 {$\lessequivlnt\eta\lessequivlnt$} 0.3. Less stringent constraints on the RGB mass-loss rate are set by the analysis of the \textasciitilde 2Gyr old NGC 6819, largely due to the lower mass-loss expected for this cluster, and to the lack of an independent and accurate distance determination. In the near future, additional constraints from frequencies of individual pulsation modes and spectroscopic effective temperatures will allow further stringent tests of the {$\Delta\nu$} and {$\nu$} max scaling relations, which provide a novel, and potentially very accurate, means of determining stellar radii and masses. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {Asteroseismology,notion,notion-database,Open clusters and associations: individual: NGC 67,Open clusters and associations: individual: NGC 68,Stars: late-type,Stars: mass-loss},
  file = {/Users/lbugnet/Zotero/storage/7Z62C3UB/Miglio et al. - 2012(2).pdf}
}

@article{Miglio2013,
  title = {Differential Population Studies Using Asteroseismology: {{Solar-like}} Oscillating Giants in {{CoRoT}} Fields {{LRc01}} and {{LRa01}}},
  author = {Miglio, A. and Chiappini, C. and Morel, T. and Barbieri, M. and Chaplin, W. J. and Girardi, L. and Montalb{\'a}n, J. and Noels, A. and Valentini, M. and Mosser, B. and Baudin, F. and Casagrande, L. and Fossati, L. and Aguirre, V. Silva and Baglin, A.},
  year = {2013},
  journal = {EPJ Web of Conferences},
  volume = {43},
  pages = {1--12},
  issn = {21016275},
  doi = {10.1051/epjconf/20134303004},
  abstract = {Solar-like oscillating giants observed by the space-borne satellites CoRoT and Kepler can be used as key tracers of stellar populations in the Milky Way. When combined with additional photometric/spectroscopic constraints, the pulsation spectra of solar-like oscillating giant stars not only reveal their radii, and hence distances, but also provide well-constrained estimates of their masses, which can be used as proxies for the ages of these evolved stars. In this contribution we provide supplementary material to the comparison we presented in Miglio et al. (2013) between populations of giants observed by CoRoT in the fields designated LRc01 and LRa01. \textcopyright{} 2013 Owned by the authors, published by EDP Sciences.},
  isbn = {9782759809691},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IY5WBLUC/Miglio et al. - 2013.pdf}
}

@article{Miglio2013a,
  title = {Galactic Archaeology: {{Mapping}} and Dating Stellar Populations with Asteroseismology of Red-Giant Stars},
  author = {Miglio, A. and Chiappini, C. and Morel, T. and Barbieri, M. and Chaplin, W. J. and Girardi, L. and Montalb'an, J. and Valentini, M. and Mosser, B. and Baudin, F. and Casagrande, L. and Fossati, L. and Silva Aguirre, V. and Baglin, A.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {429},
  number = {1},
  pages = {423--428},
  issn = {00358711},
  doi = {10.1093/mnras/sts345},
  abstract = {Our understanding of howthe Galaxywas formed and evolves is severely hampered by the lack of precise constraints on basic stellar properties such as distances, masses and ages. Here, we show that solar-like pulsating red giants represent a well-populated class of accurate distance indicators, spanning a large age range, which can be used to map and date the Galactic disc in the regions probed by observations made by the CoRoT1 and Kepler space telescopes. When combined with photometric constraints, the pulsation spectra of such evolved stars not only reveal their radii, and hence distances, but also provide well-constrained estimates of their masses, which are reliable proxies for the ages of the stars. As a first application, we consider red giants observed by CoRoT in two different parts of the Milky Way, and determine precise distances for\textasciitilde 2000 stars spread across nearly 15 000 pc of the Galactic disc, exploring regions which are a long way from the solar neighbourhood.We find significant differences in the mass distributions of these two samples which, by comparison with predictions of synthetic models of the MilkyWay,we interpret as mainly due to the vertical gradient in the distribution of stellar masses (hence ages) in the disc. In the future, the availability of spectroscopic constraints for this sample of stars will not only improve the age determination, but also provide crucial constraints on age-velocity and age-metallicity relations at different Galactocentric radii and heights from the plane \textcopyright 2012 The Authors.},
  keywords = {Asteroseismology - stars: distances,Galaxy: disc.,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CVTWWCRB/Miglio et al. - 2013(2).pdf}
}

@article{Miglio2015a,
  title = {Solar-like Oscillating Stars as Standard Clocks and Rulers for Galactic Studies},
  author = {Miglio, Andrea and Girardi, L. and Rodrigues, Tha{\'i}se S. and Stello, Dennis and Chaplin, William J.},
  year = {2015},
  journal = {Astrophysics and Space Science Proceedings},
  volume = {39},
  pages = {11--22},
  issn = {15706605},
  doi = {10.1007/978-3-319-10993-0_2},
  abstract = {The CoRoT and Kepler space missions have detected oscillations in hundreds of Sun-like stars and thousands of field red-giant stars. This has opened the door to a new era of stellar population studies in the Milky Way. We report on the current status and future prospects of harvesting space-based photometric data for ensemble asteroseismology, and highlight some of the challenges that need to be faced to use these stars as accurate clocks and rulers for Galactic studies.},
  isbn = {9783319109923},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QRRFA7CU/Miglio et al. - 2015.pdf}
}

@article{Miglio2016,
  title = {Detection of Solar-like Oscillations in Relics of the {{Milky Way}}: {{Asteroseismology}} of {{K}} Giants in {{M4}} Using Data from the {{NASA K2}} Mission},
  author = {Miglio, A. and Chaplin, W. J. and Brogaard, K. and Lund, M. N. and Mosser, B. and Davies, G. R. and Handberg, R. and Milone, A. P. and Marino, A. F. and Bossini, D. and Elsworth, Y. P. and Grundah, F. and Arentoft, T. and Bedin, L. R. and Campante, T. L. and {Jessen-Hansen}, J. and Jones, C. D. and Kuszlewicz, J. S. and Malavolta, L. and Nascimbeni, V. and Sandquist, E. L.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {461},
  number = {1},
  eprint = {1606.02115},
  pages = {760--765},
  issn = {13652966},
  doi = {10.1093/mnras/stw1555},
  abstract = {Asteroseismic constraints on K giants make it possible to infer radii, masses and ages of tens of thousands of field stars. Tests against independent estimates of these properties are however scarce, especially in themetal-poor regime. Here, we report the detection of solar-like oscillations in eight stars belonging to the red-giant branch (RGB) and red-horizontal branch (RHB) of the globular cluster M4. The detections were made in photometric observations from the K2 Mission during its Campaign 2. Making use of independent constraints on the distance, we estimate masses of the eight stars by utilizing different combinations of seismic and non-seismic inputs. When introducing a correction to the {$\delta\nu$} scaling relation as suggested by stellar models, for RGB stars we find excellent agreement with the expected masses from isochrone fitting, and with a distance modulus derived using independent methods. The offset with respect to independent masses is lower, or comparable with, the uncertainties on the average RGB mass (4-10 per cent, depending on the combination of constraints used). Our results lend confidence to asteroseismic masses in the metal-poor regime. We note that a larger sample will be needed to allow more stringent tests to be made of systematic uncertainties in all the observables (both seismic and non-seismic), and to explore the properties of RHB stars, and of different populations in the cluster.},
  archiveprefix = {arxiv},
  keywords = {Globular clusters: individual: NGC 6121 (M4),notion,notion-database,Stars: low-mass,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/DFQLNMS5/Miglio et al. - 2016.pdf}
}

@article{Miglio2017,
  title = {O {{R I G I N A L A R T I C L E PLATO}} as It Is: {{A}} Legacy Mission for {{Galactic}} Archaeology},
  author = {Miglio, A and Chiappini, C and Mosser, B and Davies, G R and Freeman, K and Girardi, L and Jofr{\'e}, P and Kawata, D and Rendle, B M and Valentini, M and Casagrande, L and Chaplin, W J and Gilmore, G and Hawkins, K and Holl, B and Appourchaux, T and Belkacem, K and Bossini, D and Brogaard, K and Goupil, M.-J and Montalb{\'a}n, J and Noels, A and Anders, F and Rodrigues, T and Piotto, G and Pollacco, D and Rauer, H and Prieto, C Allende and Avelino, P P and Babusiaux, C and Barban, C and Barbuy, B and Basu, S and Baudin, F and Benomar, O and Bienaym{\'e}, O and Binney, J and {Bland-Hawthorn}, J and Bressan, A and Cacciari, C and Campante, T L and Cassisi, S and {Christensen-Dalsgaard}, J and Katz, D and Kawaler, S D and Kjeldsen, H and Kurtz, D W and Lagarde, N and Lebreton, Y and Lund, M N and Majewski, S R and Marigo, P and Martig, M and Mathur, S and Minchev, I and Morel, T and Ortolani, S and Pinsonneault, M H and Plez, B and Prada Moroni, P G and Pricopi, D and {Recio-Blanco}, A and Reyl{\'e}, C and Robin, A and Roxburgh, I W and Salaris, M and Santiago, B X and Schiavon, R and Serenelli, A and Sharma, S and Aguirre, V Silva and Soubiran, C and Steinmetz, M and Stello, D and Strassmeier, K G and Ventura, P and Ventura, R and Walton, N A and Worley, C C},
  year = {2017},
  volume = {338},
  pages = {644--661},
  doi = {10.1002/asna.201713385},
  urldate = {2020-03-08},
  keywords = {notion,notion-database}
}

@article{Miller2010,
  title = {Tipsheet - {{Improving Response Scales}}},
  author = {Miller, Patrick R.},
  year = {2010},
  journal = {DISM Survey Research Associate},
  pages = {1--7},
  doi = {10.1146/annurev.astro.41.011802.094848},
  abstract = {As important as it is to have good question wording in a survey, it is equally important to have well constructed and reliable question response options. Researchers should first consider whether open-or closed-ended questions are more appropriate to gather the desired data. Surveys typically rely more on closed-ended questions, so researchers need to be thoughtful in how they construct closed response options. This document discusses points researchers should consider when writing responses and offers tips on how to improve those scales. Open-Ended or Closed-Ended? Open-ended questions pose a question to respondents, but allow them to answer in their own words. Closed-ended questions provide respondents with pre-set answer options, and the respondent must select the most appropriate response(s) from among those listed. Open-ended questions allow respondents to provide more nuanced answers that include a great deal of detail and rationale. Researchers often find open-ended questions useful for exploratory research in which the responses serve as a guide in writing closed-ended questions for future surveys, developing hypotheses, and shedding deeper light on why certain patterns are found in closed-ended results. The disadvantage of open-ended responses is that researchers must develop a reliable method for content analyzing those responses and devote resources to the actual content analysis. This can be a time consuming process and is one of the reasons why closed-ended questions are often preferable. Closed-ended questions offer their own advantages. Analysis of these questions is often easier than for open-ended items because no content analysis is necessary. Closed-ended questions also help standardize the survey process by presenting systematic cues to respondents that are lacking in open-ended items. The main disadvantage of closed responses is that they offer the researcher little ability to get below the surface of the superficial response and uncover the thought processes that led to it. Also, elites or experts tend to find closed-ended questions frustrating. People possessing a lot of knowledge about a specialized topic often want to share more of their},
  keywords = {but now a detailed,earlier studies revealed the,helioseismology,notion,notion-database,observational pic-,s abstract helioseismology has,s rotation,s surface rotation,solar interior convection,solar interior rotation,star rotation,sun,the sun,transformed our knowledge of,turbulent convection},
  file = {/Users/lbugnet/Zotero/storage/J59GJ9H9/Miller - 2010.pdf}
}

@article{Minchev2016,
  title = {Milky {{Way}} Chemo-Dynamics in the Era of {{Gaia}}},
  author = {Minchev, I. and Chiappini, C. and Martig, M.},
  year = {2016},
  month = sep,
  journal = {Astronomische Nachrichten},
  volume = {337},
  number = {8-9},
  eprint = {1601.01313},
  pages = {944--948},
  publisher = {{Wiley-VCH Verlag}},
  issn = {15213994},
  doi = {10.1002/asna.201612404},
  urldate = {2020-03-07},
  abstract = {The main goal of Galactic Archaeology is understanding the formation and evolution of the basic Galactic components. This requires sophisticated chemo-dynamical modeling, where disc asymmetries (e.g., perturbations from the central bar, spirals arms, and infalling satellites) and non-equilibrium processes are taken into account self-consistently. Here we discuss the current status of Galactic chemo-dynamical modeling and focus on a recent hybrid technique, which helps circumvent traditional problems with chemical enrichment and star formation encountered in fully self-consistent cosmological simulations. We show that this model can account for a number of chemo-kinematic relations in the Milky Way. In addition, we demonstrate that (1) our model matches well the observed age-[{$\alpha$}/Fe] and age-[Fe/H] relations and (2) that the scatter in the age-[Fe/H] relation cannot be simply explained by blurring (stars on apo- and pericenters visiting the solar vicinity) but significant radial migration (stars born elsewhere but ending up at the solar vicinity today because of a change in guiding radius) is needed. We emphasize the importance of accurate stellar ages, such as those obtained through asteroseismology by the CoRoT and Kepler missions, for breaking the degeneracy among different Galactic evolution scenarios.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: abundances,Galaxy: disk,Galaxy: evolution,Galaxy: formation,Galaxy: kinematics and dynamics,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2VT7CI88/1601.01313.pdf}
}

@article{Mitchell2013,
  title = {How Well Can We Really Estimate the Stellar Masses of Galaxies from Broad-Band Photometry?},
  author = {Mitchell, Peter D and Lacey, Cedric G and Baugh, Carlton M and Cole, Shaun},
  year = {2013},
  journal = {MNRAS},
  volume = {435},
  pages = {87--114},
  doi = {10.1093/mnras/stt1280},
  urldate = {2020-03-08},
  abstract = {The estimated stellar masses of galaxies are widely used to characterize how the galaxy population evolves over cosmic time. If stellar masses can be estimated in a robust manner, free from any bias, global diagnostics such as the stellar mass function can be used to constrain the physics of galaxy formation. We explore how galaxy stellar masses, estimated by fitting broad-band spectral energy distributions (SEDs) with stellar population models, can be biased as a result of commonly adopted assumptions for the star formation and chemical enrichment histories, recycled fractions and dust attenuation curves of galaxies. We apply the observational technique of broad-band SED fitting to model galaxy SEDs calculated by the theoretical galaxy formation model GALFORM, isolating the effect of each of these assumptions. We find that, averaged over the entire galaxy population, the common assumption of exponentially declining star formation histories does not, by itself, adversely affect stellar mass estimation. However, we also show that this result does not hold when considering galaxies that have undergone a recent burst of star formation. We show that fixing the metallicity in SED fitting or using sparsely sampled metallicity grids can introduce mass-dependent systematics into stellar mass estimates. We find that the common assumption of a star-dust geometry corresponding to a uniform foreground dust screen can cause the stellar masses of dusty model galaxies to be significantly underestimated. Finally, we show that stellar mass functions recovered by applying SED fitting to model galaxies at high redshift can differ significantly in both shape and normalization from the intrinsic mass functions predicted by a given model. In particular, the effects of dust can reduce the normalization at the high-mass end by up to 0.6 dex in some cases. Given these differences, our methodology of using stellar masses estimated from model galaxy SEDs offers a new, self-consistent way to compare model predictions with observations. We conclude that great care should be taken when comparing theoretical galaxy formation models to observational results based on the estimated stellar masses of high-redshift galaxies.},
  keywords = {fundamental parameters-stellar content,galaxies,notion,notion-database}
}

@article{Moarefi2005,
  title = {Influence of {{Gravity Waves}} On},
  author = {Moarefi, I and Hartl, F U and Toft, D O and Lindquist, S and Sangster, T A and Lindquist, S and Leptihn, S and Osterauer, A and Haslbeck, M and Lindquist, S and Singer, M A and Lindquist, S and Anderson, J B and Kohn, L M and Marr, K A and Bowden, R A and Brown, A J and Gow, N A and Lindquist, S and Mimnaugh, E G and Costa, B De and Neckers, L M and Lindquist, S and Queitsch, C and Sirjusingh, C and Ricker, N and Ischer, F and Marchetti, O and Entenza, J and Bille, J and Heitman, J and Yahara, I and Musiyenko, A and Barik, S and Heitman, J and Diekema, D J and Lewis, R E and Osherov, N and Albert, N D and May, G S and Lindquist, S and Ko, J R and Steinbach, W J and Perfect, J R and Whitesell, L and Boehm, M F and Burrows, F J and Fairchild, K D and Shanholtz, C and Berlin, I and Lindquist, S L and Gerhart, J and Siegal, M L and Fink, G R and Kohn, L M},
  year = {2005},
  number = {September},
  pages = {2189--2192},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YGEEY745/Moarefi et al. - 2005.pdf}
}

@article{Moffat2015,
  title = {Magnetic Relaxation and the {{Taylor}} Conjecture},
  author = {Moffatt, H. K.},
  year = {2015},
  journal = {Journal of Plasma Physics},
  volume = {81},
  number = {6},
  issn = {14697807},
  doi = {10.1017/S0022377815001269},
  abstract = {A one-dimensional model of magnetic relaxation in a pressureless low-resistivity plasma is considered. The initial two-component magnetic field b(x, t) is strongly helical, with non-uniform helicity density. The magnetic pressure gradient drives a velocity field that is dissipated by viscosity. Relaxation occurs in two phases. The first is a rapid initial phase in which the magnetic energy drops sharply and the magnetic pressure becomes approximately uniform; the helicity density is redistributed during this phase but remains non-uniform, and although the total helicity remains relatively constant, a Taylor state is not established. The second phase is one of slow diffusion, in which the velocity is weak, though still driven by persistent weak non-uniformity of magnetic pressure; during this phase, magnetic energy and helicity decay slowly and at constant ratio through the combined effects of pressure equalisation and finite resistivity. The density field, initially uniform, develops rapidly (in association with the magnetic field) during the initial phase, and continues to evolve, developing sharp maxima, throughout the diffusive stage. Finally it is proved that, if the resistivity is zero, the spatial mean {$\langle$}(b {$\cdot$} {$\nabla$} \texttimes{} b)/b2{$\rangle$} is an invariant of the governing one-dimensional induction equation.},
  isbn = {0022377815001},
  keywords = {Moffat2015,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8YYD985Y/Moffatt_2015_Journal%20of%20Plasma%20Physics_Magnetic%20relaxation%20and%20the%20Taylor%20conjecture.pdf}
}

@article{Molenda-Zakowicz2011,
  title = {Characterizing {{Kepler}} Asteroseismic Targets},
  author = {{Molenda-Zakowicz}, J. and Latham, D. W. and Catanzaro, G. and Frasca, A. and Quinn, S. N.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {412},
  number = {2},
  pages = {1210--1220},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2010.17978.x},
  abstract = {Stellar structure and evolution can be studied in great detail by asteroseismic methods, provided data of high precision are available. We determine the effective temperature (Teff), surface gravity (logg), metallicity and the projected rotational velocity (vsini) of 44 Kepler asteroseismic targets using our high-resolution (R {$>$} 20000) spectroscopic observations; these parameters will then be used to compute asteroseismic models of these stars and to interpret the Kepler light curves. We use the method of cross-correlation to measure the radial velocity (RV) of our targets, while atmospheric parameters are derived using the rotfit code and spectral synthesis method. We discover three double-lined spectroscopic binaries, HIP94924, HIP95115 and HIP97321 - for the last system, we provide the orbital solution, and we report two suspected single-lined spectroscopic binaries, HIP94112 and HIP96062. For all stars from our sample we derive RV, vsini, Teff, logg and metallicity, and for six stars, we perform a detailed abundance analysis. A spectral classification is done for 33 targets. Finally, we show that the early-type star HIP94472 is rotating slowly (vsini= 13kms-1) and we confirm its classification to the Am spectral type which makes it an interesting and promising target for asteroseismic modelling. The comparison of the results reported in this paper with the information in the Kepler Input Catalogue (KIC) shows an urgent need for verification and refinement of the atmospheric parameters listed in the KIC. That refinement is crucial for making a full use of the data delivered by Kepler and can be achieved only by a detailed ground-based study. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {Binaries: spectroscopic,notion,notion-database,Space vehicles,Stars: abundances,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/LDSSFIKE/Molenda-Zakowicz et al. - 2011.pdf}
}

@article{Molenda-Zakowicz2013,
  title = {Atmospheric Parameters of 169 {{F-}}, {{G-}}, {{K-}} and {{M-type}} Stars in the {{Kepler}} Field},
  author = {{Molenda-Zakowicz}, J. and Sousa, S. G. and Frasca, A. and Uytterhoeven, K. and Briquet, M. and Van Winckel, H. and Drobek, D. and Niemczura, E. and Lampens, P. and Lykke, J. and Bloemen, S. and Gameiro, J. F. and Jean, C. and Volpi, D. and Gorlova, N. and Mortier, A. and Tsantaki, M. and Raskin, G.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {434},
  number = {2},
  eprint = {1306.6011},
  pages = {1422--1434},
  issn = {00358711},
  doi = {10.1093/mnras/stt1095},
  abstract = {The asteroseismic and planetary studies, like all research related to stars, need precise and accurate stellar atmospheric parameters as input. We aim at deriving the effective temperature (Teff), the surface gravity (log g), the metallicity ([Fe/H]), the projected rotational velocity (v sin i) and the MK type for 169 F-, G-, K- and M-type Kepler targets which were observed spectroscopically from the ground with five different instruments. We use two different spectroscopic methods to analyse 189 high-resolution, high-signal-to-noise spectra acquired for the 169 stars. For 67 stars, the spectroscopic atmospheric parameters are derived for the first time. KIC 9693187 and 11179629 are discovered to be double-lined spectroscopic binary systems. The results obtained for those stars for which independent determinations of the atmospheric parameters are available in the literature are used for a comparative analysis. As a result, we show that for solar-type stars the accuracy of present determinations of atmospheric parameters is {$\pm$}150K in Teff, {$\pm$}0.15 dex in [Fe/H] and {$\pm$}0.3 dex in log g. Finally, we confirm that the curve-of-growth analysis and the method of spectral synthesis yield systematically different atmospheric parameters when they are applied to stars hotter than 6000 K. \textcopyright 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Open clusters and associations: Individual: NGC 68,Stars: Fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/A55CIZAG/Molenda-Zakowicz et al. - 2013.pdf}
}

@article{Molnar2018,
  title = {Gaia {{Data Release}} 2: {{Validating}} the Classification of {{RR Lyrae}} and {{Cepheid}} Variables with the {{Kepler}} and {{K2}} Missions},
  author = {Moln{\'a}r, L{\'a}szl{\'o} and Plachy, Emese and Juh{\'a}sz, {\'A}ron L. and Rimoldini, Lorenzo},
  year = {2018},
  journal = {Astronomy and Astrophysics},
  volume = {620},
  eprint = {1805.11395},
  pages = {1--16},
  issn = {14320746},
  doi = {10.1051/0004-6361/201833514},
  abstract = {Context. The second data release of the Gaia mission (DR2) includes an advance catalogue of variable stars. The classifications of these stars are based on sparse photometry from the first 22 months of the mission. Aims. We set out to investigate the purity and completeness of the all-sky Gaia classification results with the help of the continuous light curves of the observed targets from the Kepler and K2 missions, focusing specifically on RR Lyrae and Cepheid pulsators, outside the Galactic bulge region. Methods. We cross-matched the Gaia identifications with the observations collected by the Kepler space telescope. We inspected the light curves visually, then calculated the relative Fourier coefficients and period ratios for the single- and double-mode K2 RR Lyrae stars to further classify them. Results. We identified 1443 and 41 stars classified as RR Lyrae or Cepheid variables in Gaia DR2 in the targeted observations of the two missions and 263 more RR Lyre targets in the full-frame images (FFI) of the original mission. We provide the cross-match of these sources. We conclude that the RR Lyrae catalogue has a completeness between 70-78\%, and provide a purity estimate of between 92 and 98\% (targeted observations) with lower limits of 75\% (FFI stars) and 51\% (K2 worst-case scenario). The low number of Cepheids prevents us from drawing detailed conclusions, but the purity of the DR2 sample is estimated to be about 66\%.},
  archiveprefix = {arxiv},
  keywords = {Cepheids,general-stars,notion,notion-database,RR Lyrae-stars,stars,Stars: variables: Cepheids,Stars: variables: general,Stars: variables: RR Lyrae,variables},
  file = {/Users/lbugnet/Zotero/storage/E3BVNUMG/Molnár et al. - 2018.pdf}
}

@article{Mombarg2019,
  title = {Asteroseismic Masses, Ages, and Core Properties of {$\gamma$} {{Doradus}} Stars Using Gravito-Inertial Dipole Modes and Spectroscopy},
  author = {Mombarg, J. S.G. and Van Reeth, T. and Pedersen, M. G. and Molenberghs, G. and Bowman, D. M. and Johnston, C. and Tkachenko, A. and Aerts, C.},
  year = {2019},
  month = feb,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {485},
  number = {3},
  eprint = {1902.06746},
  pages = {3248--3263},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stz501},
  urldate = {2020-11-29},
  abstract = {The asteroseismic modelling of period spacing patterns from gravito-inertial modes in stars with a convective core is a high-dimensional problem. We utilize the measured period spacing pattern of prograde dipole gravity modes (acquiring 0), in combination with the effective temperature (Teff) and surface gravity (log g) derived from spectroscopy, to estimate the fundamental stellar parameters and core properties of 37 {$\gamma$} Doradus (? Dor) stars whose rotation frequency has been derived from Kepler photometry. We use two 6D grids of stellar models, one with step core overshooting and another with exponential core overshooting, to evaluate correlations between the three observables 0, T eff , and log g and the mass, age, core overshooting, metallicity, initial hydrogen mass fraction, and envelope mixing. We provide multivariate linear model recipes relating the stellar parameters to be estimated to the three observables (0, T eff , log g). We estimate the (core) mass, age, core overshooting, and metallicity of {$\gamma$} Dor stars from an ensemble analysis and achieve relative uncertainties of \textasciitilde 10 per cent for the parameters. The asteroseismic age determination allows us to conclude that efficient angular momentum transport occurs already early on during the main sequence. We find that the nine stars with observed Rossby modes occur across almost the entire mainsequence phase, except close to core-hydrogen exhaustion. Future improvements of our work will come from the inclusion of more types of detected modes per star, larger samples, and modelling of individual mode frequencies.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: statistical,notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations}
}

@misc{Mombarg2023,
  title = {Calibrating Angular Momentum Transport in Intermediate-Mass Stars from Gravity-Mode Asteroseismology},
  author = {Mombarg, Joey S. G.},
  year = {2023},
  month = jun,
  journal = {arXiv e-prints},
  doi = {10.48550/arXiv.2306.17211},
  urldate = {2023-07-27},
  abstract = {The physical mechanisms driving the transport of angular momentum in stars are not fully understood, as current models cannot explain the observed stellar rotation profiles across all stages of evolution. By making use of pulsating F-type dwarfs, this work aims at (i) observationally calibrating the efficiency of angular momentum transport, assuming a constant uniform viscosity, and (ii) testing how well state-of-the-art rotating stellar models with angular momentum (AM) transport by rotationally-induced processes can explain observed rotation profiles. In both cases, the aim is to simultaneously reproduce the measured near-core rotation and core-to-surface rotation ratio. Asteroseismic modelling is applied to a sample of seven slowly rotating pulsators, to derive (core) masses and ages from their gravity-mode oscillations. This work focuses on the main sequence, using models that start with an initial uniform rotation frequency at the start of core-hydrogen burning that is a free parameter. Two treatments of AM transport are considered: (i) a constant uniform viscosity, and (ii) rotationally-induced processes. Next, the initial rotation frequency of each star is derived from the observed present-day near-core rotation frequency for both treatments. To explain the near-core rotation rate at the inferred age, initial rotation frequencies at the zero-age main sequence need to be below 10 percent of the initial critical break-up frequency. A diffusive approximation of angular momentum transport can in general explain the observed rotation profiles of the six slowly-rotating F-type dwarfs, for average values of the viscosity between 2x10\^5 and 5x10\^7 cm\^2/s or when the viscosity is computed from rotationally-induced mechanisms. Yet, for three stars in the sample, the core-to-surface rotation fraction from rotationally-induced mechanisms is predicted to be higher than observed.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2023arXiv230617211M},
  file = {/Users/lbugnet/Zotero/storage/4AIILLX6/Mombarg - 2023 - Calibrating angular momentum transport in intermed.pdf}
}

@article{Mombarg2023a,
  title = {Calibrating Angular Momentum Transport in Intermediate-Mass Stars from Gravity-Mode Asteroseismology},
  author = {Mombarg, J. S. G.},
  year = {2023},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {677},
  pages = {A63},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202345956},
  urldate = {2023-09-28},
  abstract = {Context. The physical mechanisms driving the transport of angular momentum in stars are not fully understood, as current models cannot explain the observed stellar rotation profiles across all stages of evolution. Aims: By making use of pulsating F-type dwarfs, we aim to (i) observationally calibrate the efficiency of angular momentum transport, assuming a constant uniform viscosity, and (ii) test how well state-of-the-art rotating stellar models with angular momentum (AM) transport by rotationally induced processes can explain observed rotation profiles. In both cases, the aim is to simultaneously reproduce the measured near-core rotation and core-to-surface rotation ratio. Methods: Asteroseismic modelling is applied to a sample of seven slowly rotating pulsators in order to derive (core) masses and ages from their gravity-mode oscillations. This work focuses on the main sequence (MS), using models that start with an initial uniform rotation frequency at the start of core-hydrogen burning, which is a free parameter. Two treatments of AM transport are considered: (i) a constant uniform viscosity, and (ii) rotationally induced processes (including the Spruit-Tayler dynamo). Next, the initial rotation frequency of each star is derived from the observed present-day near-core rotation frequency for both treatments. Results: Asteroseismic modelling of gravity mode periods reveals that all seven slowly rotating stars (one of which is not further modelled) in the sample are near the end of core-hydrogen burning. To explain the near-core rotation rate at the inferred age, initial rotation frequencies at the zero-age main sequence need to be below 10\% of the initial critical break-up frequency. The derived initial rotation frequencies are consistent with previous works. Conclusions: A diffusive approximation of angular momentum transport can in general explain the observed rotation profiles of the six slowly rotating F-type dwarfs for average values of the viscosity of between 2 \texttimes{} 105 and 5 \texttimes{} 107 cm2 s-1 or when the viscosity is computed from rotationally induced mechanisms. Yet, for three stars in the sample, the core-to-surface rotation fraction from rotationally induced mechanisms is predicted to be higher than observed.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2023A\&A...677A..63M},
  file = {/Users/lbugnet/Zotero/storage/5ZJ7454I/Mombarg - 2023 - Calibrating angular momentum transport in intermed.pdf}
}

@article{Mombarg2023b,
  title = {Calibrating Angular Momentum Transport in Intermediate-Mass Stars from Gravity-Mode Asteroseismology},
  author = {Mombarg, J. S. G.},
  year = {2023},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {677},
  pages = {A63},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202345956},
  urldate = {2023-10-25},
  abstract = {Context. The physical mechanisms driving the transport of angular momentum in stars are not fully understood, as current models cannot explain the observed stellar rotation profiles across all stages of evolution. Aims: By making use of pulsating F-type dwarfs, we aim to (i) observationally calibrate the efficiency of angular momentum transport, assuming a constant uniform viscosity, and (ii) test how well state-of-the-art rotating stellar models with angular momentum (AM) transport by rotationally induced processes can explain observed rotation profiles. In both cases, the aim is to simultaneously reproduce the measured near-core rotation and core-to-surface rotation ratio. Methods: Asteroseismic modelling is applied to a sample of seven slowly rotating pulsators in order to derive (core) masses and ages from their gravity-mode oscillations. This work focuses on the main sequence (MS), using models that start with an initial uniform rotation frequency at the start of core-hydrogen burning, which is a free parameter. Two treatments of AM transport are considered: (i) a constant uniform viscosity, and (ii) rotationally induced processes (including the Spruit-Tayler dynamo). Next, the initial rotation frequency of each star is derived from the observed present-day near-core rotation frequency for both treatments. Results: Asteroseismic modelling of gravity mode periods reveals that all seven slowly rotating stars (one of which is not further modelled) in the sample are near the end of core-hydrogen burning. To explain the near-core rotation rate at the inferred age, initial rotation frequencies at the zero-age main sequence need to be below 10\% of the initial critical break-up frequency. The derived initial rotation frequencies are consistent with previous works. Conclusions: A diffusive approximation of angular momentum transport can in general explain the observed rotation profiles of the six slowly rotating F-type dwarfs for average values of the viscosity of between 2 \texttimes{} 105 and 5 \texttimes{} 107 cm2 s-1 or when the viscosity is computed from rotationally induced mechanisms. Yet, for three stars in the sample, the core-to-surface rotation fraction from rotationally induced mechanisms is predicted to be higher than observed.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2023A\&A...677A..63M},
  file = {/Users/lbugnet/Zotero/storage/4VUSDX5B/Mombarg - 2023 - Calibrating angular momentum transport in intermed.pdf}
}

@article{Montalban2010a,
  title = {Seismic Diagnostics of Red Giants: {{First}} Comparison with Stellar Models},
  author = {Montalb{\'a}n, J. and Miglio, A. and Noels, A. and Scuflaire, R. and Ventura, P.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {721},
  number = {2 PART 2},
  eprint = {1009.1754},
  pages = {1--14},
  issn = {20418213},
  doi = {10.1088/2041-8205/721/2/L182},
  abstract = {The clear detection with CoRoT and KEPLER of radial and non -radial solar-like oscillations in many red giants paves the way for seismic inferences on the structure of such stars. We present an overview of the properties of the adiabatic frequencies and frequency separations of radial and non-radial oscillation modes for an extended grid of models.We highlight how their detection allows a deeper insight into the internal structure and evolutionary state of red giants. In particular, we find that the properties of dipole modes constitute a promising seismic diagnostic tool of the evolutionary state of red giant stars.We compare our theoretical predictions with the first 34 days of KEPLER data and predict the frequency diagram expected for red giants in the CoRoT exofield in the galactic center direction. \textcopyright 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/26CIVINM/Montalbán et al. - 2010.pdf}
}

@article{Montalban2012a,
  title = {Red {{Giants}} as {{Probes}} of the {{Structure}} and {{Evolution}} of the {{Milky Way}}},
  author = {Montalban, Josefina and Miglio, Andrea and Noels, Arlette and Scuflaire, R and Ventura, Paolo and D'Antona, Francesca},
  year = {2012},
  journal = {Red Giants as Probes of the Structure and Evolution of the Milky Way, Astrophysics and Space Science Proceedings, ISBN 978-3-642-18417-8. Springer-Verlag Berlin Heidelberg, 2012, p. 23},
  eprint = {1108.4554},
  pages = {11--22},
  doi = {10.1007/978-3-642-18418-5},
  abstract = {Since the detection of non-radial solar-like oscillation modes in red giants with the CoRoT satellite, the interest in the asteroseismic properties of red giants and the link with their global properties and internal structure is substantially increasing. Moreover, more and more precise data are being collected with the space-based telescopes CoRoT and Kepler. In this paper we present a survey of the most relevant theoretical and observational results obtained up to now concerning the potential of solar-like oscillations in red giants.},
  archiveprefix = {arxiv},
  isbn = {978-3-642-18417-8},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/DAFA4QP3/Montalban et al. - 2012.pdf}
}

@article{Montalban2013a,
  title = {Testing Convective-Core Overshooting Using Period Spacings of Dipole Modes in Red Giants},
  author = {Montalb{\'a}n, J. and Miglio, A. and Noels, A. and Dupret, M. A. and Scuflaire, R. and Ventura, P.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {766},
  number = {2},
  eprint = {1302.3173},
  pages = {0--6},
  issn = {15384357},
  doi = {10.1088/0004-637X/766/2/118},
  abstract = {Uncertainties on central mixing in main-sequence (MS) and core He-burning (He-B) phases affect key predictions of stellar evolution such as late evolutionary phases, chemical enrichment, ages, etc. We propose a test of the extension of extra-mixing in two relevant evolutionary phases based on period spacing ({$\Delta$}P) of solar-like oscillating giants. From stellar models and their corresponding adiabatic frequencies (respectively, computed with ATON and LOSC codes), we provide the first predictions of the observable {$\Delta$}P for stars in the red giant branch and in the red clump (RC). We find (1) a clear correlation between {$\Delta$}P and the mass of the helium core (M He); the latter in intermediate-mass stars depends on the MS overshooting, and hence it can be used to set constraints on extra-mixing during MS when coupled with chemical composition; and (2) a linear dependence of the average value of the asymptotic period spacing ({$\langle\Delta$}P{$\rangle$}a ) on the size of the convective core during the He-B phase. A first comparison with the inferred asymptotic period spacing for Kepler RC stars also suggests the need for extra-mixing during this phase, as evinced from other observational facts. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,convection,notion,notion-database,stars: evolution,stars: late-type,stars: low-mass},
  file = {/Users/lbugnet/Zotero/storage/7WCMXBEP/Montalbán et al. - 2013.pdf}
}

@inproceedings{Monteiro1996,
  title = {Detecting Convective Overshoot in Solar-Type Stars},
  booktitle = {Inside the Stars, {{IAU Colloquium}}. {{ASP Conference Series}}, {{Vol}}.40},
  author = {Monteiro, M{\'a}rio J.P.F.G. and Christensen-Dalsgaard, J{\o}rgen and Thompson, Michael J.},
  year = {1996},
  urldate = {2020-03-08},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ACCDMDZS/Monteiro, Christensen‐Dalsgaard, Thompson - 1996.pdf}
}

@article{Montes1998a,
  title = {Multiwavelength Optical Observations of Chromospherically Active Binary Systems},
  author = {Montes, D. and {Sanz-Forcada}, J. and {Fern{\'a}ndez-Figueroa}, M. J. and De Castro, E. and Cornide, M. and Ramsey, L. W.},
  year = {1998},
  journal = {Astrophysics and Space Science},
  volume = {263},
  number = {1-4},
  pages = {279--282},
  issn = {0004640X},
  doi = {10.1051/aas:1997374},
  abstract = {We summarize here our ongoing project of multiwavelength optical observations aimed at studying the chromosphere of active binary systems, using the information provided for several optical spectroscopic features, that are formed at different heights in the chromosphere.},
  keywords = {activity,binaries,chromospheres,close,notion,notion-database,spectroscopic,stars},
  file = {/Users/lbugnet/Zotero/storage/3VEXLLHK/Montes et al. - 1998.pdf}
}

@article{Montgomery1989,
  title = {{{MHD}} Turbulance: Relaxation Processes and Variational Principles},
  author = {Montgomery, David and Phillips, Lee},
  year = {1989},
  journal = {Physica D: Nonlinear Phenomena},
  volume = {37},
  number = {1-3},
  pages = {215--226},
  issn = {01672789},
  doi = {10.1016/0167-2789(89)90131-0},
  urldate = {2020-07-02},
  abstract = {Turbulent relaxation processes seem to play a more prominent role in magnetohydrodynamics (MHD) than in hydrodynamics and exhibit a wider variety of behavior. In decaying turbulence, "relaxed" states can result from highly unequal decay rates of extensive, cascadable ideal invariants such as energy, magnetic helicity, cross helicity, etc. In externally-driven MHD systems, the relaxed states may result from other processes, less well understood. We are exploring a formulation based on a principle of the minimum rate of energy dissipation. This is a nineteenth century principle from which seems to descend the more modern (and less well accepted) principle of "the minimum rate of entropy production". Consequences of the conjectured principle are described for two cases: (1) for the reversed-field pinch (RFP), an externally-applied electric field supplies magnetic helicity at a constant rate; (2) for the case of a constant rate of dissipation of cross-helicity, a relaxed state with aligned vorticity and current densities is predicted. The former problem models the steady-state operation of a familiar fusion confinement device. The latter models certain features of solar wind turbulance, regarded as a driven, steady-state system. \textcopyright{} 1989.},
  keywords = {notion,notion-database}
}

@article{Montgomery1998,
  title = {Evidence of Plasma Fluctuations and Their Effect on the Growth of Stimulated {{Brillouin}} and Stimulated {{Raman}} Scattering in Laser Plasmas},
  author = {Montgomery, D. S. and Afeyan, B. B. and Cobble, J. A. and Fern{\'a}ndez, J. C. and Wilke, M. D. and Glenzer, S. H. and Kirkwood, R. K. and MacGowan, B. J. and Moody, J. D. and Lindman, E. L. and Munro, D. H. and Wilde, B. H. and Rose, H. A. and Dubois, D. F. and Bezzerides, B. and Vu, H. X.},
  year = {1998},
  month = may,
  journal = {Physics of Plasmas},
  volume = {5},
  number = {5},
  pages = {1973--1980},
  publisher = {{AIP Publishing}},
  issn = {1070-664X},
  doi = {10.1063/1.872868},
  urldate = {2020-07-02},
  abstract = {The reflectivity levels of stimulated Brillouin scattering (SBS) in recent large scale length laser plasma experiments is much lower than expected for conditions where the convective gain exponent is expected to be large [J. C. Fern\'andez et al., Phys. Plasmas 4, 1849 (1997)]. Long-wavelength velocity fluctuations caused during the plasma formation process, or by parametric instabilities themselves, have been proposed as a mechanism to detune SBS in these experiments and reduce its gain [W. L. Kruer et al., Phys. Plasmas 3, 382 (1996); H. A. Rose, Phys. Plasmas 4, 437 (1997)] . Evidence of large-velocity fluctuation levels is found in the time-resolved SBS spectra from these experiments, and correlates with observed changes in the reflectivity of both SBS and stimulated Raman scattering (SRS). Evidence of fluctuations that increase with increasing plasma density is presented, and their effect on the growth of parametric instabilities is discussed. \textcopyright{} 1998 American Institute of Physics.},
  keywords = {52.25.Gj,52.35.Nx,52.35.Py,52.50.Jm,Fluctuation and chaos phenomena,Macroinstabilities,notion,notion-database,Plasma production and heating by laser beams}
}

@book{Moore2014,
  title = {{{MESA Summer School}} - 2014},
  author = {Moore, Kevin},
  year = {2014},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GQ58QXQJ/Moore - 2014.pdf}
}

@article{Moradi2010,
  title = {Modeling the {{Subsurface Structure}} of {{Sunspots}}},
  author = {Moradi, H. and Baldner, C. and Birch, A. C. and Braun, D. C. and Cameron, R. H. and Duvall, T. L. and Gizon, L. and Haber, D. and Hanasoge, S. M. and Hindman, B. W. and Jackiewicz, J. and Khomenko, E. and Komm, R. and Rajaguru, P. and Rempel, M. and Roth, M. and Schlichenmaier, R. and Schunker, H. and Spruit, H. C. and Strassmeier, K. G. and Thompson, M. J. and Zharkov, S.},
  year = {2010},
  journal = {Solar Physics},
  volume = {267},
  number = {1},
  eprint = {0912.4982},
  pages = {1--62},
  issn = {00380938},
  doi = {10.1007/s11207-010-9630-4},
  abstract = {While sunspots are easily observed at the solar surface, determining their subsurface structure is not trivial. There are two main hypotheses for the subsurface structure of sunspots: the monolithic model and the cluster model. Local helioseismology is the only means by which we can investigate subphotospheric structure. However, as current linear inversion techniques do not yet allow helioseismology to probe the internal structure with sufficient confidence to distinguish between the monolith and cluster models, the development of physically realistic sunspot models are a priority for helioseismologists. This is because they are not only important indicators of the variety of physical effects that may influence helioseismic inferences in active regions, but they also enable detailed assessments of the validity of helioseismic interpretations through numerical forward modeling. In this article, we provide a critical review of the existing sunspot models and an overview of numerical methods employed to model wave propagation through model sunspots. We then carry out a helioseismic analysis of the sunspot in Active Region 9787 and address the serious inconsistencies uncovered by Gizon et al. (2009a, 2009b). We find that this sunspot is most probably associated with a shallow, positive wave-speed perturbation (unlike the traditional two-layer model) and that travel-time measurements are consistent with a horizontal outflow in the surrounding moat. \textcopyright{} 2010 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/EDP6FCZI/Moradi et al. - 2010.pdf}
}

@article{Moravveji2016,
  title = {Sub-Inertial {{Gravity Modes}} in the {{B8V Star KIC}} 7760680 {{Reveal Moderate Core Overshooting}} and {{Low Vertical Diffusive Mixing}}},
  author = {Moravveji, Ehsan and Townsend, Richard H. D. and Aerts, Conny and Mathis, St{\'e}phane},
  year = {2016},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {823},
  pages = {130},
  issn = {0004-637X},
  doi = {10.3847/0004-637X/823/2/130},
  urldate = {2023-10-15},
  abstract = {Thus far, KIC 7760680 is the richest slowly pulsating B star, exhibiting 36 consecutive dipole ({$\mathscr{l}$} = 1) gravity (g-) modes. The monotonically decreasing period spacing of the series, in addition to the local dips in the pattern, confirm that KIC 7760680 is a moderate rotator with clear mode trapping in chemically inhomogeneous layers. We employ the traditional approximation of rotation to incorporate rotational effects on g-mode frequencies. Our detailed forward asteroseismic modeling of this g-mode series reveals that KIC 7760680 is a moderately rotating B star with mass {$\sim$}3.25 M {$\odot$}. By simultaneously matching the slope of the period spacing and the number of modes in the observed frequency range, we deduce that the equatorial rotation frequency of KIC 7760680 is 0.4805 day-1, which is 26\% of its Roche break up frequency. The relative deviation of the model frequencies and those observed is less than 1\%. We succeed in tightly constraining the exponentially decaying convective core overshooting parameter to f ov {$\approx$} 0.024 {$\pm$} 0.001. This means that convective core overshooting can coexist with moderate rotation. Moreover, models with exponentially decaying overshoot from the core outperform those with the classical step-function overshoot. The best value for extra diffusive mixing in the radiatively stable envelope is confined to \{log\}\{D\}\{\{ext\}\}{$\approx$} 0.75+/- 0.25 (with D ext in cm2 s-1), which is notably smaller than theoretical predictions.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,diffusion,stars: individual: KIC 7760680,stars: interiors,stars: rotation,waves},
  annotation = {ADS Bibcode: 2016ApJ...823..130M},
  file = {/Users/lbugnet/Zotero/storage/6SYV9MBM/Moravveji et al. - 2016 - Sub-inertial Gravity Modes in the B8V Star KIC 776.pdf}
}

@article{Morel2008a,
  title = {{{CESAM}}: {{A}} Free Code for Stellar Evolution Calculations},
  author = {Morel, P. and Lebreton, Y.},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  eprint = {0801.2019},
  pages = {61--73},
  issn = {0004640X},
  doi = {10.1007/s10509-007-9663-9},
  abstract = {The cesam code is a consistent set of programs and routines which perform calculations of 1D quasi-hydrostatic stellar evolution including microscopic diffusion of chemical species and diffusion of angular momentum. The solution of the quasi-static equilibrium is performed by a collocation method based on piecewise polynomials approximations projected on a B-spline basis; that allows stable and robust calculations, and the exact restitution of the solution, not only at grid points, even for the discontinuous variables. Other advantages are the monitoring by only one parameter of the accuracy and its improvement by super-convergence. An automatic mesh refinement has been designed for adjusting the localisations of grid points according to the changes of unknowns. For standard models, the evolution of the chemical composition is solved by stiffly stable schemes of orders up to four; in the convection zones mixing and evolution of chemical are simultaneous. The solution of the diffusion equation employs the Galerkin finite elements scheme; the mixing of chemicals is then performed by a strong turbulent diffusion. A precise restoration of the atmosphere is allowed for. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {Methods: numerical,notion,notion-database,Stars: evolution,Stars: interior,Sun: evolution,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/84VYC8EC/Morel, Lebreton - 2008.pdf}
}

@article{Morel2012,
  title = {Assessing the Accuracy of the Surface Gravity Determination in Late-Type Stars with Solar-like Pulsators},
  author = {Morel, Thierry and Miglio, Andrea},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {419},
  number = {1},
  pages = {34--38},
  issn = {17453933},
  doi = {10.1111/j.1745-3933.2011.01172.x},
  abstract = {The frequency of maximum oscillation power measured in dwarfs and giants exhibiting solar-like pulsations provides a precise, and potentially accurate, inference of the stellar surface gravity. An extensive comparison for about 40 well-studied pulsating stars with gravities derived using classical methods (ionization balance, pressure-sensitive spectral features or location with respect to evolutionary tracks) supports the validity of this technique and reveals an overall remarkable agreement with mean differences not exceeding 0.05dex (although with a dispersion of up to {$\sim$}0.2dex). It is argued that interpolation in theoretical isochrones may be the most precise way of estimating the gravity by traditional means in nearby dwarfs. Attention is drawn to the usefulness of seismic targets as benchmarks in the context of large-scale surveys. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {Asteroseismology,notion,notion-database,Stars: fundamental parameters,Stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/A4TITYEN/Morel, Miglio - 2012.pdf}
}

@techreport{Morel2014,
  title = {The {{B Fields}} in {{OB Stars}} ({{BOB}}) {{Survey}}},
  author = {Morel, T. and Castro, N. and Fossati, L. and Hubrig, S. and Langer, N. and Przybilla, N. and Sch{\"o}ller, M. and Carroll, T. and Ilyin, I. and Irrgang, A. and Oskinova, L. and Schneider, F. R. N. and D{\'i}az, S. S. and Briquet, M. and Gonz{\'a}lez, J. F. and Kharchenko, N. and Nieva, M. -F. and Scholz, R. -D. and {de Koter}, A. and Hamann, W. -R. and Herrero, A. and Ma{\'i}z Apell{\'a}niz, J. and Sana, H. and Arlt, R. and Barb{\'a}, R. and Dufton, P. and Kholtygin, A. and Mathys, G. and Piskunov, A. and Reisenegger, A. and Spruit, H. and Yoon, S. -C.},
  year = {2014},
  journal = {Msngr},
  volume = {157},
  pages = {27--31},
  issn = {0722-6691},
  urldate = {2020-07-13},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3BKST25L/full-text.pdf}
}

@article{Moreno-Insertis2000a,
  title = {Distribution of Magnetic Flux on the Solar Surface and Low-Degree p-Modes},
  author = {{Moreno-Insertis}, F. and Solanki, S. K.},
  year = {2000},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {313},
  number = {2},
  pages = {411--422},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2000.03246.x},
  abstract = {The frequencies of solar p-modes are known to change over the solar cycle. There is also recent evidence that the relation between frequency shift of low-degree modes and magnetic flux or other activity indicators differs between the rising and falling phases of the solar cycle leading to a hysteresis in such diagrams. We consider the influence of the changing large-scale surface distribution of the magnetic flux on low-degree (l {$\leq$} 3) p-mode frequencies To that end, we use time-dependent models of the magnetic flux distribution and study the ensuing frequency shifts of modes with different order and degree as a function of time. The resulting curves are periodic functions (in simple cases just sine curves) shifted in time by different amounts for the different modes. We show how this may easily lead to hysteresis cycles comparable to those observed. Our models suggest that high-latitude fields are necessary to produce a significant difference in hysteresis between odd- and even-degree modes. Only magnetic field distributions within a small parameter range are consistent with the observations by Jim\'enez-Reyes et al. Observations of p-mode frequency shifts are therefore capable of providing an additional diagnostic of the magnetic field near the solar poles. The magnetic distribution that is consistent with the p-mode observations also appears reasonable compared with direct measurements of the magnetic field.},
  keywords = {notion,notion-database,Sun: activity,Sun: magnetic fields,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/JUBFU5MB/Moreno-Insertis, Solanki - 2000.pdf}
}

@article{Morgenthaler2011,
  title = {Direct Observation of Magnetic Cycles in {{Sun-like}} Stars},
  author = {Morgenthaler, A. and Petit, P. and Morin, J. and Auri{\`e}re, M. and Dintrans, B. and {Konstantinova-Antova}, R. and Marsden, S.},
  year = {2011},
  journal = {Astronomische Nachrichten},
  volume = {332},
  number = {9-10},
  pages = {866--871},
  issn = {00046337},
  doi = {10.1002/asna.201111592},
  abstract = {A sample of 19 solar-type stars, probing masses between 0.6 and 1.4 solar masses and rotation periods between 3.4 and 43 days, was regularly observed using the NARVAL spectropolarimeter at Telescope Bernard Lyot (Pic du Midi, France) between 2007 and 2011. The Zeeman-Doppler Imaging technique is employed to reconstruct the large-scale photospheric magnetic field structure of the targets and investigate its long-term temporal evolution. We present here the first results of this project with the observation of short magnetic cycles in several stars, showing up a succession of polarity reversals over the timespan of our monitoring. Preliminary trends suggest that short cycles are more frequent for stellar periods below a dozen days and for stellar masses above about one solar mass. The cycles lengths unveiled by the direct tracking of polarity switches are significantly shorter than those derived from previous studies based on chromospheric activity monitoring, suggesting the coexistence of several magnetic timescales in a same star. \textcopyright{} 2011 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {notion,notion-database,Stars: activity,Stars: magnetic fields,Stars: rotation,Techniques: polarimetric},
  file = {/Users/lbugnet/Zotero/storage/87E38SMG/Morgenthaler et al. - 2011.pdf}
}

@article{Morrow1988,
  title = {Angular Momentum Transport and Dynamo Action in the {{Sun}}: A Report on Implications of a Recent Heliospheric Estimate of Solar Rotation.},
  author = {Morrow, C. A. and Gilman, P. A. and Deluca, E. E.},
  year = {1988},
  journal = {ESASP},
  volume = {286},
  pages = {109--115},
  issn = {1609-042X},
  urldate = {2020-07-02},
  keywords = {Angular Momentum,Angular Momentum: Solar Rotation,Dynamo Theory,Helioseismology,Legendre Functions,Momentum Transfer,notion,notion-database,Solar Interior,Solar Physics,Solar Rotation,Sun: Dynamo Theory,Sunspots,Turbulence Effects}
}

@article{Morsink2002,
  title = {Normal {{Modes}} of {{Rotating Magnetic Stars}}},
  author = {Morsink, S. M. and Rezania, V.},
  year = {2002},
  journal = {The Astrophysical Journal},
  volume = {574},
  number = {2},
  pages = {908--919},
  issn = {0004-637X},
  doi = {10.1086/341190},
  abstract = {We investigate the effect of a magnetic field on the global oscillation modes of a rotating fluid star in the magnetohydrodynamic approximation. We present general equations for the modification of any type of fluid mode due to a general magnetic field that is not aligned with the star's spin axis. In the case of any internal dipole magnetic field, we derive the equations for the frequency corrections to the r-modes. We solve for the frequency correction explicitly for the case when the internal dipole field is force-free, including the uniform density case. In the weak-field limit, the spatial form of the r-mode velocity perturbation is unchanged, but the magnitude of the frequency in the rotating frame increases.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FTKB7LUJ/Morsink, Rezania - 2002.pdf}
}

@article{Mortier2014,
  title = {Astrophysics {{Correcting}} the Spectroscopic Surface Gravity Using Transits and Asteroseismology {{No}} Significant Effect on Temperatures or Metallicities with {{ARES}} and {{MOOG}} in Local Thermodynamic Equilibrium},
  author = {Mortier, A and Sousa, S G and Zh Adibekyan, V and Brand{\~a}o, I M and Santos, N C},
  year = {2014},
  journal = {A\&A},
  volume = {572},
  pages = {95},
  doi = {10.1051/0004-6361/201424537},
  urldate = {2020-03-12},
  abstract = {Context. Precise stellar parameters (effective temperature, surface gravity, metallicity, stellar mass, and radius) are crucial for several reasons, amongst which are the precise characterization of orbiting exoplanets and the correct determination of galactic chemical evolution. The atmospheric parameters are extremely important because all the other stellar parameters depend on them. Using our standard equivalent-width method on high-resolution spectroscopy, good precision can be obtained for the derived effective temperature and metallicity. The surface gravity, however, is usually not well constrained with spectroscopy. Aims. We use two different samples of FGK dwarfs to study the effect of the stellar surface gravity on the precise spectroscopic determination of the other atmospheric parameters. Furthermore, we present a straightforward formula for correcting the spectroscopic surface gravities derived by our method and with our linelists. Methods. Our spectroscopic analysis is based on Kurucz models in local thermodynamic equilibrium, performed with the MOOG code to derive the atmospheric parameters. The surface gravity was either left free or fixed to a predetermined value. The latter is either obtained through a photometric transit light curve or derived using asteroseismology. Results. We find first that, despite some minor trends, the effective temperatures and metallicities for FGK dwarfs derived with the described method and linelists are, in most cases, only affected within the errorbars by using different values for the surface gravity, even for very large differences in surface gravity, so they can be trusted. The temperatures derived with a fixed surface gravity continue to be compatible within 1 sigma with the accurate results of the infrared flux method (IRFM), as is the case for the unconstrained temperatures. Secondly, we find that the spectroscopic surface gravity can easily be corrected to a more accurate value using a linear function with the effective temperature.},
  keywords = {abundances-techniques,fundamental parameters-stars,notion,notion-database,spectroscopic-asteroseismology,stars},
  file = {/Users/lbugnet/Zotero/storage/ZWXKD6V3/full-text.pdf}
}

@article{Mortier2018,
  title = {New and Updated Stellar Parameters for 90 Transit Hosts. {{The}} Effect of the Surface Gravity},
  author = {Mortier, A. and Santos, N. C. and Sousa, S. G. and Fernandes, J. M. and Adibekyan, V. {\relax Zh}. and Mena, E. Delgado and Montalto, M. and Israelian, G.},
  year = {2018},
  month = sep,
  journal = {Astronomy and Astrophysics},
  eprint = {1309.1998},
  doi = {10.1051/0004-6361/201322240},
  urldate = {2020-01-20},
  abstract = {Context. Precise stellar parameters are crucial in exoplanet research for correctly determining of the planetary parameters. For stars hosting a transiting planet, determining of the planetary mass and radius depends on the stellar mass and radius, which in turn depend on the atmospheric stellar parameters. Different methods can provide different results, which leads to different planet characteristics.\vphantom\{\}\%Spectroscopic surface gravities have shown to be poorly constrained, but the photometry of the transiting planet can provide an independent measurement of the surface gravity. Aims. In this paper, we use a uniform method to spectroscopically derive stellar atmospheric parameters, chemical abundances, stellar masses, and stellar radii for a sample of 90 transit hosts. Surface gravities are also derived photometrically using the stellar density as derived from the light curve. We study the effect of using these different surface gravities on the determination of the chemical abundances and the stellar mass and radius. Methods. A spectroscopic analysis based on Kurucz models in LTE was performed through the MOOG code to derive the atmospheric parameters and the chemical abundances. The photometric surface gravity was determined through isochrone fitting and the use of the stellar density, directly determined from the light curve. Stellar masses and radii are determined through calibration formulae. Results. Spectroscopic and photometric surface gravities differ, but this has very little effect on the precise determination of the stellar mass in our spectroscopic analysis. The stellar radius, and hence the planetary radius, is most affected by the surface gravity discrepancies. For the chemical abundances, the difference is, as expected, only noticable for the abundances derived from analyzing of lines of ionized species.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VRHA43I4/full-text.pdf}
}

@article{Moss1986,
  title = {Magnetic Fields in Stars},
  author = {Moss, David},
  year = {1986},
  journal = {Physics Reports},
  issn = {03701573},
  doi = {10.1016/0370-1573(86)90172-9},
  abstract = {The observational evidence for stellar magnetic fields is reviewed. A detailed theoretical discussion of fields in the chemically peculiar stars of the middle main sequence is given, contrasting the rival claims of the fossil and contemporary dynamo theories for the origin of the field. It is shown how current theoretical ideas can lead to inferences about the interior field, even though only limited information about the surface field distribution is available. The solar field is discussed in terms of dynamo theory, and tentative extensions to similar, lower main sequence, stars are discussed. An account is also given of magnetic fields in degenerate objects (white dwarfs and neutron stars). Brief reference is made to magnetic fields in other stages of stellar evolution. \textcopyright{} 1986.},
  keywords = {notion,notion-database}
}

@article{Moss1989,
  title = {The Origin and Internal Structure of the Magnetic Fields of the {{CP}} Stars},
  author = {Moss, D.},
  year = {1989},
  journal = {MNRAS},
  volume = {236},
  pages = {629--644},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Moss1992,
  title = {Magnetic Fields and Differential Rotation in Stars},
  author = {Moss, David},
  year = {1992},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {257},
  number = {4},
  pages = {593--601},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BC3SPI42/1992MNRAS_257__593M.pdf}
}

@article{MossDavid,
  title = {Magnetic Fields and Differential Rotation in Stars},
  author = {{Moss, David}},
  journal = {Mnras},
  volume = {257},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5RT5PIQ2/document.pdf}
}

@article{Mosser2005a,
  title = {Seismology and Activity of the {{F}} Type Star {{HD}} 49933},
  author = {Mosser, B. and Bouchy, F. and Catala, C. and Michel, E. and Samadi, R. and Th{\'e}venin, F. and Eggenberger, P. and Sosnowska, D. and Moutou, C. and Baglin, A.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {431},
  number = {2},
  pages = {13--16},
  issn = {00046361},
  doi = {10.1051/0004-6361:200500003},
  abstract = {A 10-night asteroseismic observation programme has been conducted in January 2004 with the spectrometer HARPS at the ESO 3.6-m telescope. The selected target, the 6th magnitude F5V star HD 49933, was chosen among the prime candidates of COROT, the European space mission dedicated to characterize stellar oscillations mode with high precision photometry measurements. This star shows important line profiles variations, indicating a surprisingly high activity with respect to its low rotation rate. However, with the help of tools developed for disentangling the signatures of activity and oscillations, we are able to observe its oscillation spectrum in the frequency range [1.2, 2.2 mHz]. We measure the large separation (88.7 {$\pm$} 0.4 {$\mu$}Hz) and the maximum amplitude (around 0.4 {$\pm$}0. 1 m8-1 rms), respectively in agreement and marginal agreement with the predicted values.},
  keywords = {notion,notion-database,Stars: oscillations,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/ZWP2ZW8C/Mosser et al. - 2005.pdf}
}

@article{Mosser2008,
  title = {{{HD}} 203608, a Quiet Asteroseismic Target in the Old Galactic Disk},
  author = {Mosser, B. and Deheuvels, S. and Michel, E. and Th{\'e}venin, F. and Dupret, A. and Samadi, R. and Barban, C. and Goupil, J.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {488},
  number = {2},
  pages = {635--642},
  issn = {00046361},
  doi = {10.1051/0004-6361:200810011},
  abstract = {Context. We conducted a 5-night observing run with the spectrometer harps at the ESO 3.6-m telescope in August 2006, to continue exploring the asteroseismic properties of F-type stars. In fact, Doppler observations of F-type on the main sequence are demanding and remain currently limited to a single case (HD 49933). Comparison with photometric results obtained with the CoRoT space mission (Convection, Rotation and planetary Transits) on similar stars will be possible with an enhanced set of observations.Aims. We selected the 4th magnitude F8V star HD 203608 to investigate the oscillating properties of a low-metallicity star of the old galactic disk.Methods. We reduced the spectra with the on-line data reduction software provided by the instrument. We developed a new statistical approach for extracting the significant peaks in the Fourier domain.Results. The oscillation spectrum shows a significant excess power in the frequency range [1.5, 3.0 mHz]. It exhibits a large spacing of about 120.4 Hz at 2.5 mHz. Variations of the large spacing with frequency are clearly identified, which require an adapted asymptotic development. The modes identification is based on the unambiguous signature of 15 modes with = 0 and 1.Conclusions. These observations show the potential diagnostic of asteroseismic constraints. Including them in the stellar modeling significantly enhances the precision on the physical parameters of HD 203608, resulting in a much more precise position in the HR diagram. The age of the star is now determined in the range 7.250.07 Gyr. \textcopyright{} 2008 ESO.},
  keywords = {notion,notion-database,Stars: evolution,Stars: oscillations,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/BVK7G6YV/Mosser et al. - 2008.pdf}
}

@article{Mosser2008a,
  title = {Asteroseismology of {{Procyon}} with {{SOPHIE}}},
  author = {Mosser, B. and Bouchy, F. and Marti{\'c}, M. and Appourchaux, T. and Barban, C. and Berthomieu, G. and Garcia, R. A. and Lebrun, J. C. and Michel, E. and Provost, J. and Th{\'e}venin, F. and {Turck-Chi{\`e}ze}, S.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {478},
  number = {1},
  pages = {197--202},
  issn = {00046361},
  doi = {10.1051/0004-6361:20078337},
  abstract = {Context.This paper reports a 9-night asteroseismic observation program conducted in January 2007 with the new spectrometer SOPHIE at the OHP 193-cm telescope, on the F5 IV-V target Procyon A.Aims.This first asteroseismic program with SOPHIE was intended to test the performance of the instrument with a bright but demanding asteroseismic target and was part of a multisite network.Methods.The SOPHIE spectra have been reduced with the data reduction software provided by OHP. The Procyon asteroseismic data were then analyzed with statistical tools. The asymptotic analysis has been conducted considering possible curvature in the \'echelle diagram analysis.Results.These observations have proven the efficient performance of SOPHIE used as an asteroseismometer, and succeed in a clear detection of the large spacing. An \'echelle diagram based on the 54-Hz spacing shows clear ridges. Identification of the peaks exhibits large spacings varying from about 52 Hz to 56 Hz. Outside the frequency range [0.9, 1.0 mHz] where the identification is confused, the large spacing increases at a rate of about Hz. This may explain some of the different values of the large spacing obtained by previous observations. \textcopyright{} 2008 ESO.},
  keywords = {notion,notion-database,Stars: individual: {$\alpha$} CMi,Stars: oscillations,Techniques: radial velocities},
  file = {/Users/lbugnet/Zotero/storage/9VDXZG4B/Mosser et al. - 2008(2).pdf}
}

@article{Mosser2009a,
  title = {The {{CoRoT}} Target {{HD175726}}: {{An}} Active Star with Weak Solar-like Oscillations},
  author = {Mosser, B. and Michel, E. and Appourchaux, T. and Barban, C. and Baudin, F. and Boumier, P. and Bruntt, H. and Catala, C. and Deheuvels, S. and Garc{\'i}a, R. A. and Gaulme, P. and Regulo, C. and Roxburgh, I. and Samadi, R. and Verner, G. and Auvergne, M. and Baglin, A. and Ballot, J. and Benomar, O. and Mathur, S.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {33--40},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911917},
  abstract = {Context. The CoRoT short runs give us the opportunity to observe a large variety of late-type stars through their solar-like oscillations. We report observations of the star HD175726 that lasted for 27 days during the first short run of the mission. The time series reveals a high-activity signal and the power spectrum presents an excess due to solar-like oscillations with a low signal-to-noise ratio. Aims. Our aim is to identify the most efficient tools to extract as much information as possible from the power density spectrum. Methods. The most productive method appears to be the autocorrelation of the time series, calculated as the spectrum of the filtered spectrum. This method is efficient, very rapid computationally, and will be useful for the analysis of other targets, observed with CoRoT or with forthcoming missions such as Kepler and Plato. Results. The mean large separation has been measured to be 97.2{$\pm$}0.5 {$\mu$}Hz, slightly below the expected value determined from solar scaling laws. We also show strong evidence for variation of the large separation with frequency. The bolometric mode amplitude is only 1.7 {$\pm$} 0.25 ppm for radial modes, which is 1.7 times less than expected. Due to the low signal-to-noise ratio, mode identification is not possible for the available data set of HD175726.},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual: HD 175726,Stars: interiors,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/LHXK2GIR/Mosser et al. - 2009.pdf}
}

@article{Mosser2009b,
  title = {On Detecting the Large Separation in the Autocorrelation of Stellar Oscillation Times Series},
  author = {Mosser, B. and Appourchaux, T.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {508},
  number = {2},
  pages = {877--887},
  issn = {00046361},
  doi = {10.1051/0004-6361/200912944},
  abstract = {Context: The observations carried out by the space missions CoRoT and Kepler provide a large set of asteroseismic data. Their analysis requires an efficient procedure first to determine if a star reliably shows solar-like oscillations, second to measure the so-called large separation, third to estimate the asteroseismic information that can be retrieved from the Fourier spectrum. Aims. In this paper we develop a procedure based on the autocorrelation of the seismic Fourier spectrum that is capable of providing measurements of the large and small frequency separations. The performance of the autocorrelation method needs to be assessed and quantified. We therefore searched for criteria able to predict the output that one can expect from the analysis by autocorrelation of a seismic time series. Methods. First, the autocorrelation is properly scaled to take into account the contribution of white noise. Then we use the null hypothesis H 0 test to assess the reliability of the autocorrelation analysis. Calculations based on solar and CoRoT time series are performed to quantify the performance as a function of the amplitude of the autocorrelation signal. Results. We obtain an empirical relation for the performance of the autocorrelation method.We show that the precision of the method increases with the observation length, and with the mean seismic amplitude-to-background ratio of the pressure modes to the power 1.5{$\pm$}0.05.We propose an automated determination of the large separation, whose reliability is quantified by the H 0 test.We apply this method to analyze red giants observed by CoRoT. We estimate the expected performance for photometric time series of the Kepler mission. We demonstrate that the method makes it possible to distinguish {$\mathscr{l}$} = 0 from {$\mathscr{l}$} = 1 modes. Conclusions. The envelope autocorrelation function (EACF) has proven to be very powerful for the determination of the large separation in noisy asteroseismic data, since it enables us to quantify the precision of the performance of different measurements: mean large separation, variation of the large separation with frequency, small separation and degree identification. \textcopyright{} 2009 ESO.},
  keywords = {Methods: analytical,Methods: data analysis,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/GJ5C8JBA/Mosser, Appourchaux - 2009.pdf}
}

@article{Mosser2009d,
  title = {Short-Lived Spots in Solar-like Stars as Observed by {{CoRoT}}},
  author = {Mosser, B. and Baudin, F. and Lanza, A. F. and Hulot, J. C. and Catala, C. and Baglin, A. and Auvergne, M.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {245--254},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911942},
  abstract = {Context. CoRoT light curves have an unprecedented photometric quality, having simultaneously a high signal-to-noise ratio, a long time span and a nearly continuous duty-cycle. Aims. We analyse the light-curves of four bright targets observed in the seismology field and study short-lived small spots in solar-like stars. Methods. We present a simple spot modeling by iterative analysis. Its ability to extract relevant parameters is ensured by implementing relaxation steps to avoid convergence to local minima of the sum of the residuals between observations and modeling. The use of Monte-Carlo simulations allows us to estimate the performance of the fits. Results. Our starspot modeling gives a representation of the spots on these stars in agreement with other well tested methods. Within this framework, parameters such as rigid-body rotation and spot lifetimes seem to be precisely determined. Then, the lifetime/rotation period ratios are in the range 0.5-2, and there is clear evidence for differential rotation.},
  keywords = {notion,notion-database,Stars: activity,Stars: rotation,Starspots,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/64H99DS6/Mosser et al. - 2009(2).pdf}
}

@article{Mosser2010a,
  title = {The Universal Red-Giant Oscillation Pattern: {{An}} Automated Determination with {{CoRoT}} Data},
  author = {Mosser, B. and Belkacem, K. and Goupil, M. J. and Michel, E. and Elsworth, Y. and Barban, C. and Kallinger, T. and Hekker, S. and De Ridder, J. and Samadi, R. and Baudin, F. and Pinheiro, F. J.G. and Auvergne, M. and Baglin, A. and Catala, C.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {525},
  number = {7},
  pages = {2--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201015440},
  abstract = {Aims.The CoRoT and Kepler satellites have provided thousands of red-giant oscillation spectra. The analysis of these spectra requires efficient methods of identifying all eigenmode parameters. Methods. The assumption of new scaling laws allowed us to construct a theoretical oscillation pattern. We then obtained a highly precise determination of the large separation by correlating the observed patterns with this reference. Results.We demonstrate that this pattern is universal and are able to unambiguously assign the eigenmode radial orders and angular degrees. This solves one of the remaining problems of asteroseismology, hence allowing precise theoretical investigation of red-giant interiors. \textcopyright{} 2010 ESO.},
  keywords = {methods: analytical,methods: data analysis,notion,notion-database,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/5JBVG95E/Mosser et al. - 2010.pdf}
}

@article{Mosser2010d,
  title = {Red-Giant Seismic Properties Analyzed with {{CoRoT}}},
  author = {Mosser, B. and Belkacem, K. and Goupil, M.-J. and Miglio, A. and Morel, T. and Barban, C. and Baudin, F. and Hekker, S. and Samadi, R. and De Ridder, J. and Weiss, W. and Auvergne, M. and Baglin, A.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {517},
  pages = {A22},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201014036},
  abstract = {Context. The CoRoT 5-month long observation runs provide us with the opportunity to analyze a large variety of red-giant stars and derive their fundamental parameters from their asteroseismic properties. Aims. We perform an analysis of more than 4600 CoRoT light curves to extract as much information as possible. We take into account the characteristics of both the star sample and the method to ensure that our asteroseismic results are as unbiased as possible. We also study and compare the properties of red giants in two opposite regions of the Galaxy. Methods. We analyze the time series using the envelope autocorrelation function to extract precise asteroseismic parameters with reliable error bars. We examine first the mean wide frequency separation of solar-like oscillations and the frequency of the maximum seismic amplitude, then the parameters of the excess power envelope. With the additional information of the effective temperature, we derive the stellar mass and radius. Results. We identify more than 1800 red giants among the 4600 light curves and obtain accurate distributions of the stellar parameters for about 930 targets. We are able to reliably measure the mass and radius of several hundred red giants. We derive precise information about the stellar population distribution and the red clump. By comparing the stars observed in two different fields, we find that the stellar asteroseismic properties are globally similar, but that the characteristics are different for red-clump stars. Conclusions. This study demonstrates the efficiency of statistical asteroseismology: validating scaling relations allows us to infer fundamental stellar parameters, derive precise information about red-giant evolution and interior structure, analyze and compare stellar populations from different fields. \textcopyright{} 2010 ESO.},
  keywords = {abundances,evolution,fundamental parameters,interiors,notion,notion-database,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/LEZB4W9A/Mosser et al. - 2010(2).pdf}
}

@article{Mosser2010e,
  title = {An Alternative to Mode Fitting},
  author = {Mosser, B.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  pages = {944--948},
  issn = {00046337},
  doi = {10.1002/asna.201011432},
  abstract = {The space mission CoRoT provides us with a large amount of high-duty cycle long-duration observations. Mode fitting has proven to be efficient for the complete and detailed analysis of the oscillation pattern, but remains time consuming. Furthermore, the photometric background due to granulation severely complicates the analysis. Therefore, we attempt to provide an alternative to mode fitting, for the determination of large separations. With the envelope autocorrelation function and a dedicated filter, it is possible to measure the variation of the large separation independently for the ridges with even and odd degrees. The method appears to be as accurate as the mode fitting. It can be very easily implemented and is very rapid. \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {notion,notion-database,Stars: evolution,{Stars: individual (HD 49385, HD 49933, HD 181420,},Stars: interiors,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/XGBRXBY3/Mosser - 2010.pdf}
}

@article{Mosser2011,
  title = {Mixed Modes in Red-Giant Stars Observed with {{CoRoT}}},
  author = {Mosser, B. and Barban, C. and Montalb{\'a}n, J. and Beck, P. G. and Miglio, A. and Belkacem, K. and Goupil, M. J. and Hekker, S. and De Ridder, J. and Dupret, M. A. and Elsworth, Y. and Noels, A. and Baudin, F. and Michel, E. and Samadi, R. and Auvergne, M. and Baglin, A. and Catala, C.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {532},
  pages = {1--8},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116825},
  abstract = {Context. The CoRoT mission has provided thousands of red-giant light curves. The analysis of their solar-like oscillations allows us to characterize their stellar properties. Aims. Up to now, the global seismic parameters of the pressure modes have been unable to distinguish red-clump giants from members of the red-giant branch. As recently done with Kepler red giants, we intend to analyze and use the so-called mixed modes to determine the evolutionary status of the red giants observed with CoRoT. We also aim at deriving different seismic characteristics depending on evolution. Methods. The complete identification of the pressure eigenmodes provided by the red-giant universal oscillation pattern allows us to aim at the mixed modes surrounding the = 1 expected eigenfrequencies. A dedicated method based on the envelope autocorrelation function is proposed to analyze their period separation. Results. We have identified the mixed-mode signature separation thanks to their pattern that is compatible with the asymptotic law of gravity modes. We have shown that, independent of any modeling, the g-mode spacings help to distinguish the evolutionary status of a red-giant star. We then report the different seismic and fundamental properties of the stars, depending on their evolutionary status. In particular, we show that high-mass stars of the secondary clump present very specific seismic properties. We emphasize that stars belonging to the clump were affected by significant mass loss. We also note significant population and/or evolution differences in the different fields observed by CoRoT. \textcopyright{} 2011 ESO.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: interiors,Stars: mass-loss,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/UBGAUZNG/Mosser et al. - 2011.pdf}
}

@article{Mosser2012,
  title = {Characterization of the Power Excess of Solar-like Oscillations in Red Giants with {{Kepler}}},
  author = {Mosser, B. and Elsworth, Y. and Hekker, S. and Huber, D. and Kallinger, T. and Mathur, S. and Belkacem, K. and Goupil, M. J. and Samadi, R. and Barban, C. and Bedding, T. R. and Chaplin, W. J. and Garc{\'i}a, R. A. and Stello, D. and De Ridder, J. and Middour, C. K. and Morris, R. L. and Quintana, E. V.},
  year = {2012},
  journal = {Astronomy \& Astrophysics},
  volume = {537},
  pages = {1--15},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117352},
  abstract = {Context. The space mission Kepler provides us with long and uninterrupted photometric time series of red giants. This allows us to examine their seismic global properties and to compare these with theoretical predictions. Aims. We aim to describe the oscillation power excess observed in red giant oscillation spectra with global seismic parameters, and to investigate empirical scaling relations governing these parameters. From these scalings relations, we derive new physical properties of red giant oscillations. Methods. Various different methods were compared in order to validate the processes and to derive reliable output values. For consistency, a single method was then used to determine scaling relations for the relevant global asteroseismic parameters: mean mode height, mean height of the background signal superimposed on the oscillation power excess, width of the power excess, bolometric amplitude of the radial modes and visibility of non-radial modes. A method for deriving oscillation amplitudes is proposed, which relies on the complete identification of the red giant oscillation spectrum. Results. The comparison of the different methods has shown the important role of the way the background is modelled. The convergence reached by the collaborative work enables us to derive significant results concerning the oscillation power excess. We obtain several scaling relations, and identify the influence of the stellar mass and the evolutionary status. The effect of helium burning on the red giant interior structure is confirmed: it yields a strong mass-radius relation for clump stars. We find that none of the amplitude scaling relations motivated by physical considerations predict the observed mode amplitudes of red giant stars. In parallel, the degree-dependent mode visibility exhibits important variations. Both effects seem related to the significant influence of the high mode mass of non-radial mixed modes. A family of red giants with very weak dipole modes is identified, and its properties are analyzed. Conclusions. The clear correlation between the power densities of the background signal and of the stellar oscillation induces important consequences to be considered for deriving a reliable theoretical relation of the mode amplitude. As a by-product of this work, we have verified that red giant asteroseismology delivers new insights for stellar and Galactic physics, given the evidence for mass loss at the tip of the red giant branch. \textcopyright{} 2012 ESO.},
  keywords = {methods: data analysis,notion,notion-database,stars: evolution,stars: interiors,stars: late-type,stars: mass-loss,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/IFWMZUAN/Mosser et al. - 2012.pdf}
}

@article{Mosser2012b,
  title = {Spin down of the Core Rotation in Red Giants},
  author = {Mosser, B. and Goupil, M. J. and Belkacem, K. and Marques, J. P. and Beck, P. G. and Bloemen, S. and De Ridder, J. and Barban, C. and Deheuvels, S. and Elsworth, Y. and Hekker, S. and Kallinger, T. and Ouazzani, R. M. and Pinsonneault, M. and Samadi, R. and Stello, D. and Garc{\'i}a, R. A. and Klaus, T. C. and Li, J. and Mathur, S. and Morris, R. L.},
  year = {2012},
  journal = {Astronomy \& Astrophysics},
  volume = {548},
  eprint = {1209.3336},
  pages = {1--14},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220106},
  abstract = {Context. The space mission Kepler provides us with long and uninterrupted photometric time series of red giants. We are now able to probe the rotational behaviour in their deep interiors using the observations of mixed modes. Aims. We aim to measure the rotational splittings in red giants and to derive scaling relations for rotation related to seismic and fundamental stellar parameters. Methods. We have developed a dedicated method for automated measurements of the rotational splittings in a large number of red giants. Ensemble asteroseismology, namely the examination of a large number of red giants at different stages of their evolution, allows us to derive global information on stellar evolution. Results. We have measured rotational splittings in a sample of about 300 red giants. We have also shown that these splittings are dominated by the core rotation. Under the assumption that a linear analysis can provide the rotational splitting, we observe a small increase of the core rotation of stars ascending the red giant branch. Alternatively, an important slow down is observed for red-clump stars compared to the red giant branch. We also show that, at fixed stellar radius, the specific angular momentum increases with increasing stellar mass. Conclusions. Ensemble asteroseismology indicates what has been indirectly suspected for a while: our interpretation of the observed rotational splittings leads to the conclusion that the mean core rotation significantly slows down during the red giant phase. The slow-down occurs in the last stages of the red giant branch. This spinning down explains, for instance, the long rotation periods measured in white dwarfs. \textcopyright{} 2012 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: interiors,Stars: late-type,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/6VMCJW74/Mosser et al. - 2012(2).pdf}
}

@article{Mosser2012c,
  title = {Probing the Core Structure and Evolution of Red Giants Using Gravity-Dominated Mixed Modes Observed with {{Kepler}}},
  author = {Mosser, B. and Goupil, M. J. and Belkacem, K. and Michel, E. and Stello, D. and Marques, J. P. and Elsworth, Y. and Barban, C. and Beck, P. G. and Bedding, T. R. and De Ridder, J. and Garc{\'i}a, R. A. and Hekker, S. and Kallinger, T. and Samadi, R. and Stumpe, M. C. and Barclay, T. and Burke, C. J.},
  year = {2012},
  journal = {Astronomy \& Astrophysics},
  volume = {540},
  pages = {1--11},
  issn = {00046361},
  doi = {10.1051/0004-6361/201118519},
  abstract = {Context. There are now more than 22 months of long-cadence data available for thousands of red giants observed with the Kepler space mission. Consequently, we are able to clearly resolve fine details in their oscillation spectra and see many components of the mixed modes that probe the stellar core. Aims. We report for the first time a parametric fit to the pattern of the l = 1 mixed modes in red giants, which is a powerful tool to identify gravity-dominated mixed modes. With these modes, which share the characteristics of pressure and gravity modes, we are able to probe directly the helium core and the surrounding shell where hydrogen is burning. Methods. We propose two ways for describing the so-called mode bumping that affects the frequencies of the mixed modes. Firstly, a phenomenological approach is used to describe the main features of the mode bumping. Alternatively, a quasi-asymptotic mixed-mode relation provides a powerful link between seismic observations and the stellar interior structure. We used period \'echelle diagrams to emphasize the detection of the gravity-dominated mixed modes. Results. The asymptotic relation for mixed modes is confirmed. It allows us to measure the gravity-mode period spacings in more than two hundred red giant stars. The identification of the gravity-dominated mixed modes allows us to complete the identification of all major peaks in a red giant oscillation spectrum, with significant consequences for the true identification of l = 3 modes, of l = 2 mixed modes, for the mode widths and amplitudes, and for the l = 1 rotational splittings. Conclusions. The accurate measurement of the gravity-mode period spacing provides an effective probe of the inner, g-mode cavity. The derived value of the coupling coefficient between the cavities is different for red giant branch and clump stars. This provides a probe of the hydrogen-shell burning region that surrounds the helium core. Core contraction as red giants ascend the red giant branch can be explored using the variation of the gravity-mode spacing as a function of the mean large separation. \textcopyright{} ESO, 2012.},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: evolution,Stars: interiors,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RA2I2U2Q/Mosser et al. - 2012(3).pdf}
}

@article{Mosser2013,
  title = {Sounding Stellar Cores with Mixed Modes},
  author = {Mosser, B. and Belkacem, K. and Vrard, M.},
  year = {2013},
  journal = {EAS Publications Series},
  volume = {63},
  number = {2013},
  eprint = {1310.4752},
  pages = {137--150},
  issn = {16381963},
  doi = {10.1051/eas/1363016},
  abstract = {The space-borne missions CoRoT and Kepler have opened a new era in stellar physics, especially for evolved stars, with precise asteroseismic measurements that help determine precise stellar parameters and perform ensemble asteroseismology. This paper deals with the quality of the information that we can retrieve from the oscillations. It focusses on the conditions for obtaining the most accurate measurement of the radial and non-radial oscillation patterns. This accuracy is a prerequisite for making the best with asteroseismic data. From radial modes, we derive proxies of the stellar mass and radii with an unprecedented accuracy for field stars. For dozens of subgiants and thousands of red giants, the identification of mixed modes (corresponding to gravity waves propagating in the core coupled to pressure waves propagating in the envelope) indicates unambiguously their evolutionary status. As probes of the stellar core, these mixed modes also reveal the internal differential rotation and show the spinning down of the core rotation of stars ascending the red giant branch. A toy model of the coupling of waves constructing mixed modes is exposed, for illustrating many of their features.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LLDILXXJ/Mosser, Belkacem, Vrard - 2013.pdf}
}

@article{Mosser2013a,
  title = {Period-Luminosity Relations in Evolved Red Giants Explained by Solar-like Oscillations},
  author = {Mosser, B. and Dziembowski, W. A. and Belkacem, K. and Goupil, M. J. and Michel, E. and Samadi, R. and Soszy{\'n}ski, I. and Vrard, M. and Elsworth, Y. and Hekker, S. and Mathur, S.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {559},
  pages = {1--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/201322243},
  abstract = {Context. Solar-like oscillations in red giants have been investigated with the space-borne missions CoRoT and Kepler, while pulsations in more evolved M giants have been studied with ground-based microlensing surveys. After 3.1 years of observation with Kepler, it is now possible to link these different observations of semi-regular variables. Aims. We aim to identify period-luminosity sequences in evolved red giants identified as semi-regular variables and to interpret them in terms of solar-like oscillations. Then, we investigate the consequences of the comparison of ground-based and space-borne observations. Methods. We first measured global oscillation parameters of evolved red giants observed with Kepler with the envelope autocorrelation function method. We then used an extended form of the universal red giant oscillation pattern, extrapolated to very low frequency, to fully identify their oscillations. The comparison with ground-based results was then used to express the period-luminosity relation as a relation between the large frequency separation and the stellar luminosity. Results. From the link between red giant oscillations observed by Kepler and period-luminosity sequences, we have identified these relations in evolved red giants as radial and non-radial solar-like oscillations. We were able to expand scaling relations at very low frequency (periods as long as 100 days and large frequency separation less than 0.05 {$\mu$}Hz). This helped us identify the different sequences of period-luminosity relations, and allowed us to propose a calibration of the K magnitude with the observed large frequency separation. Conclusions. Interpreting period-luminosity relations in red giants in terms of solar-like oscillations allows us to investigate the time series obtained from ground-based microlensing surveys with a firm physical basis. This can be done with an analytical expression that describes the low-frequency oscillation spectra. The different behavior of oscillations at low frequency, with frequency separations scaling only approximately with the square root of the mean stellar density, can be used to precisely address the physics of the semi-regular variables. This will allow improved distance measurements and opens the way to extragalactic asteroseismology with the observations of M giants in the Magellanic Clouds. \textcopyright{} 2013 ESO.},
  keywords = {notion,notion-database,Stars: evolution,Stars: horizontal-branch,Stars: interiors,Stars: late-type,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TQAG3KPN/Mosser et al. - 2013.pdf}
}

@article{Mosser2013d,
  title = {Asymptotic and Measured Large Frequency Separations},
  author = {Mosser, B. and Michel, E. and Belkacem, K. and Goupil, M. J. and Baglin, A. and Barban, C. and Provost, J. and Samadi, R. and Auvergne, M. and Catala, C.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {550},
  pages = {1--12},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220435},
  abstract = {Context. With the space-borne missions CoRoT and Kepler, a large amount of asteroseismic data is now available and has led to a variety of work. So-called global oscillation parameters are inferred to characterize the large sets of stars, perform ensemble asteroseismology, and derive scaling relations. The mean large separation is such a key parameter, easily deduced from the radial-frequency differences in the observed oscillation spectrum and closely related to the mean stellar density. It is therefore crucial to measure it with the highest accuracy in order to obtain the most precise asteroseismic indices. Aims. As the conditions of measurement of the large separation do not coincide with its theoretical definition, we revisit the asymptotic expressions used for analyzing the observed oscillation spectra. Then, we examine the consequence of the difference between the observed and asymptotic values of the mean large separation. Methods. The analysis is focused on radial modes. We use series of radial-mode frequencies in published analyses of stars with solar-like oscillations to compare the asymptotic and observational values of the large separation. This comparison relies on the proper use of the second-order asymptotic expansion. Results. We propose a simple formulation to correct the observed value of the large separation and then derive its asymptotic counterpart. The measurement of the curvature of the radial ridges in the \'echelle diagram provides the correcting factor. We prove that, apart from glitches due to stellar structure discontinuities, the asymptotic expansion is valid from main-sequence stars to red giants. Our model shows that the asymptotic offset is close to 1/4, as in the theoretical development, for low-mass, main-sequence stars, subgiants and red giants. Conclusions. High-quality solar-like oscillation spectra derived from precise photometric measurements are definitely better described with the second-order asymptotic expansion. The second-order term is responsible for the curvature observed in the \'echelle diagrams used for analyzing the oscillation spectra, and this curvature is responsible for the difference between the observed and asymptotic values of the large separation. Taking it into account yields a revision of the scaling relations, which provides more accurate asteroseismic estimates of the stellar mass and radius. After correction of the bias (6\% for the stellar radius and 3\% for the mass), the performance of the calibrated relation is about 4\% and 8\% for estimating, respectively, the stellar radius and the stellar mass for masses less than 1.3 M\^a\v{S}\texttrademark; the accuracy is twice as bad for higher mass stars and red giants. \textcopyright{} ESO, 2013.},
  keywords = {Methods: analytical,Methods: data analysis,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/C2MQLPNV/Mosser et al. - 2013(2).pdf}
}

@article{Mosser2013e,
  title = {Red Giant Seismology: {{Observations}}},
  author = {Mosser, B.},
  year = {2013},
  journal = {EPJ Web of Conferences},
  volume = {43},
  issn = {21016275},
  doi = {10.1051/epjconf/20134303003},
  abstract = {The CoRoT and Kepler missions provide us with thousands of red-giant light curves that allow a very precise asteroseismic study of these objects. Before CoRoT and Kepler, the red-giant oscillation patterns remained obscure. Now, these spectra are much more clear and unveil many crucial interior structure properties. For thousands of red giants, we can derive from seismic data precise estimates of the stellar mass and radius, the evolutionary status of the giants (with a clear difference between clump and RGB stars), the internal differential rotation, the mass loss, the distance of the stars... Analyzing this amount of information is made easy by the identification of the largely homologous red-giant oscillation patterns. For the first time, both pressure and mixed mode oscillation patterns can be precisely depicted. The mixed-mode analysis allows us, for instance, to probe directly the stellar core. Fine details completing the red-giant oscillation pattern then provide further information on the interior structure, including differential rotation. \textcopyright{} 2013 Owned by the authors, published by EDP Sciences.},
  isbn = {9782759809691},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/34EJ4SFI/Mosser - 2013.pdf}
}

@article{Mosser2014,
  title = {Astrophysics {{L}} Etter to the {{E}} Ditor {{Mixed}} Modes in Red Giants : A Window on Stellar Evolution},
  author = {Mosser, B and Benomar, O and Belkacem, K and Goupil, M J and Lagarde, N and Michel, E and Lebreton, Y and Stello, Dennis},
  year = {2014},
  volume = {5},
  pages = {1--5},
  keywords = {evolution,interiors,notion,notion-database,oscillations,stars},
  file = {/Users/lbugnet/Zotero/storage/W6DJEVU3/Mosser et al. - 2014.pdf}
}

@article{Mosser2015,
  title = {Period Spacings in Red Giants: {{I}}. {{Disentangling}} Rotation and Revealing Core Structure Discontinuities},
  author = {Mosser, B. and Vrard, M. and Belkacem, K. and Deheuvels, S. and Goupil, M. J.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {584},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527075},
  abstract = {Context. Asteroseismology allows us to probe the physical conditions inside the core of red giant stars. This process relies on the properties of the global oscillations with a mixed character that are highly sensitive to the physical properties of the core. However, overlapping rotational splittings and mixed-mode spacings result in complex structures in the mixed-mode pattern, which severely complicates its identification and the measurement of the asymptotic period spacing. Aims. This work aims at disentangling the rotational splittings from the mixed-mode spacings in order to open the way to a fully automated analysis of large data sets. Methods. An analytical development of the mixed-mode asymptotic expansion is used to derive the period spacing between two consecutive mixed modes. The \'echelle diagrams constructed with the appropriately stretched periods are used to exhibit the structure of the gravity modes and of the rotational splittings. Results. We propose a new view of the mixed-mode oscillation pattern based on corrected periods, called stretched periods, that mimic the evenly spaced gravity-mode pattern. This provides a direct understanding of all oscillation components, even in the case of rapid rotation. In this way, the measurement of the asymptotic period spacing and the signature of the structural glitches on mixed modes can be performed easily. Conclusions. This work makes it possible to derive all seismic global parameters in an automated way, including the identification of the different rotational multiplets and the measurement of the rotational splitting, even when this splitting is significantly larger than the period spacing. Revealing buoyancy glitches provides a detailed view of the radiative core.},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/7D33LK6N/Mosser et al. - 2015.pdf}
}

@article{Mosser2015a,
  title = {Stellar Oscillations - {{I}} - {{The}} Adiabatic Case},
  author = {Mosser, B.},
  year = {2015},
  journal = {EAS Publications Series},
  volume = {73--74},
  eprint = {1509.08077},
  pages = {3--110},
  issn = {16381963},
  doi = {10.1051/eas/1573002},
  abstract = {This lecture on adiabatic oscillations is intended to present the basis of asteroseismology and to serve as an introduction for other lectures of the EES 2014. It also exposes the state-of-the-art of solarlike oscillation analysis, as revealed by the space missions CoRoT and Kepler. A large part of the lecture is devoted to the interpretation of the modes with a mixed character that reveal the properties of the radiative cores of subgiants and red giants.},
  archiveprefix = {arxiv},
  isbn = {9782759817351},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZIVLL9DN/Mosser - 2015.pdf}
}

@article{Mosser2017,
  title = {Dipole Modes with Depressed Amplitudes in Red Giants Are Mixed Modes},
  author = {Mosser, B. and Belkacem, K. and Pin{\c c}on, C. and Takata, M. and Vrard, M. and Barban, C. and Goupil, M. J. and Kallinger, T. and Samadi, R.},
  year = {2017},
  journal = {Astronomy \& Astrophysics},
  volume = {598},
  pages = {1--12},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629494},
  abstract = {Context. Seismic observations with the space-borne Kepler mission have shown that a number of evolved stars exhibit low-amplitude dipole modes, which is referred to as depressed modes. Recently, these low amplitudes have been attributed to the presence of a strong magnetic field in the stellar core of those stars. Subsequently, and based on this scenario, the prevalence of high magnetic fields in evolved stars has been inferred. It should be noted, however, that this conclusion remains indirect. Aims. We intend to study the properties of mode depression in evolved stars, which is a necessary condition before reaching conclusions about the physical nature of the mechanism responsible for the reduction of the dipole mode amplitudes. Methods. We perform a thorough characterization of the global seismic parameters of depressed dipole modes and show that these modes have a mixed character. The observation of stars showing dipole mixed modes that are depressed is especially useful for deriving model-independent conclusions on the dipole mode damping. We use a simple model to explain how mode visibilities are connected to the extra damping seen in depressed modes. Results. Observations prove that depressed dipole modes in red giants are not pure pressure modes but mixed modes. This result, observed in more than 90\% of the bright stars (mV {$\leq$} 11), invalidates the hypothesis that depressed dipole modes result from the suppression of the oscillation in the radiative core of the stars. Observations also show that, except for visibility, seismic properties of the stars with depressed modes are equivalent to those of normal stars. The measurement of the extra damping that is responsible for the reduction of mode amplitudes, without any prior on its physical nature, potentially provides an efficient tool for elucidating the mechanism responsible for the mode depression. Conclusions. The mixed nature of the depressed modes in red giants and their unperturbed global seismic parameters carry strong constraints on the physical mechanism responsible for the damping of the oscillation in the core. This mechanism is able to damp the oscillation in the core but cannot fully suppress it. Moreover, it cannot modify the radiative cavity probed by the gravity component of the mixed modes. The recent mechanism involving high magnetic fields proposed for explaining depressed modes is not compliant with the observations and cannot be used to infer the strength and prevalence of high magnetic fields in red giants.},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: magnetic field,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TI6AJYY7/Mosser et al. - 2017.pdf;/Users/lbugnet/Zotero/storage/VBPQKJ3G/Mosser et al. - 2017.pdf}
}

@article{Mosser2017b,
  title = {Period Spacings in Red Giants: {{III}}. {{Coupling}} Factors of Mixed Modes},
  author = {Mosser, B. and Pin{\c c}on, C. and Belkacem, K. and Takata, M. and Vrard, M.},
  year = {2017},
  month = apr,
  journal = {Astronomy \& Astrophysics},
  volume = {600},
  eprint = {1612.08453},
  pages = {A1},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201630053},
  urldate = {2021-02-18},
  abstract = {Context. The power of asteroseismology relies on the capability of global oscillations to infer the stellar structure. For evolved stars, we benefit from unique information directly carried out by mixed modes that probe their radiative cores. This third article of the series devoted to mixed modes in red giants focuses on their coupling factors, which have remained largely unexploited up to now. Aims. With the measurement of coupling factors, we intend to give physical constraints on the regions surrounding the radiative core and the hydrogen-burning shell of subgiants and red giants. Methods. A new method for measuring the coupling factor of mixed modes was implemented, which was derived from the method recently implemented for measuring period spacings. This new method was automated so that it could be applied to a large sample of stars. Results. Coupling factors of mixed modes were measured for thousands of red giants. They show specific variation with mass and evolutionary stage. Weak coupling is observed for the most evolved stars on the red giant branch only; large coupling factors are measured at the transition between subgiants and red giants as well as in the red clump. Conclusions. The measurement of coupling factors in dipole mixed modes provides a new insight into the inner interior structure of evolved stars. While the large frequency separation and the asymptotic period spacings probe the envelope and core, respectively, the coupling factor is directly sensitive to the intermediate region in between and helps determine its extent. Observationally, the determination of the coupling factor is a prior to precise fits of the mixed-mode pattern and can now be used to address further properties of the mixed-mode pattern, such as the signature of buoyancy glitches and core rotation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/97Z2A942/full-text.pdf;/Users/lbugnet/Zotero/storage/DWS82KTT/1612.08453.pdf}
}

@article{Mosser2018,
  title = {Period Spacings in Red Giants: {{IV}}. {{Toward}} a Complete Description of the Mixed-Mode Pattern},
  author = {Mosser, B. and Gehan, C. and Belkacem, K. and Samadi, R. and Michel, E. and Goupil, M. J.},
  year = {2018},
  journal = {Astronomy \& Astrophysics},
  volume = {618},
  eprint = {1807.08301},
  issn = {14320746},
  doi = {10.1051/0004-6361/201832777},
  abstract = {Context. Oscillation modes with a mixed character, as observed in evolved low-mass stars, are highly sensitive to the physical properties of the innermost regions. Measuring their properties is therefore extremely important to probe the core, but requires some care, due to the complexity of the mixed-mode pattern. Aims. The aim of this work is to provide a consistent description of the mixed-mode pattern of low-mass stars, based on the asymptotic expansion. We also study the variation of the gravity offset {$\epsilon$}g with stellar evolution. Methods. We revisit previous works about mixed modes in red giants and empirically test how period spacings, rotational splittings, mixed-mode widths, and heights can be estimated in a consistent view, based on the properties of the mode inertia ratios. Results. From the asymptotic fit of the mixed-mode pattern of a large set of red giants at various evolutionary stages, we derive unbiased and precise asymptotic parameters. As the asymptotic expansion of gravity modes is verified with a precision close to the frequency resolution for stars on the red giant branch (10-4 in relative values), we can derive accurate values of the asymptotic parameters. We decipher the complex pattern in a rapidly rotating star, and explain how asymmetrical splittings can be inferred. We also revisit the stellar inclinations in two open clusters, NGC 6819 and NGC 6791: our results show that the stellar inclinations in these clusters do not have privileged orientation in the sky. The variation of the asymptotic gravity offset with stellar evolution is investigated in detail. We also derive generic properties that explain under which conditions mixed modes can be observed.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RGEHL5UL/Mosser et al. - 2018.pdf}
}

@article{Mosser2019,
  title = {Astronomy {{Astrophysics Seismic}} Performance},
  author = {Mosser, B and Michel, E and Samadi, R and Miglio, A and Davies, G R and Girardi, L and Goupil, M J},
  year = {2019},
  journal = {A\&A},
  volume = {622},
  pages = {76},
  doi = {10.1051/0004-6361/201834607},
  urldate = {2022-01-26},
  abstract = {Context. Asteroseismology is a unique tool that can be used to study the interior of stars and hence deliver unique information for the studiy of stellar physics, stellar evolution, and Galactic archaeology. Aims. We aim to develop a simple model of the information content of asteroseismology and to characterize the ability and precision with which fundamental properties of stars can be estimated for different space missions. Methods. We defined and calibrated metrics of the seismic performance. The metrics, expressed by a seismic index E defined by simple scaling relations, are calculated for an ensemble of stars. We studied the relations between the properties of mission observations, fundamental stellar properties, and the performance index. We also defined thresholds for asteroseismic detection and measurement of different stellar properties. Results. We find two regimes of asteroseismic performance: the first where the signal strength is dominated by stellar properties and not by observational noise; and the second where observational properties dominate. Typically, for evolved stars, stellar properties provide the dominant terms in estimating the information content, while main sequence stars fall in the regime where the observational properties, especially stellar magnitude, dominate. We estimate scaling relations to predict E with an intrinsic scatter of around 21\%. Incidentally, the metrics allow us to distinguish stars burning either hydrogen or helium. Conclusions. Our predictions will help identify the nature of the cohort of existing and future asteroseismic observations. In addition, the predicted performance for PLATO will help define optimal observing strategies for defined scientific goals.},
  keywords = {evolution,interiors-stars,notion,notion-database,oscillations-stars,stars}
}

@article{Moya2004a,
  title = {Non-Adiabatic Theoretical Observables in {$\delta$} {{Scuti}} Stars},
  author = {Moya, A. and Garrido, R. and Dupret, M. A.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {414},
  number = {3},
  pages = {1081--1090},
  issn = {00046361},
  doi = {10.1051/0004-6361:20034037},
  abstract = {Phase differences and amplitude ratios at different colour photometric bands are currently being used to discriminate pulsation modes to facilitate mode identification of {$\kappa$}-driven non-radial pulsating stars. In addition to physical inputs (e.g., mass, Teff, etc.), these quantities depend on the non-adiabatic treatment of the atmosphere. This paper presents theoretical results concerning {$\delta$} Scuti pulsating stars. The envelope of each of these stellar structures possesses a convection zone whose development is determined by various factors. An interacting pulsation-atmosphere physical treatment is introduced which supplies two basic non-adiabatic physical quantities: the relative effective temperature variation and the phase lag {$\varphi$}T, defined as the angle between effective temperature variation and radial displacement. These quantities can be used to derive the phase differences and amplitude ratios. Numerical values for these quantities depend critically on the {$\alpha$} MLT parameter used to calculate the convection in the envelope. The dependence on {$\alpha$} was analyzed and it was found that the use of colour observations may be of considerable importance in testing the MLT. Finally, examples are given of how {$\alpha$} introduces uncertainties in the theoretical predictions regarding phases and amplitudes of photometric variations in {$\delta$} Scuti pulsating stars.},
  keywords = {notion,notion-database,Stars: atmosphere,Stars: oscillations,Stars: variables: {$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/FWVLSA22/Moya, Garrido, Dupret - 2004.pdf}
}

@article{Moya2008,
  title = {Inter-Comparison of the g-, f- and p-Modes Calculated Using Different Oscillation Codes for a given Stellar Model},
  author = {Moya, A. and {Christensen-Dalsgaard}, J. and Charpinet, S. and Lebreton, Y. and Miglio, A. and Montalb{\'a}n, J. and Monteiro, M. J.P.F.G. and Provost, J. and Roxburgh, I. W. and Scuflaire, R. and Su{\'a}rez, J. C. and Suran, M.},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  eprint = {0711.2587},
  pages = {231--249},
  issn = {1572946X},
  doi = {10.1007/s10509-007-9717-z},
  abstract = {In order to make asteroseismology a powerful tool to explore stellar interiors, different numerical codes should give the same oscillation frequencies for the same input physics. Any differences found when comparing the numerical values of the eigenfrequencies will be an important piece of information regarding the numerical structure of the code. The ESTA group was created to analyze the non-physical sources of these differences. The work presented in this report is a part of Task 2 of the ESTA group. Basically the work is devoted to test, compare and, if needed, optimize the seismic codes used to calculate the eigenfrequencies to be finally compared with observations. The first step in this comparison is presented here. The oscillation codes of nine research groups in the field have been used in this study. The same physics has been imposed for all the codes in order to isolate the non-physical dependence of any possible difference. Two equilibrium models with different grids, 2172 and 4042 mesh points, have been used, and the latter model includes an explicit modelling of semiconvection just outside the convective core. Comparing the results for these two models illustrates the effect of the number of mesh points and their distribution in particularly critical parts of the model, such as the steep composition gradient outside the convective core. A comprehensive study of the frequency differences found for the different codes is given as well. These differences are mainly due to the use of different numerical integration schemes. The number of mesh points and their distribution are crucial for interpreting the results. The use of a second-order integration scheme plus a Richardson extrapolation provides similar results to a fourth-order integration scheme. The proper numerical description of the Brunt-V\"ais\"al\"a frequency in the equilibrium model is also critical for some modes. This influence depends on the set of the eigenfunctions used for the solution of the differential equations. An unexpected result of this study is the high sensitivity of the frequency differences to the inconsistent use of values of the gravitational constant (G) in the oscillation codes, within the range of the experimentally determined ones, which differ from the value used to compute the equilibrium model. This effect can provide differences for a given equilibrium model substantially larger than those resulting from the use of different codes or numerical techniques; the actual differences between the values of G used by the different codes account for much of the frequency differences found here. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Numerical solution,Stars,Stellar oscillations},
  file = {/Users/lbugnet/Zotero/storage/5EVWPJER/Moya et al. - 2008.pdf}
}

@article{Moya2008b,
  title = {Granada Oscillation Code ({{GraCo}})},
  author = {Moya, A. and Garrido, R.},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  pages = {129--133},
  issn = {0004640X},
  doi = {10.1007/s10509-007-9694-2},
  abstract = {Granada oscillation code (GraCo) is a software constructed to compute adiabatic and non-adiabatic oscillation eigenfunctions and eigenvalues. The adiabatic version gives the standard numerical resolution, and also the Richardson extrapolation, different sets of eigenfunctions, different outer mechanical boundary conditions or different integration variables. The non-adiabatic version can include the atmosphere-pulsation interaction. The code has been used for intensive studies of {$\delta$} Scuti, {$\gamma$} Doradus, {$\beta$} Ceph., SdO and, SdB stars. The non adiabatic observables "phase-lag" (the phase between the effective temperature variations and the radial displacement) and {$\delta$}Teff/Teff(relative surface temperature variation) can help to the modal identification. These quantities together with the energy balance ("growth rate") provide useful additional information to the adiabatic resolution (eigenfrequencies and eigenfunctions). \textcopyright{} 2007 Springer Science+Business Media B.V.},
  keywords = {notion,notion-database,Numerical resolution,Stars,Stellar oscillations},
  file = {/Users/lbugnet/Zotero/storage/6QRYWHY6/Moya, Garrido - 2008.pdf}
}

@article{Moya2010a,
  title = {The Planetary System Host {{HR}} 8799: {{On}} Its {$\lambda$} {{Bootis}} Nature},
  author = {Moya, A. and Amado, P. J. and Barrado, D. and Hern{\'a}ndez, A. Garc{\'i}a and Aberasturi, M. and Montesinos, B. and Aceituno, F.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {406},
  number = {1},
  pages = {566--575},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2010.16699.x},
  abstract = {HR 8799 is a {$\lambda$} Bootis, {$\gamma$} Doradus star hosting a planetary system and a debris disc with two rings. This makes this system a very interesting target for asteroseismic studies. This work is devoted to the determination of the internal metallicity of this star, linked with its {$\lambda$} Bootis nature (i.e. solar surface abundances of light elements and subsolar surface abundances of heavy elements), taking advantage of its {$\gamma$} Doradus pulsations. This is the most accurate way of obtaining this information, and this is the first time that such a study is performed for a planetary-system-host star. We have used the equilibrium code cesam and the non-adiabatic pulsational code graco. We have applied the frequency ratio method (FRM) and the time-dependent convection theory to estimate the mode identification, the Brunt-Va\"is\"al\"a frequency integral and the mode instability, making the selection of the models possible. When the non-seismological constraints (i.e. HR 8799's position in the Hertzsprung-Russell diagram) are used, the solar abundance models are discarded. This result contradicts one of the main hypotheses for explaining the {$\lambda$} Bootis nature, namely the accretion/diffusion of gas by a star with solar abundance. Therefore, according to this result, a revision of this hypothesis is needed. The inclusion of accurate internal chemical mixing processes seems to be necessary to explain the peculiar abundances observed in the surface of stars with internal subsolar metallicities. The use of the asteroseismological constraints, like those provided by the FRM or the instability analysis, provides a very accurate determination of the physical characteristics of HR 8799. However, the dependence of the results on the inclination angle i still remains. The determination of this angle, more accurate multicolour photometric observations and high-resolution spectroscopy can definitively fix the mass and metallicity of this star. \textcopyright{} 2010 The Authors. Journal compilation \textcopyright{} 2010 RAS.},
  keywords = {notion,notion-database,Planetary systems,Stars: abundances,Stars: chemically peculiar,Stars: fundamental parameters,Stars: individual: HR8799,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/3A5HSRAS/Moya et al. - 2010.pdf}
}

@article{Moya2011a,
  title = {Sensitivity of the {{Calculated}} G-{{Mode Frequencies}} to {{Pulsation Codes}} and Their {{Parameters}}},
  author = {Moya, A. and Mathur, S. and Garc{\'i}a, R. A.},
  year = {2011},
  journal = {Solar Physics},
  volume = {268},
  number = {2},
  pages = {245--254},
  issn = {00380938},
  doi = {10.1007/s11207-010-9551-2},
  abstract = {From the recent work of the Evolution and Seismic Tools Activity (ESTA: Monteiro et al., ESA, SP-1306, 363 - 371, 2006 and Lebreton et al., Astrophys. Space Sci. 316, 1 - 12, 2008), whose Task 2 is devoted to comparing pulsational frequencies computed using most of the pulsational codes available in the asteroseismic community, the dependence of the theoretical frequencies on non-physical choices is now quite well specified. To ensure that the accuracy of the computed frequencies is of the same order of magnitude or better than the observational errors, some requirements in the equilibrium models and the numerical resolutions of the pulsational equations must be followed. In particular, we have verified the numerical accuracy obtained with the Saclay seismic model, which is used to study the solar g-mode region (60 to 140 {$\mu$}Hz). We have compared the results coming from the Aarhus adiabatic pulsation code (ADIPLS), with the frequencies computed with the Granada Code (GraCo) taking into account several possible non-physical choices and the effect of using two different outer mechanical boundary conditions. We have concluded that the present equilibrium models and the use of the Richardson extrapolation ensure an accuracy of the order of 0.01 {$\mu$}Hz in the determination of the frequencies, which is quite enough for our purposes. \textcopyright{} 2010 Springer Science+Business Media B.V.},
  keywords = {{Helioseismology, modelling},{Interior, radiative zone, core},notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UXZREXVN/Moya, Mathur, García - 2011.pdf}
}

@article{Moyano2022,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum: {{V}}. {{Efficiency}} of the Transport on the Red Giant Branch and in the Red Clump},
  shorttitle = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum},
  author = {Moyano, F. D. and Eggenberger, P. and Meynet, G. and Gehan, C. and Mosser, B. and Buldgen, G. and Salmon, S. J. A. J.},
  year = {2022},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {663},
  pages = {A180},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202243389},
  urldate = {2023-09-22},
  abstract = {Methods. We computed stellar evolution models with rotation and model the transport of angular momentum by the action of a sole dominant diffusive process parameterised by an additional viscosity in the equation of angular momentum transport. We constrained the values of this viscosity to match the mean core rotation rates of red giants and their behaviour with mass and evolution using asteroseismic indicators along the red giant branch and in the red clump. Results. For red giants in the hydrogen-shell burning phase, the transport of angular momentum must be more efficient in more massive stars. The additional viscosity is found to vary by approximately two orders of magnitude in the mass range M {$\sim$} 1\textendash 2.5 M . As stars evolve along the red giant branch, the efficiency of the internal transport of angular momentum must increase for low-mass stars (M 2 M ) and remain approximately constant for slightly higher masses (2.0 M M 2.5 M ). In red clump stars, the additional viscosities must be an order of magnitude higher than in younger red giants of similar mass during the hydrogen-shell burning phase. Conclusions. In combination with previous efforts, we obtain a clear picture of how the physical processes acting in stellar interiors should redistribute angular momentum from the end of the main sequence until the core-helium burning phase for low- and intermediate-mass stars to satisfy the asteroseismic constraints.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/FX3A2MTF/Moyano et al. - 2022 - Asteroseismology of evolved stars to constrain the.pdf}
}

@article{Moyano2023,
  title = {Angular Momentum Transport by Magnetic Fields in Main-Sequence Stars with {{Gamma Doradus}} Pulsators},
  author = {Moyano, F. D. and Eggenberger, P. and Salmon, S. J. A. J. and Mombarg, J. S. G. and Ekstr{\"o}m, S.},
  year = {2023},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {677},
  pages = {A6},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202346548},
  urldate = {2023-10-14},
  abstract = {Context. Asteroseismic studies show that cores of post-main-sequence stars rotate more slowly than theoretically predicted by stellar models with purely hydrodynamical transport processes. Recent studies of main-sequence stars, particularly Gamma Doradus ({$\gamma$} Dor) stars, have revealed the internal rotation rates for hundreds of stars, offering a counterpart on the main sequence for studies of angular momentum transport. Aims: We investigate whether such a disagreement between observed and predicted internal rotation rates is present in main-sequence stars by studying angular momentum transport in {$\gamma$} Dor stars. Furthermore, we test whether models of rotating stars with internal magnetic fields can reproduce their rotational properties. Methods: We computed rotating models with the Geneva stellar evolution code taking into account meridional circulation and shear instability. We also computed models with internal magnetic fields using a general formalism for transport by the Tayler-Spruit dynamo. We then compared these models to observational constraints for {$\gamma$} Dor stars that we compiled from the literature, thus combining the core rotation rates, projected rotational velocities from spectroscopy, and constraints on their fundamental parameters. Results: We show that combining the different observational constraints available for {$\gamma$} Dor stars enable us to clearly distinguish the different scenarios for internal angular momentum transport. Stellar models with purely hydrodynamical processes are in disagreement with the data, whereas models with internal magnetic fields can reproduce both core and surface constraints simultaneously. Conclusions: Similarly to results obtained for subgiant and red giant stars, angular momentum transport in radiative regions of {$\gamma$} Dor stars is highly efficient, in good agreement with predictions of models with internal magnetic fields.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,methods: numerical,stars: evolution,stars: interiors,stars: rotation,stars: variables: S Doradus},
  annotation = {ADS Bibcode: 2023A\&A...677A...6M},
  file = {/Users/lbugnet/Zotero/storage/PRSKQTK2/Moyano et al. - 2023 - Angular momentum transport by magnetic fields in m.pdf}
}

@misc{moyanoAngularMomentumTransport2023,
  title = {Angular Momentum Transport by Magnetic Fields in Main Sequence Stars with {{Gamma Doradus}} Pulsators},
  author = {Moyano, F. D. and Eggenberger, P. and Salmon, S. J. A. J. and Mombarg, J. S. G. and Ekstr{\"o}m, S.},
  year = {2023},
  month = apr,
  number = {arXiv:2304.00674},
  eprint = {2304.00674},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-04-04},
  abstract = {Context. Asteroseismic studies showed that cores of post main-sequence stars rotate slower than theoretically predicted by stellar models with purely hydrodynamical transport processes. Recent studies on main sequence stars, particularly Gamma Doradus (\$\textbackslash gamma\$ Dor) stars, revealed their internal rotation rate for hundreds of stars, offering a counterpart on the main sequence for studies of angular momentum transport. Aims. We investigate whether such a disagreement between observed and predicted internal rotation rates is present in main sequence stars by studying angular momentum transport in \$\textbackslash gamma\$ Dor stars. Furthermore, we test whether models of rotating stars with internal magnetic fields can reproduce their rotational properties. Methods. We compute rotating models with the Geneva stellar evolution code taking into account meridional circulation and the shear instability. We also compute models with internal magnetic fields using a general formalism for transport by the Tayler-Spruit dynamo. We then compare these models to observational constraints for \$\textbackslash gamma\$ Dor stars that we compiled from the literature, combining so the core rotation rates, projected rotational velocities from spectroscopy, and constraints on their fundamental parameters. Results. We show that combining the different observational constraints available for \$\textbackslash gamma\$ Dor stars enable to clearly distinguish the different scenarios for internal angular momentum transport. Stellar models with purely hydrodynamical processes are in disagreement with the data whereas models with internal magnetic fields can reproduce both core and surface constraints simultaneously. Conclusions. Similarly to results obtained for subgiant and red giant stars, angular momentum transport in radiative regions of \$\textbackslash gamma\$ Dor stars is highly efficient, in good agreement with predictions of models with internal magnetic fields.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/HRQRLGT7/Moyano et al. - 2023 - Angular momentum transport by magnetic fields in m.pdf;/Users/lbugnet/Zotero/storage/BXD9XYUG/2304.html}
}

@article{Muller1920,
  title = {Geschichte Und {{Literatur}} Des {{Lichtwechsels}}, Der Bis {{Ende}} 1915 Als Sicher Ver\"anderlich Anerkannten {{Sterne}}, Nebst Einem {{Katalog}} Der {{Elements}} Ihres {{Lichtwechsels}}},
  author = {M{\"u}ller, G. and Hartwig, E.},
  year = {1920},
  journal = {gllv},
  urldate = {2020-03-07},
  keywords = {notion,notion-database,Variable stars: catalogs}
}

@article{Muller1992,
  title = {Evolution and Advection of Solar Mesogranulation},
  author = {Muller, Richard and Auffret, Herv{\'e} and Roudier, Thierry and Vigneau, Jean and Simon, George W. and Frank, Zoe and Shine, Richard A. and Title, Alan M.},
  year = {1992},
  journal = {Nature},
  volume = {356},
  number = {6367},
  pages = {322--325},
  issn = {00280836},
  doi = {10.1038/356322a0},
  urldate = {2020-03-14},
  abstract = {GRANULAR structure on the Sun's surface, with a typical scale of 1-2 Mm, has been known since 1800, and one hundred years ago, with the first observations by spectroheliograph1,2, a mesh-like bright network was found with a characteristic scale of 30 Mm (40{${''}$}). This pattern was found, thirty years ago, to be coincident with close-packed convective cells ('supergranulation') revealed by Doppler observations3-5 to be nestling inside the bright network. More recently6,7 an intermediate 'mesogranular' structure was found, with a characteristic scale of 3-10 Mm. We have obtained a three-hour sequence of observations at the Pic du Midi observatory which shows the evolution of mesogranules from appearance to disappearance with unprecedented clarity. We see that the supergranules, which are known to carry along (advect) the granules with their convective motion, also advect the mesogranules to their boundaries. This process controls the evolution and disappearance of mesogranules. \textcopyright{} 1992 Nature Publishing Group.},
  keywords = {Advection,Astrophysics,Convection Cells,notion,notion-database,Solar Granulation,Solar Magnetic Field,Solar Physics}
}

@article{Murgas2013,
  title = {Stellar Activity as a Tracer of Moving Groups},
  author = {Murgas, F. and Jenkins, J. S. and Rojo, P. and A Jones, H. R. and Pinfield, D. J.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {552},
  pages = {1--8},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219483},
  abstract = {We present the results of a study of the stellar activity in the solar neighborhood using complete kinematics (galactocentric velocities U, V, W) and the chromospheric activity index log R'HK. We analyzed the average activity level near the centers of known moving groups using a sample of 2529 stars and found that the stars near these associations tend to be more active than field stars. This supports the hypothesis that these structures, or at least a significant part of them, are composed of kinematically bound, young stars. We confirmed our results by using GALaxy Evolution EXplorer (GALEX) UV data and kinematics taken from the Geneva-Copenhagen Survey for the stars in the sample. Finally, we present a compiled catalog with kinematics and activities for 2529 stars and a list of potential moving group members selected based on their stellar activity level. \textcopyright{} ESO, 2013.},
  keywords = {notion,notion-database,Solar neighborhood,Stars: activity,Stars: kinematics and dynamics,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/99DYJXSN/Murgas et al. - 2013.pdf}
}

@misc{Murphy,
  title = {Pulsating Stars in Binary Systems: A Review},
  author = {Murphy, Simon J},
  eprint = {1811.12659v2},
  urldate = {2020-08-31},
  abstract = {Binary systems anchor many of the fundamental relations relied upon in asteroseismology. Masses and radii are rarely constrained better than when measured via orbital dynamics and eclipse depths. Pulsating binaries have much to ooer. They are clocks, moving in space, that encode orbital motion in the Doppler-shifted pulsation frequencies. They ooer twice the opportunity to obtain an asteroseismic age, which is then applicable to both stars. They enable comparative asteroseismology-the study of two stars by their pulsation properties, whose only fundamental diierences are the mass and rotation rates with which they were born. In eccentric binaries, oscillations can be excited tidally, informing our knowledge of tidal dissipation and resonant frequency locking. Eclipsing binaries ooer benchmarks against which the asteroseismic scaling relations can be tested. We review these themes in light of both observational and theoretical developments recently made possible by space-based photometry.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CMVJBN22/full-text.pdf}
}

@article{Murphy2012,
  title = {An Examination of Some Characteristics of {{Kepler}} Short- and Long-Cadence Data},
  author = {Murphy, Simon J.},
  year = {2012},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {422},
  number = {1},
  eprint = {1201.6184},
  pages = {665--671},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.20644.x},
  abstract = {A close comparison of Kepler short- and long-cadence data released prior to 2011November1 has shown some subtle differences that make the short-cadence data superior to their long-cadence counterparts. The inevitable results of a faster sampling rate are present: the short-cadence data provide greater time resolution for short-lived events like flares, and have a much higher Nyquist frequency than the long-cadence data; however, they also contain fewer high-amplitude peaks at low frequency and allow a more precise determination of pulsation frequencies, amplitudes and phases. The latter observation indicates that Kepler data are not normally distributed. Moreover, a close inspection of the Pre-search Data Conditioned long-cadence data shows residuals that have increased noise on time-scales important to asteroseismology, but unimportant to planet searches. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,Methods: observational,notion,notion-database,Stars: activity,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/E8CQVCMX/Murphy - 2012.pdf}
}

@article{Murphy2013,
  title = {Super-{{Nyquist}} Asteroseismology with the {{Kepler}} Space Telescope},
  author = {Murphy, Simon J. and Shibahashi, Hiromoto and Kurtz, Donald W.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {430},
  number = {4},
  eprint = {1212.5603},
  pages = {2986--2998},
  issn = {00358711},
  doi = {10.1093/mnras/stt105},
  abstract = {Barycentric corrections made to the timing ofKepler observations, necessitated by variations in light arrival time at the satellite, break the regular time-sampling of the data - the time stamps are periodically modulated. A consequence is that Nyquist aliases are split into multiplets that can be identified by their shape. Real pulsation frequencies are distinguishable from these aliases and their frequencies are completely recoverable, even in the super-Nyquist regime, i.e. when the sampling interval is longer than half the pulsation period. We provide an analytical derivation of the phenomenon, alongside demonstrations with simulated and real Kepler data for {$\delta$} Sct, roAp and sdBV stars. For Kepler data sets spanning more than one Kepler orbital period (372.5 d), there are no Nyquist ambiguities on the determination of pulsation frequencies, which are the fundamental data of asteroseismology. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: oscillations,Stars: variables: general,stars: variables: {$\delta$} scuti},
  file = {/Users/lbugnet/Zotero/storage/MWE6HM5U/Murphy, Shibahashi, Kurtz - 2013.pdf}
}

@article{Murphy2014,
  title = {Finding Binaries among {{Kepler}} Pulsating Stars from Phase Modulation of Their Pulsations},
  author = {Murphy, Simon J. and Bedding, Timothy R. and Shibahashi, Hiromoto and Kurtz, Donald W. and Kjeldsen, Hans},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {441},
  number = {3},
  eprint = {1404.5649},
  pages = {2515--2527},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stu765},
  urldate = {2020-07-08},
  abstract = {We present a method for finding binaries among pulsating stars that were observed by the Kepler Mission. We use entire 4 yr light curves to accurately measure the frequencies of the strongest pulsation modes, and then track the pulsation phases at those frequencies in 10-d segments. This produces a series of time-delay measurements in which binarity is apparent as a periodic modulation whose amplitude gives the projected light travel time across the orbit. Fourier analysis of this time-delay curve provides the parameters of the orbit, including the period, eccentricity, angle of ascending node, and time of periastron passage. Differentiating the time-delay curve yields the full radial-velocity curve directly from the Kepler photometry, without the need for spectroscopy. We showexamples with {$\delta$} scuti stars having large numbers of pulsation modes, including one system in which both components of the binary are pulsating. The method is straightforward to automate, thus radial velocity curves can be derived for hundreds of non-eclipsing binary stars from Kepler photometry alone. \textcopyright{} 2014 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Binaries: General,notion,notion-database,Stars: Oscillations,Techniques:radial velocities},
  file = {/Users/lbugnet/Zotero/storage/BF47MZWT/full-text.pdf}
}

@article{Murphy2016,
  title = {Near-Uniform Internal Rotation of the Main-Sequence {$\gamma$} {{Doradus}} Pulsator {{KIC}} 7661054},
  author = {Murphy, Simon J and Fossati, Luca and Bedding, Timothy R and Saio, Hideyuki and Kurtz, Donald W and Grassitelli, Luca and Wang, Edric S},
  year = {2016},
  journal = {MNRAS},
  volume = {459},
  pages = {1201--1212},
  doi = {10.1093/mnras/stw705},
  urldate = {2020-03-24},
  abstract = {We used Kepler photometry to determine the internal rotation rate of KIC 7661054, a chemically normal {$\gamma$} Dor star on the main sequence at spectral type F2.5 V. The core rotation period of 27.25 {$\pm$} 0.06 d is obtained from the rotational splittings of a series of dipole g modes. The surface rotation period is calculated from a spectroscopic projected rotation velocity and a stellar radius computed from models. Literature data, obtained without inclusion of macrotur-bulence as a line-broadening mechanism, imply that the surface rotates much more quickly than the core, while our detailed analysis suggests that the surface may rotate slightly more quickly than the core and that the rotation profile is uniform within the 1{$\sigma$} uncertainties. We discuss the pitfalls associated with the determination of surface rotation rates of slow rotators from spectroscopy in the absence of asteroseismic constraints. A broad signal is observed at low frequency, which we show cannot be attributed to rotation, contrary to previous suggestions concerning the origin of such signals.},
  keywords = {asteroseismology-techniques,individual,KIC 7660154-stars,notion,notion-database,oscillations-stars,rotation,spectroscopic-stars}
}

@article{Murphy2018,
  title = {Finding Binaries from Phase Modulation of Pulsating Stars with {{Kepler}}: {{V}}. {{Orbital}} Parameters, with Eccentricity and Mass-Ratio Distributions of 341 New Binaries},
  author = {Murphy, Simon J. and Moe, Maxwell and Kurtz, Donald W. and Bedding, Timothy R. and Shibahashi, Hiromoto and Boffin, Henri M.J.},
  year = {2018},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {474},
  number = {4},
  eprint = {1712.00022},
  pages = {4322--4346},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stx3049},
  urldate = {2020-07-08},
  abstract = {The orbital parameters of binaries at intermediate periods (102-103 d) are difficult to measure with conventional methods and are very incomplete. We have undertaken a new survey, applying our pulsation timing method to Kepler light curves of 2224 main-sequence A/F stars and found 341 non-eclipsing binaries. We calculate the orbital parameters for 317 PB1 systems (single-pulsator binaries) and 24 PB2s (double-pulsators), tripling the number of intermediate-mass binaries with full orbital solutions. The method reaches down to small mass ratios q {$\approx$} 0.02 and yields a highly homogeneous sample. We parametrize the massratio distribution using both inversion and Markov-Chain Monte Carlo forward-modelling techniques, and find it to be skewed towards low-mass companions, peaking at q {$\approx$} 0.2. While solar-type primaries exhibit a brown dwarf desert across short and intermediate periods, we find a small but statistically significant (2.6{$\sigma$}) population of extreme-mass-ratio companions (q {$<$} 0.1) to our intermediate-mass primaries. Across periods of 100-1500 d and at q {$>$} 0.1, we measure the binary fraction of current A/F primaries to be 15.4 percent {$\pm$} 1.4 per cent, though we find that a large fraction of the companions (21 percent {$\pm$} 6 per cent) are white dwarfs in post-mass-transfer systems with primaries that are now blue stragglers, some of which are the progenitors of Type Ia supernovae, barium stars, symbiotics, and related phenomena. Excluding these white dwarfs, we determine the binary fraction of original A/F primaries to be 13.9 percent {$\pm$} 2.1 per cent over the same parameter space. Combining our measurements with those in the literature, we find the binary fraction across these periods is a constant 5 per cent for primaries M1 {$<$} 0.8M{$\odot$}, but then increases linearly with log M1, demonstrating that natal discs around more massive protostars M1 {$\greaterequivlnt$} 1M{$\odot$} become increasingly more prone to fragmentation. Finally, we find the eccentricity distribution of the main-sequence pairs to be much less eccentric than the thermal distribution.},
  archiveprefix = {arxiv},
  keywords = {Binaries: general,Blue stragglers,notion,notion-database,Stars: formation,Stars: oscillations,Stars: statistics,Stars: variables: {$\delta$}Scuti}
}

@article{Murphy2019,
  title = {Gaia-Derived Luminosities of {{Kepler A}}/{{F}} Stars and the Pulsator Fraction across the {$\delta$} {{Scuti}} Instability Strip},
  author = {Murphy, Simon J. and Hey, Daniel and Van Reeth, Timothy and Bedding, Timothy R.},
  year = {2019},
  month = feb,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {485},
  number = {2},
  eprint = {1903.00015},
  pages = {2380--2400},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stz590},
  urldate = {2020-04-13},
  abstract = {We study the fraction of stars in and around the {$\delta$} Scuti instability strip that are pulsating, using Gaia DR2 parallaxes to derive precise luminosities. We classify a sample of over 15 000 Kepler A and F stars into {$\delta$} Sct and non-{$\delta$} Sct stars, paying close attention to variability that could have other origins. We find that 18 per cent of the {$\delta$} Sct stars have their dominant frequency above the Kepler long-cadence Nyquist frequency (periods {$<$} 1 h), and 30 per cent have some super-Nyquist variability. We analyse the pulsator fraction as a function of effective temperature and luminosity, finding that many stars in the {$\delta$} Sct instability strip do not pulsate. The pulsator fraction peaks at just over 70 per cent in the middle of the instability strip. The results are insensitive to the amplitude threshold used to identify the pulsators. We define a new empirical instability strip based on the observed pulsator fraction that is systematically hotter than theoretical strips currently in use. The stellar temperatures, luminosities, and pulsation classifications are provided in an online catalogue.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Hertzsprung-Russell and colour-magnitude diagrams,notion,notion-database,Parallaxes,Stars: oscillations,Stars: variables: {$\delta$} Scuti}
}

@article{Murphy2020,
  title = {On the First {$\delta$} {{Sct-roAp}} Hybrid Pulsator and the Stability of p and g Modes in Chemically Peculiar {{A}}/{{F}} Stars},
  author = {Murphy, Simon J. and Saio, Hideyuki and {Takada-Hidai}, Masahide and Kurtz, Donald W. and Shibahashi, Hiromoto and Takata, Masao and Hey, Daniel R.},
  year = {2020},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {498},
  pages = {4272--4286},
  issn = {0035-8711},
  doi = {10.1093/mnras/staa2667},
  urldate = {2023-10-17},
  abstract = {Strong magnetic fields in chemically peculiar A-type (Ap) stars typically suppress low-overtone pressure modes (p modes) but allow high-overtone p modes to be driven. KIC 11296437 is the first star to show both. We obtained and analysed a Subaru spectrum, from which we show that KIC 11296437 has abundances similar to other magnetic Ap stars, and we estimate a mean magnetic field modulus of 2.8 {$\pm$} 0.5 kG. The same spectrum rules out a double-lined spectroscopic binary, and we use other techniques to rule out binarity over a wide parameter space, so the two pulsation types originate in one {$\delta$} Sct-roAp hybrid pulsator. We construct stellar models depleted in helium and demonstrate that helium settling is second to magnetic damping in suppressing low-overtone p modes in Ap stars. We compute the magnetic damping effect for selected p and g modes, and find that modes with frequencies similar to the fundamental mode are driven for polar field strengths {$\lessequivlnt$}4 kG, while other low-overtone p modes are driven for polar field strengths up to {$\sim$}1.5 kG. We find that the high-order g modes commonly observed in {$\gamma$} Dor stars are heavily damped by polar fields stronger than 1-4 kG, with the damping being stronger for higher radial orders. We therefore explain the observation that no magnetic Ap stars have been observed as {$\gamma$} Dor stars. We use our helium-depleted models to calculate the {$\delta$} Sct instability strip for metallic-lined A (Am) stars, and find that driving from a Rosseland mean opacity bump at {$\sim$}5 \texttimes{} 104 K caused by the discontinuous H-ionization edge in bound-free opacity explains the observation of {$\delta$} Sct pulsations in Am stars.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: chemically peculiar,stars: interiors,stars: magnetic field,stars: oscillations,stars: variables: {$\delta$} scuti},
  annotation = {ADS Bibcode: 2020MNRAS.498.4272M},
  file = {/Users/lbugnet/Zotero/storage/GEZX9SBU/Murphy et al. - 2020 - On the first δ Sct-roAp hybrid pulsator and the st.pdf}
}

@article{Mursula2003a,
  title = {Mid-Term Quasi-Periodicities in Geomagnetic Activity during the Last 15 Solar Cycles: {{Connection}} to Solar Dynamo Strength},
  author = {Mursula, K. and Zieger, B. and Vilppola, J. H.},
  year = {2003},
  journal = {Solar Physics},
  volume = {212},
  number = {1},
  pages = {201--207},
  issn = {00380938},
  doi = {10.1023/A:1022980029618},
  abstract = {Several recent studies have reported quasi-periodicities with a period between 1 and 2 years (to be called here 'mid-term quasi-periodicities') in various heliospheric parameters, like solar wind speed, interplanetary magnetic field, cosmic rays, and geomagnetic activity. Here we study their long-term occurrence in geomagnetic activity using an extended aa index which covers the last 15 solar cycles. We confirm their intermittent occurrence and the alternation of their dominant period between a slightly shorter period of about 1.2-1.4 years and a slightly longer period of about 1.5-1.7 years. We find that the mid-term quasi-periodicities were strong during two intervals of high solar activity: in the mid-19th century and since 1930. Instead, contrary to earlier studies, we find that they were consistently weak during low solar activity from 1860s to 1920s. This implies a long-term connection between the amplitude of mid-term quasi-periodicities and the solar dynamo strength. Since the rotation speed at the bottom of the solar convection layer (tachocline) has recently been found to vary at a mid-term periodicity, this suggests that the stronger the solar dynamo is, the more variable the rotation rate of the tachocline is. We also note that the disappearance of mid-term periodicities may be used as a precursor for long intervals of very weak solar activity, like great minima.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LW6INB3B/Mursula, Zieger, Vilppola - 2003.pdf}
}

@article{Nadege2015a,
  title = {Models of Red Giants in the {{CoRoT}} Asteroseismology Fields Combining Asteroseismic and Spectroscopic Constraints},
  author = {Nad{\`e}ge, Lagarde},
  year = {2015},
  journal = {Proceedings of the International Astronomical Union},
  volume = {11},
  number = {A29B},
  pages = {525--528},
  issn = {17439221},
  doi = {10.1017/S1743921316006049},
  abstract = {The availability of asteroseismic constraints for a large sample of red-giant stars from the CoRoT and Kepler missions paves the way for various statistical studies of the seismic properties of stellar populations. We use a detailed spectroscopic study of 19 CoRoT red-giant stars (Morel et al. 2014) to compare theoretical stellar evolution models to observations of the open cluster NGC 6633 and field stars. This study is already published in Lagarde et al. (2015)},
  keywords = {asteroseismology,notion,notion-database,stars: abundances,stars: evolution,stars: interiors,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/7SZPYC8B/Nadège - 2015.pdf}
}

@article{Nakamura2010,
  title = {Lunar Seismology: {{Current}} Status and Future Challenges},
  author = {Nakamura, Y.},
  year = {2010},
  journal = {DGG-Mitteilungen},
  volume = {3},
  pages = {4--13},
  keywords = {notion,notion-database}
}

@article{Natekin2013,
  title = {Gradient Boosting Machines, a Tutorial},
  author = {Natekin, Alexey and Knoll, Alois},
  year = {2013},
  month = dec,
  journal = {Frontiers in Neurorobotics},
  volume = {7},
  number = {DEC},
  pages = {21},
  publisher = {{Frontiers Research Foundation}},
  issn = {1662-5218},
  doi = {10.3389/fnbot.2013.00021},
  urldate = {2020-04-11},
  abstract = {Gradient boosting machines are a family of powerful machine-learning techniques that have shown considerable success in a wide range of practical applications. They are highly customizable to the particular needs of the application, like being learned with respect to different loss functions. This article gives a tutorial introduction into the methodology of gradient boosting methods with a strong focus on machine learning aspects of modeling. A theoretical information is complemented with descriptive examples and illustrations which cover all the stages of the gradient boosting model design. Considerations on handling the model complexity are discussed. Three practical examples of gradient boosting applications are presented and comprehensively analyzed. \textcopyright{} 2013 Natekin and Knoll.},
  keywords = {Boosting,Classification,Gradient boosting,Machine learning,notion,notion-database,Regression,Robotic control,Text classification},
  file = {/Users/lbugnet/Zotero/storage/TSYXBSS5/full-text.pdf}
}

@article{Neckel1994a,
  title = {Solar Limb Darkening 1986-1990 ({$\Lambda\lambda$}303 to 1099 Nm)},
  author = {Neckel, Heinz and Labs, Dietrich},
  year = {1994},
  journal = {Solar Physics},
  volume = {153},
  number = {1-2},
  pages = {91--114},
  issn = {00380938},
  doi = {10.1007/BF00712494},
  abstract = {The Sun's limb darkening was observed repeatedly between the 1986 minimum and the 1990 maximum of solar activity. Systematic variations, which could depend either on the momentary activity and/or the phase in the solar cycle, were not detectable, either at continuum wavelengths or in two broad-band spectral intervals. Completely irregular variations, which concern not only individual, successive scans (due to granulation, etc.), but also the daily and seasonal averages, are usually less than 1\%, but can reach occasionally 2\% or even more. Minor east-west asymmetries even in the seasonal means seem to be well established, mainly for {$\lambda$} {$<$} 400 nm. The final, mean limb-darkening coefficients agree basically with those published by Pierce and Slaughter (1977) and Pierce, Slaughter, and Weinberger (1977), but show a much lower scatter when plotted against wavelength. \textcopyright{} 1994 Kluwer Academic Publishers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/N5AQWCIA/Neckel, Labs - 1994.pdf}
}

@article{Neiner2012,
  title = {Seismic Modelling of the Late {{Be}} Stars {{HD}} 181231 and {{HD}} 175869 Observed with {{CoRoT}}: {{A}} Laboratory for Mixing Processes},
  author = {Neiner, C. and Mathis, S. and Saio, H. and Lovekin, C. and Eggenberger, P. and Lee, U.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {539},
  pages = {1--12},
  issn = {00046361},
  doi = {10.1051/0004-6361/201118151},
  abstract = {Context. HD 181231 and HD 175869 are two late rapidly rotating Be stars, which have been observed using high-precision photometry with the CoRoT satellite during about five consecutive months and 27 consecutive days, respectively. An analysis of their light curves, by Neiner and collaborators and Guti\'errez-Soto and collaborators respectively, showed that several independent pulsation g-modes are present in these stars. Fundamental parameters have also been determined by these authors using spectroscopy. Aims. We aim to model these results to infer seismic properties of HD 181231 and HD 175869, and constrain internal transport processes of rapidly rotating massive stars. Methods. We used an adiabatic (NRO) and a non-adiabatic (Tohoku) oscillation code that accounts for the combined action of Coriolis and centrifugal accelerations on stellar pulsations as needed for rapid rotator modelling. We coupled these codes with a 2D (ROTORC) stellar structure model to take the rotational deformation of the star into account. The action of transport processes was parametrised with the mixing parameter {$\alpha$} ov, which represents the "non-standard" extension of the convective core, and determined by matching observed pulsation frequencies assuming a single star evolution scenario. In a second step, we used (Geneva) evolution models to evaluate the contribution of the secular rotational transport and mixing processes in the radiative envelope. A Monte Carlo analysis of spectropolarimetric data was also performed to examine the role of a potential fossil magnetic field. Finally, based on state-of-the-art modelling of penetrative convection and internal waves, we unravelled their respective contribution to the needed "non-standard" mixing. Results. We find that extra mixing of {$\alpha$} ov = 0.3-0.35H p is needed in HD 181231 and HD 175869 to match the observed frequencies with those of prograde sectoral g-modes. We also detect the possible presence of r-modes. We investigated the respective contributions of several transport processes to this mixing: the hydrodynamical processes in particular the meridional circulation and shear-induced turbulence caused by the radiative envelope differential rotation, the possible magnetic field, the penetrative convection at the top of the convective core, and the transport by internal waves. Conclusions. We showed that the extension of the convective core needed to match observations and models may be explained by mixing induced by the penetrative movements at the bottom of the radiative envelope and by the secular hydrodynamical transport processes induced by the rotation in the envelope. We showed how asteroseismology opens a new door to probe transport processes in stellar interiors. \textcopyright{} 2012 ESO.},
  keywords = {Asteroseismology,notion,notion-database,{Stars: emission-line, Be},Stars: individual: HD 175869,Stars: individual: HD 181231,Stars: rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/C7W8EEIP/Neiner et al. - 2012.pdf}
}

@article{Neiner2015,
  title = {The Origin of Magnetic Fields in Hot Stars},
  author = {Neiner, Coralie and Mathis, St{\'e}phane and Alecian, Evelyne and Emeriau, Constance and Grunhut, Jason},
  year = {2015},
  journal = {Proceedings of the International Astronomical Union},
  volume = {10},
  eprint = {1502.00226},
  pages = {61--66},
  publisher = {{Cambridge University Press}},
  issn = {17439221},
  doi = {10.1017/S1743921315004524},
  urldate = {2022-01-20},
  abstract = {Observations of stable mainly dipolar magnetic fields at the surface of \textasciitilde 7\% of single hot stars indicate that these fields are of fossil origin, i.e. they descend from the seed field in the molecular clouds from which the stars were formed. The recent results confirm this theory. First, theoretical work and numerical simulations confirm that the properties of the observed fields correspond to those expected from fossil fields. They also showed that rapid rotation does not modify the surface dipolar magnetic configurations, but hinders the stability of fossil fields. This explains the lack of correlation between the magnetic field properties and stellar properties in massive stars. It may also explain the lack of detections of magnetic fields in Be stars, which rotate close to their break-up velocity. In addition, observations by the BinaMIcS collaboration of hot stars in binary systems show that the fraction of those hosting detectable magnetic fields is much smaller than for single hot stars. This could be related to results obtained in simulations of massive star formation, which show that the stronger the magnetic field in the original molecular cloud, the more difficult it is to fragment massive cores to form several stars. Therefore, more and more arguments support the fossil field theory.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: early-type,stars: formation,stars: magnetic fields,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/VN33QBV7/full-text.pdf}
}

@article{Neiner2017,
  title = {Discovery of Magnetic {{A}} Supergiants: {{The}} Descendants of Magnetic Main-Sequence {{B}} Stars},
  author = {Neiner, Coralie and Oksala, Mary E. and Georgy, Cyril and Przybilla, Norbert and Mathis, St{\'e}phane and Wade, Gregg and Kondrak, Matthias and Fossati, Luca and Blaz{\`e}re, Aurore and Buysschaert, Bram and Grunhut, Jason},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {471},
  number = {2},
  eprint = {1707.00560},
  pages = {1926--1935},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stx1549},
  urldate = {2020-11-29},
  abstract = {In the context of the high resolution, high signal-to-noise ratio, high sensitivity, spectropolarimetric survey BritePol, which complements observations by the BRITE constellation of nanosatellites for asteroseismology, we are looking for and measuring the magnetic field of all stars brighter than V = 4. In this paper, we present circularly polarized spectra obtained with HarpsPol at ESO in La Silla (Chile) and ESPaDOnS at CFHT (Hawaii) for three hot evolved stars: {$\mathscr{l}$} Car, HR 3890 and {$\in$} CMa. We detected a magnetic field in all three stars. Each star has been observed several times to confirm the magnetic detections and check for variability. The stellar parameters of the three objects were determined and their evolutionary status was ascertained employing evolution models computed with the Geneva code. {$\in$} CMa was already known and is confirmed to be magnetic, but our modelling indicates that it is located near the end of the main sequence, i.e. it is still in a core hydrogen burning phase. {$\mathscr{l}$} Car and HR 3890 are the first discoveries of magnetic hot supergiants located well after the end of the main sequence on the Hertzsprung-Russell diagram. These stars are probably the descendants of main-sequence magnetic massive stars. Their current field strength (a few G) is compatible with magnetic flux conservation during stellar evolution. These results provide observational constraints for the development of future evolutionary models of hot stars including a fossil magnetic field.},
  archiveprefix = {arxiv},
  keywords = {{$\in$} CMa,HR 3890,notion,notion-database,Stars: early-type,Stars: evolution,Stars: individual: {$\mathscr{l}$} Car,Stars: magnetic field}
}

@article{Neiner2017a,
  title = {Discovery of a Magnetic Field in the {$\delta$} {{Scuti F2m}} Star {$\rho$} {{Pup}}},
  author = {Neiner, C. and Wade, G. A. and Sikora, J.},
  year = {2017},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {468},
  pages = {L46-L49},
  issn = {0035-8711},
  doi = {10.1093/mnrasl/slx023},
  urldate = {2023-10-17},
  abstract = {{$\rho$} Pup is a {$\delta$} Scuti F2 pulsator, known to host a main radial mode as well as non-radial pulsations, with chemical peculiarities typical of evolved Am stars. We present a high-precision spectropolarimetric observations of this star, obtained with ESPaDOnS at the Canada-France-Hawaii Telescope in the frame of the BRITE spectropolarimetric survey. A magnetic field is clearly detected in {$\rho$} Pup, with a longitudinal field strength below 1 G. This makes {$\rho$} Pup the second known magnetic {$\delta$} Scuti discovered, after HD 188774, and a possible cool evolved counterpart of the recently discovered ultraweakly magnetic Am family.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: individual: {$\rho$} Pup,stars: magnetic field,stars: variables: {$\delta$} Scuti},
  annotation = {ADS Bibcode: 2017MNRAS.468L..46N},
  file = {/Users/lbugnet/Zotero/storage/BY4KCI76/Neiner et al. - 2017 - Discovery of a magnetic field in the δ Scuti F2m s.pdf}
}

@article{Neiner2020,
  title = {Astronomy {{Astrophysics Transport}} of Angular Momentum by Stochastically Excited Waves as an Explanation for the Outburst of the Rapidly Rotating {{Be}} Star {{HD49330}}},
  author = {Neiner, C and Lee, U and Mathis, S and Saio, H and Lovekin, C C and Augustson, K C},
  year = {2020},
  journal = {A\&A},
  volume = {644},
  pages = {9},
  doi = {10.1051/0004-6361/201935858},
  urldate = {2022-01-26},
  abstract = {Context. HD 49330 is an early Be star that underwent an outburst during its five-month observation with the CoRoT satellite. An analysis of its light curve revealed several independent p and g pulsation modes, in addition to showing that the amplitude of the modes is directly correlated with the outburst. Aims. We modelled the results obtained with CoRoT to understand the link between pulsational parameters and the outburst of this Be star. Methods. We modelled the flattening of the structure of the star due to rapid rotation in two ways: Chandrasekhar-Milne's expansion and 2D structure computed with ROTORC. We then modelled {$\kappa$}-driven pulsations. We also adapted the formalism of the excitation and amplitude of stochastically excited gravito-inertial modes to rapidly rotating stars, and we modelled those pulsations as well. Results. We find that while pulsation p modes are indeed excited by the {$\kappa$} mechanism, the observed g modes are, rather, a result of stochastic excitation. In contrast, g and r waves are stochastically excited in the convective core and transport angular momentum to the surface, increasing its rotation rate. This destabilises the external layers of the star, which then emits transient stochastically excited g waves. These transient waves produce most of the low-frequency signal detected in the CoRoT data and ignite the outburst. During this unstable phase, p modes disappear at the surface because their cavity is broken. Following the outburst and ejection of the surface layer, relaxation occurs, making the transient g waves disappear and p modes reappear. Conclusions. This work includes the first coherent model of stochastically excited gravito-inertial pulsation modes in a rapidly rotating Be star. It provides an explanation for the correlation between the variation in the amplitude of frequencies detected in the CoRoT data and the occurrence of an outburst. This scenario could apply to other pulsating Be stars, providing an explanation to the long-standing questions surrounding Be outbursts and disks.},
  keywords = {Be-stars,emission-line,HD49330,individual,notion,notion-database,oscillations-stars,rotation-stars,stars}
}

@article{Nelson2011,
  title = {Buoyant {{Magnetic Loops}} in a {{Global Dynamo Simulation}} of a {{Young Sun}}},
  author = {Nelson, Nicholas J. and Brown, Benjamin P. and Brun, Allan Sacha and Miesch, Mark S. and Toomre, Juri},
  year = {2011},
  month = aug,
  journal = {The Astrophysical Journal Letters},
  volume = {739},
  number = {2},
  eprint = {1108.4697},
  pages = {L38},
  doi = {10.1088/2041-8205/739/2/L38},
  urldate = {2020-07-06},
  abstract = {The current dynamo paradigm for the Sun and sun-like stars places the generation site for strong toroidal magnetic structures deep in the solar interior. Sunspots and star-spots on sun-like stars are believed to arise when sections of these magnetic structures become buoyantly unstable and rise from the deep interior to the photosphere. Here we present the first 3-D global magnetohydrodynamic (MHD) simulation in which turbulent convection, stratification, and rotation combine to yield a dynamo that self-consistently generates buoyant magnetic loops. We simulate stellar convection and dynamo action in a spherical shell with solar stratification, but rotating three times faster than the current solar rate. Strong wreaths of toroidal magnetic field are realized by dynamo action in the convection zone. By turning to a dynamic Smagorinsky model for subgrid-scale turbulence, we here attain considerably reduced diffusion in our simulation. This permits the regions of strongest magnetic field in these wreaths to rise toward the top of the convection zone via a combination of magnetic buoyancy instabilities and advection by convective giant cells. Such a global simulation yielding buoyant loops represents a significant step forward in combining numerical models of dynamo action and flux emergence.},
  archiveprefix = {arxiv},
  keywords = {activity-Sun,convection-magnetohydrodynamics (MHD)-stars,interior,interiors-stars,magnetic field-Sun,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8MQ8WHV8/full-text.pdf}
}

@article{Nelson2012,
  title = {Buoyant {{Magnetic Loops Generated}} by {{Global Convective Dynamo Action}}},
  author = {Nelson, Nicholas J. and Brown, Benjamin P. and Brun, A. Sacha and Miesch, Mark S. and Toomre, Juri},
  year = {2012},
  month = dec,
  journal = {Solar Physics},
  volume = {289},
  number = {2},
  eprint = {1212.5612},
  pages = {441--458},
  publisher = {{Kluwer Academic Publishers}},
  doi = {10.1007/s11207-012-0221-4},
  urldate = {2020-07-06},
  abstract = {Our global 3D simulations of convection and dynamo action in a Sun-like star reveal that persistent wreaths of strong magnetism can be built within the bulk of the convention zone. Here we examine the characteristics of buoyant magnetic structures that are self-consistently created by dynamo action and turbulent convective motions in a simulation with solar stratification but rotating at three times the current solar rate. These buoyant loops originate within sections of the magnetic wreaths in which turbulent flows amplify the fields to much larger values than is possible through laminar processes. These amplified portions can rise through the convective layer by a combination of magnetic buoyancy and advection by convective giant cells, forming buoyant loops. We measure statistical trends in the polarity, twist, and tilt of these loops. Loops are shown to preferentially arise in longitudinal patches somewhat reminiscent of active longitudes in the Sun, although broader in extent. We show that the strength of the axisymmetric toroidal field is not a good predictor of the production rate for buoyant loops or the amount of magnetic flux in the loops that are produced.},
  archiveprefix = {arxiv},
  keywords = {Convection zone,Flux emergence,Global dynamo,Magnetic buoyancy,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/J8VPZG8E/full-text.pdf}
}

@article{Nesis1993,
  title = {Dynamics of the Solar Granulation.},
  author = {Nesis, A. and Hanslmeier, A. and Hammer, R. and Komm, R. and Mattig, W. and Staiger, J. and Nesis, A. and Hanslmeier, A. and Hammer, R. and Komm, R. and Mattig, W. and Staiger, J.},
  year = {1993},
  journal = {A\&A},
  volume = {279},
  pages = {599--609},
  issn = {0004-6361},
  urldate = {2022-01-26},
  keywords = {Absorption Spectra,Astronomical Spectroscopy,Asymmetry,Cross Correlation,Flow Velocity,Line Spectra,notion,notion-database,Power Spectra,Scaling Laws,Solar Convection (Astronomy),Solar Granulation,Solar Physics,Solar Spectra,Spectral Energy Distribution,Spectrograms,Turbulent Flow,Velocity Distribution,Visible Spectrum},
  file = {/Users/lbugnet/Zotero/storage/PWUBCSAP/full-text.pdf}
}

@article{Ngeow2011,
  title = {Ground-{{Based BVRI Follow-Up Observations}} of the {{Cepheid V1154 Cyg}} in {{Kepler}}'s {{Field}}},
  author = {Ngeow, C. -C. and Szabo, R. and Szabados, L. and Henden, A. and Groenewegen, M. A. T. and Group, the Kepler Cepheid Working},
  year = {2011},
  month = nov,
  eprint = {1111.2101},
  urldate = {2020-03-27},
  abstract = {The almost un-interrupted observations from Kepler Space Telescope can be used to search for Earth-size and larger planets around other stars, as well as for stellar variability and asteroseismological study. However, the Kepler's observations are carried out with a single broad-band filter, and ground-based follow-up observations are needed to complement Kepler's light curves to fully characterize the properties of the target stars. Here we present ground-based optical (BVRI) followup observations of V1154 Cyg, the only Cepheid in the Kepler field of view, and deriving basic properties of this star.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZNJKMWIS/full-text.pdf}
}

@article{Nielsen2013,
  title = {Rotation Periods of 12 000 Main-Sequence {{Kepler}} Stars: {{Dependence}} on Stellar Spectral Type and Comparison with v Sin i Observations},
  author = {Nielsen, M. B. and Gizon, L. and Schunker, H. and Karoff, C.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {557},
  eprint = {1305.5721},
  pages = {10--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321912},
  abstract = {Aims. We aim to measure the starspot rotation periods of active stars in the Kepler field as a function of spectral type and to extend reliable rotation measurements from F-, G-, and K-type to M-type stars. Methods. Using the Lomb-Scargle periodogram we searched more than 150 000 stellar light curves for periodic brightness variations. We analyzed periods between 1 and 30 days in eight consecutive Kepler quarters, where 30 days is an estimated maximum for the validity of the PDC-MAP data correction pipeline. We selected stable rotation periods, i.e., periods that do not vary from the median by more than one day in at least six of the eight quarters. We averaged the periods for each stellar spectral class according to B-V color and compared the results to archival vsini data, using stellar radii estimates from the Kepler Input Catalog. Results. We report on the stable starspot rotation periods of 12 151 Kepler stars. We find good agreement between starspot velocities and vsini data for all F-, G-and early K-type stars. The 795 M-type stars in our sample have a median rotation period of 15.4 days. We find an excess of M-type stars with periods less than 7.5 days that are potentially fast-rotating and fully convective. Measuring photometric variability in multiple Kepler quarters appears to be a straightforward and reliable way to determine the rotation periods of a large sample of active stars, including late-type stars. \textcopyright{} 2013 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: late-type,Stars: rotation,Starspots},
  file = {/Users/lbugnet/Zotero/storage/437VMQX5/Nielsen et al. - 2013.pdf}
}

@article{Nielsen2014,
  title = {Rotational Splitting as a Function of Mode Frequency for Six {{Sun-like}} Stars},
  author = {Nielsen, M. B. and Gizon, L. and Schunker, H. and Schou, J.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {568},
  eprint = {1408.4307},
  pages = {1--4},
  issn = {14320746},
  doi = {10.1051/0004-6361/201424525},
  abstract = {Asteroseismology offers the prospect of constraining differential rotation in Sun-like stars. Here we have identified six high signal-to-noise main-sequence Sun-like stars in the Kepler field, which all have visible signs of rotational splitting of their p-mode frequencies. For each star, we extract the rotational frequency splitting and inclination angle from separate mode sets (adjacent modes with l = 2, 0, and 1) spanning the p-mode envelope. We use a Markov chain Monte Carlo method to obtain the best fit and errors associated with each parameter. We are able to make independent measurements of rotational splittings of {$\sim$}8 radial orders for each star. For all six stars, the measured splittings are consistent with uniform rotation, allowing us to exclude large radial differential rotation. This work opens the possibility of constraining internal rotation of Sun-like stars.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: rotation,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/7ND6HQGM/Nielsen et al. - 2014.pdf}
}

@article{Nielsen2015,
  title = {Constraining Differential Rotation of {{Sun-like}} Stars from Asteroseismic and Starspot Rotation Periods},
  author = {Nielsen, M. B. and Schunker, H. and Gizon, L. and Ball, W. H.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {582},
  eprint = {1508.02164},
  pages = {1--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526615},
  abstract = {In previous work, we identified six Sun-like stars observed by Kepler with exceptionally clear asteroseismic signatures of rotation. Here, we show that five of these stars exhibit surface variability suitable for measuring rotation. We compare the rotation periods obtained from light-curve variability with those from asteroseismology in order to further constrain differential rotation. The two rotation measurement methods are found to agree within uncertainties, suggesting that radial differential rotation is weak, as is the case for the Sun. Furthermore, we find significant discrepancies between ages from asteroseismology and from three different gyrochronology relations, implying that stellar age estimation is problematic even for Sun-like stars.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: rotation,Stars: solar-type,Starspots},
  file = {/Users/lbugnet/Zotero/storage/IZ38QSLN/Nielsen et al. - 2015.pdf}
}

@article{Nielsen2021,
  title = {{{PBjam}}: {{A Python Package}} for {{Automating Asteroseismology}} of {{Solar-like Oscillators}}},
  author = {Nielsen, M. B. and Davies, G. R. and Ball, W. H. and Lyttle, A. J. and Li, T. and Hall, O. J. and Chaplin, W. J. and Gaulme, P. and Carboneau, L. and Ong, J. M. J. and Garc{\'i}a, R. A. and Mosser, B. and Roxburgh, I. W. and Corsaro, E. and Benomar, O. and Moya, A. and Lund, M. N.},
  year = {2021},
  month = jan,
  journal = {The Astronomical Journal},
  volume = {161},
  number = {2},
  eprint = {2012.00580},
  pages = {62},
  publisher = {{American Astronomical Society}},
  issn = {0004-6256},
  doi = {10.3847/1538-3881/ABCD39},
  urldate = {2022-01-15},
  abstract = {Asteroseismology is an exceptional tool for studying stars by using the properties of observed modes of oscillation. So far the process of performing an asteroseismic analysis of a star has remained somewhat esoteric and inaccessible to non-experts. In this software paper we describe PBjam, an open-source Python package for analyzing the frequency spectra of solar-like oscillators in a simple but principled and automated way. The aim of PBjam is to provide a set of easy-to-use tools to extract information about the radial and quadrupole oscillations in stars that oscillate like the Sun, which may then be used to infer bulk properties such as stellar mass, radius and age or even structure. Asteroseismology and its data analysis methods are becoming increasingly important as space-based photometric observatories are producing a wealth of new data, allowing asteroseismology to be applied in a wide range of contexts such as exoplanet, stellar structure and evolution, and Galactic population studies.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/W6H7LVBQ/full-text.pdf}
}

@article{Nordstrom2004,
  title = {The {{Geneva-Copenhagen}} Survey of the Solar Neighbourhood},
  author = {Nordstr{\"o}m, B. and Andersen, J. and Holmberg, J. and J{\o}rgensen, B. R. and Mayor, M. and Pont, F.},
  year = {2004},
  journal = {Publications of the Astronomical Society of Australia},
  volume = {21},
  number = {2},
  pages = {129--133},
  issn = {14486083},
  doi = {10.1071/AS04013},
  abstract = {We report on a new survey of metallicities, ages, and Galactic orbits for a complete, magnitude-limited, and kinematically unbiased all-sky sample of 16 682 nearby F- and G-dwarfs. Our {$\sim$} 3 000 new, accurate radial velocities for nearly 13 500 of the stars, combined with Hipparcos parallaxes and Tycho-2 proper motions, complete the kinematic data for 14 139 stars and allow us to identify most of the binary stars in the sample. Isochrone ages have been determined whenever reliable results are possible, with particular attention to realistic error estimates.Among the basic properties of the Galactic disk that can be reinvestigated from our data are the metallicity distribution of G-dwarfs and the age-metallicity and age-velocity relations of the solar neighbourhood. We confirm the lack of metal-poor G-dwarfs relative to classical model predictions (the 'G-dwarf problem'), the near-constancy of the mean metallicity since the formation of the thin disk, and the appearance of the kinematic signature of the thick disk {$\sim$} 10 Gyr ago. \textcopyright{} Astronomical Society of Australia 2004.},
  keywords = {Galaxy: disk,Galaxy: evolution,Galaxy: kinematics and dynamics,Galaxy: solar neighbourhood,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MGFXXUBB/Nordström et al. - 2004.pdf}
}

@article{North2017,
  title = {A Simple Model to Describe Intrinsic Stellar Noise for Exoplanet Detection around Red Giants},
  author = {North, Thomas S. H. and Chaplin, William J. and Gilliland, Ronald L. and Huber, Daniel and Campante, Tiago L. and Handberg, Rasmus and Lund, Mikkel N. and Veras, Dimitri and Kuszlewicz, James S. and Farr, Will M.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {465},
  number = {2},
  eprint = {1610.08688},
  pages = {1308--1315},
  issn = {0035-8711},
  doi = {10.1093/mnras/stw2782},
  abstract = {In spite of the huge advances in exoplanet research provided by the NASA Kepler Mission, there remain only a small number of transit detections around evolved stars. Here we present a reformulation of the noise properties of red-giant stars, where the intrinsic stellar granulation, and the stellar oscillations described by asteroseismology play a key role. The new noise model is a significant improvement on the current Kepler results for evolved stars. Our noise model may be used to help understand planet detection thresholds for the ongoing K2 and upcoming TESS missions, and serve as a predictor of stellar noise for these missions. As an application of our noise model, we explore the minimum detectable planet radii for red giant stars, and find that Neptune sized planets should be detectable around low luminosity red giant branch stars.},
  archiveprefix = {arxiv},
  keywords = {1 i n t,and bloated massively com-,asteroseismology,fuseable hydrogen in the,notion,notion-database,of their life,photometric,planetary systems,red giants,ro d u c,stars near the end,stellar core,t i o n,techniques,which have exhausted},
  file = {/Users/lbugnet/Zotero/storage/GD5S373Y/North et al. - 2017.pdf}
}

@misc{NoTitle,
  title = {({{No Title}})},
  urldate = {2021-04-06},
  keywords = {notion,notion-database}
}

@article{November1981,
  title = {The Detection of Mesogranulation on the Sun},
  author = {November, L. J. and Toomre, J. and Gebbie, K. B. and Simon, G. W.},
  year = {1981},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {245},
  pages = {L123},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/183539},
  urldate = {2020-03-14},
  abstract = {Time averages of velocity measurements at disk center on the quiet sun reveal the presence of a fairly stationary pattern of cellular flow with a spatial scale of 5-10 Mm. Such mesogranulation has a spatial rms vertical velocity amplitude of about 60 m/s superposed on the larger scale supergranular flows. The lifetimes of mesogranules appear to be at least 2 hr.},
  keywords = {Convective Flow,notion,notion-database,Solar Atmosphere,Solar Granulation,Solar Physics,Velocity Distribution,Velocity Measurement,Vertical Motion}
}

@article{November1988,
  title = {Precise Proper-Motion Measurement of Solar Granulation},
  author = {November, Laurence J. and Simon, George W.},
  year = {1988},
  month = oct,
  journal = {The Astrophysical Journal},
  volume = {333},
  pages = {427},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/166758},
  urldate = {2020-03-14},
  abstract = {Mycotoxins are small (MW approximately 700), toxic chemical products formed as secondary metabolites by a few fungal species that readily colonise crops and contaminate them with toxins in the field or after harvest. Ochratoxins and Aflatoxins are mycotoxins of major significance and hence there has been significant research on broad range of analytical and detection techniques that could be useful and practical. Due to the variety of structures of these toxins, it is impossible to use one standard technique for analysis and/or detection. Practical requirements for high-sensitivity analysis and the need for a specialist laboratory setting create challenges for routine analysis. Several existing analytical techniques, which offer flexible and broad-based methods of analysis and in some cases detection, have been discussed in this manuscript. There are a number of methods used, of which many are lab-based, but to our knowledge there seems to be no single technique that stands out above the rest, although analytical liquid chromatography, commonly linked with mass spectroscopy is likely to be popular. This review manuscript discusses (a) sample pre-treatment methods such as liquid-liquid extraction (LLE), supercritical fluid extraction (SFE), solid phase extraction (SPE), (b) separation methods such as (TLC), high performance liquid chromatography (HPLC), gas chromatography (GC), and capillary electrophoresis (CE) and (c) others such as ELISA. Further currents trends, advantages and disadvantages and future prospects of these methods have been discussed.},
  keywords = {Cross Correlation,notion,notion-database,Power Spectra,Random Noise,Solar Atmosphere,Solar Granulation,Solar Physics,Spatial Resolution,SUN: ATMOSPHERIC MOTIONS,SUN: GRANULATION,Tracers},
  file = {/Users/lbugnet/Zotero/storage/7URQFJCW/full-text.pdf}
}

@article{Noyes1963a,
  title = {Velocity {{Fields}} in the {{Solar Atmosphere}}. {{II}}. {{The Oscillatory Field}}.},
  author = {Noyes, Robert W. and Leighton, Robert B.},
  year = {1963},
  journal = {The Astrophysical Journal},
  volume = {138},
  pages = {631},
  issn = {0004-637X},
  doi = {10.1086/147675},
  abstract = {From a systematic visual study of sets of "Doppler plates" obtained at the 13-foot spectroheliograph of the Mount Wilson Observatory during 1960 and 1961, the following results were derived: a) Vertical oscillatory motions were found in all medium-strong lines observed. The average period of the motions, about 290 sec, is a well-determined quantity for each spectral line. Slight, but apparently real, variations between the weaker and stronger lines observed suggest that the average period gradually decreases with increasing altitude in the line-forming regions of the upper photosphere. b) An oscillatory fluctuation of residual intensity was found in the cores of the stronger lines observed. The average period is somewhat shorter than that of the velocity oscillations and also exhibits an apparent decrease with increasing altitude. The two oscillations bear a definite phase relation to each other, indicating that they are physically connected. Intensity oscillations were not found in the weaker lines observed or in the core of Ha. These observations are discussed and compared with expectations for a plane wave propagating vertically through an isothermal atmosphere with an altitude-dependent radiative relaxation time.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/P6TIQESX/Noyes, Leighton - 1963.pdf}
}

@article{Noyes1984,
  title = {Rotation, Convection, and Magnetic Activity in Lower Main-Sequence Stars},
  author = {Noyes, Robert W. and Hartmann, L.W. and Baliunas, Sallie L. and Duncan, D.K. and Vaughan, A.H.},
  year = {1984},
  journal = {The Astrophysical Journal},
  pages = {763--777},
  keywords = {Ca n emission-convection-stai,notion,notion-database,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/8CGLDTMD/Noyes et al. - 1984.pdf}
}

@article{Noyes1984,
  title = {The Relation between Stellar Rotation Rate and Activity Cycle Periods},
  author = {Noyes, Robert W. and Weiss, N. O. and Vaughan, A.H.},
  year = {1984},
  journal = {The Astrophysical Journal},
  volume = {287},
  eprint = {1011.1669v3},
  pages = {769--773},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FH9HUDVL/Noyes, Weiss, Vaughan - 1984.pdf}
}

@article{Nunez2015,
  title = {{{LINKING STELLAR CORONAL ACTIVITY}} and {{ROTATION}} at 500 {{MYR}}: {{A DEEP CHANDRA OBSERVATION}} of {{M37}}},
  author = {N{\'u}{\~n}ez, Alejandro and Ag{\"u}eros, Marcel A. and Covey, Kevin R. and Hartman, Joel D. and Kraus, Adam L. and Bowsher, Emily C. and Douglas, Stephanie T. and {L{\'o}pez-Morales}, Mercedes and Pooley, David A. and Posselt, Bettina and Saar, Steven H. and West, Andrew A.},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {809},
  number = {2},
  eprint = {1507.02333},
  issn = {15384357},
  doi = {10.1088/0004-637X/809/2/161},
  abstract = {Empirical calibrations of the stellar age-rotation-activity relation (ARAR) rely on observations of the co-eval populations of stars in open clusters. We used the Chandra X-ray Observatory to study M37, a 500-Myr-old open cluster that has been extensively surveyed for rotation periods (). M37 was observed almost continuously for five days, for a total of 440.5 ks, to measure stellar X-ray luminosities (), a proxy for coronal activity, across a wide range of masses. The cluster's membership catalog was revisited to calculate updated membership probabilities from photometric data and each star's distance to the cluster center. The result is a comprehensive sample of 1699 M37 members: 426 with , 278 with X-ray detections, and 76 with both. We calculate Rossby numbers, , where {$\tau$} is the convective turnover time, and ratios of the X-ray-to-bolometric luminosity, , to minimize mass dependencies in our characterization of the rotation-coronal activity relation at 500 Myr. We find that fast rotators, for which , show saturated levels of activity, with log(). For , activity is unsaturated and follows a power law of the form , where {$\beta$} = . This is the largest sample available for analyzing the dependence of coronal emission on rotation for a single-aged population, covering stellar masses in the range 0.4-1.3 , in the range 0.4-12.8 days, and in the range . Our results make M37 a new benchmark open cluster for calibrating the ARAR at ages of Myr.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,open clusters and associations: individual (M37),stars: activity,stars: coronae,stars: rotation,X-rays: individual (M37)},
  file = {/Users/lbugnet/Zotero/storage/CKQVPL6B/Núñez et al. - 2015.pdf}
}

@article{Observatory1990,
  title = {A New Inversion of Solar Rotational Splitting Data},
  author = {Observatory, High Altitude},
  year = {1990},
  pages = {1--12},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VLQK8HJS/Observatory - 1990.pdf}
}

@article{Ogilvie2012,
  title = {On the Interaction between Tides and Convection},
  author = {Ogilvie, Gordon I. and Lesur, Geoffroy},
  year = {2012},
  month = may,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {422},
  number = {3},
  eprint = {1201.5020},
  pages = {1975--1987},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.20630.x},
  urldate = {2020-07-13},
  abstract = {We study the interaction between tides and convection in astrophysical bodies by analysing the effect of a homogeneous oscillatory shear on a fluid flow. This model can be taken to represent the interaction between a large-scale periodic tidal deformation and a smaller scale convective motion. We first consider analytically the limit in which the shear is of low amplitude and the oscillation period is short compared to the time-scales of the unperturbed flow. In this limit there is a viscoelastic response and we obtain expressions for the effective elastic modulus and viscosity coefficient. The effective viscosity is inversely proportional to the square of the oscillation frequency, with a coefficient that can be positive, negative or zero depending on the properties of the unperturbed flow. We also carry out direct numerical simulations of Boussinesq convection in an oscillatory shearing box and measure the time-dependent Reynolds stress. The results indicate that the effective viscosity of turbulent convection falls rapidly as the oscillation frequency is increased, attaining small negative values in the cases we have examined, although significant uncertainties remain because of the turbulent noise. We discuss the implications of this analysis for astrophysical tides. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  archiveprefix = {arxiv},
  keywords = {Binaries: general,Convection,Hydrodynamics,notion,notion-database,Planet-star interactions,Planets and satellites: general,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/BPCMDXMC/full-text.pdf}
}

@article{Olah2009,
  title = {Multiple and Changing Cycles of Active Stars {{II}}. {{Results}}},
  author = {Ol{\'a}h, K. and Koll{\'a}th, Z. and Granzer, T. and Strassmeier, K. G. and Lanza, A. F. and J{\"a}rvinen, S. and Korhonen, H. and Baliunas, S. L. and Soon, W. and Messina, S. and Cutispoto, G.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {501},
  number = {2},
  eprint = {0904.1747},
  pages = {703--713},
  issn = {00046361},
  doi = {10.1051/0004-6361/200811304},
  abstract = {Aims. We study the time variations in the cycles of 20 active stars based on decade-long photometric or spectroscopic observations. Methods. A method of time-frequency analysis, as discussed in a companion paper, is applied to the data. Results. Fifteen stars definitely show multiple cycles, but the records of the rest are too short to verify a timescale for a second cycle. The cycles typically show systematic changes. For three stars, we found two cycles in each of them that are not harmonics and vary in parallel, indicating a common physical mechanism arising from a dynamo construct. The positive relation between the rotational and cycle periods is confirmed for the inhomogeneous set of active stars. Conclusions. Stellar activity cycles are generally multiple and variable. \textcopyright{} 2009 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: atmospheres,Stars: late-type,Starspots},
  file = {/Users/lbugnet/Zotero/storage/H44MHEYQ/Oláh et al. - 2009.pdf}
}

@article{Olver1954,
  title = {The Asymptotic Solution of Linear Differential Equations of the Second Order for Large Values of a Parameter},
  author = {Olver, F. W. J.},
  year = {1954},
  month = dec,
  journal = {Philosophical Transactions of the Royal Society of London. Series A, Mathematical and Physical Sciences},
  volume = {247},
  number = {930},
  pages = {307--327},
  publisher = {{The Royal Society}},
  issn = {0080-4614},
  doi = {10.1098/rsta.1954.0020},
  urldate = {2020-07-14},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/H8VYJ8C8/full-text.pdf}
}

@incollection{Opa,
  title = {Chapter 7 {{TENSOR SPHERICAL HARMONICS}} 7.1.},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {3},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IDQCQRD6/Unknown - Unknown(15).pdf}
}

@misc{OpacityMechanismBtype,
  title = {The Opacity Mechanism in {{B-type}} Stars - {{II}}. {{Excitation}} of High-Order g-Modes in Main-Sequence Stars. - {{NASA}}/{{ADS}}},
  urldate = {2020-04-09},
  howpublished = {https://ui.adsabs.harvard.edu/abs/1993MNRAS.265..588D/abstract},
  keywords = {notion,notion-database}
}

@incollection{Opb,
  title = {Chapter 12 {{SUMS INVOLVING VECTOR}}, {{ADDITION M}} p {{BECOUPLING COEFFICIENTS}}},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {1},
  pages = {452--474},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/CIZ39BAX/Unknown - Unknown(13).pdf}
}

@incollection{Operator,
  title = {Chapter 2 {{ANGULAR MOMENTUM OPERATORS}} 2.1.},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  volume = {36},
  pages = {36--60},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RNFB3EI9/Unknown - Unknown(12).pdf}
}

@misc{Ordonez2015,
  title = {Population {{Effects}} on the {{Metallicity Distribution}}},
  author = {{Ordo\~nez} and {Sarajedini}},
  year = {2015},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IJEB5A3J/Ordoñez, Sarajedini - 2015.pdf}
}

@article{Oreiro2005,
  title = {Balloon 090100001: {{A}} Short and Long Period Pulsating {{sdB}} Star},
  shorttitle = {Balloon 090100001},
  author = {Oreiro, R. and P{\'e}rez Hern{\'a}ndez, F. and Ulla, A. and Garrido, R. and {\O}stensen, R. and MacDonald, J.},
  year = {2005},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {438},
  pages = {257--263},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20052681},
  urldate = {2023-10-09},
  abstract = {We report the discovery of long period oscillations in the light curve of the bright sdB pulsator Balloon 090100001. We find at least three peaks in the low frequency amplitude spectrum of the star (at periods 2733, 3665, 4378 s) and 10 certain frequencies in the short period range (118-356 s), but probably more than 25 frequencies modulate the light curve of this object. This star is one of only two sdBs, together with HS 0702+6043, known to show simultaneously short and long period pulsations. We also discuss the results of a set of multicolour photometric observations of the target, for which an amplitude-phase diagram is possible for the two dominant peaks. Comparision with theoretical models indicate that the short period peaks correspond to p modes clustered around the fundamental and the first three overtones, while the long period peaks correspond to g modes of high radial order.},
  keywords = {stars: early-type,stars: individual: Balloon 090100001,stars: oscillations,stars: subdwarfs},
  annotation = {ADS Bibcode: 2005A\&A...438..257O},
  file = {/Users/lbugnet/Zotero/storage/V7GQ87RG/Oreiro et al. - 2005 - Balloon 090100001 A short and long period pulsati.pdf}
}

@article{Osaki1975,
  title = {No Radial {{Oscillations}} of a 10 Solar Mass Star in the Main Sequence Stage},
  author = {Osaki, Yoji},
  year = {1975},
  journal = {Pas},
  volume = {27},
  pages = {237--258},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HA9Z3FNL/1975PASJ...27..237O.pdf}
}

@article{Osaki1977,
  title = {Stability of {{Cepheid-Type Stars}} against {{Nonradial Oscillations}}},
  author = {Osaki, Y.},
  year = {1977},
  journal = {PASJ},
  volume = {29},
  pages = {235--248},
  issn = {0004-6264},
  urldate = {2020-06-29},
  keywords = {notion,notion-database}
}

@article{Ouazzani2012,
  title = {Pulsations of Rapidly Rotating Stars},
  author = {Ouazzani, R.-M. and Dupret, M.-A. and Reese, D. R.},
  year = {2012},
  journal = {Astronomy \& Astrophysics},
  volume = {547},
  pages = {A75},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201219548},
  abstract = {Context. Very high precision seismic space missions such as CoRoT and Kepler provide the means of testing the modeling of transport processes in stellar interiors. For some stars, such as solar-like and red giant stars, a rotational splitting is measured. However, to fully exploit these splittings and constrain the rotation profile, one needs to be able to calculate them accurately. For some other stars, such as delta Scuti and Be stars, for instance, the observed pulsation spectra are modified by rotation to such an extent that a perturbative treatment of the effects of rotation is no longer valid.  Aims: We present here a new two-dimensional non-perturbative code called ACOR (adiabatic code of oscillation including rotation) that allows us to compute adiabatic non-radial pulsations of rotating stars without making any assumptions on the sphericity of the star, the fluid properties (i.e., baroclinicity) or the rotation profile.  Methods: The 2D non-perturbative calculations fully take into account the centrifugal distortion of the star and include the full influence of the Coriolis acceleration. The numerical method is based on a spectral approach for the angular part of the modes and a fourth-order finite differences approach for the radial part.  Results: We test and evaluate the accuracy of the calculations by comparing them with those coming from the TOP (two-dimensional oscillation program) for the same polytropic models. We illustrate the effects of rapid rotation on stellar pulsations through the phenomenon of avoided crossings.  Conclusions: As shown by the comparison with the TOP for simple models, the code is stable, and gives accurate results up to near-critical rotation rates.},
  keywords = {asteroseismology,methods,notion,notion-database,numerical,oscillations,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/IVV74H6N/Ouazzani, Dupret, Reese - 2012.pdf}
}

@article{Ouazzani2012a,
  title = {Rotational Splittings for Slow to Moderate Rotators},
  author = {Ouazzani, R.-M. and Goupil, M.-J.},
  year = {2012},
  journal = {Astronomy \& Astrophysics},
  volume = {542},
  pages = {A99},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201117151},
  abstract = {\emph{Context.{$<$}i/{$>$} The unprecedented photometric quality reached by the CoRoT and \emph{Kepler {$<$}i/{$>$}space missions opens new prospects for studying stellar rotation. Information about the rotation rate is contained on the one hand in the low frequency part of the power spectra, where signatures of nonuniform surface rotation are expected, and on the other hand in the frequency splittings induced by the internal rotation~rate.\emph{Aims.{$<$}i/{$>$} We wish to figure out whether the differences between the seismic rotation period determined by a mean rotational splitting, and the rotation period measured from the low frequency peak in the Fourier spectrum~\textendash{} observed for some of CoRoT's~targets~\textendash{} can provide constraints on the rotation profile.\emph{Methods.{$<$}i/{$>$} For uniform moderate rotators,perturbative corrections to second and third order in terms of the rotation angular velocity~{$\Omega$}, must not be neglected. These effects, in~particular, may mimic differential rotation. We apply our perturbation method to evaluate mode frequencies that are accurate up to~{$\Omega$}\textsuperscript{3{$<$}sup/{$>$} for uniform rotation. The effects of latitudinal dependence are calculated in the linear approximation. Numerical results were obtained for selected models of the upper and lower parts of the main sequence. For the latitudinal dependence, we adopt two types of rotation profile:~one with rotation uniform in depth, and one with a solar-like tachocline.\emph{Results.{$<$}i/{$>$} Deviations from the first-order splitting for a uniformly rotating star can be due to both cubic-order effects of rotation and latitudinal differential rotation. In models of \emph{{$\beta<$}i/{$>~$}Cephei pulsators, which represent upper main sequence stars, third order effects become comparable to that of a horizontal shear similar to the solar one at rotation rates well below the breakup values. These nonlinear effects are strongly mode-dependent. We show how a clean signature of the latitudinal shear may be extracted. Our models of two CoRoT~target HD~181906 and HD~181420, which are solar-like pulsators, represent lower main sequence objects. These are slow rotators and nonlinear effects in splittings are accordingly small. We use data for one low frequency peak and one splitting of a dipolar mode to constrain the rotation profile in HD~181420 and HD~181906. \emph{Conclusions.{$<$}i/{$>$} The relative influences of the two effects strongly depend on the type of oscillation modes excited in the star and the magnitude of the rotation rate. Given the mean rotational splitting and the frequency of a spot signature, it~is possible to distinguish between the two hypotheses. In the case of differential rotation in latitude, we propose a method to determine the type of rotation profile and a range of values for the~shear.}}}}}}}}},
  keywords = {asteroseismology,notion,notion-database,oscillations,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/L4KD7MH9/Ouazzani, Goupil - 2012.pdf}
}

@article{Ouazzani2013,
  title = {Non-Perturbative Effect of Rotation on Dipolar Mixed Modes in Red Giant Stars},
  author = {Ouazzani, R.-M. and Goupil, M. J. and Dupret, M.-A. and Marques, J. P.},
  year = {2013},
  journal = {Astronomy \& Astrophysics},
  volume = {554},
  pages = {A80},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201220547},
  abstract = {The space missions CoRoT and Kepler provide high quality data that allow us to test the transport of angular momentum in stars by the seismic determination of the internal rotation profile. Our aim is to test the validity of the seismic diagnostics for red giants rotation that are based on a perturbative method and to investigate the oscillation spectra when the validity does not hold. We use a non-perturbative approach implemented in the ACOR code (Ouazzani et al. 2012) that accounts for the effect of rotation on pulsations, and solves the pulsation eigenproblem directly for dipolar oscillation modes. We find that the limit of the perturbation to first order can be expressed in terms of the rotational splitting compared to the frequency separation between consecutive dipolar modes. Above this limit, non-perturbative computations are necessary but only one term in the spectral expansion of modes is sufficient as long as the core rotation rate remains significantly smaller than the pulsation frequencies. Each family of modes with different azimuthal symmetry, m, has to be considered separately. In particular, in case of rapid core rotation, the density of the spectrum differs significantly from one m-family of modes to another, so that the differences between the period spacings associated with each m-family can constitute a promising guideline toward a proper seismic diagnostic for rotation.},
  keywords = {asteroseismology,interiors,low-mass,notion,notion-database,oscillations,rotation,solar-type,stars},
  file = {/Users/lbugnet/Zotero/storage/9V7V6UMX/Ouazzani et al. - 2013.pdf}
}

@article{Ouazzani2017,
  title = {A New Asteroseismic Diagnostic for Internal Rotation in \$\textbackslash gamma\$ {{Doradus}} Stars},
  author = {Ouazzani, Rhita-Maria and Salmon, S. J. A. J. and Antoci, V. and Bedding, T. R. and Murphy, S. J. and Roxburgh, I. W.},
  year = {2017},
  month = oct,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {465},
  number = {2},
  eprint = {1610.06184},
  pages = {2294--2309},
  doi = {10.1093/mnras/stw2717},
  urldate = {2020-07-18},
  abstract = {With four years of nearly-continuous photometry from Kepler, we are finally in a good position to apply asteroseismology to \$\textbackslash gamma\$ Doradus stars. In particular several analyses have demonstrated the possibility to detect non-uniform period spacings, which have been predicted to be directly related to rotation. In the present work, we define a new seismic diagnostic for rotation in \$\textbackslash gamma\$ Doradus stars that are too rapidly rotating to present rotational splittings. Based on the non uniformity of their period spacings, we define the observable \$\textbackslash Sigma\$ as the slope of the period spacing when plotted as a function of period. We provide a one-to-one relation between this observable \$\textbackslash Sigma\$ and the internal rotation, which applies widely in the instability strip of \$\textbackslash gamma\$ Doradus stars. We apply the diagnostic to a handful of stars observed by Kepler. Thanks to g-modes in \$\textbackslash gamma\$ Doradus stars, we are now able to determine the internal rotation of stars on the lower main sequence, which is still not possible for Sun-like stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/789EF4JK/full-text.pdf}
}

@article{Ouazzani2019,
  title = {{$\gamma$} {{Doradus}} Stars as a Test of Angular Momentum Transport Models},
  author = {Ouazzani, R. -M. and Marques, J. P. and Goupil, M. -J. and Christophe, S. and Antoci, V. and Salmon, S. J. A. J. and Ballot, J.},
  year = {2019},
  month = jun,
  journal = {Astronomy and Astrophysics},
  volume = {626},
  pages = {A121},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201832607},
  urldate = {2023-11-04},
  abstract = {Helioseismology and asteroseismology of red giant stars have shown that distribution of angular momentum in stellar interiors, and the evolution of this distribution with time remains an open issue in stellar physics. Owing to the unprecedented quality and long baseline of Kepler photometry, we are able to seismically infer internal rotation rates in {$\gamma$} Doradus stars, which provide the main-sequence counterpart to the red-giants puzzle. Here, we confront these internal rotation rates to stellar evolution models which account for rotationally induced transport of angular momentum, in order to test angular momentum transport mechanisms. On the one hand, we used a stellar model-independent method developed by our team in order to obtain accurate, seismically inferred, buoyancy radii and near-core rotation for 37 {$\gamma$} Doradus stars observed by Kepler. We show that the stellar buoyancy radius can be used as a reliable evolution indicator for field stars on the main sequence. On the other hand, we computed rotating evolutionary models of intermediate-mass stars including internal transport of angular momentum in radiative zones, following the formalism developed in the series of papers started by Zahn (1992, A\&A, 265, 115), with the CESTAM code. This code calculates the rotational history of stars from the birth line to the tip of the RGB. The initial angular momentum content has to be set initially, which is done here by fitting rotation periods in young stellar clusters. We show a clear disagreement between the near-core rotation rates measured in the sample and the rotation rates obtained from the evolutionary models including rotationally induced transport of angular momentum following Zahn's prescriptions. These results show a disagreement similar to that of the Sun and red giant stars in the considered mass range. This suggests the existence of missing mechanisms responsible for the braking of the core before and along the main sequence. The efficiency of the missing mechanisms is investigated. The transport of angular momentum as formalized by Zahn and Maeder cannot explain the measurements of near-core rotation in main-sequence intermediate-mass stars we have at hand. Evolutionnary sequences (Fig. 7) and evolution of stellar global parameters are only available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr (ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/626/A121.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: low-mass,stars: oscillations,stars: rotation,stars: statistics},
  annotation = {ADS Bibcode: 2019A\&A...626A.121O},
  file = {/Users/lbugnet/Zotero/storage/DUYLWBV3/Ouazzani et al. - 2019 - γ Doradus stars as a test of angular momentum tran.pdf}
}

@article{Ouazzani2020,
  title = {First Evidence of Inertial Modes in Gamma {{Doradus}} Stars: The Core Rotation Revealed},
  author = {Ouazzani, R-M. and Ligni{\`e}res, F. and Dupret, M-A. and Salmon, S.J.A.J. and Ballot, J. and Christophe, S. and Takata, M.},
  year = {2020},
  month = jun,
  journal = {Astronomy \& Astrophysics},
  eprint = {2006.09404},
  publisher = {{EDP Sciences}},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201936653},
  urldate = {2020-07-18},
  abstract = {Gamma Doradus stars present an incredibly rich pulsation spectra, with gravito-inertial modes, in some cases supplemented with delta Scuti-like pressure modes and in numerous cases with Rossby modes. The present paper aims at showing that, in addition to these modes established in the radiative envelope, pure inertial modes, trapped in the convective core, can be detected in Kepler observations of gamma Doradus stars, thanks to their resonance with the gravito-inertial modes. We start by using a simplified model of perturbations in a full sphere of uniform density. Under these conditions, the spectrum of pure inertial modes is known from analytical solutions of the so-called Poincare equation. We then compute coupling factors which help select the pure inertial modes which interact best with the surrounding dipolar gravito-inertial modes. Using complete calculations of gravito-inertial modes in realistic models of gamma Doradus stars, we are able to show that the pure inertial/gravito-inertial resonances appear as dips in the gravito-inertial mode period spacing series at spin parameters close to those predicted by the simple model. We find the first evidence of such dips in the Kepler gamma Doradus star KIC5608334. Finally, using complete calculations in isolated convective cores, we find that the spin parameters of the pure inertial/gravito-inertial resonances are also sensitive to the density stratification of the convective core. In conclusion, we have discovered that certain dips in gravito-inertial mode period spacings observed in some Kepler stars are in fact the signatures of resonances with pure-inertial modes that are trapped in the convective core. This holds the promise to finally access the central conditions , i.e. rotation and density stratification, of intermediate-mass stars on the main sequence.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2US8VKC4/full-text.pdf}
}

@techreport{ouazzaniFirstEvidenceInertial2020,
  title = {First Evidence of Inertial Modes in {$\gamma$} {{Doradus}} Stars {{The}} Core Rotation Revealed},
  author = {Ouazzani, R-M and Lignires, F and Dupret, M-A and Salmon, S J A J and Ballot, J and Christophe, S and Takata, M},
  year = {2020},
  eprint = {2006.09404v1},
  urldate = {2021-03-02},
  abstract = {Context. The advent of space photometry with CoRoT and Kepler has allowed the gathering of exquisite and long time series for a wealth of main sequence stars, including {$\gamma$} Doradus stars whose detailed seismology was unachievable from the ground. Aims. {$\gamma$} Doradus stars present an incredibly rich pulsation spectra, with gravito-inertial modes, in some cases supplemented with {$\delta$} Scuti-like pressure modes-for the hybrid stars-and in numerous cases with Rossby modes. The present paper aims at showing that, in addition to these modes established in the radiative envelope, pure inertial modes, trapped in the convective core, can be detected in Kepler observations of {$\gamma$} Doradus stars, thanks to their resonance with the gravito-inertial modes. Methods. We start by using a simplified model of perturbations in a full sphere of uniform density. Under these conditions, the spectrum of pure inertial modes is known from analytical solutions of the so-called Poincar equation. We then compute coupling factors which help select the pure inertial modes which interact best with the surrounding dipolar gravito-inertial modes. Using complete calculations of gravito-inertial modes in realistic models of {$\gamma$} Doradus stars, we are able to show that the pure inertial/gravito-inertial resonances appear as dips in the gravito-inertial mode period spacing series at spin parameters close to those predicted by the simple model. We find the first evidence of such dips in the Kepler {$\gamma$} Doradus star KIC5608334. Finally, using complete calculations in isolated convective cores, we find that the spin parameters of the pure inertial/gravito-inertial resonances are also sensitive to the density stratification of the convective core. Results. In conclusion, we have discovered that certain dips in gravito-inertial mode period spacings observed in some Kepler stars are in fact the signatures of resonances with pure-inertial modes that are trapped in the convective core. Conclusions. This holds the promise to finally access the central conditions , i.e. rotation and density stratification, of intermediate-mass stars on the main sequence.},
  archiveprefix = {arxiv},
  isbn = {2006.09404v1},
  keywords = {asteroseismology-stars,notion,notion-database,oscillations-stars,rotation-methods},
  file = {/Users/lbugnet/Zotero/storage/8NQQSNPN/full-text.pdf}
}

@article{Ozel2013,
  title = {Differential Asteroseismic Study of Seismic Twins Observed by {{CoRoT}}: {{Comparison}} of {{HD}} 175272 with {{HD}} 181420},
  author = {Ozel, N. and Mosser, B. and Dupret, M. A. and Bruntt, H. and Barban, C. and Deheuvels, S. and Garc{\'i}a, R. A. and Michel, E. and Samadi, R. and Baudin, F. and Mathur, S. and R{\'e}gulo, C. and Auvergne, M. and Catala, C. and Morel, P. and Pichon, B.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {558},
  pages = {1--9},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321846},
  abstract = {Context. The CoRoT short asteroseismic runs give us the opportunity to observe a large variety of late-type stars through their solar-like oscillations. We report the observation and modeling of the F5V star HD 175272. Aims. Our aim is to define a method for extracting as much information as possible from a noisy oscillation spectrum. Methods. We followed a differential approach that consists of using a well-known star as a reference to characterize another star. We used classical tools such as the envelope autocorrelation function to derive the global seismic parameters of the star. We compared HD 175272 with HD 181420 through a linear approach, because they appear to be asteroseismic twins. Results. The comparison with the reference star enables us to substantially enhance the scientific output for HD 175272. First, we determined its global characteristics through a detailed seismic analysis of HD 181420. Second, with our differential approach, we measured the difference of mass, radius and age between HD 175272 and HD 181420. Conclusions. We have developed a general method able to derive asteroseismic constraints on a star even in case of low-quality data. This method can be applied to stars with interesting properties but low signal-to-noise ratio oscillation spectrum, such as stars hosting an exoplanet or members of a binary system. \textcopyright{} 2013 ESO.},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: individual: HD 175272,Stars: individual: HD 181420,Stars: interiors,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/HRTL4F4M/Ozel et al. - 2013.pdf}
}

@article{Pace2004,
  title = {The Age-Activity-Rotation Relationship in Solar-Type Stars},
  author = {Pace, G and Pasquini, L},
  year = {2004},
  volume = {1034},
  pages = {1021--1034},
  keywords = {activity,chromosphere,late-type,notion,notion-database,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/AMYFBS8C/Pace, Pasquini - 2004.pdf}
}

@article{Pace2013,
  title = {Chromospheric Activity as Age Indicator: {{An L-shaped}} Chromospheric-Activity versus Age Diagram},
  author = {Pace, G.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {551},
  pages = {1--4},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220364},
  abstract = {Context. Chromospheric activity has been calibrated and widely used as an age indicator. However, it has been suggested that the viability of this age indicator is, in the best case, limited to stars younger than about 1.5 Gyr. Aims. I aim to define the age range for which chromospheric activity is a robust astrophysical clock. Methods. I collected literature measurements of the S-index in field stars, which is a measure of the strength of the H and K lines of the Ca II and a proxy for chromospheric activity, and exploited the homogeneous database of temperature and age determinations for field stars provided by the Geneva-Copenhagen survey of the solar neighbourhood. Results. Field data, inclusive data previously used to calibrate chromospheric ages, confirm the result found using open cluster data, i.e. there is no decay of chromospheric activity after about 2 Gyr. Conclusions. The only existing indication supporting the viability of chromospheric ages older than 2 Gyr is the similarity of chromospheric activity levels in the components of 35 dwarf binaries. However, even in the most optimistic scenario, uncertainty in age determination for field stars and lack of sufficient data in open clusters make any attempt of calibrating an age activity relationship for old stars premature. The hypothesis that chromospheric activity follows the Skumanich law, i.e. that it is proportional to t-1/2, should be relaxed. \textcopyright{} 2013 ESO.},
  keywords = {notion,notion-database,Stars: activity},
  file = {/Users/lbugnet/Zotero/storage/RLVYES5Z/Pace - 2013.pdf}
}

@article{Paczynski1969,
  title = {Stellar {{Evolution}} from {{Main Sequence}} to {{White Dwarf}} or {{Supernova}}},
  author = {Paczynski, B.},
  year = {1969},
  journal = {BAAS},
  volume = {1},
  pages = {256},
  urldate = {2020-03-08},
  keywords = {notion,notion-database}
}

@article{Paczynski1970,
  title = {Evolution of {{Single Stars}}. {{I}}. {{Stellar Evolution}} from {{Main Sequence}} to {{White Dwarf}} or {{Carbon Ignition}} - {{NASA}}/{{ADS}}},
  author = {Paczy{\'n}ski, B.},
  year = {1970},
  journal = {Acta Astronomica},
  volume = {20},
  pages = {47},
  urldate = {2020-03-03},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/I8S44RRA/1970AcA____20___47P.pdf}
}

@book{PAINE1969,
  title = {Apollo 11 Preliminary {{Science Report}}},
  author = {Paine, T.O and {NATIONAL AERONAUTICS} and ADMINISTRATION, AND SPACE},
  year = {1969},
  abstract = {Paine1969},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JM393PRK/as11psr.pdf}
}

@article{Palacios2006,
  title = {Rotational Mixing in Low-Mass Stars {{II}}. {{Self-consistent}} Models of {{Pop II RGB}} Stars},
  author = {Palacios, A. and Charbonnel, C. and Talon, S. and Siess, L.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {453},
  number = {1},
  pages = {261--278},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053065},
  abstract = {Aims. In this paper we study the effects of rotation in low-mass, low-metallicity RGB stars. Methods. We present the first evolutionary models taking into account self-consistently the latest prescriptions for the transport of angular momentum by meridional circulation and shear turbulence in stellar interiors as well as the associated mixing processes for chemicals computed from the ZAMS to the upper RGB. We discuss the uncertainties associated with the physical description of the rotational mixing in detail and carefully study their effects on the rotation profile, diffusion coefficients, structural evolution, lifetimes, and chemical signatures at the stellar surface. We focus in particular on the various assumptions concerning the rotation law in the convective envelope, the initial rotation velocity distribution, the presence of {$\mu$}-gradients, and the treatment of the horizontal and vertical turbulence. Results. This exploration leads to two main conclusions. (1) After completion of the first dredge-up, the degree of differential rotation (and hence mixing) is maximised in the case of a differentially rotating convective envelope (i.e., jCE(r) - const.), as anticipated in previous studies. (2) Even with this assumption, and contrary to some previous claims, the present treatment for the evolution of the rotation profile and associated meridional circulation and shear turbulence does not lead to enough mixing of chemicals to explain the abundance anomalies in low-metallicity field and globular cluster RGB stars observed around the bump luminosity. Conclusions. This study raises questions that need to be addressed in the near future. These include, for example, the interaction between rotation and convection and the trigger of additional hydrodynamical instabilities. \textcopyright{} ESO 2006.},
  keywords = {abundances-hydrodynamics-turbulence,evolution-stars,Hydrodynamics,interiors-stars,notion,notion-database,rotation-stars,stars,Stars: abundances,Stars: evolution,Stars: interiors,Stars: rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/F4XPMQZ2/Palacios et al. - 2006.pdf}
}

@article{Palle1991,
  title = {The Search for {{Solar}} Gravity Modes},
  author = {Pall{\'e}, Pere L.},
  year = {1991},
  volume = {II},
  number = {4},
  pages = {29--38},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TX3PTPIH/Pallé - 1991.pdf}
}

@article{Palle2013,
  title = {Observations of the Radial Velocity of the {{Sun}} as Measured with the Novel {{SONG}} Spectrograph: {{Results}} from a 1-Week Campaign},
  author = {Pall{\'e}, P. L. and Grundahl, F. and Hage, A. Trivi{\~n}o and {Christensen-Dalsgaard}, J. and Frandsen, S. and Garc{\'i}a, R. A. and Uytterhoeven, K. and Andersen, M. F. and Rasmussen, P. K. and S{\o}rensen, A. N. and Kjeldsen, H. and Spano, P. and Nilsson, H. and Hartman, H. and J{\o}rgensen, U. G. and Skottfelt, J. and Harps{\o}e, K. and Andersen, M. I.},
  year = {2013},
  journal = {Journal of Physics: Conference Series},
  volume = {440},
  number = {1},
  issn = {17426596},
  doi = {10.1088/1742-6596/440/1/012051},
  abstract = {Deployment of the prototype node of the SONG project took place in April 2012 at Observatorio del Teide (Canary Islands). Its key instrument (echelle spectrograph) was installed and operational a few weeks later while its 1 m feeding telescope suffered a considerable delay to meet the required specifications. Using a fibre-feed, solar light could be fed to the spectrograph and we carried out a 1-week observing campaign in June 2012 to evaluate its performance for measuring precision radial velocities. In this work we present the first results of this campaign by comparing the sensitivity of the SONG spectrograph with other helioseismology reference instruments (Mark-I and GOLF) when simultaneous data are considered. \textcopyright{} 2013 Published under licence by IOP Publishing Ltd.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YBJNVZ2D/Pallé et al. - 2013.pdf}
}

@article{Pande2018,
  title = {Surface Gravities for 15 000 {{Kepler}} Stars Measured from Stellar Granulation and Validated with {{Gaia DR2}} Parallaxes},
  author = {Pande, Durlabh and Bedding, Timothy R. and Huber, Daniel and Kjeldsen, Hans},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {480},
  number = {1},
  eprint = {1807.03624},
  pages = {467--472},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/sty1869},
  abstract = {We have developed amethod to estimate surface gravity (log g) from light curves bymeasuring the granulation background, similar to the 'flicker' method by Bastien et al. (2016) but working in the Fourier power spectrum. We calibrated the method using Kepler stars for which asteroseismology has been possible with short-cadence data, demonstrating a precision in log g of about 0.05 dex. We also derived a correction for white noise as a function of Kepler magnitude by measuring white noise directly from observations. We then applied the method to the same sample of long-cadence stars as Bastien et al. We found that about half the stars are too faint for the granulation background to be reliably detected above the white noise. We provide a catalogue of log g values for about 15 000 stars having uncertainties better than 0.5 dex. We used Gaia DR2 parallaxes to validate that granulation is a powerful method to measure log g from light curves. Our method can also be applied to the large number of light curves collected by K2 and TESS.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: fundamental parameters,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/9KIK4URE/Pande et al. - 2018.pdf}
}

@techreport{Pande2018a,
  title = {Surface Gravities for 15,000 {{Kepler}} Stars Measured from Stellar Granulation and Validated with {{Gaia DR2}} Parallaxes},
  author = {Pande, Durlabh and Bedding, Timothy R and Huber, Daniel and Kjeldsen, Hans},
  year = {2018},
  journal = {MNRAS},
  volume = {000},
  eprint = {1807.03624v2},
  pages = {1--6},
  urldate = {2020-01-20},
  abstract = {We have developed a method to estimate surface gravity (log g) from light curves by measuring the granulation background, similar to the "flicker" method by Bastien et al. (2016) but working in the Fourier power spectrum. We calibrated the method using Kepler stars for which asteroseismology has been possible with short-cadence data, demonstrating a precision in log g of about 0.05 dex. We also derived a correction for white noise as a function of Kepler magnitude by measuring white noise directly from observations. We then applied the method to the same sample of long-cadence stars as Bastien et al. We found that about half the stars are too faint for the granulation background to be reliably detected above the white noise. We provide a catalogue of log g values for about 15,000 stars having uncertainties better than 0.5 dex. We used Gaia DR2 parallaxes to validate that granulation is a powerful method to measure log g from light curves. Our method can also be applied to the large number of light curves collected by K2 and TESS.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology-stars,fundamental parameters-stars,notion,notion-database,oscillations},
  file = {/Users/lbugnet/Zotero/storage/G73XDKAU/full-text.pdf}
}

@article{Papics2012,
  title = {Gravito-Inertial and Pressure Modes Detected in the {{B3 IV CoRoT}} Target {{HD}} 43317},
  author = {P{\'a}pics, P. I. and Briquet, M. and Baglin, A. and Poretti, E. and Aerts, C. and Degroote, P. and Tkachenko, A. and Morel, T. and Zima, W. and Niemczura, E. and Rainer, M. and Hareter, M. and Baudin, F. and Catala, C. and Michel, E. and Samadi, R. and Auvergne, M.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {542},
  eprint = {1203.5231},
  issn = {00046361},
  doi = {10.1051/0004-6361/201218809},
  urldate = {2020-06-29},
  abstract = {Context. OB stars are important building blocks of the Universe, but we have only a limited sample of them well understood enough from an asteroseismological point of view to provide feedback on the current evolutionary models. Our study adds one special case to this sample, with more observational constraints than for most of these stars. Aims. Our goal is to analyse and interpret the pulsational behaviour of the B3 IV star HD 43317 using the CoRoT light curve along with the ground-based spectroscopy gathered by the HARPS instrument. This way we continue our efforts to map the {$\beta$} Cep and SPB instability strips. Methods. We used different techniques to reveal the abundances and fundamental stellar parameters from the newly-obtained high-resolution spectra. We used various time-series analysis tools to explore the nature of variations present in the light curve. We calculated the moments and used the pixel-by-pixel method to look for line profile variations in the high-resolution spectra. Results. We find that HD 43317 is a single fast rotator (v rot {$\approx$} 50\% v crit) and hybrid SPB/{$\beta$} Cep-type pulsator with Solar metal abundances. We interpret the variations in photometry and spectroscopy as a result of rotational modulation connected to surface inhomogeneities, combined with the presence of both g and p mode pulsations. We detect a series of ten consecutive frequencies with an almost constant period spacing of 6339 s as well as a second shorter sequence consisting of seven frequencies with a spacing of 6380 s. The dominant frequencies fall in the regime of gravito-inertial modes. \textcopyright{} ESO, 2012.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: abundances,Stars: individual: HD 43317,Stars: oscillations,Stars: rotation,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/HMWDLWT3/full-text.pdf}
}

@article{Papics2017,
  title = {Signatures of Internal Rotation Discovered in the {{Kepler}} Data of Five Slowly Pulsating {{B}} Stars},
  author = {P{\'a}pics, P. I. and Tkachenko, A. and Van Reeth, T. and Aerts, C. and Moravveji, E. and {Van de Sande}, M. and De Smedt, K. and Bloemen, S. and Southworth, J. and Debosscher, J. and Niemczura, E. and Gameiro, J. F.},
  year = {2017},
  month = feb,
  journal = {Astronomy and Astrophysics},
  volume = {598},
  pages = {A74},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201629814},
  urldate = {2023-10-09},
  abstract = {Context. Massive stars are important building blocks of the Universe, and their stellar structure and evolution models are fundamental cornerstones of various fields in modern astrophysics. The precision of these models is strongly limited by our lack of understanding of various internal mixing processes that significantly influence the lifetime of these objects, such as core overshoot, chemical mixing, or the internal differential rotation. Aims: Our goal is to calibrate models by extending the sample of available seismic studies of slowly pulsating B (SPB) stars, providing input for theoretical modelling efforts that will deliver precise constraints on the parameters describing the internal mixing processes in these objects. Methods: We used spectral synthesis and disentangling techniques to derive fundamental parameters and to determine precise orbital parameters from high-resolution spectra. We employed custom masks to construct light curves from the virtually uninterrupted four year long Kepler pixel data and used standard time-series analysis tools to construct a set of significant frequencies for each target. These sets were first filtered from combination frequencies, and then screened for period spacing patterns. Results: We detect gravity mode period series of modes, of the same degree {$\mathscr{l}$} with consecutive radial order n, in four new and one revisited SPB star. These series (covering typically 10 to 40 radial orders) are clearly influenced by moderate to fast rotation and carry signatures of chemical mixing processes. Furthermore, they are predominantly prograde dipole series. Our spectroscopic analysis, in addition to placing each object inside the SPB instability strip and identifying KIC 4930889 as an SB2 binary, reveals that KIC 11971405 is a fast rotator that shows very weak Be signatures. Together with the observed photometric outbursts this illustrates that this Be star is a fast rotating SPB star. We hypothesise that the outbursts might be connected to its very densely compressed oscillation spectrum. Based on observations made with the Mercator telescope, operated by the Flemish Community, and with the William Herschel Telescope operated by the Isaac Newton Group, both on the island of La Palma at the Spanish Observatorio del Roque de los Muchachos of the Instituto de Astrof\'isica de Canarias.Based on observations obtained with the Hermes spectrograph, which is supported by the Fund for Scientific Research of Flanders (FWO), Belgium, the Research Council of KU Leuven, Belgium, the Fonds National Recherches Scientific (FNRS), Belgium, the Royal Observatory of Belgium, the Observatoire de Gen\`eve, Switzerland, and the Th\"uringer Landessternwarte Tautenburg, Germany.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: early-type,stars: fundamental parameters,stars: oscillations,stars: rotation,stars: variables: general},
  annotation = {ADS Bibcode: 2017A\&A...598A..74P},
  file = {/Users/lbugnet/Zotero/storage/53LZS3K8/Pápics et al. - 2017 - Signatures of internal rotation discovered in the .pdf}
}

@article{Parker1955,
  title = {Hydromagnetic {{Dynamo Models}}.},
  author = {Parker, Eugene N.},
  year = {1955},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {122},
  pages = {293},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/146087},
  urldate = {2020-05-14},
  abstract = {The purpose of this paper is to investigate the steady-state amplification of magnetic fields in a fluid It is shown that a rotating sphere of conducting fluid can regenerate a dipole magnetic field. It is sufficient for the angular velocity of rotation to vary with distance from the axis of rotation and for cyclonic fluid motions to be present The nonuniform rotation generates a toroidal field from the dipole field; the cyclones generate, from the toroidal field, loops of flux in the meridional plane which coalesce to amplify the dipole field The rotating sphere is discussed in relation to the liquid core of the earth and the geomagnetic dipole field. If, instead of a rotating sphere, one has a prismatic volume of fluid, it is possible to construct migratory dynamo waves The dynamo waves are discussed in relation to the solar convective zone; it is shown that such waves can account for many of the principal features of the observed solar magnetic activity},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/52D5Y7YR/Parker - 1955.pdf}
}

@article{Parker1966,
  title = {The {{Dynamical State}} of the {{Interstellar Gas}} and {{Field}}},
  author = {Parker, E. N.},
  year = {1966},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {145},
  pages = {811},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/148828},
  urldate = {2020-05-16},
  abstract = {There is now enough observational information available to show that the interstellar magnetic field in the general neighborhood of the Sun is, on the average, parallel to the plane of the Galaxy, with an average strength somewhere between 10-6 and tO-' gauss. This paper points out certain dynamical requirements for the existence of such a field. The paper is based on the assumption that the intergalactic medium, whatever it may be, exerts pressures on the Galaxy that are small compared to 10-12 dyne/cm'. It can then be shown that the galactic, or interstellar, magnetic field must be to the Galaxy by the weight of the gas threaded by the field and distributed throughout the disk of the Galaxy. It is then shown that the interstellar gas-field system is subject to a universal Rayleigh-Taylor instability of such a nature that the interstellar gas tends to concentrate into pockets suspended in the field. The cause of the instability may he thought of as a hydromagnetic self-attraction in the interstellar gas, which may be ten times larger than the gravitational self-attraction of the gas. It is this hydromagnetic self-attraction which produces the observed tendency of the interstellar gas to be confined in discrete clouds. The calculations and arguments do not restrict the over-all topology or the strength of the galactic field, which apparently must still be determined from observation.},
  keywords = {notion,notion-database}
}

@article{Parker1970a,
  title = {The Origin of Magnetic Fields},
  author = {Parker, E.n.},
  year = {1970},
  journal = {The Astrophysical Journal},
  volume = {160},
  number = {May},
  pages = {383--404},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HXYTPJP8/Parker - 1970.pdf}
}

@article{Parker1979,
  title = {Sunspots and the Physics of Magnetic Flux Tubes. {{IX}} - {{Umbral}} Dots and Longitudinal Overstability},
  author = {Parker, E. N.},
  year = {1979},
  month = nov,
  journal = {The Astrophysical Journal},
  volume = {234},
  pages = {333},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/157501},
  urldate = {2020-07-02},
  keywords = {Dynamic Stability,High Temperature Gases,Longitudinal Stability,Magnetic Flux,Magnetohydrodynamic Stability,Magnetohydrodynamic Waves,Magnetohydrodynamics:Sunspots,notion,notion-database,Perturbation Theory,Solar Magnetic Field,Solar Physics,Sunspots,Umbras}
}

@article{Parker2009,
  title = {Solar Magnetism: {{The}} State of Our Knowledge and Ignorance},
  author = {Parker, E. N.},
  year = {2009},
  month = apr,
  journal = {Space Science Reviews},
  volume = {144},
  number = {1-4},
  pages = {15--24},
  issn = {00386308},
  doi = {10.1007/s11214-008-9445-x},
  urldate = {2020-05-14},
  abstract = {We review some longstanding scientific mysteries related to solar magnetism, with final attention to the mystery of the "turbulent diffusion" essential for the theoretical {$\alpha$} {$\omega$}-dynamo that is believed to be the source of the magnetic fields of the Sun. Fundamental difficulties with the concept of turbulent diffusion of magnetic fields suggest that the solar dynamo problem needs to be reformulated. An alternative dynamo model is proposed, but it remains to be shown that the model can provide the quantitative aspects of the cyclic magnetic fields of the Sun. \textcopyright{} 2008 Springer Science+Business Media B.V.},
  keywords = {notion,notion-database,Solar dynamo,Turbulent diffusion of magnetic fields}
}

@misc{parkHorizontalShearInstabilities2020,
  title = {Horizontal Shear Instabilities in Rotating Stellar Radiation Zones: {{II}}. {{Effects}} of the Full {{Coriolis}} Acceleration},
  author = {Park, J. and Prat, V. and Mathis, S. and Bugnet, L.},
  year = {2020},
  journal = {arXiv},
  abstract = {Copyright \textcopyright{} 2020, arXiv, All rights reserved. Context. Stellar interiors are the seat of efficient transport of angular momentum all along with their evolution. In this context, understanding the dependence of the turbulent transport triggered by the instabilities of the vertical and horizontal shears of the differential rotation in stellar radiation zones as a function of their rotation, stratification, and thermal diffusivity is mandatory. Indeed, it constitutes one of the cornerstones of the rotational transport and mixing theory which is implemented in stellar evolution codes to predict the rotational and chemical evolutions of stars. Aims. We investigate horizontal shear instabilities in rotating stellar radiation zones by considering the full Coriolis acceleration with both the dimensionless horizontal Coriolis component {\~f} and the vertical component f. Methods. We performed a linear stability analysis using linearized equations derived from the Navier-Stokes and heat transport equations in the rotating non-traditional f-plane. We considered a horizontal shear flow with a hyperbolic tangent profile as the base flow. The linear stability was analyzed numerically in wide ranges of parameters, and we performed an asymptotic analysis for large vertical wavenumbers using the Wentzel-Kramers-Brillouin-Jeffreys (WKBJ) approximation for non-diffusive and highly diffusive fluids. Results. As in the traditional f-plane approximation, we identify two types of instabilities: the inflectional and inertial instabilities. The inflectional instability is destabilized as {\~f} increases and its maximum growth rate increases significantly, while the thermal diffusivity stabilizes the inflectional instability similarly to the traditional case. The inertial instability is also strongly affected; for instance, the inertially unstable regime is also extended in the non-diffusive limit as 0 {$<$} f {$<$} 1 + {\~f}2/N2, where N is the dimensionless Brunt-V\"ais\"al\"a frequency. More strikingly, in the high-thermal-diffusivity limit, it is always inertially unstable at any colatitude \texttheta{} except at the poles (i.e., 0{$\smwhtcircle$} {$<$} \texttheta{} {$<$} 180{$\smwhtcircle$}). We also derived the critical Reynolds numbers for the inertial instability using the asymptotic dispersion relations obtained from the WKBJ analysis. Using the asymptotic and numerical results, we propose a prescription for the effective turbulent viscosities induced by the inertial and inflectional instabilities that can be possibly used in stellar evolution models. The characteristic time of this turbulence is short enough so that it is efficient to redistribute angular momentum and mix chemicals in stellar radiation zones.},
  keywords = {Hydrodynamics,notion,notion-database,Stars: evolution,Stars: rotation,Turbulence}
}

@article{passeggerAstrophysicsFundamentalMdwarf2016,
  title = {Astrophysics {{Fundamental M-dwarf}} Parameters from High-Resolution Spectra Using {{PHOENIX ACES}} Models {{I}}. {{Parameter}} Accuracy and Benchmark Stars},
  author = {Passegger, V M and {Wende-Von Berg}, S and Reiners, A},
  year = {2016},
  journal = {A\&A},
  volume = {587},
  pages = {19},
  doi = {10.1051/0004-6361/201322261},
  urldate = {2021-08-02},
  abstract = {M-dwarf stars are the most numerous stars in the Universe; they span a wide range in mass and are in the focus of ongoing and planned exoplanet surveys. To investigate and understand their physical nature, detailed spectral information and accurate stellar models are needed. We use a new synthetic atmosphere model generation and compare model spectra to observations. To test the model accuracy, we compared the models to four benchmark stars with atmospheric parameters for which independent information from interfer-ometric radius measurements is available. We used {$\chi$} 2-based methods to determine parameters from high-resolution spectroscopic observations. Our synthetic spectra are based on the new PHOENIX grid that uses the ACES description for the equation of state. This is a model generation expected to be especially suitable for the low-temperature atmospheres. We identified suitable spectral tracers of atmospheric parameters and determined the uncertainties in T eff , log g, and [Fe/H] resulting from degeneracies between parameters and from shortcomings of the model atmospheres. The inherent uncertainties we find are {$\sigma$} T eff = 35 K, {$\sigma$} log g = 0.14, and {$\sigma$} [Fe/H] = 0.11. The new model spectra achieve a reliable match to our observed data; our results for T eff and log g are consistent with literature values to within 1{$\sigma$}. However, metallicities reported from earlier photometric and spectroscopic calibrations in some cases disagree with our results by more than 3{$\sigma$}. A possible explanation are systematic errors in earlier metallicity determinations that were based on insufficient descriptions of the cool atmospheres. At this point, however, we cannot definitely identify the reason for this discrepancy, but our analysis indicates that there is a large uncertainty in the accuracy of M-dwarf parameter estimates.},
  keywords = {atmospheres-brown dwarfs-line,formation-stars,low-mass-line,notion,notion-database,profiles-techniques,spectroscopic,stars},
  file = {/Users/lbugnet/Zotero/storage/HEPIN5EX/full-text.pdf}
}

@article{Pavlov2019,
  title = {Random Forests},
  author = {Pavlov, Yu L.},
  year = {2019},
  journal = {Random Forests},
  pages = {1--122},
  doi = {10.1007/978-3-662-56776-0_10},
  abstract = {The role of probabilistic methods in discrete mathematics cannot be overestimated. By defining the probability measure on a set of the studied combinatorial objects various numerical characteristics of these objects can be considered as random variables and studied using the methods of probability theory. The advantage of this approach is the well-developed probabilistic analytic techniques that allow us in many cases to obtain results, the proof of which by other methods appears too complicated, if indeed it is at all possible. The application of probabilistic methods is connected with extensive use of the terminology of probability theory. The reader will easily understand however that one speaks in fact about solving enumerative problems of discrete analysis. One of the primary research lines is the study of the limit properties of combinatorial objects manifested at the unlimited increase of the number of elements comprising such objects. It is often possible to represent the distributions of the characteristics of combinatorial objects as conditional distributions of the sums of independent random variables so that they can be studied using asymptotic methods in probability theory, namely limit theorems for sums of independent random variables.},
  isbn = {9783110941975},
  keywords = {classification,ensemble,notion,notion-database,regression},
  file = {/Users/lbugnet/Zotero/storage/959UNFD6/Pavlov - 2019.pdf}
}

@article{Paxton2011,
  title = {Modules for {{Experiments}} in {{Stellar Astrophysics}} ({{MESA}})},
  author = {Paxton, Bill and Bildsten, Lars and Dotter, Aaron and Herwig, Falk and Lesaffre, Pierre and Timmes, Frank},
  year = {2011},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {192},
  number = {1},
  eprint = {1009.1622},
  pages = {1--110},
  issn = {00670049},
  doi = {10.1088/0067-0049/192/1/3},
  abstract = {Stellar physics and evolution calculations enable a broad range of research in astrophysics. Modules for Experiments in Stellar Astrophysics (MESA) is a suite of open source, robust, efficient, thread-safe libraries for a wide range of applications in computational stellar astrophysics. A one-dimensional stellar evolution module, MESA star, combines many of the numerical and physics modules for simulations of a wide range of stellar evolution scenarios ranging from very low mass to massive stars, including advanced evolutionary phases. MESA star solves the fully coupled structure and composition equations simultaneously. It uses adaptive mesh refinement and sophisticated timestep controls, and supports shared memory parallelism based on OpenMP. State-of-the-art modules provide equation of state, opacity, nuclear reaction rates, element diffusion data, and atmosphere boundary conditions. Each module is constructed as a separate Fortran 95 library with its own explicitly defined public interface to facilitate independent development. Several detailed examples indicate the extensive verification and testing that is continuously performed and demonstrate the wide range of capabilities that MESA possesses. These examples include evolutionary tracks of very low mass stars, brown dwarfs, and gas giant planets to very old ages; the complete evolutionary track of a 1 M{$\odot$} star from the pre-main sequence (PMS) to a cooling white dwarf; the solar sound speed profile; the evolution of intermediate-mass stars through the He-core burning phase and thermal pulses on the He-shell burning asymptotic giant branch phase; the interior structure of slowly pulsating B Stars and Beta Cepheids; the complete evolutionary tracks of massive stars from the PMS to the onset of core collapse; mass transfer from stars undergoing Roche lobe overflow; and the evolution of helium accretion onto a neutron star. MESA can be downloaded from the project Web site (http://mesa.sourceforge.net/). \textcopyright{} 2011. The American Astronomical Society. All rights reserved. Printed in the U.S.A.},
  archiveprefix = {arxiv},
  keywords = {Methods: numerical,notion,notion-database,Stars: evolution,Stars: general},
  file = {/Users/lbugnet/Zotero/storage/GTS6WTH2/Paxton et al. - 2011.pdf}
}

@article{Paxton2013,
  title = {Modules for Experiments in Stellar Astrophysics ({{MESA}}): {{Planets}}, Oscillations, Rotation, and Massive Stars},
  author = {Paxton, Bill and Cantiello, Matteo and Arras, Phil and Bildsten, Lars and Brown, Edward F. and Dotter, Aaron and Mankovich, Christopher and Montgomery, M. H. and Stello, Dennis and Timmes, F. X. and Townsend, Richard},
  year = {2013},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {208},
  number = {1},
  eprint = {1301.0319},
  issn = {00670049},
  doi = {10.1088/0067-0049/208/1/4},
  abstract = {We substantially update the capabilities of the open source software package Modules for Experiments in Stellar Astrophysics (MESA), and its one-dimensional stellar evolution module, MESA star. Improvements in MESA star's ability to model the evolution of giant planets now extends its applicability down to masses as low as one-tenth that of Jupiter. The dramatic improvement in asteroseismology enabled by the space-based Kepler and CoRoT missions motivates our full coupling of the ADIPLS adiabatic pulsation code with MESA star. This also motivates a numerical recasting of the Ledoux criterion that is more easily implemented when many nuclei are present at non-negligible abundances. This impacts the way in which MESA star calculates semi-convective and thermohaline mixing. We exhibit the evolution of 3-8 M{$\odot$} stars through the end of core He burning, the onset of He thermal pulses, and arrival on the white dwarf cooling sequence. We implement diffusion of angular momentum and chemical abundances that enable calculations of rotating-star models, which we compare thoroughly with earlier work. We introduce a new treatment of radiation-dominated envelopes that allows the uninterrupted evolution of massive stars to core collapse. This enables the generation of new sets of supernovae, long gamma-ray burst, and pair-instability progenitor models. We substantially modify the way in which MESA star solves the fully coupled stellar structure and composition equations, and we show how this has improved the scaling of MESA's calculational speed on multi-core processors. Updates to the modules for equation of state, opacity, nuclear reaction rates, and atmospheric boundary conditions are also provided. We describe the MESA Software Development Kit that packages all the required components needed to form a unified, maintained, and well-validated build environment for MESA. We also highlight a few tools developed by the community for rapid visualization of MESA star results. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,methods: numerical,notion,notion-database,planets and satellites: physical evolution,stars: evolution,stars: massive,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/4XJDAX8Q/Paxton et al. - 2013.pdf}
}

@article{Paxton2019,
  title = {Modules for {{Experiments}} in {{Stellar Astrophysics}} ({{MESA}}): {{Pulsating Variable Stars}}, {{Rotation}}, {{Convective Boundaries}}, and {{Energy Conservation}}},
  shorttitle = {Modules for {{Experiments}} in {{Stellar Astrophysics}} ({{MESA}})},
  author = {Paxton, Bill and Smolec, R. and Schwab, Josiah and Gautschy, A. and Bildsten, Lars and Cantiello, Matteo and Dotter, Aaron and Farmer, R. and Goldberg, Jared A. and Jermyn, Adam S. and Kanbur, S. M. and Marchant, Pablo and Thoul, Anne and Townsend, Richard H. D. and Wolf, William M. and Zhang, Michael and Timmes, F. X.},
  year = {2019},
  month = jul,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {243},
  pages = {10},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/ab2241},
  urldate = {2023-10-12},
  abstract = {We update the capabilities of the open-knowledge software instrument Modules for Experiments in Stellar Astrophysics (MESA). RSP is a new functionality in MESAstar that models the nonlinear radial stellar pulsations that characterize RR Lyrae, Cepheids, and other classes of variable stars. We significantly enhance numerical energy conservation capabilities, including during mass changes. For example, this enables calculations through the He flash that conserve energy to better than 0.001\%. To improve the modeling of rotating stars in MESA, we introduce a new approach to modifying the pressure and temperature equations of stellar structure, as well as a formulation of the projection effects of gravity darkening. A new scheme for tracking convective boundaries yields reliable values of the convective core mass and allows the natural emergence of adiabatic semiconvection regions during both core hydrogen- and helium-burning phases. We quantify the parallel performance of MESA on current-generation multicore architectures and demonstrate improvements in the computational efficiency of radiative levitation. We report updates to the equation of state and nuclear reaction physics modules. We briefly discuss the current treatment of fallback in core-collapse supernova models and the thermodynamic evolution of supernova explosions. We close by discussing the new MESA Testhub software infrastructure to enhance source code development.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: general,stars: interiors,stars: oscillations:  including pulsations,stars: rotation,stars: variables: general},
  annotation = {ADS Bibcode: 2019ApJS..243...10P},
  file = {/Users/lbugnet/Zotero/storage/RLYQP5DT/Paxton et al. - 2019 - Modules for Experiments in Stellar Astrophysics (M.pdf}
}

@article{Paz-Chinchon2015,
  title = {The Rotational Behavior of Kepler Stars with Planets},
  author = {{Paz-Chinch{\'o}n}, F. and Le{\~a}o, I. C. and Bravo, J. P. and De Freitas, D. B. and Ferreira Lopes, C. E. and Alves, S. and Catelan, M. and Canto Martins, B. L. and De Medeiros, J. R.},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {803},
  number = {2},
  eprint = {1502.05051},
  pages = {1--11},
  issn = {15384357},
  doi = {10.1088/0004-637X/803/2/69},
  abstract = {We analyzed the host stars of the present sample of confirmed planets detected by Kepler and Kepler Objects of Interest to compute new photometric rotation periods and to study the behavior of their angular momentum. Lomb-Scargle periodograms and wavelet maps were computed for 3807 stars. For 540 of these stars, we were able to detect rotational modulation of the light curves at a significance level of greater than 99\%. For 63 of these 540 stars, no rotation measurements were previously available in the literature. According to the published masses and evolutionary tracks of the stars in this sample, the sample is composed of M- to F-type stars (with masses of 0.48-1.53 M ) with rotation periods that span a range of 2-89 days. These periods exhibit an excellent agreement with those previously reported (for the stars for which such values are available), and the observed rotational period distribution strongly agrees with theoretical predictions. Furthermore, for the 540 sources considered here, the stellar angular momentum provides an important test of Kraft's relation based on the photometric rotation periods. Finally, this study directly contributes in a direct approach to our understanding of how angular momentum is distributed between the host star and its (detected) planetary system; the role of angular momentum exchange in such systems is an unavoidable piece of the stellar rotation puzzle.},
  archiveprefix = {arxiv},
  keywords = {General - stars,Hertzsprung-Russell and C-M diagrams - stars,Kinematics and dynamics - stars,notion,notion-database,Rotation Supporting material},
  file = {/Users/lbugnet/Zotero/storage/7NX3WKUF/Paz-Chinchón et al. - 2015.pdf}
}

@article{Pech2006,
  title = {The {{ZZ Ceti}} Star {{G}} 185-32: New Insight from Asteroseismology},
  shorttitle = {The {{ZZ Ceti}} Star {{G}} 185-32},
  author = {Pech, D. and Vauclair, G.},
  year = {2006},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {453},
  number = {1},
  pages = {219--227},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361:20054370},
  urldate = {2023-10-14},
  abstract = {One of the brightest pulsating DA white dwarfs (ZZ Ceti stars), G 185-32, shows 19 periods in its power spectrum, from 71 s to 651 s. Its short periods are among the shortest ones observed in a ZZ Ceti star. The one at 141.9 s shows an amplitude which does not vary with wavelength, in contrast with what the linear theory predicts for = 1 or = 2 non-radial g-modes. The mass and Teff of G 185-32 are well constrained by spectroscopic observations and parallax measurement. The aim of the present paper is to take advantage of this rich observational background to derive the fundamental parameters of the star from asteroseismology. We computed a grid of realistic models for G 185-32 and the periods of their adiabatic = 1 and = 2 non-radial g-modes. We determined the model which fits best the observations. We identify 14 periods as real modes and determine their , k, and m values. We show that the remaining 5 periods are linear combinations.We find that G 185-32 oscillates mostly according to = 2 modes. We present a new hypothesis to account for the peculiar behaviour of the 141.9 s mode's amplitude and suggest that it is a true mode interfering with higher degree modes, involving a possible triplet resonance. We determine the main parameters of G 185-32: its total mass M{${_\ast}$} = 0.638 ({$\pm$}0.007) M , its hydrogen mass fraction MH = 1.70 ({$\pm$}0.10) \texttimes{} 10-4 M{${_\ast}$}, which implies a helium mass fraction of {$\approx$}10-2 M{${_\ast}$}, its Teff = 12 280 ({$\pm$})80 K, and estimate its rotation period to be 14.5 h.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/BIHGFC8P/Pech and Vauclair - 2006 - The ZZ Ceti star G 185-32 new insight from astero.pdf}
}

@article{Pedregosa2011,
  title = {Scikit-Learn: {{Machine Learning}} in {{Python}}},
  author = {Pedregosa, Fabian and Michel, Vincent and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Vanderplas, Jake and Cournapeau, David and Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Thirion, Bertrand and Grisel, Olivier and Dubourg, Vincent and Passos, Alexandre and Brucher, Matthieu and Perrot, Matthieu and Duchesnay, {\relax Fr{\'e}}douard},
  year = {2011},
  journal = {Journal of Machine Learning Research},
  volume = {12},
  pages = {2825--2830},
  urldate = {2020-03-20},
  abstract = {Scikit-learn is a Python module integrating a wide range of state-of-the-art machine learning algorithms for medium-scale supervised and unsupervised problems. This package focuses on bringing machine learning to non-specialists using a general-purpose high-level language. Emphasis is put on ease of use, performance, documentation, and API consistency. It has minimal dependencies and is distributed under the simplified BSD license, encouraging its use in both academic and commercial settings. Source code, binaries, and documentation can be downloaded from http://scikit-learn.sourceforge.net.},
  keywords = {model selection,notion,notion-database,Python,supervised learning,unsupervised learning},
  file = {/Users/lbugnet/Zotero/storage/KXK5UQ3Q/full-text.pdf}
}

@article{Pelisoli2018,
  title = {The {{sdA}} Problem - {{II}}. {{Photometric}} and Spectroscopic Follow-Up},
  author = {Pelisoli, Ingrid and Kepler, S. O. and Koester, D. and Castanheira, B. G. and Romero, A. D. and Fraga, L.},
  year = {2018},
  month = jul,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {478},
  pages = {867--884},
  issn = {0035-8711},
  doi = {10.1093/mnras/sty1101},
  urldate = {2023-10-09},
  abstract = {The spectral classification `subdwarf A' (sdA) is given to stars showing H-rich spectra and sub-main-sequence surface gravities, but effective temperature lower than the zero-age horizontal branch. Their evolutionary origin is an enigma. In this work, we discuss the results of follow-up observations of selected sdAs. We obtained time-resolved spectroscopy for 24 objects and time-series photometry for another 19 objects. For two targets, we report both spectroscopy and photometry observations. We confirm seven objects to be new extremely low-mass white dwarfs (ELMs), one of which is a known eclipsing star. We also find the eighth member of the pulsating ELM class.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: general,stars: evolution,subdwarfs,white dwarfs},
  annotation = {ADS Bibcode: 2018MNRAS.478..867P},
  file = {/Users/lbugnet/Zotero/storage/JR3Z9E37/Pelisoli et al. - 2018 - The sdA problem - II. Photometric and spectroscopi.pdf}
}

@article{Pelisoli2019,
  title = {Gaia {{Data Release}} 2 Catalogue of Extremely Low-Mass White Dwarf Candidates},
  author = {Pelisoli, Ingrid and Vos, Joris},
  year = {2019},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {488},
  pages = {2892--2903},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz1876},
  urldate = {2023-10-02},
  abstract = {Extremely low-mass white dwarf stars (ELMs) are M {$<$} 0.3 M{$\odot$} helium-core white dwarfs born either as a result of a common-envelope phase or after a stable Roche lobe overflow episode in a multiple system. The Universe is not old enough for ELMs to have formed through single-star evolution channels. As remnants of binary evolution, ELMs can shed light onto the poorly understood phase of common-envelope evolution and provide constraints to the physics of mass accretion. Most known ELMs will merge in less than a Hubble time, providing an important contribution to the signal to be detected by upcoming space-based gravitational wave detectors. There are currently less than 150 known ELMs; most were selected by colour, focusing on hot objects, in a magnitude-limited survey of the Northern hemisphere only. Recent theoretical models have predicted a much larger space density for ELMs than estimated observationally based on this limited sample. In order to perform meaningful comparisons with theoretical models and test their predictions, a larger well-defined sample is required. In this work, we present a catalogue of ELM candidates selected from the second data release of Gaia (DR2). We have used predictions from theoretical models and analysed the properties of the known sample to map the space spanned by ELMs in the Gaia Hertzsprung-Russell diagram. Defining a set of colour cuts and quality flags, we have obtained a final sample of 5762 ELM candidates down to Teff {$\approx$} 5000 K.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: close,catalogues,surveys,white dwarfs},
  annotation = {ADS Bibcode: 2019MNRAS.488.2892P},
  file = {/Users/lbugnet/Zotero/storage/92FU8TD8/Pelisoli and Vos - 2019 - Gaia Data Release 2 catalogue of extremely low-mas.pdf}
}

@article{Pelisoli2019a,
  title = {Gaia {{Data Release}} 2 Catalogue of Extremely Low-Mass White Dwarf Candidates},
  author = {Pelisoli, Ingrid and Vos, Joris},
  year = {2019},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {488},
  pages = {2892--2903},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz1876},
  urldate = {2023-10-09},
  abstract = {Extremely low-mass white dwarf stars (ELMs) are M {$<$} 0.3 M{$\odot$} helium-core white dwarfs born either as a result of a common-envelope phase or after a stable Roche lobe overflow episode in a multiple system. The Universe is not old enough for ELMs to have formed through single-star evolution channels. As remnants of binary evolution, ELMs can shed light onto the poorly understood phase of common-envelope evolution and provide constraints to the physics of mass accretion. Most known ELMs will merge in less than a Hubble time, providing an important contribution to the signal to be detected by upcoming space-based gravitational wave detectors. There are currently less than 150 known ELMs; most were selected by colour, focusing on hot objects, in a magnitude-limited survey of the Northern hemisphere only. Recent theoretical models have predicted a much larger space density for ELMs than estimated observationally based on this limited sample. In order to perform meaningful comparisons with theoretical models and test their predictions, a larger well-defined sample is required. In this work, we present a catalogue of ELM candidates selected from the second data release of Gaia (DR2). We have used predictions from theoretical models and analysed the properties of the known sample to map the space spanned by ELMs in the Gaia Hertzsprung-Russell diagram. Defining a set of colour cuts and quality flags, we have obtained a final sample of 5762 ELM candidates down to Teff {$\approx$} 5000 K.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: close,catalogues,surveys,white dwarfs},
  annotation = {ADS Bibcode: 2019MNRAS.488.2892P},
  file = {/Users/lbugnet/Zotero/storage/ADVL7IGJ/Pelisoli and Vos - 2019 - Gaia Data Release 2 catalogue of extremely low-mas.pdf}
}

@article{Perez-Ortiz2017,
  title = {Machine Learning Techniques to Select {{Be}} Star Candidates: {{An}} Application in the {{OGLE-IV Gaia}} South Ecliptic Pole Field},
  author = {{P{\'e}rez-Ortiz}, M. F. and {Garc{\'i}a-Varela}, A. and Quiroz, A. J. and Sabogal, B. E. and Hern{\'a}ndez, J.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {605},
  eprint = {1707.04560},
  pages = {1--14},
  issn = {14320746},
  doi = {10.1051/0004-6361/201628937},
  abstract = {Context. Optical and infrared variability surveys produce a large number of high quality light curves. Statistical pattern recognition methods have provided competitive solutions for variable star classification at a relatively low computational cost. In order to perform supervised classification, a set of features is proposed and used to train an automatic classification system. Quantities related to the magnitude density of the light curves and their Fourier coefficients have been chosen as features in previous studies. However, some of these features are not robust to the presence of outliers and the calculation of Fourier coefficients is computationally expensive for large data sets. Aims. We propose and evaluate the performance of a new robust set of features using supervised classifiers in order to look for new Be star candidates in the OGLE-IV Gaia south ecliptic pole field. Methods. We calculated the proposed set of features on six types of variable stars and also on a set of Be star candidates reported in the literature. We evaluated the performance of these features using classification trees and random forests along with the K-nearest neighbours, support vector machines, and gradient boosted trees methods. We tuned the classifiers with a 10-fold cross-validation and grid search. We then validated the performance of the best classifier on a set of OGLE-IV light curves and applied this to find new Be star candidates. Results. The random forest classifier outperformed the others. By using the random forest classifier and colours criteria we found 50 Be star candidates in the direction of the Gaia south ecliptic pole field, four of which have infrared colours that are consistent with Herbig Ae/Be stars. Conclusions. Supervised methods are very useful in order to obtain preliminary samples of variable stars extracted from large databases. As usual, the stars classified as Be stars candidates must be checked for the colours and spectroscopic characteristics expected for them.},
  archiveprefix = {arxiv},
  keywords = {Catalogs,Methods: statistical,notion,notion-database,{Stars: emission-line, Be},Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/3AG8PX62/Pérez-Ortiz et al. - 2017.pdf}
}

@article{PerezHernandez2011,
  title = {Angular Momentum Transfer between Oscillations and Rotation in Subdwarf {{B}} Hybrid Pulsators},
  author = {P{\'e}rez Hern{\'a}ndez, F. and Oreiro, R. and Hu, H.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {535},
  pages = {1--10},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117435},
  abstract = {Context. Subdwarf B pulsators exhibit pressure (p) and/or gravity (g) modes. Their frequency spectra range from very simple, with few frequencies, to very rich, with more than fifty peaks in some cases. Balloon09 is a hybrid pulsating subdwarf B, showing a great number of p-and g-modes including triplet and quintuplet-like structures, which are interpreted as p-mode frequency splittings caused by stellar rotation. Photometric observations undertaken in two subsequent years revealed a change in these rotational splittings of 0.24-0.58 {$\mu$}Hz/yr. Aims. We analyse the possibility of angular momentum interchange between stellar rotation and internal gravity waves as a mechanism for the observed rotational splitting variations. Methods. The expected change in the rotational splitting of eigenmodes resulting from this mechanism are computed in the non-adiabatic linear approximation for a stellar structure model that is representative of the target star. Balloon09 is a particularly suitable candidate for our study because the change in the rotational splittings are proportional to the amplitude squared of the g-modes which, in this case, can be estimated from the observations. Results. We find that this mechanism is able to predict changes in the splittings that can be of the same order of magnitude as the observed variations. \textcopyright{} 2011 ESO.},
  keywords = {notion,notion-database,stars: horizontal-branch,stars: oscillations,stars: rotation,subdwarfs},
  file = {/Users/lbugnet/Zotero/storage/MYAUSVUP/Pérez Hernández, Oreiro, Hu - 2011.pdf}
}

@article{Pesnell2012,
  title = {The {{Solar Dynamics Observatory}} ({{SDO}})},
  author = {Pesnell, W. Dean and Thompson, B. J. and Chamberlin, P. C.},
  year = {2012},
  journal = {Solar Physics},
  volume = {275},
  number = {1-2},
  pages = {3--15},
  issn = {00380938},
  doi = {10.1007/s11207-011-9841-3},
  abstract = {The Solar Dynamics Observatory (SDO) was launched on 11 February 2010 at 15:23 UT from Kennedy Space Center aboard an Atlas V 401 (AV-021) launch vehicle. A series of apogee-motor firings lifted SDO from an initial geosynchronous transfer orbit into a circular geosynchronous orbit inclined by 28\textdegree{} about the longitude of the SDO-dedicated ground station in New Mexico. SDO began returning science data on 1 May 2010. SDO is the first space-weather mission in NASA's Living With a Star (LWS) Program. SDO's main goal is to understand, driving toward a predictive capability, those solar variations that influence life on Earth and humanity's technological systems. The SDO science investigations will determine how the Sun's magnetic field is generated and structured, how this stored magnetic energy is released into the heliosphere and geospace as the solar wind, energetic particles, and variations in the solar irradiance. Insights gained from SDO investigations will also lead to an increased understanding of the role that solar variability plays in changes in Earth's atmospheric chemistry and climate. The SDO mission includes three scientific investigations (the Atmospheric Imaging Assembly (AIA), Extreme Ultraviolet Variability Experiment (EVE), and Helioseismic and Magnetic Imager (HMI)), a spacecraft bus, and a dedicated ground station to handle the telemetry. The Goddard Space Flight Center built and will operate the spacecraft during its planned five-year mission life; this includes: commanding the spacecraft, receiving the science data, and forwarding that data to the science teams. The science investigations teams at Stanford University, Lockheed Martin Solar Astrophysics Laboratory (LMSAL), and University of Colorado Laboratory for Atmospheric and Space Physics (LASP) will process, analyze, distribute, and archive the science data. We will describe the building of SDO and the science that it will provide to NASA. \textcopyright{} 2011 The Author(s).},
  isbn = {1120701198413},
  keywords = {Coronal,Helioseismology,notion,notion-database,SDO,Solar cycle,Space weather},
  file = {/Users/lbugnet/Zotero/storage/CSREC3TD/Pesnell, Thompson, Chamberlin - 2012.pdf}
}

@article{Peterson1983,
  title = {The Rotation of Horizontal-Branch Stars. {{II}} - {{Members}} of the Globular Clusters {{M3}}, {{M5}}, and {{M13}}},
  author = {Peterson, R. C.},
  year = {1983},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {275},
  pages = {737},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/161571},
  urldate = {2020-07-13},
  keywords = {Angular Momentum,Astrophysics,Cross Correlation,Globular Clusters,Horizontal Branch Stars,notion,notion-database,Radial Velocity,Spectral Line Width,Stellar Evolution,Stellar Rotation,Stellar Spectra}
}

@article{Petit2003,
  title = {Magnetic Topology and Surface Differential Rotation on the {{K1}} Subgiant of the {{RS CVn}} System {{HR}} 1099},
  author = {Petit, P. and Donati, J. -F. and Wade, G. A. and Landstreet, J. D. and Bagnulo, S. and Lueftinger, T. and Sigut, T. A. A. and Shorlin, S. L. S. and Strasser, S. and Auriere, M. and Oliveira, J. M.},
  year = {2003},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {348},
  number = {4},
  eprint = {astro-ph/0312238},
  pages = {1175--1190},
  publisher = {{Oxford University Press}},
  doi = {10.1111/j.1365-2966.2004.07420.x},
  urldate = {2020-07-12},
  abstract = {We present here spectropolarimetric observations of the RS CVn system HR 1099 (V711 Tau) secured from 1998 February to 2002 January with the spectropolarimeter MuSiCoS at the Telescope Bernard Lyot (Observatoire du Pic du Midi, France). We apply Zeeman-Doppler Imaging and reconstruct brightness and magnetic surface topologies of the K1 primary subgiant of the system, at five different epochs. We confirm the presence of large, axisymmetric regions where the magnetic field is mainly azimuthal, providing further support to the hypothesis that dynamo processes may be distributed throughout the whole convective zone in this star. We study the short-term evolution of surface structures from a comparison of our images with observations secured at close-by epochs by Donati et al. (2003) at the Anglo-Australian Telescope. We conclude that the small-scale brightness and magnetic patterns undergo major changes within a timescale of 4 to 6 weeks, while the largest structures remain stable over several years. We report the detection of a weak surface differential rotation (both from brightness and magnetic tracers) indicating that the equator rotates faster than the pole with a difference in rotation rate between the pole and the equator about 4 times smaller than that of the Sun. This result suggests that tidal forces also impact the global dynamic equilibrium of convective zones in cool active stars.},
  archiveprefix = {arxiv},
  keywords = {Binaries: close,notion,notion-database,Polarization,Stars: activity,Stars: imaging,Stars: magnetic fields,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/REBD6QIB/full-text.pdf}
}

@article{Petit2004,
  title = {Photospheric Magnetic Field and Surface Differential Rotation of the {{FK Com}} Star {{HD}} 199178},
  author = {Petit, P. and Donati, J. -F. and Oliveira, J. M. and Auriere, M. and Bagnulo, S. and Landstreet, J. D. and Lignieres, F. and Lueftinger, T. and Marsden, S. and Mouillet, D. and Paletou, F. and Strasser, S. and Toque, N. and Wade, G. A.},
  year = {2004},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {351},
  number = {3},
  eprint = {astro-ph/0403284},
  pages = {826--844},
  doi = {10.1111/j.1365-2966.2004.07827.x},
  urldate = {2020-07-12},
  abstract = {We present spectropolarimetric observations of the FK Com star HD 199178 obtained between 1998 December and 2003 August at the Telescope Bernard Lyot (Observatoire du Pic du Midi, France). We report the detection of a photospheric magnetic field and reconstruct its distribution by means of Zeeman-Doppler Imaging. We observe large regions where the magnetic field is mainly azimuthal, suggesting that the dynamo processes generating the magnetic activity of HD 199178 may be active very close to the stellar surface. We investigate the rapid evolution of surface brightness and magnetic structures from a continuous monitoring of the star over several weeks in 2002 and 2003. We report that significant changes occur in the distribution of cool spots and magnetic regions on typical timescales of the order of 2 weeks. Our spectropolarimetric observations also suggest that the surface of HD 199178 is sheared by differential rotation, with a difference in rotation rate between equatorial and polar regions of the order of 1.5 times that of the Sun.},
  archiveprefix = {arxiv},
  keywords = {Magnetic fields,notion,notion-database,Polarization,Stars: activity,Stars: imaging,Stars: individual: HD 199178,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/DEX75TEW/full-text.pdf}
}

@article{Petit2008,
  title = {Toroidal versus Poloidal Magnetic Fields in {{Sun-like}} Stars: {{A}} Rotation Threshold},
  author = {Petit, P. and Dintrans, B. and Solanki, S. K. and Donati, J. F. and Auri{\`e}re, M. and Ligni{\`e}res, F. and Morin, J. and Paletou, F. and Ramirez, J. and Catala, C. and Fares, R.},
  year = {2008},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {388},
  number = {1},
  pages = {80--88},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2008.13411.x},
  abstract = {From a set of stellar spectropolarimetric observations, we report the detection of surface magnetic fields in a sample of four solar-type stars, namely HD 73350, HD 76151, HD 146233 (18 Sco) and HD 190771. Assuming that the observed variability of polarimetric signal is controlled by stellar rotation, we establish the rotation periods of our targets, with values ranging from 8.8 d (for HD 190771) to 22.7 d (for HD 146233). Apart from rotation, fundamental parameters of the selected objects are very close to the Sun's, making this sample a practical basis to investigate the specific impact of rotation on magnetic properties of Sun-like stars. We reconstruct the large-scale magnetic geometry of the targets as a low-order ({$\mathscr{l}$} {$<$}10) spherical harmonic expansion of the surface magnetic field. From the set of magnetic maps, we draw two main conclusions. (i) The magnetic energy of the large-scale field increases with rotation rate. The increase in chromospheric emission with the mean magnetic field is flatter than observed in the Sun. Since the chromospheric flux is also sensitive to magnetic elements smaller than those contributing to the polarimetric signal, this observation suggests that a larger fraction of the surface magnetic energy is stored in large scales as rotation increases. (ii) Whereas the magnetic field is mostly poloidal for low rotation rates, more rapid rotators host a large-scale toroidal component in their surface field. From our observations, we infer that a rotation period lower than {$\approx$}12 d is necessary for the toroidal magnetic energy to dominate over the poloidal component. \textcopyright{} 2008 The Authors. Journal compilation \textcopyright{} 2008 RAS.},
  keywords = {notion,notion-database,Stars: individual: HD 146233,Stars: individual: HD 190771,Stars: individual: HD 73350,Stars: individual: HD 76151,Stars: magnetic fields,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/2GJAAHRI/Petit et al. - 2008.pdf}
}

@article{Petitdemange2023,
  title = {Spin-down by Dynamo Action in Simulated Radiative Stellar Layers},
  author = {Petitdemange, Ludovic and Marcotte, Florence and Gissinger, Christophe},
  year = {2023},
  month = jan,
  journal = {Science},
  volume = {379},
  pages = {300--303},
  issn = {0036-8075},
  doi = {10.1126/science.abk2169},
  urldate = {2023-10-18},
  abstract = {The evolution of a star is influenced by its internal rotation dynamics through transport and mixing mechanisms, which are poorly understood. Magnetic fields can play a role in transporting angular momentum and chemical elements, but the origin of magnetism in radiative stellar layers is unclear. Using global numerical simulations, we identify a subcritical transition from laminar flow to turbulence caused by the generation of a magnetic dynamo. Our results have many properties of the theoretically proposed Tayler-Spruit dynamo mechanism, which strongly enhances transport of angular momentum in radiative zones. The dynamo generates deep toroidal fields that are screened by the stellar outer layers. This mechanism could produce strong magnetic fields inside radiative stars without an observable field on their surface.},
  keywords = {ASTRONOMY,Astrophysics - Solar and Stellar Astrophysics,PHYSICS},
  annotation = {ADS Bibcode: 2023Sci...379..300P},
  file = {/Users/lbugnet/Zotero/storage/5C9EQIYH/Petitdemange et al. - 2023 - Spin-down by dynamo action in simulated radiative .pdf}
}

@article{Pevtsov2013,
  title = {{{ON POSSIBLE VARIATIONS OF BASAL Ca}} Ii {{K CHROMOSPHERIC LINE PROFILES WITH THE SOLAR CYCLE}}},
  author = {Pevtsov, Alexei A and Bertello, Luca and Uitenbroek, Han},
  year = {2013},
  journal = {The Astrophysical Journal},
  volume = {767},
  number = {6pp},
  pages = {56},
  doi = {10.1088/0004-637X/767/1/56},
  urldate = {2020-07-02},
  abstract = {We use daily observations of the Ca ii K line profiles of the Sun-as-a-star taken with the Integrated Sunlight Spectrometer from 2006 December through 2011 July to deconvolve the contributions from the quiet (basal) chromosphere and with magnetic network/plage areas. The 0.5 \AA{} emission index computed from basal profiles shows a significantly reduced modulation (as compared with one derived from the observed profiles) corresponding to the Sun's rotation. For basal contribution of the Ca ii K line, the peak in power spectrum corresponding to solar rotation is broad and not well defined. Power spectra for the plage contribution show two narrow well-defined peaks corresponding to solar rotation at two distinct latitudes, in agreement with the latitudinal distribution of activity on the Sun at the end of Cycle 23 and beginning of Cycle 24. We use the lack of a signature of solar rotation in the basal (quiet Sun) component as an indication of a successful removal of the active Sun (plage) component. Even though the contribution from solar activity is removed from the basal line profiles, we find a weak dependency of intensity in the line core (K3) of basal profiles with the phase of the solar cycle. Such dependency could be the result of changes in thermal properties of basal chromosphere with the solar cycle. As an alternative explanation, we also discuss a possibility that the basal component does not change with the phase of the solar cycle.},
  keywords = {activity-Sun,chromosphere,notion,notion-database,Sun},
  file = {/Users/lbugnet/Zotero/storage/GG5UILJ6/full-text.pdf}
}

@article{Philidet2019,
  title = {Magnetohydrodynamics of Stably Stratified Regions in Planets and Stars},
  author = {Philidet, J. and Gissinger, C. and Ligni{\`e}res, F. and Petitdemange, L.},
  year = {2019},
  journal = {Geophysical and Astrophysical Fluid Dynamics},
  volume = {00},
  number = {00},
  eprint = {1910.04092},
  pages = {1--18},
  issn = {10290419},
  doi = {10.1080/03091929.2019.1670827},
  abstract = {Stably stratified layers are present in stellar interiors (radiative zones) as well as planetary interiors\textendash recent observations and theoretical studies of the Earth's magnetic field seem to indicate the presence of a thin, stably stratified layer at the top of the liquid outer core. We present direct numerical simulations of this region, which is modelled as an axisymmetric spherical Couette flow for a stably stratified fluid embedded in a dipolar magnetic field. For strong magnetic fields, a super-rotating shear layer, rotating nearly 30\% faster than the imposed rotation rate difference between the inner convective dynamo region and the outer boundary, is generated in the stably stratified region. In the Earth context, and contrary to what was previously believed, we show that this super-rotation may extend towards the Earth magnetostrophic regime if the density stratification is sufficiently large. The corresponding differential rotation triggers magnetohydrodynamic instabilities and waves in the stratified region, which feature growth rates comparable to the observed timescale for geomagnetic secular variations and jerks. In the stellar context, we perform a linear analysis which shows that similar instabilities are likely to arise, and we argue that it may play a role in explaining the observed magnetic dichotomy among intermediate-mass stars.},
  archiveprefix = {arxiv},
  keywords = {Direct numerical simulations,earth: stably stratified layer,magnetic desert,notion,notion-database,outer core,stars: radiative zones},
  file = {/Users/lbugnet/Zotero/storage/BDYC8DZB/Philidet et al. - 2019.pdf}
}

@article{Piau2009,
  title = {Impact of the Physical Processes in the Modeling of {{HD49933}}},
  author = {Piau, L. and {Turck-Chi{\`e}ze}, S. and Duez, V. and Stein, R. F.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {506},
  number = {1},
  pages = {175--181},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911947},
  abstract = {Context. On its asteroseismic side, the initial run of CoRoT was partly devoted to the solar like star HD49933. The eigenmodes of this F dwarf have been observed with unprecedented accuracy. Aims. We investigate quantitatively the impact of changes in the modeling parameters like mass and composition. More importantly we investigate how a sophisticated physics affects the seismological picture of HD49933.We consider the effects of diffusion, rotation and the changes in convection efficiency. Methods. We use the CESAM stellar evolution code coupled to the ADIPLS adiabatic pulsation package to build secular models and their associated oscillation frequencies. We also exploited the hydrodynamical code STAGGER to perform surface convection calculations. The seismic variables used in this work are: the large frequency separation, the derivative of the surface phase shift, and the eigenfrequencies v{$\mathscr{l}$}=0,n=14 and v{$\mathscr{l}$}=0,n=27. Results. Mass and uncertainties on the composition have much larger impacts on the seismic variables we consider than the rotation. The derivative of the surface phase shift is a promising variable for the determination of the helium content. The seismological variables of HD49933 are sensitive to the assumed solar composition and also to the presence of diffusion in the models.},
  keywords = {Convection,notion,notion-database,Stars: interiors,Stars: late-type,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/9KD4IKXM/Piau et al. - 2009.pdf}
}

@article{Pickering1901,
  title = {Sixty-Four New Variable Stars.},
  author = {Pickering, E. C. and Colson, H. R. and Fleming, W. P. and Wells, L. D.},
  year = {1901},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {13},
  pages = {226},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/140808},
  urldate = {2020-03-07},
  keywords = {notion,notion-database}
}

@article{Pietrinferni2004a,
  title = {A {{Large Stellar Evolution Database}} for {{Population Synthesis Studies}}. {{I}}. {{Scaled Solar Models}} and {{Isochrones}}},
  author = {Pietrinferni, Adriano and Cassisi, Santi and Salaris, Maurizio and Castelli, Fiorella},
  year = {2004},
  journal = {The Astrophysical Journal},
  volume = {612},
  number = {1},
  pages = {168--190},
  issn = {0004-637X},
  doi = {10.1086/422498},
  abstract = {[Abridged] We present a large, new set of stellar evolution models and isochrones for an alpha-enhanced metal distribution typical of Galactic halo and bulge stars; it represents a homogeneous extension of our stellar model library for a distribution already presented in Pietrinferni et al.(2004). The effect of the alpha-element enhancement has been properly taken into account in the nuclear network, opacity, equation of state and, for the first time, the bolometric corrections, and color transformations. This allows us to avoid the inconsistent use - common to all alpha-enhanced model libraries currently available - of scaled-solar bolometric corrections and color transformations for alpha-enhanced models and isochrones. We show how bolometric corrections to magnitudes obtained for the U,B portion of stellar spectra for T\_\{eff\}{$<$}=6500K, are significantly affected by the metal mixture, especially at the higher metallicities. We also provide complete sets of evolutionary models for low-mass, He-burning stellar structures covering the whole metallicity range, to enable synthetic horizontal branch simulations. We compare our database with several widely used stellar model libraries from different authors, as well as with various observed color magnitude and color-color diagrams (Johnson-Cousins BVI and near infrared magnitudes, Stromgren colors) of Galactic field stars and globular clusters. We also test our isochrones comparing integrated optical colors and Surface Brightness Fluctuation magnitudes with selected globular cluster data. We find a general satisfactory agreement with the empirical constraints.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/L9EDYF67/Pietrinferni et al. - 2004.pdf}
}

@article{Pijpers1997,
  title = {Inversions in {{Astronomy}} and the {{Sola Method}}},
  author = {Pijpers, Frank P.},
  year = {1997},
  pages = {419--442},
  doi = {10.1007/978-1-4612-1878-4_21},
  abstract = {This paper was presented at the Institute for Mathematics and its Applications workshop "Inverse problems in wave propagation" and will appear in the series IMA volumes (Springer). A brief overview of applications of inversions within astronomy is presented and also an inventory of techniques commonly in use. Most of this paper is focussed on the method of Subtractive Optimally Localized Averages (SOLA) which is an adaptation of the Backus and Gilbert method. This method was originally developed for use in helioseismology where the Backus and Gilbert method is computationally too slow. Since then it has also been applied to the problem of reverberation mapping of active galactic nuclei and the differences between this inverse problem and the ones of helioseismology are also discussed.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LMN5MRGE/Pijpers - 1997.pdf}
}

@article{Pincon2017,
  title = {Can Plume-Induced Internal Gravity Waves Regulate the Core Rotation of Subgiant Stars?},
  author = {Pin{\c c}on, C. and Belkacem, K. and Goupil, M. J. and Marques, J. P.},
  year = {2017},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {605},
  eprint = {1705.10101},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201730998},
  urldate = {2020-03-09},
  abstract = {Context. The seismic data provided by the space-borne missions CoRoT and Kepler enabled us to probe the internal rotation of thousands of evolved low-mass stars. Subsequently, several studies showed that current stellar evolution codes are unable to reproduce the low core rotation rates observed in these stars. These results indicate that an additional angular momentum transport process is necessary to counteract the spin up due to the core contraction during the post-main sequence evolution. For several candidates, the transport induced by internal gravity waves (IGW) could play a non-negligible role. Aims. We aim to investigate the effect of IGW generated by penetrative convection on the internal rotation of low-mass stars from the subgiant branch to the beginning of the red giant branch. Methods. A semi-analytical excitation model was used to estimate the angular momentum wave flux. The characteristic timescale associated with the angular momentum transport by IGW was computed and compared to the contraction timescale throughout the radiative region of stellar models at different evolutionary stages. Results. We show that IGW can efficiently counteract the contraction-driven spin up of the core of subgiant stars if the amplitude of the radial-differential rotation (between the center of the star and the top of the radiative zone) is higher than a threshold value. This threshold depends on the evolutionary stage and is comparable to the differential rotation rates inferred for a sample of subgiant stars observed by the satellite Kepler. Such an agreement can therefore be interpreted as the consequence of a regulation mechanism driven by IGW. This result is obtained under the assumption of a smooth rotation profile in the radiative region and holds true even if a wide range of values is considered for the parameters of the generation model. In contrast, on the red giant branch, we find that IGW remain insufficient, on their own, to explain the observations because of an excessive radiative damping. Conclusions. IGW generated by penetrative convection are able to efficiently extract angular momentum from the core of stars on the subgiant branch and accordingly have to be taken into account. Moreover, agreements with the observations reinforce the idea that their effect is essential to regulate the amplitude of the radial-differential rotation in subgiant stars. On the red giant branch, another transport mechanism must likely be invoked.},
  archiveprefix = {arxiv},
  keywords = {Hydrodynamics,notion,notion-database,Stars: evolution,Stars: interiors,Stars: rotation,Waves},
  file = {/Users/lbugnet/Zotero/storage/6USPLXGG/full-text.pdf}
}

@article{Pincon2019,
  title = {Evolution of the Gravity Offset of Mixed Modes in {{RGB}} Stars},
  author = {Pin{\c c}on, C. and Takata, M. and Mosser, B.},
  year = {2019},
  journal = {Astronomy and Astrophysics},
  volume = {626},
  number = {35327},
  eprint = {1905.05691},
  issn = {14320746},
  doi = {10.1051/0004-6361/201935327},
  abstract = {Context. Observations of mixed modes in evolved low-mass stars enable us to probe the properties of not only the outer envelope of these stars, but also their deep layers. Among the seismic parameters associated with mixed modes, the gravity offset, denoted with {$\epsilon$}g, is expected to reveal information on the boundaries of the inner buoyancy resonant cavity. This parameter was recently measured for hundreds of stars observed by the Kepler satellite and its value was shown to change during evolution. Aims. In this article, we theoretically investigate the reasons for such a variation in terms of structure properties, focusing only on the red giant branch. Methods. Using available asymptotic analyses and a simple model of the Brunt-V\"ais\"al\"a and Lamb frequencies in the upper part of the radiative zone, we derived an analytical expression of {$\epsilon$}g for dipolar modes and compared its predictions to observations. Results. First, we show that the asymptotic value of {$\epsilon$}g well agrees with the mean value observed at the beginning of the ascent of the red giant branch, which results from the high density contrast between the helium core and the base of the convective envelope. Second, we demonstrate that the predicted value also explains the sharp decrease in {$\epsilon$}g observed for the more luminous red giant stars of the sample. This rapid drop turns out to occur just before the luminosity bump and results from the kink of the Brunt-V\"ais\"al\"a frequency near the upper turning point associated with the buoyancy cavity as stars evolve and this latter nears the base of the convective envelope. The potential of {$\epsilon$}g to probe the value and slope of the Brunt-V\"ais\"al\"a frequency below the base of the convective region is clearly highlighted. Conclusions. The observed variation in {$\epsilon$}g and its link with the internal properties on the red giant branch are now globally understood. This work motivates further analyses of the potential of this parameter as a seismic diagnosis of the region located between the hydrogen-burning shell and the base of the convective envelope, and of the local dynamical processes associated for instance with core contraction, the migration of the convective boundary, or overshooting.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/AHEPZZTA/Pinçon, Takata, Mosser - 2019.pdf}
}

@article{Pincon2020,
  title = {Probing the Mid-Layer Structure of Red Giants {{I}}. {{Mixed-mode}} Coupling Factor as a Seismic Diagnosis},
  author = {Pin{\c c}on, C. and Goupil, M. -J. and Belkacem, K.},
  year = {2020},
  month = dec,
  journal = {Astronomy \& Astrophysics},
  volume = {634},
  eprint = {1912.06008},
  doi = {10.1051/0004-6361/201936864},
  urldate = {2020-07-19},
  abstract = {The space-borne missions CoRoT and Kepler have already brought stringent constraints on the internal structure of low-mass evolved stars, a large part of which results from the detection of mixed modes. However, all the potential of these oscillation modes as a diagnosis of the stellar interior has not been fully exploited yet. In particular, the coupling factor or the gravity-offset of mixed modes, \$q\$ and \$\textbackslash varepsilon\_\{\textbackslash rm g\}\$, are expected to provide additional constraints on the mid-layers of red giants, which are located between the hydrogen-burning shell and the neighborhood of the base of the convective zone. In the present paper, we investigate the potential of the coupling factor in probing the mid-layer structure of evolved stars. Guided by typical stellar models and general physical considerations, we modeled the coupling region along with evolution. We subsequently obtained an analytical expression of \$q\$ based on the asymptotic theory of mixed modes and compared it to observations. We show that the value of \$q\$ is degenerate with respect to the thickness of the coupling evanescent region and the local density scale height. A structural interpretation of the global variations in \$q\$ observed on the subgiant and the red giant branches, as well as on the red clump, was obtained in the light of this model. We demonstrate that \$q\$ has the promising potential to probe the migration of the base of the convective region as well as convective extra-mixing in evolved red giant stars with typically \$\textbackslash nu\_\{\textbackslash rm max\} \textbackslash lesssim 100\textasciitilde\textbackslash mu\$Hz. We also show that the frequency-dependence of \$q\$ cannot be neglected in the oscillation spectra of such stars, which is in contrast with what is assumed in the current measurement methods. This analytical study paves the way for a more quantitative exploration of the link of \$q\$ with the internal properties of evolved stars using stellar models.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology-stars,evolution,interiors-stars,notion,notion-database,oscillations-stars},
  file = {/Users/lbugnet/Zotero/storage/C4IJG7ZV/full-text.pdf;/Users/lbugnet/Zotero/storage/T3GJIFBU/full-text.pdf}
}

@article{Pinsonneault1989,
  title = {Evolutionary Models of the Rotating {{Sun}}},
  author = {Pinsonneault, Marc H. and Kawaler, Steven D. and Sofia, S. and Demarque, Pierre},
  year = {1989},
  journal = {The Astrophysical Journal},
  volume = {338},
  eprint = {1011.1669v3},
  pages = {424--452},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/65PBJMTV/Pinsonneault et al. - 1989.pdf}
}

@article{Pinsonneault1997,
  title = {Mixing in {{Stars}}},
  author = {Pinsonneault, M.},
  year = {1997},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {35},
  number = {1},
  pages = {557--605},
  issn = {0066-4146},
  doi = {10.1146/annurev.astro.35.1.557},
  abstract = {Three cases for mixing not present in standard stellar models are presented: Light element depletion in low mass main-sequence stars, deep mixing in massive stars, and deep mixing in low mass giants. The review begins with the mixing indicators and the predictions of standard models. The observational evidence for anomalous mixing is then presented, followed by the physics of mixing outside the standard model. The status of theoretical models that include extra mixing is then examined.},
  keywords = {notion,notion-database,stellar abundances,stellar evolution,stellar rotation},
  file = {/Users/lbugnet/Zotero/storage/X3S4B5Q7/Pinsonneault - 1997.pdf}
}

@article{Pinsonneault2009,
  title = {Astrophysics: {{A}} Fossil Record for Exoplanets},
  author = {Pinsonneault, Marc},
  year = {2009},
  journal = {Nature},
  volume = {462},
  number = {7270},
  pages = {168--169},
  issn = {00280836},
  doi = {10.1038/462168a},
  abstract = {Stars that host planets experience more mixing of their internal elements than do stars that lack such companions. This correlation may serve as a useful diagnostic in the search for planets around stars other than the Sun. \textcopyright{} 2009 Macmillan Publishers Limited. All rights reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/EQ9RXELX/Pinsonneault - 2009.pdf}
}

@article{Pinsonneault2012,
  title = {A Revised Effective Temperature Scale for the {{Kepler}} Input Catalog},
  author = {Pinsonneault, Marc H. and An, Deokkeun and {Molenda-Zakowicz}, Joanna and Chaplin, William J. and Metcalfe, Travis S. and Bruntt, Hans},
  year = {2012},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {199},
  number = {2},
  eprint = {1110.4456},
  issn = {00670049},
  doi = {10.1088/0067-0049/199/2/30},
  abstract = {We present a catalog of revised effective temperatures for stars observed in long-cadence mode in the Kepler Input Catalog (KIC). We use Sloan Digital Sky Survey (SDSS) griz filters tied to the fundamental temperature scale. Polynomials for griz color-temperature relations are presented, along with correction terms for surface gravity effects, metallicity, and statistical corrections for binary companions or blending. We compare our temperature scale to the published infrared flux method (IRFM) scale for V TJK s in both open clusters and the Kepler fields. We find good agreement overall, with some deviations between (J - K s )-based temperatures from the IRFM and both SDSS filter and other diagnostic IRFM color-temperature relationships above 6000K. For field dwarfs, we find a mean shift toward hotter temperatures relative to the KIC, of order 215K, in the regime where the IRFM scale is well defined (4000K to 6500K). This change is of comparable magnitude in both color systems and in spectroscopy for stars with T eff below 6000K. Systematic differences between temperature estimators appear for hotter stars, and we define corrections to put the SDSS temperatures on the IRFM scale for them. When the theoretical dependence on gravity is accounted for, we find a similar temperature scale offset between the fundamental and KIC scales for giants. We demonstrate that statistical corrections to color-based temperatures from binaries are significant. Typical errors, mostly from uncertainties in extinction, are of order 100K. Implications for other applications of the KIC are discussed. \textcopyright{} 2012 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/TH4I47FE/Pinsonneault et al. - 2012.pdf}
}

@article{Pinsonneault2015,
  title = {The {{APOKASC}} Catalog: {{An}} Asteroseismic and Spectroscopic Joint Survey of Targets in the {{Kepler}} Fields},
  author = {Pinsonneault, Marc H. and Elsworth, Yvonne and Epstein, Courtney and Hekker, Saskia and M{\'e}sz{\'a}ros, Sz and Chaplin, William J. and Johnson, Jennifer A. and Garc{\'i}a, Rafael A. and Holtzman, Jon and Mathur, Savita and Garc{\'i}a P{\'e}rez, Ana and Silva Aguirre, Victor and Girardi, L{\'e}o and Basu, Sarbani and Shetrone, Matthew and Stello, Dennis and Allende Prieto, Carlos and An, Deokkeun and Beck, Paul and Beers, Timothy C. and Bizyaev, Dmitry and Bloemen, Steven and Bovy, Jo and Cunha, Katia and De Ridder, Joris and Frinchaboy, Peter M. and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Gilliland, Ronald and Harding, Paul and Hearty, Fred R. and Huber, Daniel and Ivans, Inese and Kallinger, Thomas and Majewski, Steven R. and Metcalfe, Travis S. and Miglio, Andrea and Mosser, Benoit and Muna, Demitri and Nidever, David L. and Schneider, Donald P. and Serenelli, Aldo and Smith, Verne V. and Tayar, Jamie and Zamora, Olga and Zasowski, Gail},
  year = {2015},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {215},
  number = {2},
  eprint = {1410.2503},
  issn = {00670049},
  doi = {10.1088/0067-0049/215/2/19},
  abstract = {We present the first APOKASC catalog of spectroscopic and asteroseismic properties of 1916 red giants observed in the Kepler fields. The spectroscopic parameters provided from the Apache Point Observatory Galactic Evolution Experiment project are complemented with asteroseismic surface gravities, masses, radii, and mean densities determined by members of the Kepler Asteroseismology Science Consortium. We assess both random and systematic sources of error and include a discussion of sample selection for giants in the Kepler fields. Total uncertainties in the main catalog properties are of the order of 80 K in T eff, 0.06 dex in [M/H], 0.014 dex in log g, and 12\% and 5\% in mass and radius, respectively; these reflect a combination of systematic and random errors. Asteroseismic surface gravities are substantially more precise and accurate than spectroscopic ones, and we find good agreement between their mean values and the calibrated spectroscopic surface gravities. There are, however, systematic underlying trends with T eff and log g. Our effective temperature scale is between 0 and 200 K cooler than that expected from the infrared flux method, depending on the adopted extinction map, which provides evidence for a lower value on average than that inferred for the Kepler Input Catalog (KIC). We find a reasonable correspondence between the photometric KIC and spectroscopic APOKASC metallicity scales, with increased dispersion in KIC metallicities as the absolute metal abundance decreases, and offsets in T eff and log g consistent with those derived in the literature. We present mean fitting relations between APOKASC and KIC observables and discuss future prospects, strengths, and limitations of the catalog data.},
  archiveprefix = {arxiv},
  keywords = {catalogs,notion,notion-database,stars: abundances,stars: fundamental parameters,stars: oscillations (including pulsations),surveys},
  file = {/Users/lbugnet/Zotero/storage/9UPL9KRL/Pinsonneault et al. - 2015.pdf}
}

@article{Pinsonneault2018,
  title = {The {{Second APOKASC Catalog}}: {{The Empirical Approach}}},
  author = {Pinsonneault, Marc H and Elsworth, Yvonne P and Tayar, Jamie and Serenelli, Aldo and Stello, Dennis and Zinn, Joel and Mathur, Savita and Garc{\'i}a, Rafael A and Johnson, Jennifer A and Hekker, Saskia and Huber, Daniel and Kallinger, Thomas and M{\'e}sz{\'a}ros, Szabolcs and Mosser, Benoit and Stassun, Keivan and Girardi, L{\'e}o and Rodrigues, Tha{\'i}se S and Aguirre, Victor Silva and An, Deokkeun and Basu, Sarbani and Chaplin, William J and Corsaro, Enrico and Cunha, Katia and {Garc{\'i}a-Hern{\'a}ndez}, D A and Holtzman, Jon and J{\"o}nsson, Henrik and Shetrone, Matthew and Smith, Verne V and Sobeck, Jennifer S and Stringfellow, Guy S and Zamora, Olga and Beers, Timothy C and {Fern{\'a}ndez-Trincado}, J G and Frinchaboy, Peter M and Hearty, Fred R and Nitschelm, Christian},
  year = {2018},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {239},
  number = {25pp},
  pages = {32},
  doi = {10.3847/1538-4365/aaebfd},
  urldate = {2020-03-22},
  abstract = {We present a catalog of stellar properties for a large sample of 6676 evolved stars with Apache Point Observatory Galactic Evolution Experiment spectroscopic parameters and Kepler asteroseismic data analyzed using five independent techniques. Our data include evolutionary state, surface gravity, mean density, mass, radius, age, and the spectroscopic and asteroseismic measurements used to derive them. We employ a new empirical approach for combining asteroseismic measurements from different methods, calibrating the inferred stellar parameters, and estimating uncertainties. With high statistical significance, we find that asteroseismic parameters inferred from the different pipelines have systematic offsets that are not removed by accounting for differences in their solar reference values. We include theoretically motivated corrections to the large frequency spacing ({$\Delta\nu$}) scaling relation, and we calibrate the zero-point of the frequency of the maximum power ({$\nu$} max) relation to be consistent with masses and radii for members of star clusters. For most targets, the parameters returned by different pipelines are in much better agreement than would be expected from the pipeline-predicted random errors, but 22\% of them had at least one method not return a result and a much larger measurement dispersion. This supports the usage of multiple analysis techniques for asteroseismic stellar population studies. The measured dispersion in mass estimates for fundamental calibrators is consistent with our error model, which yields median random and 1 systematic mass uncertainties for RGB stars of order 4\%. Median random and systematic mass uncertainties are at the 9\% and 8\% level, respectively, for red clump stars.},
  keywords = {notion,notion-database,stars: abundances,stars: fundamental parameters,stars: oscillations (including pulsations)},
  file = {/Users/lbugnet/Zotero/storage/VNB4P37R/full-text.pdf}
}

@article{Pires2009,
  title = {{{FAst STatistics}} for Weak {{Lensing}} ({{FASTLens}}): {{Fast}} Method for Weak Lensing Statistics and Map Making},
  author = {Pires, S. and Starck, J. L. and Amara, A. and Teyssier, R. and R{\'e}fr{\'e}gier, A. and Fadili, J.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {395},
  number = {3},
  eprint = {0804.4068},
  pages = {1265--1279},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2009.14625.x},
  abstract = {With increasingly large data sets, weak lensing measurements are able to measure cosmological parameters with ever-greater precision. However, this increased accuracy also places greater demands on the statistical tools used to extract the available information. To date, the majority of lensing analyses use the two-point statistics of the cosmic shear field. These can be either studied directly using the two-point correlation function or in Fourier space, using the power spectrum. But analysing weak lensing data inevitably involves the masking out of regions, for example to remove bright stars from the field. Masking out the stars is common practice but the gaps in the data need proper handling. In this paper, we show how an inpainting technique allows us to properly fill in these gaps with only Nlog N operations, leading to a new image from which we can compute straightforwardly and with a very good accuracy both the power spectrum and the bispectrum. We then propose a new method to compute the bispectrum with a polar fft algorithm, which has the main advantage of avoiding any interpolation in the Fourier domain. Finally, we propose a new method for dark matter mass map reconstruction from shear observations, which integrates this new inpainting concept. A range of examples based on 3D N-body simulations illustrates the results. \textcopyright{} 2009 RAS.},
  archiveprefix = {arxiv},
  keywords = {Dark matter,Methods: data analysis,Methods: statistical,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2S2ARU4V/Pires et al. - 2009.pdf}
}

@article{Pires2015,
  title = {Gap Interpolation by Inpainting Methods: {{Application}} to Ground and Space-Based Asteroseismic Data},
  author = {Pires, Sandrine and Mathur, Savita and Garc{\'i}a, Rafael A. and Ballot, J{\'e}r{\^o}me and Stello, Dennis and Sato, Kumiko},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {574},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/201322361},
  abstract = {In asteroseismology, the observed time series often suffers from incomplete time coverage due to gaps. The presence of periodic gaps may generate spurious peaks in the power spectrum that limit the analysis of the data. Various methods have been developed to deal with gaps in time series data. However, it is still important to improve these methods to be able to extract all the possible information contained in the data. In this paper, we propose a new approach to handling the problem, the so-called inpainting method. This technique, based on a prior condition of sparsity, enables the gaps in the data to be judiciously fill-in thereby preserving the asteroseismic signal as far as possible. The impact of the observational window function is reduced and the interpretation of the power spectrum simplified. This method is applied on both ground- and space-based data. It appears that the inpainting technique improves the detection and estimation of the oscillation modes. Additionally, it can be used to study very long time series of many stars because it is very fast to compute. For a time series of 50 days of CoRoT-like data, it allows a speed-up factor of 1000, if compared to methods with the same accuracy.},
  keywords = {Asteroseismology,Methods: Data analysis,Methods: Statistical,notion,notion-database,Stars: Oscillations},
  file = {/Users/lbugnet/Zotero/storage/I3B4APQR/Pires et al. - 2015.pdf}
}

@article{Pitts1985,
  title = {The Adiabatic Stability of Stars Containing Magnetic Fields - {{VI}}. {{The}} Influence of Rotation},
  author = {Pitts, E. and Tayler, R.J.},
  year = {1985},
  journal = {MNRAS},
  volume = {216},
  pages = {139--154},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Pizzolato2003,
  title = {The Stellar Activity-Rotation Relationship Revisited: {{Dependence}} of Saturated and Non-Saturated x-Ray Emission Regimes on Stellar Mass for Late-Type Dwarfs},
  author = {Pizzolato, N. and Maggio, A. and Micela, G. and Sciortino, S. and Ventura, P.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {397},
  number = {1},
  pages = {147--157},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021560},
  abstract = {We present the results of a new study on the relationship between coronal X-ray emission and stellar rotation in late-type main-sequence stars. We have selected a sample of 259 dwarfs in the B - V range 0.5-2.0, including 110 field stars and 149 members of the Pleiades, Hyades, {$\alpha$} Persei, IC 2602 and IC 2391 open clusters. All the stars have been observed with ROSAT, and most of them have photometrically-measured rotation periods available. Our results confirm that two emission regimes exist, one in which the rotation period is a good predictor of the total X-ray luminosity, and the other in which a constant saturated X-ray to bolometric luminosity ratio is attained; we present a quantitative estimate of the critical rotation periods below which stars of different masses (or spectral types) enter the saturated regime. In this work we have also empirically derived a characteristic time scale, {$\tau$}e, which we have used to investigate the relationship between the X-ray emission level and an X-ray-based Rossby number Re = Prot/{$\tau$}e: we show that our empirical time scale {$\tau$}e resembles the theoretical convective turnover time for 0.4 {$\lessequivlnt$} M/M{$\odot$} {$\lessequivlnt$} 1.2, but it also has the same functional dependence on B - V as as Lbol-1/2 in the color range 0.5 {$\lessequivlnt$} B - V {$\lessequivlnt$} 1.5. Our results imply that - for non-saturated coronae- the Lx - Prot relation is equivalent to the Lx/Lbol vs. Re relation.},
  keywords = {notion,notion-database,Stars: activity,Stars: late-type,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/8I94XCNA/Pizzolato et al. - 2003.pdf}
}

@article{plaskett1916,
  title = {A Variation in the Solar Rotation},
  author = {Plaskett, H.H},
  year = {1916},
  journal = {The Astrophysical Journal},
  number = {43},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PHH7KKKH/Plaskett - 1916.pdf}
}

@article{Platt1999,
  title = {Probabilistic {{Outputs}} for {{Support Vector Machines}} and {{Comparisons}} to {{Regularized Likelihood Methods}}},
  author = {Platt, John C.},
  year = {1999},
  journal = {ADVANCES IN LARGE MARGIN CLASSIFIERS},
  pages = {61--74},
  urldate = {2020-04-11},
  keywords = {notion,notion-database}
}

@article{Plavchan2008,
  title = {Near-{{Infrared Variability}} in the {{2MASS Calibration Fields}}: {{A Search}} for {{Planetary Transit Candidates}}},
  author = {Plavchan, Peter and Jura, M. and Kirkpatrick, J. Davy and Cutri, Roc M. and Gallagher, S. C.},
  year = {2008},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {175},
  number = {1},
  eprint = {0709.1182},
  pages = {191--228},
  issn = {0067-0049},
  doi = {10.1086/523644},
  abstract = {The 2MASS photometric calibration observations cover \textasciitilde 6 square degrees on the sky in 35 "calibration fields" each sampled in nominal photometric conditions between 562 and 3692 times during the four years of the 2MASS mission. We compile a catalog of variables from the calibration observations to search for M dwarfs transited by extra-solar planets. We present our methods for measuring periodic and non-periodic flux variability. From 7554 sources with apparent Ks magnitudes between 5.6 and 16.1, we identify 247 variables, including extragalactic variables and 23 periodic variables. We have discovered three M dwarf eclipsing systems, including two candidates for transiting extrasolar planets.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IXND766H/Plavchan et al. - 2008.pdf}
}

@inproceedings{Pokorny2014,
  title = {Grasp Moduli Spaces and Spherical Harmonics},
  booktitle = {Proceedings - {{IEEE International Conference}} on {{Robotics}} and {{Automation}}},
  author = {Pokorny, Florian T. and Bekiroglu, Yasemin and Kragic, Danica},
  year = {2014},
  month = sep,
  pages = {389--396},
  publisher = {{Institute of Electrical and Electronics Engineers Inc.}},
  issn = {10504729},
  doi = {10.1109/ICRA.2014.6906886},
  urldate = {2020-06-26},
  abstract = {In this work, we present a novel representation which enables a robot to reason about, transfer and optimize grasps on various objects by representing objects and grasps on them jointly in a common space. In our approach, objects are parametrized using smooth differentiable functions which are obtained from point cloud data via a spectral analysis. We show how, starting with point cloud data of various objects, one can utilize this space consisting of grasps and smooth surfaces in order to continuously deform various surface/grasp configurations with the goal of synthesizing force closed grasps on novel objects. We illustrate the resulting shape space for a collection of real world objects using multidimensional scaling and show that our formulation naturally enables us to use gradient ascent approaches to optimize and simultaneously deform a grasp from a known object towards a novel object.},
  keywords = {notion,notion-database}
}

@article{Pope2016,
  title = {Photometry of Very Bright Stars with {{Kepler}} and {{K2}} Smear Data},
  author = {Pope, B. J.S. and White, T. R. and Huber, D. and Murphy, S. J. and Bedding, T. R. and Caldwell, D. A. and Sarai, A. and Aigrain, S. and Barclay, T.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {455},
  number = {1},
  eprint = {1510.00008},
  pages = {L36-L40},
  issn = {13652966},
  doi = {10.1093/mnrasl/slv143},
  abstract = {High-precision time series photometry with the Kepler satellite has been crucial to our understanding both of exoplanets, and via asteroseismology, of stellar physics. After the failure of two reaction wheels, the Kepler satellite has been repurposed as Kepler-2 (K2), observing fields close to the ecliptic plane. As these fields contain many more bright stars than the original Kepler field, K2 provides an unprecedented opportunity to study nearby objects amenable to detailed follow-up with ground-based instruments. Due to bandwidth constraints, only a small fraction of pixels can be downloaded, with the result that most bright stars which saturate the detector are not observed. We show that engineering data acquired for photometric calibration, consisting of collateral 'smear' measurements, can be used to reconstruct light curves for bright targets not otherwise observable with Kepler/K2. Here we present some examples from Kepler Quarter 6 and K2 Campaign 3, including the {$\delta$} Scuti variables HD 178875 and 70 Aqr, and the red giant HR 8500 displaying solar-like oscillations. We compare aperture and smear photometry where possible, and also study targets not previously observed. These encouraging results suggest this new method can be applied to most Kepler and K2 fields.},
  archiveprefix = {arxiv},
  keywords = {70 Aqr,Asteroseismology,HD 178875,notion,notion-database,Stars: individual: HR 8500,Stars: variables: general,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/RKPHQB5C/Pope et al. - 2016.pdf}
}

@article{Poppenhaeger2010a,
  title = {Coronal Properties of Planet-Bearing Stars},
  author = {Poppenhaeger, K. and Robrade, J. and Schmitt, J. H.M.M.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {515},
  number = {11},
  pages = {1--9},
  issn = {14320746},
  doi = {10.1051/0004-6361/201014245},
  abstract = {Context. Do extrasolar planets affect the activity of their host stars? Indications for chromospheric activity enhancement have been found for a handful of targets, but in the X-ray regime, conclusive observational evidence is still missing. Aims.We want to establish a sound observational basis to confirm or reject major effects of Star-Planet Interactions (SPI) in stellar X-ray emissions. Methods.We therefore conduct a statistical analysis of stellar X-ray activity of all known planet-bearing stars within 30 pc distance for dependencies on planetary parameters such as mass and semimajor axis. Results. In our sample, there are no significant correlations of X-ray luminosity or the activity indicator LX/Lbol with planetary parameters which cannot be explained by selection effects. Conclusions.Coronal SPI seems to be a phenomenon which might only manifest itself as a strong effect for a few individual targets, but not to have a major effect on planet-bearing stars in general. \textcopyright{} 2010 ESO.},
  keywords = {notion,notion-database,Planet-star interactions,Stars: activity,Stars: coronae,Stars: statistics,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/FSNFL82E/Poppenhaeger, Robrade, Schmitt - 2010.pdf;/Users/lbugnet/Zotero/storage/VQRH8BWP/Poppenhaeger, Robrade, Schmitt - 2010(2).pdf}
}

@article{Poppenhaeger2011a,
  title = {A Search for Star-Planet Interactions in the {$\upsilon$} {{Andromedae}} System at {{X-ray}} and Optical Wavelengths},
  author = {Poppenhaeger, K. and Lenz, L. F. and Reiners, A. and Schmitt, J. H.M.M. and Shkolnik, E.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {528},
  eprint = {1010.5632},
  pages = {1--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201016008},
  abstract = {Context. Close-in, giant planets are expected to influence their host stars via tidal or magnetic interaction. But are these effects in X-rays strong enough in suitable targets known so far to be observed with today's instrumentation? Aims. The {$\upsilon$} And system, an F8V star with a Hot Jupiter, was observed to undergo cyclic changes in chromospheric activity indicators with its innermost planet's period. We aim to investigate the stellar chromospheric and coronal activity over several months. Methods. We therefore monitored the star in X-rays as well as at optical wavelengths to test coronal and chromospheric activity indicators for planet-induced variability, making use of the Chandra X-ray Observatory as well as the echelle spectrographs FOCES and HRS at Calar Alto (Spain) and the Hobby-Eberly Telescope (Texas, US). Results. The stellar activity level is low, as seen both in X-rays as in Ca\^a\texteuro{} \textperthousand{} ii line fluxes; the chromospheric data show variability with the stellar rotation period. We do not find activity variations in X-rays or in the optical that can be traced back to the planet. Conclusions. Gaining observational evidence of star-planet interactions in X-rays remains challenging. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,planet-star interactions,stars: activity,stars: chromospheres,stars: coronae,X-rays: individuals: {$\upsilon$} Andromedae,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/V384ASII/Poppenhaeger et al. - 2011.pdf}
}

@article{Poppenhaeger2011c,
  title = {A Correlation between Host Star Activity and Planet Mass for Close-in Extrasolar Planets?},
  author = {Poppenhaeger, K. and Schmitt, J. H.M.M.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {735},
  number = {1},
  eprint = {1106.0189},
  issn = {15384357},
  doi = {10.1088/0004-637X/735/1/59},
  abstract = {The activity levels of stars are influenced by several stellar properties, such as stellar rotation, spectral type, and the presence of stellar companions. Analogous to binaries, planetary companions are also thought to be able to cause higher activity levels in their host stars, although at lower levels. Especially in X-rays, such influences are hard to detect because coronae of cool stars exhibit a considerable amount of intrinsic variability. Recently, a correlation between the mass of close-in exoplanets and their host star's X-ray luminosity has been detected, based on archival X-ray data from the ROSAT All-Sky Survey. This finding has been interpreted as evidence for star-planet interactions. We show in our analysis that this correlation is caused by selection effects due to the flux limit of the X-ray data used and due to the intrinsic planet detectability of the radial velocity method, and thus does not trace possible planet-induced effects. We also show that the correlation is not present in a corresponding complete sample derived from combined XMM-Newton and ROSAT data. \textcopyright{} 2011. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,planet-star interactions,stars: activity,stars: coronae,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/EXWKV569/Poppenhaeger, Schmitt - 2011.pdf}
}

@article{Poppenhager2009,
  title = {51 {{Pegasi-a}} Planet-Bearing Maunder Minimum Candidate},
  author = {Poppenh{\"a}ger, K. and Robrade, J. and Schmitt, J. H M M and Hall, J. C.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {508},
  number = {3},
  pages = {1417--1421},
  issn = {00046361},
  doi = {10.1051/0004-6361/200912945},
  abstract = {We observed 51 Peg, the first detected planet-bearing star, in a 55 ks XMM-Newton pointing and in 5 ks pointings each with Chandra HRC-I and ACIS-S. The star has a very low count rate in the XMM observation, but is clearly visible in the Chandra images due to the detectors' different sensitivity at low X-ray energies. This allows a temperature estimate for 51 Peg's corona of T {$>$} 1 MK; the detected ACIS-S photons can be plausibly explained by emission lines of a very cool plasma near 200 eV. The constantly low X-ray surface flux and the flat-activity profile seen in optical Ca II data suggest that 51 Peg is a Maunder minimum star; an activity enhancement due to a Hot Jupiter, as proposed by recent studies, seems to be absent. The star's X-ray fluxes in different instruments are consistent with the exception of the HRC Imager, which might have a larger effective area below 200 eV than given in the calibration. \textcopyright{} 2009 ESO.},
  keywords = {notion,notion-database,Stars: activity,Stars: Coronae,Stars: individual: 51 Peg,X-rays: individuals: 51 Peg,X-rays: stars},
  file = {/Users/lbugnet/Zotero/storage/PYNZIUTD/Poppenhäger et al. - 2009.pdf}
}

@article{Poretti2009,
  title = {The Tip of the Iceberg: {{The}} Frequency Content of the {$\delta$} {{Sct}} Star {{HD}} 50844 from {{CoRoT}} Space Photometry},
  author = {Poretti, E. and Mantegazza, L. and Rainer, M. and Uytterhoeven, K. and Michel, E. and Baglin, A. and Auvergne, M. and Catala, C. and Samadi, R. and Rodr{\'i}guez, E. and Garrido, R. and Amado, P. and {Mart{\'i}n-Ruiz}, S. and Moya, A. and Su{\'a}rez, J. C. and Baudin, F. and Zima, W. and Alvarez, M. and Mathias, P. and Papar{\'o}, M. and P{\'a}pics, P. and Plachy, E.},
  year = {2009},
  journal = {AIP Conference Proceedings},
  volume = {1170},
  eprint = {0910.4079},
  pages = {435--439},
  issn = {0094243X},
  doi = {10.1063/1.3246537},
  abstract = {It has been suggested that the detection of a wealth of very low amplitude modes in {$\delta$} Sct stars was only a matter of signal-to-noise ratio. Access to this treasure, impossible from the ground, is one of the scientific aims of the space mission CoRoT, developed and operated by CNES. This work presents the results obtained on HD 50844: the 140,016 datapoints allowed us to reach the level of 10-5 mag in the amplitude spectra. The frequency analysis of the CoRoT timeseries revealed hundreds of terms in the frequency range 0-30 d-1. The initial guess that {$\delta$} Sct stars have a very rich frequency content is confirmed. The spectroscopic mode identification gives theoretical support since very high-degree modes (up to {$\mathscr{l}$}=14) are identified. We also prove that cancellation effects are not sufficient in removing the flux variations associated to these modes at the noise level of the CoRoT measurements. The ground-based observations indicate that HD 50844 is an evolved star that is slightly underabundant in heavy elements, located on the Terminal Age Main Sequence. The predominant term (f1=6.92 d -1) has been identified as the fundamental radial mode combining ground-based photometric and spectroscopic data. \textcopyright{} 2009 American Institute of Physics.},
  archiveprefix = {arxiv},
  isbn = {9780735407077},
  keywords = {notion,notion-database,Stars: Interiors,Stars: Oscillations,Stars: variables: {$\delta$} sct},
  file = {/Users/lbugnet/Zotero/storage/M6L4FI9Q/Poretti et al. - 2009.pdf}
}

@article{Pourbaix2004,
  title = {{{SB9}}: {{The}} Ninth Catalogue of Spectroscopic Binary Orbits},
  author = {Pourbaix, D. and Tokovinin, A. A. and Batten, A. H. and Fekel, F. C. and Hartkopf, W. I. and Levato, H. and Morrell, N. I. and Torres, G. and Udry, S.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {424},
  number = {2},
  eprint = {astro-ph/0406573},
  pages = {727--732},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041213},
  abstract = {The Ninth Catalogue of Spectroscopic Binary Orbits (http://sb9.astro.ulb.ac.be) continues the series of compilations of spectroscopic orbits carried out over the past 35 years by Batten and collaborators. As of 2004 May 1st, the new Catalogue holds orbits for 2386 systems. Some essential differences between this catalogue and its predecessors are out-lined and three straightforward applications are presented: (1) completeness assessment: period distribution of SB1s and SB2s; (2) shortest periods across the H-R diagram; (3) period-eccentricity relation.},
  archiveprefix = {arxiv},
  keywords = {Astronomical data bases: miscellaneous,Catalogs,notion,notion-database,Stars: binaries: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/EFV9UGQC/Pourbaix et al. - 2004.pdf}
}

@article{Prat2016,
  title = {Asymptotic Theory of Gravity Modes in Rotating Stars. {{I}}. {{Ray}} Dynamics},
  author = {Prat, V. and Ligni{\`e}res, F. and Ballot, J.},
  year = {2016},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {587},
  pages = {A110},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201527737},
  urldate = {2023-10-17},
  abstract = {Context. The seismology of early-type stars is limited by our incomplete understanding of gravito-inertial modes. Aims: We develop a short-wavelength asymptotic analysis for gravito-inertial modes in rotating stars. Methods: The Wentzel-Kramers-Brillouin approximation was applied to the equations governing adiabatic small perturbations about a model of a uniformly rotating barotropic star. Results: A general eikonal equation, including the effect of the centrifugal deformation, is derived. The dynamics of axisymmetric gravito-inertial rays is solved numerically for polytropic stellar models of increasing rotation and analysed by describing the structure of the phase space. Three different types of phase-space structures are distinguished. The first type results from the continuous evolution of structures of the non-rotating integrable phase space. It is predominant in the low-frequency region of the phase space. The second type of structures are island chains associated with stable periodic rays. The third type of structures are large chaotic regions that can be related to the envelope minimum of the Brunt-V\"ais\"al\"a frequency. Conclusions: Gravito-inertial modes are expected to follow this classification, in which the frequency spectrum is a superposition of sub-spectra associated with these different types of phase-space structures. The detailed confrontation between the predictions of this ray-based asymptotic theory and numerically computed modes will be presented in a companion paper.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,chaos,stars: oscillations,stars: rotation,waves},
  annotation = {ADS Bibcode: 2016A\&A...587A.110P},
  file = {/Users/lbugnet/Zotero/storage/ELAEQC5V/Prat et al. - 2016 - Asymptotic theory of gravity modes in rotating sta.pdf}
}

@article{Prat2017,
  title = {Period Spacing of Gravity Modes Strongly Affected by Rotation: {{Going}} beyond the Traditional Approximation},
  author = {Prat, V. and Mathis, S. and Ligni{\`e}res, F. and Ballot, J. and Culpin, P. M.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {598},
  eprint = {1611.09826},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629637},
  abstract = {Context. As of today, asteroseismology mainly allows us to probe the internal rotation of stars when modes are only weakly affected by rotation using perturbative methods. Such methods cannot be applied to rapidly rotating stars, which exhibit complex oscillation spectra. In this context, the so-called traditional approximation, which neglects the terms associated with the latitudinal component of the rotation vector, describes modes that are strongly affected by rotation. This approximation is sometimes used for interpreting asteroseismic data, however, its domain of validity is not established yet. Aims. We aim at deriving analytical prescriptions for period spacings of low-frequency gravity modes strongly affected by rotation through the full Coriolis acceleration (i.e. without neglecting any component of the rotation vector), which can be used to probe stellar internal structure and rotation. Methods. We approximated the asymptotic theory of gravito-inertial waves in uniformly rotating stars using ray theory described in a previous paper in the low-frequency regime, where waves are trapped near the equatorial plane. We put the equations of ray dynamics into a separable form and used the Einstein-Brillouin-Keller (EBK) quantisation method to compute modes frequencies from rays. Results. Two spectral patterns that depend on stratification and rotation are predicted within this new approximation: one for axisymmetric modes and one for non-axisymmetric modes. Conclusions. The detection of the predicted patterns in observed oscillation spectra would give constraints on internal rotation and chemical stratification of rapidly rotating stars exhibiting gravity modes, such as {$\gamma$} Doradus, SPB, or Be stars. The obtained results have a mathematical form that is similar to that of the traditional approximation, but the new approximation takes the full Coriolis, which allows for propagation near the centre, and centrifugal accelerations into account.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Chaos,notion,notion-database,Stars: oscillations,Stars: rotation,Waves},
  file = {/Users/lbugnet/Zotero/storage/AQ25JBSH/Prat et al. - 2017.pdf}
}

@article{Prat2018,
  title = {Asymptotic Theory of Gravity Modes in Rotating Stars. {{II}}. {{Impact}} of General Differential Rotation},
  author = {Prat, V. and Mathis, S. and Augustson, K. and Ligni{\`e}res, F. and Ballot, J. and Alvan, L. and Brun, A. S.},
  year = {2018},
  month = jul,
  journal = {Astronomy and Astrophysics},
  volume = {615},
  pages = {A106},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201832576},
  urldate = {2023-10-17},
  abstract = {Context. Differential rotation has a strong influence on stellar internal dynamics and evolution, notably by triggering hydrodynamical instabilities, by interacting with the magnetic field, and more generally by inducing transport of angular momentum and chemical elements. Moreover, it modifies the way waves propagate in stellar interiors and thus the frequency spectrum of these waves, the regions they probe, and the transport they generate. Aims: We investigate the impact of a general differential rotation (both in radius and latitude) on the propagation of axisymmetric gravito-inertial waves. Methods: We use a small-wavelength approximation to obtain a local dispersion relation for these waves. We then describe the propagation of waves thanks to a ray model that follows a Hamiltonian formalism. Finally, we numerically probe the properties of these gravito-inertial rays for different regimes of radial and latitudinal differential rotation. Results: We derive a local dispersion relation that includes the effect of a general differential rotation. Subsequently, considering a polytropic stellar model, we observe that differential rotation allows for a large variety of resonant cavities that can be probed by gravito-inertial waves. We identify that for some regimes of frequency and differential rotation, the properties of gravito-inertial rays are similar to those found in the uniformly rotating case. Furthermore, we also find new regimes specific to differential rotation, where the dynamics of rays is chaotic. Conclusions: As a consequence, we expect modes to follow the same trend. Some parts of oscillation spectra corresponding to regimes similar to those of the uniformly rotating case would exhibit regular patterns, while parts corresponding to the new regimes would be mostly constituted of chaotic modes with a spectrum rather characterised by a generic statistical distribution.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,chaos,stars: oscillations,stars: rotation,waves},
  annotation = {ADS Bibcode: 2018A\&A...615A.106P},
  file = {/Users/lbugnet/Zotero/storage/98HGPMJG/Prat et al. - 2018 - Asymptotic theory of gravity modes in rotating sta.pdf}
}

@article{Prat2019,
  title = {Period Spacings of Gravity Modes in Rapidly Rotating Magnetic Stars {{I}}. {{Axisymmetric}} Fossil Field with Poloidal and Toroidal Components},
  author = {Prat, V. and Mathis, S. and Buysschaert, B. and Van Beeck, J. and Bowman, D. M. and Aerts, C. and Neiner, C.},
  year = {2019},
  journal = {Astronomy and Astrophysics},
  volume = {64},
  eprint = {1903.05620},
  pages = {1--9},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201935462},
  abstract = {Context. Stellar magnetic fields are one of the candidates often invoked to explain the missing transport of angular momentum observed in the models of stellar interiors. However, the properties of an internal magnetic field and the consequences of its presence on stellar evolution are largely unknown. Aims. We study the effect of an axisymmetric internal magnetic field on the frequency of gravity modes in rapidly rotating stars to check whether gravity modes can be used to detect and probe such a field. Methods. Rotation is taken into account using the traditional approximation of rotation and the effect of the magnetic field is computed using a perturbative approach. As a proof of concept, we compute frequency shifts due to a mixed (i.e. with both poloidal and toroidal components) fossil magnetic field for a representative model of a known magnetic, rapidly rotating, slowly pulsating B-type star, namely HD 43317. Results. We find that frequency shifts induced by the magnetic field scale with the square of its amplitude. A magnetic field with a near-core strength of order 150 kG (which is consistent with the observed surface field strength of order 1 kG) leads to signatures that are detectable in period spacings for high-radial-order gravity modes. Conclusions. The predicted frequency shifts can be used to constrain internal magnetic fields and offers the potential for a significant step forward in our interpretation of the observed structure of gravity-mode period spacing patterns in rapidly rotating stars.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,magnetic field,notion,notion-database,oscillations,rotation,stars,waves},
  file = {/Users/lbugnet/Zotero/storage/RDZP9DRU/Prat et al. - 2019(2).pdf}
}

@article{Prat2020,
  title = {Period Spacings of Gravity Modes in Rapidly Rotating Magnetic Stars {{II}}. {{The}} Case of an Oblique Dipolar Fossil Magnetic Field},
  author = {Prat, Vincent and Mathis, St{\'e}phane and Neiner, Coralie and Van Beeck, Jordan and Bowman, Dominic M. and Aerts, Conny},
  year = {2020},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {636},
  eprint = {2003.08218},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201937398},
  urldate = {2020-06-29},
  abstract = {Context. Stellar internal magnetic fields have recently been shown to leave a detectable signature on period spacing patterns of gravity modes. Aims. We investigate the effect of the obliquity of a mixed (poloidal and toroidal) dipolar internal fossil magnetic field with respect to the rotation axis on the frequency of gravity modes in rapidly rotating stars. Methods. We use the traditional approximation of rotation to compute non-magnetic modes, and a perturbative treatment of the magnetic field to compute the corresponding frequency shifts. We apply the new formalism to HD 43317, a magnetic, rapidly rotating, slowly pulsating B-type star, whose field has an obliquity angle of about 80\{\textbackslash deg\}. Results. We find that frequency shifts induced by the magnetic field on high-radial-order gravity modes are larger with increasing obliquity angle, when the magnetic axis is closer to the equatorial region, where these modes are trapped. The maximum value is reached for an obliquity angle of 90\{\textbackslash deg\}. This trend is observed for all mode geometries. Conclusions. Our results predict that the signature of an internal oblique dipolar magnetic field is detectable using asteroseismology of gravity modes.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HTTVWFWF/full-text.pdf}
}

@article{Prendergast1956,
  title = {The {{Equilibrium}} of a {{Self-Gravitating Incompressible Fluid Sphere}} with a {{Magnetic Field}}. {{I}}.},
  author = {Prendergast, Kevin H.},
  year = {1956},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {123},
  pages = {498},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/146186},
  urldate = {2020-07-02},
  abstract = {Abstract image available at:\textbackslash nhttp://adsabs.harvard.edu/abs/1956ApJ...123..498P},
  keywords = {notion,notion-database}
}

@article{Preston1959,
  title = {A {{Spectroscopic Study}} of the {{RR Lyrae Stars}}.},
  author = {Preston, George W.},
  year = {1959},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {130},
  pages = {507},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/146743},
  urldate = {2020-03-31},
  keywords = {notion,notion-database}
}

@article{Price-Whelan2018,
  title = {Binary {{Companions}} of {{Evolved Stars}} in {{APOGEE DR14}}: {{Search Method}} and {{Catalog}} of {$\sim$}5000 {{Companions}}},
  author = {{Price-Whelan}, Adrian M. and Hogg, David W. and Rix, Hans-Walter and De Lee, Nathan and Majewski, Steven R. and Nidever, David L. and Troup, Nicholas and {Fern{\'a}ndez-Trincado}, Jos{\'e} G. and {Garc{\'i}a-Hern{\'a}ndez}, Domingo A. and {Longa-Pe{\~n}a}, Pen{\'e}lope and Nitschelm, Christian and Sobeck, Jennifer and Zamora, Olga},
  year = {2018},
  month = jun,
  journal = {The Astronomical Journal},
  volume = {156},
  number = {1},
  eprint = {1804.04662},
  pages = {18},
  publisher = {{American Astronomical Society}},
  issn = {0004-6256},
  doi = {10.3847/1538-3881/aac387},
  urldate = {2020-08-31},
  abstract = {Multi-epoch radial velocity measurements of stars can be used to identify stellar, sub-stellar, and planetary-mass companions. Even a small number of observation epochs can be informative about companions, though there can be multiple qualitatively different orbital solutions that fit the data. We have custom-built a Monte Carlo sampler (The Joker) that delivers reliable (and often highly multi-modal) posterior samplings for companion orbital parameters given sparse radial-velocity data. Here we use The Joker to perform a search for companions to 96,231 red-giant stars observed in the APOGEE survey (DR14) with \$\textbackslash geq 3\$ spectroscopic epochs. We select stars with probable companions by making a cut on our posterior belief about the amplitude of the stellar radial-velocity variation induced by the orbit. We provide (1) a catalog of 320 companions for which the stellar companion properties can be confidently determined, (2) a catalog of 4,898 stars that likely have companions, but would require more observations to uniquely determine the orbital properties, and (3) posterior samplings for the full orbital parameters for all stars in the parent sample. We show the characteristics of systems with confidently determined companion properties and highlight interesting systems with candidate compact object companions.},
  archiveprefix = {arxiv},
  keywords = {binaries: spectroscopic,methods: data analysis,methods: statistical,notion,notion-database,planets and satellites: fundamental parameters,surveys,techniques: radial velocities}
}

@article{Price-Whelan2018,
  title = {The {{Astropy Project}}: {{Building}} an Inclusive, Open-Science Project and Status of the v2.0 Core Package},
  shorttitle = {The {{Astropy Project}}},
  author = {The Astropy Collaboration and {Price-Whelan}, A. M. and Sip{\H o}cz, B. M. and G{\"u}nther, H. M. and Lim, P. L. and Crawford, S. M. and Conseil, S. and Shupe, D. L. and Craig, M. W. and Dencheva, N. and Ginsburg, A. and VanderPlas, J. T. and Bradley, L. D. and {P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and Aldcroft, T. L. and Cruz, K. L. and Robitaille, T. P. and Tollerud, E. J. and Ardelean, C. and Babej, T. and Bachetti, M. and Bakanov, A. V. and Bamford, S. P. and Barentsen, G. and Barmby, P. and Baumbach, A. and Berry, K. L. and Biscani, F. and Boquien, M. and Bostroem, K. A. and Bouma, L. G. and Brammer, G. B. and Bray, E. M. and Breytenbach, H. and Buddelmeijer, H. and Burke, D. J. and Calderone, G. and Rodr{\'i}guez, J. L. Cano and Cara, M. and Cardoso, J. V. M. and Cheedella, S. and Copin, Y. and Crichton, D. and D{\'A}vella, D. and Deil, C. and Depagne, {\'E} and Dietrich, J. P. and Donath, A. and Droettboom, M. and Earl, N. and Erben, T. and Fabbro, S. and Ferreira, L. A. and Finethy, T. and Fox, R. T. and Garrison, L. H. and Gibbons, S. L. J. and Goldstein, D. A. and Gommers, R. and Greco, J. P. and Greenfield, P. and Groener, A. M. and Grollier, F. and Hagen, A. and Hirst, P. and Homeier, D. and Horton, A. J. and Hosseinzadeh, G. and Hu, L. and Hunkeler, J. S. and Ivezi{\'c}, {\v Z} and Jain, A. and Jenness, T. and Kanarek, G. and Kendrew, S. and Kern, N. S. and Kerzendorf, W. E. and Khvalko, A. and King, J. and Kirkby, D. and Kulkarni, A. M. and Kumar, A. and Lee, A. and Lenz, D. and Littlefair, S. P. and Ma, Z. and Macleod, D. M. and Mastropietro, M. and McCully, C. and Montagnac, S. and Morris, B. M. and Mueller, M. and Mumford, S. J. and Muna, D. and Murphy, N. A. and Nelson, S. and Nguyen, G. H. and Ninan, J. P. and N{\"o}the, M. and Ogaz, S. and Oh, S. and Parejko, J. K. and Parley, N. and Pascual, S. and Patil, R. and Patil, A. A. and Plunkett, A. L. and Prochaska, J. X. and Rastogi, T. and Janga, V. Reddy and Sabater, J. and Sakurikar, P. and Seifert, M. and Sherbert, L. E. and {Sherwood-Taylor}, H. and Shih, A. Y. and Sick, J. and Silbiger, M. T. and Singanamalla, S. and Singer, L. P. and Sladen, P. H. and Sooley, K. A. and Sornarajah, S. and Streicher, O. and Teuben, P. and Thomas, S. W. and Tremblay, G. R. and Turner, J. E. H. and Terr{\'o}n, V. and {van Kerkwijk}, M. H. and {de la Vega}, A. and Watkins, L. L. and Weaver, B. A. and Whitmore, J. B. and Woillez, J. and Zabalza, V.},
  year = {2018},
  month = aug,
  journal = {The Astronomical Journal},
  volume = {156},
  number = {3},
  eprint = {1801.02634},
  primaryclass = {astro-ph},
  pages = {123},
  issn = {1538-3881},
  doi = {10.3847/1538-3881/aabc4f},
  urldate = {2022-07-26},
  abstract = {The Astropy project supports and fosters the development of open-source and openly-developed Python packages that provide commonly-needed functionality to the astronomical community. A key element of the Astropy project is the core package Astropy, which serves as the foundation for more specialized projects and packages. In this article, we provide an overview of the organization of the Astropy project and summarize key features in the core package as of the recent major release, version 2.0. We then describe the project infrastructure designed to facilitate and support development for a broader ecosystem of inter-operable packages. We conclude with a future outlook of planned new features and directions for the broader Astropy project.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/76DDA6BW/The Astropy Collaboration et al. - 2018 - The Astropy Project Building an inclusive, open-s.pdf;/Users/lbugnet/Zotero/storage/69PFTZFH/1801.html}
}

@article{Priest2010a,
  title = {Magnetic {{Coupling}} between the {{Interior}} and {{Atmosphere}} of the {{Sun}}},
  author = {Priest, E},
  year = {2010},
  journal = {Astrophysics and Space Science},
  number = {1908},
  eprint = {0903.4935},
  pages = {10--12},
  doi = {10.1007/978-3-642-02859-5},
  abstract = {Astronomical observation of stellar rotation suggests that at least the surface layers of the Sun have lost a substantial amount of the angular momentum that they possessed at the beginning of the main-sequence phase of evolution, and solar-wind observations indicate that magnetic coupling is still draining angular momentum from the Sun today. In addition, helioseismological analysis has shown that the specific angular momentum at the top of the almost uniformly rotating radiative interior is approximately (although not exactly) the same as the spherically averaged value at the base of the (differentially rotating) convection zone, suggesting that angular momentum is being transported through the tachocline. The mechanism by which that transport is taking place is not understood. Nor is there a consensus of opinion. I review some of the suggestions that have been put forward, biassing my discussion, no doubt, according to my own opinions.},
  archiveprefix = {arxiv},
  isbn = {978-3-642-02858-8},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GQ7EEHDJ/Priest - 2010.pdf;/Users/lbugnet/Zotero/storage/LEYAGLAN/Priest - 2010(2).pdf}
}

@article{Prieto2016,
  title = {The Rotation-Metallicity Relation for the {{Galactic}} Disk as Measured in the {{Gaia DR1 TGAS}} and {{APOGEE}} Data},
  author = {Prieto, Carlos Allende and Kawata, Daisuke and Cropper, Mark},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {596},
  eprint = {1609.07821},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629787},
  abstract = {Aims. Previous studies have found that the Galactic rotation velocity-metallicity (V-[Fe/H]) relations for the thin and thick disk populations show negative and positive slopes, respectively. The first Gaia data release includes the Tycho-Gaia Astrometric Solution (TGAS) information, which we use to analyze the V-[Fe/H] relation for a strictly selected sample with high enough astrometric accuracy. We aim to present an explanation for the slopes of the V-[Fe/H] relationship. Methods. We have identified a sample of stars with accurate Gaia TGAS data and SDSS APOGEE [{$\alpha$}/Fe] and [Fe/H] measurements. We measured the V-[Fe/H] relation for thin and thick disk stars classified on the basis of their [{$\alpha$}/Fe] and [Fe/H] abundances. Results. We find dV/d [Fe/H] =-18 {$\pm$} 2 km s-1 dex-1 for stars in the thin disk and dV/d [Fe/H] = +23 {$\pm$} 10 km s-1 dex-1 for thick disk stars, and thus we confirm the different signs for the slopes. The negative value of dV/d[Fe/H] for thin disk stars is consistent with previous work, but the combination of TGAS and APOGEE data provides higher precision, even though systematic errors could exceed {$\pm$}5 km s-1 dex-1. Our average measurement of dV/d[Fe/H] for local thick disk stars shows a somewhat flatter slope than in previous studies, but we confirm a significant spread and a dependence of the slope on the [{$\alpha$}/Fe] ratio of the stars. Using a simple N-body model, we demonstrate that the observed trends for the thick and thin disk can be explained by the measured radial metallicity gradients and the correlation between orbital eccentricity and metallicity in the thick disk. Conclusions. We conclude that the V-[Fe/H] relation for thin disk stars is well determined from our TGAS-APOGEE sample, and a direct consequence of the radial metallicity gradient and the correlation between Galactic rotation and mean Galactocentric distance. Stars formed farther away from the solar circle tend to be near their orbital pericenter, showing larger velocities and on average lower metallicities, while those closer to the Galactic center are usually closer to their orbital apocenter, therefore moving slower and with higher metallicities. The positive dV/d[Fe/H] for the thick disk sample is likely connected to the correlation between orbital eccentricity and metallicity for that population.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: disk,Galaxy: stellar content,notion,notion-database,Solar neighborhood,Stars: kinematics and dynamics,Stars: late-type},
  file = {/Users/lbugnet/Zotero/storage/QXLBPUBS/Prieto, Kawata, Cropper - 2016.pdf}
}

@article{Project1989,
  title = {National {{Optical Astronomy Observatories}}},
  author = {Project, International Gemini},
  year = {1989},
  number = {February 1999},
  pages = {2--3},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5GPQQLBX/Project - 1989.pdf}
}

@article{Provencal2013,
  title = {Empirical {{Determination}} of {{Convection}} in {{Pulsating White Dwarfs}}},
  author = {Provencal, Judith L. and Hermes, J. J. and Montgomery, M. and Reed, Mike and Shipman, Harry and Fraga, Luciano},
  year = {2013},
  month = feb,
  journal = {NOAO Proposal},
  pages = {100},
  urldate = {2023-10-02},
  abstract = {We propose high speed photometric observations of WD J1518+0658 with SOAR and the KPNO 2m as important components of a coordinated international campaign designed to survey the properties of convection in white dwarf atmospheres. Convection remains the largest source of theoretical uncertainty in our understanding of stellar physics. Asteroseismology has proven a powerful tool to attack this problem. White dwarf pulsations appear as local surface temperature variations. The extreme temperature sensitivity of convection leads to local variations in the convection zone's depth. This in turn modulates the local energy flux, producing nonsinusoidal light curves. The observed nonlinearities provide a self-consistent observational test of convection in white dwarf atmospheres. WD J1518+0658 is a member of the newly discovered class of extremely low mass white dwarf pulsators (ELMVs). ELMVs offer the opportunity to extend our investigation to unexplored regions of lower effective temperatures and surface gravities, where conditions are closer to those found in main sequence stars. High precision light curves from SOAR, combined with frequency, amplitude, and phase information provided by the KPNO 2m and the entire WET run, will allow us to recover WD J1518+0658's convective thermal response timescale.},
  annotation = {ADS Bibcode: 2013noao.prop..100P}
}

@article{Provost2006,
  title = {Asteroseismology and Evolutionary Status of {{Procyon A}}},
  author = {Provost, J. and Berthomieu, G. and Marti{\'c}, M. and Morel, P.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {460},
  number = {3},
  pages = {759--767},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065251},
  abstract = {Models of Procyon A satisfying the actual observational constraints, particularly the asteroseismic ones, are discussed. The oscillations of these models were computed and analysed. We looked for seismic signatures of the evolutionary status of Procyon A. We show that the behavior of the small frequency spacings, particularly {$\delta$}v01 allows us to distinguish between main sequence and post-main sequence models, all satisfying the observational constraints on mass, effective temperature, radius, and surface metallicity of Procyon A. We also introduce a new seismic evolution criterion, {$\epsilon$}, based on the comparison of the low and high frequency parts of the power spectrum. The comparison of the seismic properties of the models with the available asteroseismic observations does not allow us to definitely decide on the stage of evolution of Procyon A. Much more accurate frequencies must be obtained especially in the low-frequency domain to distinguish between the models. \textcopyright{} ESO 2006.},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual: Procyon A,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/DTFDJZVG/Provost et al. - 2006.pdf}
}

@article{Prusti2016,
  title = {The {{Gaia}} Mission},
  author = {Prusti, T. and De Bruijne, J. H.J. and Brown, A. G.A. and Vallenari, A. and Babusiaux, C. and {Bailer-Jones}, C. A.L. and Bastian, U. and Biermann, M. and Evans, D. W. and Eyer, L. and Jansen, F. and Jordi, C. and Klioner, S. A. and Lammers, U. and Lindegren, L. and Luri, X. and Mignard, F. and Milligan, D. J. and Panem, C. and Poinsignon, V. and Pourbaix, D. and Randich, S. and Sarri, G. and Sartoretti, P. and Siddiqui, H. I. and Soubiran, C. and Valette, V. and Van Leeuwen, F. and Walton, N. A. and Aerts, C. and Arenou, F. and Cropper, M. and Drimmel, R. and H{\o}g, E. and Katz, D. and Lattanzi, M. G. and O'Mullane, W. and Grebel, E. K. and Holland, A. D. and Huc, C. and Passot, X. and Bramante, L. and Cacciari, C. and Casta{\~n}eda, J. and Chaoul, L. and Cheek, N. and De Angeli, F. and Fabricius, C. and Guerra, R. and Hern{\'a}ndez, J. and {Jean-Antoine-Piccolo}, A. and Masana, E. and Messineo, R. and Mowlavi, N. and Nienartowicz, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and Panuzzo, P. and Portell, J. and Richards, P. J. and Riello, M. and Seabroke, G. M. and Tanga, P. and Th{\'e}venin, F. and Torra, J. and Els, S. G. and {Gracia-Abril}, G. and Comoretto, G. and {Garcia-Reinaldos}, M. and Lock, T. and Mercier, E. and Altmann, M. and Andrae, R. and Astraatmadja, T. L. and {Bellas-Velidis}, I. and Benson, K. and Berthier, J. and Blomme, R. and Busso, G. and Carry, B. and Cellino, A. and Clementini, G. and Cowell, S. and Creevey, O. and Cuypers, J. and Davidson, M. and De Ridder, J. and De Torres, A. and Delchambre, L. and Dell'Oro, A. and Ducourant, C. and Fr{\'e}mat, Y. and {Garc{\'i}a-Torres}, M. and Gosset, E. and Halbwachs, J. L. and Hambly, N. C. and Harrison, D. L. and Hauser, M. and Hestroffer, D. and Hodgkin, S. T. and Huckle, H. E. and Hutton, A. and Jasniewicz, G. and Jordan, S. and Kontizas, M. and Korn, A. J. and Lanzafame, A. C. and Manteiga, M. and Moitinho, A. and Muinonen, K. and Osinde, J. and Pancino, E. and Pauwels, T. and Petit, J. M. and {Recio-Blanco}, A. and Robin, A. C. and Sarro, L. M. and Siopis, C. and Smith, M. and Smith, K. W. and Sozzetti, A. and Thuillot, W. and Van Reeven, W. and Viala, Y. and Abbas, U. and Abreu Aramburu, A. and Accart, S. and Aguado, J. J. and Allan, P. M. and Allasia, W. and Altavilla, G. and {\'A}lvarez, M. A. and Alves, J. and Anderson, R. I. and Andrei, A. H. and Anglada Varela, E. and Antiche, E. and Antoja, T. and Ant{\'o}n, S. and Arcay, B. and Atzei, A. and Ayache, L. and Bach, N. and Baker, S. G. and {Balaguer-N{\'u}{\~n}ez}, L. and Barache, C. and Barata, C. and Barbier, A. and Barblan, F. and Baroni, M. and Barrado Y Navascu{\'e}s, D. and Barros, M. and Barstow, M. A. and Becciani, U. and Bellazzini, M. and Bellei, G. and Bello Garc{\'i}a, A. and Belokurov, V. and Bendjoya, P. and Berihuete, A. and Bianchi, L. and Bienaym{\'e}, O. and Billebaud, F. and Blagorodnova, N. and {Blanco-Cuaresma}, S. and Boch, T. and Bombrun, A. and Borrachero, R. and Bouquillon, S. and Bourda, G. and Bouy, H. and Bragaglia, A. and Breddels, M. A. and Brouillet, N. and Br{\"u}semeister, T. and Bucciarelli, B. and Budnik, F. and Burgess, P. and Burgon, R. and Burlacu, A. and Busonero, D. and Buzzi, R. and Caffau, E. and Cambras, J. and Campbell, H. and Cancelliere, R. and {Cantat-Gaudin}, T. and Carlucci, T. and Carrasco, J. M. and Castellani, M. and Charlot, P. and Charnas, J. and Charvet, P. and Chassat, F. and Chiavassa, A. and Clotet, M. and Cocozza, G. and Collins, R. S. and Collins, P. and Costigan, G. and Crifo, F. and Cross, N. J.G. and Crosta, M. and Crowley, C. and Dafonte, C. and Damerdji, Y. and Dapergolas, A. and David, P. and David, M. and De Cat, P. and De Felice, F. and De Laverny, P. and De Luise, F. and De March, R. and De Martino, D. and De Souza, R. and Debosscher, J. and Del Pozo, E. and Delbo, M. and Delgado, A. and Delgado, H. E. and Di Marco, F. and Di Matteo, P. and Diakite, S. and Distefano, E. and Dolding, C. and Dos Anjos, S. and Drazinos, P. and Dur{\'a}n, J. and Dzigan, Y. and Ecale, E. and Edvardsson, B. and Enke, H. and Erdmann, M. and Escolar, D. and Espina, M. and Evans, N. W. and Eynard Bontemps, G. and Fabre, C. and Fabrizio, M. and Faigler, S. and Falc{\~a}o, A. J. and Farr{\`a}s Casas, M. and Faye, F. and Federici, L. and Fedorets, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and Fernique, P. and Fienga, A. and Figueras, F. and Filippi, F. and Findeisen, K. and Fonti, A. and Fouesneau, M. and Fraile, E. and Fraser, M. and Fuchs, J. and Furnell, R. and Gai, M. and Galleti, S. and Galluccio, L. and Garabato, D. and {Garc{\'i}a-Sedano}, F. and Gar{\'e}, P. and Garofalo, A. and Garralda, N. and Gavras, P. and Gerssen, J. and Geyer, R. and Gilmore, G. and Girona, S. and Giuffrida, G. and Gomes, M. and {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J. J. and Granvik, M. and Guerrier, A. and Guillout, P. and Guiraud, J. and G{\'u}rpide, A. and {Guti{\'e}rrez-S{\'a}nchez}, R. and Guy, L. P. and Haigron, R. and Hatzidimitriou, D. and Haywood, M. and Heiter, U. and Helmi, A. and Hobbs, D. and Hofmann, W. and Holl, B. and Holland, G. and Hunt, J. A.S. and Hypki, A. and Icardi, V. and Irwin, M. and Jevardat De Fombelle, G. and Jofr{\'e}, P. and Jonker, P. G. and Jorissen, A. and Julbe, F. and Karampelas, A. and Kochoska, A. and Kohley, R. and Kolenberg, K. and Kontizas, E. and Koposov, S. E. and Kordopatis, G. and Koubsky, P. and Kowalczyk, A. and {Krone-Martins}, A. and Kudryashova, M. and Kull, I. and Bachchan, R. K. and {Lacoste-Seris}, F. and Lanza, A. F. and Lavigne, J. B. and {Le Poncin-Lafitte}, C. and Lebreton, Y. and Lebzelter, T. and Leccia, S. and Leclerc, N. and {Lecoeur-Taibi}, I. and Lemaitre, V. and Lenhardt, H. and Leroux, F. and Liao, S. and Licata, E. and Lindstr{\o}m, H. E.P. and Lister, T. A. and Livanou, E. and Lobel, A. and L{\"o}ffler, W. and L{\'o}pez, M. and {Lopez-Lozano}, A. and Lorenz, D. and Loureiro, T. and MacDonald, I. and Magalh{\~a}es Fernandes, T. and Managau, S. and Mann, R. G. and Mantelet, G. and Marchal, O. and Marchant, J. M. and Marconi, M. and Marie, J. and Marinoni, S. and Marrese, P. M. and Marschalk{\'o}, G. and Marshall, D. J. and {Mart{\'i}n-Fleitas}, J. M. and Martino, M. and Mary, N. and Matijevi{\v c}, G. and Mazeh, T. and McMillan, P. J. and Messina, S. and Mestre, A. and Michalik, D. and Millar, N. R. and Miranda, B. M.H. and Molina, D. and Molinaro, R. and Molinaro, M. and Moln{\'a}r, L. and Moniez, M. and Montegriffo, P. and Monteiro, D. and Mor, R. and Mora, A. and Morbidelli, R. and Morel, T. and Morgenthaler, S. and Morley, T. and Morris, D. and Mulone, A. F. and Muraveva, T. and Musella, I. and Narbonne, J. and Nelemans, G. and Nicastro, L. and Noval, L. and Ord{\'e}novic, C. and {Ordieres-Mer{\'e}}, J. and Osborne, P. and Pagani, C. and Pagano, I. and Pailler, F. and Palacin, H. and Palaversa, L. and Parsons, P. and Paulsen, T. and Pecoraro, M. and Pedrosa, R. and Pentik{\"a}inen, H. and Pereira, J. and Pichon, B. and Piersimoni, A. M. and Pineau, F. X. and Plachy, E. and Plum, G. and Poujoulet, E. and Pr{\v s}a, A. and Pulone, L. and Ragaini, S. and Rago, S. and Rambaux, N. and {Ramos-Lerate}, M. and Ranalli, P. and Rauw, G. and Read, A. and Regibo, S. and Renk, F. and Reyl{\'e}, C. and Ribeiro, R. A. and Rimoldini, L. and Ripepi, V. and Riva, A. and Rixon, G. and Roelens, M. and {Romero-G{\'o}mez}, M. and Rowell, N. and Royer, F. and Rudolph, A. and {Ruiz-Dern}, L. and Sadowski, G. and Sagrist{\`a} Sell{\'e}s, T. and Sahlmann, J. and Salgado, J. and Salguero, E. and Sarasso, M. and Savietto, H. and Schnorhk, A. and Schultheis, M. and Sciacca, E. and Segol, M. and Segovia, J. C. and Segransan, D. and Serpell, E. and Shih, I. C. and Smareglia, R. and Smart, R. L. and Smith, C. and Solano, E. and Solitro, F. and Sordo, R. and Soria Nieto, S. and Souchay, J. and Spagna, A. and Spoto, F. and Stampa, U. and Steele, I. A. and Steidelm{\"u}ller, H. and Stephenson, C. A. and Stoev, H. and Suess, F. F. and S{\"u}veges, M. and Surdej, J. and Szabados, L. and {Szegedi-Elek}, E. and Tapiador, D. and Taris, F. and Tauran, G. and Taylor, M. B. and Teixeira, R. and Terrett, D. and Tingley, B. and Trager, S. C. and Turon, C. and Ulla, A. and Utrilla, E. and Valentini, G. and Van Elteren, A. and Van Hemelryck, E. and Van Leeuwen, M. and Varadi, M. and Vecchiato, A. and Veljanoski, J. and Via, T. and Vicente, D. and Vogt, S. and Voss, H. and Votruba, V. and Voutsinas, S. and Walmsley, G. and Weiler, M. and Weingrill, K. and Werner, D. and Wevers, T. and Whitehead, G. and {Wyrzykowski} and Yoldas, A. and {\v Z}erjal, M. and Zucker, S. and Zurbach, C. and Zwitter, T. and Alecu, A. and Allen, M. and Allende Prieto, C. and Amorim, A. and {Anglada-Escud{\'e}}, G. and Arsenijevic, V. and Azaz, S. and Balm, P. and Beck, M. and Bernstein, H. H. and Bigot, L. and Bijaoui, A. and Blasco, C. and Bonfigli, M. and Bono, G. and Boudreault, S. and Bressan, A. and Brown, S. and Brunet, P. M. and Bunclark, P. and Buonanno, R. and Butkevich, A. G. and Carret, C. and Carrion, C. and Chemin, L. and Ch{\'e}reau, F. and Corcione, L. and Darmigny, E. and De Boer, K. S. and De Teodoro, P. and De Zeeuw, P. T. and Delle Luche, C. and Domingues, C. D. and Dubath, P. and Fodor, F. and Fr{\'e}zouls, B. and Fries, A. and Fustes, D. and Fyfe, D. and Gallardo, E. and Gallegos, J. and Gardiol, D. and Gebran, M. and Gomboc, A. and G{\'o}mez, A. and Grux, E. and Gueguen, A. and Heyrovsky, A. and Hoar, J. and Iannicola, G. and Isasi Parache, Y. and Janotto, A. M. and Joliet, E. and Jonckheere, A. and Keil, R. and Kim, D. W. and Klagyivik, P. and Klar, J. and Knude, J. and Kochukhov, O. and Kolka, I. and Kos, J. and Kutka, A. and Lainey, V. and Lebouquin, D. and Liu, C. and Loreggia, D. and Makarov, V. V. and Marseille, M. G. and Martayan, C. and {Martinez-Rubi}, O. and Massart, B. and Meynadier, F. and Mignot, S. and Munari, U. and Nguyen, A. T. and Nordlander, T. and Ocvirk, P. and O'Flaherty, K. S. and Olias Sanz, A. and Ortiz, P. and Osorio, J. and Oszkiewicz, D. and Ouzounis, A. and Palmer, M. and Park, P. and Pasquato, E. and Peltzer, C. and Peralta, J. and P{\'e}turaud, F. and Pieniluoma, T. and Pigozzi, E. and Poels, J. and Prat, G. and Prod'homme, T. and Raison, F. and Rebordao, J. M. and Risquez, D. and {Rocca-Volmerange}, B. and Rosen, S. and {Ruiz-Fuertes}, M. I. and Russo, F. and Sembay, S. and Serraller Vizcaino, I. and Short, A. and Siebert, A. and Silva, H. and Sinachopoulos, D. and Slezak, E. and Soffel, M. and Sosnowska, D. and Strai{\v z}ys, V. and Ter Linden, M. and Terrell, D. and Theil, S. and Tiede, C. and Troisi, L. and Tsalmantza, P. and Tur, D. and Vaccari, M. and Vachier, F. and Valles, P. and Van Hamme, W. and Veltz, L. and Virtanen, J. and Wallut, J. M. and Wichmann, R. and Wilkinson, M. I. and Ziaeepour, H. and Zschocke, S.},
  year = {2016},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {595},
  eprint = {1609.04153},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629272},
  urldate = {2020-03-06},
  abstract = {Gaia is a cornerstone mission in the science programme of the European Space Agency (ESA). The spacecraft construction was approved in 2006, following a study in which the original interferometric concept was changed to a direct-imaging approach. Both the spacecraft and the payload were built by European industry. The involvement of the scientific community focusses on data processing for which the international Gaia Data Processing and Analysis Consortium (DPAC) was selected in 2007. Gaia was launched on 19 December 2013 and arrived at its operating point, the second Lagrange point of the Sun-Earth-Moon system, a few weeks later. The commissioning of the spacecraft and payload was completed on 19 July 2014. The nominal five-year mission started with four weeks of special, ecliptic-pole scanning and subsequently transferred into full-sky scanning mode. We recall the scientific goals of Gaia and give a description of the as-built spacecraft that is currently (mid-2016) being operated to achieve these goals. We pay special attention to the payload module, the performance of which is closely related to the scientific performance of the mission. We provide a summary of the commissioning activities and findings, followed by a description of the routine operational mode. We summarise scientific performance estimates on the basis of in-orbit operations. Several intermediate Gaia data releases are planned and the data can be retrieved from the Gaia Archive, which is available through the Gaia home page.},
  archiveprefix = {arxiv},
  keywords = {Astrometry,Galaxy: structure,notion,notion-database,Parallaxes,Proper motions,Space vehicles: instruments,Telescopes},
  file = {/Users/lbugnet/Zotero/storage/YI5UFLME/full-text.pdf}
}

@article{Prusti2017,
  title = {The {{Gaia}} Mission Status},
  author = {Prusti, T.},
  year = {2017},
  month = apr,
  journal = {Proceedings of the International Astronomical Union},
  volume = {12},
  number = {S330},
  pages = {7--12},
  publisher = {{Cambridge University Press}},
  issn = {17439221},
  doi = {10.1017/S1743921317005816},
  urldate = {2020-03-06},
  abstract = {Gaia is an ESA cornerstone mission conducting a full sky survey over its 5 year operational period. Gaia performs astrometric, photometric and spectroscopic measurements. The data processing is entrusted to scientists and engineers who have formed the Gaia Data Processing and Analysis Consortium (DPAC). The photometric science alerts started in 2014. The first intermediate data release (Gaia DR1) took place 14 September 2016 and it has been extensively used by the community. Gaia DR2 is scheduled for April 2018. Gaia is expected to be able to continue observations roughly for another 5 years after the nominal phase. The procedure to grant funding for the extension period has been initiated. In case funding is granted, the total operational time of Gaia may be 10 years.},
  keywords = {astrometry,catalogs,notion,notion-database,space vehicles,surveys,techniques: photometric,techniques: radial velocities}
}

@misc{PslsPyPI,
  title = {Psls {$\cdot$} {{PyPI}}},
  urldate = {2021-04-06},
  howpublished = {https://pypi.org/project/psls/},
  keywords = {notion,notion-database}
}

@article{Psra2011,
  title = {Kepler Eclipsing Binary Stars. {{I}}. Catalog and Principal Characterization of 1879 Eclipsing Binaries in the First Data Release},
  author = {Psra, Andrej and Batalha, Natalie and Slawson, Robert W. and Doyle, Laurance R. and Welsh, William F. and Orosz, Jerome A. and Seager, Sara and Rucker, Michael and Mjaseth, Kimberly and Engle, Scott G. and Conroy, Kyle and Jenkins, Jon and Caldwell, Douglas and Koch, David and Borucki, William},
  year = {2011},
  month = mar,
  journal = {Astronomical Journal},
  volume = {141},
  number = {3},
  eprint = {1006.2815},
  pages = {83},
  issn = {00046256},
  doi = {10.1088/0004-6256/141/3/83},
  urldate = {2020-04-14},
  abstract = {The Kepler space mission is devoted to finding Earth-size planets orbiting other stars in their habitable zones. Its large, 105 deg2 field of view features over 156,000 stars that are observed continuously to detect and characterize planet transits. Yet, this high-precision instrument holds great promise for other types of objects as well. Here we present a comprehensive catalog of eclipsing binary stars observed by Kepler in the first 44 days of operation, the data being publicly available through MAST as of 2010 June 15. The catalog contains 1879 unique objects. For each object, we provide its Kepler ID (KID), ephemeris (BJD0, P 0), morphology type, physical parameters (T eff, log g, E(B - V)), the estimate of third light contamination (crowding), and principal parameters (T 2/T 1, q, fillout factor, and sin i for overcontacts, and T 2/T 1, (R 1 + R 2)/a, esin {$\omega$}, ecos {$\omega$}, and sin i for detached binaries). We present statistics based on the determined periods and measure the average occurrence rate of eclipsing binaries to be 1.2\% across the Kepler field. We further discuss the distribution of binaries as a function of galactic latitude and thoroughly explain the application of artificial intelligence to obtain principal parameters in a matter of seconds for the whole sample. The catalog was envisioned to serve as a bridge between the now public Kepler data and the scientific community interested in eclipsing binary stars. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {binaries: eclipsing,catalogs,methods: data analysis,methods: numerical,methods: statistical,notion,notion-database,stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/WGLPWAHN/full-text.pdf}
}

@article{Puschmann2005,
  title = {Time Series of High Resolution Photospheric Spectra in a Quiet Region of the {{Sun II}}. {{Analysis}} of the Variation of Physical Quantities of Granular Structures},
  author = {Puschmann, K. G. and Cobo, B. Ruiz and V{\'a}zquez, M. and Bonet, J. A. and Hanslmeier, A.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {441},
  number = {3},
  eprint = {1205.1723},
  pages = {1157--1169},
  issn = {00046361},
  doi = {10.1051/0004-6361:20047193},
  abstract = {From the inversion of a time series of high resolution slit spectrograms obtained from the quiet sun, the spatial and temporal distribution of the thermodynamical quantities and the vertical flow velocity is derived as a function of optical depth (log {$\tau$}) and geometrical height (z). Spatial coherence and phase shift analyses between temperature and vertical velocity depict the height variation of these physical quantities for structures of different size. An average granular cell model is presented, showing the granule-intergranular lane stratification of temperature, vertical velocity, gas pressure and density as a function of log {$\tau$} and z. Studies of a specific small and a specific large granular cell complement these results. A strong decay of the temperature fluctuations with increasing height together with a less efficient penetration of smaller cells is revealed. The T - T coherence at all granular scales is broken already at log {$\tau$} = -1 or z {$\sim$} 170km. At the layers beyond, an inversion of the temperature contrast at granular scales {$>$}1{${''}$}5 is revealed, both in log {$\tau$} and z. At deeper layers the temperature sensitivity of the H- opacity leeds to much smaller temperature fluctuations at equal log {$\tau$} than at equal z, in concordance with Stein \& Nordlund (1998, ApJ, 499, 914). Vertical velocities are in phase throughout the photosphere and penetrate into the highest layers under study. Velocities at the largest granular scales ({$\sim$}4{${''}$}) are still found even at log {$\tau$} {$\sim$} -2.8 or z {$\sim$} 370km. Again a less efficient height penetration of smaller cells concerning convective velocities is revealed, although still at log {$\tau$} {$\sim$} -2 or z {$\sim$} 280 km structures {$>$} 1{${''}$}.4 are detected. A similar size distribution of velocity and temperature structures with height provides observational evidence for substantial overshoot into the photosphere. At deep photospheric layers, the behaviour of the vertical velocities reflected in simulations is for the first time qualitatively reproduced by observations: intergranular velocities are larger than the granular ones and, both reach extrema, where the granular one is shifted towards higher layers. \textcopyright{} ESO 2005.},
  archiveprefix = {arxiv},
  keywords = {Hydrodynamics,notion,notion-database,Radiative transfer,Sun: granulation,Sun: photosphere,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/LY7ECEQ3/Puschmann et al. - 2005.pdf}
}

@inproceedings{Putnet1999,
  title = {Magnetic White Darf Stars - a Review},
  booktitle = {11th {{European Workshop}} on {{White Dwarfs}}},
  author = {Putney, Angela},
  year = {1999},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NQZU5PTR/Putney - 1999.pdf}
}

@article{Quentin2018,
  title = {Rotation and Magnetism in Intermediate-Mass Stars},
  author = {Quentin, L{\'e}o G. and Tout, Christopher A.},
  year = {2018},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {477},
  pages = {2298--2309},
  issn = {0035-8711},
  doi = {10.1093/mnras/sty770},
  urldate = {2023-10-05},
  abstract = {Rotation and magnetism are increasingly recognized as important phenomena in stellar evolution. Surface magnetic fields from a few to 20 000 G have been observed and models have suggested that magnetohydrodynamic transport of angular momentum and chemical composition could explain the peculiar composition of some stars. Stellar remnants such as white dwarfs have been observed with fields from a few to more than 109 G. We investigate the origin of and the evolution, on thermal and nuclear rather than dynamical time-scales, of an averaged large-scale magnetic field throughout a star's life and its coupling to stellar rotation. Large-scale magnetic fields sustained until late stages of stellar evolution with conservation of magnetic flux could explain the very high fields observed in white dwarfs. We include these effects in the Cambridge stellar evolution code using three time-dependant advection-diffusion equations coupled to the structural and composition equations of stars to model the evolution of angular momentum and the two components of the magnetic field. We present the evolution in various cases for a 3 M\_\{{$\odot\rbrace$} star from the beginning to the late stages of its life. Our particular model assumes that turbulent motions, including convection, favour small-scale field at the expense of large-scale field. As a result, the large-scale field concentrates in radiative zones of the star and so is exchanged between the core and the envelope of the star as it evolves. The field is sustained until the end of the asymptotic giant branch, when it concentrates in the degenerate core.\vphantom\}},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: general,stars: magnetic field,stars: rotation,white dwarfs},
  annotation = {ADS Bibcode: 2018MNRAS.477.2298Q},
  file = {/Users/lbugnet/Zotero/storage/P948YTZM/Quentin and Tout - 2018 - Rotation and magnetism in intermediate-mass stars.pdf}
}

@article{Quintana2010,
  title = {Pixel-Level Calibration in the {{Kepler Science Operations Center}} Pipeline},
  author = {Quintana, Elisa V. and Jenkins, Jon M. and Clarke, Bruce D. and Chandrasekaran, Hema and Twicken, Joseph D. and McCauliff, Sean D. and Cote, Miles T. and Klaus, Todd C. and Allen, Christopher and Caldwell, Douglas A. and Bryson, Stephen T.},
  year = {2010},
  journal = {Software and Cyberinfrastructure for Astronomy},
  volume = {7740},
  number = {1},
  pages = {77401X},
  issn = {0277786X},
  doi = {10.1117/12.857678},
  abstract = {We present an overview of the pixel-level calibration of flight data from the Kepler Mission performed within the Kepler Science Operations Center Science Processing Pipeline. This article describes the calibration (CAL) module, which operates on original spacecraft data to remove instrument effects and other artifacts that pollute the data. Traditional CCD data reduction is performed (removal of instrument/detector effects such as bias and dark current), in addition to pixel-level calibration (correcting for cosmic rays and variations in pixel sensitivity), Kepler-specific corrections (removing smear signals which result from the lack of a shutter on the photometer and correcting for distortions induced by the readout electronics), and additional operations that are needed due to the complexity and large volume of flight data. CAL operates on long (\textasciitilde 30 min) and short (\textasciitilde 1 min) sampled data, as well as full-frame images, and produces calibrated pixel flux time series, uncertainties, and other metrics that are used in subsequent Pipeline modules. The raw and calibrated data are also archived in the Multi-mission Archive at Space Telescope at the Space Telescope Science Institute for use by the astronomical community. \textcopyright{} 2010 SPIE.},
  isbn = {9780819482303},
  keywords = {calibration,kepler,notion,notion-database,space telescope,transit photometry},
  file = {/Users/lbugnet/Zotero/storage/ABSC3VIL/Quintana et al. - 2010.pdf}
}

@article{Radler1987,
  title = {On the Oscillatory Behaviour of Kinematic Mean-field Dynamos},
  author = {R{\"a}dler, K. -H and Br{\"a}uer, H. -J},
  year = {1987},
  journal = {Astronomische Nachrichten},
  volume = {308},
  number = {2},
  pages = {101--109},
  issn = {15213994},
  doi = {10.1002/asna.2113080203},
  urldate = {2020-07-13},
  abstract = {The paper considers the question after the circumstances in which kinematic mean-field dynamos can have oscillatory magnetic field modes. The conducting fluid body is allowed to be of almost arbitrary shape; its surroundings are vacuum. A general relation for the frequency of oscillation is derived. This relation is discussed more closely for models with pure {$\alpha$}2-mechanism. Proof is given that no oscillations can occur for constant {$\alpha$}. The investigations published so far on spherical models with pure {$\alpha$}2-mechanism call up the question whether there is a chance for axisymmetric modes to be oscillatory. For both spherical models and disk models the possibility of oscillatory axisymmetric modes is demonstrated by examples. Copyright \textcopyright{} 1987 WILEY-VCH Verlag GmbH \& Co. KGaA},
  keywords = {dynamo theory,magnetic fields,notion,notion-database,oscillations}
}

@article{Raghavan2010,
  title = {A {{Survey}} of {{Stellar Families}}: {{Multiplicity}} of {{Solar-Type Stars}}},
  author = {Raghavan, Deepak and McAlister, Harold A. and Henry, Todd J. and Latham, David W. and Marcy, Geoffrey W. and Mason, Brian D. and Gies, Douglas R. and White, Russel J. and ten Brummelaar, Theo A.},
  year = {2010},
  month = jul,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {190},
  number = {1},
  eprint = {1007.0414},
  pages = {1--42},
  doi = {10.1088/0067-0049/190/1/1},
  urldate = {2020-07-14},
  abstract = {We present the results of a comprehensive assessment of companions to solar-type stars. A sample of 454 stars, including the Sun, was selected from the Hipparcos catalog with \{\textbackslash pi\} {$>$} 40 mas, \{\textbackslash sigma\}\_\{\textbackslash pi\}/\{\textbackslash pi\} {$<$} 0.05, 0.5 {$<$} B - V {$<$} 1.0 (\textasciitilde{} F6-K3), and constrained by absolute magnitude and color to exclude evolved stars. New observational aspects of this work include surveys for (1) very close companions with long-baseline interferometry at the CHARA Array, (2) close companions with speckle interferometry, and (3) wide proper motion companions identified by blinking multi-epoch archival images. In addition, we include the results from extensive radial-velocity monitoring programs and evaluate companion information from various catalogs. The overall observed fractions of single, double, triple, and higher order systems are 56\% \textbackslash pm 2\%, 33\% \textbackslash pm 2\%, 8\% \textbackslash pm 1\%, and 3\% \textbackslash pm 1\%, respectively, counting all confirmed stellar and brown dwarf companions. Our completeness analysis indicates that only a few undiscovered companions remain in this well-studied sample, implying that the majority (54\% \textbackslash pm 2\%) of solar-type stars are single, in contrast to the results of prior multiplicity studies. The orbital-period distribution of companions is unimodal and roughly log-normal with a peak of about 300 years. The period-eccentricity relation shows a roughly flat distribution beyond the expected circularization for periods below 12 days. The mass-ratio distribution shows a preference for like-mass pairs, which occur more frequently in relatively close pairs. The fraction of planet hosts among single, binary, and multiple systems are statistically indistinguishable, suggesting that planets are as likely to form around single stars as they are around components of binary or multiple systems with sufficiently wide separations.},
  archiveprefix = {arxiv},
  keywords = {binaries,general-planetary systems-stars,machine-readable tables,notion,notion-database,solar-type-stars,statistics-surveys Online-only material},
  file = {/Users/lbugnet/Zotero/storage/MHGNVQL5/full-text.pdf}
}

@article{rajpurohitExploringStellarProperties2018,
  title = {Exploring the Stellar Properties of {{M}} Dwarfs with High-Resolution Spectroscopy from the Optical to the near-Infrared *},
  author = {Rajpurohit, A S and Allard, F and Rajpurohit, S and Sharma, R and Teixeira, G D C and Mousis, O and Kamlesh, R},
  year = {2018},
  eprint = {1810.13252v3},
  urldate = {2021-08-01},
  abstract = {Context. Being the most numerous and oldest stars in the galaxy, M dwarfs are objects of great interest for exoplanet searches. The presence of molecules in their atmosphere complicates our understanding of their atmospheric properties. But great advances have recently been made in the modeling of M dwarfs due to the revision of solar abundances. Aims. We aim to determine stellar parameters of M dwarfs using high resolution spectra (R{$\sim$}90 000) simultaneously in the visible and the near-infrared. The high resolution spectra and broad wavelength coverage provide an unique opportunity to understand the onset of dust and cloud formation at cool temperatures. Furthermore, this study will help in understanding the physical processes which occur in a cool atmospheres, particularly, the redistribution of energy from the optical to the near-infrared. Methods. The stellar parameters of M dwarfs in our sample have been determined by comparing the high resolution spectra both in the optical and in the near-infrared simultaneously observed by CARMENES with the synthetic spectra obtained from the BT-Settl model atmosphere. The detailed spectral synthesis of these observed spectra both in the optical and in the near-infrared helps to understand the missing continuum opacity. Results. For the first time, we derive fundamental stellar parameters of M dwarfs using the high resolution optical and near-infrared spectra simultaneously. We determine T eff , log g and [M/H] for 292 M dwarfs of spectral type M0 to M9, where the formation of dust and clouds are important. The derived T eff for the sample ranges from 2300 to 4000 K, values of log g ranges from 4.5 {$\leq$} log g {$\leq$} 5.5 and the resulting metallicity ranges from-0.5 {$\leq$} [M/H] {$\leq$} +0.5. We have also explored the possible differences in T eff , log g and [M/H] by comparing them with other studies of the same sample of M dwarfs.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars},
  file = {/Users/lbugnet/Zotero/storage/F3CWG846/full-text.pdf}
}

@article{Ramirez2005a,
  title = {The {{Effective Temperature Scale}} of {{FGK Stars}}. {{II}}. {{T}} Eff : {{Color}} : [{{Fe}}/{{H}}] {{Calibrations}}},
  author = {Ramirez, Ivan and Melendez, Jorge},
  year = {2005},
  journal = {The Astrophysical Journal},
  volume = {626},
  number = {1},
  eprint = {astro-ph/0503110},
  pages = {465--485},
  issn = {0004-637X},
  doi = {10.1086/430102},
  abstract = {We present up-to-date metallicity-dependent temperature versus color calibrations for main-sequence and giant stars based on temperatures derived with the infrared flux method (IRFM). Seventeen colors in the photometric systems UBV, uvby, Vilnius, Geneva, RI(Cousins), DDO, Hipparcos-Tycho, and Two Micron All Sky Survey (2MASS) have been calibrated. The spectral types covered by the calibrations range from F0 to K5 (7000K{$>\sptilde$}Teff{$>\sptilde$}4000K) with some relations extending below 4000 K or up to 8000 K. Most of the calibrations are valid in the metallicity range -3.5{$>\sptilde$}[Fe/H]{$>\sptilde$}0.4, although some of them extend to as low as [Fe/H]\textasciitilde -4.0. All fits to the data have been performed with more than 100 stars; standard deviations range from 30 to 120 K. Fits were carefully performed and corrected to eliminate the small systematic errors introduced by the calibration formulae. Tables of colors as a function of Teff and [Fe/H] are provided. This work is largely based on the study by A. Alonso and collaborators; thus, our relations do not significantly differ from theirs except for the very metal-poor hot stars. From the calibrations, the temperatures of 44 dwarf and giant stars with direct temperatures available are obtained. The comparison with direct temperatures confirms our finding in Paper I that the zero point of the IRFM temperature scale is in agreement, to the 10 K level, with the absolute temperature scale (that based on stellar angular diameters) within the ranges of atmospheric parameters covered by those 44 stars. The colors of the Sun are derived from the present IRFM Teff scale and they compare well with those of five solar analogs. It is shown that if the IRFM Teff scale accurately reproduces the temperatures of very metal-poor stars, systematic errors of the order of 200 K, introduced by the assumption of (V-K) being completely metallicity independent when studying very metal-poor dwarf stars, are no longer acceptable. Comparisons with other Teff scales, both empirical and theoretical, are also shown to be in reasonable agreement with our results, although it seems that both Kurucz and MARCS synthetic colors fail to predict the detailed metallicity dependence, given that for [Fe/H]=-2.0, differences as high as approximately +/-200 K are found.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/FGIK9QCK/Ramirez, Melendez - 2005.pdf}
}

@article{Rao2018,
  title = {Star-Planet Interactions: {{V}}. {{Dynamical}} and Equilibrium Tides in Convective Zones},
  author = {Rao, Suvrat and Meynet, Georges and Eggenberger, Patrick and Haemmerl{\'e}, Lionel and Privitera, Giovanni and Georgy, Cyril and Ekstr{\"o}m, Sylvia and Mordasini, Christoph},
  year = {2018},
  journal = {Astronomy and Astrophysics},
  volume = {618},
  eprint = {1807.01474},
  pages = {1--13},
  issn = {14320746},
  doi = {10.1051/0004-6361/201833107},
  abstract = {Context. When planets are formed from the protoplanetary disk and after the disk has dissipated, the evolution of their orbits is governed by tidal interactions, friction, and gravitational drag, and also by changes in the mass of the star and planet. These interactions may change the initial distribution of the distances between the planets and their host star by expanding the original orbit, by contracting it (which may cause an engulfment of the planet by the star), or by destroying the planet. Aims. We study the evolution of the orbit of a planet orbiting its host star under the effects of equilibrium tides, dynamical tides, drag (frictional and gravitational), and stellar mass loss. Methods. We used the Geneva stellar evolution code to compute the evolution of stars with initial masses of 1 and 1.5 M{$\odot$} with different rotation rates at solar metallicity. The star is evolved from the pre-main-sequence (PMS) up to the tip of the red giant branch. We used these models as input for computing the evolution of the planetary orbits. We explored the effects of changing the planet masses (of 1 Earth mass up to 20 Jupiter masses), the distance between the planet and the star (of 0.015 and more than 3 au), the mass, and the spin of the star. We present results when only the equilibrium tide was accounted for and when both equilibrium and dynamical tides were accounted for. The expression for the dynamical tide is a frequency-Averaged dissipation of tidally excited inertial waves, obtained from a piecewise homogeneous two-layer stellar model. Gravity wave damping was neglected. Results. Dynamical tides in convective zones have a significant effect on planetary orbits only during the PMS phase and only for fast-rotating stars. They have no significant effects during the PMS phase for initially slow-rotating stars and during the red giant branch phase, regardless of the initial rotation. In the plots of initial orbital distance versus planetary mass, we show the regions that lead to engulfment or any significant changes in the orbit. As a result of orbital evolution, a region near the star can become devoid of planets after the PMS phase. We call this zone the planet desert, and its extent depends sensitively on stellar rotation. An examination of the planet distribution as a function of distance to the host star and mass can provide constraints on current computations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planet-star interactions,Planetary systems},
  file = {/Users/lbugnet/Zotero/storage/6C573HLW/Rao et al. - 2018(2).pdf}
}

@article{Rashba2007,
  title = {Probing the Internal Solar Magnetic Field through g Modes},
  author = {Rashba, T. I. and Semikoz, V. B. and {Turck-Chi{\`e}ze}, S. and Valle, J. W.F.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {377},
  number = {1},
  eprint = {astro-ph/0611728},
  pages = {453--458},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.11626.x},
  abstract = {The observation of g-mode candidates by the Solar and Heliospheric Observatory (SOHO) mission opens the possibility of probing the internal structure of the solar radiative zone (RZ) and the solar core more directly than possible via the use of the p-mode helioseismology data. We study the effect of rotation and RZ magnetic fields on g-mode frequencies. Using a self-consistent static magnetohydrodynamics magnetic field model, we show that a 1 per cent g-mode frequency shift with respect to the Solar Seismic Model (SSEM) prediction, currently hinted in the Global Oscillation at Low Frequencies (GOLF) data, can be obtained for magnetic fields as low as 300 kG, for current measured modes of radial order. On the other hand, we also argue that a similar shift for the case of the low-order g-mode candidate frequencies cannot result from rotation effects nor from central magnetic fields, unless these exceed 8 MG. \textcopyright{} 2007 RAS.},
  archiveprefix = {arxiv},
  keywords = {MHD,notion,notion-database,Sun: helioseismology,Sun: interior,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/NT2N29V9/Rashba et al. - 2007.pdf;/Users/lbugnet/Zotero/storage/UAHLUDVK/Rashba et al. - 2007(2).pdf}
}

@article{Raskin2011,
  title = {Astrophysics {{HERMES}} : A High-Resolution Fibre-Fed Spectrograph},
  author = {Raskin, G. and Van Winckel, H. and Hensberge, H. and Jorissen, A. and Lehmann, H. and Waelkens, C. and Avila, G. and De Cuyper, J.},
  year = {2011},
  journal = {Astronomy \& Astrophysics},
  volume = {69},
  number = {April 2009},
  pages = {1--12},
  doi = {10.1051/0004-6361/201015435},
  abstract = {The HERMES high-resolution spectrograph project aims at exploiting the specific potential of small but flexible telescopes in ob- servational astrophysics. The optimised optical design of the spectrograph is based on the well-proven concept of white-pupil beam folding for high-resolution spectroscopy. In this contribution we present the complete project, including the spectrograph design and procurement details, the telescope adaptor and calibration unit, the detector system, as well as the optimised data-reduction pipeline. We present a detailed performance analysis to show that the spectrograph performs as specified both in optical quality and in total efficiency. With a spectral resolution of 85 000 (63 000 for the low-resolution fibre), a spectral coverage from 377 to 900 nm in a single exposure and a peak efficiency of 28\%, HERMES proves to be an ideal instrument for building up time series of high-quality data of variable (stellar) phenomena. Key},
  keywords = {abundances,instrumentation,notion,notion-database,radial velocities,spectrographs,spectroscopic,stars,techniques},
  file = {/Users/lbugnet/Zotero/storage/D2UDMKWS/Raskin et al. - 2011.pdf}
}

@article{Rast1995,
  title = {On the Nature of 'exploding' Granules and Granule Fragmentation},
  author = {Rast, Mark Peter},
  year = {1995},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {443},
  pages = {863},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/175576},
  urldate = {2020-03-14},
  abstract = {The morphological evolution of solar granulation is dominated by granule expansion and fragmentation. 'Exploding' granules undergo these processes in a particularly vigorous manner, rapidly expanding to a large size, darkening in the center, and splitting by the formation of dark interior radially directed lanes. We argue that such events can be better understood if granulation is viewed as downflow-dominated surface-driven convection rather than as a collection of more deeply driven upflowing thermal plumes. Regions of maximum granular upflow lie not in the centers of the granules but along their sides, immediately adjacent to the intergranular downflow lanes. These upflows occur primarily in response to the buoyancy and pressure gradient forces induced in proximity to the strongly driven downflow plumes. The upflows are thus dynamically linked to the downflow sites, and granular expansion results in a weakening to the central flow. Radiative losses can then exceed the advected heat supply in the granule center, with the fluid cooling until buoyancy forces becomes sufficient to trigger the formation of a new downflow plume there. Lateral propagation proceeds as neighboring flows are distributed, with propagation preferentially occurring in directions predisposed to weak upflow by the strength and shape of the downflows defining the granule boundary. Thus the radially oriented structures seen in observations of some fragmenting granules may be formed. Finally, the strong downflow plumes initiated in the solar photosphere entrain surrounding material as they descend. With depth this more weakly downflowing material establishes a connectivity which is strikingly of mesogranular scale. This may help to explain the observed correlation between the spatial distribution of exploding granules and mesogranular flows, and suggests that both mesogranulation and supergranulation are secondary manifestations of granulation itself.},
  keywords = {Advection,Buoyancy,CONVECTION,Expansion,Fragmentation,Morphology,notion,notion-database,Photosphere,Plumes,Pressure Distribution,Radiative Heat Transfer,Solar Convection (Astronomy),Solar Granulation,Solar Physics,SUN: GRANULATION}
}

@article{Rast2003,
  title = {{{THE SCALES OF GRANULATION}}, {{MESOGRANULATION}}, {{AND SUPERGRANULATION}}},
  author = {Rast, Mark Peter},
  year = {2003},
  journal = {The Astronomy and Astrophysics Review},
  volume = {597},
  urldate = {2020-03-14},
  abstract = {Solar granulation is described as an advection-fragmentation process in the upper layers of the convection zone. The fundamental hydrodynamic unit is the downflow plume, and from its structure the granular scale follows. Moreover, through the collective advective interaction of many small-scale and short-lived granular plumes, large spatial and long temporal mesogranular and supergranular scales naturally arise. We illustrate and examine this process of scale selection using a simplified n-body advective-interaction model. For parameters set by granulation observations and numerical plume simulations, clustering scales remarkably close to observed mesogranulation and supergranulation result.},
  keywords = {convection-hydrodynamics-Sun,granulation-Sun,mpeg animation,notion,notion-database,photosphere On-line material,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/XZ8MN5AG/full-text.pdf}
}

@book{Rauer2014,
  title = {The {{PLATO}} 2.0 Mission},
  author = {Rauer, H. and Catala, C. and Aerts, C. and Appourchaux, T. and Benz, W. and Brandeker, A. and {Christensen-Dalsgaard}, J. and Deleuil, M. and Gizon, L. and Goupil, M. J. and G{\"u}del, M. and {Janot-Pacheco}, E. and {Mas-Hesse}, M. and Pagano, I. and Piotto, G. and Pollacco, D. and {Santos} and Smith, A. and Su{\'a}rez, J. C. and Szab{\'o}, R. and Udry, S. and Adibekyan, V. and Alibert, Y. and Almenara, J. M. and {Amaro-Seoane}, P. and Eiff, M. A.V. and Asplund, M. and Antonello, E. and Barnes, S. and Baudin, F. and Belkacem, K. and Bergemann, M. and Bihain, G. and Birch, A. C. and Bonfils, X. and Boisse, I. and Bonomo, A. S. and Borsa, F. and Brand{\~a}o, I. M. and Brocato, E. and Brun, S. and Burleigh, M. and Burston, R. and Cabrera, J. and Cassisi, S. and Chaplin, W. and Charpinet, S. and Chiappini, C. and Church, R. P. and Csizmadia, Sz and Cunha, M. and Damasso, M. and Davies, M. B. and Deeg, H. J. and D{\'i}az, R. F. and Dreizler, S. and Dreyer, C. and Eggenberger, P. and Ehrenreich, D. and Eigm{\"u}ller, P. and Erikson, A. and Farmer, R. and Feltzing, S. and {de Oliveira Fialho}, F. and Figueira, P. and Forveille, T. and Fridlund, M. and Garc{\'i}a, R. A. and Giommi, P. and Giuffrida, G. and Godolt, M. and {da Silva}, J. Gomes and Granzer, T. and Grenfell, J. L. and {Grotsch-Noels}, A. and G{\"u}nther, E. and Haswell, C. A. and Hatzes, A. P. and H{\'e}brard, G. and Hekker, S. and Helled, R. and Heng, K. and Jenkins, J. M. and Johansen, A. and Khodachenko, M. L. and Kislyakova, K. G. and Kley, W. and Kolb, U. and Krivova, N. and Kupka, F. and Lammer, H. and Lanza, A. F. and Lebreton, Y. and Magrin, D. and {Marcos-Arenal}, P. and Marrese, P. M. and Marques, J. P. and Martins, J. and Mathis, S. and Mathur, S. and Messina, S. and Miglio, A. and Montalban, J. and Montalto, M. and P. F. G. Monteiro, M. J. and Moradi, H. and Moravveji, E. and Mordasini, C. and Morel, T. and Mortier, A. and Nascimbeni, V. and Nelson, R. P. and Nielsen, M. B. and Noack, L. and Norton, A. J. and Ofir, A. and Oshagh, M. and Ouazzani, R. M. and P{\'a}pics, P. and Parro, V. C. and Petit, P. and Plez, B. and Poretti, E. and Quirrenbach, A. and Ragazzoni, R. and Raimondo, G. and Rainer, M. and Reese, D. R. and Redmer, R. and Reffert, S. and {Rojas-Ayala}, B. and Roxburgh, I. W. and Salmon, S. and Santerne, A. and Schneider, J. and Schou, J. and Schuh, S. and Schunker, H. and {Silva-Valio}, A. and Silvotti, R. and Skillen, I. and Snellen, I. and Sohl, F. and Sousa, S. G. and Sozzetti, A. and Stello, D. and Strassmeier, K. G. and {\v S}vanda, M. and Szab{\'o}, Gy M. and Tkachenko, A. and Valencia, D. and Van Grootel, V. and Vauclair, S. D. and Ventura, P. and Wagner, F. W. and Walton, N. A. and Weingrill, J. and Werner, S. C. and Wheatley, P. J. and Zwintz, K.},
  year = {2014},
  journal = {Experimental Astronomy},
  volume = {38},
  eprint = {1310.0696},
  issn = {09226435},
  doi = {10.1007/s10686-014-9383-4},
  abstract = {PLATO 2.0 has recently been selected for ESA's M3 launch opportunity (2022/24). Providing accurate key planet parameters (radius, mass, density and age) in statistical numbers, it addresses fundamental questions such as: How do planetary systems form and evolve? Are there other systems with planets like ours, including potentially habitable planets? The PLATO 2.0 instrument consists of 34 small aperture telescopes (32 with 25 s readout cadence and 2 with 2.5 s candence) providing a wide field-of-view (2232 deg \textsuperscript{2}) and a large photometric magnitude range (4\textendash 16 mag). It focusses on bright (4\textendash 11 mag) stars in wide fields to detect and characterize planets down to Earth-size by photometric transits, whose masses can then be determined by ground-based radial-velocity follow-up measurements. Asteroseismology will be performed for these bright stars to obtain highly accurate stellar parameters, including masses and ages. The combination of bright targets and asteroseismology results in high accuracy for the bulk planet parameters: 2 \%, 4\textendash 10 \% and 10 \% for planet radii, masses and ages, respectively. The planned baseline observing strategy includes two long pointings (2\textendash 3 years) to detect and bulk characterize planets reaching into the habitable zone (HZ) of solar-like stars and an additional step-and-stare phase to cover in total about 50 \% of the sky. PLATO 2.0 will observe up to 1,000,000 stars and detect and characterize hundreds of small planets, and thousands of planets in the Neptune to gas giant regime out to the HZ. It will therefore provide the first large-scale catalogue of bulk characterized planets with accurate radii, masses, mean densities and ages. This catalogue will include terrestrial planets at intermediate orbital distances, where surface temperatures are moderate. Coverage of this parameter range with statistical numbers of bulk characterized planets is unique to PLATO 2.0. The PLATO 2.0 catalogue allows us to e.g.: - complete our knowledge of planet diversity for low-mass objects, - correlate the planet mean density-orbital distance distribution with predictions from planet formation theories,- constrain the influence of planet migration and scattering on the architecture of multiple systems, and - specify how planet and system parameters change with host star characteristics, such as type, metallicity and age. The catalogue will allow us to study planets and planetary systems at different evolutionary phases. It will further provide a census for small, low-mass planets. This will serve to identify objects which retained their primordial hydrogen atmosphere and in general the typical characteristics of planets in such low-mass, low-density range. Planets detected by PLATO 2.0 will orbit bright stars and many of them will be targets for future atmosphere spectroscopy exploring their atmosphere. Furthermore, the mission has the potential to detect exomoons, planetary rings, binary and Trojan planets. The planetary science possible with PLATO 2.0 is complemented by its impact on stellar and galactic science via asteroseismology as well as light curves of all kinds of variable stars, together with observations of stellar clusters of different ages. This will allow us to improve stellar models and study stellar activity. A large number of well-known ages from red giant stars will probe the structure and evolution of our Galaxy. Asteroseismic ages of bright stars for different phases of stellar evolution allow calibrating stellar age-rotation relationships. Together with the results of ESA's Gaia mission, the results of PLATO 2.0 will provide a huge legacy to planetary, stellar and galactic science.},
  archiveprefix = {arxiv},
  isbn = {1-06-860149-3},
  keywords = {Asteroseismology,Exoplanetary science,Exoplanets,notion,notion-database,Stellar science,Transit survey},
  file = {/Users/lbugnet/Zotero/storage/MVXJD36P/Rauer et al. - 2014.pdf}
}

@article{Rauer2014a,
  title = {The {{PLATO}} 2.0 Mission},
  author = {Rauer, H. and Catala, C. and Aerts, C. and Appourchaux, T. and Benz, W. and Brandeker, A. and {Christensen-Dalsgaard}, J. and Deleuil, M. and Gizon, L. and Goupil, M. J. and G{\"u}del, M. and {Janot-Pacheco}, E. and {Mas-Hesse}, M. and Pagano, I. and Piotto, G. and Pollacco, D. and {Santos} and Smith, A. and Su{\'a}rez, J. C. and Szab{\'o}, R. and Udry, S. and Adibekyan, V. and Alibert, Y. and Almenara, J. M. and {Amaro-Seoane}, P. and Eiff, M. A.V. and Asplund, M. and Antonello, E. and Barnes, S. and Baudin, F. and Belkacem, K. and Bergemann, M. and Bihain, G. and Birch, A. C. and Bonfils, X. and Boisse, I. and Bonomo, A. S. and Borsa, F. and Brand{\~a}o, I. M. and Brocato, E. and Brun, S. and Burleigh, M. and Burston, R. and Cabrera, J. and Cassisi, S. and Chaplin, W. and Charpinet, S. and Chiappini, C. and Church, R. P. and Csizmadia, Sz and Cunha, M. and Damasso, M. and Davies, M. B. and Deeg, H. J. and D{\'i}az, R. F. and Dreizler, S. and Dreyer, C. and Eggenberger, P. and Ehrenreich, D. and Eigm{\"u}ller, P. and Erikson, A. and Farmer, R. and Feltzing, S. and {de Oliveira Fialho}, F. and Figueira, P. and Forveille, T. and Fridlund, M. and Garc{\'i}a, R. A. and Giommi, P. and Giuffrida, G. and Godolt, M. and {da Silva}, J. Gomes and Granzer, T. and Grenfell, J. L. and {Grotsch-Noels}, A. and G{\"u}nther, E. and Haswell, C. A. and Hatzes, A. P. and H{\'e}brard, G. and Hekker, S. and Helled, R. and Heng, K. and Jenkins, J. M. and Johansen, A. and Khodachenko, M. L. and Kislyakova, K. G. and Kley, W. and Kolb, U. and Krivova, N. and Kupka, F. and Lammer, H. and Lanza, A. F. and Lebreton, Y. and Magrin, D. and {Marcos-Arenal}, P. and Marrese, P. M. and Marques, J. P. and Martins, J. and Mathis, S. and Mathur, S. and Messina, S. and Miglio, A. and Montalban, J. and Montalto, M. and P. F. G. Monteiro, M. J. and Moradi, H. and Moravveji, E. and Mordasini, C. and Morel, T. and Mortier, A. and Nascimbeni, V. and Nelson, R. P. and Nielsen, M. B. and Noack, L. and Norton, A. J. and Ofir, A. and Oshagh, M. and Ouazzani, R. M. and P{\'a}pics, P. and Parro, V. C. and Petit, P. and Plez, B. and Poretti, E. and Quirrenbach, A. and Ragazzoni, R. and Raimondo, G. and Rainer, M. and Reese, D. R. and Redmer, R. and Reffert, S. and {Rojas-Ayala}, B. and Roxburgh, I. W. and Salmon, S. and Santerne, A. and Schneider, J. and Schou, J. and Schuh, S. and Schunker, H. and {Silva-Valio}, A. and Silvotti, R. and Skillen, I. and Snellen, I. and Sohl, F. and Sousa, S. G. and Sozzetti, A. and Stello, D. and Strassmeier, K. G. and {\v S}vanda, M. and Szab{\'o}, Gy M. and Tkachenko, A. and Valencia, D. and Van Grootel, V. and Vauclair, S. D. and Ventura, P. and Wagner, F. W. and Walton, N. A. and Weingrill, J. and Werner, S. C. and Wheatley, P. J. and Zwintz, K.},
  year = {2014},
  journal = {Experimental Astronomy},
  volume = {38},
  number = {1-2},
  eprint = {1310.0696},
  pages = {249--330},
  publisher = {{Kluwer Academic Publishers}},
  issn = {09226435},
  doi = {10.1007/s10686-014-9383-4},
  urldate = {2020-03-08},
  abstract = {PLATO 2.0 has recently been selected for ESA's M3 launch opportunity (2022/24). Providing accurate key planet parameters (radius, mass, density and age) in statistical numbers, it addresses fundamental questions such as: How do planetary systems form and evolve? Are there other systems with planets like ours, including potentially habitable planets? The PLATO 2.0 instrument consists of 34 small aperture telescopes (32 with 25 s readout cadence and 2 with 2.5 s candence) providing a wide field-of-view (2232 deg \textsuperscript{2}) and a large photometric magnitude range (4\textendash 16 mag). It focusses on bright (4\textendash 11 mag) stars in wide fields to detect and characterize planets down to Earth-size by photometric transits, whose masses can then be determined by ground-based radial-velocity follow-up measurements. Asteroseismology will be performed for these bright stars to obtain highly accurate stellar parameters, including masses and ages. The combination of bright targets and asteroseismology results in high accuracy for the bulk planet parameters: 2 \%, 4\textendash 10 \% and 10 \% for planet radii, masses and ages, respectively. The planned baseline observing strategy includes two long pointings (2\textendash 3 years) to detect and bulk characterize planets reaching into the habitable zone (HZ) of solar-like stars and an additional step-and-stare phase to cover in total about 50 \% of the sky. PLATO 2.0 will observe up to 1,000,000 stars and detect and characterize hundreds of small planets, and thousands of planets in the Neptune to gas giant regime out to the HZ. It will therefore provide the first large-scale catalogue of bulk characterized planets with accurate radii, masses, mean densities and ages. This catalogue will include terrestrial planets at intermediate orbital distances, where surface temperatures are moderate. Coverage of this parameter range with statistical numbers of bulk characterized planets is unique to PLATO 2.0. The PLATO 2.0 catalogue allows us to e.g.: - complete our knowledge of planet diversity for low-mass objects, - correlate the planet mean density-orbital distance distribution with predictions from planet formation theories,- constrain the influence of planet migration and scattering on the architecture of multiple systems, and - specify how planet and system parameters change with host star characteristics, such as type, metallicity and age. The catalogue will allow us to study planets and planetary systems at different evolutionary phases. It will further provide a census for small, low-mass planets. This will serve to identify objects which retained their primordial hydrogen atmosphere and in general the typical characteristics of planets in such low-mass, low-density range. Planets detected by PLATO 2.0 will orbit bright stars and many of them will be targets for future atmosphere spectroscopy exploring their atmosphere. Furthermore, the mission has the potential to detect exomoons, planetary rings, binary and Trojan planets. The planetary science possible with PLATO 2.0 is complemented by its impact on stellar and galactic science via asteroseismology as well as light curves of all kinds of variable stars, together with observations of stellar clusters of different ages. This will allow us to improve stellar models and study stellar activity. A large number of well-known ages from red giant stars will probe the structure and evolution of our Galaxy. Asteroseismic ages of bright stars for different phases of stellar evolution allow calibrating stellar age-rotation relationships. Together with the results of ESA's Gaia mission, the results of PLATO 2.0 will provide a huge legacy to planetary, stellar and galactic science.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Exoplanetary science,Exoplanets,notion,notion-database,Stellar science,Transit survey}
}

@article{Rawls2016,
  title = {Kic 9246715: The {{Double Red Giant Eclipsing Binary With Odd Oscillations}}},
  author = {Rawls, Meredith L. and Gaulme, Patrick and McKeever, Jean and Jackiewicz, Jason and Orosz, Jerome A. and Corsaro, Enrico and Beck, Paul G. and Mosser, Beno{\^i}t and Latham, David W. and Latham, Christian A.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {818},
  number = {2},
  eprint = {1601.00038},
  pages = {108},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/818/2/108},
  abstract = {We combine Kepler photometry with ground-based spectra to present a comprehensive dynamical model of the double red giant eclipsing binary KIC 9246715. While the two stars are very similar in mass (M1 = 2.171 [+0.006 / -0.008], M2 = 2.149 [+0.006 / -0.008] Msun) and radius (R1 = 8.37 [+0.03 / -0.07], R2 = 8.30 [+0.04 / -0.03] Rsun), an asteroseismic analysis finds one main set of solar-like oscillations with unusually low-amplitude, wide modes. A second set of oscillations from the other star may exist, but this marginal detection is extremely faint. Because the two stars are nearly twins, KIC 9246715 is a difficult target for a precise test of the asteroseismic scaling relations, which yield M = 2.17 +/- 0.14 Msun and R = 8.26 +/- 0.18 Rsun. Both stars are consistent with the inferred asteroseismic properties, but we suspect the main oscillator is Star 2 because it is less active than Star 1. We find evidence for stellar activity and modest tidal forces acting over the 171-day eccentric orbit, which are likely responsible for the essential lack of solar-like oscillations in one star and weak oscillations in the other. Mixed modes indicate the main oscillating star is on the secondary red clump (a core-He-burning star), and stellar evolution modeling supports this with a coeval history for a pair of red clump stars. This system is a useful case study and paves the way for a detailed analysis of more red giants in eclipsing binaries, an important benchmark for asteroseismology.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/J3YU2EJY/Rawls et al. - 2016.pdf}
}

@article{Read2014,
  title = {The Local Dark Matter Density},
  author = {Read, J. I.},
  year = {2014},
  journal = {Journal of Physics G: Nuclear and Particle Physics},
  volume = {41},
  number = {6},
  eprint = {1404.1938},
  pages = {063101},
  publisher = {{Institute of Physics Publishing}},
  issn = {13616471},
  doi = {10.1088/0954-3899/41/6/063101},
  urldate = {2020-03-06},
  abstract = {I review current efforts to measure the mean density of dark matter near the Sun. This encodes valuable dynamical information about our Galaxy and is also of great importance for 'direct detection' dark matter experiments. I discuss theoretical expectations in our current cosmology; the theory behind mass modelling of the Galaxy; and I show how combining local and global measures probes the shape of the Milky Way dark matter halo and the possible presence of a 'dark disc'. I stress the strengths and weaknesses of different methodologies and highlight the continuing need for detailed tests on mock data - particularly in the light of recently discovered evidence for disequilibria in the Milky Way disc. I collate the latest measurements of {$\rho$}dm and show that, once the baryonic surface density contribution {$\Sigma$}b is normalized across different groups, there is remarkably good agreement. Compiling data from the literature, I estimate {$\Sigma$}b = 54.2 {$\pm$}4.9 M{\.o}pc-2, where the dominant source of uncertainty is in the Hi gas contribution. Assuming this contribution from the baryons, I highlight several recent measurements of {$\rho$}dm in order of increasing data complexity and prior, and, correspondingly, decreasing formal error bars. Comparing these measurements with spherical extrapolations from the Milky Way's rotation curve, I show that the Milky Way is consistent with having a spherical dark matter halo at R0 {$\sim$} 8 kpc. The very latest measures of {$\rho$}dm based on {$\sim$}10000 stars from the Sloan Digital Sky Survey appear to favour little halo flattening at R0, suggesting that the Galaxy has a rather weak dark matter disc, with a correspondingly quiescent merger history. I caution, however, that this result hinges on there being no large systematics that remain to be uncovered in the SDSS data, and on the local baryonic surface density being {$\Sigma$}b {$\sim$} 55 M{\.o}pc-2. I conclude by discussing how the new Gaia satellite will be transformative. We will obtain much tighter constraints on both {$\Sigma$}b and {$\rho$}dm by having accurate 6D phase space data for millions of stars near the Sun. These data will drive us towards fully three dimensional models of our Galactic potential, moving us into the realm of precision measurements of{$\rho$}dm. \textcopyright{} 2014 IOP Publishing Ltd.},
  archiveprefix = {arxiv},
  keywords = {dark matter,direct dark matter detection,local dark matter density,mass modelling,MilkyWay,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/S3UV8GXU/full-text.pdf}
}

@article{Reed2018,
  title = {A Review of Seismic Observations of {{Kepler}} and {{K2-Observed sdBV}} Stars},
  author = {Reed, Michael D. and Baran, Andrzej S. and Telting, John H. and {\O}stensen, Roy H. and Jeffery, Christopher S. and Kern, Joshua W. and Ketzer, Laura and Crooke, John and Slayton, A.},
  year = {2018},
  journal = {Open Astronomy},
  volume = {27},
  number = {1},
  pages = {157--166},
  issn = {25436376},
  doi = {10.1515/astro-2018-0015},
  abstract = {This paper reviews recent seismic findings from Kepler and K2 data. Using three years of short cadence Kepler (K1) data, it is possible to examine time evolution of pulsations in an unprecedented way. While K2 observations are shorter, only three months, they are important as they are finding more sdBV stars than K1 did. Most importantly, K2 is discovering more p-mode pulsators with coverage not possible to get from the ground.},
  keywords = {Kepler \& K2 observations of sdBV stars,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AUZ5WW9F/Reed et al. - 2018.pdf}
}

@article{Reed2021,
  title = {Pulsating Subdwarf {{B}} Stars Observed with {{K2}} during {{Campaign}} 7 and an Examination of Seismic Group Properties},
  author = {Reed, M. D. and Slayton, A. and Baran, A. S. and Telting, J. H. and {\O}stensen, R. H. and Jeffery, C. S. and Uzundag, M. and Sanjayan, S.},
  year = {2021},
  month = nov,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {507},
  pages = {4178--4195},
  issn = {0035-8711},
  doi = {10.1093/mnras/stab2405},
  urldate = {2023-10-14},
  abstract = {We report the discovery of four new pulsating subdwarf B (sdBV) stars from Campaign 7 of the Kepler spacecraft's K2 mission. EPIC 215776487, EPIC 217280630, EPIC 218366972, and EPIC 218717602 are all gravity (g)-mode pulsators and we also detect two pressure (p)-mode pulsations in EPIC 218717602. We detect asymptotic \$\textbackslash ell \textbackslash, =\textbackslash, 1\$ sequences in all four stars, allowing us to identify nearly all of the g modes. We detect evenly spaced frequency multiplets in EPIC 218717602 from which we determine a rotation period near 7 d. Spectroscopic observations determine that EPIC 218366972 is in a 5.92 d binary with most likely a white dwarf companion of canonical mass while the others have no detected companions. As we detect no multiplets in EPIC 218366972, it is added to the growing list of subsynchronously rotating stars. With 40 Kepler-detected sdBV stars and a growing number of Transiting Exoplanet Survey Satellite (TESS) publications, we update an examination of the group properties to provide direction for models. We notice a correlation between effective temperature and period of maximum pulsation amplitude, at least for g-mode pulsations, and update the previously observed effective temperature-rotation period relation.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: oscillations,subdwarfs},
  annotation = {ADS Bibcode: 2021MNRAS.507.4178R},
  file = {/Users/lbugnet/Zotero/storage/DG4IDYAF/Reed et al. - 2021 - Pulsating subdwarf B stars observed with K2 during.pdf}
}

@article{Reese2004,
  title = {Oscillations of Magnetic Stars {{II}}. {{Axisymmetric}} Toroidal and Non-Axisymmetric Shear {{Alfv\'en}} Modes in a Spherical Shell},
  author = {Reese, D. and Rincon, F. and Rieutord, M.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {427},
  number = {1},
  pages = {279--292},
  issn = {00046361},
  doi = {10.1051/0004-6361:20040539},
  abstract = {We carry out numerical and mathematical investigations of shear Alfv\'en waves inside of a spherical shell filled with an incompressible conducting fluid, and bathed in a strong dipolar magnetic field. We focus on axisymmetric toroidal and non-axisymmetric modes, in continuation of a previous work by Rincon \& Rieutord (2003, A\&A, 398, 663). Analytical expressions are obtained for toroidal eigenmodes and their corresponding frequencies at low diffusivities. These oscillations behave like magnetic shear layers, in which the magnetic poles play a key role, and hence become singular when diffusivities vanish. It is also demonstrated that non-axisymmetric modes are split into two categories, namely poloidal or toroidal types, following similar asymptotic behaviours as their axisymmetric counterparts when the diffusivities become arbitrarily small.},
  keywords = {Magnetohydrodynamics (MHD),notion,notion-database,Stars: magnetic fields,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RFTXC48M/Reese, Rincon, Rieutord - 2004.pdf}
}

@article{Reese2006,
  title = {La Mod\'elisation Des Oscillations d ' \'Etoiles En Rotation Rapide {{To}} Cite This Version : {{HAL Id}} : Tel-00120334 {{La}} Mod \textasciiacute{} Elisation Des Oscillations d ' \textasciiacute{} Etoiles En Rotation Rapide},
  author = {Reese, Daniel},
  year = {2006},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZW7HDPE8/Reese - 2006.pdf}
}

@article{Reese2006a,
  title = {Acoustic Oscillations of Rapidly Rotating Polytropic Stars. {{II}}. {{Effects}} of the {{Coriolis}} and Centrifugal Accelerations},
  author = {Reese, D. and Ligni{\`e}res, F. and Rieutord, M.},
  year = {2006},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {455},
  number = {2},
  eprint = {astro-ph/0605503},
  pages = {621--637},
  doi = {10.1051/0004-6361:20065269},
  urldate = {2020-08-10},
  abstract = {Context: With the launch of space missions devoted to asteroseismology (like COROT), the scientific community will soon have accurate measurements of pulsation frequencies in many rapidly rotating stars. Aims: The present work focuses on the effects of rotation on pulsations of rapidly rotating stars when both the Coriolis and centrifugal accelerations require a non-perturbative treatment. Method: We develop a 2-dimensional spectral numerical approach which allows us to compute acoustic modes in centrifugally distorted polytropes including the full influence of the Coriolis force. This method is validated through comparisons with previous studies, and the results are shown to be highly accurate. Results: In the frequency range considered and with COROT's accuracy, we establish a domain of validity for perturbative methods, thus showing the need for complete calculations beyond v.sin i = 50 km/s for a R = 2.3 R\_\textbackslash odot, M = 1.9 M\_\textbackslash odot polytropic star. Furthermore, it is shown that the main differences between complete and perturbative calculations come essentially from the centrifugal distortion.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/Y2XRLMHH/full-text.pdf}
}

@article{Reese2013,
  title = {Mode Visibilities in Rapidly Rotating Stars},
  author = {Reese, D. R. and Prat, V. and Barban, C. and {Van 'T Veer-Menneret}, C. and MacGregor, K. B.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {550},
  pages = {1--28},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220506},
  abstract = {Context. Mode identification is a crucial step to comparing observed frequencies with theoretical ones. However, it has proven to be particularly difficult in rapidly rotating stars. An important reason for this is the lack of simple frequency patterns such as those present in solar-type pulsators. This problem is further aggravated in {$\delta$} Scuti stars by their particularly rich frequency spectra. Aims. As a first step to obtaining further observational constraints towards mode identification in rapid rotators, we aim to accurately calculate mode visibilities and amplitude ratios while fully taking into account the effects of rotation. Methods. We derive the relevant equations for calculating mode visibilities in different photometric bands while fully taking into account the geometric distortion from both the centrifugal deformation and the pulsation modes, the variations in effective gravity, and an approximate treatment of the temperature variations, given the adiabatic nature of the pulsation modes. These equations are then applied to 2D oscillation modes, calculated using the TOP code (Two-dimension Oscillation Program), in fully distorted 2D models based on the self-consistent field (SCF) method. The specific intensities come from a grid of Kurucz atmospheres, thereby taking into account limb and gravity darkening. Results. We obtain mode visibilities and amplitude ratios for 2 M{\.i} models with rotation rates ranging from 0 to 80\% of the critical rotation rate. Based on these calculations, we confirm a number of results from earlier studies, such as the increased visibility of numerous chaotic modes at sufficient rotation rates, the simpler frequency spectra with dominant island modes for pole-on configurations, or the dependence of amplitude ratios on inclination and azimuthal order in rotating stars. In addition, we explain how the geometric shape of the star leads to a smaller contrast between pole-on and equator-on visibilities of equatorially-focused island modes. We also show that modes with similar ({$\mathscr{l}$}, |m|) values frequently have similar amplitude ratios, even in the most rapidly rotating models. \textcopyright{} ESO, 2013.},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations,Stars: rotation,Stars: variables:{$\delta$}Scuti},
  file = {/Users/lbugnet/Zotero/storage/6TMTSSGA/Reese et al. - 2013.pdf}
}

@article{Reeth2016,
  title = {Astrophysics {{Interior}} Rotation of a Sample of {$\gamma$} {{Doradus}} Stars from Ensemble Modelling of Their Gravity-Mode Period Spacings},
  author = {Reeth, T Van and Tkachenko, A and Aerts, C},
  year = {2016},
  journal = {Astronomy \& Astrophysics},
  volume = {593},
  pages = {120},
  doi = {10.1051/0004-6361/201628616},
  urldate = {2020-03-24},
  abstract = {Context. Gamma Doradus stars (hereafter {$\gamma$} Dor stars) are known to exhibit gravity-and/or gravito-intertial modes that probe the inner stellar region near the convective core boundary. The non-equidistant spacing of the pulsation periods is an observational signature of the stellar evolutions and current internal structure and is heavily influenced by rotation. Aims. We aim to constrain the near-core rotation rates for a sample of {$\gamma$} Dor stars for which we have detected period spacing patterns. Methods. We combined the asymptotic period spacing with the traditional approximation of stellar pulsation to fit the observed period spacing patterns using {$\chi$} 2-optimisation. The method was applied to the observed period spacing patterns of a sample of stars and used for ensemble modelling. Results. For the majority of stars with an observed period spacing pattern we successfully determined the rotation rates and the asymptotic period spacing values, although the uncertainty margins on the latter were typically large. This also resulted directly in the identification of the modes that correspond to the detected pulsation frequencies, which for most stars were prograde dipole gravity and gravito-inertial modes. The majority of the observed retrograde modes were found to be Rossby modes. We also discuss the limitations of the method that are due to the neglect of the centrifugal force and the incomplete treatment of the Coriolis force. Conclusions. Despite its current limitations, the proposed method was successful to derive the rotation rates and to identify the modes from the observed period spacing patterns. It forms the first step towards detailed seismic modelling based on observed period spacing patterns of moderately to rapidly rotating {$\gamma$} Dor stars.},
  keywords = {asteroseismology-methods,data analysis-stars,fundamental parameters-stars,general-stars,notion,notion-database,oscillations,variables},
  file = {/Users/lbugnet/Zotero/storage/R233UJ8W/full-text.pdf}
}

@article{Regulo2002,
  title = {A Method to Detect P-Mode Oscillations in Solar-like Star Signals},
  author = {R{\'e}gulo, C. and Roca Cort{\'e}s, T.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {396},
  number = {2},
  pages = {745--751},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021441},
  abstract = {A good example of finding a signal buried in noise, a common problem in Astrophysics, is the search for stellar oscillations in the acoustic power spectrum of solar-like stars. In this work it is shown that it is possible to find this type of signal in the power spectrum of stellar oscillations if the peaks are "almost" equally spaced in frequency, as the asymptotic theory for acoustic modes predicts. This signature of the power spectra of the p-mode oscillations in solar-like stars is used to design a method that allows the identification of the signal even when this signal is completely buried in noise, {$\sigma$}signal/{$\sigma$}signal+noise {$<$} 1/25.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RL7TCSL9/Régulo, Roca Cortés - 2002.pdf}
}

@article{Regulo2005,
  title = {An Observational Approach to Convection in Main Sequence Stars},
  author = {R{\'e}gulo, C. and Rami{\'o}, H. V{\'a}zquez and Cort{\'e}s, T. Roca},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {443},
  number = {3},
  pages = {1013--1019},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053620},
  abstract = {Observational results concerning possible changes in the granulation of Main Sequence stars were found by analysing their seismic power spectra obtained from photometric microvariability. We analysed as many as 178 stars with spectral types F, G, K, and M observed for 54 days. We present evidence of changes in the lifetime and contrast of the granulation, which both increase from F to M stars, although within the limit of resolution. \textcopyright{} ESO 2005.},
  keywords = {Convection,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/EMHEMJ7Z/Régulo, Ramió, Cortés - 2005.pdf}
}

@article{Regulo2005a,
  title = {Stellar P-Mode Oscillations Signal in {{Procyon}} a from {{MOST}} Data},
  author = {R{\'e}gulo, C. and Cort{\'e}s, T. R.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {444},
  number = {1},
  pages = {6--9},
  issn = {00046361},
  doi = {10.1051/0004-6361:200500192},
  abstract = {Recently, Matthews et al. (2004, Nature, 430, 51) claim a null detection of p-mode oscillations in Procyon A from 32 days of nearly continuous photometric satellite-based observations (MOST). They did not even find evidence in the Fourier amplitude spectrum of Procyon of the uniform frequency spacing signature that solar-like stars acoustic spectrum must show according to asymptotic theory. However, re-analysing his data, we have found a clear evidence of signal fully compatible with what is expected from p-mode oscillations in Procyon A. Using the method developed in R\'egulo \& Roca Cort\'es (2002, A\&A, 396, 745), that allows the analysis of stellar oscillations in the acoustic power spectrum of solar-like stars when the signal is buried in noise, we have found a frequency spacing in the power spectrum of the data of 54.5 {$\mu$}Hz, that agrees well with the expectations of the theory of stellar oscillation as well as with previous estimations from ground-based observations. Moreover, our method allows the recovery of the power spectrum of the signal from the knowledge of the frequency spacing present in the data, which yields clear peaks that can be identified as acoustic p-modes. Nonetheless, as the frequency spacing coincides with the second sub-multiple of the orbital frequency of the satellite (164.34 {$\mu$}Hz) the above findings must be taken with caution. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Stars: individual: Procyon,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VHZ74YEU/Régulo, Cortés - 2005.pdf}
}

@article{Regulo2007a,
  title = {Stellar P-Modes Oscillation Measurements in Solar-like Star Signals: {$\alpha$} {{Centauri A}} as an Example},
  author = {R{\'e}gulo, C. and Cort{\'e}s, T. Roca},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {469},
  number = {1},
  pages = {233--237},
  issn = {00046361},
  doi = {10.1051/0004-6361:20065985},
  abstract = {Context. This paper deals with the analysis of observational data series of solar-like stars. In dealing with observations of solar-like stellar oscillations from ground observatories, to achieve the necessary level of signal to noise to measure individual acoustic modes in their power spectra it is necessary to have access to large telescopes and preferably more than one used simultaneously at appropriate longitudes. It is very difficult to obtain observing time to cover more than a few day series of data, which usually implies difficulties in obtaining a precise determination of the acoustic frequencies. Aims. To find the acoustic frequencies of solar-like stars from short duration data series. Methods. The analysis technique is based on an earlier work by the authors that allows the recovery of the acoustic power spectrum of solar-like stars even in cases with poor S/N ratios. The method is applied to solar data to show how it works and also it is used to re-analyse the recently published ultra-high-precision velocity measurements in {$\alpha$} Cen A. Results. The method is shown to work well with solar observations and allows us to obtain the acoustic frequencies of solar-like stars from short-duration data series with a precision comparable with that obtained from standard methods in longer data series. Conclusions. This method can be used with currently observed data series to provide useful information on the structure of stars. \textcopyright{} ESO 2007.},
  keywords = {notion,notion-database,Stars: individual: {$\alpha$} Cen A,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/HQD36G6H/Régulo, Cortés - 2007.pdf}
}

@article{Regulo2007b,
  title = {{{TRUFAS}}, a Wavelet-Based Algorithm for the Rapid Detection of Planetary Transits},
  author = {R{\'e}gulo, C. and Almenara, J. M. and Alonso, R. and Deeg, H. and Cort{\'e}s, T. Roca},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {467},
  number = {3},
  pages = {1345--1352},
  issn = {00046361},
  doi = {10.1051/0004-6361:20066827},
  abstract = {Aims. We describe a fast, robust and automatic detection algorithm, TRUFAS, and apply it to data that are being expected from the CoRoT mission. Methods. The procedure proposed for the detection of planetary transits in light curves works in two steps: 1) a continuous wavelet transformation of the detrended light curve with posterior selection of the optimum scale for transit detection, and 2) a period search in that selected wavelet transformation. The detrending of the light curves are based on Fourier filtering or a discrete wavelet transformation. TRUFAS requires the presence of at least 3 transit events in the data. Results. The proposed algorithm is shown to identify reliably and quickly the transits that had been included in a standard set of 999 light curves that simulate CoRoT data. Variations in the pre-processing of the light curves and in the selection of the scale of the wavelet transform have only little effect on TRUFAS' results. Conclusions. TRUFAS is a robust and quick transit detection algorithm, especially well suited for the analysis of very large volumes of data from space or ground-based experiments, with long enough durations for the target-planets to produce multiple transit events. \textcopyright{} ESO 2007.},
  keywords = {Methods: data analysis,notion,notion-database,Planetary systems},
  file = {/Users/lbugnet/Zotero/storage/9PZKPNTR/Régulo et al. - 2007.pdf}
}

@article{Regulo2016,
  title = {Magnetic Activity Cycles in Solar-like Stars: {{The}} Cross-Correlation Technique of p-Mode Frequency Shifts},
  author = {R{\'e}gulo, C. and Garc{\'i}a, R. A. and Ballot, J.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {589},
  pages = {1--7},
  issn = {14320746},
  doi = {10.1051/0004-6361/201425408},
  abstract = {Aims. We set out to study the use of cross-correlation techniques to infer the frequency shifts that are induced by changing magnetic fields in p-mode frequencies and to provide a precise estimation of error bars. Methods. This technique and the calculation of the associated errors is first tested and validated on the Sun where p-mode magnetic behaviour is very well known. These validation tests are performed on 6000-day time series of Sun-as-a-star observations delivered by the SoHO spacecraft. Errors of the frequency shifts are quantified through Monte Carlo simulations. The same methodology is then applied to three solar-like oscillating stars: HD 49933, observed by CoRoT, as well as KIC 3733735 and KIC 7940546, observed by Kepler. Results. We first demonstrate the reliability of the error bars computed with the Monte Carlo simulations using the Sun. From the three stars analyzed, we confirm the presence of a magnetic activity cycle in HD 49933 with this methodology and we unveil the seismic signature of ongoing magnetic variations in KIC 3733735. Finally, the third star, KIC 7940546, seems to be in a quiet regime.},
  keywords = {asteroseismology,notion,notion-database,stars: activity,stars: oscillations,stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/UGG6YQJJ/Régulo, García, Ballot - 2016.pdf}
}

@article{Reimers1975,
  title = {Circumstellar Absorption Lines and Mass Loss from Red Giants.},
  author = {Reimers, D.},
  year = {1975},
  journal = {Memoires of the Societe Royale des Sciences de Liege},
  volume = {8},
  pages = {369},
  urldate = {2020-07-02},
  keywords = {Absorption Spectra,Astrophysics,Doppler Effect,Giant Stars,Ionization,K Lines,Line Spectra,M Stars,notion,notion-database,Spectral Line Width,Stellar Envelopes,Stellar Evolution,Stellar Mass Ejection,Stellar Spectra,Velocity Distribution}
}

@article{Reiners2006,
  title = {Rotation- and Temperature-Dependence of Stellar Latitudinal Differential Rotation},
  author = {Reiners, A.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {446},
  number = {1},
  pages = {267--277},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053911},
  abstract = {More than 600 high resolution spectra of stars with spectral type F and later were obtained in order to search for signatures of differential rotation in line profiles. In 147 stars the rotation law could be measured, with 28 of them found to be differentially rotating. Comparison to rotation laws in stars of spectral type A reveals that differential rotation sets in at the convection boundary in the HR-diagram; no star that is significantly hotter than the convection boundary exhibits the signatures of differential rotation. Four late A-/early F-type stars close to the convection boundary and at v sin i {$\approx$}100kms-1 show extraordinarily strong absolute shear at short rotation periods around one day. It is suggested that this is due to their small convection zone depth and that it is connected to a narrow range in surface velocity; the four stars are very similar in Teff and v sin i. Detection frequencies of differential rotation {$\alpha$} = {$\Delta\Omega$}/{$\Omega$} {$>$} 0 were analyzed in stars with varying temperature and rotation velocity. Measurable differential rotation is more frequent in late-type stars and slow rotators. The strength of absolute shear, {$\Delta\Omega$}, and differential rotation {$\alpha$} are examined as functions of the stellar effective temperature and rotation period. The highest values of {$\Delta\Omega$} are found at rotation periods between two and three days. In slower rotators, the strongest absolute shear at a given rotation rate {$\Delta\Omega$}max is given approximately by {$\Delta\Omega$} max {$\propto$} P-1 i-e., {$\alpha$}max {$\approx$} const. In faster rotators, both {$\alpha$}max and {$\Delta\Omega$}max diminish less rapidly. A comparison with differential rotation measurements in stars of later spectral type shows that F-stars exhibit stronger shear than cooler stars do and the upper boundary in absolute shear {$\Delta\Omega$} with temperature is consistent with the temperature-scaling law found in Doppler Imaging measurements. \textcopyright{} ESO 2006.},
  keywords = {notion,notion-database,Stars: activity,Stars: general,Stars: late-type,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/AEBM85R2/Reiners - 2006.pdf}
}

@article{Reiners2010,
  title = {A Volume-Limited Sample of 63 {{M7-M9}}.5 Dwarfs. {{II}}. {{Activity}}, Magnetism, and the Fade of the Rotation-Dominated Dynamo},
  author = {Reiners, A. and Basri, G.},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {710},
  number = {2},
  eprint = {0912.4259},
  pages = {924--935},
  issn = {15384357},
  doi = {10.1088/0004-637X/710/2/924},
  abstract = {In a volume-limited sample of 63 ultracool dwarfs of spectral type M7-M9.5, we have obtained high-resolution spectroscopy with UVES at the Very Large Telescope and HIRES at Keck Observatory. In this second paper, we present projected rotation velocities, average magnetic field strengths, and chromospheric emission from the H{$\alpha$} line. We confirm earlier results that the mean level of normalized H{$\alpha$} luminosity decreases with lower temperature, and we find that the scatter among H{$\alpha$} luminosities is larger at lower temperature. We measure average magnetic fields between 0 and 4kG with no indication for a dependence on temperature between M7 and M9.5. For a given temperature, H{$\alpha$} luminosity is related to magnetic field strength, consistent with results in earlier stars. A few very slowly rotating stars show very weak magnetic fields and H{$\alpha$} emission, and all stars rotating faster than our detection limit show magnetic fields of at least a few hundred Gauss. In contrast to earlier-type stars, we observe magnetic fields weaker than 1kG in stars rotating faster than {$\sim$}3kms-1, but we find no correlation between rotation and magnetic flux generation among them. We interpret this as a fundamental change in the dynamo mechanism; in ultracool dwarfs, magnetic field generation is predominantly achieved by a turbulent dynamo, while other mechanisms can operate more efficiently at earlier spectral types. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Brown dwarfs,notion,notion-database,Stars: low-mass,Stars: magnetic field},
  file = {/Users/lbugnet/Zotero/storage/SZDY8RL7/Reiners, Basri - 2010.pdf}
}

@article{Reiners2011,
  title = {Radius {{Dependent Angular Momentum Evolution}} in {{Low-Mass Stars}}. {{I}}},
  author = {Reiners, Ansgar and Mohanty, Subhanjoy},
  year = {2011},
  eprint = {1111.7071},
  pages = {1--34},
  doi = {10.1088/0004-637X/746/1/43},
  abstract = {Angular momentum evolution in low-mass stars is determined by initial conditions during star formation, stellar structure evolution, and the behaviour of stellar magnetic fields. Here we show that the empirical picture of angular momentum evolution arises naturally if rotation is related to magnetic field strength instead of to magnetic flux, and formulate a corrected braking law based on this. Angular momentum evolution then becomes a strong function of stellar radius, explaining the main trends observed in open clusters and field stars at a few Gyr: the steep transition in rotation at the boundary to full convection arises primarily from the large change in radius across this boundary, and does not require changes in dynamo mode or field topology. Additionally, the data suggest transient core-envelope decoupling among solar-type stars, and field saturation at longer periods in very low-mass stars. For solar-type stars, our model is also in good agreement with the empirical Skumanich law. Finally, in further support of the theory, we show that the predicted age at which low-mass stars spin down from the saturated to unsaturated field regimes in our model corresponds remarkably well to the observed lifetime of magnetic activity in these stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WXMIJUQP/Reiners, Mohanty - 2011.pdf}
}

@article{Reinhold2013,
  title = {Fast and Reliable Method for Measuring Stellar Differential Rotation from Photometric Data},
  author = {Reinhold, T. and Reiners, A.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {557},
  eprint = {1306.2176},
  pages = {1--10},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321161},
  abstract = {Context. Co-rotating spots at different latitudes on the stellar surface generate periodic photometric variability and can be useful proxies for detecting differential rotation (DR). This is a major ingredient of the solar dynamo, but observations of stellar DR are very sparse. Because the Kepler space telescope steadily collects more data, we are interested in detecting DR using photometric information of a star. Aims. The main goal of this paper is to develop a fast method for determining stellar DR from photometric data. Methods. We ran an extensive Monte Carlo simulation of differentially rotating spotted stars with very different properties to investigate the detectability of DR. For different noise levels the resulting light curves were prewhitened using Lomb-Scargle periodograms to derive parameters for a global sine fit to detect periodicities. Results. We show under which conditions DR can successfully be detected from photometric data, and in which cases the light curve provides insufficient or even misleading information on the stellar rotation law. In our simulations, the most significant period P1out is on average 2.4\% shorter than the actual spot rotation-rate. This period was detected in 96.2\% of all light curves. The signature of DR is a second period close to P1 out in our model. For the noise-free case, we found such a period in 64.2\% of all stars. Calculating the measured latitudinal shear of two distinct spots {$\alpha$}out, and comparing this with the known original spot rotation-rates shows that the real value is on average 3.2\% lower. Comparing the total equator-to-pole shear {$\alpha$} to {$\alpha$}out, we find that {$\alpha$} is underestimated by 8.8\%, especially the detection of DR for stars with {$\alpha$} {$<$} 6\% is challenging. Finally, we applied our method to four differentially rotating Kepler stars and found close agreement with results from detailed modeling. Conclusions. The method we developed is capable of measuring stellar rotation periods and detecting DR with relatively high accuracy and is suitable for large data sets. We will apply our analysis to more Kepler data in a forthcoming paper. \textcopyright{} 2013 ESO.},
  archiveprefix = {arxiv},
  keywords = {Methods: analytical,Methods: statistical,notion,notion-database,Stars: rotation,Starspots,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/ZTXFYH2U/Reinhold, Reiners - 2013.pdf}
}

@article{Reinhold2014,
  title = {Rotation \& Differential Rotation of the Active {{Kepler}} Stars},
  author = {Reinhold, Timo and Reiners, Ansgar and Basri, Gibor},
  year = {2014},
  journal = {Proceedings of the International Astronomical Union},
  volume = {9},
  number = {S302},
  pages = {216--219},
  issn = {17439221},
  doi = {10.1017/S1743921314002117},
  abstract = {Stellar rotation is a well-known quantity for tens of thousands of stars. In contrast, differential rotation (DR) is only known for a handful of stars because DR cannot be measured directly. We present rotation periods for more than 24,000 active stars in the Kepler field. Thereof, more than 18,000 stars show a second period, which we attribute to surface differential rotation. Our rotation periods are consistent with previous measurements and the theory of magnetic braking. Our results on DR paint a rather different picture: The temperature dependence of the absolute shear {$\delta$} is split into two groups separated around 6000 K. For the cooler stars {$\delta$} only slightly increases with temperature, whereas stars hotter than 6000 K show large scatter. This is the first time that DR has been measured for such a large number of stars. \textcopyright{} International Astronomical Union 2014.},
  isbn = {9781107044982},
  keywords = {activity,differential rotation,Kepler,notion,notion-database,Rotation},
  file = {/Users/lbugnet/Zotero/storage/4QPDUGZ2/Reinhold, Reiners, Basri - 2014.pdf}
}

@article{Reinhold2015,
  title = {Discriminating Solar and Antisolar Differential Rotation in High-Precision Light Curves},
  author = {Reinhold, Timo and Arlt, Rainer},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {576},
  issn = {14320746},
  doi = {10.1051/0004-6361/201425337},
  abstract = {Context. Surface differential rotation (DR) is one major ingredient of the magnetic field generation process in the Sun and likely in other stars. The term solar-like differential rotation describes the observation that solar equatorial regions rotate faster than polar ones. The opposite effect of polar regions rotating faster than equatorial ones (termed as antisolar DR) has only been observed in a few stars, although there is evidence from theoretical dynamo models. Aims. We present a new method of detecting the sign of DR (i.e., solar-like or antisolar DR) by analyzing long-term high-precision light curves with the Lomb-Scargle periodogram. Methods. We compute the Lomb-Scargle periodogram and identify a set of significant periods Pk, which we associate with active regions located at different latitudes on the stellar surface. If detectable, the first harmonics (P{${'}$}k) of these periods were identified to compute their peak-height-ratios rk:= h(P{${'}$}k)/h(Pk). Spots rotating at lower latitudes generate less sine-shaped light curves, which requires additional power in the harmonics, and results in larger ratios rk. Comparing different ratios rk and the associated periods Pk yields information about the spot latitudes, and reveals the sign of DR. Results. We tested our method on different sets of synthetic light curves all exhibiting solar-like DR. The number of cases where our method detects antisolar DR is the false-positive rate of our method. Depending on the set of light curves, the noise level, the required minimum peak separation, and the presence or absence of spot evolution, our method fails to detect the correct sign in at most 20\%. We applied our method to 50 Kepler G stars and found 21-34 stars with solar-like DR and 5-10 stars with antisolar DR, depending on the minimum peak separation. Conclusions. The method is able to determine the sign of DR in a statistical way with a low false-positive rate. Applying our method to real data might suggest that - within the uncertainties - antisolar DR was detected in 5-10 Kepler stars.},
  keywords = {notion,notion-database,Stars: rotation,Starspots},
  file = {/Users/lbugnet/Zotero/storage/7DWSAF4A/Reinhold, Arlt - 2015.pdf}
}

@article{Reinhold2015a,
  title = {Rotation, Differential Rotation, and Gyrochronology of Active {{Kepler}} Stars},
  author = {Reinhold, Timo and Gizon, Laurent},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {583},
  eprint = {1507.07757},
  pages = {1--15},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526216},
  abstract = {Context. In addition to the discovery of hundreds of exoplanets, the high-precision photometry from the CoRoT and Kepler satellites has led to measurements of surface rotation periods for tens of thousands of stars, which can potentially be used to infer stellar ages via gyrochronology. Aims. Our main goal is to derive ages of thousands of field stars using consistent rotation period measurements derived by different methods. Multiple rotation periods are interpreted as surface differential rotation (DR). We study the dependence of DR with rotation period and effective temperature. Methods. We reanalyze a previously studied sample of 24 124 Kepler stars using different approaches based on the Lomb-Scargle periodogram. Each quarter (Q1-Q14) is treated individually using a prewhitening approach. Additionally, the full time series and their different segments are analyzed. Results. For more than 18 500 stars our results are consistent with the rotation periods from McQuillan et al. (2014, ApJS, 211, 24). Of these, more than 12 300 stars show multiple significant peaks, which we interpret as DR. Dependencies of the DR with rotation period and effective temperature could be confirmed, e.g., the relative DR increases with rotation period. Gyrochronology ages between 100 Myr and 10 Gyr were derived for more than 17 000 stars using different gyrochronology relations, most of them with uncertainties dominated by period variations. We find a bimodal age distribution for Teff between 3200-4700 K. The derived ages reveal an empirical activity-age relation using photometric variability as stellar activity proxy. Additionally, we found 1079 stars with extremely stable (mostly short) periods. Half of these periods may be associated with rotation stabilized by non-eclipsing companions, the other half might be due to pulsations. Conclusions. The derived gyrochronology ages are well constrained since more than 93.0\% of the stars seem to be younger than the Sun where calibration is most reliable. Explaining the bimodality in the age distribution is challenging, and limits accurate stellar age predictions. The relation between activity and age is interesting, and requires further investigation. The existence of cool stars with almost constant rotation period over more than three years of observation might be explained by synchronization with stellar companions, or a dynamo mechanism keeping the spot configurations extremely stable.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: rotation,Starspots},
  file = {/Users/lbugnet/Zotero/storage/M227AN7S/Reinhold, Gizon - 2015.pdf}
}

@article{Reisenegger2009,
  title = {Stable Magnetic Equilibria and Their Evolution in the Upper Main Sequence, White Dwarfs, and Neutron Stars},
  author = {Reisenegger, A.},
  year = {2009},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {499},
  number = {2},
  eprint = {0809.0361},
  pages = {557--566},
  issn = {00046361},
  doi = {10.1051/0004-6361/200810895},
  urldate = {2020-07-02},
  abstract = {Context. Long-lived, large-scale magnetic field configurations exist in upper main sequence, white dwarf, and neutron stars. Externally, these fields have a strong dipolar component, while their internal structure and evolution are uncertain but highly relevant to several problems in stellar and high-energy astrophysics.Aims. We discuss the main properties expected for the stable magnetic configurations in these stars from physical arguments and the ways these properties may determine the modes of decay of these configurations. Methods. We explain and emphasize the likely importance of the non-barotropic, stable stratification of matter in all these stars (due to entropy gradients in main-sequence envelopes and white dwarfs, due to composition gradients in neutron stars). We first illustrate it in a toy model involving a single, azimuthal magnetic flux tube. We then discuss the effect of stable stratification or its absence on more general configurations, such as axisymmetric equilibria involving poloidal and toroidal field components. We argue that the main mode of decay for these configurations are processes that lift the constraints set by stable stratification, such as heat diffusion in main-sequence envelopes and white dwarfs, and beta decays or particle diffusion in neutron stars. We estimate the time scales for these processes, as well as their interplay with the cooling processes in the case of neutron stars.Results. Stable magneto-hydrostatic equilibria appear to exist in stars whenever the matter in their interior is stably stratified (not barotropic). These equilibria are not force-free and not required to satisfy the Grad-Shafranov equation, but they do involve both toroidal and poloidal field components. In main sequence stars with radiative envelopes and in white dwarfs, heat diffusion is not fast enough to make these equilibria evolve over the stellar lifetime. In neutron stars, a strong enough field might decay by overcoming the compositional stratification through beta decays (at the highest field strengths) or through ambipolar diffusion (for somewhat weaker fields). These processes convert magnetic energy to thermal energy, and they occur at significant rates only once the latter is less than the former; therefore, they substantially delay the cooling of the neutron star, while slowly decreasing its magnetic energy. \textcopyright{} 2009 ESO.},
  archiveprefix = {arxiv},
  keywords = {Magnetic fields,Magnetohydrodynamics (MHD),notion,notion-database,Stars: early-type,Stars: magnetic fields,Stars: neutron,Stars: white dwarfs},
  file = {/Users/lbugnet/Zotero/storage/SACHHB64/full-text.pdf}
}

@article{Reisman2008,
  title = {On the {{Scale}} of {{History}}},
  author = {Reisman, Susana},
  year = {2008},
  journal = {Afterimage: The Journal of Media Arts and Cultural Criticism},
  volume = {35},
  number = {4},
  pages = {37--37},
  issn = {0300-7472},
  doi = {10.1525/aft.2008.35.4.37},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MX3BRRKM/Reisman - 2008.pdf}
}

@article{Reiter2015,
  title = {A Method for the Estimation of P-Mode Parameters from Averaged Solar Oscillation Power Spectra},
  author = {Reiter, J. and Rhodes, E. J. and Kosovichev, A. G. and Schou, J. and Scherrer, P. H. and Larson, T. P.},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {803},
  number = {2},
  eprint = {1504.07493},
  pages = {1--105},
  issn = {15384357},
  doi = {10.1088/0004-637X/803/2/92},
  abstract = {A new fitting methodology is presented that is equally well suited for the estimation of low-, medium-, and high-degree mode parameters from m-averaged solar oscillation power spectra of widely differing spectral resolution. This method, which we call the "Windowed, MuLTiple-Peak, averaged-spectrum" or WMLTP Method, constructs a theoretical profile by convolving the weighted sum of the profiles of the modes appearing in the fitting box with the power spectrum of the window function of the observing run, using weights from a leakage matrix that takes into accountobservational and physical effects, such as the distortion of modes by solar latitudinal differential rotation. We demonstrate that the WMLTP Method makes substantial improvements in the inferences of the properties of the solar oscillations in comparison with a previous method, which employed a single profile to represent each spectral peak. We also present an inversion for the internal solar structure, which is based upon 6366 modes that we computed using the WMLTP method on the 66 day 2010 Solar and Heliospheric Observatory/MDI Dynamics Run. To improve both the numerical stability and reliability of the inversion, we developed a new procedure for the identification and correction of outliers in a frequency dataset. We present evidence for a pronounced departure of the sound speed in the outer half of the solar convection zone and in the subsurface shear layer from the radial sound speed profile contained in Model S of Christensen-Dalsgaard and his collaborators that existed in the rising phase of Solar Cycle 24 during mid-2010.},
  archiveprefix = {arxiv},
  keywords = {methods: data analysis,methods: numerical,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/8PA93T52/Reiter et al. - 2015.pdf}
}

@techreport{Rempel2010,
  title = {Solar Convection Zone Dynamics},
  author = {Rempel, Matthias},
  year = {2010},
  eprint = {1010.5858v1},
  urldate = {2020-05-13},
  abstract = {A comprehensive understanding of the solar magnetic cycle requires detailed modeling of the solar interior including the maintenance and variation of large scale flows (differential rotation and meridional flow), the solar dynamo and the flux emergence process connecting the magnetic field in the solar convection zone with magnetic field in the photosphere and above. Due to the vast range of time and length scales encountered, a single model of the entire convection zone is still out of reach. However, a variety of aspects can be modeled through a combined approach of 3D MHD models and simplified descriptions. We will briefly review our current theoretical understanding of these processes based on numerical models of the solar interior.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LTJ5N5LV/full-text.pdf}
}

@article{Rempel2013,
  title = {Coherent Structures and the Saturation of a Nonlinear Dynamo},
  author = {Rempel, Erico L. and Chian, Abraham C.L. and Brandenburg, Axel and Mu{\~n}oz, Pablo R. and Shadden, Shawn C.},
  year = {2013},
  month = aug,
  journal = {Journal of Fluid Mechanics},
  volume = {729},
  number = {1},
  eprint = {1210.6637},
  pages = {309--329},
  issn = {00221120},
  doi = {10.1017/jfm.2013.290},
  urldate = {2020-05-14},
  abstract = {Eulerian and Lagrangian tools are used to detect coherent structures in the velocity and magnetic fields of a mean-field dynamo, produced by direct numerical simulations of the three-dimensional compressible magnetohydrodynamic equations with an isotropic helical forcing and moderate Reynolds number. Two distinct stages of the dynamo are studied: the kinematic stage, where a seed magnetic field undergoes exponential growth; and the saturated regime. It is shown that the Lagrangian analysis detects structures with greater detail, in addition to providing information on the chaotic mixing properties of the flow and the magnetic fields. The traditional way of detecting Lagrangian coherent structures using finite-time Lyapunov exponents is compared with a recently developed method called function M. The latter is shown to produce clearer pictures which readily permit the identification of hyperbolic regions in the magnetic field, where chaotic transport/dispersion of magnetic field lines is highly enhanced. \textcopyright{} 2013 Cambridge University Press.},
  archiveprefix = {arxiv},
  keywords = {Chaotic advection,Dynamo theory,MHD turbulence,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8K2VTUXS/full-text.pdf}
}

@article{Reville2015,
  title = {{{FROM SOLAR TO STELLAR CORONA}}: {{THE ROLE OF WIND}}, {{ROTATION}}, {{AND MAGNETISM}}},
  author = {R{\'e}ville, Victor and Brun, Allan Sacha and Strugarek, Antoine and Matt, Sean P and Bouvier, J{\'e}r{\^o}me and Folsom, Colin P and Petit, Pascal},
  year = {2015},
  journal = {The Astrophysical Journal},
  volume = {814},
  number = {2},
  pages = {99},
  doi = {10.1088/0004-637X/814/2/99},
  urldate = {2020-07-02},
  abstract = {Observations of surface magnetic fields are now within reach for many stellar types thanks to the development of Zeeman-Doppler Imaging. These observations are extremely useful for constraining rotational evolution models of stars, as well as for characterizing the generation of the magnetic field. We recently demonstrated that the impact of coronal magnetic field topology on the rotational braking of a star can be parameterized with a scalar parameter: the open magnetic flux. However, without running costly numerical simulations of the stellar wind, reconstructing the coronal structure of the large-scale magnetic field is not trivial. An alternative-broadly used in solar physics-is to extrapolate the surface magnetic field assuming a potential field in the corona, to describe the opening of the field lines by the magnetized wind. This technique relies on the definition of a so-called source surface radius, which is often fixed to the canonical value of R 2.5.  However this value likely varies from star to star. To resolve this issue, we use our extended set of 2.5D wind simulations published in 2015 to provide a criterion for the opening of field lines as well as a simple tool to assess the source surface radius and the open magnetic flux. This allows us to derive the magnetic torque applied to the star by the wind from any spectropolarimetric observation. We conclude by discussing some estimations of spin-down timescales made using our technique and compare them to observational requirements.},
  keywords = {MHD,notion,notion-database,outflows,stars: coronae,stars: magnetic field,stars: rotation,stars: winds,Sun: corona},
  file = {/Users/lbugnet/Zotero/storage/ECHPK25M/full-text.pdf}
}

@article{Ribas2009,
  title = {The {{Sun}} and Stars as the Primary Energy Input in Planetary Atmospheres},
  author = {Ribas, Ignasi},
  year = {2009},
  journal = {Proceedings of the International Astronomical Union},
  volume = {5},
  number = {S264},
  eprint = {0911.4872},
  pages = {3--18},
  issn = {1743-9213},
  doi = {10.1017/s1743921309992298},
  abstract = {Proper characterization of the host star to a planet is a key element to the understanding of its overall properties. The star has a direct impact through the modification of the structure and evolution of the planet atmosphere by being the overwhelmingly larger source of energy. The star plays a central role in shaping the structure, evolution, and even determining the mere existence of planetary atmospheres. The vast majority of the stellar flux is well understood thanks to the impressive progress made in the modeling of stellar atmospheres. At short wavelengths (X-rays to UV), however, the information is scarcer since the stellar emission does not originate in the photosphere but in the chromospheric and coronal regions, which are much less understood. The same can be said about particle emissions, with a strong impact on planetary atmospheres, because a detailed description of the time-evolution of stellar wind is still lacking. Here we review our current understanding of the flux and particle emissions of the Sun and low-mass stars and briefly address their impact in the context of planetary atmospheres.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/KCLQZRU3/Ribas - 2009.pdf}
}

@article{Ribas2010,
  title = {Evolution of the Solar Activity over Time and Effects on Planetary Atmospheres. {{II}}. {$K$}1 {{Ceti}}, an Analog of the Sun When Life Arose on Earth},
  author = {Ribas, I. and Porto De Mello, G. F. and Ferreira, L. D. and H{\'e}brard, E. and Selsis, F. and Catal{\'a}n, S. and Garc{\'e}s, A. and Do Nascimento, J. D. and De Medeiros, J. R.},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {714},
  number = {1},
  eprint = {1003.3561},
  pages = {384--395},
  issn = {15384357},
  doi = {10.1088/0004-637X/714/1/384},
  abstract = {The early evolution of Earth's atmosphere and the origin of life took place at a time when physical conditions at the Earth were radically different from its present state. The radiative input from the Sun was much enhanced in the high-energy spectral domain, and in order to model early planetary atmospheres in detail, a knowledge of the solar radiative input is needed. We present an investigation of the atmospheric parameters, state of evolution, and high-energy fluxes of the nearby star {$\kappa$}1 Cet, previously thought to have properties resembling those of the early Sun. Atmospheric parameters were derived from the excitation/ionization equilibrium of Fe I and Fe II, profile fitting of H{$\alpha$}, and the spectral energy distribution. The UV irradiance was derived from Far-Ultraviolet Spectroscopic Explorer and Hubble Space Telescope data, and the absolute chromospheric flux from the H{$\alpha$} line core. From careful spectral analysis and the comparison of different methods, we propose for {$\kappa$}1 Cet the following atmospheric parameters: T eff = 5665 {$\pm$} 30K (H{$\alpha$} profile and energy distribution), log g = 4.49 {$\pm$} 0.05 dex (evolutionary and spectroscopic), and [Fe/H] = +0.10 {$\pm$} 0.05 (Fe II lines). The UV radiative properties of {$\kappa$}1 Cet indicate that its flux is some 35\% lower than the current Sun's between 210 and 300nm, it matches the Sun's at 170nm, and increases to at least 2-7 times higher than the Sun's between 110 and 140nm. The use of several indicators ascribes an age to {$\kappa$}1 Cet in the interval {$\sim$}0.4-0.8Gyr and the analysis of the theoretical Hertzsprung-Russell diagram (H-R) suggests a mass {$\sim$}1.04 M{$\odot$}. This star is thus a very close analog of the Sun when life arose on Earth and Mars is thought to have lost its surface bodies of liquid water. Photochemical models indicate that the enhanced UV emission leads to a significant increase in photodissociation rates compared with those commonly assumed of the early Earth. Our results show that reliable calculations of the chemical composition of early planetary atmospheres need to account for the stronger solar photodissociating UV irradiation. \textcopyright{} 2010 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planets and satellites: atmospheres,Stars: abundances,Stars: activity,Stars: late-type,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/GLMZUNC4/Ribas et al. - 2010.pdf}
}

@article{Richardson2012,
  title = {No {{Evidence Supporting Flare-Driven High-Frequency Global Oscillations}}},
  author = {Richardson, M. and Hill, F. and Stassun, K. G.},
  year = {2012},
  journal = {Solar Physics},
  volume = {281},
  number = {1},
  pages = {21--35},
  issn = {00380938},
  doi = {10.1007/s11207-012-0057-y},
  abstract = {The underlying physics that generates the excitations in the global low-frequency ({$<$} 5. 3 mHz) solar acoustic power spectrum is a well-known process that is attributed to solar convection; however, a definitive explanation as to what causes excitations in the high-frequency regime ({$>$} 5. 3 mHz) has yet to be found. Karoff and Kjeldsen (Astrophys. J. 678, 73-76, 2008) concluded that there is a correlation between solar flares and the global high-frequency solar acoustic waves. We have used Global Oscillation Network Group (GONG) helioseismic data in an attempt to verify the Karoff and Kjeldsen (2008) results as well as compare the post-flare acoustic power spectrum to the pre-flare acoustic power spectrum for 31 solar flares. Among the 31 flares analyzed, we observe that a decrease in acoustic power after the solar flare is just as likely as an increase. Furthermore, while we do observe variations in acoustic power that are most likely associated with the usual p-modes associated with solar convection, these variations do not show any significant temporal association with flares. We find no evidence that consistently supports flare-driven high-frequency waves. \textcopyright{} 2012 Springer Science+Business Media B.V.},
  keywords = {{Flares, waves},{Helioseismology, observations},notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/8WZATTC9/Richardson, Hill, Stassun - 2012.pdf}
}

@article{Ricker2014,
  title = {Transiting {{Exoplanet Survey Satellite}} ({{TESS}})},
  author = {Ricker, George R. and Winn, Joshua N. and Vanderspek, Roland and Latham, David W. and Bakos, G{\'a}sp{\'a}r {\'A}. and Bean, Jacob L. and {Berta-Thompson}, Zachory K. and Brown, Timothy M. and Buchhave, Lars and Butler, Nathaniel R. and Butler, R. Paul and Chaplin, William J. and Charbonneau, David and {Christensen-Dalsgaard}, J{\o}rgen and Clampin, Mark and Deming, Drake and Doty, John and De Lee, Nathan and Dressing, Courtney and Dunham, E. W. and Endl, Michael and Fressin, Francois and Ge, Jian and Henning, Thomas and Holman, Matthew J. and Howard, Andrew W. and Ida, Shigeru and Jenkins, Jon and Jernigan, Garrett and Johnson, John A. and Kaltenegger, Lisa and Kawai, Nobuyuki and Kjeldsen, Hans and Laughlin, Gregory and Levine, Alan M. and Lin, Douglas and Lissauer, Jack J. and MacQueen, Phillip and Marcy, Geoffrey and McCullough, P. R. and Morton, Timothy D. and Narita, Norio and Paegert, Martin and Palle, Enric and Pepe, Francesco and Pepper, Joshua and Quirrenbach, Andreas and Rinehart, S. A. and Sasselov, Dimitar and Sato, Bun'ei and Seager, Sara and Sozzetti, Alessandro and Stassun, Keivan G. and Sullivan, Peter and Szentgyorgyi, Andrew and Torres, Guillermo and Udry, Stephane and Villasenor, Joel},
  year = {2014},
  journal = {Space Telescopes and Instrumentation 2014: Optical, Infrared, and Millimeter Wave},
  volume = {9143},
  pages = {914320},
  issn = {1996756X},
  doi = {10.1117/12.2063489},
  abstract = {TESS is a low-cost SMEX-class satellite mission. In a two-year all-sky \textbackslash nsurvey, TESS will observe more than 2,000,000 nearby stars, searching \textbackslash nfor temporary drops in brightness caused by planetary transits. \textbackslash n\textbackslash nTESS is expected to identify more than 1000 transiting exoplanet \textbackslash ncandidates, including a sample of about 100 Super Earths---small \textbackslash nrock-and-ice planets in the range 1 to 10 Earth masses---orbiting F, G, \textbackslash nK, and M dwarfs. TESS's "wide-shallow'' survey complements the \textbackslash n"narrow-deep'' CoRoT and Kepler surveys. TESS-discovered transiting \textbackslash nsystems will be nearby ({$<$} 50 pc), and typically 10-20 x brighter than \textbackslash nthose discovered by CoRoT and Kepler. Thus, the resulting TESS Transit \textbackslash nCatalog will comprise all of the best transiting systems for follow-up \textbackslash nobservations. TESS will identify Super Earths orbiting IR-bright stars, \textbackslash nwithin reach of JWST spectroscopic searches for planetary water and \textbackslash ncarbon dioxide. \textbackslash n\textbackslash nTESS is a collaborative effort led by researchers at the Massachusetts \textbackslash nInstitute of Technology, the Harvard-Smithsonian Center for \textbackslash nAstrophysics, and the NASA Ames Research Center. Additional TESS \textbackslash nscientific partners include Las Cumbres Observatory Global Telescope, \textbackslash nLowell Observatory, the NASA Goddard Space Flight Center, the Infrared \textbackslash nProcessing and Analysis Center at the California Institute of \textbackslash nTechnology, the Geneva Observatory (Switzerland), the Tokyo Institute of \textbackslash nTechnology (Japan), and Institut Sup\'erieur de \textbackslash nl'A\'eronautique et de l'Espace (France). \textbackslash n\textbackslash nTESS was funded by NASA for a Phase A study from May 2008 - June 2009, \textbackslash nbut was not selected for flight. Additional funding leading to a flight \textbackslash nopportunity is being sought. Support has also been provided by the Kavli \textbackslash nFoundation, Google, and the Smithsonian Institution. TESS could launch \textbackslash nas early as 2013-2014.},
  isbn = {9780819496119},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TB5HHJYH/Ricker et al. - 2014.pdf}
}

@techreport{Rieutord2000,
  title = {On Mesogranulation, Network Formation and Supergranulation},
  author = {Rieutord, M and Roudier, T and Malherbe, J M and Rincon, F},
  year = {2000},
  journal = {Astron. Astrophys},
  volume = {357},
  pages = {1063--1072},
  urldate = {2020-03-14},
  abstract = {We present arguments which show that in all likelihood mesogranulation is not a true scale of solar convection but the combination of the effects of both highly energetic granules , which give birth to strong positive divergences (SPDs) among which we find exploders, and averaging effects of data processing. The important role played by SPDs in horizontal velocity fields appears in the spectra of these fields where the scale {$\sim$}4 Mm is most energetic; we illustrate the effect of averaging with a one-dimensional toy model which shows how two independent non-moving (but evolving) structures can be transformed into a single moving structure when time and space resolution are degraded. The role of SPDs in the formation of the photospheric network is shown by computing the advection of floating corks by the granular flow. The coincidence of the network bright points distribution and that of the corks is remarkable. We conclude with the possibility that supergranulation is not a proper scale of convection but the result of a large-scale instability of the granular flow, which manifests itself through a correlation of the flows generated by SPDs.},
  keywords = {convection-turbulence-Sun,granulation-Sun,notion,notion-database,photosphere}
}

@article{Rieutord2010,
  title = {The {{Sun}}'s Supergranulation},
  author = {Rieutord, Michel and Rincon, Fran{\c c}ois},
  year = {2010},
  journal = {Living Reviews in Solar Physics},
  volume = {7},
  number = {1},
  eprint = {1005.5376},
  pages = {2},
  publisher = {{Max Planck Institute for Solar System Research}},
  issn = {16144961},
  doi = {10.12942/lrsp-2010-2},
  urldate = {2020-03-15},
  abstract = {The Sun's supergranulation refers to a physical pattern covering the surface of the quiet Sun with a typical horizontal scale of approximately 30,000 km and a lifetime of around 1.8 d. Its most noticeable observable signature is as a fluctuating velocity field of 360 m s-1 rms whose components are mostly horizontal. Supergranulation was discovered more than fifty years ago, however explaining why and how it originates still represents one of the main challenges of modern solar physics. A lot of work has been devoted to the subject over the years, but observational constraints, conceptual difficulties and numerical limitations have all concurred to prevent a detailed understanding of the supergranulation phenomenon so far. With the advent of 21st century supercomputing resources and the availability of unprecedented high-resolution observations of the Sun, a stage at which key progress can be made has now been reached. A unifying strategy between observations and modelling is more than ever required for this to be possible. The primary aim of this review is therefore to provide readers with a detailed interdisciplinary description of past and current research on the problem, from the most elaborate observational strategies to recent theoretical and numerical modelling efforts that have all taken up the challenge of uncovering the origins of supergranulation. Throughout the text, we attempt to pick up the most robust findings so far, but we also outline the difficulties, limitations and open questions that the community has been confronted with over the years. In the light of the current understanding of the multiscale dynamics of the quiet photosphere, we finally suggest a tentative picture of supergranulation as a dynamical feature of turbulent magnetohydrodynamic convection in an extended spatial domain, with the aim of stimulating future research and discussions. \textcopyright{} Max-Planck-Gesellschaft.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,convection,MHD,notion,notion-database,Solar and Stellar Astrophysics,supergranulation,turbulence},
  file = {/Users/lbugnet/Zotero/storage/PRT8GD8M/full-text.pdf}
}

@article{Rieutord2013,
  title = {Studying {{Stellar Rotation}} and {{Convection}}},
  author = {Rieutord, Michel and Espinosa Lara, Francisco},
  year = {2013},
  journal = {Studying Stellar Rotation and Convection},
  volume = {865},
  pages = {219--237},
  doi = {10.1007/978-3-642-33380-4},
  abstract = {Modelling isolated rotating stars at any rotation rate is a challenge for the next generation of stellar models. These models will couple dynamical aspects of rotating stars, like angular momentum and chemicals transport, with classical chemical evolution, gravitational contraction or mass-loss. Such modelling needs to be achieved in two dimensions, combining the calculation of the structure of the star, its mean flows and the time-evolution of the whole. We present here a first step in this challenging programme. It leads to the first self-consistent two-dimensional models of rotating stars in a steady state generated by the ESTER code. In these models the structure (pressure, density and temperature) and the flow fields are computed in a self-consistent way allowing the prediction of the differential rotation and the associated meridian circulation of the stars. After a presentation of the physical properties of such models and the numerical methods at work, we give the first grid of such models describing massive and intermediate-mass stars for a selection of rotation rates up to 90 \% of the breakup angular velocity.},
  isbn = {978-3-642-33379-8},
  keywords = {notion,notion-database,Physics},
  file = {/Users/lbugnet/Zotero/storage/6LN2ZZ73/Rieutord, Espinosa Lara - 2013.pdf;/Users/lbugnet/Zotero/storage/XMCSDFDJ/Rieutord, Espinosa Lara - 2013(2).pdf}
}

@article{Rieutord2017,
  title = {On the Oscillation Spectrum of a Magnetized Core in a Giant Star},
  author = {Rieutord, Michel},
  year = {2017},
  journal = {EPJWC},
  volume = {160},
  pages = {02011},
  doi = {10.1051/EPJCONF/201716002011},
  urldate = {2020-07-20},
  keywords = {notion,notion-database}
}

@article{Riley1996,
  title = {Interplanetary Observations of Solar G-Mode Oscillations?},
  author = {Riley, Pete and Sonett, C. P.},
  year = {1996},
  journal = {Geophysical Research Letters},
  volume = {23},
  number = {12},
  pages = {1541--1544},
  issn = {00948276},
  doi = {10.1029/96GL01409},
  abstract = {By applying spectral techniques to magnetic field and plasma data from Helios 1 and 2, Pioneer 1 and 2, and Voyager 1 and 2 missions, an attempt has been made to find evidence for solar g-mode oscillations in the solar wind. It is demonstrated that analysis employing simple spectral techniques is unlikely to detect such oscillations. Using the multi-taper method, however, many 'significant' lines are identified. Unfortunately, we cannot conclude that such lines are necessarily the signature of solar g-mode oscillations because (i) these lines do not appear to be stationary; (ii) there is no evidence for the predicted signatures of asymptotic g-rhodes; and (iii) the statistics of these lines do not deviate significantly from pseudo-randomly generated data. We suggest that the difference between our conclusions and previous studies lies in the criteria used to identify these lines. Copyright 1996 by the American Geophysical Union.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PWB9KKBW/Riley, Sonett - 1996.pdf}
}

@article{Rincon2018,
  title = {The {{Sun}}'s Supergranulation},
  author = {Rincon, Fran{\c c}ois and Rieutord, Michel and Eu, Omp and Rincon, F and Rieutord, M},
  year = {2018},
  journal = {Living Reviews in Solar Physics},
  volume = {15},
  pages = {6},
  doi = {10.1007/s41116-018-0013-5},
  urldate = {2020-03-15},
  abstract = {Supergranulation is a fluid-dynamical phenomenon taking place in the solar photo-sphere, primarily detected in the form of a vigorous cellular flow pattern with a typical horizontal scale of approximately 30-35 Mm, a dynamical evolution time of 24-48 h, a strong 300-400 m/s (rms) horizontal flow component and a much weaker 20-30 m/s vertical component. Supergranulation was discovered more than 60 years ago, however , explaining its physical origin and most important observational characteristics has proven extremely challenging ever since, as a result of the intrinsic multiscale, nonlinear dynamical complexity of the problem concurring with strong observational and computational limitations. Key progress on this problem is now taking place with the advent of twenty-first-century supercomputing resources and the availability of global observations of the dynamics of the solar surface with high spatial and temporal resolutions. This article provides an exhaustive review of observational, numerical and theoretical research on supergranulation, and discusses the current status of our understanding of its origin and dynamics, most importantly in terms of large-scale nonlinear thermal convection, in the light of a selection of recent findings. This article is a revised version of https://doi.org/10.12942/lrsp-2010-2. Change summary: Major revision, updated and expanded. Switched author order. About 40 new references. Change details: This new text represents a major update of our 2010 review on supergranulation. It is more readable and significantly more concise than the original publication in our view, yet (hopefully) addresses the many exciting theoretical, numerical and observational developments on the problem since 2010. All sections have been revised in a holistic way in the light of these new results. The general discussion has also been almost entirely rewritten to reflect recent evolutions in the understanding and perception of supergranulation in the broader solar dynamics context.},
  keywords = {Convection,MHD,notion,notion-database,Supergranulation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/LZTSLLIL/full-text.pdf}
}

@article{Rix2013,
  title = {The {{Milky Way}}'s Stellar Disk},
  author = {Rix, Hans-Walter and Bovy, Jo},
  year = {2013},
  month = nov,
  journal = {The Astronomy and Astrophysics Review},
  volume = {21},
  number = {1},
  eprint = {1301.3168},
  pages = {61},
  publisher = {{Springer Nature}},
  issn = {0935-4956},
  doi = {10.1007/s00159-013-0061-8},
  urldate = {2020-03-06},
  abstract = {A suite of vast stellar surveys mapping the Milky Way, culminating in the Gaia mission, is revolutionizing the empirical information about the distribution and properties of stars in the Galactic stellar disk. We review and lay out what analysis and modeling machinery needs to be in place to test mechanisms of disk galaxy evolution and to stringently constrain the Galactic gravitational potential, using such Galactic star-by-star measurements. We stress the crucial role of stellar survey selection functions in any such modeling; and we advocate the utility of viewing the Galactic stellar disk as made up from `mono-abundance populations' (MAPs), both for dynamical modeling and for constraining the Milky Way's evolutionary processes. We review recent work on the spatial and kinematical distribution of MAPs, and lay out how further study of MAPs in the Gaia era should lead to a decisively clearer picture of the Milky Way's dark matter distribution and formation history.},
  archiveprefix = {arxiv},
  keywords = {{Galaxy: Disk, dynamics and kinematics, formation a},notion,notion-database,Surveys},
  file = {/Users/lbugnet/Zotero/storage/29F9EKAH/full-text.pdf}
}

@article{Roberts1983,
  title = {The Effect of a Weak Magnetic Field on Stellar Oscillations},
  author = {Roberts, P. H. and Soward, A. M.},
  year = {1983},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {205},
  number = {4},
  pages = {1171--1189},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/205.4.1171},
  urldate = {2020-08-10},
  abstract = {We take further a recent study by Biront et al of the effect of a weak magnetic field on the pulsations of a star, in the limit in which the magnetic energy of the star is small compared with its gravitational energy. We discover that short wavelength waves of Alfv\'en type are necessarily generated in the pulsation, and that these dominate the horizontal surface motions, which nevertheless are an order of magnitude smaller than the radial motions. These waves may also provide an important source of damping of the pulsation.},
  keywords = {Astrophysics,Magnetic Effects,Magnetic Flux,Magnetohydrodynamic Waves,notion,notion-database,Pulsations:Stars,Stars:Pulsations,Stellar Gravitation,Stellar Magnetic Fields,Stellar Models,Stellar Oscillations},
  file = {/Users/lbugnet/Zotero/storage/9K4YED6H/full-text.pdf}
}

@article{Roberts2013,
  title = {Astrophysically Robust Systematics Removal Using Variational Inference: {{Application}} to the First Month of Kepler Data},
  author = {Roberts, S. and McQuillan, A. and Reece, S. and Aigrain, S.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {435},
  number = {4},
  eprint = {1308.3644},
  pages = {3639--3653},
  issn = {00358711},
  doi = {10.1093/mnras/stt1555},
  abstract = {Space-based transit search missions such as Kepler are collecting large numbers of stellar light curves of unprecedented photometric precision and time coverage. However, before this scientific goldmine can be exploited fully, the data must be cleaned of instrumental artefacts. We present a new method to correct common-mode systematics in large ensembles of very high precision light curves. It is based on a Bayesian linear basis model and uses shrinkage priors for robustness, variational inference for speed and a de-noising step based on empirical mode decomposition to prevent the introduction of spurious noise into the corrected light curves. After demonstrating the performance of our method on a synthetic data set, we apply it to the first month of Kepler data. We compare the results, which are publicly available, to the output of the Kepler pipeline's pre-search data conditioning, and show that the two generally give similar results, but the light curves corrected using our approach have lower scatter, on average, on both long and short time-scales. We finish by discussing some limitations of our method and outlining some avenues for further development. The trend-corrected data produced by our approach are publicly available. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Data analysis-techniques,Methods,notion,notion-database,Photometric},
  file = {/Users/lbugnet/Zotero/storage/HQYTUWAV/Roberts et al. - 2013.pdf}
}

@article{Robinson2005,
  title = {Simulating the Outer Layers of {{Procyon A}}: {{A}} Comparison with the {{Sun}}},
  author = {Robinson, F. J. and Demarque, P. and Guenther, D. B. and Kim, Y. C. and Chan, K. L.},
  year = {2005},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {362},
  number = {3},
  pages = {1031--1037},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2005.09376.x},
  abstract = {We compare a new 3D radiative hydrodynamical simulation of the surface layers of Procyon A to a similar 3D simulation of the surface layers of the Sun. Both simulations include realistic input physics and are performed using the same numerical techniques and computer codes. Convection in the surface layers of Procyon A is very different from the Sun. Compared with the Sun, the atmospheric structure and convective flow in Procyon A exhibit the following characteristics. (i)The highly superadiabatic transition layer (SAL) is located at a much shallower optical depth; it is in a dynamically active region and its outer region is sometimes located in the optically thin atmosphere. (ii)The outer region of the SAL moves from an optically thin region to a thick region and back again over a time of 20-30 min. This motion, which is driven by the granulation, takes place in a time approximately half the turnover time of the largest granules. (iii)The peak rms velocity in the vertical direction is much larger in Procyon A. The main reason for the radically different radiative-convective behaviour in Procyon A compared with the Sun is the role played by turbulent eddies in determining the overall flow/thermal structure. The turbulent pressure and turbulent kinetic energy can exceed 50 per cent of the local gas pressure (compared with about 10-20 per cent in the Sun). In such regions, the mixing lengthy theory is a poor approximation. The Procyon A simulation thus reveals two distinct time-scales: the autocorrelation time of the vertical velocity and the characteristic time-scale of the SAL, which is tied to granulation. Just below the surface, the autocorrelation decay time is about 5 min in Procyon A and the SAL motion time-scale is 20-30 min. In the simulations, the peak value of the superadiabaticity varies between 0.5 and 3. When the SAL penetrates the optically thin region, there are efficient radiative losses and the peak of the SAL is low. We speculate that these losses damp out the relative amplitudes in luminosity (temperature fluctuations) compared with velocity (Doppler). Although this will not affect the frequencies of the peaks in the power spectrum, it will probably lower the average amplitude of the peaks relative to the noise background. \textcopyright{} 2005 RAS.},
  keywords = {notion,notion-database,Stars: atmospheres,Stars: individual: Procyon A,Stars: Oscillations},
  file = {/Users/lbugnet/Zotero/storage/H26IYEJN/Robinson et al. - 2005.pdf}
}

@article{robitaille2013,
  title = {Astropy: {{A}} Community {{Python}} Package for Astronomy},
  shorttitle = {Astropy},
  author = {Robitaille, Thomas P. and Tollerud, Erik J. and Greenfield, Perry and Droettboom, Michael and Bray, Erik and Aldcroft, Tom and Davis, Matt and Ginsburg, Adam and {Price-Whelan}, Adrian M. and Kerzendorf, Wolfgang E. and Conley, Alexander and Crighton, Neil and Barbary, Kyle and Muna, Demitri and Ferguson, Henry and Grollier, Fr{\'e}d{\'e}ric and Parikh, Madhura M. and Nair, Prasanth H. and G{\"u}nther, Hans M. and Deil, Christoph and Woillez, Julien and Conseil, Simon and Kramer, Roban and Turner, James E. H. and Singer, Leo and Fox, Ryan and Weaver, Benjamin A. and Zabalza, Victor and Edwards, Zachary I. and Bostroem, K. Azalee and Burke, D. J. and Casey, Andrew R. and Crawford, Steven M. and Dencheva, Nadia and Ely, Justin and Jenness, Tim and Labrie, Kathleen and Lim, Pey Lian and Pierfederici, Francesco and Pontzen, Andrew and Ptak, Andy and Refsdal, Brian and Servillat, Mathieu and Streicher, Ole},
  year = {2013},
  month = oct,
  journal = {Astronomy \& Astrophysics},
  volume = {558},
  pages = {A33},
  publisher = {{EDP Sciences}},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201322068},
  urldate = {2022-07-26},
  abstract = {We present the first public version (v0.2) of the open-source and community-developed Python package, Astropy. This package provides core astronomy-related functionality to the community, including support for domain-specific file formats such as flexible image transport system (FITS) files, Virtual Observatory (VO) tables, and common ASCII table formats, unit and physical quantity conversions, physical constants specific to astronomy, celestial coordinate and time transformations, world coordinate system (WCS) support, generalized containers for representing gridded as well as tabular data, and a framework for cosmological transformations and conversions. Significant functionality is under activedevelopment, such as a model fitting framework, VO client and server tools, and aperture and point spread function (PSF) photometry tools. The core development team is actively making additions and enhancements to the current code base, and we encourage anyone interested to participate in the development of future Astropy versions.},
  copyright = {\textcopyright{} ESO, 2013},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/JGKZJVTK/Robitaille et al. - 2013 - Astropy A community Python package for astronomy.pdf;/Users/lbugnet/Zotero/storage/AJLTAWNV/aa22068-13.html}
}

@article{Rodrigues2014,
  title = {Bayesian Distances and Extinctions for Giants Observed by {{Kepler}} and {{APOGEE}}},
  author = {Rodrigues, Tha{\'i}se S. and Girardi, L{\'e}o and Miglio, Andrea and Bossini, Diego and Bovy, Jo and Epstein, Courtney and Pinsonneault, Marc H. and Stello, Dennis and Zasowski, Gail and Prieto, Carlos Allende and Chaplin, William J. and Hekker, Saskia and Johnson, Jennifer A. and M{\'e}sz{\'a}ros, Szabolcs and Mosser, Beno{\^i}t and Anders, Friedrich and Basu, Sarbani and Beers, Timothy C. and Chiappini, Cristina and {da Costa}, Luiz A.N. and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Garc{\'i}a P{\'e}rez, Ana E. and Hearty, Fred R. and Maia, Marcio A.G. and Majewski, Steven R. and Mathur, Savita and Montalb{\'a}n, Josefina and Nidever, David L. and Santiago, Basilio and Schultheis, Mathias and Serenelli, Aldo and Shetrone, Matthew},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {445},
  number = {3},
  pages = {2758--2776},
  issn = {13652966},
  doi = {10.1093/mnras/stu1907},
  abstract = {We present a first determination of distances and extinctions for individual stars in the first release of the APOKASC catalogue, built from the joint efforts of the Apache Point Observatory Galactic Evolution Experiment (APOGEE) and the Kepler Asteroseismic Science Consortium (KASC). Our method takes into account the spectroscopic constraints derived from the APOGEE Stellar Parameters and Chemical Abundances Pipeline, together with the asteroseismic parameters from KASC. These parameters are then employed to estimate intrinsic stellar properties, including absolute magnitudes, using the Bayesian tool PARAM. We then find the distance and extinction that best fit the observed photometry in Sloan Digital Sky Survey (SDSS), 2MASS, and WISE passbands. The first 1989 giants targetted by APOKASC are found at typical distances between 0.5 and 5 kpc, with individual uncertainties of just \textasciitilde 1.8 per cent. Our extinction estimates are systematically smaller than provided in the Kepler Input Catalogue and by the Schlegel et al. maps. Distances to individual stars in the NGC 6791 and NGC 6819 star clusters agree to within their credible intervals. Comparison with the APOGEE red clump and SAGA catalogues provide another useful check, exhibiting agreement with our measurements to within a few per cent. Overall, present methods seem to provide excellent distance and extinction determinations for the bulk of the APOKASC sample. Approximately one third of the stars present broad or multiple-peaked probability density functions and hence increased uncertainties. Uncertainties are expected to be reduced in future releases of the catalogue, when a larger fraction of the stars will have seismically determined evolutionary status classifications.},
  keywords = {notion,notion-database,Stars: distances,Stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/IMP87FJZ/Rodrigues et al. - 2014.pdf}
}

@article{Roettenbacher2017,
  title = {No {{Sun-like}} Dynamo on the Active Star \$\textbackslash zeta\$ {{Andromedae}} from Starspot Asymmetry},
  author = {Roettenbacher, Rachael M. and Monnier, John D. and Korhonen, Heidi and Aarnio, Alicia N. and Baron, Fabien and Che, Xiao and Harmon, Robert O. and Kovari, Zsolt and Kraus, Stefan and Schaefer, Gail H. and Torres, Guillermo and Zhao, Ming and ten Brummelaar, Theo A. and Sturmann, Judit and Sturmann, Laszlo},
  year = {2017},
  month = sep,
  journal = {Nature},
  volume = {533},
  number = {7602},
  eprint = {1709.10107},
  pages = {217--220},
  publisher = {{Nature Publishing Group}},
  doi = {10.1038/nature17444},
  urldate = {2020-07-02},
  abstract = {Sunspots are cool areas caused by strong surface magnetic fields inhibiting convection. Moreover, strong magnetic fields can alter the average atmospheric structure, degrading our ability to measure stellar masses and ages. Stars more active than the Sun have more and stronger dark spots than in the solar case, including on the rotational pole itself. Doppler imaging, which has so far produced the most detailed images of surface structures on other stars than the Sun, cannot always distinguish the hemisphere in which the starspots are located, especially in the equatorial region and if the data quality is not optimal. This leads to problems in investigating the north-south distribution of starspot active latitudes (those latitudes with more spot activity), which are crucial constraints of dynamo theory. Polar spots, inferred only from Doppler tomography, could plausibly be observational artifacts, casting some doubt on their very existence. Here we report imaging of the old, magnetically-active star \$\textbackslash zeta\$ Andromedae using long-baseline infrared interferometry. In our data, a dark polar spot is seen in each of two epochs, while lower-latitude spot structures in both hemispheres do not persist between observations revealing global starspot asymmetries. The north-south symmetry of active latitudes observed on the Sun is absent on \$\textbackslash zeta\$ And, which hosts global spot patterns that cannot be produced by solar-type dynamos.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics}
}

@misc{Roettenbacher2019,
  title = {High {{Angular Resolution Astrophysics}}: {{Resolving Stellar Surface Features}}},
  shorttitle = {High {{Angular Resolution Astrophysics}}},
  author = {Roettenbacher, Rachael M. and Norris, Ryan P. and Baron, Fabien and Carpenter, Kenneth G. and {Creech-Eakman}, Michelle J. and Gies, Douglas and Maccarone, Thomas and Monnier, John D. and Rau, Gioia and Ridgway, Stephen and Schaefer, Gail H. and ten Brummelaar, Theo},
  year = {2019},
  month = mar,
  number = {arXiv:1903.04660},
  eprint = {1903.04660},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-08-16},
  abstract = {We are now in an era where we can image details on the surfaces of stars. When resolving stellar surfaces, we see that every surface is uniquely complicated. Each imaged star provides insight into not only the stellar surface structures, but also the stellar interiors suggesting constraints on evolution and dynamo models. As more resources become operational in the coming years, imaging stellar surfaces should become commonplace for revealing the true nature of stars. Here, we discuss the main types of stars for which imaging surface features is currently useful and what improved observing techniques would provide for imaging stellar surface features.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/EDWXRBTK/Roettenbacher et al. - 2019 - High Angular Resolution Astrophysics Resolving St.pdf;/Users/lbugnet/Zotero/storage/IVWRSIFE/1903.html}
}

@misc{Roettenbacher2019a,
  title = {High {{Angular Resolution Astrophysics}}: {{Resolving Stellar Surface Features}}},
  shorttitle = {High {{Angular Resolution Astrophysics}}},
  author = {Roettenbacher, Rachael M. and Norris, Ryan P. and Baron, Fabien and Carpenter, Kenneth G. and {Creech-Eakman}, Michelle J. and Gies, Douglas and Maccarone, Thomas and Monnier, John D. and Rau, Gioia and Ridgway, Stephen and Schaefer, Gail H. and ten Brummelaar, Theo},
  year = {2019},
  month = mar,
  number = {arXiv:1903.04660},
  eprint = {1903.04660},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-08-16},
  abstract = {We are now in an era where we can image details on the surfaces of stars. When resolving stellar surfaces, we see that every surface is uniquely complicated. Each imaged star provides insight into not only the stellar surface structures, but also the stellar interiors suggesting constraints on evolution and dynamo models. As more resources become operational in the coming years, imaging stellar surfaces should become commonplace for revealing the true nature of stars. Here, we discuss the main types of stars for which imaging surface features is currently useful and what improved observing techniques would provide for imaging stellar surface features.},
  archiveprefix = {arxiv},
  langid = {english},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/HNCYLTA7/Roettenbacher et al. - 2019 - High Angular Resolution Astrophysics Resolving St.pdf}
}

@article{Rogers2005,
  title = {Gravity Waves in the {{Sun}}},
  author = {Rogers, Tamara M. and Glatzmaier, Gary A.},
  year = {2005},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {364},
  number = {4},
  pages = {1135--1146},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2005.09659.x},
  abstract = {We present numerical simulations of penetrative convection and gravity wave excitation in the Sun. Gravity waves are self-consistently generated by a convective zone overlying a radiative interior. We produce power spectra for gravity waves in the radiative region as well as estimates for the energy flux of gravity waves below the convection zone. We calculate a peak energy flux in waves below the convection zone to be three orders of magnitude smaller than previous estimates for m = 1. The simulations show that the linear dispersion relation is a good approximation only deep below the convective-radiative boundary. Both low-frequency propagating gravity waves as well as higher frequency standing modes are generated although we find that convection does not continually drive the standing g-mode frequencies. \textcopyright{} 2005 RAS.},
  keywords = {Convection,Hydrodynamics,notion,notion-database,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/RIFGRX3X/Rogers, Glatzmaier - 2005.pdf}
}

@article{Rogers2011,
  title = {On {{Limiting}} the {{Thickness}} of the {{Solar Tachocline}}},
  author = {Rogers, T. M.},
  year = {2011},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {733},
  pages = {12},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/733/1/12},
  urldate = {2023-10-11},
  abstract = {We present axisymmetric simulations of the coupled convective and radiative regions in the Sun in order to investigate the angular momentum evolution of the radiative interior. Both hydrodynamic and magnetohydrodynamic models were run. We find an initial rapid adjustment in which the differential rotation of the convection zone viscously spreads into the radiative interior, thus forming a "tachocline." In polar regions, the subsequent spread of the tachocline is halted by a counterrotating meridional circulation cell which develops in the tachocline. Near the equator such a counterrotating cell is more intermittent and the tachocline penetration depth continues to increase, albeit more slowly than previously predicted. In the magnetic models, we impose a dipolar field initially confined to the radiative interior. The behavior of the magnetic models is very similar to their non-magnetic counterparts. Despite being connected to the convection zone, very little angular momentum is transferred between the convective and radiative regions. Therefore, while it appears that a magnetic field is not necessary to stop the tachocline spread, it also does not promote such a spread if connected to the convection zone.},
  keywords = {Astrophysics - Earth and Planetary Astrophysics,Astrophysics - Solar and Stellar Astrophysics,hydrodynamics,magnetohydrodynamics: MHD,Sun: rotation},
  annotation = {ADS Bibcode: 2011ApJ...733...12R},
  file = {/Users/lbugnet/Zotero/storage/82UR2AL3/Rogers - 2011 - On Limiting the Thickness of the Solar Tachocline.pdf}
}

@article{Rogers2015,
  title = {On the {{Differential Rotation}} of {{Massive Main-sequence Stars}}},
  author = {Rogers, T. M.},
  year = {2015},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {815},
  pages = {L30},
  issn = {0004-637X},
  doi = {10.1088/2041-8205/815/2/L30},
  urldate = {2023-11-06},
  abstract = {To date, asteroseismology has provided core-to-surface differential rotation measurements in eight main-sequence stars. These stars, ranging in mass from {$\sim$}1.5-9 M{$\odot$}, show rotation profiles ranging from uniform to counter-rotation. Although they have a variety of masses, these stars all have convective cores and overlying radiative regions, conducive to angular momentum transport by internal gravity waves (IGWs). Using two-dimensional numerical simulations, we show that angular momentum transport by IGWs can explain all of these rotation profiles. We further predict that, should high mass, faster rotating stars be observed, the core-to-envelope differential rotation will be positive, but less than one.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: rotation,waves},
  annotation = {ADS Bibcode: 2015ApJ...815L..30R},
  file = {/Users/lbugnet/Zotero/storage/G5UFQ83B/Rogers - 2015 - On the Differential Rotation of Massive Main-seque.pdf}
}

@article{Romanyuk2022,
  title = {Magnetic {{Fields}} of {{Chemically Peculiar}} and {{Related Stars}}. {{VIII}}. {{Main Results}} of 2021 and {{Near-Future Prospects}}},
  author = {Romanyuk, I. I.},
  year = {2022},
  month = dec,
  journal = {Astrophysical Bulletin},
  volume = {77},
  pages = {437--445},
  doi = {10.1134/S1990341322040095},
  urldate = {2023-10-05},
  abstract = {\textemdash We present a review of the papers written in the research field of stellar magnetism in 2021. The instruments, observation, and data analysis methods, photometry, spectroscopy, and spectropolarimetry results are considered. We present new data on magnetic fields of chemically peculiar stars and other objects of various types.},
  keywords = {stars: chemically peculiar,stars: magnetic field,stars: solar-type,stars: white dwarfs},
  annotation = {ADS Bibcode: 2022AstBu..77..437R},
  file = {/Users/lbugnet/Zotero/storage/789YJCE7/Romanyuk - 2022 - Magnetic Fields of Chemically Peculiar and Related.pdf}
}

@article{Romero2022,
  title = {Discovery of 74 New Bright {{ZZ Ceti}} Stars in the First Three Years of {{TESS}}},
  author = {Romero, Alejandra D. and Kepler, S. O. and Hermes, J. J. and Amaral, Larissa Antunes and Uzundag, Murat and Bogn{\'a}r, Zs{\'o}fia and Bell, Keaton J. and VanWyngarden, Madison and Baran, Andy and Pelisoli, Ingrid and Oliveira, Gabriela da Rosa and Koester, Detlev and Klippel, T. S. and Fraga, Luciano and Bradley, Paul A. and Vu{\v c}kovi{\'c}, Maja and Heintz, Tyler M. and Reding, Joshua S. and Kaiser, B. C. and Charpinet, St{\'e}phane},
  year = {2022},
  month = apr,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {511},
  pages = {1574--1590},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac093},
  urldate = {2023-10-14},
  abstract = {We report the discovery of 74 new pulsating DA white dwarf stars, or ZZ Cetis, from the data obtained by the Transiting Exoplanet Survey Satellite mission, from Sectors 1 to 39, corresponding to the first 3 cycles. This includes objects from the Southern hemisphere (Sectors 1-13 and 27-39) and the Northern hemisphere (Sectors 14-26), observed with 120 s- and 20 s-cadence. Our sample likely includes 13 low-mass and one extremely low-mass white dwarf candidate, considering the mass determinations from fitting Gaia magnitudes and parallax. In addition, we present follow-up time series photometry from ground-based telescopes for 11 objects, which allowed us to detect a larger number of periods. For each object, we analysed the period spectra and performed an asteroseismological analysis, and we estimate the structure parameters of the sample, i.e. stellar mass, effective temperature, and hydrogen envelope mass. We estimate a mean asteroseismological mass of {$\langle$}Msis{$\rangle$} = 0.635 {$\pm$} 0.015 M{$\odot$}, excluding the candidate low or extremely low-mass objects. This value is in agreement with the mean mass using estimates from Gaia data, which is {$\langle$}Mphot{$\rangle$} = 0.631 {$\pm$} 0.040 M{$\odot$}, and with the mean mass of previously known ZZ Cetis of {$\langle$}M*{$\rangle$} = 0.644 {$\pm$} 0.034 M{$\odot$}. Our sample of 74 new bright ZZ Cetis increases the number of known ZZ Cetis by \textasciitilde 20 per cent.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: oscillations,stars: white dwarfs,surveys},
  annotation = {ADS Bibcode: 2022MNRAS.511.1574R},
  file = {/Users/lbugnet/Zotero/storage/LTFAZXP3/Romero et al. - 2022 - Discovery of 74 new bright ZZ Ceti stars in the fi.pdf}
}

@article{Romero2022a,
  title = {Discovery of 74 New Bright {{ZZ Ceti}} Stars in the First Three Years of {{TESS}}},
  author = {Romero, Alejandra D. and Kepler, S. O. and Hermes, J. J. and Amaral, Larissa Antunes and Uzundag, Murat and Bogn{\'a}r, Zs{\'o}fia and Bell, Keaton J. and VanWyngarden, Madison and Baran, Andy and Pelisoli, Ingrid and Oliveira, Gabriela da Rosa and Koester, Detlev and Klippel, T. S. and Fraga, Luciano and Bradley, Paul A. and Vu{\v c}kovi{\'c}, Maja and Heintz, Tyler M. and Reding, Joshua S. and Kaiser, B. C. and Charpinet, St{\'e}phane},
  year = {2022},
  month = apr,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {511},
  pages = {1574--1590},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac093},
  urldate = {2023-10-14},
  abstract = {We report the discovery of 74 new pulsating DA white dwarf stars, or ZZ Cetis, from the data obtained by the Transiting Exoplanet Survey Satellite mission, from Sectors 1 to 39, corresponding to the first 3 cycles. This includes objects from the Southern hemisphere (Sectors 1-13 and 27-39) and the Northern hemisphere (Sectors 14-26), observed with 120 s- and 20 s-cadence. Our sample likely includes 13 low-mass and one extremely low-mass white dwarf candidate, considering the mass determinations from fitting Gaia magnitudes and parallax. In addition, we present follow-up time series photometry from ground-based telescopes for 11 objects, which allowed us to detect a larger number of periods. For each object, we analysed the period spectra and performed an asteroseismological analysis, and we estimate the structure parameters of the sample, i.e. stellar mass, effective temperature, and hydrogen envelope mass. We estimate a mean asteroseismological mass of {$\langle$}Msis{$\rangle$} = 0.635 {$\pm$} 0.015 M{$\odot$}, excluding the candidate low or extremely low-mass objects. This value is in agreement with the mean mass using estimates from Gaia data, which is {$\langle$}Mphot{$\rangle$} = 0.631 {$\pm$} 0.040 M{$\odot$}, and with the mean mass of previously known ZZ Cetis of {$\langle$}M*{$\rangle$} = 0.644 {$\pm$} 0.034 M{$\odot$}. Our sample of 74 new bright ZZ Cetis increases the number of known ZZ Cetis by \textasciitilde 20 per cent.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: oscillations,stars: white dwarfs,surveys},
  annotation = {ADS Bibcode: 2022MNRAS.511.1574R}
}

@article{Romero2023,
  title = {Asteroseismology of {{PG}} 1541 + 651 and {{BPM}} 31594 with {{TESS}}},
  author = {Romero, Alejandra D. and {da Rosa}, Gabriela Oliveira and Kepler, S. O. and Bradley, Paul A. and Uzundag, Murat and Bell, Keaton J. and Hermes, J. J. and Lauffer, G. R.},
  year = {2023},
  month = jan,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {518},
  pages = {1448--1458},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac3113},
  urldate = {2023-10-22},
  abstract = {We present the photometric data from TESS for two known ZZ Ceti stars, PG 1541 + 651 and BPM 31594. Before TESS, both objects only had observations from short runs from ground-based facilities, with three and one period detected, respectively. The TESS data allowed the detection of multiple periodicities, 12 for PG 1541 + 651, and six for BPM 31594, which enables us to perform a detailed asteroseismological study. For both objects, we found a representative asteroseismic model with canonical stellar mass \textasciitilde 0.61M{$\odot$} and thick hydrogen envelopes, thicker than 10-5.3M*. The detection of triplets in the Fourier transform also allowed us to estimate mean rotation periods, being \textasciitilde 22 h for PG 1541 + 651 and 11.6 h for BPM 31594, which is consistent with a range of values reported for other ZZ Ceti stars.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: variables: general,surveys,white dwarfs},
  annotation = {ADS Bibcode: 2023MNRAS.518.1448R},
  file = {/Users/lbugnet/Zotero/storage/GCAH6IX5/Romero et al. - 2023 - Asteroseismology of PG 1541 + 651 and BPM 31594 wi.pdf}
}

@article{Ronan1994,
  title = {Solar {{Cycle}} Changes in the {{High Frequency Spectrum}}},
  author = {Ronan, R. S. and Cadora, K. and Labonte, B. J.},
  year = {1994},
  journal = {Solar Physics},
  volume = {150},
  pages = {389--392},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/EKWBI95G/Ronan, Cadora, Labonte - 1994.pdf}
}

@article{Ronan1994,
  title = {Intermediate Degree P-Mode Frequency Splittings near Solar Maximum},
  author = {Ronan, R. S. and Labonte, B. J.},
  year = {1994},
  journal = {Solar Physics},
  volume = {149},
  number = {1},
  pages = {1--21},
  issn = {00380938},
  doi = {10.1007/BF00645174},
  abstract = {We report on observations of global solar Ca K-line intensity oscillations taken in May 1991 from Mees Solar Observatory, Hawaii. We measure p-mode frequency splittings for modes of spherical harmonic degrees between 20 and 129 averaged over the radial order of the modes. Our measurement of the antisymmetric component of the splittings is comparable with previous measurements and thus indicates a decrease in the latitudinal differential rotation with depth into the convection zone and the upper radiative zone. We find evidence for a 1\% variation in the rotation rate of the upper convection zone roughly in phase with the solar activity cycle. Our measurement of the symmetric component of the splittings is of the same order as was reported from the previous solar maximum and is an order of magnitude larger than has been measured near solar minimum. From the degree dependence of the symmetric component of the splittings, we find evidence for an aspherical fractional sound speed perturbation located at a depth of 0.85 {$\pm$} 0.05 solar radii. This perturbation has a magnitude of {$\delta$}c/c {$\approx$} +9 \texttimes{} 10-4 at the equator relative to the poles. Additionally, there is evidence for a near-surface aspherical sound speed perturbation of smaller magnitude {$\delta$}c/c {$\approx$} +4 \texttimes{} 10-4 at the equator relative to the poles. If an intense global magnetic field were the dominant source of the observed symmetric component of the splittings, instead of latitudinal gradients in the sound speed, then global fields of order 105 G would be required in the convection zone. \textcopyright{} 1994 Kluwer Academic Publishers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/85245R9A/Ronan, Labonte - 1994.pdf}
}

@techreport{Roudier1998,
  title = {Solar Mesogranule Lifetime Measurements},
  author = {Roudier, Th and Malherbe, J M and Vigneau, J and Pfeiffer, B},
  year = {1998},
  journal = {Astron. Astrophys},
  volume = {330},
  pages = {1136--1144},
  urldate = {2020-03-14},
  abstract = {We present a study in which the solar lifetime of mesocells (4-10 arcsec) was determined from a long time sequence (6 h 40 min) obtained at the Pic du Midi Observatory. The mesocell detection was performed by local correlation tracking, using various spatial and temporal windows. The histograms derived from the visual measurements reveal that mesoscale lifetime is between 10 min and 160 min, with peaked distributions around 30-40 min. The indirect method for lifetime estimation using a correlation coefficient, gives a mesocale lifetime from 16 to 185 min depending on the temporal window and the methods used. The proper motions of the long-living mesocells are found to be random with respect to the super-ganule flows, with the peak distribution of horizontal velocities at 0.5 km/s. The results of this mesocell lifetime determination method are smaller by a factor of 2 to 5 with respect to the previous results. This difference could be attributed to the mesocell definition, the method of measurement or the different location of the mesocell field of view in the supergranular network.},
  keywords = {granulation-convection,notion,notion-database,photosphere-Sun,Sun},
  file = {/Users/lbugnet/Zotero/storage/R4L8G2RT/full-text.pdf}
}

@article{Roxburgh2003a,
  title = {The Ratio of Small to Large Separations of Acoustic Oscillations as a Diagnostic of the Interior of Solar-like Stars},
  author = {Roxburgh, I. W. and Vorontsov, S. V.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {411},
  number = {2},
  pages = {215--220},
  issn = {00046361},
  doi = {10.1051/0004-6361:20031318},
  abstract = {By considering stellar models with the same interior structure but different outer layers we demonstrate that the ratio of the small to large separations of acoustic oscillations in solar-like stars is essentially independent of the structure of the outer layers, and is determined solely by the interior structure. Defining the scaled Eulerian pressure perturbation {$\psi$}ell;({$\omega$},t),= rp{${'}$}/({$\rho$}c)1/2 we define the internal phase shift {$\delta\mathscr{l}$}({$\omega$}, t) through the relation {$\omega\psi$}/(d{$\psi$}/dt) = tan({$\omega$}t - {$\pi\mathscr{l}$}/2 + {$\delta$} {$\mathscr{l}$}). The {$\delta\mathscr{l}$} are almost independent of acoustic radius t = {$\int$} dr/c outside the stellar core and can be determined as a continuous functions of {$\omega$} from partial wave solutions for the interior - that is solutions of the oscillation equations for any {$\omega$} that satisfy the Laplace boundary condition at a sufficiently large acoustic radius tf outside the stellar core. If the {$\omega$} are eigenfrequencies then they satisfy the Eigenfrequency Equation {$\omega$}T = (n + {$\mathscr{l}$}/2){$\pi$} + {$\alpha$}({$\omega$}) - {$\delta\mathscr{l}$}({$\omega$}) where {$\alpha$}({$\omega$}) is the {$\mathscr{l}$} independent surface phase shift (Roxburgh \& Vorontsov 2000). Using this result we show that the ratio of small to large separations is determined to high accuracy solely by the internal phase shifts {$\delta$} {$\mathscr{l}$}({$\omega$}) and hence by the interior structure alone. The error in this result is estimated and shown to be smaller than that associated with the errors in the determination of the frequencies ({$\approx$}0.1-0.3 {$\mu$}Hz) from the upcoming space missions MOST, COROT and Eddington.},
  keywords = {notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/IKT3RND4/Roxburgh, Vorontsov - 2003.pdf}
}

@article{Roxburgh2006,
  title = {The Autocorrelation Function of Stellar P-Mode Measurements and Its Diagnostic Properties},
  author = {Roxburgh, I. W. and Vorontsov, S. V.},
  year = {2006},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {369},
  number = {3},
  pages = {1491--1496},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2006.10396.x},
  abstract = {The basic properties of acoustic wave propagation in stellar interiors can be analysed from the autocorrelation function (ACF) of intensity (or velocity) observations without measuring the resonant p-mode frequencies. We show how the strength of acoustic wave refraction in the stellar core, or forward acoustic amplitude, can be measured from a modulation in the ACF. This is the basic physical quantity which governs the so-called 'small frequency separations', and its measurement from the ACF can be used for determining the small frequency separations when the data is of insufficient quality for a reliable identification of the stellar p-mode frequencies. \textcopyright{} 2006 RAS.},
  keywords = {Methods: numerical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/AFGJJZD5/Roxburgh, Vorontsov - 2006.pdf}
}

@article{Roxburgh2007,
  title = {Acoustic Wave Reflection by Stellar Cores: {{Can}} It Be Seen in the Autocorrelation Function of p-Mode Measurements?},
  author = {Roxburgh, I. W. and Vorontsov, S. V.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {379},
  number = {2},
  pages = {801--806},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.11979.x},
  abstract = {The rapid variation of density with depth in a stellar core can distort acoustic wave propagation in stellar interiors, producing a reflected wave. The reflectivity can come from a rapid density change at the boundary of a convective core, or from the steep gradients established in a radiative core during chemical evolution. We analyse this wave reflection within the framework of wave scattering theory, and address the question of the detectability of the reflected wave in the autocorrelation function of stellar p-mode measurements. \textcopyright{} 2007 RAS.},
  keywords = {Methods: numerical,notion,notion-database,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/39QF2AXX/Roxburgh, Vorontsov - 2007.pdf}
}

@article{Roxburgh2009,
  title = {Small Separations and Phase Shift Differences of L=0, 1 p-Modes},
  author = {Roxburgh, I. W.},
  year = {2009},
  journal = {Astronomy and Astrophysics},
  volume = {493},
  number = {1},
  pages = {185--191},
  issn = {00046361},
  doi = {10.1051/0004-6361:200811047},
  abstract = {Aims. We investigate the diagnostic potential of l = 0,1 p-modes and the origin of the periodicity in their small separations. Methods. We used theoretical analysis, phase-shifts, modelling. and data analysis.Results. The periodicity in the small separations between modes of l = 0, 1 is determined by the acoustic radius of the base of the outer convective envelope. The mean variation is determined primarily by the structure of the inner core. The separations are related to the inner phase shifts differences l which we show can be determined directly from the frequencies. The modulation period is shifted slightly by the frequency dependence of the phase shifts and the amplitudes. We present results using data from the BiSON, IRIS, and GOLF experiments, and a solar model, all of which give a modulation period of \textasciitilde 359l5 lHz corresponding to an acoustic radius \textasciitilde 1422l20 s.. \textcopyright{} 2008 ESO.},
  keywords = {notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/MZ2LSK7M/Roxburgh - 2009.pdf}
}

@article{Roxburgh2015,
  title = {Scaled Models, Scaled Frequencies, and Model Fitting},
  author = {Roxburgh, Ian W.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {584},
  pages = {2--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527447},
  abstract = {I show that given a model star of mass M, radius R, and density profile {$\rho$}(x) [x = r/R], there exists a two parameter family of models with masses Mk, radii Rk, density profile {$\rho$}k(x) = {$\lambda\rho$}(x) and frequencies {$\nu$}kn{$\mathscr{l}$} = {$\lambda$}1/2{$\nu$}n{$\mathscr{l}$}, where {$\lambda$},Rk/RA are scaling factors. These models have different internal structures, but all have the same value of separation ratios calculated at given radial orders n, and all exactly satisfy a frequency matching algorithm with an offset function determined as part of the fitting procedure. But they do not satisfy ratio matching at given frequencies nor phase shift matching. This illustrates that erroneous results may be obtained when model fitting with ratios at given n values or frequency matching. I give examples from scaled models and from non scaled evolutionary models.},
  keywords = {Asteroseismology,Methods: analytical,Methods: numerical,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TL5UCCQR/Roxburgh - 2015.pdf}
}

@article{Rudiger1997,
  title = {The Slender Solar Tachocline: {{A}} Magnetic Model},
  author = {R{\"u}diger, G. and Kitchatinov, L. L.},
  year = {1997},
  journal = {Astronomische Nachrichten},
  volume = {318},
  number = {5},
  pages = {273--279},
  publisher = {{Wiley-VCH Verlag}},
  issn = {00046337},
  doi = {10.1002/asna.2113180504},
  urldate = {2020-06-19},
  abstract = {A model for the sharp transition from differential rotation in the solar convection zone to rigid rotation in the radiative interior is presented. Differential rotation in the radiative zone is shown to be quenched efficiently by an internal magnetic field. The poloidal field amplitude, B0, is the input parameter for our model which determines the transition layer thickness and the toroidal field strength. It is illustrated analytically and confirmed numerically that a rather small field, B0 = 10-4 Gauss, suffices to satisfy the helioseismological restrictions on the depth of the differential rotation penetration below the convection zone. The transition layer thickness decreases further with increasing B0. The toroidal field amplitude B {$\simeq$} 200 Gauss is almost independent of B0.},
  keywords = {Diffusion,MHD,notion,notion-database,Turbulence}
}

@article{Rudiger2007,
  title = {Structure and Stability of the Magnetic Solar Tachocline},
  author = {R{\"u}diger, G. and Kitchatinov, L. L.},
  year = {2007},
  month = aug,
  journal = {New Journal of Physics},
  volume = {9},
  pages = {302},
  issn = {1367-2630},
  doi = {10.1088/1367-2630/9/8/302},
  urldate = {2023-10-18},
  abstract = {Rather weak fossil magnetic fields in the radiative core can produce the solar tachocline if the field is almost horizontal in the tachocline region, i.e. if the field is confined within the core. This particular field geometry is shown to result from a shallow (\{\textbackslash lesssim\} 1\textbackslash,Mm) penetration of the meridional flow existing in the convection zone into the radiative core. Two conditions are thus crucial for a magnetic tachocline theory: (i) the presence of meridional flow of a few metres per second at the base of the convection zone, and (ii) a magnetic diffusivity inside the tachocline smaller than 108 cm2 s-1. Numerical solutions for the confined poloidal fields and the resulting tachocline structures are presented. We find that the tachocline thickness runs as Bp-1/2 with the poloidal field amplitude falling below 5\% of the solar radius for Bp {$>$} 5 mG. The resulting toroidal field amplitude inside the tachocline of about 100 G does not depend on the Bp. The hydromagnetic stability of the tachocline is only briefly discussed. For the hydrodynamic stability of latitudinal differential rotation we found that the critical 29\% of the 2D theory of Watson (1981 Geophys. Astrophys. Fluid Dyn. 16 285) are reduced to only 21\% in 3D for marginal modes of about 6 Mm radial scale.},
  keywords = {Astrophysics},
  annotation = {ADS Bibcode: 2007NJPh....9..302R},
  file = {/Users/lbugnet/Zotero/storage/LYF7ETQQ/Rüdiger and Kitchatinov - 2007 - Structure and stability of the magnetic solar tach.pdf}
}

@article{Rudiger2012,
  title = {Helicity and Dynamo Action in Magnetized Stellar Radiation Zones},
  author = {R{\"u}diger, G. and Kitchatinov, L. L. and Elstner, D.},
  year = {2012},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {425},
  number = {3},
  pages = {2267--2276},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2012.21569.x},
  urldate = {2020-07-13},
  abstract = {The helicity and {$\alpha$} effect driven by the non-axisymmetric Tayler instability of toroidal magnetic fields in stellar radiation zones are computed. In the linear approximation, a purely toroidal field always excites pairs of modes with identical growth rates but with opposite helicity so that the net helicity vanishes. If the magnetic background field has a helical structure by an extra (weak) poloidal component then one of the modes dominates, producing a net kinetic helicity anticorrelated with the current helicity of the background field. The mean electromotive force is computed with the result that the {$\alpha$} effect by the most rapidly growing mode has the same sign as the current helicity of the background field. The {$\alpha$} effect is found to be too small to drive an {$\alpha$} 2 dynamo, but the excitation conditions for an {$\alpha\Omega$} dynamo can be fulfilled for weak poloidal fields. Moreover, if the dynamo produces its own {$\alpha$} effect by the magnetic instability, then problems with its sign do not arise. For all cases, however, the {$\alpha$} effect shows an extremely strong concentration to the poles so that a possible {$\alpha\Omega$} dynamo might only work at the polar regions. Hence, the results of our linear theory lead to a new topological problem for the existence of large-scale dynamos in stellar radiation zones on the basis of the current-driven instability of toroidal fields. \textcopyright{} 2012 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2012 RAS.},
  keywords = {Instabilities,Interiors,Magnetic field,MHD,notion,notion-database,Stars},
  file = {/Users/lbugnet/Zotero/storage/E3M8YLAE/full-text.pdf}
}

@article{Rudiger2016,
  title = {Instability of Magnetized and Differentially Rotating Stellar Radiation Zones with High Magnetic {{Mach}} Number},
  author = {R{\"u}diger, G. and Schultz, M. and Kitchatinov, L. L.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {456},
  number = {3},
  pages = {3004--3010},
  issn = {13652966},
  doi = {10.1093/mnras/stv2838},
  abstract = {With applications to inner solar-type radiative zones, a linear theory is used to analyse the instability of a toroidal background field of dipolar parity, in the presence of density stratification, differential rotation and realistically small Prandtl numbers. The physical parameters are the Alfv\'en frequency {$\Omega$}A, the global rotation rate {$\Omega$} and the buoyancy frequency N with {$\Omega$}A {$<$} {$\Omega$}},
  keywords = {Instabilities,MHD,notion,notion-database,Stars: interiors,Stars: magnetic field,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/YJJQD595/Rüdiger, Schultz, Kitchatinov - 2016.pdf}
}

@misc{Rui2023,
  title = {Gravity Waves in Strong Magnetic Fields},
  author = {Rui, Nicholas Z. and Fuller, Jim},
  year = {2023},
  month = mar,
  number = {arXiv:2303.08147},
  eprint = {2303.08147},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-05-09},
  abstract = {Strong magnetic fields in the cores of stars are expected to significantly modify the behavior of gravity waves, which is likely the origin of suppressed dipole modes observed in many red giants. However, a detailed understanding of how such fields alter the spectrum and spatial structure of magnetogravity waves has been elusive. For a dipole field, we analytically characterize the horizontal eigenfunctions of magnetogravity modes, assuming that the wavevector is primarily radial. For axisymmetric modes (\$m=0\$), the magnetogravity wave eigenfunctions become Hough functions, and they have a radial turning point for sufficiently strong magnetic fields. For non-axisymmetric modes (\$m\textbackslash neq0\$), the interaction between the discrete \$g\$ mode spectrum and a continuum of Alfv\textbackslash 'en waves produces nearly discontinuous features in the fluid displacements at critical latitudes associated with a singularity in the fluid equations. We find that magnetogravity modes cannot propagate in regions with sufficiently strong magnetic fields, instead becoming evanescent. When encountering strong magnetic fields, ingoing gravity waves are likely refracted into outgoing slow magnetic waves. These outgoing waves approach infinite radial wavenumbers, which are likely to be damped efficiently. However, it may be possible for a small fraction of the wave power to escape the stellar core as pure Alfv\textbackslash 'en waves or magnetogravity waves confined to a very narrow equatorial band. The artificially sharp features in the WKB-separated solutions suggest the need for global mode solutions which include small terms neglected in our analysis.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/CCCQ5S62/Rui and Fuller - 2023 - Gravity waves in strong magnetic fields.pdf;/Users/lbugnet/Zotero/storage/HEDK5U6I/2303.html}
}

@misc{Rui2023a,
  title = {Asteroseismic G-Mode Period Spacings in Strongly Magnetic Rotating Stars},
  author = {Rui, Nicholas Z. and Ong, J. M. Joel and Mathis, St{\'e}phane},
  year = {2023},
  month = oct,
  journal = {arXiv e-prints},
  doi = {10.48550/arXiv.2310.19873},
  urldate = {2023-11-03},
  abstract = {Strong magnetic fields are expected to significantly modify the pulsation frequencies of waves propagating in the cores of red giants or in the radiative envelopes of intermediate- and high-mass main-sequence stars. We calculate the g-mode frequencies of stars with magnetic dipole fields which are aligned with their rotational axes, treating both the Lorentz and Coriolis forces non-perturbatively. We provide a compact asymptotic formula for the g-mode period spacing, and universally find that strong magnetism decreases this period spacing substantially more than is predicted by perturbation theory. These results are validated with explicit numerical mode calculations for realistic stellar models. The approach we present is highly versatile: once the eigenvalues \$\textbackslash lambda\$ of a certain differential operator are precomputed as a function of the magnetogravity and rotational frequencies (in units of the mode frequency), the non-perturbative impact of the Coriolis and Lorentz forces is understood under a broad domain of validity, and is readily incorporated into asteroseismic modeling.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  annotation = {ADS Bibcode: 2023arXiv231019873R},
  file = {/Users/lbugnet/Zotero/storage/24NW2MAW/Rui et al. - 2023 - Asteroseismic g-mode period spacings in strongly m.pdf}
}

@article{Saar1999,
  title = {Time Evolution of the Magnetic Activity Cycle Period. Ii. Results for an Expanded Stellar Sample s Teven h. s Aar},
  author = {Saar, Steven H},
  year = {1999},
  volume = {10},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZJYZ2IUX/Saar - 1999.pdf}
}

@article{Saar2002,
  title = {A New Look at Dynamo Cycle Amplitudes},
  author = {Saar, S. H. and Brandenburg, A.},
  year = {2002},
  journal = {Astronomische Nachrichten},
  volume = {323},
  number = {3-4},
  eprint = {astro-ph/0207392},
  pages = {357--360},
  issn = {00046337},
  doi = {10.1002/1521-3994(200208)323:3/4<357::AID-ASNA357>3.0.CO;2-I},
  abstract = {We explore the dependence of the amplitude of stellar dynamo cycle variability (as seen in the Mount Wilson Ca II HK timeseries data) on other stellar parameters. We find that the fractional cycle amplitude Acyc (i.e. the ratio of the peak-to-peak variation to the average) decreases somewhat with mean activity, increases with decreasing effective temperature, but is not correlated with inverse Rossby number Ro-1. We find that Acyc increases with the ratio of cycle and rotational frequencies {$\omega$}cyc/{$\Omega$} along two, nearly parallel branches.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: chromospheres,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/3VGJRXIV/Saar, Brandenburg - 2002.pdf}
}

@article{Sachkov2014,
  title = {Study of Pulsations of Chemically Peculiar a Stars},
  author = {Sachkov, M. E.},
  year = {2014},
  journal = {Astrophysical Bulletin},
  volume = {69},
  number = {1},
  pages = {40--45},
  issn = {19903413},
  doi = {10.1134/S1990341314010040},
  urldate = {2020-04-13},
  abstract = {Rapidly oscillating chemically peculiar A stars (roAp) pulsate in high-overtone, low degree p-modes and form a sub-group of chemically peculiar magnetic A stars (Ap). Until recently, the classical asteroseismic research, i.e., frequency analysis, of these stars was based on photometric observations both ground-based and space-based. Significant progress has been achieved by obtaining uninterrupted, ultra-high precision data from the MOST, COROT, and Kepler satellites. Over the last ten years, a real breakthrough was achieved in the study of roAp stars due to the time-resolved, high spectral resolution spectroscopic observations. Unusual pulsational characteristics of these stars, caused by the interaction between propagating pulsationwaves and strong stratification of chemical elements, provide an opportunity to study the upper roAp star atmosphere in more detail than is possible for any star but the Sun, using spectroscopic data. In this paper the results of recent pulsation studies of these stars are reviewed. \textcopyright{} 2014 Pleiades Publishing, Ltd.},
  keywords = {notion,notion-database,stars: chemically peculiar,stars: oscillations}
}

@techreport{SachkovM2014,
  title = {Observational Studies of {{roAp}} Stars},
  author = {{Sachkov M}},
  year = {2014},
  journal = {psce},
  pages = {315--322},
  urldate = {2020-03-27},
  abstract = {Rapidly oscillating Ap (roAp) stars are high-overtone, low-degree p-mode pulsators that are also chemically peculiar magnetic A stars. Until recently the classical asteroseismic analysis i.e. frequency analysis, of these stars was based on ground and space photometric observations. Significant progress was achieved through access to uninterrupted, ultra-high-precision data from MOST, COROT and Kepler satellites. Over the last ten years the study of roAp stars has been altered drastically from an observational point of view through studies of time-resolved, high-resolution spectra. Their unusual pulsational characteristics, caused by an interplay between the short vertical lengths of the pulsation waves and strong stratification of chemical elements, allow us to examine the upper roAp atmosphere in more detail than is possible for any star except the Sun. In this paper I review the results of recent studies of the pulsations of roAp stars.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BITQMAYJ/full-text.pdf}
}

@article{Saio2005,
  title = {A Non-Adiabatic Analysis for Axisymmetric Pulsations of Magnetic Stars},
  author = {Saio, Hideyuki},
  year = {2005},
  month = jul,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {360},
  pages = {1022--1032},
  issn = {0035-8711},
  doi = {10.1111/j.1365-2966.2005.09091.x},
  urldate = {2023-10-17},
  abstract = {This paper presents the results of a non-adiabatic analysis for axisymmetric non-radial pulsations including the effect of a dipole magnetic field. Convection is assumed to be suppressed in the stellar envelope, and the diffusion approximation is used to radiative transport. As in a previous adiabatic analysis, the eigenfunctions are expanded in a series of spherical harmonics. The analysis is applied to a 1.9-Msolar, main-sequence model (logTeff= 3.913). The presence of a magnetic field always stabilizes low-order acoustic modes. All the low-order modes of the model that are excited by the {$\kappa$}-mechanism in the HeII ionization zone in the absence of a magnetic field are found to be stabilized if the polar strength of the dipole magnetic field is larger than about 1 kG. For high-order p modes, on the other hand, distorted dipole and quadrupole modes excited by the {$\kappa$}-mechanism in the H ionization zone remain overstable, even in the presence of a strong magnetic field. It is found, however, that all the distorted radial high-order modes are stabilized by the effect of the magnetic field. Thus, our non-adiabatic analysis suggests that distorted dipole modes and distorted quadrupole modes are most likely excited in rapidly oscillating Ap stars. The latitudinal amplitude dependence is found to be in reasonable agreement with the observationally determined one for HR 3831. Finally, the expected amplitude of magnetic perturbations at the surface is found to be very small.},
  keywords = {stars: chemically peculiar,stars: magnetic fields,stars: oscillations,stars: variables: other},
  annotation = {ADS Bibcode: 2005MNRAS.360.1022S},
  file = {/Users/lbugnet/Zotero/storage/IFI65IHX/Saio - 2005 - A non-adiabatic analysis for axisymmetric pulsatio.pdf}
}

@article{Saio2015,
  title = {Asteroseismic Measurement of Slow, Nearly Uniform Surface-to-Core Rotation in the Main-Sequence {{F}} Star {{KIC}} 9244992},
  author = {Saio, Hideyuki and Kurtz, Donald W. and Takata, Masao and Shibahashi, Hiromoto and Murphy, Simon J. and Sekii, Takashi and Bedding, Timothy R.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {447},
  number = {4},
  pages = {3264--3277},
  issn = {13652966},
  doi = {10.1093/mnras/stu2696},
  abstract = {We have found a rotationally split series of core g-mode triplets and surface p-mode multiplets in a main-sequence F star, KIC 9244992. Comparison with models shows that the star has a mass of about 1.45 M{$\odot$}, and is at an advanced stage of main-sequence evolution in which the central hydrogen abundance mass fraction is reduced to about 0.1. This is the second case, following KIC 11145123, of an asteroseismic determination of the rotation of the deep core and surface of an A-F main-sequence star. We have found, essentially model independently, that the rotation near the surface, obtained from p-mode splittings, is 66 d, slightly slower than the rotation of 64 d in the core, measured by g-mode splittings. KIC 9244992 is similar to KIC 11145123 in that both are near the end of main-sequence stage with very slow and nearly uniform rotation. This indicates the angular momentum transport in the interior of an A-F star during the main-sequence stage is much stronger than that expected from standard theoretical formulations.},
  keywords = {Asteroseismology,notion,notion-database,Stars: individual: KIC 9244992,Stars: interiors,Stars: oscillations,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/X54WFXQR/Saio et al. - 2015.pdf}
}

@article{Saio2021,
  title = {Rotation of the Convective Core in \$\textbackslash gamma\$ {{Dor}} Stars Measured by Dips in Period Spacings of g Modes Coupled with Inertial Modes},
  author = {Saio, Hideyuki and Takata, Masao and Lee, Umin and Li, Gang and Van Reeth, Timothy},
  year = {2021},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {502},
  number = {4},
  eprint = {2102.08548},
  primaryclass = {astro-ph},
  pages = {5856--5874},
  issn = {0035-8711, 1365-2966},
  doi = {10.1093/mnras/stab482},
  urldate = {2023-10-17},
  abstract = {The relation of period spacing (\$\textbackslash Delta P\$) versus period (\$P\$) of dipole prograde g modes is known to be useful to measure rotation rates in the g-mode cavity of rapidly rotating \$\textbackslash gamma\$ Dor and slowly pulsating B (SPB) stars. In a rapidly rotating star, an inertial mode in the convective core can resonantly couple with g modes propagative in the surrounding radiative region. The resonant coupling causes a dip in the \$P\$-\$\textbackslash Delta P\$ relation, distinct from the modulations due to the chemical composition gradient. Such a resonance dip in \$\textbackslash Delta P\$ of prograde dipole g modes appears around a frequency corresponding to a spin parameter \$2f\_\{\textbackslash rm rot\}\{\textbackslash rm(cc)\}/\textbackslash nu\_\{\textbackslash rm co-rot\} \textbackslash sim 8-11\$ with \$f\_\{\textbackslash rm rot\}\$(cc) being the rotation frequency of the convective core and \$\textbackslash nu\_\{\textbackslash rm co-rot\}\$ the pulsation frequency in the co-rotating frame. The spin parameter at the resonance depends somewhat on the extent of core overshooting, central hydrogen abundance, and other stellar parameters. We can fit the period at the observed dip with the prediction from prograde dipole g modes of a main-sequence model, allowing the convective core to rotate differentially from the surrounding g-mode cavity. We have performed such fittings for 16 selected \$\textbackslash gamma\$ Dor stars having well defined dips, and found that the majority of \$\textbackslash gamma\$ Dor stars we studied rotate nearly uniformly, while convective cores tend to rotate slightly faster than the g-mode cavity in less evolved stars.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/ABALHHJM/Saio et al. - 2021 - Rotation of the convective core in $gamma$ Dor st.pdf;/Users/lbugnet/Zotero/storage/S64R3JA4/2102.html}
}

@article{saioRotationConvectiveCore2021,
  title = {Rotation of the Convective Core in {$\gamma$} {{Dor}} Stars Measured by Dips in Period Spacings of g Modes Coupled with Inertial Modes},
  author = {Saio, Hideyuki and Takata, Masao and Lee, Umin and Li, Gang and Van Reeth, Timothy},
  year = {2021},
  month = feb,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {000},
  pages = {1--15},
  issn = {0035-8711},
  doi = {10.1093/mnras/stab482},
  urldate = {2021-03-02},
  abstract = {{$<$}p{$>$}The relation of period spacing ({$\Delta$}P) versus period (P) of dipole prograde g modes is known to be useful to measure rotation rates in the g-mode cavity of rapidly rotating {$\gamma$} Dor and slowly pulsating B (SPB) stars. In a rapidly rotating star, an inertial mode in the convective core can resonantly couple with g modes propagative in the surrounding radiative region. The resonant coupling causes a dip in the P~-~{$\Delta$}P relation, distinct from the modulations due to the chemical composition gradient. Such a resonance dip in {$\Delta$}P of prograde dipole g modes appears around a frequency corresponding to a spin parameter 2frot(cc)/{$\nu$}co-rot {$\sim$} 8 - 11 with frot(cc) being the rotation frequency of the convective core and {$\nu$}co-rot the pulsation frequency in the co-rotating frame. The spin parameter at the resonance depends somewhat on the extent of core overshooting, central hydrogen abundance, and other stellar parameters. We can fit the period at the observed dip with the prediction from prograde dipole g modes of a main-sequence model, allowing the convective core to rotate differentially from the surrounding g-mode cavity. We have performed such fittings for 16 selected {$\gamma$} Dor stars having well defined dips, and found that the majority of {$\gamma$} Dor stars we studied rotate nearly uniformly, while convective cores tend to rotate slightly faster than the g-mode cavity in less evolved stars.{$<$}/p{$>$}},
  keywords = {asteroseismology-stars,general,interiors-stars,notion,notion-database,oscillations-stars,rotation-stars,variables},
  file = {/Users/lbugnet/Zotero/storage/GZL6D73N/full-text.pdf}
}

@article{Salabert2004,
  title = {Solar p Modes in 10 Years of the {{IRIS}} Network},
  author = {Salabert, D. and Fossat, E. and Gelly, B. and Kholikov, S. and Grec, G. and Lazrek, M. and Schmider, F. X.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {413},
  number = {3},
  pages = {1135--1142},
  issn = {00046361},
  doi = {10.1051/0004-6361:20031541},
  abstract = {IRIS data (the low degree l {$\leq$} 3 helioseismology network) have been analysed for the study of p-mode parameters variability over the falling phase of the solar activity cycle 22 and the rising phase of the solar activity cycle 23. The IRIS duty cycle has been improved by the so-called "repetitive music method", a method of partial gap filling. We present in this paper an analysis of the dependence of p-mode frequencies and linewidths with frequency and with solar magnetic activity. We confirm also the periodicity of about 70 {$\mu$}Hz of the high-frequency pseudo modes, with a much reduced visibility during the phase of higher activity.},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/XYT6SFHA/Salabert et al. - 2004.pdf}
}

@article{Salabert2006,
  title = {Damping and {{Excitation Variations}} of the {{Solar Acoustic Modes Using LOWL Observations}}},
  author = {Salabert, D. and Jimenez-Reyes, S. J.},
  year = {2006},
  journal = {The Astrophysical Journal},
  volume = {650},
  number = {1},
  eprint = {astro-ph/0607346},
  pages = {451--460},
  issn = {0004-637X},
  doi = {10.1086/507177},
  abstract = {We have used observations made with the helioseismic instrument LOWL collected over \textasciitilde 6 years to carry out an independent study of the variations of the p-mode damping and excitation rates with solar activity. We observe significant variations in the mode height, mode width, and mode velocity power over a wide range of angular-degree values. Their sensitivities to solar activity show clear evidence of frequency dependence, with the modes in the frequency range from 2700 to 3300 {$\mu$}Hz showing the largest variations and exhibiting a maximum change centered around 3100 {$\mu$}Hz. The mode energy-supply rate is consistent, at the level of precision of the observations, with a zero change during the solar cycle and over the range of studied frequencies. Moreover, the variations with solar activity of each of these parameters are observed to be more or less independent of l over the range of studied angular degrees. Our results provide the first in-depth confirmation of the findings obtained from GONG measurements for intermediate angular degrees.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NBJN9ESX/Salabert, Jimenez‐Reyes - 2006.pdf}
}

@article{Salabert2007a,
  title = {Sun-as-a-Star Observations: {{Evidence}} for Degree Dependence of Changes in Damping of Low-{$\mathscr{l}$} p Modes along the Solar Cycle},
  author = {Salabert, D. and Chaplin, W. J. and Elsworth, Y. and New, R. and Verner, G. A.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {463},
  number = {3},
  pages = {1181--1187},
  issn = {00046361},
  doi = {10.1051/0004-6361:20066419},
  abstract = {Aims. We use 9.5-yr of BiSON Sun-as-a-star data to search for dependence of solar-cycle parameter changes on the angular degree, {$\mathscr{l}$}, of the data. The nature of the Sun-as-a-star observations is such that for changes measured at fixed frequency, or for changes averaged across the same range in frequency, any {$\mathscr{l}$} dependence present carries information on the latitudinal distribution of the agent (i.e., the activity) responsible for those changes. Methods. We split the 9.5-yr timeseries into contiguous 108-d pieces, and determine mean changes in the damping of, power in, and energy supplied to the modes through the solar cycle. We also apply a careful correction to account for the deleterious effects of the ground-based BiSON window function on the results. Results. From our full analysis we obtain a marginally significant result for the damping parameter, where the mean change is found to be weakest at {$\mathscr{l}$} = 0. The other parameters show hints of some dependence in {$\mathscr{l}$}. Conclusions. Our main conclusion is that the mean fractional solar-cycle change in the {$\mathscr{l}$} = 0 damping rates is approximately 50\% smaller than was previously assumed. It had been common practice to use an average over all low-{$\mathscr{l}$} modes; our downward revision of the radial-mode value has implications for comparisons with models of the global solar cycle changes, which are usually based on a spherically symmetric geometry. \textcopyright{} ESO 2007.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/3WLSK56I/Salabert et al. - 2007.pdf}
}

@article{Salabert2009,
  title = {Measurement of Low Signal-to-Noise-Ratio Solar p Modes in Spatially-Resolved Helioseismic Data},
  author = {Salabert, D. and Leibacher, J. and Appourchaux, T. and Hill, F.},
  year = {2009},
  number = {1985},
  eprint = {0902.2561},
  doi = {10.1088/0004-637X/696/1/653},
  abstract = {We present an adaptation of the rotation-corrected, m-averaged spectrum technique designed to observe low signal-to-noise-ratio, low-frequency solar p modes. The frequency shift of each of the 2l+1 m spectra of a given (n,l) multiplet is chosen that maximizes the likelihood of the m-averaged spectrum. A high signal-to-noise ratio can result from combining individual low signal-to-noise-ratio, individual-m spectra, none of which would yield a strong enough peak to measure. We apply the technique to GONG and MDI data and show that it allows us to measure modes with lower frequencies than those obtained with classic peak-fitting analysis of the individual-m spectra. We measure their central frequencies, splittings, asymmetries, lifetimes, and amplitudes. The low-frequency, low- and intermediate-angular degrees rendered accessible by this new method correspond to modes that are sensitive to the deep solar interior down to the core and to the radiative interior. Moreover, the low-frequency modes have deeper upper turning points, and are thus less sensitive to the turbulence and magnetic fields of the outer layers, as well as uncertainties in the nature of the external boundary condition. As a result of their longer lifetimes (narrower linewidths) at the same signal-to-noise ratio the determination of the frequencies of lower-frequency modes is more accurate, and the resulting inversions should be more precise.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/S5AIMF2N/Salabert et al. - 2009.pdf}
}

@article{Salabert2011a,
  title = {Mode Visibilities in Radial Velocity and Intensity {{Sun-as-a-star}} Helioseismic Measurements},
  author = {Salabert, D. and Ballot, J. and Garc{\'i}a, R. A.},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  pages = {1--9},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012053},
  abstract = {We analyze more than 5000 days of Sun-as-a-star radial velocity GOLF and intensity VIRGO observations to measure the visibilities of the I = 0, 1, 2, and 3 modes and the m-amplitude ratios of the I = 2 and 3 modes in the solar acoustic spectrum. We provide observational values that we compare to theoretical predictions. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  keywords = {data analysis,helioseismology,methods,notion,notion-database,sun},
  file = {/Users/lbugnet/Zotero/storage/LTFCJJLL/Salabert, Ballot, García - 2011.pdf;/Users/lbugnet/Zotero/storage/S93JQTUR/Salabert, Ballot, García - 2011(2).pdf}
}

@article{Salabert2011b,
  title = {About the P-Mode Frequency Shifts in {{HD}} 49933},
  author = {Salabert, D. and R{\'e}gulo, C. and Ballot, J. and Garc{\'i}a, R. A. and Mathur, S.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {530},
  pages = {1--5},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116633},
  abstract = {We study the frequency dependence of the frequency shifts of the low-degree p modes measured in the F5V star HD 49933, by analyzing the second run of observations collected by the CoRoT satellite. The 137-day light curve is divided into two subseries corresponding to periods of low and high stellar activity. The activity-frequency relationship is obtained independently from the analysis of the mode frequencies extracted by both a local and a global peak-fitting analyses, and from a cross-correlation technique in the frequency range between 1450 {$\mu$}Hz and 2500 {$\mu$}Hz. The three methods return consistent results. We show that the frequency shifts measured in HD 49933 present a frequency dependence with a clear increase with frequency, reaching a maximal shift of about 2 {$\mu$}Hz around 2100 {$\mu$}Hz. Similar variations are obtained between the l = 0 and l = 1 modes. At higher frequencies, the frequency shifts show indications of a downturn followed by an upturn, consistent between the l = 0 and 1 modes. We show that the frequency variation of the p-mode frequency shifts of the solar-like oscillating star HD 49933 has a comparable shape to the one observed in the Sun, which is understood to arise from changes in the outer layers due to its magnetic activity. \textcopyright{} 2011 ESO.},
  keywords = {Methods: data analysis,notion,notion-database,Stars: activity,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/KTHTRNXW/Salabert et al. - 2011.pdf}
}

@article{Salabert2011c,
  title = {Global P-Mode Oscillations throughout the Complete Solar Cycle 23 and the Beginning of Cycle 24},
  author = {Salabert, D. and Garc{\'i}a, R. A. and Pall{\'e}, P. L. and Jim{\'e}nez, A.},
  year = {2011},
  journal = {Journal of Physics: Conference Series},
  volume = {271},
  number = {1},
  eprint = {1011.4966},
  pages = {1998--1999},
  issn = {17426596},
  doi = {10.1088/1742-6596/271/1/012030},
  abstract = {The parameters of the p-mode oscillations vary with solar activity. Such temporal variations provide insights for the study of the structural and dynamical changes occurring in the Sun's interior throughout the solar cycle. We present here a complete picture of the temporal variations of the global p-mode parameters (excitation, damping, frequency, peak asymmetry, and rotational splitting) over the entire solar cycle 23 and the beginning of cycle 24 as observed by the space-based, Sun-as-a-star helioseismic GOLF and VIRGO instruments onboard SoHO. \textcopyright{} Published under licence by IOP Publishing Ltd.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/F44IQPBP/Salabert et al. - 2011(2).pdf}
}

@article{Salabert2015,
  title = {Seismic Sensitivity to Sub-Surface Solar Activity from 18 Yr of {{GOLF}}/{{SoHO}} Observations},
  author = {Salabert, D. and Garc{\'i}a, R. A. and {Turck-Chi{\`e}ze}, S.},
  year = {2015},
  journal = {Astronomy and Astrophysics},
  volume = {578},
  eprint = {1502.07607},
  pages = {1--12},
  issn = {14320746},
  doi = {10.1051/0004-6361/201425236},
  abstract = {Solar activity has significantly changed over the last two Schwabe cycles. After a long and deep minimum at the end of Cycle 23, the weaker activity of Cycle 24 contrasts with the previous cycles. In this work, the response of the solar acoustic oscillations to solar activity is used in order to provide insights into the structural and magnetic changes in the sub-surface layers of the Sun during this on-going unusual period of low activity. We analyze 18 yr of continuous observations of the solar acoustic oscillations collected by the Sun-as-a-star GOLF instrument on board the SoHO spacecraft. From the fitted mode frequencies, the temporal variability of the frequency shifts of the radial, dipolar, and quadrupolar modes are studied for different frequency ranges that are sensitive to different layers in the solar sub-surface interior. The low-frequency modes show nearly unchanged frequency shifts between Cycles 23 and 24, with a time evolving signature of the quasi-biennial oscillation, which is particularly visible for the quadrupole component revealing the presence of a complex magnetic structure. The modes at higher frequencies show frequency shifts that are 30\% smaller during Cycle 24, which is in agreement with the decrease observed in the surface activity between Cycles 23 and 24. The analysis of 18 yr of GOLF oscillations indicates that the structural and magnetic changes responsible for the frequency shifts remained comparable between Cycle 23 and Cycle 24 in the deeper sub-surface layers below 1400 km as revealed by the low-frequency modes. The frequency shifts of the higher-frequency modes, sensitive to shallower regions, show that Cycle 24 is magnetically weaker in the upper layers of Sun.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/42RXCSGW/Salabert, García, Turck-Chièze - 2015.pdf}
}

@article{Salabert2016,
  title = {The Solar-Stellar Connection: {{Magnetic}} Activity of Seismic Solar Analogs},
  author = {Salabert, D. and Garcia, R. A. and Beck, P. G. and Regulo, C. and Ballot, J. and Creevey, O. L. and Egeland, R. and do Nascimento, J. -D. and Hernandez, F. Perez and Bigot, L. and Mathur, S. and Metcalfe, T. S. and Corsaro, E. and Palle, P. L.},
  year = {2016},
  number = {1996},
  eprint = {1610.00990},
  pages = {1--7},
  doi = {10.5281/zenodo.159255},
  abstract = {Finding solar-analog stars with fundamental properties as close as possible to the Sun and studying the characteristics of their surface magnetic activity is a very promising way to understand the solar variability and its associated dynamo process. However, the identification of solar-analog stars depends on the accuracy of the estimated stellar parameters. Thanks to the photometric CoROT and Kepler space missions, the addition of asteroseismic data was proven to provide the most accurate fundamental properties that can be derived from stellar modeling today. Here, we present our latest results on the solar-stellar connection by studying 18 solar analogs that we identified among the Kepler seismic sample (Salabert et al., 2016a). We measured their magnetic activity properties using the observations collected by the Kepler satellite and the ground-based, high-resolution HERMES spectrograph. The photospheric (Sph) and chromospheric (S) magnetic activity proxies of these seismic solar analogs are compared in relation to the solar activity. We show that the activity of the Sun is comparable to the activity of the seismic solar analogs, within the maximum-to-minimum temporal variations of the 11-year solar activity cycle. Furthermore, we report on the discovery of temporal variability in the acoustic frequencies of the young (1 Gyr-old) solar analog KIC10644253 with a modulation of about 1.5 years, which agrees with the derived photospheric activity Sph (Salabert et al, 2016b). It could be the signature of the short-period modulation, or quasi-biennal oscillation, of its magnetic activity as observed in the Sun and in the 1-Gyr-old solar analog HD30495. In addition, the lithium abundance and the chromospheric activity estimated from HERMES confirms that KIC10644253 is a young and more active star than the Sun.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UWTGEICY/Salabert et al. - 2016(2).pdf}
}

@article{Salabert2016a,
  title = {Magnetic Variability in the Young Solar Analog {{KIC}} 10644253},
  author = {Salabert, D. and R{\'e}gulo, C. and Garc{\'i}a, R. A. and Beck, P. G. and Ballot, J. and Creevey, O. L. and P{\'e}rez Hern{\'a}ndez, F. and {do Nascimento Jr.}, J.-D. and Corsaro, E. and Egeland, R. and Mathur, S. and Metcalfe, T. S. and Bigot, L. and Ceillier, T. and Pall{\'e}, P. L.},
  year = {2016},
  journal = {Astronomy \& Astrophysics},
  volume = {589},
  pages = {A118},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201527978},
  keywords = {activity,data analysis,methods,notion,notion-database,observational,oscillations,solar-type,stars},
  file = {/Users/lbugnet/Zotero/storage/P5RD9SFH/Salabert et al. - 2016.pdf}
}

@article{Salabert2018,
  title = {Frequency Dependence of P-Mode Frequency Shifts Induced by Magnetic Activity in {{Kepler}} Solar-like Stars},
  author = {Salabert, D. and R{\'e}gulo, C. and Hern{\'a}ndez, F. P{\'e}rez and Garc{\'i}a, R. A.},
  year = {2018},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {611},
  eprint = {1712.05691},
  pages = {A84},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201731714},
  urldate = {2021-01-06},
  abstract = {The variations of the frequencies of the low-degree acoustic oscillations in the Sun induced by magnetic activity show a dependence on radial order. The frequency shifts are observed to increase towards higher-order modes to reach a maximum of about 0.8 {$\mu$}Hz over the 11-yr solar cycle. A comparable frequency dependence is also measured in two other main sequence solar-like stars, the F-star HD 49933, and the young 1 Gyr-old solar analog KIC 10644253, although with different amplitudes of the shifts of about 2 {$\mu$}Hz and 0.5 {$\mu$}Hz, respectively. Our objective here is to extend this analysis to stars with different masses, metallicities, and evolutionary stages. From an initial set of 87 Kepler solar-like oscillating stars with known individual p-mode frequencies, we identify five stars showing frequency shifts that can be considered reliable using selection criteria based on Monte Carlo simulations and on the photospheric magnetic activity proxy Sph. The frequency dependence of the frequency shifts of four of these stars could be measured for the l = 0 and l = 1 modes individually. Given the quality of the data, the results could indicate that a physical source of perturbation different from that in the Sun is dominating in this sample of solar-like stars.},
  archiveprefix = {arxiv},
  keywords = {activity,data analysis,Methods,notion,notion-database,oscillations,solar type,Stars},
  file = {/Users/lbugnet/Zotero/storage/G7PMV7M5/full-text.pdf}
}

@article{Salaris2015,
  title = {Post First Dredge-up [{{C}}/{{N}}] Ratio as Age Indicator. {{Theoretical}} Calibration},
  author = {Salaris, Maurizio and Pietrinferni, Adriano and Piersimoni, Anna M. and Cassisi, Santi},
  year = {2015},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {583},
  eprint = {1509.06904},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201526951},
  urldate = {2020-07-03},
  abstract = {We performed a detailed analysis of the use of [C/N] measured in red giant branch stars between the completion of the first dredge up and the red giant branch bump ([C/N] FDU) as age indicator. [C/N] FDU cannot give accurate ages for individual stars, but may provide a general chronology for the formation of composite populations and add constraints to analyses of red giants from surface gravity-effective temperature diagrams. We provide a theoretical calibration of [C/N] FDU in terms of total metallicity [M/H] and age, for ages greater than 1 Gyr, which we tested against variations in the initial heavy element distribution (scaled-solar vs. {$\alpha$}-enhanced), efficiency of overshooting from MS convective cores and from the convective envelopes, variations in the initial He abundance and in the mixing length parameter. Our calibration is compared with a small sample of available measurements of [C/N] FDU in star clusters and halo field stars, which at least qualitatively confirm the overall trend of the predicted [C/N] FDU with age and [M/H]. The use of [C/N] FDU-[M/H]-age relations obtained from independent sets of stellar evolution calculations cause age differences (for a given [C/N] FDU and [M/H] pair) up to 2 Gyr. More accurate spectroscopic measurements of [C/N] FDU in star clusters with well-established ages and metallicities are required to better test theoretical calibrations of this age indicator.},
  archiveprefix = {arxiv},
  keywords = {Convection,Galaxies: formation,notion,notion-database,Stars: abundances,Stars: evolution,Stars: interiors},
  file = {/Users/lbugnet/Zotero/storage/D7S5V32B/full-text.pdf}
}

@article{Samadi2001,
  title = {Excitation of Stellar P-Modes by Turbulent Convection: 1. {{Theoretical}} Formulation},
  author = {Samadi, Reza and Goupil, Marie-Jo},
  year = {2001},
  month = jan,
  journal = {Astronomy and Astrophysics},
  volume = {370},
  number = {1},
  eprint = {astro-ph/0101109},
  pages = {136--146},
  publisher = {{EDP Sciences}},
  doi = {10.1051/0004-6361:20010212},
  urldate = {2020-07-04},
  abstract = {Stochatic excitation of stellar oscillations by turbulent convection is investigated and an expression for the power injected into the oscillations by the turbulent convection of the outer layers is derived which takes into account excitation through turbulent Reynolds stresses and turbulent entropy fluctuations. This formulation generalizes results from previous works and is built so as to enable investigations of various possible spatial and temporal spectra of stellar turbulent convection. For the Reynolds stress contribution and assuming the Kolmogorov spectrum we obtain a similar formulation than those derived by previous authors. The entropy contribution to excitation is found to originate from the advection of the Eulerian entropy fluctuations by the turbulent velocity field. Numerical computations in the solar case in a companion paper indicate that the entropy source term is dominant over Reynold stress contribution to mode excitation, except at high frequencies.},
  archiveprefix = {arxiv},
  keywords = {Convection,notion,notion-database,Stars: oscillations,Sun: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/2GFMLZUX/full-text.pdf}
}

@article{Samadi2002,
  title = {Solar-like Oscillations in {$\delta$} {{Scuti}} Stars},
  author = {Samadi, R. and Goupil, M. J. and Houdek, G.},
  year = {2002},
  journal = {Astronomy and Astrophysics},
  volume = {395},
  number = {2},
  pages = {563--571},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021322},
  abstract = {Model computations of {$\delta$} Scuti stars, located in the vicinity of the red edge of the classical instability strip, suggest amplitudes of solar-like oscillations larger than in cooler models located outside the instability strip. Solar-like amplitudes in our {$\delta$} Scuti models are found to be large enough to be detectable with ground-based instruments provided they can be distinguished from the opacity-driven large-amplitude pulsations. There would be advantages in observing simultaneously opacity-driven and stochastically excited modes in the same star. We anticipate their possible detection in the context of the planned asteroseismic space missions, such as the French mission COROT (COnvection ROtation and planetary Transits). We propose known {$\delta$} Scuti stars as potential candidates for the target selection of these upcoming space missions.},
  keywords = {notion,notion-database,Stars: interiors,Stars: variables: {$\delta$}Sct},
  file = {/Users/lbugnet/Zotero/storage/5B6STWLL/Samadi, Goupil, Houdek - 2002.pdf}
}

@article{Samadi2005,
  title = {Excitation of Solar-like Oscillations: {{From PMS}} to {{MS}} Stellar Models},
  author = {Samadi, R. and Goupil, M. J. and Alecian, E. and Baudin, F. and Georgobiani, D. and Trampedach, R. and Stein, R. and Nordlund, {\AA}},
  year = {2005},
  journal = {Journal of Astrophysics and Astronomy},
  volume = {26},
  number = {2-3},
  pages = {171--184},
  publisher = {{Indian Academy of Sciences}},
  issn = {02506335},
  doi = {10.1007/BF02702325},
  urldate = {2020-07-04},
  abstract = {The amplitude of solar-like oscillations results from a balance between excitation and damping. As in the sun, the excitation is attributed to turbulent motions that stochastically excite the p modes in the uppermost part of the convective zone. We present here a model for the excitation mechanism. Comparisons between modeled amplitudes and helio and stellar seismic constraints are presented and the discrepancies discussed. Finally the possibility and the interest of detecting such stochastically excited modes in pre-main sequence stars are also discussed.},
  keywords = {Convection,Excitation,notion,notion-database,Oscillations,Stars: main and pre-main sequence stars,stars: {$\alpha$} Cen A,Sun,Turbulence}
}

@article{Samadi2007,
  title = {Excitation of Solar-like Oscillations across the {{HR}} Diagram},
  author = {Samadi, R. and Georgobiani, D. and Trampedach, R. and Goupil, M. J. and Stein, R. F. and Nordlund, {\AA}},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {463},
  number = {1},
  eprint = {astro-ph/0611762},
  pages = {297--308},
  issn = {00046361},
  doi = {10.1051/0004-6361:20041953},
  abstract = {Aims. We extend semi-analytical computations of excitation rates for solar oscillation modes to those of other solar-like oscillating stars to compare them with recent observations Methods. Numerical 3D simulations of surface convective zones of several solar-type oscillating stars are used to characterize the turbulent spectra as well as to constrain the convective velocities and turbulent entropy fluctuations in the uppermost part of the convective zone of such stars. These constraints, coupled with a theoretical model for stochastic excitation, provide the rate P at which energy is injected into the p-modes by turbulent convection. These energy rates are compared with those derived directly from the 3D simulations. Results. The excitation rates obtained from the 3D simulations are systematically lower than those computed from the semi-analytical excitation model. We find that Pmax, the P maximum, scales as (L/M)S where s is the slope of the power law and L and M are the mass and luminosity of the 1D stellar model built consistently with the associated 3D simulation. The slope is found to depend significantly on the adopted form of {$\chi$}k, the eddy time-correlation; using a Lorentzian, {$\chi$}kL, results in s = 2.6, whereas a Gaussian, {$\chi$}kG, gives s = 3.1. Finally, values of V, the maximum in the mode velocity, are estimated from the computed power laws for fm-dx and we find that Vmax increases as (L/M)SD. Comparisons with the currently available ground-based observations show that the computations assuming a Lorentzian {$\chi$}k yield a slope, sv, closer to the observed one than the slope obtained when assuming a Gaussian. We show that the spatial resolution of the 3D simulations must be high enough to obtain accurate computed energy rates. \textcopyright{} ESO 2007.},
  archiveprefix = {arxiv},
  keywords = {Convection,Hertzsprung-russell (hr) and c-m,notion,notion-database,Stars: Variables: general methods: numerical,Sun: oscillations,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/AWVQ7KLZ/Samadi et al. - 2007.pdf}
}

@article{Samadi2013,
  title = {Stellar Granulation as Seen in Disk-Integrated Intensity},
  author = {Samadi, R. and Belkacem, K. and Ludwig, H.-G. and Caffau, E. and Campante, T. L. and Davies, G. R. and Kallinger, T. and Lund, M. N. and Mosser, B. and Baglin, A. and Mathur, S. and Garcia, R. A.},
  year = {2013},
  journal = {Astronomy \& Astrophysics},
  volume = {559},
  pages = {A40},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201220817},
  abstract = {Context. Solar granulation has been known for a long time to be a surface manifestation of convection. The space-borne missions CoRoT and Kepler enable us to observe the signature of this phenomena in disk-integrated intensity on a large number of stars. Aims. The space-based photometric measurements show that the global brightness fluctuations and the lifetime associated with granulation obeys characteristic scaling relations. We thus aimed at providing simple theoretical modeling to reproduce these scaling relations, and subsequently at inferring the physical properties of granulation across the Hertzsprung-Russell diagram. Methods. We developed a simple 1D theoretical model. The input parameters were extracted from 3D hydrodynamical models of the surface layers of stars, and the free parameters involved in the model were calibrated with solar observations. Two different prescriptions for representing the Fourier transform of the time-correlation of the eddy velocity were compared: a Lorentzian and an exponential form. Finally, we compared our theoretical prediction with 3D radiative hydrodynamical (RHD) numerical modeling of stellar granulation (hereafter ab initio approach). Results. Provided that the free parameters are appropriately adjusted, our theoretical model reproduces the observed solar granulation spectrum quite satisfactorily; the best agreement is obtained for an exponential form. Furthermore, our model results in granulation spectra that agree well with the ab initio approach using two 3D RHD models that are representative of the surface layers of an F-dwarf and a red-giant star. Conclusions. We have developed a theoretical model that satisfactory reproduces the solar granulation spectrum and gives results consistent with the ab initio approach. The model is used in a companion paper as theoretical framework for interpretating the observed scaling relations.},
  keywords = {atmospheres,convection,granulation,notion,notion-database,oscillations,stars,sun,turbulence},
  file = {/Users/lbugnet/Zotero/storage/Z7SD3I5L/Samadi et al. - 2013.pdf}
}

@article{Samadi2013a,
  title = {Stellar Granulation as Seen in Disk-Integrated Intensity. {{II}}. {{Theoretical}} Scaling Relations Compared with Observations},
  author = {Samadi, R. and Belkacem, K. and Ludwig, H. -G. and Caffau, E. and Campante, T. L. and Davies, G. R. and Kallinger, T. and Lund, M. N. and Mosser, B. and Baglin, A. and Mathur, S. and Garcia, R.},
  year = {2013},
  month = sep,
  eprint = {1309.1488},
  doi = {10.1051/0004-6361/201220817},
  urldate = {2020-03-14},
  abstract = {A large set of stars observed by CoRoT and Kepler shows clear evidence for the presence of a stellar background, which is interpreted to arise from surface convection, i.e., granulation. These observations show that the characteristic time-scale (tau\_eff) and the root-mean-square (rms) brightness fluctuations (sigma) associated with the granulation scale as a function of the peak frequency (nu\_max) of the solar-like oscillations. We aim at providing a theoretical background to the observed scaling relations based on a model developed in the companion paper. We computed for each 3D model the theoretical power density spectrum (PDS) associated with the granulation as seen in disk-integrated intensity on the basis of the theoretical model. For each PDS we derived tau\_eff and sigma and compared these theoretical values with the theoretical scaling relations derived from the theoretical model and the Kepler measurements. We derive theoretical scaling relations for tau\_eff and sigma, which show the same dependence on nu\_max as the observed scaling relations. In addition, we show that these quantities also scale as a function of the turbulent Mach number (Ma) estimated at the photosphere. The theoretical scaling relations for tau\_eff and sigma match the observations well on a global scale. Our modelling provides additional theoretical support for the observed variations of sigma and tau\_eff with nu\_m max. It also highlights the important role of Ma in controlling the properties of the stellar granulation. However, the observations made with Kepler on a wide variety of stars cannot confirm the dependence of our scaling relations on Ma. Measurements of the granulation background and detections of solar-like oscillations in a statistically sufficient number of cool dwarf stars will be required for confirming the dependence of the theoretical scaling relations with Ma.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@inproceedings{Samadi2015,
  title = {Stellar Oscillations - {{II}} - {{The}} Non-Adiabatic Case},
  booktitle = {{{EAS Publications Series}}},
  author = {Samadi, R. and Belkacem, K. and Sonoi, T.},
  year = {2015},
  volume = {73--74},
  eprint = {1510.01151},
  pages = {111--191},
  publisher = {{EDP Sciences}},
  issn = {16381963},
  doi = {10.1051/eas/1573003},
  urldate = {2020-03-08},
  abstract = {A leap forward has been performed due to the space-borne missions, MOST, CoRoT and Kepler. They provided a wealth of observational data, and more precisely oscillation spectra, which have been (and are still) exploited to infer the internal structure of stars. While an adiabatic approach is often sufficient to get information on the stellar equilibrium structures it is not sufficient to get a full understanding of the physics of the oscillation. Indeed, it does not permit one to answer some fundamental questions about the oscillations, such as: What are the physical mechanisms responsible for the pulsations inside stars? What determines the amplitudes? To what extent the adiabatic approximation is valid? All these questions can only be addressed by considering the energy exchanges between the oscillations and the surrounding medium. This lecture therefore aims at considering the energetical aspects of stellar pulsations with particular emphasis on the driving and damping mechanisms. To this end, the full non-adiabatic equations are introduced and thoroughly discussed. Two types of pulsation are distinguished, namely the self-excited oscillations that result from an instability and the solar-like oscillations that result from a balance between driving and damping by turbulent convection. For each type, the main physical principles are presented and illustrated using recent observations obtained with the ultra-high precision photometry spaceborne missions (MOST, CoRoT and Kepler). Finally, we consider in detail the physics of scaling relations, which relates the seismic global indices with the global stellar parameters and gave birth to the development of statistical (or ensemble) asteroseismology. Indeed, several of these relations rely on the same cause: the physics of non-adiabatic oscillations.},
  archiveprefix = {arxiv},
  isbn = {978-2-7598-1735-1},
  keywords = {notion,notion-database}
}

@article{samadiPLATOSolarlikeLightcurve2019,
  title = {The {{PLATO Solar-like Light-curve Simulator A}} Tool to Generate Realistic Stellar Light-Curves with Instrumental Effects Representative of the {{PLATO}} Mission},
  author = {Samadi, R and Deru, A and Reese, D and Marchiori, V and Grolleau, E and Green, J J and Pertenais, M and Lebreton, Y and Deheuvels, S and Mosser, B and Belkacem, K and B{\"o}rner, A and Smith, A M S},
  year = {2019},
  journal = {A\&A},
  volume = {624},
  pages = {117},
  doi = {10.1051/0004-6361/201834822},
  urldate = {2021-04-09},
  abstract = {Context. ESA's PLATO space mission, to be launched by the end of 2026, aims to detect and characterise Earth-like planets in their habitable zone using asteroseismology and the analysis of the transit events. The preparation of science objectives will require the implementation of hare-and-hound exercises relying on the massive generation of representative simulated light-curves. Aims. We developed a light-curve simulator named the PLATO Solar-like Light-curve Simulator (PSLS) in order to generate light-curves representative of typical PLATO targets, that is showing simultaneously solar-like oscillations, stellar granulation, and magnetic activity. At the same time, PSLS also aims at mimicking in a realistic way the random noise and the systematic errors representative of the PLATO multi-telescope concept. Methods. To quantify the instrumental systematic errors, we performed a series of simulations at pixel level that include various relevant sources of perturbations expected for PLATO. From the simulated pixels, we extract the photometry as planned on-board and also simulate the quasi-regular updates of the aperture masks during the observations. The simulated light-curves are then corrected for instrumental effects using the instrument point spread functions reconstructed on the basis of a microscanning technique that will be operated during the in-flight calibration phases of the mission. These corrected and simulated light-curves are then fitted by a parametric model, which we incorporated in PSLS. Simulation of the oscillations and granulation signals rely on current state-of-the-art stellar seismology. Results. We show that the instrumental systematic errors dominate the signal only at frequencies below {$\sim$}20 \textmu Hz. The systematic errors level is found to mainly depend on stellar magnitude and on the detector charge transfer inefficiency. To illustrate how realistic our simulator is, we compared its predictions with observations made by Kepler on three typical targets and found a good qualitative agreement with the observations. Conclusions. PSLS reproduces the main properties of expected PLATO light-curves. Its speed of execution and its inclusion of relevant stellar signals as well as sources of noises representative of the PLATO cameras make it an indispensable tool for the scientific preparation of the PLATO mission.},
  keywords = {asteroseismology-stars,image processing-techniques,notion,notion-database,numerical,oscillations-techniques,photometric-methods},
  file = {/Users/lbugnet/Zotero/storage/YUCZQ9KS/full-text.pdf}
}

@article{Sana2012,
  title = {Binary Interaction Dominates the Evolution of Massive Stars},
  author = {Sana, H. and {de Mink}, S. E. and {de Koter}, A. and Langer, N. and Evans, C. J. and Gieles, M. and Gosset, E. and Izzard, R. G. and Bouquin, J. -B. Le and Schneider, F. R. N.},
  year = {2012},
  month = jul,
  journal = {Science},
  volume = {337},
  number = {6093},
  eprint = {1207.6397},
  pages = {444--446},
  publisher = {{American Association for the Advancement of Science}},
  doi = {10.1126/science.1223344},
  urldate = {2020-08-31},
  abstract = {The presence of a nearby companion alters the evolution of massive stars in binary systems, leading to phenomena such as stellar mergers, X-ray binaries and gamma-ray bursts. Unambiguous constraints on the fraction of massive stars affected by binary interaction were lacking. We simultaneously measured all relevant binary characteristics in a sample of Galactic massive O stars and quantified the frequency and nature of binary interactions. Over seventy per cent of all massive stars will exchange mass with a companion, leading to a binary merger in one third of the cases. These numbers greatly exceed previous estimates and imply that binary interaction dominates the evolution of massive stars, with implications for populations of massive stars and their supernovae.},
  archiveprefix = {arxiv},
  keywords = {ASTRONOMY,Astrophysics,Cosmology and Extragalactic Astrophysics,notion,notion-database,Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/ZUHSLB4G/full-text.pdf}
}

@article{Sanchez2014,
  title = {A Mean-Field {{Babcock-Leighton}} Solar Dynamo Model with Long-Term Variability},
  author = {Sanchez, Sabrina and Fournier, Alexandre and Pinheiro, Katia J and Aubert, Julien},
  year = {2014},
  journal = {An Acad Bras Cienc},
  volume = {86},
  number = {1},
  issn = {1678-2690},
  doi = {10.1590/0001-37652014111212},
  urldate = {2020-05-14},
  abstract = {Dynamo models relying on the Babcock-Leighton mechanism are successful in reproducing most of the solar magnetic field dynamical characteristics. However, considering that such models operate only above a lower magnetic field threshold, they do not provide an appropriate magnetic field regeneration process characterizing a self-sustainable dynamo. In this work we consider the existence of an additional {$\alpha$}-effect to the Babcock-Leighton scenario in a mean-field axisymmetric kinematic numerical model. Both poloidal field regeneration mechanisms are treated with two different strength-limiting factors. Apart from the solar antisymmetric parity behavior, the main solar features are reproduced: cyclic polarity reversals, mid-latitudinal equatorward migration of strong toroidal field, poleward migration of polar surface radial fields, and the quadrature phase shift between both. Long-term variability of the solutions exhibits lenghty periods of minimum activity followed by posterior recovery, akin to the observed Maunder Minimum. Based on the analysis of the residual activity during periods of minimum activity, we suggest that these are caused by a predominance of the {$\alpha$}-effect over the Babcock-Leighton mechanism in regenerating the poloidal field.},
  keywords = {magnetohydrodynamics,notion,notion-database,solar cycle,solar dynamo,sunspots},
  file = {/Users/lbugnet/Zotero/storage/DX6NWVM9/full-text.pdf}
}

@article{SanchezArias2023,
  title = {Frequency Analysis of the Hybrid {$\delta$} {{Sct-$\gamma$ Dor}} Star {{CoRoT-102314644}}},
  author = {S{\'a}nchez Arias, J. P. and Creevey, O. L. and Chapellier, E. and Pichon, B.},
  year = {2023},
  month = aug,
  journal = {Astronomy and Astrophysics},
  volume = {676},
  pages = {A96},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202141610},
  urldate = {2023-10-17},
  abstract = {Context. Observations from space missions allowed significant progress due to the absence of atmospheric noise contributions and having uninterrupted data sets. This has been extremely beneficial in asteroseismology because many oscillation frequencies, not observable from the ground, can be detected. One example of this success is the large number of hybrid {$\delta$} Sct-{$\gamma$} Dor stars discovered. These stars have radial and non-radial p and g modes simultaneously excited, allowing us to probe both the external and near-to-core layers. Aims: We aim to analyse the light curve of the hybrid {$\delta$} Sct-{$\gamma$} Dor star CoRoT ID 102314644 and characterise its frequency spectrum. Using the detected frequencies, we intend to perform an initial interpretation developing stellar models. Methods: The frequency analysis was obtained with a classical Fourier analysis. A detailed analysis of the individual frequencies is performed using phase diagrams and other light curve characteristics. Initial stellar modelling was performed using the Cesam2k and the GYRE code. Results: We detected 29 {$\gamma$} Dor type frequencies in the [0.32 - 3.66] c/d range and a series of six equidistant periods with a mean period spacing of {$\Delta\Pi$} = 1612 s. In the {$\delta$} Sct domain, we found 38 frequencies in the [8.63 - 24.73] c/d range and a quintuplet centred on the frequency p1 = 11.39 c/d, which suggests a rotational period of 3.06 d. The frequency analysis suggests the presence of spots. Nevertheless, we could not dismiss the possibility of a binary system. The initial modelling of the frequency data allowed us to refine its astrophysical parameters. Conclusions: The observed period spacing, a p-mode quintuplet, the possible rotation period, and the analysis of the individual frequencies impose significant constraints on our understanding of differential rotation and magnetic fields operating in A-F-type stars. Nevertheless, it is fundamental to accompany photometric data with spectroscopic measurements to distinguish variations between surface activity from a companion.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: oscillations,stars: variables: {$\delta$} Scuti,techniques: photometric},
  annotation = {ADS Bibcode: 2023A\&A...676A..96S},
  file = {/Users/lbugnet/Zotero/storage/IIMGWQQ3/Sánchez Arias et al. - 2023 - Frequency analysis of the hybrid δ Sct-γ Dor star .pdf}
}

@article{Santos2004,
  title = {Spectroscopic [{{Fe}}/{{H}}] for 98 Extra-Solar Planet-Host Stars. {{Exploring}} the Probability of Planet Formation},
  author = {Santos, N. C. and Israelian, G. and Mayor, M.},
  year = {2004},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {415},
  number = {3},
  eprint = {astro-ph/0311541},
  pages = {1153--1166},
  issn = {00046361},
  doi = {10.1051/0004-6361:20034469},
  urldate = {2020-03-12},
  abstract = {We present stellar parameters and metallicities, obtained from a detailed spectroscopic analysis, for a large sample of 98 stars known to be orbited by planetary mass companions (almost all known targets), as well as for a volume-limited sample of 41 stars not known to host any planet. For most of the stars the stellar parameters are revised versions of the ones presented in our previous work. However, we also present parameters for 18 stars with planets not previously published, and a compilation of stellar parameters for the remaining 4 planet-hosts for which we could not obtain a spectrum. A comparison of our stellar parameters with values of Teff, log g, and [Fe/H] available in the literature shows a remarkable agreement. In particular, our spectroscopic log g values are now very close to trigonometric log g estimates based on Hipparcos parallaxes. The derived [Fe/H] values are then used to confirm the previously known result that planets are more prevalent around metal-rich stars. Furthermore, we confirm that the frequency of planets is a strongly rising function of the stellar metallicity, at least for stars with [Fe/H] {$>$} 0. While only about 3\% of the solar metallicity stars in the CORALIE planet search sample were found to be orbited by a planet, this number increases to more than 25\% for stars with [Fe/H] above +0.3. Curiously, our results also suggest that these percentages might remain relatively constant for values of [Fe/H] lower than about solar, increasing then linearly with the mass fraction of heavy elements. These results are discussed in the context of the theories of planetary formation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: Abundances,Stars: Chemically peculiar,Stars: Fundamental parameters,Stars: Planetary systems,Stars: Planetary systems: formation},
  file = {/Users/lbugnet/Zotero/storage/LGU5YYNJ/full-text.pdf}
}

@article{Santos2010,
  title = {Do Stellar Magnetic Cycles Influence the Measurement of Precise Radial Velocities?},
  author = {Santos, N. C. and Gomes Da Silva, J. and Lovis, C. and Melo, C.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {511},
  number = {1},
  eprint = {0912.2901},
  pages = {1--10},
  issn = {00046361},
  doi = {10.1051/0004-6361/200913433},
  abstract = {The ever increasing level of precision achieved by present and future radial-velocity instruments is opening the way to discovering very low-mass, long-period planets (e.g. solar-system analogs). These systems will be detectable as low-amplitude signals in radial-velocity (RV). However, an important obstacle to their detection may be the existence of stellar magnetic cycles on similar timescales. Here we present the results of a long-term program to simultaneously measure radial-velocities and stellar-activity indicators (CaII, H{$\alpha$}, Hei) for a sample of stars with known activity cycles. Our results suggest that all these stellar activity indexes can be used to trace the stellar magnetic cycle in solar-type stars. Likewise, we find clear indications that different parameters of the HARPS cross-correlation function (BIS, FWHM, and contrast) are also sensitive to activity level variations. Finally, we show that, although in a few cases slight correlations or anti-correlations between radial-velocity and the activity level of the star exist, their origin is still not clear. We can, however, conclude that for our targets (early-K dwarfs) we do not find evidence of any radial-velocity variations induced by variations of the stellar magnetic cycle with amplitudes significantly above {$\sim$}1 m/s. \textcopyright{} 2010 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: activity,Stars: fundamental parameters,Starspots,Techniques: radial velocities,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/LDGYQLPV/Santos et al. - 2010.pdf}
}

@article{Santos2017,
  title = {Starspot Signature on the Light Curve: {{Learning}} about the Latitudinal Distribution of Spots},
  author = {Santos, A. R.G. and Cunha, M. S. and Avelino, P. P. and Garc{\'i}a, R. A. and Mathur, S.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {599},
  pages = {4--11},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629923},
  abstract = {Context. Quasi-periodic modulations of the stellar light curve may result from dark spots crossing the visible stellar disc. Owing to differential rotation, spots at different latitudes generally have different rotation periods. Hence, by studying spot-induced modulations, it is possible to learn about stellar surface (differential) rotation and magnetic activity. Recently, a method based on the Lomb-Scargle periodogram of light curves has been proposed to identify the sign of the differential rotation at the stellar surface. Aims. Our goal is to understand how the modulation of the stellar light curve due to the presence of spots and the corresponding periodogram are affected by both the stellar and spot properties. Methods. We generate synthetic light curves of stars with different properties (inclination angle, limb darkening, and rotation rate) and spot configurations (number of spots, latitude, intensity contrast, and size). By analysing their Lomb-Scargle periodograms, we compute the ratio between the heights of the second and first harmonics of the rotation period (peak-height ratio). Results. We find that the peak-height ratios are essentially a function of a single parameter, the fraction of time the spot is visible, which is related to the sinusoidality of the spot modulation. We identify the conditions under which the periodogram analysis can actually provide an estimate of the spot latitudes and/or the stellar inclination angle. We also identify possible sources of error in the identification of the sign of the differential rotation.},
  keywords = {notion,notion-database,Stars: activity,Stars: rotation,Stars: solar-type,Starspots,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/D74SEM36/Santos et al. - 2017.pdf}
}

@article{Santos2018,
  title = {Signatures of {{Magnetic Activity}} in the {{Seismic Data}} of {{Solar-type Stars Observed}} by {{Kepler}}},
  author = {Santos, A. R. G. and Campante, T. L. and Chaplin, W. J. and Cunha, M. S. and Lund, M. N. and Kiefer, R. and Salabert, D. and Garc{\'i}a, R. A. and Davies, G. R. and Elsworth, Y. and Howe, R.},
  year = {2018},
  journal = {The Astrophysical Journal Supplement Series},
  doi = {10.3847/1538-4365/aac9b6},
  keywords = {notion,notion-database}
}

@article{Santos2019,
  title = {Surface {{Rotation}} and {{Photometric Activity}} for {{Kepler Targets}}. {{I}}. {{M}} and {{K Main-sequence Stars}}},
  author = {Santos, A. R. G. and Garc{\'i}a, R. A. and Mathur, S. and Bugnet, L. and {van Saders}, J. L. and Metcalfe, T. S. and Simonian, G. V. A. and Pinsonneault, M. H.},
  year = {2019},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {244},
  number = {1},
  eprint = {1908.05222},
  pages = {21},
  doi = {10.3847/1538-4365/ab3b56},
  abstract = {Brightness variations due to dark spots on the stellar surface encode information about stellar surface rotation and magnetic activity. In this work, we analyze the Kepler long-cadence data of 26,521 main-sequence stars of spectral types M and K in order to measure their surface rotation and photometric activity level. Rotation-period estimates are obtained by the combination of a wavelet analysis and autocorrelation function of the light curves. Reliable rotation estimates are determined by comparing the results from the different rotation diagnostics and four data sets. We also measure the photometric activity proxy Sph using the amplitude of the flux variations on an appropriate timescale. We report rotation periods and photometric activity proxies for about 60 per cent of the sample, including 4,431 targets for which McQuillan et al. (2013a,2014) did not report a rotation period. For the common targets with rotation estimates in this study and in McQuillan et al. (2013a,2014), our rotation periods agree within 99 per cent. In this work, we also identify potential polluters, such as misclassified red giants and classical pulsator candidates. Within the parameter range we study, there is a mild tendency for hotter stars to have shorter rotation periods. The photometric activity proxy spans a wider range of values with increasing effective temperature. The rotation period and photometric activity proxy are also related, with Sph being larger for fast rotators. Similar to McQuillan et al. (2013a,2014), we find a bimodal distribution of rotation periods.},
  archiveprefix = {arxiv},
  keywords = {activity,catalogs,data analysis,low-mass,methods,notion,notion-database,photometric,rotation,stars,starspots,techniques},
  file = {/Users/lbugnet/Zotero/storage/FX79B6IX/Santos et al. - 2019.pdf}
}

@misc{santosSurfaceRotationPhotometric2019,
  title = {Surface Rotation and Photometric Activity for Kepler Targets {{I}}. {{M}} and {{K}} Main-Sequence Stars},
  author = {Santos, A.R.G. and Garc{\'i}a, R.A. and Mathur, S. and Bugnet, L. and {van Saders}, J.L. and Metcalfe, T.S. and Simonian, G.V.A. and Pinsonneault, M.H.},
  year = {2019},
  journal = {arXiv},
  abstract = {Copyright \textcopyright{} 2019, arXiv, All rights reserved. Brightness variations due to dark spots on the stellar surface encode information about stellar surface rotation and magnetic activity. In this work, we analyze the Kepler long-cadence data of 26,521 main-sequence stars of spectral types M and K in order to measure their surface rotation and photometric activity level. Rotation-period estimates are obtained by the combination of a wavelet analysis and autocorrelation function of the light curves. Reliable rotation estimates are determined by comparing the results from the different rotation diagnostics and four data sets. We also measure the photometric activity proxy Sph using the amplitude of the flux variations on an appropriate timescale. We report rotation periods and photometric activity proxies for about 60 per cent of the sample, including 4,431 targets for which McQuillan et al. (2013b, 2014) did not report a rotation period. For the common targets with rotation estimates in this study and in McQuillan et al. (2013b, 2014), our rotation periods agree within 99 per cent. In this work, we also identify potential polluters, such as misclassified red giants and classical pulsator candidates. Within the parameter range we study, there is a mild tendency for hotter stars to have shorter rotation periods. The photometric activity proxy spans a wider range of values with increasing effective temperature. The rotation period and photometric activity proxy are also related, with Sph being larger for fast rotators. Similar to McQuillan et al. (2013b, 2014), we find a bimodal distribution of rotation periods.},
  keywords = {Catalogs,Methods: data analysis,notion,notion-database,Stars: activity,Stars: low-mass,Stars: rotation,Starspots,Techniques: photometric}
}

@article{Sanyal2017,
  title = {Astrophysics {{Metallicity}} Dependence of Envelope Inflation in Massive Stars},
  author = {Sanyal, D and Langer, N and Sz{\'e}csi, D and Yoon, S.-C and Grassitelli, L},
  year = {2017},
  journal = {A\&A},
  volume = {597},
  pages = {71},
  doi = {10.1051/0004-6361/201629612},
  urldate = {2020-06-08},
  abstract = {Context. Recently it has been found that models of massive stars reach the Eddington limit in their interior, which leads to dilute extended envelopes. Aims. We perform a comparative study of the envelope properties of massive stars at different metallicities, with the aim to establish the impact of the stellar metallicity on the effect of envelope inflation. Methods. We analysed published grids of core-hydrogen burning massive star models computed with metallicities appropriate for massive stars in the Milky Way, the Large Magellanic Cloud, and the Small Magellanic Cloud, the very metal poor dwarf galaxy I Zwicky 18, and for metal-free chemical composition. Results. Stellar models of all the investigated metallicities reach and exceed the Eddington limit in their interior, aided by the opacity peaks of iron, helium, and hydrogen, and consequently develop inflated envelopes. Envelope inflation leads to a redward bending of the zero-age main sequence and a broadening of the main-sequence band in the upper part of the Hertzsprung-Russell diagram. We derive the limiting L/M-values as a function of the stellar surface temperature above which inflation occurs, and find them to be higher for lower metallicity. While Galactic models show inflation above {$\sim$}29 M , the corresponding mass limit for Population III stars is {$\sim$}150 M. While the masses of the inflated envelopes are generally low, we find that they can reach 1-100 M in models with effective temperatures below {$\sim$}8000 K, with higher masses reached by models of lower metallicity. Conclusions. Envelope inflation is expected to occur in sufficiently massive stars at all metallicities, and is expected to lead to rapidly growing pulsations, high macroturbulent velocities, and might well be related to the unexplained variability observed in luminous blue variables such as S Doradus and {$\eta$} Carina.},
  keywords = {evolution-stars,interiors-stars,mass-loss,massive-stars,notion,notion-database,stars},
  file = {/Users/lbugnet/Zotero/storage/XCFNLYFT/full-text.pdf}
}

@article{Sanz-Forcada2013,
  title = {{$\iota$} {{Horologi}}, the First Coronal Activity Cycle in a Young Solar-like Star},
  author = {{Sanz-Forcada}, J. and Stelzer, B. and Metcalfe, T. S.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {553},
  pages = {1--5},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321388},
  abstract = {Context. The shortest chromospheric (Ca ii H\&K) activity cycle (1.6 yr) has been recently discovered in the young (\textasciitilde 600 Myr) solar-like star {$\iota$} Hor. Coronal X-ray activity cycles have only been discovered in a few stars other than the Sun, all of them with an older age and a lower activity level than {$\iota$} Hor. Aims. We intended to find the X-ray coronal counterpart of the chromospheric cycle for {$\iota$} Hor. This represents the first X-ray cycle observed in an active star, as well as the paradigm of the first coronal cycles in the life of a solar-like star. Methods. We monitored {$\iota$} Hor with XMM-Newton observations spanning almost two years. The spectra of each observation are fit with two-temperature coronal models to study the long-term variability of the star. Results. We find a cyclic behavior in X-rays very similar to the contemporaneous chromospheric cycle. The continuous chromospheric monitoring for more than three cycle lengths shows a trend toward decreasing amplitude, apparently modulated by a longer term trend. The second cycle is disrupted prior to reaching its maximum, followed by a brief episode of chaotic variability before the cyclic behavior resumes, only to be disrupted again after slightly more than one cycle. Conclusions. We confirm the presence of an activity cycle of \textasciitilde 1.6 yr in {$\iota$} Hor both in X-rays and Ca ii H\&K. It is likely subject to the modulation of a longer, not yet constrained second cycle. The 1.6 yr cycle is the shortest coronal one observed to date, and {$\iota$} Hor represents the most active star for which a coronal activity cycle has been found. This cycle is probably representative of the first coronal cycles in the life of a solar-like star, at the age when life started on Earth. \textcopyright{} ESO, 2013.},
  keywords = {Astrobiology,notion,notion-database,Planetary systems,Stars: activity,Stars: chromospheres,Stars: coronae,Stars: individual:{$\iota$}Horologi},
  file = {/Users/lbugnet/Zotero/storage/9YTAB8PD/Sanz-Forcada, Stelzer, Metcalfe - 2013.pdf}
}

@book{Saslaw1985,
  title = {Gravitational Physics of Stellar and Galactic Systems},
  author = {Saslaw, W. C. and C., W.},
  year = {1985},
  urldate = {2020-03-07},
  keywords = {Astronomical Models,Astrophysics,Boltzmann Transport Equation,CLUSTERING,CLUSTERS OF GALAXIES,Cosmology,Fokker,Galactic Clusters,Galactic Evolution,Galactic Nuclei,Galactic Rotation,Galaxies,GALAXIES,Globular Clusters,GRAVITATION,Gravitational Collapse,Gravitational Effects,Gravitational Fields,GRAVITATIONAL FIELDS,GRAVITATIONAL INTERACTIONS,Many Body Problem,notion,notion-database,Orbital Mechanics,Planck Equation,Spiral Galaxies,Star Clusters,STARS,Stellar Evolution,Stellar Gravitation,Stellar Physics,STELLAR SYSTEMS,THEORY}
}

@article{saundersEvolutionaryObservationalProperties2023,
  title = {Evolutionary and {{Observational Properties}} of {{Red Giant Acoustic Glitch Signatures}}},
  author = {Saunders, David P. and Ong, J. M. Joel and Basu, Sarbani},
  year = {2023},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {947},
  pages = {22},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/acbdf3},
  urldate = {2023-05-28},
  abstract = {While solar-like oscillations in red giants have been observed at massive scales by the Kepler mission, few features of these oscillation mode frequencies, other than their global properties, have been exploited for stellar characterization. The signatures of acoustic glitches in mode frequencies have been used for studying main-sequence stars, but the validity of applying such techniques to evolved red giants, particularly pertaining to the inclusion of nonradial modes, has been less well examined. Making use of new theoretical developments, we characterize glitches using the {$\pi$} modes associated with red giant stellar models, and use our procedure to examine for the first time how the properties of the He II acoustic glitch-specifically its amplitude and associated acoustic depth-vary over the course of evolution up the red giant branch, and with respect to other fundamental stellar properties. We find that the acoustic depths of these glitches, in conjunction with other spectroscopic information, discriminate between red giants in the first-ascent and core-helium-burning phases. We critically reexamine previous attempts to constrain acoustic glitches from nonradial (in particular dipole) modes in red giants. Finally, we apply our fitting procedure to Kepler data, to evaluate its robustness to noise and other observational systematics.},
  keywords = {1372,1965,73,Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,Computational methods,Red giant stars},
  annotation = {ADS Bibcode: 2023ApJ...947...22S},
  file = {/Users/lbugnet/Zotero/storage/DXCXYFL3/Saunders et al. - 2023 - Evolutionary and Observational Properties of Red G.pdf}
}

@article{Saux2019,
  title = {Automatic Classification of {{K2}} Pulsating Stars Using Machine Learning Techniques},
  author = {Saux, A. Le and Bugnet, L. and Mathur, S. and Breton, S. N. and Garcia, R. A.},
  year = {2019},
  month = jun,
  eprint = {1906.09611},
  urldate = {2020-07-08},
  abstract = {The second mission of the NASA Kepler satellite, K2, has collected hundreds of thousands of lightcurves for stars close to the ecliptic plane. This new sample could increase the number of known pulsating stars and then improve our understanding of those stars. For the moment only a few stars have been properly classified and published. In this work, we present a method to automaticly classify K2 pulsating stars using a Machine Learning technique called Random Forest. The objective is to sort out the stars in four classes: red giant (RG), main-sequence Solar-like stars (SL), classical pulsators (PULS) and Other. To do this we use the effective temperatures and the luminosities of the stars as well as the FliPer features, that measures the amount of power contained in the power spectral density. The classifier now retrieves the right classification for more than 80\% of the stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SN69UU36/full-text.pdf}
}

@inproceedings{sauxAutomaticClassificationK22019,
  title = {Automatic Classification of K2 Pulsating Stars Using Machine Learning Techniques},
  booktitle = {{{arXiv}}},
  author = {Saux, A.L. and Bugnet, L. and Mathur, S. and Breton, S.N. and Garca, R.A.},
  year = {2019},
  abstract = {Copyright \textcopyright{} 2019, arXiv, All rights reserved. The second mission of NASA's Kepler satellite, K2, has collected hundreds of thousands of lightcurves for stars close to the ecliptic plane. This new sample could increase the number of known pulsating stars and then improve our understanding of those stars. For the moment only a few stars have been properly classified and published. In this work, we present a method to automaticly classify K2 pulsating stars using a Machine Learning technique called Random Forest. The objective is to sort out the stars in four classes: red giant (RG), main-sequence Solar-like stars (SL), classical pulsators (PULS) and Other. To do this we use the effective temperatures and the luminosities of the stars as well as the FliPer features, that measures the amount of power contained in the power spectral density. The classifier now retrieves the right classification for more than 80\% of the stars.},
  keywords = {Asteroseismology,Methods: Data Analysis,notion,notion-database,Stars: Oscillations,Thecniques: Machine Learning}
}

@article{Savanov2013,
  title = {The Presence of a Magnetic Field on the Pulsating Subdwarf {{Balloon}} 090100001. {{Observations}} of 2012},
  author = {Savanov, I. S. and Romaniuk, I. I. and Semenko, E. A. and Dmitrienko, E. S.},
  year = {2013},
  month = oct,
  journal = {Astronomy Reports},
  volume = {57},
  pages = {751--756},
  issn = {1063-7729},
  doi = {10.1134/S1063772913090059},
  urldate = {2023-10-09},
  abstract = {New polarization observations of the subdwarf Bal 09 are analyzed. Bal 09 belongs to the group of hybrid sdB stars, which display both short- and long-period pulsations. Explaining certain properties of Bal 09 that were previously unknown in relation to subdwarfs (variations of the amplitude of the fundamental pulsation mode, rotational splitting of line multiplets and variation of this splitting) requires invoking information about the magnetic field of the star. According to estimates made in 2010, the longitudinal component of the magnetic field of Bal 09 is 34{$\pm$}63 G. This value is significantly lower than the fields found earlier for six other hot subdwarfs. New observational data for the longitudinal magnetic field of Bal 09 was obtained on July 27, 2012, using the main stellar spectrograph of the 6-m telescope of the Special Astrophysical Observatory (SAO). The longitudinal component of the magnetic field {$<$} B z {$>$} was found via a regression analysis. When applied to the star HD 210762 with a zero total magnetic field, this method yielded the value {$<$} B z {$>$} = -12 {$\pm$} 9 G. The observations also included measurements of {$<$} B z {$>$} for the well-studied magnetic star {$\gamma$} Equ, which is used at the SAO for calibration and testing of the polarimetric instruments. The estimate obtained for {$\gamma$} Equ is {$<$} B z {$>$} = -546{$\pm$}16G, consistentwith the general variations of the longitudinal magnetic-field component of this star. This new study, based on data obtained on July 27, 2012, leads to a similar estimate of the longitudinal magnetic field, {$<$} B z {$>$} = -23{$\pm$}53 G. This estimate of {$<$} B z {$>$} was obtained for the full analyzed spectral range (4400-4958 \AA ). The corresponding "limited" solution yielded -32{$\pm$}63 G. The regression analysis for the individual spectral sub-bands and for bands containing characteristic spectral features, did not provide firm evidence of the presence of a magnetic field, with a strength exceeding the error in {$<$} B z {$>$}. The data analysis leads to the conclusion that the errors of the measurements made in 2010 and 2012 are in good agreement. This testifies to the reliability of the method applied and of the resulting observational material. In addition, the estimates are in good agreement among themselves and with estimates obtained earlier, in 2010. The results unambiguously confirm the earlier conclusion that the subdwarf Bal 09 does not have magnetic field with a strength comparable to those detected earlier for six sdB and sdO stars. Estimates of {$<$} B z {$>$} for hot subdwarfs that have appeared in the literature since the 2010 study also provide trustworthy evidence for the absence of magnetic fields {$\sim$} 1 kG in these objects.},
  annotation = {ADS Bibcode: 2013ARep...57..751S}
}

@article{sayeedSWANDATADRIVENINFERENCE2021,
  title = {{{THE SWAN}}: {{DATA-DRIVEN INFERENCE OF STELLAR SURFACE GRAVITIES FOR COOL STARS FROM PHOTOMETRIC LIGHT CURVES}}},
  author = {Sayeed, Maryum and Huber, Daniel and Wheeler, Adam and Ness, Melissa},
  year = {2021},
  eprint = {2011.10062v2},
  urldate = {2021-08-01},
  abstract = {Stellar light curves are well known to encode physical stellar properties. Precise, automated and computationally inexpensive methods to derive physical parameters from light curves are needed to cope with the large influx of these data from space-based missions such as Kepler and TESS. Here we present a new methodology which we call The Swan, a fast, generalizable and effective approach for deriving stellar surface gravity (log g) for main sequence, subgiant and red giant stars from Kepler light curves using local linear regression on the full frequency content of Kepler long cadence power spectra. With this inexpensive data-driven approach, we recover log g to a precision of {$\sim$}0.02 dex for 13,822 stars with seismic log g values between 0.2-4.4 dex, and {$\sim$}0.11 dex for 4,646 stars with Gaia derived log g values between 2.3-4.6 dex. We further develop a signal-to-noise metric and find that granulation is difficult to detect in many cool main sequence stars (T eff 5500 K), in particular K dwarfs. By combining our log g measurements with Gaia radii, we derive empirical masses for 4,646 subgiant and main sequence stars with a median precision of {$\sim$}7\%. Finally, we demonstrate that our method can be used to recover log g to a similar mean absolute deviation precision for TESS-baseline of 27 days. Our methodology can be readily applied to photometric time-series observations to infer stellar surface gravities to high precision across evolutionary states.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology-stars,data analysis,fundamental parameters-Techniques,Kepler-methods,notion,notion-database,photometric-surveys},
  file = {/Users/lbugnet/Zotero/storage/6FMMTTJ4/full-text.pdf}
}

@article{Scargle1982,
  title = {Statistical Aspects of Spectral Analysis of Unevenly Spaced Data},
  author = {Scargle, J D},
  year = {1982},
  journal = {Astrophysical Journal},
  volume = {263},
  eprint = {hep-ph/0003129v2},
  pages = {835--853},
  issn = {0004-637X},
  doi = {10.1086/160554},
  abstract = {Detection of a periodic signal hidden in noise is frequently a goal in astronomical data analysis. This paper does not introduce a new detection technique, but instead studies the reliability and efficiency of detection with the most commonly used technique, the periodogram, in the case where the observation times are unevenly spaced. This choice was made because, of the methods in current use, it appears to have the simplest statistical behavior. A modification of the classical definition of the periodogram is necessary in order to retain the simple statistical behavior of the evenly spaced case. With this modification, periodogram analysis and least-squares fitting of sine waves to the data are exactly equivalent. Certain difficulties with the use of the periodogram are less important than commonly beheved in the case of detection of strictly periodic signals. In addition, the standard method for mitigating these difficulties (tapering) can be used just as well if the sampling is uneven. An analysis of the statistical significance of signal detections is presented, with examples.},
  archiveprefix = {arxiv},
  pmid = {15003161},
  keywords = {notion,notion-database,time series analysis},
  file = {/Users/lbugnet/Zotero/storage/YLFSW99V/Scargle - 1982.pdf}
}

@techreport{Schad2020,
  title = {Inference of Solar Rotation from Perturbations of Acoustic Mode Eigenfunctions},
  author = {Schad, Ariane and Roth, Markus},
  year = {2020},
  eprint = {2002.06114v1},
  urldate = {2020-02-17},
  abstract = {Today's picture of the internal solar rotation rate profile results essentially from helio-seismic analyses of frequency splittings of resonant acoustic waves. Here we present another , complementary estimation of the internal solar rotation rate using the perturbation of the shape of the acoustic waves. For this purpose we extend a global helioseismic approach developed previously for the investigation of the meridional flow Schad et al. (2011, 2012, 2013) to work on the components of the differential rotation. We discuss the effect of rotation on mode eigenfunctions and thereon based observables. Based on a numerical study using a simulated rotation rate profile we tailor an inversion approach and also consider the case of the presence of an additional meridional flow. This inversion approach is then applied to data from the MDI (Michelson Doppler Imager aboard the Solar Heliospheric Observator (SoHO)) instrument and the HMI (Helioseismic and Magnetic Imager aboard the Solar Dynamics Observatory (SDO)) instrument. In the end, rotation rate profiles estimated from eigenfunction perturbation and frequency splittings are compared. The rotation rate profiles from the two different approaches are qualitatively in good agreement, especially for the MDI data. Significant differences are obtained at high latitudes {$>$} 50 \textbullet{} and near the subsurface. The result from HMI data shows larger discrepancies between the different methods. We find that the two global helioseismic approaches provide complementary methods for measuring the solar rotation. Comparing the results from different methods may help to reveal systematic influences that affect analyses based on eigenfunction perturbations, like meridional flow measurements.},
  archiveprefix = {arxiv},
  keywords = {data analysis,helioseismology-Sun,notion,notion-database,observation-Methods,Sun},
  file = {/Users/lbugnet/Zotero/storage/AHE8PLVB/full-text.pdf}
}

@article{Schatzman1962,
  title = {A Theory of the Role of Magnetic Activity during Star Formation},
  author = {Schatzman, E.},
  year = {1962},
  journal = {AnAp},
  volume = {25},
  pages = {18},
  issn = {0365-0499},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Scherrer1995,
  title = {The {{Solar Oscillations Investigation}} - {{Michelson Doppler Imager}}},
  author = {Scherrer, P. H. and Bogart, R. S. and Bush, R. I. and Hoeksema, J. T. and Kosovichev, A. G. and Schou, J. and Rosenberg, W. and Springer, L. and Tarbell, T. D. and Title, A. and Wolfson, C. J. and Zayer, I.},
  year = {1995},
  month = dec,
  journal = {Solar Physics},
  volume = {162},
  number = {1-2},
  pages = {129--188},
  publisher = {{Kluwer Academic Publishers}},
  issn = {00380938},
  doi = {10.1007/BF00733429},
  urldate = {2020-07-14},
  abstract = {The Solar Oscillations Investigation (SOI) uses the Michelson Doppler Imager (MDI) instrument to probe the interior of the Sun by measuring the photospheric manifestations of solar oscillations. Characteristics of the modes reveal the static and dynamic properties of the convection zone and core. Knowledge of these properties will improve our understanding of the solar cycle and of stellar evolution. Other photospheric observations will contribute to our knowledge of the solar magnetic field and surface motions. The investigation consists of coordinated efforts by several teams pursuing specific scientific objectives. The instrument images the Sun on a 10242 CCD camera through a series of increasingly narrow spectral filters. The final elements, a pair of tunable Michelson interferometers, enable MDI to record filtergrams with a FWHM bandwidth of 94 m\AA. Normally 20 images centered at 5 wavelengths near the Ni I 6768 spectral line are recorded each minute. MDI calculates velocity and continuum intensity from the filtergrams with a resolution of 4{${''}$} over the whole disk. An extensive calibration program has verified the end-to-end performance of the instrument. To provide continuous observations of the longest-lived modes that reveal the internal structure of the Sun, a carefully-selected set of spatial averages are computed and downlinked at all times. About half the time MDI will also be able to downlink complete velocity and intensity images each minute. This high rate telemetry (HRT) coverage is available for at least a continuous 60-day interval each year and for 8 hours each day during the rest of the year. During the 8-hour HRT intervals, 10 of the exposures each minute can be programmed for other observations, such as measurements in MDI's higher resolution (1.25{${''}$}) field centered about 160{${''}$} north of the equator; meanwhile, the continuous structure program proceeds during the other half minute. Several times each day, polarizers will be inserted to measure the line-of-sight magnetic field. MDI operations will be scheduled well in advance and will vary only during the daily 8-hour campaigns. Quick-look and summary data, including magnetograms, will be processed immediately. Most high-rate data will be delivered only by mail to the SOI Science Support Center (SSSC) at Stanford, where a processing pipeline will produce 3 Terabytes of calibrated data products each year. These data products will be analyzed using the SSSC and the distributed resources of the co-investigators. The data will be available for collaborative investigations. \textcopyright{} 1995 Kluwer Academic Publishers.},
  keywords = {notion,notion-database}
}

@article{Scherrer2012,
  title = {The {{Helioseismic}} and {{Magnetic Imager}} ({{HMI}}) {{Investigation}} for the {{Solar Dynamics Observatory}} ({{SDO}})},
  author = {Scherrer, P. H. and Schou, J. and Bush, R. I. and Kosovichev, A. G. and Bogart, R. S. and Hoeksema, J. T. and Liu, Y. and Duvall, T. L. and Zhao, J. and Title, A. M. and Schrijver, C. J. and Tarbell, T. D. and Tomczyk, S.},
  year = {2012},
  journal = {Solar Physics},
  volume = {275},
  number = {1-2},
  pages = {207--227},
  issn = {00380938},
  doi = {10.1007/s11207-011-9834-2},
  abstract = {The Helioseismic and Magnetic Imager (HMI) instrument and investigation as a part of the NASA Solar Dynamics Observatory (SDO) is designed to study convection-zone dynamics and the solar dynamo, the origin and evolution of sunspots, active regions, and complexes of activity, the sources and drivers of solar magnetic activity and disturbances, links between the internal processes and dynamics of the corona and heliosphere, and precursors of solar disturbances for space-weather forecasts. A brief overview of the instrument, investigation objectives, and standard data products is presented. \textcopyright{} 2011 The Author(s).},
  isbn = {1120701198},
  keywords = {Helioseismology,Instrumentation and data management,{Magnetic fields, photosphere},notion,notion-database,Solar Dynamics Observatory},
  file = {/Users/lbugnet/Zotero/storage/EDFHMGD4/Scherrer et al. - 2012.pdf}
}

@article{Scherrer2019,
  title = {A {{Critical Evaluation}} of {{Recent Claims Concerning Solar Rotation}}},
  author = {Scherrer, P. H. and Gough, D. O.},
  year = {2019},
  journal = {The Astrophysical Journal},
  volume = {877},
  number = {1},
  eprint = {1904.02820},
  pages = {42},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/ab13ad},
  abstract = {Fossat et al. (2017) recently reported detecting rotational splitting of g modes indirectly via the interaction with p modes observed directly by the GOLF instrument on SOHO. They concluded that the core of the Sun is rotating 3:8 ? 0:1 times faster than the surrounding radiative envelope. This is startling, partly because such rapid rotation almost contradicts direct inferences from the p-mode rotational splitting inferred from the same data. Moreover, the inferred amplitudes of the g modes appear to exceed the upper bound reported by Appourchaux et al. (2010). It is also suspect because the theory of the procedure implies that the principal modes claimed to have been measured should be undetectable. We point out that there are other interpretations: one leads to a core rotation about twice faster than the surrounding envelope; another, to a core rotating more slowly than the envelope. Here we also report on an independent assessment of the Fossat et al. analysis by applying their procedure to different representations of the GOLF data, expanding on Schunker et al. (2018). We also analyze seismic data obtained from LOI and MDI (both also on SOHO), from HMI (on SDO) and from the ground-based BiSON and GONG, and found the evidence reported by Fossat et al. not to be robust. We also illustrate that merely fitting model spectra to observations, which Fossat et al. do to support their g-mode detections and as Fossat \& Schmider (2018) do for extracting additional g-mode splittings, is not necessarily reliable. We are therefore led to doubt the claim.},
  archiveprefix = {arxiv},
  keywords = {helioseismology,notion,notion-database,oscillations,rotation,sun},
  file = {/Users/lbugnet/Zotero/storage/Y2IGT23Z/Scherrer, Gough - 2019.pdf}
}

@article{Schmid2016,
  title = {Asteroseismic Modelling of the Two {{F-type}} Hybrid Pulsators {{KIC 10080943A}} and {{KIC 10080943B}}},
  author = {Schmid, V. S. and Aerts, C.},
  year = {2016},
  month = aug,
  journal = {Astronomy \& Astrophysics},
  volume = {592},
  pages = {A116},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201628617},
  urldate = {2023-10-28},
  abstract = {Context. Pulsating binary stars are ideal targets for testing the theory of stellar structure and evolution. Fundamental parameters can be derived to high precision from binary modelling and provide crucial constraints for seismic modelling. High-order gravity modes are sensitive to the conditions near the convective core and therefore allow for a determination of parameters describing interior physics, especially the convective-core overshooting parameter. KIC 10080943 is a binary system that contains two gravity- and pressure-mode hybrid pulsators. A detailed observational study has provided fundamental and seismic parameters for both components. Aims: We aim to find a model that is able to predict the observed g-mode period spacings and stellar parameters of both components of KIC 10080943. Methods: By calculating model grids with the stellar evolution code MESA and the seismic code GYRE, we can compare theoretical properties to the observed mean period spacing and position in the Hertzsprung-Russell diagram. Results: The masses of our best models are somewhat below the values estimated from binarity, which is a consequence of the low observed mean g-mode period spacing. We find that the amount of core overshooting and diffusive mixing can be well constrained by the equal-age requirement for the two stars, however, we find no significant difference for different shapes of core overshooting. The measured rotation rates are within the limit of validity for the first-order perturbation approximation. We can find a good fit by using the traditional approximation for the pulsations, when taking slightly younger models with a higher asymptotic period spacing. This is because the zonal modes experience a slight shift due to the Coriolis force, which the first-order perturbation approximation ignores.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: spectroscopic,stars: evolution,stars: individual: KIC 10080943,stars: oscillations},
  annotation = {ADS Bibcode: 2016A\&A...592A.116S},
  file = {/Users/lbugnet/Zotero/storage/QUM69CWV/Schmid and Aerts - 2016 - Asteroseismic modelling of the two F-type hybrid p.pdf}
}

@article{Schmidt2001,
  title = {Studies of Magnetic and Suspected-Magnetic Southern White Dwarfs},
  author = {Schmidt, Gary D. and Vennes, Stephane and Wickramasinghe, D. T. and Ferrario, L.},
  year = {2001},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {328},
  number = {1},
  pages = {203--210},
  issn = {00358711},
  doi = {10.1046/j.1365-8711.2001.04853.x},
  abstract = {Optical spectrophotometry and circular spectropolarimetry are presented for several candidate magnetic white dwarfs that were identified during the Hamburg/ESO survey for bright quasi-stellar objects. Two objects, HE 1211-1707 and HE 1043-0502, are shown to be rare examples of white dwarfs that show neutral helium lines in a high magnetic field, in these cases {$\sim$} 50 and {$\sim$} 800 MG, respectively. The former is also found to be rotating with a period of {$\sim$}2h. HE 1045-0908 is a hydrogen-line star with a polar field strength of {$\sim$} 20 MG, spinning with a period in the range {$\sim$} 2-4 h. Attempts at modelling the limited amount of phase-resolved data that is available suggest that the field structure on this star departs substantially from a simple centred dipolar geometry. Two cool white dwarfs with unidentified broad absorption spectral features, HE 0236-2656 and HE 0330-0002, are polarimetrically confirmed to be magnetic. Line identifications for these stars are not yet possible, but the atmospheres are probably helium-rich, with spectral features formed by trace compounds of hydrogen, carbon, and perhaps other metals. HE 0003-5701 and HE 0338-3853 were proposed by Reimers et al. alongside two similar objects to be magnetic DB white dwarfs, with Zeeman-split lines of helium in magnetic fields all near 20 MG. However, our observations show that the first two, and by extension all four, are non-magnetic white dwarf + cool dwarf pairs. They deserve to be studied in their own right as possible close binaries. Finally, a lack of circular polarization suggests that HE 0000-3430 and HE 0127-3110 are also non-magnetic. HE 0000-3430 appears to be a featureless DC white dwarf over the spectral range observed here, while the sole absorption line near 5890 \AA{} in HE 0127-3110 could be either He I {$\lambda$}5876 or the Na I D doublet, but there are difficulties with either interpretation.},
  keywords = {Binaries: general,notion,notion-database,Stars: individual: HE 1043-0502,Stars: individual: HE 1211-1707,Stars: magnetic fields,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/IJ6MB2QV/Schmidt et al. - 2001.pdf}
}

@article{Schofield2019,
  title = {The {{Asteroseismic Target List}} for {{Solar-like Oscillators Observed}} in 2 Minute {{Cadence}} with the {{Transiting Exoplanet Survey Satellite}}},
  author = {Schofield, Mathew and Chaplin, William J. and Huber, Daniel and Campante, Tiago L. and Davies, Guy R. and Miglio, Andrea and Ball, Warrick H. and Appourchaux, Thierry and Basu, Sarbani and Bedding, Timothy R. and {Christensen-Dalsgaard}, J{\o}rgen and Creevey, Orlagh and Garc{\'i}a, Rafael A. and Handberg, Rasmus and Kawaler, Steven D. and Kjeldsen, Hans and Latham, David W. and Lund, Mikkel N. and Metcalfe, Travis S. and Ricker, George R. and Serenelli, Aldo and Aguirre, Victor Silva and Stello, Dennis and Vanderspek, Roland},
  year = {2019},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {241},
  number = {1},
  eprint = {1901.10148},
  pages = {12},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/ab04f5},
  abstract = {We present the target list of solar-type stars to be observed in short-cadence (2-min) for asteroseismology by the NASA Transiting Exoplanet Survey Satellite (TESS) during its 2-year nominal survey mission. The solar-like Asteroseismic Target List (ATL) is comprised of bright, cool main-sequence and subgiant stars and forms part of the larger target list of the TESS Asteroseismic Science Consortium (TASC). The ATL uses Gaia DR2 and the Extended Hipparcos Compilation (XHIP) to derive fundamental stellar properties, calculate detection probabilities and produce a rank-ordered target list. We provide a detailed description of how the ATL was produced and calculate expected yields for solar-like oscillators based on the nominal photometric performance by TESS. We also provide publicly available source code which can be used to reproduce the ATL, thereby enabling comparisons of asteroseismic results from TESS with predictions from synthetic stellar populations.},
  archiveprefix = {arxiv},
  keywords = {catalogs,funda-,instruments,notion,notion-database,oscillations,space vehicles,stars,surveys},
  file = {/Users/lbugnet/Zotero/storage/H3EC5KNL/Schofield et al. - 2019.pdf}
}

@article{Scholler2017,
  title = {B Fields in {{OB}} Stars ({{BOB}}): {{Concluding}} the {{FORS}} 2 Observing Campaign},
  shorttitle = {B Fields in {{OB}} Stars ({{BOB}})},
  author = {Sch{\"o}ller, M. and Hubrig, S. and Fossati, L. and Carroll, T. A. and Briquet, M. and Oskinova, L. M. and J{\"a}rvinen, S. and Ilyin, I. and Castro, N. and Morel, T. and Langer, N. and Przybilla, N. and Nieva, M. -F. and Kholtygin, A. F. and Sana, H. and Herrero, A. and Barb{\'a}, R. H. and {de Koter}, A. and {BOB Collaboration}},
  year = {2017},
  month = mar,
  journal = {Astronomy and Astrophysics},
  volume = {599},
  pages = {A66},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201628905},
  urldate = {2023-06-05},
  abstract = {Aims: The B fields in OB stars (BOB) Collaboration is based on an ESO Large Programme to study the occurrence rate, properties, and ultimately the origin of magnetic fields in massive stars. Methods: In the framework of this program, we carried out low-resolution spectropolarimetric observations of a large sample of massive stars using FORS 2 installed at the ESO VLT 8 m telescope. Results: We determined the magnetic field values with two completely independent reduction and analysis pipelines. Our in-depth study of the magnetic field measurements shows that differences between our two pipelines are usually well within 3{$\sigma$} errors. From the 32 observations of 28 OB stars, we were able to monitor the magnetic fields in CPD -57\textdegree{} 3509 and HD 164492C, confirm the magnetic field in HD 54879, and detect a magnetic field in CPD -62\textdegree{} 2124. We obtain a magnetic field detection rate of 6 {$\pm$} 3\% for the full sample of 69 OB stars observed with FORS 2 within the BOB program. For the preselected objects with a v sin I below 60 km s-1, we obtain a magnetic field detection rate of 5 {$\pm$} 5\%. We also discuss X-ray properties and multiplicity of the objects in our FORS 2 sample with respect to the magnetic field detections. Based on observations made with ESO Telescopes at the La Silla Paranal Observatory under program ID 191.D-0255(E,G).},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,polarization,stars: early-type,stars: magnetic field,stars: massive},
  annotation = {ADS Bibcode: 2017A\&A...599A..66S},
  file = {/Users/lbugnet/Zotero/storage/QYDTPQIJ/Schöller et al. - 2017 - B fields in OB stars (BOB) Concluding the FORS 2 .pdf}
}

@article{Schonberg1942,
  title = {On the {{Evolution}} of the {{Main-Sequence Stars}}.},
  author = {Sch{\"o}nberg, M. and Chandrasekhar, S.},
  year = {1942},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {96},
  pages = {161},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/144444},
  urldate = {2020-07-12},
  keywords = {notion,notion-database}
}

@article{Schonhut-Stasik2019,
  title = {Robo-{{AO Kepler Asteroseismic Survey}}. {{II}}. {{Do Stellar Companions Inhibit Stellar Oscillations}}?},
  author = {{Schonhut-Stasik}, Jessica and Huber, Daniel and Baranec, Christoph and Lamman, Claire and Salama, Maissa and {Jensen-Clem}, Reecca and Duev, Dmitry A. and Riddle, Reed and Kulkarni, S. R. and Law, Nicholas M.},
  year = {2019},
  eprint = {1910.03803},
  abstract = {The Kepler space telescope observed over 15,000 stars for asteroseismic studies. Of these, 75\% of dwarfs (and 8\% of giants) were found to show anomalous behavior: such as suppressed oscillations (low amplitude) or no oscillations at all. The lack of solar-like oscillations may be a consequence of multiplicity, due to physical interactions with spectroscopic companions or due to the dilution of oscillation amplitudes from "wide'" (AO detected; visual) or spectroscopic companions introducing contaminating flux. We present a search for stellar companions to 327 of the Kepler asteroseismic sample, which were expected to display solar-like oscillations. We used direct imaging with Robo-AO, which can resolve secondary sources at \textasciitilde 0."15, and followed up detected companions with Keck AO. Directly imaged companion systems with both separations of \$\textbackslash leq\$0."5 and amplitude dilutions {$>$}10\% all have anomalous primaries, suggesting these oscillation signals are diluted by a sufficient amount of excess flux. We also used the high-resolution spectrometer ESPaDOnS at CFHT to search for spectroscopic binaries. We find tentative evidence for a higher fraction of spectroscopic binaries with high radial velocity scatter in anomalous systems, which would be consistent with previous results suggesting that oscillations are suppressed by tidal interactions in close eclipsing binaries.},
  archiveprefix = {arxiv},
  keywords = {adaptive optics - techniques,binaries,data analysis - methods,fun-,high angular res-,notion,notion-database,observational - asteroseismology -,olution - methods,spectroscopic - instrumentation,stars},
  file = {/Users/lbugnet/Zotero/storage/A5KZBKGW/Schonhut-Stasik et al. - 2019.pdf}
}

@article{Schroder2007,
  title = {A Critical Test of Empirical Mass Loss Formulae Applied to Individual Giants and Supergiants},
  author = {Schroder, Klaus-Peter and Cuntz, Manfred},
  year = {2007},
  month = feb,
  journal = {Astronomy and Astrophysics},
  volume = {465},
  number = {2},
  eprint = {astro-ph/0702172},
  pages = {593--601},
  doi = {10.1051/0004-6361:20066633},
  urldate = {2020-07-02},
  abstract = {To test our new, improved Reimers-type mass-loss relation, given by Schroder \& Cuntz in 2005 (ApJL 630, L73), we take a look at the best studied galactic giants and supergiants - particularly those with spatially resolved circumstellar shells and winds, obtained directly or by means of a companion acting as a probing light source. Together with well-known physical parameters, the selected stars provide the most powerful and critical observational venues for assessing the validity of parameterized mass-loss relations for cool winds not driven by molecules or dust. In this study, star by star, we compare our previously published relation with the original Reimers relation (1975), the Lamers relation (1981), and the two relations by de Jager and his group (1988, 1990). The input data, especially the stellar masses, have been constrained using detailed stellar evolution models. We find that only the relationship by Schroder \& Cuntz agrees, within the error bars, with the observed mass-loss rates for all giants and supergiants.},
  archiveprefix = {arxiv},
  keywords = {Methods: statistical,notion,notion-database,Stars: general,Stars: late-type,Stars: mass-loss,{Stars: winds, outflows}},
  file = {/Users/lbugnet/Zotero/storage/VI3K3EA9/full-text.pdf}
}

@article{Schroder2013,
  title = {What Do the {{Mt}}. {{Wilson}} Stars Tell Us about Solar Activity?},
  author = {Schr{\"o}der, K. P. and Mittag, M. and Hempelmann, A. and {Gonz{\'a}lez-P{\'e}rez}, J. N. and Schmitt, J. H.M.M.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {554},
  pages = {1--7},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219830},
  abstract = {We relate the evolutionary status and mass of the Mt. Wilson project stars with the type and strength of stellar activity as established in decades of monitoring their chromospheric Ca II K line emission. We specifically derive their positions in the Hertzsprung-Russell-diagram (HRD) from Hipparcos parallaxes and SIMBAD B - V data, considering and correcting for the effects of different individual stellar metallicities, and place different activity groups of the Mt. Wilson stars on a common set of Z = 0.02 evolution tracks to obtain a quantitative picture of their relative evolutionary status and mass distribution. We find that, first, the downturn in stellar activity does not depend on absolute age but instead decreases with the relative age as stars advance on the main sequence and thus confirm theoretical expectations, while the most active of the irregularly variable stars are found to scatter around the zero-age main-sequence (ZAMS). Moderately active stars, both with clear cycles like the Sun and those without a dominant activity period, populate the 2nd quarter of main-sequence (MS) evolution. Almost inactive stars are mostly in their 3rd quarter of MS evolution and seem to represent stellar analogues of the solar Maunder minimum state. Totally inactive stars are all in the final quarter of their MS evolution and make up for over 70\% of the Mt. Wilson stars that far evolved (the remainders being only weakly active). Most of these are more massive and younger than the Sun. Accordingly, less massive stars did not have enough time to significantly decrease their activity, since they generally evolve more slowly. We find, second, that the Sun is near an apparent upper mass limit for cyclic activity on the MS, because there are no cyclic MS stars much above one solar mass, at least not in the Mt. Wilson sample. Once put in proper perspective with the other Mt. Wilson stars, the Sun indeed ought to be approaching a gradual transition from moderate cyclic activity to a weak, Maunder-minimum-type state, as historic Maunder-type minima seem to indicate already. In addition, the apparent upper mass limit for MS stars to solar-like cyclic activity, not much above one solar mass, is providing dynamo theory with an interesting new challenge. \textcopyright{} 2013 ESO.},
  keywords = {notion,notion-database,Stars: activity,Stars: chromospheres,Stars: evolution,Stars: solar-type,Sun: activity,Sun: chromosphere},
  file = {/Users/lbugnet/Zotero/storage/XWWTCCUS/Schröder et al. - 2013.pdf}
}

@article{Schuh2006,
  title = {Exciting New Features in the Frequency Spectrum of the {{EC}} 14026 Star {{HS}} 0702+6043. {{Simultaneous}} g-Modes and p-Modes in a {{sdB}} Pulsator},
  author = {Schuh, S. and Huber, J. and Dreizler, S. and Green, E. M. and Stahn, T. and Randall, S. and Husser, T. -O. and Heber, U. and O'Toole, S. and Fontaine, G.},
  year = {2006},
  month = jan,
  journal = {Memorie della Societa Astronomica Italiana},
  volume = {77},
  pages = {480},
  issn = {0037-8720},
  doi = {10.48550/arXiv.astro-ph/0510832},
  urldate = {2023-10-09},
  abstract = {The discovery of a long-period g-mode oscillation in the previously known short-period p-mode sdB pulsator HS 0702+6043 makes this star an extraordinary object, unique as a member of the family of sdB pulsators, and one of the very few known pulsating stars overall exhibiting excited modes along both the acoustic and gravity branches of the nonradial pulsation spectrum. Because p-modes and g-modes probe different regions of a pulsating star, HS 0702+6043 holds a tremendous potential for asteroseismological investigations. We present preliminary results from the first extended campaign on this object.},
  keywords = {Astrophysics,stars: individual: HS 0702+6043,stars: oscillations,stars: subdwarfs},
  annotation = {ADS Bibcode: 2006MmSAI..77..480S},
  file = {/Users/lbugnet/Zotero/storage/FFT3SD6T/Schuh et al. - 2006 - Exciting new features in the frequency spectrum of.pdf}
}

@article{Schunker2011a,
  title = {Constructing and {{Characterising Solar Structure Models}} for {{Computational Helioseismology}}},
  author = {Schunker, H. and Cameron, R. H. and Gizon, L. and Moradi, H.},
  year = {2011},
  journal = {Solar Physics},
  volume = {271},
  number = {1},
  pages = {1--26},
  issn = {00380938},
  doi = {10.1007/s11207-011-9790-x},
  abstract = {In local helioseismology, numerical simulations of wave propagation are useful to model the interaction of solar waves with perturbations to a background solar model. However, the solution to the linearised equations of motion include convective modes that can swamp the helioseismic waves that we are interested in. In this article, we construct background solar models that are stable against convection, by modifying the vertical pressure gradient of Model S (Christensen-Dalsgaard et al., 1996, Science272, 1286) relinquishing hydrostatic equilibrium. However, the stabilisation affects the eigenmodes that we wish to remain as close to Model S as possible. In a bid to recover the Model S eigenmodes, we choose to make additional corrections to the sound speed of Model S before stabilisation. No stabilised model can be perfectly solar-like, so we present three stabilised models with slightly different eigenmodes. The models are appropriate to study the f and p1 to p4 modes with spherical harmonic degrees in the range from 400 to 900. Background model CSM has a modified pressure gradient for stabilisation and has eigenfrequencies within 2\% of Model S. Model CSM\_A has an additional 10\% increase in sound speed in the top 1 Mm resulting in eigenfrequencies within 2\% of Model S and eigenfunctions that are, in comparison with CSM, closest to those of Model S. Model CSM\_B has a 3\% decrease in sound speed in the top 5 Mm resulting in eigenfrequencies within 1\% of Model S and eigenfunctions that are only marginally adversely affected. These models are useful to study the interaction of solar waves with embedded three-dimensional heterogeneities, such as convective flows and model sunspots. We have also calculated the response of the stabilised models to excitation by random near-surface sources, using simulations of the propagation of linear waves. We find that the simulated power spectra of wave motion are in good agreement with an observed SOHO/MDI power spectrum. Overall, our convectively stabilised background models provide a good basis for quantitative numerical local helioseismology. The models are available for download from http://www.mps.mpg.de/projects/seismo/NA4/. \textcopyright{} 2011 The Author(s).},
  keywords = {Helioseismology,notion,notion-database,Numerical methods,Solar models},
  file = {/Users/lbugnet/Zotero/storage/RKWDR86P/Schunker et al. - 2011.pdf}
}

@article{Schunker2018,
  title = {Fragile {{Detection}} of {{Solar}} g -{{Modes}} by {{Fossat}} et Al},
  author = {Schunker, Hannah and Schou, Jesper and Gaulme, Patrick and Gizon, Laurent},
  year = {2018},
  month = jun,
  journal = {Solar Physics},
  volume = {293},
  number = {6},
  eprint = {1804.04407},
  pages = {95},
  publisher = {{Springer Netherlands}},
  issn = {1573093X},
  doi = {10.1007/s11207-018-1313-6},
  urldate = {2020-07-29},
  abstract = {The internal gravity modes of the Sun are notoriously difficult to detect, and the claimed detection of gravity modes presented by Fossat et~al. (Astron. Astrophys.604, A40, 2017) is thus very exciting. Given the importance of these modes for understanding solar structure and dynamics, the results must be robust. While Fossat et al. described their method and parameter choices in detail, the sensitivity of their results to several parameters was not presented. Therefore, we test the sensitivity of the results to a selection of the parameters. The most concerning result is that the detection vanishes when we adjust the start time of the 16.5-year velocity time-series by a few hours. We conclude that this reported detection of gravity modes is extremely fragile and should be treated with utmost caution.},
  archiveprefix = {arxiv},
  keywords = {{Helioseismology, observations},Interior,notion,notion-database,Oscillations},
  file = {/Users/lbugnet/Zotero/storage/492W87ML/full-text.pdf}
}

@article{Schussler1996,
  title = {Distribution of Starspots on Cool Stars},
  author = {Sch{\"u}ssler, M. and Caligari, P. and {Ferriz-Mas}, A. and Solanki, S.K and Stix, M.},
  year = {1996},
  journal = {A\&A},
  volume = {314},
  pages = {503--513},
  urldate = {2020-05-14},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ASDTNFEC/full-text.pdf}
}

@article{Schwarzschild1975,
  title = {{{ON THE SCALE OF PHOTOSPHERIC CONVECTION IN RED GIANTS AND SUPERGIANTS}}},
  author = {Schwarzschild, Martin},
  year = {1975},
  journal = {The Astrophysical Journal},
  volume = {195},
  pages = {137--144},
  urldate = {2020-03-13},
  abstract = {An attempt is made to estimate the sizes of the convective elements which dominate the brightness variations on the photospheres of red giants and supergiants. The data assembled permit the extreme hypothesis that these dominant convective elements are so large that only a modest number of them exists at any one time on the entire surface of such a star-in contrast with two million granules on the Sun.},
  keywords = {Astronomical Models,Astrophysics,convection-interiors,Convective Flow,Gas Ionization,Giant Stars,Late Stars,notion,notion-database,Photosphere,Solar Granulation,Stellar Mass Ejection,Stellar Winds,stellar-late-type stars,Subject headings,Supergiant Stars},
  file = {/Users/lbugnet/Zotero/storage/WRUXHP7L/full-text.pdf}
}

@article{schweitzerCARMENESSearchExoplanets2019,
  title = {The {{CARMENES}} Search for Exoplanets around {{M}} Dwarfs {{Different}} Roads to Radii and Masses of the Target Stars},
  author = {Schweitzer, A and Passegger, V M and Cifuentes, C and B{\'e}jar, V J S and {Cort{\'e}s-Contreras}, M and Caballero, J A and Del Burgo, C and Czesla, S and K{\"u}rster, M and Montes, D and Zapatero Osorio, M R and Ribas, I and Reiners, A and Quirrenbach, A and Amado, P J and Aceituno, J and {Anglada-Escud{\'e}}, G and Bauer, F F and Dreizler, S and Jeffers, S V and Guenther, E W and Henning, T and Kaminski, A and Lafarga, M and Marfil, E and Morales, J C and Schmitt, J H M M and Seifert, W and Solano, E and Tabernero, H M and Zechmeister, M},
  year = {2019},
  journal = {A\&A},
  volume = {625},
  pages = {68},
  doi = {10.1051/0004-6361/201834965},
  urldate = {2021-08-02},
  abstract = {Aims. We determine the radii and masses of 293 nearby, bright M dwarfs of the CARMENES survey. This is the first time that such a large and homogeneous high-resolution (R {$>$} 80 000) spectroscopic survey has been used to derive these fundamental stellar parameters. Methods. We derived the radii using Stefan-Boltzmann's law. We obtained the required effective temperatures T eff from a spectral analysis and we obtained the required luminosities L from integrated broadband photometry together with the Gaia DR2 parallaxes. The mass was then determined using a mass-radius relation that we derived from eclipsing binaries known in the literature. We compared this method with three other methods: (1) We calculated the mass from the radius and the surface gravity log g, which was obtained from the same spectral analysis as T eff. (2) We used a widely used infrared mass-magnitude relation. (3) We used a Bayesian approach to infer stellar parameters from the comparison of the absolute magnitudes and colors of our targets with evolutionary models. Results. Between spectral types M0 V and M7 V our radii cover the range 0.1 R {$<$} R {$<$} 0.6 R with an error of 2-3\% and our masses cover 0.09 M {$<$} M {$<$} 0.6 M with an error of 3-5\%. We find good agreement between the masses determined with these different methods for most of our targets. Only the masses of very young objects show discrepancies. This can be well explained with the assumptions that we used for our methods.},
  keywords = {fundamental parameters-stars,general,late-type-stars,low-mass-stars,notion,notion-database,stars}
}

@article{scienceEstec,
  title = {Estec},
  author = {Science, Plato and Team, Working},
  pages = {1--53},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WAIBLTEJ/PTO-EST-SCI-RS-0150_SciRD_7_0.pdf}
}

@article{Sciences2017,
  title = {Verlinde ' s New Theory of Gravity Passes First Test {{Verlinde}} ' s New Theory of Gravity Passes First Test},
  author = {Sciences, Other},
  year = {2017},
  journal = {27 Janeiro, 2019},
  volume = {236},
  eprint = {1905.02730},
  pages = {1--21},
  doi = {10.1093/mnras},
  urldate = {2020-07-02},
  abstract = {A quest\~ao de qu\~ao rapidamente o Universo est\'a a expandir-se tem intrigado os astr\'onomos h\'a quase um s\'eculo. Estudos diferentes continuam a obter novas respostas \textendash{} o que faz com que alguns investigadores se perguntem se est\~ao a negligenciar um mecanismo-chave na ``maquinaria'' que impulsiona o cosmos.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,Convective Heat Transfer,Dynamo Theory,Magnetic Field Configurations,notion,notion-database,Peculiar Stars,Stellar Evolution,Stellar Magnetic Fields,Stellar Models,Stellar Structure}
}

@article{Scornet2015,
  title = {{{CONSISTENCY OF RANDOM FORESTS}} 1},
  author = {Scornet, Erwan and Biau, G{\'e}rard and Vert, Jean-Philippe},
  year = {2015},
  journal = {The Annals of Statistics},
  volume = {43},
  number = {4},
  eprint = {1405.2881v4},
  pages = {1716--1741},
  doi = {10.1214/15-AOS1321},
  urldate = {2020-03-23},
  abstract = {Random forests are a learning algorithm proposed by Breiman [Mach. Learn. 45 (2001) 5-32] that combines several randomized decision trees and aggregates their predictions by averaging. Despite its wide usage and outstanding practical performance, little is known about the mathematical properties of the procedure. This disparity between theory and practice originates in the difficulty to simultaneously analyze both the randomization process and the highly data-dependent tree structure. In the present paper, we take a step forward in forest exploration by proving a consistency result for Breiman's [Mach. Learn. 45 (2001) 5-32] original algorithm in the context of additive regression models. Our analysis also sheds an interesting light on how random forests can nicely adapt to sparsity.},
  archiveprefix = {arxiv},
  keywords = {62G05,62G20,additive model,consistency,dimension reduction,notion,notion-database,Random forests,randomization,sparsity}
}

@article{Seach2020,
  title = {A {{Magnetic Snapshot Survey}} of {{F-Type Stars}}},
  author = {Seach, J M and Marsden, S C and Carter, B D and Neiner, C and Folsom, C P and Mengel, M W and Oksala, M E and Buysschaert, B},
  year = {2020},
  month = apr,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {494},
  number = {4},
  pages = {5682--5703},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/staa1107},
  urldate = {2020-11-29},
  abstract = {We present a spectropolarimetric magnetic snapshot survey of 55 stars which includes 53 F-type stars ranging from spectral types F0 to F9 plus 2 chemically peculiar stars {$\beta$} CrB, and {$\delta$} Cap. We look for magnetic fields in stars spanning a range of effective temperatures where the transition from fossil to dynamo magnetic fields is believed to occur. High-resolution spectropolarimetry using circularly polarized spectra is used to look for a magnetic detection in the Stokes V profile, determine the mean longitudinal magnetic field (Bl), and to look for correlations with stellar parameters. Surface magnetic fields are detected on 14 F-stars, and present in every spectral class from F3V-F9V ranging in strength from 0.3 {$\pm$} 0.1 G (36 UMa, F8V) to 8.3 {$\pm$} 0.9 G (h Dra, F8V). Thus we find photospheric magnetic fields are present in stars as early as spectral type F3V with an outer convection zone thickness less than a few per cent of the stellar radius.},
  keywords = {notion,notion-database,stars: early,stars: late,stars: magnetic field,type}
}

@article{Seager2003,
  title = {A {{Unique Solution}} of {{Planet}} and {{Star Parameters}} from an {{Extrasolar Planet Transit Light Curve}}},
  author = {Seager, S. and Mallen-Ornelas, G.},
  year = {2003},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {585},
  number = {2},
  eprint = {astro-ph/0206228},
  pages = {1038--1055},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/346105},
  urldate = {2020-07-07},
  abstract = {There is a unique solution of the planet and star parameters from a planet transit light curve with two or more transits if the planet has a circular orbit and the light curve is observed in a band pass where limb darkening is negligible. The existence of this unique solution is very useful for current planet transit surveys for several reasons. First, there is an analytic solution that allows a quick parameter estimate, in particular of Rp. Second, the stellar density can be uniquely derived from the transit light curve alone. The stellar density can be used to immediately rule out a giant star (and hence a much larger than planetary companion) and can also be used to put an upper limit on the stellar and planet radius even considering slightly evolved stars. Third, the presence of an additional fully blended star that contaminates an eclipsing system to mimic a planet transit can be largely ruled out from the transit light curve given a spectral type for the central star. Fourth, the period can be estimated from a single-transit light curve and a measured spectral type. All of these applications can be used to select the best planet transit candidates for mass determination by radial velocity follow-up. To use these applications in practice, the photometric precision and time sampling of the light curve must be high (better than 0.005 mag precision and 5 minute time sampling).},
  archiveprefix = {arxiv},
  keywords = {binaries,eclipsing-planetary systems-techniques,notion,notion-database,photometric,Subject headings},
  file = {/Users/lbugnet/Zotero/storage/4B2TFPKP/full-text.pdf}
}

@article{See2017,
  title = {Studying Stellar Spin-down with {{Zeeman-Doppler}} Magnetograms},
  author = {See, V. and Jardine, M. and Vidotto, A. A. and Donati, J. F. and Saikia, S. Boro and Fares, R. and Folsom, C. P. and H{\'e}brard, E. M. and Jeffers, S. V. and Marsden, S. C. and Morin, J. and Petit, P. and Waite, I. A.},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {466},
  number = {2},
  eprint = {1705.01835},
  pages = {1542--1554},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stw3094},
  urldate = {2020-07-13},
  abstract = {Magnetic activity and rotation are known to be intimately linked for low-mass stars. Understanding rotation evolution over the stellar lifetime is therefore an important goal within stellar astrophysics. In recent years, there has been increased focus on how the complexity of the stellar magnetic field affects the rate of angular-momentum loss from a star. This is a topic that Zeeman-Doppler imaging (ZDI), a technique that is capable of reconstructing the large-scale magnetic field topology of a star, can uniquely address. Using a potential field source surface model, we estimate the open flux, mass-loss rate and angular-momentum-loss rates for a sample of 66 stars that have been mapped with ZDI.We show that the open flux of a star is predominantly determined by the dipolar component of its magnetic field for our choice of source surface radius. We also show that, on the main sequence, the open flux, mass-loss and angular-momentum-loss rates increase with decreasing Rossby number. The exception to this rule is stars less massive than 0.3M{$\odot$}. Previous work suggests that low-mass M dwarfs may possess either strong, ordered and dipolar fields or weak and complex fields. This range of field strengths results in a large spread of angular-momentum-loss rates for these stars and has important consequences for their spin-down behaviour. Additionally, our models do not predict a transition in the mass-loss rates at the so-called wind-dividing line noted from Ly{$\alpha$} studies.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: activity,Stars: evolution,Stars: magnetic field,Stars: rotation,Techniques: polarimetric},
  file = {/Users/lbugnet/Zotero/storage/T9JC277M/full-text.pdf}
}

@article{Semel1989,
  title = {Zeeman-{{Doppler}} Imaging of Active Stars. {{I}} - {{Basic}} Principles.},
  author = {Semel, M.},
  year = {1989},
  journal = {A\&A},
  volume = {225},
  pages = {456--466},
  issn = {0004-6361},
  urldate = {2020-07-02},
  keywords = {Astrophysics,Computational Astrophysics,Doppler Effect,Fourier Transformation,Integral Equations,Magnetic Field Configurations,notion,notion-database,Polarimetry,Stellar Activity,Stellar Rotation,Stellar Spectra,Zeeman Effect}
}

@article{Serenelli2017,
  title = {The {{First APOKASC Catalog}} of {{Kepler Dwarf}} and {{Subgiant Stars}}},
  author = {Serenelli, Aldo and Johnson, Jennifer and Huber, Daniel and Pinsonneault, Marc and Ball, Warrick H. and Tayar, Jamie and Aguirre, Victor Silva and Basu, Sarbani and Troup, Nicholas and Hekker, Saskia and Kallinger, Thomas and Stello, Dennis and Davies, Guy R. and Lund, Mikkel N. and Mathur, Savita and Mosser, Benoit and Stassun, Keivan G. and Chaplin, William J. and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Handberg, Rasmus and Holtzman, Jon and Hearty, Fred and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Gaulme, Patrick and Zamora, Olga},
  year = {2017},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {233},
  number = {2},
  eprint = {1710.06858},
  pages = {23},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/aa97df},
  abstract = {(Abridged) We present the first APOKASC catalog of spectroscopic and asteroseismic data for 415 dwarfs and subgiants. Asteroseismic data have been obtained by Kepler in short cadence. The spectroscopic parameters are based on spectra taken as part of APOGEE and correspond to DR13 of SDSS. We analyze our data using two Teff scales, the spectroscopic values from DR13 and those derived from SDSS griz photometry. We use the differences in our results arising from these choices as a test of systematic Teff, and find that they can lead to significant differences in the derived stellar properties. Determinations of surface gravity (\$\textbackslash log\{g\}\$), mean density (\$\textbackslash rho\$), radius (\$R\$), mass (\$M\$), and age (\$\textbackslash tau\$) for the whole sample have been carried out with stellar grid-based modeling. We have assessed random and systematic error sources in the spectroscopic and seismic data, as well as in the grid-based modeling determination of the stellar quantities in the catalog. We provide stellar properties for both Teff scales. The median combined (random and systematic) uncertainties are 2\% (0.01 dex; \$\textbackslash log\{g\}\$), 3.4\% (\$\textbackslash rho\$), 2.6\% (\$R\$), 5.1\% (\$M\$), and 19\% (\$\textbackslash tau\$) for the photometric Teff scale and 2\% (\$\textbackslash log\{g\}\$), 3.5\% (\$\textbackslash rho\$), 2.7\% (\$R\$), 6.3\% (\$M\$), and 23\% (\$\textbackslash tau\$) for the spectroscopic scale. Comparisons with stellar quantities in the catalog by Chaplin et al.(2014) highlight the importance of metallicity measurements for determining stellar parameters accurately. We compare our results with those from other sources, including stellar radii determined from TGAS parallaxes and asteroseismic analyses based on individual frequencies. We find a very good agreement in all cases. Comparisons give strong support to the determination of stellar quantities based on global seismology, a relevant result for future missions such as TESS and PLATO. Table 5 corrected (wrongly listed SDSS Teff before).},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9NB4H78E/Serenelli et al. - 2017.pdf}
}

@article{serrano-InstrumentSignalNoise,
  title = {Instrument {{Signal}} and {{Noise Budget}}},
  author = {{Serrano-}, Dimitri and Cabrera, Juan},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZTJDR6GB/PLATO-DLR-PL-RP-0001_i4.0_Instrument-Signal-and-Noise-Budget.pdf}
}

@article{Shafranov1966,
  title = {Plasma {{Equilibrium}} in a {{Magnetic Field}}},
  author = {Shafranov, V. D. and D., V.},
  year = {1966},
  journal = {RvPP},
  volume = {2},
  pages = {103},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Shapiro2013,
  title = {The Place of the {{Sun}} among the {{Sun-like}} Stars},
  author = {Shapiro, A. I. and Schmutz, W. and Cessateur, G. and Rozanov, E.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {552},
  pages = {1--8},
  issn = {00046361},
  doi = {10.1051/0004-6361/201220512},
  abstract = {Context. Monitoring of the photometric and chromospheric HK emission data series of stars similar to the Sun in age and average activity level showed that there is an empirical correlation between the average stellar chromospheric activity level and the photometric variability. In general, more active stars show larger photometric variability. Interestingly, the measurements and reconstructions of the solar irradiance show that the Sun is significantly less variable than indicated by the empirical relationship. Aims. We aim to identify possible reasons for the Sun to be currently outside of this relationship. Methods. We employed different scenarios of solar HK emission and irradiance variability and compared them with available time series of Sun-like stars. Results. We show that the position of the Sun on the diagram of photometric variability versus chromospheric activity changes with time. The present solar position is different from its temporal mean position as the satellite era of continuous solar irradiance measurements has accidentally coincided with a period of unusually high and stable solar activity. Our analysis suggests that although present solar variability is significantly smaller than indicated by the stellar data, the temporal mean solar variability might be in agreement with the stellar data. We propose that the continuation of the photometric program and its expansion to a larger stellar sample will ultimately allow us to constrain the historical solar variability. \textcopyright{} 2013 ESO.},
  keywords = {notion,notion-database,Stars: activity,Stars: solar-type,Stars: variables: general,Sun: activity,Sun: atmosphere},
  file = {/Users/lbugnet/Zotero/storage/XYNUH9TW/Shapiro et al. - 2013.pdf}
}

@article{Shapiro2014,
  title = {Variability of {{Sun-like}} Stars: {{Reproducing}} Observed Photometric Trends},
  author = {Shapiro, A. I. and Solanki, S. K. and Krivova, N. A. and Schmutz, W. K. and Ball, W. T. and Knaack, R. and Rozanov, E. V. and Unruh, Y. C.},
  year = {2014},
  journal = {Astronomy and Astrophysics},
  volume = {569},
  eprint = {1406.2383},
  issn = {14320746},
  doi = {10.1051/0004-6361/201323086},
  abstract = {Context. The Sun and stars with low magnetic activity levels become photometrically brighter when their activity increases. Magnetically more active stars display the opposite behavior and become fainter when their activity increases. Aims. We reproduce the observed photometric trends in stellar variations with a model thattreats stars as hypothetical suns with coverage by magnetic features different from that of the Sun. Methods. The model attributes the variability of stellar spectra to the imbalance between the contributions from different components of the solar atmosphere, such as dark starspots and bright faculae. A stellar spectrum is calculated from spectra of the individual components by weighting them with corresponding disk-area coverages. The latter are obtained by extrapolating the solar dependences of spot and facular disk-area coverages on chromospheric activity to stars with different levels of mean chromospheric activity. Results. We find that the contribution by starspots to the variability increases faster with chromospheric activity than the facular contribution. This causes the transition from faculae-dominated variability and direct activity-brightness correlation to spot-dominated variability and inverse activity-brightness correlation with increasing chromospheric activity level. We show that the regime of the variability also depends on the angle between the stellar rotation axis and the line-of-sight and on the latitudinal distribution of active regions on the stellar surface. Our model can be used as a tool for extrapolating the observed photometric variability of the Sun to Sun-like stars at different activity levels, which makes a direct comparison between solar and stellar irradiance data possible.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Solar-terrestrial relations,Stars: activity,Stars: solar-type,Stars: variables: general,Sun: activity,Sun: atmosphere},
  file = {/Users/lbugnet/Zotero/storage/JZRNXQDB/Shapiro et al. - 2014.pdf}
}

@article{Shapiro2016,
  title = {Are Solar Brightness Variations Faculae- or Spot-Dominated?},
  author = {Shapiro, A. I. and Solanki, S. K. and Krivova, N. A. and Yeo, K. L. and Schmutz, W. K.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {589},
  eprint = {1602.04447},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527527},
  abstract = {Context. Regular spaceborne measurements have revealed that solar brightness varies on multiple timescales, variations on timescales greater than a day being attributed to a surface magnetic field. Independently, ground-based and spaceborne measurements suggest that Sun-like stars show a similar, but significantly broader pattern of photometric variability. Aims. To understand whether the broader pattern of stellar variations is consistent with the solar paradigm, we assess relative contributions of faculae and spots to solar magnetically-driven brightness variability. We investigate how the solar brightness variability and its facular and spot contributions depend on the wavelength, timescale of variability, and position of the observer relative to the ecliptic plane. Methods. We performed calculations with the SATIRE model, which returns solar brightness with daily cadence from solar disc area coverages of various magnetic features. We took coverages as seen by an Earth-based observer from full-disc SoHO/MDI and SDO/HMI data and projected them to mimic out-of-ecliptic viewing by an appropriate transformation. Results. Moving the observer away from the ecliptic plane increases the amplitude of 11-year variability as it would be seen in Str\"omgren (b + y)/2 photometry, but decreases the amplitude of the rotational brightness variations as it would appear in Kepler and CoRoT passbands. The spot and facular contributions to the 11-year solar variability in the Str\"omgren (b + y)/2 photometry almost fully compensate each other so that the Sun appears anomalously quiet with respect to its stellar cohort. Such a compensation does not occur on the rotational timescale. Conclusions. The rotational solar brightness variability as it would appear in the Kepler and CoRoT passbands from the ecliptic plane is spot-dominated, but the relative contribution of faculae increases for out-of-ecliptic viewing so that the apparent brightness variations are faculae-dominated for inclinations less than about i = 45\textdegree. Over the course of the 11-year activity cycle, the solar brightness variability is faculae-dominated shortwards of 1.2 {$\mu$}m independently of the inclination.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: solar-type,Stars: variables: general,Starspots,Sun: activity,{Sun: faculae, plages}},
  file = {/Users/lbugnet/Zotero/storage/JKLCMPTQ/Shapiro et al. - 2016.pdf}
}

@article{Sharma2011,
  title = {Galaxia: {{A}} Code to Generate a Synthetic Survey of the {{Milky}} Way},
  author = {Sharma, Sanjib and {Bland-Hawthorn}, Joss and Johnston, Kathryn V. and Binney, James},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {730},
  number = {1},
  eprint = {1101.3561},
  issn = {15384357},
  doi = {10.1088/0004-637X/730/1/3},
  abstract = {We present here a fast code for creating a synthetic survey of the Milky Way. Given one or more color-magnitude bounds, a survey size, and geometry, the code returns a catalog of stars in accordance with a given model of the Milky Way. The model can be specified by a set of density distributions or as an N-body realization. We provide fast and efficient algorithms for sampling both types of models. As compared to earlier sampling schemes which generate stars at specified locations along a line of sight, our scheme can generate a continuous and smooth distribution of stars over any given volume. The code is quite general and flexible and can accept input in the form of a star formation rate, age-metallicity relation, age-velocity-dispersion relation, and analytic density distribution functions. Theoretical isochrones are then used to generate a catalog of stars, and support is available for a wide range of photometric bands. As a concrete example, we implement the Besan\c{c}on Milky Way model for the disk. For the stellar halo we employ the simulated stellar halo N-body models of Bullock \& Johnston. In order to sample N-body models, we present a scheme that disperses the stars spawned by an N-body particle, in such a way that the phase-space density of the spawned stars is consistent with that of the N-body particles. The code is ideally suited to generating synthetic data sets that mimic near future wide area surveys such as GAIA, LSST, and HERMES. As an application we study the prospect of identifying structures in the stellar halo with a simulated GAIA survey. We plan to make the code publicly available. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: stellar content,Galaxy: structure,methods: data analysis,methods: numerical,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/85VDHIME/Sharma et al. - 2011.pdf}
}

@article{Sharma2016a,
  title = {Stellar {{Population Synthesis Based Modeling}} of the {{Milky Way Using Asteroseismology}} of 13,000 {{Kepler Red Giants}}},
  author = {Sharma, Sanjib and Stello, Dennis and {Bland-Hawthorn}, Joss and Huber, Daniel and Bedding, Timothy R.},
  year = {2016},
  journal = {The Astrophysical Journal},
  volume = {822},
  number = {1},
  eprint = {1603.05661},
  pages = {15},
  issn = {1538-4357},
  doi = {10.3847/0004-637x/822/1/15},
  abstract = {With current space-based missions it is now possible to obtain age-sensitive asteroseismic information for tens of thousands of red giants. This provides a promising opportunity to study the Galactic structure and evolution. We use asteroseismic data of red giants, observed by Kepler, to test the current theoretical framework of modelling the Galaxy based on population synthesis modeling and the use of asteroseismic scaling relations for giants. We use the open source code Galaxia to model the Milky Way and find the distribution of the masses predicted by Galaxia to be systematically offset with respect to the seismically-inferred observed masses. The Galactic model overestimates the number of low mass stars, and these stars are predominantly old and of low metallicity. Using corrections to the \$\textbackslash Delta \textbackslash nu\$ scaling relation suggested by stellar models (available for download) significantly reduces the disagreement between predicted and observed masses. For a few cases where non-seismic mass estimates are available, the corrections to \$\textbackslash Delta \textbackslash nu\$ also improve the agreement between seismic and non-seismic mass estimates. The disagreement between predictions of the Galactic model and the observations is most pronounced for stars with \$\{\textbackslash rm [Fe/H]\}{$<$}-0.5\$ and \$\{\textbackslash rm [Fe/H]\}{$>$}0\$ or for \$T\_\{\textbackslash rm eff\}{$>$}4700\$ K. Altering the star formation rate in order to suppress stars older than 10 Gyr improves the agreement for mass but leads to inconsistent color distributions. We also tested the predictions of the TRILEGAL Galactic model. However, unlike \{\textbackslash sl Galaxia\}, it had difficulties in reproducing the photometric properties of the Kepler Input Catalog because it overestimates the number of blue stars. We conclude that either the scaling relations and/or the Galactic models need to be revised to reconcile predictions of theory with asteroseismic observations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/LG2K4LEM/Sharma et al. - 2016.pdf}
}

@article{sharmaTESSHERMESSurveyData2004,
  title = {The {{TESS-HERMES}} Survey Data Release 1: High-Resolution Spectroscopy of the {{TESS}} Southern Continuous Viewing Zone},
  author = {Sharma, Sanjib and Stello, Dennis and Buder, Sven and Kos, Janez and {Bland-Hawthorn}, Joss and Asplund, Martin and Duong, Ly and Lin, Jane and Lind, Karin and Ness, Melissa and Huber, Daniel and Zwitter, Tomaz and Traven, Gregor and Hon, Marc and Kafle, Prajwal R and Khanna, Shourya and Saddon, Hafiz and Anguiano, Borja and Casey, Andrew R and Freeman, Ken and Martell, Sarah and De Silva, Gayandhi M and Simpson, Jeffrey D and Wittenmyer, Rob A and Zucker, Daniel B},
  year = {2004},
  journal = {MNRAS},
  volume = {473},
  doi = {10.1093/mnras/stx2582},
  urldate = {2021-08-12},
  keywords = {notion,notion-database}
}

@misc{shenarWolfRayetStarsRecent2022,
  title = {Wolf-{{Rayet}} Stars: Recent Advances and Persisting Problems},
  shorttitle = {Wolf-{{Rayet}} Stars},
  author = {Shenar, Tomer},
  year = {2022},
  month = aug,
  number = {arXiv:2208.02614},
  eprint = {2208.02614},
  primaryclass = {astro-ph},
  institution = {{arXiv}},
  urldate = {2022-08-08},
  abstract = {Wolf-Rayet (WR) stars comprise a class of stars whose spectra are dominated by strong, broad emission lines that are associated with copious mass loss. In the massive-star regime, roughly 90\% of the known WR stars are thought to have evolved off the main sequence. Dubbed classical WR (cWR) stars, these hydrogen-depleted objects represent a crucial evolutionary phase preceding core collapse into black holes, and offer a unique window into hot-star wind physics. Their formation is thought to be rooted in either intrinsic mass-loss or binary interactions. Results obtained from analyses using contemporary model atmospheres still fail to reconcile the derived properties of WR stars with predictions from stellar evolution. Importantly, stellar evolution models cannot reproduce the the bulk of cWR stars, a problem that becomes especially severe at subsolar metallicity. Next-generation model atmospheres and upcoming observational campaigns to hunt for undetected companions promise a venue for progress.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/84E6N4HW/Shenar - 2022 - Wolf-Rayet stars recent advances and persisting p.pdf;/Users/lbugnet/Zotero/storage/NAG5PMZG/2208.html}
}

@book{shewhartIntroductionProbabilityStatistics2000,
  title = {An {{Introduction}} to {{Probability}} and {{Statistics}}},
  author = {Shewhart, Walter A and Wilks, Samuel S and Cressie, Noel A C and Fisher, Nicholas I and Johnstone, Iain M and Kadane, J B and Scott, David W and Silverman, Bernard W and Smith, Adrian F M and Teugels, Jozefl and Barnett, Vic and Bradley, Ralph A and Hunter, J Stuart and Kendall, David G},
  year = {2000},
  month = sep,
  publisher = {{John Wiley \& Sons, Inc.}},
  address = {{Hoboken, NJ, USA}},
  doi = {10.1002/9781118165676},
  urldate = {2021-11-29},
  abstract = {A complete list of the titles in this series appears at the end of this volume.},
  isbn = {978-1-118-16567-6},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZS4SLMXS/full-text.pdf}
}

@article{Shi2023,
  title = {A {{Catalog}} of {{New Slowly Pulsating B-type Stars}}},
  author = {Shi, Xiang-dong and Qian, Sheng-bang and Zhu, Li-ying and Li, Lin-jia},
  year = {2023},
  month = sep,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {268},
  pages = {16},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/ace88c},
  urldate = {2023-10-17},
  abstract = {This paper reports the discovery of new slowly pulsating B-type stars. Based on the photometric, spectral, and astrometric data of the TESS, LAMOST, and Gaia surveys, we have found 286 new slowly pulsating B-type (SPB) stars and 21 candidates. Among these, 20 are Be stars or candidates with emission-line profiles. It is shown that these SPB stars have luminosities between 40 and 2850 L {$\odot$} and effective temperatures ranging from 10,000 to 21,000 K. Their pulsation periods are from 0.14 to 6.5 days with amplitude ranges of 0.2-20 mmag in the TESS band. It is indicated that these targets follow the distribution of the SPB stars in the period-luminosity and the period-temperature diagrams. Their positions on the H-R diagram reveal that most of these pulsators are distributed in the instability region of SPB stars, in the main-sequence evolutionary stage, and with mass ranges of 2.5-7 M {$\odot$}. However, there are some targets beyond the red edge of the theoretical instability region, which should be caused by the rapid rotation reducing the measured effective temperature. The discovery of these new SPB stars increases the total number by over 60\%, which are significant samples for further investigating the structure and evolution of intermediate-mass and even massive stars by asteroseismology.},
  keywords = {1307,732,Massive stars,Pulsating variable stars},
  annotation = {ADS Bibcode: 2023ApJS..268...16S},
  file = {/Users/lbugnet/Zotero/storage/4GDH974A/Shi et al. - 2023 - A Catalog of New Slowly Pulsating B-type Stars.pdf}
}

@article{Shibahashi1976,
  title = {Overstability of {{Gravity Modes}} in {{Massive Stars}} with the {{Semiconvective Zone}}},
  author = {Shibahashi, H. and Osaki, Y.},
  year = {1976},
  journal = {PASJ},
  volume = {28},
  pages = {199--214},
  issn = {0004-6264},
  urldate = {2020-06-26},
  keywords = {notion,notion-database}
}

@article{Shibahashi1979,
  title = {Modal {{Analysis}} of {{Stellar Nonradial Oscillations}} by an {{Asymptotic Method}}},
  author = {Shibahashi, H.},
  year = {1979},
  journal = {PASJ},
  volume = {31},
  pages = {87--104},
  issn = {0004-6264},
  urldate = {2020-06-26},
  keywords = {notion,notion-database}
}

@article{Shibahashi2000,
  title = {Asteroseismology and {{Oblique Pulsator Model}} of {{Beta Cephei}}},
  author = {Shibahashi, H. and Aerts, C.},
  year = {2000},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {531},
  number = {2},
  eprint = {astro-ph/0001372},
  pages = {L143-L146},
  publisher = {{IOP Publishing}},
  doi = {10.1086/312533},
  urldate = {2020-06-29},
  abstract = {We discuss the oscillation features of Beta Cephei, which is a magnetic star in which the magnetic axis seems to be oblique to the rotation axis. We interpret the observed equi-distant fine structures of the frequency spectrum as a manifestation of a magnetic perturbation of an eigenmode, which would be a radial mode in the absence of the magnetic field. Besides these frequency components, we interpret another peak in the frequency spectrum as an independent quadrupole mode. By this mode identification, we deduce the mass, the evolutionary stage, the rotational frequency, the magnetic field strength, and the geometrical configuration of Beta Cephei.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,STARS: EARLY,STARS: INDIVIDUAL: CONSTELLATION NAME: {$\beta$} CEPHEI,STARS: MAGNETIC FIELDS,STARS: OSCILLATIONS,STARS: ROTATION,TYPE},
  file = {/Users/lbugnet/Zotero/storage/465YJ599/full-text.pdf}
}

@article{Shine2000,
  title = {Supergranule and {{Mesogranule Evolution}}},
  author = {Shine, R.A. and Simon, G.W. and Hurlburt, N.E.},
  year = {2000},
  journal = {Solar Physics},
  volume = {193},
  number = {1/2},
  pages = {313--331},
  issn = {00380938},
  doi = {10.1023/A:1005207625696},
  urldate = {2020-03-14},
  keywords = {notion,notion-database}
}

@article{Shiode2013,
  title = {The Observational Signatures of Convectively Excited Gravity Modes in Main-Sequence Stars},
  author = {Shiode, Joshua H. and Quataert, Eliot and Cantiello, Matteo and Bildsten, Lars},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {430},
  number = {3},
  eprint = {1210.5525},
  pages = {1736--1745},
  issn = {00358711},
  doi = {10.1093/mnras/sts719},
  abstract = {We predict the flux and surface velocity perturbations produced by convectively excited gravity modes (g-modes) in main-sequence stars. Core convection in massive stars can excite g-modes to sufficient amplitudes to be detectable with high-precision photometry by Kepler and Convection, Rotation and planetary Transits (CoRoT), if the thickness of the convective overshoot region is {$\lessequivlnt$}30 per cent of a pressure scale height. The g-modes manifest as excess photometric variability, with amplitudes of \textasciitilde 10 {$\mu$}mag at frequencies {$\lessequivlnt$}10 {$\mu$}Hz (0.8 d-1) near the solar metallicity zero-age main sequence. The flux variations are largest for stars with M {$\greaterequivlnt$} 5M{$\odot$}, but are potentially detectable down to M \textasciitilde{} 2-3M{$\odot$}. During the main-sequence evolution, radiative damping decreases such that ever lower frequency modes reach the stellar surface and flux perturbations reach up to \textasciitilde 100 {$\mu$}mag at the terminal-age main sequence. Using the same convective excitation model, we confirm previous predictions that solar gmodes produce surface velocity perturbations of{$\lessequivlnt$}0.3mm s-1. This implies that stochastically excited g-modes are more easily detectable in the photometry of massive main-sequence stars than in the Sun. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Convection,notion,notion-database,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/77DLXYVL/Shiode et al. - 2013.pdf}
}

@article{Shultz2019,
  title = {The Magnetic Early {{B-type}} Stars \textendash{} {{III}}. {{A}} Main-Sequence Magnetic, Rotational, and Magnetospheric Biography},
  author = {Shultz, M. E. and Wade, G. A. and Rivinius, T. and Alecian, E. and Neiner, C. and Petit, V. and Owocki, S. and {Ud-Doula}, A. and Kochukhov, O. and Bohlender, D. and Keszthelyi, Z.},
  year = {2019},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {490},
  number = {1},
  eprint = {1909.02530},
  pages = {274--295},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stz2551},
  urldate = {2021-01-03},
  abstract = {Magnetic confinement of stellar winds leads to the formation of magnetospheres, which can be sculpted into centrifugal magnetospheres (CMs) by rotational support of the corotating plasma. The conditions required for the CMs of magnetic early B-type stars to yield detectable emission in H {$\alpha$} \textendash{} the principal diagnostic of these structures \textendash{} are poorly constrained. A key reason is that no detailed study of the magnetic and rotational evolution of this population has yet been performed. Using newly determined rotational periods, modern magnetic measurements, and atmospheric parameters determined via spectroscopic modelling, we have derived fundamental parameters, dipolar oblique rotator models, and magnetospheric parameters for 56 early B-type stars. Comparison to magnetic A- and O-type stars shows that the range of surface magnetic field strength is essentially constant with stellar mass, but that the unsigned surface magnetic flux increases with mass. Both the surface magnetic dipole strength and the total magnetic flux decrease with stellar age, with the rate of flux decay apparently increasing with stellar mass. We find tentative evidence that multipolar magnetic fields may decay more rapidly than dipoles. Rotational periods increase with stellar age, as expected for a magnetic braking scenario. Without exception, all stars with H {$\alpha$} emission originating in a CM are (1) rapid rotators, (2) strongly magnetic, and (3) young, with the latter property consistent with the observation that magnetic fields and rotation both decrease over time.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: chemically peculiar,Stars: early-type,Stars: evolution,Stars: magnetic field,Stars: massive,Stars: rotation}
}

@article{Siegel2010,
  title = {Excitation of Non-Radial Stellar Oscillations by Gravitational Waves: {{A}} First Model},
  author = {Siegel, D. M. and Roth, M.},
  year = {2010},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {408},
  number = {3},
  eprint = {1103.0373},
  pages = {1742--1748},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2010.17240.x},
  abstract = {The excitation of solar and solar-like g modes in non-relativistic stars by arbitrary external gravitational wave fields is studied starting from the full field equations of general relativity. We develop a formalism that yields the mean-square amplitudes and surface velocities of global normal modes excited in such a way. The isotropic elastic sphere model of a star is adopted to demonstrate this formalism and for calculative simplicity. It is shown that gravitational waves solely couple to quadrupolar spheroidal eigenmodes and that normal modes are only sensitive to the spherical component of the gravitational waves having the same azimuthal order. The mean-square amplitudes in case of stationary external gravitational waves are given by a simple expression, a product of a factor depending on the resonant properties of the star and the power spectral density of the gravitational waves' spherical accelerations. Both mean-square amplitudes and surface velocities show a characteristic R8-dependence (effective R2-dependence) on the radius of the star. This finding increases the relevance of this excitation mechanism in case of stars larger than the Sun. \textcopyright{} 2010 The Authors. Journal compilation \textcopyright{} 2010 RAS.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Gravitation,Gravitational waves,notion,notion-database,Stars: oscillations,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/29TJ3BCH/Siegel, Roth - 2010(2).pdf;/Users/lbugnet/Zotero/storage/QBYBZ4C3/Siegel, Roth - 2010.pdf}
}

@article{Siess2000,
  title = {An Internet Server for Pre-Main Sequence Tracks of Low- and Intermediate-Mass Stars},
  author = {Siess, L. and Dufour, E. and Forestini, M.},
  year = {2000},
  journal = {Astronomy and Astrophysics},
  volume = {358},
  number = {2},
  eprint = {astro-ph/0003477},
  pages = {593--599},
  issn = {00046361},
  urldate = {2020-07-13},
  abstract = {We present new grids of pre-main sequence (PMS) tracks for stars in the mass range 0.1 to 7.0 M{$\odot$}. The computations were performed for four different metallicities (Z=0.01,0.02,0.03 and 0.04). A fifth table has been computed for the solar composition (Z=0.02), including a moderate overshooting. We describe the update in the physics of the Grenoble stellar evolution code which concerns mostly changes in the equation of state (EOS) adopting the formalism proposed by Pols et al. (1995) and in the treatment of the boundary condition. Comparisons of our models with other grids demonstrate the validity of this EOS in the domain of very low-mass stars. Finally, we present a new server dedicated to PMS stellar evolution which allows the determination of stellar parameters from observational data, the calculation of isochrones, the retrieval of evolutionary files and the possibility to generate graphic outputs.},
  archiveprefix = {arxiv},
  keywords = {Astronomical data bases: miscellaneous,Equation of state,notion,notion-database,Stars: evolution,Stars: Hertzsprung-Russel (HR) and C-M diagrams,Stars: pre-main sequence}
}

@article{Sills2000a,
  title = {Rotation of {{Horizontal}}-{{Branch Stars}} in {{Globular Clusters}}},
  author = {Sills, Alison and Pinsonneault, M. H.},
  year = {2000},
  journal = {The Astrophysical Journal},
  volume = {540},
  number = {1},
  pages = {489--503},
  issn = {0004-637X},
  doi = {10.1086/309306},
  abstract = {The rotation of horizontal-branch stars places important constraints on angular momentum evolution in evolved stars and therefore on rotational mixing on the giant branch. Prompted by new observations of rotation rates of horizontal-branch stars, we calculate simple models for the angular momentum evolution of a globular cluster giant star from the base of the giant branch to the star's appearance on the horizontal branch. We include mass loss and infer the accompanied loss of angular momentum for each of four assumptions about the internal angular momentum profile. Mass loss is found to have important implications for angular momentum evolution. These models are compared to observations of horizontal-branch rotation rates in M13. We find that rapid rotation on the horizontal branch can be reconciled with slow solid body main-sequence rotation if giant-branch stars have differential rotation in their convective envelopes and a rapidly rotating core, which is then followed by a redistribution of angular momentum on the horizontal branch. We discuss the physical reasons that these very different properties relative to the solar case may exist in giants. Rapid rotation in the core of the main-sequence precursors of the rapidly rotating horizontal-branch star or an angular momentum source on the giant branch is required for all cases if the rotational velocity of turnoff stars is less than 4 km s-1. We suggest that the observed range in rotation rates on the horizontal branch is caused by internal angular momentum redistribution, which occurs on a timescale comparable to the evolution of the stars on the horizontal branch. The apparent lack of rapid horizontal-branch rotators hotter than 12,000 K in M13 could be a consequence of gravitational settling, which inhibits internal angular momentum transport. Alternative explanations and observational tests are discussed.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/X4IPPAGR/Sills, Pinsonneault - 2000.pdf}
}

@article{SilvaAguirre2011,
  title = {Constraining Mixing Processes in Stellar Cores Using Asteroseismology},
  author = {Silva Aguirre, V. and Ballot, J. and Serenelli, A. M. and Weiss, A.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {529},
  pages = {1--13},
  issn = {00046361},
  doi = {10.1051/0004-6361/201015847},
  abstract = {Context. The overall evolution of low-mass stars is heavily influenced by the processes occurring in the stellar interior. In particular, mixing processes in convectively unstable zones and overshooting regions affect the resulting observables and main sequence lifetime. Aims. We aim to study the effects of different convective boundary definitions and mixing prescriptions in convective cores of low-mass stars and to distinguish the existence, size, and evolutionary stage of the central mixed zone by means of asteroseismology. Methods. We implemented the Ledoux criterion for convection in our stellar evolution code, together with a time-dependent diffusive approach for mixing of elements when semiconvective zones are present. We compared models with masses ranging from 1.1 M{$\odot$} to 2 M{$\odot$} computed with two different criteria for convective boundary definition and included different mixing prescriptions within and beyond the formal limits of the convective regions. Using calculations of adiabatic oscillations frequencies for a large set of models, we developed an asteroseismic diagnosis using only l = 0 and l = 1 modes based on the ratios of small to large separations r01 and r10 defined by Roxburgh \& Vorontsov (2003, A\&A, 411, 215). We analyzed the sensitivity of this seismic tool to the central conditions of the star during the main sequence evolution. Results. The seismic variables r 01 and r10 are almost linear in the expected observable frequency range, and we show that their slope depends simultaneously on the central hydrogen content, the extent of the convective core, and the amplitude of the sound-speed discontinuity at the core boundary. By considering about 25 modes and an accuracy in the frequency determinations as expected from the CoRoT and Kepler missions, the technique we propose allows us to detect the presence of a convective core and to discriminate the different sizes of the homogeneously mixed central region without the need for a strong prior knowledge on the stellar mass. \textcopyright{} 2011 ESO.},
  keywords = {Asteroseismology,Convection,notion,notion-database,Stars: evolution,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/BFDG5PBV/Silva Aguirre et al. - 2011.pdf}
}

@article{SilvaAguirre2011b,
  title = {Constructing a One-Solar-Mass Evolutionary Sequence Using Asteroseismic Data from {{Kepler}}},
  author = {Silva Aguirre, V. and Chaplin, W. J. and Ballot, J. and Basu, S. and Bedding, T. R. and Serenelli, A. M. and Verner, G. A. and Miglio, A. and Monteiro, M. J.P.F.G. and Weiss, A. and Appourchaux, T. and Bonanno, A. and Broomhall, A. M. and Bruntt, H. and Campante, T. L. and Casagrande, L. and Corsaro, E. and Elsworth, Y. and Garc{\'i}a, R. A. and Gaulme, P. and Handberg, R. and Hekker, S. and Huber, D. and Karoff, C. and Mathur, S. and Mosser, B. and Salabert, D. and Sch{\"o}nrich, R. and Sousa, S. G. and Stello, D. and White, T. R. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kawaler, S. D. and Kjeldsen, H. and Houdek, G. and Metcalfe, T. S. and {Molenda-Akowicz}, J. and Thompson, M. J. and Caldwell, D. A. and Christiansen, J. L. and Wohler, B.},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {740},
  number = {1},
  issn = {20418205},
  doi = {10.1088/2041-8205/740/1/L2},
  abstract = {Asteroseismology of solar-type stars has entered a new era of large surveys with the success of the NASA Kepler mission, which is providing exquisite data on oscillations of stars across the Hertzsprung-Russell diagram. From the time-series photometry, the two seismic parameters that can be most readily extracted are the large frequency separation ({$\Delta\nu$}) and the frequency of maximum oscillation power ({$\nu$}max). After the survey phase, these quantities are available for hundreds of solar-type stars. By scaling from solar values, we use these two asteroseismic observables to identify for the first time an evolutionary sequence of 1 M {$\infty$} field stars, without the need for further information from stellar models. Comparison of our determinations with the few available spectroscopic results shows an excellent level of agreement. We discuss the potential of the method for differential analysis throughout the main-sequence evolution and the possibility of detecting twins of very well-known stars. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  keywords = {asteroseismology,notion,notion-database,stars: evolution,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/ULAWDXK4/Silva Aguirre et al. - 2011(2).pdf}
}

@article{SilvaAguirre2012a,
  title = {Verifying Asteroseismically Determined Parameters of {{Kepler}} Stars Using {{Hipparcos}} Parallaxes: {{Self-consistent}} Stellar Properties and Distances},
  author = {Silva Aguirre, V. and Casagrande, L. and Basu, S. and Campante, T. L. and Chaplin, W. J. and Huber, D. and Miglio, A. and Serenelli, A. M. and Ballot, J. and Bedding, T. R. and {Christensen-Dalsgaard}, J. and Creevey, O. L. and Elsworth, Y. and Garc{\'i}a, R. A. and Gilliland, R. L. and Hekker, S. and Kjeldsen, H. and Mathur, S. and Metcalfe, T. S. and Monteiro, M. J.P.F.G. and Mosser, B. and Pinsonneault, M. H. and Stello, D. and Weiss, A. and Tenenbaum, P. and Twicken, J. D. and Uddin, K.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {757},
  number = {1},
  issn = {15384357},
  doi = {10.1088/0004-637X/757/1/99},
  abstract = {Accurately determining the properties of stars is of prime importance for characterizing stellar populations in our Galaxy. The field of asteroseismology has been thought to be particularly successful in such an endeavor for stars in different evolutionary stages. However, to fully exploit its potential, robust methods for estimating stellar parameters are required and independent verification of the results is mandatory. With this purpose, we present a new technique to obtain stellar properties by coupling asteroseismic analysis with the InfraRed Flux Method. By using two global seismic observables and multi-band photometry, the technique allows us to obtain masses, radii, effective temperatures, bolometric fluxes, and hence distances for field stars in a self-consistent manner. We apply our method to 22 solar-like oscillators in the Kepler short-cadence sample, that have accurate Hipparcos parallaxes. Our distance determinations agree to better than 5\%, while measurements of spectroscopic effective temperatures and interferometric radii also validate our results. We briefly discuss the potential of our technique for stellar population analysis and models of Galactic Chemical Evolution. \textcopyright{} 2012. The American Astronomical Society. All rights reserved.},
  keywords = {asteroseismology,notion,notion-database,parallaxes,stars: distances,stars: fundamental parameters,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/HLVNZITY/Silva Aguirre et al. - 2012.pdf}
}

@article{SilvaAguirre2013,
  title = {Determining Distances Using Asteroseismic Methods},
  author = {Silva Aguirre, V. and Casagrande, L. and Basu, S. and Campante, T. L. and Chaplin, W. J. and Huber, D. and Miglio, A. and Serenelli, A. M.},
  year = {2013},
  journal = {Astronomische Nachrichten},
  volume = {334},
  number = {1-2},
  eprint = {1210.7343},
  pages = {22--25},
  issn = {00046337},
  doi = {10.1002/asna.201211774},
  abstract = {Asteroseismology has been extremely successful in determining the properties of stars in different evolutionary stages with a remarkable level of precision. However, to fully exploit its potential, robust methods for estimating stellar parameters are required and independent verification of the results is needed. In this talk, I present a new technique developed to obtain stellar properties by coupling asteroseismic analysis with the infrared flux method. Using two global seismic observables and multi-band photometry, the technique determines masses, radii, effective temperatures, bolometric fluxes, and thus distances for field stars in a self-consistent manner. Applying our method to a sample of solar-like oscillators in the Kepler field that have accurate Hipparcos parallaxes, we find agreement in our distance determinations to better than 5 \%. Comparison with measurements of spectroscopic effective temperatures and interferometric radii also validate our results, and show that our technique can be applied to stars evolved beyond the main-sequence phase. \textcopyright{} 2013 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: distances,Stars: fundamental parameters,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/MZIHUHYV/Silva Aguirre et al. - 2013.pdf}
}

@article{SilvaAguirre2013a,
  title = {Stellar Ages and Convective Cores in Field Main-Sequence Stars: {{First}} Asteroseismic Application to Two Kepler Targets},
  author = {Silva Aguirre, V. and Basu, S. and Brand{\~a}o, I. M. and {Christensen-Dalsgaard}, J. and Deheuvels, S. and Do{\v g}an, G. and Metcalfe, T. S. and Serenelli, A. M. and Ballot, J. and Chaplin, W. J. and Cunha, M. S. and Weiss, A. and Appourchaux, T. and Casagrande, L. and Cassisi, S. and Creevey, O. L. and Garc{\'i}a, R. A. and Lebreton, Y. and Noels, A. and Sousa, S. G. and Stello, D. and White, T. R. and Kawaler, S. D. and Kjeldsen, H.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {769},
  number = {2},
  issn = {15384357},
  doi = {10.1088/0004-637X/769/2/141},
  abstract = {Using asteroseismic data and stellar evolution models we obtain the first detection of a convective core in a Kepler field main-sequence star, putting a stringent constraint on the total size of the mixed zone and showing that extra mixing beyond the formal convective boundary exists. In a slightly less massive target the presence of a convective core cannot be conclusively discarded, and thus its remaining main-sequence lifetime is uncertain. Our results reveal that best-fit models found solely by matching individual frequencies of oscillations corrected for surface effects do not always properly reproduce frequency combinations. Moreover, slightly different criteria to define what the best-fit model is can lead to solutions with similar global properties but very different interior structures. We argue that the use of frequency ratios is a more reliable way to obtain accurate stellar parameters, and show that our analysis in field main-sequence stars can yield an overall precision of 1.5\%, 4\%, and 10\% in radius, mass, and age, respectively. We compare our results with those obtained from global oscillation properties, and discuss the possible sources of uncertainties in asteroseismic stellar modeling where further studies are still needed. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  keywords = {asteroseismology,notion,notion-database,stars: fundamental parameters,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/JIB4JQ74/Silva Aguirre et al. - 2013(2).pdf}
}

@article{SilvaAguirre2015,
  title = {Ages and Fundamental Properties of {{Kepler}} Exoplanet Host Stars from Asteroseismology},
  author = {Silva Aguirre, V. and Davies, G. R. and Basu, S. and {Christensen-Dalsgaard}, J. and Creevey, O. and Metcalfe, T. S. and Bedding, T. R. and Casagrande, L. and Handberg, R. and Lund, M. N. and Nissen, P. E. and Chaplin, W. J. and Huber, D. and Serenelli, A. M. and Stello, D. and Van Eylen, V. and Campante, T. L. and Elsworth, Y. and Gilliland, R. L. and Hekker, S. and Karoff, C. and Kawaler, S. D. and Kjeldsen, H. and Lundkvist, M. S.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {452},
  number = {2},
  eprint = {1504.07992},
  pages = {2127--2148},
  issn = {13652966},
  doi = {10.1093/mnras/stv1388},
  abstract = {We present a study of 33 Kepler planet-candidate host stars for which asteroseismic observations have sufficiently high signal-to-noise ratio to allow extraction of individual pulsation frequencies. We implement a new Bayesian scheme that is flexible in its input to process individual oscillation frequencies, combinations of them, and average asteroseismic parameters, and derive robust fundamental properties for these targets. Applying this scheme to grids of evolutionary models yields stellar properties with median statistical uncertainties of 1.2 per cent (radius), 1.7 per cent (density), 3.3 per cent (mass), 4.4 per cent (distance), and 14 per cent (age), making this the exoplanet host-star sample with the most precise and uniformly determined fundamental parameters to date. We assess the systematics from changes in the solar abundances and mixing-length parameter, showing that they are smaller than the statistical errors.We also determine the stellar propertieswith three other fitting algorithms and explore the systematics arising from using different evolution and pulsation codes, resulting in 1 per cent in density and radius, and 2 per cent and 7 per cent in mass and age, respectively. We confirm previous findings of the initial helium abundance being a source of systematics comparable to our statistical uncertainties, and discuss future prospects for constraining this parameter by combining asteroseismology and data from space missions. Finally, we compare our derived properties with those obtained using the global average asteroseismic observables along with effective temperature and metallicity, finding excellent level of agreement. Owing to selection effects, our results show that the majority of the high signal-to-noise ratio asteroseismic Kepler host stars are older than the Sun.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Planetary systems,Planets and satellites: fundamental parameters,Stars: evolution,Stars: fundamental parameters,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/5VQ8K4GG/Silva Aguirre et al. - 2015.pdf}
}

@article{Simoniello2008,
  title = {Reliability of {{P}} Mode Event Classification Using Contemporaneous {{BiSON}} and {{GOLF}} Observations},
  author = {Simoniello, R. and Chaplin, W. J. and Elsworth, Y. P. and Garc{\'i}a, R. A.},
  year = {2008},
  journal = {Journal of Physics: Conference Series},
  volume = {118},
  number = {1},
  eprint = {0808.1668},
  issn = {17426596},
  doi = {10.1088/1742-6596/118/1/012088},
  abstract = {We carried out a comparison of the signals seen in contemporaneous BiSON and GOLF data sets. Both instruments perform Doppler shift velocity measurements in integrated sunlight, although BiSON perform measurements from the two wings of potassium absorption line and GOLF from one wing of the NaD1 line. Discrepancies between the two datasets have been observed. We show,in fact, that the relative power depends on the wing in which GOLF data observes. During the blue wing period, the relative power is mugh higher than in BiSON datasets, while a good agreement has been observed during the red period. \textcopyright{} 2008 IOP Publishing Ltd.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NLIIXBB3/Simoniello et al. - 2008.pdf}
}

@article{Simoniello2008a,
  title = {P-Mode Power Variation with Solar Atmosphere as Observed in the {{NaD1}} and {{K}} Spectral Lines},
  author = {Simoniello, R. and {Jim{\'e}nez-Reyes}, S. J. and Garc{\'i}a, R. A. and Pall{\'e}, P. L.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  pages = {494--497},
  issn = {00046337},
  doi = {10.1002/asna.200710983},
  abstract = {In this work we investigate p-mode power variation with solar atmosphere. To this aim, we use TH\'EMIS observations of the NaD1 ({$\lambda$}5896 \AA ) and K ({$\lambda$}7699 \AA ) spectral lines. While the formation heights of the K spectral line are essentially located in the photospheric layer, the formation heights of the NaD1 line span a much wider region: from photosphere up to chromosphere. Hence, we had the opportunity to infer p-mode power variation up to the chromospheric layer. By analyzing power spectra obtained by temporal series at different points of the Na D1 and K spectral lines, we confirm and quantify the increase in p-mode power towards higher atmospheric layers. Furthermore, the large span in formation heights of the NaD1 line induces a larger enhancement of p-mode power with solar atmosphere compared to the K spectral line. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {notion,notion-database,Sun: atmosphere,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/649P62GZ/Simoniello et al. - 2008(2).pdf}
}

@article{Simoniello2010,
  title = {Acoustic Power Absorption and Enhancement Generated by Slow and Fast {{MHD}} Waves: {{Evidence}} of Solar Cycle Velocity/Intensity Amplitude Changes Consistent with the Mode Conversion Theory},
  author = {Simoniello, R. and Finsterle, W. and Garc{\'i}a, R. A. and Salabert, D. and Jim{\'e}nez, A. and Elsworth, Y. and Schunker, H.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {516},
  number = {18},
  pages = {1--10},
  issn = {14320746},
  doi = {10.1051/0004-6361/200913091},
  abstract = {We used long duration, high quality, unresolved (Sun-as-a star) observations collected by the ground based network BiSON and by the instruments GOLF and VIRGO on board the ESA/NASA SOHO satellite to search for solar-cycle-related changes in mode characteristics in velocity and continuum intensity for the frequency range between 2.5 mHz {$<\backslash$}nu{$<$}6.8 mHz. Over the ascending phase of solar cycle 23 we found a suppression in the p-mode amplitudes both in the velocity and intensity data between 2.5 mHz lt;\textbackslash nu{$<$} 4.5 mHz with a maximum suppression for frequencies in the range between 2.5 mHz {$<\backslash$}nu{$<$} 3.5 mHz. The size of the amplitude suppression is 13 {$\pm$} 2 per cent for the velocity and 9 {$\pm$} 2 per cent for the intensity observations. Over the range of 4.5 mHz {$<\backslash$}nu{$<$}5.5 mHz the findings hint within the errors to a null change both in the velocity and intensity amplitudes. At still higher frequencies, in the so called High-frequency Interference Peaks (HIPs) between 5.8 mHz {$<\backslash$}nu{$<$}6.8 mHz, we found an enhancement in the velocity amplitudes with the maximum 36 {$\pm$} 7 per cent occurring for 6.3 mHz {$<\backslash$}nu{$<$} 6.8 mHz. However, in intensity observations we found a rather smaller enhancement of about 5 {$\pm$} 2 per cent in the same interval. There is evidence that the frequency dependence of solar-cycle velocity amplitude changes is consistent with the theory behind the mode conversion of acoustic waves in a non-vertical magnetic field, but there are some problems with the intensity data, which may be due to the height in the solar atmosphere at which the VIRGO data are taken. \textcopyright{} 2010 ESO.},
  keywords = {methods: data analysis,methods: observational,notion,notion-database,Sun: oscillation,Sun: surface magnetism},
  file = {/Users/lbugnet/Zotero/storage/32R6V8A2/Simoniello et al. - 2010.pdf}
}

@article{Simoniello2012,
  title = {The Quasi-Biennial Periodicity ({{QBP}}) in Velocity and Intensity Helioseismic Observations: {{The}} Seismic {{QBP}} over Solar Cycle 23},
  author = {Simoniello, R. and Finsterle, W. and Salabert, D. and Garc{\'i}a, R. A. and {Turck-Chi{\`e}ze}, S. and Jim{\'e}nez, A. and Roth, M.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {539},
  pages = {1--9},
  issn = {00046361},
  doi = {10.1051/0004-6361/201118057},
  abstract = {Aims. We looked for signatures of quasi-biennial periodicity (QBP) over diff erent phases of solar cycle by means of acoustic modes of oscillation. Low-degree p-mode frequencies are shown to be sensitive to changes in magnetic activity due to the global dynamo. Recently there has been reported evidence of two-year variations in p-mode frequencies. Methods. Long high-quality helioseismic data are provided by BiSON (Birmingham Solar Oscillation Network), GONG (Global Oscillation Network Group), GOLF (Global Oscillation at Low Frequency) and VIRGO (Variability of Solar IRradiance and Gravity Oscillation) instruments. We determined the solar cycle changes in p-mode frequencies for spherical degree t = 0, 1, 2 with their azimuthal components in the frequency range 2.5 mHz {$\leq$} v {$\leq$} 3. 5mHz. Results. We found signatures of QBP at all levels of solar activity in the modes more sensitive tohigher latitudes. The signal strength increases with latitude and the equatorial component also seems to be modulated by the 11-year envelope. Conclusions. The persistent nature of the seismic QBP is not observed in the surface activity indices, where mid-term variations are found only from time to time and mainly in periods of high activity. This feature, together with the latitudinal dependence, provides more evidence of a mechanism that is almost independent and diff erent from the one that brings the active regions up to the surface. Therefore, these findings can be used to provide more constraints on dynamo models that consider a further cyclic component on top of the 11-year cycle. \textcopyright{} ESO 2012.},
  keywords = {Methods: data analysis,notion,notion-database,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/UB7SRV4S/Simoniello et al. - 2012.pdf}
}

@article{Simoniello2013,
  title = {The Quasi-Biennial Periodicity as a Window on the Solar Magnetic Dynamo Configuration},
  author = {Simoniello, R. and Jain, K. and Tripathy, S. C. and {Turck-Chi{\`e}ze}, S. and Baldner, C. and Finsterle, W. and Hill, F. and Roth, M.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {765},
  number = {2},
  eprint = {1210.6796},
  issn = {15384357},
  doi = {10.1088/0004-637X/765/2/100},
  abstract = {Manifestations of the solar magnetic activity through periodicities of about 11 and 2 years are now clearly seen in all solar activity indices. In this paper, we add information about the mechanism driving the 2-year period by studying the time and latitudinal properties of acoustic modes that are sensitive probes of the subsurface layers. We use almost 17 years of high-quality resolved data provided by the Global Oscillation Network Group to investigate the solar cycle changes in p-mode frequencies for spherical degrees {$\mathscr{l}$} from 0 to 120 and 1600 {$\mu$}Hz {$\leq\nu$} {$\leq$} 3500 {$\mu$}Hz. For both periodic components of solar activity, we locate the origin of the frequency shift in the subsurface layers and find evidence that a sudden enhancement in amplitude occurs in just the last few hundred kilometers. We also show that, in both cases, the size of the shift increases toward equatorial latitudes and from minimum to maximum solar activity, but, in agreement with previous findings, the quasi-biennial periodicity (QBP) causes a weaker shift in mode frequencies and a slower enhancement than that caused by the 11-year cycle. We compare our observational findings with the features predicted by different models, that try to explain the origin of this QBP and conclude that the observed properties could result from the beating between a dipole and quadrupole magnetic configuration of the dynamo. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {dynamo,notion,notion-database,Sun: activity,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/ANHFT7XN/Simoniello et al. - 2013.pdf}
}

@article{Skarka2022,
  title = {Periodic Variable {{A-F}} Spectral Type Stars in the Northern {{TESS}} Continuous Viewing Zone. {{I}}. {{Identification}} and Classification},
  author = {Skarka, M. and {\v Z}{\'a}k, J. and Fedurco, M. and Paunzen, E. and Henzl, Z. and Ma{\v s}ek, M. and Karjalainen, R. and Sanchez Arias, J. P. and S{\'o}dor, {\'A}. and Auer, R. F. and Kab{\'a}th, P. and Karjalainen, M. and Li{\v s}ka, J. and {\v S}tegner, D.},
  year = {2022},
  month = oct,
  journal = {Astronomy \& Astrophysics},
  volume = {666},
  pages = {A142},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202244037},
  urldate = {2023-10-17},
  abstract = {Context. In the time of large space surveys that provide tremendous amounts of precise data, it is highly desirable to have a commonly accepted methodology and system for the classification of variable stars. This is especially important for A-F stars, which can show intrinsic brightness variations due to both rotation and pulsations. Aims: The goal of our study is to provide a reliable classification of the variability of A-F stars brighter than 11 mag located in the northern TESS continuous viewing zone. We also aim to provide a thorough discussion about issues in the classification related to data characteristics and the issues arising from the similar light-curve shape generated by different physical mechanisms. Methods: We used TESS long- and short-cadence photometric data and corresponding Fourier transform to classify the variability type of the stars. We also used spectroscopic observations to determine the projected rotational velocity of a few stars. Results: We present a clear and concise classification system that is demonstrated on many examples. We find clear signs of variability in 3025 of 5923 studied stars (51\%). For 1813 of these 3025 stars, we provide a classification; the rest cannot be unambiguously classified. Of the classified stars, 64.5\% are pulsating stars of g-mode {$\gamma$} Doradus (GDOR) and p-mode {$\delta$} Scuti types and their hybrids. We realised that the long- and short-cadence pre-search data conditioning simple aperture photometry data can differ significantly not only in amplitude but also in the content of instrumental and data-reduction artefacts, making the long-cadence data less reliable. We identified a new group of stars that show stable light curves and characteristic frequency spectrum patterns (8.5\% of the classified stars). According to the position in the Hertzsprung-Russell diagram, these stars are likely GDOR stars but are on average about 200 K cooler than GDORs and have smaller amplitudes and longer periods. With the help of spectroscopic measurements of v sin i, we show that the variability of stars with unresolved groups of peaks located close to the positions of the harmonics in their frequency spectra (16\% of the classified stars) can be caused by rotation rather than by pulsations. We show that without spectroscopic observations it can be impossible to unambiguously distinguish between ellipsoidal variability and rotational variability. We also applied our methodology to three previous studies and find significant discrepancies in the classification. Conclusions: We demonstrate how difficult the classification of variable A-F stars can be when using only photometric data, how the residual artefacts can produce false positives, and that some types cannot actually be distinguished without spectroscopic observations. Our analysis provides collections that can be used as training samples for automatic classification. Full Table 5 is only available at the CDS via anonymous ftp to cdsarc.u-strasbg.fr (ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/cat/J/A+A/666/A142},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,catalogs,methods: data analysis,stars: oscillations,stars: rotation,stars: variables: general},
  annotation = {ADS Bibcode: 2022A\&A...666A.142S},
  file = {/Users/lbugnet/Zotero/storage/2SRVYUGH/Skarka et al. - 2022 - Periodic variable A-F spectral type stars in the n.pdf}
}

@article{skumanich1972,
  title = {Time Scale for {{Ca II}} Emission Decay, Rotational Braking, and Lithium Depletion},
  author = {Skumanich, A.},
  year = {1972},
  journal = {The Astrophysical Journal},
  volume = {767},
  number = {11},
  pages = {1--34},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/46S83GVZ/Skumanich - 1972.pdf}
}

@article{Smak1966,
  title = {{{THE LONG-PERIOD VARIABLE STARSl}}},
  author = {Smak, Jozef I.},
  year = {1966},
  journal = {Annual Review of Astronomie and Astrophysics},
  pages = {19--34},
  urldate = {2020-04-09},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NHC498MX/full-text.pdf}
}

@article{Smalley2015,
  title = {{{KIC}} 4768731: {{A}} Bright Long-Period {{roAp}} Star in the {{Kepler}} Field},
  author = {Smalley, B. and Niemczura, E. and Murphy, S. J. and Lehmann, H. and Kurtz, D. W. and Holdsworth, D. L. and Cunha, M. S. and Balona, L. A. and Briquet, M. and Bruntt, H. and De Cat, P. and Lampens, P. and Thygesen, A. O. and Uytterhoeven, K.},
  year = {2015},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {452},
  number = {4},
  pages = {3334--3345},
  issn = {13652966},
  doi = {10.1093/mnras/stv1515},
  abstract = {We report the identification of 61.45 d\textsuperscript{-1} (711.2 {$\mu$}Hz) oscillations, with amplitudes of 62.6 {$\mu$}mag, in KIC 4768731 (HD 225914) using Kepler photometry. This relatively bright (V = 9.17) chemically peculiar star with spectral type A5 Vp SrCr(Eu) has previously been found to exhibit rotational modulation with a period of 5.21 d. Fourier analysis reveals a simple dipole pulsator with an amplitude that has remained stable over a 4-yr time span, but with a frequency that is variable. Analysis of high-resolution spectra yields stellar parameters of T{$<$}inf{$>$}eff{$<$}/inf{$>$} =8100{$\pm$}200 K, log g=4.0{$\pm$}0.2, [Fe/H]=+0.31{$\pm$}0.24 and v sin i=14.8{$\pm$}1.6 kms\textsuperscript{-1}. Line profile variations caused by rotation are also evident. Lines of Sr, Cr, Eu, Mg and Si are strongest when the star is brightest, while Y and Ba vary in antiphase with the other elements. The abundances of rare earth elements are only modestly enhanced compared to other roAp stars of similar Teffand log g. Radial velocities in the literature suggest a significant change over the past 30 yr, but the radial velocities presented here show no significant change over a period of 4 yr.},
  keywords = {Asteroseismology,notion,notion-database,Stars: abundances,Stars: chemically peculiar,Stars: individual: KIC 4768731,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/794FERFH/Smalley et al. - 2015.pdf}
}

@article{Smith2012,
  title = {Kepler {{Presearch Data Conditioning II}} - {{A Bayesian Approach}} to {{Systematic Error Correction}}},
  author = {Smith, Jeffrey C. and Stumpe, Martin C. and Van Cleve, Jeffrey E. and Jenkins, Jon M. and Barclay, Thomas S. and Fanelli, Michael N. and Girouard, Forrest R. and Kolodziejczak, Jeffery J. and McCauliff, Sean D. and Morris, Robert L. and Twicken, Joseph D.},
  year = {2012},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {124},
  number = {919},
  eprint = {1203.1383},
  pages = {1000--1014},
  issn = {00046280},
  doi = {10.1086/667697},
  abstract = {With the unprecedented photometric precision of the Kepler Spacecraft, significant systematic and stochastic errors on transit signal levels are observable in the Kepler photometric data. These errors, which include discontinuities, outliers, systematic trends and other instrumental signatures, obscure astrophysical signals. The Presearch Data Conditioning (PDC) module of the Kepler data analysis pipeline tries to remove these errors while preserving planet transits and other astrophysically interesting signals. The completely new noise and stellar variability regime observed in Kepler data poses a significant problem to standard cotrending methods such as SYSREM and TFA. Variable stars are often of particular astrophysical interest so the preservation of their signals is of significant importance to the astrophysical community. We present a Bayesian Maximum A Posteriori (MAP) approach where a subset of highly correlated and quiet stars is used to generate a cotrending basis vector set which is in turn used to establish a range of "reasonable" robust fit parameters. These robust fit parameters are then used to generate a Bayesian Prior and a Bayesian Posterior Probability Distribution Function (PDF) which when maximized finds the best fit that simultaneously removes systematic effects while reducing the signal distortion and noise injection which commonly afflicts simple least-squares (LS) fitting. A numerical and empirical approach is taken where the Bayesian Prior PDFs are generated from fits to the light curve distributions themselves.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/3DHSSAP4/Smith et al. - 2012.pdf}
}

@article{Soderblom2010,
  title = {The {{Ages}} of {{Stars}}},
  author = {Soderblom, David R.},
  year = {2010},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {48},
  number = {1},
  eprint = {1003.6074},
  pages = {581--629},
  issn = {0066-4146},
  doi = {10.1146/annurev-astro-081309-130806},
  abstract = {The age of an individual star cannot be measured, only estimated through mostly model-dependent or empirical methods, and no single method works well for a broad range of stellar types or for a full range in age. This review presents a summary of the available techniques for age-dating stars and ensembles of stars, their realms of applicability, and their strengths and weaknesses. My emphasis is on low-mass stars because they are present from all epochs of star formation in the Galaxy and because they present both special opportunities and problems. The ages of open clusters are important for understanding the limitations of stellar models and for calibrating empirical age indicators. For individual stars, a hierarchy of quality for the available age-dating methods is described. Although our present ability to determine the ages of even the nearest stars is mediocre, the next few years hold great promise as asteroseismology probes beyond stellar surfaces and starts to provide precise interior properties of stars and as models continue to improve when stressed by better observations.},
  archiveprefix = {arxiv},
  keywords = {ages,evolution,galaxy,low-mass,notion,notion-database,open clusters and associations,pre-main sequence,solar-type,stars},
  file = {/Users/lbugnet/Zotero/storage/78MYRG7G/Soderblom - 2010.pdf}
}

@article{Soderblom2015a,
  title = {Ages of Stars: {{Methods}} and Uncertainties},
  author = {Soderblom, David R.},
  year = {2015},
  journal = {Astrophysics and Space Science Proceedings},
  volume = {39},
  eprint = {1409.2266},
  pages = {3--9},
  issn = {15706605},
  doi = {10.1007/978-3-319-10993-0_1},
  abstract = {Estimating ages for stars is difficult at best, but Galactic problems have their own requirements that go beyond those for other areas of astrophysics. As in other areas, asteroseismology is helping, and in this review I discuss some of the general problems encountered and some specific to large-scale studies of the Milky Way.},
  archiveprefix = {arxiv},
  isbn = {9783319109923},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PWFRG4BQ/Soderblom - 2015.pdf}
}

@article{Soker2004,
  title = {Why a {{Single-Star Model Cannot Explain}} the {{Bipolar Nebula}} of {{Eta Carinae}}},
  author = {Soker, Noam},
  year = {2004},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {612},
  number = {2},
  eprint = {astro-ph/0403674},
  pages = {1060--1064},
  publisher = {{IOP Publishing}},
  doi = {10.1086/422599},
  urldate = {2020-07-13},
  abstract = {I examine the angular momentum evolution during the 1837-1856 Great Eruption of the massive star Eta Carinae. I find that the new estimate of the mass blown during that eruption implies that the envelope of Eta Car substantially spun-down during the 20 years eruption. Single-star models, most of which require the envelope to rotate close to the break-up velocity, cannot account for the bipolar nebula (the Homunculus) formed from matter expelled in that eruption. The kinetic energy and momentum of the Homunculus further constrains single-star models. I discuss how Eta Car can fit into a unified model for the formation of bipolar lobes where two oppositely ejected jets inflate two lobes (or bubbles). These jets are blown by an accretion disk, which requires stellar companions in the case of bipolar nebulae around stellar objects.},
  archiveprefix = {arxiv},
  keywords = {binaries,close-circumstellar matter-stars,individual ( Carinae)-stars,mass loss-stars,notion,notion-database,outflows,Subject headingg s,winds},
  file = {/Users/lbugnet/Zotero/storage/S6QZ2E6J/full-text.pdf}
}

@article{Solanki2013,
  title = {Solar Irradiance Variability},
  author = {Solanki, S. K. and Unruh, Y. C.},
  year = {2013},
  journal = {Astronomische Nachrichten},
  volume = {334},
  number = {1-2},
  pages = {145--150},
  issn = {00046337},
  doi = {10.1002/asna.201211752},
  abstract = {The Sun has long been considered a constant star, to the extent that its total irradiance was termed the solar constant. It required radiometers in space to detect the small variations in solar irradiance on timescales of the solar rotation and the solar cycle. A part of the difficulty is that there are no other constant natural daytime sources to which the Sun's brightness can be compared. The discovery of solar irradiance variability rekindled a long-running discussion on how strongly the Sun affects our climate. A non-negligible influence is suggested by correlation studies between solar variability and climate indicators. The mechanism for solar irradiance variations that fits the observations best is that magnetic features at the solar surface, i.e. sunspots, faculae and the magnetic network, are responsible for almost all variations (although on short timescales convection and p-mode oscillations also contribute). In spite of significant progress important questions are still open. Thus there is a debate on how strongly irradiance varies on timescales of centuries (i.e. how much darker the Sun was during the Maunder minimum than it is today). It is also not clear how the solar spectrum changes over the solar cycle. Both these questions are of fundamental importance for working out just how strongly the Sun influences our climate. Another interesting question is how solar irradiance variability compares with that of other cool dwarfs, particularly now that observations from space are available also for stars. \textcopyright{} 2013 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {notion,notion-database,Stars: activity,Stars: magnetic fields,Sun: activity,Sun: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/8EG2P45L/Solanki, Unruh - 2013.pdf}
}

@article{Somers2016,
  title = {Lithium {{Depletion}} Is a {{Strong Test}} of {{Core-envelope Recoupling}}},
  author = {Somers, Garrett and Pinsonneault, Marc H.},
  year = {2016},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {829},
  pages = {32},
  issn = {0004-637X},
  doi = {10.3847/0004-637X/829/1/32},
  urldate = {2023-10-10},
  abstract = {Rotational mixing is a prime candidate for explaining the gradual depletion of lithium from the photospheres of cool stars during the main sequence. However, previous mixing calculations have relied primarily on treatments of angular momentum transport in stellar interiors incompatible with solar and stellar data in the sense that they overestimate the internal differential rotation. Instead, recent studies suggest that stars are strongly differentially rotating at young ages but approach a solid body rotation during their lifetimes. We modify our rotating stellar evolution code to include an additional source of angular momentum transport, a necessary ingredient for explaining the open cluster rotation pattern, and examine the consequences for mixing. We confirm that core-envelope recoupling with a {$\sim$}20 Myr timescale is required to explain the evolution of the mean rotation pattern along the main sequence, and demonstrate that it also provides a more accurate description of the Li depletion pattern seen in open clusters. Recoupling produces a characteristic pattern of efficient mixing at early ages and little mixing at late ages, thus predicting a flattening of Li depletion at a few Gyr, in agreement with the observed late-time evolution. Using Li abundances we argue that the timescale for core-envelope recoupling during the main sequence decreases sharply with increasing mass. We discuss the implications of this finding for stellar physics, including the viability of gravity waves and magnetic fields as agents of angular momentum transport. We also raise the possibility of intrinsic differences in initial conditions in star clusters using M67 as an example.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: abundances,stars: rotation,stars: solar-type},
  annotation = {ADS Bibcode: 2016ApJ...829...32S},
  file = {/Users/lbugnet/Zotero/storage/LHTTCAJ9/Somers and Pinsonneault - 2016 - Lithium Depletion is a Strong Test of Core-envelop.pdf}
}

@article{Soriano2007,
  title = {The {{CoRoT}} Primary Target {{HD}} 52265: {{Models}} and Seismic Tests},
  author = {Soriano, M. and Vauclair, S. and Vauclair, G. and Laymand, M.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {471},
  number = {3},
  pages = {885--892},
  issn = {00046361},
  doi = {10.1051/0004-6361:20066798},
  abstract = {HD 52265 is the only known exoplanet-host star selected as a main target for the seismology programme of the CoRoT satellite. As such, it will be observed continuously during five months, which is of particular interest when studying planetary systems. This star was misclassified as a giant in the Bright Star Catalog, while it is more probably on the main-sequence or at the beginning of the subgiant branch. We performed an extensive analysis of this star, showing how asteroseismology may lead to a precise determination of its external parameters and internal structure. Methods. We first reviewed the observational constraints on the metallicity, the gravity, and the effective temperature derived from the spectroscopic observations of HD 52265. We also derived its luminosity using the Hipparcos parallax. We computed the evolutionary tracks for models of various metallicities that cross the relevant observational error boxes in the gravity-effective temperature plane. We selected eight different stellar models that satisfy the observational constraints, computed their p-modes frequencies, and analysed specific seismic tests. Results. The possible models for HD 52265, which satisfy the constraints derived from the spectroscopic observations, are different in both their external and internal parameters. They lie either on the main sequence or at the beginning of the subgiant branch. The differences in the models lead to quite different properties of their oscillation frequencies. We give evidence of an interesting specific behaviour of these frequencies in the case of helium-rich cores: the "small separations" may become negative and give constraints on the size of the core. We expect that the observations of this star by the CoRoT satellite will allow a choice between these possible models. \textcopyright{} ESO 2007.},
  keywords = {notion,notion-database,Planetary systems,Stars: abundances,Stars: individual: HD 52265,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/CGJ883MY/Soriano et al. - 2007.pdf}
}

@article{Soriano2008,
  title = {Asteroseismology of Solar-Type Stars: {{Signatures}} of Convective and/or Helium Cores},
  author = {Soriano, M. and Vauclair, S.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {488},
  number = {3},
  pages = {975--985},
  issn = {00046361},
  doi = {10.1051/0004-6361:200809977},
  abstract = {Aims. Several frequency combinations are widely used in the analysis of stellar oscillations for comparisons between models and observations. In particular, the "small separations" can help constraining the stellar cores. We showed in a previous paper that they can change sign, in contradiction with the "asymptotic theory", and that this behaviour could correspond to signatures of convective and/or helium cores. Here we analyse this behaviour in detail by systematic modelling during stellar evolution.Methods. We computed evolutionary tracks for models with various masses (from 1.05 to 1.25 ) and various chemical compositions, with and without overshooting. We computed the adiabatic oscillation frequencies of the models and analysed the evolution of their small separations along an evolutionary track.Results. We find that, for all cases, the stars go through a stage during their evolution, where the small separations computed between degrees and become negative in the observed range of frequencies. This behaviour is clearly related to the signature of a helium-rich core. We discuss the consequences for interpreting of the acoustic frequencies observed in solar-type stars.. \textcopyright{} 2008 ESO.},
  keywords = {Galaxy: kinematics and dynamics,Galaxy: open clusters and associations: general,notion,notion-database,Stars: abundances,Stars: evolution,Stars: oscillations,Stars: planetary systems},
  file = {/Users/lbugnet/Zotero/storage/V2DJI9EC/Soriano, Vauclair - 2008.pdf}
}

@article{Soriano2010a,
  title = {New Seismic Analysis of the Exoplanet-Host Star {$\mu$} {{Arae}}},
  author = {Soriano, M. and Vauclair, S.},
  year = {2010},
  journal = {Astronomy and Astrophysics},
  volume = {513},
  number = {8},
  pages = {1--8},
  issn = {14320746},
  doi = {10.1051/0004-6361/200911862},
  abstract = {Aims. We present detailed modelling of the exoplanet-host star {$\mu$} Arae, using a new method for the asteroseismic analysis, and taking into account the new value recently derived for the Hipparcos parallax. The aim is to obtain precise parameters for this star and its internal structure, including constraints on the core overshooting. Methods. We computed new stellar models in a wider range than Bazot et al. (2005, A\&A, 440, 615), with various chemical compositions ([Fe/H] and Y), with or without overshooting at the edge of the core. We computed their adiabatic oscillation frequencies and compared them to the seismic observations. For each set of chemical parameters, we kept the model which represented the best fit to the echelle diagram. Then, by comparing the effective temperatures, gravities and luminosities of these models with the spectroscopic error boxes, we were able to derive precise parameters for this star. Results. First we find that all the models which correctly fit the echelle diagram have the same mass and radius, with an uncertainty of the order of one percent. Second, the final comparison with spectroscopic observations leads to the conclusion that besides its high metallicity, {$\mu$} Arae has a high helium abundance of the order of Y = 0.3. Knowing this allows finding precise values for all the other parameters, mass, radius and age. \textcopyright{} ESO, 2010.},
  keywords = {notion,notion-database,Planetary systems,Stars: abundances,Stars: evolution,Stars: individual: {$\mu$} Arae,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/KEIXHBEY/Soriano, Vauclair - 2010.pdf}
}

@article{Southworth2007,
  title = {A Method for the Direct Determination of the Surface Gravities of Transiting Extrasolar Planets},
  author = {Southworth, John and Wheatley, Peter J and Sams, Giles},
  year = {2007},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {379},
  pages = {11--15},
  doi = {10.1111/j.1745-3933.2007.00324.x},
  urldate = {2020-07-07},
  abstract = {We show that the surface gravity of a transiting extrasolar planet can be calculated from only the spectroscopic orbit of its parent star and the analysis of its transit light curve. This does not require additional constraints, such as are often inferred from theoretical stellar models or model atmospheres. The surface gravity of the planet can therefore be measured precisely and from only directly observable quantities. We outline the method and apply it to the case of the first known transiting extrasolar planet, HD 209458b. We find a surface gravity of g p = 9.28 {$\pm$} 0.15 m s -2 , which is an order of magnitude more precise than the best available measurements of its mass, radius and density. This confirms that the planet has a much lower surface gravity than that predicted by published theoretical models of gas giant planets. We apply our method to all 14 known transiting extrasolar planets and find a significant correlation between surface gravity and orbital period, which is related to the known correlation between mass and period. This correlation may be the underlying effect as surface gravity is a fundamental parameter in the evaporation of planetary atmospheres.},
  keywords = {data analysis-binaries,eclipsing-binaries,HD 209458-planetary systems,individual,methods,notion,notion-database,spectroscopic-stars}
}

@article{Sowicka2017,
  title = {Search for Exoplanets around Pulsating Stars of {{A-F}} Type in {{Kepler}} Short-Cadence Data and the Case of {{KIC}} 8197761},
  author = {Sowicka, Paulina and Handler, Gerald and D{\k{e}}bski, Bart{\l}omiej and Jones, David and {Van de Sande}, Marie and P{\'a}pics, P{\'e}ter I.},
  year = {2017},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {467},
  pages = {4663--4673},
  issn = {0035-8711},
  doi = {10.1093/mnras/stx413},
  urldate = {2023-10-28},
  abstract = {We searched for extrasolar planets around pulsating stars by examining Kepler data for transit-like events hidden in the intrinsic variability. All short-cadence observations for targets with 6000 {$<$} Teff {$<$} 8500 K were visually inspected for transit-like events following the removal of pulsational signals by sinusoidal fits. Clear transit-like events were detected in KIC 5613330 and KIC 8197761. KIC 5613330 is a confirmed exoplanet host (Kepler-635b), where the transit period determined here is consistent with the literature value. KIC 8197761 is a {$\gamma$} Doradus-{$\delta$} Scuti star exhibiting eclipses/transits occurring every 9.868 6667(27) d, having durations of 8.37 h and causing brightness drops {$\Delta$} F/F = 0.006 29(29). The star's pulsation spectrum contains several mode doublets and triplets, identified as l = 1, with a mean spacing of 0.001 659(15) d-1 , implying an internal rotation period of 301 {$\pm$} 3 d. Trials to calculate the size of the light travel time effect (LTTE) from the pulsations to constrain the companion's mass ended inconclusive. Finding planets around {$\gamma$} Doradus stars from the pulsational LTTE, therefore, is concluded to be unrealistic. Spectroscopic monitoring of KIC 8197761 revealed sinusoidal radial velocity variations with a semi-amplitude of 19.75 {$\pm$} 0.32 km s-1, while individual spectra present rotational broadening consistent with vsin I = 9 {$\pm$} 1 km s-1. This suggests that the stellar surface rotation is synchronized with the orbit, whereas the stellar core rotates {$\sim$}30 times slower. Combining the observed radial velocity variability with the transit photometry, constrains the companion's mass to be {$\approx$}0.28 M{$\odot$}, ruling out an exoplanet hypothesis.},
  keywords = {Astrophysics - Earth and Planetary Astrophysics,Astrophysics - Solar and Stellar Astrophysics,binaries: eclipsing,planetary systems,planets and satellites: detection,stars: individual: KIC 8197761,stars: variables: general},
  annotation = {ADS Bibcode: 2017MNRAS.467.4663S},
  file = {/Users/lbugnet/Zotero/storage/9M7GM3RK/Sowicka et al. - 2017 - Search for exoplanets around pulsating stars of A-.pdf}
}

@techreport{Sozzetti2007,
  title = {Improving {{Stellar}} and {{Planetary Parameters}} of {{Transiting Planet Systems}}: {{The Case}} of {{TrES-2}}},
  author = {Sozzetti, Alessandro and Torres, Guillermo and Charbonneau, David and Latham, David W and Holman, Matthew J and Winn, Joshua N and Laird, John B and O'donovan, Francis T and Sloan, Alfred P and Fellow, Research},
  year = {2007},
  eprint = {0704.2938v1},
  urldate = {2020-01-20},
  abstract = {We report on a spectroscopic determination of the atmospheric parameters and chemical abundance of the parent star of the recently discovered transiting planet TrES-2. A detailed LTE analysis of a set of Fe I and Fe II lines from our Keck spectra yields T eff = 5850 {$\pm$} 50 K, log g = 4.4 {$\pm$} 0.1, and [Fe/H] = -0.15 {$\pm$} 0.10. Several independent checks (e.g., additional spectroscopy, line-depth ratios) confirm the reliability of our spectroscopic T eff estimate. The mass and radius of the star, needed to determine the properties of the planet, are traditionally inferred by comparison with stellar evolution models using T eff and some measure of the stellar luminosity, such as the spectroscopic surface gravity (when a trigonometric parallax is unavailable, as in this case). We apply here a new method in which we use instead of log g the normalized separation a/R {$\star$} (related to the stellar density), which can be determined directly from the light curves of transiting planets with much greater precision. With the a/R {$\star$} value from the light curve analysis of Holman et al. (2007b) and our T eff estimate we obtain M {$\star$} = 0.980 {$\pm$} 0.062 M {$\odot$} and R {$\star$} = 1.000 +0.036 -0.033 R {$\odot$} , and an evolutionary age of 5.1 +2.7 -2.3 Gyr, in good agreement with other constraints based on the strength of the emission in the Ca II H \& K line cores, the Lithium abundance, and rotation. The new stellar parameters yield improved values for the planetary mass and radius of M p = 1.198 {$\pm$} 0.053 M Jup and R p = 1.220 +0.045 -0.042 R Jup , confirming that},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/XR2K7X43/full-text.pdf}
}

@article{Sozzetti2007a,
  title = {Improving {{Stellar}} and {{Planetary Parameters}} of {{Transiting Planet Systems}}: {{The Case}} of {{TrES-2}}},
  author = {Sozzetti, A. and Torres, G. and Charbonneau, D. and Latham, D. W. and Holman, M. J. and Winn, J. N. and Laird, J. B. and O'Donovan, F. T.},
  year = {2007},
  month = apr,
  eprint = {0704.2938},
  doi = {10.1086/519214},
  abstract = {We report on a spectroscopic determination of the atmospheric parameters and chemical abundance of the parent star of the recently discovered transiting planet \{TrES-2\}. A detailed LTE analysis of a set of \textbackslash ion\{Fe\}\{1\} and \textbackslash ion\{Fe\}\{2\} lines from our Keck spectra yields \$T\_\textbackslash mathrm\{eff\} = 5850\textbackslash pm 50\$ K, \$\textbackslash log g = 4.4\textbackslash pm 0.1\$, and [Fe/H] \$= -0.15\textbackslash pm 0.10\$. Several independent checks (e.g., additional spectroscopy, line-depth ratios) confirm the reliability of our spectroscopic \$T\_\textbackslash mathrm\{eff\}\$ estimate. The mass and radius of the star, needed to determine the properties of the planet, are traditionally inferred by comparison with stellar evolution models using \$T\_\textbackslash mathrm\{eff\}\$ and some measure of the stellar luminosity, such as the spectroscopic surface gravity (when a trigonometric parallax is unavailable, as in this case). We apply here a new method in which we use instead of \$\textbackslash log g\$ the normalized separation \$a/R\_\textbackslash star\$ (related to the stellar density), which can be determined directly from the light curves of transiting planets with much greater precision. With the \$a/R\_\textbackslash star\$ value from the light curve analysis of Holman et al. \textbackslash citeyearpar\{holman07b\} and our \$T\_\textbackslash mathrm\{eff\}\$ estimate we obtain \$M\_\textbackslash star = 0.980\textbackslash pm0.062 M\_\textbackslash odot\$ and \$R\_\textbackslash star = 1.000\_\{-0.033\}\^\{+0.036\} R\_\textbackslash odot\$, and an evolutionary age of \$5.1\^\{+2.7\}\_\{-2.3\}\$ Gyr, in good agreement with other constraints based on the strength of the emission in the \textbackslash ion\{Ca\}\{2\} H \& K line cores, the Lithium abundance, and rotation. The new stellar parameters yield improved values for the planetary mass and radius of \$M\_p = 1.198 \textbackslash pm 0.053 M\_\textbackslash mathrm\{Jup\}\$ and \$R\_p = 1.220\^\{+0.045\}\_\{-0.042\} R\_\textbackslash mathrm\{Jup\}\$, confirming that \{TrES-2\} is the most massive among the currently known nearby (\$d\textbackslash lesssim 300\$ pc) transiting hot Jupiters. [Abridged]},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/X353ZSR7/0704.2938.pdf}
}

@article{Spada2016,
  title = {Angular Momentum Transport Efficiency in Post-Main Sequence Low-Mass Stars},
  author = {Spada, F. and Gellert, M. and Arlt, R. and Deheuvels, S.},
  year = {2016},
  month = may,
  journal = {Astronomy and Astrophysics},
  volume = {589},
  pages = {A23},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201527591},
  urldate = {2023-10-26},
  abstract = {Context. Using asteroseismic techniques, it has recently become possible to probe the internal rotation profile of low-mass ({$\approx$}1.1-1.5 M{$\odot$}) subgiant and red giant stars. Under the assumption of local angular momentum conservation, the core contraction and envelope expansion occurring at the end of the main sequence would result in a much larger internal differential rotation than observed. This suggests that angular momentum redistribution must be taking place in the interior of these stars. Aims: We investigate the physical nature of the angular momentum redistribution mechanisms operating in stellar interiors by constraining the efficiency of post-main sequence rotational coupling. Methods: We model the rotational evolution of a 1.25M{$\odot$} star using the Yale Rotational stellar Evolution Code. Our models take into account the magnetic wind braking occurring at the surface of the star and the angular momentum transport in the interior, with an efficiency dependent on the degree of internal differential rotation. Results: We find that models including a dependence of the angular momentum transport efficiency on the radial rotational shear reproduce very well the observations. The best fit of the data is obtained with an angular momentum transport coefficient scaling with the ratio of the rotation rate of the radiative interior over that of the convective envelope of the star as a power law of exponent {$\approx$}3. This scaling is consistent with the predictions of recent numerical simulations of the Azimuthal Magneto-Rotational Instability. Conclusions: We show that an angular momentum transport process whose efficiency varies during the stellar evolution through a dependence on the level of internal differential rotation is required to explain the observed post-main sequence rotational evolution of low-mass stars.},
  keywords = {asteroseismology,Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,magnetohydrodynamics (MHD),Magnetohydrodynamics (MHD),notion,notion-database,stars: interiors,Stars: interiors,stars: magnetic field,Stars: magnetic field,stars: rotation,Stars: rotation,stars: solar-type,Stars: solar-type},
  annotation = {ADS Bibcode: 2016A\&A...589A..23S},
  file = {/Users/lbugnet/Zotero/storage/GY6L7244/Spada et al. - 2016.pdf;/Users/lbugnet/Zotero/storage/H77IMNZ6/Spada et al. - 2016 - Angular momentum transport efficiency in post-main.pdf}
}

@article{Spada2020b,
  title = {Competing Effect of Wind Braking and Interior Coupling in the Rotational Evolution of Solar-like Stars},
  author = {Spada, F. and Lanzafame, A. C.},
  year = {2020},
  month = apr,
  journal = {Astronomy \& Astrophysics},
  volume = {636},
  pages = {A76},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201936384},
  urldate = {2023-10-26},
  abstract = {Solar-like stars (M {$\lessequivlnt$} 1.3 M{$\odot$}) lose angular momentum through their magnetized winds. The resulting evolution of the surface rotation period, which can be directly measured photometrically, has the potential to be an accurate indicator of stellar age, and is constrained by observations of rotation periods of coeval stars, such as members of Galactic open clusters. A prominent observational feature of the mass-rotation period diagrams of open clusters is a sequence of relatively slower rotators. The formation and persistence of this slow-rotator sequence across several billion years imply an approximately coherent spin-down of the stars that belong to it. In particular, the sequence is observed to evolve coherently toward longer periods in progressively older clusters. Recent observations of the {$\approx$}700 Myr Praesepe and the 1 Gyr NGC 6811 clusters, however, are not fully consistent with this general pattern. While the stars of 1 M{$\odot$} on the slow-rotator sequence of the older NGC 6811 have longer periods than their counterparts in the younger Praesepe, as expected, the two sequences essentially merge at lower masses ({$\lessequivlnt$}0.8 M{$\odot$}). In other words, it seems that low-mass stars have not been spinning down in the intervening 300 Myr. Here we show that this behavior is a manifestation of the variable rotational coupling in solar-like stars. The resurfacing of angular momentum from the interior can temporarily compensate for that lost at the surface due to wind braking. In our model the internal redistribution of angular momentum has a steep mass dependence; as a result, the re-coupling occurs at different ages for stars of different masses. The semi-empirical mass dependence of the rotational coupling timescale included in our model produces an evolution of the slow-rotator sequence in very good agreement with the observations. Our model, in particular, explains the stalled surface spin-down of low-mass stars between Praesepe and NGC 6811, and predicts that the same behavior should be observable at other ages in other mass ranges.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,notion,notion-database,Open clusters and associations: individual: NGC 68,open clusters and associations: individual: NGC 6811,Open clusters and associations: individual: Pleiad,open clusters and associations: individual: Pleiades,Open clusters and associations: individual: Praese,open clusters and associations: individual: Praesepe,stars: evolution,Stars: evolution,stars: late-type,Stars: late-type,stars: rotation,Stars: rotation},
  annotation = {ADS Bibcode: 2020A\&A...636A..76S},
  file = {/Users/lbugnet/Zotero/storage/9J7CQ4YR/full-text.pdf;/Users/lbugnet/Zotero/storage/JA3XZYTT/Spada and Lanzafame - 2020 - Competing effect of wind braking and interior coup.pdf}
}

@article{Spruit1999,
  title = {Differential Rotation and Magnetic Fields in Stellar Interiors},
  author = {Spruit, H. C.},
  year = {1999},
  journal = {Astronomy \& Astrophysics},
  volume = {349},
  number = {1},
  eprint = {astro-ph/9907138},
  pages = {189--202},
  issn = {00046361},
  abstract = {The processes contributing to the evolution of an initially weak magnetic field in a differentially rotating star are reviewed. These include rotational smoothing (akin to convective expulsion) and a list of about 5 instabilities, among them magnetorotational instability, buoyancy instability, and pinch-type instabilities. The important effects of thermal and magnetic diffusion on these instabilities are analyzed in some detail. The first instability to set in is a pinch-type instability. It becomes important in modifying the field configuration before magnetic buoyancy-driven instabilities set in. The evolution of an initially strong field remains a more open question, including the old problem whether dynamically stable magnetic equilibria exist in stars.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,Magnetohydrodynamics (MHD),notion,notion-database,Stars: magnetic fields,Stars: rotation,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/2L7B5W3P/Spruit - 1999.pdf}
}

@article{Spruit2002,
  title = {Dynamo Action by Differential Rotation in a Stably Stratified Stellar Interior},
  author = {Spruit, H. C.},
  year = {2002},
  journal = {Astronomy \& Astrophysics},
  volume = {381},
  number = {3},
  eprint = {astro-ph/0108207},
  pages = {923--932},
  publisher = {{EDP Sciences}},
  issn = {00046361},
  doi = {10.1051/0004-6361:20011465},
  urldate = {2020-03-09},
  abstract = {Magnetic fields can be created in stably stratified (non-convective) layers in a differentially rotating star. A magnetic instability in the toroidal field (wound up by differential rotation) replaces the role of convection in closing the field amplification loop. Tayler instability is likely to be the most relevant magnetic instability. A dynamo model is developed from these ingredients, and applied to the problem of angular momentum transport in stellar interiors. It produces a predominantly horizontal field. This dynamo process is found to be more effective in transporting angular momentum than the known hydrodynamic mechanisms. It might account for the observed pattern of rotation in the solar core.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,Magnetohydrodynamics (MHD),notion,notion-database,Stars: magnetic fields},
  file = {/Users/lbugnet/Zotero/storage/MBBUEVG5/full-text.pdf}
}

@article{Spruit2003,
  title = {Origin of the Torsional Oscillation Pattern of Solar Rotation},
  author = {Spruit, H. C.},
  year = {2003},
  month = mar,
  journal = {Solar Physics},
  volume = {213},
  number = {1},
  eprint = {astro-ph/0209146},
  pages = {1--21},
  issn = {00380938},
  doi = {10.1023/A:1023202605379},
  urldate = {2020-07-13},
  abstract = {A model is presented that explains the 'torsional oscillation' pattern of deviations in the solar rotation rate as a geostrophic flow. The flow is driven by temperature variations near the surface due to the enhanced emission of radiation by the small-scale magnetic field. The model explains the sign of the flow, its amplitude and the fact that the maxima occur near the boundaries of the main activity belts. The amplitude of the flow decreases with depth from its maximum at the surface but penetrates over much of the depth of the convection zone, in agreement with the data from helioseismology. It predicts that the flow is axisymmetric only on average, and in reality consists of a superposition of circulations around areas of enhanced magnetic activity. It must be accompanied by a meridional flow component, which declines more rapidly with depth.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database}
}

@article{Starck2003,
  title = {Astronomical Image Representation by the Curvelet Transform},
  author = {Starck, J. L. and Donoho, D. L. and Cand{\`e}s, E. J.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {398},
  number = {2},
  pages = {785--800},
  issn = {00046361},
  doi = {10.1051/0004-6361:20021571},
  abstract = {We outline digital implementations of two newly developed multiscale representation systems, namely, the ridgelet and curvelet transforms. We apply these digital transforms to the problem of restoring an image from noisy data and compare our results with those obtained via well established methods based on the thresholding of wavelet coefficients. We show that the curvelet transform allows us also to well enhance elongated features contained in the data. Finally, we describe the Morphological Component Analysis, which consists in separating features in an image which do not present the same morphological characteristics. A range of examples illustrates the results.},
  keywords = {Methods: data analysis,notion,notion-database,Techniques: image processing},
  file = {/Users/lbugnet/Zotero/storage/XHJN8SAQ/Starck, Donoho, Candès - 2003.pdf}
}

@article{Starck2013,
  title = {Sparsity and the {{Bayesian}} Perspective},
  author = {Starck, J. L. and Donoho, D. L. and Fadili, M. J. and Rassat, A.},
  year = {2013},
  journal = {Astronomy and Astrophysics},
  volume = {552},
  pages = {1--5},
  issn = {00046361},
  doi = {10.1051/0004-6361/201321257},
  abstract = {Sparsity has recently been introduced in cosmology for weak-lensing and cosmic microwave background (CMB) data analysis for different applications such as denoising, component separation, or inpainting (i.e., filling the missing data or the mask). Although it gives very nice numerical results, CMB sparse inpainting has been severely criticized by top researchers in cosmology using arguments derived from a Bayesian perspective. In an attempt to understand their point of view, we realize that interpreting a regularization penalty term as a prior in a Bayesian framework can lead to erroneous conclusions. This paper is by no means against the Bayesian approach, which has proven to be very useful for many applications, but warns against a Bayesian-only interpretation in data analysis, which can be misleading in some cases. \textcopyright{} 2013 ESO.},
  keywords = {Cosmic background radiation,Methods: data analysis,Methods: statistical,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TVETFFQW/Starck et al. - 2013.pdf}
}

@article{Stassun2018,
  title = {The {{TESS Input Catalog}} and {{Candidate Target List}}},
  author = {Stassun, Keivan G. and Oelkers, Ryan J. and Pepper, Joshua and Paegert, Martin and Lee, Nathan De and Torres, Guillermo and Latham, David W. and Charpinet, St{\'e}phane and Dressing, Courtney D. and Huber, Daniel and Kane, Stephen R. and L{\'e}pine, S{\'e}bastien and Mann, Andrew and Muirhead, Philip S. and {Rojas-Ayala}, B{\'a}rbara and Silvotti, Roberto and Fleming, Scott W. and Levine, Al and Plavchan, Peter},
  year = {2018},
  journal = {The Astronomical Journal},
  volume = {156},
  number = {3},
  eprint = {1706.00495},
  pages = {102},
  publisher = {{IOP Publishing}},
  issn = {0004-6256},
  doi = {10.3847/1538-3881/aad050},
  abstract = {The Transiting Exoplanet Survey Satellite (TESS) will be conducting a nearly all-sky photometric survey over two years, with a core mission goal to discover small transiting exoplanets orbiting nearby bright stars. It will obtain 30-minute cadence observations of all objects in the TESS fields of view, along with 2-minute cadence observations of 200,000 to 400,000 selected stars. The choice of which stars to observe at the 2-min cadence is driven by the need to detect small transiting planets, which leads to the selection of primarily bright, cool dwarfs. We describe the catalogs assembled and the algorithms used to populate the TESS Input Catalog (TIC). We also describe a ranking system for prioritizing stars according to the smallest transiting planet detectable, and assemble a Candidate Target List (CTL) using that ranking. We discuss additional factors that affect the ability to photometrically detect and dynamically confirm small planets, and we note additional stellar populations of interest that may be added to the final target list. The TIC is available on the STScI MAST server, and an enhanced CTL is available through the Filtergraph data visualization portal system at the URL https://filtergraph.vanderbilt.edu/tess\_ctl .},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/YU77ZIM5/Stassun et al. - 2018.pdf}
}

@book{Stein2003,
  title = {An {{Introduction}} to {{Seismology}}, {{Earthquakes}}, and {{Earth Structure}}},
  author = {Stein, Seth and Wysession, Michael},
  year = {2003},
  publisher = {{Blackwell}},
  urldate = {2020-03-02},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZZTXTJKT/full-text.pdf}
}

@article{steinGenerationAcousticGravity1967,
  title = {Generation of {{Acoustic}} and {{Gravity Waves}} by {{Turbulence}} in an {{Isothermal Stratified Atmosphere}}},
  author = {Stein, Robert F.},
  year = {1967},
  month = dec,
  journal = {Solar Physics, Volume 2, Issue 4, pp.385-432},
  volume = {2},
  number = {4},
  pages = {385},
  publisher = {{Kluwer Academic Publishers}},
  issn = {0038-0938},
  doi = {10.1007/BF00146490},
  urldate = {2022-02-02},
  abstract = {Lighthill's method of calculating the aerodynamic emission of sound waves in a homogeneous atmosphere is extended to calculate the acoustic and gravity-wave emission by turbulent motions in a stratified atmosphere. The acoustic power output is Pac {$\approx$} 103\texttheta ouo3/loM5 ergs/cm3 sec, and the upward gravity wave flux is Fzgr {$\approx$} 102\texttheta oUo3/lo (lo ergs/cm3 sec. Here u0 is the turbulence velocity scale, l0 is its length scale, and H the scale height at the atmosphere. M = u0/c0 is the Mach number of the turbulence. The acoustic power output is proportional to the maximum value of the turbulence spectrum, and inversely to its rate of falloff at high frequencies. The stratification cuts off the acoustic emission at low Mach numbers. The gravity emission occurs near the critical angle to the vertical \texttheta c = cos-1{$\omega$}/{$\omega$}2, where {$\omega$}22 = ({$\gamma$} - 1)/{$\gamma$}2 (c0/H), and at very short wavelengths. It is proportional to the large wave number tail of the turbulence spectrum. On the sun, gravity-wave emission is much more efficient than acoustic, but can occur only from turbulent motions in stable regions, whereas acoustic waves are produced by turbulence in the convection zone. \textcopyright{} 1967 D. Reidel Publishing Company.},
  keywords = {notion,notion-database}
}

@article{Stellingwerf1979,
  title = {Pulsation in the Lower {{Cepheid}} Strip. {{I}} - {{Linear}} Survey},
  author = {Stellingwerf, R. F.},
  year = {1979},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {227},
  pages = {935},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/156802},
  urldate = {2020-03-31},
  keywords = {Astronomy,Cepheid Variables,Cepheids:Pulsations,Delta Scuti Stars:Models,Dwarf Cepheids:Models,Dwarf Stars,Helium,notion,notion-database,Pulsars,Star Distribution,Stellar Mass,Stellar Models}
}

@article{Stello2006,
  title = {Oscillation Mode Lifetimes in {$\xi$} {{Hydrae}}: {{Will}} Strong Mode Damping Limit Asteroseismology of Red Giant Stars?},
  author = {Stello, D. and Kjeldsen, H. and Bedding, T. R. and Buzasi, D.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {448},
  number = {2},
  eprint = {astro-ph/0511344},
  pages = {709--715},
  issn = {00046361},
  doi = {10.1051/0004-6361:20054016},
  abstract = {We introduce a new method to measure frequency separations and mode lifetimes of stochastically excited and damped oscillations, so-called solar-like oscillations. Our method shows that velocity data of the red giant star \textsterling Hya (Frandsen et al. 2002) support a large frequency separation between modes of roughly 7 {$\mu$}Hz. We also conclude that the data are consistent with a mode lifetime of 2 days, which is so short relative to its pulsation period that none of the observed frequencies are unambiguous. Hence, we argue that the maximum asteroseismic output that can be obtained from these data is an average large frequency separation, the oscillation amplitude and the average mode lifetime. However, the significant discrepancy between the theoretical calculations of the mode lifetime (Houdek \& Gough 2002) and our result based on the observations of {$\xi$} implies that red giant stars can help us better understand the damping and driving mechanisms of solar-like p-modes by convection. \textcopyright{} ESO 2006.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: individual: {$\xi$} Hya,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/XYHAI9EA/Stello et al. - 2006.pdf}
}

@article{Stello2006b,
  title = {Multisite Campaign on the Open Cluster {{M67}} - {{I}}. {{Observations}} and Photometric Reductions},
  author = {Stello, D. and Arentoft, T. and Bedding, T. R. and Bouzid, M. Y. and Bruntt, H. and Csubry, Z. and Dall, T. H. and Dind, Z. E. and Frandsen, S. and Gilliland, R. L. and Jacob, A. P. and Jensen, H. R. and Kang, Y. B. and Kim, S. L. and Kiss, L. L. and Kjeldsen, H. and Koo, J. R. and Lee, J. A. and Lee, C. U. and Nuspl, J. and Sterken, C. and Szab{\'o}, R.},
  year = {2006},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {373},
  number = {3},
  eprint = {astro-ph/0609340},
  pages = {1141--1150},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2006.11060.x},
  abstract = {We report on an ambitious multisite campaign aimed at detecting stellar variability, particularly solar-like oscillations, in the red giant stars in the open cluster M67 (NGC 2682). During the six-week observing run, which comprised 164 telescope nights, we used nine 0.6-m to 2.1-m class telescopes located around the world to obtain uninterrupted time series photometry. We outline here the data acquisition and reduction, with emphasis on the optimization of the signal-to-noise ratio of the low-amplitude (50-500 {$\mu$}mag) solar-like oscillations. This includes a new and efficient method for obtaining the linearity profile of the CCD response at ultrahigh precision ({$\sim$}10 parts per million). The noise in the final time series is 0.50 mmag per minute integration for the best site, while the noise in the Fourier spectrum of all sites combined is 20 {$\mu$}mag. In addition to the red giant stars, this data set proves to be very valuable for studying high-amplitude variable stars such as eclipsing binaries, W UMa systems and {$\delta$} Scuti stars. \textcopyright{} 2006 RAS.},
  archiveprefix = {arxiv},
  keywords = {Blue stragglers,notion,notion-database,Open clusters and associations: individual: M67 (N,Stars: oscillations,Stars: variables: other,Techniques: photometric,{$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/KZSYBCUH/Stello et al. - 2006(2).pdf}
}

@article{Stello2007,
  title = {Multisite Campaign on the Open Cluster {{M67}} - {{II}}. {{Evidence}} for Solar-like Oscillations in Red Giant Stars},
  author = {Stello, D. and Bruntt, H. and Kjeldsen, H. and Bedding, T. R. and Arentoft, T. and Gilliland, R. L. and Nuspl, J. and Kim, S. L. and Kang, Y. B. and Koo, J. R. and Lee, J. A. and Sterken, C. and Lee, C. U. and Jensen, H. R. and Jacob, A. P. and Szab{\'o}, R. and Frandsen, S. and Csubry, Z. and Dind, Z. E. and Bouzid, M. Y. and Dall, T. H. and Kiss, L. L.},
  year = {2007},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {377},
  number = {2},
  pages = {584--594},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2007.11585.x},
  abstract = {ABSTRACT Measuring solar-like oscillations in an ensemble of stars in a cluster, holds promise for testing stellar structure and evolution more stringently than just fitting parameters to single field stars. The most-ambitious attempt to pursue these prospects was by Gilliland et al. who targeted 11 turn-off stars in the open cluster M67 (NGC 2682), but the oscillation amplitudes were too small ({$<$}20 {$\mu$}mag) to obtain unambiguous detections. Like Gilliland et al. we also aim at detecting solar-like oscillations in M67, but we target red giant stars with expected amplitudes in the range 50- and periods of 1 to 8 h. We analyse our recently published photometry measurements, obtained during a six-week multisite campaign using nine telescopes around the world. The observations are compared with simulations and with estimated properties of the stellar oscillations. Noise levels in the Fourier spectra as low as are obtained for single sites, while the combined data reach, making this the best photometric time series of an ensemble of red giant stars. These data enable us to make the first test of the scaling relations (used to estimate frequency and amplitude) with an homogeneous ensemble of stars. The detected excess power is consistent with the expected signal from stellar oscillations, both in terms of its frequency range and amplitude. However, our results are limited by apparent high levels of non-white noise, which cannot be clearly separated from the stellar signal. \textcopyright{} 2007 The Authors. Journal compilation \textcopyright{} 2007 RAS.},
  keywords = {notion,notion-database,Open clusters and associations: individual: M67 (N,Stars: oscillations,Stars: variables: other,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/ZECH5CEW/Stello et al. - 2007.pdf}
}

@article{Stello2008,
  title = {Oscillating {{K Giants}} with the {{WIRE Satellite}}: {{Determination}} of {{Their Asteroseismic Masses}}},
  author = {Stello, D. and Bruntt, H. and Preston, H. and Buzasi, D.},
  year = {2008},
  journal = {The Astrophysical Journal},
  volume = {674},
  number = {1},
  eprint = {0801.2155},
  pages = {L53-L56},
  issn = {0004-637X},
  doi = {10.1086/528936},
  abstract = {Mass estimates of K giants are generally very uncertain. Traditionally, stellar masses of single field stars are determined by comparing their location in the Hertzsprung-Russell diagram with stellar evolutionary models. Applying an additional method to determine the mass is therefore of significant interest for understanding stellar evolution. We present the time series analysis of 11 K giants recently observed with the WIRE satellite. With this comprehensive sample, we report the first confirmation that the characteristic acoustic frequency, nu\_max, can be predicted for K giants by scaling from the solar acoustic cut-off frequency. We are further able to utilize our measurements of nu\_max to determine an asteroseismic mass for each star with a lower uncertainty compared to the traditional method, for most stars in our sample. This indicates good prospects for the application of our method on the vast amounts of data that will soon come from the COROT and Kepler space missions.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/B6B7XTDX/Stello et al. - 2008.pdf}
}

@article{Stello2009,
  title = {Radius Determination of Solar-Type Stars Using Asteroseismology: {{What}} to Expect from the Kepler Mission},
  author = {Stello, Dennis and Chaplin, William J. and Bruntt, Hans and Creevey, Orlagh L. and {Garc{\'i}a-Hernndez}, Antonio and Monteiro, Mario J.P.F.G. and Moya, Andr{\'e}s and Quirion, Pierre Olivier and Sousa, Sergio G. and Surez, Juan Carlos and Appourchaux, Thierry and Arentoft, Torben and Ballot, Jerome and Bedding, Timothy R. and {Christensen-Dalsgaard}, J{\o}rgen and Elsworth, Yvonne and Fletcher, Stephen T. and Garc{\'i}a, Rafael A. and Houdek, G{\"u}nter and {Jim{\'e}nez-Reyes}, Sebastian J. and Kjeldsen, Hans and New, Roger and R{\'e}gulo, Clara and Salabert, David and Toutain, Thierry},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {700},
  number = {2},
  pages = {1589--1602},
  issn = {15384357},
  doi = {10.1088/0004-637X/700/2/1589},
  abstract = {For distant stars, as observed by the NASA Kepler satellite, parallax information is currently of fairly low quality and is not complete. This limits the precision with which the absolute sizes of the stars and their potential transiting planets can be determined by traditional methods. Asteroseismology will be used to aid the radius determination of stars observed during NASA's Kepler mission. We report on the recent asteroFLAG hare-and-hounds Exercise\#2, where a group of "hares" simulated data of F-K main-sequence stars that a group of "hounds" sought to analyze, aimed at determining the stellar radii. We investigated stars in the range 9 {$<$} V {$<$} 15, both with and without parallaxes. We further test different uncertainties in T eff, and compare results with and without using asteroseismic constraints. Based on the asteroseismic large frequency spacing, obtained from simulations of 4 yr time series data from the Kepler mission, we demonstrate that the stellar radii can be correctly and precisely determined, when combined with traditional stellar parameters from the Kepler Input Catalogue. The radii found by the various methods used by each independent hound generally agree with the true values of the artificial stars to within 3\%, when the large frequency spacing is used. This is 5-10 times better than the results where seismology is not applied. These results give strong confidence that radius estimation can be performed to better than 3\% for solar-like stars using automatic pipeline reduction. Even when the stellar distance and luminosity are unknown we can obtain the same level of agreement. Given the uncertainties used for this exercise we find that the input log g and parallax do not help to constrain the radius, and that T eff and metallicity are the only parameters we need in addition to the large frequency spacing. It is the uncertainty in the metallicity that dominates the uncertainty in the radius. \textcopyright{} 2009 The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WBC7IZMH/Stello et al. - 2009.pdf}
}

@article{Stello2009a,
  title = {The Relation between {{$\Delta\nu$}} and {$N$}max for Solar-like Oscillations},
  author = {Stello, D. and Chaplin, W. J. and Basu, S. and Elsworth, Y. and Bedding, T. R.},
  year = {2009},
  journal = {Monthly Notices of the Royal Astronomical Society: Letters},
  volume = {400},
  number = {1},
  eprint = {0909.5193},
  pages = {80--84},
  issn = {17453933},
  doi = {10.1111/j.1745-3933.2009.00767.x},
  abstract = {Establishing relations between global stellar parameters and asteroseismic quantities can help improve our understanding of stellar astrophysics and facilitate the interpretation of observations. We present an observed relation between the large frequency separation, {$\Delta\nu$}, and the frequency of maximum power, {$\nu$}max. We find that {$\Delta\nu$} {$\alpha$} {$\nu$}0.77max, allowing prediction of {$\Delta\nu$} to about 15 per cent given {$\nu$}max. Our result is further supported by established scaling relations for {$\Delta\nu$} and {$\nu$}max and by extended stellar model calculations, which confirm that {$\Delta\nu$} can be estimated using this relation for basically any star showing solar-like oscillations in the investigated range (0.5 {$<$} M/M {$\odot$} {$<$} 4.0). \textcopyright{} 2009 The Authors. Journal compilation \textcopyright{} 2009 RAS.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/4ACDWZKN/Stello et al. - 2009(2).pdf}
}

@article{Stello2010a,
  title = {Detection of Solar-like Oscillations from Kepler Photometry of the Open Cluster {{NGC}} 6819},
  author = {Stello, Dennis and Basu, Sarbani and Bruntt, Hans and Mosser, Benot and Stevens, Ian R. and Brown, Timothy M. and {Christensen-Dalsgaard}, J{\o}rgen and Gilliland, Ronald L. and Kjeldsen, Hans and Arentoft, Torben and Ballot, J{\'e}rme and Barban, Caroline and Bedding, Timothy R. and Chaplin, William J. and Elsworth, Yvonne P. and Garc{\'i}a, Rafael A. and Goupil, Marie Jo and Hekker, Saskia and Huber, Daniel and Mathur, Savita and Meibom, S{\o}ren and Sangaralingam, Vinothini and Baldner, Charles S. and Belkacem, Kevin and Biazzo, Katia and Brogaard, Karsten and Su{\'a}rez, Juan Carlos and D'Antona, Francesca and Demarque, Pierre and Esch, Lisa and Gai, Ning and Grundahl, Frank and Lebreton, Yveline and Jiang, Biwei and Jevtic, Nada and Karoff, Christoffer and Miglio, Andrea and {Molenda-Akowicz}, Joanna and Montalbn, Josefina and Noels, Arlette and Cort{\'e}s, Teodoro Roca and Roxburgh, Ian W. and Serenelli, Aldo M. and Aguirre, Victor Silva and Sterken, Christiaan and Stine, Peter and Szab{\'o}, Robert and Weiss, Achim and Borucki, William J. and Koch, David and Jenkins, Jon M.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {713},
  number = {2 PART 2},
  issn = {20418213},
  doi = {10.1088/2041-8205/713/2/L182},
  abstract = {Asteroseismology of stars in clusters has been a long-sought goal because the assumption of a common age, distance, and initial chemical composition allows strong tests of the theory of stellar evolution. We report results from the first 34days of science data from the Kepler Mission for the open cluster NGC 6819 - one of the four clusters in the field of view. We obtain the first clear detections of solar-like oscillations in the cluster red giants and are able to measure the large frequency separation, {$\Delta\nu$}, and the frequency of maximum oscillation power, {$\nu$}max. We find that the asteroseismic parameters allow us to test cluster membership of the stars, and even with the limited seismic data in hand, we can already identify four possible non-members despite their having a better than 80\% membership probability from radial velocity measurements. We are also able to determine the oscillation amplitudes for stars that span about 2 orders of magnitude in luminosity and find good agreement with the prediction that oscillation amplitudes scale as the luminosity to the power of 0.7. These early results demonstrate the unique potential of asteroseismology of the stellar clusters observed by Kepler. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  keywords = {notion,notion-database,Open clusters and associations: individual (NGC 68,Stars: fundamental parameters,Stars: Interiors,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/WUI6DN6Z/Stello et al. - 2010.pdf}
}

@article{Stello2010b,
  title = {Solar-like Oscillations in Cluster Stars},
  author = {Stello, D. and Basu, S. and Bedding, T. R. and Brogaard, K. and Bruntt, H. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Demarque, P. and Elsworth, Y. P. and Garc{\'i}a, R. A. and Gilliland, R. L. and Hekker, S. and Huber, D. and Karoff, C. and Kjeldsen, H. and Lebreton, Y. and Mathur, S. and Meibom, S. and {Molenda-Zakowicz}, J. and Noels, A. and Roxburgh, I. W. and Aguirre, V. S. and Sterken, C. and Szab{\"o}, R.},
  year = {2010},
  journal = {Astronomische Nachrichten},
  volume = {331},
  number = {9-10},
  eprint = {1007.0009},
  pages = {985--988},
  issn = {00046337},
  doi = {10.1002/asna.201011442},
  abstract = {We present a brief overview of the history of attempts to obtain a clear detection of solar-like oscillations in cluster stars, and discuss the results on the first clear detection, which was made by the Kepler Asteroseismic Science Consortium (KASC) Working Group 2. \textcopyright{} 2010 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Open clusters and associations: individual (NGC 68,Stars: fundamental parameters,Stars: interiors,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/9C6DEP66/Stello et al. - 2010(2).pdf}
}

@article{Stello2011,
  title = {Amplitudes of Solar-like Oscillations: {{Constraints}} from Red Giants in Open Clusters Observed by {{Kepler}}},
  author = {Stello, Dennis and Huber, Daniel and Kallinger, Thomas and Basu, Sarbani and Mosser, Beno{\^i}t and Hekker, Saskia and Mathur, Savita and Garc{\'i}a, Rafael A. and Bedding, Timothy R. and Kjeldsen, Hans and Gilliland, Ronald L. and Verner, Graham A. and Chaplin, William J. and Benomar, Othman and Meibom, S{\o}ren and Grundahl, Frank and Elsworth, Yvonne P. and {Molenda-Zakowicz}, Joanna and Szab{\'o}, Robert and {Christensen-Dalsgaard}, J{\o}rgen and Tenenbaum, Peter and Twicken, Joseph D. and Uddin, Kamal},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {737},
  number = {1},
  eprint = {1107.0490},
  issn = {20418205},
  doi = {10.1088/2041-8205/737/1/L10},
  abstract = {Scaling relations that link asteroseismic quantities to global stellar properties are important for gaining understanding of the intricate physics that underpins stellar pulsations. The common notion that all stars in an open cluster have essentially the same distance, age, and initial composition implies that the stellar parameters can be measured to much higher precision than what is usually achievable for single stars. This makes clusters ideal for exploring the relation between the mode amplitude of solar-like oscillations and the global stellar properties. We have analyzed data obtained with NASA's Kepler space telescope to study solar-like oscillations in 100 red giant stars located in either of the three open clusters, NGC6791, NGC6819, and NGC6811. By fitting the measured amplitudes to predictions from simple scaling relations that depend on luminosity, mass, and effective temperature, we find that the data cannot be described by any power of the luminosity-to-mass ratio as previously assumed. As a result we provide a new improved empirical relation which treats luminosity and mass separately. This relation turns out to also work remarkably well for main-sequence and subgiant stars. In addition, the measured amplitudes reveal the potential presence of a number of previously unknown unresolved binaries in the red clump in NGC6791 and NGC6819, pointing to an interesting new application for asteroseismology as a probe into the formation history of open clusters. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {binaries: general,notion,notion-database,open clusters and associations: individual (NGC 67,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TDF4IH6Z/Stello et al. - 2011.pdf}
}

@article{Stello2011a,
  title = {An Asteroseismic Membership Study of the Red Giants in Three Open Clusters Observed by {{Kepler}}: {{NGC}} 6791, {{NGC}} 6819, and {{NGC}} 6811},
  author = {Stello, Dennis and Meibom, S{\o}ren and Gilliland, Ronald L. and Grundahl, Frank and Hekker, Saskia and Mosser, Beno{\^i}t and Kallinger, Thomas and Mathur, Savita and Garc{\'i}a, Rafael A. and Huber, Daniel and Basu, Sarbani and Bedding, Timothy R. and Brogaard, Karsten and Chaplin, William J. and Elsworth, Yvonne P. and {Molenda-Zakowicz}, Joanna and Szab{\'o}, Robert and Still, Martin and Jenkins, Jon M. and {Christensen-Dalsgaard}, J{\o}rgen and Kjeldsen, Hans and Serenelli, Aldo M. and Wohler, Bill},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {739},
  number = {1},
  eprint = {1107.1234},
  issn = {15384357},
  doi = {10.1088/0004-637X/739/1/13},
  abstract = {Studying star clusters offers significant advances in stellar astrophysics due to the combined power of having many stars with essentially the same distance, age, and initial composition. This makes clusters excellent test benches for verification of stellar evolution theory. To fully exploit this potential, it is vital that the star sample is uncontaminated by stars that are not members of the cluster. Techniques for determining cluster membership therefore play a key role in the investigation of clusters. We present results on three clusters in the Kepler field of view based on a newly established technique that uses asteroseismology to identify fore- or background stars in the field, which demonstrates advantages over classical methods such as kinematic and photometry measurements. Four previously identified seismic non-members in NGC 6819 are confirmed in this study, and three additional non-members are found - two in NGC 6819 and one in NGC 6791. We further highlight which stars are, or might be, affected by blending, which needs to be taken into account when analyzing these Kepler data. \textcopyright{} 2011. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,open clusters and associations: individual (NGC 67,stars: fundamental Parameters,stars: interiors,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/6S8CFF7I/Stello et al. - 2011(2).pdf}
}

@article{Stello2013a,
  title = {Asteroseismic Classification of Stellar Populations among 13,000 Red Giants Observed by Kepler},
  author = {Stello, Dennis and Huber, Daniel and Bedding, Timothy R. and Benomar, Othman and Bildsten, Lars and Elsworth, Yvonne P. and Gilliland, Ronald L. and Mosser, Beno{\^i}t and Paxton, Bill and White, Timothy R.},
  year = {2013},
  journal = {Astrophysical Journal Letters},
  volume = {765},
  number = {2},
  eprint = {1302.0858},
  issn = {20418205},
  doi = {10.1088/2041-8205/765/2/L41},
  abstract = {Of the more than 150,000 targets followed by the Kepler Mission, about 10\% were selected as red giants. Due to their high scientific value, in particular for Galaxy population studies and stellar structure and evolution, their Kepler light curves were made public in late 2011. More than 13,000 (over 85\%) of these stars show intrinsic flux variability caused by solar-like oscillations making them ideal for large-scale asteroseismic investigations. We automatically extracted individual frequencies and measured the period spacings of the dipole modes in nearly every red giant. These measurements naturally classify the stars into various populations, such as the red giant branch, the low-mass (M/M {$\odot$} {$\lessequivlnt$} 1.8) helium-core-burning red clump, and the higher-mass (M/M {$\odot$} {$\greaterequivlnt$} 1.8) secondary clump. The period spacings also reveal that a large fraction of the stars show rotationally induced frequency splittings. This sample of stars will undoubtedly provide an extremely valuable source for studying the stellar population in the direction of the Kepler field, in particular when combined with complementary spectroscopic surveys. \textcopyright{} 2013 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,stars: evolution,stars: fundamental parameters,stars: interiors,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/E2WYM4LE/Stello et al. - 2013.pdf}
}

@article{Stello2014,
  title = {Non-Radial Oscillations in m-Giant Semi-Regular Variables: {{Stellar}} Models and Kepler Observations},
  author = {Stello, Dennis and Compton, Douglas L. and Bedding, Timothy R. and {Christensen-Dalsgaard}, J{\o}rgen and Kiss, Laszlo L. and Kjeldsen, Hans and Bellamy, Beau and Garc{\'i}a, Rafael A. and Mathur, Savita},
  year = {2014},
  journal = {Astrophysical Journal Letters},
  volume = {788},
  number = {1},
  eprint = {1406.0003},
  issn = {20418213},
  doi = {10.1088/2041-8205/788/1/L10},
  abstract = {The success of asteroseismology relies heavily on our ability to identify the frequency patterns of stellar oscillation modes. For stars like the Sun this is relatively easy because the mode frequencies follow a regular pattern described by a well-founded asymptotic relation. When a solar-like star evolves off the main sequence and onto the red giant branch its structure changes dramatically, resulting in changes in the frequency pattern of the modes. We follow the evolution of the adiabatic frequency pattern from the main sequence to near the tip of the red giant branch for a series of models. We find a significant departure from the asymptotic relation for the non-radial modes near the red giant branch tip, resulting in a triplet frequency pattern. To support our investigation we analyze almost four years of Kepler data of the most luminous stars in the field (late K and early M type) and find that their frequency spectra indeed show a triplet pattern dominated by dipole modes even for the most luminous stars in our sample. Our identification explains previous results from ground-based observations reporting fine structure in the Petersen diagram and sub-ridges in the period-luminosity diagram. Finally, we find "new ridges" of non-radial modes with frequencies below the fundamental mode in our model calculations, and we speculate they are related to f modes. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/VAA8DFYQ/Stello et al. - 2014.pdf}
}

@article{Stello2015,
  title = {Oscillating Red Giants Observed during Campaign 1 of the {{Kepler K2}} Mission: {{New}} Prospects for Galactic Archaeology},
  author = {Stello, Dennis and Huber, Daniel and Sharma, Sanjib and Johnson, Jennifer and Lund, Mikkel N. and Handberg, Rasmus and Buzasi, Derek L. and Aguirre, Victor Silva and Chaplin, William J. and Miglio, Andrea and Pinsonneault, Marc and Basu, Sarbani and Bedding, Tim R. and {Bland-Hawthorn}, Joss and Casagrande, Luca and Davies, Guy and Elsworth, Yvonne and Garcia, Rafael A. and Mathur, Savita and Mauro, Maria Pia Di and Mosser, Benoit and Schneider, Donald P. and Serenelli, Aldo and Valentini, Marica},
  year = {2015},
  journal = {Astrophysical Journal Letters},
  volume = {809},
  number = {1},
  eprint = {1506.08931},
  pages = {L3},
  publisher = {{IOP Publishing}},
  issn = {20418213},
  doi = {10.1088/2041-8205/809/1/L3},
  abstract = {NASA's re-purposed Kepler mission - dubbed K2 - has brought new scientific opportunities that were not anticipated for the original Kepler mission. One science goal that makes optimal use of K2's capabilities, in particular its 360\textdegree{} ecliptic field of view, is galactic archaeology - the study of the evolution of the Galaxy from the fossil stellar record. The thrust of this research is to exploit high-precision, time-resolved photometry from K2 in order to detect oscillations in red giant stars. This asteroseismic information can provide estimates of stellar radius (hence distance), mass, and age of vast numbers of stars across the Galaxy. Here we present the initial analysis of a subset of red giants, observed toward the north galactic gap, during the mission's first full science campaign. We investigate the feasibility of using K2 data for detecting oscillations in red giants that span a range in apparent magnitude and evolutionary state (hence intrinsic luminosity). We demonstrate that oscillations are detectable for essentially all cool giants within the range {$\sim$}1.9-3.2. Our detection is complete down to , which results in a seismic sample with little or no detection bias. This sample is ideally suited to stellar population studies that seek to investigate potential shortcomings of contemporary Galaxy models.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: evolution,Galaxy: stellar content,Galaxy: structure,notion,notion-database,stars: fundamental parameters,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/EBBRRAYW/Stello et al. - 2015.pdf}
}

@article{Stello2016,
  title = {The {{K2 Galactic Archaeology Program Data Release}} 1: {{Asteroseismic}} Results from {{Campaign}} 1},
  author = {Stello, D. and Zinn, J. and Elsworth, Y. and Garcia, R. A. and Kallinger, T. and Mathur, S. and Mosser, B. and Sharma, S. and Chaplin, W. J. and Davies, G. and Huber, D. and Jones, C. D. and Miglio, A. and Aguirre, V. S.},
  year = {2016},
  eprint = {1611.09852},
  doi = {10.3847/1538-4357/835/1/83},
  abstract = {NASA's K2 mission is observing tens of thousands of stars along the ecliptic, providing data suitable for large scale asteroseismic analyses to inform galactic archaeology studies. Its first campaign covered a field near the north galactic cap, a region never covered before by large asteroseismic-ensemble investigations, and was therefore of particular interest for exploring this part of our Galaxy. Here we report the asteroseismic analysis of all stars selected by the K2 Galactic Archaeology Program during the mission's "North Galactic Cap" campaign 1. Our consolidated analysis uses six independent methods to measure the global seismic properties, in particular the large frequency separation, and the frequency of maximum power. From the full target sample of 8630 stars we find about 1200 oscillating red giants, a number comparable with estimates from galactic synthesis modeling. Thus, as a valuable by-product we find roughly 7500 stars to be dwarfs, which provide a sample well suited for galactic exoplanet occurrence studies because they originate from our simple and easily reproducible selection function. In addition, to facilitate the full potential of the data set for galactic archaeology we assess the detection completeness of our sample of oscillating red giants. We find the sample is at least near complete for stars with 40 {$<$} numax/microHz {$<$} 270, and numax\_detec {$<$} 2.6*1e6 * 2e-Kp microHz. There is a detection bias against helium core burning stars with numax \textasciitilde{} 30 microHz, affecting the number of measurements of DeltaNu and possibly also numax. Although we can detect oscillations down to Kp = 15, our campaign 1 sample lacks enough faint giants to assess the detection completeness for stars fainter than Kp \textasciitilde{} 14.5.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/57VWQHTW/Stello et al. - 2016.pdf}
}

@article{Stello2016a,
  title = {Suppression of Quadrupole and Octupole Modes in Red Giants Observed by {{Kepler}}},
  author = {Stello, Dennis and Cantiello, Matteo and Fuller, Jim and Garcia, Rafael A. and Huber, Daniel},
  year = {2016},
  journal = {Publications of the Astronomical Society of Australia},
  volume = {33},
  pages = {1--6},
  issn = {14486083},
  doi = {10.1017/pasa.2016.9},
  abstract = {An exciting new theoretical result shows that observing suppression of dipole oscillation modes in red giant stars can be used to detect strong magnetic fields in the stellar cores. A fundamental facet of the theory is that nearly all the mode energy leaking into the core is trapped by the magnetic greenhouse effect. This results in clear predictions for how the mode visibility changes as a star evolves up the red giant branch, and how that depends on stellar mass, spherical degree, and mode lifetime. Here, we investigate the validity of these predictions with a focus on the visibility of different spherical degrees. We find that mode suppression weakens for higher degree modes with a reduction in the quadrupole mode visibility of up to 49\%, and no detectable suppression of octupole modes, in agreement with theory. We find evidence for the influence of increasing mode lifetimes on the visibilities along the red giant branch, in agreement with previous independent observations. These results support the theory that strong internal magnetic fields cause suppression of non-radial modes in red giants. We also find preliminary evidence that stars with suppressed dipole modes on average have slightly lower metallicity than normal stars.},
  keywords = {notion,notion-database,Stars: Fundamental parameters,Stars: Interiors,Stars: Magnetic field,Stars: Oscillations},
  file = {/Users/lbugnet/Zotero/storage/8JWLLFFI/Stello et al. - 2016(2).pdf}
}

@article{Stello2016b,
  title = {A Prevalence of Dynamo-Generated Magnetic Fields in the Cores of Intermediate-Mass Stars},
  author = {Stello, Dennis and Cantiello, Matteo and Fuller, Jim and Huber, Daniel and Garci{\'a}, Rafael A. and Bedding, Timothy R. and Bildsten, Lars and Aguirre, Victor Silva},
  year = {2016},
  journal = {Nature},
  volume = {529},
  number = {7586},
  eprint = {1601.00004},
  pages = {364--367},
  publisher = {{Nature Publishing Group}},
  issn = {14764687},
  doi = {10.1038/nature16171},
  abstract = {Magnetic fields play a part in almost all stages of stellar evolution. Most low-mass stars, including the Sun, show surface fields that are generated by dynamo processes in their convective envelopes. Intermediate-mass stars do not have deep convective envelopes, although 10 per cent exhibit strong surface fields that are presumed to be residuals from the star formation process. These stars do have convective cores that might produce internal magnetic fields, and these fields might survive into later stages of stellar evolution, but information has been limited by our inability to measure the fields below the stellar surface. Here we report the strength of dipolar oscillation modes for a sample of 3,600 red giant stars. About 20 per cent of our sample show mode suppression, by strong magnetic fields in the cores, but this fraction is a strong function of mass. Strong core fields occur only in red giants heavier than 1.1 solar masses, and the occurrence rate is at least 50 per cent for intermediate-mass stars (1.6-2.0 solar masses), indicating that powerful dynamos were very common in the previously convective cores of these stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AMGMPFLX/Stello et al. - 2016(5).pdf}
}

@article{Stello2017,
  title = {Asteroseismic Masses of Retired Planet-Hosting {{A-stars}} Using {{SONG}}},
  author = {Stello, Dennis and Huber, Daniel and Grundahl, Frank and Lloyd, James and Ireland, Mike and Casagrande, Luca and Fredslund, Mads and Bedding, Timothy R. and Palle, Pere L. and Antoci, Victoria and Kjeldsen, Hans and {Christensen-Dalsgaard}, J{\o}rgen},
  year = {2017},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {472},
  number = {4},
  eprint = {1708.09613},
  issn = {13652966},
  doi = {10.1093/mnras/stx2295},
  abstract = {To better understand how planets form, it is important to study planet occurrence rates as a function of stellar mass. However, estimating masses of field stars is often difficult. Over the past decade, a controversy has arisen about the inferred occurrence rate of gas-giant planets around evolved intermediate-mass stars - the so-called 'retired A-stars'. The high masses of these red-giant planet hosts, derived using spectroscopic information and stellar evolution models, have been called into question. Here, we address the controversy by determining the masses of eight evolved planet-hosting stars using asteroseismology. We compare the masses with spectroscopic-based masses from the Exoplanet Orbit Database,which were previously adopted to infer properties of the exoplanets and their hosts. We find a significant one-sided offset between the two sets of masses for stars with spectroscopic masses above roughly 1.6 MO\textperiodcentered, suggestive of an average 15-20 per cent overestimate of the adopted spectroscopic-based masses. The only star in our sample well below this mass limit is also the only one not showing this offset. Finally, we note that the scatter across literature values of spectroscopic-based masses often exceeds their formal uncertainties, making it comparable to the offset we report here.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Stevenson1978,
  title = {Turbulent Thermal Convection in the Presence of Rotation and a Magnetic Field: {{A}} Heuristic Theory},
  author = {Stevenson, David J.},
  year = {1978},
  month = jan,
  journal = {http://dx.doi.org/10.1080/03091927908242681},
  volume = {12},
  number = {1},
  pages = {139--169},
  publisher = {{Taylor \& Francis Group}},
  issn = {10290419},
  doi = {10.1080/03091927908242681},
  urldate = {2022-01-26},
  abstract = {The growth of linear, Boussinesq convective modes for a superadiabatic fluid in a planar geometry with negligible thermal diffusion or molecular viscosity is analysed. Small and large magnetic diff...},
  keywords = {notion,notion-database}
}

@article{Stone1996,
  title = {Three-Dimensional {{Magnetohydrodynamical Simulations}} of {{Vertically Stratified Accretion Disks}}},
  author = {Stone, James M. and Hawley, John F. and Gammie, Charles F. and Balbus, Steven A.},
  year = {1996},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {463},
  pages = {656},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/177280},
  urldate = {2020-07-02},
  abstract = {We present three-dimensional magnetohydrodynamical simulations of the nonlinear evolution of the magnetorotational instability (Balbus \& Hawley 1991) in an initially isothermal, vertically stratified accretion disk. The simulations are local in the plane of the disk, but are global in the vertical direction in the sense that the computational domain encompasses several scale heights. We find that the instability generates and maintains magnetohydrodynamic turbulence in stratified disks. The properties of the saturated, turbulent state are similar to those reported for nonstratified homogeneous boxes, e.g., the power-law spectral distribution is consistent with Kolmogorov. The angular momentum transport rate is proportional to the magnetic pressure; if the average rate is scaled to the equatorial pressure, as in a standard ''alpha-disk'' model, the constant of proportionality is alpha less than or similar to 0.01 for most of our simulations. This value may be limited somewhat by the numerical resolution of our simulations. We find buoyancy does not play an important role as a saturation mechanism. The nonlinear evolution of disks that begin with a variety of initial magnetic field geometries and strengths is similar. In particular, models in which the most unstable wavelengths are initially well resolved saturate at and maintain roughly the same magnetic energy density, suggesting dynamo action in the disk.We use the simulations to study the effect of the instability on the vertical structure of magnetic accretion disks. After saturation, the disk consists of a weakly magnetized core surrounded by a strongly magnetized corona. Changing the vertical boundary conditions does not significantly alter this structure. The vertical flux of magnetic energy is small compared to the local magnetic energy generation and dissipation rates; The disk is stable to Parker and buoyancy modes. Models evolved with an adiabatic equation of state undergo substantial heating due to nonlinear dissipation, resulting in an increase in the scale height of the disk. The vertical structure produced by the instability, particularly the presence of a strongly magnetized corona, may have relevance to the production of MHD winds from disks.},
  keywords = {ACCRETION,ACCRETION DISKS,INSTABILITIES,MAGNETOHYDRODYNAMICS: MHD,METHODS: NUMERICAL,notion,notion-database}
}

@article{Strassmeier2008,
  title = {Starspots: Signatures of Stellar Magnetic Activity},
  author = {Strassmeier, Klaus G.},
  year = {2008},
  journal = {Proceedings of the International Astronomical Union},
  volume = {4},
  number = {S259},
  pages = {363--368},
  issn = {1743-9213},
  doi = {10.1017/s1743921309030737},
  abstract = {Starspots, just as Sunspots, are among the most obvious tracers and signatures of stellar surface magnetic activity. Emphasized already several decades ago as the origin for the rotationally modulated brightness of cool late-type stars, it is just now that we start to trace individual surface features in great enough detail to understand their magnetic behavior and interaction. Starspots also became the most important ``noise'' for detecting extra-solar planets and could possibly be decisive when it comes to detect another Earth. Since this is not a review, and because indirect imaging techniques are covered in other papers in this volume, I focus in this paper on some specific detections of starspots and introduce four new facilities particularly suited for starspot research in the near future.},
  keywords = {instrumentation,magnetic fields,meth-,methods,notion,notion-database,ods,photometric,rotation,spectrographs,spectroscopic,spots,stars},
  file = {/Users/lbugnet/Zotero/storage/B84BS7AK/Strassmeier - 2008.pdf}
}

@book{Strassmeier2009,
  title = {Starspots},
  author = {Strassmeier, Klaus G.},
  year = {2009},
  journal = {Astronomy and Astrophysics Review},
  volume = {17},
  issn = {09354956},
  doi = {10.1007/s00159-009-0020-6},
  abstract = {Starspots are created by local magnetic fields on the surfaces of stars, just as sunspots. Their fields are strong enough to suppress the overturning convective motion and thus block or redirect the flow of energy from the stellar interior outwards to the surface and consequently appear as locally cool and therefore dark regions against an otherwise bright photosphere (Biermann in Astronomische Nachrichten 264:361, 1938; Z Astrophysik 25:135, 1948). As such, starspots are observable tracers of the yet unknown internal dynamo activity and allow a glimpse into the complex internal stellar magnetic field structure. Starspots also enable the precise measurement of stellar rotation which is among the key ingredients for the expected internal magnetic topology. But whether starspots are just blown-up sunspot analogs, we do not know yet. This article is an attempt to review our current knowledge of starspots. A comparison of a white-light image of the Sun (G2V, 5 Gyr) with a Doppler image of a young solar-like star (EK Draconis; G1.5V, age 100 Myr, rotation 10 \texttimes{} {$\Omega$} Sun) and with a mean-field dynamo simulation suggests that starspots can be of significantly different appearance and cannot be explained with a scaling of the solar model, even for a star of same mass and effective temperature. Starspots, their surface location and migration pattern, and their link with the stellar dynamo and its internal energy transport, may have far reaching impact also for our understanding of low-mass stellar evolution and formation. Emphasis is given in this review to their importance as activity tracers in particular in the light of more and more precise exoplanet detections around solar-like, and therefore likely spotted, host stars. \textcopyright{} 2009 Springer-Verlag.},
  isbn = {0015900900206},
  keywords = {Exoplanets,Magnetic fields,notion,notion-database,Stars: activity,Stars: imaging,Stars: rotation,Starspots,Sunspots,Techniques: polarimetric},
  file = {/Users/lbugnet/Zotero/storage/RP8EKQE9/Strassmeier - 2009.pdf}
}

@article{Strugarek2011,
  title = {Magnetic Confinement of the Solar Tachocline: {{II}}. {{Coupling}} to a Convection Zone},
  author = {Strugarek, A. and Brun, A. S. and Zahn, J. P.},
  year = {2011},
  journal = {Astronomy \& Astrophysics},
  volume = {532},
  eprint = {1107.3665},
  issn = {00046361},
  doi = {10.1051/0004-6361/201116518},
  abstract = {Context. The reason for the observed thinness of the solar tachocline is still not well understood. One of the explanations that have been proposed is that a primordial magnetic field renders the rotation uniform in the radiation zone. Aims. We test here the validity of this magnetic scenario through 3D numerical MHD simulations that encompass both the radiation zone and the convection zone. Methods. The numerical simulations are performed with the anelastic spherical harmonics (ASH) code. The computational domain extends from 0.07R{$\cdot$} to 0.97R{$\cdot$}. Results. In the parameter regime we explored, a dipolar fossil field aligned with the rotation axis cannot remain confined in the radiation zone. When the field lines are allowed to interact with turbulent unstationary convective motions at the base of the convection zone, 3D effects prevent the field confinement. Conclusions. In agreement with previous work, we find that a dipolar fossil field, even when it is initially buried deep inside the radiation zone, will spread into the convective zone. According to Ferraro's law of iso-rotation, it then imprints on the radiation zone the latitudinal differential rotation of the convection zone, which is not observed. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  keywords = {Convection,Magnetic fields,Magnetohydrodynamics (MHD),notion,notion-database,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/N8SHYINE/Strugarek, Brun, Zahn - 2011.pdf}
}

@article{Strugarek2011a,
  title = {Magnetic Confinement of the Solar Tachocline: {{The}} Oblique Dipole},
  author = {Strugarek, A. and Brun, A. S. and Zahn, J. P.},
  year = {2011},
  journal = {Astronomische Nachrichten},
  volume = {332},
  number = {9-10},
  pages = {891--896},
  issn = {00046337},
  doi = {10.1002/asna.201111613},
  abstract = {3D MHD global solar simulations coupling the turbulent convective zone and the radiative zone have been carried out. Essential features of the Sun such as differential rotation, meridional circulation and internal waves excitation are recovered. These realistic models are used to test the possibility of having the solar tachocline confined by a primordial inner magnetic field. We find that the initially confined magnetic fields we consider open into the convective envelope. Angular momentum is transported across the two zones by magnetic torques and stresses, establishing the so-called Ferarro's law of isorotation. In the parameter space studied, the confinement of the magnetic field by meridional circulation penetration fails, also implying the failure of the tachocline confinement by the magnetic field. Three-dimensional convective motions are proven responsible for the lack of magnetic field confinement. Those results are robust for the different magnetic field topologies considered, i.e. aligned or oblique dipole. \textcopyright{} 2011 WILEY-VCH Verlag GmbH \& Co. KGaA, Weinheim.},
  keywords = {Convection,Magnetohydrodynamics (MHD),notion,notion-database,Sun: interior,Sun: magnetic fields,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/926JGBQL/Strugarek, Brun, Zahn - 2011(2).pdf}
}

@article{Strugarek2011b,
  title = {Magnetic Confinement of the Solar Tachocline: {{II}}. {{Coupling}} to a Convection Zone},
  shorttitle = {Magnetic Confinement of the Solar Tachocline},
  author = {Strugarek, A. and Brun, A. S. and Zahn, J. -P.},
  year = {2011},
  month = aug,
  journal = {Astronomy \& Astrophysics},
  volume = {532},
  pages = {A34},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201116518},
  urldate = {2023-10-11},
  abstract = {Context. The reason for the observed thinness of the solar tachocline is still not well understood. One of the explanations that have been proposed is that a primordial magnetic field renders the rotation uniform in the radiation zone. Aims: We test here the validity of this magnetic scenario through 3D numerical MHD simulations that encompass both the radiation zone and the convection zone. Methods: The numerical simulations are performed with the anelastic spherical harmonics (ASH) code. The computational domain extends from 0.07R{$\odot$} to 0.97R{$\odot$}. Results: In the parameter regime we explored, a dipolar fossil field aligned with the rotation axis cannot remain confined in the radiation zone. When the field lines are allowed to interact with turbulent unstationary convective motions at the base of the convection zone, 3D effects prevent the field confinement. Conclusions: In agreement with previous work, we find that a dipolar fossil field, even when it is initially buried deep inside the radiation zone, will spread into the convective zone. According to Ferraro's law of iso-rotation, it then imprints on the radiation zone the latitudinal differential rotation of the convection zone, which is not observed.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,convection,magnetic fields,magnetohydrodynamics (MHD),Sun: interior,Sun: rotation},
  annotation = {ADS Bibcode: 2011A\&A...532A..34S},
  file = {/Users/lbugnet/Zotero/storage/342XHX7J/Strugarek et al. - 2011 - Magnetic confinement of the solar tachocline II. .pdf}
}

@article{Strugarek2014,
  title = {On the Diversity of Magnetic Interactions in Close-in Star-Planet Systems},
  author = {Strugarek, A. and Brun, A. S. and Matt, S. P. and R{\'e}ville, V.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {795},
  number = {1},
  eprint = {1409.5268},
  issn = {15384357},
  doi = {10.1088/0004-637X/795/1/86},
  abstract = {Magnetic interactions between close-in planets and their host star can play an important role in the secular orbital evolution of the planets, as well as the rotational evolution of their host. As long as the planet orbits inside the Alfv\'en surface of the stellar wind, the magnetic interaction between the star and the planet can modify the wind properties and also lead to direct angular momentum transfers between the two. We model these star-planet interactions using compressible magnetohydrodynamic (MHD) simulations, and quantify the angular momentum transfers between the star, the planet, and the stellar wind. We study the cases of magnetized and non-magnetized planets and vary the orbital radius inside the Alfv\'en surface of the stellar wind. Based on a grid of numerical simulations, we propose general scaling laws for the modification of the stellar wind torque, for the torque between the star and the planet, and for the planet migration associated with the star-planet magnetic interactions. We show that when the coronal magnetic field is large enough and the star is rotating sufficiently slowly, the effect of the magnetic star-planet interaction is comparable to tidal effects and can lead to a rapid orbital decay.},
  archiveprefix = {arxiv},
  keywords = {magnetohydrodynamics (MHD),notion,notion-database,outflows,planet,planets and satellites: dynamical evolution and st,star interactions,stars: winds},
  file = {/Users/lbugnet/Zotero/storage/E22I7L9G/Strugarek et al. - 2014.pdf}
}

@article{Strugarek2017,
  title = {Reconciling Solar and Stellar Magnetic Cycles with Nonlinear Dynamo Simulations},
  author = {Strugarek, A. and Beaudoin, P. and Charbonneau, P. and Brun, A. S. and do Nascimento, J. -D.},
  year = {2017},
  month = jul,
  journal = {Science},
  volume = {357},
  number = {6347},
  eprint = {1707.04335},
  pages = {185--187},
  publisher = {{American Association for the Advancement of Science}},
  doi = {10.1126/science.aal3999},
  urldate = {2020-07-03},
  abstract = {The magnetic fields of solar-type stars are observed to cycle over decadal periods -11 years in the case of the Sun. The fields originate in the turbulent convective layers of stars and have a complex dependency upon stellar rotation rate. We have performed a set of turbulent global simulations that exhibit magnetic cycles varying systematically with stellar rotation and luminosity. We find that the magnetic cycle period is inversely proportional to the Rossby number, which quantifies the influence of rotation on turbulent convection. The trend relies on a fundamentally non-linear dynamo process and is compatible with the Sun's cycle and those of other solar-type stars.},
  archiveprefix = {arxiv},
  keywords = {ASTRONOMY,Astrophysics,notion,notion-database,Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/6N9Z3V9Z/full-text.pdf}
}

@article{Sturrock2005,
  title = {Combined and Comparative Analysis of Power Spectra},
  author = {Sturrock, P. A. and Scargle, J. D. and Walther, G. and Wheatland, M. S.},
  year = {2005},
  journal = {Solar Physics},
  volume = {227},
  number = {1},
  pages = {137--153},
  issn = {00380938},
  doi = {10.1007/s11207-005-7424-x},
  abstract = {In solar physics, especially in exploratory stages of research, it is often necessary to compare the power spectra of two or more time series. One may, for instance, wish to estimate what the power spectrum of the combined data sets might have been, or one may wish to estimate the significance of a particular peak that shows up in two or more power spectra. One may also on occasion need to search for a complex of peaks in a single power spectrum, such as a fundamental and one or more harmonics, or a fundamental plus sidebands, etc. Visual inspection can be revealing, but it can also be misleading. This leads one to look for one or more ways of forming statistics, which readily lend themselves to significance estimation, from two or more power spectra. We derive formulas for statistics formed from the sum, the minimum, and the product of two or more power spectra. A distinguishing feature of our formulae is that, if each power spectrum has an exponential distribution, each statistic also has an exponential distribution. The statistic formed from the minimum power of two or more power spectra is well known and has an exponential distribution. The sum of two or more powers also has a well-known distribution that is not exponential, but a simple operation does lead to an exponential distribution. Concerning the product of two or more power spectra, we find an analytical expression for the case n = 2, and a procedure for computing the statistic for n {$>$} 2. We also show that some quite simple expressions give surprisingly good approximations. \textcopyright{} Springer Science + Business Media, Inc. 2005.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WWXNX38C/Sturrock et al. - 2005.pdf}
}

@article{Su2023,
  title = {Asteroseismology of the {{Pulsating Extremely Low-mass White Dwarf SDSS J111215}}.82 + 111745.0: {{A Model}} with p-Mode {{Pulsations Consistent}} with the {{Observations}}},
  shorttitle = {Asteroseismology of the {{Pulsating Extremely Low-mass White Dwarf SDSS J111215}}.82 + 111745.0},
  author = {Su, Jie and Li, Yan},
  year = {2023},
  month = feb,
  journal = {The Astrophysical Journal},
  volume = {943},
  pages = {113},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/aca533},
  urldate = {2023-10-14},
  abstract = {SDSS J111215.82+111745.0 is the second pulsating extremely low-mass white dwarf discovered. Two short-period pulsations, 107.56 and 134.275 s, were detected on this star, which would be the first observed pressure mode (p-mode) pulsations observed on a white dwarf. While the two potential p-modes have yet to be confirmed, they make SDSS J111215.82+111745.0 an interesting object. In this work, we analyzed the whole set of seven periods observed on SDSS J111215.82+111745.0. We adopt three independent period-spacing tests to reveal a roughly 93.4 s mean period spacing of {$\mathscr{l}$} = 1 g-modes, which gives added credence to the {$\mathscr{l}$} = 1 identifications. Then we perform asteroseismic modeling for this star, in which the H chemical profile is taken as a variable. The stellar parameters M = 0.1650 {$\pm$} 0.0137 M {$\Sun$} and T eff = 9750 {$\pm$} 560 K are determined from the best-fit model, and the H/He chemical profiles are also defined. The two suspected p-modes are also well represented in the best-fit model, and both the stellar parameters and the pulsation frequencies are in good agreement with the values derived from spectroscopy.},
  keywords = {1309,1625,1799,73,Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,Pulsation modes,Stellar pulsations,White dwarf stars},
  annotation = {ADS Bibcode: 2023ApJ...943..113S},
  file = {/Users/lbugnet/Zotero/storage/3FH2II6G/Su and Li - 2023 - Asteroseismology of the Pulsating Extremely Low-ma.pdf}
}

@article{Suarez2006,
  title = {Effects of Moderately Fast Shellular Rotation on Adiabatic Oscillations},
  author = {Su{\'a}rez, J. C. and Goupil, M. J. and Morel, P.},
  year = {2006},
  month = apr,
  journal = {Astronomy and Astrophysics},
  volume = {449},
  number = {2},
  pages = {673--685},
  issn = {00046361},
  doi = {10.1051/0004-6361:20054181},
  urldate = {2020-06-02},
  abstract = {We investigate adiabatic oscillations for {$\delta$} Scuti star models, taking a moderate rotation velocity (around 100 km s-1) into account. The resulting oscillation frequencies include corrections for rotation up to second order in the rotation rate including those of near degeneracy. Effects of either a uniform rotation or a rotation profile assuming local angular momentum conservation of the form {$\Omega$} = {$\Omega$}(r) on oscillation frequencies are compared. As expected, important differences (around 3 {$\mu$}Hz) are obtained in the g and mixed-mode regions. For higher-frequency p modes, differences range between 1 {$\mu$}Hz and 3 {$\mu$}Hz. Such differences are likely to be detectable with future space missions such as COROT, where precisions in frequency around 0.5 {$\mu$}Hz are expected to be reached. \textcopyright{} ESO 2006.},
  keywords = {notion,notion-database,Stars: evolution,Stars: fundamental parameters,Stars: interiors,Stars: oscillations,Stars: rotation,Stars: variables: {$\delta$} Sct},
  file = {/Users/lbugnet/Zotero/storage/FQQ5IR5Q/full-text.pdf}
}

@article{Suarez2009,
  title = {Seismology of {$\beta$} {{Cephei}} Stars: {{Differentially}} Rotating Models for Interpreting the Oscillation Spectrum of {$\nu$} {{Eridani}}},
  author = {Su{\'a}rez, J. C. and Moya, A. and Amado, P. J. and {Mart{\'i}n-Ruiz}, S. and {Rodr{\'i}guez-L{\'o}pez}, C. and Garrido, R.},
  year = {2009},
  journal = {Astrophysical Journal},
  volume = {690},
  number = {2},
  eprint = {0811.1436},
  pages = {1401--1411},
  issn = {15384357},
  doi = {10.1088/0004-637X/690/2/1401},
  abstract = {A method for the asteroseismic analysis of {$\beta$} Cephei stars is presented and applied to the star {$\nu$} Eridani. The method is based on the analysis of rotational splittings and their asymmetries using differentially rotating asteroseismic models. Models with masses around 7.13 M {$\odot$}, and ages around 14.9 Myr, were found to fit better in 10 of the 14 observed frequencies, which were identified as the fundamental radial mode and the three {$\mathscr{l}$} = 1 triplets g1, p1, and p2. The splittings and aymmetries found for these modes recover those provided in the literature, except for p2. For this last mode, all its non-axysimmetric components are predicted by the models. Moreover, opposite signs of the observed and predicted splitting asymmetries are found. If identification is confirmed, this can be a very interesting source of information about the internal rotation profile, in particular in the outer regions of the star. In general, the seismic models that include a description for shellular rotation yield slightly better results as compared with those given by uniformly rotating models. Furthermore, we show that asymmetries are quite dependent on the overshooting of the convective core, which makes the present technique suitable for testing the theories describing the angular momentum redistribution and chemical mixing due to rotationally induced turbulence. \textcopyright{} 2009. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual ({$\nu$} Eridani),Stars: interiors,Stars: oscillations (including pulsations),Stars: rotation,Stars: variables: other},
  file = {/Users/lbugnet/Zotero/storage/3J28EUWE/Suárez et al. - 2009.pdf}
}

@article{Suarez2010a,
  title = {On the Interpretation of Echelle Diagrams for Solar-like Oscillations Effect of Centrifugal Distortion},
  author = {Su{\'a}rez, J. C. and Goupil, M. J. and Reese, D. R. and Samadi, R. and Ligni{\`e}res, F. and Rieutord, M. and Lochard, J.},
  year = {2006},
  journal = {Astrophysical Journal},
  volume = {721},
  number = {1},
  eprint = {1009.0123},
  pages = {537--546},
  issn = {15384357},
  doi = {10.1088/0004-637X/721/1/537},
  abstract = {This work aims at determining the impact of slow to moderate rotation on the regular patterns often present in solar-like oscillation spectra, i.e., the frequency spacings. We focus on the well-known asteroseismic diagnostic echelle diagrams, examining how rotation may modify the estimates of the large and small spacings, as well as the identification ofmodes.We illustrate theworkwith a real case: the solar-like star {$\eta$} Bootis.We study amain-sequence 1.3M {$\odot$} star as a typical case. The modeling takes into account rotation effects on the equilibrium models through an effective gravity and on the oscillation frequencies through both perturbative and non-perturbative calculations. We compare the results of both type of calculations in the context of the regular spacings (like the small spacings and the scaled small spacings) and echelle diagrams. We show that for echelle diagrams the perturbative approach remains valid for rotational velocities up to 40-50 km s-1. We show that for the rotational velocities measured in solar-like stars, i.e., v sin i up to 20-30 km s-1, rotation effects must be taken into account in the modeling for a correct interpretation of the observed oscillations. In particular, theoretical oscillation frequencies must be corrected up to the second order in terms of rotation rate, including near degeneracy effects. For rotational velocities of about 16 km s-1 and higher, diagnostics on large spacings and on modal identification through echelle diagrams can be significantly altered by the presence of the m {$\neq$} 0 components of the rotationally split modes. We found these effects to be detectable in the observed frequency range. Analysis of the effects of rotation on small spacings and scaled small spacings reveals that these can be of the order of or even larger than surface effects, typically turbulence, microscopic diffusion, etc. Furthermore, we show that scaled spacings are significantly affected by stellar distortion even for small stellar rotational velocities (from 10 to 15 km s-1) and therefore some care must be taken when using them as indicators for probing deep stellar interiors. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: individual (eta Bootis),Stars: interiors,Stars: oscillations,Stars: rotation,Stars: solar-type,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/MQ8RLNIC/Suárez et al. - 2010.pdf}
}

@article{Suijs2008,
  title = {White Dwarf Spins from Low-Mass Stellar Evolution Models},
  author = {Suijs, L. and Langer, N. and Poelarends, A. J. and Yoon, S. C. and Heger, A. and Herwig, F.},
  year = {2008},
  month = apr,
  journal = {Astronomy \& Astrophysics},
  volume = {481},
  number = {3},
  eprint = {0802.3286},
  pages = {87--90},
  issn = {00046361},
  doi = {10.1051/0004-6361:200809411},
  urldate = {2020-07-05},
  abstract = {Context: The prediction of the spins of the compact remnants is a fundamental goal of the theory of stellar evolution. Aims: Here, we confront the predictions for white dwarf spins from evolutionary models, including rotation with observational constraints.Methods. We perform stellar evolution calculations for stars in the mass range 1... 3, including the physics of rotation, from the zero age main sequence into the TP-AGB stage. We calculate two sets of model sequences, with and without inclusion of magnetic fields. From the final computed models of each sequence, we deduce the angular momenta and rotational velocities of the emerging white dwarfs. Results: While models including magnetic torques predict white dwarf rotational velocities between 2 and 10 km s-1, those from the nonmagnetic sequences are found to be one to two orders of magnitude larger, well above empirical upper limits. Conclusions: We find the situation analogous to that in the neutron star progenitor mass range, and conclude that magnetic torques may be required to understand the slow rotation of compact stellar remnants in general. \textcopyright{} 2008 ESO.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: evolution,Stars: magnetic fields,Stars: rotation,Stars: white dwarfs},
  file = {/Users/lbugnet/Zotero/storage/F2ZPRNP5/full-text.pdf}
}

@article{Sule2005,
  title = {A Numerical {{MHD}} Model for the Solar Tachocline with Meridional Flow},
  author = {Sule, A. and R{\"u}diger, G. and Arlt, R.},
  year = {2005},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {437},
  pages = {1061--1067},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20042086},
  urldate = {2023-10-18},
  abstract = {There are successful approaches to explain the formation of the tachocline by a poloidal magnetic field in the solar core. We present here the first MHD simulations of the solar tachocline which self-consistently include the meridional circulation. We show that the meridional flow significantly changes the shape and the characteristics of the tachocline. We find that after the inclusion of the meridional circulation, a tachocline can be formed even when the poloidal field lines are crossing the boundary between the radiative zone and the convection zone. We also discuss the effects of the magnetic Prandtl number as well as of the magnetic Reynolds number on the properties of the tachocline. The tachocline is much thinner for higher magnetic Reynolds numbers and/or lower magnetic Prandtl numbers. We expect that a poloidal magnetic seed field of around 1 G will be sufficient to produce the tachocline of the Sun. However, the model requires the initial magnetic field to be in a narrow range to satisfy tachocline solutions. The simulations including a stable temperature gradient produce a shallower as well as slower meridional circulation than the ones without it, as required from the lithium abundance at the solar surface.},
  keywords = {magnetohydrodynamics (MHD),Sun: interior,Sun: magnetic fields,Sun: rotation},
  annotation = {ADS Bibcode: 2005A\&A...437.1061S},
  file = {/Users/lbugnet/Zotero/storage/XRF3JV2Q/Sule et al. - 2005 - A numerical MHD model for the solar tachocline wit.pdf}
}

@article{Sun2018,
  title = {Formation of {{Extremely Low-mass White Dwarf Binaries}}},
  author = {Sun, M. and Arras, P.},
  year = {2018},
  month = may,
  journal = {The Astrophysical Journal},
  volume = {858},
  pages = {14},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/aab9a4},
  urldate = {2023-10-02},
  abstract = {Motivated by the discovery of several pulsating, extremely low-mass white dwarfs (ELM WDs, mass M {$\lessequivlnt$} 0.18 M {$\odot$}) that likely have WD companions, this paper discusses binary formation models for these systems. ELM WDs are formed using angular momentum losses by magnetic braking. Evolutionary models are constructed using the Modules for Experiments in Stellar Astrophysics (MESA), with ELM WD progenitors in the range 1.0 {$\lessequivlnt$} M d/M {$\odot$} {$\lessequivlnt$} 1.5 and WD companions in the range 0.4 {$\lessequivlnt$} M a/M {$\odot$} {$\lessequivlnt$} 0.9. A prescription to reduce magnetic braking for thin surface convection zones is included. Upon the thinning of the evolved donor envelope, the donor star shrinks out of contact and mass transfer (MT) ceases, revealing the ELM WD. Systems with low masses have previously been suggested as possible AM CVNs. Systems with high masses, up to the limit M {$\simeq$} 0.18 M {$\odot$} at which shell flashes occur on the WD cooling track, tend to expand out to orbital periods P orb {$\greaterequivlnt$} 15 hr. In between this range, ELM WDs may become pulsators both as pre-WDs and on the WD cooling track. Brickhill's criterion for convective mode driving is used to estimate the location of the blue edge of the g-mode instability strip. In the appendix, we show that the formation of an ELM WD by unstable MT or a common-envelope event is unlikely. Stable Roche-lobe overflow with conservative MT produces only M {$\greaterequivlnt$} 0.2 M {$\odot$}.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,binaries: close,stars: variables: general,white dwarfs},
  annotation = {ADS Bibcode: 2018ApJ...858...14S},
  file = {/Users/lbugnet/Zotero/storage/CKDCIWTV/Sun and Arras - 2018 - Formation of Extremely Low-mass White Dwarf Binari.pdf}
}

@article{Svanda2011,
  title = {Validated Helioseismic Inversions for {{3D}} Vector Flows},
  author = {{\v S}vanda, M. and Gizon, L. and Hanasoge, S. M. and Ustyugov, S. D.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {530},
  eprint = {1104.4083},
  issn = {00046361},
  doi = {10.1051/0004-6361/201016426},
  abstract = {Context. According to time-distance helioseismology, information about internal fluid motions is encoded in the travel times of solar waves. The inverse problem consists of inferring three-dimensional vector flows from a set of travel-time measurements. While only few tests of the inversions have been done, it is known that the retrieval of the small-amplitude vertical flow velocities is problematic. A thorough study of biases and noise has not been carried out in realistic conditions. Aims. Here we investigate the potential of time-distance helioseismology to infer three-dimensional convective velocities in the near-surface layers of the Sun. We developed a new subtractive optimally localised averaging (SOLA) code suitable for pipeline pseudo-automatic processing. Compared to its predecessor, the code was improved by accounting for additional constraints in order to get the right answer within a given noise level. The main aim of this study is to validate results obtained by our inversion code. Methods. We simulate travel-time maps using a snapshot from a numerical simulation of solar convective flows, realistic Born travel-time sensitivity kernels, and a realistic model of travel-time noise. These synthetic travel times are inverted for flows and the results compared with the known input flow field. Additional constraints are implemented in the inversion: cross-talk minimization between flow components and spatial localization of inversion coefficients. Results. Using modes f, p1 through p 4, we show that horizontal convective flow velocities can be inferred without bias, at a signal-to-noise ratio greater than one in the top 3.5 Mm, provided that observations span at least four days. The vertical component of velocity (vz), if it were to be weak, is more difficult to infer and is seriously affected by cross-talk from horizontal velocity components. We emphasise that this cross-talk must be explicitly minimised in order to retrieve vz in the top 1 Mm. We also show that statistical averaging over many different areas of the Sun allows for reliably measuring of average properties of all three flow components in the top 5.5 Mm of the convection zone. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/7TVYWJZT/Švanda et al. - 2011.pdf}
}

@techreport{Szegedy,
  title = {Inception-v4, {{Inception-ResNet}} and the {{Impact}} of {{Residual Connections}} on {{Learning}}},
  author = {Szegedy, Christian and Ioffe, Sergey and Vanhoucke, Vincent and Alemi, Alex},
  eprint = {1602.07261v2},
  urldate = {2020-06-19},
  abstract = {Very deep convolutional networks have been central to the largest advances in image recognition performance in recent years. One example is the Inception architecture that has been shown to achieve very good performance at relatively low computational cost. Recently, the introduction of residual connections in conjunction with a more traditional architecture has yielded state-of-the-art performance in the 2015 ILSVRC challenge; its performance was similar to the latest generation Inception-v3 network. This raises the question of whether there are any benefit in combining the Inception architecture with residual connections. Here we give clear empirical evidence that training with residual connections accelerates the training of Inception networks significantly. There is also some evidence of residual Inception networks outperforming similarly expensive Inception networks without residual connections by a thin margin. We also present several new streamlined architectures for both residual and non-residual Inception networks. These variations improve the single-frame recognition performance on the ILSVRC 2012 classification task significantly. We further demonstrate how proper activation scaling stabilizes the training of very wide residual Inception networks. With an ensemble of three residual and one Inception-v4, we achieve 3.08\% top-5 error on the test set of the ImageNet classification (CLS) challenge.},
  archiveprefix = {arxiv},
  isbn = {1602.07261v2},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/482UI5ZR/full-text.pdf}
}

@article{Szegedy2015,
  title = {Going Deeper with Convolutions {{Christian}}},
  author = {Szegedy, Christian and Wei, Liu and Yangqing, Jia and Pierre, Sermanet and Scott, Reed and Dragomir, Anguelov and Dumitru, Erham and Vincent, Vanhoucke and Andrew, Rabinovich},
  year = {2015},
  journal = {Population Health Management},
  volume = {18},
  number = {3},
  eprint = {1409.4842v1},
  pages = {186--191},
  issn = {1942-7891},
  doi = {10.1089/pop.2014.0089},
  urldate = {2020-06-19},
  abstract = {Very deep convolutional networks have been central to the largest advances in image recognition performance in recent years. One example is the Inception architecture that has been shown to achieve very good performance at relatively low computational cost. Recently, the introduction of residual connections in conjunction with a more traditional architecture has yielded state-of-the-art performance in the 2015 ILSVRC challenge; its performance was similar to the latest generation Inception-v3 network. This raises the question of whether there are any benefit in combining the Inception architecture with residual connections. Here we give clear empirical evidence that training with residual connections accelerates the training of Inception networks significantly. There is also some evidence of residual Inception networks outperforming similarly expensive Inception networks without residual connections by a thin margin. We also present several new streamlined architectures for both residual and non-residual Inception networks. These variations improve the single-frame recognition performance on the ILSVRC 2012 classification task significantly. We further demonstrate how proper activation scaling stabilizes the training of very wide residual Inception networks. With an ensemble of three residual and one Inception-v4, we achieve 3.08 percent top-5 error on the test set of the ImageNet classification (CLS) challenge},
  archiveprefix = {arxiv},
  isbn = {9781467369640},
  pmid = {25291085},
  keywords = {notion,notion-database,Vision}
}

@inproceedings{Szegedy2015a,
  title = {Going Deeper with Convolutions},
  booktitle = {Proceedings of the {{IEEE Computer Society Conference}} on {{Computer Vision}} and {{Pattern Recognition}}},
  author = {Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  year = {2015},
  month = oct,
  volume = {07-12-June},
  eprint = {1409.4842},
  pages = {1--9},
  publisher = {{IEEE Computer Society}},
  issn = {10636919},
  doi = {10.1109/CVPR.2015.7298594},
  urldate = {2020-07-20},
  abstract = {We propose a deep convolutional neural network architecture codenamed Inception that achieves the new state of the art for classification and detection in the ImageNet Large-Scale Visual Recognition Challenge 2014 (ILSVRC14). The main hallmark of this architecture is the improved utilization of the computing resources inside the network. By a carefully crafted design, we increased the depth and width of the network while keeping the computational budget constant. To optimize quality, the architectural decisions were based on the Hebbian principle and the intuition of multi-scale processing. One particular incarnation used in our submission for ILSVRC14 is called GoogLeNet, a 22 layers deep network, the quality of which is assessed in the context of classification and detection.},
  archiveprefix = {arxiv},
  isbn = {978-1-4673-6964-0},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/YWGCS2VH/full-text.pdf}
}

@article{Szegedy2015nn,
  title = {Going Deeper with Convolutions},
  author = {Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  year = {2015},
  month = oct,
  journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
  volume = {07-12-June},
  eprint = {1409.4842},
  pages = {1--9},
  publisher = {{IEEE Computer Society}},
  issn = {10636919},
  doi = {10.1109/CVPR.2015.7298594},
  urldate = {2021-01-02},
  abstract = {We propose a deep convolutional neural network architecture codenamed Inception that achieves the new state of the art for classification and detection in the ImageNet Large-Scale Visual Recognition Challenge 2014 (ILSVRC14). The main hallmark of this architecture is the improved utilization of the computing resources inside the network. By a carefully crafted design, we increased the depth and width of the network while keeping the computational budget constant. To optimize quality, the architectural decisions were based on the Hebbian principle and the intuition of multi-scale processing. One particular incarnation used in our submission for ILSVRC14 is called GoogLeNet, a 22 layers deep network, the quality of which is assessed in the context of classification and detection.},
  archiveprefix = {arxiv},
  isbn = {9781467369640},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WBQYQ292/full-text.pdf}
}

@inproceedings{Szegedy2017,
  title = {Inception-v4, Inception-{{ResNet}} and the Impact of Residual Connections on Learning},
  booktitle = {31st {{AAAI Conference}} on {{Artificial Intelligence}}, {{AAAI}} 2017},
  author = {Szegedy, Christian and Ioffe, Sergey and Vanhoucke, Vincent and Alemi, Alexander A.},
  year = {2017},
  month = feb,
  eprint = {1602.07261},
  pages = {4278--4284},
  publisher = {{AAAI press}},
  urldate = {2020-07-20},
  abstract = {Very deep convolutional networks have been central to the largest advances in image recognition performance in recent years. One example is the Inception architecture that has been shown to achieve very good performance at relatively low computational cost. Recently, the introduction of residual connections in conjunction with a more traditional architecture has yielded state-of-the-art performance in the 2015 ILSVRC challenge; its performance was similar to the latest generation Inception-v3 network. This raises the question: Are there any benefits to combining Inception architectures with residual connections? Here we give clear empirical evidence that training with residual connections accelerates the training of Inception networks significantly. There is also some evidence of residual Inception networks outperforming similarly expensive Inception networks without residual connections by a thin margin. We also present several new streamlined architectures for both residual and nonresidual Inception networks. These variations improve the single-frame recognition performance on the ILSVRC 2012 classification task significantly. We further demonstrate how proper activation scaling stabilizes the training of very wide residual Inception networks. With an ensemble of three residual and one Inception-v4 networks, we achieve 3.08\% top-5 error on the test set of the ImageNet classification (CLS) challenge.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NNR4FRJ9/full-text.pdf}
}

@article{Szewczuk2018,
  title = {{{KIC}} 3240411 - the Hottest Known {{SPB}} Star with the Asymptotic g-Mode Period Spacing},
  author = {Szewczuk, Wojciech and {Daszy{\'n}ska-Daszkiewicz}, Jadwiga},
  year = {2018},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {478},
  pages = {2243--2256},
  issn = {0035-8711},
  doi = {10.1093/mnras/sty1126},
  urldate = {2023-10-15},
  abstract = {We report the discovery of the hottest hybrid B-type pulsator, KIC 3240411, that exhibits the period spacing in the low-frequency range. This pattern is associated with asymptotic properties of high-order gravity (g-) modes. Our seismic modelling made simultaneously with the mode identification shows that dipole axisymmetric modes best fit the observations. Evolutionary models are computed with MESA code and pulsational models with the linear non-adiabatic code employing the traditional approximation to include the effects of rotation. The problem of mode excitation is discussed. We confirm that significant modification is indispensable to explain an instability of both pressure and gravity modes in the observed frequency ranges of KIC 3240411.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: early-type,stars: individual: KIC 3240411,stars: opacity,stars: oscillations,stars: rotation},
  annotation = {ADS Bibcode: 2018MNRAS.478.2243S},
  file = {/Users/lbugnet/Zotero/storage/UP6S9JBT/Szewczuk and Daszyńska-Daszkiewicz - 2018 - KIC 3240411 - the hottest known SPB star with the .pdf}
}

@article{Takahashi2021,
  title = {Modeling of Magneto-Rotational Stellar Evolution. {{I}}. {{Method}} and First Applications},
  author = {Takahashi, K. and Langer, N.},
  year = {2021},
  month = feb,
  journal = {Astronomy \& Astrophysics},
  volume = {646},
  pages = {A19},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202039253},
  urldate = {2023-10-06},
  abstract = {While magnetic fields have long been considered significant for the evolution of magnetic non-degenerate stars and compact stars, it has become clear in recent years that, in fact, all stars are deeply affected by their effects. This is particularly true regarding their internal angular momentum distribution, but magnetic fields may also influence internal mixing processes and even the fate of the star. We propose a new framework for stellar evolution simulations in which the interplay between magnetic field, rotation, mass loss, and changes in the stellar density and temperature distributions are treated self-consistently. For average large-scale stellar magnetic fields that are symmetric to the axis of the rotation of the star, we derive 1D evolution equations for the toroidal and poloidal components from the mean-field magnetohydrodynamic equation by applying Alfv\'en's theorem; and, hence, a conservative form of the angular momentum transfer due to the Lorentz force is formulated. We implement our formalism into a numerical stellar evolution code and simulate the magneto-rotational evolution of 1.5 M{$\odot$} stars. The Lorentz force aided by the {$\Omega$} effect imposes torsional Alfv\'en waves propagating through the magnetized medium, leading to near-rigid rotation within the Alfv\'en timescale. Our models, with different initial spins and B-fields, can reproduce the main observed properties of Ap/Bp stars. Calculations that are extended to the red-giant regime show a pronounced core-envelope coupling, which are capable of reproducing the core and surface rotation periods already determined by asteroseismic observations. Movie associated to Fig. 3 is available at https://www.aanda.org},
  keywords = {Astrophysics - High Energy Astrophysical Phenomena,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: magnetic field,stars: rotation},
  annotation = {ADS Bibcode: 2021A\&A...646A..19T},
  file = {/Users/lbugnet/Zotero/storage/RPQHM6VM/Takahashi and Langer - 2021 - Modeling of magneto-rotational stellar evolution. .pdf}
}

@article{takahashiModelingMagnetorotationalStellar2020,
  title = {Modeling of Magneto-Rotational Stellar Evolution. {{I}}. {{Method}} and First Applications},
  author = {Takahashi, K. and Langer, N.},
  year = {2020},
  month = nov,
  journal = {Astronomy \& Astrophysics},
  eprint = {2010.13909},
  publisher = {{EDP Sciences}},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202039253},
  urldate = {2020-12-04},
  abstract = {While magnetic fields have long been considered to be important for the evolution of magnetic non-degenerate stars and compact stars, it has become clear in recent years that actually all of the stars are deeply affected. This is particularly true regarding their internal angular momentum distribution, but magnetic fields may also influence internal mixing processes and even the fate of the star. We propose a new framework for stellar evolution simulations, in which the interplay between magnetic field, rotation, mass loss, and changes in the stellar density and temperature distributions are treated self-consistently. For average large-scale stellar magnetic fields which are symmetric to the axis of rotation of the star, we derive 1D evolution equations for the toroidal and poloidal components from the mean-field MHD equation by applying Alfven's theorem, and a conservative form of the angular momentum transfer due to the Lorentz force is formulated. We implement our formalism into a numerical stellar evolution code and simulate the magneto-rotational evolution of 1.5 M\$\_\textbackslash odot\$ stars. The Lorentz force aided by the \$\textbackslash Omega\$ effect imposes torsional Alfven waves propagating through the magnetized medium, leading to near-rigid rotation within the Alfven timescale. Our models with different initial spins and B-fields can reproduce the main observed properties of Ap/Bp stars. Calculations continued to the red-giant regime show a pronounced core-envelope coupling, which reproduces the core and surface rotation periods determined by asteroseismic observations.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Takata1994,
  title = {Selection Rules for Perturbations to the Eigenfunctions of the Pulsations of Stars Due to the Rotation and Magnetic Field},
  author = {Takata, M and Shibahashi, H},
  year = {1994},
  journal = {Publications of the Astronomical Society of Japan},
  volume = {46},
  pages = {301--314},
  urldate = {2020-05-01},
  keywords = {Astrophysics,Eigenvectors,Magnetic Fields,Magnetic Stars,notion,notion-database,Peculiar Stars,Perturbation,Stellar Oscillations,Stellar Rotation},
  file = {/Users/lbugnet/Zotero/storage/PWJRFIAT/full-text.pdf}
}

@article{Takata2016,
  title = {Physical Formulation of Mixed Modes of Stellar Oscillations},
  author = {Takata, Masao},
  year = {2016},
  month = dec,
  journal = {Publ. Astron. Soc. Japan},
  volume = {68},
  number = {6},
  pages = {91--92},
  publisher = {{Oxford Academic}},
  doi = {10.1093/pasj/psw093},
  urldate = {2020-07-14},
  abstract = {The frequency condition for eigenmodes of nonradial stellar oscillations with a mixed character, which have been extensively detected in red giants and subgiants, is generally examined by a simple physical model based on a progressive-wave picture. The coupling coefficient between the gravity-wave oscillation in the core and the acoustic-wave oscillation in the envelope is expressed in terms of the reflection coefficient at the intermediate evanescent region. This relation is fully consistent with the recent asymptotic analysis for dipolar modes, but disagrees with the conventional asymptotic analysis, which assumes that the coupling is weak. The expression for the amplitude ratio between the core and envelope oscillations is also derived. The upper and lower bounds of the ratio are found to be determined by the reflection coefficient at the intermediate region. It is also argued that the eigenmode condition should appropriately be modified if the wave generated near the surface and transmitted to the core is (partially) lost either by damping or scattering in the core. The developed formulation opens a possibility to characterize the core damping (or scattering) of the red giant stars in terms of the formal reflection coefficient at the inner boundary of the inner cavity, which would provide a valuable insight into those physical processes.},
  keywords = {analytical-stars,asteroseismology-methods,general-waves,notion,notion-database,oscillations-stars,variables}
}

@article{Takata2020,
  title = {Inferring the Internal Structure of {\emph{{$\gamma$}}} {{Doradus}} Variables from {{Rossby}} Modes: {{Extension}} of the {\emph{{$\nu$}}} - {$\surd$}{{$\Delta$}} {\emph{{$\nu$}}} Diagram},
  shorttitle = {Inferring the Internal Structure of {\emph{{$\gamma$}}} {{Doradus}} Variables from {{Rossby}} Modes},
  author = {Takata, M. and Ouazzani, R.-M. and Saio, H. and Christophe, S. and Ballot, J. and Antoci, V. and Salmon, S. J. A. J.},
  year = {2020},
  month = dec,
  journal = {Astronomy \& Astrophysics},
  volume = {644},
  pages = {A138},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/202038098},
  urldate = {2023-09-19},
  abstract = {A unique type of oscillation modes has recently been identified in {$\gamma$} Doradus variables. These low-frequency modes are called Rossby modes (or r modes) because they consist of Rossby waves in each spherical layer. These waves are characterised by toroidal motions that are restored by the latitudinal variation in the Coriolis force. The horizontal oscillations are we{$\surd$}akly coupled in the radial direction. We show that these modes can be used to probe the interior of the stars. The method of the {$\nu$} - {$\increment\nu$} diagram, which has originally been developed to analyse another type of modes, Kelvin g-modes (or prograde sectoral g-modes), is extended to take Rossby modes into account. We first show based on a theoretical model and then on two stars, KIC 3240967 and KIC 12066947, that the method can be adapted to Rossby modes straightforwardly. In addition, we demonstrate that simultaneous analysis of Kelvin and Rossby modes results in (1) smaller uncertainties in the internal rotation rate and the characteristic period of gravity modes, and (2) a substantial reduction of the correlation between the estimates of the two parameters.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/SIKJRDGF/Takata et al. - 2020 - Inferring the internal structure of γ Dorad.pdf}
}

@article{Takata2020a,
  title = {A Diagnostic Diagram for {\emph{{$\gamma$}}} {{Doradus}} Variables and Slowly Pulsating {{B-type}} Stars},
  author = {Takata, M. and Ouazzani, R.-M. and Saio, H. and Christophe, S. and Ballot, J. and Antoci, V. and Salmon, S. J. A. J. and Hijikawa, K.},
  year = {2020},
  month = mar,
  journal = {Astronomy \& Astrophysics},
  volume = {635},
  pages = {A106},
  issn = {0004-6361, 1432-0746},
  doi = {10.1051/0004-6361/201936297},
  urldate = {2023-09-19},
  abstract = {Pulsating variables of {$\gamma$} Doradus type ({$\gamma$} Dor) and slowly pulsating B-type (SPB) stars are found on and near the main sequence with typical periods varying between one and several days, making them rather hard to detect from the ground. It is only with space missions such as CoRoT and Kepler that we became truly capable of determining their oscillation frequencies with enough precision to perform in-depth analyses. Here we p{$\surd$}resent an efficient and easy-to-implement seismic tool, in which the frequency ({$\nu$}) and the square root of the frequency difference ( {$\increment\nu$}) are plotted against each other as the abscissa and the ordinate, respectively. This allows us to immediately (1) perform mode identification; (2) estimate the average rotation rate and the characteristic period of gravity modes; and (3) recognise certain physical effects, including buoyancy glitches and avoided crossings. This diagnostic tool can only be applied to prograde sectoral g modes. To validate the tool presented here, we used stellar models and also applied it to three {$\gamma$} Dor (KIC 12066947, KIC 5608334 and KIC 4846809) and one SPB star (KIC 3459297), all observed with Kepler. Furthermore, we show that the rotation rates determined using this new tool are consistent with the results of previous studies.},
  langid = {english},
  file = {/Users/lbugnet/Zotero/storage/53IVQHHK/Takata et al. - 2020 - A diagnostic diagram for γ Doradus variable.pdf}
}

@article{Talon1997,
  title = {Anisotropic Diffusion and Shear Instabilities},
  author = {Talon, S. and Zahn, J. -P.},
  year = {1997},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {317},
  eprint = {astro-ph/9609010},
  pages = {749--751},
  urldate = {2020-07-17},
  abstract = {We examine the role of anisotropic turbulence on the shear instabilities in a stratified flow. Such turbulence is expected to occur in the radiative interiors of stars, due to their differential rotation and their strong stratification, and the turbulent transport associated with it will be much stronger in the horizontal than in the vertical direction. It will thus weaken the restoring force which is caused by the gradient of mean molecular weight (\$\textbackslash mu\$). We find that the critical shear which is able to overcome the \$\textbackslash mu\$-gradient is substantially reduced by this anisotropic turbulence, and we derive an estimate for the resulting turbulent diffusivity in the vertical direction.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/R6KWRETP/full-text.pdf}
}

@article{Talon2002,
  title = {Angular Momentum Extraction by Gravoty Waves in the {{Sun}}},
  author = {Talon, Suzanne and Kumar, P. and Zahn, J.P.},
  year = {2002},
  journal = {Astrophysical Journal Letters},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/RVES5LMJ/Talon, Kumar, Zahn - 2002.pdf}
}

@article{Talon2003,
  title = {Angular Momentum Transport by Internal Gravity Waves {{I}} - {{Pop I}} Main Sequence Stars},
  author = {Talon, S. and Charbonnel, C.},
  year = {2003},
  journal = {Astronomy and Astrophysics},
  volume = {405},
  number = {3},
  pages = {1025--1032},
  issn = {00046361},
  doi = {10.1051/0004-6361:20030672},
  abstract = {We examine the generation of gravity waves by the surface convection zone of low-mass main sequence stars with solar metallicity. It is found that the total momentum luminosity in waves rises with stellar mass, up to the quasi-disappearance of the convection zone around 6500 K (corresponding to a mass of {$\sim$} 1.4 M{$\odot$} for solar metallicity) where the luminosity drastically drops. We calculate the net momentum extraction associated with these waves and explain how the calculated mass dependence helps resolve the enigma of the Li dip in terms of rotational mixing, forming a coherent picture of mixing in all main sequence stars.},
  keywords = {Hydrodynamics,notion,notion-database,Stars: abundances,Stars: interiors,Stars: late-type,Stars: rotation,Turbulence},
  file = {/Users/lbugnet/Zotero/storage/XVJ2K8VI/Talon, Charbonnel - 2003.pdf}
}

@article{Talon2004,
  title = {Angular Momentum Transport by Internal Gravity Waves {{II}}. {{Pop II}} Stars from the {{Li}} Plateau to the Horizontal Branch},
  author = {Talon, S. and Charbonnel, C.},
  year = {2004},
  journal = {Astronomy and Astrophysics},
  volume = {418},
  number = {3},
  pages = {1051--1060},
  issn = {00046361},
  doi = {10.1051/0004-6361:20034334},
  abstract = {This paper is the second in a series where we examine the generation and filtering of internal gravity waves in stars and the consequences of wave-induced transport of angular momentum at various stages of stellar evolution. Here we concentrate on Pop II dwarf stars and we focus in particular on the differential properties of internal gravity waves as a function of the stellar mass. We show that, for the range of masses corresponding to the lithium plateau, gravity waves are fully efficient and should thus lead to a quasi-solid rotation state, similar to that of the Sun. In the slightly more massive progenitors of currently observed horizontal branch star however, internal wave generation is not efficient on the main sequence, and large internal differential rotation can thus be maintained. This leads to a natural explanation of the large rotational velocities measured on the horizontal branch in some globular clusters.},
  keywords = {Hydrodynamics,notion,notion-database,Stars: abundances,Stars: interiors,Stars: Population II,Stars: rotation,Waves},
  file = {/Users/lbugnet/Zotero/storage/P8N65YWX/Talon, Charbonnel - 2004.pdf}
}

@article{Talon2005,
  title = {Hydrodynamical Stellar Models Including Rotation, Internal Gravity Waves, and Atomic Diffusion. {{I}}. {{Formalism}} and Tests on {{Pop}} i Dwarfs},
  author = {Talon, S. and Charbonnel, C.},
  year = {2005},
  journal = {Astronomy \& Astrophysics},
  volume = {440},
  number = {3},
  pages = {981--994},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053020},
  abstract = {In this paper, we develop a formalism, in order to incorporate the contribution of internal gravity waves to the transport of angular momentum and chemicals over long time-scales in stars. We show that the development of a doublepeaked shear layer acts as a filter for waves, and also how the asymmetry of this filter produces momentum extraction from the core when it is rotating faster than the surface. Using only this filtered flux, it is possible to follow the contribution of internal waves over long (evolutionary) time-scales. We then present the evolution of the internal rotation profile using this formalism for stars which are spun down via magnetic torquing. We show that waves tend to slow down the core, creating a "slow" front that may then propagate from the core to the surface. Further spin down of the surface leads to the formation of a new front. Finally we show how this momentum transport reduces rotational mixing in a 1.2 M{$\odot$}, Z = 0.02 model, leading to a surface lithium abundance in agreement with observations in the Hyades. \textcopyright{} ESO 2005.},
  keywords = {Hydrodynamics,notion,notion-database,Stars: abundances,Stars: evolution,Turbulence,Waves},
  file = {/Users/lbugnet/Zotero/storage/VV2KMKV5/Talon, Charbonnel - 2005.pdf}
}

@article{Talon2008,
  title = {Astrophysics {{Angular}} Momentum Transport by Internal Gravity Waves {{IV}}. {{Wave}} Generation by Surface Convection Zone, from the Pre-Main Sequence to the Early-{{AGB}} in Intermediate Mass Stars},
  author = {Talon, S and Charbonnel, C},
  year = {2008},
  journal = {A\&A},
  volume = {482},
  pages = {597--605},
  doi = {10.1051/0004-6361:20078620},
  urldate = {2022-01-20},
  abstract = {Context. This is the fourth in a series of papers that deal with angular momentum transport by internal gravity waves in stellar interiors. Aims. Here, we want to examine the potential role of waves in other evolutionary phases than the main sequence. Methods. We study the evolution of a 3 M Population I model from the pre-main sequence to the early-AGB phase and examine whether waves can lead to angular momentum redistribution and/or element diffusion at the external convection zone boundary. Results. We find that, although waves produced by the surface convection zone can be ignored safely for such a star during the main sequence, it is not the case for later evolutionary stages. In particular, angular momentum transport by internal waves could be quite important at the end of the sub-giant branch and during the early-AGB phase. Wave-induced mixing of chemicals is expected during the early-AGB phase.},
  keywords = {hydrodynamics-turbulence-waves-methods,interiors-stars,notion,notion-database,numerical-stars,rotation}
}

@article{Talon2009,
  title = {Session {{IV Sources}} and Sinks of Light Elements},
  author = {Talon, Suzanne and Charbonnel, Corinne},
  year = {2009},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/46KDRJIY/Talon, Charbonnel - 2009.pdf}
}

@article{Tamuz2005,
  title = {Correcting Systematic Effects in a Large Set of Photometric Light Curves},
  author = {Tamuz, O. and Mazeh, T. and Zucker, S.},
  year = {2005},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {356},
  number = {4},
  eprint = {astro-ph/0502056},
  pages = {1466--1470},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2004.08585.x},
  abstract = {We suggest a new algorithm to remove systematic effects in a large set of light curves obtained by a photometric survey. The algorithm can remove systematic effects, such as those associated with atmospheric extinction, detector efficiency, or point spread function changes over the detector. The algorithm works without any prior knowledge of the effects, as long as they linearly appear in many stars of the sample. The approach, which was originally developed to remove atmospheric extinction effects, is based on a lower rank approximation of matrices, an approach which has already been suggested and used in chemometrics, for example. The proposed algorithm is especially useful in cases where the uncertainties of the measurements are unequal. For equal uncertainties, the algorithm reduces to the Principal Component Analysis (PCA) algorithm. We present a simulation to demonstrate the effectiveness of the proposed algorithm and we point out its potential, in the search for transit candidates in particular.},
  archiveprefix = {arxiv},
  keywords = {Atmospheric effects,Methods: data analysis,Methods: statistical,notion,notion-database,Planetary systems,Surveys,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/M8IFRB2D/Tamuz, Mazeh, Zucker - 2005.pdf}
}

@article{Tassoul1968,
  title = {Asymptotic {{Approximations}} for {{Stellar Pulsations}}},
  author = {Tassoul, Monique and Tassoul, Jean Louis},
  year = {1968},
  month = jul,
  journal = {The Astrophysical Journal},
  volume = {153},
  pages = {127},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/149642},
  urldate = {2020-06-26},
  keywords = {notion,notion-database}
}

@article{Tassoul1980,
  title = {Asymptotic Approximations for Stellar Nonradial Pulsations},
  author = {Tassoul, M.},
  year = {1980},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {43},
  eprint = {1011.1669v3},
  pages = {469--490},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AQGNULPC/Tassoul - 1980.pdf}
}

@article{Tayar2013,
  title = {Implications of Rapid Core Rotation in Red Giants for Internal Angular Momentum Transport in Stars},
  author = {Tayar, Jamie and Pinsonneault, Marc H.},
  year = {2013},
  journal = {Astrophysical Journal Letters},
  volume = {775},
  number = {1},
  eprint = {1306.3986},
  pages = {1--13},
  issn = {20418205},
  doi = {10.1088/2041-8205/775/1/L1},
  abstract = {Core rotation rates have been measured for red giant stars using asteroseismology. These data, along with helioseismic measurements and open cluster spin-down studies, provide powerful clues about the nature and timescale for internal angular momentum transport in stars. We focus on two cases: the metal-poor red giant KIC 7341231 ("Otto") and intermediate-mass core helium burning stars. For both, we examine limiting case studies for angular momentum coupling between cores and envelopes under the assumption of rigid rotation on the main sequence. We discuss the expected pattern of core rotation as a function of mass and radius. In the case of Otto, strong post-main-sequence coupling is ruled out and the measured core rotation rate is in the range of 23-33 times the surface value expected from standard spin-down models. The minimum coupling timescale (0.17-0.45 Gyr) is significantly longer than that inferred for young open cluster stars. This implies ineffective internal angular momentum transport in early first ascent giants. By contrast, the core rotation rates of evolved secondary clump stars are found to be consistent with strong coupling given their rapid main-sequence rotation. An extrapolation to the white dwarf regime predicts rotation periods between 330 and 0.0052 days, depending on mass and decoupling time. We identify two key ingredients that explain these features: the presence of a convective core and inefficient angular momentum transport in the presence of larger mean molecular weight gradients. Observational tests that can disentangle these effects are discussed. \textcopyright{} 2013. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: evolution,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/6HQIXSUL/Tayar, Pinsonneault - 2013.pdf}
}

@article{Tayar2015,
  title = {Rapid {{Rotation}} of {{Low-Mass Red Giants Using Apokasc}}: A {{Measure}} of {{Interaction Rates}} on the {{Post-Main-Sequence}}},
  author = {Tayar, Jamie and Ceillier, Tugdual and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Troup, Nicholas W. and Mathur, Savita and Garc{\'i}a, Rafael A. and Zamora, O. and Johnson, Jennifer A. and Pinsonneault, Marc H. and M{\'e}sz{\'a}ros, Szabolcs and Prieto, Carlos Allende and Chaplin, William J. and Elsworth, Yvonne and Hekker, Saskia and Nidever, David L. and Salabert, David and Schneider, Donald P. and Serenelli, Aldo and Shetrone, Matthew and Stello, Dennis},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {807},
  number = {1},
  eprint = {1505.03536},
  issn = {15384357},
  doi = {10.1088/0004-637X/807/1/82},
  abstract = {We investigate the occurrence rate of rapidly rotating ({$\nu$} sin i {$>$}10 km s-1), low-mass giant stars in the Apache Point Observatory Galaxy Evolution Experiment-Kepler (APOKASC) fields with asteroseismic mass and surface gravity measurements. Such stars are likely merger products and their frequency places interesting constraints on stellar population models. We also identify anomalous rotators, i.e., stars with 5 km s-1 {$<$} {$\nu$} sin i {$<$} 10 km s-1 that are rotating significantly faster than both angular momentum evolution predictions and the measured rates of similar stars. Our data set contains fewer rapid rotators than one would expect given measurements of the Galactic field star population, which likely indicates that asteroseismic detections are less common in rapidly rotating red giants. The number of low-mass moderate (5-10 km s-1) rotators in our sample gives a lower limit of 7\% for the rate at which low-mass stars interact on the upper red giant branch because single stars in this mass range are expected to rotate slowly. Finally, we classify the likely origin of the rapid or anomalous rotation where possible. KIC 10293335 is identified as a merger product and KIC 6501237 is a possible binary system of two oscillating red giants.},
  archiveprefix = {arxiv},
  keywords = {binaries: close,notion,notion-database,stars: late-type,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/2UXWXGF8/full-text.pdf;/Users/lbugnet/Zotero/storage/66DFML6I/Tayar et al. - 2015.pdf}
}

@article{Tayar2017,
  title = {The {{Correlation}} between {{Mixing Length}} and {{Metallicity}} on the {{Giant Branch}}: {{Implications}} for {{Ages}} in the {{Gaia Era}}},
  author = {Tayar, Jamie and Somers, Garrett and Pinsonneault, Marc H. and Stello, Dennis and Mints, Alexey and Johnson, Jennifer A. and Zamora, O. and {Garc{\'i}a-Hern{\'a}ndez}, D. A. and Maraston, Claudia and Serenelli, Aldo and Prieto, Carlos Allende and Bastien, Fabienne A. and Basu, Sarbani and Bird, J. C. and Cohen, R. E. and Cunha, Katia and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Girardi, Leo and Hekker, Saskia and Holtzman, Jon and Huber, Daniel and Mathur, Savita and M{\'e}sz{\'a}ros, Szabolcs and Mosser, B. and Shetrone, Matthew and Aguirre, Victor Silva and Stassun, Keivan and Stringfellow, Guy S. and Zasowski, Gail and {Roman-Lopes}, A.},
  year = {2017},
  journal = {The Astrophysical Journal},
  volume = {840},
  number = {1},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/aa6a1e},
  abstract = {\textcopyright{} 2017. The American Astronomical Society. All rights reserved.. In the updated APOGEE-Kepler catalog, we have asteroseismic and spectroscopic data for over 3000 first ascent red giants. Given the size and accuracy of this sample, these data offer an unprecedented test of the accuracy of stellar models on the post-main-sequence. When we compare these data to theoretical predictions, we find a metallicity dependent temperature offset with a slope of around 100 K per dex in metallicity. We find that this effect is present in all model grids tested, and that theoretical uncertainties in the models, correlated spectroscopic errors, and shifts in the asteroseismic mass scale are insufficient to explain this effect. Stellar models can be brought into agreement with the data if a metallicity-dependent convective mixing length is used, with {$\Delta\alpha$} ML,YREC {$\sim$}0.2 per dex in metallicity, a trend inconsistent with the predictions of three-dimensional stellar convection simulations. If this effect is not taken into account, isochrone ages for red giants from the Gaia data will be off by as much as a factor of two even at modest deviations from solar metallicity ([Fe/H] =-0.5).},
  keywords = {notion,notion-database}
}

@article{Tayar2019,
  title = {{{CORE-ENVELOPE COUPLING IN INTERMEDIATE-MASS CORE-HELIUM BURNING STARS}}},
  author = {Tayar, Jamie and Beck, Paul G and Pinsonneault, Marc H and Garc{\'i}a, Rafael A and Mathur, Savita},
  year = {2019},
  journal = {The Astrophysical Journal},
  volume = {887},
  number = {2},
  eprint = {1911.01443v1},
  urldate = {2020-07-05},
  abstract = {Stars between two and three solar masses rotate rapidly on the main sequence, and the detection of slow core and surface rotation in the core-helium burning phase for these stars places strong constraints on their angular momentum transport and loss. From a detailed asteroseismic study of the mixed-dipole mode pattern in a carefully selected, representative sample of stars, we find that slow core rotation rates in the range reported by prior studies are a general phenomenon and not a selection effect. We show that the core rotation rates of these stars decline strongly with decreasing surface gravity during the core He-burning phase. We argue that this is a model-independent indication of significant rapid angular momentum transport between the cores and envelopes of these stars. We see a significant range in core rotation rates at all surface gravities, with little evidence for a convergence towards a uniform value. We demonstrate using evolutionary models that measured surface rotation periods are a biased tracer of the true surface rotation distribution, and argue for using stellar models for interpreting the contrast between core and surface rotation rates. The core rotation rates we measure do not have a strong mass or metallicity dependence. We argue that the emerging data strongly favors a model where angular momentum transport is much more efficient during the core He burning phase than in the shell burning phases which precede and follow it.},
  archiveprefix = {arxiv},
  keywords = {evolution,notion,notion-database,rotation,stars},
  file = {/Users/lbugnet/Zotero/storage/B8HJTZPE/full-text.pdf}
}

@article{Tayler1971,
  title = {Magnetohydrodynamic {{Stability Problems}} in {{Astrophysics}}},
  author = {Tayler, R.J.},
  year = {1971},
  journal = {Q. Jl R. astr. Soc.},
  number = {2},
  pages = {352--362},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JMSUF52M/Tayler - 1971.pdf}
}

@article{Tayler1973,
  title = {The Adiabatic Stability of Stars Containing Magnetic Fields-{{I}}.{{Toroidal}} Fields},
  author = {Tayler, R. J.},
  year = {1973},
  month = jan,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {161},
  pages = {365},
  issn = {0035-8711},
  doi = {10.1093/mnras/161.4.365},
  urldate = {2023-10-09},
  abstract = {Conditions for the stability against adiabatic perturbations of a star containing a purely toroidal magnetic field are established. These conditions are necessary and sufficient for stability, if the change in gravitational field produced by the perturbation is neglected. They remain necessary for stability if the change in gravitational field is included. The criteria are given in closed algebraic form so that they can be applied readily, if an equilibrium model of a star with a toroidal magnetic field is proposed. Because the criteria are complicated, it is difficult to draw general conclusions from them. It is however possible to show that instability must occur close to the axis of symmetry of the star, if there is a non-zero electric current density on the axis. This proves that a large class of configurations are unstable. The occurrence of this instability depends only on the shape of the field and not on its strength, whereas in general the field strength will be important in determining instability. It is not easy to predict the ultimate effect of such instabilities. They have very short growth times compared to characteristic times of stellar evolution and, even if the instability is initially contained as an oscillation of finite amplitude, it may lead to a considerably enhanced decay of the magnetic field. It is unlikely that stars exist with a purely toroidal field, although it may be stronger than the poloidal component. However, models have previously been obtained of stars with only a toroidal field and their oscillation properties have been discussed. Because these discussions by other authors have involved integrals over the whole star, the localized instabilities found in this paper have not been discovered.},
  annotation = {ADS Bibcode: 1973MNRAS.161..365T},
  file = {/Users/lbugnet/Zotero/storage/E76KGN48/Tayler - 1973 - The adiabatic stability of stars containing magnet.pdf}
}

@article{Tayler1980,
  title = {The Adiabatic Stability of Stars Containing Magnetic Fields-{{IV}}. {{Mixed}} Poloidal and Toroidal Fields},
  author = {Tayler, R.J.},
  year = {1980},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {191},
  pages = {151--163},
  urldate = {2020-05-01},
  abstract = {The stability of axisymmetric non-rotating stars containing mixed poloidal and toroidal magnetic fields is studied. It is shown that, if there is a non-zero current density on the axis of symmetry, the system is unstable. If the current density on the symmetry axis vanishes, the magnitude of the toroidal field is comparable with that of the poloidal field and the magnetic pressure is very small compared with the gas pressure, it seems probable that the system is stable but this result can only be confirmed by a much more detailed investigation of particular stellar models. A previous result concerning the instability of purely toroidal fields, which has recently been questioned, is confirmed and discussed further.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TGH25CD5/full-text.pdf}
}

@article{tedmackerethProspectsGalacticStellar2020,
  title = {Prospects for {{Galactic}} and Stellar Astrophysics with Asteroseismology of Giant Stars in the {{TESS Continuous Viewing Zones}} and Beyond},
  author = {Ted Mackereth, J and Miglio, Andrea and Elsworth, Yvonne and Mosser, Benoit and Mathur, Savita and Garcia, Rafael A and Nardiello, Domenico and Hall, Oliver J and Vrard, Mathieu and Ball, Warrick H and Basu, Sarbani and Beaton, Rachael L and Beck, Paul G and Bergemann, Maria and Bossini, Diego and Casagrande, Luca and Campante, Tiago L and Chaplin, William J and Chiappini, Cristina and Girardi, L{\'e}o and Christ S{\o}lvsten J{\o}rgensen, Andreas and Khan, Saniya and Montalb{\'a}n, Josefina and Nielsen, Martin B and Pinsonneault, Marc H and Rodrigues, Tha{\'i}se S and Serenelli, Aldo and Silva Aguirre, Victor and Stello, Dennis and Tayar, Jamie and Teske, Johanna and {van Saders}, Jennifer L and Willett, Emma},
  year = {2020},
  journal = {MNRAS},
  volume = {000},
  eprint = {2012.00140v2},
  pages = {1--21},
  urldate = {2021-08-12},
  abstract = {The NASA-TESS mission presents a treasure trove for understanding the stars it observes and the Milky Way, in which they reside. We present a first look at the prospects for Galactic and stellar astrophysics by performing initial asteroseismic analyses of bright (G {$<$} 11) red giant stars in the TESS Southern Continuous Viewing Zone (SCVZ). Using three independent pipelines, we detect {$\nu$} max and {$\increment\nu$} in 41\% of the 15,405 star parent sample (6,388 stars), with consistency at a level of {$\sim$} 2\% in {$\nu$} max and {$\sim$} 5\% in {$\increment\nu$}. Based on this, we predict that seismol-ogy will be attainable for {$\sim$} 3 \texttimes{} 10 5 giants across the whole sky and at least 10 4 giants with {$\geq$} 1 year of observations in the TESS-CVZs, subject to improvements in analysis and data reduction techniques. The best quality TESS-CVZ data, for 5,574 stars where pipelines returned consistent results, provide high quality power spectra across a number of stellar evolutionary states. This makes possible studies of, for example, the Asymptotic Giant Branch bump (AGBb). Furthermore, we demonstrate that mixed = 1 modes and rotational splitting are cleanly observed in the 1-year data set. By combining TESS-CVZ data with TESS-HERMES, SkyMapper, APOGEE and Gaia we demonstrate its strong potential for Galactic archaeology studies, providing good age precision and accuracy that reproduces well the age of high [{$\alpha$}/Fe] stars and relationships between mass and kinematics from previous studies based on e.g. Kepler. Better quality astrometry and simpler target selection than the Kepler sample makes this data ideal for studies of the local star formation history and evolution of the Galac-tic disc. These results provide a strong case for detailed spectroscopic follow-up in the CVZs to complement that which has been (or will be) collected by current surveys.},
  archiveprefix = {arxiv},
  keywords = {fundamental pa-rameters-Galaxy,fundamental parameters-stars,kinematics and dynamics-Galaxy,notion,notion-database,oscillations-Galaxy,stars,stellar content,structure-Galaxy},
  file = {/Users/lbugnet/Zotero/storage/I4D3QDJV/full-text.pdf}
}

@article{Theado2008,
  title = {New Light on the Driving Mechanism in {{roAp}} Stars. {{Part I}}. {{Effects}} of Metallicity},
  author = {Th{\'e}ado, S. and Dupret, M. -A. and Noels, A. and Ferguson, J. W.},
  year = {2008},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {493},
  number = {1},
  eprint = {0811.3495},
  pages = {159--174},
  doi = {10.1051/0004-6361:200810494},
  urldate = {2020-04-09},
  abstract = {Observations suggest that a relationship exists between the driving mechanism of roAp star pulsations and the heavy element distribution in these stars. We attempt to study the effects of local and global metallicity variations on the excitation mechanism of high order p-modes in A star models. We developed stellar evolutionary models to describe magnetic A stars with different global metallicity or local metal accumulation profiles. These models were computed with CLES ("Code Li\textbackslash `egeois d'\textbackslash 'evolution stellaire"), and the stability of our models was assessed with the non-adiabatic oscillation code MAD. Our models reproduce the blue edge of the roAp star instability strip, but generate a red edge hotter than the observed one, regardless of metallicity. Surprisingly, we find that an increase in opacity inside the driving region can produce a lower amount of driving, which we refer to as the "inverse \$\textbackslash kappa\$-mechanism".},
  archiveprefix = {arxiv},
  keywords = {Diffusion,notion,notion-database,Stars: abundances,Stars: chemically peculiar,Stars: evolution,Stars: interiors,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/96N894H4/full-text.pdf}
}

@article{Thompson2003a,
  title = {The Internal Rotation of the Sun},
  author = {Thompson, M.J. and {Christensen-Dalsgaard}, J{\o}rgen and Miesch, Mark S. and Toomre, Juri},
  year = {2003},
  journal = {Annual Review of Astronomy \& Astrophysics},
  volume = {41},
  number = {517},
  pages = {81--86},
  issn = {03796566},
  doi = {10.1146/annurev.astro.41.011802.094848},
  urldate = {2020-03-10},
  abstract = {Helioseismology has transformed our knowledge of the Sun's rotation. Earlier studies revealed the Sun's surface rotation, but now a detailed observational picture has been built up of the internal rotation of our nearest star. Unlike the predictions of stellar-evolution models, the radiative interior is found to rotate roughly uniformly. The rotation within the convection zone is also very different from prior expectations, which had been that the rotation rate would depend primarily on the distance from the rotation axis. Layers of rotational shear have been discovered at the base of the convection zone and in the subphotospheric layers. Studies of the time variation of rotation have uncovered zonal-flow bands, extending through a substantial fraction of the convection zone, which migrate over the course of the solar cycle, and there are hints of other temporal variations and of a jet-like structure. At the same time, building on earlier work with mean-field models, researchers have made great progress in supercomputer simulations of the intricate interplay between turbulent convection and rotation in the Sun's interior. Such studies are beginning to transform our understanding of how rotation organizes itself in a stellar interior.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BKAA9ZDP/full-text.pdf}
}

@article{Thompson2012,
  title = {A Class of Eccentric Binaries with Dynamic Tidal Distortions Discovered with {{Kepler}}},
  author = {Thompson, Susan E. and Everett, Mark and Mullally, Fergal and Barclay, Thomas and Howell, Steve B. and Still, Martin and Rowe, Jason and Christiansen, Jessie L. and Kurtz, Donald W. and Hambleton, Kelly and Twicken, Joseph D. and Ibrahim, Khadeejah A. and Clarke, Bruce D.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {753},
  number = {1},
  eprint = {1203.6115},
  issn = {15384357},
  doi = {10.1088/0004-637X/753/1/86},
  abstract = {We have discovered a class of eccentric binary systems within the Kepler data archive that have dynamic tidal distortions and tidally induced pulsations. Each has a uniquely shaped light curve that is characterized by periodic brightening or variability at timescales of 4-20days, frequently accompanied by shorter period oscillations. We can explain the dominant features of the entire class with orbitally varying tidal forces that occur in close, eccentric binary systems. The large variety of light curve shapes arises from viewing systems at different angles. This hypothesis is supported by spectroscopic radial velocity measurements for five systems, each showing evidence of being in an eccentric binary system. Prior to the discovery of these 17 new systems, only four stars, where KOI-54 is the best example, were known to have evidence of these dynamic tides and tidally induced oscillations. We perform preliminary fits to the light curves and radial velocity data, present the overall properties of this class, and discuss the work required to accurately model these systems. \textcopyright{} 2012 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Binaries: general,notion,notion-database,Stars: evolution,Stars: oscillations (including pulsations),Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/FJ3HU946/Thompson et al. - 2012.pdf}
}

@article{Thomson-Paressant2023,
  title = {A Search for Magnetic {$\delta$} {{Scuti}} Stars in {{Kepler}} Hybrid Candidates},
  author = {{Thomson-Paressant}, K. and Neiner, C. and Lampens, P. and {Labadie-Bartz}, J. and Monier, R. and Mathias, P. and Tkachenko, A.},
  year = {2023},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {526},
  pages = {1728--1741},
  issn = {0035-8711},
  doi = {10.1093/mnras/stad2798},
  urldate = {2023-10-17},
  abstract = {Numerous candidate hybrid stars of type {$\delta$} Scuti-{$\gamma$} Doradus have been identified with the Kepler satellite. However, many of them lie outside the theoretically expected instability strip for hybrid pulsation, where {$\delta$} Sct and {$\gamma$} Dor pulsations can be simultaneously excited. We postulate that some of these pulsating stars may not be genuine hybrid pulsators but rather magnetic {$\delta$} Sct stars, for which the rotational modulation from spots on the surface associated with the magnetic field produces frequencies in the same domain as {$\gamma$} Dor pulsations. We search for the presence of a magnetic field in a small sample of selected hybrid {$\delta$} Sct-{$\gamma$} Dor stars using spectropolarimetry. At the time of observations, the only {$\delta$} Sct star known to have a magnetic field was HD 188774 with a field strength of a few hundred Gauss. Our observations were thus tailored to detect fields of this typical strength. We find no magnetic field in the hybrid candidate stars we observed. However, two of the three other magnetic {$\delta$} Sct stars discovered since these observations have much weaker fields than HD 188774, and are of dynamo origin rather than fossil fields. It is likely that our observations are not sensitive enough to detect such dynamo magnetic fields in the cooler stars of our sample if they are present. This work nevertheless provides reliable upper limits on possible fossil fields in the hotter stars, pointing towards typically weaker fields in {$\delta$} Sct stars than in OBA stars in general.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: magnetic field,stars: oscillations,stars: variables: S Doradus,stars: variables: Scuti},
  annotation = {ADS Bibcode: 2023MNRAS.526.1728T}
}

@article{Thomson1995,
  title = {Propagation of Solar Oscillations through the Interplanetary Medium},
  author = {Thomson, David J. and Maclennan, Carol G. and Lanzerotti, Louis J.},
  year = {1995},
  journal = {Nature},
  volume = {376},
  number = {6536},
  pages = {139--144},
  issn = {00280836},
  doi = {10.1038/376139a0},
  abstract = {Time-series analysis of the fluxes of interplanetary charged particles measured by the Ulysses and Voyager spacecraft reveals many periodic components. From 1 to 140 {$\mu$}Hz, the spectral components are consistent with those estimated (but not confirmed) for gravity-mode oscillations of the Sun: from 1, 000 to 4, 000 {$\mu$}Hz, the spectral lines closely match the frequencies of known solar pressure modes. These concordances imply that the solar wind and the interplanetary magnetic field transmit solar oscillations and thus might be used to probe the interior structure of the Sun. \textcopyright{} 1995 Nature Publishing Groups. All Rights Reserved.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/MWWQ256F/Thomson, Maclennan, Lanzerotti - 1995.pdf}
}

@article{Thygesen2012a,
  title = {Atmospheric Parameters of 82 Red Giants in the {{Kepler}} Field},
  author = {Thygesen, A. O. and Frandsen, S. and Bruntt, H. and Kallinger, T. and Andersen, M. F. and Elsworth, Y. P. and Hekker, S. and Karoff, C. and Stello, D. and Brogaard, K. and Burke, C. and Caldwell, D. A. and Christiansen, J. L.},
  year = {2012},
  journal = {Astronomy and Astrophysics},
  volume = {543},
  eprint = {1205.5642},
  pages = {1--15},
  issn = {00046361},
  doi = {10.1051/0004-6361/201219237},
  abstract = {Context. Accurate fundamental parameters of stars are essential for the asteroseismic analysis of data from the NASA Kepler mission. Aims. We aim at determining accurate atmospheric parameters and the abundance pattern for a sample of 82 red giants that are targets for the Kepler mission. Methods. We have used high-resolution, high signal-to-noise spectra from three different spectrographs. We used the iterative spectral synthesis method VWA to derive the fundamental parameters from carefully selected high-quality iron lines. After determination of the fundamental parameters, abundances of 13 elements were measured using equivalent widths of the spectral lines. Results. We identify discrepancies in log g and [Fe/H], compared to the parameters based on photometric indices in the Kepler Input Catalogue (larger than 2.0 dex for log g and [Fe/H] for individual stars). The T eff found from spectroscopy and photometry shows good agreement within the uncertainties. We find good agreement between the spectroscopic log g and the log g derived from asteroseismology. Also, we see indications of a potential metallicity effect on the stellar oscillations. Conclusions. We have determined the fundamental parameters and element abundances of 82 red giants. The large discrepancies between the spectroscopic log g and [Fe/H] and values in the Kepler Input Catalogue emphasize the need for further detailed spectroscopic follow-up of the Kepler targets in order to produce reliable results from the asteroseismic analysis. \textcopyright{} 2012 ESO.},
  archiveprefix = {arxiv},
  keywords = {Methods: observational,notion,notion-database,Stars: abundances,Stars: fundamental parameters,Techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/ERBEAIG3/Thygesen et al. - 2012.pdf}
}

@article{tingLargePristineSample2018,
  title = {A {{Large}} and {{Pristine Sample}} of {{Standard Candles}} across the {{Milky Way}}: {$\sim$}100,000 {{Red Clump Stars}} with 3\% {{Contamination}}},
  author = {Ting, Yuan-Sen and Hawkins, Keith and Rix, Hans-Walter},
  year = {2018},
  journal = {The Astrophysical Journal Letters},
  volume = {858},
  pages = {L7},
  doi = {10.3847/2041-8213/aabf8e},
  urldate = {2021-05-18},
  abstract = {Core helium-burning red clump (RC) stars are excellent standard candles in the Milky Way. These stars may have more precise distance estimates from spectrophotometry than from Gaia parallaxes beyond 3 kpc. However, RC stars have values of T eff and g log that are very similar to some red giant branch (RGB) stars. Especially for low-resolution spectroscopic studies where T eff , g log , and [Fe/H] can only be estimated with limited precision, separating RC stars from RGB through established methods can incur {$\sim$}20\% contamination. Recently, Hawkins et al. demonstrated that the additional information in single-epoch spectra, such as the C/N ratio, can be exploited to cleanly differentiate RC and RGB stars. In this second paper of the series, we establish a data-driven mapping from spectral flux space to independently determined asteroseismic parameters, the frequency and the period spacing. From this, we identify 210,371 RC stars from the publicly available LAMOST DR3 and APOGEE DR14 data, with {$\sim$}9\% of contamination. We provide an RC sample of 92249 stars with a contamination of only {$\sim$}3\%, by restricting the combined analysis to LAMOST stars with S/N pix 75. This demonstrates that high-signal-to-noise ratio (S/N), low-resolution spectra covering a broad wavelength range can identify RC samples at least as pristine as their high-resolution counterparts. As coming and ongoing surveys such as TESS, DESI, and LAMOST will continue to improve the overlapping training spectroscopic-asteroseismic sample, the method presented in this study provides an efficient and straightforward way to derive a vast yet pristine sample of RC stars to reveal the three-dimensional (3D) structure of the Milky Way.},
  keywords = {methods: data analysis,notion,notion-database,stars: distances,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/EUZA55LU/full-text.pdf}
}

@article{Title1989,
  title = {Statistical Properties of Solar Granulation Derived from the {{SOUP}} Instrument on {{Spacelab}} 2},
  author = {Title, A. M. and Tarbell, T. D. and Topka, K. P. and Ferguson, S. H. and Shine, R. A. and {SOUP Team}},
  year = {1989},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {336},
  pages = {475},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/167026},
  urldate = {2020-03-15},
  abstract = {Computer algorithms and statistical techniques were used to identify, measure, and quantify the properties of solar granulation derived from movies collected by the Solar Optical Universal Polarimeter on Spacelab 2. The results show that there is neither a typical solar granule nor a typical granule evolution. A granule's evolution is dependent on local magnetic flux density, its position with respect to the active region plage, its position in the mesogranulation pattern, and the evolution of granules in its immediate neighborhood.},
  keywords = {Earth Atmosphere,Image Processing,Mean,notion,notion-database,Root,Solar Atmosphere,Solar Granulation,Solar Magnetic Field,Solar Oscillations,Solar Physics,Spacelab,Square Errors,Statistical Analysis,SUN: ATMOSPHERIC MOTIONS,SUN: GRANULATION,SUN: OSCILLATIONS}
}

@article{Tkachenko2012,
  title = {Spectrum {{Analysis}} of {{Bright Kepler Gamma Doradus Candidate Stars}}},
  author = {Tkachenko, Andrew and Lehmann, Holger and Smalley, Barry and Debosscher, Jonas and Aerts, Conny},
  year = {2012},
  month = feb,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {422},
  number = {4},
  eprint = {1202.1116},
  pages = {2960--2968},
  doi = {10.1111/j.1365-2966.2012.20687.x},
  urldate = {2020-03-31},
  abstract = {Ground-based spectroscopic follow-up observations of the pulsating stars observed by the Kepler satellite mission are needed for their asteroseismic modelling. We aim to derive the fundamental parameters for a sample of 26 Gamma Doradus candidate stars observed by the Kepler satellite mission to accomplish one of the required preconditions for their asteroseismic modelling and to compare our results with the types of pulsators expected from the existing light curve analysis. We use the spectrum synthesis method to derive the fundamental parameters like Teff, logg, [M/H], and vsini from newly obtained spectra and compute the spectral energy distribution from literature photometry to get an independent measure of Teff. We find that most of the derived Teff values agree with the values given in the Kepler Input Catalogue. According to their positions in the HR-diagram three stars are expected Gamma Dor stars, ten stars are expected Delta Sct stars, and seven stars are possibly Delta Sct stars at the hot border of the instability strip. Four stars in our sample are found to be spectroscopic binary candidates and four stars have very low metallicity where two show about solar C abundance. Six of the 10 stars located in the Delta Sct instability region of the HR-diagram show both Delta Sct and Gamma Dor-type oscillations in their light curves implying that Gamma Dor-like oscillations are much more common among the Delta Sct stars than predicted by theory. Moreover, seven stars showing periods in the Delta Sct and the Delta Sct-Gamma Dor range in their light curves are located in the HR-diagram left of the blue edge of the theoretical Delta Sct instability strip. The consistency of these findings with recent investigations based on high-quality Kepler data implies the need for a revision of the theoretical Gamma Dor and Delta Sct instability strips.},
  archiveprefix = {arxiv},
  keywords = {abundances-stars,fundamental parameters-stars,notion,notion-database,stars,Stars: abundances,Stars: fundamental parameters,Stars: variables: {$\delta$} Scuti,variables,{$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/DTLH35YQ/full-text.pdf}
}

@article{Tobias2001,
  title = {Transport and {{Storage}} of {{Magnetic Field}} by {{Overshooting Turbulent Compressible Convection}}},
  author = {Tobias, Steven M. and Brummell, Nicholas H. and Clune, Thomas L. and Toomre, Juri},
  year = {2001},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {549},
  pages = {1183--1203},
  issn = {0004-637X},
  doi = {10.1086/319448},
  urldate = {2023-10-18},
  abstract = {We present the results of a series of numerical experiments that investigate the transport of magnetic fields by turbulent penetrative compressible convection. We find that magnetic flux is preferentially transported downward out of a turbulent convecting region and stored in a stably stratified region below. This pumping mechanism is believed to be a crucial component for the operation of a large-scale solar interface dynamo since it may be responsible for the transport of flux from the solar convection zone to the stable overshoot region. The high-resolution three-dimensional simulations show that efficient pumping occurs as a result of the action of strong coherent downflowing plumes. The properties of the transport are evaluated as a function of magnetic field strength, rotation rate, supercriticality, stiffness of the interface, and configuration. The turbulent pumping of magnetic flux is remarkably robust and more efficient than its laminar counterpart. The turbulent convection naturally amplifies magnetic energy from any existing mean field. The transport of flux from the convection zone removes the source for this local amplification there, and thus the peak magnetic energy also comes to reside in the stable region. This is important for an effective interface dynamo.},
  keywords = {Convection,Magnetohydrodynamics: MHD,Sun: Interior,Sun: Magnetic Fields},
  annotation = {ADS Bibcode: 2001ApJ...549.1183T},
  file = {/Users/lbugnet/Zotero/storage/X6FPASGQ/Tobias et al. - 2001 - Transport and Storage of Magnetic Field by Oversho.pdf}
}

@article{Tobias2007,
  title = {Stellar {{Dynamos}}},
  author = {Tobias, Steven and Weiss, Nigel},
  year = {2007},
  pages = {282--311},
  doi = {10.1201/9781420055269.ch6},
  keywords = {notion,notion-database}
}

@article{Tokuno2022,
  title = {Asteroseismology of the Dip Structure in Period-Spacings of Rapidly Rotating {$\gamma$} {{Doradus}} Stars Caused by the Coupling between Core and Envelope Oscillations},
  author = {Tokuno, Takato and Takata, Masao},
  year = {2022},
  month = aug,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {514},
  pages = {4140--4159},
  issn = {0035-8711},
  doi = {10.1093/mnras/stac1492},
  urldate = {2023-10-09},
  abstract = {Recent asteroseismic observations by the Kepler space mission have revealed the dip fine structure in the period-spacing versus period diagram of rapidly rotating {$\gamma$} Doradus stars. Following the successful reproduction of the dip structure by numerical calculations in previous studies, we present in this paper the physical mechanism of how the dip is formed as a result of the interaction between the gravito-inertial waves in the radiative envelope and the pure inertial waves in the convective core. We analytically describe the wave solutions in both of the radiative envelope and the convective core, and match them at the interface to construct an eigenmode. We have found from the analysis the following points: the dip structure is mainly controlled by a parameter that has an inverse correlation with Brunt-V\"ais\"al\"a frequency at the interface; the depth and the width of the dip is shallower and larger, respectively, as the parameter gets large; the shape of the dip can be approximated by the Lorentzian function; the period at the central position of the dip is equal to or slightly smaller than that of the involved pure inertial mode in the convective core. We have also understood based on the evolutionary models of main-sequence stars that the parameter is inversely correlated with the chemical composition gradient at the convective-core boundary. The dip structure thus would provide information about the poorly-understood physical processes, such as diffusion, convective overshooting and rotational mixing, around the boundary between the convective core and the radiative envelope.},
  keywords = {Asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: interiors,stars: oscillations,stars: rotation,stars: variables: general},
  annotation = {ADS Bibcode: 2022MNRAS.514.4140T},
  file = {/Users/lbugnet/Zotero/storage/GWGQRLET/Tokuno and Takata - 2022 - Asteroseismology of the dip structure in period-sp.pdf}
}

@article{Tomczyk1995,
  title = {An Instrument to Observe Low-Degree Solar Oscilaltions},
  author = {Tomczyk, S and Streander, K and Card, G and Elmore, D and Hull, H},
  year = {1995},
  pages = {1--21},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/2Z4F8GTI/Tomczyk et al. - 1995.pdf}
}

@book{Tong2015,
  title = {Extraterrestrial Seismology},
  author = {Tong, Vincent C. H. and Garc{\'i}a, Rafael A.},
  year = {2015},
  isbn = {978-1-107-04172-1},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UYKCMATH/Extra_seismo_Proof_RAG.pdf}
}

@article{Torrence1998,
  title = {A {{Practical Guide}} to {{Wavelet Analysis}}.},
  author = {Torrence, Christopher and Compo, Gilbert P.},
  year = {1998},
  journal = {BAMS},
  volume = {79},
  number = {1},
  pages = {61--78},
  doi = {10.1175/1520-0477(1998)079<0061:APGTWA>2.0.CO;2},
  urldate = {2020-04-09},
  keywords = {notion,notion-database}
}

@article{Torres2011,
  title = {Modeling {{Kepler}} Transit Light Curves as False Positives: {{Rejection}} of Blend Scenarios for {{Kepler-9}}, and Validation of {{Kepler-9}} d, a Super-Earth-Size Planet in a Multiple System},
  author = {Torres, Guillermo and Fressin, Fran{\c c}ois and Batalha, Natalie M. and Borucki, William J. and Brown, Timothy M. and Bryson, Stephen T. and Buchhave, Lars A. and Charbonneau, David and Ciardi, David R. and Dunham, Edward W. and Fabrycky, Daniel C. and Ford, Eric B. and Gautier, Thomas N. and Gilliland, Ronald L. and Holman, Matthew J. and Howell, Steve B. and Isaacson, Howard and Jenkins, Jon M. and Koch, David G. and Latham, David W. and Lissauer, Jack J. and Marcy, Geoffrey W. and Monet, David G. and Prsa, Andrej and Quinn, Samuel N. and Ragozzine, Darin and Rowe, Jason F. and Sasselov, Dimitar D. and Steffen, Jason H. and Welsh, William F.},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {727},
  number = {1},
  eprint = {1008.4393},
  issn = {15384357},
  doi = {10.1088/0004-637X/727/1/24},
  abstract = {Light curves from the Kepler Mission contain valuable information on the nature of the phenomena producing the transit-like signals. To assist in exploring the possibility that they are due to an astrophysical false positive, we describe a procedure (BLENDER) to model the photometry in terms of a "blend" rather than a planet orbiting a star. A blend may consist of a background or foreground eclipsing binary (or star-planet pair) whose eclipses are attenuated by the light of the candidate and possibly other stars within the photometric aperture. We apply BLENDER to the case of Kepler-9 (KIC 3323887), a target harboring two previously confirmed Saturn-size planets (Kepler-9 b and Kepler-9 c) showing transit timing variations, and an additional shallower signal with a 1.59 day period suggesting the presence of a super-Earth-size planet. Using BLENDER together with constraints from other follow-up observations we are able to rule out all blends for the two deeper signals and provide independent validation of their planetary nature. For the shallower signal, we rule out a large fraction of the false positives that might mimic the transits. The false alarm rate for remaining blends depends in part (and inversely) on the unknown frequency of small-size planets. Based on several realistic estimates of this frequency, we conclude with very high confidence that this small signal is due to a super-Earth-size planet (Kepler-9 d) in a multiple system, rather than a false positive. The radius is determined to be 1.64+0.19-0.14 R., and current spectroscopic observations are as yet insufficient to establish its mass. \textcopyright{} 2011 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {Binaries: eclipsing,notion,notion-database,Planetary systems,{Stars: individual (Kepler-9, KIC 3323887, KOI-377)},Stars: statistics},
  file = {/Users/lbugnet/Zotero/storage/MASHC56A/Torres et al. - 2011.pdf}
}

@article{Tout2004,
  title = {Magnetic Fields in White Dwarfs and Stellar Evolution},
  author = {Tout, C. A. and Wickramasinghe, D. T. and Ferrario, L.},
  year = {2004},
  month = dec,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {355},
  number = {3},
  pages = {L13-L16},
  publisher = {{Oxford University Press}},
  issn = {0035-8711},
  doi = {10.1111/j.1365-2966.2004.08482.x},
  urldate = {2020-07-22},
  abstract = {The surface magnetic field strengths observed in the magnetic Ap, Bp stars (100-20000 G) and in the high field magnetic white dwarfs (106-109 G) cover many decades but nevertheless the range of magnetic fluxes observed in each of these stellar groups is similar. An evolutionary link between them therefore appears plausible. For both groups of stars there is also information on field complexity. The magnetic white dwarfs in general show non-dipole field structures which can be best modelled if we assume contributions from higher order multipoles. The field structures of the Ap and Bp stars are similarly complex. We investigate the hypothesis that the magnetic fields of the white dwarfs could be fossil remnants from the main-sequence phase by focussing on the problem of how field complexity may arise and be maintained during evolution to the compact star state. We also address the question of to what extent magnetic fields seen in the early type stars could be fossil remnants from the pre-main-sequence phases of stellar evolution dating back perhaps to the time of star formation.},
  keywords = {notion,notion-database,Stars: Evolution,Stars: Formation,Stars: Magnetic fields,Stars: Neutron,White dwarfs},
  file = {/Users/lbugnet/Zotero/storage/GQ5DPD4C/full-text.pdf}
}

@article{Toutain1997,
  title = {Tri-Phonic Helioseismology: {{Comparison}} of Solar p Modes Observed by the Helioseismology Instruments Aboard {{SOHO}}},
  author = {Toutain, T. and Appourchaux, T. and Baudin, F. and Fr{\"o}hlich, C. and Gabriel, A. and Scherrer, P. and Andersen, B. N. and Bogart, R. and Bush, R. and Finsterle, W. and Garc{\'i}a, R. A. and Grec, G. and Henney, C. J. and Hoeksema, J. T. and Jim{\'e}nez, A. and Kosovichev, A. and Roca Cort{\'e}s, T. and {Turck-Chi{\`e}ze}, S. and Ulrich, R. and Wehrli, C.},
  year = {1997},
  journal = {Solar Physics},
  volume = {175},
  number = {2},
  pages = {311--328},
  issn = {00380938},
  doi = {10.1023/A:1004949832159},
  abstract = {The three helioseismology instruments aboard SOHO observe solar p modes in velocity (GOLF and MDI) and in intensity (VIRGO and MDI). Time series of two months duration are compared and confirm that the instruments indeed observe the same Sun to a high degree of precision. Power spectra of 108 days are compared showing systematic differences between mode frequencies measured in intensity and in velocity. Data coverage exceeds 97\% for all the instruments during this interval. The weighted mean differences (V - I) are -0.1 {$\mu$}Hz for l = 0, and -0.16 {$\mu$}Hz for l = 1. The source of this systematic difference may be due to an asymmetry effect that is stronger for modes seen in intensity. Wavelet analysis is also used to compare the shape of the forcing functions. In these data sets nearly all of the variations in mode amplitude are of solar origin. Some implications for structure inversions are discussed.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HZ4EI9MA/Toutain et al. - 1997.pdf}
}

@article{Toutain2000,
  title = {Optimal {{Masks}} for {{Low-Degree Solar Acoustic Modes}}},
  author = {Toutain, T. and Kosovichev, A. G.},
  year = {2000},
  journal = {The Astrophysical Journal},
  volume = {534},
  number = {2},
  eprint = {astro-ph/0004153},
  pages = {L211-L214},
  issn = {0004637X},
  doi = {10.1086/312682},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TFLHPEQP/Toutain, Kosovichev - 2000.pdf}
}

@article{Toutain2005,
  title = {Monte {{Carlo}} Simulation of Solar P-Mode Profiles Revisited: {{Bias}} and Uncertainty Estimation from One, Not Many, Fits},
  author = {Toutain, T. and Elsworth, Y. and Chaplin, W. J.},
  year = {2005},
  journal = {Astronomy and Astrophysics},
  volume = {433},
  number = {2},
  pages = {713--715},
  issn = {00046361},
  doi = {10.1051/0004-6361:20042508},
  abstract = {It is quite common in helioseismology to use extensive Monte Carlo simulations to investigate the bias and associated uncertainties in fitted p-mode parameters. This can, however, be very time-intensive if the fitting problem is complicated or large datasets (in time or resolution) are involved. Here, we show that it is often possible to reduce significantly the task by taking advantage of the statistical properties of the p-mode profiles. \textcopyright{} ESO 2005.},
  keywords = {Methods: data analysis,Methods: statistical,notion,notion-database,Sun: helioseismology},
  file = {/Users/lbugnet/Zotero/storage/UMC6A2FZ/Toutain, Elsworth, Chaplin - 2005.pdf}
}

@article{Townsend2003,
  title = {Asymptotic Expressions for the Angular Dependence of Low-Frequency Pulsation Modes in Rotating Stars},
  author = {Townsend, R. H. D.},
  year = {2003},
  month = apr,
  journal = {MNRAS},
  volume = {340},
  number = {3},
  pages = {1020--1030},
  issn = {0035-8711},
  doi = {10.1046/J.1365-8711.2003.06379.X},
  urldate = {2021-12-22},
  abstract = {Through the solution of Laplace's tidal equations, approximated to describe equatorially trapped wave propagation, analytical expressions are obtained for the angular dependence of pulsation modes in uniformly rotating stars. As the ratio between rotation and pulsation frequencies becomes large, these expressions approach the exact solutions of the governing low-frequency pulsation equations. Four classes of asymptotic solution are found, corresponding to g (gravito-inertial), r (Rossby), Kelvin and Yanai modes. The Kelvin modes arise through the conservation of specific vorticity, much like the r modes, but propagate in the same sense as the rotation; they are found to be the equivalents of prograde sectoral modes. The prograde Yanai modes behave like g modes, as do the retrograde ones if the rotation is sufficiently rapid; otherwise, the latter exhibit the character of r modes. Comparison between asymptotic and numerical solutions to the tidal equations reveals that the former converge rapidly towards the latter, for g and Yanai modes. The convergence is slower for Kelvin and r modes, as these become equatorially trapped only when the rotation is very rapid. It is argued that the utility of the asymptotic solutions does not rest on their accuracy alone, but also on the valuable physical insights that they are capable of providing.},
  keywords = {hydrodynamics,methods: analytical,notion,notion-database,stars: oscillations,stars: rotation,waves},
  file = {/Users/lbugnet/Zotero/storage/UQZ9JA3Z/full-text.pdf}
}

@article{Townsend2005,
  title = {Kappa-Mechanism Excitation of Retrograde Mixed Modes in Rotating {{B-type}} Stars},
  author = {Townsend, R. H. D.},
  year = {2005},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {364},
  number = {2},
  eprint = {astro-ph/0506580},
  pages = {573--582},
  doi = {10.1111/j.1365-2966.2005.09585.x},
  urldate = {2020-04-09},
  abstract = {I examine the stability of retrograde mixed modes in rotating B-type stars. These modes can be regarded as a hybrid between the Rossby modes that arise from conservation of vorticity, and the Poincare modes that are gravity waves modified by the Coriolis force. Using a non-adiabatic pulsation code based around the traditional approximation, I find that the modes are unstable in mid- to late-B type stars, due to the same iron-bump opacity mechanism usually associated with SPB and \$\textbackslash beta\$ Cep stars. At one half of the critical rotation rate, the instability for \$m=1...4\$ modes spans the spectral types B4 to A0. Inertial-frame periods of the unstable modes range from 100 days down to a fraction of a day, while normalized growth rates can reach in excess of \$10\^\{-5\}\$. I discuss the relevance of these findings to SPB and pulsating Be stars, and to the putative Maia class of variable star. I also outline some of the questions raised by this discovery of a wholly-new class of pulsational instability in early-type stars.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,notion,notion-database,Stars: early-type,{Stars: emission-line, Be},Stars: oscillations,Stars: rotation,Stars: variables: other},
  file = {/Users/lbugnet/Zotero/storage/92ZKQRFW/full-text.pdf}
}

@article{Townsend2013,
  title = {{{GYRE}}: {{An}} Open-{{Source}} Stellar Oscillation Code Based on a New Magnus Multiple Shooting Scheme},
  author = {Townsend, R. H.D. and Teitler, S. A.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {435},
  number = {4},
  eprint = {1308.2965},
  pages = {3406--3418},
  issn = {00358711},
  doi = {10.1093/mnras/stt1533},
  abstract = {We present a new oscillation code, GYRE, which solves the stellar pulsation equations (both adiabatic and non-adiabatic) using a novel Magnus Multiple Shooting numerical scheme devised to overcome certain weaknesses of the usual relaxation and shooting schemes appearing in the literature. The codeis accurate (up to sixth-order in the number of grid points), robust, efficiently makes use of multiple processor cores and/or nodes and is freely available in source form for use and distribution. We verify the code against analytic solutions and results from other oscillation codes, in all cases finding good agreement. Then, we use the code to explore how the asteroseismic observables of a 1.5M{$\odot$} star change as it evolves through the red-giant bump. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Methods: numerical,notion,notion-database,Stars: evolution,Stars: interiors,Stars: oscillations,Stars: variables:general},
  file = {/Users/lbugnet/Zotero/storage/N6B3QM8C/Townsend, Teitler - 2013.pdf}
}

@article{Townsend2014a,
  title = {{{GYRE}}: {{A}} New Open-Source Stellar Oscillation Code},
  author = {Townsend, Rich and Teitler, Seth and Paxton, Bill},
  year = {2014},
  journal = {Proceedings of the International Astronomical Union},
  volume = {9},
  number = {S301},
  eprint = {1309.4455},
  pages = {505--506},
  issn = {17439213},
  doi = {10.1017/S1743921313015275},
  abstract = {We introduce GYRE, a new open-source stellar oscillation code which solves the adiabatic/non-adiabatic pulsation equations using a novel Magnus Multiple Shooting (MMS) numerical scheme. The code has a global error scaling of up to 6th order in the grid spacing, and can therefore achieve high accuracy with few grid points. It is moreover robust and efficiently makes use of multiple processor cores and/or nodes. We present an example calculation using GYRE, and discuss recent work to integrate GYRE into the asteroseismic optimization module of the MESA stellar evolution code. Copyright \textcopyright{} International Astronomical Union 2014.},
  archiveprefix = {arxiv},
  isbn = {9781107045170},
  keywords = {methods: numerical,notion,notion-database,stars: evolution,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/GZAT3NWP/Townsend, Teitler, Paxton - 2014(2).pdf;/Users/lbugnet/Zotero/storage/WITYQ6GC/Townsend, Teitler, Paxton - 2014.pdf}
}

@inproceedings{Townsend2018,
  title = {{{MESA SDK}} for {{Linux}}},
  booktitle = {Zndo},
  author = {Townsend, Richard and {Richard}},
  doi = {10.5281/ZENODO.2603170},
  urldate = {2020-11-29},
  keywords = {notion,notion-database}
}

@article{Townsenda,
  title = {Asteroseismology with {{MESA The MESA Software Development Kit}} ( {{SDK}} )},
  author = {Townsend, Rich},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/U4QLMVMH/Townsend - Unknown.pdf}
}

@article{Trampedach2013,
  title = {A {{GRID OF THREE-DIMENSIONAL STELLAR ATMOSPHERE MODELS OF SOLAR METALLICITY}}. {{I}}. {{GENERAL PROPERTIES}}, {{GRANULATION}}, {{AND ATMOSPHERIC EXPANSION}}},
  author = {Trampedach, Regner and Asplund, Martin and Collet, Remo and Nordlund, {\AA}ke and Stein, Robert F},
  year = {2013},
  journal = {The Astrophysical Journal},
  volume = {769},
  number = {15pp},
  pages = {18},
  doi = {10.1088/0004-637X/769/1/18},
  urldate = {2020-03-13},
  abstract = {Present grids of stellar atmosphere models are the workhorses in interpreting stellar observations and determining their fundamental parameters. These models rely on greatly simplified models of convection, however, lending less predictive power to such models of late-type stars. We present a grid of improved and more reliable stellar atmosphere models of late-type stars, based on deep, three-dimensional (3D), convective, stellar atmosphere simulations. This grid is to be used in general for interpreting observations and improving stellar and asteroseismic modeling. We solve the Navier Stokes equations in 3D and concurrent with the radiative transfer equation, for a range of atmospheric parameters, covering most of stellar evolution with convection at the surface. We emphasize the use of the best available atomic physics for quantitative predictions and comparisons with observations. We present granulation size, convective expansion of the acoustic cavity, and asymptotic adiabat as functions of atmospheric parameters.},
  keywords = {atmospheres-stars,convection-stars,interiors-stars,late-type,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/98VXT7P2/full-text.pdf}
}

@article{Triana2015,
  title = {{{THE INTERNAL ROTATION PROFILE OF THE B-TYPE STAR KIC}} 10526294 {{FROM FREQUENCY INVERSION OF ITS DIPOLE GRAVITY MODES}}},
  author = {Triana, S A and Moravveji, E and P{\'a}pics, P I and Aerts, C and Kawaler, S D and {Christensen-Dalsgaard}, J},
  year = {2015},
  journal = {The Astrophysical Journal},
  volume = {810},
  pages = {16},
  doi = {10.1088/0004-637X/810/1/16},
  urldate = {2020-03-10},
  abstract = {The internal angular momentum distribution of a star is the key to determining its evolution. Fortunately, stellar internal rotation can be probed through studies of rotationally split nonradial oscillation modes. In particular, the detection of nonradial gravity modes (g modes) in massive young stars has recently become feasible thanks to the Kepler space mission. Our goal is to derive the internal rotation profile of the Kepler B8V star KIC 10526294 through asteroseismology. We interpret the observed rotational splittings of its dipole g modes using four different approaches based on the best seismic models of the star and their rotational kernels. We show that these kernels can resolve differential rotation within the radiative envelope if a smooth rotational profile is assumed and if the observational errors are small. Based on Kepler data, we find that the rotation rate near the core-envelope boundary is well constrained to 163 {$\pm$} 89 nHz. The seismic data are consistent with rigid rotation but a profile with counter-rotation within the envelope has a statistical advantage over constant rotation. Our study should be repeated for other massive stars with a variety of stellar parameters in order to determine the physical conditions that control the internal rotation profile of young massive stars, with the aim of improving the input physics of their models.},
  keywords = {asteroseismology,notion,notion-database,stars: individual (KIC 10526294),stars: oscillations,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/EHIP4JB3/full-text.pdf}
}

@article{Triana2017,
  title = {Internal Rotation of 13 Low-Mass Low-Luminosity Red Giants in the {{Kepler}} Field},
  author = {Triana, S. A. and Corsaro, E. and De Ridder, J. and Bonanno, A. and P{\'e}rez Hern{\'a}ndez, F. and Garc{\'i}a, R. A.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {602},
  eprint = {1702.07910},
  pages = {1--16},
  issn = {14320746},
  doi = {10.1051/0004-6361/201629186},
  abstract = {Context. The Kepler space telescope has provided time series of red giants of such unprecedented quality that a detailed asteroseismic analysis becomes possible. For a limited set of about a dozen red giants, the observed oscillation frequencies obtained by peak-bagging together with the most recent pulsation codes allowed us to reliably determine the core/envelope rotation ratio. The results so far show that the current models are unable to reproduce the rotation ratios, predicting higher values than what is observed and thus indicating that an efficient angular momentum transport mechanism should be at work. Here we provide an asteroseismic analysis of a sample of 13 low-luminosity low-mass red giant stars observed by Kepler during its first nominal mission. These targets form a subsample of the 19 red giants studied previously, which not only have a large number of extracted oscillation frequencies, but also unambiguous mode identifications. Aims. We aim to extend the sample of red giants for which internal rotation ratios obtained by theoretical modeling of peak-bagged frequencies are available. We also derive the rotation ratios using different methods, and compare the results of these methods with each other. Methods. We built seismic models using a grid search combined with a Nelder-Mead simplex algorithm and obtained rotation averages employing Bayesian inference and inversion methods. We compared these averages with those obtained using a previously developed model-independent method. Results. We find that the cores of the red giants in this sample are rotating 5 to 10 times faster than their envelopes, which is consistent with earlier results. The rotation rates computed from the different methods show good agreement for some targets, while some discrepancies exist for others.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Stars: evolution,Stars: interiors,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/7EIGRTWA/Triana et al. - 2017.pdf}
}

@article{Trimble2004a,
  title = {Astrophysics in 2003},
  author = {Trimble, Virginia and Aschwanden, Markus~J.},
  year = {2004},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {116},
  number = {817},
  pages = {187--265},
  issn = {0004-6280},
  doi = {10.1086/383241},
  abstract = {Five coherent sections appear this year, addressing solar physics,\textbackslash ncosmology (with WMAP highlights), gamma-ray bursters (and their\textbackslash nassociation with Type Ia supernovae), extra-solar-system planets, and\textbackslash nthe formation and evolution of galaxies (from reionization to assemblage\textbackslash nof Local Group galaxies). There are also eight incoherent sections that\textbackslash ndeal with other topics in stellar, galactic, and planetary astronomy and\textbackslash nthe people who study them.\textbackslash n},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/H8QUZAMI/Trimble, Aschwanden - 2004.pdf}
}

@article{Trimble2007,
  title = {Astrophysics in 2006},
  author = {Trimble, Virginia and Aschwanden, Markus J. and Hansen, Carl J.},
  year = {2007},
  journal = {Space Science Reviews},
  volume = {132},
  number = {1},
  pages = {1--182},
  issn = {00386308},
  doi = {10.1007/s11214-007-9224-0},
  abstract = {The fastest pulsar and the slowest nova; the oldest galaxies and the youngest stars; the weirdest life forms and the commonest dwarfs; the highest energy particles and the lowest energy photons. These were some of the extremes of Astrophysics 2006. We attempt also to bring you updates on things of which there is currently only one (habitable planets, the Sun, and the Universe) and others of which there are always many, like meteors and molecules, black holes and binaries. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  keywords = {Active galaxies,Astrobiology,Binary stars,Clusters of galaxies,Cosmology: general,Earth,Galaxies: general,Gamma-ray bursts,ISM: general,Milky Way,notion,notion-database,Planets and satellites: general,Star clusters,Stars: general,Sun: general,Supernovae},
  file = {/Users/lbugnet/Zotero/storage/ATXKQJ2L/Trimble, Aschwanden, Hansen - 2007.pdf}
}

@article{Tripathy2010,
  title = {Unusual Trends in Solar {{P-mode}} Frequencies during the Current Extended Minimum},
  author = {Tripathy, S. C. and Jain, K. and Hill, F. and Leibacher, J. W.},
  year = {2010},
  journal = {Astrophysical Journal Letters},
  volume = {711},
  number = {2 PART 2},
  eprint = {1002.1690},
  issn = {20418213},
  doi = {10.1088/2041-8205/711/2/L84},
  abstract = {We investigate the behavior of the intermediate-degree mode frequencies of the Sun during the current extended minimum phase to explore the time-varying conditions in the solar interior. Using contemporaneous helioseismic data from the Global Oscillation Network Group (GONG) and the Michelson Doppler Imager (MDI), we find that the changes in resonant mode frequencies during the activity minimum period are significantly greater than the changes in solar activity as measured by different proxies. We detect a seismic minimum in MDI p-mode frequency shifts during 2008 July-August but no such signature is seen in mean shifts computed from GONG frequencies. We also analyze the frequencies of individual oscillation modes from GONG data as a function of latitude and observe a signature of the onset of the solar cycle 24 in early 2009. Thus, the intermediate-degree modes do not confirm the onset of the cycle 24 during late 2007 as reported from the analysis of the low-degree Global Oscillations at Low Frequency frequencies. Further, both the GONG and MDI frequencies show a surprising anti-correlation between frequencies and activity proxies during the current minimum, in contrast to the behavior during the minimum between cycles 22 and 23. \textcopyright{} 2010. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Sun: activity,Sun: helioseismology,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/WAMQ6KYZ/Tripathy et al. - 2010.pdf}
}

@article{Tromp2001,
  title = {Inner-{{Core Anisotropy}} and {{Rotation}}},
  author = {Tromp, Jeroen},
  year = {2001},
  month = may,
  journal = {Annual Review of Earth and Planetary Sciences},
  volume = {29},
  number = {1},
  pages = {47--69},
  publisher = {{Annual Reviews}},
  issn = {0084-6597},
  doi = {10.1146/annurev.earth.29.1.47},
  urldate = {2020-07-04},
  abstract = {{$\blacksquare$} Abstract This paper reviews recent research focused on the Earth's inner core. Large inner-core traveltime anomalies and the anomalous splitting of core-sensitive free oscillations strongly suggest that the inner core is anisotropic. Initial models involved a simple, constant or depth-dependent cylindrical anisotropy at a level less than a few percent. Recent observations suggest that its eastern hemisphere is largely isotropic, whereas its western hemisphere is highly anisotropic, and there are indications that its top 100 km may be isotropic. The coda of inner-core reflected phases has been used to infer strong heterogeneities with a length scale of just a few kilometers. Thus, a complicated three-dimensional picture of the inner core is beginning to emerge, although it has been suggested that much of this complexity may be the misinterpretation of signals that have their origin in the lowermost mantle. Numerical models of the geodynamo suggest that the inner core may rotate at a slightly different ra...},
  keywords = {inner-core attenuation,inner-core boundary,inner-core shear waves,inner-core viscosity,notion,notion-database,seismology of the core}
}

@article{Trott2016,
  title = {Australian {{Aboriginal Astronomy}} and {{Navigation arXiv}}:1607.02215v1},
  author = {Trott, Cathryn M. and Wayth, Randall B.},
  year = {2016},
  journal = {arXiv preprint arXiv: \ldots},
  volume = {447},
  number = {3},
  eprint = {1604.03273},
  pages = {15},
  issn = {14486083},
  doi = {10.1017/pas.2016.xxx},
  abstract = {Spectral features introduced by instrumental chromaticity of radio interferometers have the potential to negatively impact the ability to perform Epoch of Reionisation (EoR) and Cosmic Dawn (CD) science using the redshifted neutral hydrogen emission line from the early Universe. We describe instrument calibration choices that influence the spectral characteristics of the science data, and assess their impact on EoR statistical and tomographic experiments. Principally, we consider the intrinsic spectral response of the receiving antennas, embedded within a complete frequency-dependent primary beam response, and frequency-dependent instrument sampling. We assess different options for bandpass calibration. The analysis is applied to the proposed SKA1-Low EoR/CD experiments. We provide tolerances on the smoothness of the SKA station primary beam bandpass, to meet the scientific goals of statistical and tomographic (imaging) EoR programs. Two calibration strategies are tested: (1) fitting of each fine channel independently, and (2) fitting of an nth-order polynomial for each \textasciitilde 1\textasciitilde MHz coarse channel with (n+1)th-order residuals (n=2,3,4). Strategy (1) leads to uncorrelated power in the 2D power spectrum proportional to the thermal noise power, thereby reducing the overall array sensitivity. Strategy (2) leads to correlated residuals from the fitting, and residual signal power with (n+1)th-order curvature. For the residual power to be less than the thermal noise, the fractional amplitude of a fourth-order term in the bandpass across a single coarse channel must be {$<$}2.5\% (50\textasciitilde MHz), {$<$}0.5\% (150\textasciitilde MHz), {$<$}0.8\% (200\textasciitilde MHz). The tomographic experiment places stringent constraints on phase residuals in the bandpass. We find that the root-mean-square variability over all stations of the change in phase across any fine channel (4.578\textasciitilde kHz) should not exceed 0.2 degrees.},
  archiveprefix = {arxiv},
  keywords = {aboriginal astronomy,ethnoastronomy,history of astronomy,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/9H9MKMDH/Trott, Wayth - 2016.pdf}
}

@article{Tsantaki2013,
  title = {Astronomy {{Astrophysics Deriving}} Precise Parameters for Cool Solar-Type Stars {{Optimizing}} the Iron Line List},
  author = {Tsantaki, M and Sousa, S G and Zh Adibekyan, V and Santos, N C and Mortier, A and Israelian, G},
  year = {2013},
  journal = {A\&A},
  volume = {555},
  pages = {150},
  doi = {10.1051/0004-6361/201321103},
  urldate = {2020-03-12},
  abstract = {Context. Temperature, surface gravity, and metallicitity are basic stellar atmospheric parameters necessary to characterize a star. There are several methods to derive these parameters and a comparison of their results often shows considerable discrepancies, even in the restricted group of solar-type FGK dwarfs. Aims. We want to check the differences in temperature between the standard spectroscopic technique based on iron lines and the infrared flux method (IRFM). We aim to improve the description of the spectroscopic temperatures especially for the cooler stars where the differences between the two methods are higher, as presented in a previous work. Methods. Our spectroscopic analysis was based on the iron excitation and ionization balance, assuming Kurucz model atmospheres in LTE. The abundance analysis was determined using the code MOOG. We optimized the line list using a cool star (HD 21749) with high resolution and high signal-to-noise spectrum, as a reference in order to check for weak, isolated lines. Results. We test the quality of the new line list by re-deriving stellar parameters for 451 stars with high resolution and signal-to-noise HARPS spectra, that were analyzed in a previous work with a larger line list. The comparison in temperatures between this work and the latest IRFM for the stars in common shows that the differences for the cooler stars are significantly smaller and more homogeneously distributed than in previous studies for stars with temperatures below 5000 K. Moreover, a comparison is presented between interferometric temperatures with our results that shows good agreement, even though the sample is small and the errors of the mean differences are large. We use the new line list to re-derive parameters for some of the cooler stars that host planets. Finally, we present the impact of the new temperatures on the [Cr /Cr ] and [Ti /Ti ] abundance ratios that previously showed systematic trends with temperature. We show that the slopes of these trends for the cooler stars become drastically smaller.},
  keywords = {fundamental parameters-techniques,notion,notion-database,spectroscopic,stars}
}

@article{Turck-Chieze1993,
  title = {The Solar Interior},
  author = {{Turck-Chi{\`e}ze}, S. and D{\"a}ppen, W. and Fossat, E. and Provost, J. and Schatzman, E. and Vignaud, D.},
  year = {1993},
  journal = {Physics Reports},
  volume = {230},
  number = {2-4},
  pages = {57--235},
  issn = {03701573},
  doi = {10.1016/0370-1573(93)90020-E},
  abstract = {This report confronts the different aspects of the solar interior from the experimental and theoretical points of view, discussing photospheric abundances, neutrinos and acoustic mode measurements. The theoretical approach mainly concerns the classical framework of stellar evolution, nevertheless, particle interpretation of the data and astrophysical solutions invoked in the last 10 years are coherently examined. \textcopyright{} 1993.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4RGJXXGU/Turck-Chièze et al. - 1993.pdf}
}

@article{Turck-Chieze1997a,
  title = {First View of the Solar Core from {{GOLF}} Acoustic Modes},
  author = {{Turck-Chi{\'e}ze}, S. and Basu, S. and Brun, A. S. and {Christensen-Dalsgaard}, J. and {Eff-Darwich}, A. and Lopes, I. and P{\'e}rez Hern{\'a}ndez, F. and Berthomieu, G. and Provost, J. and Ulrich, R. K. and Baudin, F. and Boumier, P. and Charra, J. and Gabriel, A. H. and Garcia, R. A. and Grec, G. and Renaud, C. and Robillot, J. M. and Roca Cort{\'e}s, T.},
  year = {1997},
  journal = {Solar Physics},
  volume = {175},
  number = {2},
  pages = {247--265},
  issn = {00380938},
  doi = {10.1023/A:1004992727541},
  abstract = {After 8 months of nearly continuous measurements the GOLF instrument, aboard SOHO, has detected acoustic mode frequencies of more than 100 modes, extending from 1.4 mHz to 4.9 mHz. In this paper, we compare these results with the best available predictions coming from solar models. To verify the quality of the data, we examine the asymptotic seismic parameters; this confirms the improvements achieved in solar models during the last decade. Using the GOLF set of frequencies for l = 0, 1, 2, 3 combined with the LOWL second year data set for l {$>$} 3, we then carry out inversions to infer properties of the solar core. This largely confirms the previous results down to around 0.1 R{$\odot$}, while there remain differences, even closer to the centre, where the present study shows an extreme sensitivity of the inversion results to the values of the frequencies. We finally consider physical processes which may influence directly or indirectly the solar core structure.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/BLXIN7SS/Turck-Chiéze et al. - 1997.pdf}
}

@article{Turck-Chieze2004,
  title = {Erratum: ``{{Looking}} for {{Gravity-Mode Multiplets}} with the {{GOLF Experiment}} Aboard {{SOHO}} '' ({{ApJ}}, 604, 455 [2004])},
  author = {{Turck-Chieze}, S. and Garcia, R. A. and Couvidat, S. and Ulrich, R. K. and Bertello, L. and Varadi, F. and Kosovichev, A. G. and Gabriel, A. H. and Berthomieu, G. and Brun, A. S. and Lopes, I. and Palle, P. and Provost, J. and Robillot, J. M. and Roca Cortes, T.},
  year = {2004},
  journal = {The Astrophysical Journal},
  volume = {608},
  number = {1},
  pages = {610--610},
  issn = {0004-637X},
  doi = {10.1086/421487},
  abstract = {This paper is focused on the search for low-amplitude solar gravity modes between 150 and 400 {$\mu$}Hz, corresponding to low-degree, low-order modes. It presents results based on an original strategy that looks for multiplets instead of single peaks, taking into consideration our knowledge of the solar interior from acoustic modes. Five years of quasi-continuous measurements collected with the helioseismic GOLF experiment aboard the SOHO spacecraft are analyzed. We use different power spectrum estimators and calculate confidence levels for the most significant peaks. This approach allows us to look for signals with velocities down to 2 mm s-1, not far from the limit of existing instruments aboard SOHO, amplitudes that have never been investigated up to now. We apply the method to series of 1290 days, beginning in 1996 April, near the solar cycle minimum. An automatic detection algorithm lists those peaks and multiplets that have a probability of more than 90\% of not being pure noise. The detected patterns are then followed in time, considering also series of 1768 and 2034 days, partly covering the solar cycle maximum. In the analyzed frequency range, the probability of detection of the multiplets does not increase with time as for very long lifetime modes. This is partly due to the observational conditions after 1998 October and the degradation of these observational conditions near the solar maximum, since these modes have a ``mixed'' character and probably behave as acoustic modes. Several structures retain our attention because of the presence of persistent peaks along the whole time span. These features may support the idea of an increase of the rotation in the inner core. There are good arguments for thinking that complementary observations up to the solar activity minimum in 2007 will be decisive for drawing conclusions on the presence or absence of gravity modes detected aboard the SOHO satellite.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZZIWKFHQ/Turck-Chieze et al. - 2004.pdf}
}

@article{Turck-Chieze2004a,
  title = {Surprising Sun: {{A}} New Step towards a Complete Picture?},
  author = {{Turck-Chi{\`e}ze}, S. and Couvidat, S. and Piau, L. and Ferguson, J. and Lambert, P. and Ballot, J. and Garcia, R. A. and Nghiem, P.},
  year = {2004},
  journal = {Physical Review Letters},
  volume = {93},
  number = {21},
  pages = {19--22},
  issn = {00319007},
  doi = {10.1103/PhysRevLett.93.211102},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WUGI7GLJ/Turck-Chièze et al. - 2004.pdf}
}

@article{Turck-Chieze2004b,
  title = {Looking for {{Gravity-Mode Multiplets}} with the {{GOLF Experiment}} Aboard {{SOHO}}},
  author = {{Turck-Chi{\`e}ze}, S. and Garc{\'i}a, R. A. and Couvidat, S. and Ulrich, R. K. and Bertello, L. and Varadi, F. and Kosovichev, A. G. and Gabriel, A. H. and Berthomieu, G. and Brun, A. S. and Lopes, I. and Pall{\'e}, P. and Provost, J. and Robillot, J. M. and Roca Cort{\'e}s, T.},
  year = {2004},
  month = mar,
  journal = {The Astrophysical Journal},
  volume = {604},
  pages = {455--468},
  issn = {0004-637X},
  doi = {10.1086/381743},
  urldate = {2023-07-27},
  abstract = {This paper is focused on the search for low-amplitude solar gravity modes between 150 and 400 {$\mu$}Hz, corresponding to low-degree, low-order modes. It presents results based on an original strategy that looks for multiplets instead of single peaks, taking into consideration our knowledge of the solar interior from acoustic modes. Five years of quasi-continuous measurements collected with the helioseismic GOLF experiment aboard the SOHO spacecraft are analyzed. We use different power spectrum estimators and calculate confidence levels for the most significant peaks. This approach allows us to look for signals with velocities down to 2 mm s-1, not far from the limit of existing instruments aboard SOHO, amplitudes that have never been investigated up to now. We apply the method to series of 1290 days, beginning in 1996 April, near the solar cycle minimum. An automatic detection algorithm lists those peaks and multiplets that have a probability of more than 90\% of not being pure noise. The detected patterns are then followed in time, considering also series of 1768 and 2034 days, partly covering the solar cycle maximum. In the analyzed frequency range, the probability of detection of the multiplets does not increase with time as for very long lifetime modes. This is partly due to the observational conditions after 1998 October and the degradation of these observational conditions near the solar maximum, since these modes have a ``mixed'' character and probably behave as acoustic modes. Several structures retain our attention because of the presence of persistent peaks along the whole time span. These features may support the idea of an increase of the rotation in the inner core. There are good arguments for thinking that complementary observations up to the solar activity minimum in 2007 will be decisive for drawing conclusions on the presence or absence of gravity modes detected aboard the SOHO satellite.},
  keywords = {Sun: Helioseismology,Sun: Interior,Sun: Oscillations},
  annotation = {ADS Bibcode: 2004ApJ...604..455T},
  file = {/Users/lbugnet/Zotero/storage/EMNSHLCQ/Turck-Chièze et al. - 2004 - Looking for Gravity-Mode Multiplets with the GOLF .pdf}
}

@article{Turck-Chieze2005,
  title = {The Magnetism of the Solar Interior for a Complete {{MHD}} Solar Vision},
  author = {{Turck-Chi{\`e}ze}, S. and Appourchaux, T. and Ballot, J. and Berthomieu, G. and Boumier, P. and Brun, A. S. and Cacciani, A. and {Christensen-Dalsgaard}, J. and Corbard, T. and Couvidat, S. and {Eff-Darwich}, A. and Dintrans, B. and Fossat, E. and Garcia, R. A. and Gelly, B. and Gizon, L. and Gough, D. and Jimenez, A. and {Jimenez-Reyes}, S. and Kosovishev, A. and Lambert, P. and Lopes, I. and Martic, M. and Mathis, S. and Meunier, N. and Nghiem, P. A. and Palle, P. and Piau, L. and Provost, J. and Rieutord, M. and Robillot, J. M. and Rodier, T. and Roxburgh, I. and Rozelot, J. P. and Solanki, S. and Talon, S. and Thompson, M. and Thuillier, G. and Vauclair, S. and Zahn, J. P.},
  year = {2005},
  journal = {European Space Agency, (Special Publication) ESA SP},
  number = {588},
  eprint = {astro-ph/0510854},
  pages = {193--202},
  issn = {03796566},
  abstract = {The solar magnetism is no more considered as a purely superficial phenomenon. The SoHO community has shown that the length of the solar cycle depends on the transition region between radiation and convection. Nevertheless, the internal solar (stellar) magnetism stays poorly known. Starting in 2008, the American instrument HMI/SDO and the European microsatellite PICARD will enrich our view of the Sun-Earth relationship. Thus obtaining a complete MHD solar picture is a clear objective for the next decades and it requires complementary observations of the dynamics of the radiative zone. For that ambitious goal, space prototypes are being developed to improve gravity mode detection. The Sun is unique to progress on the topology of deep internal magnetic fields and to nderstand the complex mechanisms which provoke photospheric and coronal magnetic changes and possible longer cycles important for human life. We propose the following roadmap in Europe to contribute to this "impressive" revolution in Astronomy and in our Sun-Earth relationship: SoHO (1995-2007), PI-CARD (2008-2010), DynaMICS (2009-2017) in parallel to SDO (2008-2017) then a world-class mission located at the L1 orbit or above the solar poles.},
  archiveprefix = {arxiv},
  isbn = {9290928999},
  keywords = {Celestial mechanics,General relativity,Gravitational moments,notion,notion-database,Solar magnetism,Solar rotation,Sun},
  file = {/Users/lbugnet/Zotero/storage/AQ5MPYC9/Turck-Chièze et al. - 2005.pdf}
}

@article{Turck-Chieze2006,
  title = {{{GOLF-NG}} Spectrometer, a Space Prototype for Studying the Dynamics of the Deep Solar Interior},
  author = {{Turck-Chi{\`e}ze}, Sylvaine and Carton, Pierre Henri and Ballot, J{\'e}rome and Barri{\`e}re, Jean Christophe and {Daniel-Thomas}, Philippe and Delbart, Alain and Desforges, Daniel and Garcia, Rafa{\"e}l A. and Granelli, R{\'e}mi and Mathur, Savita and Nunio, Fran{\c c}ois and Piret, Yves and Pall{\'e}, Pere L. and Jim{\'e}nez, Antonio J. and {Jim{\'e}nez-Reyes}, Sebastian J. and Robillot, Jean Maurice and Fossat, Eric and {Eff-Darwich}, Antonio M. and Gelly, Bernard},
  year = {2006},
  journal = {Advances in Space Research},
  volume = {38},
  number = {8},
  pages = {1812--1818},
  issn = {02731177},
  doi = {10.1016/j.asr.2005.09.033},
  abstract = {The GOLF-NG (Global Oscillations at Low Frequency New Generation) instrument is devoted to the search for solar gravity and acoustic modes, and also chromospheric modes from space. This instrument which is a successor to GOLF/SOHO will contribute to improve our knowledge of the dynamics of the solar radiative zone. It is a 15 points resonant scattering spectrometer, working on the D1 sodium line. A ground-based prototype is under construction to validate the difficult issues. It will be installed at the Teide Observatory, on Tenerife in 2006 to analyse the separation of the effects of the magnetic turbulence of the line from the solar oscillations. We are prepared to put a space version of this instrument including a capability of identification of the modes, in orbit during the next decade. This instrument should be included in the ILWS program as it offers a key to the improvement of our knowledge of the solar core in combination with observations from SDO and PICARD. We hope to determine the core rotation and magnetic field, through precise measurements of oscillation mode frequency splittings. Understanding the magnetic field of the radiative zone is important for progress in the study of solar activity sources, an important player for the long-term Sun-Earth relationship. \textcopyright{} 2006.},
  keywords = {notion,notion-database,Resonant spectrometer,Solar acoustic modes,Solar Doppler velocity,Solar gravity modes,Space instrument},
  file = {/Users/lbugnet/Zotero/storage/FB95DCV4/Turck-Chièze et al. - 2006.pdf}
}

@article{Turck-Chieze2006a,
  title = {Solar Gravity Modes: {{Present}} and Future},
  author = {{Turck-Chi{\`e}ze}, Sylvaine},
  year = {2006},
  journal = {Advances in Space Research},
  volume = {37},
  number = {8},
  pages = {1569--1575},
  issn = {02731177},
  doi = {10.1016/j.asr.2005.08.003},
  abstract = {Gravity modes are the best probes to study the solar radiative zone dynamics, especially in the nuclear core. These modes remain difficult to observe, but they are essential ingredients for progressing on the evolution of the Sun-Earth relationship at the level of centuries. Today, the knowledge of the internal dynamics comes from acoustic modes and concerns mainly the external 2\% of the solar mass. Nevertheless, the flat rotation profile of the radiative zone compels physics beyond the standard framework. I summarize different attempts to look for gravity modes and the results obtained after 8 years of observation with the GOLF/SoHO instrument. Some gravity mode candidates (at 1 mm/s level) have appeared with more than 98\% confidence level as quadruplets or quintuplets. These patterns, if confirmed as gravity modes, may reveal very exciting physics of the solar core. Getting information on rotation and magnetic field in the solar core are real keys to simulate a complete dynamical solar picture. The understanding of the solar dynamics, the precise energetic balance and its temporal evolution necessitate more observations of the radiative zone which constitutes 98\% of the Sun by mass. Our expertise in Doppler velocity measurements allows a step further and a new instrumental concept to reach velocities as low as 0.1 mm/s. A prototype will join the Tenerife site in 2006 and a space version is proposed to CNES and ESA as a microsatellite or part of a payload at the L1 Lagrange point. \textcopyright{} 2006.},
  keywords = {Acoustic modes,ILWS program,MHD calculation,notion,notion-database,Resonant spectrometer,Solar model,Sun: gravity modes},
  file = {/Users/lbugnet/Zotero/storage/PLMDZ3KC/Turck-Chièze - 2006.pdf}
}

@article{Turck-Chieze2007,
  title = {Understanding the Origin of the Solar Cyclic Activity for an Improved Earth Climate Prediction},
  author = {{Turck-Chi{\`e}ze}, Sylvaine and Lambert, Pascal},
  year = {2007},
  journal = {Advances in Space Research},
  volume = {40},
  number = {7},
  pages = {907--914},
  issn = {02731177},
  doi = {10.1016/j.asr.2007.01.090},
  abstract = {This review is dedicated to the processes which could explain the origin of the great extrema of the solar activity. We would like to reach a more suitable estimate and prediction of the temporal solar variability and its real impact on the Earth climatic models. The development of this new field is stimulated by the SoHO helioseismic measurements and by some recent solar modelling improvement which aims to describe the dynamical processes from the core to the surface. We first recall assumptions on the potential different solar variabilities. Then, we introduce stellar seismology and summarize the main SOHO results which are relevant for this field. Finally we mention the dynamical processes which are presently introduced in new solar models. We believe that the knowledge of two important elements: (1) the magnetic field interplay between the radiative zone and the convective zone and (2) the role of the gravity waves, would allow to understand the origin of the grand minima and maxima observed during the last millennium. Complementary observables like acoustic and gravity modes, radius and spectral irradiance from far UV to visible in parallel to the development of 1D-2D-3D simulations will improve this field. PICARD, SDO, DynaMICCS are key projects for a prediction of the next century variability. Some helioseismic indicators constitute the first necessary information to properly describe the Sun-Earth climatic connection. \textcopyright{} 2007 COSPAR.},
  keywords = {Gravity waves,Helioseismology,notion,notion-database,Solar interior,Solar magnetic field},
  file = {/Users/lbugnet/Zotero/storage/FSCVV7LT/Turck-Chièze, Lambert - 2007.pdf}
}

@article{Turck-Chieze2008,
  title = {Laboratory Performances of the Solar Multichannel Resonant Scattering Spectrometer Prototype of the {{GOLF-New Generation}} Instrument},
  author = {{Turck-Chi{\`e}ze}, S. and Carton, P. H. and Mathur, S. and Barri{\`e}re, J. C. and {Daniel-Thomas}, P. and {Lahonde-Hamdoun}, C. and Granelli, R. and Loiseau, D. and Nunio, F. and Piret, Y. and Robillot, J. M.},
  year = {2008},
  journal = {Astronomische Nachrichten},
  volume = {329},
  number = {5},
  pages = {521--528},
  issn = {00046337},
  doi = {10.1002/asna.200710989},
  abstract = {This article quickly summarizes the performances and results of the GOLF/SoHO resonant spectrometer, thus justifying to go a step further. We then recall the characteristics of the multichannel resonant GOLF-NG spectrometer and present the first successful performances of the laboratory tests on the prototype and also the limitations of this first technological instrument. Scientific questions and an observation strategy are discussed. \textcopyright{} 2008 Wiley-VCH Verlag GmbH \& Co. KGaA.},
  keywords = {notion,notion-database,Space vehicles: instruments,Sun: oscillations},
  file = {/Users/lbugnet/Zotero/storage/TVF7EHNU/Turck-Chièze et al. - 2008.pdf}
}

@article{Turck-Chieze2009,
  title = {The {{DynaMICCS}} Perspective: {{A}} Mission for a Complete and Continuous View of the {{Sun}} Dedicated to Magnetism, Space Weather and Space Climate},
  author = {{Turck-Chi{\`e}ze}, S. and Lamy, P. and Carr, C. and Carton, P. H. and Chevalier, A. and Dandouras, I. and Defise, J. M. and Dewitte, S. and {de Wit}, T. Dudok and Halain, J. P. and Hasan, S. and Hochedez, J. F. and Horbury, T. and Levacher, P. and Meissonier, M. and Murphy, N. and Rochus, P. and Ruzmaikin, A. and Schmutz, W. and Thuillier, G. and Viv{\`e}s, S.},
  year = {2009},
  journal = {Experimental Astronomy},
  volume = {23},
  number = {3},
  pages = {1017--1055},
  issn = {09226435},
  doi = {10.1007/s10686-008-9111-z},
  abstract = {The DynaMICCS mission is designed to probe and understand the dynamics of crucial regions of the Sun that determine solar variability, including the previously unexplored inner core, the radiative/convective zone interface layers, the photosphere/chromosphere layers and the low corona. The mission delivers data and knowledge that no other known mission provides for understanding space weather and space climate and for advancing stellar physics (internal dynamics) and fundamental physics (neutrino properties, atomic physics, gravitational moments...). The science objectives are achieved using Doppler and magnetic measurements of the solar surface, helioseismic and coronographic measurements, solar irradiance at different wavelengths and in-situ measurements of plasma/energetic particles/magnetic fields. The DynaMICCS payload uses an original concept studied by Thal\`es Alenia Space in the framework of the CNES call for formation flying missions: an external occultation of the solar light is obtained by putting an occulter spacecraft 150 m (or more) in front of a second spacecraft. The occulter spacecraft, a LEO platform of the mini sat class, e.g. PROTEUS, type carries the helioseismic and irradiance instruments and the formation flying technologies. The latter spacecraft of the same type carries a visible and infrared coronagraph for a unique observation of the solar corona and instrumentation for the study of the solar wind and imagers. This mission must guarantee long (one 11-year solar cycle) and continuous observations (duty cycle {$>$} 94\%) of signals that can be very weak (the gravity mode detection supposes the measurement of velocity smaller than 1 mm/s). This assumes no interruption in observation and very stable thermal conditions. The preferred orbit therefore is the L1 orbit, which fits these requirements very well and is also an attractive environment for the spacecraft due to its low radiation and low perturbation (solar pressure) environment. This mission is secured by instrumental R and D activities during the present and coming years. Some prototypes of different instruments are already built (GOLFNG, SDM) and the performances will be checked before launch on the ground or in space through planned missions of CNES and PROBA ESA missions (PICARD, LYRA, maybe ASPIICS). \textcopyright{} The Author(s) 2008.},
  keywords = {Acoustic modes,Formation flying,Global solar magnetism,notion,notion-database,Solar activity,Solar gravity,Solar variability,Solar wind-irradiance},
  file = {/Users/lbugnet/Zotero/storage/M6YZ8W5A/Turck-Chièze et al. - 2009.pdf}
}

@article{Turck-Chieze2010a,
  title = {Seismic and Dynamical Solar Models. {{I}}. the Impact of the Solar Rotation History on Neutrinos and Seismic Indicators},
  author = {{Turck-Chi{\`e}ze}, S. and Palacios, A. and Marques, J. P. and Nghiem, P. A.P.},
  year = {2010},
  journal = {Astrophysical Journal},
  volume = {715},
  number = {2},
  eprint = {1004.1657},
  pages = {1539--1555},
  issn = {15384357},
  doi = {10.1088/0004-637X/715/2/1539},
  abstract = {Solar activity and helioseismology show the limitation of the standard solar model and call for the inclusion of dynamical processes in both convective and radiative zones. In this paper, we concentrate on the radiative zone. We first recall the sensitivity of boron neutrinos to the microscopic physics included in solar standard and seismic models. We confront the neutrino predictions of the seismic model with all the detected neutrino fluxes. Then, we compute new models of the Sun including a detailed transport of angular momentum and chemicals due to internal rotation that includes meridional circulation and shear-induced turbulence. We use two stellar evolution codes: CESAM and STAREVOL to estimate the different terms. We follow three temporal evolutions of the internal rotation which differ by their initial conditions: very slow, moderate, and fast rotation, with magnetic braking at the arrival on the main sequence for the last two. We find that the meridional velocities in the present solar radiative zone are extremely small in comparison with those of the convective zone (smaller than 10-6 cm s-1 instead of ms-1). All models lead to a radial differential rotation profile in the radiative zone but with a significantly different contrast. We compare these profiles to the presumed solar internal rotation and show that if meridional circulation and shear turbulence were the only mechanisms transporting angular momentum within the Sun, a rather slow rotation in the young Sun is favored. We confirm the small influence of the transport by rotation on the sound speed profile but its potential impact on the chemicals in the transition region between radiation and convective zones. These models are physically more representative of the real Sun than the standard or seismic solar models but a high initial rotation, as has been considered previously, increases the disagreement with neutrinos and the sound speed in the radiative zone. This present work pushes us to pursue the inclusion of the other dynamical processes to better reproduce the observed solar profile in the whole radiative zone and to better describe the young active Sun. We also need to get a better knowledge of solar gravity mode splittings to use their constraints. \textcopyright{} 2010. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {Hydrodynamics,Neutrinos,notion,notion-database,Sun: evolution,Sun: helioseismology,Sun: interior,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/E92KEXN5/Turck-Chièze et al. - 2010.pdf}
}

@article{Turck-Chieze2011,
  title = {Solar Neutrinos, Helioseismology and the Solar Internal Dynamics},
  author = {{Turck-Chi{\`e}ze}, Sylvaine and Couvidat, S{\'e}bastien},
  year = {2011},
  journal = {Reports on Progress in Physics},
  volume = {74},
  number = {8},
  eprint = {1009.0852},
  issn = {00344885},
  doi = {10.1088/0034-4885/74/8/086901},
  abstract = {Neutrinos are fundamental particles ubiquitous in the Universe and whose properties remain elusive despite more than 50 years of intense research activity. This review illustrates the importance of solar neutrinos in astrophysics, nuclear physics and particle physics. After a description of the historical context, we remind the reader of the noticeable properties of these particles and of the stakes of the solar neutrino puzzle. The standard solar model triggered persistent efforts in fundamental physics to predict the solar neutrino fluxes, and its constantly evolving predictions have been regularly compared with the detected neutrino signals. Anticipating that this standard model could not reproduce the internal solar dynamics, a seismic solar model was developed which enriched theoretical neutrino flux predictions with in situ observation of acoustic and gravity waves propagating in the Sun. This seismic model contributed to the stabilization of the neutrino flux predictions. This review recalls the main historical steps, from the pioneering Homestake mine experiment and the GALLEX-SAGE experiments capturing the first proton-proton neutrinos. It emphasizes the importance of the SuperKamiokande and SNO detectors. Both experiments demonstrated that the solar-emitted electron neutrinos are partially transformed into other neutrino flavors before reaching the Earth. This sustained experimental effort opens the door to neutrino astronomy, with long-base lines and underground detectors. The success of BOREXINO in detecting the 7Be neutrino signal alone instills confidence in physicists' ability to detect each neutrino source separately. It justifies the building of a new generation of detectors to measure the entire solar neutrino spectrum in greater detail, as well as supernova neutrinos. A coherent picture has emerged from neutrino physics and helioseismology. Today, new paradigms take shape in these two fields: neutrinos are massive particles, but their masses are still unknown, and the research on the solar interior focuses on the dynamical aspects and on the signature of dark matter. The magnetic moment of the neutrino begins to be an actor in stellar evolution. The third part of the review is dedicated to this prospect. The understanding of the crucial role of both rotation and magnetism in solar physics benefits from SoHO, SDO and PICARD space observations, and from a new prototype, GOLF-NG. The magnetohydrodynamical view of the solar interior is a new way of understanding the impact of the Sun on the Earth's environment and climate. For now, the particle and stellar challenges seem decoupled, but this is only a superficial appearance. The development of asteroseismology - with the COROT and KEPLER spacecraft - and of neutrino physics will both contribute to improvements in our understanding of, for instance, supernova explosions. This shows the far-reaching impact of neutrino and stellar astronomy. \textcopyright{} 2011 IOP Publishing Ltd.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Q6UVCSLQ/Turck-Chièze, Couvidat - 2011.pdf}
}

@techreport{Turck2011,
  title = {Report on {{Progress}} in {{Physics}}, Final Version},
  author = {Turck, Sylvaine and Eze, Ch{\`i} and Couvidat, S{\'e}bastien},
  year = {2011},
  month = sep,
  eprint = {1009.0852v2},
  urldate = {2020-07-04},
  abstract = {Neutrinos are fundamental particles ubiquitous in the Universe and whose properties remain elusive despite more than 50 years of intense research activity. This review illustrates the importance of solar neutrinos in Astrophysics, Nuclear Physics, and Particle Physics. After a description of the historical context, we remind the reader of the noticeable properties of these particles and of the stakes of the solar neutrino puzzle. The Standard Solar Model triggered persistent efforts in fundamental Physics to predict the solar neutrino fluxes, and its constantly evolving predictions have been regularly compared to the detected neutrino signals. Anticipating that this standard model could not reproduce the internal solar dynamics, a Seismic Solar Model was developed which enriched theoretical neutrino flux predictions with in situ observation of acoustic and gravity waves propagating in the Sun. This seismic model contributed to the stabilization of the neutrino flux predictions. This review reminds the main historical steps, from the pioneering Homestake mine experiment and the GALLEX-SAGE experiments capturing the first pp neutrinos. It emphasizes the importance of the Superkamiokande and SNO detectors. Both experiments demonstrated that the solar-emitted electronic neutrinos are partially transformed into other neutrino flavors before reaching the Earth. This sustained experimental effort opens the door to Neutrino Astronomy, with long-base lines and underground detectors. The success of BOREXINO in detecting the 7 Be neutrino signal alone instills confidence in the physicists ability to detect each neutrino source separately. It justifies the building of a new generation of detectors to measure the entire solar neutrino spectrum with greater detail, as well as supernova neutrinos. A coherent picture emerged from neutrino physics and helioseismology. Today, new paradigms take shape in these two fields: the neutrinos are massive particles, but their masses are still unknown, and the research on the solar interior is focusing on the dynamical aspects and on signature of dark matter. The magnetic moment of the neutrino begins to be an actor of stellar evolution. The third part of the review is dedicated to this prospect. The understanding of the crucial role of both rotation and magnetism in solar physics benefit from SoHO, SDO, and PICARD space observations, and from new prototype like GOLF-NG. The magneto-hydrodynamical view of the solar interior is a new way of understanding the impact of the Sun on the Earth environment and climate. For now, the particle and stellar challenges seem decoupled, but this is only a superficial appearance. The development of asteroseismology-with the COROT and KEPLER spacecrafts-and of neutrino physics will both contribute to improvements in our understanding of, for instance, supernova explosions. This shows the far-reaching impact of Neutrino and Stellar Astronomy.},
  archiveprefix = {arxiv},
  keywords = {global helioseismology,internal solar magnetic fields,internal solar rotation,local helioseismology,neutrino properties,notion,notion-database,numbers: solar neutrinos,Sun-Earth relationship},
  file = {/Users/lbugnet/Zotero/storage/W9L9X47U/full-text.pdf}
}

@misc{Tutar2011,
  title = {Unno {{Chapter}} 4: {{NONADIABATIC OSCILLATIONS}}},
  author = {Unno, Wasaburo},
  year = {1989},
  isbn = {1030328129},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JMBN6TZY/Unno - 1989(9).pdf}
}

@article{Udalski2008,
  title = {The Optical Gravitational Lensing Experiment. {{OGLE-III}} Photometric Maps of the Small Magellanic Cloud},
  author = {Udalski, A. and Soszy{\'n}ski, I. and Szyma{\'n}ski, M. K. and Kubiak, M. and Pietrzy{\'n}ski, G. and {Wyrzykowski} and Szewczyk, O. and Ulaczyk, K. and Poleski, R.},
  year = {2008},
  journal = {Acta Astronomica},
  volume = {58},
  number = {4},
  eprint = {0901.4632},
  pages = {329--343},
  issn = {00015237},
  urldate = {2020-04-11},
  abstract = {We present OGLE-III Photometric Maps of the Small Magellanic Cloud. They contain precise, calibrated VI photometry of about 6.2 million stars from 41 OGLE-III fields in the SMC observed regularly in the years 2001-2008 and covering about 14 square degrees in the sky. Also precise astrometry of these objects is provided. One of the fields, SMC140, is centered on the 47 Tucanae Galactic globular cluster providing unique data on this object. We discuss quality of the data and present a few color-magnitude diagrams of the observed fields. All photometric data are available to the astronomical community from the OGLE Internet archive.},
  archiveprefix = {arxiv},
  keywords = {Catalogs,Magellanic clouds,notion,notion-database,Surveys,Techniques: Photometric}
}

@article{Udalski2015,
  title = {{{OGLE-IV}}: {{Fourth}} Phase of the {{Optical Gravitational Lensing Experiment}}},
  author = {Udalski, A. and Szyma{\'n}ski, M. K. and Szyma{\'n}ski, G.},
  year = {2015},
  journal = {Acta Astronomica},
  volume = {65},
  number = {1},
  eprint = {1504.05966},
  pages = {1--38},
  publisher = {{Copernicus Foundation for Polish Astronomy}},
  issn = {00015237},
  urldate = {2020-04-11},
  abstract = {We present both the technical overview and main science drivers of the fourth phase of the Optical Gravitational Lensing Experiment (hereafter OGLE-IV). OGLE-IV is currently one of the largest sky variability surveys worldwide, targeting the densest stellar regions of the sky. The survey covers over 3000 square degrees in the sky and monitors regularly over a billion sources. The main targets include the inner Galactic Bulge and the Magellanic System. Their photometry spans the range of 12 {$<$} I {$<$} 21 mag and 13 {$<$} I {$<$} 21.7 mag, respectively. Supplementary shallower Galaxy Variability Survey covers the extended Galactic bulge and 2/3 of the whole Galactic disk within the magnitude range of 10 {$<$} I {$<$} 19 mag. All OGLE-IV surveys provide photometry with milli-magnitude accuracy at the bright end. The cadence of observations varies from 19-60 minutes in the inner Galactic bulge to 1-3 days in the remaining Galactic bulge fields, Magellanic System and the Galactic disk. OGLE-IV provides the astronomical community with a number of real time services. The Early Warning System (EWS) contains information on two thousand gravitational microlensing events being discovered in real time annually, the OGLE Transient Detection System (OTDS) delivers over 200 supernovae a year. We also provide the real time photometry of unpredictable variables such as optical counterparts to the X-ray sources and R Coronae Borealis stars. Hundreds of thousands new variable stars have already been discovered and classified by the OGLE survey. The number of new detections will be at least doubled during the current OGLE-IV phase. The survey was designed and optimized primarily to conduct the second generation microlensing survey for exoplanets. It has already contributed significantly to the increase of the discovery rate of microlensing exoplanets and free-floating planets.},
  archiveprefix = {arxiv},
  keywords = {Galaxy: bulge,Galaxy: disk,Magellanic Clouds,notion,notion-database,Surveys,Techniques: Photometric}
}

@article{Ueno1998,
  title = {{{3D Velocity-Field Observation}} of {{Solar Convection I}}. {{Characteristics}} of {{Mesogranulation}}},
  author = {Ueno, Satoru and Kitai, Reizaburo},
  year = {1998},
  journal = {PASJ},
  volume = {50},
  pages = {125--139},
  issn = {0004-6264},
  doi = {10.1093/PASJ/50.1.125},
  urldate = {2020-03-14},
  keywords = {CONVECTION,notion,notion-database,SUN: ATMOSPHERIC MOTION,SUN: MESOGRANULATION,SUN: PHOTOSPHERE}
}

@article{Ulrich1970,
  title = {The {{Five-Minute Oscillations}} on the {{Solar Surface}}},
  author = {Ulrich, Roger K.},
  year = {1970},
  month = dec,
  journal = {The Astrophysical Journal},
  volume = {162},
  pages = {993},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/150731},
  urldate = {2020-02-28},
  abstract = {The acoustic properties of the subphotospheric layers are examined. It is shown that standing acoustic waves may be trapped in a layer below the photosphere. These standing waves may exist only along discrete lines in the diagnostic diagram of horizontal wavenumber versus frequency. The positions of these lines are derived from a modal analysis of the solar envelope. The lines for the fundamental mode and the first-overtone mode pass through the centers of the two peaks observed by Frazier. An examination of the energy balance of the oscillations shows that they are overstable. When they are assigned an amplitude of 0.2 km , they generate about (5-7) x 106 ergs . This power output suggests that the dissipation of the 5-minute oscillations above the temperature minimum is responsible for heating the chromosphere and corona.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/HHGJTZG9/full-text.pdf}
}

@inproceedings{Ulrich1983,
  title = {Solar Seismology from Space},
  author = {Ulrich, R., K.},
  year = {1983},
  urldate = {2020-03-02},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AUJGHH4N/full-text.pdf}
}

@article{Ulrich1986,
  title = {Determination of Stellar Ages from Asteroseismology},
  author = {Ulrich, R. K.},
  year = {1986},
  journal = {The Astrophysical Journal},
  volume = {306},
  pages = {L37},
  issn = {0004-637X},
  doi = {10.1086/184700},
  abstract = {This Letter shows that measurements of the stellar analog of the solar 5 minute oscillations can permit the determination of the radius and age of isolated stars. The key frequencies of oscillation correspond to pairs of modes differing by two in the degree of the spherical harmonic describing the angular dependence of the motion and by one in the overtone order of the modes. The frequency pairs are very nearly degenerate, and adequate frequency resolution will require a nearly unbroken time sequence extending over 15 days.},
  keywords = {Astrophysics,Cepheid Variables,Chronology,notion,notion-database,Plasma Diagnostics,Plasma Frequencies,Seismology,STARS: EVOLUTION,STARS: PULSATION,Stellar Evolution,Stellar Models,Stellar Oscillations},
  file = {/Users/lbugnet/Zotero/storage/9UBUC6WI/Ulrich - 1986.pdf}
}

@book{Unno1989,
  title = {Nonradial Oscillations of Stars},
  author = {Unno, Wasaburo and Osaki, Yoji and Ando, Hiroyasu and Saio, H and Shibahashi, H},
  year = {1989},
  publisher = {{University of Tokyo Press}},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JXRSZEF6/Unno et al. - 1989.pdf}
}

@incollection{Unno1989a,
  title = {Unno {{Chapter}} 5: {{EXCITATION AND DAMPING OF OSCILLATIONS}}},
  author = {Unno, Wasaburo},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GQTEGWHG/Unno - 1989.pdf}
}

@incollection{Unno1989b,
  title = {Unno {{Introduction}}},
  author = {Unno, Wasaburo},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6T76CPDC/Unno - 1989(3).pdf}
}

@misc{Unno1989c,
  title = {Unno {{Chapter}} 3:{{BASIC EQUATIONS AND ADIABATIC OSCILLATIONS}}},
  author = {Unno, Wasaburo},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VI6A5B8Y/Unno - 1989(5).pdf}
}

@incollection{Unno1989d,
  title = {Unno {{Chapter}} 2: {{OBSERVATIONAL ASPECTS OF NONRADIAL OSCILLATIONS}}},
  author = {{Unno}},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/96TMGV3B/Unno - 1989(6).pdf}
}

@incollection{Unno1989e,
  title = {Unno {{Chapter}} 3: {{ADIABATIC OSCILLATIONS}} Suite},
  author = {Unno, Wasaburo},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6WIY77J4/Unno - 1989(7).pdf}
}

@incollection{Unno1989f,
  title = {Unno: References},
  author = {Unno, Wasaburo},
  year = {1989},
  pages = {380--399},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/M68KY472/Unno - 1989(4).pdf}
}

@incollection{Unno1989g,
  title = {Unno {{Chapter}} 7: {{HELIO}}\_ {{AND ASTEROSEISMOLOGY}}},
  author = {Unno, Wasaburo},
  year = {1989},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZSUYJHJ3/Unno - 1989(2).pdf}
}

@article{Uytterhoeven2008a,
  title = {The {$\gamma$} {{Doradus CoRoT}} Target {{HD}} 49434: {{I}}. {{Results}} from the Ground-Based Campaign},
  author = {Uytterhoeven, K. and Mathias, P. and Poretti, E. and Rainer, M. and {Mart{\'i}n-Ruiz}, S. and Rodr{\'i}guez, E. and Amado, P. J. and Le Contel, D. and Jankov, S. and Niemczura, E. and Pollard, K. R. and Brunsden, E. and Papar{\'o}, M. and Costa, V. and Valtier, J. C. and Garrido, R. and Su{\'a}rez, J. C. and Kilmartin, P. M. and Chapellier, E. and {Rodr{\'i}guez-L{\'o}pez}, C. and Marin, A. J. and Aceituno, F. J. and Casanova, V. and Rolland, A. and Olivares, I.},
  year = {2008},
  journal = {Astronomy and Astrophysics},
  volume = {489},
  number = {3},
  pages = {1213--1224},
  issn = {00046361},
  doi = {10.1051/0004-6361:200809992},
  abstract = {Context. We present an extensive ground-based photometric and spectroscopic campaign of the {$\gamma$} Dor CoRoT target HD 49434. This campaign was a preparatory step of the CoRoT satellite observations, which occurred between October 2007 and March 2008.Aims. With satellite data, detection of low-degree pulsation modes only is achievable, and, as no filters are available, with poor identification. Ground-based data promise eventually to identify additional modes and provide extra input for the identification: spectroscopic data allows the detection of high-degree modes and an estimate of the azimuthal number . We attempt to detect and identify as many pulsation modes as possible from the ground-based dataset of the {$\gamma$} Dor star HD 49434, and anticipate the CoRoT results. Methods. We searched for frequencies in the multi-colour variations, the pixel-to-pixel variations across the line profiles, and the moments variations in a large dataset, consisting of both multi-colour photometric and spectroscopic data from different observatories, using different frequency analysis methods. We performed a tentative mode identification of the spectroscopic frequencies using the Moment Method and the Intensity Period Search Method. We also completed an abundance analysis.Results. The frequency analysis clearly indicates the presence of four frequencies in the 0.2-1.7 d-1 interval, as well as six frequencies in the 5-12 d -1domain. The low frequencies are typical of {$\gamma$} Dor variables, while the high frequencies are common to {$\lambda$} Sct pulsators. We propose that the frequency 2.666 dd-1 is the rotational frequency. All modes, for which an identification was possible, appear to be high-degree modes (3 {$\leq$} {$\mathscr{l}$} {$\leq$} 8). We did not find evidence for a possible binary nature of the star HD 49434. The element abundances that we derived are consistent with values obtained in previous analyses. Conclusions. We classify the {$\gamma$} Dor star HD 49434 as a hybrid pulsator, which pulsates simultaneously in p- and q-modes. This implies that HD 49434 is an extremely interesting target for asteroseismic modelling. \textcopyright{} 2008 ESO.},
  keywords = {Line: profiles,notion,notion-database,Stars: individual: HD 49434,Stars: oscillations,Stars: variables: {$\delta$} Sct},
  file = {/Users/lbugnet/Zotero/storage/563SLSAL/Uytterhoeven et al. - 2008.pdf}
}

@article{Uytterhoeven2011,
  title = {The {{Kepler}} Characterization of the Variability among {{A-and F-type}} Stars: {{I}}. {{General}} Overview},
  author = {Uytterhoeven, K. and Moya, A. and Grigahc{\`e}ne, A. and Guzik, J. A. and {Guti{\'e}rrez-Soto}, J. and Smalley, B. and Handler, G. and Balona, L. A. and Niemczura, E. and Fox MacHado, L. and Benatti, S. and Chapellier, E. and Tkachenko, A. and Szab{\'o}, R. and Su{\'a}rez, J. C. and Ripepi, V. and Pascual, J. and Mathias, P. and {Mart{\'i}n-Ru{\'i}z}, S. and Lehmann, H. and Jackiewicz, J. and Hekker, S. and Gruberbauer, M. and Garc{\'i}a, R. A. and Dumusque, X. and {D{\'i}az-Fraile}, D. and Bradley, P. and Antoci, V. and Roth, M. and Leroy, B. and Murphy, S. J. and De Cat, P. and Cuypers, J. and Kjeldsen, H. and {Christensen-Dalsgaard}, J. and Breger, M. and Pigulski, A. and Kiss, L. L. and Still, M. and Thompson, S. E. and Van Cleve, J.},
  year = {2011},
  journal = {Astronomy and Astrophysics},
  volume = {534},
  eprint = {1107.0335},
  issn = {00046361},
  doi = {10.1051/0004-6361/201117368},
  abstract = {Context. The Kepler spacecraft is providing time series of photometric data with micromagnitude precision for hundreds of A-F type stars. Aims. We present a first general characterization of the pulsational behaviour of A-F type stars as observed in the Kepler light curves of a sample of 750 candidate A-F type stars, and observationally investigate the relation between {$\gamma$} Doradus ({$\gamma$} Dor), {$\delta$} Scuti ({$\delta$} Sct), and hybrid stars. Methods. We compile a database of physical parameters for the sample stars from the literature and new ground-based observations. We analyse the Kepler light curve of each star and extract the pulsational frequencies using different frequency analysis methods. We construct two new observables, "energy" and "efficiency", related to the driving energy of the pulsation mode and the convective efficiency of the outer convective zone, respectively. Results. We propose three main groups to describe the observed variety in pulsating A-F type stars: {$\gamma$} Dor, {$\delta$} Sct, and hybrid stars. We assign 63\% of our sample to one of the three groups, and identify the remaining part as rotationally modulated/active stars, binaries, stars of different spectral type, or stars that show no clear periodic variability. 23\% of the stars (171 stars) are hybrid stars, which is a much higher fraction than what has been observed before. We characterize for the first time a large number of A-F type stars (475 stars) in terms of number of detected frequencies, frequency range, and typical pulsation amplitudes. The majority of hybrid stars show frequencies with all kinds of periodicities within the {$\gamma$} Dor and {$\delta$} Sct range, also between 5 and 10 d-1, which is a challenge for the current models. We find indications for the existence of {$\delta$} Sct and {$\gamma$} Dor stars beyond the edges of the current observational instability strips. The hybrid stars occupy the entire region within the {$\delta$} Sct and {$\gamma$} Dor instability strips and beyond. Non-variable stars seem to exist within the instability strips. The location of {$\gamma$} Dor and {$\delta$} Sct classes in the (T eff, log g)-diagram has been extended. We investigate two newly constructed variables, "efficiency" and "energy", as a means to explore the relation between {$\gamma$} Dor and {$\delta$} Sct stars. Conclusions. Our results suggest a revision of the current observational instability strips of {$\delta$} Sct and {$\gamma$} Dor stars and imply an investigation of pulsation mechanisms to supplement the {$\kappa$} mechanism and convective blocking effect to drive hybrid pulsations. Accurate physical parameters for all stars are needed to confirm these findings. \textcopyright{} 2011 ESO.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Binaries: general,notion,notion-database,Stars: fundamental parameters,Stars: oscillations,Stars: statistics,Stars: variables:{$\delta$}Scuti},
  file = {/Users/lbugnet/Zotero/storage/SRUSRKVB/Uytterhoeven et al. - 2011.pdf}
}

@article{Uzundag2021,
  title = {Asteroseismic Analysis of Variable Hot Subdwarf Stars Observed with {{TESS}}. {{I}}. {{The}} Mean g-Mode Period Spacings in Hot Subdwarf {{B}} Stars},
  author = {Uzundag, Murat and Vu{\v c}kovi{\'c}, Maja and N{\'e}meth, P{\'e}ter and Miller Bertolami, M. and Silvotti, Roberto and Baran, Andrzej S. and Telting, John H. and Reed, Mike and Shoaf, K. A. and {\O}stensen, Roy H. and Sahoo, Sumanta K.},
  year = {2021},
  month = jul,
  journal = {Astronomy \& Astrophysics},
  volume = {651},
  pages = {A121},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202140961},
  urldate = {2023-10-14},
  abstract = {Context. We present photometric and spectroscopic analyses of gravity (g-mode) long-period pulsating hot subdwarf B (sdB) stars, also called V1093 Her stars, observed by the TESS space telescope in both 120 s short-cadence and 20 s ultra-short-cadence mode during the survey observation and the extended mission of the southern ecliptic hemisphere. Aims: We performed a detailed asteroseismic and spectroscopic analysis of five pulsating sdB stars observed with TESS in order to compare the observations with model predictions based on our stellar evolution computations coupled with adiabatic pulsation computations. Methods: We processed and analyzed TESS observations of long-period pulsating hot subdwarf B stars. We used standard pre-whitening techniques on the datasets to extract the pulsation periods from the TESS light curves. We applied standard seismic tools for mode identification, including asymptotic period spacings and rotational frequency multiplets. Based on the values obtained from Kolmogorov-Smirnov and Inverse Variance tests, we searched for a constant period spacing for dipole (l = 1) and quadrupole (l = 2) modes. We calculated the mean period spacing for l = 1 and l = 2 modes and estimated the errors by means of a statistical resampling analysis. For all stars, atmospheric parameters were derived by fitting synthetic spectra to the newly obtained low-resolution spectra. We computed stellar evolution models using the LPCODE stellar evolution code, and computed l = 1 g-mode frequencies with the adiabatic nonradial pulsation code LP-PUL. Derived observational mean period spacings were then compared to the mean period spacings from detailed stellar evolution computations coupled with the adiabatic pulsation computations of g-modes. Results: We detect 73 frequencies, most of which are identified as dipole and quadrupole g-modes with periods spanning from {$\sim$}3000 s to {$\sim$}14 500 s. The derived mean period spacing of dipole modes is concentrated in a narrow region ranging from 251 s to 256 s, while the mean period spacing for quadrupole modes spans from 145 s to 154 s. The atmospheric parameters derived from spectroscopic data are typical of long-period pulsating sdB stars with an effective temperature ranging from 23 700 K to 27 600 K and surface gravity spanning from 5.3 dex to 5.5 dex. In agreement with the expectations from theoretical arguments and previous asteroseismological works, we find that the mean period spacings obtained for models with small convective cores, as predicted by a pure Schwarzschild criterion, are incompatible with the observations. We find that models with a standard, modest convective boundary mixing at the boundary of the convective core are in better agreement with the observed mean period spacings and are therefore more realistic. Conclusions: Using high-quality space-based photometry collected by the TESS mission coupled with low-resolution spectroscopy from the ground, we provide a global comparison of the observations with model predictions by means of a robust indicator such as the mean period spacing. All five objects that we analyze in this work show remarkable homogeneity in both seismic and spectroscopic properties. Based on observations at the La Silla Observatory of the European Southern Observatory for programs number 0103.D-0511 and 0104.D-0514. Based on observations obtained at Las Campanas Observatory under the run code 0KJ21U8U.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: horizontal-branch,stars: interiors,stars: oscillations,subdwarfs},
  annotation = {ADS Bibcode: 2021A\&A...651A.121U},
  file = {/Users/lbugnet/Zotero/storage/6USGIH5H/Uzundag et al. - 2021 - Asteroseismic analysis of variable hot subdwarf st.pdf}
}

@article{Uzundag2023,
  title = {Asteroseismological Analysis of the Polluted {{ZZ Ceti}} Star {{G}} 29-38 with {{TESS}}},
  author = {Uzundag, Murat and De Ger{\'o}nimo, Francisco C. and C{\'o}rsico, Alejandro H. and Silvotti, Roberto and Bradley, Paul A. and Montgomery, Michael H. and Catelan, M{\'a}rcio and Toloza, Odette and Bell, Keaton J. and Kepler, S. O. and Althaus, Leandro G. and Kleinman, Scot J. and Kilic, Mukremin and Mullally, Susan E. and G{\"a}nsicke, Boris T. and B{\k{a}}kowska, Karolina and Barber, Sam and Nitta, Atsuko},
  year = {2023},
  month = sep,
  journal = {Monthly Notices of the Royal Astronomical Society},
  issn = {0035-8711},
  doi = {10.1093/mnras/stad2776},
  urldate = {2023-09-22},
  abstract = {G 29-38 (TIC 422526868) is one of the brightest (V = 13.1) and closest (d = 17.51 pc) pulsating white dwarfs with a hydrogen-rich atmosphere (DAV/ZZ Ceti class). It was observed by the TESS spacecraft in sectors 42 and 56. The atmosphere of G 29-38 is polluted by heavy elements that are expected to sink out of visible layers on short timescales. The photometric TESS data set spans \textasciitilde 51 days in total, and from this, we identified 56 significant pulsation frequencies, that include rotational frequency multiplets. In addition, we identified 30 combination frequencies in each sector. The oscillation frequencies that we found are associated with g-mode pulsations, with periods spanning from \textasciitilde{} 260 s to \textasciitilde{} 1400 s. We identified rotational frequency triplets with a mean separation {$\delta\nu\mathscr{l}$} = 1 of 4.67 {$\mu$}Hz and a quintuplet with a mean separation {$\delta\nu\mathscr{l}$} = 2 of 6.67 {$\mu$}Hz, from which we estimated a rotation period of about 1.35 {$\pm$} 0.1 days. We determined a constant period spacing of 41.20 s for {$\mathscr{l}$} = 1 modes and 22.58 s for {$\mathscr{l}$} = 2 modes. We performed period-to-period fit analyses and found an asteroseismological model with M{$\star$}/M{$\odot$} = 0.632 {$\pm$} 0.03, Teff = 11 635 {$\pm$} 178 K, and log g = 8.048 {$\pm$} 0.005 (with a hydrogen envelope mass of MH \textasciitilde{} 5.6 \texttimes{} 10-5M{$\star$}), in good agreement with the values derived from spectroscopy. We obtained an asteroseismic distance of 17.54 pc, which is in excellent agreement with that provided by Gaia (17.51 pc).},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: evolution,stars: interiors,stars: oscillations (including pulsations),stars: white dwarfs},
  annotation = {ADS Bibcode: 2023MNRAS.tmp.2656U},
  file = {/Users/lbugnet/Zotero/storage/GVZNUKF7/Uzundag et al. - 2023 - Asteroseismological analysis of the polluted ZZ Ce.pdf}
}

@article{Valenti2005,
  title = {Spectroscopic {{Properties}} of {{Cool Stars}} ({{SPOCS}}). {{I}}. 1040 {{F}}, {{G}}, and {{K Dwarfs}} from {{Keck}}, {{Lick}}, and {{AAT Planet Search Programs}}},
  author = {Valenti, Jeff A. and Fischer, Debra A.},
  year = {2005},
  month = jul,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {159},
  number = {1},
  pages = {141--166},
  publisher = {{IOP Publishing}},
  issn = {0067-0049},
  doi = {10.1086/430500},
  urldate = {2020-03-16},
  abstract = {We present a uniform catalog of stellar properties for 1040 nearby F, G, and K stars that have been observed by the Keck, Lick, and AAT planet search programs. Fitting observed echelle spectra with synthetic spectra yielded effective temperature, surface gravity, metallicity, projected rotational velocity, and abundances of the elements Na, Si, Ti, Fe, and Ni, for every star in the catalog. Combining V-band photometry and Hipparcos parallaxes with a bolometric correction based on the spectroscopic results yielded stellar luminosity, radius, and mass. Interpolating Yonsei-Yale isochrones to the luminosity, effective temperature, metallicity, and {$\alpha$}-element enhancement of each star yielded a theoretical mass, radius, gravity, and age range for most stars in the catalog. Automated tools provide uniform results and make analysis of such a large sample practical. Our analysis method differs from traditional abundance analyses in that we fit the observed spectrum directly, rather than trying to match equivalent widths, and we determine effective temperature and surface gravity from the spectrum itself, rather than adopting values based on measured photometry or parallax. As part of our analysis, we determined a new relationship between macroturbulence and effective temperature on the main sequence. Detailed error analysis revealed small systematic offsets with respect to the Sun and spurious abundance trends as a function of effective temperature that would be inobvious in smaller samples. We attempted to remove these errors by applying empirical corrections, achieving a precision per spectrum of 44 K in effective temperature, 0.03 dex in metallicity, 0.06 dex in the logarithm of gravity, and 0.5 km s-1 in projected rotational velocity. Comparisons with previous studies show only small discrepancies. Our spectroscopically determined masses have a median fractional precision of 15\%, but they are systematically 10\% higher than masses obtained by interpolating isochrones. Our spectroscopic radii have a median fractional precision of 3\%. Our ages from isochrones have a precision that varies dramatically with location in the Hertzsprung-Russell diagram. We plan to extend the catalog by applying our automated analysis technique to other large stellar samples.},
  keywords = {Catalogs,notion,notion-database,Stars: Abundances,Stars: Fundamental Parameters,Stars: Late,Techniques: Spectroscopic,Type},
  file = {/Users/lbugnet/Zotero/storage/8SDBVSVY/full-text.pdf}
}

@article{Valyavin2005,
  title = {Rotation Period and Magnetic Field Morphology of the White Dwarf {{WD}}\,0009+501},
  author = {Valyavin, G. and Bagnulo, S. and Monin, D. and Fabrika, S. and Lee, B.-C. and Galazutdinov, G. and Wade, G. A. and Burlakova, T.},
  year = {2005},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {439},
  number = {3},
  pages = {1099--1106},
  publisher = {{EDP Sciences}},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20052642},
  urldate = {2020-07-16},
  abstract = {We present new spectropolarimetric observations of the weak-field magnetic white dwarf WD 0009+501. From these data we estimate that the star's longitudinal magnetic field varies with the rotation phase from about -120kG to about +50 kG, and that the surface magnetic field varies from about 150kG to about 300 kG. Earlier estimates of the stellar rotation period are revised anew, and we find that the most probable period is about 8 h. We have attempted to recover the star's magnetic morphology by modelling the available magnetic observables, assuming that the field is described by the superposition of a dipole and a quadrupole. According to the best-fit model, the inclination of the rotation axis with respect to the line of sight is i = 60\textdegree{} {$\pm$} 20\textdegree, and the angle between the rotation axis and the dipolar axis is {$\beta$} = 111\textdegree{} {$\pm$} 17\textdegree. The dipole strength at the pole is about 340 kG, and the quadrupolar strength is about 300 kG. \textcopyright{} ESO 2005.},
  keywords = {notion,notion-database,Stars: individual: WD 0009+501,Stars: magnetic fields,Stars: rotation,Stars: white dwarfs},
  file = {/Users/lbugnet/Zotero/storage/3MUEIYJH/full-text.pdf}
}

@article{vanBallegooijen1982,
  title = {The Overshoot Layer at the Base of the Solar Convective Zone and the Problem of Magnetic Flux Storage.},
  author = {{van Ballegooijen}, A. A.},
  year = {1982},
  month = sep,
  journal = {Astronomy and Astrophysics},
  volume = {113},
  pages = {99--112},
  issn = {0004-6361},
  urldate = {2023-10-18},
  abstract = {Possibilities for storing a horizontal magnetic field in the overshoot layer at the base of the solar convective zone, or in the radiative zone below it, are studied using a one-dimensional model of the overshoot layer. The convective energy flux is estimated using a linear mode analysis. The thickness of the overshoot layer is found to be a few tenths of the pressure scale height, with an abrupt temperature gradient change at the base of the layer. Neutrally buoyant horizontal flux tubes, with an equipartition field strength greater than or about equal to 10 to the fourth Gauss, could be stabilized in the overshoot layer, but an additional force is needed to counteract the buoyancy force from an inflow of heat into the tubes. The Coriolis force on a mass flow along the toroidal flux with a flow velocity of 8 m/s may hold tubes with an equipartition field strength of about 10 to the fourth Gauss in the overshoot layer, and such flux tubes may be stable for solar cycle periods.},
  keywords = {Astrophysics,Convective Heat Transfer,Coriolis Effect,Entropy,Layers,Magnetic Flux,Solar Flux,Solar Magnetic Field,Solar Physics,Stellar Structure,Velocity Distribution},
  annotation = {ADS Bibcode: 1982A\&A...113...99V},
  file = {/Users/lbugnet/Zotero/storage/X5LI3LGI/van Ballegooijen - 1982 - The overshoot layer at the base of the solar conve.pdf}
}

@article{VanBeeck2020,
  title = {Detecting Axisymmetric Magnetic Fields Using Gravity Modes in Intermediate-Mass Stars},
  author = {{van Beeck}, J. and Prat, V. and Van Reeth, T. and Mathis, S. and Bowman, D.M. and Neiner, C. and Aerts, C.},
  year = {2020},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {638},
  number = {A149},
  eprint = {2005.02411},
  publisher = {{EDP Sciences}},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201937363},
  urldate = {2020-05-31},
  abstract = {Context: Angular momentum (AM) transport models of stellar interiors require improvements to explain the strong extraction of AM from stellar cores that is observed with asteroseismology. One of the often invoked mediators of AM transport are internal magnetic fields, even though their properties, observational signatures and influence on stellar evolution are largely unknown. Aims: We study how a fossil, axisymmetric internal magnetic field affects period spacing patterns of dipolar gravity mode oscillations in main-sequence stars with masses of 1.3, 2.0 and 3.0 M\$\_\textbackslash odot\$. We assess the influence of fundamental stellar parameters on the magnitude of pulsation mode frequency shifts. Methods: We compute dipolar gravity mode frequency shifts due to a fossil, axisymmetric poloidal-toroidal internal magnetic field for a grid of stellar evolution models, varying stellar fundamental parameters. Rigid rotation is taken into account using the traditional approximation of rotation and the influence of the magnetic field is computed using a perturbative approach. Results: We find magnetic signatures for dipolar gravity mode oscillations in terminal-age main-sequence stars that are measurable for a near-core field strength larger than \$10\^\{5\}\$ G. The predicted signatures differ appreciably from those due to rotation. Conclusions: Our formalism demonstrates the potential for the future detection and characterization of strong fossil, axisymmetric internal magnetic fields in gravity-mode pulsators near the end of core-hydrogen burning from Kepler photometry, if such fields exist.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,magnetic field,notion,notion-database,oscillations,rotation,stars,waves},
  file = {/Users/lbugnet/Zotero/storage/7LK4KM6A/Van Beeck et al. - 2020.pdf}
}

@article{Vanderburg2014,
  title = {A {{Technique}} for {{Extracting Highly Precise Photometry}} for the {{Two-Wheeled Kepler Mission}}},
  author = {Vanderburg, Andrew and Johnson, John Asher},
  year = {2014},
  journal = {Publications of the Astronomical Society of the Pacific},
  volume = {126},
  number = {944},
  eprint = {1408.3853},
  pages = {948--958},
  issn = {00046280},
  doi = {10.1086/678764},
  abstract = {The original Kepler mission achieved high photometric precision thanks to ultra-stable pointing enabled by use of four reaction wheels. The loss of two of these reaction wheels reduced the telescope's ability to point precisely for extended periods of time, and as a result, the photometric precision has suffered. We present a technique for generating photometric light curves from pixel-level data obtained with the two-wheeled extended Kepler mission, K2. Our photometric technique accounts for the non-uniform pixel response function of the Kepler detectors by correlating flux measurements with the spacecraft's pointing and removing the dependence. When we apply our technique to the ensemble of stars observed during the Kepler Two-Wheel Concept Engineering Test, we find improvements over raw K2 photometry by factors of 2-5, with noise properties qualitatively similar to Kepler targets at the same magnitudes. We find evidence that the improvement in photometric precision depends on each target's position in the Kepler field of view, with worst precision near the edges of the field. Overall, this technique restores the median attainable photometric precision to within a factor of two of the original Kepler photometric precision for targets ranging from 10\$\^\{th\}\$ to 15\$\^\{th\}\$ magnitude in the Kepler bandpass, peaking with a median precision within 35\% that of Kepler for stars between 12\$\^\{th\}\$ and 13\$\^\{th\}\$ magnitude in the Kepler bandpass.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PGZDKRBQ/Vanderburg, Johnson - 2014.pdf}
}

@article{VanDerMaaten2008,
  title = {Visualizing {{Data}} Using T-{{SNE}}},
  author = {{van der Maaten}, Laurens and Hinton, Geoffrey},
  year = {2008},
  journal = {Journal of Machine Learning Research},
  volume = {9},
  pages = {2579--2605},
  urldate = {2020-07-20},
  abstract = {We present a new technique called "t-SNE" that visualizes high-dimensional data by giving each datapoint a location in a two or three-dimensional map. The technique is a variation of Stochastic Neighbor Embedding (Hinton and Roweis, 2002) that is much easier to optimize, and produces significantly better visualizations by reducing the tendency to crowd points together in the center of the map. t-SNE is better than existing techniques at creating a single map that reveals structure at many different scales. This is particularly important for high-dimensional data that lie on several different, but related, low-dimensional manifolds, such as images of objects from multiple classes seen from multiple viewpoints. For visualizing the structure of very large data sets, we show how t-SNE can use random walks on neighborhood graphs to allow the implicit structure of all of the data to influence the way in which a subset of the data is displayed. We illustrate the performance of t-SNE on a wide variety of data sets and compare it with many other non-parametric visualization techniques, including Sammon mapping, Isomap, and Locally Linear Embedding. The visualiza-tions produced by t-SNE are significantly better than those produced by the other techniques on almost all of the data sets.},
  keywords = {dimensionality reduction,embedding algorithms,manifold learning,multidimensional scaling,notion,notion-database,visualization},
  file = {/Users/lbugnet/Zotero/storage/FI9XPVLE/full-text.pdf}
}

@article{VanderPlas2018,
  title = {Understanding the {{Lomb}}\textendash{{Scargle Periodogram}}},
  author = {VanderPlas, Jacob T.},
  year = {2018},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {236},
  number = {1},
  eprint = {1703.09824},
  pages = {16},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/aab766},
  abstract = {The Lomb-Scargle periodogram is a well-known algorithm for detecting and characterizing periodic signals in unevenly-sampled data. This paper presents a conceptual introduction to the Lomb-Scargle periodogram and important practical considerations for its use. Rather than a rigorous mathematical treatment, the goal of this paper is to build intuition about what assumptions are implicit in the use of the Lomb-Scargle periodogram and related estimators of periodicity, so as to motivate important practical considerations required in its proper application and interpretation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/77SJ5KSM/VanderPlas - 2018.pdf}
}

@article{VanEylen2018,
  title = {{{HD}} 89345: {{A}} Bright Oscillating Star Hosting a Transiting Warm {{Saturn-sized}} Planet Observed by {{K2}}},
  author = {{van Eylen}, V. and Dai, F. and Mathur, S. and Gandolfi, D. and Albrecht, S. and Fridlund, M. and Garc{\'i}a, R. A. and Guenther, E. and Hjorth, M. and Justesen, A. B. and Livingston, J. and Lund, M. N. and P{\'e}rez Hern{\'a}ndez, F. and {Prieto-Arranz}, J. and Regulo, C. and Bugnet, L. and Everett, M. E. and Hirano, T. and Nespral, D. and Nowak, G. and Palle, E. and Silva Aguirre, V. and Trifonov, T. and Winn, J. N. and Barrag{\'a}n, O. and Beck, P. G. and Chaplin, W. J. and Cochran, W. D. and Csizmadia, S. and Deeg, H. and Endl, M. and Heeren, P. and Grziwa, S. and Hatzes, A. P. and Hidalgo, D. and Korth, J. and Mathis, S. and Rodriguez, P. Monta{\~n}es and Narita, N. and Patzold, M. and Persson, C. M. and Rodler, F. and Smith, A. M.S.},
  year = {2018},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {478},
  number = {4},
  eprint = {1805.01860},
  pages = {4866--4880},
  issn = {13652966},
  doi = {10.1093/mnras/sty1390},
  abstract = {We report the discovery and characterization of HD 89345b (K2-234b; EPIC 248777106b), a Saturn-sized planet orbiting a slightly evolved star. HD 89345 is a bright star (V = 9.3 mag) observed by the K2 mission with 1 min time sampling. It exhibits solar-like oscillations. We conducted asteroseismology to determine the parameters of the star, finding themass and radius to be 1.12-0.01+0.04 M{$\odot$} and 1.657 -0.004+0.020 R{$\odot$}, respectively. The star appears to have recently left the main sequence, based on the inferred age, 9.4-1.3+0.4 Gyr, and the non-detection of mixed modes. The star hosts a 'warm Saturn' (P = 11.8 d, Rp = 6.86 {$\pm$} 0.14 R{$\oplus$}). Radial-velocity follow-up observations performed with the FIbre-fed Echelle Spectrograph, HARPS, and HARPS-N spectrographs show that the planet has a mass of 35.7 {$\pm$} 3.3 M{$\oplus$}. The data also show that the planet's orbit is eccentric (e{$\approx$}0.2). An investigation of the rotational splitting of the oscillation frequencies of the star yields no conclusive evidence on the stellar inclination angle. We further obtained Rossiter-McLaughlin observations, which result in a broad posterior of the stellar obliquity. The planet seems to confirm to the same patterns that have been observed for other sub-Saturns regarding planet mass and multiplicity, orbital eccentricity, and stellar metallicity.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,notion,notion-database,Planets and satellites: composition,Planets and satellites: formation,Planets and satellites: fundamental parameters},
  file = {/Users/lbugnet/Zotero/storage/YPDKCSCI/Van Eylen et al. - 2018.pdf}
}

@article{VanLeeuwen2007a,
  title = {Validation of the New {{Hipparcos}} Reduction},
  author = {Van Leeuwen, F.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {474},
  number = {2},
  eprint = {0708.1752},
  pages = {653--664},
  issn = {00046361},
  doi = {10.1051/0004-6361:20078357},
  abstract = {Context. A new reduction of the astrometric data as produced by the Hipparcos mission has been published, claiming accuracies for nearly all stars brighter than magnitude Hp = 8 to be better, by up to a factor 4, than in the original catalogue. Aims. The new Hipparcos astrometric catalogue is checked for the quality of the data and the consistency of the formal errors as well as the possible presence of error correlations. The differences with the earlier publication are explained. Methods. The internal errors are followed through the reduction process, and the external errors are investigated on the basis of a comparison with radio observations of a small selection of stars, and the distribution of negative parallaxes. Error correlation levels are investigated and the reduction by more than a factor 10 as obtained in the new catalogue is explained. Results. The formal errors on the parallaxes for the new catalogue are confirmed. The presence of a small amount of additional noise, though unlikely, cannot be ruled out. Conclusions. The new reduction of the Hipparcos astrometric data provides an improvement by a factor 2.2 in the total weight compared to the catalogue published in 1997, and provides much improved data for a wide range of studies on stellar luminosities and local galactic kinematics. \textcopyright ESO 2007.},
  archiveprefix = {arxiv},
  keywords = {Astrometry,Catalogs,Instrumentation: miscellaneous,Methods: data analysis,notion,notion-database,Space vehicles: instruments},
  file = {/Users/lbugnet/Zotero/storage/Z3HBPN46/Van Leeuwen - 2007.pdf}
}

@misc{vanoniNotero2022,
  title = {Notero},
  author = {Vanoni, David},
  year = {2022},
  month = jul,
  urldate = {2022-07-18},
  abstract = {A Zotero plugin for syncing items into Notion},
  copyright = {MIT},
  keywords = {notion,notion-database,typescript,zotero,zotero-plugin,zotero-sync}
}

@article{Vanreeth2015,
  title = {{{GRAVITY-MODE PERIOD SPACINGS AS A SEISMIC DIAGNOSTIC}} for {{A SAMPLE}} of {$\gamma$} {{DORADUS STARS}} from {{KEPLER SPACE PHOTOMETRY}} and {{HIGH-RESOLUTION GROUND-BASED SPECTROSCOPY}}},
  author = {Van Reeth, T. and Tkachenko, A. and Aerts, C. and P{\'a}pics, P. I. and Triana, S. A. and Zwintz, K. and Degroote, P. and Debosscher, J. and Bloemen, S. and Schmid, V. S. and De Smedt, K. and Fremat, Y. and Fuentes, A. S. and Homan, W. and Hrudkova, M. and Karjalainen, R. and Lombaert, R. and Nemeth, P. and {\O}stensen, R. and Van De Steene, G. and Vos, J. and Raskin, G. and Van Winckel, H.},
  year = {2015},
  month = jun,
  journal = {Astrophysical Journal, Supplement Series},
  volume = {218},
  number = {2},
  eprint = {1504.02119},
  pages = {27},
  publisher = {{Institute of Physics Publishing}},
  issn = {00670049},
  doi = {10.1088/0067-0049/218/2/27},
  urldate = {2020-11-29},
  abstract = {Gamma Doradus stars (hereafter {$\gamma$} Dor stars) are gravity-mode pulsators of spectral type A or F. Such modes probe the deep stellar interior, offering a detailed fingerprint of their structure. Four-year high-precision space-based Kepler photometry of {$\gamma$} Dor stars has become available, allowing us to study these stars with unprecedented detail. We selected, analyzed, and characterized a sample of 67 {$\gamma$} Dor stars for which we have Kepler observations available. For all the targets in the sample we assembled high-resolution spectroscopy to confirm their F-type nature. We found fourteen binaries, among which are four single-lined binaries, five double-lined binaries, two triple systems, and three binaries with no detected radial velocity variations. We estimated the orbital parameters whenever possible. For the single stars and the single-lined binaries, fundamental parameter values were determined from spectroscopy. We searched for period spacing patterns in the photometric data and identified this diagnostic for 50 of the stars in the sample, 46 of which are single stars or single-lined binaries. We found a strong correlation between the spectroscopic v sin i and the period spacing values, confirming the influence of rotation on {$\gamma$} Dor-type pulsations as predicted by theory. We also found relations between the dominant g-mode frequency, the longest pulsation period detected in series of prograde modes, v sin i, and Teff.},
  archiveprefix = {arxiv},
  keywords = {asteroseismology,notion,notion-database,stars: fundamental parameters,stars: oscillations,stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/LGT3U59F/full-text.pdf}
}

@article{VanReeth2016,
  title = {Interior Rotation of a Sample of {$\gamma$} {{Doradus}} Stars from Ensemble Modelling of Their Gravity-Mode Period Spacings},
  author = {Van Reeth, T. and Tkachenko, A. and Aerts, C.},
  year = {2016},
  month = oct,
  journal = {Astronomy \& Astrophysics},
  volume = {593},
  pages = {A120},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201628616},
  urldate = {2023-10-17},
  abstract = {Context. Gamma Doradus stars (hereafter {$\gamma$} Dor stars) are known to exhibit gravity- and/or gravito-intertial modes that probe the inner stellar region near the convective core boundary. The non-equidistant spacing of the pulsation periods is an observational signature of the stellar evolutions and current internal structure and is heavily influenced by rotation. Aims: We aim to constrain the near-core rotation rates for a sample of {$\gamma$} Dor stars for which we have detected period spacing patterns. Methods: We combined the asymptotic period spacing with the traditional approximation of stellar pulsation to fit the observed period spacing patterns using {$\chi$}2-optimisation. The method was applied to the observed period spacing patterns of a sample of stars and used for ensemble modelling. Results: For the majority of stars with an observed period spacing pattern we successfully determined the rotation rates and the asymptotic period spacing values, although the uncertainty margins on the latter were typically large. This also resulted directly in the identification of the modes that correspond to the detected pulsation frequencies, which for most stars were prograde dipole gravity and gravito-inertial modes. The majority of the observed retrograde modes were found to be Rossby modes. We also discuss the limitations of the method that are due to the neglect of the centrifugal force and the incomplete treatment of the Coriolis force. Conclusions: Despite its current limitations, the proposed method was successful to derive the rotation rates and to identify the modes from the observed period spacing patterns. It forms the first step towards detailed seismic modelling based on observed period spacing patterns of moderately to rapidly rotating {$\gamma$}Dor stars. Based on data gathered with the NASA Discovery mission Kepler and the HERMES spectrograph, which is installed at the Mercator Telescope, operated on the island of La Palma by the Flemish Community at the Spanish Observatorio del Roque de los Muchachos of the Instituto de Astrof\'isica de Canarias, and supported by the Fund for Scientific Research of Flanders (FWO), Belgium, the Research Council of KU Leuven, Belgium, the Fonds National de la Recherche Scientifique (F.R.S.-FNRS), Belgium, the Royal Observatory of Belgium, the Observatoire de Gen\`eve, Switzerland, and the Th\"uringer Landessternwarte Tautenburg, Germany.},
  keywords = {asteroseismology,Astrophysics - Solar and Stellar Astrophysics,methods: data analysis,stars: fundamental parameters,stars: oscillations,stars: variables: general},
  annotation = {ADS Bibcode: 2016A\&A...593A.120V},
  file = {/Users/lbugnet/Zotero/storage/686HZ9TL/Van Reeth et al. - 2016 - Interior rotation of a sample of γ Doradus stars f.pdf}
}

@article{Vanreeth2018,
  title = {Sensitivity of Gravito-Inertial Modes to Differential Rotation in Intermediate-Mass Main-Sequence Stars},
  author = {Van Reeth, T. and Mombarg, J. S.G. and Mathis, S. and Tkachenko, A. and Fuller, J. and Bowman, D. M. and Buysschaert, B. and Johnston, C. and Garc{\'i}a Hern{\'a}ndez, A. and Goldstein, J. and Townsend, R. H.D. and Aerts, C.},
  year = {2018},
  month = oct,
  journal = {Astronomy \& Astrophysics},
  volume = {618},
  eprint = {1806.03586},
  pages = {A24},
  publisher = {{EDP Sciences}},
  issn = {14320746},
  doi = {10.1051/0004-6361/201832718},
  urldate = {2020-11-29},
  abstract = {Context. While rotation has a major impact on stellar structure and evolution, its effects are not well understood. Thanks to high-quality and long-Time base photometric observations obtained with recent space missions, we are now able to study stellar rotation more precisely. Aims. We aim to constrain radial differential rotation profiles in {$\gamma$} Doradus ({$\gamma$} Dor) stars, and to develop new theoretical seismic diagnosis for such stars with rapid and potentially non-uniform rotation. Methods. We have derived a new asymptotic description which accounts for the impact of weak differential near-core rotation on gravity-mode period spacings. The theoretical predictions are illustrated from pulsation computations with the code GYRE and compared with observations of {$\gamma$} Dor stars. When possible, we also derived the surface rotation rates in these stars by detecting and analysing signatures of rotational modulation, and computed the core-To-surface rotation ratios. Results. Stellar rotation must be strongly differential before its effects on period spacing patterns can be detected, unless multiple period spacing patterns can be compared. Six stars in our sample exhibit a single unexplained period spacing pattern of retrograde modes. We hypothesise that these are Yanai modes. Finally, we find signatures of rotational spot modulation in the photometric data of eight targets. Conclusions. If only one period spacing pattern is detected and analysed for a star, it is difficult to detect differential rotation. A rigidly rotating model will often provide the best solution. Differential rotation can only be detected when multiple period spacing patterns have been found for a single star or its surface rotation rate is known as well. This is the case for eight of the stars in our sample, revealing surface-To-core rotation ratios between 0.95 and 1.05.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: fundamental parameters,Stars: oscillations,Stars: rotation,Stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/MS7UCUW3/full-text.pdf}
}

@article{vanRoestel2018,
  title = {Discovery of 36 Eclipsing {{EL CVn}} Binaries Found by the {{Palomar Transient Factory}}},
  author = {{van Roestel}, J. and Kupfer, T. and {Ruiz-Carmona}, R. and Groot, P. J. and Prince, T. A. and Burdge, K. and Laher, R. and Shupe, D. L. and Bellm, E.},
  year = {2018},
  month = apr,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {475},
  pages = {2560--2590},
  issn = {0035-8711},
  doi = {10.1093/mnras/stx3291},
  urldate = {2023-10-09},
  abstract = {We report on the discovery and analysis of 36 new eclipsing EL CVn-type binaries, consisting of a core helium-composition pre-white dwarf (pre-He-WD) and an early-type main-sequence companion. This more than doubles the known population of these systems. We have used supervised machine learning methods to search 0.8 million light curves from the Palomar Transient Factory (PTF), combined with Sloan Digital Sky Survey (SDSS), Panoramic Survey Telescope and Rapid Response System (Pan-STARRS) and Two-Micron All-Sky Survey (2MASS) colours. The new systems range in orbital periods from 0.46 to 3.8 d and in apparent brightness from {$\sim$}14 to 16 mag in the PTF R or g΄ filters. For 12 of the systems, we obtained radial velocity curves with the Intermediate Dispersion Spectrograph at the Isaac Newton Telescope. We modelled the light curves, radial velocity curves and spectral energy distributions to determine the system parameters. The radii (0.3-0.7 R{$\odot$}) and effective temperatures (8000-17 000 K) of the pre-He-WDs are consistent with stellar evolution models, but the masses (0.12-0.28 M{$\odot$}) show more variance than models have predicted. This study shows that using machine learning techniques on large synoptic survey data is a powerful way to discover substantial samples of binary systems in short-lived evolutionary stages.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,binaries: close,binaries: eclipsing,stars: individual: EL CVn,white dwarfs},
  annotation = {ADS Bibcode: 2018MNRAS.475.2560V},
  file = {/Users/lbugnet/Zotero/storage/RYKSBQ5Z/van Roestel et al. - 2018 - Discovery of 36 eclipsing EL CVn binaries found by.pdf}
}

@article{VanSaders2013,
  title = {Fast Star, Slow Star; {{Old}} Star, Young Star: {{Subgiant}} Rotation as a Population and Stellar Physics Diagnostic},
  author = {{van Saders}, Jennifer L. and Pinsonneault, Marc H.},
  year = {2013},
  journal = {Astrophysical Journal},
  volume = {776},
  number = {2},
  eprint = {1306.3701},
  issn = {15384357},
  doi = {10.1088/0004-637X/776/2/67},
  abstract = {Stellar rotation is a strong function of both mass and evolutionary state. Missions such as Kepler and CoRoT provide tens of thousands of rotation periods, drawn from stellar populations that contain objects at a range of masses, ages, and evolutionary states. Given a set of reasonable starting conditions and a prescription for angular momentum loss, we address the expected range of rotation periods for cool field stellar populations ({$\sim$}0.4-2.0 M {$\odot$}). We find that cool stars fall into three distinct regimes in rotation. Rapid rotators with surface periods less than 10 days are either young low-mass main sequence (MS) stars, or higher mass subgiants which leave the MS with high rotation rates. Intermediate rotators (10-40 days) can be either cool MS dwarfs, suitable for gyrochronology, or crossing subgiants at a range of masses. Gyrochronology relations must therefore be applied cautiously, since there is an abundant population of subgiant contaminants. The slowest rotators, at periods greater than 40 days, are lower mass subgiants undergoing envelope expansion. We identify additional diagnostic uses of rotation periods. There exists a period-age relation for subgiants distinct from the MS period-age relations. There is also a period-radius relation that can be used as a constraint on the stellar radius, particularly in the interesting case of planet host stars. The high-mass/low-mass break in the rotation distribution on the MS persists onto the subgiant branch, and has potential as a diagnostic of stellar mass. Finally, this set of theoretical predictions can be compared to extensive datasets to motivate improved modeling. \textcopyright{} 2013. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: evolution,stars: fundamental parameters,stars: interiors,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/H93HVITW/Van Saders, Pinsonneault - 2013.pdf}
}

@article{VanSaders2016,
  title = {Weakened Magnetic Braking as the Origin of Anomalously Rapid Rotation in Old Field Stars},
  author = {{van Saders}, Jennifer L. and Ceillier, Tugdual and Metcalfe, Travis S. and Aguirre, Victor Silva and Pinsonneault, Marc H. and Garc{\'i}a, Rafael A. and Mathur, Savita and Davies, Guy R.},
  year = {2016},
  journal = {Nature},
  volume = {529},
  number = {7585},
  pages = {181--184},
  publisher = {{Nature Publishing Group}},
  issn = {14764687},
  doi = {10.1038/nature16168},
  abstract = {A knowledge of stellar ages is crucial for our understanding of many astrophysical phenomena, and yet ages can be difficult to determine. As they become older, stars lose mass and angular momentum, resulting in an observed slowdown in surface rotation. The technique of gyrochronology uses the rotation period of a star to calculate its age. However, stars of known age must be used for calibration, and, until recently, the approach was untested for old stars (older than 1 gigayear, Gyr). Rotation periods are now known for stars in an open cluster of intermediate age (NGC 6819; 2.5 Gyr old), and for old field stars whose ages have been determined with asteroseismology. The data for the cluster agree with previous period-age relations, but these relations fail to describe the asteroseismic sample. Here we report stellar evolutionary modelling, and confirm the presence of unexpectedly rapid rotation in stars that are more evolved than the Sun. We demonstrate that models that incorporate dramatically weakened magnetic braking for old stars can - unlike existing models - reproduce both the asteroseismic and the cluster data. Our findings might suggest a fundamental change in the nature of ageing stellar dynamos, with the Sun being close to the critical transition to much weaker magnetized winds. This weakened braking limits the diagnostic power of gyrochronology for those stars that are more than halfway through their main-sequence lifetimes.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ZYB38BD6/Van Saders et al. - 2016.pdf}
}

@article{Varshalovich1988,
  title = {The {{Graphical Method}} in {{Angular Momentum Theory}}},
  author = {Varshalovich, D A and Moskalev, A N and Khersonskii, V K},
  year = {1988},
  journal = {Quantum Theory of Angular Momentum},
  pages = {412--451},
  doi = {10.1142/9789814415491_0012},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GV7C88TU/Varshalovich, Moskalev, Khersonskii - 1988.pdf}
}

@article{Varshalovich1988a,
  title = {Introduction: {{Basic Concepts}}},
  author = {Varshalovich, D A and Moskalev, A N and Khersonskii, V K},
  year = {1988},
  journal = {Quantum Theory of Angular Momentum},
  pages = {1--2},
  doi = {10.1142/9789814415491_0001},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6ZGBBLLF/Varshalovich, Moskalev, Khersonskii - 1988(2).pdf}
}

@article{Vauclair2008,
  title = {Astrophysics {{L}} Etter to the {{E}} Ditor {{The}} Exoplanet-Host Star {$\iota$} {{Horologii}} : An Evaporated},
  author = {Vauclair, S and Laymand, M and Bouchy, F and Vauclair, G and Hoa, A Hui Bon and Charpinet, S and Bazot, M},
  year = {2008},
  volume = {8},
  number = {November 2006},
  pages = {5--8},
  keywords = {abundances,galaxy,hyades,individual,notion,notion-database,open cluster and associations,oscillations,planetary systems,stars,{stars: oscillations, stars: planetary systems, sta}},
  file = {/Users/lbugnet/Zotero/storage/75LJ7KRP/Vauclair et al. - 2008.pdf}
}

@article{Vauclair2010,
  title = {Precise Characterisation of Exoplanet-Host Stars Parameters},
  author = {Vauclair, Sylvie},
  year = {2010},
  journal = {Proceedings of the International Astronomical Union},
  volume = {6},
  number = {S276},
  pages = {30--33},
  issn = {17439213},
  doi = {10.1017/S1743921311019892},
  abstract = {Studying the internal structure of exoplanet-host stars compared to that of similar stars without detected planets is particularly important for the understanding of planetary formation. In this framework, asteroseismic studies represent an excellent tool for a better characterization of stars and for a precise determination of the stellar parameters like mass, radius, gravity, effective temperature. The detection of stellar oscillations is obtained with the same instruments as used for the discovery of exoplanets, both from the ground and from space, although the time scales are very different. Here I discuss some details about the characterization of exoplanethost stars from seismology and the importance of the helium and heavy element abundances in this respect. \textcopyright{} International Astronomical Union 2011.},
  isbn = {9780521196529},
  keywords = {Abundances,Interiors,notion,notion-database,Oscillations,Stars},
  file = {/Users/lbugnet/Zotero/storage/X8U74QS8/Vauclair - 2010.pdf}
}

@incollection{Vectorsa,
  title = {Chapter 1 {{ELEMENTS OF VECTOR AND TENSOR THEORY}}},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {i},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4ZMUTU8Y/Unknown - Unknown(16).pdf}
}

@techreport{Velikhov1959,
  title = {Stability of an Ideally Conducting Liquid  Flowing between Cylinders Rotating in a Magnetic Field},
  author = {Velikhov, E P},
  year = {1959},
  journal = {J. Exptl. Theoret. Phys. (U.S.S.R.)},
  volume = {36},
  number = {9},
  pages = {1398--1404},
  urldate = {2020-07-02},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/4JX5S99K/full-text.pdf}
}

@article{Ventura2008,
  title = {The {{ATON}} 3.1 Stellar Evolutionary Code: {{A}} Version for Asteroseismology},
  author = {Ventura, Paolo and D'Antona, Francesca and Mazzitelli, Italo},
  year = {2008},
  journal = {Astrophysics and Space Science},
  volume = {316},
  number = {1-4},
  pages = {93--98},
  issn = {0004640X},
  doi = {10.1007/s10509-007-9672-8},
  abstract = {We describe the main features of the evolutionary code ATON 3.1 and its latest version, particularly deviced to be apt for follow up asteroseismology applications. An older version of the code including rotational evolution is also shortly described. \textcopyright{} 2007 Springer Science+Business Media B.V.},
  keywords = {Convection,Diffusion,notion,notion-database,Stellar oscillations,Stellar structure},
  file = {/Users/lbugnet/Zotero/storage/FRGA3IC3/Ventura, D'Antona, Mazzitelli - 2008.pdf}
}

@article{Verma2014a,
  title = {Asteroseismic Estimate of Helium Abundance of a Solar Analog Binary System},
  author = {Verma, Kuldeep and Faria, Jo{\~a}o P. and Antia, H. M. and Basu, Sarbani and Mazumdar, Anwesh and Monteiro, M{\'a}rio J.P.F.G. and Appourchaux, Thierry and Chaplin, William J. and Garc{\'i}a, Rafael A. and Metcalfe, Travis S.},
  year = {2014},
  journal = {Astrophysical Journal},
  volume = {790},
  number = {2},
  eprint = {1405.7512},
  pages = {1--43},
  issn = {15384357},
  doi = {10.1088/0004-637X/790/2/138},
  abstract = {16 Cyg A and B are among the brightest stars observed by Kepler. What makes these stars more interesting is that they are solar analogs. 16 Cyg A and B exhibit solar-like oscillations. In this work we use oscillation frequencies obtained using 2.5 yr of Kepler data to determine the current helium abundance of these stars. For this we use the fact that the helium ionization zone leaves a signature on the oscillation frequencies and that this signature can be calibrated to determine the helium abundance of that layer. By calibrating the signature of the helium ionization zone against models of known helium abundance, the helium abundance in the envelope of 16 Cyg A is found to lie in the range of 0.231 to 0.251 and that of 16 Cyg B lies in the range of 0.218 to 0.266. \textcopyright{} 2014. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,{stars: Abundancesstars: individual (HD 186408, HD}},
  file = {/Users/lbugnet/Zotero/storage/YSWA4W2Q/Verma et al. - 2014.pdf}
}

@article{Verner2011,
  title = {Global Asteroseismic Properties of Solar-like Oscillations Observed by {{Kepler}}: {{A}} Comparison of Complementary Analysis Methods},
  author = {Verner, G. A. and Elsworth, Y. and Chaplin, W. J. and Campante, T. L. and Corsaro, E. and Gaulme, P. and Hekker, S. and Huber, D. and Karoff, C. and Mathur, S. and Mosser, B. and Appourchaux, T. and Ballot, J. and Bedding, T. R. and Bonanno, A. and Broomhall, A. M. and Garc{\'i}a, R. A. and Handberg, R. and New, R. and Stello, D. and R{\'e}gulo, C. and Roxburgh, I. W. and Salabert, D. and White, T. R. and Caldwell, D. A. and Christiansen, J. L. and Fanelli, M. N.},
  year = {2011},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {415},
  number = {4},
  pages = {3539--3551},
  issn = {00358711},
  doi = {10.1111/j.1365-2966.2011.18968.x},
  abstract = {We present the asteroseismic analysis of 1948 F-, G- and K-type main-sequence and subgiant stars observed by the National Aeronautics and Space Administration Kepler mission. We detect and characterize solar-like oscillations in 642 of these stars. This represents the largest cohort of main-sequence and subgiant solar-like oscillators observed to date. The photometric observations are analysed using the methods developed by nine independent research teams. The results are combined to validate the determined global asteroseismic parameters and calculate the relative precision by which the parameters can be obtained. We correlate the relative number of detected solar-like oscillators with stellar parameters from the Kepler Input Catalogue and find a deficiency for stars with effective temperatures in the range 5300 {$\lessequivlnt$}Teff{$\lessequivlnt$} 5700K and a drop-off in detected oscillations in stars approaching the red edge of the classical instability strip. We compare the power-law relationships between the frequency of peak power, {$\nu$}max, the mean large frequency separation, {$\Delta\nu$}, and the maximum mode amplitude, Amax, and show that there are significant method-dependent differences in the results obtained. This illustrates the need for multiple complementary analysis methods to be used to assess the robustness and reproducibility of results derived from global asteroseismic parameters. \textcopyright{} 2011 The Authors Monthly Notices of the Royal Astronomical Society \textcopyright{} 2011 RAS.},
  keywords = {notion,notion-database,Stars: fundamental parameters,Stars: interiors,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/F5B8KKPZ/Verner et al. - 2011.pdf}
}

@article{Verner2011a,
  title = {Verification of the Kepler Input Catalog from Asteroseismology of Solar-Type Stars},
  author = {Verner, G. A. and Chaplin, W. J. and Basu, S. and Brown, T. M. and Hekker, S. and Huber, D. and Karoff, C. and Mathur, S. and Metcalfe, T. S. and Mosser, B. and Quirion, P. O. and Appourchaux, T. and Bedding, T. R. and Bruntt, H. and Campante, T. L. and Elsworth, Y. and Garc{\'i}a, R. A. and Handberg, R. and R{\'e}gulo, C. and Roxburgh, I. W. and Stello, D. and {Christensen-Dalsgaard}, J. and Gilliland, R. L. and Kawaler, S. D. and Kjeldsen, H. and Allen, C. and Clarke, B. D. and Girouard, F. R.},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {738},
  number = {2},
  eprint = {1109.0869},
  pages = {1--12},
  issn = {20418205},
  doi = {10.1088/2041-8205/738/2/L28},
  abstract = {We calculate precise stellar radii and surface gravities from the asteroseismic analysis of over 500 solar-type pulsating stars observed by the Kepler space telescope. These physical stellar properties are compared with those given in the Kepler Input Catalog (KIC), determined from ground-based multi-color photometry. For the stars in our sample, we find general agreement but we detect an average overestimation bias of 0.23dex in the KIC determination of log (g) for stars with log (g)KIC {$>$} 4.0dex, and a resultant underestimation bias of up to 50\% in the KIC radii estimates for stars with R KIC {$<$} 2 R. Part of the difference may arise from selection bias in the asteroseismic sample; nevertheless, this result implies there may be fewer stars characterized in the KIC with R 1 R {$\odot$} than is suggested by the physical properties in the KIC. Furthermore, if the radius estimates are taken from the KIC for these affected stars and then used to calculate the size of transiting planets, a similar underestimation bias may be applied to the planetary radii. \textcopyright{} 2011 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: fundamental parameters,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/3IXZ4ZRC/Verner et al. - 2011(2).pdf}
}

@article{Vida2013,
  title = {Detecting Activity Cycles of Late-Type Dwarfs in {{Kepler}} Data},
  author = {Vida, K. and Ol{\'a}h, K.},
  year = {2013},
  month = aug,
  journal = {Proceedings of the International Astronomical Union},
  volume = {9},
  number = {S302},
  eprint = {1308.2641},
  pages = {224--227},
  publisher = {{Cambridge University Press}},
  doi = {10.1017/S1743921314002142},
  urldate = {2020-07-12},
  abstract = {Using data of fast-rotating active dwarf stars in the Kepler database, we perform time-frequency analysis of the light curves in order to search for signs of activity cycles. We use the phenomenon that the active region latitudes vary with the cycle (like the solar butterfly diagram), which causes the observed rotation period to change as a consequence of differential rotation. We find cycles in 8 cases of the 39 promising targets with periods between of 300-900 days.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: activity,stars: low-mass,stars: magnetic fields,stars: rotation,stars: spots}
}

@article{Vida2018,
  title = {Finding Flares in {{Kepler}} Data Using Machine-Learning Tools},
  author = {Vida, Kriszti{\'a}n and Roettenbacher, Rachael M.},
  year = {2018},
  journal = {Astronomy and Astrophysics},
  volume = {616},
  eprint = {1806.00334},
  pages = {1--5},
  issn = {14320746},
  doi = {10.1051/0004-6361/201833194},
  abstract = {Context. Archives of long photometric surveys, such as the Kepler database, are a great basis for studying flares. However, identifying the flares is a complex task; it is easily done in the case of single-target observations by visual inspection, but is nearly impossible for several year-long time series for several thousand targets. Although automated methods for this task exist, several problems are difficult (or impossible) to overcome with traditional fitting and analysis approaches. Aims. We introduce a code for identifying and analyzing flares based on machine-learning methods, which are intrinsically adept at handling such data sets. Methods. We used the RANSAC (RANdom SAmple Consensus) algorithm to model light curves, as it yields robust fits even in the case of several outliers, such as flares. The light curves were divided into search windows, approximately on the order of the stellar rotation period. This search window was shifted over the data set, and a voting system was used to keep false positives to a minimum: only those flare candidate points were kept that were identified as a flare in several windows. Results. The code was tested on short-cadence K2 observations of TRAPPIST-1 and on long-cadence Kepler data of KIC 1722506. The detected flare events and flare energies are consistent with earlier results from manual inspections.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,notion,notion-database,Stars: activity,Stars: flare,Stars: late-type,Stars: low-mass,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/EVBKTXWH/Vida, Roettenbacher - 2018.pdf}
}

@article{Vidotto2014,
  title = {Stellar Magnetism: {{Empirical}} Trends with Age and Rotation},
  author = {Vidotto, A. A. and Gregory, S. G. and Jardine, M. and Donati, J. F. and Petit, P. and Morin, J. and Folsom, C. P. and Bouvier, J. and Cameron, A. C. and Hussain, G. and Marsden, S. and Waite, I. A. and Fares, R. and Jeffers, S. and Do Nascimento, J. D.},
  year = {2014},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {441},
  number = {3},
  eprint = {1404.2733},
  pages = {2361--2374},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stu728},
  urldate = {2020-07-17},
  abstract = {We investigate how the observed large-scale surface magnetic fields of low-mass stars {\~(}0.1-2M{$\odot$}), reconstructed through Zeeman-Doppler imaging, vary with age t, rotation and X-ray emission. Our sample consists of 104 magnetic maps of 73 stars, from accreting premain sequence to main-sequence objects (1 Myr {$\lessequivlnt$} t {$\lessequivlnt$} 10 Gyr). For non-accreting dwarfs we empirically find that the unsigned average large-scale surface field is related to age as t-0.655 {$\pm$} 0.045. This relation has a similar dependence to that identified by Skumanich, used as the basis for gyrochronology. Likewise, our relation could be used as an age-dating method ('magnetochronology'). The trends with rotation we find for the large-scale stellar magnetism are consistent with the trends found from Zeeman broadening measurements (sensitive to large-and small-scale fields). These similarities indicate that the fields recovered from both techniques are coupled to each other, suggesting that small-and large-scale fields could share the same dynamo field generation processes. For the accreting objects, fewer statistically significant relations are found, with one being a correlation between the unsigned magnetic flux and rotation period. We attribute this to a signature of star-disc interaction, rather than being driven by the dynamo. \textcopyright{} 2014 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Planetary systems,Stars: Activity,Stars: Evolution,Stars: Magnetic field,Stars: Rotation,Techniques: Polarimetric},
  file = {/Users/lbugnet/Zotero/storage/XL4HT3UK/full-text.pdf}
}

@article{Vieytes2004,
  title = {Chromospheric Models of Solar Type Stars: {{The Vaughan-Preston}} Gap},
  author = {Vieytes, M. and Mauas, P. J.D.},
  year = {2004},
  journal = {Astrophysics and Space Science},
  volume = {290},
  number = {3-4},
  pages = {311--318},
  issn = {0004640X},
  doi = {10.1023/b:astr.0000032532.94509.5d},
  abstract = {We have built different models for stars of the same spectral type than the Sun but with different levels of chromospheric activity, to study the response of the S index of activity built from the emission of the Ca II H and K lines to changes in the chromospheric structure. We found that the fact that there are many stars with either strong or weak emission, but few with intermediate values of S, the so-called Vaughan-Preston gap, can be due to a discontinuity in the response of the Ca II lines to chromospheric heating. In fact, we are able to reproduce the observed distribution of the number of stars as a function of S.},
  keywords = {notion,notion-database,Stars: activity,Stars: atmospheres,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/DJYSHCGN/Vieytes, Mauas - 2004.pdf}
}

@article{Villebrun2019,
  title = {Astronomy {{Astrophysics Magnetic}} Fields of Intermediate-Mass {{T Tauri}} Stars {{I}}. {{Magnetic}} Detections and Fundamental Stellar Parameters},
  author = {Villebrun, F and Alecian, E and Hussain, G and Bouvier, J and Folsom, C P and Lebreton, Y and Amard, L and Charbonnel, C and Gallet, F and Haemmerl{\'e}, L and B{\"o}hm, T and {Johns-Krull}, C and Kochukhov, O and Marsden, S C and Morin, J and Petit, P},
  year = {2019},
  journal = {Astronomy \& Astrophysics},
  volume = {622},
  pages = {72},
  doi = {10.1051/0004-6361/201833545},
  urldate = {2020-07-31},
  abstract = {Context. The origin of the fossil magnetic fields detected in 5 to 10\% of intermediate-mass main sequence stars is still highly debated. Aims. We want to bring observational constraints to a large population of intermediate-mass pre-main sequence (PMS) stars in order to test the theory that convective-dynamo fields generated during the PMS phases of stellar evolution can occasionally relax into fossil fields on the main sequence. Methods. Using distance estimations, photometric measurements, and spectropolarimetric data from HARPSpol and ESPaDOnS of 38 intermediate-mass PMS stars, we determined fundamental stellar parameters (T eff , L and v sin i) and measured surface magnetic field characteristics (including detection limits for non-detections, and longitudinal fields and basic topologies for positive detections). Using PMS evolutionary models, we determined the mass, radius, and internal structure of these stars. We compared different PMS models to check that our determinations were not model-dependant. We then compared the magnetic characteristics of our sample accounting for their stellar parameters and internal structures. Results. We detect magnetic fields in about half of our sample. About 90\% of the magnetic stars have outer convective envelopes larger than {$\sim$}25\% of the stellar radii, and heavier than {$\sim$}2\% of the stellar mass. Going to higher mass, we find that the magnetic incidence in intermediate-mass stars drops very quickly, within a timescale on the order of few times 0.1 Myr. Finally, we propose that intermediate-mass T Tauri stars with large convective envelopes, close to the fully convective limit, have complex fields and that their dipole component strengths may decrease as the sizes of their convective envelopes decrease, similar to lower-mass T Tauri stars.},
  keywords = {activity-stars,fundamental parameters-stars,Herbig Ae/Be,magnetic field-stars,notion,notion-database,pre-main sequence-stars,stars,T Tauri,variables},
  file = {/Users/lbugnet/Zotero/storage/XYBWMIJ3/full-text.pdf}
}

@article{Vorontsov2002,
  title = {Helioseismic Measurement of Solar Torsional Oscillations},
  author = {Vorontsov, S. V. and {Christensen-Dalsgaard}, J. and Schou, J. and Strakhov, V. N. and Thompson, M. J.},
  year = {2002},
  journal = {Science},
  volume = {296},
  number = {5565},
  pages = {101--103},
  issn = {00368075},
  doi = {10.1126/science.1069190},
  abstract = {Bands of slower and faster rotation, the so-called torsional oscillations, are observed at the Sun's surface to migrate in latitude over the 11-year solar cycle. Here, we report on the temporal variations of the Sun's internal rotation from solar p-mode frequencies obtained over nearly 6 years by the Michelson Doppler Imager (MDI) instrument on board the Solar and Heliospheric Observatory (SOHO) satellite. The entire solar convective envelope appears to be involved in the torsional oscillations, with phase propagating poleward and equatorward from midlatitudes at all depths throughout the convective envelope.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/SIFAZMAU/Vorontsov et al. - 2002.pdf}
}

@article{Vos2015,
  title = {Testing Eccentricity Pumping Mechanisms to Model Eccentric Long Period {{sdB}} Binaries with {{MESA}}},
  author = {Vos, Joris and {\O}stensen, Roy and Marchant, Pablo and Winckel, Hans},
  year = {2015},
  month = may,
  journal = {Astronomy \& Astrophysics},
  volume = {579},
  doi = {10.1051/0004-6361/201526019},
  abstract = {Hot subdwarf-B stars in long-period binaries are found to be on eccentric orbits, even though current binary-evolution theory predicts those objects to be circularised before the onset of Roche-lobe overflow (RLOF). We aim to find binary-evolution mechanisms that can explain these eccentric long-period orbits, and reproduce the currently observed period-eccentricity diagram. Three different processes are considered; tidally-enhanced wind mass-loss, phase-dependent RLOF on eccentric orbits and the interaction between a circumbinary disk and the binary. The binary module of the stellar-evolution code MESA (Modules for Experiments in Stellar Astrophysics) is extended to include the eccentricity-pumping processes. The effects of different input parameters on the final period and eccentricity of a binary-evolution model are tested with MESA. The end products of models with only tidally-enhanced wind mass-loss can indeed be eccentric, but these models need to lose too much mass, and invariably end up with a helium white dwarf that is too light to ignite helium. Within the tested parameter space, no sdBs in eccentric systems are formed. Phase-dependent RLOF can reintroduce eccentricity during RLOF, and could help to populate the short-period part of the period-eccentricity diagram. When phase-dependent RLOF is combined with eccentricity pumping via a circumbinary disk, the higher eccentricities can be reached as well. A remaining problem is that these models favour a distribution of higher eccentricities at lower periods, while the observed systems show the opposite. The models presented here are potentially capable of explaining the period-eccentricity distribution of long-period sdB binaries, but further theoretical work on the physical mechanisms is necessary.},
  file = {/Users/lbugnet/Zotero/storage/55EN2A4R/Vos et al. - 2015 - Testing eccentricity pumping mechanisms to model e.pdf}
}

@article{Vousden2016a,
  title = {Dynamic Temperature Selection for Parallel Tempering in {{Markov}} Chain {{Monte Carlo}} Simulations},
  author = {Vousden, W. D. and Farr, W. M. and Mandel, I.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {455},
  number = {2},
  eprint = {1501.05823},
  pages = {1919--1937},
  issn = {13652966},
  doi = {10.1093/MNRAS/STV2422},
  abstract = {Modern problems in astronomical Bayesian inference require efficient methods for sampling from complex, high-dimensional, often multimodal probability distributions. Most popular methods, such as MCMC sampling, perform poorly on strongly multimodal probability distributions, rarely jumping between modes or settling on just one mode without finding others. Parallel tempering addresses this problem by sampling simultaneously with separate Markov chains from tempered versions of the target distribution with reduced contrast levels. Gaps between modes can be traversed at higher temperatures, while individual modes can be efficiently explored at lower temperatures. In this paper, we investigate how one might choose the ladder of temperatures to achieve more efficient sampling, as measured by the autocorrelation time of the sampler. In particular, we present a simple, easily implemented algorithm for dynamically adapting the temperature configuration of a sampler while sampling. This algorithm dynamically adjusts the temperature spacing to achieve a uniform rate of exchanges between chains at neighbouring temperatures. We compare the algorithm to conventional geometric temperature configurations on a number of test distributions and on an astrophysical inference problem, reporting efficiency gains by a factor of 1.2-2.5 over a well-chosen geometric temperature configuration and by a factor of 1.5-5 over a poorly chosen configuration. On all of these problems, a sampler using the dynamical adaptations to achieve uniform acceptance ratios between neighbouring chains outperforms one that does not.},
  archiveprefix = {arxiv},
  keywords = {Methods: data analysis,Methods: numerical,Methods: statistical,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/IHYZ528K/Vousden, Farr, Mandel - 2016.pdf}
}

@article{Vrard2015,
  title = {Influence of Helium Ionisation on Red Giant Oscillation Spectra},
  author = {Vrard, M. and Mosser, B. and Barban, C.},
  year = {2015},
  journal = {EPJ Web of Conferences},
  volume = {101},
  pages = {06067},
  publisher = {{EDP Sciences}},
  issn = {2100-014X},
  doi = {10.1051/EPJCONF/201510106067},
  urldate = {2020-06-02},
  abstract = {Since its launch in 2009, the space mission \emph{Kepler{$<$}i/{$>$} has provided an amount of data of unprecedented quality. In particular, red giants exhibit an oscillation spectrum arranged in a regular pattern called the universal oscillation pattern. Here we analyse and characterize the departures observed from this universal pattern. We measured the deviation for more than one hundred red giants and attribute it to glitches related to the region of second ionisation of helium.}},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/E9W6ZLRZ/full-text.pdf}
}

@article{Vrard2016,
  title = {Period Spacings in Red Giants: {{II}}. {{Automated}} Measurement},
  author = {Vrard, M. and Mosser, B. and Samadi, R.},
  year = {2016},
  journal = {Astronomy and Astrophysics},
  volume = {588},
  eprint = {1602.04940},
  pages = {1--13},
  issn = {14320746},
  doi = {10.1051/0004-6361/201527259},
  abstract = {Context. The space missions CoRoT and Kepler have provided photometric data of unprecedented quality for asteroseismology. A very rich oscillation pattern has been discovered for red giants, including mixed modes that are used to decipher the red giants' interiors. They carry information on the radiative core of red giant stars and bring strong constraints on stellar evolution. Aims. Since more than 15 000 red giant light curves have been observed by Kepler, we have developed a simple and efficient method for automatically characterizing the mixed-mode pattern and measuring the asymptotic period spacing. Methods. With the asymptotic expansion of the mixed modes, we have revealed the regularity of the gravity-mode pattern. The stretched periods were used to study the evenly space periods with a Fourier analysis and to measure the gravity period spacing, even when rotation severely complicates the oscillation spectra. Results. We automatically measured gravity period spacing for more than 6100 Kepler red giants. The results confirm and extend previous measurements made by semi-automated methods. We also unveil the mass and metallicity dependence of the relation between the frequency spacings and the period spacings for stars on the red giant branch. Conclusions. The delivery of thousands of period spacings combined with all other seismic and non-seismic information provides a new basis for detailed ensemble asteroseismology.},
  archiveprefix = {arxiv},
  keywords = {Asteroseismology,Methods: data analysis,notion,notion-database,Stars: evolution,Stars: oscillations,Stars: solar-type},
  file = {/Users/lbugnet/Zotero/storage/QFJJTHRG/Vrard, Mosser, Samadi - 2016.pdf}
}

@article{Vrard2017,
  title = {Radial Mode Widths in Red Giant Stars Spectra Observed by {{Kepler}}},
  author = {Vrard, Mathieu and Mosser, Beno{\^i}t and Barban, Caroline},
  year = {2017},
  journal = {EPJ Web of Conferences},
  volume = {160},
  pages = {2--4},
  issn = {2100014X},
  doi = {10.1051/epjconf/201716004012},
  abstract = {The Kepler space mission has observed many solar-like pulsators, and helped to decipher their fundamental parameters (e.g: mass, radius, rotation). Most of the achievements recently obtained in that domain result from the analysis of the mode frequencies. However, unique information on non-adiabatic physics derives from the height and width of the modes. In this study, we aim at measuring the mode widths of the pressure modes in thousands of Kepler red giants and to analyze their variations in function of stellar parameters. To achieve that, we used a peakbagging technique on the star radial modes. The results show a relation between the radial mode linewidth and the effective temperature of the star as theoretically predicted. We also unveil a clear dependence with mass and stellar evolution for the radial mode width. This means that the mode damping depends on the evolutionary status of the stars.},
  isbn = {2017160040},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/Q8I2TASS/Vrard, Mosser, Barban - 2017.pdf}
}

@article{Vrard2019,
  title = {Analyse Sismique Des G\'eantes Rouges : Une Vision D\'etaill\'ee \`a Grande \'Echelle de La Structure Du Coeur et de l ' Enveloppe {{To}} Cite This Version :},
  author = {Vrard, Mathieu},
  year = {2019},
  keywords = {notion,notion-database}
}

@article{vrardAstrophysicsAmplitudeLifetime2018,
  title = {Astrophysics {{Amplitude}} and Lifetime of Radial Modes in Red Giant Star Spectra Observed by {{Kepler}}},
  author = {Vrard, M and Kallinger, T and Mosser, B and Barban, C and Baudin, F and Belkacem, K and Cunha, M S},
  year = {2018},
  journal = {A\&A},
  volume = {616},
  doi = {10.1051/0004-6361/201832477},
  urldate = {2021-09-03},
  abstract = {Context. The space-borne missions CoRoT and Kepler have provided photometric observations of unprecedented quality. The study of solar-like oscillations observed in red giant stars by these satellites allows a better understanding of the different physical processes occurring in their interiors. In particular, the study of the mode excitation and damping is a promising way to improve our understanding of stellar physics that has, so far, been performed only on a limited number of targets. Aims. The recent asteroseismic characterization of the evolutionary status for a large number of red giants allows us to study the physical processes acting in the interior of red giants and how they are modified during stellar evolution. In this work, we aim to obtain information on the excitation and damping of pressure modes through the measurement of the stars' pressure mode widths and amplitudes and to analyze how they are modified with stellar evolution. The objective is to bring observational constraints on the modeling of the physical processes behind mode excitation and damping. Methods. We fit the frequency spectra of red giants with well-defined evolutionary status using Lorentzian functions to derive the pressure mode widths and amplitudes. To strengthen our conclusions, we used two different fitting techniques. Results. Pressure mode widths and amplitudes were determined for more than 5000 red giants. With a stellar sample two orders of magnitude larger than previous results, we confirmed that the mode width depends on stellar evolution and varies with stellar effective temperature. In addition, we discovered that the mode width depends on stellar mass. We also confirmed observationally the influence of the stellar metallicity on the mode amplitudes, as predicted by models.},
  keywords = {asteroseismology-convection-stars,data analysis,evolution-stars,interiors-methods,notion,notion-database,solar-type-stars},
  file = {/Users/lbugnet/Zotero/storage/JSWFPP4Y/full-text.pdf}
}

@techreport{Wade2002,
  title = {The {{MiMeS Survey}} of {{Magnetism}} in {{Massive Stars}}: {{Introduction}} and Overview *},
  author = {Wade, G A and Neiner, C and Alecian, E and Grunhut, J H and Petit, V and De Batz, B and Bohlender, D A and Cohen, D H and Henrichs, H F and Kochukhov, O and Landstreet, J D and Manset, N and Martins, F and Mathis, S and Oksala, M E and Owocki, S P and Rivinius, Th and Shultz, M E and Sundqvist, J O and Townsend, R H D and {Ud-Doula}, A and Bouret, J.-C and Braithwaite, J and Briquet, M and Carciofi, A C and {David-Uraz}, A and Folsom, C P and Fullerton, A W and Leroy, B and Marcolino, W L F and Moffat, A F J and Naz{\'e}, Y and Louis, N St and Aur{\`i} Ere, M and Bagnulo, S and Bailey, J D and Barb{\'a}, R H and Blaz{\`e}re, A},
  year = {2002},
  journal = {Mon. Not. R. Astron. Soc},
  volume = {000},
  eprint = {1511.08425v1},
  pages = {41},
  urldate = {2020-07-13},
  abstract = {The MiMeS project is a large-scale, high resolution, sensitive spectropolarimetric investigation of the magnetic properties of O and early B type stars. Initiated in 2008 and completed in 2013, the project was supported by 3 Large Program allocations, as well as various programs initiated by independent PIs and archival resources. Ultimately, over 4800 circularly polarized spectra of 560 O and B stars were collected with the instruments ESPaDOnS at the Canada-France-Hawaii Telescope, Narval at the T\'elescope Bernard Lyot, and HARPSpol at the European Southern Observatory La Silla 3.6m telescope, making MiMeS by far the largest systematic investigation of massive star magnetism ever undertaken. In this paper, the first in a series reporting the general results of the survey, we introduce the scientific motivation and goals, describe the sample of targets, review the instrumentation and observational techniques used, explain the exposure time calculation designed to provide sensitivity to surface dipole fields above approximately 100 G, discuss the polarimetric performance, stability and uncertainty of the instrumentation, and summarize the previous and forthcoming publications.},
  archiveprefix = {arxiv},
  isbn = {1511.08425v1},
  keywords = {magnetic fields,massive-Instrumentation,notion,notion-database,rotation-Stars,spectropolarimetry-Stars,Stars},
  file = {/Users/lbugnet/Zotero/storage/XL9TX5Q2/full-text.pdf}
}

@techreport{Wade2013,
  title = {The Magnetic Characteristics of {{Galactic OB}} Stars from the {{MiMeS}} Survey of Magnetism in Massive Stars},
  author = {Wade, G A and Grunhut, J and Alecian, E and Neiner, C and Aur{\`i} Ere, M and Bohlender, D A and {David-Uraz}, A and Folsom, C and Henrichs, H F},
  year = {2013},
  eprint = {1310.3965v1},
  urldate = {2020-04-30},
  abstract = {The Magnetism in Massive Stars (MiMeS) project represents the largest systematic survey of stellar magnetism ever undertaken. Based on a sample of over 550 Galactic B and O-type stars, the MiMeS project has derived the basic characteristics of magnetism in hot, massive stars. Herein we report preliminary results.},
  archiveprefix = {arxiv},
  keywords = {early-type,magnetic fields,notion,notion-database,Stars},
  file = {/Users/lbugnet/Zotero/storage/JMKXZBVI/full-text.pdf}
}

@inproceedings{Wade2014,
  title = {Magnetic Fields and Internal Mixing of Main Sequence {{B}} Stars},
  booktitle = {Proceedings of the {{International Astronomical Union}}},
  author = {Wade, G. A. and Folsom, C. P. and Grunhut, J. and Landstreet, J. D. and Petit, V.},
  year = {2014},
  volume = {9},
  pages = {401--403},
  publisher = {{Cambridge University Press}},
  issn = {17439221},
  doi = {10.1017/S1743921314007273},
  urldate = {2020-05-14},
  abstract = {We have obtained high-quality magnetic field measurements of 19 sharp-lined B-type stars with precisely-measured N/C abundance ratios (Nieva \& Przybilla 2012). Our primary goal is to test the idea (Meynet et al. 2011) that a magnetic field may explain extra drag (through the wind) on the surface rotation, thus producing more internal shear and mixing, and thus could provide an explanation for the appearance of slowly rotating N-rich main sequence B stars.},
  keywords = {notion,notion-database,stars: abundances,stars: early-type,stars: evolution,stars: magnetic fields}
}

@article{Wade2016,
  title = {The {{MiMeS}} Survey of Magnetism in Massive Stars: {{Introduction}} and Overview},
  author = {Wade, G. A. and Neiner, C. and Alecian, E. and Grunhut, J. H. and Petit, V. and {de Batz}, B. and Bohlender, D. A. and Cohen, D. H. and Henrichs, H. F. and Kochukhov, O. and Landstreet, J. D. and Manset, N. and Martins, F. and Mathis, S. and Oksala, M. E. and Owocki, S. P. and Rivinius, T. and Shultz, M. E. and Sundqvist, J. O. and Townsend, R. H.D. and {Ud-Doula}, A. and Bouret, J. C. and Braithwaite, J. and Briquet, M. and Carciofi, A. C. and {David-Uraz}, A. and Folsom, C. P. and Fullerton, A. W. and Leroy, B. and Marcolino, W. L.F. and Moffat, A. F.J. and Naz{\'e}, Y. and St Louis, N. and Auri{\`e}re, M. and Bagnulo, S. and Bailey, J. D. and Barb{\'a}, R. H. and Blaz{\`e}re, A. and B{\"o}hm, T. and Catala, C. and Donati, J. F. and Ferrario, L. and Harrington, D. and Howarth, I. D. and Ignace, R. and Kaper, L. 9. and L{\"u}ftinger, T. and Prinja, R. and Vink, J. S. and Weiss, W. W. and Yakunin, I.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {456},
  number = {1},
  eprint = {1511.08425},
  pages = {2--22},
  publisher = {{Oxford University Press}},
  issn = {13652966},
  doi = {10.1093/mnras/stv2568},
  urldate = {2020-07-13},
  abstract = {The MiMeS (Magnetism in Massive Stars) project is a large-scale, high-resolution, sensitive spectropolarimetric investigation of the magnetic properties of O- and early B-type stars. Initiated in 2008 and completed in 2013, the project was supported by three Large Program allocations, as well as various programmes initiated by independent principal investigators, and archival resources. Ultimately, over 4800 circularly polarized spectra of 560 O and B stars were collected with the instruments ESPaDOnS (Echelle SpectroPolarimetric Device for the Observation of Stars) at the Canada-France-Hawaii Telescope, Narval at the T\'elescope Bernard Lyot and HARPSpol at the European Southern Observatory La Silla 3.6 m telescope, making MiMeS by far the largest systematic investigation of massive star magnetism ever undertaken. In this paper, the first in a series reporting the general results of the survey, we introduce the scientific motivation and goals, describe the sample of targets, review the instrumentation and observational techniques used, explain the exposure time calculation designed to provide sensitivity to surface dipole fields above approximately 100 G, discuss the polarimetric performance, stability and uncertainty of the instrumentation, and summarize the previous and forthcoming publications.},
  archiveprefix = {arxiv},
  keywords = {Instrumentation: polarimeters,notion,notion-database,Stars: early-type,Stars: magnetic field,Stars: massive,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/3GXXYD9C/full-text.pdf}
}

@article{Wade2018,
  title = {Magnetism of Hot Stars},
  author = {Wade, G. A. and Neiner, C.},
  year = {2018},
  journal = {Contributions of the Astronomical Observatory Skalnate Pleso},
  volume = {48},
  number = {1},
  eprint = {1712.09747},
  pages = {106--115},
  publisher = {{Astronomical Institute, Slovak Academy of Sciences}},
  issn = {13360337},
  urldate = {2020-04-30},
  abstract = {Strong, stable, and organised magnetic fields are present at the surfaces of a small fraction of OBA stars. These "fossil fields" exhibit uniform characteristics in stars over a tremendous range of stellar mass, age, temperature, and rotation rate. In hot O- and B-type stars, these magnetic fields couple efficiently to the stellar radiatively driven winds, strongly influencing stellar mass loss and rotation. In this article we review the characteristics of the known magnetic hot stars, discuss recent discoveries and insights, and describe recent theoretical progress toward understanding basic field properties and the influence of magnetic fields on hot star evolution.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Outflows,Stars: evolution,Stars: magnetic fields,Stars: rotation,Stars: winds}
}

@article{Waelkens1991,
  title = {Slowly {{Pulsating B}} Stars},
  author = {Waelkens, C.},
  year = {1991},
  journal = {Astronomy and Astrophysics},
  volume = {246},
  pages = {453--468},
  urldate = {2020-03-31},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/K5CUVPTK/full-text.pdf}
}

@article{Waldmann2012,
  title = {{{OF}} "Cocktail Parties" and Exoplanets},
  author = {Waldmann, I. P.},
  year = {2012},
  journal = {Astrophysical Journal},
  volume = {747},
  number = {1},
  eprint = {1106.1989},
  issn = {15384357},
  doi = {10.1088/0004-637X/747/1/12},
  abstract = {The characterization of ever smaller and fainter extrasolar planets requires an intricate understanding of one's data and the analysis techniques used. Correcting the raw data at the 10-4 level of accuracy in flux is one of the central challenges. This can be difficult for instruments that do not feature a calibration plan for such high precision measurements. Here, it is not always obvious how to de-correlate the data using auxiliary information of the instrument and it becomes paramount to know how well one can disentangle instrument systematics from one's data, given nothing but the data themselves. We propose a non-parametric machine learning algorithm, based on the concept of independent component analysis, to de-convolve the systematic noise and all non-Gaussian signals from the desired astrophysical signal. Such a "blind" signal de-mixing is commonly known as the "Cocktail Party problem" in signal processing. Given multiple simultaneous observations of the same exoplanetary eclipse, as in the case of spectrophotometry, we show that we can often disentangle systematic noise from the original light-curve signal without the use of any complementary information of the instrument. In this paper, we explore these signal extraction techniques using simulated data and two data sets observed with the Hubble Space Telescope NICMOS instrument. Another important application is the de-correlation of the exoplanetary signal from time-correlated stellar variability. Using data obtained by the Kepler mission we show that the desired signal can be de-convolved from the stellar noise using a single time series spanning several eclipse events. Such non-parametric techniques can provide important confirmations of the existent parametric corrections reported in the literature, and their associated results. Additionally they can substantially improve the precision exoplanetary light-curve analysis in the future. \textcopyright{} 2012 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {methods: data analysis,methods: statistical,notion,notion-database,techniques: photometric,techniques: spectroscopic},
  file = {/Users/lbugnet/Zotero/storage/EAEKKQZ9/Waldmann - 2012.pdf}
}

@article{Walker2007,
  title = {The {{Differential Rotation}} of {$\kappa$} 1 {{Ceti}} as {{Observed}} by {{MOST}}},
  author = {Walker, Gordon A. H. and Croll, Bryce and Kuschnig, Rainer and Walker, Andrew and Rucinski, Slavek M. and Matthews, Jaymie M. and Guenther, David B. and Moffat, Anthony F. J. and Sasselov, Dimitar and Weiss, Werner W.},
  year = {2007},
  journal = {The Astrophysical Journal},
  volume = {659},
  number = {2},
  eprint = {0704.2204},
  pages = {1611--1622},
  issn = {0004-637X},
  doi = {10.1086/511851},
  abstract = {We first reported evidence for differential rotation of {$\kappa$}1 Ceti in Paper I. In this paper we demonstrate that the differential rotation pattern closely matches that for the Sun. This result is based on additional MOST observations in 2004 and 2005, as well as those from 2003. Using StarSpotz, a program developed specifically to analyze MOST photometry, we have solved for k, the differential rotation coefficient, and Peq, the equatorial rotation period using the light curves from all three years. The absolute range in spot latitudes is 10\textdegree -75\textdegree{} and k=0.090+0.006-0.005, less than the solar value but consistent with the younger age of the star; k is also well constrained by the independent spectroscopic estimate of vsini. We demonstrate independently that the pattern of differential rotation with latitude is indeed solar. Details are given of the parallel tempering formalism used in finding the most robust solution, which gives Peq=8.77+0.03-0.04 days, smaller than that usually adopted, implying an age {$<$}750 My. Our values of Peq and k can explain the range of rotation periods others have found by spots or activity at a variety of latitudes. Historically, Ca II activity seems to occur consistently between latitudes 50\textdegree{} and 60\textdegree, which might indicate a permanent magnetic feature. Knowledge of k and Peq is key to understanding the dynamo mechanism and rotation structure in the convective zone, as well assessing age for solar-type stars. We recently published values of k and Peq for {$\varepsilon$} Eri based on MOST photometry and expect to analyze MOST light curves for several more spotted, solar-type stars. Based on data from the MOST satellite, a Canadian Space Agency mission, jointly operated by Dynacon, Inc., the University of Toronto Institute of Aerospace Studies, and the University of British Columbia with the assistance of the University of Vienna.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GBT35ING/Walker et al. - 2007.pdf}
}

@article{Walkowicz2011,
  title = {White-Light Flares on Cool Stars in the Kepler Quarter 1 Data},
  author = {Walkowicz, Lucianne M. and Basri, Gibor and Batalha, Natalie and Gilliland, Ronald L. and Jenkins, Jon and Borucki, William J. and Koch, David and Caldwell, Doug and Dupree, Andrea K. and Latham, David W. and Meibom, Soeren and Howell, Steve and Brown, Timothy M. and Bryson, Steve},
  year = {2011},
  journal = {Astronomical Journal},
  volume = {141},
  number = {2},
  eprint = {1008.0853},
  issn = {00046256},
  doi = {10.1088/0004-6256/141/2/50},
  abstract = {We present the results of a search for white-light flares on {$\sim$} 23,000 cool dwarfs in the Kepler Quarter 1 long cadence data. We have identified 373 flaring stars, some of which flare multiple times during the observation period. We calculate relative flare energies, flare rates, and durations and compare these with the quiescent photometric variability of our sample. We find that M dwarfs tend to flare more frequently but for shorter durations than K dwarfs and that they emit more energy relative to their quiescent luminosity in a given flare than K dwarfs. Stars that are more photometrically variable in quiescence tend to emit relatively more energy during flares, but variability is only weakly correlated with flare frequency. We estimate distances for our sample of flare stars and find that the flaring fraction agrees well with other observations of flare statistics for stars within 300 pc above the Galactic plane. These observations provide a more rounded view of stellar flares by sampling stars that have not been pre-selected by their activity, and are informative for understanding the influence of these flares on planetary habitability. \textcopyright{} 2011. The American Astronomical Society.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: Emission-line: Be,Stars: Flare,Stars: Low-mass},
  file = {/Users/lbugnet/Zotero/storage/BGMG3X76/Walkowicz et al. - 2011.pdf}
}

@article{Walkowicz2012,
  title = {The {{Information Content}} in {{Analytic Spot Models}} of {{Broadband Precision Lightcurves}}},
  author = {Walkowicz, Lucianne M. and Basri, Gibor S. and Valenti, Jeff A.},
  year = {2012},
  eprint = {1212.1672},
  doi = {10.1088/0067-0049/205/2/17},
  abstract = {We present the results of numerical experiments to assess degeneracies in lightcurve models of starspots. Using synthetic lightcurves generated with the Cheetah starspot modeling code, we explore the extent to which photometric light curves constrain spot model parameters, including spot latitudes and stellar inclination. We also investigate the effects of spot parameters and differential rotation on one's ability to correctly recover rotation periods and differential rotation in the Kepler lightcurves. We confirm that in the absence of additional constraints on the stellar inclination, such as spectroscopic measurements of vsini or occultations of starspots by planetary transits, the spot latitude and stellar inclination are difficult to determine uniquely from the photometry alone. We find that for models with no differential rotation, spots that appear on opposite hemispheres of the star may cause one to interpret the rotation period to be half of the true period. When differential rotation is included, the changing longitude separation between spots breaks the symmetry of the hemispheres and the correct rotation period is more likely to be found. The dominant period found via periodogram analysis is typically that of the largest spot. Even when multiple spots with periods representative of the star's differential rotation exist, if one spot dominates the lightcurve the signal of differential rotation may not be detectable from the periodogram alone. Starspot modeling is applicable to stars with a wider range of rotation rates than other surface imaging techniques (such as Doppler imaging), allows subtle signatures of differential rotation to be measured, and may provide valuable information on the distribution of stellar spots. However, given the inherent degeneracies and uncertainty present in starspot models, caution should be exercised in their interpretation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/AF92KLCA/Walkowicz, Basri, Valenti - 2012.pdf}
}

@article{Wang2016,
  title = {On Computation of {{Hough}} Functions},
  author = {Wang, Houjun and Boyd, John P. and Akmaev, Rashid A.},
  year = {2016},
  journal = {Geoscientific Model Development},
  volume = {9},
  number = {4},
  pages = {1477--1488},
  issn = {19919603},
  doi = {10.5194/gmd-9-1477-2016},
  abstract = {Hough functions are the eigenfunctions of the Laplace tidal equation governing fluid motion on a rotating sphere with a resting basic state. Several numerical methods have been used in the past. In this paper, we compare two of those methods: \emph{normalized} associated Legendre polynomial expansion and Chebyshev collocation. Both methods are not widely used, but both have some advantages over the commonly used unnormalized associated Legendre polynomial expansion method. Comparable results are obtained using both methods. For the first method we note some details on numerical implementation. The Chebyshev collocation method was first used for the Laplace tidal problem by Boyd (1976) and is relatively easy to use. A compact MATLAB code is provided for this method. We also illustrate the importance and effect of including a \emph{parity factor} in Chebyshev polynomial expansions for modes with \emph{odd} zonal wave numbers.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/222MNBCQ/Wang, Boyd, Akmaev - 2016.pdf}
}

@article{Wang2018,
  title = {Revisiting the Mass-Luminosity Relation with an Effective Temperature Modifier},
  author = {Wang, Jifei and Zhong, Zehao},
  year = {2018},
  journal = {A\&A},
  volume = {619},
  pages = {1},
  doi = {10.1051/0004-6361/201834109},
  urldate = {2020-07-12},
  abstract = {The mass-luminosity relation (MLR) is commonly used to estimate the stellar mass. The classical MLR can hardly fit data of all the stellar mass range, thus researchers have generally adopted piecewise MLRs based on the classical MLR with different exponents for different mass ranges. However, varying turning points for the piecewise MLRs and for the exponent of each segment were used, and the estimated stellar masses are not always as good as those obtained by dynamical methods. We suggest an alternative way to improve the mass estimation accuracy: adding an effective temperature modifier to modify every segment MLR. We use a corresponding estimating equation for G-and K-type main-sequence stars, and verify this equation on two eclipsing binary catalogs. We compare the estimated results with those from a classical MLR and several piecewise MLRs. We find that the new estimates are significantly more accurate than those from the classical MLR and some piecewise MLRs, and they are not inferior to the stellar masses from other piecewise MLRs. This indicates that the temperature modifier can effectively help improve the estimation accuracy. In addition, we discuss the effect of adding the temperature modifier on the practicability of estimating stellar masses.},
  keywords = {binaries,eclipsing-stars,fundamental parameters,notion,notion-database}
}

@article{Wang2019,
  title = {Two New {{R CMa-type}} Eclipsing Binaries Containing a Possible Low-Mass {{Helium}} White Dwarf Precursor: {{KIC}} 7368103 and {{KIC}} 8823397},
  shorttitle = {Two New {{R CMa-type}} Eclipsing Binaries Containing a Possible Low-Mass {{Helium}} White Dwarf Precursor},
  author = {Wang, Kun and Zhang, Xiaobin and Luo, Yangping and Luo, Changqing},
  year = {2019},
  month = jun,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {486},
  pages = {2462--2470},
  issn = {0035-8711},
  doi = {10.1093/mnras/stz1033},
  urldate = {2023-10-09},
  abstract = {We report the discovery of two new R CMa-type eclipsing binaries, each consisting of a possible low-mass Helium white dwarf precursor. Based on the Kepler long-cadence photometry and the radial-velocity measurements given by Matson et al., we determined comprehensive photometric solutions and physical parameters of two binaries KIC 7368103 and KIC 8823397. Light-curve modelling reveals that they are both short-period detached system with very low mass ratios q {$\simeq$} 0.1. The derived physical parameters show that the two binary systems consist of an extremely low-mass ({$\simeq$}0.2 M{$\odot$}), oversized ({$>$}1 R{$\odot$}), and overluminous secondary component, accompanied by a less-evolved early A-type primary star. We therefore introduce KIC 7368103 and KIC 8823397 as two new R CMa-type binaries, which are probably evolving into EL CVn stars. After subtracting the synthetic eclipsing curve from the de-trended Kepler data, we carried out a preliminary frequency analysis of their light-curve residuals. KIC 7368103 was found to pulsate in 35 independent frequencies in the range from 14 to 31 d-1, which could be due to the intrinsic pulsations of the {$\delta$} Sct-type primary star. However, no significant frequencies above the confidence level were detected in the binary KIC 8823397.},
  keywords = {KIC 8823397),stars: binaries: eclipsing,stars: individual (KIC 7368103,stars: variables: delta Scuti},
  annotation = {ADS Bibcode: 2019MNRAS.486.2462W},
  file = {/Users/lbugnet/Zotero/storage/5Q2BPSZ3/Wang et al. - 2019 - Two new R CMa-type eclipsing binaries containing a.pdf}
}

@article{Wang2020,
  title = {Discovery of {{Two Pulsating Extremely Low-mass Pre-white Dwarf Candidates}} in the {{TESS Eclipsing Binaries}}},
  author = {Wang, Kun and Zhang, Xiaobin and Dai, Min},
  year = {2020},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {888},
  pages = {49},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ab584c},
  urldate = {2023-10-02},
  abstract = {We report the discovery of two new pulsating extremely low-mass pre-white dwarf (pre-ELMV) candidates in the Transiting Exoplanet Survey Satellite (TESS) eclipsing binaries, TIC 149160359 and TIC 416264037. Their light curves show a typical feature of EL CVn-type binaries. The light-curve modeling indicates that they are both detached systems with very low-mass ratios (q {$\simeq$} 0.1). Based on the photometric solutions, the masses and radii of the two main-sequence primary components are estimated, and those of the secondaries are deduced. The results show that the less-massive components of the two binaries are both probably thermally bloated, pre-ELMVs. Apart from the eclipsing light changes, short-period light variations are clearly shown in their residual light curves. We have made the Fourier analysis of their light-curve residuals with the Period04 program. TIC 149160359 was found to pulsate in 21 independent frequencies, 17 of which are between 21 and 35 day-1 and the others are between 63 and 77 day-1. The Fourier amplitude spectrum of TIC 416264037 also shows two frequency concentration ranges. Out of nine independent frequencies, seven reside within the low-frequency range of 12.5-19.9 day-1. Two pulsating signals, f 4 = 122.2698 day-1 and f 10 = 112.3603 day-1, were detected in the high-frequency region. These low-frequency signals that are detected on TIC 149160359 and TIC 416264037 are probably due to the intrinsic pulsations of their {$\delta$} Sct-type primary components. However, the high-frequency signals are likely to come from the pulsations of the pre-ELM WD components. This brings the number of pre-ELMV candidates to 12.},
  keywords = {1799,370,444,Delta Scuti variable stars,Eclipsing binary stars,White dwarf stars},
  annotation = {ADS Bibcode: 2020ApJ...888...49W}
}

@article{Wang2020a,
  title = {Discovery of {{Two Pulsating Extremely Low-mass Pre-white Dwarf Candidates}} in the {{TESS Eclipsing Binaries}}},
  author = {Wang, Kun and Zhang, Xiaobin and Dai, Min},
  year = {2020},
  month = jan,
  journal = {The Astrophysical Journal},
  volume = {888},
  pages = {49},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ab584c},
  urldate = {2023-10-09},
  abstract = {We report the discovery of two new pulsating extremely low-mass pre-white dwarf (pre-ELMV) candidates in the Transiting Exoplanet Survey Satellite (TESS) eclipsing binaries, TIC 149160359 and TIC 416264037. Their light curves show a typical feature of EL CVn-type binaries. The light-curve modeling indicates that they are both detached systems with very low-mass ratios (q {$\simeq$} 0.1). Based on the photometric solutions, the masses and radii of the two main-sequence primary components are estimated, and those of the secondaries are deduced. The results show that the less-massive components of the two binaries are both probably thermally bloated, pre-ELMVs. Apart from the eclipsing light changes, short-period light variations are clearly shown in their residual light curves. We have made the Fourier analysis of their light-curve residuals with the Period04 program. TIC 149160359 was found to pulsate in 21 independent frequencies, 17 of which are between 21 and 35 day-1 and the others are between 63 and 77 day-1. The Fourier amplitude spectrum of TIC 416264037 also shows two frequency concentration ranges. Out of nine independent frequencies, seven reside within the low-frequency range of 12.5-19.9 day-1. Two pulsating signals, f 4 = 122.2698 day-1 and f 10 = 112.3603 day-1, were detected in the high-frequency region. These low-frequency signals that are detected on TIC 149160359 and TIC 416264037 are probably due to the intrinsic pulsations of their {$\delta$} Sct-type primary components. However, the high-frequency signals are likely to come from the pulsations of the pre-ELM WD components. This brings the number of pre-ELMV candidates to 12.},
  keywords = {1799,370,444,Delta Scuti variable stars,Eclipsing binary stars,White dwarf stars},
  annotation = {ADS Bibcode: 2020ApJ...888...49W}
}

@article{Wang2022,
  title = {Extremely {{Low-mass White Dwarf Stars Observed}} in {{Gaia DR2}} and {{LAMOST DR8}}},
  author = {Wang, Kun and N{\'e}meth, P{\'e}ter and Luo, Yangping and Chen, Xiaodian and Jiang, Qingquan and Cao, Xingmei},
  year = {2022},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {936},
  pages = {5},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac847c},
  urldate = {2023-10-14},
  abstract = {We present the first results from our ongoing project to study extremely low-mass (ELM) white dwarfs (WDs) (M {$\leq$} 0.3M {$\odot$}) with the Large Sky Area Multi-Object Fiber Spectroscopic Telescope (LAMOST) spectra. Based on the LAMOST DR8 spectral database, we analyzed 136 ELM WD candidates selected from Gaia DR2 data and 12 known objects previously identified by the ELM Survey. The atmospheric parameters and radial velocities of these stars were obtained by fitting the LAMOST low-resolution spectra. After comparing the atmospheric parameters of the 12 known objects from this work to the results reported by the ELM Survey, we demonstrated the potential of LAMOST spectra in probing into the nature of ELM WDs. Based on the atmospheric parameters and Gaia EDR3 data, we identified 21 new high-probability ELM WDs with masses M {$\leq$} 0.3M {$\odot$} and parallax estimates that agree to within a factor of 3. Two of them, J0338+4134 and J1129+4715, show significant radial velocity variability and are very likely to be binary systems containing at least one ELM WD.},
  keywords = {1799,288,Astrophysics - Solar and Stellar Astrophysics,Compact objects,White dwarf stars},
  annotation = {ADS Bibcode: 2022ApJ...936....5W},
  file = {/Users/lbugnet/Zotero/storage/7WZPL5BG/Wang et al. - 2022 - Extremely Low-mass White Dwarf Stars Observed in G.pdf}
}

@article{Wang2022a,
  title = {Extremely {{Low-mass White Dwarf Stars Observed}} in {{Gaia DR2}} and {{LAMOST DR8}}},
  author = {Wang, Kun and N{\'e}meth, P{\'e}ter and Luo, Yangping and Chen, Xiaodian and Jiang, Qingquan and Cao, Xingmei},
  year = {2022},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {936},
  pages = {5},
  issn = {0004-637X},
  doi = {10.3847/1538-4357/ac847c},
  urldate = {2023-10-14},
  abstract = {We present the first results from our ongoing project to study extremely low-mass (ELM) white dwarfs (WDs) (M {$\leq$} 0.3M {$\odot$}) with the Large Sky Area Multi-Object Fiber Spectroscopic Telescope (LAMOST) spectra. Based on the LAMOST DR8 spectral database, we analyzed 136 ELM WD candidates selected from Gaia DR2 data and 12 known objects previously identified by the ELM Survey. The atmospheric parameters and radial velocities of these stars were obtained by fitting the LAMOST low-resolution spectra. After comparing the atmospheric parameters of the 12 known objects from this work to the results reported by the ELM Survey, we demonstrated the potential of LAMOST spectra in probing into the nature of ELM WDs. Based on the atmospheric parameters and Gaia EDR3 data, we identified 21 new high-probability ELM WDs with masses M {$\leq$} 0.3M {$\odot$} and parallax estimates that agree to within a factor of 3. Two of them, J0338+4134 and J1129+4715, show significant radial velocity variability and are very likely to be binary systems containing at least one ELM WD.},
  keywords = {1799,288,Astrophysics - Solar and Stellar Astrophysics,Compact objects,White dwarf stars},
  annotation = {ADS Bibcode: 2022ApJ...936....5W}
}

@article{Watters2019,
  title = {Shallow Seismic Activity and Young Thrust Faults on the {{Moon}}},
  author = {Watters, Thomas R. and Weber, Renee C. and Collins, Geoffrey C. and Howley, Ian J. and Schmerr, Nicholas C. and Johnson, Catherine L.},
  year = {2019},
  month = jun,
  journal = {Nature Geoscience},
  volume = {12},
  number = {6},
  pages = {411--417},
  publisher = {{Nature Publishing Group}},
  issn = {17520908},
  doi = {10.1038/s41561-019-0362-2},
  urldate = {2020-02-28},
  abstract = {The discovery of young thrust faults on the Moon is evidence of recent tectonic activity, but how recent is unknown. Seismometers at four Apollo landing sites recorded 28 shallow moonquakes between 1969 and 1977. Some of these shallow quakes could be associated with activity on the young faults. However, the epicentre locations of these quakes are poorly constrained. Here we present more-accurate estimates of the epicentre locations, based on an algorithm for sparse seismic networks. We found that the epicentres of eight near-surface quakes fall within 30 km of a fault scarp, the distance of the expected strong ground shaking. From an analysis of the timing of these eight events, we found that six occurred when the Moon was less than 15,000 km from the apogee distance. Analytical modelling of tidal forces that contribute to the current lunar stress state indicates that seven near-apogee events within 60 km of a fault scarp occur at or near the time of peak compressional stresses, when fault slip events are most likely. We conclude that the proximity of moonquakes to the young thrust faults together with evidence of regolith disturbance and boulder movements on and near the fault scarps strongly suggest the Moon is tectonically active.},
  keywords = {notion,notion-database,Planetary science,Seismology,Tectonics},
  file = {/Users/lbugnet/Zotero/storage/I675FJ3C/full-text.pdf}
}

@article{Weber1967,
  title = {The {{Angular Momentum}} of the {{Solar Wind}}},
  author = {Weber, Edmund J. and Davis, Jr., Leverett},
  year = {1967},
  month = apr,
  journal = {The Astrophysical Journal},
  volume = {148},
  pages = {217},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/149138},
  urldate = {2020-07-02},
  abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein-protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-{$\alpha$}-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD {$\leq$} 2.0 \AA{} for the interface backbone atoms) increased from 21\% with default Glide SP settings to 58\% with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63\% success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40\% of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
  keywords = {notion,notion-database}
}

@article{Wei2015,
  title = {On Obliquely Magnetized and Differentially Rotating Stars},
  author = {Wei, Xing and Goodman, Jeremy},
  year = {2015},
  month = jan,
  journal = {ApJ},
  volume = {806},
  number = {1},
  eprint = {1501.04211},
  pages = {50},
  doi = {10.1088/0004-637X/806/1/50},
  urldate = {2020-07-13},
  abstract = {We investigate the interaction of differential rotation and a misaligned magnetic field. The incompressible magnetohydrodynamic equations are solved numerically for a free-decay problem. In the kinematic limit, differential rotation annihilates the non-axisymmetric field on a timescale proportional to the cube root of magnetic Reynolds number (\$Rm\$), as predicted by R\textbackslash "adler. Nonlinearly, the outcome depends upon the initial energy in the non-axisymmetric part of the field. Sufficiently weak fields approach axisymmetry as in the kinematic limit; some differential rotation survives across magnetic surfaces, at least on intermediate timescales. Stronger fields enforce uniform rotation and remain non-axisymmetric. The initial field strength that divides these two regimes does not follow the scaling \$Rm\^\{-1/3\}\$ predicted by quasi-kinematic arguments, perhaps because our \$Rm\$ is never sufficiently large or because of reconnection. We discuss the possible relevance of these results to tidal synchronization and tidal heating of close binary stars, particularly double white dwarfs.},
  archiveprefix = {arxiv},
  keywords = {magnetohydrodynamics (MHD),notion,notion-database,stars: rotation,white dwarfs},
  file = {/Users/lbugnet/Zotero/storage/3KYFJD2E/full-text.pdf}
}

@article{Wei2018,
  title = {The {{Magnetic Effect}} on {{Dynamical Tide}} in {{Rapidly Rotating Astronomical Objects}}},
  author = {Wei, Xing},
  year = {2018},
  journal = {The Astrophysical Journal},
  volume = {854},
  number = {1},
  pages = {34},
  doi = {10.3847/1538-4357/aaa54d},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/P6E4FBJC/document.pdf}
}

@article{Weiss2013a,
  title = {{{BRITE-Constellation}} : {{Nanosatellites}} for Precision Photometry of Bright Stars},
  author = {Weiss, W. W. and Moffat, A. F. J. and {Schwarzenberg-Czerny}, A. and Koudelka, O. F. and Grant, C. C. and Zee, R. E. and Kuschnig, R. and Mochnacki, {\relax St}. and Rucinski, S. M. and Matthews, J. M. and Orlea{\'n}ski, P. and Pamyatnykh, A. A. and Pigulski, A. and Alves, J. and Guedel, M. and Handler, G. and Wade, G. A. and Scholtz, A. L.},
  year = {2013},
  journal = {Proceedings of the International Astronomical Union},
  volume = {9},
  number = {S301},
  eprint = {1309.5531},
  pages = {67--68},
  issn = {1743-9213},
  doi = {10.1017/s1743921313014105},
  abstract = {BRITE-Constellation (where BRITE stands for BRI ght T arget E xplorer) is an international nanosatellite mission to monitor photometrically, in two colours, brightness and temperature variations of stars brighter than V {$\approx$} 4, with precision and time coverage not possible from the ground. The current mission design consists of three pairs of 7 kg nanosats (hence ``Constellation'') from Austria, Canada and Poland carrying optical telescopes (3 cm aperture) and CCDs. One instrument in each pair is equipped with a blue filter; the other, a red filter. The first two nanosats (funded by Austria) are UniBRITE , designed and built by UTIAS-SFL (University of Toronto Institute for Aerospace Studies-Space Flight Laboratory) and its twin, BRITE-Austria , built by the Technical University Graz (TUG) with support of UTIAS-SFL. They were launched on 25 February 2013 by the Indian Space Agency, under contract to the Canadian Space Agency.  Each BRITE instrument has a wide field of view ({$\approx$} 24 degrees), so up to 15 bright stars can be observed simultaneously in 32 \texttimes{} 32 sub-rasters. Photometry (with reduced precision but thorough time sampling) of additional fainter targets will be possible through on-board data processing. A critical technical element of the BRITE mission is the three-axis attitude control system to stabilize a nanosat with very low inertia. The pointing stability is better than 1.5 arcminutes rms, a significant advance by UTIAS-SFL over any previous nanosatellite.  BRITE-Constellation will primarily measure p- and g-mode pulsations to probe the interiors and ages of stars through asteroseismology. The BRITE sample of many of the brightest stars in the night sky is dominated by the most intrinsically luminous stars: massive stars seen at all evolutionary stages, and evolved medium-mass stars at the very end of their nuclear burning phases (cool giants and AGB stars). The Hertzsprung-Russell diagram for stars brighter than mag V =4 from which the BRITE-Constellation sample will be selected is shown in Fig. 1. This sample falls into two principal classes of stars: (1) Hot luminous H-burning stars (O to F stars). Analyses of OB star variability have the potential to help solve two outstanding problems: the sizes of convective (mixed) cores in massive stars and the influence of rapid rotation on their structure and evolution.(2) Cool luminous stars (AGB stars, cool giants and cool supergiants). Measurements of the time scales involved in surface granulation and differential rotation will constrain turbulent convection models.Mass loss from these stars (especially the massive supernova progenitors) is a major contributor to the evolution of the interstellar medium, so in a sense, this sample dominates cosmic ``ecology'' in terms of future generations of star formation. The massive stars are believed to share many characteristics of the lower mass range of the first generation of stars ever formed (although the original examples are of course long gone). BRITE observations will also be used to detect some Jupiter- and even Neptune-sized planets around bright host stars via transits, as expected on the basis of statistics from the Kepler exoplanet mission. Detecting planets around such very bright stars will greatly facilitate their subsequent characterization. BRITE will also use surface spots to investigate stellar rotation.  The following Table summarizes launch and orbit parameters of BRITE-Constellation components.  The full version of this paper describing in more detail BRITE-Constellation will be published separately in a journal. The symposium presentation is available at http://iaus301.astro.uni.wroc.pl/program.php},
  archiveprefix = {arxiv},
  isbn = {0000000000000},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/K973W8QT/Weiss et al. - 2013.pdf}
}

@article{Welsh2011a,
  title = {{{KOI-54}}: {{The Kepler}} Discovery of Tidally Excited Pulsations and Brightenings in a Highly Eccentric Binary},
  author = {Welsh, William F. and Orosz, Jerome A. and Aerts, Conny and Brown, Timothy M. and Brugamyer, Erik and Cochran, William D. and Gilliland, Ronald L. and Guzik, Joyce Ann and Kurtz, D. W. and Latham, David W. and Marcy, Geoffrey W. and Quinn, Samuel N. and Zima, Wolfgang and Allen, Christopher and Batalha, Natalie M. and Bryson, Steve and Buchhave, Lars A. and Caldwell, Douglas A. and Gautier, Thomas N. and Howell, Steve B. and Kinemuchi, K. and Ibrahim, Khadeejah A. and Isaacson, Howard and Jenkins, Jon M. and Prsa, Andrej and Still, Martin and Street, Rachel and Wohler, Bill and Koch, David G. and Borucki, William J.},
  year = {2011},
  journal = {Astrophysical Journal, Supplement Series},
  volume = {197},
  number = {1},
  eprint = {1102.1730},
  issn = {00670049},
  doi = {10.1088/0067-0049/197/1/4},
  abstract = {Kepler observations of the star HD 187091 (KIC 8112039, hereafter KOI-54) revealed a remarkable light curve exhibiting sharp periodic brightening events every 41.8 days with a superimposed set of oscillations forming a beating pattern in phase with the brightenings. Spectroscopic observations revealed that this is a binary star with a highly eccentric orbit, e = 0.83. We are able to match the Kepler light curve and radial velocities with a nearly face-on (i = 55) binary star model in which the brightening events are caused by tidal distortion and irradiation of nearly identical A stars during their close periastron passage. The two dominant oscillations in the light curve, responsible for the beating pattern, have frequencies that are the 91st and 90th harmonic of the orbital frequency. The power spectrum of the light curve, after removing the binary star brightening component, reveals a large number of pulsations, 30 of which have a signal-to-noise ratio {$\greaterequivlnt$}7. Nearly all of these pulsations have frequencies that are either integer multiples of the orbital frequency or are tidally split multiples of the orbital frequency. This pattern of frequencies unambiguously establishes the pulsations as resonances between the dynamic tides at periastron and the free oscillation modes of one or both of the stars. KOI-54 is only the fourth star to show such a phenomenon and is by far the richest in terms of excited modes. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {binaries: close,binaries: spectroscopic,notion,notion-database,{stars: individual (KID 8112039, HD 187091, 2MASS J},stars: oscillations,stars: variables: general},
  file = {/Users/lbugnet/Zotero/storage/8C7T7HFB/Welsh et al. - 2011.pdf}
}

@article{Wheeler2015,
  title = {The Role of the Magnetorotational Instability in Massive Stars},
  author = {Wheeler, J. Craig and Kagan, Daniel and Chatzopoulos, Emmanouil},
  year = {2015},
  journal = {Astrophysical Journal},
  volume = {799},
  number = {1},
  eprint = {1411.5714},
  issn = {15384357},
  doi = {10.1088/0004-637X/799/1/85},
  abstract = {The magnetorotational instability (MRI) is key to physics in accretion disks and is widely considered to play some role in massive star core collapse. Models of rotating massive stars naturally develop very strong shear at composition boundaries, a necessary condition for MRI instability, and the MRI is subject to triply diffusive destabilizing effects in radiative regions. We have used the MESA stellar evolution code to compute magnetic effects due to the Spruit-Tayler (ST) mechanism and the MRI, separately and together, in a sample of massive star models. We find that the MRI can be active in the later stages of massive star evolution, leading to mixing effects that are not captured in models that neglect the MRI. The MRI and related magnetorotational effects can move models of given zero-age main sequence mass across "boundaries" from degenerate CO cores to degenerate O/Ne/Mg cores and from degenerate O/Ne/Mg cores to iron cores, thus affecting the final evolution and the physics of core collapse. The MRI acting alone can slow the rotation of the inner core in general agreement with the observed "initial" rotation rates of pulsars. The MRI analysis suggests that localized fields {$\sim$}1012 G may exist at the boundary of the iron core. With both the ST and MRI mechanisms active in the 20 M{$\odot$} model, we find that the helium shell mixes entirely out into the envelope. Enhanced mixing could yield a population of yellow or even blue supergiant supernova progenitors that would not be standard SN IIP.},
  archiveprefix = {arxiv},
  keywords = {Instabilities,Magnetohydrodynamics (MHD),notion,notion-database,Stars: Magnetic fields,Stars: Neutron,Stars: Rotation,Supernovae: General},
  file = {/Users/lbugnet/Zotero/storage/EG3787FR/Wheeler, Kagan, Chatzopoulos - 2015.pdf}
}

@article{White2011,
  title = {Calculating Asteroseismic Diagrams for Solar-like Oscillations},
  author = {White, Timothy R. and Bedding, Timothy R. and Stello, Dennis and {Christensen-Dalsgaard}, J{\o}rgen and Huber, Daniel and Kjeldsen, Hans},
  year = {2011},
  journal = {Astrophysical Journal},
  volume = {743},
  number = {2},
  eprint = {1109.3455},
  issn = {15384357},
  doi = {10.1088/0004-637X/743/2/161},
  abstract = {With the success of the Kepler and CoRoT missions, the number of stars with detected solar-like oscillations has increased by several orders of magnitude; for the first time we are able to perform large-scale ensemble asteroseismology of these stars. In preparation for this golden age of asteroseismology we have computed expected values of various asteroseismic observables from models of varying mass and metallicity. The relationships between these asteroseismic observables, such as the separations between mode frequencies, are able to significantly constrain estimates of the ages and masses of these stars. We investigate the scaling relation between the large frequency separation, {$\Delta\nu$}, and mean stellar density. Furthermore we present model evolutionary tracks for several asteroseismic diagrams. We have extended the so-called C-D diagram beyond the main sequence to the subgiants and the red giant branch. We also consider another asteroseismic diagram, the {$\epsilon$} diagram, which is more sensitive to variations in stellar properties at the subgiant stages and can aid in determining the correct mode identification. The recent discovery of gravity-mode period spacings in red giants forms the basis for a third asteroseismic diagram. We compare the evolutionary model tracks in these asteroseismic diagrams with results from pre-Kepler studies of solar-like oscillations and early results from Kepler. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: fundamental parameters,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/9UKESN9L/White et al. - 2011.pdf}
}

@article{White2011a,
  title = {Asteroseismic Diagrams from a Survey of Solar-like Oscillations with {{Kepler}}},
  author = {White, Timothy R. and Bedding, Timothy R. and Stello, Dennis and Appourchaux, Thierry and Ballot, J{\'e}rme and Benomar, Othman and Bonanno, Alfio and Broomhall, Anne Marie and Campante, Tiago L. and Chaplin, William J. and {Christensen-Dalsgaard}, J{\o}rgen and Corsaro, Enrico and Do{\v g}an, G{\"u}lnur and Elsworth, Yvonne P. and Fletcher, Stephen T. and Garc{\'i}a, Rafael A. and Gaulme, Patrick and Handberg, Rasmus and Hekker, Saskia and Huber, Daniel and Karoff, Christoffer and Kjeldsen, Hans and Mathur, Savita and Mosser, Benoit and Monteiro, Mario J.P.F.G. and R{\'e}gulo, Clara and Salabert, David and Silva Aguirre, Victor and Thompson, Michael J. and Verner, Graham and Morris, Robert L. and Sanderfer, Dwight T. and Seader, Shawn E.},
  year = {2011},
  journal = {Astrophysical Journal Letters},
  volume = {742},
  number = {1},
  eprint = {1110.1375},
  pages = {0--5},
  issn = {20418205},
  doi = {10.1088/2041-8205/742/1/L3},
  abstract = {Photometric observations made by the NASA Kepler Mission have led to a dramatic increase in the number of main-sequence and subgiant stars with detected solar-like oscillations. We present an ensemble asteroseismic analysis of 76 solar-type stars. Using frequencies determined from the Kepler time-series photometry, we have measured three asteroseismic parameters that characterize the oscillations: the large frequency separation ({$\Delta\nu$}), the small frequency separation between modes of l = 0 and l = 2 ({$\delta\nu$}02) , and the dimensionless offset ({$\epsilon$}). These measurements allow us to construct asteroseismic diagrams, namely the so-called Christensen-Dalsgaard diagram of {$\delta\nu$}02 versus{$\Delta\nu$}, and the recently re-introduced {$\epsilon$} diagram. We compare the Kepler results with previously observed solar-type stars and with theoretical models. The positions of stars in these diagrams places constraints on their masses and ages. Additionally, we confirm the observational relationship between {$\epsilon$} and T eff that allows for the unambiguous determination of radial order and should help resolve the problem of mode identification in F stars. \textcopyright{} 2011. The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/T94PM7TD/White et al. - 2011(2).pdf}
}

@article{White2012,
  title = {Solving the Mode Identification Problem in Asteroseismology of {{F}} Stars Observed with {{Kepler}}},
  author = {White, Timothy R. and Bedding, Timothy R. and Gruberbauer, Michael and Benomar, Othman and Stello, Dennis and Appourchaux, Thierry and Chaplin, William J. and {Christensen-Dalsgaard}, Jorgen and Elsworth, Yvonne P. and Garc{\'i}a, Rafael A. and Hekker, Saskia and Huber, Daniel and Kjeldsen, Hans and Mosser, Beno{\^i}t and Kinemuchi, Karen and Mullally, Fergal and Still, Martin},
  year = {2012},
  journal = {Astrophysical Journal Letters},
  volume = {751},
  number = {2},
  eprint = {1205.0544},
  pages = {1--7},
  issn = {20418205},
  doi = {10.1088/2041-8205/751/2/L36},
  abstract = {Asteroseismology of F-type stars has been hindered by an ambiguity in identification of their oscillation modes. The regular mode pattern that makes this task trivial in cooler stars is masked by increased line widths. The absolute mode frequencies, encapsulated in the asteroseismic variable {$\epsilon$}, can help solve this impasse because the values of {$\epsilon$} implied by the two possible mode identifications are distinct. We find that the correct {$\epsilon$} can be deduced from the effective temperature and the line widths and we apply these methods to a sample of solar-like oscillators observed with Kepler. \textcopyright{} 2012. The American Astronomical Society. All rights reserved..},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: fundamental parameters,stars: interiors,stars: oscillations},
  file = {/Users/lbugnet/Zotero/storage/52GMLBV2/White et al. - 2012.pdf}
}

@article{White2013,
  title = {Interferometric Radii of Bright {{Kepler}} Stars with the {{CHARA Array}}: \texttheta{} {{Cygni}} and 16 {{Cygni A}} and {{B}}},
  author = {White, T. R. and Huber, D. and Maestro, V. and Bedding, T. R. and Ireland, M. J. and Baron, F. and Boyajian, T. S. and Che, X. and Monnier, J. D. and Pope, B. J.S. and Roettenbacher, R. M. and Stello, D. and Tuthill, P. G. and Farrington, C. D. and Goldfinger, P. J. and McAlister, H. A. and Schaefer, G. H. and Sturmann, J. and Sturmann, L. and {ten Brummelaar}, T. A. and Turner, N. H.},
  year = {2013},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {433},
  number = {2},
  pages = {1262--1270},
  issn = {00358711},
  doi = {10.1093/mnras/stt802},
  abstract = {We present the results of long-baseline optical interferometry observations using the Precision Astronomical Visual Observations (PAVO) beam combiner at the Center for High Angular Resolution Astronomy (CHARA) Array to measure the angular sizes of three bright Kepler stars: \texttheta{} Cygni, and both components of the binary system 16 Cygni. Supporting infrared observations were made with the Michigan Infrared Combiner (MIRC) and Classic beam combiner, also at the CHARA Array. We find limb-darkened angular diameters of 0.753 {$\pm$} 0.009 mas for \texttheta{} Cyg, 0.539 {$\pm$} 0.007 mas for 16 Cyg A and 0.490 {$\pm$} 0.006 mas for 16 Cyg B. The Kepler Mission has observed these stars with outstanding photometric precision, revealing the presence of solar-like oscillations. Due to the brightness of these stars the oscillations have exceptional signal-to-noise, allowing for detailed study through asteroseismology, and are well constrained by other observations. We have combined our interferometric diameters with Hipparcos parallaxes, spectrophotometric bolometric fluxes and the asteroseismic large frequency separation to measure linear radii (\texttheta{} Cyg: 1.48 {$\pm$} 0.02 R, 16 Cyg A: 1.22 {$\pm$} 0.02 R, 16 Cyg B: 1.12 {$\pm$} 0.02 R), effective temperatures (\texttheta{} Cyg: 6749 {$\pm$} 44 K, 16 Cyg A: 5839 {$\pm$} 42 K, 16 Cyg B: 5809 {$\pm$} 39 K) and masses (\texttheta{} Cyg: 1.37 {$\pm$} 0.04 M, 16 Cyg A: 1.07 {$\pm$} 0.05M, 16 Cyg B: 1.05 {$\pm$} 0.04M) for each star with very little model dependence. The measurements presented here will provide strong constraints for future stellar modelling efforts. \textcopyright{} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
  keywords = {notion,notion-database,Stars: individual: 16 Cygni A,Stars: individual: 16 Cygni B,Stars: individual: \texttheta Cygni,Stars: oscillations,Techniques: interferometric},
  file = {/Users/lbugnet/Zotero/storage/3VCM238S/White et al. - 2013.pdf}
}

@article{White2015,
  title = {Testing {{Asteroseismic Scaling Relations}} with {{Interferometry}}},
  author = {White, T. R. and Aguirre, V. Silva and Boyajian, T. and Creevey, O. and Huber, D. and Von Braun, K. and Bedding, T. R. and Elsworth, Y. and Hekker, S. and Stello, D. and Weiss, A.},
  year = {2015},
  journal = {EPJ Web of Conferences},
  volume = {101},
  pages = {8--9},
  issn = {2100014X},
  doi = {10.1051/epjconf/201510106068},
  abstract = {The asteroseismic scaling relations for the frequency of maximum oscillation power, v max , and the large frequency separation, {$\Delta\nu$}, provide an easy way to directly determine the masses and radii of stars with detected solar-like oscillations. With the vast amount of data available from the CoRoT and Kepler missions, the convenience of the scaling relations has resulted in their wide-spread use. But how valid are the scaling relations when applied to red giants, which have a substantially different structure than the Sun? Verifying the scaling relations empirically requires independent measurements. We report on the current state and future prospects of interferometric tests of the scaling relations.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/VH4626PK/White et al. - 2015.pdf}
}

@article{White2017,
  title = {Kepler Observations of the Asteroseismic Binary {{HD}} 176465},
  author = {White, T. R. and Benomar, O. and Silva Aguirre, V. and Ball, W. H. and Bedding, T. R. and Chaplin, W. J. and {Christensen-Dalsgaard}, J. and Garcia, R. A. and Gizon, L. and Stello, D. and Aigrain, S. and Antia, H. M. and Appourchaux, T. and Bazot, M. and Campante, T. L. and Creevey, O. L. and Davies, G. R. and Elsworth, Y. P. and Gaulme, P. and Handberg, R. and Hekker, S. and Houdek, G. and Howe, R. and Huber, D. and Karoff, C. and Marques, J. P. and Mathur, S. and McQuillan, A. and Metcalfe, T. S. and Mosser, B. and Nielsen, M. B. and R{\'e}gulo, C. and Salabert, D. and Stahn, T.},
  year = {2017},
  journal = {Astronomy and Astrophysics},
  volume = {601},
  eprint = {1609.09581},
  issn = {14320746},
  doi = {10.1051/0004-6361/201628706},
  abstract = {Binary star systems are important for understanding stellar structure and evolution, and are especially useful when oscillations can be detected and analysed with asteroseismology. However, only four systems are known in which solar-like oscillations are detected in both components. Here, we analyse the fifth such system, HD 176465, which was observed by Kepler. We carefully analysed the system's power spectrum to measure individual mode frequencies, adapting our methods where necessary to accommodate the fact that both stars oscillate in a similar frequency range. We also modelled the two stars independently by fitting stellar models to the frequencies and complementaryparameters. We are able to cleanly separate the oscillation modes in both systems. The stellar models produce compatible ages and initial compositions for the stars, as is expected from their common and contemporaneous origin. Combining the individual ages, the system is about 3.0 {$\pm$} 0.5 Gyr old. The two components of HD 176465 are young physically-similar oscillating solar analogues, the first such system to be found, and provide important constraints for stellar evolution and asteroseismology.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Widrow2002a,
  title = {Origin of Galactic and Extragalactic Magnetic Fields},
  author = {Widrow, Lawrence M.},
  year = {2002},
  journal = {Reviews of Modern Physics},
  volume = {74},
  number = {3},
  eprint = {astro-ph/0207240},
  pages = {775--823},
  issn = {00346861},
  doi = {10.1103/RevModPhys.74.775},
  abstract = {A variety of observations suggest that magnetic fields are present in all galaxies and galaxy clusters. These fields are characterized by a modest strength (10-7 - 10-5 G) and huge spatial scale ({$\lessequivlnt$} 1 Mpc). It is generally assumed that magnetic fields in spiral galaxies arise from the combined action of differential rotation and helical turbulence, a process known as the {$\alpha\omega$} dynamo. However, fundamental questions concerning the nature of the dynamo as well as the origin of the seed fields necessary to prime it remain unclear. Moreover, the standard {$\alpha\omega$} dynamo does not explain the existence of magnetic fields in elliptical galaxies and clusters. The author summarizes what is known observationally about magnetic fields in galaxies, clusters, superclusters, and beyond. He then reviews the standard dynamo paradigm, the challenges that have been leveled against it, and several alternative scenarios. He concludes with a discussion of astrophysical and early-Universe candidates for seed fields.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/ATYS5DUW/Widrow - 2002.pdf}
}

@article{Wieczorek2006,
  title = {The Constitution and Structure of the {{Lunar}} Interior},
  author = {Wieczorek, Mark A. and Jolliff, Bradley L. and Khan, Amir and Pritchard, Matthew E. and Weiss, Benjamin P. and Williams, James G. and Hood, Lon L. and Righter, Kevin and Neal, Clive R. and Shearer, Charles K. and McCallum, I. Stewart and Tompkins, Stephanie and Hawke, B. Ray and Peterson, Chris and Gillis, Jeffrey J. and Bussey, Ben},
  year = {2006},
  journal = {Reviews in Mineralogy and Geochemistry},
  volume = {60},
  pages = {221--364},
  issn = {15296466},
  doi = {10.2138/rmg.2006.60.3},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/JWD3PX2X/The_Constitution_and_Structure_of_the_Lunar_Interi.pdf}
}

@incollection{Wigner,
  title = {Chapter 9: 6j {{SYMBOLS AND THE}} |{{IACAH COEFFICIENTS}} 9.1.},
  booktitle = {Quantum {{Theory}} of {{Angular Momentum}}},
  number = {4},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/NTWXWWXV/Unknown - Unknown(11).pdf}
}

@article{WILCOX1981a,
  title = {Stellar {{Oscillations}}},
  author = {WILCOX, J. M.},
  year = {1981},
  journal = {Science},
  volume = {211},
  number = {4488},
  pages = {1341--1342},
  issn = {0036-8075},
  doi = {10.1126/science.211.4488.1341-a},
  abstract = {Lecture notes},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5WLUK56F/WILCOX - 1981.pdf}
}

@article{Willson1984,
  title = {Measurements of Solar Total Irradiance and Its Variability},
  author = {Willson, Richard C.},
  year = {1984},
  journal = {Space Science Reviews},
  volume = {38},
  number = {3-4},
  pages = {203--242},
  issn = {00386308},
  doi = {10.1007/BF00176830},
  abstract = {The development of electrically self calibrated cavity pyrheliometric instrumentation that occurred in the early 20th century provided the technological base for experiments to detect variability of the solar total irradiance. Experiments from ground based observatories, aircraft and balloons during the 1st half of the 20th century were unable to achieve sufficient accuracy or long term precision to unambiguously detect irradiance variations of solar origin. Refinements in pyrheliometric technology during the 1960's and 1970's and the accessibility of extended experimental opportunities above the Earth's atmosphere in recent years have provided the first direct observations of solar total irradiance variability and provided the cornerstone observations of a long term database on solar irradiance. A program of solar irradiance monitoring has evolved to sustain the database over at least 22 years, corresponding to a single cycle of solar magnetic activity, and the shortest well identified cycle of climate variation. Direct links between total irradiance variations, solar magnetic activity and the solar global '5 min' oscillation phenomena have been derived from recent space flight observations by the SMM/ACRIM I experiment. \textcopyright{} 1984 D. Reidel Publishing Company.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/QMNZY7DN/Willson - 1984.pdf}
}

@article{Willson2000,
  title = {Mass {{Loss}} from {{Cool Stars}}: {{Impact}} on the {{Evolution}} of {{Stars}} and {{Stellar Populations}}},
  author = {Willson, Lee Anne},
  year = {2000},
  journal = {Annual Review of Astronomy and Astrophysics},
  volume = {38},
  number = {1},
  pages = {573--611},
  issn = {0066-4146},
  doi = {10.1146/annurev.astro.38.1.573},
  abstract = {This review emphasizes the mass loss processes that affect the fates of single stars with initial masses between one and nine solar masses. Just one epoch of mass loss has been clearly demonstrated to be important for these stars; that is the episode that ends their evolution up the asymptotic giant branch. Quite a clear picture of this evolutionary stage is emerging from current studies. Mass loss rates increase precipitously as stars evolve toward greater luminosity and radius and decreased effective temperature. As a result, empirical relationships between mass loss rates and stellar parameters are determined mostly by selection effects and tell us which stars are losing mass rather than how stars lose mass. After detailed theoretical models are found to match observational constraints, the models may be used to extrapolate to populations not available for study nearby, such as young stars with low metallicity. The fates of stars are found to depend on both their initial masses and their initial metallicities; a larger proportion of low-metallicity stars should end up with core masses reaching the Chandrasekhar limit, giving rise to Type 1.5 supernovae, and the remnant white dwarfs of low-Z populations will be both fewer and more massive than those in Population I. There are also clear indications that some stars lose one to several tenths of a solar mass during the helium core flash, but neither models nor observations reveal any details of this process yet. The observational and theoretical bases for a variety of mass loss formulae in current use are also reviewed in this article, and the relations are compared in a series of figures.},
  keywords = {and nine solar masses,asymptotic giant stars,circumstellar,dust,emphasizes the mass loss,fates,initial masses between one,just one epoch,mira variables,notion,notion-database,of single stars with,processes that affect the,s abstract this review,stellar evolution,stellar winds},
  file = {/Users/lbugnet/Zotero/storage/9Y5NUFMC/Willson - 2000.pdf}
}

@inproceedings{Winget1988,
  title = {Seismological {{Investigations}} of Compact Stars},
  booktitle = {{{IAUS}}},
  author = {Winget, D.E.},
  year = {1988},
  volume = {123},
  urldate = {2020-11-10},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/UEIEQJT4/m-api-04edd2c2-7ce7-ae99-6427-8e3c83955aaa.pdf}
}

@article{Winn2010,
  title = {Hot {{Stars}} with {{Hot Jupiters Have High Obliquities}}},
  author = {Winn, Joshua N. and Fabrycky, Daniel and Albrecht, Simon and Johnson, John Asher},
  year = {2010},
  month = jun,
  journal = {The Astrophysical Journal Letters},
  volume = {718},
  number = {2},
  eprint = {1006.4161},
  pages = {145--149},
  doi = {10.1088/2041-8205/718/2/L145},
  urldate = {2020-07-07},
  abstract = {We show that stars with transiting planets for which the stellar obliquity is large are preferentially hot (T\_eff {$>$} 6250 K). This could explain why small obliquities were observed in the earliest measurements, which focused on relatively cool stars drawn from Doppler surveys, as opposed to hotter stars that emerged later from transit surveys. The observed trend could be due to differences in planet formation and migration around stars of varying mass. Alternatively, we speculate that hot-Jupiter systems begin with a wide range of obliquities, but the photospheres of cool stars realign with the orbits due to tidal dissipation in their convective zones, while hot stars cannot realign because of their thinner convective zones. This in turn would suggest that hot Jupiters originate from few-body gravitational dynamics, and that disk migration plays at most a supporting role.},
  archiveprefix = {arxiv},
  keywords = {formation-planet-star interactions-stars,notion,notion-database,planetary systems-planets and satellites,rotation},
  file = {/Users/lbugnet/Zotero/storage/44T74K5U/full-text.pdf}
}

@article{Witze2019,
  title = {'{{Marsquakes}}' Reveal Red Planet's Hidden Geology},
  author = {Witze, Alexandra},
  year = {2019},
  month = dec,
  journal = {Nature},
  volume = {576},
  number = {7787},
  pages = {348},
  publisher = {{NLM (Medline)}},
  issn = {14764687},
  doi = {10.1038/d41586-019-03796-7},
  urldate = {2020-03-07},
  pmid = {31848480},
  keywords = {notion,notion-database,Planetary science},
  file = {/Users/lbugnet/Zotero/storage/HEKAHQI4/full-text.pdf}
}

@article{wolff1986,
  title = {Activity in {{F}} Stars},
  author = {Wolff, Sidney C. and Boesgaard, Ann Merchant and Simon, Theodore},
  year = {1986},
  journal = {The Astrophysical Journal},
  volume = {310},
  number = {9},
  eprint = {1011.1669v3},
  pages = {360--370},
  issn = {1098-6596},
  doi = {10.1017/CBO9781107415324.004},
  archiveprefix = {arxiv},
  isbn = {9788578110796},
  pmid = {25246403},
  keywords = {icle,notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/TTVMAQRX/Wolff, Boesgaard, Simon - 1986.pdf}
}

@article{Woltjer1959,
  title = {Hydromagnetic {{Equilibrium IV}}. {{Axisymmetric Compressible Media}}.},
  author = {Woltjer, L.},
  year = {1959},
  month = sep,
  journal = {The Astrophysical Journal},
  volume = {130},
  pages = {405},
  publisher = {{IOP Publishing}},
  issn = {0004-637X},
  doi = {10.1086/146732},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Wood2011,
  title = {The {{Sun}}'s Meridional Circulation and Interior Magnetic Field},
  author = {Wood, Toby S. and McCaslin, Jeremy O. and Garaud, Pascale},
  year = {2011},
  month = jun,
  journal = {The Astrophysical Journal},
  volume = {738},
  number = {21pp},
  eprint = {1106.5250},
  pages = {47},
  doi = {10.1088/0004-637X/738/1/47},
  urldate = {2020-07-06},
  abstract = {To date, no self-consistent numerical simulation of the solar interior has succeeded in reproducing the observed thinness of the solar tachocline, and the persistence of uniform rotation beneath it. Although it is known that the uniform rotation can be explained by the presence of a global-scale confined magnetic field, numerical simulations have thus far failed to produce any solution where such a field remains confined against outward diffusion. We argue that the problem lies in the choice of parameters for which these numerical simulations have been performed. We construct a simple analytical magneto-hydrodynamic model of the solar interior and identify several distinct parameter regimes. For realistic solar parameter values, our results are in broad agreement with the tachocline model of Gough \& McIntyre. In this regime, meridional flows driven at the base of the convection zone are of sufficient amplitude to hold back the interior magnetic field against diffusion. For the parameter values used in existing numerical simulations, on the other hand, we find that meridional flows are significantly weaker and, we argue, unable to confine the interior field. We propose a method for selecting parameter values in future numerical models.},
  archiveprefix = {arxiv},
  keywords = {interior-Sun,magnetohydrodynamics (MHD)-Sun,notion,notion-database,rotation},
  file = {/Users/lbugnet/Zotero/storage/FZKZLWUH/full-text.pdf}
}

@article{Woodard1985,
  title = {Change of Solar Oscillation Eigenfrequencies with the Solar Cycle},
  author = {Woodard, Martin F. and Noyes, Robert W.},
  year = {1985},
  journal = {Nature},
  volume = {318},
  number = {6045},
  pages = {449--450},
  issn = {00280836},
  doi = {10.1038/318449a0},
  abstract = {Solar acoustic eigenfrequencies depend on the internal structure of the Sun, which may change during the 11-yr cycle of magnetic activity as a result of various effects associated with the solar dynamo. Observations of low-degree acoustic frequencies were made, using the ACRIM instrument on the Solar Maximum Mission (SMM) satellite, in 1980 (near solar maximum) and 1984 (near solar minimum). The analysis of these data, presented here, indicates that the frequencies of l = 0 and l = 1 acoustic modes in the 5-min band have decreased from 1980 to 1984, by {$\sim$}0.42 Hz or 1.3 parts in 104. This finding may have important implications for our understanding of the mechanism of the solar activity cycle. \textcopyright{} 1985 Nature Publishing Group.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/E3A7MF2P/Woodard, Noyes - 1985.pdf}
}

@article{wpSolarlikeLightcurveSimulator2016,
  title = {The {{Solar-like Light-curve Simulator}} ( {{SLS}} ) {{In}} Short},
  author = {Wp, Plato- Pspsm and Samadi, R},
  year = {2016},
  number = {May},
  pages = {23--24},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/B7Q8Z766/samadi_16_05_24_sls.pdf}
}

@article{Wright1973,
  title = {{{PINCH INSTABILITIES IN MAGNETIC STARS}}},
  author = {Wright, G A E},
  year = {1973},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {162},
  pages = {339--358},
  urldate = {2020-07-02},
  keywords = {notion,notion-database}
}

@article{Wright2004,
  title = {Do {{We Know}} of {{Any Maunder Minimum Stars}}?},
  author = {Wright, J. T.},
  year = {2004},
  journal = {The Astronomical Journal},
  volume = {128},
  number = {3},
  eprint = {astro-ph/0406338},
  pages = {1273--1278},
  issn = {0004-6256},
  doi = {10.1086/423221},
  abstract = {Most stars previously identified as Maunder minimum stars are old stars evolved off of the main sequence. Analysis of activity measurements from the California and Carnegie Planet Search program stars and Hipparcos parallaxes implies that the canonical age-chromospheric activity relation breaks down for stars older than \$\textbackslash sim 6\$ Gyr when activity is calculated from Mount Wilson S values. Stars only 1 magnitude above the main sequence exhibit significantly suppressed activity levels which have been mistaken for examples of Maunder minimum behavior.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/6PMY73VH/Wright - 2004.pdf}
}

@article{Wright2004a,
  title = {Chromospheric {{Ca}} Ii {{Emission}} in {{Nearby F}}, {{G}}, {{K}}, and {{M Stars}}},
  author = {Wright, J. T. and Marcy, G. W. and Butler, R. Paul and Vogt, S. S.},
  year = {2004},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {152},
  number = {2},
  eprint = {astro-ph/0402582},
  pages = {261--295},
  issn = {0067-0049},
  doi = {10.1086/386283},
  abstract = {We present chromospheric Ca II H and K activity measurements, rotation periods, and ages for \textasciitilde 1200 F, G, K, and M type main-sequence stars from \textasciitilde 18,000 archival spectra taken at Keck and Lick Observatories as a part of the California and Carnegie Planet Search Project. We have calibrated our chromospheric S-values against the Mount Wilson chromospheric activity data. From these measurements we have calculated median activity levels and derived R'HK, stellar ages, and rotation periods from general parameterizations for 1228 stars, \textasciitilde 1000 of which have no previously published S-values. We also present precise time series of activity measurements for these stars. Based on observations obtained at Lick Observatory, which is operated by the University of California, and on observations obtained at the W. M. Keck Observatory, which is operated jointly by the University of California and the California Institute of Technology. The Keck Observatory was made possible by the generous financial support of the W. M. Keck Foundation.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/I8XWKLZL/Wright et al. - 2004.pdf}
}

@article{Wright2016,
  title = {Solar-Type Dynamo Behaviour in Fully Convective Stars without a Tachocline},
  author = {Wright, Nicholas J. and Drake, Jeremy J.},
  year = {2016},
  journal = {Nature},
  eprint = {1607.07870},
  issn = {14764687},
  doi = {10.1038/nature18638},
  abstract = {In solar-type stars (with radiative cores and convective envelopes like our Sun), the magnetic field powers star spots, flares and other solar phenomena, as well as chromospheric and coronal emission at ultraviolet to X-ray wavelengths. The dynamo responsible for generating the field depends on the shearing of internal magnetic fields by differential rotation. The shearing has long been thought to take place in a boundary layer known as the tachocline between the radiative core and the convective envelope. Fully convective stars do not have a tachocline and their dynamo mechanism is expected to be very different, although its exact form and physical dependencies are not known. Here we report observations of four fully convective stars whose X-ray emission correlates with their rotation periods in the same way as in solar-type stars. As the X-ray activity-rotation relationship is a well-established proxy for the behaviour of the magnetic dynamo, these results imply that fully convective stars also operate a solar-type dynamo. The lack of a tachocline in fully convective stars therefore suggests that this is not a critical ingredient in the solar dynamo and supports models in which the dynamo originates throughout the convection zone.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Xiang-Gruess2016,
  title = {On the Formation of a Quasi-Stationary Twisted Disc after a Tidal Disruption Event},
  author = {{Xiang-Gruess}, M. and Ivanov, P. B. and Papaloizou, J. C.B.},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {463},
  number = {2},
  pages = {2242--2264},
  issn = {13652966},
  doi = {10.1093/mnras/stw2130},
  abstract = {We investigate misaligned accretion discs formed after tidal disruption events that occur when a star encounters a supermassive black hole. We employ the linear theory of warped accretion discs to find the shape of a disc for which the stream arising from the disrupted star provides a source of angular momentum that is misaligned with that of the black hole. For quasi-steady configurations, we find that when the warp diffusion or propagation time is large compared to the local mass accretion time and/or the natural disc alignment radius is small, misalignment is favoured. These results have been verified using smoothed particle hydrodynamics simulations. We also simulated 1D model discs including gas and radiation pressure. As accretion rates initially exceed the Eddington limit, the disc is initially advection dominated. Assuming the {$\alpha$} model for the disc, where it can be thermally unstable, it subsequently undergoes cyclic transitions between high and low states. During these transitions, the aspect ratio varies from \textasciitilde{} 1 to \textasciitilde{} 10-3 which is reflected in changes in the degree of disc misalignment at the stream impact location. For maximal black hole rotation and sufficiently large values of viscosity parameter {$\alpha$} {$>$} \textasciitilde{} 0.01-0.1, the ratio of the disc inclination to that of the initial stellar orbit is estimated to be 0.1-0.2 in the advection-dominated state, while reaching of order unity in the low state. Misalignment decreases with decrease of {$\alpha$}, but increases as the black hole rotation parameter decreases. Thus, it is always significant when the latter is small.},
  keywords = {Accretion,Accretion discs,Hydrodynamics,notion,notion-database,Quasars: supermassive black holes,Relativistic processes},
  file = {/Users/lbugnet/Zotero/storage/2BSQBUMD/Xiang-Gruess, Ivanov, Papaloizou - 2016.pdf}
}

@article{Xiang2018,
  title = {Stellar Mass Distribution and Star Formation History of the {{Galactic}} Disk Revealed by Mono-Age Stellar Populations from {{LAMOST}}},
  author = {Xiang, Maosheng and Shi, Jianrong and Liu, Xiaowei and Yuan, Haibo and Chen, Bingqiu and Huang, Yang and Wang, Chun and Tian, Zhijia and Huo, Zhiying and Zhang, Huawei and Zhang, And Meng},
  year = {2018},
  journal = {The Astrophysical Journal},
  volume = {237},
  number = {2},
  eprint = {1807.04592v1},
  urldate = {2020-03-06},
  abstract = {We present a detailed determination and analysis of 3D stellar mass distribution of the Galactic disk for mono-age populations using a sample of 0.93 million main-sequence turn-off and subgiant stars from the LAMOST Galactic Surveys. Our results show (1) all stellar populations younger than 10 Gyr exhibit strong disk flaring, which is accompanied with a dumpy vertical density profile that is best described by a sech n function with index depending on both radius and age; (2) Asymmetries and wave-like oscillations are presented in both the radial and vertical direction, with strength varying with stellar populations; (3) As a contribution by the Local spiral arm, the mid-plane stellar mass density at solar radius but 400-800 pc (3-6 \textbullet ) away from the Sun in the azimuthal direction has a value of 0.0594 {$\pm$} 0.0008 M {$\odot$} /pc 3 , which is 0.0164 M {$\odot$} /pc 3 higher than previous estimates at the solar neighborhood. The result causes doubts on the current estimate of local dark matter density; (4) The radial distribution of surface mass density yields a disk scale length evolving from {$\sim$}4 kpc for the young to {$\sim$}2 kpc for the old populations. The overall population exhibits a disk scale length of 2.48 {$\pm$} 0.05 kpc, and a total stellar mass of 3.6({$\pm$}0.1) \texttimes{} 10 10 M {$\odot$} assuming R {$\odot$} = 8.0 kpc, and the value becomes 4.1({$\pm$}0.1) \texttimes{} 10 10 M {$\odot$} if R {$\odot$} = 8.3 kpc; (5) The disk has a peak star formation rate (SFR) changing from 6-8 Gyr at the inner to 4-6 Gyr ago at the outer part, indicating an inside-out assemblage history. The 0-1 Gyr population yields a recent disk total SFR of 1.96 {$\pm$} 0.12 M {$\odot$} /yr.},
  archiveprefix = {arxiv},
  keywords = {disk-Galaxy,evolution-Galaxy,formation,Galaxy,notion,notion-database,structure-Galaxy},
  file = {/Users/lbugnet/Zotero/storage/36SD24SX/full-text.pdf}
}

@article{Yang2006,
  title = {Angular Momentum Transport and Element Mixing in the Stellar Interior {{I}}. {{Application}} to the Rotating {{Sun}}},
  author = {Yang, W. M. and Bi, S. L.},
  year = {2006},
  journal = {Astronomy and Astrophysics},
  volume = {449},
  number = {3},
  pages = {1161--1168},
  issn = {00046361},
  doi = {10.1051/0004-6361:20053577},
  abstract = {Aims. The purpose of this work was to obtain diffusion coefficient for the magnetic angular momentum transport and material transport in a rotating solar model. Methods. We assumed that the transport of both angular momentum and chemical elements caused by magnetic fields could be treated as a diffusion process. Results. The diffusion coefficient depends on the stellar radius, angular velocity, and the configuration of magnetic fields. By using of this coefficient, it is found that our model becomes more consistent with the helioseismic results of total angular momentum, angular momentum density, and the rotation rate in a radiative region than the one without magnetic fields. Not only can the magnetic fields redistribute angular momentum efficiently, but they can also strengthen the coupling between the radiative and convective zones. As a result, the sharp gradient of the rotation rate is reduced at the bottom of the convective zone. The thickness of the layer of sharp radial change in the rotation rate is about 0.036 R {$\odot$} in our model. Furthermore, the difference of the sound-speed square between the seismic Sun and the model is improved by mixing the material that is associated with angular momentum transport. \textcopyright{} ESO 2006.},
  keywords = {Diffusion,notion,notion-database,Sun: magnetic fields,Sun: rotation},
  file = {/Users/lbugnet/Zotero/storage/UKN8ZDTU/Yang, Bi - 2006.pdf}
}

@article{Yang2013,
  title = {Evolution of Rotational Velocities of {{A-type}} Stars},
  author = {Yang, Wuming and Bi, Shaolan and Meng, Xiangcun and Tian, Zhijia},
  year = {2013},
  journal = {Astrophysical Journal Letters},
  volume = {765},
  number = {2},
  eprint = {1302.0448},
  issn = {20418205},
  doi = {10.1088/2041-8205/765/2/L36},
  abstract = {The equatorial velocity of A-type stars undergoes an acceleration in the first third of the main sequence (MS) stage, but the velocity decreases as if the stars were not undergoing any redistribution of angular momentum in the external layers in the last stage of the MS phase. Our calculations show that the acceleration and the decrease of the equatorial velocity can be reproduced by the evolution of the differential rotation zero-age MS model with the angular momentum transport caused by hydrodynamic instabilities during the MS stage. The acceleration results from the fact that the angular momentum stored in the interiors of the stars is transported outward. In the last stage, the core and the radiative envelope are uncoupling, and the rotation of the envelope is a quasi-solid rotation; the uncoupling and the expansion of the envelope indicate that the decrease of the equatorial velocity approximately follows the slope for the change in the equatorial velocity of the model without any redistribution of angular momentum. When the fractional age 0.3 {$\lessequivlnt$} t/t MS {$\lessequivlnt$} 0.5, the equatorial velocity remains almost constant for stars whose central density increases with age in the early stage of the MS phase, while the velocity decreases with age for stars whose central density decreases with age in the early stage of the MS phase. \textcopyright{} 2013 The American Astronomical Society. All rights reserved.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,stars: early-type,stars: evolution,stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/ERBKV88J/Yang et al. - 2013.pdf}
}

@article{Yoon2005,
  title = {On the Evolution of Rapidly Rotating Massive White Dwarfs towards Supernovae or Collapses},
  author = {Yoon, S. -C. and Langer, N.},
  year = {2005},
  month = jun,
  journal = {Astronomy \& Astrophysics},
  volume = {435},
  pages = {967--985},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20042542},
  urldate = {2023-10-09},
  abstract = {A recent study indicated that the inner cores of rapidly accreting (dot M {$>$} 10-7 M\_{$\odot$} yr-1) CO white dwarfs may rotate differentially, with a shear rate near the threshold value for the onset of the dynamical shear instability. Such differentially rotating white dwarfs have critical masses for thermonuclear explosion or electron-capture induced collapse that significantly exceed the canonical Chandrasekhar limit. Here, we construct two-dimensional differentially rotating white dwarf models with rotation laws resembling those of the one-dimensional models of the previous work. We derive analytic relations between the white dwarf mass, its angular momentum, and its rotational-, gravitational- and binding energy. We show that these relations are applicable for a wide range of angular velocity profiles, including solid body rotation. Taken at a central density of 2 \texttimes{} 10\^9 g cm-3 they specify initial models for the thermonuclear explosion of rotating CO white dwarfs. At {$\rho$}c = 1010 g cm-3 and 4 \texttimes{} 109 g cm-3, they give criteria for the electron-capture induced collapse of rotating CO and ONeMg white dwarfs, respectively. We demonstrate that pre-explosion and pre-collapse conditions of both rigidly and differentially rotating white dwarfs are well established by the present work, which may facilitate future multi-dimensional simulations of type Ia supernova explosions and studies of the formation of millisecond pulsars and gamma-ray bursts from collapsing white dwarfs. Our results lead us to suggest various possible evolutionary scenarios for progenitors of type Ia supernovae, leading to a new paradigm of a variable mass of exploding white dwarfs, at values well above the classical Chandrasekhar mass. Based on our 2D-models, we argue that the supernova peak brightness is proportional to the white dwarf mass, which could explain various aspects of the diversity of type Ia supernovae, such as their variation in brightness, the dependence of their mean luminosity on the host galaxy type, and the weak correlation between ejecta velocity and peak brightness.},
  keywords = {Astrophysics,gamma rays: bursts,stars: neutron,stars: rotation,stars: supernovae: general,stars: white dwarfs},
  annotation = {ADS Bibcode: 2005A\&A...435..967Y},
  file = {/Users/lbugnet/Zotero/storage/L8TVYFX7/Yoon and Langer - 2005 - On the evolution of rapidly rotating massive white.pdf}
}

@article{Yoon2012,
  title = {Evolution of Massive {{Population III}} Stars with Rotation and Magnetic Fields},
  author = {Yoon, S. -C. and Dierks, A. and Langer, N.},
  year = {2012},
  month = jun,
  journal = {Astronomy \& Astrophysics},
  volume = {542},
  pages = {A113},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/201117769},
  urldate = {2023-10-09},
  abstract = {Aims: We present a new grid of massive Population III (Pop III) star models including the effects of rotation on the stellar structure and chemical mixing, and magnetic torques for the transport of angular momentum. This grid covers the range of mass from 10 to 1000 M{$\odot$}, and rotational velocity from zero to 100\% of the critical rotation on the zero-age main sequence. Based on the grid, we also present a phase diagram for the expected final fates (i.e., core-collapse supernova, gamma-ray bursts (GRBs) and pair-instability supernovae of diverse types) of rotating massive Pop III stars. Methods: The model grid has been calculated with a stellar evolution code. We adopted the recent calibration made with the VLT-FLAMES data for the overshooting parameter and the chemical mixing efficiency due to rotation. The Spruit-Tayler dynamo was assumed for magnetic torques. Results: Our non-rotating models become redder than the previous models in the literature because of the larger overshooting parameter adopted in this study. In particular, convective dredge-up of the helium core material into the hydrogen envelope is observed in our non-rotating very massive star models ({$\greaterequivlnt$}200 M{$\odot$}), which is potentially important for the chemical yields. On the other hand, the stars become bluer and more luminous with a higher rotational velocity. With the Spruit-Tayler dynamo, our models with a sufficiently high initial rotational velocity can reach the critical rotation earlier and lose more mass as a result, compared to the previous models without magnetic fields. The most dramatic effect of rotation is found with the so-called chemically homogeneous evolution (CHE), which is observed for a limited mass and rotational velocity range. CHE has several important consequences: 1) both primary nitrogen and ionizing photons are abundantly produced; 2) conditions for GRB progenitors are fulfilled for an initial mass range of 13-84 M{$\odot$}; 3) pair instability supernovae of type Ibc are expected for 84-190 M{$\odot$}; 4) both a pulsational pair instability supernova and a GRB may occur from the same progenitor of \textasciitilde 56-84 M{$\odot$}, which might significantly influence the consequent GRB afterglow. We find that CHE does not occur for very massive stars ({$>$}190 M{$\odot$}), in which case the hydrogen envelope expands to the red-supergiant phase and the final angular momentum is too low to generate any explosive event powered by rotation. Tables 3-5 and Appendix A are available in electronic form at http://www.aanda.org},
  keywords = {Astrophysics - High Energy Astrophysical Phenomena,Astrophysics - Solar and Stellar Astrophysics,dark ages,first stars,gamma-ray burst: general,reionization,stars: evolution,stars: Population III,stars: rotation,supernovae: general},
  annotation = {ADS Bibcode: 2012A\&A...542A.113Y},
  file = {/Users/lbugnet/Zotero/storage/MLMRIIZL/Yoon et al. - 2012 - Evolution of massive Population III stars with rot.pdf}
}

@article{Yu2016,
  title = {Asteroseismology of 1523 Misclassified Red Giants Using {{Kepler}} Data},
  author = {Yu, Jie and Huber, Daniel and Bedding, Timothy R. and Stello, Dennis and Murphy, Simon J. and Xiang, Maosheng and Bi, Shaolan and Li, Tanda},
  year = {2016},
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {463},
  number = {2},
  eprint = {1608.05803},
  pages = {1297--1306},
  issn = {13652966},
  doi = {10.1093/mnras/stw2074},
  abstract = {We analysed solar-like oscillations in 1523 Kepler red giants which have previously been misclassified as subgiants, with predicted {$\upsilon$}max values [based on the Kepler Input Catalogue (KIC)] between 280 and 700 {$\mu$}Hz. We report the discovery of 626 new oscillating red giants in our sample, in addition to 897 oscillators that were previously characterized by Hekker et al. from one quarter of Kepler data. Our sample increases the known number of oscillating low-luminosity red giants by 26 per cent (up to \textasciitilde 1900 stars). About three quarters of our sample are classified as ascending red giant branch stars, while the remainder are red-clump stars. A novel scheme was applied to determine {$\Delta\upsilon$} for 108 stars with {$\upsilon$}max close to the Nyquist frequency (240 {$\mu$}Hz {$<$} {$\upsilon$}max {$<$} 320 {$\mu$}Hz). Additionally, we identified 47 stars oscillating in the super-Nyquist frequency regime, up to 387 {$\mu$}Hz, using long-cadence light curves. We show that the misclassifications are most likely due to large uncertainties in KIC surface gravities, and do not result from the absence of broad-band colours or from different physical properties such as reddening, spatial distribution, mass or metallicity. The sample will be valuable to study oscillations in low-luminosity red giants and to characterize planet candidates around those stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database,Stars: oscillations,Techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/QZB4S9RU/Yu et al. - 2016.pdf}
}

@article{Yu2018,
  title = {Asteroseismology of 16,000 {{Kepler Red Giants}}: {{Global Oscillation Parameters}}, {{Masses}}, and {{Radii}}},
  author = {Yu, Jie and Huber, Daniel and Bedding, Timothy R and Stello, Dennis and Hon, Marc and Murphy, Simon J and Khanna, Shourya},
  year = {2018},
  journal = {The Astrophysical Journal Supplement Series},
  volume = {236},
  pages = {42},
  doi = {10.3847/1538-4365/aaaf74},
  urldate = {2020-03-31},
  abstract = {The Kepler mission has provided exquisite data to perform an ensemble asteroseismic analysis on evolved stars. In this work we systematically characterize solar-like oscillations and granulation for 16,094 oscillating red giants, using end-of-mission long-cadence data. We produced a homogeneous catalog of the frequency of maximum power (typical uncertainty s = n 1.6\% max), the mean large frequency separation (s = n D 0.6\%), oscillation amplitude (s = 4.7\% A), granulation power (s = 8.6\% gran), power excess width (s = 8.8\% width), seismically derived stellar mass (s = 7.8\% M), radius (s = 2.9\% R), and thus surface gravity (s = 0.01 g log dex). Thanks to the large red giant sample, we confirm that red-giant-branch (RGB) and helium-core-burning (HeB) stars collectively differ in the distribution of oscillation amplitude, granulation power, and width of power excess, which is mainly due to the mass difference. The distribution of oscillation amplitudes shows an extremely sharp upper edge at fixed n max , which might hold clues for understanding the excitation and damping mechanisms of the oscillation modes. We find that both oscillation amplitude and granulation power depend on metallicity, causing a spread of 15\% in oscillation amplitudes and a spread of 25\% in granulation power from [Fe/H]=-0.7 to 0.5 dex. Our asteroseismic stellar properties can be used as reliable distance indicators and age proxies for mapping and dating galactic stellar populations observed by Kepler. They will also provide an excellent opportunity to test asteroseismology using Gaia parallaxes, and lift degeneracies in deriving atmospheric parameters in large spectroscopic surveys such as APOGEE and LAMOST.},
  keywords = {catalogs,notion,notion-database,stars: fundamental parameters,stars: oscillations,techniques: photometric},
  file = {/Users/lbugnet/Zotero/storage/JFJ6X9LN/full-text.pdf}
}

@article{Yu2020,
  title = {Asteroseismology of Luminous Red Giants with {{Kepler I}}: Long-Period Variables with Radial and Non-Radial Modes},
  author = {Yu, Jie and Bedding, Timothy R and Stello, Dennis and Huber, Daniel and Compton, Douglas L and Gizon, Laurent and Hekker, Saskia},
  year = {2020},
  month = mar,
  journal = {Monthly Notices of the Royal Astronomical Society},
  volume = {493},
  number = {1},
  eprint = {2001.10878},
  pages = {1388--1403},
  publisher = {{Oxford University Press (OUP)}},
  issn = {0035-8711},
  doi = {10.1093/mnras/staa300},
  urldate = {2020-07-04},
  abstract = {While long-period variables (LPVs) have been extensively investigated, especially with MACHO and OGLE data for the Magellanic Clouds, there still exist open questions in their pulsations regarding the excitation mechanisms, radial order, and angular degree assignment. Here, we perform asteroseismic analyses on LPVs observed by the 4-year Kepler mission. Using a cross-correlation method, we detect unambiguous pulsation ridges associated with radial fundamental modes (n~= 1) and overtones (n {$\geq$} 2), where the radial order assignment is made using theoretical frequencies and observed frequencies. Our results confirm that the amplitude variability seen in semiregulars is consistent with oscillations being solar-like. We identify that the dipole modes, l~= 1, are dominant in the radial orders of 3 {$\leq$} n {$\leq$} 6, and that quadrupole modes, l~= 2, are dominant in the first overtone n~= 2. A test of seismic scaling relations using Gaia DR2 parallaxes reveals the possibility that the relations break down when {$\nu$}max~{$\lessequivlnt~$}3 \$\textbackslash mu \{\textbackslash rm Hz\}\$ (R~{$\greaterequivlnt~$}40 R{$\odot$}, or log \$\textbackslash rm L/L\_\{\textbackslash odot \}\$~{$\greaterequivlnt~$}2.6). Our homogeneous measurements of pulsation amplitude and period for 3213 LPVs will be valuable for probing effects of pulsation on mass-loss, in particular in those stars with periods around 60 d, which has been argued as a threshold of substantial pulsation-triggered mass-loss.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database}
}

@article{Zaatri2007,
  title = {Sensitivity of Low Degree Oscillations to the Change in Solar Abundances},
  author = {Zaatri, A. and Provost, J. and Berthomieu, G. and Morel, P. and Corbard, T.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {469},
  number = {3},
  pages = {1145--1149},
  issn = {00046361},
  doi = {10.1051/0004-6361:20077212},
  abstract = {Context. The most recent determination of the solar chemical composition, using a time-dependent, 3D hydrodynamical model of the solar atmosphere, exhibits a significant decrease of C, N, O abundances compared to their previous values. Solar models that use these new abundances are not consistent with helioseismological determinations of the sound speed profile, the surface helium abundance and the convection zone depth. Aims. We investigate the effect of changes of solar abundances on low degree p-mode and g-mode characteristics which are strong constraints of the solar core. We consider particularly the increase of neon abundance in the new solar mixture in order to reduce the discrepancy between models using new abundances and helioseismology. Methods. The observational determinations of solar frequencies from the GOLF instrument are used to test solar models computed with different chemical compositions. We consider in particular the normalized small frequency spacings in the low degree p-mode frequency range. Results. Low-degree small frequency spacings are very sensitive to changes in the heavy-element abundances, notably neon. We show that by considering all the seismic constraints, including the small frequency spacings, a rather large increase of neon abundance by about (0.5 {$\pm$} 0.05) dex can be a good solution to the discrepancy between solar models that use new abundances and low degree helioseismology, subject to adjusting slightly the solar age and the highest abundances. We also show that the change in solar abundances, notably neon, considerably affects g-mode frequencies, with relative frequency differences between the old and the new models higher than 1.5\%. \textcopyright{} ESO 2007.},
  keywords = {notion,notion-database,Sun: abundances,Sun: helioseismology,Sun: interior},
  file = {/Users/lbugnet/Zotero/storage/CNYUPA2F/Zaatri et al. - 2007.pdf}
}

@inproceedings{Zadrozny2001,
  title = {Obtaining Calibrated Probability Estimates from Decision Trees and Naive {{Bayesian}} Classifiers},
  booktitle = {In {{Proceedings}} of the {{Eighteenth International Conference}} on {{Machine Learning}}},
  author = {Zadrozny, Bianca and Elkan, Charles},
  year = {2001},
  urldate = {2020-04-11},
  abstract = {Accurate, well-calibrated estimates of class membership probabilities are needed in many supervised learning applications, in particular when a cost-sensitive decision must be made about examples with example-dependent costs. This paper presents simple but successful methods for obtaining calibrated probability estimates from decision tree and naive Bayesian classi-fiers. Using the large and challenging KDD'98 contest dataset as a testbed, we report the results of a detailed experimental comparison of ten methods, according to four evaluation measures. We conclude that binning succeeds in significantly improving naive Bayesian probability estimates, while for improving decision tree probability estimates, we recommend smoothing by-estimation and a new variant of pruning that we call curtailment.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/GFUAJC8J/full-text.pdf}
}

@techreport{Zadrozny2002,
  title = {Transforming {{Classifier Scores}} into {{Accurate Multiclass Probability Estimates}}},
  author = {Zadrozny, Bianca and Elkan, Charles},
  year = {2002},
  urldate = {2020-04-04},
  abstract = {Class membership probability estimates are important for many applications of data mining in which classification outputs are combined with other sources of information for decision-making, such as example-dependent misclassification costs, the outputs of other classifiers, or domain knowledge. Previous calibration methods apply only to two-class problems. Here, we show how to obtain accurate probability estimates for multiclass problems by combining calibrated binary probability estimates. We also propose a new method for obtaining calibrated two-class probability estimates that can be applied to any classifier that produces a ranking of examples. Using naive Bayes and support vector machine classifiers, we give experimental results from a variety of two-class and multiclass domains, including direct marketing, text categorization and digit recognition.},
  isbn = {158113567X},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/WJ6BNUP4/full-text.pdf}
}

@article{Zahn1966,
  title = {Les Mar\'ees Dans Une \'Etoile Double Serr\'ee (Suite)},
  author = {Zahn, J. P. and P., J.},
  year = {1966},
  journal = {AnAp},
  volume = {29},
  pages = {489},
  issn = {0365-0499},
  urldate = {2020-07-13},
  keywords = {notion,notion-database}
}

@article{Zahn1989,
  title = {Tidal Evolution of Close Binary Stars. {{I}} - {{Revisiting}} the Theory of the Equilibrium Tide},
  author = {Zahn, J. -P. and {-P.}, J.},
  year = {1989},
  journal = {A\&A},
  volume = {220},
  number = {1-2},
  pages = {112--116},
  issn = {0004-6361},
  urldate = {2020-07-13},
  keywords = {Astrophysics,Binary Stars,Mixing Length Flow Theory,notion,notion-database,Stellar Envelopes,Stellar Evolution,Tides,Turbulence Effects,Viscosity}
}

@article{Zahn1992,
  title = {Circulation and Turbulence in Rotating Stars.},
  author = {Zahn, J.P.},
  year = {1992},
  journal = {A\&A},
  volume = {265},
  pages = {115--132},
  issn = {0004-6361},
  urldate = {2020-07-02},
  keywords = {Angular Momentum,Astrophysics,Meridional Flow,Momentum Transfer,notion,notion-database,Stellar Composition,Stellar Interiors,Stellar Models,Stellar Physics,Stellar Rotation,Turbulence}
}

@article{Zahn2007,
  title = {On Magnetic Instabilities and Dynamo Action in Stellar Radiation Zones},
  author = {Zahn, J. P. and Brun, A. S. and Mathis, S.},
  year = {2007},
  journal = {Astronomy and Astrophysics},
  volume = {474},
  number = {1},
  pages = {145--154},
  issn = {00046361},
  doi = {10.1051/0004-6361:20077653},
  abstract = {Context. We examine the MHD instabilities arising in the radiation zone of a differentially rotating star, in which a poloidal field of fossil origin is sheared into a toroidal field. Aims. We focus on the non-axisymmetric instability that affects the toroidal magnetic field in a rotating star, which was first studied by Pitts and Tayler in the non-dissipative limit. If such an instability were able to mix the stellar material, it could have an impact on the evolution of the star. According to Spruit, it could also drive a dynamo. Methods. We compare the numerical solutions built with the 3-dimensional ASH code with the predictions drawn from an analytical study of the Pitts \& Tayler instability. Results. The Pitts \& Tayler instability is manifestly present in our simulations, with its conspicuous m = 1 dependence in azimuth. But its analytic treatment used so far is too simplified to be applied to the real stellar situation. Although the instability generated field reaches an energy comparable to that of the mean poloidal field, that field seems unaffected by the instability: it undergoes Ohmic decline, and is neither eroded nor regenerated by the instability. The toroidal field is produced by shearing the poloidal field and it draws its energy from the differential rotation. The small scale motions behave as Alfv\'en waves; they cause negligible eddy-diffusivity and contribute little to the net transport of angular momentum. Conclusions. In our simulations we observe no sign of dynamo action, of either mean field or fluctuation type, up to a magnetic Reynolds number of 10 5. However the Pitts \& Tayler instability is sustained as long as the differential rotation acting on the poloidal field is able to generate a toroidal field of sufficient strength. But in the Sun such a poloidal field of fossil origin is ruled out by the nearly uniform rotation of the deep interior. \textcopyright{} ESO 2007.},
  keywords = {Instabilities,Magnetohydrodynamics (MHD),notion,notion-database,Stars: magnetic fields,Stars: rotation},
  file = {/Users/lbugnet/Zotero/storage/9XSDSB4B/Zahn, Brun, Mathis - 2007.pdf}
}

@inproceedings{Zahn2008,
  title = {Instabilities and Mixing in Stellar Radiation Zones},
  booktitle = {Proceedings of the {{International Astronomical Union}}},
  author = {Zahn, Jean Paul},
  year = {2008},
  volume = {4},
  pages = {47--59},
  issn = {17439213},
  doi = {10.1017/S1743921308022424},
  urldate = {2020-07-02},
  abstract = {The standard model of stellar structure is unable to account for various observational facts, and there is now a large consensus that some 'extra mixing' must occur in the radiation zones. The possible causes for such mixing are briefly reviewed. The most efficient among them is probably the shear-turbulence generated by the differential rotation, which itself results from the transport of angular momentum that can be mediated through the large-scale circulation induced by structural adjustments or by the applied torques (stellar wind, accretion, tides). In solar-type stars this angular momentum transport is ensured mainly by internal gravity waves that are excited at the boundary with convection zones. Another cause of mixing manifests itself in the red giant phase, namely the thermohaline instability due to an inversion of the molecular weight gradient. The implementation of these processes in stellar evolution codes is giving rise to a new generation of stellar models, which are in much better agreement with the observational constraints. \textcopyright{} 2008 International Astronomical Union.},
  keywords = {Instabilities,Interiors,notion,notion-database,Rotation,Stars: evolution,Turbulence}
}

@article{Zakharov1994,
  title = {The {{Mars-94}} and {{Mars-96}} Missions},
  author = {Zakharov, Alexander V. and V., Alexander},
  year = {1994},
  month = nov,
  journal = {Philosophical Transactions of the Royal Society of London. Series A: Physical and Engineering Sciences},
  volume = {349},
  number = {1690},
  pages = {295--307},
  publisher = {{The Royal Society}},
  issn = {0962-8428},
  doi = {10.1098/rsta.1994.0133},
  urldate = {2020-03-07},
  abstract = {The main goal of Solar System studies in Russia for the next 10-15 years is Mars and the Mars-94 project is the first stage of this long-term space programme. In October 1994 it is planned to launch a spacecraft with the following components onboard: an orbiter, two small autonomous stations to be landed on the surface of Mars and two penetrators to analyse the underlying surface layers. The main scientific objectives of this mission are to investigate the evolution and contemporary physics of Mars, and to make, using various methods, a wide range of comprehensive studies of those physical and chemical processes which took place in the past and which continue there now. The payload of the Mars-94 orbiter includes 23 scientific instruments to study the Martian surface, the inner structure of the planet, its atmosphere, and its plasma envelope, as well as instruments for astrophysical studies. The next stage of the programme is a mission to Mars in 1996. At present the Mars-96 project includes a spacecraft with an orbiter, a Martian rover, a balloon, penetrators and small stations. A short description of the scenario, payload, and scientific objectives of these missions is presented in this paper.},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/PQLX444A/full-text.pdf}
}

@article{zhangPremainsequenceDordSct2020,
  title = {A {{Pre-main-sequence}} {$\gamma$} {{Dor-$\delta$ Sct Hybrid}} with {{Extremely Slow Internal Rotation}} in a {{Short-period Eclipsing Binary KIC}} 9850387 {{Revealed}} by {{Asteroseismology}}},
  author = {Zhang, X and Chen, X and Zhang, H and Fu, J.N.},
  year = {2020},
  journal = {The Astrophysical journal},
  volume = {895},
  pages = {124},
  urldate = {2021-01-26},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/97JKQH2M/Zhang_2020_ApJ_895_124.pdf}
}

@article{Zhou2019,
  title = {The {{Amplitude}} of {{Solar}} P-Mode {{Oscillations}} from {{Three-dimensional Convection Simulations}}},
  author = {Zhou, Yixiao and Asplund, Martin and Collet, Remo},
  year = {2019},
  journal = {The Astrophysical Journal},
  volume = {880},
  number = {1},
  eprint = {1905.13397},
  pages = {13},
  issn = {1538-4357},
  doi = {10.3847/1538-4357/ab262c},
  abstract = {The amplitude of solar p-mode oscillations is governed by stochastic excitation and mode damping, both of which take place in the surface convection zone. However, the time-dependent, turbulent nature of convection makes it difficult to self-consistently study excitation and damping processes through the use of traditional one-dimensional hydrostatic models. To this end, we carried out \textbackslash textit\{ab initio\} three-dimensional, hydrodynamical numerical simulations of the solar atmosphere to investigate how p-modes are driven and dissipated in the Sun. The description of surface convection in the simulations is free from the tuneable parameters typically adopted in traditional one-dimensional models. Mode excitation and damping rates are computed based on analytical expressions whose ingredients are evaluated directly from the three-dimensional model. With excitation and damping rates both available, we estimate the theoretical oscillation amplitude and frequency of maximum power, \$\textbackslash nu\_\{\textbackslash max\}\$, for the Sun. We compare our numerical results with helioseismic observations, finding encouraging agreement between the two. The numerical method presented here provides a novel way to investigate the physical processes responsible for mode driving and damping, and should be valid for all solar-type oscillating stars.},
  archiveprefix = {arxiv},
  keywords = {notion,notion-database},
  file = {/Users/lbugnet/Zotero/storage/5CZH763U/Zhou, Asplund, Collet - 2019.pdf}
}

@techreport{Ziegler2000,
  title = {Angular Momentum Transport and Dynamo-Effect in Stratified, Weakly Magnetic Disks},
  author = {Ziegler, U},
  year = {2000},
  journal = {Astron. Astrophys},
  volume = {356},
  pages = {1141--1148},
  issn = {0004-6361},
  urldate = {2020-07-02},
  abstract = {The magnetic shear instability is reviewed numerically in the local box approximation for a Kepler disk. Special emphasis is laid on the relation between the viscosity-alpha and dynamo-alpha in case a mean magnetic field is generated. Self-sustaining 'turbulence' is initiated by the instability which acts simultaneously as dynamo and efficient outward transporter for angular momentum. The Shakura-Sunyaev parameter {$\alpha$} SS is estimated to {$\approx$} 1.5 {$\cdot$} 10 -2 for an adiabatic disk model, and the contribution from the Maxwell stress dominates over that of the Reynolds stress by a factor of 4. In case of stress-free, normal-B vertical boundary conditions , a non-zero mean magnetic field mainly oriented in az-imuthal direction is generated. This mean field turns out time-dependent in a quasi-periodic manner. Box resonance oscillations in the horizontal velocities for a limited time lead to an enhanced, violently fluctuating Reynolds stress associated with a reduced magnetic activity. The resulting (dynamo-) {$\alpha$}-effect is negative in the upper disk plane and positive in the lower disk plane, it is small and highly noisy.},
  keywords = {INSTABILITIES,MAGNETIC FIELDS,MAGNETOHYDRODYNAMICS (MHD),notion,notion-database,TURBULENCE},
  file = {/Users/lbugnet/Zotero/storage/RZB6UTUG/full-text.pdf}
}

@article{Ziegler2003,
  title = {Box Simulations of Rotating Magnetoconvection. {{Effects}} of Penetration and Turbulent Pumping},
  author = {Ziegler, U. and R{\"u}diger, G.},
  year = {2003},
  month = apr,
  journal = {Astronomy and Astrophysics},
  volume = {401},
  pages = {433--442},
  issn = {0004-6361},
  doi = {10.1051/0004-6361:20030207},
  urldate = {2023-10-18},
  abstract = {Various effects of penetration in rotating magnetoconvection are studied by means of three-dimensional numerical simulations employing the code NIRVANA. A local, 2-layer model is applied dividing the computational domain (which is a rectangular box placed tangentially on a sphere at latitude 45deg) in an unstable polytropic region on top of a stable polytropic region. Different realizations of convection are examined parameterized by Taylor numbers Ta=0,6 x 104, 6x 105 and magnetic field strengths {$\beta$} = 5,50,500,5000,infty . We find a rather distinctive behavior of the penetration depth Delta on the system parameters (Ta,{$\beta$}). In non-rotating convection Delta is a monotonically decreasing function of {$\beta$}-1 which is due to magnetic quenching effects. Also, penetration is subject to rotational quenching, i.e. Delta is reduced for increasing rotation rate. In the intermediate regime of (Ta,{$\beta$}), the effects of rotation and magnetic field on Delta do not simply add (see Fig. 3). We find, nevertheless, a very strong reduction of the penetration depth of overshooting turbulence by both rotation and magnetism. Penetrative convection is closely associated with the mixing of a passive scalar quantity advected with the flow. In the long term, the tracer material penetrates significantly deeper into the stable layer than suggested by Delta which is due to the cumulative effect of isolated, fast-moving plumes. In case of a weak magnetic field, penetrative convection also serves to ensure a downward transport of magnetic flux by turbulent pumping with an average rate gammaz \textasciitilde{} -7x 10-3 measured in units of the sound speed at the top z-boundary. For larger magnetic fields the pumping effect is quenched and even changes sign in the convection zone. This effect is suggested as being due to the effect of ``turbulent buoyancy'' which in density-stratified media transports a given magnetic field upwards if it is not too strong (Kichatinov \& R\"udiger \textbackslash cite\{Kichatinov92\}).},
  keywords = {convection,magnetic fields,magnetohydrodynamics,turbulence},
  annotation = {ADS Bibcode: 2003A\&A...401..433Z},
  file = {/Users/lbugnet/Zotero/storage/QYL4AZ8T/Ziegler and Rüdiger - 2003 - Box simulations of rotating magnetoconvection. Eff.pdf}
}

@article{Zinn2020,
  title = {The {{K2 Galactic Archaeology Program Data Release}} 2: {{Asteroseismic Results}} from {{Campaigns}} 4, 6, and 7},
  author = {Zinn, Joel C. and Stello, Dennis and Elsworth, Yvonne and Garc{\'i}a, Rafael A. and Kallinger, Thomas and Mathur, Savita and Mosser, Beno{\^i}t and Bugnet, Lisa and Jones, Caitlin and Hon, Marc and Sharma, Sanjib and Sch{\"o}nrich, Ralph and Warfield, Jack T. and Luger, Rodrigo and Pinsonneault, Marc H. and Johnson, Jennifer A. and Huber, Daniel and Aguirre, Victor Silva and Chaplin, William J. and Davies, Guy R. and Miglio, Andrea},
  year = {2020},
  month = dec,
  journal = {The Astrophysical Journal Supplement Series},
  volume = {251},
  number = {2},
  eprint = {2012.04051},
  pages = {23},
  publisher = {{American Astronomical Society}},
  doi = {10.3847/1538-4365/abbee3},
  urldate = {2020-12-30},
  archiveprefix = {arxiv},
  keywords = {1368,1370,1614,1626,205,73,Asteroseismology,Astrophysics,Astrophysics of Galaxies,Catalogs,notion,notion-database,Red giant branch,Red giant clump,Solar and Stellar Astrophysics,Stellar masses,Stellar radii}
}

@article{zinnK2GalacticArchaeology2020,
  title = {The {{K2}} Galactic Archaeology Program Data Release 2: {{Asteroseismic}} Results from Campaigns 4, 6, \&amp; 7},
  author = {Zinn, J.C. and Stello, D. and Elsworth, Y. and Garc{\'i}a, R.A. and Kallinger, T. and Mathur, S. and Mosser, B. and Bugnet, L. and Jones, C. and Hon, M. and Sharma, S. and Sch{\"o}nrich, R. and Warfield, J.T. and Luger, R. and Pinsonneault, M.H. and Johnson, J.A. and Huber, D. and Aguirre, V.S. and Chaplin, W.J. and Davies, G.R. and Miglio, A.},
  year = {2020},
  journal = {arXiv},
  issn = {23318422},
  abstract = {Copyright \textcopyright{} 2020, The Authors. All rights reserved. Studies of Galactic structure and evolution have benefitted enormously from Gaia kinematic information, though additional, intrinsic stellar parameters like age are required to best constrain Galactic models. Asteroseismology is the most precise method of providing such information for field star populations en masse, but existing samples for the most part have been limited to a few narrow fields of view by the CoRoT and Kepler missions. In an effort to provide well-characterized stellar parameters across a wide range in Galactic position, we present the second data release of red giant asteroseismic parameters for the K2 Galactic Archaeology Program (GAP). We provide {$\nu$}max and {$\increment\nu$} based on six independent pipeline analyses; first-ascent red giant branch (RGB) and red clump (RC) evolutionary state classifications from machine learning; and ready-to-use radius \& mass coefficients, {$\kappa$}R \& {$\kappa$}M, which, when appropriately multiplied by a solar-scaled effective temperature factor, yield physical stellar radii and masses. In total, we report 4395 radius and mass coefficients, with typical uncertainties of 3.3\% (stat.) {$\pm$} 1\% (syst.) for {$\kappa$}R and 7.7\% (stat.) {$\pm$} 2\% (syst.) for {$\kappa$}M among RGB stars, and 5.0\% (stat.){$\pm$}1\% (syst.) for {$\kappa$}R and 10.5\% (stat.){$\pm$}2\% (syst.) for {$\kappa$}M among RC stars. We verify that the sample is nearly complete \textemdash{} except for a dearth of stars with {$\nu$}max . 10-20\textmu Hz \textemdash{} by comparing to Galactic models and visual inspection. Our asteroseismic radii agree with radii derived from Gaia Data Release 2 parallaxes to within 2.2 {$\pm$} 0.3\% for RGB stars and 2.0 {$\pm$} 0.6\% for RC stars.},
  keywords = {notion,notion-database}
}

@misc{Zong2023,
  title = {The Cradle of Nonlinear Asteroseismology: Observations of Oscillation Mode Variability in Compact Pulsating Stars},
  shorttitle = {The Cradle of Nonlinear Asteroseismology},
  author = {Zong, Weikai and Charpinet, St{\'e}phane and Vauclair, G{\'e}rard and Fu, Jian-Ning and Ma, Xiao-Yu},
  year = {2023},
  month = feb,
  number = {arXiv:2302.02166},
  eprint = {2302.02166},
  primaryclass = {astro-ph},
  publisher = {{arXiv}},
  urldate = {2023-09-19},
  abstract = {We briefly review progress in developing a pathway to nonlinear astereoseismology, both from theoretical and observational aspects. As predicted by the theory of weak nonlinear interactions between resonant modes, their amplitude and frequency can be modulated according to various kinds of patterns. However, those subtle modulations could hardly be well characterized from ground-based photometric monitoring. The \{\textbackslash sl Kepler\} spacecraft offered a new window to find clear-cut evidence of well-determined amplitude and frequency modulations, leading to the first discoveries of such variations in pulsating white dwarf and hot B subdwarf stars. Following that direction, a systematic survey of oscillation mode properties in compact pulsators monitored by \{\textbackslash sl Kepler\} suggests that mode variability is likely a common phenomenon, which remain unaccounted for by standard linear non-radial pulsation theory. To reach this conclusion firmly, the survey has now been extended to a larger context including compact stars observed by K2 and TESS. We expect that this extended survey will help to constrain key parameters governing weak nonlinear effects in stellar oscillations.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics - Solar and Stellar Astrophysics},
  file = {/Users/lbugnet/Zotero/storage/87L873LL/Zong et al. - 2023 - The cradle of nonlinear asteroseismology observat.pdf;/Users/lbugnet/Zotero/storage/L2JTTX9R/2302.html}
}

@misc{zotero-4242,
  title = {Evidence of Structural Discontinuities in the Inner Core of Red-Giant Stars | {{Nature Communications}}},
  urldate = {2023-08-01},
  howpublished = {https://www.nature.com/articles/s41467-022-34986-z},
  file = {/Users/lbugnet/Zotero/storage/E4IFP4L9/s41467-022-34986-z.html}
}

@misc{zotero-4284,
  title = {White-Dwarf Asteroseismology with the {{TESS}} Space Telescope - {{NASA}}/{{ADS}}},
  urldate = {2023-09-19},
  howpublished = {https://ui.adsabs.harvard.edu/abs/2022BAAA...63...48C/abstract},
  file = {/Users/lbugnet/Zotero/storage/G8ADEZZ8/abstract.html}
}

@misc{zotero-4326,
  title = {Zotero | {{Your}} Personal Research Assistant},
  urldate = {2022-07-26},
  howpublished = {https://www.zotero.org/},
  file = {/Users/lbugnet/Zotero/storage/LDYLB5AH/www.zotero.org.html}
}

@misc{zotero-4358,
  title = {Hot {{Subdwarf Stars}} | {{Annual Review}} of {{Astronomy}} and {{Astrophysics}}},
  urldate = {2023-10-02},
  howpublished = {https://www.annualreviews.org/doi/pdf/10.1146/annurev-astro-082708-101836},
  file = {/Users/lbugnet/Zotero/storage/2UNMLNIF/annurev-astro-082708-101836.html}
}

@misc{zotero-4452,
  title = {I {{Spy Transits}} and {{Pulsations}}: {{Empirical Variability}} in {{White Dwarfs Using Gaia}} and the {{Zwicky Transient Facility}} - {{NASA}}/{{ADS}}},
  urldate = {2023-10-09},
  howpublished = {https://ui.adsabs.harvard.edu/abs/2021ApJ...912..125G/abstract},
  file = {/Users/lbugnet/Zotero/storage/FCGS8WQR/abstract.html}
}

@misc{zotero-4651,
  title = {Presupernova {{Evolution}} of {{Rotating Massive Stars}}. {{II}}. {{Evolution}} of the {{Surface Properties}} - {{NASA}}/{{ADS}}},
  urldate = {2023-10-28},
  howpublished = {https://ui.adsabs.harvard.edu/abs/2000ApJ...544.1016H/abstract},
  file = {/Users/lbugnet/Zotero/storage/82TGB8Y6/abstract.html}
}

@misc{zotero-4667,
  title = {Asteroseismology of Evolved Stars to Constrain the Internal Transport of Angular Momentum. {{VI}}. {{Testing}} a Parametric Formulation for the Azimuthal Magneto-Rotational Instability - {{NASA}}/{{ADS}}},
  urldate = {2023-11-05},
  howpublished = {https://ui.adsabs.harvard.edu/abs/2023A\%26A...673A.110M/abstract},
  file = {/Users/lbugnet/Zotero/storage/SKBQTZBU/abstract.html}
}

@article{Zwintz2019,
  title = {The {{Power}} of {{Asteroseismology}} for {{Early Stellar Evolution}}},
  author = {Zwintz, Konstanze},
  year = {2019},
  month = dec,
  journal = {Frontiers in Astronomy and Space Sciences},
  volume = {6},
  pages = {68},
  publisher = {{Frontiers Media S.A.}},
  issn = {2296-987X},
  doi = {10.3389/fspas.2019.00068},
  urldate = {2020-03-03},
  abstract = {Stars are the building blocks of planetary systems, clusters, associations, and galaxies. The evolution of stars is driven by physical processes in their interiors making theory of stellar interior structure and evolution an important ingredient of contemporary astrophysics. Despite its importance, this theory contains major shortcomings starting from the early stages of stellar evolution which significantly impact all subsequent evolutionary phases. Studying the pulsations of young intermediate-mass stars, i.e., conducting pre-main sequence (pre-MS) asteroseismology, has the potential to contribute to a better understanding of the processes acting during the earliest phases of stellar evolution. With ultra-precise observational data obtained from space and from ground in combination with improvements of our theoretical models for pre-MS stars, the field of pre-MS asteroseismology will advance in the future and provide important constraints for the input physics of early stellar evolution.},
  keywords = {early stellar evolution,notion,notion-database,p- and g-mode pulsations,pre-main sequence,solar-like,space telescopes,SPB,{$\gamma$} Doradus,{$\delta$} Scuti},
  file = {/Users/lbugnet/Zotero/storage/DWGG48ZH/full-text.pdf}
}

@article{Zwintz2020,
  title = {Beta {{Cas}}: The First Delta {{Scuti}} Star with a Dynamo Magnetic Field},
  author = {Zwintz, K. and Neiner, C. and Kochukhov, O. and Rybchikova, T. and Pigulski, A. and Muellner, M. and Steindl, T. and Kuschnig, R. and Handler, G. and Moffat, A. F. J. and Pablo, H. and Popowicz, A. and Wade, G. A.},
  year = {2020},
  month = sep,
  journal = {Astronomy \& Astrophysics},
  volume = {643},
  eprint = {2009.04784},
  pages = {A110},
  publisher = {{EDP Sciences}},
  doi = {10.1051/0004-6361/202038210},
  urldate = {2020-11-29},
  abstract = {F type stars are characterised by several physical processes such as different pulsation mechanisms, rotation, convection, diffusion, and magnetic fields. The rapidly rotating delta Scuti star beta Cas can be considered as a benchmark star to study the interaction of several of these effects. We investigate the pulsational and magnetic field properties of beta Cas. We also determine the star's apparent fundamental parameters and chemical abundances. Based on photometric time series obtained from three different space missions (BRITE-Constellation, SMEI, and TESS), we conduct a frequency analysis and investigate the stability of the pulsation amplitudes over four years of observations. We investigate the presence of a magnetic field and its properties using spectropolarimetric observations taken with the Narval instrument by applying the Least Square Deconvolution and Zeeman Doppler Imaging techniques. beta Cas shows only three independent p-mode frequencies down to the few ppm-level; its highest amplitude frequency is suggested to be a \$n=3\$, \$\textbackslash ell = 2\$, \$m=0\$ mode. Its magnetic field structure is quite complex and almost certainly of a dynamo origin. beta Cas' atmosphere is slightly deficient in iron peak elements and slightly overabundant in C, O, and heavier elements. Atypically for delta Scuti stars, we can only detect three pulsation modes down to exceptionally low noise levels for beta Cas. The star is also one of very few delta Scuti pulsators known to date to show a measurable magnetic field, and the first delta Scuti star with a dynamo magnetic field. These characteristics make beta Cas an interesting target for future studies of dynamo processes in the thin convective envelopes of F-type stars, of the transition region between fossil and dynamo fields, and the interaction between pulsations and magnetic field.},
  archiveprefix = {arxiv},
  keywords = {Astrophysics,notion,notion-database,Solar and Stellar Astrophysics,stars: abundances,stars: atmospheres,stars: individual: {$\beta$} Cas,stars: magnetic field,stars: variables: {$\delta$}}
}

@article{Zwintz2020a,
  title = {{$\beta$} {{Cas}}: {{The}} First {$\delta$} {{Scuti}} Star with a Dynamo Magnetic Field{$\star$}},
  shorttitle = {{$\beta$} {{Cas}}},
  author = {Zwintz, K. and Neiner, C. and Kochukhov, O. and Ryabchikova, T. and Pigulski, A. and M{\"u}llner, M. and Steindl, T. and Kuschnig, R. and Handler, G. and Moffat, A. F. J. and Pablo, H. and Popowicz, A. and Wade, G. A.},
  year = {2020},
  month = nov,
  journal = {Astronomy and Astrophysics},
  volume = {643},
  pages = {A110},
  issn = {0004-6361},
  doi = {10.1051/0004-6361/202038210},
  urldate = {2023-10-17},
  abstract = {Context. F-type stars are characterised by several physical processes such as different pulsation mechanisms, rotation, convection, diffusion, and magnetic fields. The rapidly rotating {$\delta$} Scuti star {$\beta$} Cas can be considered as a benchmark star to study the interaction of several of these effects. Aims: We investigate the pulsational and magnetic field properties of {$\beta$} Cas. We also determine the star's apparent fundamental parameters and chemical abundances. Methods: Based on photometric time series obtained from three different space missions (BRITE-Constellation, SMEI, and TESS), we conduct a frequency analysis and investigate the stability of the pulsation amplitudes over four years of observations. We investigate the presence of a magnetic field and its properties using spectropolarimetric observations taken with the Narval instrument by applying the least-squares deconvolution and Zeeman-Doppler imaging techniques. Results: The star {$\beta$} Cas shows only three independent p-mode frequencies down to the few ppm-level; its highest amplitude frequency is suggested to be an n = 3, {$\mathscr{l}$} = 2, m = 0 mode. Its magnetic field structure is quite complex and almost certainly of a dynamo origin. The atmosphere of {$\beta$} Cas is slightly deficient in iron peak elements and slightly overabundant in C, O, and heavier elements. Conclusions: Atypically for {$\delta$} Scuti stars, we can only detect three pulsation modes down to exceptionally low noise levels for {$\beta$} Cas. The star is also one of very few {$\delta$} Scuti pulsators known to date to show a measurable magnetic field and the first {$\delta$} Scuti star with a dynamo magnetic field. These characteristics make {$\beta$} Cas an interesting target for future studies of dynamo processes in the thin convective envelopes of F-type stars, the transition region between fossil and dynamo fields, and the interaction between pulsations and magnetic field. The BRITE data are only available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr (ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/cat/J/A+A/643/A110 Based on data collected by the BRITE Constellation satellite mission, designed, built, launched, operated and supported by the Austrian Research Promotion Agency (FFG), the University of Vienna, the Technical University of Graz, the University of Innsbruck, the Canadian Space Agency (CSA), the University of Toronto Institute for Aerospace Studies (UTIAS), the Foundation for Polish Science \& Technology (FNiTP MNiSW), and National Science Centre (NCN). Also based on observations obtained at the Telescope Bernard Lyot (USR5026) operated by the Observatoire Midi-Pyr\'en\'ees, Universit\'e de Toulouse (Paul Sabatier), Centre National de la Recherche Scientifique (CNRS) of France.},
  keywords = {Astrophysics - Solar and Stellar Astrophysics,stars: abundances,stars: atmospheres,stars: individual: {$\beta$} Cas,stars: magnetic field,stars: variables: {$\delta$}},
  annotation = {ADS Bibcode: 2020A\&A...643A.110Z},
  file = {/Users/lbugnet/Zotero/storage/NR5TYCE4/Zwintz et al. - 2020 - β Cas The first δ Scuti star with a dynamo magnet.pdf}
}


==> refs_old <==
@article{Broderick2007,
	title = {Magnetic helicity and the relaxation of fossil fields},
	volume = {383},
	doi = {10.1111/j.1365-2966.2007.12634.x},
	number = {3},
	urldate = {2021-01-01},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Broderick, Avery E. and Narayan, Ramesh},
	year = {2007},
	pages = {943--956},
}

@book{ismail_2005, place={Cambridge}, series={Encyclopedia of Mathematics and its Applications}, title={Classical and Quantum Orthogonal Polynomials in One Variable}, DOI={10.1017/CBO9781107325982}, publisher={Cambridge University Press}, author={Ismail, Mourad E. H.}, year={2005}, collection={Encyclopedia of Mathematics and its Applications}}

@book{szegö1975orthogonal,
  title={Orthogonal Polynomials},
  author={Szeg{\"o}, G.},
  number={v. 23; v. 1975},
  lccn={77476087},
  series={American Mathematical Society: Colloquium publications},
  url={https://books.google.at/books?id=ntCoxgEACAAJ},
  year={1975},
  publisher={American Mathematical Society}
}


@book{DT98,
	Author = {{Dahlen}, F.~A. and {Tromp}, J.},
	Date-Added = {2012-06-01 15:44:37 +0000},
	Date-Modified = {2012-06-01 15:45:39 +0000},
	Publisher = {{Princeton University Press}},
	Title = {{Theoretical Global Seismology}},
	Year = {1998}}

@ARTICLE{Bhattacharya_etal_2024,
       author = {{Bhattacharya}, Shatanik and {Bharati Das}, Srijan and {Bugnet}, Lisa and {Panda}, Subrata and {Hanasoge}, Shravan M.},
        title = "{Detectability of axisymmetric magnetic fields from the core to the surface of oscillating post-main sequence stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = apr,
          eid = {arXiv:2404.17167},
        pages = {arXiv:2404.17167},
          doi = {10.48550/arXiv.2404.17167},
archivePrefix = {arXiv},
       eprint = {2404.17167},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240417167B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
